Persistent Dirac for molecular representation

Molecular representations are of fundamental importance for the modeling and analysis of molecular systems. Representation models and in general approaches based on topological data analysis (TDA) have demonstrated great success in various steps of drug design and materials discovery. Here we develop a mathematically rigorous computational framework for molecular representation based on the persistent Dirac operator. The properties of the spectrum of the discrete weighted and unweighted Dirac matrices are systemically discussed and used to demonstrate the geometric and topological properties of both non-homology and homology eigenvectors of real molecular structures. This allows us to asses the influence of weighting schemes on the information encoded in the Dirac eigenspectrum. A series of physical persistent attributes, which characterize the spectrum of the Dirac matrices across a filtration, are proposed and used as efficient molecular fingerprints. Finally, our persistent Dirac-based model is used for clustering molecular configurations from nine types of organic-inorganic halide perovskites. We found that our model can cluster the structures very well, demonstrating the representation and featurization power of the current approach.

==> refs.tex <==
% This file was created with JabRef 2.6.
% Encoding: Cp1252

@PREAMBLE{
 "\providecommand{\noopsort}[1]{}"
 # "\providecommand{\singleletter}[1]{#1}%"
}

%%%%%%%%%%%%%%%%%%%% my works

@incollection{vaccarino2022persistent,
  title={Persistent Homology: A Topological Tool for Higher-Interaction Systems},
  author={Vaccarino, Francesco and Fugacci, Ulderico and Scaramuccia, Sara},
  booktitle={Higher-Order Systems},
  pages={97--139},
  year={2022},
  publisher={Springer}
}



@article{wee2022persistent,
  title={Persistent spectral based ensemble learning (PerSpect-EL) for protein--protein binding affinity prediction},
  author={Wee, JunJie and Xia, Kelin},
  journal={Briefings in Bioinformatics},
  volume={23},
  number={2},
  pages={bbac024},
  year={2022},
  publisher={Oxford Academic}
}

@inproceedings{post2009first,
  title={First order approach and index theorems for discrete and metric graphs},
  author={Post, Olaf},
  booktitle={Annales Henri Poincar{\'e}},
  volume={10},
  number={5},
  pages={823--866},
  year={2009},
  organization={Springer}
}

@article{calmon2023dirac,
  title={Dirac signal processing of higher-order topological signals},
  author={Calmon, Lucille, and Schaub, Michael T. and Bianconi, Ginestra},
  journal={arXiv preprint arXiv:2301.10137},
  year={2023},
  publisher={arXiv}
}

@article{bianconi2022dirac,
  title={Dirac gauge theory for topological spinors in 3+ 1 dimensional networks},
  author={Bianconi, Ginestra},
  journal={arXiv preprint arXiv:2212.05621},
  year={2022}
}



@article{liu2021persistent,
  title={Persistent spectral hypergraph based machine learning ({PSH-ML}) for protein-ligand binding affinity prediction},
  author={Liu, Xiang and Feng, Huitao and Wu, Jie and Xia, Kelin},
  journal={Briefings in Bioinformatics},
  volume={22},
  number={5},
  pages={bbab127},
  year={2021},
  publisher={Oxford University Press}
}

@article{wee2021forman,
  title={Forman persistent Ricci curvature {(FPRC)}-based machine learning models for protein--ligand binding affinity prediction},
  author={Wee, JunJie and Xia, Kelin},
  journal={Briefings in Bioinformatics},
  volume={22},
  number={6},
  pages={bbab136},
  year={2021},
  publisher={Oxford University Press}
}


@article{wee2021ollivier,
  title={Ollivier {P}ersistent {R}icci {C}urvature-{B}ased {M}achine {L}earning for the {P}rotein--{L}igand {B}inding {A}ffinity {P}rediction},
  author={Wee, JunJie and Xia, Kelin},
  journal={Journal of Chemical Information and Modeling},
  volume={61},
  number={4},
  pages={1617--1626},
  year={2021},
  publisher={ACS Publications}
}

@article{meng2021persistent,
  title={Persistent spectral--based machine learning {(PerSpect ML)} for protein-ligand binding affinity prediction},
  author={Meng, Zhenyu and Xia, Kelin},
  journal={Science Advances},
  volume={7},
  number={19},
  pages={eabc5329},
  year={2021},
  publisher={American Association for the Advancement of Science}
}

@article{Liu2020hypergraph,
  title={Hypergraph based persistent cohomology {(HPC)} for molecular representations in drug design},
  author={Liu, X. and Wang X. J. and Wu, J. and Xia, K. L.},
  journal={Briefings in Bioinformatics},
  year={2021}
}

@ARTICLE{KLXia:2010,
  author = {Xia, K. L. and Zhan, Meng and Wei, G. W.},
  title = {Poster: Matched interface and boundary {(MIB)} method for multi-domain
	elliptic interface problems, in {Workshop on Fluid Motion Driven
	by Immersed Structures, Fields Institute, Toronto} },
  year = {2010},
  pages = { },
  month = {August 9-13}
}

@ARTICLE{KLXia:2011,
  author = {Xia, K. L. and Zhan, Meng and Wei, Guo-Wei},
  title = {The matched interface and boundary {(MIB)} method for multi-domain
	elliptic interface problems},
  journal = {Journal of Computational Physics},
  year = {2011},
  volume = {230},
  pages = {8231-8258}
}

@ARTICLE{KLXia:2012a,
  author = {Xia, K. L. and Zhan, Meng and Wan, D. C. and Wei, G. W. },
  title = {Adaptively deformed mesh based matched interface and boundary {(MIB)}
	method for elliptic interface problems},
  journal = {Journal of Computational Physics},
  year = {2012},
  volume = {231},
  pages = {1440 -1461}
}

@ARTICLE{KLXia:2013b,
  author = {Xia, K. L. and Wei, G. W. },
  title = {Three-dimensional {MIB} galerkin method for elliptic interface problems },
  year = {2013},
  journal = {submitted to Journal of Computational Physics},
  volume = {},
  pages = {}
  }


@ARTICLE{KLXia:2013e,
  author = {Xia, K. L.  and Wei, G. W. },
  title = {Protein folding tames chaos  },
  year = {2013},
  journal = { arXiv:1308.2953v1},
  volume = {},
  pages = {arXiv:1308.2953v1}
  }


@article{KLXia:2013f,
Author = {Xia, K. L.  and Wei, G. W.},
Title = {A stochastic model for protein flexibility analysis
},
Journal = {   Physical Review E },
Year = {2013},
Volume = {88},
Number = {},
Pages = {062709},
}

@article{KLXia:2013d,
Author = { Xia, K. L.  and Opron, K. and Wei, G. W.},
Title = {Multiscale multiphysics and multidomain models - { Flexibility and Rigidity}
},
Journal = {Journal of Chemical Physics },
Year = {2013},
Volume = {139},
Number = {},
Pages = { 194109},
}

@ARTICLE{XFeng:2013b,
  AUTHOR =       {Feng, X. and  Xia, K. L. and Tong, Y. Y. and Wei, G. W.},
  TITLE =        {Multiscale  geometric modeling of macromolecules {II:} Lagrangian representation},
  JOURNAL =      {Journal of Computational Chemistry},
  YEAR =         {2013},
  volume =       {34},
  number =       {},
  pages =        {2100-2120}
}

@article{Opron:2014,
Author = { Opron, K. and Xia, K. L. and Wei, G. W.},
Title = {Fast and anisotropic flexibility-rigidity index for protein flexibility and fluctuation analysis
},
Journal = {Journal of  Chemical Physics },
Year = {2014},
Volume = {140},
Number = {},
Pages = {234105},
}

@article{Opron:2014b,
Author = { Opron, K. and Xia, K. L. and Z. F. Burton and Wei, G. W.},
Title = {Flexibility–rigidity index for protein–nucleic acid flexibility and fluctuation analysis},
Journal = {Journal of  Computational Chemistry },
Year = {2016},
Volume = {37},
Number = {14},
Pages = {1283--1295},
}




@ARTICLE{KLXia:2014a,
  author = {Xia, K. L. and  Feng, X. and  Tong, Y. Y.  and Wei, G. W. },
  title = {Multiscale geometric modeling of macromolecules  I:  Cartesian representation},
  year = {2014},
  journal = {Journal of Computational Physics},
  volume = {275},
  pages = {912-936 }
  }

	
@ARTICLE{KLXia:2014b,
  author = {Xia, K. L.   and Wei, G. W. },
  title = { Molecular nonlinear dynamics and protein thermal uncertainty quantification },
  year = {2014},
  journal = {Chaos},
  volume = {24},
  pages = {013103 }
  }



@article{Xia:2014molecular,
  title={Molecular nonlinear dynamics and protein thermal uncertainty quantification},
  author={Xia, K. L. and Wei, G. W.},
  journal={Chaos: An Interdisciplinary Journal of Nonlinear Science},
  volume={24},
  number={1},
  pages={013103},
  year={2014},
  publisher={AIP Publishing}
}
	
@ARTICLE{KLXia:2014c,
  author = {Xia, K. L.   and Wei, G. W. },
  title = { Persistent homology  analysis of protein structure, flexibility and folding },
  year = {2014},
  journal = {International  Journal  for  Numerical    Methods  in    Biomedical    Engineerings},
  volume = {30 },
  pages = {814-844 }
  }

	
	
@ARTICLE{KLXia:2014e,
  author = {Xia, K. L. and  Meng, Z.  and Wei, G. W. },
  title = { {MIB  Galerkin}  method  for  elliptic  interface  problems},
  year = {  2014},
  journal = { Journal of Computational and Applied Mathematics},
  volume = {272},
  pages = {195- 220}
  }
	
	
@ARTICLE{KLXia:2014f,
  author = {Xia, K. L.  and Wei, G. W. },
  title = {A  {Galerkin formulation of the MIB} method for three dimensional elliptic interface problems},
  year = { 2014},
  journal = {Computers and Mathematics with Applications},
  volume = {68 },
  pages = {719-745  }
  }
	

@article{KLXia:2014persistent,
  title={Persistent homology analysis of protein structure, flexibility, and folding},
  author={Xia, K. L.  and Wei, G. W. },
  journal={International journal for numerical methods in biomedical engineering},
  volume={30},
  number={8},
  pages={814--844},
  year={2014},
  publisher={Wiley Online Library}
}

@ARTICLE{KLXia:2015a,
  author = {Xia, K. L. and  Feng, X. and  Tong, Y. Y.  and Wei, G. W. },
  title = {Persistent Homology for the quantitative prediction of fullerene stability},
  year = {2015},
  journal = {Journal of Computational Chemsitry},
  volume = {36},
  pages = { 408-422}
  }

@ARTICLE{ZXCang:2015,
  author = {Cang, Z. X. and  Mu, L. and Wu, K. D. and  Opron, K. and Xia, K. L. and Wei, G.W.},
   title = {A topological approach to protein classificationy},
  journal = {Molecular based Mathematical Biologys},
     year = {2015},
    volume={3},
  number={},
  pages={140-162}
}
	
@ARTICLE{KLXia:2015b,
  author = {Xia, K. L. and Wei, G. W. },
   title = {Persistent topology for {cryo-EM} data analysis},
  journal = {International Journal for Numerical Methods in Biomedical Engineering},
     year = {2015},
    volume={31},
  number={ },
  pages={e02719},
}

@ARTICLE{KLXia:2015c,
  author = {Xia, K. L.  and Wei, G. W. },
   title = {Multidimensional persistence in biomolecular data},
  journal = {  Journal Computational Chemistry },
    year = {2015},
    volume={36},
  number={},
  pages={1502-1520},
}


@ARTICLE{KLXia:2015d,
  author = {Xia, K. L. and Zhao, Z. X.   and Wei, G. W. },
   title = {Multiresolution topological simplification},
  journal = {  Journal Computational Biology},
     year = { 2015},
    volume={22},
  number={},
  pages={1-5},
}

@article{xia2015multiresolution,
  title={Multiresolution persistent homology for excessively large biomolecular datasets},
  author={Xia, K. L. and Zhao, Z. X.   and Wei, G. W. },
  journal={The Journal of chemical physics},
  volume={143},
  number={13},
  pages={10B603\_1},
  year={2015},
  publisher={AIP Publishing}
}

@article{Xia:2015multiscale,
  title={Multiscale {Gaussian} network model {(mGNM)} and multiscale anisotropic network model (mANM)},
  author={Xia, K. L. and Opron, K. and Wei, G. W.},
  journal={The Journal of chemical physics},
  volume={143},
  number={20},
  pages={204106},
  year={2015},
  publisher={AIP Publishing}
}

@article{Opron:2015communication,
  title={Communication: Capturing protein multiscale thermal fluctuations},
  author={Opron, K. and Xia, K. L. and Wei, G.W.},
  journal={The Journal of chemical physics},
  volume={142},
  number={21},
  pages={211101},
  year={2015},
  publisher={AIP Publishing}
}

@article{Nguyen:2016generalized,
  title={Generalized flexibility-rigidity index},
  author={Nguyen, D. and Xia, K. L. and Wei, G. W.},
  journal={The Journal of Chemical Physics},
  volume={144},
  number={23},
  pages={234106},
  year={2016},
  publisher={AIP Publishing}
}


@article{Xia:2018multiscale,
  title={Multiscale persistent functions for biomolecular structure characterization},
  author={Xia, K. L. and Li, Z. M. and Mu, L.},
  journal={Bulletin of mathematical biology},
  volume={80},
  number={1},
  pages={1--31},
  year={2018},
  publisher={Springer}
}

@article{Xia:2018multiscale,
  title={Multiscale virtual particle based elastic network model {(MVP-ENM)} for normal mode analysis of large-sized biomolecules},
  author={Xia, K. L. },
  journal={Physical Chemistry Chemical Physics},
  volume={20},
  number={1},
  pages={658--669},
  year={2018},
  publisher={Royal Society of Chemistry}
}

@article{Xia:2018sequence,
  title={Sequence-based multiscale modeling for high-throughput chromosome conformation capture {(Hi-C)} data analysis},
  author={Xia, K. L.},
  journal={PloS one},
  volume={13},
  number={2},
  pages={e0191899},
  year={2018},
  publisher={Public Library of Science}
}

@article{Xia:2016review,
  title={A review of geometric, topological and graph theory apparatuses for the modeling and analysis of biomolecular data},
  author={Xia, K. L. and Wei, G. W.},
  journal={arXiv preprint arXiv:1612.01735},
  year={2016}
}

@article{xia2018persistent,
  title={Persistent homology analysis of ion aggregations and hydrogen-bonding networks},
  author={Xia, K. L.},
  journal={Physical Chemistry Chemical Physics},
  volume={20},
  number={19},
  pages={13448--13460},
  year={2018},
  publisher={Royal Society of Chemistry}
}

@article{pun2018persistent,
  title={Persistent-Homology-based Machine Learning and its Applications--A Survey},
  author={Pun, C. S. and Xia, K. L. and Lee, S. X.},
  journal={arXiv preprint arXiv:1811.00252},
  year={2018}
}

@article{meng2019weighted,
  title={Weighted persistent homology for biomolecular data analysis},
  author={Meng, Z. Y. and Anand, D. V. and Lu, Y. P. and Wu, J. and Xia, K. L.},
  journal={Scientific Reports},
  volume={10},
  number={1},
  pages={1--15},
  year={2020},
  publisher={Nature Publishing Group}
}

@article{xia2019persistent,
  title={Persistent homology analysis of osmolyte molecular aggregation and their hydrogen-bonding networks},
  author={Xia, K. L. and Anand, D. V. and Saxena, S. and Mu, Y. G.},
  journal={Physical Chemistry Chemical Physics},
  volume={21},
  number={37},
  pages={21038--21048},
  year={2019},
  publisher={Royal Society of Chemistry}
}

@article{anand2020weighted,
  title={Weighted persistent homology for osmolyte molecular aggregation and hydrogen-bonding network analysis},
  author={Anand, D. V. and Meng, Z. Y. and Xia, K. L. and Mu, Y. G.},
  journal={Scientific reports},
  volume={10},
  number={1},
  pages={1--17},
  year={2020},
  publisher={Nature Publishing Group}
}

%%%%%%%%%%  group papers

%% Review
@article{wei2017mathematics,
  title={Mathematics at the eve of a historic transition in biology},
  author={Wei, G. W.},
  journal={Computational and Mathematical Biophysics},
  volume={5},
  number={1},
  year={2017}
}

@article{wei2017persistent,
  title={Persistent homology analysis of biomolecular data},
  author={Wei, G. W.},
  journal={Journal of Computational Physics},
  volume={305},
  pages={276--299},
  year={2017}
}

@article{nguyen2020review,
  title={A review of mathematical representations of biomolecular data},
  author={Nguyen, D. D. and Cang, Z. X. and Wei, G. W.},
  journal={Physical Chemistry Chemical Physics},
  year={2020},
  publisher={Royal Society of Chemistry}
}

%% ESPH
@article{cang:2017analysis,
  title={Analysis and prediction of protein folding energy changes upon mutation by element specific persistent homology},
  author={Cang, Z. X. and Wei, G. W.},
  journal={Bioinformatics},
  volume={33},
  number={22},
  pages={3549--3557},
  year={2017},
  publisher={Oxford University Press}
}

@article{cang:2017topologynet,
  title={{TopologyNet: Topology} based deep convolutional and multi-task neural networks for biomolecular property predictions},
  author={Cang, Z. X. and Wei, G. W.},
  journal={PLOS Computational Biology},
  volume={13},
  number={7},
  pages={e1005690},
  year={2017},
  publisher={Public Library of Science}
}

@article{cang:2017integration,
  title={Integration of element specific persistent homology and machine learning for protein-ligand binding affinity prediction},
   author={Cang, Z. X. and Wei, G. W.},
  journal={International journal for numerical methods in biomedical engineering},
  year={2017},
  pages={{10.1002/cnm.2914}},
  publisher={Wiley Online Library}
}

@article{nguyen:2017rigidity,
  title={Rigidity {S}trengthening: {A} {M}echanism for {P}rotein--{L}igand {B}inding},
  author={Nguyen, D. D. and Xiao, T. and Wang, M. L. and Wei, G. W.},
  journal={Journal of chemical information and modeling},
  volume={57},
  number={7},
  pages={1715--1721},
  year={2017},
  publisher={ACS Publications}
}

@article{cang:2018representability,
  title={Representability of algebraic topology for biomolecules in machine learning based scoring and virtual screening},
  author={Cang, Z. X. and Mu, L. and Wei, G. W.},
  journal={PLoS computational biology},
  volume={14},
  number={1},
  pages={e1005929},
  year={2018},
  publisher={Public Library of Science}
}

@article{wu:2018quantitative,
  title={Quantitative toxicity prediction using topology based multi-task deep neural networks},
  author={Wu, K. D. and Wei, G. W.},
  journal={Journal of chemical information and modeling},
  year={2018},
  pages={{10.1021/acs.jcim.7b00558}},
  publisher={ACS Publications}
}

@article{cang2018integration,
  title={Integration of element specific persistent homology and machine learning for protein-ligand binding affinity prediction},
  author={Cang, Z. X. and Wei, G. W.},
  journal={International journal for numerical methods in biomedical engineering},
  volume={34},
  number={2},
  pages={e2914},
  year={2018},
  publisher={Wiley Online Library}
}

@article{nguyen2019agl,
  title={{AGL}-{S}core: {A}lgebraic {G}raph {L}earning {S}core for {P}rotein-{L}igand {B}inding {S}coring, {R}anking, {D}ocking, and {S}creening},
  author={Nguyen, D. D. and Wei, G. W.},
  journal={Journal of chemical information and modeling},
  volume={59},
  number={7},
  pages={3291--3304},
  year={2019},
  publisher={ACS Publications}
}

@article{nguyen2019dg,
  title={{DG-GL}: {D}ifferential geometry-based geometric learning of molecular datasets},
  author={Nguyen, D. D. and Wei, G. W.},
  journal={International journal for numerical methods in biomedical engineering},
  volume={35},
  number={3},
  pages={e3179},
  year={2019},
  publisher={Wiley Online Library}
}

@article{zhao2018protein,
  title={Protein pocket detection via convex hull surface evolution and associated {Reeb} graph},
  author={Zhao, R. D. and Cang, Z. X. and Tong, Y. Y. and Wei, G. W.},
  journal={Bioinformatics},
  volume={34},
  number={17},
  pages={i830--i837},
  year={2018},
  publisher={Oxford University Press}
}

@article{wu2018topp,
  title={{TopP--S}: {P}ersistent homology-based multi-task deep neural networks for simultaneous predictions of partition coefficient and aqueous solubility},
  author={Wu, K. D. and Zhao, Z. X. and Wang, R. X. and Wei, G. W.},
  journal={Journal of computational chemistry},
  volume={39},
  number={20},
  pages={1444--1454},
  year={2018},
  publisher={Wiley Online Library}
}

%%%%%%%%% solvation free energy
@article{wang2015parameter,
  title={Parameter optimization in differential geometry based solvation models},
  author={Wang, B. and Wei, G. W.},
  journal={The Journal of chemical physics},
  volume={143},
  number={13},
  pages={10B608\_1},
  year={2015},
  publisher={AIP Publishing LLC}
}

@article{wang2016automatic,
  title={Automatic parametrization of non-polar implicit solvent models for the blind prediction of solvation free energies},
  author={Wang, B. and Zhao, Z. X. and Wei, G. W.},
  journal={The Journal of chemical physics},
  volume={145},
  number={12},
  pages={124110},
  year={2016},
  publisher={AIP Publishing LLC}
}

@article{wang2018breaking,
  title={Breaking the polar-nonpolar division in solvation free energy prediction},
  author={Wang, B. and Wang, C. Z. and Wu, K. D. and Wei, G. W.},
  journal={Journal of computational chemistry},
  volume={39},
  number={4},
  pages={217--233},
  year={2018},
  publisher={Wiley Online Library}
}




%%%%% D3R
@article{nguyen2018mathematical,
  title={Mathematical deep learning for pose and binding affinity prediction and ranking in {D3R Grand Challenges}},
  author={Nguyen, D. D. and Cang, Z. X. and Wu, K. D. and Wang, M. L. and Cao, Y. and Wei, G. Wei.},
  journal={Journal of computer-aided molecular design},
  volume={33},
  number={1},
  pages={71--82},
  year={2019},
  publisher={Springer}
}

@article{nguyen2019mathdl,
  title={{MathDL}: {M}athematical deep learning for {D3R Grand Challenge} 4},
  author={Nguyen, D. D. and Gao, K. F. and Wang, M. L. and Wei, G. W.},
  journal={Journal of computer-aided molecular design},
  pages={1--17},
  year={2019},
  publisher={Springer}
}

%% Generative model

@article{gao2020generative,
  title={Generative {N}etwork {C}omplex for the {A}utomated {G}eneration of {D}rug-like {M}olecules},
  author={Gao, Kaifu and Nguyen, Duc Duy and Tu, Meihua and Wei, Guo-Wei},
  journal={Journal of chemical information and modeling},
  volume={60},
  number={12},
  pages={5682--5698},
  year={2020},
  publisher={ACS Publications}
}

@article{wang2020persistent,
  title={Persistent spectral graph},
  author={Wang, R. and Nguyen, D. D. and Wei, Guo-Wei},
  journal={International Journal for Numerical Methods in Biomedical Engineering},
  pages={e3376},
  year={2020},
  publisher={Wiley Online Library}
}



%%%%%%%%%%%%%% Prof.Wei drug design
@Online{Wei2019,
 author = {Wei, G. W.},
 year = {2019},
 title = {I build mathematical programs that could discover the drugs of the future},
 journal = {The Conversation},
 url = {https://theconversation.com/i-build-mathematical-programs-that-could-discover-the-drugs-of-the-future-110689},
 urldate = {2019-02-26}
}


%%% COVID19

@article{nguyen2020potentially,
  title={Potentially highly potent drugs for {2019-nCoV}},
  author={Nguyen, Duc and Gao, Kaifu and Chen, Jiahui and Wang, Rui and Wei, Guewei},
  journal={bioRxiv},
  year={2020},
  publisher={Cold Spring Harbor Laboratory}
}

%%%%%%%%% cohomology

@article{cang2020persistent,
  title={Persistent cohomology for data with multicomponent heterogeneous information},
  author={Cang, Z. X. and Wei, G. W.},
  journal={SIAM Journal on Mathematics of Data Science},
  volume={2},
  number={2},
  pages={396--418},
  year={2020},
  publisher={SIAM}
}


%%% TopNetTree
@article{wang2020topology,
  title={A topology-based network tree for the prediction of protein--protein binding affinity changes following mutation},
  author={Wang, Menglun and Cang, Zixuan and Wei, Guo-Wei},
  journal={Nature Machine Intelligence},
  volume={2},
  number={2},
  pages={116--123},
  year={2020},
  publisher={Nature Publishing Group}
}


@article{chen2021algebraic,
  title={Algebraic graph-assisted bidirectional transformers for molecular property prediction},
  author={Chen, Dong and Gao, Kaifu and Nguyen, Duc Duy and Chen, Xin and Jiang, Yi and Wei, Guo-Wei and Pan, Feng},
  journal={Nature Communications},
  volume={12},
  number={1},
  pages={1--9},
  year={2021},
  publisher={Nature Publishing Group}
}

@article{jiang2021ggl,
  title={{GGL-Tox:} {G}eometric {G}raph {L}earning for {T}oxicity {P}rediction},
  author={Jiang, Jian and Wang, Rui and Wei, Guo-Wei},
  journal={Journal of chemical information and modeling},
  volume={61},
  number={4},
  pages={1691--1700},
  year={2021},
  publisher={ACS Publications}
}



%%%%%%%%%%%%% SARS-CoV-2


@article{chen2020mutations,
  title={Mutations strengthened {SARS-CoV-2} infectivity},
  author={Chen, Jiahui and Wang, Rui and Wang, Menglun and Wei, Guo-Wei},
  journal={Journal of molecular biology},
  volume={432},
  number={19},
  pages={5212--5226},
  year={2020},
  publisher={Elsevier}
}

@article{wang2020mutations,
  title={Mutations on {COVID-19} diagnostic targets},
  author={Wang, Rui and Hozumi, Yuta and Yin, Changchuan and Wei, Guo-Wei},
  journal={Genomics},
  volume={112},
  number={6},
  pages={5204--5213},
  year={2020},
  publisher={Elsevier}
}


%%%%%%%%%%%% Guowei works end







%%%%%%%%%%% Jie Wu

@article{ren2017weighted,
  title={Weighted {P}ersistent {H}omology},
  author={Ren, S. Q. and Wu, C. Y. and Wu, J.},
  journal={arXiv preprint arXiv:1708.06722},
  year={2017}
}


@article{wu2018weighted,
  title={Weighted ({C}o)homology and {W}eighted {L}aplacian},
  author={Wu, C. Y. and Ren, S. Q. and Wu, J. and Xia, K. L.},
  journal={SCIENCE CHINA Mathematics},
  publisher={Science China Press}
}

@article{ren2018hodge,
  title={{Hodge} {D}ecompositions for {W}eighted {H}ypergraphs},
  author={Ren, S. Q. and Wu, C. Y. and Wu, J.},
  journal={arXiv preprint arXiv:1805.11331},
  year={2018}
}

@article{bressan2016embedded,
  title={The embedded homology of hypergraphs and applications},
  author={Bressan, S. and Li, J. Y. and Ren, S. Q. and Wu, J.},
  journal={arXiv preprint arXiv:1610.00890},
  year={2016}
}

@article{ren2018discrete,
  title={A Discrete Morse Theory for Hypergraphs},
  author={Ren, S. Q. and Wang, C. and Wu, C. Y. and Wu, J.},
  journal={arXiv preprint arXiv:1804.07132},
  year={2018}
}


%%%% Hypergraph

@techreport{parks1991homology,
  title={Homology and hypergraph acyclicity: a combinatorial invariant for hypergraphs},
  author={Parks, A. D. and Lipscomb, S. L.},
  year={1991},
  institution={NAVAL SURFACE WARFARE CENTER DAHLGREN VA}
}

@article{chung1992cohomological,
  title={Cohomological aspects of hypergraphs},
  author={Chung, F. and Graham, R. L.},
  journal={Transactions of the American Mathematical Society},
  volume={334},
  number={1},
  pages={365--388},
  year={1992}
}

@inproceedings{johnson2009hypernetworks,
  title={Hypernetworks of complex systems},
  author={J. Johnson},
  booktitle={International Conference on Complex Sciences},
  pages={364--375},
  year={2009},
  organization={Springer}
}

@article{emtander2009betti,
  title={Betti numbers of hypergraphs},
  author={Emtander, E.},
  journal={Communications in algebra},
  volume={37},
  number={5},
  pages={1545--1571},
  year={2009},
  publisher={Taylor \& Francis}
}

@article{bressan2016embedded,
  title={The embedded homology of hypergraphs and applications},
  author={Bressan, S. and Li, J. Y. and Ren, S. Q. and Wu, J.},
  journal={arXiv preprint arXiv:1610.00890},
  year={2016}
}

@article{ren2020stability,
  title={Stability of persistent homology for hypergraphs},
  author={Ren, S. Q. and Wu, J.},
  journal={arXiv preprint arXiv:2002.02237},
  year={2020}
}

@article{ren2017computing,
  title={Computing the Homology of Hypergraphs},
  author={Ren, S. Q. and Wu, C. Y. and Bressan, S. and Wu, J.},
  journal={arXiv preprint arXiv:1705.00151},
  year={2017}
}

@article{ren2018evolutions,
  title={Evolutions of hypergraphs and their embedded homology},
  author={Ren, S. Q. and Wu, C. Y. and Wu, J.},
  journal={arXiv preprint arXiv:1804.07132},
  year={2018}
}

@article{ren2018hodge,
  title={Hodge Decompositions for Weighted Hypergraphs},
  author={Ren, S. Q. and Wu, C. Y. and Wu, J.},
  journal={arXiv preprint arXiv:1805.11331},
  year={2018}
}


@book{qi2017tensor,
  title={Tensor analysis: spectral theory and special tensors},
  author={Qi, Liqun and Luo, Ziyan},
  year={2017},
  publisher={SIAM}
}

@article{cooper2012spectra,
  title={Spectra of uniform hypergraphs},
  author={Cooper, Joshua and Dutle, Aaron},
  journal={Linear Algebra and its applications},
  volume={436},
  number={9},
  pages={3268--3292},
  year={2012},
  publisher={Elsevier}
}

@article{banerjee2017spectra,
  title={Spectra of general hypergraphs},
  author={Banerjee, Anirban and Char, Arnab and Mondal, Bibhash},
  journal={Linear Algebra and its Applications},
  volume={518},
  pages={14--30},
  year={2017},
  publisher={Elsevier}
}



%%%%%%%%%% Cohomology

@article{de2011persistent,
  title={Persistent cohomology and circular coordinates},
  author={De Silva, Vin and Morozov, Dmitriy and Vejdemo-Johansson, Mikael},
  journal={Discrete \& Computational Geometry},
  volume={45},
  number={4},
  pages={737--759},
  year={2011},
  publisher={Springer}
}











%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

@ARTICLE{ukherjee:2009,
  author = {ukherjee, S. and Zhang, Y.},
  title = {{MM-align: a quick algorithm for aligning multiple-chain protein
	complex structures using iterative dynamic programming}},
  journal = {Nucleic Acids Res},
	volume = {},
  year = {2009},
  pages = {1-12}
}

@ARTICLE{Abaid:2008,
  author = { Abaid, N. and Eisenberg, B. S. and Liu, W. S. },
  title = {Asymptotic Expansions of {I-V} Relations via a {Poisson-Nernst-Planck}
	System},
  journal = {SIAM Journal on Applied Dynamical Systems},
  year = {2008},
  volume = {7},
  pages = {1507-1526 },
  number = {4 }
}

@ARTICLE{gottlieb86,
  author = {Abarbanel, S. and Gottlieb, D. and Tadmor, E.},
  title = {Spectral methods for discontinuous problems},
  journal = {Numerical Methods for Fluid Dynamics},
  year = {1986},
  pages = {129-153 },
  publisher = {(K. Morton and M. Baines eds.), Oxford University Press, New York}
}

@ARTICLE{Abraham:1998,
  author = {Abraham, F. F. and Broughton, J. Q. and Bernstein, N. and Kaxiras,
	E.},
  title = {Spanning the continuum to quantum length scales in a dynamic simulation
	of brittle fracture},
  journal = {Europhys. Lett.},
  year = {1998},
  volume = {44},
  pages = {783 - 787}
}

@ARTICLE{Abrams:2006a,
  author = {Abrams, Jerry B. and Rosso, Lula and Tuckerman, Mark E. },
  title = {Efficient and precise solvation free energies via alchemical adiabatic
	molecular dynamics},
  journal = {The Journal of Chemical Physics},
  year = {2006},
  volume = {125},
  pages = {074115},
  number = {7}
}

@ARTICLE{Abrashkin:2007,
  author = {Abrashkin, A. and Andelman, D. and Orland, H.},
  title = {Dipolar Poisson-Boltzmann Equation: Ions and Dipoles Close to Charge
	Interfaces},
  journal = { Phys. Rev. Lett. },
  year = {2007},
  volume = {99},
  pages = {077801},
  abstract = {In the DPB model we coarse grain the interaction of individual ions
	and dipoles interacting together.It includes some aspects of the
	discrete nature of the dipolar solvent molecules and how they modify
	the ion?Csolvent interactions.}
}

@ARTICLE{VelocityExtrapolation,
  author = {D. Adalsteinsson and J.A. Sethian},
  title = {{The Fast Construction of Extension Velocities in Level Set Methods}},
  journal = {J. Computational Physics},
  year = {1999},
  volume = {148},
  pages = {2--22}
}

@ARTICLE{Adalsteinsson:2008,
  author = {Adalsteinsson, H. and Debusschere, B. J. and Long, K. R. and Najm,
	H. N.},
  title = {Components for atomistic-to-continuum multiscale modeling of flow
	in micro- and nanofluidic systems },
  journal = {Scient. Program.},
  year = {2008},
  volume = {16},
  pages = {297-313}
}

@ARTICLE{Adams:2002,
  author = {Adams, L. and Li, Z. L.},
  title = {The immersed interface/multigrid methods for interface problems},
  journal = {SIAM J. Sci. Comput. },
  year = {2002},
  volume = {24},
  pages = {463-479},
  annote = {The immersed interface/multigrid methods for interface problems},
  date-added = {2008-09-19 10:28:56 -0500},
  date-modified = {2008-09-19 10:28:56 -0500},
  ty = {JOUR}
}

@ARTICLE{Adcock:2006,
  author = {Adcock, S. A. and McCammon, J. A.},
  title = {Molecular Dynamics: Survey of Methods for Simulating the Activity
	of Protein},
  journal = {Chemical Reviews},
  year = {2006},
  volume = {106},
  pages = {1589-615},
  number = {5},
  annote = {Molecular Dynamics: Survey of Methods for Simulating the Activity
	of Protein},
  bdsk-url-1 = {http://dx.doi.org/10.1021/cr040426m},
  date-added = {2008-06-28 10:28:56 -0500},
  date-modified = {2008-06-28 10:28:56 -0500},
  keywords = {molecular\_simulation; molecular\_dynamics},
  ty = {JOUR},
  url = {http://dx.doi.org/10.1021/cr040426m}
}

@ARTICLE{Agmon:1995,
  author = {Agmon, N.},
  title = {The Grotthuss Mechanism},
  journal = {Chem. Phys. Lett},
  year = {1995},
  volume = {244},
  pages = {456-462},
  number = { }
}

@ARTICLE{Agrawal:2002,
  author = {Agrawal, O. P.},
  title = {Formulation of Euler?Lagrange equations for fractional variational
	problems},
  journal = {J. Math. Anal. Appl. },
  year = {2002},
  volume = {272},
  pages = {368 -79}
}

@ARTICLE{Ahmed:2005,
  author = {Ahmed, S. S. and Ringhofer, C. and Vasileska, D.},
  title = {Parameter-Free Effective Potential Method for Use in Particle-Based
	Device Simulations},
  journal = {IEEE Tran. Nanotech.},
  year = {2008},
  volume = {4},
  pages = {456 -471}
}

@ARTICLE{Ahmend:2004,
  author = {Ahmend, S. S. and Vasileska, D. },
  title = {Modelling of narrow-width {SOI} devices},
  journal = {Semicond. Sci. Technol},
  year = {2004},
  volume = {19},
  pages = {S131-133}
}

@ARTICLE{Akeson:1991,
  author = {Akeson, M. and Deamer, D.W.},
  title = {Proton conductance by the {Gramicidin} water wire. {Model} for proton
	conductance in the $\mathrm{F}_0\mathrm{F}_1\mathrm{ATP}$ases?},
  journal = {Biophys J.},
  year = {1991},
  volume = {60},
  pages = {101-109},
  number = { }
}

@ARTICLE{Akiyama:1998,
  author = {Akiyama, Ryo and Hirata, Fumio},
  title = {Theoretical study for water structure at highly ordered surface:
	Effect of surface structure},
  journal = {Journal of Chemical Physics},
  year = {1998},
  volume = {108},
  pages = {4904-4911}
}


@ARTICLE{MultiSolvers,
  author = {Burak Aksoylu and Andrei Khodakovsky and Peter Schr{\"o}der},
  title = {Multilevel Solvers for Unstructured Surface Meshes},
  journal = {SIAM J. Sci. Comput.},
  year = {2005},
  volume = {26},
  pages = {1146--1165},
  number = {4}
}

@ARTICLE{Alavi:1998,
  author = {Alavi, S. and Wei, G. W. and Snider, R. F.},
  title = {Chain relations of reduced distribution functions and their associated
	correlation functions},
  journal = {J. Chem. Phys. },
  year = {1998},
  volume = {108},
  pages = {706-714 },
  annote = {Chain relations of reduced distribution functions and their associated
	correlation functions},
  date-added = {2008-11-25 10:28:56 -0500},
  date-modified = {2008-11-25 10:28:56 -0500},
  ty = {JOUR}
}

@ARTICLE{Alavi:1997,
  author = {Alavi, S. and Wei, G. W. and Snider, R. F.},
  title = {Chain relations of reduced distribution functions and their associated
	correlation functions},
  journal = {J. Chem. Phys.},
  year = {1997},
  volume = {108},
  pages = {706 -714}
}

@MISC{PointSetCourse,
  author = {M. Alexa and M. Gross and M. Pauly and H.P. Pfister and M. Stamminger
	and M. Zwicke},
  title = {Point-Based Computer Graphics},
  year = {2006},
  note = {ACM SIGGRAPH Course}
}

@ARTICLE{Alexandrovsky:2004,
  author = {Alexandrovsky, V. V. and Basilevsky, M. V. and Leontyev, I. V. and
	Mazo, M. A. and Sulimov, V. B.},
  title = {The Binomial Cell Model of Hydrophobic Solvation},
  journal = {Journal of Physical Chemistry B},
  year = {2004},
  volume = {108},
  pages = {15830-40},
  number = {40},
  abstract = {On the basis of the cell model of dense fluids, we derive the binomial
	distribution law for a number of solvent particles occupying a given
	void of excluded volume (a cavity) which arises in a bulk solvent
	as a fluctuation. It is inserted as a default distribution in the
	information theory approach (Hummer, G.; Garde, S.; Garcia, A. E.;
	Paulaitis, M. E.; Pratt, L. R. J. Phys. Chem. B 1998, 102, 10469)
	for treating the thermodynamics of cavitation; the imaginary process
	is considered as a component of the total solvation process. Computations
	of cavitation free energies, entropies, and enthalpies for 11 hydrocarbons
	in water solvent are compared with results of the computer simulation
	of these properties reported by E. Gallicchio et al. (Gallicchio,
	E.; Kubo, M. M.; Levy, R. J. Phys. Chem. B 2000, 104, 6271). A similar
	analysis of cavitation for model spherical solutes in water in a
	wide range of cavity radii is also provided. Linear correlation between
	the cavitation free energy and the cavity volume is observed and
	justified. The present binomial approach for treating cavitation
	effects efficiently covers a large range of cavity volumes 's (102
	Ãƒ 3 < <103 Ãƒ 3).},
  annote = {The Binomial Cell Model of Hydrophobic Solvation},
  bdsk-url-1 = {http://dx.doi.org/10.1021/jp031189e},
  date-added = {2008-08-29 15:50:55 -0500},
  date-modified = {2008-08-29 15:50:55 -0500},
  keywords = {Solvation},
  ty = {JOUR},
  url = {http://dx.doi.org/10.1021/jp031189e}
}

@ARTICLE{Alexov:1999,
  author = {Alexov, E.G. and Gunner, M. R.},
  title = {{Calculated Protein and Proton Motions Coupled to Electron Transfer:
	Electron Transfer from $Q_A^-$ to $Q_B$ in Bacterial Photosynthetic
	Reaction Centers}},
  journal = {Biochemistry},
  year = {1999},
  volume = {38},
  pages = {8253-8270}
}

@ARTICLE{Alikakos:2006,
  author = {Alikakos, N. D. and Bates, P. W. and Cahn, J. W. and Fife, P. C.
	and Fusco, G. and Tanoglu, G. B.},
  title = {Analysis of a corner layer problem in anisotropic interfaces},
  journal = {Discrete Contin. Dyn. Syst. Ser. B},
  year = {2006},
  volume = {6},
  pages = {237-255},
  annote = {Analysis of a corner layer problem in anisotropic interfaces},
  date-added = {2008-09-19 10:28:56 -0500},
  date-modified = {2008-09-19 10:28:56 -0500},
  ty = {JOUR}
}

@ARTICLE{Alikakos:1994,
  author = {Alikakos, N. D. and Bates, P. W. and Chen, X. F.},
  title = {Convergence of the {Cahn-Hilliard} equation to the {Hele-Shaw} model},
  journal = {Arch. Rational Mech. Anal. },
  year = {1994},
  volume = {128},
  pages = {165--205},
  annote = {Convergence of the {Cahn-Hilliard} equation to the {Hele-Shaw} model},
  date-added = {2008-09-19 10:28:56 -0500},
  date-modified = {2008-09-19 10:28:56 -0500},
  ty = {JOUR}
}

@ARTICLE{Alikakos:2000,
  author = {Alikakos, N. D. and Bates, P. W. and Chen, X. F. and Fusco, G.},
  title = {Mullins-Sekerka motion of small droplets on a fixed boundary},
  journal = {J. Geom. Anal. },
  year = {2000},
  volume = {10},
  pages = {575-596},
  annote = {{Mullins-Sekerka} motion of small droplets on a fixed boundary},
  date-added = {2008-09-19 10:28:56 -0500},
  date-modified = {2008-09-19 10:28:56 -0500},
  ty = {JOUR}
}

@ARTICLE{allen2003shb,
  author = {Allen, B. and Curless, B. and Popovi{\'c}, Z.},
  title = {{The space of human body shapes: reconstruction and parameterization
	from range scans}},
  journal = {ACM SIGGRAPH},
  year = {2003},
  pages = {587--594}
}

@ARTICLE{UoW,
  author = {Brett Allen and Brian Curless and Zoran Popovi{\'c}},
  title = {Articulated Body Deformation from Range Scan Data},
  journal = {ACM Trans. on Graphics (SIGGRAPH)},
  year = {2002},
  volume = {21},
  pages = {612--619},
  number = {3}
}

@ARTICLE{Allen:2001,
  author = {Allen, R. and Hansen, J.-P. and Melchionna, S. },
  title = {{Electrostatic potential inside ionic solutions confined by dielectrics:
	a variational approach}},
  journal = {Phys Chem Chem Physics},
  year = {2001},
  volume = {3},
  pages = {4177-4186}
}

@ARTICLE{ACDLD03,
  author = {Pierre Alliez and David Cohen-Steiner and Bruno L{\'e}vy and Olivier
	Devillers and Mathieu Desbrun},
  title = {Anisotropic Polygonal Remeshing},
  journal = {ACM Trans. on Graphics (SIGGRAPH)},
  year = {2003},
  volume = {22},
  pages = {485--493},
  number = {3},
  month = {jun}
}

@INPROCEEDINGS{ACTD07,
  author = {Pierre Alliez and David Cohen-Steiner and Yiying Tong and Mathieu
	Desbrun},
  title = {Voronoi-based Variational Reconstruction of Unoriented Point Sets},
  booktitle = {Symposium on Geometry Processing},
  year = {2007},
  pages = {39--48},
  month = Jul
}

@ARTICLE{ACYD05,
  author = {Pierre Alliez and David Cohen-Steiner and Mariette Yvinec and Mathieu
	Desbrun},
  title = {Variational Tetrahedral Meshing},
  journal = {ACM Trans. on Graphics (SIGGRAPH)},
  year = {2005},
  volume = {24},
  pages = {617--625},
  number = {3},
  month = {jul}
}

@INPROCEEDINGS{AD01,
  author = {Pierre Alliez and Mathieu Desbrun},
  title = {Progressive Compression for Lossless Transmission of Triangle Meshes},
  booktitle = {ACM SIGGRAPH Conference},
  year = {2001},
  pages = {195--202},
  month = Aug
}

@INPROCEEDINGS{ADEG01,
  author = {Pierre Alliez and Mathieu Desbrun},
  title = {Valence-Driven Connectivity Encoding of 3D Meshes},
  booktitle = {Eurographics Conference Proceedings},
  year = {2001},
  pages = {480--489},
  month = aug
}

@INPROCEEDINGS{AMD02,
  author = {Pierre Alliez and Mark Meyer and Mathieu Desbrun},
  title = {Interactive Geometry Remeshing},
  booktitle = {ACM SIGGRAPH Conference},
  year = {2002},
  pages = {347--354},
  month = Jul
}

@INCOLLECTION{Alliez2007,
  author = {Alliez, P. and Ucelli, G. and Gotsman, C. and Attene, M.},
  title = {Recent Advances in Remeshing of Surfaces},
  booktitle = {Shape Analysis and Structuring},
  publisher = {Springer-Verlag},
  year = {2007},
  editor = {{Leila de Floriani and Michela Spagnuolo}},
  pages = {53--82}
}

@INPROCEEDINGS{Alumbaugh2005,
  author = {Alumbaugh, Tyler J and Jiao, Xiangmin},
  title = {{Compact Array-Based Mesh Data Structures}},
  booktitle = {Engineering},
  year = {2005},
  editor = {Hanks, Byron W},
  series = {IMR '05},
  pages = {485--503},
  publisher = {Springer Berlin Heidelberg},
  doi = {10.1007/3-540-29090-7_29},
  file = {:C\:/Dropbox/Dropbox/Paper/alumbaugh.pdf:pdf},
  keywords = {half edge,half face,mesh data structures,parallel computing},
  owner = {doubletony},
  timestamp = {2012.04.26},
  url = {http://www.springerlink.com/index/r15m46761414351g.pdf}
}

@ARTICLE{Ameur:2004,
  author = {Hend Ben Ameur and Martin Burger and Benjamin Hackl},
  title = {Level set methods for geometric inverse problems in linear elasticity},
  journal = {Inverse Problems},
  year = {2004},
  volume = {20},
  pages = {673-696},
  number = {3},
  abstract = {In this paper, we investigate the regularization and numerical solution
	of geometric inverse problems related to linear elasticity with minimal
	assumptions on the geometry of the solution. In particular, we consider
	the probably severely ill-posed reconstruction problem of a two-dimensional
	inclusion from a single boundary measurement. In order to avoid parametrizations,
	which would introduce a priori assumptions on the geometric structure
	of the solution, we employ the level set method for the numerical
	solution of the reconstruction problem. With this approach, we construct
	an evolution of shapes with a normal velocity chosen depending on
	the shape derivative of the corresponding least-squares functional
	in order to guarantee its descent. Moreover, we analyse penalization
	by perimeter as a regularization method, based on recent results
	on the convergence of Neumann problems and a generalization of Golab's
	theorem. The behaviour of the level set method and of the regularization
	procedure in the presence of noise are tested in several numerical
	examples. It turns out that reconstructions of good quality can be
	obtained only for simple shapes or for unreasonably low noise levels.
	However, it seems reasonable that the quality of reconstructions
	improves by using more than a single boundary measurement, which
	is an interesting topic for future research.},
  bdsk-url-1 = {http://stacks.iop.org/0266-5611/20/673},
  date-added = {2008-09-14 15:32:12 -0500},
  date-modified = {2008-09-14 15:32:12 -0500},
  doi = {10.1088/0266-5611/20/3/003},
  keywords = {Mathematics; Mechanics},
  url = {http://stacks.iop.org/0266-5611/20/673}
}

@ARTICLE{Amovilli:1997,
  author = {Amovilli, C. and Mennucci, B. },
  title = {Self-Consistent-Field Calculation of {Pauli} Repulsion and Dispersion
	Contributions to the Solvation Free Energy in the Polarizable Continuum
	Model},
  journal = {Journal of Physical Chemistry B},
  year = {1997},
  volume = {101},
  pages = {1051--1057},
  number = {6},
  abstract = {Abstract: By using the theory of intermolecular forces, two new expressions
	for {Pauli} repulsion and dispersion contributions to the solvation
	free energy are derived. These expressions contain explicitly the
	solute electron density and, therefore, can be used directly in the
	SCF calculation of the solute wave function within the polarizable
	continuum model (PCM). The final expressions are very simple and
	include also some intrinsic solvent properties which are, for repulsion,
	the density, the molecular weight, the number of valence electrons,
	and for dispersion, the refractive index and the ionization potential.
	This new approach does not depend on any given intermolecular potential
	and it can be adapted to any choice of basis set. For small-size
	basis sets, even minimal, the dispersion contribution is obtained
	in two steps and includes the effect of adding diffuse and polarization
	functions, not used in the wave function itself. This method has
	been implemented in our HONDO package, in a version which includes
	the cavitation contribution, determined by the Pierotti-Claverie
	method, and the polarization contribution determined by the Miertus-Scrocco-Tomasi
	method. Some preliminary results on solutes containing C, H, O, and
	N are presented for solvation in water, n-hexane, and 1-octanol.
	The quality of these results, given the simplicity of the PCM, is
	acceptable and of great interest for future developments.},
  address = {Dipartimento di Chimica e Chimica Industriale, Universit\`{a} di
	Pisa, Via Risorgimento 35, 56126 Pisa, Italy},
  bdsk-url-1 = {http://dx.doi.org/10.1021/jp9621991},
  date-added = {2008-06-29 15:18:18 -0500},
  date-modified = {2008-06-29 15:18:18 -0500},
  doi = {10.1021/jp9621991},
  keywords = {nonpolar, quantum\_mechanics, solvation},
  posted-at = {2008-06-29 21:17:39},
  priority = {0},
  url = {http://dx.doi.org/10.1021/jp9621991}
}

@ARTICLE{Ancona:1989,
  author = {Ancona, M. G. and Iafrate, G. J.},
  title = {Quantum correction to the equation of state of an electron gas in
	a semiconductor},
  journal = {Physical Review B},
  year = {1989},
  volume = {39},
  pages = {9536-9540}
}

@ARTICLE{Anderson:2009,
  author = {Anderson, C. R.},
  title = {Efficient solution of the {Schr\"{o}dinger-Poisson} equations in
	layered semiconductor devices},
  journal = {J. Comput. Phys.},
  year = {2009},
  volume = {228},
  pages = {4745-4756}
}

@BOOK{roberts,
  title = {Computational Fluid Mechanics and Heat Transfer},
  publisher = {McGraw-Hill, New York},
  year = {1984},
  author = {Anderson, D. A. and Tannehill, J. C. and Pletcher, R. H.}
}

@ARTICLE{DiffuseInterface,
  author = {D. M. Anderson and G. B. McFadden and A. A. Wheeler},
  title = {{Diffuse-Interface Methods In Fluid Mechanics}},
  journal = {Annual Review of Fluid Mechanics},
  year = {1998},
  volume = {30},
  pages = {139--165}
}

@ARTICLE{Andrei:2004,
  author = { Andrei, P. and Mayergoyz, I.},
  title = {Analysis of fluctuations in semiconductor devices through self-consistent
	{Poisson-Schr\"{o}dinger} computations },
  journal = {J. Applied Physics},
  year = {2004},
  volume = {96},
  pages = {2071-2079 },
  annote = {Analysis of fluctuations in semiconductor devices through self-consistent
	Poisson-Schrodinger computations },
  date-added = {2008-11-25 10:28:56 -0500},
  date-modified = {2008-11-25 10:28:56 -0500},
  ty = {JOUR}
}

@ARTICLE{Anguelov:2005:SSC,
  author = {Dragomir Anguelov and Praveen Srinivasan and Daphne Koller and Sebastian
	Thrun and Jim Rodgers and James Davis},
  title = {SCAPE: shape completion and animation of people},
  journal = {ACM Trans. on Graphics (SIGGRAPH)},
  year = {2005},
  volume = {24},
  pages = {408--416},
  number = {3},
  month = aug
}

@INPROCEEDINGS{anguelov-srinivasan-etal:04,
  author = {Anguelov, D. and Srinivasan, P. and Pang, H.-C. and Koller, D. and
	Thrun, S. and Davis, J.},
  title = {The Correlated Correspondence Algorithm for Unsupervised Registration
	of Nonrigid Surfaces},
  booktitle = {Advances in Neural Information Processing Systems},
  year = {2004}
}

@ARTICLE{Antosiewicz:1996,
  author = {Antosiewicz, J. and McCammon, J. A. and Gilson, M. K.},
  title = {The determinants of {p$K_a$s} in proteins},
  journal = {Biochemistry},
  year = {1996},
  volume = {35},
  pages = {7819-7833},
  number = {24},
  abstract = {Although validation studies show that theoretical models for predicting
	the pKas of ionizable groups in proteins are increasingly accurate,
	a number of important questions remain: (1) What factors limit the
	accuracy of current models? (2) How can conformational flexibility
	of proteins best be accounted for? (3) Will use of solution structures
	in the calculations, rather than crystal structures, improve the
	accuracy of the computed pKas? and (4) Why does accurate prediction
	of protein pKas seem to require that a high dielectric constant be
	assigned to the protein interior? This paper addresses these and
	related issues. Among the conclusions are the following: (1) computed
	pKas averaged over NMR structure sets are more accurate than those
	based upon single crystal structures; (2) use of atomic parameters
	optimized to reproduce hydration energies of small molecules improves
	agreement with experiment when a low protein dielectric constant
	is assumed; (3) despite use of NMR structures and optimized atomic
	parameters, pKas computed with a protein dielectric constant of 20
	are more accurate than those computed with a low protein dielectric
	constant; (4) the pKa shifts in ribonuclease A that result from phosphate
	binding are reproduced reasonably well by calculations; (5) the substantial
	pKa shifts observed in turkey ovomucoid third domain result largely
	from interactions among ionized groups; and (6) both experimental
	data and calculations indicate that proteins tend to lower the pKas
	of Asp side chains but have little overall effect upon the pKas of
	other ionizable groups.},
  address = {Nist,ctr adv res biotechnol,9600 gudelsky dr rockville, md usa 20850
	Nist,ctr adv res biotechnol rockville, md usa 20850 Univ calif san
	diego,dept chem \& biochem la jolla, ca usa 92093 Univ calif san
	diego,dept pharmacol la jolla, ca usa 92093},
  annote = {The determinants of pK(a)s in proteins; JUN 18},
  bdsk-url-1 = {http://pubs.acs.org/cgi-bin/pagelookup?bichaw/35/7819},
  date-added = {2008-09-01 13:51:26 -0500},
  date-modified = {2008-09-01 13:51:26 -0500},
  journal1 = {Biochemistry-USA},
  keywords = {Electrostatics},
  ty = {JOUR},
  url = {http://pubs.acs.org/cgi-bin/pagelookup?bichaw/35/7819}
}

@ARTICLE{Antypov:2005,
  author = {Antypov, D. and Barbosa, M. C. and Holm, C.},
  title = {Incorporation of excluded-volume correlations into Poisson-Boltzmann
	theory},
  journal = {Physical Review E},
  year = {2005},
  volume = {71},
  pages = {061106.}
}

@ARTICLE{Arakaki:2004,
  author = {Arakaki, A. K. and Zhang, Y. and Skolnick, J.},
  title = {{Large scale assesment of the utility of low resolution protein structures
	for biochemical function assignment}},
  journal = {Bioinformatics},
  year = {2004},
  volume = {20},
  pages = {1087-1096}
}

@ARTICLE{Archibald:2009b,
  author = {Archibald, R. and Gelb, A. and Saxena, R.},
  title = {Adjusting for noise in the polynomial annihilation edge detection
	method},
  year = {in preparation, 2009},
  annote = {Adjusting for noise in the polynomial annihilation edge detection
	method},
  date-added = {2008-11-25 10:28:56 -0500},
  date-modified = {2008-11-25 10:28:56 -0500},
  ty = {JOUR}
}

@ARTICLE{Archibald:2009,
  author = {Archibald, R. and Gelb, A. and Saxena, R. and Xiu, D. B.},
  title = {Discontinuity detection in multivariate space for stochastic simulations},
  journal = {J. Comput. Phys.},
  year = {2009},
  volume = {228},
  pages = {2676-2689 },
  annote = {Discontinuity detection in multivariate space for stochastic simulations},
  date-added = {2008-11-25 10:28:56 -0500},
  date-modified = {2008-11-25 10:28:56 -0500},
  ty = {JOUR}
}

@ARTICLE{Arkhipov:2006,
  author = {Arkhipov, A. and Freddolino, P. L. and Schulten, K.},
  title = {Stability and dynamics of virus capsids described by coarse-grained
	modeling},
  journal = {Structure},
  year = {2006},
  volume = {14},
  pages = {1767-1777},
  annote = {Stability and dynamics of virus capsids described by coarse-grained
	modeling},
  date-added = {2009-03-10 },
  date-modified = {2009-03-10},
  ty = {JOUR}
}

@ARTICLE{Arkhipov:2008,
  author = {Arkhipov, A. and Yin, Ying and Schulten K.},
  title = { {Four-Scale} Description of Membrane Sculpting by BAR Domains},
  journal = {Biophysical Journal},
  year = {2008},
  volume = {95},
  pages = {2806 - 2821},
  number = { }
}

@ARTICLE{Artacho:2008,
  author = {Artacho, E.},
  title = {The SIESTA method; developments and applicability},
  journal = {J. Phys.: Condens. Matter},
  year = {2008},
  volume = {20},
  pages = {064208}
}

@ARTICLE{Asenov:1998,
  author = {Asenov, A.},
  title = {Random dopant induced threshold voltage lowering and fluctuations
	in {Sub-0.1 $\mu$m MOSFET: A 3-D 'atomistic' simulation study}},
  journal = {IEEE TRansactions on Electron Devices},
  year = {1998},
  volume = {45},
  pages = {2505-2513}
}

@ARTICLE{Ashbaugh:2000,
  author = {Ashbaugh, H. S.},
  title = {Convergence of Molecular and Macroscopic Continuum Descriptions of
	Ion Hydration},
  journal = {Journal of Physical Chemistry B},
  year = {2000},
  volume = {104},
  pages = {7235-7238},
  number = {31},
  abstract = {Using computer simulations we study the boundary between explicit
	molecular and macroscopic continuum dielectric descriptions of ion
	hydration. The continuum model reasonably describes electrostatic
	potential fluctuation contributions to the hydration free energy,
	but fails to capture first-order potential contributions in the uncharged
	state. Once this contribution is accounted for, cationic and anionic
	free energies become indistinguishable with increasing size, in agreement
	with continuum model predictions. The ion radius at which the hydration
	free energies converge scales as the square root of the absolute
	charge (v = 0.54 Ã-\pm \$0.04) and compares to the length scale
	ion-water dipole interactions equal the thermal energy.},
  annote = {Convergence of Molecular and Macroscopic Continuum Descriptions of
	Ion Hydration},
  bdsk-url-1 = {http://dx.doi.org/10.1021/jp0015067},
  date-added = {2008-06-28 10:30:24 -0500},
  date-modified = {2008-06-28 10:30:24 -0500},
  keywords = {Electrostatics; Solvation},
  ty = {JOUR},
  url = {http://dx.doi.org/10.1021/jp0015067}
}

@ARTICLE{Ashbaugh:2006,
  author = {Ashbaugh, H. S. and Pratt, L. R.},
  title = {Colloquium: Scaled particle theory and the length scales of hydrophobicity},
  journal = {Reviews of Modern Physics},
  year = {2006},
  volume = {78},
  pages = {159-78},
  number = {1},
  abstract = {Hydrophobic hydration plays a crucial role in self-assembly processes
	over multiple length scales, from the microscopic origins of inert
	gas solubility in water, to the mesoscopic organization of proteins
	and surfactant structures, to macroscopic phase separation. Many
	theoretical studies focus on the molecularly detailed interactions
	between oil and water, but the extrapolation of molecular-scale models
	to larger-length-scale hydration phenomena is sometimes not warranted.
	Scaled particle theories are based upon an interpolative view of
	that microscopic<-->macroscopic issue. This Colloquium revisits the
	scaled particle theory proposed 30 years ago by Stillinger {$[$}J.
	Solution Chem. 2, 141 (1973){$]$}, adopts a practical generalization,
	and considers the implications for hydrophobic hydration in light
	of our current understanding. The generalization is based upon identifying
	a molecular length, implicit in previous applications of scaled particle
	models, which provides an effective radius for joining microscopic
	and macroscopic descriptions. It will be demonstrated that the generalized
	theory correctly reproduces many of the anomalous thermodynamic properties
	of hydrophobic hydration for molecularly sized solutes, including
	solubility minima and entropy convergence, successfully interpolates
	between the microscopic and macroscopic extremes, and provides new
	insights into the underlying molecular mechanisms. The model considered
	here serves as a reference for theories that bridge microscopic and
	macroscopic hydrophobic effects. The results are discussed in terms
	of length scales associated with component phenomena. In particular,
	first there is a discussion of the microscopic-macroscopic joining
	radius identified by the theory; then follows a discussion of the
	Tolman length that describes curvature corrections to a surface area
	model of hydrophobic hydration free energies and the length scales
	on which entropy convergence of hydration free energies are expected.},
  annote = {Colloquium: Scaled particle theory and the length scales of hydrophobicity},
  bdsk-url-1 = {http://dx.doi.org/10.1103/RevModPhys.78.159},
  date-added = {2008-09-17 09:14:02 -0500},
  date-modified = {2008-09-17 09:14:02 -0500},
  keywords = {Solvation; StatisticalMechanics},
  ty = {JOUR},
  url = {http://dx.doi.org/10.1103/RevModPhys.78.159}
}

@ARTICLE{Atalay2007,
  author = {Atalay, F Betul and Mount, David M},
  title = {{Pointerless Implementation of Hierarchical Simplicial Meshes and
	Efficient Neighbor Finding in Arbitrary Dimensions}},
  journal = {International Journal of Computational Geometry Applications},
  year = {2007},
  volume = {17},
  pages = {595},
  number = {06},
  abstract = {We describe a pointerless representation of hierarchical regular simplicial
	meshes, based on a bisection approach proposed by Maubach. We introduce
	a new labeling scheme, called an LPT code, which uniquely encodes
	the geometry of each simplex of the hi- erarchy, and we present rules
	to compute the neighbors of a given simplex efficiently through the
	use of these codes. In addition, we show how to traverse the associated
	tree and how to answer point location and interpolation queries.
	Our system works in arbitrary dimensions.},
  doi = {10.1142/S0218195907002495},
  file = {:C\:/Dropbox/Dropbox/Paper/ijcga-simplex.pdf:pdf},
  issn = {02181959},
  keywords = {hierarchical meshes,neighbor finding,pointerless data structures,simplicial
	meshes},
  owner = {doubletony},
  timestamp = {2012.04.26},
  url = {http://www.worldscinet.com/ijcga/17/1706/S0218195907002495.html}
}

@ARTICLE{Attard:1996,
  author = {Attard, P.},
  title = {Electrolytes and the Electric Double Layer},
  journal = {Adv. Chem. Phys.},
  year = {1996},
  volume = {92},
  pages = {1-159.}
}

@ARTICLE{Auffray:2008,
  author = {Auffray, C. and Nottale, L.},
  title = {Scale relativity theory and integrative systems biology: 1 Founding
	principles and scale laws },
  journal = {Prog. Biophy. Mole. Biol.},
  year = {2008},
  volume = {97},
  pages = {79-114}
}

@ARTICLE{AreaVOF,
  author = {Eugenio Aulisa and Sandro Manservisi and Ruben Scardovelli and Stephane
	Zaleski},
  title = {A Geometrical Area-preserving Volume-of-fluid Advection Method},
  journal = {J. Comput. Phys.},
  year = {2003},
  volume = {192},
  pages = {355--364},
  number = {1}
}

@INCOLLECTION{Ayers0489,
  author = {Ayers, Paul W. and Yang, W. T.},
  title = {Density-Functional Theory},
  booktitle = {Computational Medicinal Chemistry and Drug Discovery},
  publisher = {Marcel Dekker, Inc},
  year = {2004},
  editor = {Bultinck, Patrick and Winter, Hans De and Langenaeker, Wilfried and
	Tollenaere, Jan P.},
  pages = {89--118},
  address = {New York},
  endnotereftype = {Book Section},
  shorttitle = {Density-Functional Theory}
}

@ARTICLE{Ayers06224108,
  author = {Ayers, P. W. and Yang, W. T.},
  title = {Legendre-transform functionals for spin-density-functional theory},
  journal = {Journal of Chemical Physics},
  year = {2006},
  volume = {124},
  pages = {224108},
  number = {22},
  month = {Jun},
  abstract = {We provide a rigorous proof that the Hohenberg-Kohn theorem holds
	for spin densities by extending Lieb's Legendre-transform formulation
	to spin densities. The resulting spin-density-functional theory resolves
	several troublesome issues. Most importantly, the present paper provides
	an explicit construction for the spin potentials at any point along
	the adiabatic connection curve, thus providing a formal basis for
	the use of exchange-correlation functionals of the spin density in
	the Kohn-Sham density-functional theory (DFT). The practical implications
	of this result for unrestricted Kohn-Sham DFT calculations is considered,
	and the existence of holes below the Fermi level is discussed. We
	argue that an orbital's energy tends to increase as its occupation
	number increases, which provides the basis for a computational algorithm
	for determining the occupation numbers in Kohn-Sham DFT and helps
	explain the origin of Hund's rules and holes below the Fermi level.
	(c) 2006 American Institute of Physics.},
  endnotereftype = {Journal Article},
  issn = {0021-9606},
  shorttitle = {Legendre-transform functionals for spin-density-functional theory},
  url = {<Go to ISI>://000238279800012}
}

@ARTICLE{Ayyadi:2005,
  author = {Ayyadi, A. E. and J\"{u}ngel, A.},
  title = {Semiconductor simulations using a coulped quantum drift-diffusion
	{Schr\"{o}dinger-Poisson} model},
  journal = {SIAM J. Appl. Math},
  year = {2005},
  volume = {66},
  pages = {544-572}
}

@ARTICLE{Azuara:2006,
  author = {Azuara, C. and Lindahl E. and Koehl, P. and Orland, H. and Delarue, M.},
  title = {PDB-Hydro: incorporating dipolar solvents with variable density in
	the Poisson-Boltzmann treatment of macromolecule electrostatics},
  journal = {Nucleic Acids Research},
  year = {2006},
  volume = {34},
  pages = {W38-CW42},
  abstract = {This is in effect a generalization of the Langevin Dipoles-Protein
	Dipoles (LDPD) model advocated by Warshel and colleagues, with the
	key additional feature that the dipoles are now allowed to have a
	variable density at each grid point around the solute. Also, it leads
	to a solvent with a variable dielectric constant that is self-consistently
	determined by the system.}
}

@ARTICLE{Azuara:2008,
  author = {Azuara, C. and Orland, H. and Bon, M. and Koehl, P. and Delarue,
	M.},
  title = {Incorporating Dipolar Solvents with Variable Density in Poisson-Boltzmann
	Electrostatics},
  journal = {Biophysical Journal},
  year = {2008},
  volume = {95},
  pages = {5587?C5605},
  abstract = {The solvent region is no longer modeled as a homogeneous dielectric
	media but rather as an assembly of self-orienting interacting dipoles
	of variable density. The method effectively unifies both the Poisson-centric
	view and the Langevin Dipole model. The model results in a variable
	dielectric constant in the solvent region and also in a variable
	solvent density that depends on the nature of the closest exposed
	solute atoms.}
}

@ARTICLE{Babuska:1970,
  author = {Babu{\v s}ka, I.},
  title = {The finite element method for elliptic equations with discontinuous
	coefficients},
  journal = { Computing},
  year = {1970},
  volume = {5},
  pages = {207-213},
  annote = {The finite element method for elliptic equations with discontinuous
	coefficients},
  date-added = {2008-09-19 10:28:56 -0500},
  date-modified = {2008-09-19 10:28:56 -0500},
  ty = {JOUR}
}

@ARTICLE{MAZC10,
  author = {Badieirostami, M. and Adibi, A. and Zhou, H. M. and Chow, S.N.},
  title = {Wiener Chaos Expansion and Simulation of Electromagnetic Wave Propagation
	Excited by a Spatially Incoherent Source},
  journal = {SIAM Multiscale Modeling and Simulation},
  year = {2010},
  volume = {8}
}

@ARTICLE{MAZC07,
  author = {Badieirostami, M. and Adibi, A. and Zhou, H. M. and Chow, S.N.},
  title = {Model for efficient simulation of spatially incoherent light using
	the Wiener chaos expansion method},
  journal = {Opt. Lett.},
  year = {2007},
  volume = {32},
  pages = {3188-3190}
}

@ARTICLE{Baeumer:2008,
  author = {Baeumer, B. and Kovacs, M. and Meerschaert, M.M.},
  title = {Numerical solutions for fractional reaction-diffusion equations},
  journal = {Computers and Mathematics with Applications},
  year = {2008},
  volume = {55},
  pages = {2212-2226},
  number = { }
}

@ARTICLE{Baeumer:2001,
  author = {Baeumer,B. and Meerschaert,M.M. and Benson,D.A. and Wheatcraft,S.W.},
  title = {Subordinated advection-dispersion equation for contaminant transport},
  journal = {Water Resour.Res.},
  year = {2001},
  volume = {37},
  pages = {1543-1550},
  number = { }
}

@ARTICLE{Bai:2007a,
  author = {Bai, J and Feng, XC},
  title = {Fractional-order anisotropic diffusion for image denoising},
  journal = {IEEE Trans Image Process},
  year = {2007},
  volume = {16},
  pages = {2492-2502},
  number = {10}
}

@ARTICLE{JBai:2007,
  author = {Bai, J and Feng, X. C.},
  title = {Fractional-Order Anisotropic Diffusion for Image Denoising},
  journal = {IEEE Trans. Image Proc. },
  year = {2007},
  volume = {16},
  pages = {2492 -502}
}

@ARTICLE{Baik016437,
  author = {Baik, M. H. and Silverman, J. S. and Yang, I. V. and Ropp, P. A.
	and Szalai, V. A. and Yang, W. T. and Thorp, H. H.},
  title = {Using density functional theory to design DNA base analogues with
	low oxidation potentials},
  journal = {Journal of Physical Chemistry B},
  year = {2001},
  volume = {105},
  pages = {6437-6444},
  number = {27},
  month = {Jul}
}

@ARTICLE{BXZ09,
  author = {C. Bajaj and G. Xu and Q. Zhang},
  title = {A Fast Variational Method for the Construction of Smooth Molecular
	Surfaces},
  journal = {Computer Methods in Applied Mechanics and Engineering},
  year = {2009},
  owner = {Yiying},
  timestamp = {2009.03.26}
}

@INCOLLECTION{Baker:2005a,
  author = {Baker, N. A.},
  title = {Biomolecular Applications of {{Poisson-Boltzmann}} Methods},
  booktitle = {Reviews in Computational Chemistry},
  publisher = {John Wiley and Sons},
  year = {2005},
  editor = {Lipkowitz, K. B. and Larter, R. and Cundari, T. R.},
  volume = {21},
  address = {Hoboken, NJ},
  address1 = {21},
  annote = {Biomolecular Applications of PoissonÃ¢Â€Â“Boltzmann Methods},
  date-added = {2008-09-03 13:21:41 -0500},
  date-modified = {2008-09-03 13:21:41 -0500},
  ty = {CHAP}
}

@ARTICLE{Baker:2005,
  author = {Baker, N. A.},
  title = {Improving implicit solvent simulations: a {Poisson}-centric view},
  journal = {Current Opinion in Structural Biology},
  year = {2005},
  volume = {15},
  pages = {137-43},
  number = {2},
  abstract = {Recent developments in implicit solvent models may be compared in
	terms of accuracy and computational efficiency. Based on improvements
	in the accuracy of generalized Born methods and the speed of PoissonÃ¢Â€Â“Boltzmann
	solvers, it appears that the two techniques are converging to a point
	at which both will be suitable for simulating certain types of biomolecular
	systems over sizable time and length scales.},
  keywords = {Electrostatics},
  ty = {JOUR},
  url = {http://dx.doi.org/10.1016/j.sbi.2005.02.001}
}

@ARTICLE{Baker:2004,
  author = {Baker, N. A.},
  title = {{P}oisson-{B}oltzmann Methods for Biomolecular Electrostatics},
  journal = {Methods in Enzymology},
  year = {2004},
  volume = {383},
  pages = {94-118},
  annote = {{Poisson-Boltzmann} Methods for Biomolecular Electrostatics; Baker2004},
  bdsk-file-1 = {YnBsaXN0MDDUAQIDBAUGCQpYJHZlcnNpb25UJHRvcFkkYXJjaGl2ZXJYJG9iamVjdHMSAAGGoNE
	HCFRyb290gAFfEA9OU0tleWVkQXJjaGl2ZXKoCwwXGBkdJCVVJG51bGzTDQ4PEBEUViRjbGFzc1
	dOUy5rZXlzWk5TLm9iamVjdHOAB6ISE4ACgAOiFRaABIAGWWFsaWFzRGF0YVxyZWxhdGl2ZVBhd
	GjSDRobHFdOUy5kYXRhgAVPEQGmAAAAAAGmAAIAAAxNYWNpbnRvc2ggSEQAAAAAAAAAAAAAAAAA
	AADD4v5NSCsAAAAZYksOMjAwNC1CYWtlci5wZGYAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAA
	AAAAAAAAAAAAAAAAAAAAAAAAAAAAAABliUL8eZUIAAAAAAAAAAAAEAAQAAAkgAAAAAAAAAAAAAA
	AAAAAAB0FyY2hpdmUAABAACAAAw+NSrQAAABEACAAAvx6rkgAAAAEAFAAZYksAGWIDAAqkKAAKp
	BEAAHrcAAIARE1hY2ludG9zaCBIRDpVc2VyczpiYWtlcjpEb2N1bWVudHM6UmVmZXJlbmNlczpB
	cmNoaXZlOjIwMDQtQmFrZXIucGRmAA4AHgAOADIAMAAwADQALQBCAGEAawBlAHIALgBwAGQAZgA
	PABoADABNAGEAYwBpAG4AdABvAHMAaAAgAEgARAASADdVc2Vycy9iYWtlci9Eb2N1bWVudHMvUm
	VmZXJlbmNlcy9BcmNoaXZlLzIwMDQtQmFrZXIucGRmAAATAAEvAAAVAAIADP//AADSHh8gIVgkY
	2xhc3Nlc1okY2xhc3NuYW1loyEiI11OU011dGFibGVEYXRhVk5TRGF0YVhOU09iamVjdF8QNy4u
	Ly4uLy4uLy4uL0RvY3VtZW50cy9SZWZlcmVuY2VzL0FyY2hpdmUvMjAwNC1CYWtlci5wZGbSHh8
	mJ6InI1xOU0RpY3Rpb25hcnkACAARABoAHwApADIANwA6AD8AQQBTAFwAYgBpAHAAeACDAIUAiA
	CKAIwAjwCRAJMAnQCqAK8AtwC5AmMCaAJxAnwCgAKOApUCngLYAt0C4AAAAAAAAAIBAAAAAAAAA
	CgAAAAAAAAAAAAAAAAAAALt},
  bdsk-url-1 = {http://www.sciencedirect.com/science/article/B7CV2-4C47J19-6/2/5c077798e7534bffa0a9b9e2c6959e22},
  date-added = {2008-09-01 13:56:16 -0500},
  date-modified = {2008-09-01 13:56:16 -0500},
  keywords = {Electrostatics},
  ty = {JOUR},
  url = {http://www.sciencedirect.com/science/article/B7CV2-4C47J19-6/2/5c077798e7534bffa0a9b9e2c6959e22}
}

@INCOLLECTION{Baker:2006,
  author = {Baker, N. A. and Bashford, D. and Case, D. A.},
  title = {Implicit solvent electrostatics in biomolecular simulation},
  booktitle = {New Algorithms for Macromolecular Simulation},
  publisher = {Springer},
  year = {2006},
  editor = {Leimkuhler, B. and Chipot, C. and Elber, R. and Laaksonen, A. and
	Mark, A. and Schlick, T. and Schutte, C. and Skeel, R.},
  bdsk-file-1 = {YnBsaXN0MDDUAQIDBAUGCQpYJHZlcnNpb25UJHRvcFkkYXJjaGl2ZXJYJG9iamVjdHMSAAGGoNE
	HCFRyb290gAFfEA9OU0tleWVkQXJjaGl2ZXKoCwwXGBkdJCVVJG51bGzTDQ4PEBEUViRjbGFzc1
	dOUy5rZXlzWk5TLm9iamVjdHOAB6ISE4ACgAOiFRaABIAGWWFsaWFzRGF0YVxyZWxhdGl2ZVBhd
	GjSDRobHFdOUy5kYXRhgAVPEQHWAAAAAAHWAAIAAAxNYWNpbnRvc2ggSEQAAAAAAAAAAAAAAAAA
	AADD4v5NSCsAAAAZYksaMjAwNi1CYWtlckJhc2hmb3JkQ2FzZS5wZGYAAAAAAAAAAAAAAAAAAAA
	AAAAAAAAAAAAAAAAAAAAAAAAAAAAAABliUsA/IcwAAAAAAAAAAAAEAAQAAAkgAAAAAAAAAAAAAA
	AAAAAAB0FyY2hpdmUAABAACAAAw+NSrQAAABEACAAAwD92LAAAAAEAFAAZYksAGWIDAAqkKAAKp
	BEAAHrcAAIAUE1hY2ludG9zaCBIRDpVc2VyczpiYWtlcjpEb2N1bWVudHM6UmVmZXJlbmNlczpB
	cmNoaXZlOjIwMDYtQmFrZXJCYXNoZm9yZENhc2UucGRmAA4ANgAaADIAMAAwADYALQBCAGEAawB
	lAHIAQgBhAHMAaABmAG8AcgBkAEMAYQBzAGUALgBwAGQAZgAPABoADABNAGEAYwBpAG4AdABvAH
	MAaAAgAEgARAASAENVc2Vycy9iYWtlci9Eb2N1bWVudHMvUmVmZXJlbmNlcy9BcmNoaXZlLzIwM
	DYtQmFrZXJCYXNoZm9yZENhc2UucGRmAAATAAEvAAAVAAIADP//AADSHh8gIVgkY2xhc3Nlc1ok
	Y2xhc3NuYW1loyEiI11OU011dGFibGVEYXRhVk5TRGF0YVhOU09iamVjdF8QQy4uLy4uLy4uLy4
	uL0RvY3VtZW50cy9SZWZlcmVuY2VzL0FyY2hpdmUvMjAwNi1CYWtlckJhc2hmb3JkQ2FzZS5wZG
	bSHh8mJ6InI1xOU0RpY3Rpb25hcnkACAARABoAHwApADIANwA6AD8AQQBTAFwAYgBpAHAAeACDA
	IUAiACKAIwAjwCRAJMAnQCqAK8AtwC5ApMCmAKhAqwCsAK+AsUCzgMUAxkDHAAAAAAAAAIBAAAA
	AAAAACgAAAAAAAAAAAAAAAAAAAMp},
  date-added = {2008-09-01 13:58:22 -0500},
  date-modified = {2008-09-01 13:58:22 -0500},
  keywords = {Mathematics, Electrostatics}
}

@INCOLLECTION{Baker:2003,
  author = {Baker, N. A. and McCammon, J. A.},
  title = {Electrostatic Interactions},
  booktitle = {Structural Bioinformatics},
  publisher = {John Wiley \& Sons, Inc.},
  year = {2003},
  editor = {Bourne, P. and Weissig, H.},
  pages = {427-440},
  address = {New York},
  annote = {Electrostatic interactions},
  date-added = {2008-09-01 13:56:00 -0500},
  date-modified = {2008-09-01 13:56:00 -0500},
  keywords = {Electrostatics},
  ty = {CHAP}
}

@ARTICLE{Baker:2001b,
  author = {Nathan A. Baker and David Sept and Michael J. Holst and J. Andrew
	Mccammon},
  title = {The adaptive multilevel finite element solution of the {{Poisson-Boltzmann}}
	equation on massively parallel computers},
  journal = {IBM Journal of Research and Development},
  year = {2001},
  volume = {45},
  pages = {427-438},
  number = {3-4},
  address = {Univ Calif San Diego La Jolla, CA USA 92093 Baker, NA nbaker{\char64}wasabi.ucsd.edu
	Dept Chem \& Biochem, 9500 Gilman Dr,Mail Code 0365 Sept, D dsept@biomed.wustl.edu
	Holst, MJ mholst@math.ucsd.edu McCammon, JA jmccammon@ucsd.edu Univ
	Calif San Diego La Jolla, CA USA 92093 Dept Chem \& Biochem Univ
	Calif San Diego La Jolla, CA USA 92093 Dept Math Washington Univ
	St Louis, MO USA 63130 Dept Biomed Engn Univ Calif San Diego La Jolla,
	CA USA 92093 Dept Pharmacol},
  annote = {The adaptive multilevel finite element solution of the {Poisson-Boltzmann}
	equation on massively parallel computers},
  bdsk-file-1 = {YnBsaXN0MDDUAQIDBAUGCQpYJHZlcnNpb25UJHRvcFkkYXJjaGl2ZXJYJG9iamVjdHMSAAGGoNE
	HCFRyb290gAFfEA9OU0tleWVkQXJjaGl2ZXKoCwwXGBkdJCVVJG51bGzTDQ4PEBEUViRjbGFzc1
	dOUy5rZXlzWk5TLm9iamVjdHOAB6ISE4ACgAOiFRaABIAGWWFsaWFzRGF0YVxyZWxhdGl2ZVBhd
	GjSDRobHFdOUy5kYXRhgAVPEQHqAAAAAAHqAAIAAAxNYWNpbnRvc2ggSEQAAAAAAAAAAAAAAAAA
	AADD4v5NSCsAAAAZYksfMjAwMS1CYWtlclNlcHRIb2xzdE1jQ2FtbW9uLnBkZgAAAAAAAAAAAAA
	AAAAAAAAAAAAAAAAAAAAAAAAAAAAAABlidcM6CM9QREYgcHJ2dwAEAAQAAAkgAAAAAAAAAAAAAA
	AAAAAAB0FyY2hpdmUAABAACAAAw+NSrQAAABEACAAAwzpPHwAAAAEAFAAZYksAGWIDAAqkKAAKp
	BEAAHrcAAIAVU1hY2ludG9zaCBIRDpVc2VyczpiYWtlcjpEb2N1bWVudHM6UmVmZXJlbmNlczpB
	cmNoaXZlOjIwMDEtQmFrZXJTZXB0SG9sc3RNY0NhbW1vbi5wZGYAAA4AQAAfADIAMAAwADEALQB
	CAGEAawBlAHIAUwBlAHAAdABIAG8AbABzAHQATQBjAEMAYQBtAG0AbwBuAC4AcABkAGYADwAaAA
	wATQBhAGMAaQBuAHQAbwBzAGgAIABIAEQAEgBIVXNlcnMvYmFrZXIvRG9jdW1lbnRzL1JlZmVyZ
	W5jZXMvQXJjaGl2ZS8yMDAxLUJha2VyU2VwdEhvbHN0TWNDYW1tb24ucGRmABMAAS8AABUAAgAM
	//8AANIeHyAhWCRjbGFzc2VzWiRjbGFzc25hbWWjISIjXU5TTXV0YWJsZURhdGFWTlNEYXRhWE5
	TT2JqZWN0XxBILi4vLi4vLi4vLi4vRG9jdW1lbnRzL1JlZmVyZW5jZXMvQXJjaGl2ZS8yMDAxLU
	Jha2VyU2VwdEhvbHN0TWNDYW1tb24ucGRm0h4fJieiJyNcTlNEaWN0aW9uYXJ5AAgAEQAaAB8AK
	QAyADcAOgA/AEEAUwBcAGIAaQBwAHgAgwCFAIgAigCMAI8AkQCTAJ0AqgCvALcAuQKnAqwCtQLA
	AsQC0gLZAuIDLQMyAzUAAAAAAAACAQAAAAAAAAAoAAAAAAAAAAAAAAAAAAADQg==},
  bdsk-url-1 = {http://www.research.ibm.com/journal/rd/453/baker.html},
  bdsk-url-2 = {http://dx.doi.org/10.1147/rd.453.0427},
  journal1 = {Ibm J Res Develop},
  keywords = {Electrostatics},
  ty = {JOUR},
  url = {http://www.research.ibm.com/journal/rd/453/baker.html}
}

@ARTICLE{Baker:2001,
  author = {Baker, N. A. and Sept, D. and Joseph, S. and Holst, M. J. and McCammon,
	J. A.},
  title = {Electrostatics of nanosystems: Application to microtubules and the
	ribosome},
  journal = {Proceedings of the National Academy of Sciences of the United States
	of America},
  year = {2001},
  volume = {98},
  pages = {10037-10041},
  number = {18},
  abstract = {Evaluation of the electrostatic properties of biomolecules has become
	a standard practice in molecular biophysics. Foremost among the models
	used to elucidate the electrostatic potential is the {Poisson-Boltzmann}
	equation; however, existing methods for solving this equation have
	limited the scope of accurate electrostatic calculations to relatively
	small biomolecular systems. Here we present the application of numerical
	methods to enable the trivially parallel solution of the {Poisson-Boltzmann}
	equation for supramolecular structures that are orders of magnitude
	larger in size. As a demonstration of this methodology, electrostatic
	potentials have been calculated for large microtubule and ribosome
	structures. The results point to the likely role of electrostatics
	in a variety of activities of these structures.},
  annote = {Electrostatics of nanosystems: Application to microtubules and the
	ribosome; APBS},
  bdsk-file-1 = {YnBsaXN0MDDUAQIDBAUGCQpYJHZlcnNpb25UJHRvcFkkYXJjaGl2ZXJYJG9iamVjdHMSAAGGoNE
	HCFRyb290gAFfEA9OU0tleWVkQXJjaGl2ZXKoCwwXGBkdJCVVJG51bGzTDQ4PEBEUViRjbGFzc1
	dOUy5rZXlzWk5TLm9iamVjdHOAB6ISE4ACgAOiFRaABIAGWWFsaWFzRGF0YVxyZWxhdGl2ZVBhd
	GjSDRobHFdOUy5kYXRhgAVPEQH8AAAAAAH8AAIAAAxNYWNpbnRvc2ggSEQAAAAAAAAAAAAAAAAA
	AADD4v5NSCsAAAAZYksfMjAwMS1CYWtlclNlcHRKb3NlcGgjMTk2MjU4LnBkZgAAAAAAAAAAAAA
	AAAAAAAAAAAAAAAAAAAAAAAAAAAAAABliWMM6C7hQREYgcHJ2dwAEAAQAAAkgAAAAAAAAAAAAAA
	AAAAAAB0FyY2hpdmUAABAACAAAw+NSrQAAABEACAAAwzpSCAAAAAEAFAAZYksAGWIDAAqkKAAKp
	BEAAHrcAAIAVU1hY2ludG9zaCBIRDpVc2VyczpiYWtlcjpEb2N1bWVudHM6UmVmZXJlbmNlczpB
	cmNoaXZlOjIwMDEtQmFrZXJTZXB0Sm9zZXBoIzE5NjI1OC5wZGYAAA4ATAAlADIAMAAwADEALQB
	CAGEAawBlAHIAUwBlAHAAdABKAG8AcwBlAHAAaABIAG8AbABzAHQATQBjAEMAYQBtAG0AbwBuAC
	4AcABkAGYADwAaAAwATQBhAGMAaQBuAHQAbwBzAGgAIABIAEQAEgBOVXNlcnMvYmFrZXIvRG9jd
	W1lbnRzL1JlZmVyZW5jZXMvQXJjaGl2ZS8yMDAxLUJha2VyU2VwdEpvc2VwaEhvbHN0TWNDYW1t
	b24ucGRmABMAAS8AABUAAgAM//8AANIeHyAhWCRjbGFzc2VzWiRjbGFzc25hbWWjISIjXU5TTXV
	0YWJsZURhdGFWTlNEYXRhWE5TT2JqZWN0XxBOLi4vLi4vLi4vLi4vRG9jdW1lbnRzL1JlZmVyZW
	5jZXMvQXJjaGl2ZS8yMDAxLUJha2VyU2VwdEpvc2VwaEhvbHN0TWNDYW1tb24ucGRm0h4fJieiJ
	yNcTlNEaWN0aW9uYXJ5AAgAEQAaAB8AKQAyADcAOgA/AEEAUwBcAGIAaQBwAHgAgwCFAIgAigCM
	AI8AkQCTAJ0AqgCvALcAuQK5Ar4CxwLSAtYC5ALrAvQDRQNKA00AAAAAAAACAQAAAAAAAAAoAAA
	AAAAAAAAAAAAAAAADWg==},
  bdsk-url-1 = {http://www.pnas.org/cgi/content/full/98/18/10037},
  date-added = {2008-06-28 10:34:42 -0500},
  date-modified = {2008-06-28 10:34:42 -0500},
  journal1 = {Proc Nat Acad Sci USA},
  keywords = {Electrostatics; Biological_systems},
  ty = {JOUR},
  url = {http://www.pnas.org/cgi/content/full/98/18/10037}
}

@ARTICLE{Baker:2000a,
  author = {Baker, N. and Holst, M. and Wang, F.},
  title = {Adaptive multilevel finite element solution of the {{Poisson-Boltzmann}}
	equation {II}. {R}efinement at solvent-accessible surfaces in biomolecular
	systems},
  journal = {Journal of Computational Chemistry},
  year = {2000},
  volume = {21},
  pages = {1343-1352},
  number = {15},
  abstract = {We apply the adaptive multilevel finite element techniques (Holst,
	Baker, and Wang {$[$}21{$]$}) to the nonlinear {Poisson-Boltzmann}
	equation (PBE) in the context of biomolecules. Fast and accurate
	numerical solution of the PBE in this setting is usually difficult
	to accomplish due to presence of discontinuous coefficients, delta
	functions, three spatial dimensions, unbounded domains, and rapid
	(exponential) nonlinearity. However, these adaptive techniques have
	shown substantial improvement in solution time over conventional
	uniform-mesh finite difference methods. One important aspect of the
	adaptive multilevel finite element method is the robust a posteriori
	error estimators necessary to drive the adaptive refinement routines.
	This article discusses the choice of solvent accessibility for a
	posteriori error estimation of PBE solutions and the implementation
	of such routines in the Adaptive {Poisson-Boltzmann} Solver (APBS)
	software package based on the Manifold Code (MC) libraries. Results
	are shown for the application of this method to several biomolecular
	systems. Ã‚Â??000 John Wiley \& Sons, Inc. J Comput Chem 21:
	1343-1352, 2000},
  annote = {Adaptive multilevel finite element solution of the {Poisson-Boltzmann}
	equation {II}. Refinement at solvent-accessible surfaces in biomolecular
	systems; BakerEtal2000},
  bdsk-file-1 = {YnBsaXN0MDDUAQIDBAUGCQpYJHZlcnNpb25UJHRvcFkkYXJjaGl2ZXJYJG9iamVjdHMSAAGGoNE
	HCFRyb290gAFfEA9OU0tleWVkQXJjaGl2ZXKoCwwXGBkdJCVVJG51bGzTDQ4PEBEUViRjbGFzc1
	dOUy5rZXlzWk5TLm9iamVjdHOAB6ISE4ACgAOiFRaABIAGWWFsaWFzRGF0YVxyZWxhdGl2ZVBhd
	GjSDRobHFdOUy5kYXRhgAVPEQHKAAAAAAHKAAIAAAxNYWNpbnRvc2ggSEQAAAAAAAAAAAAAAAAA
	AADD4v5NSCsAAAAZYksXMjAwMC1CYWtlckhvbHN0V2FuZy5wZGYAAAAAAAAAAAAAAAAAAAAAAAA
	AAAAAAAAAAAAAAAAAAAAAAAAAAAAAABlijMNHOBtQREYgcHJ2dwAEAAQAAAkgAAAAAAAAAAAAAA
	AAAAAAB0FyY2hpdmUAABAACAAAw+NSrQAAABEACAAAw0d+awAAAAEAFAAZYksAGWIDAAqkKAAKp
	BEAAHrcAAIATU1hY2ludG9zaCBIRDpVc2VyczpiYWtlcjpEb2N1bWVudHM6UmVmZXJlbmNlczpB
	cmNoaXZlOjIwMDAtQmFrZXJIb2xzdFdhbmcucGRmAAAOADAAFwAyADAAMAAwAC0AQgBhAGsAZQB
	yAEgAbwBsAHMAdABXAGEAbgBnAC4AcABkAGYADwAaAAwATQBhAGMAaQBuAHQAbwBzAGgAIABIAE
	QAEgBAVXNlcnMvYmFrZXIvRG9jdW1lbnRzL1JlZmVyZW5jZXMvQXJjaGl2ZS8yMDAwLUJha2VyS
	G9sc3RXYW5nLnBkZgATAAEvAAAVAAIADP//AADSHh8gIVgkY2xhc3Nlc1okY2xhc3NuYW1loyEi
	I11OU011dGFibGVEYXRhVk5TRGF0YVhOU09iamVjdF8QQC4uLy4uLy4uLy4uL0RvY3VtZW50cy9
	SZWZlcmVuY2VzL0FyY2hpdmUvMjAwMC1CYWtlckhvbHN0V2FuZy5wZGbSHh8mJ6InI1xOU0RpY3
	Rpb25hcnkACAARABoAHwApADIANwA6AD8AQQBTAFwAYgBpAHAAeACDAIUAiACKAIwAjwCRAJMAn
	QCqAK8AtwC5AocCjAKVAqACpAKyArkCwgMFAwoDDQAAAAAAAAIBAAAAAAAAACgAAAAAAAAAAAAA
	AAAAAAMa},
  bdsk-url-1 = {http://dx.doi.org/10.1002/1096-987X(20001130)21:15%3C1343::AID-JCC2%3E3.0.CO;2-K},
  bdsk-url-2 = {http://dx.doi.org/10.1002/1096-987X(20001130)21:15%3C1343::AID-JCC2%3E3.0.CO;2-K},
  date-added = {2008-06-29 14:46:01 -0500},
  date-modified = {2008-06-29 14:46:01 -0500},
  doi = {10.1002/1096-987X(20001130)21:15<1343::AID-JCC2>3.0.CO;2-K},
  journal1 = {J Comput Chem},
  keywords = {Electrostatics},
  ty = {JOUR},
  url = {http://dx.doi.org/10.1002/1096-987X(20001130)21:15<1343::AID-JCC2>3.0.CO;2-K}
}

@ARTICLE{Baker:1999g,
  author = {Baker, T.S. and Olson, N. H. and Fuller, S. D.},
  title = {Adding the third dimension to virus life cycles: three-dimensional
	reconstruction of icosahedral viruses from cryo-electron micrographs},
  journal = {Microbiol. Molec. Biol. Rev.},
  year = {1999},
  volume = {63},
  pages = {862-922},
  annote = {Adding the third dimension to virus life cycles: three-dimensional
	reconstruction of icosahedral viruses from cryo-electron micrographs},
  date-added = {2009-03-10 },
  date-modified = {2009-03-10},
  ty = {JOUR}
}

@ARTICLE{Balamurugan08174105,
  author = {Balamurugan, D. and Yang, W. T. and Beratan, D. N.},
  title = {Exploring chemical space with discrete, gradient, and hybrid optimization
	methods},
  journal = {Journal of Chemical Physics},
  year = {2008},
  volume = {129},
  pages = {174105},
  number = {17},
  month = {Nov},
  abstract = {Discrete, gradient, and hybrid optimization methods are applied to
	the challenge of discovering molecules with optimized properties.
	The cost and performance of the approaches were studied using a tight-binding
	model to maximize the static first electronic hyperpolarizability
	of molecules. Our analysis shows that discrete branch and bound methods
	provide robust strategies for inverse chemical design involving diverse
	chemical structures. Based on the linear combination of atomic potentials,
	a hybrid discrete-gradient optimization strategy significantly improves
	the performance of the gradient methods. The hybrid method performs
	better than dead-end elimination and competes with branch and bound
	and genetic algorithms. The branch and bound methods for these model
	Hamiltonians are more cost effective than genetic algorithms for
	moderate-sized molecular optimization.},
  endnotereftype = {Journal Article},
  issn = {0021-9606},
  shorttitle = {Exploring chemical space with discrete, gradient, and hybrid optimization
	methods},
  url = {<Go to ISI>://000260777400009}
}

@ARTICLE{Ball:2001,
  author = {Ball, F. G. and Rice, J. A. },
  title = {Stochastic models for ion channels: Introduction and bibliography},
  journal = {Mathematical Biosciences},
  year = {1992},
  volume = {112},
  pages = {189-206},
  number = {2}
}

@ARTICLE{Banavali:2002,
  author = {Banavali, N. K. and Im, W. and Roux, B.},
  title = {Electrostatic free energy calculations using the generalized solvent
	boundary potential method},
  journal = {Journal of Chemical Physics},
  year = {2002},
  volume = {117},
  pages = {7381-8},
  number = {15},
  abstract = {Free energy perturbation (FEP) calculations using all-atom molecular
	dynamics simulations with a large number of explicit solvent molecules
	are a powerful approach to study ligandÃ¢Â€Â“macromolecule
	association processes at the atomic level. One strategy to carry
	out FEP calculations efficiently and reduce computational time is
	to consider the explicit dynamics of only a small number of atoms
	in a localized region around the ligand. Such an approximation is
	motivated by the observation that the factors governing binding specificity
	are dominated by interactions in the vicinity of the ligand. However,
	a straightforward truncation of the system may yield inaccurate results
	as the influence exerted by the remote regions of the macromolecule
	and the surrounding solvent through long-range electrostatic effects
	may be significant. To obtain meaningful results, it is important
	to incorporate the influence of the remote regions of the ligandÃ¢Â€Â“macromolecule
	complex implicitly using some effective potential. The generalized
	solvent boundary potential (GSBP) that was developed recently {$[$}W.
	Im, S. BernÃƒÂ¨che, and B. Roux, J. Chem. Phys. 114, 2924 (2001){$]$}
	is an efficient computational method to represent the long-range
	electrostatic interactions arising from remote (outer) regions in
	simulations of a localized (inner) region with a small number of
	explicit atoms. In the present work, FEP calculations combined with
	GSBP are used to illustrate the importance of these long-range electrostatic
	factors in estimation of the charging free energy of an aspartate
	ligand bound to the aspartyl-tRNA synthetase. Calculations with explicit
	spherical simulation inner regions of different radii are used to
	test the accuracy of the GSBP method and also illustrate the importance
	of explicit protein and solvent dynamics in the free energy estimation.
	The influence of the represented outer region is tested using separate
	simulations in which the reaction field and/or the protein static
	field are excluded. Both components are shown to be essential to
	obtain quantitatively meaningful results. The ability of implicitly
	treating the influence of protein fluctuations in the outer region
	using a protein dielectric constant is examined. It is shown that
	accurate charging free energy calculations can be performed for this
	system with a spherical region of 15 to 20 Ãƒ radius, which roughly
	corresponds to 1500Ã¢Â€Â-500 moving atoms. The results indicate
	that GSBP in combination with FEP calculations is a precise and efficient
	approach to include long-range electrostatic effects in the study
	of ligand binding to large macromolecules.},
  annote = {Electrostatic free energy calculations using the generalized solvent
	boundary potential method; *; This describes the application of a
	hybrid explicit-implicit solvent method to free energy calculations
	and demonstrates good accuracy with significant speed-up in the calculation.
	In general, this hybrid method appears to be very useful for relatively
	rigid sites but may require some modification to handles systems
	undergoing substantial conformational changes.},
  bdsk-url-1 = {http://dx.doi.org/10.1063/1.1507108},
  date-added = {2008-09-15 10:07:25 -0500},
  date-modified = {2008-09-15 10:07:25 -0500},
  keywords = {Multiscale; Electrostatics; Solvation},
  ty = {JOUR},
  url = {http://dx.doi.org/10.1063/1.1507108}
}

@ARTICLE{Bank:2003,
  author = {Bank, R. E. and Holst, M.},
  title = {A New Paradigm for Parallel Adaptive Meshing Algorithms},
  journal = {SIAM Review},
  year = {2003},
  volume = {45},
  pages = {291-323},
  number = {2},
  abstract = {We present a new approach to the use of parallel computers with adaptive
	finite element methods. This approach addresses the load balancing
	problem in a new way, requiring far less communication than current
	approaches. It also allows existing sequential adaptive PDE codes
	such as PLTMG and MC to run in a parallel environment without a large
	investment in recoding. In this new approach, the load balancing
	problem is reduced to the numerical solution of a small elliptic
	problem on a single processor, using a sequential adaptive solver,
	without requiring any modifications to the sequential solver. The
	small elliptic problem is used to produce a posteriori error estimates
	to predict future element densities in the mesh, which are then used
	in a weighted recursive spectral bisection of the initial mesh. The
	bulk of the calculation then takes place independently on each processor,
	with no communication, using possibly the same sequential adaptive
	solver. Each processor adapts its region of the mesh independently,
	and a nearly load-balanced mesh distribution is usually obtained
	as a result of the initial weighted spectral bisection. Only the
	initial fan-out of the mesh decomposition to the processors requires
	communication. Two additional steps requiring boundary exchange communication
	may be employed after the individual processors reach an adapted
	solution, namely, the construction of a global conforming mesh from
	the independent subproblems, followed by a final smoothing phase
	using the subdomain solutions as an initial guess. We present a series
	of convincing numerical experiments that illustrate the effectiveness
	of this approach. The justification of the initial refinement prediction
	step, as well as the justification of skipping the two communication-intensive
	steps, is supported by some recent {$[$}J. Xu and A. Zhou, Math.
	Comp., 69 (2000), pp. 881--909{$]$} and not so recent {$[$}J. A.
	Nitsche and A. H. Schatz, Math. Comp., 28 (1974), pp. 937--958; A.
	H. Schatz and L. B. Wahlbin, Math. Comp., 31 (1977), pp. 414--442;
	A. H. Schatz and L. B. Wahlbin, Math. Comp., 64 (1995), pp. 907--928{$]$}
	results on local a priori and a posteriori error estimation. This
	revision of the original article {$[$}R. E. Bank and M. J. Holst,
	SIAM J. Sci. Comput., 22 (2000), pp. 1411--1443{$]$} updates the
	numerical experiments and reflects the knowledge we have gained since
	the original paper appeared.},
  annote = {A New Paradigm for Parallel Adaptive Meshing Algorithms},
  bdsk-url-1 = {http://dx.doi.org/10.1137/S003614450342061},
  date-added = {2008-09-16 15:54:11 -0500},
  date-modified = {2008-09-16 15:54:11 -0500},
  keywords = {Mathematics},
  ty = {JOUR},
  url = {http://dx.doi.org/10.1137/S003614450342061}
}

@ARTICLE{Bank:2000,
  author = {Bank, R. E. and Holst, M.},
  title = {A new paradigm for parallel adaptive meshing algorithms},
  journal = {Siam Journal on Scientific Computing},
  year = {2000},
  volume = {22},
  pages = {1411-1443},
  number = {4},
  abstract = {We present a new approach to the use of parallel computers with adaptive
	finite element methods. This approach addresses the load balancing
	problem in a new way, requiring far less communication than current
	approaches. It also allows existing sequential adaptive PDE codes
	such as PLTMG and MC to run in a parallel environment without a large
	investment in recoding. In this new approach, the load balancing
	problem is reduced to the numerical solution of a small elliptic
	problem on a single processor, using a sequential adaptive solver,
	without requiring any modifications to the sequential solver. The
	small elliptic problem is used to produce a posteriori error estimates
	to predict future element densities in the mesh, which are then used
	in a weighted recursive spectral bisection of the initial mesh. The
	bulk of the calculation then takes place independently on each processor,
	with no communication, using possibly the same sequential adaptive
	solver. Each processor adapts its region of the mesh independently,
	and a nearly load-balanced mesh distribution is usually obtained
	as a result of the initial weighted spectral bisection. Only the
	initial fan-out of the mesh decomposition to the processors requires
	communication. Two additional steps requiring boundary exchange communication
	may be employed after the individual processors reach an adapted
	solution, namely, the construction of a global conforming mesh from
	the independent subproblems, followed by a final smoothing phase
	using the subdomain solutions as an initial guess. We present a series
	of convincing numerical experiments which illustrate the effectiveness
	of this approach. The justification of the initial refinement prediction
	step, as well as the justification of skipping the two communication-intensive
	steps, is supported by some recent {$[$}J. Xu and A. Zhou, Math.
	Comp., to appear{$]$} and not so recent {$[$}J. A. Nitsche and A.
	H. Schatz, Math. Comp., 28 (1974), pp. 937--958; A. H. Schatz and
	L. B. Wahlbin, Math. Comp., 31 (1977), pp. 414--442; A. H. Schatz
	and L. B. Wahlbin, Math. Comp., 64 (1995), pp. 907--928{$]$} results
	on local a priori and a posteriori error estimation.},
  address = {Univ Calif San Diego La Jolla, CA USA 92093 Bank, RE rbank{\char64}ucsd.edu
	Dept Math Holst, M mholst@math.ucsd.edu Univ Calif San Diego La Jolla,
	CA USA 92093 Dept Math},
  annote = {A new paradigm for parallel adaptive meshing algorithms; NOV 8},
  bdsk-url-1 = {http://epubs.siam.org/sam-bin/jvip.pl?journal=SISC&vol=22&iss=4&pg=1411},
  date-added = {2008-09-16 15:54:11 -0500},
  date-modified = {2008-09-16 15:54:11 -0500},
  journal1 = {Siam J Sci Comput},
  keywords = {Mathematics},
  ty = {JOUR},
  url = {http://epubs.siam.org/sam-bin/jvip.pl?journal=SISC&vol=22&iss=4&pg=1411}
}

@ARTICLE{BCLZ10-2,
  author = {Bao, G. and Chow, S. N. and Li, P. and Zhou, H. M.},
  title = {An Inverse Random Source Problem for the { Helmholtz } Equation},
  journal = { AMS Mathematics of Computation},
  year = {submitted 2010},
  number = { }
}

@ARTICLE{BCLZ10-1,
  author = {Bao, G. and Chow, S. N. and Li, P. and Zhou, H. M.},
  title = {Numerical Solution of an Inverse Medium Scattering Problem with a
	Stochastic Source},
  journal = { Inverse Problems },
  year = {2010},
  volume = {26},
  number = { 074014 }
}

@ARTICLE{Barcilon:1992b,
  author = {Barcilon, V. },
  title = {Ion flow through narrow membran channels: part $\mathbf{I}$},
  journal = {SIAM J. Appl. Math.},
  year = {1992},
  volume = {52},
  pages = {1391-1404},
  number = { 5}
}

@ARTICLE{Barcilon:1992,
  author = {Barcilon, Victor and Chen, D.P. and Eisenberg, B. S. },
  title = {Ion flow through narrow membrane channels: Part II},
  journal = {SIAM J. Appl. Math},
  year = {1992},
  volume = {52},
  pages = {1405-1425},
  month = {October}
}

@ARTICLE{Bardhan:2009,
  author = {Bardhan, J. P. and Eisenberg, B. S. and Gillespie, D. },
  title = {{Discretization of the induced-charge boundary integral equation}},
  journal = {Physical Review E (Statistical, Nonlinear, and Soft Matter Physics).
	},
  year = {2009},
  volume = {80(1)},
  pages = {011906-10}
}

@ARTICLE{Bargteil:SLC,
  author = {Adam W. Bargteil and Tolga G. Goktekin and James F. O'Brien and John
	A. Strain},
  title = {{A Semi-Lagrangian Contouring Method for Fluid Simulation}},
  journal = {ACM Trans. Graph.},
  year = {2006},
  volume = {25},
  pages = {19--38},
  number = {1}
}

@ARTICLE{Barles:1991,
  author = {Barles, G. and Souganidis, P. E.},
  title = {Convergence of approximation schemes for fully nonlinear second order
	equations},
  journal = {Asymptotic Analysis},
  year = {1991},
  volume = {5},
  pages = {271-283},
  annote = {Convergence of approximation schemes for fully nonlinear second order
	equations},
  date-added = {2008-09-19 10:28:56 -0500},
  date-modified = {2008-09-19 10:28:56 -0500},
  ty = {JOUR}
}

@INPROCEEDINGS{SparseMatrices,
  author = {S. T. Barnard and A. Pothen and H. D. Simon},
  title = {A spectral algorithm for envelope reduction of sparse matrices},
  booktitle = {ACM/IEEE Supercomputing},
  year = {1993},
  pages = {493--502}
}

@ARTICLE{Barone:1997,
  author = {Barone, V and Cossi, M. and Tomasi, J.},
  title = {A new definition of cavities for the computation of solvation free
	energies by the polarizable continuum model },
  journal = {Journal of Chemical Physics},
  year = {1997},
  volume = {107},
  pages = {3210-3221}
}

@ARTICLE{Barraud:2007,
  author = {Barraud, S.},
  title = {Quantization effects on the phonon-limited electron mobility in ultrathin
	SOI, sSOI and GeOI devices},
  journal = {Semiconductor Scienec and Technology},
  year = {2007},
  volume = {22},
  pages = {413-417 },
  annote = {Quantization effects on the phonon-limited electron mobility in ultrathin
	SOI, sSOI and GeOI devices},
  date-added = {2008-11-25 10:28:56 -0500},
  date-modified = {2008-11-25 10:28:56 -0500},
  ty = {JOUR}
}

@BOOK{barret-berry-etal:94,
  title = {Templates for the Solution of Linear Systems: Building Blocks for
	Iterative Methods},
  publisher = {SIAM},
  year = {1994},
  author = {Barret, R. and Berry, M. and Chan, T.F. and Demmel, J. and Donato,
	J. and Dongarra, J. and Eijkhout, V. and Pozo, R. and Romine, C.
	and van der Vonst, H.}
}

@INBOOK{FV-Barth,
  pages = {439--474},
  title = {{Finite volume methods: foundation and analysis}},
  publisher = {John Wiley and Sons Ltd},
  year = {2004},
  author = {T. Barth and M. Ohlberger},
  volume = {1},
  series = {Encyclopedia of Computational Mechanics, E. Stein, R. de Borst, T.J.R.
	Hughes (Eds.)}
}

@ARTICLE{BarthSethian,
  author = {Timothy J. Barth and James A. Sethian},
  title = {Numerical Schemes for the Hamilton-Jacobi and Level Set Equations
	on Triangulated Domains},
  journal = {J. Comput. Phys.},
  year = {1998},
  volume = {145},
  pages = {1--40},
  number = {1}
}

@ARTICLE{Bashford:2000,
  author = {Bashford, D. and Case, D. A.},
  title = {Generalized {Born} models of macromolecular solvation effects},
  journal = {Annual Review of Physical Chemistry},
  year = {2000},
  volume = {51},
  pages = {129-152},
  abstract = {It would often be useful in computer simulations to use a simple description
	of solvation effects, instead of explicitly representing the individual
	solvent molecules. Continuum dielectric models often work well in
	describing the thermodynamic aspects of aqueous solvation, and approximations
	to such models that avoid the need to solve the Poisson equation
	are attractive because of their computational efficiency. Here we
	give an overview of one such approximation, the generalized Born
	model, which is simple and fast enough to be used for molecular dynamics
	simulations of proteins and nucleic acids. We discuss its strengths
	and weaknesses, both for its fidelity to the underlying continuum
	model and for its ability to replace explicit consideration of solvent
	molecules in macromolecular simulations. We focus particularly on
	versions of the generalized Born model that have a pair-wise analytical
	form, and therefore fit most naturally into conventional molecular
	mechanics calculations.},
  address = {Scripps Clin \& Res Inst La Jolla, CA USA 92037 Bashford, D bashford{\char64}scripps.edu
	Dept Mol Biol Case, DA case@scripps.edu Scripps Clin \& Res Inst
	La Jolla, CA USA 92037 Dept Mol Biol},
  annote = {Generalized Born models of macromolecular solvation effects; BashfordCaseGB},
  bdsk-url-1 = {http://physchem.AnnualReviews.org/cgi/content/full/51/1/129},
  date-added = {2008-09-01 13:58:51 -0500},
  date-modified = {2008-09-01 13:58:51 -0500},
  journal1 = {Annu Rev Phys Chem},
  keywords = {Electrostatics},
  ty = {JOUR},
  url = {http://physchem.AnnualReviews.org/cgi/content/full/51/1/129}
}

@ARTICLE{Bashford:1990,
  author = {Bashford, D. and Karplus, M.},
  title = {{p$K_a$'s} of ionizable groups in proteins: atomic detail from a
	continuum electrostatic model},
  journal = {Biochemistry},
  year = {1990},
  volume = {29},
  pages = {10219-25},
  number = {44},
  abstract = {A macroscopic electrostatic model is used to calculate the pKa values
	of the titratable groups in lysozyme. The model makes use of detailed
	structural information and treats solvation self-energies and interactions
	arising from permanent partial charges and titratable charges. Both
	the tetragonal and triclinic crystal structures are analyzed. Half
	of the experimentally observed pKa shifts (11 out of 21) are well
	reproduced by calculations for both structures; this includes the
	unusually high pKa of Glu 35 in the active site. For more than half
	the pKa's (13 out of 21), there is a large difference (1-3.3 pK units)
	between the results from the two structures. Many of these correspond
	to the titrating groups for which the calculations are in error.
	Since for an ionic strength of 0.1 M the Debye screening between
	titratable groups leads to a very high effective dielectric constant
	(the average value for all pairs of titrating groups is approximately
	900), near-neighbor interactions dominate the pKa perturbations.
	Thus, the pKa values are very sensitive to the details of the local
	protein conformation, and it is likely that side-chain mobility has
	an important role in determining the observed pKa shifts.},
  address = {Department of Chemistry, Harvard University, Cambridge, Massachusetts
	02138.},
  annote = {Nov 6; pKa's of ionizable groups in proteins: atomic detail from
	a continuum electrostatic model; 2271649; 0006-2960 Journal Article},
  bdsk-url-1 = {http://www.ncbi.nlm.nih.gov/entrez/query.fcgi?cmd=Retrieve&db=PubMed&dopt=Citation&list_uids=2271649},
  date-added = {2008-06-28 10:41:20 -0500},
  date-modified = {2008-06-28 10:41:20 -0500},
  keywords = {Electrostatics},
  read = {Yes},
  ty = {JOUR},
  url = {http://www.ncbi.nlm.nih.gov/entrez/query.fcgi?cmd=Retrieve&db=PubMed&dopt=Citation&list_uids=2271649}
}

@ARTICLE{Bates:2003,
  author = {Bates, P. B. and Chen, X. F. and Chmaj, A. J. J.},
  title = {Traveling waves of bistable dynamics on a lattice},
  journal = {SIAM J. Math. Anal. },
  year = {2003},
  volume = {35},
  pages = {520-546},
  annote = {Traveling waves of bistable dynamics on a lattice},
  date-added = {2008-09-19 10:28:56 -0500},
  date-modified = {2008-09-19 10:28:56 -0500},
  ty = {JOUR}
}

@ARTICLE{Bates:2008c,
  author = {Bates, P. W. and Brown, S. and Han, J.},
  title = {Numerical analysis for a nonlocal Allen-Cahn equation},
  journal = {International Journal of Numerical Analysis and Modeling},
  year = {in press, 2008},
  annote = {Numerical analysis for a nonlocal Allen-Cahn equation},
  date-added = {2008-09-19 10:28:56 -0500},
  date-modified = {2008-09-19 10:28:56 -0500},
  ty = {JOUR}
}

@ARTICLE{Bates:2006b,
  author = {Bates, P. W. and Chen, F.},
  title = {Spectral analysis of traveling waves for nonlocal evolution equations},
  journal = {SIAM J. Math. Anal. },
  year = {2006},
  volume = {38},
  pages = {116-126},
  annote = {Spectral analysis of traveling waves for nonlocal evolution equations},
  date-added = {2008-09-19 10:28:56 -0500},
  date-modified = {2008-09-19 10:28:56 -0500},
  ty = {JOUR}
}

@ARTICLE{Bates:2002b,
  author = {Bates, P. W. and Chen, F. X.},
  title = {Traveling wave solutions for a nonlocal phase-field system},
  journal = {Interfaces Free Bound. },
  year = {2002},
  volume = {4},
  pages = {227-238},
  annote = {Traveling wave solutions for a nonlocal phase-field system},
  date-added = {2008-09-19 10:28:56 -0500},
  date-modified = {2008-09-19 10:28:56 -0500},
  ty = {JOUR}
}

@ARTICLE{Bates:2002c,
  author = {Bates, P. W. and Chen, F. X.},
  title = {Spectral analysis and multidimensional stability of traveling waves
	for nonlocal Allen-Cahn equation},
  journal = {J. Math. Anal. Appl. },
  year = {2002},
  volume = {273},
  pages = {45-57},
  annote = {Spectral analysis and multidimensional stability of traveling waves
	for nonlocal Allen-Cahn equation},
  date-added = {2008-09-19 10:28:56 -0500},
  date-modified = {2008-09-19 10:28:56 -0500},
  ty = {JOUR}
}

@ARTICLE{Bates:2005,
  author = {Bates, P. W. and Chen, X. F. and Chmaj, A. J. J.},
  title = {Heteroclinic solutions of a {van der Waals} model with indefinite
	nonlocal interactions},
  journal = {Calc. Var. Partial Differential Equations },
  year = {2005},
  volume = {24},
  pages = {261-281},
  annote = {Heteroclinic solutions of a {van der Waals} model with indefinite
	nonlocal interactions},
  date-added = {2008-09-19 10:28:56 -0500},
  date-modified = {2008-09-19 10:28:56 -0500},
  ty = {JOUR}
}

@ARTICLE{Bates:2009,
  author = {Bates, P. W. and Chen, Z. and Sun, Y. H. and Wei, G. W. and Zhao,
	S.},
  title = {Geometric and potential driving formation and evolution of biomolecular
	surfaces},
  journal = {J. Math. Biol. },
  year = {2009},
  volume = {59},
  pages = {193-231},
  annote = {Geometric and potential driving formation and evolution of biomolecular
	surfaces},
  date-added = {2008-09-19 10:28:56 -0500},
  date-modified = {2008-09-19 10:28:56 -0500},
  ty = {JOUR}
}

@ARTICLE{Bates:2005b,
  author = {Bates, P. W. and Fusco, G.},
  title = {Equilibria with many nuclei for the {Cahn-Hilliard} equation},
  journal = {J. Differential Equations },
  year = {2005},
  volume = {160},
  pages = {283-356},
  annote = {Equilibria with many nuclei for the {Cahn-Hilliard} equation},
  date-added = {2008-09-19 10:28:56 -0500},
  date-modified = {2008-09-19 10:28:56 -0500},
  ty = {JOUR}
}

@ARTICLE{Bates:2005d,
  author = {Bates, P. W. and Han, J. H.},
  title = {The Neumann boundary problem for a nonlocal {Cahn-Hilliard} equation},
  journal = {J. Differential Equations },
  year = {2005},
  volume = {212},
  pages = {235-277},
  annote = {The Neumann boundary problem for a nonlocal {Cahn-Hilliard} equation},
  date-added = {2008-09-19 10:28:56 -0500},
  date-modified = {2008-09-19 10:28:56 -0500},
  ty = {JOUR}
}

@ARTICLE{Bates:2005c,
  author = {Bates, P. W. and Han, J. L.},
  title = {The {Dirichlet} boundary problem for a nonlinear {Cahn-Hilliard}
	equation},
  journal = {J. Math. Anal. Appl. },
  year = {2005},
  volume = {311},
  pages = {289-312},
  annote = {The {Dirichlet} boundary problem for a nonlinear {Cahn-Hilliard}
	equation},
  date-added = {2008-09-19 10:28:56 -0500},
  date-modified = {2008-09-19 10:28:56 -0500},
  ty = {JOUR}
}

@ARTICLE{Bates:2006d,
  author = {Bates, P. W. and Han, J. L. and Zhao, G. Y.},
  title = {On a nonlocal phase-field system},
  journal = {Nonlin. Anal. Theory Meth. Appl. },
  year = {2006},
  volume = {64},
  pages = {2251-2278},
  annote = {On a nonlocal phase-field system},
  date-added = {2008-09-19 10:28:56 -0500},
  date-modified = {2008-09-19 10:28:56 -0500},
  ty = {JOUR}
}

@ARTICLE{Bates:2006e,
  author = {Bates, P. W. and Lisei, H. and Lu, K. N.},
  title = {Attractors for Stochastic lattice dynamical systems},
  journal = {Stoch. Dyn. },
  year = {2006},
  volume = {6},
  pages = {1-21},
  annote = {Attractors for Stochastic lattice dynamical systems},
  date-added = {2008-09-19 10:28:56 -0500},
  date-modified = {2008-09-19 10:28:56 -0500},
  ty = {JOUR}
}

@ARTICLE{Bates:2008e,
  author = {Bates, P. W. and Lu, K. and Wang, B.},
  title = {Random Attractors for Stochastic Reaction-Diffusion Equations on
	Unbounded Domains},
  journal = {J. Differential Equations},
  year = {in press, 2008},
  annote = {Random Attractors for Stochastic Reaction-Diffusion Equations on
	Unbounded Domains},
  date-added = {2008-09-19 10:28:56 -0500},
  date-modified = {2008-09-19 10:28:56 -0500},
  ty = {JOUR}
}

@ARTICLE{Bates:2008d,
  author = {Bates, P. W. and Lu, K. L. and C Zeng, C.},
  title = {Approximately Invariant Manifolds and Global Dynamics of Spike States},
  journal = {Inventiones Mathematicae},
  year = {79 pages, in press, 2008},
  annote = {Approximately Invariant Manifolds and Global Dynamics of Spike States},
  date-added = {2008-09-19 10:28:56 -0500},
  date-modified = {2008-09-19 10:28:56 -0500},
  ty = {JOUR}
}

@ARTICLE{Bates:2001,
  author = {Bates, P. W. and Lu, K. N. and Wang, B. X.},
  title = {Attractors for lattice dynamical systems},
  journal = {Internat. J. Bifur. Chaos Appl. Sci. Engrg. },
  year = {2001},
  volume = {11},
  pages = {143-153},
  annote = {Attractors for lattice dynamical systems},
  date-added = {2008-09-19 10:28:56 -0500},
  date-modified = {2008-09-19 10:28:56 -0500},
  ty = {JOUR}
}

@ARTICLE{Bates:2007b,
  author = {Bates, P. W. and Pan, X. B.},
  title = {Nucleation of instability of the {Meissner} state of 3-dimensional
	superconductors},
  journal = {Comm. Math. Phys. },
  year = {2007},
  volume = {276},
  number = {571-610},
  annote = {Nucleation of instability of the {Meissner} state of 3-dimensional
	superconductors},
  date-added = {2008-09-19 10:28:56 -0500},
  date-modified = {2008-09-19 10:28:56 -0500},
  ty = {JOUR}
}

@ARTICLE{Bates:2002,
  author = {Bates, P. W. and Shi, J. P.},
  title = {Existence and instability of spike layer solutions to singular perturbation
	problems},
  journal = {J. Funct. Anal. },
  year = {2002},
  volume = {196},
  pages = {211-264},
  annote = {Existence and instability of spike layer solutions to singular perturbation
	problems},
  date-added = {2008-09-19 10:28:56 -0500},
  date-modified = {2008-09-19 10:28:56 -0500},
  ty = {JOUR}
}

@ARTICLE{Bates:2008,
  author = {Bates, P. W. and Wei, G. W. and Zhao, Shan},
  title = {Minimal molecular surfaces and their applications},
  journal = {Journal of Computational Chemistry},
  year = {2008},
  volume = {29},
  pages = {380-91},
  number = {3},
  abstract = {This article presents a novel concept, the minimal molecular surface
	(MMS), for the theoretical modeling of biomolecules. The MMS can
	be viewed as a result of the surface free energy minimization when
	an apolar molecule, such as protein, DNA or RNA is immersed in a
	polar solvent. Based on the theory of differential geometry, the
	MMS is created via the mean curvature minimization of molecular hypersurface
	functions. A detailed numerical algorithm is presented for the practical
	generation of MMSs. Extensive numerical experiments, including those
	with internal and open cavities, are carried out to demonstrated
	the proposed concept and algorithms. The proposed MMS is typically
	free of geometric singularities. Application of the MMS to the electrostatic
	analysis is considered for a set of twenty six proteins. Â© 2007
	Wiley Periodicals, Inc. J Comput Chem, 2007},
  address = {Department of Mathematics, Michigan State University, Michigan 48824;
	Department of Electrical and Computer Engineering, Michigan State
	University, Michigan 48824; Department of Mathematics, University
	of Alabama, Albama 35487},
  bdsk-url-1 = {http://dx.doi.org/10.1002/jcc.20796},
  bdsk-url-2 = {http://dx.doi.org/10.1002/jcc.20796},
  date-added = {2008-06-28 10:45:03 -0500},
  date-modified = {2008-06-28 10:45:03 -0500},
  doi = {10.1002/jcc.20796},
  keywords = {electrostatics; mathematics},
  url = {http://dx.doi.org/10.1002/jcc.20796}
}

@ARTICLE{Bates:2006,
  author = {Bates, P. W. and Wei, G. W. and Zhao, S.},
  title = {The minimal molecular surface},
  journal = {arXiv:q-bio/0610038v1 },
  year = {2006},
  volume = {[q-bio.BM]},
  annote = {The minimal molecular surface},
  date-added = {2008-09-19 10:28:56 -0500},
  date-modified = {2008-09-19 10:28:56 -0500},
  ty = {JOUR}
}

@ARTICLE{Bates:2006f,
  author = {Bates, P. W. and Wei, G. W. and Zhao, S.},
  title = {The minimal molecular surface},
  journal = {Midwest Quantitative Biology Conference},
  year = {2006},
  volume = {Mission Point Resort, Mackinac Island, MI},
  pages = {September 29 - October 1},
  annote = {The minimal molecular surface},
  date-added = {2008-09-19 10:28:56 -0500},
  date-modified = {2008-09-19 10:28:56 -0500},
  ty = {JOUR}
}

@ARTICLE{Bates:2006c,
  author = {Bates, P. W. and Zhang, C. L.},
  title = {Traveling pulses for the {Klein-Gordon} equation on a lattice or
	continuum with long-range interaction},
  journal = {Discr. Contin. Dyn. Syst. },
  year = {2006},
  volume = {16},
  pages = {235-252},
  annote = {Traveling pulses for the {Klein-Gordon} equation on a lattice or
	continuum with long-range interaction},
  date-added = {2008-09-19 10:28:56 -0500},
  date-modified = {2008-09-19 10:28:56 -0500},
  ty = {JOUR}
}

@ARTICLE{Bates:2007,
  author = {Bates, P. W. and Zhao, G. Y.},
  title = {Existence, uniqueness and stability of the stationary solution to
	a nonlocal evolution equation arising in population dispersal},
  journal = {J. math. Anal. Appl. },
  year = {2007},
  volume = {332},
  pages = {428-440},
  annote = {Existence, uniqueness and stability of the stationary solution to
	a nonlocal evolution equation arising in population dispersal},
  date-added = {2008-09-19 10:28:56 -0500},
  date-modified = {2008-09-19 10:28:56 -0500},
  ty = {JOUR}
}

@ARTICLE{Battey:2007,
  author = {Battey, J. N. and Kopp, J. and Bordoli, L. and Read, R. J. and Clarke,
	N. D. and Schwede, T.},
  title = {{Automated server predictions in CASP7}},
  journal = {Proteins},
  year = {2007},
  volume = {69},
  pages = {68-82},
  number = {S8}
}

@ARTICLE{Bazant:2009,
  author = { Bazant, M. Z. and Kilic, M. S. and Storey, B. D. and Ajdari, A.
	},
  title = {Towards an understanding of induced-charge electrokinetics at large
	applied voltages in concentrated solutions},
  journal = {Advances in Colloid and Interface Science},
  year = {2009},
  volume = {152},
  pages = {48-88 }
}

@ARTICLE{Bazant:2011,
  author = {Bazant, M. Z. and Storey, B. D and Kornyshev, A. A.},
  title = {Double Layer in Ionic Liquids: Overscreening versus Crowding},
  journal = {Physical Review Letters},
  year = {2011},
  volume = {106},
  pages = {046102.}
}

@ARTICLE{Bazant:2005,
  author = {Bazant, M. Z. and Thornton, K. and Ajdari, A. },
  title = {Diffuse-charge dynamics in electrochemical systems},
  journal = {Physical Review E},
  year = {2004},
  volume = {70},
  pages = {021506}
}

@ARTICLE{Beale:2006,
  author = {Beale, J. T. and Layton, A. T.},
  title = {On the accuracy of finite difference methods for elliptic problems
	with interfaces },
  journal = {Comm. Appl. Math. Comp. Sci.,},
  year = {2006},
  volume = {1},
  pages = { 91-119}
}

@ARTICLE{Beall1997,
  author = {Beall, Mark W and Shephard, Mark S},
  title = {{A general topology-based mesh data structure}},
  journal = {International Journal for Numerical Methods in Engineering},
  year = {1997},
  volume = {40},
  pages = {1573--1596},
  number = {9},
  abstract = {A representation for a mesh based on the topological hierarchy of
	vertices, edges, faces and regions, is described. The representation
	is general and easily supports procedures ranging from mesh generation
	to adaptive analysis processes. Three implementations are given which
	concentrate on different aspects of performance (storage requirements
	and speed). Comparisons are made to other published. representations.
	(C) 1997 by John Wiley & Sons, Ltd.},
  doi = {10.1002/(SICI)1097-0207(19970515)40:9<1573::AID-NME128>3.0.CO;2-9},
  file = {:C\:/Users/doubletony/AppData/Local/Mendeley Ltd./Mendeley Desktop/Downloaded/Beall, Shephard - 1997 - A general topology-based mesh data structure(2).pdf:pdf},
  issn = {00295981},
  owner = {doubletony},
  publisher = {Chichester, New York, Wiley [etc.] 1969-},
  timestamp = {2012.04.26},
  url = {http://doi.wiley.com/10.1002/%28SICI%291097-0207%2819970515%2940%3A9%3C1573%3A%3AAID-NME128%3E3.0.CO%3B2-9}
}

@ARTICLE{Beck:2000,
  author = {Beck, T. L.},
  title = {Real-space mesh techniques in density-functional theory},
  journal = {REVIEWS OF MODERN PHYSICS },
  year = {2000},
  volume = {72},
  pages = {1041-1080}
}

@ARTICLE{Becke:1993,
  author = {Becke, A. D.},
  title = {Density functional thermochemistry III. The role of exact exchange},
  journal = {J. Chem. Phys.},
  year = {1993},
  volume = {98},
  pages = {5648}
}

@ARTICLE{Becke:1993,
  author = {Becke, A. D.},
  title = {Density functional thermochemistry {III}. The role of exact exchange},
  journal = {J. Chem. Phys.},
  year = {1993},
  volume = {98},
  pages = {5648}
}

@ARTICLE{Bednarek:2000,
  author = {Bednarek, S. and Szafran, B. and Adamowski, J.},
  title = {Solution of the {Poisson-Schr\"{o}dinger} problem for a single-electron
	transistor },
  journal = {Zeitschrift fur Angewandte Mathematik und Physik},
  year = {2000},
  volume = {61},
  pages = { 4461-4464},
  annote = {Solution of the Poisson-Schrodinger problem for a single-electron
	transistor },
  date-added = {2008-11-25 10:28:56 -0500},
  date-modified = {2008-11-25 10:28:56 -0500},
  ty = {JOUR}
}

@ARTICLE{Bedrossian:2010,
  author = { Bedrossian, J. and von Brecht, J. H. and Zhu, S. W. and Sifakis,
	E. and Teran, J. M.},
  title = { A finite element method for interface problems in domains with smooth
	boundaries and interfaces
	
	},
  journal = {J. Comput. Phys.},
  year = {2010},
  volume = {229},
  pages = {6405-6426}
}


@ARTICLE{Beglov:1996,
  author = {Beglov, D. and Roux, B.},
  title = {Solvation of complex molecules in a polar liquid: an integral equation
	theory},
  journal = {Journal of Chemical Physics},
  year = {1996},
  volume = {104},
  pages = {8678-8689},
  number = {21},
  abstract = {A statistical mechanical integral equation theory is developed to
	describe the average structure of a polar liquid around a complex
	molecular solute of irregular shape. The integral equation is formulated
	in three-dimensional Cartesian coordinates from the hypernetted chain
	(HNC) equation for a solute at infinite dilution. The direct correlation
	function of the pure solvent used in the theory is taken from the
	analytical solution of the mean spherical approximation (MSA) equation
	for a liquid constituted of nonpolarizable hard spheres with an embedded
	dipole at their center. It is demonstrated explicitly that, in the
	limit where the size of the solvent particles becomes very small,
	the present theory reduces to the well-known equations for macroscopic
	electrostatics in which the solvent is represented in terms of a
	dielectric continuum. A linearized version of the integral equation
	corresponds to a three-dimensional extension of the familiar MSA
	equation. This 3D-MSA integral equation is illustrated with numerical
	applications to the case of an ion, a water molecule, and N-methylacetamide.
	The numerical solution, obtained on a discrete three-dimensional
	cubic grid in Cartesian coordinates, yields the average solvent density
	and polarization density at all the points x,y,z around the solute.
	All spatial convolutions appearing in the theory are calculated using
	three-dimensional numerical fast Fourier transforms (FFT). Ã‚Â??996
	American Institute of Physics.},
  annote = {Solvation of complex molecules in a polar liquid: an integral equation
	theory; BeglovRoux},
  bdsk-file-1 = {YnBsaXN0MDDUAQIDBAUGCQpYJHZlcnNpb25UJHRvcFkkYXJjaGl2ZXJYJG9iamVjdHMSAAGGoNE
	HCFRyb290gAFfEA9OU0tleWVkQXJjaGl2ZXKoCwwXGBkdJCVVJG51bGzTDQ4PEBEUViRjbGFzc1
	dOUy5rZXlzWk5TLm9iamVjdHOAB6ISE4ACgAOiFRaABIAGWWFsaWFzRGF0YVxyZWxhdGl2ZVBhd
	GjSDRobHFdOUy5kYXRhgAVPEQG6AAAAAAG6AAIAAAxNYWNpbnRvc2ggSEQAAAAAAAAAAAAAAAAA
	AADD4v5NSCsAAAAZYksTMTk5Ni1CZWdsb3ZSb3V4LnBkZgAAAAAAAAAAAAAAAAAAAAAAAAAAAAA
	AAAAAAAAAAAAAAAAAAAAAAAAAAAAAABlidr8eaiMAAAAAAAAAAAAEAAQAAAkgAAAAAAAAAAAAAA
	AAAAAAB0FyY2hpdmUAABAACAAAw+NSrQAAABEACAAAvx6wcwAAAAEAFAAZYksAGWIDAAqkKAAKp
	BEAAHrcAAIASU1hY2ludG9zaCBIRDpVc2VyczpiYWtlcjpEb2N1bWVudHM6UmVmZXJlbmNlczpB
	cmNoaXZlOjE5OTYtQmVnbG92Um91eC5wZGYAAA4AKAATADEAOQA5ADYALQBCAGUAZwBsAG8AdgB
	SAG8AdQB4AC4AcABkAGYADwAaAAwATQBhAGMAaQBuAHQAbwBzAGgAIABIAEQAEgA8VXNlcnMvYm
	FrZXIvRG9jdW1lbnRzL1JlZmVyZW5jZXMvQXJjaGl2ZS8xOTk2LUJlZ2xvdlJvdXgucGRmABMAA
	S8AABUAAgAM//8AANIeHyAhWCRjbGFzc2VzWiRjbGFzc25hbWWjISIjXU5TTXV0YWJsZURhdGFW
	TlNEYXRhWE5TT2JqZWN0XxA8Li4vLi4vLi4vLi4vRG9jdW1lbnRzL1JlZmVyZW5jZXMvQXJjaGl
	2ZS8xOTk2LUJlZ2xvdlJvdXgucGRm0h4fJieiJyNcTlNEaWN0aW9uYXJ5AAgAEQAaAB8AKQAyAD
	cAOgA/AEEAUwBcAGIAaQBwAHgAgwCFAIgAigCMAI8AkQCTAJ0AqgCvALcAuQJ3AnwChQKQApQCo
	gKpArIC8QL2AvkAAAAAAAACAQAAAAAAAAAoAAAAAAAAAAAAAAAAAAADBg==},
  bdsk-url-1 = {http://dx.doi.org/10.1063/1.471557},
  date-added = {2008-06-29 08:34:47 -0500},
  date-modified = {2008-06-29 08:34:47 -0500},
  keywords = {Solvation; Misc; Electrostatics},
  ty = {JOUR},
  url = {http://dx.doi.org/10.1063/1.471557}
}

@ARTICLE{Belgrader:2000,
  author = {Belgrader, P. and Okuzumi, M. and Pourahmadi, F. and Borkholder,
	D. A. and Northrup, M. A.},
  title = {A microfluidic cartridge to prepare spores for PCR analysis},
  journal = {Biosensors Bioelectronics},
  year = {2000},
  volume = {14},
  pages = {849-852}
}

@ARTICLE{LaplaceEigenmaps,
  author = {Mikhail Belkin and Partha Niyogi},
  title = {Laplacian Eigenmaps for Dimensionality Reduction and Data Representation},
  journal = {Neural Comput.},
  year = {2003},
  volume = {15},
  pages = {1373--1396},
  number = {6}
}

@ARTICLE{belongie2002sma,
  author = {Belongie, S. and Malik, J. and Puzicha, J.},
  title = {{Shape matching and object recognition using shape contexts}},
  journal = {IEEE Trans. on PAMI},
  year = {2002},
  volume = {24},
  pages = {509-522},
  number = {4}
}

@ARTICLE{Bemish938585,
  author = {Bemish, R. J. and Block, P. A. and Pedersen, L. G. and Yang, W. T.
	and Miller, R. E.},
  title = {The Ar-C2h2 Intermolecular Potential from High-Resolution Spectroscopy
	and Ab-Initio Theory - a Case for Multicenter Interactions},
  journal = {Journal of Chemical Physics},
  year = {1993},
  volume = {99},
  pages = {8585-8598},
  number = {11},
  month = {Dec},
  abstract = {Infrared spectra have been obtained for the Ar-C2H2 complex, which
	include a combination band associated with the low frequency bending
	mode. These data are used, together with ab initio calculations and
	the results of previous studies of this system, to construct a two-dimensional
	Hartree-Fock plus damped dispersion (HFD) intermolecular potential
	surface corresponding to the C-H stretch excited vibrational state.
	A high quality SCF surface, which includes ghost orbital corrections,
	has been used to fix the repulsive part of the potential. The remaining
	potential parameters were initially estimated with the aid of various
	combining rules and the collocation technique was used to solve the
	bound state problem for this potential and to calculate the spectrum
	of the Ar-C2H2 complex. To obtain good agreement between the calculated
	and experimental spectra it was necessary to distribute the dispersion
	interaction over the length of the acetylene subunit. The result
	is a double minimum potential upon which the complex executes wide
	amplitude bending motion.},
  endnotereftype = {Journal Article},
  issn = {0021-9606},
  shorttitle = {The Ar-C2h2 Intermolecular Potential from High-Resolution Spectroscopy
	and Ab-Initio Theory - a Case for Multicenter Interactions},
  url = {<Go to ISI>://A1993MJ90200025}
}

@ARTICLE{BenAbdallah:2007,
  author = {Ben Abdallah, N. and Mouis, M. and Negulescu, C.},
  title = {An accelerated algorithm for 2D simulations of the quantum ballistic
	transport in nanoscale MOSFETs },
  journal = {J. Comput. Phys.},
  year = {2007},
  volume = {225},
  pages = {74-99},
  annote = {An accelerated algorithm for 2D simulations of the quantum ballistic
	transport in nanoscale MOSFETs },
  date-added = {2008-11-25 10:28:56 -0500},
  date-modified = {2008-11-25 10:28:56 -0500},
  ty = {JOUR}
}

@ARTICLE{GotsmanCompression2,
  author = {Mirela Ben-Chen and Craig Gotsman},
  title = {On the optimality of spectral compression of mesh data},
  journal = {ACM Trans. Graph.},
  year = {2005},
  volume = {24},
  pages = {60--80},
  number = {1}
}

@BOOK{Berger:1988,
  title = {Differential Geometry: Manifolds, Curves, and Surfaces},
  publisher = {Springer-Verlag},
  year = {1988},
  author = {Berger, M. and Gostiaux, B.}
}

@ARTICLE{Bergstrom:2003,
  author = {Bergstrom, C. A. S. and Strafford, M. and Lazorova, L. and Avdeef,
	A. and Luthman, K. and Artursson, P. },
  title = {Absorption Classification of Oral Drugs Based on Molecular Surface
	Properties},
  journal = {Journal of Medicinal Chemistry},
  year = {2003},
  volume = {46},
  pages = {558--570},
  number = {4},
  abstract = {Abstract: The aim of this study was to investigate whether easily
	calculated and comprehended molecular surface properties can predict
	drug solubility and permeability with sufficient accuracy to allow
	theoretical absorption classification of drug molecules. For this
	purpose, structurally diverse, orally administered model drugs were
	selected from the World Health Organization (WHO)'s list of essential
	drugs. The solubility and permeability of the drugs were determined
	using well-established in vitro methods in highly accurate experimental
	settings. Descriptors for molecular surface area were generated from
	low-energy conformations obtained by conformational analysis using
	molecular mechanics calculations. Correlations between the calculated
	molecular surface area descriptors, on one hand, and solubility and
	permeability, on the other, were established with multivariate data
	analysis (partial least squares projection to latent structures (PLS))
	using training and test sets. The obtained models were challenged
	with external test sets. Both solubility and permeability of the
	druglike molecules could be predicted with high accuracy from the
	calculated molecular surface properties alone. The established correlations
	were used to perform a theoretical biopharmaceutical classification
	of the WHO-listed drugs into six classes, resulting in a correct
	prediction for 87\% of the essential drugs. An external test set
	consisting of Food and Drug Administration (FDA) standard compounds
	for biopharmaceutical classification was predicted with 77\% accuracy.
	We conclude that PLS models of easily comprehended molecular surface
	properties can be used to rapidly provide absorption profiles of
	druglike molecules early on in drug discovery.},
  address = {Center of Pharmaceutical Informatics, Department of Pharmacy, Uppsala
	University, Uppsala Biomedical Center, P.O. Box 580, SE-751 23 Uppsala,
	Sweden, pION Inc., 5 Constitution Way, Woburn, Massachusetts 01801,
	and Department of Chemistry, Medicinal Chemistry, G\"{o}teborg University,
	SE-412 96 G\"{o}teborg, Sweden},
  bdsk-url-1 = {http://dx.doi.org/10.1021/jm020986i},
  date-added = {2008-06-30 09:29:38 -0500},
  date-modified = {2008-06-30 09:29:38 -0500},
  doi = {10.1021/jm020986i},
  keywords = {bioinformatics, drug\_design, electrostatics, solvation},
  posted-at = {2008-06-30 15:29:06},
  priority = {0},
  url = {http://dx.doi.org/10.1021/jm020986i}
}

@ARTICLE{Bergstrom,
  author = {Bergstrom, C.A.S. and Strafford, M. and Lazorova, L. and Avdeef,
	A. and Luthman, K. and Artursson, P. },
  title = {Absorption classification of oral drugs based on molecular surface
	properties},
  journal = {J. Medicinal Chem.},
  year = {2003},
  volume = {46},
  pages = {558-570}
}

@ARTICLE{Bernal:1933,
  author = {Bernal, JD and Fowler, RH},
  title = {A theory of water and ionic solution, with particular reference to
	hydrogen and hydroxyl ions},
  journal = {J Chem Phys},
  year = {1933},
  volume = {1},
  pages = {515-548}
}

@ARTICLE{Berthelsen:2004,
  author = {Berthelsen, Petter Andreas},
  title = {A decomposed immersed interface method for variable coefficient elliptic
	equations with non-smooth and discontinuous solutions},
  journal = {J. Comput. Phys.},
  year = {2004},
  volume = {197},
  pages = {364--386},
  number = {1},
  abstract = { A second order accurate finite difference method is presented for
	solving two-dimensional variable coefficient elliptic equations on
	{Cartesian grids}, in which the coefficients, the source term, the
	solution and its derivatives may be non-smooth or discontinuous across
	an interface. A correction term is introduced to the standard central
	difference stencil so that the numerical discretization is well-defined
	across the interface. We also propose a new method to approximate
	the correction term as part of the iterative procedure. The method
	is easy to implement since the correction term only needs to be added
	to the right-hand-side of the system. Therefore, the coefficient
	matrix remains symmetric and diagonally dominant, allowing for most
	standard solvers to be used. Numerical examples show good agreements
	with exact solutions, and the order of accuracy is comparable with
	other immersed interface methods.},
  bdsk-url-1 = {http://www.sciencedirect.com/science/article/B6WHY-4BHJW0W-5/2/3dd90f981d3410c22c6ffffe133f83c8},
  date-added = {2008-09-14 15:32:12 -0500},
  date-modified = {2008-09-14 15:32:12 -0500},
  doi = {10.1016/j.jcp.2003.12.003 },
  keywords = {Mathematics},
  ty = {JOUR},
  url = {http://www.sciencedirect.com/science/article/B6WHY-4BHJW0W-5/2/3dd90f981d3410c22c6ffffe133f83c8}
}

@ARTICLE{Bertonati:2007,
  author = {Bertonati, C. and Honig, B. and Alexov, E.},
  title = {{Poisson-Boltzmann} calculations of nonspecific salt effects on protein-protein
	binding free energy},
  journal = {Biophysical Journal},
  year = {2007},
  volume = {92},
  pages = {1891-1899}
}

@ARTICLE{ABertozzi:2004,
  author = {Bertozzi, A. L. and Greer, J. B.},
  title = {Low-curvature image simplifiers: Global regularity of smooth solutions
	and Laplacian limiting schemes},
  journal = {Communications on Pure and Applied Mathematics},
  year = {2004},
  volume = {57},
  pages = {764-790},
  number = {6}
}

@ARTICLE{Bertozzi:2004,
  author = {Bertozzi, Andrea L. and Greer, John B. },
  title = {Low-curvature image simplifiers: Global regularity of smooth solutions
	and {Laplacian} limiting schemes},
  journal = {Communications on Pure and Applied Mathematics},
  year = {2004},
  volume = {57},
  pages = {764-790},
  number = {6},
  abstract = {We consider a class of fourth-order nonlinear diffusion equations
	motivated by Tumblin and Turk's ldquolow-curvature image simplifiersrdquo
	for image denoising and segmentation. The PDE for the image intensity
	u is of the formwhere g(s) = k2/(k2 + s2) is a ldquocurvaturerdquo
	threshold and &lgr; denotes a fidelity-matching parameter. We derive
	a priori bounds for &Dgr;u that allow us to prove global regularity
	of smooth solutions in one space dimension, and a geometric constraint
	for finite-time singularities from smooth initial data in two space
	dimensions. This is in sharp contrast to the second-order Perona-Malik
	equation (an ill-posed problem), on which the original LCIS method
	is modeled. The estimates also allow us to design a finite difference
	scheme that satisfies discrete versions of the estimates, in particular,
	a priori bounds on the smoothness estimator in both one and two space
	dimensions. We present computational results that show the effectiveness
	of such algorithms. Our results are connected to recent results for
	fourth-order lubrication-type equations and the design of positivity-preserving
	schemes for such equations. This connection also has relevance for
	other related fourth-order imaging equations. Â© 2004 Wiley Periodicals,
	Inc.},
  bdsk-url-1 = {http://dx.doi.org/10.1002/cpa.20019},
  date = {2004 %@ 1097-0312 %+ University of California, Los Angeles, Department
	of Mathematics, Box 951555, Los Angeles, CA 90095-1555},
  date-added = {2008-09-14 15:32:12 -0500},
  date-modified = {2008-09-14 15:32:12 -0500},
  doi = {10.1002/cpa.20019},
  keywords = {Mathematics; Visualization},
  refer1 = {10.1002/cpa.20019},
  url = {http://dx.doi.org/10.1002/cpa.20019}
}

@ARTICLE{besl-mckay:92,
  author = {Besl, P.J. and McKay, N.D.},
  title = {A Method for Registration of 3{D} Shapes},
  journal = {IEEE Transactions on PAMI},
  year = {1992},
  volume = {14},
  pages = {239--256},
  number = {2}
}

@ARTICLE{Besler:1990,
  author = {Besler, B. H. and Merz, K. M., Jr. and Kollman, P. A.},
  title = {Atomic charges derived from semiempirical methods.},
  journal = {J. Comput. Chem.},
  year = {1990},
  volume = {11},
  pages = {431-439}
}

@ARTICLE{Bhat:2006,
  author = {Bhat, S. and Purisima, E. O. },
  title = {Molecular surface generation using a variable{-}radius solvent probe},
  journal = {Proteins: Structure, Function, and Bioinformatics},
  year = {2006},
  volume = {62},
  pages = {244-261}
}

@ARTICLE{Bianco,
  author = {Bianco, F. and Puppo, G. and Russo, G.},
  title = {High-order central differencing for hyperbolic conservation laws},
  journal = {SIAM J. Sci. Comput.},
  year = {1999},
  pages = {294-322},
  issn = {21}
}

@ARTICLE{Billeter:1998,
  author = {Billeter, S.R. and van Gunsteren, W.F.},
  title = {{Protonizable Water Model for Quantum Dynamical Simulations}},
  journal = {Journal of Physical Chemistry},
  year = {1998},
  volume = {102},
  pages = {4669-4678}
}

@ARTICLE{Billeter:1997,
  author = {Billeter, S.R. and van Gunsteren, W.F.},
  title = {A modular molecular dynamics/quantum dynamics program for non-adiabatic
	proton transfers in solution},
  journal = {Computer Physics Communications},
  year = {1997},
  volume = {107},
  pages = {61-91}
}

@ARTICLE{Biros:2004,
  author = {Biros, George and Ying, Lexing and Zorin, Denis},
  title = {A fast solver for the {Stokes} equations with distributed forces
	in complex geometries},
  journal = {J. Comput. Phys.},
  year = {2004},
  volume = {193},
  pages = {317--348},
  number = {1},
  abstract = { We present a new method for the solution of the Stokes equations.
	The main features of our method are: (1) it can be applied to arbitrary
	geometries in a black-box fashion; (2) it is second-order accurate;
	and (3) it has optimal algorithmic complexity. Our approach, to which
	we refer as the embedded boundary integral method (EBI), is based
	on Anita Mayo's work for the Poisson's equation: "The Fast Solution
	of Poisson's and the Biharmonic Equations on Irregular Regions",
	SIAM Journal on Numerical Analysis, 21 (1984) 285-299. We embed the
	domain in a rectangular domain, for which fast solvers are available,
	and we impose the boundary conditions as interface (jump) conditions
	on the velocities and tractions. We use an indirect boundary integral
	formulation for the homogeneous Stokes equations to compute the jumps.
	The resulting equations are discretized by NystrÃ¶m's method. The
	rectangular domain problem is discretized by finite elements for
	a velocity-pressure formulation with equal order interpolation bilinear
	elements (Q1-Q1). Stabilization is used to circumvent the inf-sup
	condition for the pressure space. For the integral equations, fast
	matrix-vector multiplications are achieved via an NlogN algorithm
	based on a block representation of the discrete integral operator,
	combined with (kernel independent) singular value decomposition to
	sparsify low-rank blocks. The regular grid solver is a Krylov method
	(conjugate residuals) combined with an optimal two-level Schwartz-preconditioner.
	For the integral equation we use GMRES. We have tested our algorithm
	on several numerical examples and we have observed optimal convergence
	rates.},
  bdsk-url-1 = {http://www.sciencedirect.com/science/article/B6WHY-49M6NCJ-1/2/5bcaf7ba2244022cb062bb139ee8ecf6},
  date-added = {2008-09-14 15:32:12 -0500},
  date-modified = {2008-09-14 15:32:12 -0500},
  doi = {10.1016/j.jcp.2003.08.011 },
  keywords = {Mathematics; IntegralEquation},
  ty = {JOUR},
  url = {http://www.sciencedirect.com/science/article/B6WHY-49M6NCJ-1/2/5bcaf7ba2244022cb062bb139ee8ecf6}
}

@ARTICLE{Bischoff2005,
  author = {Bischoff, Stephan and Pavic, Darko and Kobbelt, Leif},
  title = {Automatic restoration of polygon models},
  journal = {ACM Trans. Graph.},
  year = {2005},
  volume = {24},
  pages = {1332--1352},
  number = {4},
  month = oct,
  acmid = {1095883},
  address = {New York, NY, USA},
  doi = {10.1145/1095878.1095883},
  issn = {0730-0301},
  issue_date = {October 2005},
  keywords = {Mesh repair, polygon meshes, surface extraction, voxelization},
  numpages = {21},
  publisher = {ACM},
  url = {http://doi.acm.org/10.1145/1095878.1095883}
}

@ARTICLE{Bischoff05,
  author = {Bischoff, S. and Weyand, T. and Kobbelt, L.},
  title = {Snakes on Triangle Meshes},
  journal = {Bild. für die Medizin},
  year = {2005},
  pages = {208--212}
}

@ARTICLE{Bissonnette:2009,
  author = {Bissonnette, M. L. Z. and Donald, J. E. and DeGrado, W. F. and Jardetzky,
	T. S. and Lamb, R. A.},
  title = {Functional analysis of the transmembrane domain in paramyxovirus
	F protein-mediated membrane fusion },
  journal = {Journal of Molecular Biology},
  year = {2009},
  volume = {386},
  pages = {14-36},
  annote = {Functional analysis of the transmembrane domain in paramyxovirus
	F protein-mediated membrane fusion },
  date-added = {2009-03-10 },
  date-modified = {2009-03-10},
  ty = {JOUR}
}

@ARTICLE{Blandford2005,
  author = {Blandford, Daniel K and Blelloch, Guy E and Cardoze, David E and
	Kadow, Clemens},
  title = {{Compact Representations of Simplicial Meshes in Two and Three Dimensions}},
  journal = {International Journal of Computational Geometry and Applications},
  year = {2005},
  volume = {15},
  pages = {3--24},
  number = {1},
  abstract = {We describe data structures for representing simplicial meshes compactly
	while supporting online queries and updates efficiently. Our data
	structure requires about a factor of five less memory than the most
	efficient standard data structures for triangular or tetrahedral
	meshes, while efficiently supporting traversal among simplices, storing
	data on simplices, and insertion and deletion of simplices. Our implementation
	of the data structures uses about 5 bytes/triangle in two dimensions
	(2D) and 7.5 bytes/tetrahedron in three dimensions (3D). We use the
	data structures to implement 2D and 3D incremental algorithms for
	generating a Delaunay mesh. The 3D algorithm can generate 100 Million
	tetrahedra with 1 Gbyte of memory, including the space for the coordinates
	and all data used by the algorithm. The runtime of the algorithm
	is as fast as Shewchuk's Pyramid code, the most efficient we know
	of, and uses a factor of 3.5 less memory overall.},
  editor = {Ungor, Alper},
  owner = {doubletony},
  publisher = {Citeseer},
  timestamp = {2012.04.26},
  url = {http://www.worldscinet.com/ijcga/15/1501/S0218195905001580.html}
}

@ARTICLE{Blinn:1982,
  author = {Blinn, J.},
  title = {A generalization of algebraic surface drawing},
  journal = {ACM Transactions on Graphics},
  year = {1982},
  volume = {1},
  pages = {235-256},
  number = {3}
}

@ARTICLE{Blomberg:1999,
  author = {Blomberg, N. and Gabdoulline, R. R. and Nilges, M. and Wade, R. C.},
  title = {Classification of protein sequences by homology modeling and quantitative
	analysis of electrostatic similarity},
  journal = {Proteins},
  year = {1999},
  volume = {37},
  pages = {379-387},
  number = {3},
  abstract = {Protein electrostatics plays a key role in ligand binding and protein-protein
	interactions. Therefore, similarities or dissimilarities in electrostatic
	potentials can be used as indicators of similarities or dissimilarities
	in protein function. We here describe a method to compare the electrostatic
	properties within protein families objectively and quantitatively.
	Three-dimensional structures are built from database sequences by
	comparative modeling. Molecular potentials are then computed for
	these with a continuum solvation model by finite difference solution
	of the {Poisson-Boltzmann} equation or analytically as a multipole
	expansion that permits rapid comparison of very large datasets. This
	approach is applied to 104 members of the Pleckstrin homology (PH)
	domain family. The deviation of the potentials of the homology models
	from those of the corresponding experimental structures is comparable
	to the variation of the potential in an ensemble of structures from
	nuclear magnetic resonance data or between snapshots from a molecular
	dynamics simulation. For this dataset, the results for analysis of
	the full electrostatic potential and the analysis using only monopole
	and dipole terms are very similar. The electrostatic properties of
	the PH domains are generally conserved despite the extreme sequence
	divergence in this family. Notable exceptions from this conservation
	are seen for PH domains linked to a Dbl homology (DH) domain and
	in proteins with internal PH domain repeats. Proteins 1999;37:379-387.
	Ã‚Â??999 Wiley-Liss, Inc.},
  address = {European Mol Biol Lab Heidelberg Germany D-69117 Nilges, M Meyerhofstr
	1 European Mol Biol Lab Heidelberg Germany D-69117},
  annote = {Classification of protein sequences by homology modeling and quantitative
	analysis of electrostatic similarity; NOV 15},
  bdsk-url-1 = {http://www3.interscience.wiley.com/cgi-bin/fulltext/68502071/HTMLSTART},
  date-added = {2008-09-15 10:05:57 -0500},
  date-modified = {2008-09-15 10:05:57 -0500},
  journal1 = {Protein-Struct Funct Genet},
  keywords = {Electrostatics; BiologicalSystems; Bioinformatics},
  read = {Yes},
  ty = {JOUR},
  url = {http://www3.interscience.wiley.com/cgi-bin/fulltext/68502071/HTMLSTART}
}

@ARTICLE{Blomgren:1998,
  author = {Blomgren, P. and Chan, T.F.},
  title = {Color {TV}: total variation methods for restoration of vector-valued
	images},
  journal = {Image Processing, IEEE Transactions on},
  year = {1998},
  volume = {7},
  pages = {304-309},
  number = {3},
  abstract = {We propose a new definition of the total variation (TV) norm for vector-valued
	functions that can be applied to restore color and other vector-valued
	images. The new TV norm has the desirable properties of (1) not penalizing
	discontinuities (edges) in the image, (2) being rotationally invariant
	in the image space, and (3) reducing to the usual TV norm in the
	scalar case. Some numerical experiments on denoising simple color
	images in red-green-blue (RGB) color space are presented },
  bdsk-url-1 = {http://dx.doi.org/10.1109/83.661180},
  date-added = {2008-09-16 14:47:28 -0500},
  date-modified = {2008-09-16 14:47:28 -0500},
  doi = {10.1109/83.661180},
  issn = {1057-7149},
  keywords = {Mathematics; Visualization}
}

@ARTICLE{Blumen:1989,
  author = {Blumen,A. and Zumofen,G. and Klafter,J.},
  title = {Transport aspects in anomalous diffusion: L'evy walks},
  journal = {Phys.Rev.A},
  year = {1989},
  volume = {40},
  pages = {3964?C3973},
  number = { }
}

@INPROCEEDINGS{Bobenko:2005:DWF,
  author = {Alexander I. Bobenko and Peter Schr{\"{o}}der},
  title = {Discrete Willmore Flow},
  booktitle = {Symp. on Geometry Processing},
  year = {2005},
  pages = {101--110},
  month = jul
}

@ARTICLE{Bochev:1996,
  author = {Bochev, P. and Liao, G. and Pena, G. dela},
  title = {{Analysis and computation of adaptive moving grids by deformation}},
  journal = {Numerical Methods for Partial Differential Equations},
  year = {1996},
  volume = {12},
  pages = {489--506}
}

@ARTICLE{Boda:2004-1,
  author = {Boda, D. and Gillespie, D. and Nonner, W. and Henderson, D. and Eisenberg,
	B. S.},
  title = {{Computing induced charges in inhomogeneous dielectric media: application
	in a Monte Carlo simulation of complex ionic systems.}},
  journal = {Phys Rev E Stat Nonlin Soft Matter Phys},
  year = {2004},
  volume = {69},
  pages = {046702}
}

@ARTICLE{Boda:2008,
  author = {Boda, D. and Nonner, W. and Henderson, D. and Eisenberg, B. S. and
	Gillespie, D. },
  title = {{Volume Exclusion in Calcium Selective Channels}},
  journal = {Biophys. J.},
  year = {2008},
  volume = {94},
  pages = {3486-3496}
}

@ARTICLE{Boda:2007-1,
  author = {Boda, D. and Nonner, W. and Valisko, M. and Henderson, D. and Eisenberg,
	B. S. and Gillespie, D. },
  title = {Steric Selectivity in {Na} Channels Arising from Protein Polarization
	and Mobile Side Chains},
  journal = {Biophys. J.},
  year = {2007},
  volume = {93(6)},
  pages = {1960-1980}
}

@ARTICLE{Boda:2007-2,
  author = {Boda, D. and Valisko, M. and Eisenberg, B. S. and Nonner, W. and
	Henderson, D. and Gillespie, D. },
  title = {{The combined effect of pore radius and protein dielectric coefficient
	on the selectivity of a calcium channel}},
  journal = {Physical Review Letters,},
  year = {2007},
  volume = {98},
  pages = {168102}
}

@ARTICLE{Boda:2009,
  author = {Boda, D. and Valisko, M. and Henderson, D. and Eisenberg, B. S. and
	Gillespie, D. and Nonner, W. },
  title = {{Ionic selectivity in L-type calcium channels by electrostatics and
	hard-core repulsion}},
  journal = {J. Gen. Physiol},
  year = {2009},
  volume = {133},
  pages = {497-509}
}

@ARTICLE{Boda:2004-2,
  author = {Boda, D. and Varga, T. and Henderson, D. and Busath, D. and Nonner,
	W. and Gillespie, D. and Eisenberg, B. S.},
  title = {Monte Carlo simulation study of a system with a dielectric boundary:
	application to calcium channel selectivity},
  journal = {Molecular Simulation},
  year = {2004},
  volume = {30},
  pages = {89-96}
}

@ARTICLE{Boissonnat2005,
  author = {Boissonnat, Jean-Daniel and Oudot, Steve},
  title = {Provably good sampling and meshing of surfaces},
  journal = {Graph. Models},
  year = {2005},
  volume = {67},
  pages = {405--451},
  number = {5},
  month = sep,
  acmid = {1120643},
  address = {San Diego, CA, USA},
  doi = {10.1016/j.gmod.2005.01.004},
  issn = {1524-0703},
  issue_date = {September 2005},
  keywords = {{\$\epsilon\$}-sampling, mesh refinement, restricted delaunay triangulation,
	surface approximation, surface mesh generation},
  numpages = {47},
  publisher = {Academic Press Professional, Inc.},
  url = {http://dx.doi.org/10.1016/j.gmod.2005.01.004}
}

@INPROCEEDINGS{Bolz03,
  author = {Jeff Bolz and Ian Farmer and Eitan Grinspun and Peter Schr\"{o}der},
  title = {Sparse Matrix Solvers on the GPU: conjugate gradients and multigrid},
  booktitle = {ACM SIGGRAPH},
  year = {2003},
  pages = {917--924}
}

@ARTICLE{Boor:1974,
  author = {Boor, C. D.},
  title = {{Good approximation by splines with variable knots {II}. Lecture
	Notes in Mathematics}},
  journal = {Spring-Verlag},
  year = {1974},
  pages = {12--20},
  address = {New York}
}

@ARTICLE{Borgis:2012,
  author = {Borgis, D. and Gendre, L. and Ramirez, R. },
  title = {Molecular density functional theory: application to solvation and
	electron-transfer thermodynamics in polar solvents},
  journal = {Journal of physical chemistry.},
  year = {2012},
  volume = {116},
  pages = {2504- 2512},
  number = {8}
}

@ARTICLE{Borli:2008,
  author = {Borli, H. and Kolberg, S. and Fjeldly, T. A. and Iniguez, B.},
  title = {Precise Modeling Framework for Short-Channel Double-Gate and Gate-All-Around
	MOSFETs},
  journal = {IEEE T Electron Devices},
  year = {2008},
  volume = {55},
  pages = {2678-2686},
  annote = {Precise Modeling Framework for Short-Channel Double-Gate and Gate-All-Around
	MOSFETs},
  date-added = {2008-11-25 10:28:56 -0500},
  date-modified = {2008-11-25 10:28:56 -0500},
  ty = {JOUR}
}

@ARTICLE{Borukhov:1997,
  author = {Borukhov,I. and Andelman,D.},
  title = {Steric Effects in Electrolytes: A Modified Poisson-Boltzmann Equation},
  journal = {Phys. Rev. Lett. },
  year = {1997},
  volume = {79},
  pages = {435-438},
  number = {3},
  abstract = {The adsorption of large ions from solution to a charged surface is
	investigated theoretically. A generalized Poisson-Boltzmann equation
	which takes into account the finite size of the ions is presented.
	We obtain analytical expressions for the electrostatic potential
	and ion concentrations at the surface, leading to a modified Grahame
	equation. At high surface charge densities the ionic concentration
	saturates to its maximum value. Our results are in agreement with
	recent experiments.}
}

@ARTICLE{AMG,
  author = {Alfio Borz?and Giuseppe Borzì},
  title = {Algebraic multigrid methods for solving generalized eigenvalue problems},
  journal = {Int. J. Numer. Meth. Engng},
  year = {2006},
  volume = {65},
  pages = {1186--1196}
}

@ARTICLE{Boschitsch:2007,
  author = {Boschitsch, A. H. and Fenley, M. O.},
  title = {A new outer boundary formulation and energy corrections for the nonlinear
	{{Poisson-Boltzmann}} equation},
  journal = {Journal of Computational Chemistry},
  year = {2007},
  volume = {28},
  pages = {909-21},
  number = {5},
  abstract = {The nonlinear {Poisson-Boltzmann} equation (PBE) has been successfully
	used for the prediction of numerous electrostatic properties of highly
	charged biopolyelectrolytes immersed in aqueous salt solutions. While
	numerous numerical solvers for the 3D PBE have been developed, the
	formulation of the outer boundary treatments used in these methods
	has only been loosely addressed, especially in the nonlinear case.
	The de facto standard in current nonlinear PBE implementations is
	to either set the potential at the outer boundaries to zero or estimate
	it using the (linear) Debye-HÃƒÂ¼ckel (DH) approximation. However,
	an assessment of how these outer boundary treatments affect the overall
	solution accuracy does not appear to have been previously made. As
	will be demonstrated here, both approximations can, under certain
	conditions, produce completely erroneous estimates of the potential
	and energy salt dependencies. A related concern for calculations
	carried out on grids of finite extent (e.g., all current finite difference
	and finite element implementations) is the contribution to the energy
	and salt dependence from the exterior region outside the computational
	grid. This too is shown to be significant, especially at low salt
	concentration where essentially all of the contributions to the excess
	osmotic pressure and ion stress energies originate from this exterior
	region. In this paper the authors introduce a new outer boundary
	treatment that is valid for both the linear and nonlinear PBE. The
	authors also formulate energy corrections to account for contributions
	from outside the computational domain. Finally, the authors also
	consider the effects of general ion exclusion layers upon biomolecular
	electrostatics. It is shown that while these layers tend to increase
	the surface electrostatic potential, under physiological salt conditions
	and high net charges their effect on the excess osmotic pressure
	term, which is a measure of the salt dependence of the total electrostatic
	free energy, is weak. To facilitate presentation and allow very fine
	resolutions and/or large computational domains to be considered,
	attention is restricted to the 1D spherically symmetric nonlinear
	PBE. Though geometrically limited, the modeling principles nevertheless
	extend to general PBE solvers as discussed in the Appendix. The 1D
	model can also be used to benchmark and validate the salt effect
	prediction capabilities of existing PBE solvers.},
  annote = {A new outer boundary formulation and energy corrections for the nonlinear
	{Poisson-Boltzmann} equation},
  bdsk-file-1 = {YnBsaXN0MDDUAQIDBAUGCQpYJHZlcnNpb25UJHRvcFkkYXJjaGl2ZXJYJG9iamVjdHMSAAGGoNE
	HCFRyb290gAFfEA9OU0tleWVkQXJjaGl2ZXKoCwwXGBkdJCVVJG51bGzTDQ4PEBEUViRjbGFzc1
	dOUy5rZXlzWk5TLm9iamVjdHOAB6ISE4ACgAOiFRaABIAGWWFsaWFzRGF0YVxyZWxhdGl2ZVBhd
	GjSDRobHFdOUy5kYXRhgAVPEQHSAAAAAAHSAAIAAAxNYWNpbnRvc2ggSEQAAAAAAAAAAAAAAAAA
	AADD4v5NSCsAAAAZYksZMjAwNy1Cb3NjaGl0c2NoRmVubGV5LnBkZgAAAAAAAAAAAAAAAAAAAAA
	AAAAAAAAAAAAAAAAAAAAAAAAAAAAAABliiMKAsuUAAAAAAAAAAAAEAAQAAAkgAAAAAAAAAAAAAA
	AAAAAAB0FyY2hpdmUAABAACAAAw+NSrQAAABEACAAAwoD5NQAAAAEAFAAZYksAGWIDAAqkKAAKp
	BEAAHrcAAIAT01hY2ludG9zaCBIRDpVc2VyczpiYWtlcjpEb2N1bWVudHM6UmVmZXJlbmNlczpB
	cmNoaXZlOjIwMDctQm9zY2hpdHNjaEZlbmxleS5wZGYAAA4ANAAZADIAMAAwADcALQBCAG8AcwB
	jAGgAaQB0AHMAYwBoAEYAZQBuAGwAZQB5AC4AcABkAGYADwAaAAwATQBhAGMAaQBuAHQAbwBzAG
	gAIABIAEQAEgBCVXNlcnMvYmFrZXIvRG9jdW1lbnRzL1JlZmVyZW5jZXMvQXJjaGl2ZS8yMDA3L
	UJvc2NoaXRzY2hGZW5sZXkucGRmABMAAS8AABUAAgAM//8AANIeHyAhWCRjbGFzc2VzWiRjbGFz
	c25hbWWjISIjXU5TTXV0YWJsZURhdGFWTlNEYXRhWE5TT2JqZWN0XxBCLi4vLi4vLi4vLi4vRG9
	jdW1lbnRzL1JlZmVyZW5jZXMvQXJjaGl2ZS8yMDA3LUJvc2NoaXRzY2hGZW5sZXkucGRm0h4fJi
	eiJyNcTlNEaWN0aW9uYXJ5AAgAEQAaAB8AKQAyADcAOgA/AEEAUwBcAGIAaQBwAHgAgwCFAIgAi
	gCMAI8AkQCTAJ0AqgCvALcAuQKPApQCnQKoAqwCugLBAsoDDwMUAxcAAAAAAAACAQAAAAAAAAAo
	AAAAAAAAAAAAAAAAAAADJA==},
  bdsk-url-1 = {http://dx.doi.org/10.1002/jcc.20565},
  date-added = {2008-09-01 14:02:52 -0500},
  date-modified = {2008-09-01 14:02:52 -0500},
  keywords = {Electrostatics},
  read = {Yes},
  ty = {JOUR},
  url = {http://dx.doi.org/10.1002/jcc.20565}
}

@ARTICLE{Boschitsch:2004,
  author = {Boschitsch, A. H. and Fenley, M. O.},
  title = {Hybrid boundary element and finite difference method for solving
	the nonlinear {{Poisson-Boltzmann}} equation},
  journal = {Journal of Computational Chemistry},
  year = {2004},
  volume = {25},
  pages = {935-955},
  number = {7},
  abstract = {A hybrid approach for solving the nonlinear {Poisson-Boltzmann} equation
	(PBE) is presented. Under this approach, the electrostatic potential
	is separated into (1) a linear component satisfying the linear PBE
	and solved using a fast boundary element method and (2) a correction
	term accounting for nonlinear effects and optionally, the presence
	of an ion-exclusion layer. Because the correction potential contains
	no singularities (in particular, it is smooth at charge sites) it
	can be accurately and efficiently solved using a finite difference
	method. The motivation for and formulation of such a decomposition
	are presented together with the numerical method for calculating
	the linear and correction potentials. For comparison, we also develop
	an integral equation representation of the solution to the nonlinear
	PBE. When implemented upon regular lattice grids, the hybrid scheme
	is found to outperform the integral equation method when treating
	nonlinear PBE problems. Results are presented for a spherical cavity
	containing a central charge, where the objective is to compare computed
	1D nonlinear PBE solutions against ones obtained with alternate numerical
	solution methods. This is followed by examination of the electrostatic
	properties of nucleic acid structures.},
  annote = {Hybrid boundary element and finite difference method for solving
	the nonlinear {Poisson-Boltzmann} equation; FenBo},
  bdsk-url-1 = {http://www3.interscience.wiley.com/cgi-bin/abstract/107632573/ABSTRACT},
  date-added = {2008-09-17 09:08:11 -0500},
  date-modified = {2008-09-17 09:08:11 -0500},
  keywords = {Electrostatics},
  ty = {JOUR},
  url = {http://www3.interscience.wiley.com/cgi-bin/abstract/107632573/ABSTRACT}
}

@ARTICLE{Bostrom:2005,
  author = {Bostrom, M. and Tavares, F. W. and Bratko, D. and Ninham, B. W.},
  title = {Specific Ion Effects in Solutions of Globular Proteins: Comparison
	between Analytical Models and Simulation},
  journal = {Journal of Physical Chemistry B},
  year = {2005},
  volume = {109},
  pages = {24489-94},
  number = {51},
  abstract = {Monte Carlo simulations have been performed for ion distributions
	outside a single globular macroion and for a pair of macroions, in
	different salt solutions. The model that we use includes both electrostatic
	and {van der waals} interactions between ions and between ions and
	macroions. Simulation results are compared with the predictions of
	the Ornstein-Zernike equation with the hypernetted chain closure
	approximation and the nonlinear {Poisson-Boltzmann} equation, both
	augmented by pertinent {van der waals} terms. Ion distributions from
	analytical approximations are generally very close to the simulation
	results. This demonstrates that properties that are related to ion
	distributions in the double layer outside a single interface can
	to a good approximation be obtained from the {Poisson-Boltzmann}
	equation. We also present simulation and integral equation results
	for the mean force between two globular macroions (with properties
	corresponding to those of hen-egg-white lysozyme protein at pH 4.3)
	in different salt solutions. The mean force and potential of mean
	force between the macroions become more attractive upon increasing
	the polarizability of the counterions (anions), in qualitative agreement
	with experiments. We finally show that the deduced second virial
	coefficients agree quite well with experimental results.},
  annote = {Specific Ion Effects in Solutions of Globular Proteins: Comparison
	between Analytical Models and Simulation; Compares PB with OZ equation
	and Monte Carlo simulations.},
  bdsk-url-1 = {http://dx.doi.org/10.1021/jp0551869},
  date-added = {2008-06-28 10:48:03 -0500},
  date-modified = {2008-06-28 10:48:03 -0500},
  keywords = {Solvation; Electrostatics; Protein-protein_interactions},
  ty = {JOUR},
  url = {http://dx.doi.org/10.1021/jp0551869}
}

@ARTICLE{Bothma:2010,
  author = {Bothma, J.P. and Gilmore, J.B. and McKenzie, R.H.},
  title = {The role of quantum effects in proton transfer reactions in enzymes:
	quantum tunneling in a noisy environment?},
  journal = {New Journal of Physics},
  year = {2010},
  volume = {12},
  number = { 055002 }
}

@BOOK{Botsch2010,
  title = {Polygon Mesh Processing},
  publisher = {A K Peters},
  year = {2010},
  author = {Botsch, M. and Kobbelt, L. and Pauly, M. and Alliez, P. and L{\'e}vy,
	B.},
  series = {Ak Peters Series},
  isbn = {9781568814261},
  lccn = {2009024954},
  url = {http://books.google.com/books?id=8zX-2VRqBAkC}
}

@ARTICLE{Botsch2002,
  author = {Botsch, M and Kobbelt, S Steinberg S Bischoff L},
  title = {{OpenMesh - a generic and efficient polygon mesh data structure}},
  journal = {Structure},
  year = {2002},
  volume = {2002},
  abstract = {We describe the implementation of a half-edge data structure for the
	static representation and dynamic handling of arbitrary polygonal
	meshes. The particular design of the data structures and classes
	aims at maximum flexibility and high performance. We achieve this
	by using generative programming concepts which allow the compiler
	to resolve most of the special case handling decisions at compile
	time. We evaluate our data structure based on prototypic implementations
	of mesh processing applications such as decimation and smoothing.},
  owner = {doubletony},
  publisher = {Copyright 2001, Society of Petroleum Engineers Inc.},
  timestamp = {2012.04.26},
  url = {http://citeseerx.ist.psu.edu/viewdoc/summary?doi=10.1.1.16.3900}
}

@MISC{MeshCourse,
  author = {Mario Botsch and Mark Pauly},
  title = {Geometric Modeling based on Triangle Meshes},
  year = {2006},
  note = {ACM SIGGRAPH Course}
}

@INPROCEEDINGS{MeshCourse2007,
  author = {Mario Botsch and Mark Pauly and Leif Kobbelt and Pierre Alliez and
	and Stephan Bischoff and Christian R{\"o}ssl},
  title = {Geometric Modeling Based on Polygonal Meshes},
  year = {2007},
  proceeding = {ACM SIGGRAPH Course Notes}
}

@ARTICLE{DefoMethods,
  author = {Mario Botsch and Olga Sorkine},
  title = {On Linear Variational Surface Deformation Methods},
  journal = {IEEE Transaction on Visualization on Computer Graphics},
  year = {2008},
  pages = {"to appear"}
}

@ARTICLE{Brackbill:1993,
  author = {Brackbill, J. U.},
  title = {{An adaptive grid with directional control}},
  journal = {J. Comput. Phys.},
  year = {1993},
  volume = {108},
  pages = {38--50}
}

@ARTICLE{CSF,
  author = {J. U. Brackbill and D. B. Kothe and C. Zemach},
  title = {{A Continuum Method for Modeling Surface Tension}},
  journal = {J. Comput. Phys.},
  year = {1992},
  volume = {100},
  pages = {335--354},
  number = {2}
}

@ARTICLE{Brackbill:1982,
  author = {Brackbill, J. U. and Saltzman, J. S.},
  title = {{Adaptive zoning for singular problem in two dimensions}},
  journal = {J. Comput. Phys.},
  year = {1982},
  volume = {46},
  pages = {342--368}
}

@ARTICLE{Bradley:2008,
  author = {Bradley, Michael J. and Chivers, Peter T. and Baker, Nathan A. },
  title = {Molecular Dynamics Simulation of the Escherichia coli NikR Protein:
	Equilibrium Conformational Fluctuations Reveal Interdomain Allosteric
	Communication Pathways},
  journal = {Journal of Molecular Biology},
  year = {2008},
  volume = {378},
  pages = {1155-73},
  number = {5},
  abstract = {Escherichia coli NikR is a homotetrameric Ni2+- and DNA-binding protein
	that functions as a transcriptional repressor of the NikABCDE nickel
	permease. The protein is composed of two distinct domains. The N-terminal
	50 amino acids of each chain forms part of the dimeric ribbon-helix-helix
	(RHH) domains, a well-studied DNA-binding fold. The 83-residue C-terminal
	nickel-binding domain forms an ACT (aspartokinase, chorismate mutase,
	and TyrA) fold and contains the tetrameric interface. In this study,
	we have utilized an equilibrium molecular dynamics simulation in
	order to explore the conformational dynamics of the NikR tetramer
	and determine important residue interactions within and between the
	RHH and ACT domains to gain insight into the effects of Ni2+ on DNA-binding
	activity. The molecular simulation data were analyzed using two different
	correlation measures based on fluctuations in atomic position and
	noncovalent contacts together with a clustering algorithm to define
	groups of residues with similar correlation patterns for both types
	of correlation measure. Based on these analyses, we have defined
	a series of residue interrelationships that describe an allosteric
	communication pathway between the Ni2+- and DNA-binding sites, which
	are separated by 40 \r{A}. Several of the residues identified by
	our analyses have been previously shown experimentally to be important
	for NikR function. An additional subset of the identified residues
	structurally connects the experimentally implicated residues and
	may help coordinate the allosteric communication between the ACT
	and RHH domains.},
  bdsk-file-1 = {YnBsaXN0MDDUAQIDBAUGCQpYJHZlcnNpb25UJHRvcFkkYXJjaGl2ZXJYJG9iamVjdHMSAAGGoNE
	HCFRyb290gAFfEA9OU0tleWVkQXJjaGl2ZXKoCwwXGBkdJCVVJG51bGzTDQ4PEBEUViRjbGFzc1
	dOUy5rZXlzWk5TLm9iamVjdHOAB6ISE4ACgAOiFRaABIAGWWFsaWFzRGF0YVxyZWxhdGl2ZVBhd
	GjSDRobHFdOUy5kYXRhgAVPEQHeAAAAAAHeAAIAAAxNYWNpbnRvc2ggSEQAAAAAAAAAAAAAAAAA
	AADD4v5NSCsAAAAZYkscMjAwOC1CcmFkbGV5Q2hpdmVyc0Jha2VyLnBkZgAAAAAAAAAAAAAAAAA
	AAAAAAAAAAAAAAAAAAAAAAAAAAAAAAD0rFcQ4nBwAAAAAAAAAAAAEAAQAAAkgAAAAAAAAAAAAAA
	AAAAAAB0FyY2hpdmUAABAACAAAw+NSrQAAABEACAAAxDjibAAAAAEAFAAZYksAGWIDAAqkKAAKp
	BEAAHrcAAIAUk1hY2ludG9zaCBIRDpVc2VyczpiYWtlcjpEb2N1bWVudHM6UmVmZXJlbmNlczpB
	cmNoaXZlOjIwMDgtQnJhZGxleUNoaXZlcnNCYWtlci5wZGYADgA6ABwAMgAwADAAOAAtAEIAcgB
	hAGQAbABlAHkAQwBoAGkAdgBlAHIAcwBCAGEAawBlAHIALgBwAGQAZgAPABoADABNAGEAYwBpAG
	4AdABvAHMAaAAgAEgARAASAEVVc2Vycy9iYWtlci9Eb2N1bWVudHMvUmVmZXJlbmNlcy9BcmNoa
	XZlLzIwMDgtQnJhZGxleUNoaXZlcnNCYWtlci5wZGYAABMAAS8AABUAAgAM//8AANIeHyAhWCRj
	bGFzc2VzWiRjbGFzc25hbWWjISIjXU5TTXV0YWJsZURhdGFWTlNEYXRhWE5TT2JqZWN0XxBFLi4
	vLi4vLi4vLi4vRG9jdW1lbnRzL1JlZmVyZW5jZXMvQXJjaGl2ZS8yMDA4LUJyYWRsZXlDaGl2ZX
	JzQmFrZXIucGRm0h4fJieiJyNcTlNEaWN0aW9uYXJ5AAgAEQAaAB8AKQAyADcAOgA/AEEAUwBcA
	GIAaQBwAHgAgwCFAIgAigCMAI8AkQCTAJ0AqgCvALcAuQKbAqACqQK0ArgCxgLNAtYDHgMjAyYA
	AAAAAAACAQAAAAAAAAAoAAAAAAAAAAAAAAAAAAADMw==},
  bdsk-url-1 = {http://dx.doi.org/10.1016/j.jmb.2008.03.010},
  bdsk-url-2 = {http://dx.doi.org/10.1016/j.jmb.2008.03.010},
  date-added = {2008-09-16 15:46:13 -0500},
  date-modified = {2008-09-16 15:46:13 -0500},
  doi = {10.1016/j.jmb.2008.03.010},
  keywords = {Allostery, Metalloregulation, MolecularDynamics},
  posted-at = {2008-04-26 14:52:57},
  priority = {0},
  url = {http://dx.doi.org/10.1016/j.jmb.2008.03.010}
}

@ARTICLE{Bradley:2005(a),
  author = {Bradley, P. and Malmstrom, L. and Qian, B. and Schonbrun, J. and
	Chivian, D. and Kim, D. E. and Meiler, J. and Misura, K. M. and Baker,
	D.},
  title = {{Free modeling with Rosetta in CASP6}},
  journal = {Proteins},
  year = {2005},
  volume = {61},
  pages = {91-98},
  number = {Suppl 7}
}

@ARTICLE{Bradley:2005(b),
  author = {Bradley, P. and Misura, K. M. and Baker, D.},
  title = {{Toward high-resolution de novo structure prediction for small proteins}},
  journal = {Science},
  year = {2005},
  volume = {309},
  pages = {1868-1871},
  number = {5742}
}

@ARTICLE{Bramble:1996,
  author = {Bramble, J. and King, J.},
  title = {A finite element method for interface problems in domains with smooth
	boundaries and interfaces},
  journal = {Adv. Comput. Math. },
  year = {1996},
  volume = {6},
  pages = {109-138},
  annote = {A finite element method for interface problems in domains with smooth
	boundaries and interfaces},
  date-added = {2008-09-19 10:28:56 -0500},
  date-modified = {2008-09-19 10:28:56 -0500},
  ty = {JOUR}
}



@ARTICLE{Brandsburg:2000,
  author = {Brandsburg-zabary, S and Fried, O and Marantz ,Y and Nachliel ,E
	and Gutman,M},
  title = {Biophysical aspects of intra-protein proton transfer},
  journal = {Biochim Biophys Acta},
  year = {2000},
  volume = {1458},
  pages = {120-134}
}

@ARTICLE{Braun-Sand:2005,
  author = {Braun-Sand, Sonja and Burykin, Anton and Chu, Zhen Tao and Warshel,
	Arieh },
  title = {Realistic Simulations of Proton Transport along the Gramicidin Channel:
	Demonstrating the Importance of Solvation Effects},
  journal = {J. Phys. Chem. B},
  year = {2005},
  volume = {109},
  pages = {583-592}
}

@ARTICLE{Breed:1996,
  author = {Breed, J and Sankararamakrishnan, R and Kerr ID and Sansom, Msp},
  title = {Molecular dynamics simulations of water within models of ion channels},
  journal = {Biophys J},
  year = {1996},
  volume = {70},
  pages = {1643-1661}
}

@INPROCEEDINGS{BreenOffset,
  author = {D.E. Breen and S. Mauch},
  title = {{Generating Shaded Offset Surfaces with Distance, Closest-Point and
	Color Volumes}},
  booktitle = {International Workshop on Volume Graphics},
  year = {1999},
  pages = {307--320},
  month = {March}
}

@INPROCEEDINGS{Bridson,
  author = {R. Bridson and R. Fedkiw and M. M{\"u}ller-Fischer},
  title = {Fluid Simulation},
  booktitle = {ACM SIGGRAPH Course Notes},
  year = {2006}
}

@INPROCEEDINGS{Brisson1989,
  author = {Brisson, Erik},
  title = {{Representing geometric structures in d dimensions: topology and
	order}},
  booktitle = {SCG 89 Proceedings of the fifth annual symposium on Computational
	geometry},
  year = {1989},
  volume = {9},
  pages = {218--227},
  publisher = {ACM Press},
  abstract = {We develop a representation for the topological structure of subdivided
	manifolds (with and without boundary) of dimension d &ge; 1 which
	allows straightforward access of the available order information.
	It is shown that there exists a large amount of ordering information
	in subdivided manifolds: given a k -2)-cell in the boundary of a
	k +1)-cell, 1 &le; k &le; d , all of the k - and k -1)-cells 'between
	them' can be ordered 'around' the k -2)-cell. This includes the usual
	orderings in 2- and 3-dimensional objects. We introduce the 'cell-tuple
	structure', a simple, uniform representation of the incidence and
	ordering information in a subdivided manifold. It includes the quad-edge
	data structure of Guibas and Stolfi GS 85 and the facet-edge data
	structure of Dobkin and Laszlo DL 87 as special cases in dimensions
	2 and 3, respectively.},
  doi = {10.1145/73833.73858},
  file = {:C\:/Dropbox/Dropbox/Paper/p218-brisson.pdf:pdf},
  isbn = {0897913183},
  issn = {01795376},
  issue = {1},
  owner = {doubletony},
  timestamp = {2012.04.26},
  url = {http://www.springerlink.com/index/10.1007/BF02189330}
}

@ARTICLE{Broekaert:1998,
  author = { Broekaert, T. P. E. and Brar, B. and van der Wagt J. P. A. and Seabaugh,
	A. C. and Morris, F. J. and Moise, T. S. and Beam, E. A. and Frazier,
	G. A.},
  title = { A monolithic 4-bit 2-Gsps resonant tunneling analog-to-digital converter
	},
  journal = {IEEE JOURNAL OF SOLID-STATE CIRCUITS},
  year = {1998},
  volume = {33},
  pages = {1342-1349 }
}

@ARTICLE{bronstein2007cnr,
  author = {Bronstein, A.M. and Bronstein, M.M. and Kimmel, R.},
  title = {{Calculus of non-rigid surfaces for geometry and texture manipulation}},
  journal = {IEEE Trans. on Vis. and Comp. Graphics, \emph{to appear}},
  year = {2007}
}

@TECHREPORT{bronstein2007jie,
  author = {Bronstein, A.M. and Bronstein, M.M. and Kimmel, R.},
  title = {{Joint intrinsic and extrinsic similarity for recognition of non-rigid
	shapes}},
  institution = {Dept. of CS, Technion},
  year = {2007},
  number = {CIS-2007-01}
}

@ARTICLE{bronstein2006gms,
  author = {Bronstein, A.M. and Bronstein, M.M. and Kimmel, R.},
  title = {{Generalized multidimensional scaling: A framework for isometry-invariant
	partial surface matching}},
  journal = {Proceedings of the National Academy of Sciences},
  year = {2006},
  volume = {103},
  pages = {1168--1172},
  number = {5},
  publisher = {The National Academy of Sciences}
}

@ARTICLE{bronstein2005mam,
  author = {Bronstein, M.M. and Bronstein, A.M. and Kimmel, R. and Yavneh, I.},
  title = {{A multigrid approach for multi-dimensional scaling}},
  journal = {Proc. Copper Mountain Conf. Multigrid Methods},
  year = {2005}
}

@ARTICLE{Brooks:1983,
  author = {Brooks, B. R. and Bruccoleri, R. E. and Olafson, B. D. and States,
	D.J. and Swaminathan, S. and Karplus, M.},
  title = {CHARMM: A program for macromolecular energy, minimization, and dynamics
	calculations},
  journal = {J. Comput. Chem.},
  year = {1983},
  volume = {4},
  pages = {187-217}
}


@ARTICLE{Brown:2002,
  author = {Brown, A. R. and Asenov, A. and Watling, J. R.},
  title = {Intrinsic fluctuations in sub 10-nm double-gate MOSFETs introduced
	by discreteness of charge and matter},
  journal = {IEEE Trans. Nanotechnol.},
  year = {2002},
  volume = {4},
  pages = {195-200}
}

@ARTICLE{brown2004nrr,
  author = {Brown, BJ and Rusinkiewicz, S.},
  title = {{Non-rigid range-scan alignment using thin-plate splines}},
  journal = {Int. Symp. on 3D Data Processing, Visualization and Transmission},
  year = {2004},
  pages = {759--765}
}

@ARTICLE{Buckingham:1955,
  author = { Buckingham, A. D. and Pople, J. A.},
  title = {Theoretical Studies of the Kerr Effect I: Deviations from a Linear
	Polarization Law},
  journal = {Proc. Phys. Soc. A},
  year = {1955},
  volume = {68},
  pages = {905- 909}
}

@ARTICLE{Budiono:2008,
  author = {Budiono, and Byun, D. and Nyugen, V. D. and Kim, J. and Ko, H. S.},
  title = {Free surface transition and momentum augmentation of liquid flow
	in Micro/Nano-scale channels with hydrophobic and hydrophilic surfaces},
  journal = {J. Mech. Sci. Techn.},
  year = {2008},
  volume = {22},
  pages = {2554-2562}
}

@ARTICLE{Bufler:2000,
  author = {Bufler, F. M. and Schenk, A. and Fichtner, W.},
  title = {Efficient Monte Carlo device modeling },
  journal = {IEEE T Electron Devices},
  year = {2000},
  volume = {47},
  pages = {1891-1897 },
  annote = {{Efficient Monte Carlo device modeling} },
  date-added = {2008-11-25 10:28:56 -0500},
  date-modified = {2008-11-25 10:28:56 -0500},
  ty = {JOUR}
}

@ARTICLE{Bulat07174101,
  author = {Bulat, F. A. and Heaton-Burgess, T. and Cohen, A. J. and Yang, W.
	T.},
  title = {Optimized effective potentials from electron densities in finite
	basis sets},
  journal = {Journal of Chemical Physics},
  year = {2007},
  volume = {127},
  pages = {174101},
  number = {17},
  month = {Nov},
  abstract = {The Wu-Yang method for determining the optimized effective potential
	(OEP) and implicit density functionals from a given electron density
	is revisited to account for its ill-posed nature, as recently done
	for the direct minimization method for OEP's from a given orbital
	functional [T. Heaton-Burgess, F. A. Bulat, and W. Yang, Phys. Rev.
	Lett. 98, 256401 (2007)]. To address the issues on the general validity
	and practical applicability of methods that determine the Kohn-Sham
	(local) multiplicative potential in a finite basis expansion, a new
	functional is introduced as a regularized version of the original
	work of Wu and Yang. It is shown that the unphysical, highly oscillatory
	potentials that can be obtained when unbalanced basis sets are used
	are the controllable manifestation of the ill-posed nature of the
	problem. The new method ensures that well behaved potentials are
	obtained for arbitrary basis sets. (c) 2007 American Institute of
	Physics.},
  endnotereftype = {Journal Article},
  issn = {0021-9606},
  shorttitle = {Optimized effective potentials from electron densities in finite basis
	sets},
  url = {<Go to ISI>://000250787300003}
}

@ARTICLE{Bulat08153401,
  author = {Bulat, F. A. and Ke, S. H. and Yang, W. and Couchman, L.},
  title = {Lead-molecule coupling effects on the distortion-dependent conductance
	of carbon nanotubes},
  journal = {Physical Review B},
  year = {2008},
  volume = {77},
  pages = {153401},
  number = {15},
  month = {Apr},
  abstract = {The effect of the lead-molecule coupling on the zero-bias conductance
	of carbon nanotubes as a function of tube distortion is studied.
	It is shown that the coupling strength can have a dramatic effect
	on the electromechanical characteristics. Robust conductance as a
	function of distortion is realized in the strong coupling regime,
	while sharp oscillations on the conductance for small geometrical
	changes can be observed in the weak coupling regime. The origin of
	the phenomenon is traced to the combined effect of the coupling-induced
	broadening and distortion-induced shifts of the energy levels.},
  endnotereftype = {Journal Article},
  issn = {1098-0121},
  shorttitle = {Lead-molecule coupling effects on the distortion-dependent conductance
	of carbon nanotubes},
  url = {<Go to ISI>://000255457400013 }
}

@ARTICLE{Bulat0514319,
  author = {Bulat, F. A. and Toro-Labbe, A. and Champagne, B. and Kirtman, B.
	and Yang, W. T.},
  title = {Density-functional theory (hyper)polarizabilities of push-pull pi-conjugated
	systems: Treatment of exact exchange and role of correlation - art.
	no. 014309},
  journal = {Journal of Chemical Physics},
  year = {2005},
  volume = {123},
  pages = {14319},
  number = {1},
  month = {Jul},
  abstract = {The performance of the optimized effective potential procedure for
	exact exchange in calculating static electric-field response properties
	of push-pull pi-conjugated systems has been studied, with an emphasis
	on NO2-(CH = CH)(n)-NH2 chains. Good agreement with Hartree-Fock
	dipole moments and (hyper)polarizabilities is obtained; particularly
	noteworthy is the chain length dependence for beta/n. Thus, the problem
	that conventional density-functional theory functionals dramatically
	overestimate these properties is largely solved, although there remains
	a significant correlation contribution that cannot be accounted for
	with current correlation functionals. (c) 2005 American Institute
	of Physics.},
  endnotereftype = {Journal Article},
  issn = {0021-9606},
  shorttitle = {Density-functional theory (hyper)polarizabilities of push-pull pi-conjugated
	systems: Treatment of exact exchange and role of correlation - art.
	no. 014309},
  url = {<Go to ISI>://000230493600022}
}

@ARTICLE{Bultrini:2009,
  author = {Bultrini, E. and Brick, K. and Mukherjee, S. and Zhang, Y. and Silvestrini,
	F. and Alano, P. and Pizzi, E.},
  title = {{Revisiting the Plasmodium falciparum RIFIN family: from comparative
	genomics to 3D-model prediction}},
  journal = {BMC Genomics},
  year = {2009},
  volume = {10},
  pages = {445}
}

@ARTICLE{Burch:2009,
  author = {Burch, D. and Bazant, M. Z.},
  title = {Size-Dependent Spinodal and Miscibility Gaps for Intercalation in
	Nanoparticles},
  journal = {Nano Letters},
  year = {2009},
  volume = {9},
  pages = {3795-3800.},
  number = {11}
}

@ARTICLE{Burger:2007,
  author = {Burger, Martin and Eisenberg, B. S. and Heinz, Engl},
  title = {Inverse Problems Related to Ion Channel Selectivity},
  journal = {SIAM J Applied Math},
  year = {2002},
  volume = {67},
  pages = {960-989},
  number = {4},
  month = { }
}

@ARTICLE{Burger07164107,
  author = {Burger, S. K. and Yang, W.},
  title = {Sequential quadratic programming method for determining the minimum
	energy path},
  journal = {Journal of Chemical Physics},
  year = {2007},
  volume = {127},
  pages = {164107},
  number = {16},
  month = {Oct},
  abstract = {A new method, referred to as the sequential quadratic programming
	method, is presented for determining minimum energy paths. The method
	is based on minimizing the points representing the path in the subspace
	perpendicular to the tangent of the path while using a penalty term
	to prevent kinks from forming. Rather than taking one full step,
	the minimization is divided into a number of sequential steps on
	an approximate quadratic surface. The resulting method can efficiently
	determine the reaction mechanism, from which transition state can
	be easily identified and refined with other methods. To improve the
	resolution of the path close to the transition state, points are
	clustered close to this region with a reparametrization scheme. The
	usefulness of the algorithm is demonstrated for the Muller-Brown
	potential, amide hydrolysis, and an 89 atom cluster taken from the
	active site of 4-oxalocrotonate tautomerase for the reaction which
	catalyzes 2-oxo-4-hexenedioate to the intermediate 2-hydroxy-2,4-hexadienedioate.
	(C) 2007 American Institute of Physics.},
  endnotereftype = {Journal Article},
  issn = {0021-9606},
  shorttitle = {Sequential quadratic programming method for determining the minimum
	energy path},
  url = {<Go to ISI>://000250589400009}
}

@ARTICLE{Burger08294209,
  author = {Burger, S. K. and Yang, W. T.},
  title = {Linear-scaling quantum calculations using non-orthogonal localized
	molecular orbitals},
  journal = {Journal of Physics-Condensed Matter},
  year = {2008},
  volume = {20},
  pages = {294209},
  number = {29},
  month = {Jul},
  abstract = {An absolute energy minimum variational principle is used for carrying
	out linear-scaling calculations with non-orthogonal localized orbitals.
	Comparing with results based on orthogonal localized molecular orbitals,
	the method is shown to give significantly more accurate results when
	the localized molecular orbitals are allowed to be non-orthogonal.
	This is made possible by introducing a second minimization for approximating
	the inverse overlap matrix. We also show how an exact line search
	may be used efficiently with the conjugate gradient method for minimizing
	the energy functional.},
  endnotereftype = {Journal Article},
  issn = {0953-8984},
  shorttitle = {Linear-scaling quantum calculations using non-orthogonal localized
	molecular orbitals},
  url = {<Go to ISI>://000257325900014}
}

@ARTICLE{Burger:2008,
  author = {Burger, S. K. and Yang, W. T.},
  title = {Linear-scaling quantum calculations using non-orthogonal localized
	molecular orbitals},
  journal = {J. Phys. Conden Matter},
  year = {2008},
  volume = {20},
  number = {294209 }
}

@ARTICLE{Burger06224102,
  author = {Burger, S. K. and Yang, W. T.},
  title = {A combined explicit-implicit method for high accuracy reaction path
	integration},
  journal = {Journal of Chemical Physics},
  year = {2006},
  volume = {124},
  pages = {224102},
  number = {22},
  month = {Jun},
  abstract = {We present the use of an optimal combined explicit-implicit method
	for following the reaction path to high accuracy. This is in contrast
	to most purely implicit reaction path integration algorithms, which
	are only efficient on stiff ordinary differential equations. The
	defining equation for the reaction path is considered to be stiff,
	however, we show here that the reaction path is not uniformly stiff
	and instead is only stiff near stationary points. The optimal algorithm
	developed in this work is a combination of explicit and implicit
	methods with a simple criterion to switch between the two. Using
	three different chemical reactions, we combine and compare three
	different integration methods: the implicit trapezoidal method [C.
	Gonzalez and H. Schlegel, J. Chem. Phys. 90, 2154 (1989)], an explicit
	stabilized third order algorithm [A. A. Medovikov, BIT 38, 372 (1998)]
	implemented in the code DUMKA3 and the traditional explicit fourth
	order Runge-Kutta method written in the code DUMKA3. The results
	for high accuracy show that when the implicit trapezoidal method
	is combined with either explicit method the number of energy and
	gradient calculations can potentially be reduced by almost a half
	compared with integrating either method alone. Finally, to explain
	the improvements of the combined method we expand on the concepts
	of stability and stiffness and relate them to the efficiency of integration
	methods. (c) 2006 American Institute of Physics.},
  endnotereftype = {Journal Article},
  issn = {0021-9606},
  shorttitle = {A combined explicit-implicit method for high accuracy reaction path
	integration},
  url = {<Go to ISI>://000238279800006}
}

@ARTICLE{Burger06244108,
  author = {Burger, S. K. and Yang, W. T.},
  title = {Automatic integration of the reaction path using diagonally implicit
	Runge-Kutta methods},
  journal = {Journal of Chemical Physics},
  year = {2006},
  volume = {125},
  pages = {244108},
  number = {24},
  month = {Dec},
  abstract = {The diagonally implicit Runge-Kutta framework is shown to be a general
	form for constructing stable, efficient steepest descent reaction
	path integrators, of any order. With this framework tolerance driven,
	adaptive step-size methods can be constructed by embedding methods
	to obtain error estimates of each step without additional computational
	cost. There are many embedded and nonembedded, diagonally implicit
	Runge-Kutta methods available from the numerical analysis literature
	and these are reviewed for orders two, three, and four. New embedded
	methods are also developed which are tailored to the application
	of reaction path following. All integrators are summarized and compared
	for three systems: the Muller-Brown [Theor. Chem. Acta 53, 75 (1979)]
	potential and two gas phase chemical reactions. The results show
	that many of the methods are capable of integrating efficiently while
	reliably keeping the error bound within the desired tolerance. This
	allows the reaction path to be determined through automatic integration
	by only specifying the desired accuracy and transition state. (c)
	2006 American Institute of Physics.},
  endnotereftype = {Journal Article},
  issn = {0021-9606},
  shorttitle = {Automatic integration of the reaction path using diagonally implicit
	Runge-Kutta methods},
  url = {<Go to ISI>://000243158000010}
}

@ARTICLE{Burger0654109,
  author = {Burger, S. K. and Yang, W. T.},
  title = {Quadratic string method for determining the minimum-energy path based
	on multiobjective optimization},
  journal = {Journal of Chemical Physics},
  year = {2006},
  volume = {124},
  pages = {54109},
  number = {5},
  month = {Feb},
  abstract = {Based on a multiobjective optimization framework, we develop a new
	quadratic string method for finding the minimum-energy path. In the
	method, each point on the minimum-energy path is minimized by integration
	in the descent direction perpendicular to path. Each local integration
	is done on a quadratic surface approximated by a damped Broyden-Fletcher-Goldfarb-Shanno
	updated Hessian, allowing the algorithm to take many steps between
	energy and gradient calls. The integration is performed with an adaptive
	step-size solver, which is restricted in length to the trust radius
	of the approximate Hessian. The full algorithm is shown to be capable
	of practical superlinear convergence, in contrast to the linear convergence
	of other methods. The method also eliminates the need for predetermining
	such parameters as step size and spring constants, and is applicable
	to reactions with multiple barriers. The effectiveness of this method
	is demonstrated for the Muller-Brown potential, a seven-atom Lennard-Jones
	cluster, and the enolation of acetaldehyde to vinyl alcohol. (c)
	2006 American Institute of Physics.},
  endnotereftype = {Journal Article},
  issn = {0021-9606},
  shorttitle = {Quadratic string method for determining the minimum-energy path based
	on multiobjective optimization},
  url = {<Go to ISI>://000235171100009}
}

@ARTICLE{Burke:2005,
  author = {Burke, K. and Werschnik, J. and Gross, E. K. U.},
  title = { Time-dependent density functional theory: Past, present, and future},
  journal = {J. Chem. Phys.},
  year = {2005},
  volume = {123},
  pages = {062206}
}

@ARTICLE{Burke:2005,
  author = {Burke, K. and Werschnik, J. and Gross, E. K. U.},
  title = { Time-dependent density functional theory: Past, present, and future},
  journal = {J. Chem. Phys.},
  year = {2005},
  volume = {123},
  pages = {062206}
}

@ARTICLE{Burman:2010,
  author = {Burman, Erik and Hansbo, Peter},
  title = {Interior-penalty-stabilized {Lagrange} multiplier methods for the
	finite-element solution of elliptic interface problems
	
	},
  journal = {IAM J. Numer. Anal.},
  year = {2010},
  volume = {30},
  pages = {870-885}
}

@ARTICLE{Cai:2003,
  author = {Cai, W. and Deng, S. Z.},
  title = {An upwinding embedded boundary method for {Maxwell's} equations in
	media with material interfaces: 2D case},
  journal = {J. Comput. Phys.},
  year = {2003},
  volume = {190},
  pages = {159-183},
  annote = {An upwinding embedded boundary method for {Maxwell's} equations in
	media with material interfaces: 2D case},
  date-added = {2008-09-19 10:28:56 -0500},
  date-modified = {2008-09-19 10:28:56 -0500},
  ty = {JOUR}
}

@ARTICLE{cai89,
  author = {Cai, W. and Gottlieb, D. and Shu, C.-W.}
}

@ARTICLE{cai93,
  author = {Cai, W. and Shu, C. -W.},
  title = {Uniform high-order spectral methods for one- and two-dimensional
	Euler equations},
  journal = {J. Comput. Phys.},
  year = {1993},
  volume = {104},
  pages = {427-443}
}


@ARTICLE{ZXu:2011,
  author = {Xu, Z. L. and  Cai, W.},
  title = {Fast Analytical Methods for Macroscopic Electrostatic Models in Biomolecular Simulations},
  journal = {SIAM REVIEW},
  year = {2011},
  volume = {53},
  pages = {683-720}
}

@ARTICLE{ZXu:2011b,
  author = {Xu, Z. L. and  Cai, W. and Cheng, Xiaolin},
  title = { Image Charge Method for Reaction Fields in a Hybrid Ion-Channel Model},
  journal = { Commun. Comput. Phys.},
  year = {2011},
  volume = {9},
  pages = {1056-1070}
}

@ARTICLE{ZCai:2011,
  author = {Cai, Zhiqiang and Ye, Xiu and Zhang, Shun},
  title = {Discontinuous {Galerkin} Finite Element Methods for Interface Problems:
	{A} Priori and A Posteriori Error Estimations		},
  journal = {SIAM J. Numer. Anal.},
  year = {2011},
  volume = {49},
  pages = {1761-1787}
}

@ARTICLE{Cances:1997,
  author = {Cances, E. and Mennucci, B. and Tomasi, J.},
  title = {A new integral equation formalism for the polarizable continuum model:
	Theoretical background and applications to isotropic and anisotropic
	dielectrics},
  journal = {Journal of Chemical Physics},
  year = {1997},
  volume = {107},
  pages = {3032 -- 3041}
}

@ARTICLE{Canham:1970,
  author = {Canham, P. B.},
  title = { The Minimum Energy of Bending as a Possible Explanation of the Biconcave
	Shape of the Human Red Blood Cell},
  journal = {Journal of Theoretical Biology},
  year = {1970},
  volume = {26},
  pages = {61 - 81}
}

@ARTICLE{Canutescu:2003,
  author = {Canutescu, A. A. and Shelenkov, A. A. and Dunbrack, R. L. Jr.},
  title = {{A graph-theory algorithm for rapid protein side-chain prediction}},
  journal = {Protein Sci},
  year = {2003},
  volume = {12},
  pages = {2001-2014},
  number = {9}
}

@ARTICLE{CHQZ,
  author = {Canuto, C. and Hussaini, M. Y. and Quarteroni, A. and Zang, T. A.
	},
  title = {Spectral methods in fluid dynamics},
  journal = {Springer-Verlag, Berlin},
  year = {1988}
}

@ARTICLE{HCao:2002,
  author = {Cao, H. and Yu, Z. N. and Wang, J. and Tegenfeldt, J. O. and Austin,
	R. H. and Chen, E. and Wu, W. and Chou, S. Y. },
  title = {Fabrication of 10 nm enclosed nanofluidic channels },
  journal = {Appl. Phys. Lett. },
  year = {2002},
  volume = {81},
  pages = {174-176 },
  number = { }
}

@ARTICLE{Weiming:1999,
  author = {Cao, W. and Huang, W. and Russell, R. D. },
  title = {{An $r-$adaptive finite element method based upon moving mesh PDEs}},
  journal = {J. Comput. Phys.},
  year = {1999},
  volume = {149},
  pages = {221--244}
}

@ARTICLE{Caputo:1997,
  author = {Caputo, M.},
  title = {Linear model of dissipation whose W is almost frequency independent},
  journal = {Geophys. J. R. Astr. Soc. },
  year = {1997},
  volume = {13},
  pages = {529 -539}
}

@ARTICLE{Cardenas:2000,
  author = {Cardenas, Alfredo E. and Coalson, Rob D. and Kurnikova, Maria G.
	},
  title = {Three{-}Dimensional {Poisson-Nernst-Planck} Theory Studies: Influence
	of Membrane Electrostatics on {Gramicidin A} Channel Conductance},
  journal = {Biophysical Journal},
  year = {2000},
  volume = {79},
  pages = {80-93},
  month = {July}
}

@ARTICLE{CZCG05,
  author = {Carlsson, G. and Zomorodian, A. and Collins, A. and Guibas, L. J.},
  title = {Persistence Barcodes for Shapes},
  journal = {International Journal of Shape Modeling},
  year = {2005},
  volume = {11},
  pages = {149--187},
  number = {2},
  owner = {Yiying},
  timestamp = {2009.03.28}
}

@ARTICLE{Carstensen:1997,
  author = {Carstensen, V. and Kimmel, R. and Sapiro, G.},
  title = {Geodesic active contours},
  journal = {International Journal of Computer Vision},
  year = {1997},
  volume = {22},
  pages = {61-79},
  date-added = {2008-09-16 14:49:04 -0500},
  date-modified = {2008-09-16 14:49:41 -0500}
}

@ARTICLE{caselles-kimmel-etal:97,
  author = {Caselles, V. and Kimmel, R. and Sapiro, G.},
  title = {Geodesic Active Contours},
  journal = {IJCV},
  year = {1997},
  volume = {22},
  pages = {61--79},
  number = {1}
}

@ARTICLE{Caughey:1967,
  author = { Caughey, D. M. and Thomas, R. E. },
  title = {Carrier mobilities in silicon empirically related to doping and field},
  journal = {IEEE Proc.},
  year = {1967},
  volume = {55},
  pages = {2192-2193},
  annote = {Carrier mobilities in silicon empirically related to doping and field},
  date-added = {2008-11-25 10:28:56 -0500},
  date-modified = {2008-11-25 10:28:56 -0500},
  ty = {JOUR}
}

@ARTICLE{Cecil:2005,
  author = {Cecil, Thomas},
  title = {A numerical method for computing minimal surfaces in arbitrary dimension},
  journal = {J. Comput. Phys.},
  year = {2005},
  volume = {206},
  pages = {650--660},
  number = {2},
  abstract = { In this paper we propose a numerical method for computing minimal
	surfaces with fixed boundaries. The level set method is used to evolve
	a codimension-1 surface with fixed codimension-2 boundary in under
	mean curvature flow. For n = 3 the problem has been approached in
	D.L. Chopp, 1993 and L.-T. Cheng [D.L. Chopp, Computing minimal surfaces
	via level set curvature flow, J. Comput. Phys. 106(1) (1993) 77-91
	and L.-T. Cheng, The level set method applied to geometrically based
	motion, materials science, and image processing, UCLA CAM Report,
	00-20] using the level set method, but with a more complicated boundary
	conditions. The method we present can be generalized straightforward
	to arbitrary dimension, and the framework in which it is presented
	is dimension independent. Examples are shown for n = 2, 3, 4.},
  bdsk-url-1 = {http://www.sciencedirect.com/science/article/B6WHY-4FF9HGD-4/2/dca5a02d04877693eab264a92996ea97},
  date-added = {2008-09-16 14:37:53 -0500},
  date-modified = {2008-09-16 14:37:53 -0500},
  doi = {10.1016/j.jcp.2004.12.022},
  keywords = {Mathematics},
  ty = {JOUR},
  url = {http://www.sciencedirect.com/science/article/B6WHY-4FF9HGD-4/2/dca5a02d04877693eab264a92996ea97}
}

@ARTICLE{Celes2005,
  author = {Celes, Waldemar and Paulino, Glaucio H. and Espinha, Rodrigo},
  title = {{A compact adjacency-based topological data structure for finite
	element mesh representation}},
  journal = {International Journal for Numerical Methods in Engineering},
  year = {2005},
  volume = {64},
  pages = {1529--1556},
  number = {11},
  month = nov,
  doi = {10.1002/nme.1440},
  file = {:C\:/Dropbox/Dropbox/Paper/05celes_compactadjacency.pdf:pdf},
  issn = {0029-5981},
  keywords = {finite element,implicit entities,reduced representation,topological
	data structure},
  owner = {doubletony},
  timestamp = {2012.04.26},
  url = {http://doi.wiley.com/10.1002/nme.1440}
}

@ARTICLE{Cerutti:2007,
  author = {Cerutti, D. S. and Baker, N. A. and McCammon, J. A.},
  title = {Solvent reaction field potential inside an uncharged globular protein:
	A bridge between implicit and explicit solvent models?},
  journal = {The Journal of Chemical Physics},
  year = {2007},
  volume = {127},
  pages = {155101},
  number = {15},
  abstract = {The solvent reaction field potential of an uncharged protein immersed
	in simple point charge/extended explicit solvent was computed over
	a series of molecular dynamics trajectories, in total 1560 ns of
	simulation time. A finite, positive potential of 13--24 kbTec-1"
	align="middle"> (where T=300 K), dependent on the geometry of the
	solvent-accessible surface, was observed inside the biomolecule.
	The primary contribution to this potential arose from a layer of
	positive charge density 1.0 Ã-from the solute surface, on average
	0.008 ec/Ã-, which we found to be the product of a highly ordered
	first solvation shell. Significant second solvation shell effects,
	including additional layers of charge density and a slight decrease
	in the short-range solvent-solvent interaction strength, were also
	observed. The impact of these findings on implicit solvent models
	was assessed by running similar explicit solvent simulations on the
	fully charged protein system. When the energy due to the solvent
	reaction field in the uncharged system is accounted for, correlation
	between per-atom electrostatic energies for the explicit solvent
	model and a simple implicit (Poisson) calculation is 0.97, and correlation
	between per-atom energies for the explicit solvent model and a previously
	published, optimized Poisson model is 0.99. Â©2007 American Institute
	of Physics},
  bdsk-file-1 = {YnBsaXN0MDDUAQIDBAUGCQpYJHZlcnNpb25UJHRvcFkkYXJjaGl2ZXJYJG9iamVjdHMSAAGGoNE
	HCFRyb290gAFfEA9OU0tleWVkQXJjaGl2ZXKoCwwXGBkdJCVVJG51bGzTDQ4PEBEUViRjbGFzc1
	dOUy5rZXlzWk5TLm9iamVjdHOAB6ISE4ACgAOiFRaABIAGWWFsaWFzRGF0YVxyZWxhdGl2ZVBhd
	GjSDRobHFdOUy5kYXRhgAVPEQHiAAAAAAHiAAIAAAxNYWNpbnRvc2ggSEQAAAAAAAAAAAAAAAAA
	AADD4v5NSCsAAAAZYksdMjAwNy1DZXJ1dHRpQmFrZXJNY2NhbW1vbi5wZGYAAAAAAAAAAAAAAAA
	AAAAAAAAAAAAAAAAAAAAAAAAAAAAAABlimcM6BydQREYgcHJ2dwAEAAQAAAkgAAAAAAAAAAAAAA
	AAAAAAB0FyY2hpdmUAABAACAAAw+NSrQAAABEACAAAwzpNdwAAAAEAFAAZYksAGWIDAAqkKAAKp
	BEAAHrcAAIAU01hY2ludG9zaCBIRDpVc2VyczpiYWtlcjpEb2N1bWVudHM6UmVmZXJlbmNlczpB
	cmNoaXZlOjIwMDctQ2VydXR0aUJha2VyTWNjYW1tb24ucGRmAAAOADwAHQAyADAAMAA3AC0AQwB
	lAHIAdQB0AHQAaQBCAGEAawBlAHIATQBjAGMAYQBtAG0AbwBuAC4AcABkAGYADwAaAAwATQBhAG
	MAaQBuAHQAbwBzAGgAIABIAEQAEgBGVXNlcnMvYmFrZXIvRG9jdW1lbnRzL1JlZmVyZW5jZXMvQ
	XJjaGl2ZS8yMDA3LUNlcnV0dGlCYWtlck1jY2FtbW9uLnBkZgATAAEvAAAVAAIADP//AADSHh8g
	IVgkY2xhc3Nlc1okY2xhc3NuYW1loyEiI11OU011dGFibGVEYXRhVk5TRGF0YVhOU09iamVjdF8
	QRi4uLy4uLy4uLy4uL0RvY3VtZW50cy9SZWZlcmVuY2VzL0FyY2hpdmUvMjAwNy1DZXJ1dHRpQm
	FrZXJNY2NhbW1vbi5wZGbSHh8mJ6InI1xOU0RpY3Rpb25hcnkACAARABoAHwApADIANwA6AD8AQ
	QBTAFwAYgBpAHAAeACDAIUAiACKAIwAjwCRAJMAnQCqAK8AtwC5Ap8CpAKtArgCvALKAtEC2gMj
	AygDKwAAAAAAAAIBAAAAAAAAACgAAAAAAAAAAAAAAAAAAAM4},
  bdsk-url-1 = {http://dx.doi.org/10.1063/1.2771171},
  bdsk-url-2 = {http://dx.doi.org/10.1063/1.2771171},
  date-added = {2008-06-28 10:49:26 -0500},
  date-modified = {2008-06-28 10:49:26 -0500},
  doi = {10.1063/1.2771171},
  keywords = {solvation, nonpolar, molecular\_simulation, electrostatics},
  priority = {0},
  publisher = {AIP},
  url = {http://dx.doi.org/10.1063/1.2771171}
}

@ARTICLE{Truhlar:2006,
  author = {Chamberlin, A. and Cramer, C. and Truhlar, D.},
  title = {Predicting Aqueous Free Energies of Solvation as Functions of Temperature},
  journal = {J. Phys. Chem. B},
  year = {2006},
  volume = {110},
  pages = {5665-5675}
}

@ARTICLE{AChambolle:1997,
  author = {Chambolle, A. and Lions, P. L.},
  title = {Image recovery via total variation minimization and related problems},
  journal = {Numerische Mathematik},
  year = {1997},
  volume = {76},
  pages = {167-188},
  number = {2},
  abstract = {We study here a classical image denoising technique introduced by
	L. Rudin and S. Osher a few years ago, namely the constrained minimization
	of the total variation (TV) of the image. First, we give results
	of existence and uniqueness and prove the link between the constrained
	minimization problem and the minimization of an associated Lagrangian
	functional. Then we describe a relaxation method for computing the
	solution, and give a proof of convergence. After this, we explain
	why the TV-based model is well suited to the recovery of some images
	and not of others. We eventually propose an alternative approach
	whose purpose is to handle the minimization of the minimum of several
	convex functionals. We propose for instance a variant of the original
	TV minimization problem that handles correctly some situations where
	TV fails.}
}

@ARTICLE{Champagne06194114,
  author = {Champagne, B. and Bulat, F. A. and Yang, W. T. and Bonness, S. and
	Kirtman, B.},
  title = {Density functional theory investigation of the polarizability and
	second hyperpolarizability of polydiacetylene and polybutatriene
	chains: Treatment of exact exchange and role of correlation},
  journal = {Journal of Chemical Physics},
  year = {2006},
  volume = {125},
  pages = {194114},
  number = {19},
  month = {Nov},
  abstract = {The static polarizability and second hyperpolarizability of increasingly
	large polydiacetylene and polybutatriene (PBT) chains have been evaluated
	using the optimized effective potential for exact exchange (OEP-EXX)
	method developed by Yang and Wu [Phys. Rev. Lett. 89, 143002 (2002)],
	where the unknown part of the effective potential is expressed as
	a linear combination of Gaussian functions. Various conventional
	atomic orbital basis sets were employed for the exchange potential
	(X basis) as well as for the Kohn-Sham orbitals [molecular orbital
	(MO) basis]. Our results were compared to coupled-perturbed Hartree-Fock
	(CPHF) calculations and to ab initio correlated values obtained at
	various levels of approximation. It turns out that (a) small conventional
	basis sets are, in general, unsatisfactory for the X basis; (b) the
	performance of a given X basis depends on the MO basis and is generally
	improved when using a larger MO basis; (c) these effects are exaggerated
	for the second hyperpolarizability compared to the polarizability;
	(d) except for the second hyperpolarizability of PBT chains, using
	6-311++G** for the X basis gives reasonable agreement with the CPHF
	results for all MO basis sets; (e) our results suggest that in the
	limit of a complete X basis the OEP-EXX values may approach the CPHF
	data; and (f) in general, the quality of a given conventional X basis
	degrades with the length of the oligomer, which correlates with the
	fact that the number of X basis functions becomes a smaller fraction
	of the number required to reproduce exactly the finite-basis-set
	Hartree-Fock energies. Linear and especially nonlinear electric field
	responses constitute a very stringent test for assessing the quality
	of functionals and potentials; appropriately tailored basis sets
	are needed to describe the latter. Finally, this study further highlights
	the importance of electron correlation effects on linear and nonlinear
	responses, for which correlated functionals with OEP are required.
	(c) 2006 American Institute of Physics.},
  endnotereftype = {Journal Article},
  issn = {0021-9606},
  shorttitle = {Density functional theory investigation of the polarizability and
	second hyperpolarizability of polydiacetylene and polybutatriene
	chains: Treatment of exact exchange and role of correlation},
  url = {<Go to ISI>://000242181800016}
}

@ARTICLE{TChan:2000,
  author = {Chan, T. and Marquina, A. and Mulet, P.},
  title = {High-order total variation-based image restoration},
  journal = {{SIAM} Journal on Scientific Computing},
  year = {2000},
  volume = {22},
  pages = {503-516},
  number = {2},
  abstract = {The total variation ( TV) denoising method is a {{PDE}}-based technique
	that preserves edges well but has the sometimes undesirable staircase
	effect, namely, the transformation of smooth regions ( ramps) into
	piecewise constant regions ( stairs). In this paper we present an
	improved model, constructed by adding a nonlinear fourth order diffusive
	term to the Euler-Lagrange equations of the variational TV model.
	Our technique substantially reduces the staircase effect, while preserving
	sharp jump discontinuities ( edges). We show numerical evidence of
	the power of resolution of this novel model with respect to the TV
	model in some 1D and 2D numerical examples.}
}

@ARTICLE{ChanVese,
  author = {Tony Chan and Luminita Vese},
  title = {{Active Contours without Edges}},
  journal = {IEEE Trans. Image Processing},
  year = {2001},
  volume = {10},
  pages = {266--277},
  number = {2}
}

@ARTICLE{Chan:2009,
  author = {Chan, T. and Wang, Y. and Zhou, H.},
  title = {Multiscale total variation and multiscale anisotropic diusion algorithms
	for image denoising},
  journal = {Preprint},
  year = {2009}
}

@ARTICLE{Chan:2009b,
  author = {Chan, T. and Wang, Y. and Zhou, H.},
  title = {Denoising natural color images},
  journal = {Preprint},
  year = {2009}
}

@ARTICLE{ChaZho07,
  author = {Chan, T.F. and Zhou, H. M.},
  title = {Total Variation Wavelet Thresholding},
  journal = {Scientific Computing},
  year = {2007},
  volume = {32},
  pages = {315-341}
}

@ARTICLE{ChShZh06,
  author = {Chan, T. F. and J. Shen and Zhou, H. M.},
  title = { Total Variation Wavelet Inpainting},
  journal = {Journal of Mathematical Imaging and Vision},
  year = {2006},
  volume = {25},
  pages = {107-125},
  number = { }
}

@ARTICLE{ChaZho02,
  author = {Chan, T. F. and Zhou, H. M.},
  title = { {ENO-wavelet} Transforms for Piecewise Smooth Functions},
  journal = {SIAM J. Numer. Anal.},
  year = {2002},
  volume = {40},
  pages = {1369--1404},
  number = { }
}

@ARTICLE{Chang:2009,
  author = {Chang, C. C. and Yang, R. J.},
  title = {A perspective on streaming current in silica nanofluidic channels:
	{Poisson-Boltzmann} model versus {Poisson-Nernst-Planck} model},
  journal = {J. Colliod Interface Sci.},
  year = {2009},
  volume = {339},
  pages = {517-520}
}

@ARTICLE{QSChang:2010,
  author = {Chang, Q.S. and Tai, X.C. and Xing, L.},
  title = {A Compound Algorithm of Denoising Using Second-Order and Fourth-Order
	Partial Differential Equations },
  journal = {NUMERICAL MATHEMATICS-THEORY METHODS AND APPLICATIONS},
  year = {2010},
  volume = {2},
  pages = {353-376}
}

@ARTICLE{charpiat-faugeras-etal:05,
  author = {Charpiat, G. and Faugeras, O. and Keriven, R.},
  title = {Approximations of Shape Metrics and Application to Shape Warping
	and Empirical Shape Statistics},
  journal = {FoCM},
  year = {2005},
  volume = {5},
  pages = {1--58},
  number = {1}
}

@INPROCEEDINGS{charpiat-keriven-etal:05,
  author = {Charpiat, G. and Keriven, R. and Pons, J.-P. and Faugeras, O.},
  title = {Designing Spatially Coherent Minimizing Flows for Variational Problems
	Based on Active Contours},
  booktitle = {International Conference on Computer Vision},
  year = {2005},
  volume = {2},
  pages = {1403--1408}
}

@TECHREPORT{charpiat-maurel-etal:06,
  author = {Charpiat, G. and Maurel, P. and Pons, J.-P. and Keriven, R. and Faugeras,
	O.},
  title = {Generalized Gradients: Priors on Minimization Flows},
  institution = {ENPC-CERTIS},
  year = {2006},
  number = {06-23},
  month = {march}
}

@ARTICLE{Che:2008,
  author = {Che, J. and Dzubiella, J. and Li, B. and McCammon, J. A. },
  title = {Electrostatic Free Energy and Its Variations in Implicit Solvent
	Models},
  journal = {Journal of Physical Chemistry B},
  year = {2008},
  volume = {112},
  pages = {3058-69},
  number = {10},
  abstract = {Abstract: A mean-field approach to the electrostatics for solutes
	in electrolyte solution is revisited and rigorously justified. In
	this approach, an electrostatic free energy functional is constructed
	that depends solely on the local ionic concentrations. The unique
	set of such concentrations that minimize this free energy are given
	by the usual Boltzmann distributions through the electrostatic potential
	which is determined by the {Poisson-Boltzmann} equation. This approach
	is then applied to the variational implicit solvent description of
	the solvation of molecules [Dzubiella, Swanson, McCammon, Phys. Rev.
	Lett. 2006, 96, 087802; J. Chem. Phys. 2006, 124, 084905]. Care is
	taken for the singularities of the potential generated by the solute
	point charges. The variation of the electrostatic free energy with
	respect to the location change of solute-solvent interfaces, that
	is, dielectric boundaries, is derived. Such a variation gives rise
	to the normal component of the effective surface force per unit surface
	area that is shown to be attractive to the fixed point charges in
	the solutes. Two examples of applications are given to validate the
	analytical results. The first one is a one-dimensional model system
	resembling, for example, a charged solute or cavity in a one-dimensional
	channel. The second one, which is of its own interest, is the electrostatic
	free energy of a charged sphercal solute immersed in an ionic solution.
	An analytical formula is derived for the Debye-H\"{u}ckel approximation
	of the free energy, extending the classical Born's formula to one
	that includes ionic concentrations. Variations of the nonlinear {Poisson-Boltzmann}
	free energy are also obtained.},
  address = {The Genomics Institute of the Novartis Research Foundation, 10675
	John Jay Hopkins Drive, San Diego, California 92121, Physik Department
	(T37), Technische Universit\"{a}t M\"{u}nchen (TUM), James-Franck-Strasse,
	85748 Garching, Germany, Department of Mathematics and NSF Center
	for Theoretical Biological Physics (CTBP), University of California,
	San Diego, La Jolla, California 92093-0112, and Department of Chemistry
	and Biochemistry, Department of Pharmacology, and NSF Center for
	Theoretical Biological Physics (CTBP), University of California,
	San Diego, La Jolla, California 92093-0365},
  bdsk-file-1 = {YnBsaXN0MDDUAQIDBAUGCQpYJHZlcnNpb25UJHRvcFkkYXJjaGl2ZXJYJG9iamVjdHMSAAGGoNE
	HCFRyb290gAFfEA9OU0tleWVkQXJjaGl2ZXKoCwwXGBkdJCVVJG51bGzTDQ4PEBEUViRjbGFzc1
	dOUy5rZXlzWk5TLm9iamVjdHOAB6ISE4ACgAOiFRaABIAGWWFsaWFzRGF0YVxyZWxhdGl2ZVBhd
	GjSDRobHFdOUy5kYXRhgAVPEQHqAAAAAAHqAAIAAAxNYWNpbnRvc2ggSEQAAAAAAAAAAAAAAAAA
	AADD4v5NSCsAAAAZYksfMjAwOC1DaGVEenViaWVsbGFMaU1jY2FtbW9uLnBkZgAAAAAAAAAAAAA
	AAAAAAAAAAAAAAAAAAAAAAAAAAAAAABlinMP9I7BQREYgcHJ2dwAEAAQAAAkgAAAAAAAAAAAAAA
	AAAAAAB0FyY2hpdmUAABAACAAAw+NSrQAAABEACAAAw/1qAAAAAAEAFAAZYksAGWIDAAqkKAAKp
	BEAAHrcAAIAVU1hY2ludG9zaCBIRDpVc2VyczpiYWtlcjpEb2N1bWVudHM6UmVmZXJlbmNlczpB
	cmNoaXZlOjIwMDgtQ2hlRHp1YmllbGxhTGlNY2NhbW1vbi5wZGYAAA4AQAAfADIAMAAwADgALQB
	DAGgAZQBEAHoAdQBiAGkAZQBsAGwAYQBMAGkATQBjAGMAYQBtAG0AbwBuAC4AcABkAGYADwAaAA
	wATQBhAGMAaQBuAHQAbwBzAGgAIABIAEQAEgBIVXNlcnMvYmFrZXIvRG9jdW1lbnRzL1JlZmVyZ
	W5jZXMvQXJjaGl2ZS8yMDA4LUNoZUR6dWJpZWxsYUxpTWNjYW1tb24ucGRmABMAAS8AABUAAgAM
	//8AANIeHyAhWCRjbGFzc2VzWiRjbGFzc25hbWWjISIjXU5TTXV0YWJsZURhdGFWTlNEYXRhWE5
	TT2JqZWN0XxBILi4vLi4vLi4vLi4vRG9jdW1lbnRzL1JlZmVyZW5jZXMvQXJjaGl2ZS8yMDA4LU
	NoZUR6dWJpZWxsYUxpTWNjYW1tb24ucGRm0h4fJieiJyNcTlNEaWN0aW9uYXJ5AAgAEQAaAB8AK
	QAyADcAOgA/AEEAUwBcAGIAaQBwAHgAgwCFAIgAigCMAI8AkQCTAJ0AqgCvALcAuQKnAqwCtQLA
	AsQC0gLZAuIDLQMyAzUAAAAAAAACAQAAAAAAAAAoAAAAAAAAAAAAAAAAAAADQg==},
  bdsk-url-1 = {http://dx.doi.org/10.1021/jp7101012},
  bdsk-url-2 = {http://dx.doi.org/10.1021/jp7101012},
  date-added = {2008-06-28 10:51:15 -0500},
  date-modified = {2008-06-28 10:51:15 -0500},
  doi = {10.1021/jp7101012},
  keywords = {electrostatics, solvation, statistical\_mechanics},
  priority = {0},
  url = {http://dx.doi.org/10.1021/jp7101012}
}

@ARTICLE{CChen:2009,
  author = {Chen, C. J. and Saxena, Rishu and Wei, G. W.},
  title = {Differential geometry based multiscale models for virus formation
	and evolution},
  journal = {Int. J. Biomed. Imaging},
  year = {2010},
  volume = {2010},
  pages = {308627}
}

@ARTICLE{CMChen:2007,
  author = {Chen, C. M.and Liu, F. and Turner, I. and Anh, V.},
  title = {A Fourier method for the fractional diffusion equation describing
	sub-diffusion},
  journal = {Journal of Computational Physics },
  year = {2007},
  volume = {227},
  pages = {886 -897}
}

@ARTICLE{DuanChen:2011a,
  author = {Chen, Duan and Chen, Zhan and Chen, Changjun and Geng, W. H. and
	Wei, G. W.},
  title = {{MIBPB}: A software package for electrostatic analysis },
  journal = {J. Comput. Chem.},
  year = {2011},
  volume = {32},
  pages = {657 - 670}
}

@ARTICLE{DuanChen:2012a,
  author = {Chen, Duan and Chen, Zhan and Wei, G. W.},
  title = {Quantum dynamics in continuum for proton transport {II: Variational}
	solvent-solute interface},
  journal = {International Journal for Numerical Methods in Biomedical Engineering},
  year = { 2012},
  volume = {28},
  pages = {25 - 51 }
}

@ARTICLE{DuanChen:2012b,
  author = {Chen, Duan and Wei, G. W.},
  title = {Quantum dynamics in continuum for proton transport---{Generalized}	correlation},
  journal = {J Chem. Phys.},
  volume = {136},
  pages = {134109},
  year = {2012}
}
@ARTICLE{EisenbergR:1993,
  author = {Chen, D. and Eisenberg, B. S.},
  title = {Charges, currents, and potentials in ionic channels of one conformation},
  journal = {Biophys J.},
  year = {1993},
  volume = {64},
  pages = {1405 - 1421},
  number = {5}
}

@ARTICLE{Chen:1997,
  author = {Chen, Duan and Lear, James and Eisenberg, B. S.},
  title = {Permeation through an open channel: {Poisson-Nernst-Planck} theory
	of a synthetic ionic channel.},
  journal = {Biophys J.},
  year = {1997},
  volume = {72},
  pages = {97-116},
  number = {1}
}

@ARTICLE{DuanChen:2013,
  author = {Chen, Duan and Wei, G. W.},
  title = {Quantum dynamics in continuum for proton transport {I: Basic} formulation
	},
  journal = {Commun. Comput. Phys.},
  volume = {13},
  year = { 2013},
  pages = {285-324 }
}


@ARTICLE{DuanChen:2010,
  author = {Chen, D. and Wei, G. W.},
  title = {Modeling and simulation of electronic structure, material interface
	and random doping in nano-electronic devices},
  journal = {J. Comput. Phys.},
  year = {2010},
  volume = {229},
  pages = { 4431-4460}
}

@ARTICLE{DuanChen:2010c,
  author = {Chen, Duan and Wei, G. W.},
  title = {Multi-scale Modeling and Simulation for Proton Trans-location in
	the Ion Channel, in {Workshop on Fluid Motion Driven by Immersed
	Structures, Fields Institute, Toronto} },
  year = {2010},
  pages = { },
  month = {August 9-13}
}

@ARTICLE{Chen:2008,
  author = {Chen, D. and Wei, G. W. and Cong, X. and Wang, G.},
  title = {Computational methods for optical molecular imaging},
  journal = {Communications in Numerical Methods in Engineering},
  year = {2009},
  volume = {25},
  pages = {1137-1161},
  date-added = {2008-06-30 22:16:14 -0400},
  date-modified = {2008-06-30 22:16:39 -0400}
}

@ARTICLE{DPChen:1995,
  author = {Chen, D. P. and Eisenberg, R. S. and Jerome, J. W. and Shu, C. W.},
  title = {Hydrodynamic model of temperature change in open ionic channels},
  journal = {Biophys. J.},
  year = {1995},
  volume = {69},
  pages = {2304 - 2322}
}

@BOOK{chenGQ:2005,
  title = {Nonlinear partial differential equations and related analysis},
  publisher = {the American Mathematical Society},
  year = {2005},
  author = {Chen, G. -Q. and Gasper, G. and Jerome, J. W. }
}

@ARTICLE{HNChen:2007,
  author = {Chen, H. N. and Wu, Y. J. and Voth, G. A.},
  title = {Proton transport Behavior through the {influenza A} {M2} channel:
	Insights from molecular simulation},
  journal = {Biophys J.},
  year = {2007},
  volume = {93},
  pages = {3470-3479},
  number = { }
}

@ARTICLE{Chen:2008d,
  author = {Chen, J. and Brooks III, C. L.},
  title = {Implicit modeling of nonpolar solvation for simulating protein folding
	and conformational transitions},
  journal = {Physical Chemistry Chemical Physics},
  year = {2008},
  volume = {10},
  pages = {471-81},
  abstract = {Accurate description of the solvent environment is critical in computer
	simulations of protein structure and dynamics. An implicit treatment
	of solvent aims to capture the mean influence of water molecules
	on the solute via direct estimation of the solvation free energy.
	It has emerged as a powerful alternative to explicit solvent, and
	provides a favorable compromise between computational cost and level
	of detail. We review the current theory and techniques for implicit
	modeling of nonpolar solvation in the context of simulating protein
	folding and conformational transitions, and discuss the main directions
	for further development. It is demonstrated that the current surface
	area based nonpolar models have severe limitations, including insufficient
	description of the conformational dependence of solvation, over-estimation
	of the strength of pair-wise nonpolar interactions, and incorrect
	prediction of anti-cooperativity for three-body hydrophobic associations.
	We argue that, to improve beyond current level of accuracy of implicit
	solvent models, two important aspects of nonpolar solvation need
	to be incorporated, namely, the length-scale dependence of hydrophobic
	association and solvent screening of solute--solute dispersion interactions.
	We recognize that substantial challenges exist in constructing a
	sufficiently balanced, yet reasonably efficient, implicit solvent
	protein force field. Nonetheless, most of the fundamental problems
	are understood, and exciting progress has been made over the last
	few years. We believe that continual work along the frontiers outlined
	will greatly improve ones ability to study protein folding and large
	conformational transitions at atomistic detail.},
  bdsk-url-1 = {http://www.rsc.org/publishing/journals/CP/article.asp?doi=b714141f},
  date-added = {2008-06-28 10:53:30 -0500},
  date-modified = {2008-06-28 10:53:30 -0500},
  keywords = {nonpolar, solvation},
  priority = {0},
  url = {http://www.rsc.org/publishing/journals/CP/article.asp?doi=b714141f}
}

@ARTICLE{Chen:2007,
  author = {Chen, J. and Brooks, C. L. 3rd.},
  title = {{Can molecular dynamics simulations provide high-resolution refinement
	of protein structure?}},
  journal = {Proteins},
  year = {2007},
  volume = {67},
  pages = {922-930},
  number = {4}
}

@ARTICLE{Bashford:1994,
  author = {Chen, J.L. and Noodleman, L. and Case, D.A. and Bashford, D.},
  title = {Incorporating Solvation Effects into Density Functional Electronic
	Structure Calculations},
  journal = {J. Phys. Chem.},
  year = {1994},
  volume = {98},
  pages = {11059- 11068},
  abstract = {An improved approach to the calculation of molecular electronic structures,
	solvation energies, and pK, values in condensed phases is described.
	The electronic structure of the solute is described by density functional
	quantum mechanics, and electrostatic features of environmental effects
	are modeled through external charge distributions and continuum dielectrics.
	The reaction potential produced by atom-centered point-charge and
	dipole fits to the molecular charge distribution is computed via
	finite-difference solutions to the Poisson- Boltzmann equation. The
	coupling of the reaction potential into the molecular Hamiltonian
	is achieved through numerical integration, and the entire system
	is iterated to self-consistency. Sample calculations of solvation
	energies, solvated dipole moments, and absolute pK, values are provided
	for a variety of small organic molecules to illustrate applications
	of the method.}
}

@ARTICLE{LeiChen:2008,
  author = {Chen, Lei and Conlisk, A. T.},
  title = {Electroosmotic flow and particle transport in micro/nano nozzles
	and diffusers},
  journal = {Biomedical Microdevices},
  year = {2008},
  volume = {10},
  pages = {289 - 289}
}

@ARTICLE{Chen:2007f,
  author = {Chen, Long and Holst, Michael J. and Xu, Jinchao},
  title = {The Finite Element Approximation of the Nonlinear Poisson--Boltzmann
	Equation},
  journal = {SIAM Journal on Numerical Analysis},
  year = {2007},
  volume = {45},
  pages = {2298--2320},
  number = {6},
  abstract = {A widely used electrostatics model in the biomolecular modeling community,
	the nonlinear Poisson\&ndash;Boltzmann equation, along with its finite
	element approximation, are analyzed in this paper. A regularized
	Poisson\&ndash;Boltzmann equation is introduced as an auxiliary problem,
	making it possible to study the original nonlinear equation with
	delta distribution sources. A priori error estimates for the finite
	element approximation are obtained for the regularized Poisson\&ndash;Boltzmann
	equation based on certain quasi-uniform grids in two and three dimensions.
	Adaptive finite element approximation through local refinement driven
	by an a posteriori error estimate is shown to converge. The Poisson\&ndash;Boltzmann
	equation does not appear to have been previously studied in detail
	theoretically, and it is hoped that this paper will help provide
	molecular modelers with a better foundation for their analytical
	and computational work with the Poisson\&ndash;Boltzmann equation.
	Note that this article apparently gives the first rigorous convergence
	result for a numerical discretization technique for the nonlinear
	Poisson\&ndash;Boltzmann equation with delta distribution sources,
	and it also introduces the first provably convergent adaptive method
	for the equation. This last result is currently one of only a handful
	of existing convergence results of this type for nonlinear problems.},
  bdsk-file-1 = {YnBsaXN0MDDUAQIDBAUGCQpYJHZlcnNpb25UJHRvcFkkYXJjaGl2ZXJYJG9iamVjdHMSAAGGoNE
	HCFRyb290gAFfEA9OU0tleWVkQXJjaGl2ZXKoCwwXGBkdJCVVJG51bGzTDQ4PEBEUViRjbGFzc1
	dOUy5rZXlzWk5TLm9iamVjdHOAB6ISE4ACgAOiFRaABIAGWWFsaWFzRGF0YVxyZWxhdGl2ZVBhd
	GjSDRobHFdOUy5kYXRhgAVPEQG+AAAAAAG+AAIAAAxNYWNpbnRvc2ggSEQAAAAAAAAAAAAAAAAA
	AADD4v5NSCsAAAAZYksUMjAwNy1DaGVuSG9sc3RYdS5wZGYAAAAAAAAAAAAAAAAAAAAAAAAAAAA
	AAAAAAAAAAAAAAAAAAAAAAAAAAAAAABlissNZp+UAAAAAAAAAAAAEAAQAAAkgAAAAAAAAAAAAAA
	AAAAAAB0FyY2hpdmUAABAACAAAw+NSrQAAABEACAAAw1n8RQAAAAEAFAAZYksAGWIDAAqkKAAKp
	BEAAHrcAAIASk1hY2ludG9zaCBIRDpVc2VyczpiYWtlcjpEb2N1bWVudHM6UmVmZXJlbmNlczpB
	cmNoaXZlOjIwMDctQ2hlbkhvbHN0WHUucGRmAA4AKgAUADIAMAAwADcALQBDAGgAZQBuAEgAbwB
	sAHMAdABYAHUALgBwAGQAZgAPABoADABNAGEAYwBpAG4AdABvAHMAaAAgAEgARAASAD1Vc2Vycy
	9iYWtlci9Eb2N1bWVudHMvUmVmZXJlbmNlcy9BcmNoaXZlLzIwMDctQ2hlbkhvbHN0WHUucGRmA
	AATAAEvAAAVAAIADP//AADSHh8gIVgkY2xhc3Nlc1okY2xhc3NuYW1loyEiI11OU011dGFibGVE
	YXRhVk5TRGF0YVhOU09iamVjdF8QPS4uLy4uLy4uLy4uL0RvY3VtZW50cy9SZWZlcmVuY2VzL0F
	yY2hpdmUvMjAwNy1DaGVuSG9sc3RYdS5wZGbSHh8mJ6InI1xOU0RpY3Rpb25hcnkACAARABoAHw
	ApADIANwA6AD8AQQBTAFwAYgBpAHAAeACDAIUAiACKAIwAjwCRAJMAnQCqAK8AtwC5AnsCgAKJA
	pQCmAKmAq0CtgL2AvsC/gAAAAAAAAIBAAAAAAAAACgAAAAAAAAAAAAAAAAAAAML},
  bdsk-url-1 = {http://link.aip.org/link/?SNA/45/2298},
  date-added = {2008-09-17 09:05:38 -0500},
  date-modified = {2008-09-17 09:05:38 -0500},
  keywords = {Electrostatics, Mathematics, Solvation},
  priority = {0},
  publisher = {SIAM},
  url = {http://link.aip.org/link/?SNA/45/2298}
}

@ARTICLE{TChen:2008,
  author = {Chen, T. and Strain, J.},
  title = {Piecewise-polynomial discretization and {Krylov-accelerated} multigrid
	for elliptic interface problems},
  journal = {J. Comput. Phys.},
  year = {2008},
  volume = {16},
  pages = {7503-7542}
}

@INPROCEEDINGS{chen-medioni:91,
  author = {Chen, Y. and Medioni, G.},
  title = {Object Modeling by Registration of Multiple Range Images},
  booktitle = {IEEE Conference on Robotics and Automation},
  year = {1991},
  volume = {3},
  pages = {2724--2729}
}

@ARTICLE{Chen:2006a,
  author = {Chen, Y. -G. and Weeks, J. D.},
  title = {Local molecular field theory for effective attractions between like
	charged objects in systems with strong {Coulomb} interactions},
  journal = {Proceedings of the National Academy of Sciences of the United States
	of America},
  year = {2006},
  volume = {103},
  pages = {7560-5},
  number = {20},
  abstract = {Strong, short-ranged positional correlations involving counterions
	can induce a net attractive force between negatively charged strands
	of DNA and lead to the formation of ion pairs in dilute ionic solutions.
	However, the long range of the Coulomb interactions impedes the development
	of a simple local picture. We address this general problem by mapping
	the properties of a nonuniform system with Coulomb interactions onto
	those of a simpler system with short-ranged intermolecular interactions
	in an effective external field that accounts for the averaged effects
	of appropriately chosen long-ranged and slowly varying components
	of the Coulomb interactions. The remaining short-ranged components
	combine with the other molecular core interactions and strongly affect
	pair correlations in dense or strongly coupled systems. We show that
	pair correlation functions in the effective short-ranged system closely
	resemble those in the uniform primitive model of ionic solutions
	and illustrate the formation of ion pairs and clusters at low densities.
	The theory accurately describes detailed features of the effective
	attraction between two equally charged walls at strong coupling and
	intermediate separations of the walls. Analytical results for the
	minimal coupling strength needed to get any attraction and for the
	separation at which the attractive force is a maximum are presented.},
  annote = {Local molecular field theory for effective attractions between like
	charged objects in systems with strong Coulomb interactions},
  bdsk-url-1 = {http://dx.doi.org/10.1073/pnas.0600282103},
  date-added = {2008-09-01 14:06:13 -0500},
  date-modified = {2008-09-01 14:06:13 -0500},
  keywords = {Electrostatics; StatisticalMechanics; Solvation; BeyondMeanField},
  ty = {JOUR},
  url = {http://dx.doi.org/10.1073/pnas.0600282103}
}



@ARTICLE{ZhanChen:2010b,
  author = {Chen, Z. and Baker, N. A. and Wei, G. W. },
  title = {Differential geometry based solvation models {II}: Lagrangian formulation},
  journal = {J. Math. Biol.},
  year = {2011},
  volume = {63},
  pages = {1139- 1200}
}

@ARTICLE{ZhanChen:2010a,
  author = {Chen, Z. and Baker, N. A. and Wei, G. W. },
  title = {Differential geometry based solvation models {I}: Eulerian formulation},
  journal = {J. Comput. Phys.},
  year = {2010},
  volume = {229},
  pages = {8231-8258}
}

@ARTICLE{ZhanChen:2012,
  author = {Chen, Z. and Zhao, Shan and  Chun, J.  and Thomas, D. G. and  Baker, N. A. and
Bates, P. B.  and Wei, G. W. },
  title = {Variational approach for nonpolar solvation analysis},
  journal = {Journal of Chemical Physics},
  year = {2012},
  Volume ={137},
  number ={084101}
}

@ARTICLE{ZhanChen:2011a,
  author = {Chen, Z. and Wei, G. W. },
  title = {Differential geometry based solvation models {III}: Quantum formulation},
  journal = {J. Chem. Phys.},
  year = {2011},
  volume = {135},
  pages = {194108}
}

@ARTICLE{Cheng:2007e,
  author = {Cheng, L. T. and Dzubiella, Joachim and McCammon, Andrew J. and Li,
	B.},
  title = {Application of the level-set method to the implicit solvation of
	nonpolar molecules},
  journal = {Journal of Chemical Physics},
  year = {2007},
  volume = {127},
  number = {8},
  abstract = {A level-set method is developed for numerically capturing the equilibrium
	solute-solvent interface that is defined by the recently proposed
	variational implicit solvent model [Dzubiella, Swanson, and McCammon,
	Phys. Rev. Lett. 104, 527 (2006); J. Chem. Phys. 124, 084905 (2006)].
	In the level-set method, a possible solute-solvent interface is represented
	by the zero level set (i.e., the zero level surface) of a level-set
	function and is eventually evolved into the equilibrium solute-solvent
	interface. The evolution law is determined by minimization of a solvation
	free energy functional that couples both the interfacial energy and
	the {van der waals} type solute-solvent interaction energy. The surface
	evolution is thus an energy minimizing process, and the equilibrium
	solute-solvent interface is an output of this process. The method
	is implemented and applied to the solvation of nonpolar molecules
	such as two xenon atoms, two parallel paraffin plates, helical alkane
	chains, and a single fullerence C60. The level-set solutions show
	good agreement for the solvation energies when compared to available
	molecular dynamics simulations. In particular, the method captures
	solvent dewetting (nanobubble formation) and quantitatively describes
	the interaction in the strongly hydrophobic plate system.
	
	 \&copy;2007 American Institute of Physics},
  bdsk-url-1 = {http://dx.doi.org/10.1063/1.2757169},
  bdsk-url-2 = {http://dx.doi.org/10.1063/1.2757169},
  date-added = {2008-06-28 10:54:54 -0500},
  date-modified = {2008-06-28 10:54:54 -0500},
  doi = {10.1063/1.2757169},
  keywords = {mathematics; solvation},
  priority = {0},
  publisher = {AIP},
  url = {http://dx.doi.org/10.1063/1.2757169}
}

@ARTICLE{Cheng2:2009,
  author = { Cheng, Li-Tien and Xie, Yang and Dzubiella, Joachim and McCammon,
	J. Andrew and Che, Jianwei and Li, Bo },
  title = {{Coupling the level-set method with molecular mechanics for variational
	implicit solvation of nonpolar molecules}},
  journal = {J. Chem. Theory Comput.},
  year = {2009},
  volume = {5},
  pages = {257-266}
}

@ARTICLE{Cheng:2005,
  author = {Cheng, M. H. and Coalson, R. D. },
  title = {{An accurate and efficient empirical approach for calculating the
	dielectric self-energy and ion-ion pair potential in continuum models
	of biological ion channels}},
  journal = {J Phys Chem B},
  year = {2005},
  volume = {109(1)},
  pages = {488-98}
}

@ARTICLE{Cheng:2010,
  author = {Cheng, M. H. and Coalson, R. D. and Tang, P.},
  title = {{Molecular dynamics and brownian dynamics investigation of ion permeation
	and anesthetic halothane effects on a proton-gated ion channel}},
  journal = {J Am Chem Soc},
  year = {2010},
  volume = {132(46)},
  pages = {16442-9}
}

@ARTICLE{Cheng:2009,
  author = {Cheng, X. L. and Ivanov, I. and Wang, H. L. and Sine, S. M. and McCammon,
	J. A.},
  title = {Molecular Dynamics Simulations of a Prokaryotic Homologue of the
	Nicotinic Acetylcholine Receptor},
  journal = { Biophysical Journal},
  year = {2009},
  volume = {96},
  pages = {4502-4513 }
}

@ARTICLE{YCheng:2009,
  author = {Cheng, Y. and Gamba, I. M. and Majorana, A. and Shu, Chi-Wang},
  title = {A discontinuous Galerkin solver for Boltzmann?Poisson systems in
	nano devices},
  journal = {Computer Methods in Applied Mechanics and Engineering},
  year = {2009},
  volume = {198},
  pages = {3130-3150}
}

@ARTICLE{Cheng:2007,
  author = {Cheng, Y. and Suen, J. K. and RadiÄ- Z. and Bond, S. D. and Holst,
	M. J. and McCammon, J. A.},
  title = {Continuum simulations of acetylcholine diffusion with reaction-determined
	boundaries in neuromuscular junction models},
  journal = {Biophysical Chemistry},
  year = {2007},
  volume = {127},
  pages = {129-39},
  number = {3},
  abstract = {The reaction-diffusion system of the neuromuscular junction has been
	modeled in 3D using the finite element package FEtk. The numerical
	solution of the dynamics of acetylcholine with the detailed reaction
	processes of acetylcholinesterases and nicotinic acetylcholine receptors
	has been discussed with the reaction-determined boundary conditions.
	The simulation results describe the detailed acetylcholine hydrolysis
	process, and reveal the time-dependent interconversion of the closed
	and open states of the acetylcholine receptors as well as the percentages
	of unliganded/monoliganded/diliganded states during the neuro-transmission.
	The finite element method has demonstrated its flexibility and robustness
	in modeling large biological systems.},
  bdsk-url-1 = {http://dx.doi.org/10.1016/j.bpc.2007.01.003},
  date-added = {2008-09-03 13:30:19 -0500},
  date-modified = {2008-09-03 13:30:19 -0500},
  keywords = {Diffusion; NeuromuscularJunctions},
  read = {Yes},
  url = {http://dx.doi.org/10.1016/j.bpc.2007.01.003}
}

@ARTICLE{Cheng:2007a,
  author = {Cheng, Y. and Suen, J. K. and Zhang, D. and Bond, S. D. and Zhang,
	Y. and Song, Y. and Baker, N. A. and Bajaj, C. L. and Holst, M. J.
	and McCammon, J. A.},
  title = {Finite Element Analysis of the Time-Dependent {Smoluchowski} Equation
	for Acetylcholinesterase Reaction Rate Calculations},
  journal = {Biophysical Journal},
  year = {2007},
  volume = {92},
  pages = {3397-406},
  number = {10},
  abstract = {This article describes the numerical solution of the time-dependent
	Smoluchowski equation to study diffusion in biomolecular systems.
	Specifically, finite element methods have been developed to calculate
	ligand binding rate constants for large biomolecules. The resulting
	software has been validated and applied to the mouse acetylcholinesterase
	(mAChE) monomer and several tetramers. Rates for inhibitor binding
	to mAChE were calculated at various ionic strengths with several
	different time steps. Calculated rates show very good agreement with
	experimental and theoretical steady-state studies. Furthermore, these
	finite element methods require significantly fewer computational
	resources than existing particle-based Brownian dynamics methods
	and are robust for complicated geometries. The key finding of biological
	importance is that the rate accelerations of the monomeric and tetrameric
	mAChE that result from electrostatic steering are preserved under
	the non-steady-state conditions that are expected to occur in physiological
	circumstances.},
  bdsk-file-1 = {YnBsaXN0MDDUAQIDBAUGCQpYJHZlcnNpb25UJHRvcFkkYXJjaGl2ZXJYJG9iamVjdHMSAAGGoNE
	HCFRyb290gAFfEA9OU0tleWVkQXJjaGl2ZXKoCwwXGBkdJCVVJG51bGzTDQ4PEBEUViRjbGFzc1
	dOUy5rZXlzWk5TLm9iamVjdHOAB6ISE4ACgAOiFRaABIAGWWFsaWFzRGF0YVxyZWxhdGl2ZVBhd
	GjSDRobHFdOUy5kYXRhgAVPEQI+AAAAAAI+AAIAAAxNYWNpbnRvc2ggSEQAAAAAAAAAAAAAAAAA
	AADD4v5NSCsAAAAZYksfMjAwNy1DaGVuZ1N1ZW5aaGFuZ0IjMTk2MjY4LnBkZgAAAAAAAAAAAAA
	AAAAAAAAAAAAAAAAAAAAAAAAAAAAAABliaMM6CU5QREYgcHJ2dwAEAAQAAAkgAAAAAAAAAAAAAA
	AAAAAAB0FyY2hpdmUAABAACAAAw+NSrQAAABEACAAAwzpPngAAAAEAFAAZYksAGWIDAAqkKAAKp
	BEAAHrcAAIAVU1hY2ludG9zaCBIRDpVc2VyczpiYWtlcjpEb2N1bWVudHM6UmVmZXJlbmNlczpB
	cmNoaXZlOjIwMDctQ2hlbmdTdWVuWmhhbmdCIzE5NjI2OC5wZGYAAA4AeAA7ADIAMAAwADcALQB
	DAGgAZQBuAGcAUwB1AGUAbgBaAGgAYQBuAGcAQgBvAG4AZABaAGgAYQBuAGcAUwBvAG4AZwBCAG
	EAawBlAHIAQgBhAGoAYQBqAEgAbwBsAHMAdABNAGMAQwBhAG0AbQBvAG4ALgBwAGQAZgAPABoAD
	ABNAGEAYwBpAG4AdABvAHMAaAAgAEgARAASAGRVc2Vycy9iYWtlci9Eb2N1bWVudHMvUmVmZXJl
	bmNlcy9BcmNoaXZlLzIwMDctQ2hlbmdTdWVuWmhhbmdCb25kWmhhbmdTb25nQmFrZXJCYWphakh
	vbHN0TWNDYW1tb24ucGRmABMAAS8AABUAAgAM//8AANIeHyAhWCRjbGFzc2VzWiRjbGFzc25hbW
	WjISIjXU5TTXV0YWJsZURhdGFWTlNEYXRhWE5TT2JqZWN0XxBkLi4vLi4vLi4vLi4vRG9jdW1lb
	nRzL1JlZmVyZW5jZXMvQXJjaGl2ZS8yMDA3LUNoZW5nU3VlblpoYW5nQm9uZFpoYW5nU29uZ0Jh
	a2VyQmFqYWpIb2xzdE1jQ2FtbW9uLnBkZtIeHyYnoicjXE5TRGljdGlvbmFyeQAIABEAGgAfACk
	AMgA3ADoAPwBBAFMAXABiAGkAcAB4AIMAhQCIAIoAjACPAJEAkwCdAKoArwC3ALkC+wMAAwkDFA
	MYAyYDLQM2A50DogOlAAAAAAAAAgEAAAAAAAAAKAAAAAAAAAAAAAAAAAAAA7I=},
  bdsk-url-1 = {http://dx.doi.org/10.1529/biophysj.106.102533},
  date-added = {2008-09-03 13:30:19 -0500},
  date-modified = {2008-09-03 13:30:19 -0500},
  keywords = {Diffusion; Acetylcholinesterase},
  url = {http://dx.doi.org/10.1529/biophysj.106.102533}
}

@ARTICLE{YDCheng:2009,
  author = {Cheng, Y. D. and Gamba, I. M. and Majorana, A. and Shu, C. W.},
  title = {A discontinuous Galerkin solver for {Boltzmann-Poisson} systems in
	nano devices},
  journal = {Comput. Methods Appl. Mech. Engrg.},
  year = {2009},
  volume = {198},
  pages = {3130-3150}
}

@ARTICLE{Chern:2007,
  author = {Chern, I. and Shu, Y. C.},
  title = {A coupling interface method for elliptic interface problems},
  journal = {J. Comput. Phys.},
  year = {2007},
  volume = {225},
  pages = {2138 - 2174}
}

@ARTICLE{Chern:2003,
  author = {Chern, I. -L. and Liu, J.-G. and Weng, W.-C.},
  title = {Accurate Evaluation of Electrostatics for Macromolecules in Solution},
  journal = {Methods and Applications of Analysis},
  year = {2003},
  volume = {10},
  pages = {309-28},
  number = {2},
  bdsk-url-1 = {http://www.intlpress.com/MAA/p/2003/10_2/MAA-10-2-309-328.pdf},
  date-added = {2008-06-30 21:42:46 -0400},
  date-modified = {2008-06-30 21:44:20 -0400},
  url = {http://www.intlpress.com/MAA/p/2003/10_2/MAA-10-2-309-328.pdf}
}

@ARTICLE{Cukierman:2006,
  author = {Chernyshev, Anatoly and Cukierman, Samuel},
  title = {Proton Transfer in { Gramicidin} Water Wires in Phosphlipid Bilayers:
	Attenuation by Phosphoethanolamine},
  journal = {Biophys J.},
  year = {1997},
  volume = {91},
  pages = {580-587},
  number = { }
}

@ARTICLE{Chiba:2008,
  author = {Mahito Chiba and Dmitri G. Fedorov and Kazuo Kitaura},
  title = {Polarizable continuum model with the fragment molecular orbital-based
	time-dependent density functional theory},
  journal = {Journal of Computational Chemistry},
  year = {2008},
  volume = {29},
  pages = {2667--2676}
}

@ARTICLE{Chirlian:1987,
  author = {Chirlian, L. E. and Francl, M. M.},
  title = { Atomic charges derived from electrostatic potentials: A detailed
	study.},
  journal = {J. Comput. Chem.},
  year = {1987},
  volume = {8},
  pages = {894-905}
}

@ARTICLE{Chopp:1993,
  author = {Chopp, David L. },
  title = {Computing Minimal Surfaces via Level Set Curvature Flow},
  journal = {J. Comput. Phys.},
  year = {1993},
  volume = {106},
  pages = {77--91},
  number = {1},
  bdsk-url-1 = {http://www.sciencedirect.com/science/article/B6WHY-45P1273-4J/2/588cc6c35517b35e0158b9218e8b9bda},
  date-added = {2008-09-16 14:39:43 -0500},
  date-modified = {2008-09-16 14:39:43 -0500},
  doi = {10.1006/jcph.1993.1092 },
  keywords = {Mathematics},
  ty = {JOUR},
  url = {http://www.sciencedirect.com/science/article/B6WHY-45P1273-4J/2/588cc6c35517b35e0158b9218e8b9bda}
}

@ARTICLE{Chorny:2005,
  author = {Chorny, I. and Dill, K. A. and Jacobson, M. P.},
  title = {Surfaces Affect Ion Pairing},
  journal = {Journal of Physical Chemistry B},
  year = {2005},
  volume = {109},
  pages = {24056-60},
  number = {50},
  abstract = {In water, positive ions attract negative ions. That attraction can
	be modulated if a hydrophobic surface is present near the two ions
	in water. Using computer simulations with explicit and implicit water,
	we study how an ion embedded on a hydrophobic surface interacts with
	another nearby ion in water. Using hydrophobic surfaces with different
	curvatures, we find that the contact interaction between a positive
	and negative ion is strongly affected by the curvature of an adjacent
	surface, either stabilizing or destabilizing the ion pair. We also
	find that the solvent-separated ion pair (SSIP) can be made more
	stable than the contacting ion pair by the presence of a surface.
	This may account for why bridging waters are often found in protein
	crystal structures. We also note that implicit solvent models do
	not account for SSIPs. Finally, we find that there are charge asymmetries:
	an embedded positive charge attracting a negative ion is different
	than an embedded negative charge attracting a positive ion. Such
	asymmetries are also not predicted by implicit solvent models. These
	results may be useful for improving computational models of solvation
	in biology and chemistry.},
  annote = {Surfaces Affect Ion Pairing; Failure of {Poisson-Boltzmann} to predict
	solvent-separated ion pairs and to include the effects of nearby
	surfaces.},
  bdsk-url-1 = {http://dx.doi.org/10.1021/jp055043m},
  date-added = {2008-06-28 10:57:04 -0500},
  date-modified = {2008-06-28 10:57:04 -0500},
  keywords = {Solvation; Electrostatics},
  ty = {JOUR},
  url = {http://dx.doi.org/10.1021/jp055043m}
}

@ARTICLE{Chou:2009,
  author = {Chou, T. },
  title = {Enhancement of charged macromolecule capture by nanopores in a salt
	gradient},
  journal = {J. Chem. Phys.},
  year = {2009},
  volume = {131},
  number = {034703 }
}

@ARTICLE{Choudhary:2010,
  author = {Choudhary, O. P. and Ujwal, R. and Kowallis, W. and Coalson, R. and
	Abramson, J. and Grabe, M.},
  title = {{The electrostatics of VDAC: implications for selectivity and gating}},
  journal = {J Mol Biol},
  year = {2010},
  volume = {396(3)},
  pages = {580-92}
}

@ARTICLE{ChYaZh09,
  author = {Chow, S.N. and Yang, T. S. and Zhou, H. M.},
  title = {Global Optimizations by Intermittent Diffusion},
  journal = {SIAM J. Optimization},
  year = {2010},
  number = { }
}

@ARTICLE{ChShZh07,
  author = {Chow, S. N. and Shen, W. X. and Zhou, H. M.},
  title = {Dynamical Order in Systems of Coupled Noisy Oscillators},
  journal = {J. of Dynamics and Differential Equations},
  year = {2007},
  volume = {19},
  pages = {1007-1036}
}

@ARTICLE{ChoZho07,
  author = {Chow, S. N. and Zhou, H. M.},
  title = {An Analysis of Phase Noise and {Fokker-Planck} Equations},
  journal = {J. of Differential Equations},
  year = {2007},
  volume = {234},
  pages = {391-411}
}

@ARTICLE{KTZhu:2006,
  author = {Chu, K. T. and Bazant, M. Z.},
  title = {Nonlinear electrochemical relaxation around conductors},
  journal = {Phys. Rev. E},
  year = {2006},
  volume = {74},
  number = {011501}
}

@ARTICLE{SMPBE,
  author = {Chu, Vincent B. and Bai, Y. and Lipfert, Jan and Herschlag, Daniel
	and Doniach, Sebastian},
  title = {Evaluation of Ion Binding to {DNA} Duplexes Using a Size-Modified
	{Poisson-Boltzmann} Theory},
  journal = {Biophysical Journal},
  year = {2007},
  volume = {93},
  pages = {3202--3209},
  number = {9}
}

@ARTICLE{chui2003npm,
  author = {Chui, H. and Rangarajan, A.},
  title = {{A new point matching algorithm for non-rigid registration}},
  journal = {Computer Vision and Image Understanding},
  year = {2003},
  volume = {89},
  pages = {114--141},
  number = {2-3},
  publisher = {Elsevier}
}

@BOOK{ChungOverview,
  title = {Spectral graph theory},
  publisher = {American Mathematical Society},
  year = {1997},
  author = {F. Chung}
}

@ARTICLE{Chung2:2002,
  author = {Chung, Shin-Ho and Allen, T. W. and Kuyucak, Serdar },
  title = {Conducting-state properties of the {KcsA} potassium channel from
	molecular and {Brownian} dynamics simulations },
  journal = {Biophysical Journal},
  year = {2002},
  volume = {82},
  pages = {628-645},
  month = { }
}

@ARTICLE{Chung:2002,
  author = {Chung, Shin-Ho and Kuyucak, Serdar },
  title = {Recent advances in ion channel research},
  journal = {Biochimica et Biophysica Acta},
  year = {2002},
  volume = {1565},
  pages = {267-286}
}

@ARTICLE{CG07,
  author = {Gregory Cipriano and Michael Gleicher},
  title = {Molecular Surface Abstraction},
  journal = {IEEE Transactions on Visualization and Computer Graphics},
  year = {2007},
  volume = {13},
  pages = {1608-1615},
  number = {6},
  address = {Los Alamitos, CA, USA},
  doi = {http://doi.ieeecomputersociety.org/10.1109/TVCG.2007.70578},
  issn = {1077-2626},
  owner = {Yiying},
  publisher = {IEEE Computer Society},
  timestamp = {2009.03.25}
}

@ARTICLE{Cisneros05114502,
  author = {Cisneros, G. A. and Liu, H. Y. and Lu, Z. Y. and Yang, W. T.},
  title = {Reaction path determination for quantum mechanical/molecular mechanical
	modeling of enzyme reactions by combining first order and second
	order "chain-of-replicas" methods},
  journal = {Journal of Chemical Physics},
  year = {2005},
  volume = {122},
  pages = {114502},
  number = {11},
  month = {Mar},
  abstract = {A two-step procedure for the determination of reaction paths in enzyme
	systems is presented. This procedure combines. two chain-of-states
	methods: a quantum mechanical/molecular mechanical (QM/MM) implementation
	of the nudged elastic band (NEB) method and a second order parallel
	path optimizer method both recently developed in our laboratory.
	In the first step, a reaction path determination is performed with
	the NEB method, along with a restrained minimization procedure for
	the MM environment to obtain a first approximation to the reaction
	path. In the second step; the calculated path is refined with the
	parallel path optimizer method. By combining these two methods the
	reaction paths are determined accurately, and in addition, the number
	of path optimization iterations are significantly reduced. This procedure
	is tested by calculating both steps of the isomerization of 2-oxo-4-hexenedioate
	I by 4-oxalocrotonate, tautomerase, which have been previously determined
	by our group. The calculated paths agree with the previously reported
	results and we obtain a reduction of 45%-55% in the number of path
	optimization cycles. (c) 2005 American Institute of Physics.},
  endnotereftype = {Journal Article},
  issn = {0021-9606},
  shorttitle = {Reaction path determination for quantum mechanical/molecular mechanical
	modeling of enzyme reactions by combining first order and second
	order "chain-of-replicas" methods},
  url = {<Go to ISI>://000228389900035}
}

@ARTICLE{Cisneros0310384,
  author = {Cisneros, G. A. and Liu, H. Y. and Zhang, Y. K. and Yang, W. T.},
  title = {Ab initio QM/MM study shows there is no general acid in the reaction
	catalyzed by 4-oxalocrotonate tautornerase},
  journal = {Journal of the American Chemical Society},
  year = {2003},
  volume = {125},
  pages = {10384-10393},
  number = {34},
  month = {Aug},
  abstract = {The mechanism for the reaction catalyzed by the 4-oxalocrotonate tautomerase
	(4-OT) enzyme has been studied using a quantum mechanical/molecular
	mechanical (QM/MM) method developed in our laboratory. Total free
	energy barriers were obtained for the two steps involved in this
	reaction. In the first step, Pro-1 acts as a general base to abstract
	a proton from the third carbon of the substrate, 2-oxo-4-hexenedioate,
	creating a negative charge on the oxygen at C-2 of this substrate.
	In the second step, the same hydrogen abstracted by the N-terminal
	Pro-1 is shuttled back to the fifth carbon of the substrate to form
	the product, 2-oxo-3-hexenedioate. The calculated total free energy
	barriers are 14.54 and 16.45 kcal/mol for the first and second steps,
	respectively. Our calculations clearly show that there is no general
	acid in the reaction. Arg-39", which is hydrogen bonded to the carboxylate
	group of the substrate, and an ordered water, which moves closer
	to the site of the charge formed in the transition state and intermediate,
	play the main role in transition state/intermediate stabilization
	without acting as general acids in the reaction.},
  endnotereftype = {Journal Article},
  issn = {0002-7863},
  shorttitle = {Ab initio QM/MM study shows there is no general acid in the reaction
	catalyzed by 4-oxalocrotonate tautornerase},
  url = {<Go to ISI>://000184919600046}
}

@ARTICLE{Cisneros06700,
  author = {Cisneros, G. A. and Wang, M. and Silinski, P. and Fitzgerald, M.
	C. and Yang, W. T.},
  title = {Theoretical and experimental determination on two substrates turned
	over by 4-oxalocrotonate tautomerase},
  journal = {Journal of Physical Chemistry A},
  year = {2006},
  volume = {110},
  pages = {700-708},
  number = {2},
  month = {Jan},
  abstract = {Quantum mechanical/molecular mechanical (QM/MM) calculations and experimental
	kinetic studies have been performed on 4-oxalocrotonate tautomerase
	(4OT) for two different substrates, 2-hydroxymuconate (2HM) and 2-oxo-4-hexenedioate
	(2o4hex). Potential (Delta E) and free energy (Delta G) paths for
	both steps of the reaction using both substrates were calculated
	to determine the free energy barriers and compared to the experimental
	values obtained from the kinetic studies via the transition state
	theory. In the first step, a proton from the hydroxyl oxygen on the
	second carbon of 2HM, or from the third carbon of 2o4hex, is abstracted
	by Pro-1. In the second step, the proton is transferred to the fifth
	carbon of the substrate to form the product, 2-oxo-3-hexenedioate
	(2o3hex). For both substrates we obtain a calculated Delta G of approximate
	to 13 kcal/mol, in agreement with experimental determinations. The
	calculated free energy barrier difference Delta G(2o4hex) -Delta
	G(2HM) (Delta Delta G) is 0.87 kcal/mol. We obtained an experimental
	AAG of 0.85 kcal/mol. These results suggest that 2HM is turned over
	faster than 2o4hex by 4OT. However, these energy differences are
	so small that both 2HM and 2o4hex need to be taken into account in
	considering the mechanism of catalysis of 4OT.},
  endnotereftype = {Journal Article},
  issn = {1089-5639},
  shorttitle = {Theoretical and experimental determination on two substrates turned
	over by 4-oxalocrotonate tautomerase},
  url = {<Go to ISI>://000234699000039}
}

@ARTICLE{Cisneros046885,
  author = {Cisneros, G. A. and Wang, M. and Silinski, P. and Fitzgerald, M.
	C. and Yang, W. T.},
  title = {The protein backbone makes important contributions to 4-oxalocrotonate
	tautomerase enzyme catalysis: Understanding from theory and experiment},
  journal = {Biochemistry},
  year = {2004},
  volume = {43},
  pages = {6885-6892},
  number = {22},
  month = {Jun},
  abstract = {The role of polypeptide backbone interactions in 4-oxalocrotonate
	tautomerase (4OT) catalysis has been investigated using a combination
	of site-directed mutagenesis experiments with unnatural amino acids
	and quantum mechanical/molecular mechanical (QM/MM) calculations
	of the 4OT reaction mechanism. Energy barriers for the wild-type
	enzyme (wt-4OT) and for a 4OT analogue containing a backbone amide
	to ester bond mutation between Ile-7 and Leu-8 [(OL8)4OT] were determined
	by both theory and experiment. The amide to ester bond mutation in
	(OL8)4OT effectively deleted a putative hydrogen bonding interaction
	between the enzyme's polypeptide backbone and its substrate. Recent
	theoretical calculations for the 4OT reaction mechanism suggested
	that this hydrogen bonding interaction helps properly position the
	substrate in the active site [Cisneros, G. A., et al. (2003) J. Am.
	Chem. Soc. 125, 10384-10393]. Our experimental results for (OL8)4OT
	reveal that the energy barrier for the (OL8)4OT-catalyzed reaction
	was increased 1.8 kcal/mol over that of the wild-type enzyme. This
	increase was in good agreement with the 1.0 kcal/mol increase obtained
	from QM/MM calculations for this analogue. Our theoretical calculations
	further suggest the hydrogen bond deletion in (OL8)4OT results in
	a rearrangement of the substrate in the active site. In this rearrangement,
	an ordered water molecule loses its ability to stabilize the transition
	state (TS), and Arg-61 gains the ability to stabilize the TS. The
	predicted role of Arg-61 in (OL8)4OT catalysis was confirmed in kinetic
	experiments with an analogue of (OL8)4OT containing an Arg to Ala
	mutation at position 61.},
  endnotereftype = {Journal Article},
  issn = {0006-2960},
  shorttitle = {The protein backbone makes important contributions to 4-oxalocrotonate
	tautomerase enzyme catalysis: Understanding from theory and experiment},
  url = {<Go to ISI>://000221807500006}
}

@ARTICLE{Param,
  author = {U. Clarenz and N. Litke and M. Rumpf},
  title = {{Axioms and Variational Problems in Surface Parameterization}},
  journal = {CAGD},
  year = {2004},
  volume = {21},
  pages = {727--749},
  number = {8}
}

@ARTICLE{Clarke:2006,
  author = {Clarke, N. },
  title = {{Free Modeling Assessment at CASP7, in{Assessment talk given at CASP7
	conference. Asilomar Conference Center, Pacific Grove, CA}}},
  year = {2006}
}

@ARTICLE{Coalson:2005,
  author = {Coalson, R. D. and Kurnikova, M. G. },
  title = {{Poisson-Nernst-Planck theory approach to the calculation of current
	through biological ion channels}},
  journal = {IEEE Trans Nanobioscience},
  year = {2005},
  volume = {4(1)},
  pages = {81-93}
}

@ARTICLE{Cohen09786,
  author = {Cohen, A. J. and Mori-Sanchez, P. and Yang, W. T.},
  title = {Second-Order Perturbation Theory with Fractional Charges and Fractional
	Spins},
  journal = {J. Chem. Theory Comput.},
  year = {2009},
  volume = {5},
  pages = {786-792},
  number = {4},
  endnotereftype = {Journal Article}
}

@ARTICLE{Mori-Sanchez09xxx,
  author = {Cohen, A. J. and Mori-Sanchez, P. and Yang, W. T.},
  title = {Failure of the random phase approximation correlation energy},
  journal = {J. Chem. Phys.},
  year = {2009},
  note = {submitted}
}

@ARTICLE{Cohen08115123,
  author = {Cohen, A. J. and Mori-Sanchez, P. and Yang, W. T.},
  title = {Fractional charge perspective on the band gap in density-functional
	theory},
  journal = {Physical Review B},
  year = {2008},
  volume = {77},
  pages = {115123},
  number = {11},
  month = {Mar},
  abstract = {The calculation of the band gap by density-functional theory (DFT)
	is examined by considering the behavior of the energy as a originates
	mainly from errors in describing systems with fractional charges.
	Formulas for the energy derivatives with respect to number of electrons
	are derived, which clarify the role of optimized effective potentials
	in prediction of the band gap. Calculations with a recent functional
	that has much improved behavior for fractional charges give a good
	prediction of the energy gap and also epsilon(HOMO)similar or equal
	to-I for finite systems. Our results indicate that it is possible,
	within DFT, to have a functional whose eigenvalues or derivatives
	accurately predict the band gap.},
  endnotereftype = {Journal Article},
  issn = {1098-0121},
  shorttitle = {Fractional charge perspective on the band gap in density-functional
	theory},
  url = {<Go to ISI>://000254542800062}
}

@ARTICLE{Cohen08121104,
  author = {Cohen, A. J. and Mori-Sanchez, P. and Yang, W. T.},
  title = {Fractional spins and static correlation error in density functional
	theory},
  journal = {Journal of Chemical Physics},
  year = {2008},
  volume = {129},
  pages = {121104},
  number = {12},
  month = {Sep},
  abstract = {Electronic states with fractional spins arise in systems with large
	static correlation (strongly correlated systems). Such fractional-spin
	states are shown to be ensembles of degenerate ground states with
	normal spins. It is proven here that the energy of the exact functional
	for fractional-spin states is a constant, equal to the energy of
	the comprising degenerate pure-spin states. Dramatic deviations from
	this exact constancy condition exist with all approximate functionals,
	leading to large static correlation errors for strongly correlated
	systems, such as chemical bond dissociation and band structure of
	Mott insulators. This is demonstrated with numerical calculations
	for several molecular systems. Approximating the constancy behavior
	for fractional spins should be a major aim in functional constructions
	and should open the frontier for density functional theory to describe
	strongly correlated systems. The key results are also shown to apply
	in reduced density-matrix functional theory. (C) 2008 American Institute
	of Physics.},
  endnotereftype = {Journal Article},
  issn = {0021-9606},
  shorttitle = {Fractional spins and static correlation error in density functional
	theory},
  url = {<Go to ISI>://000259884600004}
}

@ARTICLE{Cohen08792,
  author = {Cohen, A. J. and Mori-Sanchez, P. and Yang, W. T.},
  title = {Insights into current limitations of density functional theory},
  journal = {Science},
  year = {2008},
  volume = {321},
  pages = {792-794},
  number = {5890},
  month = {Aug},
  endnotereftype = {Journal Article},
  issn = {0036-8075},
  shorttitle = {Insights into current limitations of density functional theory},
  url = {<Go to ISI>://000258261000032}
}

@ARTICLE{Cohen07191109,
  author = {Cohen, A. J. and Mori-Sanchez, P. and Yang, W. T.},
  title = {Development of exchange-correlation functionals with minimal many-electron
	self-interaction error},
  journal = {Journal of Chemical Physics},
  year = {2007},
  volume = {126},
  pages = {191109},
  number = {19},
  month = {May},
  abstract = {New exchange-correlation functionals that address the important issue
	of many-electron self-interaction are developed. This is carried
	out by considering the performance of the functional on systems with
	fractional numbers of electrons at the same time as more standard
	thermochemical tests. The inclusion of Coulomb-attenuated exchange
	in the functional is facilitated by use of the adiabatic connection
	coupled with a short-range and long-range splittings. The new functionals
	have a good performance on thermochemistry and a much improved description
	of the total energy versus number of electrons and henceforth a much
	smaller many-electron self-interaction error. (C) 2007 American Institute
	of Physics.},
  endnotereftype = {Journal Article},
  issn = {0021-9606},
  shorttitle = {Development of exchange-correlation functionals with minimal many-electron
	self-interaction error},
  url = {<Go to ISI>://000246646600009}
}

@ARTICLE{Cohen0734101,
  author = {Cohen, A. J. and Mori-Sanchez, P. and Yang, W. T.},
  title = {Assessment and formal properties of exchange-correlation functionals
	constructed from the adiabatic connection},
  journal = {Journal of Chemical Physics},
  year = {2007},
  volume = {127},
  pages = {34101},
  number = {3},
  month = {Jul},
  abstract = {We examine the development and investigate the performance of exchange-correlation
	functionals constructed from the adiabatic connection. Our method
	is based on a direct modeling of the adiabatic connection curve in
	the coupling-constant space and is very flexible in the models. Several
	different models are investigated in the construction of new families
	of exchange-correlation functionals. Also the performance of two
	of these models (MCY1 and MCY2) is investigated over a wider range
	of systems and properties, with comparison made to the performance
	of established functionals. Overall, the adiabatic functionals improve
	upon widely used hybrid and generalized gradient approximation functionals,
	particularly in correctly describing one-electron systems and reaction
	energy barriers. (C) 2007 American Institute of Physics.},
  endnotereftype = {Journal Article},
  issn = {0021-9606},
  shorttitle = {Assessment and formal properties of exchange-correlation functionals
	constructed from the adiabatic connection},
  url = {<Go to ISI>://000248194300003}
}

@ARTICLE{Cohen0484,
  author = {Cohen, A. J. and Wu, Q. and Yang, W. T.},
  title = {Calculation of nuclear magnetic resonance shielding constants using
	potential-based methods},
  journal = {Chemical Physics Letters},
  year = {2004},
  volume = {399},
  pages = {84-88},
  number = {1-3},
  month = {Nov},
  abstract = {We present the calculation of nuclear magnetic resonance shielding
	constants using a range of different methods. In particular we examine
	two new methods proposed by Yang and Wu which are based on the Kohn-Sham
	potential. The first is a method which reproduces an accurate input
	density (WY) and the second is an implementation of the optimised
	effective potential method. We find that these methods give results
	which are very similar to each other and when the methods are applied
	to a hybrid functional (e.g. B3LYP) we obtain good agreement with
	experiment. (C) 2004 Elsevier B.V. All rights reserved.},
  endnotereftype = {Journal Article},
  issn = {0009-2614},
  shorttitle = {Calculation of nuclear magnetic resonance shielding constants using
	potential-based methods},
  url = {<Go to ISI>://000225324400015}
}

@ARTICLE{CAD04,
  author = {David Cohen-Steiner and Pierre Alliez and Mathieu Desbrun},
  title = {Variational Shape Approximation},
  journal = {ACM Trans. on Graphics (SIGGRAPH)},
  year = {2004},
  volume = {23},
  pages = {985--995},
  number = {3}
}

@ARTICLE{cohensteiner2004vsa,
  author = {Cohen-Steiner, D. and Alliez, P. and Desbrun, M.},
  title = {{Variational shape approximation}},
  journal = {ACM Trans. on Graphics},
  year = {2004},
  volume = {23},
  pages = {905-914},
  number = {3},
  publisher = {ACM Press New York, NY, USA}
}

@ARTICLE{Cohen-Steiner2006,
  author = {Cohen-Steiner, David and Morvan, Jean-Marie},
  title = {{Second fundamental measure of geometric sets and local approximation of curvatures }},
  journal = {J. Diff. Geom.},
  year = {2006},
  volume = {74},
  pages = {391--404},
  number = {3}
}

@INPROCEEDINGS{Coifman05geometricdiffusions,
  author = {R. R. Coifman and S. Lafon and A. B. Lee and M. Maggioni and F. Warner
	and S. Zucker},
  title = {Geometric diffusions as a tool for harmonic analysis and structure
	definition of data: Diffusion maps},
  booktitle = {Proceedings of the National Academy of Sciences},
  year = {2005},
  pages = {7426--7431},
  owner = {Yiying},
  timestamp = {2009.03.28}
}

@ARTICLE{Cole:2002,
  author = {Cole, C. D. and Frost, A. S. and Thompson, N. and Cotten, M. and
	Cross, T. A. and Busath, D. D.},
  title = {Noncontact Dipole Effects on Channel Permeation. VI. 5F- and {6F-Trp}
	{Gramicidin} Channel Currents},
  journal = {Biophysical Journal},
  year = {2002},
  volume = {83},
  pages = {1974-1986},
  number = { }
}

@ARTICLE{Colella,
  author = {Phillip Colella},
  title = {{Multidimensional Upwind Methods for Hyperbolic Conservation Laws}},
  journal = {J. Comput. Phys.},
  year = {1990},
  volume = {87},
  pages = {171--200},
  number = {1}
}

@ARTICLE{Collier:1996,
  author = {Collier, J. R. and Monk, N. A. M. and Maini, P. K. and Lewis, J.
	H.},
  title = {Pattern formation by lateral inhibition with feedback: A mathematical
	model of Delta-Notch intercellular signalling
	
	},
  journal = {J. Theor. Biol.},
  year = {1996},
  volume = {183},
  pages = {429 - 446 },
  number = { }
}

@ARTICLE{Connolly85,
  author = {Connolly, M. L.},
  title = {Depth buffer algorithms for molecular modeling},
  journal = {J. Mol. Graphics},
  year = {1985},
  volume = {3},
  pages = {19-24}
}

@ARTICLE{Connolly:1983,
  author = {Connolly, M. L. },
  title = {Analytical molecular surface calculation},
  journal = {Journal of Applied Crystallography},
  year = {1983},
  volume = {16},
  pages = {548--558},
  number = {5},
  abstract = {A computer algorithm is presented for calculating the part of the
	{van der waals} surface of molecule that is accessible to solvent.
	The solvent molecule is modeled by a sphere. This sphere is, in effect,
	rolled over the molecule to generate a smooth outer-surface contour.
	This surface contour is made up of pieces of spheres and tori that
	join at circular arcs. The spheres, tori and arcs are defined by
	analytical expressions in terms of the atomic coordinates, {van der
	waals} radii and the probe radius. The area of each surface piece
	may be calculated analytically and the surface may be displayed on
	either vector or raster computer-graphics systems. These methods
	are useful for studying the structure and interactions of proteins
	and nucleic acids.},
  bdsk-url-1 = {http://dx.doi.org/10.1107/S0021889883010985},
  date-added = {2008-06-30 06:51:44 -0500},
  date-modified = {2008-06-30 06:51:44 -0500},
  doi = {10.1107/S0021889883010985},
  keywords = {electrostatics, mathematics, solvation},
  posted-at = {2008-06-30 12:50:46},
  priority = {0},
  url = {http://dx.doi.org/10.1107/S0021889883010985}
}

@ARTICLE{Constantin:2007,
  author = {Constantin, D. and Siwy, Z. S.},
  title = {{Poisson-Nernst -Planck} model of ion current rectification through
	a nanofluidic diode },
  journal = {Phys. Rev. E },
  year = {2007},
  volume = {76},
  pages = { 041202},
  number = {  }
}

@ARTICLE{Corey:1953,
  author = {Corey, R. B. and Pauling, L.},
  title = {Molecular models of amino acids, peptides and proteins},
  journal = {Rev. Sci. Instr.},
  year = {1953},
  volume = {24},
  pages = { 621-627}
}

@ARTICLE{Cornell:1995,
  author = {Cornell, W. D. and Cieplak, P. and Bayly, C. and Gould, I. R. and
	Merz, K. M. J. and Ferguson, D. M. and Spellmeyer, D. C. and Fox,
	T. and Caldwell, J. W. and Kollman, P. A.},
  title = {A second generation force field for the simulation of proteins and
	nucleic acids},
  journal = {J. Am. Chem. Soc.},
  year = {1995},
  volume = {117},
  pages = { 5179 -- 5197}
}

@ARTICLE{Corry:2003,
  author = {Corry, B. and Kuyucak, S. and Chung, S.-H. },
  title = {Dielectric Self-Energy in {Poisson-Boltzmann and Poisson-Nernst-Planck}
	Models of Ion Channels},
  journal = {Biophysical Journal},
  year = {2003},
  volume = {84},
  pages = {3594-3606},
  number = {6}
}

@ARTICLE{Corry:1999,
  author = {Corry, Ben and Kuyucak, Serdar and Chung, Shin-Ho},
  title = {Test of {Poisson-Nernst-Planck} Theory in Ion Channels},
  journal = {The Rockefeller University Press},
  year = {1999},
  volume = {114},
  pages = {597-599},
  number = {4},
  month = { October}
}

@ARTICLE{Cortis:1997,
  author = {Cortis, C. M. and Friesner, R. A.},
  title = {Numerical solution of the {{Poisson-Boltzmann}} equation using tetrahedral
	finite-element meshes},
  journal = {Journal of Computational Chemistry},
  year = {1997},
  volume = {18},
  pages = {1591-1608},
  abstract = {The automatic three-dimensional mesh generation system for molecular
	geometries developed in our laboratory is used to solve the {Poisson-Boltzmann}
	equation numerically using a finite element method. For a number
	of different systems, the results are found to be in good agreement
	with those obtained in finite difference calculations using the DelPhi
	program as well as with those from boundary element calculations
	using our triangulated molecular surface. The overall scaling of
	the method is found to be approximately linear in the number of atoms
	in the system. The finite element mesh structure can be exploited
	to compute the gradient of the polarization energy in 10-20{\%} of
	the time required to solve the equation itself. The resulting timings
	for the larger systems considered indicate that energies and gradients
	can be obtained in about half the time required for a finite difference
	solution to the equation. The development of a multilevel version
	of the algorithm as well as future applications to structure optimization
	using molecular mechanics force fields are also discussed. Ã‚Â??997
	John Wiley \& Sons, Inc.},
  annote = {Numerical solution of the {Poisson-Boltzmann} equation using tetrahedral
	finite-element meshes},
  bdsk-url-1 = {http://www3.interscience.wiley.com/cgi-bin/abstract/48415/ABSTRACT},
  date-added = {2008-06-28 10:58:19 -0500},
  date-modified = {2008-06-28 10:58:19 -0500},
  keywords = {Electrostatics; Mathematics},
  ty = {JOUR},
  url = {http://www3.interscience.wiley.com/cgi-bin/abstract/48415/ABSTRACT}
}

@ARTICLE{Cossi:1996,
  author = {Cossi, M. and Barone, V. and Cammi, R. and Tomasi, J.},
  title = {Ab initio study of solvated molecules: A new implementation of the
	polarizable continuum model},
  journal = {Chemical Physics Letters},
  year = {1996},
  volume = {255},
  pages = {327-335}
}

@ARTICLE{Cox:1981,
  author = {Cox, S. R. and Williams, D. E.},
  title = {Representation of the molecular electrostatic potential by a net
	atomic charge model.},
  journal = { J.Comput. Chem.},
  year = {1981},
  volume = {2},
  pages = {304-323}
}

@ARTICLE{Cozzetto:2009,
  author = {Cozzetto, D. and Kryshtafovych, A. and Fidelis, K. and Moult, J.
	and Rost, B. and Tramontano, A.},
  title = {{Evaluation of template-based models in CASP8 with standard measures}},
  journal = {Proteins},
  year = {2009},
  volume = {77},
  pages = {18-28},
  number = {S9}
}

@BOOK{spectralGeo,
  title = {Old and New Aspects in Spectral Geometry},
  publisher = {Kluwer Academic},
  year = {2001},
  author = {M. Craioveanu and M. Puta and and T. Rassias},
  series = {Mathematics and Applications}
}

@ARTICLE{Cramer:1999,
  author = {Cramer, C. J. and Truhlar, D. G.},
  title = {Implicit Solvation Models: Equilibria, Structure, Spectra, and Dynamics},
  journal = {Chem. Rev.},
  year = {1999},
  volume = {99},
  pages = {2161-2200}
}

@ARTICLE{Crawford9245,
  author = {Crawford, T. D. and Yang, W.},
  title = {The Hartley Basis Functions and Transform - Alternatives to Plane-Waves
	and the Fourier-Transform},
  journal = {Chemical Physics Letters},
  year = {1992},
  volume = {192},
  pages = {45-48},
  number = {1},
  month = {Apr},
  abstract = {The Hartley "cas" basis functions are presented as alternatives to
	the well-known plane waves in electronic structure and molecular
	dynamics calculations. The cas functions are real, amenable to a
	fast transform, and thus offer the advantage of improved computational
	efficiency. The basis functions are tested in the calculation of
	the energy eigenvalues of a Morse oscillator, and are found to give
	results equal in accuracy to the plane waves.},
  endnotereftype = {Journal Article},
  issn = {0009-2614},
  shorttitle = {The Hartley Basis Functions and Transform - Alternatives to Plane-Waves
	and the Fourier-Transform},
  url = {<Go to ISI>://A1992HR94400008}
}

@ARTICLE{CrHuZh08,
  author = {Crosby, F. and Huynh, Q. and Zhou, H. M.},
  title = {Total Variation Methods for Three Dimensional Lidar Image Denoising},
  journal = {Photogrammetric Engineering and Remote Sensing},
  year = {in press 2010}
}

@ARTICLE{Crowley,
  author = {Crowley , P.B. and Golovin, A. },
  title = {Cation{-}pi interactions in protein-protein interfaces},
  journal = {Proteins {-} Struct. Func. Bioinf.},
  year = {2005},
  volume = {59},
  pages = {231-239}
}

@ARTICLE{Crowley:2005,
  author = {Crowley, Peter B. and Golovin, Adel },
  title = {Cation-pi interactions in protein-protein interfaces},
  journal = {Proteins: Structure, Function, and Bioinformatics},
  year = {2005},
  volume = {59},
  pages = {231--239},
  number = {2},
  abstract = {Arginine is an abundant residue in protein-protein interfaces. The
	importance of this residue relates to the versatility of its side
	chain in intermolecular interactions. Different classes of protein-protein
	interfaces were surveyed for cation-pi interactions. Approximately
	half of the protein complexes and one-third of the homodimers analyzed
	were found to contain at least one intermolecular cation-pi pair.
	Interactions between arginine and tyrosine were found to be the most
	abundant. The electrostatic interaction energy was calculated to
	be sim3 kcal/mol, on average. A distance-based search of guanidinium:aromatic
	interactions was also performed using the Macromolecular Structure
	Database (MSD). This search revealed that half of the guanidinium:aromatic
	pairs pack in a coplanar manner. Furthermore, it was found that the
	cationic group of the cation-pi pair is frequently involved in intermolecular
	hydrogen bonds. In this manner the arginine side chain can participate
	in multiple interactions, providing a mechanism for inter-protein
	specificity. Thus, the cation-pi interaction is established as an
	important contributor to protein-protein interfaces. Proteins 2005.
	Â© 2005 Wiley-Liss, Inc.},
  address = {Instituto de Tecnologia Qu\'{i}mica e Biol\'{o}gica, Universidade
	Nova de Lisboa, Oeiras, Portugal; EMBL Bioinformatics Institute,
	Wellcome Trust Genome Campus, Hinxton, Cambridge, United Kingdom},
  bdsk-url-1 = {http://dx.doi.org/10.1002/prot.20417},
  date-added = {2008-06-30 09:21:15 -0500},
  date-modified = {2008-06-30 09:21:15 -0500},
  doi = {10.1002/prot.20417},
  keywords = {electrostatics, protein-protein\_interactions},
  posted-at = {2008-06-30 12:55:23},
  priority = {0},
  url = {http://dx.doi.org/10.1002/prot.20417}
}

@ARTICLE{Cui:2002,
  author = {Cui, Q.},
  title = {Combining implicit solvation models with hybrid quantum mechanical/molecular
	mechanical methods: A critical test with glycine},
  journal = {Journal of Chemical Physics},
  year = {2002},
  volume = {117},
  pages = {4720},
  number = {10},
  abstract = {A combined approach to study reactions in solution in which the solute
	and a number of solvent molecules are described with a hybrid quantum
	mechanical/molecular mechanical (QM/MM) method, and the bulk solvent
	is represented by a polarizable continuum model (PCM) has been implemented.
	In this way, both short-range effects of the first-solvation shell
	and long-range electrostatics due to the bulk solvent can be taken
	into account. By carefully choosing the size of the solute--solvent
	cluster and the QM/MM partition, the current QM/MM/PCM approach can
	offer both computational efficiency and accuracy. The approach has
	been illustrated by two simple systems: water-dimer and glycine in
	water. The results demonstrated that the current approach offers
	a satisfactory description of solvation effects on the geometry and
	energetics of neutral and charged hydrogen-bonding systems. The method
	correctly produced the relative stability of the zwitterionic and
	neutral forms of glycine in solution, which was found to be a subtle
	issue in previous studies. The approach can be extended to study
	reactions in biomolecules in which part of the system is treated
	with QM/MM, and the bulk solvent plus part of the protein or nucleic
	acids are described with either a continuum or approximate microscopic
	representation. Â©2002 American Institute of Physics.},
  bdsk-url-1 = {http://link.aip.org/link/?JCPSA6/117/4720/1},
  bdsk-url-2 = {http://dx.doi.org/10.1063/1.1499481},
  date-added = {2008-06-29 14:38:43 -0500},
  date-modified = {2008-06-29 14:39:39 -0500},
  doi = {10.1063/1.1499481},
  url = {http://link.aip.org/link/?JCPSA6/117/4720/1}
}

@ARTICLE{Cui:2003,
  author = {Cui, Y. and Zhong, Z. and Wang, D. and Wang, W. U. and Lieber, C.
	M.},
  title = {High performance silicon nanowire field effect transistors},
  journal = {Nano Letters},
  year = {2003},
  volume = {3},
  pages = {149-152},
  annote = {High performance silicon nanowire field effect transistors},
  date-added = {2008-11-25 10:28:56 -0500},
  date-modified = {2008-11-25 10:28:56 -0500},
  ty = {JOUR}
}

@ARTICLE{Cukier:2004,
  author = {Cukier, R. I.},
  title = {Theory and simulation of proton-coupled electron transfer, hydrogen-atom
	transfer, and proton translocation in proteins},
  journal = {Biochimica Et Biophysica Acta-Bioenergetics },
  year = {2004},
  volume = {1655},
  pages = {37-44},
  number = { }
}

@ARTICLE{Cukier:2004b,
  author = {Cukier, R. I.},
  title = {Quantum molecular dynamics simulation of proton transfer in cytochrome
	c oxidase},
  journal = {Biochimica Et Biophysica Acta-Bioenergetics },
  year = {2004},
  volume = {1656},
  pages = {189 - 202},
  number = { }
}

@ARTICLE{Cukierman:1997,
  author = {Cukierman, Samuel and Quigley, Edward P. and Crumrine, David S.},
  title = {Proton Conduction in {Gramicidin A} and in Its Dioxolane{-}Linked
	Dimer in Different Lipid Bilayers},
  journal = {Biophys J.},
  year = {1997},
  volume = {73},
  pages = {2489-2502},
  number = { }
}

@ARTICLE{Curatola:2005,
  author = {Curatola, G. and Doornbos, G. and Loo, J. and Ponomarev, Y. V. and
	Iannaccone, G.},
  title = {{Detailed modeling of sub-100-nm MOSFETs based on Schr\"{o}dinger
	DD per subband and experiments and evaluation of the performance
	gap to ballistic transport}},
  journal = {IEEE Trans. Electron Devices},
  year = {2005},
  volume = {52},
  pages = {1851-1858},
  annote = {Detailed modeling of sub-100-nm MOSFETs based on Schrodinger DD per
	subband and experiments and evaluation of the performance gap to
	ballistic transport},
  date-added = {2008-11-25 10:28:56 -0500},
  date-modified = {2008-11-25 10:28:56 -0500},
  ty = {JOUR}
}

@INPROCEEDINGS{VRIP,
  author = {B. Curless and M. Levoy},
  title = {A Volumetric Method for Building Complex Models from Range Images},
  booktitle = {Proc. of ACM SIGGRAPH},
  year = {1996},
  pages = {303--312}
}

@ARTICLE{Curutchet:2006,
  author = {Curutchet, C. and Orozco, M. and Luque, F. J. and Mennucci, B. and
	Tomasi, J.},
  title = {Dispersion and repulsion contributions to the solvation free energy:
	Comparison of quantum mechanical and classical approaches in the
	polarizable continuum model},
  journal = {Journal of Computational Chemistry},
  year = {2006},
  volume = {27},
  pages = {1769-80},
  number = {15},
  abstract = {We report a systematic comparison of the dispersion and repulsion
	contributions to the free energy of solvation determined using quantum
	mechanical self-consistent reaction field (QM-SCRF) and classical
	methods. In particular, QM-SCRF computations have been performed
	using the dispersion and repulsion expressions developed in the framework
	of the integral equation formalism of the polarizable continuum model,
	whereas classical methods involve both empirical pairwise potential
	and surface-dependent approaches. Calculations have been performed
	for a series of aliphatic and aromatic compounds containing prototypical
	functional groups in four solvents: water, octanol, chloroform, and
	carbon tetrachloride. The analysis is focused on the dependence of
	the dispersion and repulsion components on the level of theory used
	in QM-SCRF computations, the contribution of those terms in different
	solvents, and the magnitude of the coupling between electrostatic
	and dispersion-repulsion components. Finally, comparison is made
	between the dispersion-repulsion contributions obtained from QM-SCRF
	calculations and the results determined from classical approaches.},
  annote = {Dispersion and repulsion contributions to the solvation free energy:
	Comparison of quantum mechanical and classical approaches in the
	polarizable continuum model},
  bdsk-url-1 = {http://dx.doi.org/10.1002/jcc.20480},
  date-added = {2008-08-29 15:52:17 -0500},
  date-modified = {2008-08-29 15:52:17 -0500},
  keywords = {Solvation},
  ty = {JOUR},
  url = {http://dx.doi.org/10.1002/jcc.20480}
}

@INCOLLECTION{CGAL,
  author = {Guillaume Damiand},
  title = {Combinatorial Maps},
  booktitle = {{CGAL} User and Reference Manual},
  publisher = {{CGAL Editorial Board}},
  year = {2012},
  edition = {{4.0}},
  note = {\string www.cgal.org/Manual/4.0/doc\_html/cgal\_manual/packages.html\\
	\#Pkg\string:CombinatorialMaps},
  altnote = {\url{www.cgal.org/Manual/4.0/doc_html/cgal_manual/packages.html\\
	#Pkg:CombinatorialMaps}}
}

@ARTICLE{Damjanovic:2007,
  author = {Damjanovic, A. and Schlessman, J. L. and Fitch, C. A. and Garcia,
	A. E. and Garcia-Moreno, B.},
  title = {Role of flexibility and polarity as determinants of the hydration
	of internal cavities and pockets in proteins},
  journal = {Biophysical Journal},
  year = {in press},
  abstract = {Molecular dynamics simulations of Staphylococcal nuclease and of ten
	variants with internal polar or ionizable groups were performed to
	investigate systematically the molecular determinants of hydration
	of internal cavities and pockets in proteins. In contrast to apolar
	cavities in rigid carbon structures, such as nanotubes or buckeyballs,
	internal cavities in proteins that are large enough to house a few
	water molecules will most likely be dehydrated unless they contain
	a source of polarity. The water content in the protein interior can
	be modulated by the flexibility of protein elements that interact
	with water, which can impart positional disorder to water molecules,
	or bias the pattern of internal hydration that is stabilized. This
	might explain differences in the patterns of hydration observed in
	crystal structures obtained at cryogenic and room temperature conditions.
	The ability of molecular dynamics simulations to determine the most
	likely sites of water binding in internal pockets and cavities depends
	on its ability to sample efficiently the hydration of internal sites
	and alternative protein and water conformations. This can be enhanced
	significantly by performing multiple molecular dynamics simulations
	as well as simulations started from different initial hydration states.},
  bdsk-url-1 = {http://dx.doi.org/10.1529/biophysj.107.104182},
  date-added = {2008-09-16 15:43:26 -0500},
  date-modified = {2008-09-16 15:43:26 -0500},
  keywords = {Solvation; MolecularDynamics},
  url = {http://dx.doi.org/10.1529/biophysj.107.104182}
}

@ARTICLE{Darcy:2000,
  author = {Darcy, I.K. and Sumners, D.W.},
  title = {Rational tangle distances on knots and links},
  journal = {MATHEMATICAL PROCEEDINGS OF THE CAMBRIDGE PHILOSOPHICAL SOCIETY },
  year = {2000},
  volume = {128},
  pages = {497-510 },
  number = { }
}

@ARTICLE{Das:1999,
  author = {Das Sarma, S. and Hwang, E. H.},
  title = {Charged impurity-scattering-limited low-temperature resistivity of
	low-density silicon inversion layers },
  journal = {Phys. Rev. Lett.},
  year = {1999},
  volume = {83},
  pages = {164-167},
  annote = {Charged impurity-scattering-limited low-temperature resistivity of
	low-density silicon inversion layers },
  date-added = {2008-11-25 10:28:56 -0500},
  date-modified = {2008-11-25 10:28:56 -0500},
  ty = {JOUR}
}

@BOOK{Datta:1995,
  title = {Electronic Transport in Mesoscopic Systems },
  year = {Cambridge University Press, 1995},
  author = {Datta, S.},
  annote = {Electronic Transport in Mesoscopic Systems, Cambridge University
	Press },
  date-added = {2008-11-25 10:28:56 -0500},
  date-modified = {2008-11-25 10:28:56 -0500},
  ty = {BOOK}
}

@ARTICLE{Datta:2000,
  author = {Datta, S.},
  title = {{Nanoscale device modeling: the Green's function method}},
  journal = {Superlattices and Microstructures},
  year = {2000},
  volume = {28},
  pages = {253-278}
}

@ARTICLE{Daubechies:2009,
  author = {Daubechies, I. and Gunturk, S. and Yilmaz, O. and Wang, Y.},
  title = {The Golden Ratio encoder},
  journal = {IEEE Trans. Information Theory},
  year = {submitted, 2009}
}

@ARTICLE{Daubechies,
  author = {I. Daubechies and I. Guskov and W. Sweldens},
  title = {Regularity of Irregular Subdivision},
  journal = {Constructive Approximation},
  year = {1999},
  volume = {15},
  pages = {381-426}
}

@ARTICLE{David:2000,
  author = {David, L. and Luo, R. and Gilson, M. K.},
  title = {Comparison of generalized {Born} and {Poisson} models: Energetics
	and dynamics of {HIV} protease},
  journal = {Journal of Computational Chemistry},
  year = {2000},
  volume = {21},
  pages = {295-309},
  number = {4},
  abstract = {This study characterizes the accuracy of energies and forces computed
	with a generalized Born (GB) model and the distance-dependent dielectric
	(DDD) model with respect to detailed finite solutions of the Poisson
	equation (FDPE). Tests are done for a small molecule in solution
	and for HIV-1 protease with inhibitor, KNI-272. GB agrees well with
	FDPE for the small molecule, but less well for the protein system.
	The correlation between GB and FDPE energies is poorest in calculations
	of changes upon binding. Also, forces computed with the GB model
	are less accurate than energies. The DDD model is far less accurate
	than GB. Nanosecond stochastic dynamics simulations of HIV-1 protease
	with an empty active site are used to examine the consequence of
	the models for the conformational preferences of the active site.
	Interestingly, the active site flaps remain near their starting conformations
	in the FDPE and GB simulations but collapse into the active site
	in the DDD simulation. Ã‚Â??000 John Wiley \& Sons, Inc. J Comput
	Chem 21: 295-309, 2000},
  address = {NIST Rockville, MD USA 20850 Gilson, MK Ctr Adv Res Biotechnol, 9600
	Gudelsky Dr Gilson, MK gilson@carb.nist.gov NIST Rockville, MD USA
	20850 Ctr Adv Res Biotechnol},
  annote = {Comparison of generalized Born and Poisson models: Energetics and
	dynamics of HIV protease; MAR},
  bdsk-url-1 = {http://www3.interscience.wiley.com/cgi-bin/fulltext/69504135/HTMLSTART},
  date-added = {2008-09-01 14:00:20 -0500},
  date-modified = {2008-09-01 14:00:20 -0500},
  journal1 = {J Comput Chem},
  keywords = {Electrostatics},
  ty = {JOUR},
  url = {http://www3.interscience.wiley.com/cgi-bin/fulltext/69504135/HTMLSTART}
}

@ARTICLE{Davies:2006,
  author = {Davies, M. N. and Toseland, C. P. and Moss, D. S. and Flower, D.
	R.},
  title = {Benchmarking {pKa} prediction},
  journal = {BMC Biochemistry},
  year = {2006},
  volume = {7},
  pages = {18},
  abstract = {Background pKa values are a measure of the protonation of ionizable
	groups in proteins. Ionizable groups are involved in intra-protein,
	protein-solvent and protein-ligand interactions as well as solubility,
	protein folding and catalytic activity. The pKa shift of a group
	from its intrinsic value is determined by the perturbation of the
	residue by the environment and can be calculated from three-dimensional
	structural data. Results Here we use a large dataset of experimentally-determined
	pKas to analyse the performance of different prediction techniques.
	Our work provides a benchmark of available software implementations:
	MCCE, MEAD, PROPKA and UHBD. Combinatorial and regression analysis
	is also used in an attempt to find a consensus approach towards pKa
	prediction. The tendency of individual programs to over- or underpredict
	the pKa value is related to the underlying methodology of the individual
	programs. Conclusion Overall, PROPKA is more accurate than the other
	three programs. Key to developing accurate predictive software will
	be a complete sampling of conformations accessible to protein structures.},
  annote = {Benchmarking {pKa} prediction},
  bdsk-url-1 = {http://dx.doi.org/10.1186/1471-2091-7-18},
  date-added = {2008-09-16 15:40:23 -0500},
  date-modified = {2008-09-16 15:40:23 -0500},
  keywords = {Solvation; pKa; Electrostatics},
  ty = {JOUR},
  url = {http://dx.doi.org/10.1186/1471-2091-7-18}
}

@ARTICLE{Davis:1991b,
  author = {Davis, M. E. and Madura, J. D. and Sines, J. and Luty, B. A. and
	Allison, S. A. and McCammon, J. A.},
  title = {Diffusion-controlled enzymatic reactions},
  journal = {Methods in Enzymology},
  year = {1991},
  volume = {202},
  pages = {473-497},
  annote = {Diffusion-controlled enzymatic reactions},
  date-added = {2008-09-01 14:01:36 -0500},
  date-modified = {2008-09-01 14:01:36 -0500},
  keywords = {Diffusion},
  ty = {JOUR},
  url = {http://www.sciencedirect.com/science?_ob=ArticleURL&_udi=B7CV2-4B3T11F-5C&_user=4275&_handle=B-WA-A-A-BE-MsSAYZW-UUA-AUYCZYEUUV-AUYBWZEYUV-BYVVDEVUD-BE-U&_fmt=summary&_coverDate=12%2F31%2F1991&_rdoc=22&_orig=browse&_srch=%23toc%2318066%231991%23997979999%23472502!&_cdi=18066&view=c&_acct=C000000938&_version=1&_urlVersion=0&_userid=4275&md5=6dfa241aba9433c0409af47b6576d902}
}

@ARTICLE{Davis:1990a,
  author = {Davis, M. E. and McCammon, J. A.},
  title = {Electrostatics in biomolecular structure and dynamics},
  journal = {Chemical Reviews},
  year = {1990},
  volume = {94},
  pages = {509-21},
  annote = {Electrostatics in biomolecular structure and dynamics; DavisMcCammon},
  bdsk-url-1 = {http://dx.doi.org/10.1021/cr00101a005},
  date-added = {2008-09-01 13:57:15 -0500},
  date-modified = {2008-09-01 13:57:15 -0500},
  doi = {http://dx.doi.org/10.1021/cr00101a005},
  keywords = {Electrostatics},
  ty = {JOUR}
}

@ARTICLE{Day:2003,
  author = {Day, Tyler J. F. and Soudackov, Alexander V. and Cuma,Martin and
	Schmitt, Udo W. and Voth, Gregory A. },
  title = {{A second generation multistate empirical valence bond model for
	proton transport in aqueous systems}},
  journal = {Journal of Chemical Physics},
  year = {2002},
  volume = {117},
  pages = {5840-5849}
}

@ARTICLE{De-Rienzo:2001,
  author = {De Rienzo, F. and Gabdoulline, R. R. and Menziani, M. C. and De Benedetti,
	P. G. and Wade, R. C.},
  title = {Electrostatic analysis and {Brownian} dynamics simulation of the
	association of plastocyanin and cytochrome {F}},
  journal = {Biophysical Journal},
  year = {2001},
  volume = {81},
  pages = {3090-3104},
  number = {6},
  abstract = {The oxidation of cytochrome f by the soluble cupredoxin plastocyanin
	is a central reaction in the photosynthetic electron transfer chain
	of all oxygenic organisms. Here, two different computational approaches
	are used to gain new insights into the role of molecular recognition
	and protein-protein association processes in this redox reaction.
	First, a comparative analysis of the computed molecular electrostatic
	potentials of seven single and multiple point mutants of spinach
	plastocyanin (D42N, E43K, E43N, E43Q/D44N, E59K/E60Q, E59K/E60Q/E43N,
	Q88E) and the wt protein was carried out. The experimentally determined
	relative rates (k2) for the set of plastocyanin mutants are found
	to correlate well (r2 = 0.90 0.97) with the computed measure of the
	similarity of the plastocyanin electrostatic potentials. Second,
	the effects on the plastocyanin/cytochrome f association rate of
	these mutations in the plastocyanin {\tt{}"{}}eastern site{\tt{}"{}}
	were evaluated by simulating the association of the wild type and
	mutant plastocyanins with cytochrome f by Brownian dynamics. Good
	agreement between the computed and experimental relative rates (k2)
	(r2 = 0.89 0.92) was achieved for the plastocyanin mutants. The results
	obtained by applying both computational techniques provide support
	for the fundamental role of the acidic residues at the plastocyanin
	eastern site in the association with cytochrome f and in the overall
	electron-transfer process.},
  address = {Univ Modena Reggio Emilia Modena Italy I-41100 Menziani, MC Dipartimento
	Chim, Via Campi 183 Menziani, MC menziani@unimo.it Univ Modena Reggio
	Emilia Modena Italy I-41100 Dipartimento Chim European Mol Biol Lab
	Heidelberg Germany D-69012 European Media Lab Heidelberg Germany
	D-69118},
  annote = {Electrostatic analysis and Brownian dynamics simulation of the association
	of plastocyanin and cytochrome F; DEC},
  bdsk-url-1 = {http://www.biophysj.org/cgi/content/abstract/81/6/3090},
  date-added = {2008-09-15 10:06:38 -0500},
  date-modified = {2008-09-15 10:06:38 -0500},
  journal1 = {Biophys J},
  keywords = {Electrostatics; Bioinformatics; Diffusion},
  read = {Yes},
  ty = {JOUR},
  url = {http://www.biophysj.org/cgi/content/abstract/81/6/3090}
}

@INPROCEEDINGS{DDCB01,
  author = {Gilles Debunne and Mathieu Desbrun and Marie-Paule Cani and Alan
	Barr},
  title = {Dynamic Real-Time Deformations using Space \& Time Adaptive Sampling},
  booktitle = {ACM SIGGRAPH Conference},
  year = {2001},
  pages = {31--36},
  month = {August}
}

@INPROCEEDINGS{DDCB00,
  author = {Gilles Debunne and Mathieu Desbrun and Marie-Paule Cani and Alan
	Barr},
  title = {Adaptive Simulation of Soft Bodies in Real-Time},
  booktitle = {Computer Animation Conference Proceedings},
  year = {2000},
  month = {May}
}

@INPROCEEDINGS{DDCB00,
  author = {Gilles Debunne and Mathieu Desbrun and Marie-Paule Cani and Alan
	H. Barr},
  title = {Adaptive Simulation of Soft Bodies in Real-Time},
  booktitle = {Computer Animation},
  year = {2000},
  pages = {133-144},
  month = {May}
}

@ARTICLE{Decornez:1999,
  author = {Decornez, H. and Drukker, K. and Hammes-Schiffer, H.},
  title = {Solvation and hydrogen-bonding effects on proton wires},
  journal = {J. Phys. Chem. A },
  year = {1999},
  volume = {103},
  pages = {2891- 2898}
}

@ARTICLE{Decoursey:2003,
  author = {Decoursey, Thomas},
  title = {Voltage-gated proton channels and other proton transfer pathways},
  journal = {Physiol Rev},
  year = {2003},
  volume = {83},
  pages = {475-579}
}




@ARTICLE{Musset:2011,
  author = {Musset, B and Smith, S. M. E. and  Rajan, S.  and  Morgan, D.  and  Cherny, V. V.  and  DeCoursey, T. E.},
  title = {Aspartate 112 is the selectivity filter of the human voltage-gated proton channel},
  journal = {Nature},
  year = {2011},
  volume = {480},
  pages = {273-U167}
}



@ARTICLE{Degond:2007,
  author = {Degond, P. and Gallego, S. and Mehats, F.},
  title = {An entropic quantum drift-diffusion model for electron transport
	in resonant tunneling diodes},
  journal = {J. Comput. Phys.},
  year = {2007},
  volume = {221},
  pages = {226-249 },
  annote = {An entropic quantum drift-diffusion model for electron transport
	in resonant tunneling diodes},
  date-added = {2008-11-25 10:28:56 -0500},
  date-modified = {2008-11-25 10:28:56 -0500},
  ty = {JOUR}
}

@MISC{PyMOL,
  author = {DeLano, W. L.},
  title = {The {PyMOL} Molecular Graphics System},
  howpublished = {http://www.pymol.org/},
  year = {2002},
  address = {Palo Alto, CAThe PyMOL Molecular Graphics System},
  annote = {PyMOL; The PyMOL Molecular Graphics System},
  bdsk-url-1 = {http://www.pymol.org/},
  date-added = {2008-09-17 09:18:58 -0500},
  date-modified = {2008-09-17 09:18:58 -0500},
  keywords = {Electrostatics; Software},
  ty = {COMP}
}

@ARTICLE{Deng:2003,
  author = {Deng, S. Z. and Ito, K. and Li, Z. L.},
  title = {Three-dimensional elliptic solvers for interface problems and applications},
  journal = {J. Comput. Phys. },
  year = {2003},
  volume = {184},
  pages = {215-243},
  annote = {Three-dimensional elliptic solvers for interface problems and applications},
  date-added = {2008-09-19 10:28:56 -0500},
  date-modified = {2008-09-19 10:28:56 -0500},
  ty = {JOUR}
}

@ARTICLE{Denisov:2004,
  author = {Denisov, V. P. and Schlessman, J. L. and GarcÃ­a-Moreno, B. E.
	and Halle, B.},
  title = {Stabilization of Internal Charges in a Protein: Water Penetration
	or Conformational Change?},
  journal = {Biophysical Journal},
  year = {2004},
  volume = {87},
  pages = {3982-94},
  number = {6},
  abstract = {The ionizable amino acid side chains of proteins are usually located
	at the surface. However, in some proteins an ionizable group is embedded
	in an apolar internal region. Such buried ionizable groups destabilize
	the protein and may trigger conformational changes in response to
	pH variations. Because of the prohibitive energetic cost of transferring
	a charged group from water to an apolar medium, other stabilizing
	factors must be invoked, such as ionization-induced water penetration
	or structural changes. To examine the role of water penetration,
	we have measured the 17O and 2H magnetic relaxation dispersions (MRD)
	for the V66E and V66K mutants of staphylococcal nuclease, where glutamic
	acid and lysine residues are buried in predominantly apolar environments.
	At neutral pH, where these residues are uncharged, we find no evidence
	of buried water molecules near the mutation site. This contrasts
	with a previous cryogenic crystal structure of the V66E mutant, but
	is consistent with the room-temperature crystal structure reported
	here. MRD measurements at different pH values show that ionization
	of Glu-66 or Lys-66 is not accompanied by penetration of long-lived
	water molecules. On the other hand, the MRD data are consistent with
	a local conformational change in response to ionization of the internal
	residues.},
  annote = {Stabilization of Internal Charges in a Protein: Water Penetration
	or Conformational Change?},
  bdsk-url-1 = {http://dx.doi.org/10.1529/biophysj.104.048454},
  date-added = {2008-09-16 15:43:22 -0500},
  date-modified = {2008-09-16 15:43:22 -0500},
  keywords = {Solvation},
  ty = {JOUR},
  url = {http://dx.doi.org/10.1529/biophysj.104.048454}
}

@INPROCEEDINGS{Des02,
  author = {Mathieu Desbrun},
  title = {Processing Irregular Meshes},
  booktitle = {Shape Modeling International (paper for invited talk)},
  year = {2002},
  month = Jun
}

@INPROCEEDINGS{DDG,
  author = {Mathieu Desbrun and Eitan Grinspun and Peter Schr{\"o}der},
  title = {Discrete Differential Geometry: An Applied Introduction},
  year = {2006},
  proceeding = {ACM SIGGRAPH Course Notes}
}

@INPROCEEDINGS{DHM03,
  author = {Mathieu Desbrun and Anil Hirani and Jerrold E. Marsden},
  title = {Discrete Exterior Calculus for Variational Problems in Computer Vision
	and Graphics},
  booktitle = {IEEE Conference on Decision and Control (CDC'03)},
  year = {2003},
  volume = {42},
  pages = {4903--4907},
  month = jun
}

@INCOLLECTION{DKT07,
  author = {Mathieu Desbrun and Eva Kanso and Yiying Tong},
  title = {Discrete Differential Forms for Computational Modeling},
  booktitle = {Discrete Differential Geometry},
  publisher = {Springer},
  year = {2007},
  editor = {A. Bobenko and P. Schr{\"o}der}
}

@INCOLLECTION{Desbrun2008,
  author = {Desbrun, Mathieu and Kanso, Eva and Tong, Yiying},
  title = {{Discrete Differential Forms for Computational Modeling}},
  booktitle = {Discrete Differential Geometry},
  publisher = {Springer},
  year = {2008},
  editor = {{Bobenko, A. Schr\"{o}der, P. Sullivan, J. Ziegler}, G.},
  pages = {287--324},
  doi = {10.1007/978-3-7643-8621-4_16},
  file = {:C\:/Users/yiying/Desktop/SVN/geometrycode/references/Desbrun, Kanso, Tong - 2008 - Discrete Differential Forms for Computational Modeling.pdf:pdf}
}

@INCOLLECTION{DKT06,
  author = {Mathieu Desbrun and Eva Kanso and Yiying Tong},
  title = {{Discrete Differential Forms for Computational Sciences}},
  booktitle = {Discrete Differential Geometry},
  publisher = {ACM SIGGRAPH},
  year = {2006},
  editor = {Eitan Grinspun and Peter Schr{\"o}der and Mathieu Desbrun},
  series = {Course Notes}
}

@INCOLLECTION{DKT06,
  author = {Mathieu Desbrun and Eva Kanso and Yiying Tong},
  title = {Discrete Differential Forms for Computational Modeling},
  booktitle = {ACM SIGGRAPH'06 Course Notes on Discrete Differential Geometry},
  publisher = {ACM Press},
  year = {2006}
}

@ARTICLE{DLM05,
  author = {Mathieu Desbrun and Melvin Leok and Jerrold E. Marsden},
  title = {Discrete Poincar{\'e} Lemma},
  journal = {Applied Numerical Mathematics},
  year = {2005},
  volume = {53},
  pages = {231--248}
}

@INPROCEEDINGS{DMA02,
  author = {Mathieu Desbrun and Mark Meyer and Pierre Alliez},
  title = {Intrinsic Parameterizations of Surface Meshes},
  booktitle = {Eurographics Conference},
  year = {2002},
  volume = {21},
  month = sep,
  issue = {3}
}

@INCOLLECTION{DMB00,
  author = {Mathieu Desbrun and Mark Meyer and Alan H. Barr},
  title = {Interactive Animation of Cloth-like Objects for Virtual Reality},
  booktitle = {Cloth Modeling and Animation},
  publisher = {A.K. Peters},
  year = {2000},
  editor = {Donald House and David Breen},
  chapter = {9}
}

@ARTICLE{desbrun-meyer-etal:99,
  author = {Desbrun, M. and Meyer, M. and Schr\"oder, P. and Barr, A.H.},
  title = {Implicit Fairing of Irregular Meshes using Diffusion and Curvature
	Flow},
  journal = {ACM SIGGRAPH},
  year = {1999},
  pages = {317--324}
}

@INPROCEEDINGS{DMSB98,
  author = {Mathieu Desbrun and Mark Meyer and Peter Schr\"{o}der and Alan H.
	Barr},
  title = {Implicit fairing of irregular meshes using diffusion and curvature
	flow},
  booktitle = {ACM SIGGRAPH},
  year = {1999},
  pages = {317--324}
}

@INPROCEEDINGS{DMSB00,
  author = {Mathieu Desbrun and Mark Meyer and Peter Schr{\"o}der and Alan H.
	Barr},
  title = {Anisotropic Feature-Preserving Denoising of Height Fields and Bivariate
	Data},
  booktitle = {Proceedings of Graphics Interface},
  year = {2000}
}

@INPROCEEDINGS{Dey-Giesen-etal:04,
  author = {Dey, T. K. and Giesen, J. and Goswami, S.},
  title = {Shape Segmentation and Matching with Flow Discretization},
  booktitle = {Workshop on Algorithms and Data Structures},
  year = {2003},
  pages = {25--36}
}

@ARTICLE{DeyLS09,
  author = {Dey, Tamal. K. and Li, Kuiyu and Sun, Jian},
  title = {Computing handle and tunnel loops with knot linking},
  journal = {Computer Aided Design},
  year = {2009},
  volume = {41},
  pages = {730--738},
  number = {10},
  address = {Newton, MA, USA},
  doi = {http://dx.doi.org/10.1016/j.cad.2009.01.001},
  issn = {0010-4485},
  publisher = {Butterworth-Heinemann}
}

@ARTICLE{DeyLSC08,
  author = {Tamal. K. Dey and Kuiyu Li and Jian Sun and David Cohen-Steiner},
  title = {Computing geometry-aware handle and tunnel loops in 3D models.},
  journal = {ACM Trans. Graph. (SIGGRAPH 08)},
  year = {2008},
  volume = {27},
  number = {3},
  ee = {http://doi.acm.org/10.1145/1360612.1360644},
  url = {http://dblp.uni-trier.de/db/journals/tog/tog27.html#DeyLSC08}
}

@ARTICLE{YDi:2005,
  author = {Di, Y. and Li, R. and Tang, T. and Zhang, P.},
  title = {{Moving mesh finite element methods for the incompressible {{Navier-Stokes}}
	equations}},
  journal = {SIAM J.SCI.COMPUT},
  year = {2005},
  volume = {26},
  pages = {1036-1056}
}

@INPROCEEDINGS{TVMin,
  author = {Fran{\,c}oise Dibos and Georges Koepfler},
  title = {Total Variation Minimization by the Fast Level Sets Transform},
  booktitle = {Proc. of IEEE Workshop on Variational and Level Set Methods (VLSM)},
  year = {2001},
  pages = {179--185}
}

@ARTICLE{SDidas:2009,
  author = {Didas, S. and Weickert, J. and Burgeth, B.},
  title = {{Properties of higher order nonlinear diffusion filtering}},
  journal = {Journal of mathematical imaging and vision},
  year = {2009},
  volume = {35},
  pages = {208--226},
  number = {3},
  issn = {0924-9907},
  publisher = {Springer}
}

@ARTICLE{BayesianPriors,
  author = {James R. Diebel and Sebastian Thrun and Michael Br{\"u}nig},
  title = {A {B}ayesian Method for Probable Surface Reconstruction \& Decimation},
  journal = {ACM Trans. Graphics},
  year = {2006},
  volume = {25},
  pages = {39--59},
  number = {1}
}

@ARTICLE{DSSCNS09,
  author = {Dietrich, C.A. and Scheidegger, C. E. and Schreiner, J. and Comba,
	J. L. D. and Nedel, L. P. and Silva, C. T.},
  title = {Edge Transformations for Improving Mesh Quality of Marching Cubes},
  journal = {IEEE Transactions on Visualization and Computer Graphics},
  year = {2009},
  volume = {15},
  pages = {150--159},
  number = {1},
  address = {Piscataway, NJ, USA},
  doi = {http://dx.doi.org/10.1109/TVCG.2008.60},
  issn = {1077-2626},
  owner = {Yiying},
  publisher = {IEEE Educational Activities Department},
  timestamp = {2009.03.26}
}

@ARTICLE{FDing:2003,
  author = {Ding, F. and Borreguero, J.M. and Buldyrey, S.V. and Stanley, H.E.
	and Dokholyan, N.V.},
  title = {Mechanism for the alpha-helix to beta-hairpin transition},
  journal = {J Am Chem Soc},
  year = {2003},
  volume = {53},
  pages = {220-228},
  number = { }
}

@ARTICLE{DYT05,
  author = {Dinh,, Huong Quynh and Yezzi,, Anthony and Turk,, Greg},
  title = {Texture transfer during shape transformation},
  journal = {ACM Trans. Graph.},
  year = {2005},
  volume = {24},
  pages = {289--310},
  number = {2},
  address = {New York, NY, USA},
  doi = {http://doi.acm.org/10.1145/1061347.1061353},
  issn = {0730-0301},
  owner = {Yiying},
  publisher = {ACM},
  timestamp = {2009.03.26}
}

@ARTICLE{MP-FEMLSM,
  author = {Daniele A. DiPietro and Stefania LoForte and Nicola Parolini},
  title = {{Mass Preserving Finite Element Implementations of the Level Set
	Method}},
  journal = {Applied Numerical Mathematics},
  year = {2006},
  volume = {56},
  pages = {1179--1195},
  number = {9}
}

@ARTICLE{Ditkowski:2008,
  author = {Ditkowski, Adi and Suhov, Alexander},
  title = {Near-field infinity-simulating boundary conditions for the heat equation},
  journal = {Proceedings of the National Academy of Sciences},
  year = {2008},
  volume = {105},
  pages = {10646-10648},
  number = {31},
  abstract = {The numerical simulation of various physical phenomena in infinite
	domains poses great difficulties. Truncation of the domain is usually
	necessary in such cases. To ensure stability of the resulting problem
	on the restricted domain, appropriate boundary conditions should
	be applied. Here, we develop a boundary condition for the case in
	which the heat equation is satisfied outside the domain of interest
	with no restrictions on the equation inside. The condition employs
	a thin layer encasing the computational domain. The resulting condition,
	combined with techniques similar to those proposed by Jiang and Greengard
	[Jiang S, Greengard L (2004) Fast evaluation of nonreflecting boundary
	conditions for the SchrÃ¶dinger equation in one dimension. 47:955â-66.]
	promises to be more accurate and computationally efficient than previously
	described techniques.},
  bdsk-url-1 = {http://www.pnas.org/content/105/31/10646.abstract},
  bdsk-url-2 = {http://dx.doi.org/10.1073/pnas.0802671105},
  date-added = {2008-09-14 15:32:12 -0500},
  date-modified = {2008-09-14 15:32:12 -0500},
  doi = {10.1073/pnas.0802671105},
  eprint = {http://www.pnas.org/content/105/31/10646.full.pdf+html},
  keywords = {Mathematics; Diffusion},
  url = {http://www.pnas.org/content/105/31/10646.abstract}
}

@INPROCEEDINGS{Dobkin1987,
  author = {Dobkin, D. P. and Laszlo, M. J.},
  title = {Primitives for the manipulation of three-dimensional subdivisions},
  booktitle = {Proceedings of the third annual Symposium on Computational Geometry},
  year = {1987},
  series = {SCG '87},
  pages = {86--99},
  address = {New York, NY, USA},
  publisher = {ACM},
  acmid = {41967},
  doi = {10.1145/41958.41967},
  isbn = {0-89791-231-4},
  location = {Waterloo, Ontario, Canada},
  numpages = {14},
  url = {http://doi.acm.org/10.1145/41958.41967}
}

@ARTICLE{Dolinsky:2007,
  author = {Dolinsky, T. J. and Czodrowski, P. and Li, H. and Nielsen, J. E.
	and Jensen, J. H. and Klebe, G. and Baker, N. A. },
  title = {PDB2PQR: Expanding and upgrading automated preparation of biomolecular
	structures for molecular simulations},
  journal = {Nucleic Acids Res},
  year = {2007},
  volume = {35},
  pages = {W522-525}
}

@ARTICLE{PDB2PQR2,
  author = {Dolinsky, T. J. and Czodrowski, P. and Li, H. and Nielsen, J. E.
	and Jensen, J. H. and Klebe, G. and Baker, N. A.},
  title = {{PDB2PQR}: expanding and upgrading automated preparation of biomolecular
	structures for molecular simulations},
  journal = {Nucleic Acids Research},
  year = {2007},
  volume = {35},
  pages = {W522-5},
  number = {S2},
  abstract = {Real-world observable physical and chemical characteristics are increasingly
	being calculated from the 3D structures of biomolecules. Methods
	for calculating pKa values, binding constants of ligands, and changes
	in protein stability are readily available, but often the limiting
	step in computational biology is the conversion of PDB structures
	into formats ready for use with biomolecular simulation software.
	The continued sophistication and integration of biomolecular simulation
	methods for systems- and genome-wide studies requires a fast, robust,
	physically realistic and standardized protocol for preparing macromolecular
	structures for biophysical algorithms. As described previously, the
	PDB2PQR web server addresses this need for electrostatic field calculations
	(Dolinsky et al., Nucleic Acids Research, 32, W665--W667, 2004).
	Here we report the significantly expanded PDB2PQR that includes the
	following features: robust standalone command line support, improved
	pKa estimation via the PROPKA framework, ligand parameterization
	via PEOE_PB charge methodology, expanded set of force fields and
	easily incorporated user-defined parameters via XML input files,
	and improvement of atom addition and optimization code. These features
	are available through a new web interface (http://pdb2pqr.sourceforge.net/),
	which offers users a wide range of options for PDB file conversion,
	modification and parameterization.},
  bdsk-file-1 = {YnBsaXN0MDDUAQIDBAUGCQpYJHZlcnNpb25UJHRvcFkkYXJjaGl2ZXJYJG9iamVjdHMSAAGGoNE
	HCFRyb290gAFfEA9OU0tleWVkQXJjaGl2ZXKoCwwXGBkdJCVVJG51bGzTDQ4PEBEUViRjbGFzc1
	dOUy5rZXlzWk5TLm9iamVjdHOAB6ISE4ACgAOiFRaABIAGWWFsaWFzRGF0YVxyZWxhdGl2ZVBhd
	GjSDRobHFdOUy5kYXRhgAVPEQIqAAAAAAIqAAIAAAxNYWNpbnRvc2ggSEQAAAAAAAAAAAAAAAAA
	AADD4v5NSCsAAAAZYksfMjAwNy1Eb2xpbnNreUN6b2Ryb3cjMTk2MjhGLnBkZgAAAAAAAAAAAAA
	AAAAAAAAAAAAAAAAAAAAAAAAAAAAAABlij8JmEbAAAAAAAAAAAAAEAAQAAAkgAAAAAAAAAAAAAA
	AAAAAAB0FyY2hpdmUAABAACAAAw+NSrQAAABEACAAAwmZYAAAAAAEAFAAZYksAGWIDAAqkKAAKp
	BEAAHrcAAIAVU1hY2ludG9zaCBIRDpVc2VyczpiYWtlcjpEb2N1bWVudHM6UmVmZXJlbmNlczpB
	cmNoaXZlOjIwMDctRG9saW5za3lDem9kcm93IzE5NjI4Ri5wZGYAAA4AagA0ADIAMAAwADcALQB
	EAG8AbABpAG4AcwBrAHkAQwB6AG8AZAByAG8AdwBzAGsAaQBMAGkATgBpAGUAbABzAGUAbgBKAG
	UAbgBzAGUAbgBLAGwAZQBiAGUAQgBhAGsAZQByAC4AcABkAGYADwAaAAwATQBhAGMAaQBuAHQAb
	wBzAGgAIABIAEQAEgBdVXNlcnMvYmFrZXIvRG9jdW1lbnRzL1JlZmVyZW5jZXMvQXJjaGl2ZS8y
	MDA3LURvbGluc2t5Q3pvZHJvd3NraUxpTmllbHNlbkplbnNlbktsZWJlQmFrZXIucGRmAAATAAE
	vAAAVAAIADP//AADSHh8gIVgkY2xhc3Nlc1okY2xhc3NuYW1loyEiI11OU011dGFibGVEYXRhVk
	5TRGF0YVhOU09iamVjdF8QXS4uLy4uLy4uLy4uL0RvY3VtZW50cy9SZWZlcmVuY2VzL0FyY2hpd
	mUvMjAwNy1Eb2xpbnNreUN6b2Ryb3dza2lMaU5pZWxzZW5KZW5zZW5LbGViZUJha2VyLnBkZtIe
	HyYnoicjXE5TRGljdGlvbmFyeQAIABEAGgAfACkAMgA3ADoAPwBBAFMAXABiAGkAcAB4AIMAhQC
	IAIoAjACPAJEAkwCdAKoArwC3ALkC5wLsAvUDAAMEAxIDGQMiA4IDhwOKAAAAAAAAAgEAAAAAAA
	AAKAAAAAAAAAAAAAAAAAAAA5c=},
  bdsk-url-1 = {http://tinyurl.com/25e9ff},
  date-added = {2008-09-17 09:18:10 -0500},
  date-modified = {2008-09-17 09:18:10 -0500},
  keywords = {pKa; Solvation; Software},
  url = {http://tinyurl.com/25e9ff}
}

@ARTICLE{Dolinsky:2004,
  author = {Dolinsky, T. J. and Nielsen, J. E. and McCammon, J. A. and Baker,
	N. A. },
  title = {PDB2PQR: an automated pipeline for the setup, execution, and analysis
	of {Poisson-Boltzmann} electrostatics calculations},
  journal = {Nucleic Acids Res},
  year = {2004},
  volume = {32},
  pages = {W665-W667}
}

@ARTICLE{Pdb2pqr,
  author = {Dolinsky, T. J. and Nielsen, J. E. and McCammon, J. A. and Baker,
	N. A.},
  title = {{PDB2PQR}: {A}n automated pipeline for the setup, execution, and
	analysis of {Poisson-Boltzmann} electrostatics calculations},
  journal = {Nucleic Acids Research},
  year = {2004},
  volume = {32},
  pages = {W665-W667}
}

@ARTICLE{PDB2PQR1,
  author = {Dolinsky, T. J. and Nielsen, J. E. and McCammon, J. A. and Baker,
	N. A.},
  title = {{PDB2PQR}: an automated pipeline for the setup, execution, and analysis
	of {Poisson-Boltzmann} electrostatics calculations},
  journal = {Nucleic Acids Research},
  year = {2004},
  volume = {32},
  pages = {W665-W667},
  number = {S2},
  abstract = {Continuum solvation models, such as {Poisson-Boltzmann} and Generalized
	Born methods, have become increasingly popular tools for investigating
	the influence of electrostatics on biomolecular structure, energetics
	and dynamics. However, the use of such methods requires accurate
	and complete structural data as well as force field parameters such
	as atomic charges and radii. Unfortunately, the limiting step in
	continuum electrostatics calculations is often addition of missing
	atomic coordinates to molecular structures from the Protein Data
	Bank and the assignment of parameters to biomolecular structures.
	To address this problem, we have developed the PDB2PQR web service
	(http://agave.wustl.edu/pdb2pqr/). This server automates many of
	the common tasks of preparing structures for continuum electrostatics
	calculations, including: adding a limited number of missing heavy
	atoms to biomolecular structures, estimating titration states and
	protonating biomolecules in a manner consistent with favorable hydrogen-bonding,
	assigning charge and radius parameters from a variety of force fields,
	and finally generating {\tt{}"{}}PQR{\tt{}"{}} output compatible
	with several popular computational biology packages. This service
	is intended to facilitate the setup and execution of electrostatics
	calculations for both experts and non-experts and thereby broaden
	the accessibility of the biological community to continuum electrostatics
	analyses of biomolecular systems.},
  annote = {PDB2PQR: an automated pipeline for the setup, execution, and analysis
	of {Poisson-Boltzmann} electrostatics calculations; PDB2PQR},
  bdsk-file-1 = {YnBsaXN0MDDUAQIDBAUGCQpYJHZlcnNpb25UJHRvcFkkYXJjaGl2ZXJYJG9iamVjdHMSAAGGoNE
	HCFRyb290gAFfEA9OU0tleWVkQXJjaGl2ZXKoCwwXGBkdJCVVJG51bGzTDQ4PEBEUViRjbGFzc1
	dOUy5rZXlzWk5TLm9iamVjdHOAB6ISE4ACgAOiFRaABIAGWWFsaWFzRGF0YVxyZWxhdGl2ZVBhd
	GjSDRobHFdOUy5kYXRhgAVPEQH8AAAAAAH8AAIAAAxNYWNpbnRvc2ggSEQAAAAAAAAAAAAAAAAA
	AADD4v5NSCsAAAAZYksfMjAwNC1Eb2xpbnNreU5pZWxzZW4jMTk2MkIzLnBkZgAAAAAAAAAAAAA
	AAAAAAAAAAAAAAAAAAAAAAAAAAAAAABlis8M6CndQREYgcHJ2dwAEAAQAAAkgAAAAAAAAAAAAAA
	AAAAAAB0FyY2hpdmUAABAACAAAw+NSrQAAABEACAAAwzpQxwAAAAEAFAAZYksAGWIDAAqkKAAKp
	BEAAHrcAAIAVU1hY2ludG9zaCBIRDpVc2VyczpiYWtlcjpEb2N1bWVudHM6UmVmZXJlbmNlczpB
	cmNoaXZlOjIwMDQtRG9saW5za3lOaWVsc2VuIzE5NjJCMy5wZGYAAA4ATAAlADIAMAAwADQALQB
	EAG8AbABpAG4AcwBrAHkATgBpAGUAbABzAGUAbgBNAGMAQwBhAG0AbQBvAG4AQgBhAGsAZQByAC
	4AcABkAGYADwAaAAwATQBhAGMAaQBuAHQAbwBzAGgAIABIAEQAEgBOVXNlcnMvYmFrZXIvRG9jd
	W1lbnRzL1JlZmVyZW5jZXMvQXJjaGl2ZS8yMDA0LURvbGluc2t5TmllbHNlbk1jQ2FtbW9uQmFr
	ZXIucGRmABMAAS8AABUAAgAM//8AANIeHyAhWCRjbGFzc2VzWiRjbGFzc25hbWWjISIjXU5TTXV
	0YWJsZURhdGFWTlNEYXRhWE5TT2JqZWN0XxBOLi4vLi4vLi4vLi4vRG9jdW1lbnRzL1JlZmVyZW
	5jZXMvQXJjaGl2ZS8yMDA0LURvbGluc2t5TmllbHNlbk1jQ2FtbW9uQmFrZXIucGRm0h4fJieiJ
	yNcTlNEaWN0aW9uYXJ5AAgAEQAaAB8AKQAyADcAOgA/AEEAUwBcAGIAaQBwAHgAgwCFAIgAigCM
	AI8AkQCTAJ0AqgCvALcAuQK5Ar4CxwLSAtYC5ALrAvQDRQNKA00AAAAAAAACAQAAAAAAAAAoAAA
	AAAAAAAAAAAAAAAADWg==},
  bdsk-url-1 = {http://dx.doi.org/10.1093/nar/gkh381},
  date-added = {2008-09-17 09:18:08 -0500},
  date-modified = {2008-09-17 09:18:08 -0500},
  keywords = {Software; MolecularDynamics; Electrostatics},
  ty = {JOUR},
  url = {http://dx.doi.org/10.1093/nar/gkh381}
}

@ARTICLE{Dominy:2002,
  author = {Dominy, B. N. and Brooks, C. L.},
  title = {{Identifying native-like protein structures using physics-based potentials.}},
  journal = {J Comput Chem},
  year = {2002},
  volume = {23},
  pages = {147-160},
  number = {1}
}

@ARTICLE{Dominy:1999,
  author = {Dominy, B. N. and Brooks, {III}, C. L.},
  title = {Development of a generalized {Born} model parameterization for proteins
	and nucleic acids},
  journal = {Journal of Physical Chemistry B},
  year = {1999},
  volume = {103},
  pages = {3765-3773},
  number = {18},
  abstract = {The generalized Born model proposed by Still and co-workers (Qui,
	D.; Shenkin, P. S.; Hollinger, F. P.; Still, W. C. J. Phys. Chem.
	A 1997, 101, 3005-3014) is parametrized specifically for proteins,
	peptides, and nucleic acids within the CHARMM all hydrogen and polar
	hydrogen force fields. A database of atomic electrostatic environments
	and molecular electrostatic solvation free energies comprising amino
	acid residues, nucleic acid bases, dipeptides, dinucleotides, proteins,
	and DNA strands is established, and numerical finite difference Poisson
	calculations are solved using atomic radii and charges from the corresponding
	force field parameters. These data provide the necessary input to
	parametrize generalized Born models for a particular force field.
	The performance of these models in reproducing overall molecular
	solvation trends is examined and found to be quite good. Furthermore,
	calculations of electrostatic solvation free energy differences suggest
	that conformational free energy changes are well reproduced. Finally,
	the utilization of this generalized Born model in molecular dynamics
	simulations (both with and without cutoffs) is shown to give excellent
	agreement with explicit solvent simulations of a small 56-residue
	protein in water.},
  address = {Scripps Clin \& Res Inst La Jolla, CA USA 92037 Brooks, CL Dept Mol
	Biol, TPC6,10550 N Torrey Pines Rd Brooks, CL brooks@scripps.edu
	Scripps Clin \& Res Inst La Jolla, CA USA 92037 Dept Mol Biol},
  annote = {Development of a generalized Born model parameterization for proteins
	and nucleic acids; MAY 6},
  bdsk-url-1 = {http://dx.doi.org/10.1021/jp984440c},
  date-added = {2008-09-01 13:59:55 -0500},
  date-modified = {2008-09-01 13:59:55 -0500},
  journal1 = {J Phys Chem B},
  keywords = {Electrostatics; MolecularSimulation},
  ty = {JOUR},
  url = {http://dx.doi.org/10.1021/jp984440c}
}

@ARTICLE{wai94,
  author = {Don, W. S.},
  title = {Numerical study of pseudospectral methods in shock wave applications},
  journal = {J. Comput. Phys},
  year = {1994},
  volume = {110},
  pages = {103-111}
}

@ARTICLE{Don98,
  author = {Don, W. S. and Gottlieb, D.},
  title = {Spectral simulation of supersonic reactive flows},
  journal = {SIAM J. Numer Anal.},
  year = {1998},
  volume = {35},
  pages = {2370--2384}
}

@INPROCEEDINGS{InPreparation,
  author = {Roger D Donaldson and Yiying Tong and Mathieu Desbrun and Houman
	Owhadi},
  title = {Discrete geometric homogenisation},
  booktitle = {in preparation},
  year = {2008}
}

@ARTICLE{Dong:2008MCB,
  author = {Dong, F. and Olsen, B. and Baker, N. A.},
  title = {Computational Methods for Biomolecular Electrostatics},
  journal = {Methods in Cell Biology},
  year = {2008},
  volume = {84},
  pages = {843-70},
  abstract = {An understanding of intermolecular interactions is essential for insight
	into how cells develop, operate, communicate, and control their activities.
	Such interactions include several components: contributions from
	linear, angular, and torsional forces in covalent bonds, {van der
	waals} forces, as well as electrostatics. Among the various components
	of molecular interactions, electrostatics are of special importance
	because of their long range and their influence on polar or charged
	molecules, including water, aqueous ions, and amino or nucleic acids,
	which are some of the primary components of living systems. Electrostatics,
	therefore, play important roles in determining the structure, motion,
	and function of a wide range of biological molecules. This chapter
	presents a brief overview of electrostatic interactions in cellular
	systems, with a particular focus on how computational tools can be
	used to investigate these types of interactions.},
  bdsk-file-1 = {YnBsaXN0MDDUAQIDBAUGCQpYJHZlcnNpb25UJHRvcFkkYXJjaGl2ZXJYJG9iamVjdHMSAAGGoNE
	HCFRyb290gAFfEA9OU0tleWVkQXJjaGl2ZXKoCwwXGBkdJCVVJG51bGzTDQ4PEBEUViRjbGFzc1
	dOUy5rZXlzWk5TLm9iamVjdHOAB6ISE4ACgAOiFRaABIAGWWFsaWFzRGF0YVxyZWxhdGl2ZVBhd
	GjSDRobHFdOUy5kYXRhgAVPEQHKAAAAAAHKAAIAAAxNYWNpbnRvc2ggSEQAAAAAAAAAAAAAAAAA
	AADD4v5NSCsAAAAZYksXMjAwOC1Eb25nT2xzZW5CYWtlci5wZGYAAAAAAAAAAAAAAAAAAAAAAAA
	AAAAAAAAAAAAAAAAAAAAAAAAAAAAAABliqsNMibMAAAAAAAAAAAAEAAQAAAkgAAAAAAAAAAAAAA
	AAAAAAB0FyY2hpdmUAABAACAAAw+NSrQAAABEACAAAw0zQAwAAAAEAFAAZYksAGWIDAAqkKAAKp
	BEAAHrcAAIATU1hY2ludG9zaCBIRDpVc2VyczpiYWtlcjpEb2N1bWVudHM6UmVmZXJlbmNlczpB
	cmNoaXZlOjIwMDgtRG9uZ09sc2VuQmFrZXIucGRmAAAOADAAFwAyADAAMAA4AC0ARABvAG4AZwB
	PAGwAcwBlAG4AQgBhAGsAZQByAC4AcABkAGYADwAaAAwATQBhAGMAaQBuAHQAbwBzAGgAIABIAE
	QAEgBAVXNlcnMvYmFrZXIvRG9jdW1lbnRzL1JlZmVyZW5jZXMvQXJjaGl2ZS8yMDA4LURvbmdPb
	HNlbkJha2VyLnBkZgATAAEvAAAVAAIADP//AADSHh8gIVgkY2xhc3Nlc1okY2xhc3NuYW1loyEi
	I11OU011dGFibGVEYXRhVk5TRGF0YVhOU09iamVjdF8QQC4uLy4uLy4uLy4uL0RvY3VtZW50cy9
	SZWZlcmVuY2VzL0FyY2hpdmUvMjAwOC1Eb25nT2xzZW5CYWtlci5wZGbSHh8mJ6InI1xOU0RpY3
	Rpb25hcnkACAARABoAHwApADIANwA6AD8AQQBTAFwAYgBpAHAAeACDAIUAiACKAIwAjwCRAJMAn
	QCqAK8AtwC5AocCjAKVAqACpAKyArkCwgMFAwoDDQAAAAAAAAIBAAAAAAAAACgAAAAAAAAAAAAA
	AAAAAAMa},
  bdsk-url-1 = {http://dx.doi.org/10.1016/S0091-679X(07)84026-X},
  bdsk-url-2 = {http://dx.doi.org/10.1016/S0091-679X(07)84026-X},
  booktitle = {Methods in Cell Biology},
  date-added = {2008-09-01 14:03:23 -0500},
  date-modified = {2008-09-01 14:04:12 -0500},
  doi = {10.1016/S0091-679X(07)84026-X},
  keywords = {Electrostatics; Solvation},
  url = {http://dx.doi.org/10.1016/S0091-679X(07)84026-X}
}

@ARTICLE{Dong:2003,
  author = {Dong, F. and Vijaykumar, M. and Zhou, H. X.},
  title = {Comparison of Calculation and Experiment Implicates Significant Electrostatic
	Contributions to the Binding Stability of Barnase and Barstar},
  journal = {Biophysical Journal},
  year = {2003},
  volume = {85},
  pages = {49-60},
  number = {1},
  abstract = {The contributions of electrostatic interactions to the binding stability
	of barnase and barstar were studied by the {Poisson-Boltzmann} model
	with three different protocols: a), the dielectric boundary specified
	as the {van der Waals} (vdW) surface of the protein along with a
	protein dielectric constant (p) of 4; b), the dielectric boundary
	specified as the molecular (i.e., solvent-exclusion (SE)) surface
	along with p = 4; and c), {\tt{}"{}}SE + p = 20.{\tt{}"{}} The {\tt{}"{}}vdW
	+ p = 4{\tt{}"{}} and {\tt{}"{}}SE + p = 20{\tt{}"{}} protocols predicted
	an overall electrostatic stabilization whereas the {\tt{}"{}}SE +
	p = 4{\tt{}"{}} protocol predicted an overall electrostatic destabilization.
	The {\tt{}"{}}vdW + p = 4{\tt{}"{}} protocol was most consistent
	with experiment. It quantitatively reproduced the observed effects
	of 17 mutations neutralizing charged residues lining the binding
	interface and the measured coupling energies of six charge pairs
	across the interface and reasonably rationalized the experimental
	ionic strength and pH dependences of the binding constant. In contrast,
	the {\tt{}"{}}SE + p = 4{\tt{}"{}} protocol predicted significantly
	larger coupling energies of charge pairs whereas the {\tt{}"{}}SE
	+ p = 20{\tt{}"{}} protocol did not predict any pH dependence. This
	study calls for further scrutiny of the different {Poisson-Boltzmann}
	protocols and demonstrates potential danger in drawing conclusions
	on electrostatic contributions based on a particular calculation
	protocol.},
  annote = {Comparison of Calculation and Experiment Implicates Significant Electrostatic
	Contributions to the Binding Stability of Barnase and Barstar; *;
	This paper reveals one of PB theory's {\tt{}"{}}dirty little secrets{\tt{}"{}}:
	one can obtain very different results using different discontinuous
	dielectric functions (e.g., {van der Waals} vs. Connolly surfaces).
	Furthermore, the choice of SA apolar coefficients to use also depends
	on the surface definition. This isn't terribly surprising -- nor
	troubling, considering the shift to continuous dielectric functions
	in the PB community -- however, it is a good fact to keep in mind
	when running or analyzing PB calculations.},
  bdsk-url-1 = {http://www.biophysj.org/cgi/content/abstract/85/1/49},
  date-added = {2008-09-16 14:29:58 -0500},
  date-modified = {2008-09-16 14:29:58 -0500},
  keywords = {Electrostatics},
  ty = {JOUR},
  url = {http://www.biophysj.org/cgi/content/abstract/85/1/49}
}

@ARTICLE{Dong:2008PCCP,
  author = {Dong, F. and Wagoner, J. A. and Baker, N. A. },
  title = {Assessing the performance of implicit solvation models at a nucleic
	acid surface},
  journal = {Physical Chemistry Chemical Physics},
  year = {2008},
  volume = {10},
  pages = {4889-902},
  abstract = {Implicit solvation models are popular alternatives to explicit solvent
	methods due to their ability to pre-average solvent behavior and
	thus reduce the need for computationally-expensive sampling. Previously,
	we have demonstrated that Poisson--Boltzmann models for polar solvation
	and integral-based models for nonpolar solvation can reproduce explicit
	solvation forces in a low-charge density protein system. In the present
	work, we examine the ability of these continuum models to describe
	solvation forces at the surface of a RNA hairpin. While these models
	do not completely describe all of the details of solvent behavior
	at this highly-charged biomolecular interface, they do provide a
	reasonable description of average solvation forces and therefore
	show significant promise for developing more robust implicit descriptions
	of solvent around nucleic acid systems for use in biomolecular simulation
	and modeling. Additionally, we observe fairly good transferability
	in the nonpolar model parameters optimized for protein systems, suggesting
	its robustness for modeling general nonpolar solvation phenomena
	in biomolecular systems.},
  bdsk-file-1 = {YnBsaXN0MDDUAQIDBAUGCQpYJHZlcnNpb25UJHRvcFkkYXJjaGl2ZXJYJG9iamVjdHMSAAGGoNE
	HCFRyb290gAFfEA9OU0tleWVkQXJjaGl2ZXKoCwwXGBkdJCVVJG51bGzTDQ4PEBEUViRjbGFzc1
	dOUy5rZXlzWk5TLm9iamVjdHOAB6ISE4ACgAOiFRaABIAGWWFsaWFzRGF0YVxyZWxhdGl2ZVBhd
	GjSDRobHFdOUy5kYXRhgAVPEQHSAAAAAAHSAAIAAAxNYWNpbnRvc2ggSEQAAAAAAAAAAAAAAAAA
	AADD4v5NSCsAAAAZYksZMjAwOC1Eb25nV2Fnb25lckJha2VyLnBkZgAAAAAAAAAAAAAAAAAAAAA
	AAAAAAAAAAAAAAAAAAAAAAAAAAAAAAyOFbsTOz7kAAAAAAAAAAAAEAAQAAAkgAAAAAAAAAAAAAA
	AAAAAAB0FyY2hpdmUAABAACAAAw+NSrQAAABEACAAAxM8WCQAAAAEAFAAZYksAGWIDAAqkKAAKp
	BEAAHrcAAIAT01hY2ludG9zaCBIRDpVc2VyczpiYWtlcjpEb2N1bWVudHM6UmVmZXJlbmNlczpB
	cmNoaXZlOjIwMDgtRG9uZ1dhZ29uZXJCYWtlci5wZGYAAA4ANAAZADIAMAAwADgALQBEAG8AbgB
	nAFcAYQBnAG8AbgBlAHIAQgBhAGsAZQByAC4AcABkAGYADwAaAAwATQBhAGMAaQBuAHQAbwBzAG
	gAIABIAEQAEgBCVXNlcnMvYmFrZXIvRG9jdW1lbnRzL1JlZmVyZW5jZXMvQXJjaGl2ZS8yMDA4L
	URvbmdXYWdvbmVyQmFrZXIucGRmABMAAS8AABUAAgAM//8AANIeHyAhWCRjbGFzc2VzWiRjbGFz
	c25hbWWjISIjXU5TTXV0YWJsZURhdGFWTlNEYXRhWE5TT2JqZWN0XxBCLi4vLi4vLi4vLi4vRG9
	jdW1lbnRzL1JlZmVyZW5jZXMvQXJjaGl2ZS8yMDA4LURvbmdXYWdvbmVyQmFrZXIucGRm0h4fJi
	eiJyNcTlNEaWN0aW9uYXJ5AAgAEQAaAB8AKQAyADcAOgA/AEEAUwBcAGIAaQBwAHgAgwCFAIgAi
	gCMAI8AkQCTAJ0AqgCvALcAuQKPApQCnQKoAqwCugLBAsoDDwMUAxcAAAAAAAACAQAAAAAAAAAo
	AAAAAAAAAAAAAAAAAAADJA==},
  bdsk-url-1 = {http://www.rsc.org/publishing/journals/CP/article.asp?doi=b807384h},
  date-added = {2008-09-01 14:04:17 -0500},
  date-modified = {2008-09-01 14:04:28 -0500},
  keywords = {Electrostatics, Nonpolar, NucleicAcids, Solvation},
  posted-at = {2008-07-08 12:27:15},
  priority = {0},
  url = {http://www.rsc.org/publishing/journals/CP/article.asp?doi=b807384h}
}

@ARTICLE{Dong:2006,
  author = {Dong, F. and Zhou, H. -X.},
  title = {Electrostatic contribution to the binding stability of protein-protein
	complexes},
  journal = {Proteins},
  year = {2006},
  volume = {65},
  pages = {87-102},
  number = {1},
  abstract = {To investigate roles of electrostatic interactions in protein binding
	stability, electrostatic calculations were carried out on a set of
	64 mutations over six protein-protein complexes. These mutations
	alter polar interactions across the interface and were selected for
	putative dominance of electrostatic contributions to the binding
	stability. Three protocols of implementing the {Poisson-Boltzmann}
	model were tested. In vdW4 the dielectric boundary between the protein
	low dielectric and the solvent high dielectric is defined as the
	protein {van der Waals} surface and the protein dielectric constant
	is set to 4. In SE4 and SE20, the dielectric boundary is defined
	as the surface of the protein interior inaccessible to a 1.4-Ãƒ
	solvent probe, and the protein dielectric constant is set to 4 and
	20, respectively. In line with earlier studies on the barnase-barstar
	complex, the vdW4 results on the large set of mutations showed the
	closest agreement with experimental data. The agreement between vdW4
	and experiment supports the contention of dominant electrostatic
	contributions for the mutations, but their differences also suggest
	{van der Waals} and hydrophobic contributions. The results presented
	here will serve as a guide for future refinement in electrostatic
	calculation and inclusion of nonelectrostatic effects.},
  annote = {Electrostatic contribution to the binding stability of protein-protein
	complexes},
  bdsk-url-1 = {http://dx.doi.org/10.1002/prot.21070},
  date-added = {2008-09-16 14:30:35 -0500},
  date-modified = {2008-09-16 14:30:35 -0500},
  keywords = {Electrostatics; Protein-proteinInteractions},
  ty = {JOUR},
  url = {http://dx.doi.org/10.1002/prot.21070}
}

@ARTICLE{spectralQuad,
  author = {Shen Dong and Peer-Timo Bremer and Michael Garland and Valerio Pascucci
	and John C. Hart},
  title = {Spectral surface quadrangulation},
  year = {2006},
  pages = {1057--1066},
  booktitle = {ACM Transactions on Graphics(SIGGRAPH)}
}

@ARTICLE{Dorfi:1987,
  author = {Dorfi, E. A. and Drury, L. O. C.},
  title = {{Simple adaptive grid for 1-D initial value problems}},
  journal = {J. Comput. Phys.},
  year = {1987},
  volume = {69},
  pages = {175--195}
}

@ARTICLE{Doyle:2003,
  author = {Doyle, B. S. and Datta, S. and Doczy, M. and Hareland, S. and Kavalieros,
	B. J. and Linton, T. and Murthy, A. and Rios, R. and Chau, R.},
  title = {{High performance fully-depleted tri-gate CMOS transistors}},
  journal = {IEEE Trans. Electron Devices},
  year = {2003},
  volume = {24},
  pages = {263-265},
  annote = {High performance fully-depleted tri-gate CMOS transistors},
  date-added = {2008-11-25 10:28:56 -0500},
  date-modified = {2008-11-25 10:28:56 -0500},
  ty = {JOUR}
}

@ARTICLE{Dragan,
  author = {Dragan, A.I. and Read, C.M. and Makeyeva, E.N. and Milgotina, E.I.
	and Churchill, M.E.A. and Crane{-}Robinson, C. and Privalov, P.L.
	},
  title = {DNA binding and bending by HMG boxes: Energetic determinants of specificity},
  journal = {J. Mol. Biol.},
  year = {2004},
  volume = {343},
  pages = {371-393}
}

@ARTICLE{Dragan:2004,
  author = {Dragan, Anatoly I. and Read, Christopher M. and Makeyeva, Elena N.
	and Milgotina, Ekaterina I. and Churchill, Mair E. and Crane-Robinson,
	Colyn and Privalov, Peter L. },
  title = {{DNA} Binding and Bending by {HMG} Boxes: Energetic Determinants
	of Specificity},
  journal = {Journal of Molecular Biology},
  year = {2004},
  volume = {343},
  pages = {371--393},
  number = {2},
  abstract = {To clarify the physical basis of DNA binding specificity, the thermodynamic
	properties and DNA binding and bending abilities of the DNA binding
	domains (DBDs) of sequence-specific (SS) and non-sequence-specific
	(NSS) HMG box proteins were studied with various DNA recognition
	sequences using micro-calorimetric and optical methods. Temperature-induced
	unfolding of the free DBDs showed that their structure does not represent
	a single cooperative unit but is subdivided into two (in the case
	of NSS DBDs) or three (in the case of SS DBDs) sub-domains, which
	differ in stability. Both types of HMG box, most particularly SS,
	are partially unfolded even at room temperature but association with
	DNA results in stabilization and cooperation of all the sub-domains.
	Binding and bending measurements using fluorescence spectroscopy
	over a range of ionic strengths, combined with calorimetric data,
	allowed separation of the electrostatic and non-electrostatic components
	of the Gibbs energies of DNA binding, yielding their enthalpic and
	entropic terms and an estimate of their contributions to DNA binding
	and bending. In all cases electrostatic interactions dominate non-electrostatic
	in the association of a DBD with DNA. The main difference between
	SS and NSS complexes is that SS are formed with an enthalpy close
	to zero and a negative heat capacity effect, while NSS are formed
	with a very positive enthalpy and a positive heat capacity effect.
	This indicates that formation of SS HMG box-DNA complexes is specified
	by extensive {van der waals} contacts between apolar groups, i.e.
	a more tightly packed interface forms than in NSS complexes. The
	other principal difference is that DNA bending by the NSS DBDs is
	driven almost entirely by the electrostatic component of the binding
	energy, while DNA bending by SS DBDs is driven mainly by the non-electrostatic
	component. The basic extensions of both categories of HMG box play
	a similar role in DNA binding and bending, making solely electrostatic
	interactions with the DNA.},
  bdsk-url-1 = {http://dx.doi.org/10.1016/j.jmb.2004.08.035},
  date-added = {2008-06-30 09:35:32 -0500},
  date-modified = {2008-06-30 09:35:32 -0500},
  doi = {10.1016/j.jmb.2004.08.035},
  keywords = {electrostatics, protein-nucleic\_acid\_interactions, solvation},
  posted-at = {2008-06-30 15:33:24},
  priority = {0},
  url = {http://dx.doi.org/10.1016/j.jmb.2004.08.035}
}

@ARTICLE{RumpfLSM,
  author = {Droske, M. and Rumpf, M.},
  title = {A Level Set Formulation for Willmore Flow},
  journal = {Interfaces and Free Boundaries},
  year = {2004},
  volume = {6},
  pages = {361--378},
  number = {3},
  abstract = {A level set formulation of Willmore flow is derived using the gradient
	flow perspective. Starting from single embedded surfaces and the
	corresponding gradient flow, the metric is generalized to sets of
	level set surfaces using the identification of normal velocities
	and variations of the level set function in time via the level set
	equation. The approach in particular allows to identify the natural
	dependent quantities of the derived variational formulation. Furthermore,
	spatial and temporal discretization are discussed and some numerical
	simulations are presented.},
  file = {DrRu03b.pdf:http\://numod.ins.uni-bonn.de/research/papers/public/DrRu03b.pdf:PDF}
}

@ARTICLE{Drukker:1998,
  author = {Drukker, K. and de Leeuw, S. H. and Hammes-Schiffer, H.},
  title = {Proton transport along water chains in an electric field},
  journal = {J. Chem. Phys. },
  year = {1998},
  volume = {108},
  pages = {6799  -6808}
}

@ARTICLE{Dryjaa:2007,
  author = { Dryjaa, M and Galvisb, J. and Sarkisb, M.},
  title = {{BDDC methods for discontinuous Galerkin discretization of elliptic
	problems}},
  journal = {Journal of Complexity},
  year = {2007},
  volume = {23},
  pages = {715-739}
}

@ARTICLE{Du:2000,
  author = {Du, Q. and Beglov, D. and Roux, B. },
  title = {Solvation Free Energy of Polar and Nonpolar Molecules in Water: An
	Extended Interaction Site Integral Equation Theory in Three Dimensions},
  journal = {Journal of Physical Chemistry B},
  year = {2000},
  volume = {104},
  pages = {796--805},
  number = {4},
  abstract = {Abstract: The solvation free energy of polar and nonpolar molecules
	in water is examined using the statistical mechanical integral equation
	theory which was recently introduced by Beglov and Roux (J. Phys.
	Chem. 1997, 101, 7821). The integral equation is an extension of
	previous theories based on the reference interaction site model (RISM)
	and the hypernetted chain equation (HNC) to determine the one-dimensional
	site-site radial pair correlation functions. Since the integral equation
	provides the average density of the solvent interaction sites in
	three-dimensional (3d) space around a complex molecular solute of
	arbitrary shape, it is thereby referred to as the 3d-RISM-HNC integral
	equation. In the present paper, the accuracy of the 3d-RISM-HNC integral
	equation is examined by comparing the calculated excess solvation
	free energy at infinite dilution with experimental data for a set
	of nonpolar (n-alkanes) and polar (n-alcohols, n-carboxylic acids,
	and simple amides) molecules. Thermodynamic integration is used to
	calculate the excess solvation free energy on the basis of the average
	site densities obtained by the 3d-RISM-HNC equation. Two extensions
	were made to improve the accuracy of the integral equation. First,
	the susceptibility of pure liquid water (an input for calculating
	the excess solvation free energy of molecules in the infinite dilution
	limit) was obtained by combining information from a molecular dynamics
	simulation with the RISM-HNC integral equation. Second, empirical
	water hydrogen and water oxygen bridge functions were introduced
	and optimized for improving the accuracy of the theory. The calculated
	solvation free energies are in good accord with experimental data,
	although further work will be required for quantitatively accurate
	results. These preliminary results indicate that the 3d-RISM-HNC
	equation with well-calibrated optimized bridge functions is a promising
	approach for calculating the hydration free energy of complex molecules.},
  address = {Centre de Recherche en Calcul Appliqu\'{e} (CERCA), D\'{e}partements
	de physique et de chimie, Universit\'{e} de Montr\'{e}al, C.P. 6128,
	succ. Centre-Ville, Montreal, Quebec, Canada H3C 3J7},
  bdsk-url-1 = {http://dx.doi.org/10.1021/jp992712l},
  date-added = {2008-06-30 06:38:32 -0500},
  date-modified = {2008-06-30 06:38:32 -0500},
  doi = {10.1021/jp992712l},
  keywords = {solvation, statistical\_mechanics},
  posted-at = {2008-06-30 12:37:45},
  priority = {0},
  url = {http://dx.doi.org/10.1021/jp992712l}
}

@ARTICLE{Du-phase:2004,
  author = {Du, Q. and Liu, C. and Wang, X. Q.},
  title = {A phase field approach in the numerical study of the elastic bending
	energy for vesicle membranes},
  journal = {J. Comput. Phys.},
  year = {2004},
  volume = {198},
  pages = {450-468},
  annote = {A phase field approach in the numerical study of the elastic bending
	energy for vesicle membranes},
  date-added = {2008-09-19 10:28:56 -0500},
  date-modified = {2008-09-19 10:28:56 -0500},
  ty = {JOUR}
}

@ARTICLE{Du:2005,
  author = {Du, Yan and Bock, Barbara C. and Schachter, Karen A. and Chao, Mary
	and Gallo, Kathleen A. },
  title = {Cdc42 Induces Activation Loop Phosphorylation and Membrane Targeting
	of Mixed Lineage Kinase 3},
  journal = {Journal of Biological Chemistry},
  year = {2005},
  volume = {280},
  pages = {42984--42993},
  number = {52},
  abstract = {Mixed lineage kinase 3 (MLK3) functions as a mitogen-activated protein
	kinase kinase kinase to activate multiple mitogen-activated protein
	kinase pathways. Our current studies demonstrate that lack of MLK3
	blocks signaling of activated Cdc42 to c-Jun N-terminal kinase, giving
	strong support for the idea that Cdc42 is a physiological activator
	of MLK3. We show herein that Cdc42, in a prenylation-dependent manner,
	targets MLK3 from a perinuclear region to membranes, including the
	plasma membrane. Cdc42-induced membrane targeting of MLK3 is independent
	of MLK3 catalytic activity but depends upon an intact Cdc42/Rac-interactive
	binding motif, consistent with MLK3 membrane translocation being
	mediated through direct binding of Cdc42. Phosphorylation of the
	activation loop of MLK3 requires MLK3 catalytic activity and is induced
	by Cdc42 in a prenylation-independent manner, arguing that Cdc42
	binding is sufficient for activation loop autophosphorylation of
	MLK3. However, membrane targeting is necessary for full activation
	of MLK3 and maximal signaling to JNK. We previously reported that
	MLK3 is autoinhibited through an interaction between its N-terminal
	SH3 domain and a proline-containing sequence found between the leucine
	zipper and the CRIB motif of MLK3. Thus we propose a model in which
	GTP-bound Cdc42/Rac binds MLK3 and disrupts SH3-mediated autoinhibition
	leading to dimerization and activation loop autophosphorylation.
	Targeting of this partially active MLK3 to membranes likely results
	in additional phosphorylation events that fully activate MLK3 and
	its ability to maximally signal through the JNK pathway. 10.1074/jbc.M502671200},
  bdsk-url-1 = {http://dx.doi.org/10.1074/jbc.M502671200},
  date-added = {2008-06-30 21:57:28 -0400},
  date-modified = {2008-06-30 21:57:28 -0400},
  doi = {10.1074/jbc.M502671200},
  keywords = {misc},
  posted-at = {2008-07-01 02:56:56},
  priority = {0},
  url = {http://dx.doi.org/10.1074/jbc.M502671200}
}

@ARTICLE{Duan:2001,
  author = {Duan, X. F. and Huang, Y. and Ciu, Y. and Wang, J. F. and Lieber,
	C. M.},
  title = {Indium phosphide nanowires as building blocks for nanoscale electronic
	and optoelectronics devices},
  journal = {Nature},
  year = {2001},
  volume = {409},
  pages = {66-69},
  annote = {Indium phosphide nanowires as building blocks for nanoscale electronic
	and optoelectronics devices},
  date-added = {2008-11-25 10:28:56 -0500},
  date-modified = {2008-11-25 10:28:56 -0500},
  ty = {JOUR}
}

@ARTICLE{Duan:1998,
  author = {Duan, Y. and Kollman, P. A.},
  title = {{Pathways to a protein folding intermediate observed in a 1-microsecond
	simulation in aqueous solution}},
  journal = {Science},
  year = {1998},
  volume = {282},
  pages = {740-744},
  number = {5389}
}

@ARTICLE{Duffy:1999,
  author = {Duffy, D. C. and Gillis, H. L. and Lin, J. and Sheppard, N. F. and
	Kellogg, G. J.},
  title = {Microfabricated centrifugal microfluidic systems: Characterization
	and multiple enzymatic assay},
  journal = {Analytical Chemistry },
  year = {1999},
  volume = {71},
  pages = {5206-5212}
}

@ARTICLE{Dumett:2003,
  author = {Miguel A. Dumett and James P. Keener},
  title = {An Immersed Interface Method for Solving Anisotropic Elliptic Boundary
	Value Problems in Three Dimensions},
  journal = {SIAM Journal on Scientific Computing},
  year = {2003},
  volume = {25},
  pages = {348-367},
  number = {1},
  abstract = {We have developed a first-order stable {Cartesian grid} discretization
	that uses only interior grid points for inhomogeneous anisotropic
	elliptic operators subject to Neumann boundary conditions on a bounded
	nonrectangular geometry in three dimensions. For this discretization
	method, a necessary and sufficient condition depending on the mesh
	size h for the existence of this first-order stable scheme at a regular
	(i.e., interior) grid point is found in terms of the anisotropy matrix.
	For this discretization method, a way to analyze the existence of
	a first-order stable scheme at an irregular (i.e., boundary) grid
	point is also given. The arguments are identical to those for the
	two-dimensional case [M. A. Dumett and J. P. Keener, A Numerical
	Method for Solving Anisotropic Elliptic Boundary Value Problems on
	an Irregular Domain in 2D, manuscript]; only the details change.
	Unlike in [M. A. Dumett and J. P. Keener, A Numerical Method for
	Solving Anisotropic Elliptic Boundary Value Problems on an Irregular
	Domain in 2D, manuscript], a discussion of {Dirichlet} and {Robin}
	boundary conditions is also included. In particular, it is shown
	that the Gerschgorin condition does not impose sign restrictions
	on irregular grid points stencil coefficients as in the Neumann case.},
  bdsk-url-1 = {http://link.aip.org/link/?SCE/25/348/1},
  bdsk-url-2 = {http://dx.doi.org/10.1137/S106482750240697X},
  date-added = {2008-09-14 15:32:12 -0500},
  date-modified = {2008-09-14 15:32:12 -0500},
  doi = {10.1137/S106482750240697X},
  keywords = {Mathematics},
  publisher = {SIAM},
  url = {http://link.aip.org/link/?SCE/25/348/1}
}

@ARTICLE{Dunbrack:1997,
  author = {Dunbrack, R. L. Jr. and Cohen, F. E.},
  title = {{Bayesian statistical analysis of protein side-chain rotamer preferences}},
  journal = {Protein Sci},
  year = {1997},
  volume = {6},
  pages = {1661-1681},
  number = {8}
}

@ARTICLE{Duncan:2005,
  author = {Duncan, A. and Sedgewick, R. D. and Coalson, R. D. },
  title = {{Improved local lattice approach for Coulombic simulations}},
  journal = {Phys Rev E Stat Nonlin Soft Matter Phys},
  year = {2005},
  volume = {71},
  pages = {046702}
}

@ARTICLE{Dunker:1978,
  author = {Dunker, AK and Marvin, DA },
  title = {A model for membrane transport through $\alpha$-helical protein pores},
  journal = {J Theor Biol},
  year = {1978},
  volume = {72},
  pages = {9-16}
}

@ARTICLE{Dutta:2005,
  author = { Dutta, S. and Berman, H. M.},
  title = {Large macromolecular complexes in the Protein Data Bank: a status
	report},
  journal = {Structure},
  year = {2005},
  volume = {13},
  pages = {381 - 388},
  annote = {Large macromolecular complexes in the Protein Data Bank: a status
	report},
  date-added = {2009-03-10 },
  date-modified = {2009-03-10},
  ty = {JOUR}
}

@ARTICLE{Dvinsky:1991,
  author = {Dvinsky, A. S.},
  title = {{Adaptive grid generation from harmonic maps on Riemannian manifolds}},
  journal = {J. Comput. Phys.},
  year = {1991},
  volume = {95},
  pages = {450--476}
}

@BOOK{Deamer:1982,
  title = {Proton permeability in biological and model membranes. In: Intracellular
	pH: Its Measurement, Regulation, and Utilization in Cellular Functions},
  publisher = {New York: Liss},
  year = {1982},
  author = {Deamer DW},
  address = { },
  date-added = { },
  date-modified = { },
  keywords = { }
}

@MISC{MOF,
  author = {V. Dyadechko and M. Shashkov},
  title = {{Moment-of-Fluid Interface Reconstruction}},
  howpublished = {LANL Technical Report LA-UR-05-7571},
  year = {2006}
}

@ARTICLE{Dyrka:2008,
  author = {Dyrka, Witold and Augousti, Andy T. and Kotulska, Malgorzata },
  title = {Ion Flux Through Membrane Channels: An Enhanced Algorithm for the
	{Poisson-Nernst-Planck} Model},
  journal = {J. Comput Chem},
  year = {2008},
  volume = {29},
  pages = {1876-1888}
}

@ARTICLE{Dziuk,
  author = {Gerhard Dziuk and Ernst Kuwert and Reiner Schatzle},
  title = {Evolution of Elastic Curves in $\mathbb{R}^n$: Existence and Computation},
  journal = {SIAM J. Math. Anal.},
  year = {2002},
  volume = {33},
  pages = {1228--1245},
  number = {5}
}

@ARTICLE{Dzubiella:2006,
  author = {Dzubiella, J. and Swanson, J. M. J. and McCammon, J. A.},
  title = {Coupling Hydrophobicity, Dispersion, and Electrostatics in Continuum
	Solvent Models},
  journal = {Physical Review Letters},
  year = {2006},
  volume = {96},
  pages = {087802},
  abstract = {An implicit solvent model is presented that couples hydrophobic, dispersion,
	and electrostatic solvation energies by minimizing the system Gibbs
	free energy with respect to the solvent volume exclusion function.
	The solvent accessible surface is the output of the theory. The method
	is illustrated with the solvation of simple solutes on different
	length scales and captures the sensitivity of hydration to the particular
	form of the solute-solvent interactions in agreement with recent
	computer simulations.},
  annote = {Coupling Hydrophobicity, Dispersion, and Electrostatics in Continuum
	Solvent Models},
  bdsk-url-1 = {http://dx.doi.org/10.1103/PhysRevLett.96.087802},
  date-added = {2008-09-03 13:25:19 -0500},
  date-modified = {2008-09-03 13:25:19 -0500},
  keywords = {Solvation; Electrostatics; StatisticalMechanics},
  ty = {JOUR},
  url = {http://dx.doi.org/10.1103/PhysRevLett.96.087802}
}

@ARTICLE{Dzubiella:2006a,
  author = {Dzubiella, J. and Swanson, J. M. J. and McCammon, J. A.},
  title = {Coupling nonpolar and polar solvation free energies in implicit solvent
	models},
  journal = {Journal of Chemical Physics},
  year = {2006},
  volume = {124},
  pages = {084905},
  abstract = {Recent studies on the solvation of atomistic and nanoscale solutes
	indicate that a strong coupling exists between the hydrophobic, dispersion,
	and electrostatic contributions to the solvation free energy, a facet
	not considered in current implicit solvent models. We suggest a theoretical
	formalism which accounts for coupling by minimizing the Gibbs free
	energy of the solvent with respect to a solvent volume exclusion
	function. The resulting differential equation is similar to the Laplace-Young
	equation for the geometrical description of capillary interfaces
	but is extended to microscopic scales by explicitly considering curvature
	corrections as well as dispersion and electrostatic contributions.
	Unlike existing implicit solvent approaches, the solvent accessible
	surface is an output of our model. The presented formalism is illustrated
	on spherically or cylindrically symmetrical systems of neutral or
	charged solutes on different length scales. The results are in agreement
	with computer simulations and, most importantly, demonstrate that
	our method captures the strong sensitivity of solvent expulsion and
	dewetting to the particular form of the solvent-solute interactions.},
  annote = {Coupling nonpolar and polar solvation free energies in implicit solvent
	models},
  bdsk-file-1 = {YnBsaXN0MDDUAQIDBAUGCQpYJHZlcnNpb25UJHRvcFkkYXJjaGl2ZXJYJG9iamVjdHMSAAGGoNE
	HCFRyb290gAFfEA9OU0tleWVkQXJjaGl2ZXKoCwwXGBkdJCVVJG51bGzTDQ4PEBEUViRjbGFzc1
	dOUy5rZXlzWk5TLm9iamVjdHOAB6ISE4ACgAOiFRaABIAGWWFsaWFzRGF0YVxyZWxhdGl2ZVBhd
	GjSDRobHFdOUy5kYXRhgAVPEQHwAAAAAAHwAAIAAAxNYWNpbnRvc2ggSEQAAAAAAAAAAAAAAAAA
	AADD4v5NSCsAAAAZYksfMjAwNi1EenViaWVsbGFTd2FucyMxQUJCREZBLnBkZgAAAAAAAAAAAAA
	AAAAAAAAAAAAAAAAAAAAAAAAAAAAAAau9+sSX0toAAAAAAAAAAAAEAAQAAAkgAAAAAAAAAAAAAA
	AAAAAAB0FyY2hpdmUAABAACAAAw+NSrQAAABEACAAAxJgZKgAAAAEAFAAZYksAGWIDAAqkKAAKp
	BEAAHrcAAIAVU1hY2ludG9zaCBIRDpVc2VyczpiYWtlcjpEb2N1bWVudHM6UmVmZXJlbmNlczpB
	cmNoaXZlOjIwMDYtRHp1YmllbGxhU3dhbnMjMUFCQkRGQS5wZGYAAA4ARAAhADIAMAAwADYALQB
	EAHoAdQBiAGkAZQBsAGwAYQBTAHcAYQBuAHMAbwBuAE0AYwBDAGEAbQBtAG8AbgAuAHAAZABmAA
	8AGgAMAE0AYQBjAGkAbgB0AG8AcwBoACAASABEABIASlVzZXJzL2Jha2VyL0RvY3VtZW50cy9SZ
	WZlcmVuY2VzL0FyY2hpdmUvMjAwNi1EenViaWVsbGFTd2Fuc29uTWNDYW1tb24ucGRmABMAAS8A
	ABUAAgAM//8AANIeHyAhWCRjbGFzc2VzWiRjbGFzc25hbWWjISIjXU5TTXV0YWJsZURhdGFWTlN
	EYXRhWE5TT2JqZWN0XxBKLi4vLi4vLi4vLi4vRG9jdW1lbnRzL1JlZmVyZW5jZXMvQXJjaGl2ZS
	8yMDA2LUR6dWJpZWxsYVN3YW5zb25NY0NhbW1vbi5wZGbSHh8mJ6InI1xOU0RpY3Rpb25hcnkAC
	AARABoAHwApADIANwA6AD8AQQBTAFwAYgBpAHAAeACDAIUAiACKAIwAjwCRAJMAnQCqAK8AtwC5
	Aq0CsgK7AsYCygLYAt8C6AM1AzoDPQAAAAAAAAIBAAAAAAAAACgAAAAAAAAAAAAAAAAAAANK},
  bdsk-url-1 = {http://link.aip.org/link/?JCPSA6/124/084905/1},
  date-added = {2008-08-28 09:43:49 -0500},
  date-modified = {2008-08-28 09:43:49 -0500},
  doi = {10.1063/1.2171192},
  keywords = {Solvation; Electrostatics},
  ty = {JOUR},
  url = {http://link.aip.org/link/?JCPSA6/124/084905/1}
}

@ARTICLE{W.E:2007,
  author = {E, W. N. and Engquist, B. and Li, X. and Ren, W. and Vanden-Eijnden,
	E.},
  title = {Heterogeneous multiscale methods: A review},
  journal = {Commun. Comput. Phys. },
  year = {2007},
  volume = {2},
  pages = {367 -450}
}

@INPROCEEDINGS{EDK06,
  author = { Eckstein, Ilya and  Desbrun,  Mathieuand  Kuo, C. C. Jay},
  title = {Compression of Time Varying Isosurfaces},
  booktitle = {Graphics Interface},
  year = {2006},
  pages = {99--105},
  month = Jul
}

@INPROCEEDINGS{EPTKD07,
  author = {Ilya Eckstein and Jean-Philippe Pons and Yiying Tong and C.C. Jay
	Kuo and Mathieu Desbrun},
  title = {Generalized Surface Flows for Mesh Processing},
  booktitle = {Symposium on Geometry Processing},
  year = {2007},
  pages = {183--192},
  month = Jul
}

@ARTICLE{Edelman1988,
  author = {Edelman, PaulH and Saks, MichaelE},
  title = {{Combinatorial representation and convex dimension of convex geometries}},
  journal = {Order A Journal On The Theory Of Ordered Sets And Its Applications},
  year = {1988},
  volume = {5},
  pages = {23--32},
  number = {1},
  doi = {10.1007/BF00143895},
  issn = {01678094},
  keywords = {1,a representation theory,convex,convex dimension,convex geometries,introduction
	notation,lattices,meet distributive,paper develop,purpose},
  owner = {doubletony},
  timestamp = {2012.04.26},
  url = {http://www.springerlink.com/index/10.1007/BF00143895}
}

@TECHREPORT{Alpha,
  author = {Herbert Edelsbrunner},
  title = {Weighted alpha shapes},
  year = {1992},
  address = {Champaign, IL, USA},
  publisher = {University of Illinois at Urbana-Champaign},
  source = {http://www.ncstrl.org:8900/ncstrl/servlet/search?formname=detail\&id=oai%3Ancstrlh%3Auiuc_cs%3Ancstrl.uiuc_cs%2F%2FUIUCDCS-R-92-1760}
}


@INPROCEEDINGS{AlphaOld,
  author = {Herbert Edelsbrunner and Ernst P. M\"{u}cke},
  title = {Three-dimensional alpha shapes},
  booktitle = {VVS '92: Proceedings of the 1992 workshop on Volume visualization},
  year = {1992},
  pages = {75--82},
  address = {New York, NY, USA},
  publisher = {ACM},
  doi = {http://doi.acm.org/10.1145/147130.147153},
  isbn = {0-89791-527-5},
  location = {Boston, Massachusetts, United States}
}

@ARTICLE{Edinger:1997,
  author = {Edinger, S. R. and Cortis, C. and Shenkin, P. S. and Friesner, R.
	A. },
  title = {Solvation Free Energies of Peptides: Comparison of Approximate Continuum
	Solvation Models with Accurate Solution of the {{Poisson-Boltzmann}}
	Equation},
  journal = {Journal of Physical Chemistry B},
  year = {1997},
  volume = {101},
  pages = {1190--1197},
  number = {7},
  abstract = {Abstract: We have compared solvation free energies obtained from a
	number of approximate solvation models with an accurate solution
	of the {Poisson-Boltzmann} equation for a large data set of peptide
	structures, ranging from a single amino acid to a peptide sequence
	of length nine. The models are assessed for their ability to predict
	relative energetics of different peptide conformations (of the same
	sequence) as determined from the {Poisson-Boltzmann} results. We
	find that the widely used distance dependent dielectric model yields
	qualitatively erroneous results; in contrast, the generalized Born
	model of Still and co-workers, an approximation to the {Poisson-Boltzmann}
	equation, provides reasonably good solvation free energies and performs
	rather well in rank ordering of conformations. A surface area based
	model produces results of intermediate quality. Our results suggest
	that the generalized Born model is presently the clearly preferred
	alternative if one wishes to carry out molecular dynamics simulations
	with a fast, approximate solvation model.},
  address = {Department of Chemistry and Center for Biomolecular Simulation, Columbia
	University, New York, New York 10027, and Department of Biochemistry
	and Molecular Biophysics and Center for Biomolecular Simulation,
	Columbia University, 630 West 168th Street, New York, New York 10032},
  bdsk-url-1 = {http://dx.doi.org/10.1021/jp962156k},
  date-added = {2008-06-29 15:21:42 -0500},
  date-modified = {2008-06-29 15:21:42 -0500},
  doi = {10.1021/jp962156k},
  keywords = {electrostatics, solvation},
  posted-at = {2008-06-29 21:20:51},
  priority = {0},
  url = {http://dx.doi.org/10.1021/jp962156k}
}

@ARTICLE{Edmonds1960abs,
  author = {Edmonds, J.},
  title = {{A Combinatorial Representation of Polyhedral Surfaces (Abstract)}},
  journal = {Notices of the American Mathematical Society},
  year = {1960},
  volume = {7},
  citeulike-article-id = {381506},
  comment = {This is an abstract for the seminar on the topic. There is no publication
	otherwise available for the description of graph rotation systems
	by Edmonds.},
  keywords = {polygon\_meshes, vv},
  posted-at = {2005-11-05 09:05:59},
  priority = {0}
}

@ARTICLE{Edmonds1960,
  author = {Edmonds, J R},
  title = {{A combinatorial representation for polyhedral surfaces}},
  journal = {Notices Amer Math Soc},
  year = {1960},
  volume = {7},
  pages = {646},
  owner = {doubletony},
  timestamp = {2012.04.26}
}

@ARTICLE{Edwards:2002,
  author = {Edwards, Scott and Corry, Ben and Kuyucak, Serdar and Chung, Shin-Ho},
  title = {Continuum Electrostatics Fails to Describe Ion Permeation in the
	{Gramicidin} Channel},
  journal = {Biophysical Journal},
  year = {2002},
  volume = {83},
  pages = {1348-1360},
  month = {September}
}

@ARTICLE{Egwolf:2004,
  author = {Egwolf, B. and Tavan, P.},
  title = {Continuum description of ionic and dielectric shielding for molecular-dynamics
	simulations of proteins in solution},
  journal = {Journal of Chemical Physics},
  year = {2004},
  volume = {120},
  pages = {2056-2068},
  number = {4},
  abstract = {We extend our continuum description of solvent dielectrics in molecular-dynamics
	(MD) simulations {$[$}B. Egwolf and P. Tavan, J. Chem. Phys. 118,
	2039 (2003){$]$}, which has provided an efficient and accurate solution
	of the Poisson equation, to ionic solvents as described by the linearized
	PoissonÃ¢Â€Â“Boltzmann (LPB) equation. We start with the
	formulation of a general theory for the electrostatics of an arbitrarily
	shaped molecular system, which consists of partially charged atoms
	and is embedded in a LPB continuum. This theory represents the reaction
	field induced by the continuum in terms of charge and dipole densities
	localized within the molecular system. Because these densities cannot
	be calculated analytically for systems of arbitrary shape, we introduce
	an atom-based discretization and a set of carefully designed approximations.
	This allows us to represent the densities by charges and dipoles
	located at the atoms. Coupled systems of linear equations determine
	these multipoles and can be rapidly solved by iteration during a
	MD simulation. The multipoles yield the reaction field forces and
	energies. Finally, we scrutinize the quality of our approach by comparisons
	with an analytical solution restricted to perfectly spherical systems
	and with results of a finite difference method},
  annote = {Continuum description of ionic and dielectric shielding for molecular-dynamics
	simulations of proteins in solution; *; The extension of a novel
	approach for approximating the solution to the Poisson or PB equations
	using atom-centered inducible dipoles.},
  bdsk-url-1 = {http://dx.doi.org/10.1063/1.1636154},
  date-added = {2008-06-29 08:38:13 -0500},
  date-modified = {2008-06-29 08:38:13 -0500},
  keywords = {Electrostatics},
  ty = {JOUR},
  url = {http://dx.doi.org/10.1063/1.1636154}
}

@ARTICLE{Eisenberg:2010c,
  author = {Eisenberg, B. S.},
  title = {{Crowded Charges in Ion Channels}},
  journal = {Advances in Chemical Physics},
  year = {2010},
  volume = {in the press}
}

@ARTICLE{Eisenberg:2003,
  author = {Eisenberg, B. S.},
  title = {Ion Channels as Devices},
  journal = {Journal of Computational Electronics},
  year = {2003},
  volume = {2},
  pages = {245-249},
  month = { }
}

@ARTICLE{Eisenberg:1996,
  author = {Eisenberg, B. S.},
  title = {Computing the field in proteins and channels},
  journal = {J. Membrane Biol.},
  year = {1996},
  volume = {150},
  pages = {1-25}
}

@ARTICLE{Eisenberg:1993,
  author = {Eisenberg, B. S. and Chen, D},
  title = {{Poisson-Nernst-Planck (PNP) theory of an open ionic channel}},
  journal = {Biophysical Journal},
  year = {1993},
  volume = {64},
  pages = {A22}
}

@ARTICLE{Eisenberg:2010,
  author = {Eisenberg, B. S. and Hyon, Yun Kyong and Liu, Chun },
  title = {{Energy variational analysis of ions in water and channels: Field
	theory for primitive models of complex ionic fluids}},
  journal = {Journal of Chemical Physics},
  year = {2010},
  volume = {133},
  pages = {104104}
}

@ARTICLE{Eisenberg:2006,
  author = {Eisenberg, B. S. and Liu, W. S. },
  title = {{Poisson-Nernst-Planck} systems for ion channels with permanent charges},
  journal = {SIAM Journal on Applied Dynamical Systems},
  year = {2006},
  volume = {38},
  pages = {1932-1966},
  number = { 6}
}

@ARTICLE{Eisenhaber,
  author = {Eisenhaber, F. and Argos, P. },
  title = {Improved strategy in analytic surface calculation for molecular systems:
	Handling of singularities and computational efficiency},
  journal = {J. Comput. Chem.},
  year = {1993},
  volume = {14},
  pages = {1272-1280}
}

@ARTICLE{Eisenhaber:1993,
  author = {Eisenhaber, F. and Argos, P.},
  title = {Improved strategy in analytic surface calculation for molecular systems:
	Handling of singularities and computational efficiency},
  journal = {J. Comput. Chem.},
  year = {1993},
  volume = {14},
  pages = {1272-1280}
}

@ARTICLE{Eisenman:1987,
  author = {Eisenman, G. and Dani, J. A. },
  title = {An Introduction to Molecular Architecture and Permeability of Ion
	Channels},
  journal = {Annual Review of Biophysics and Biophysical Chemistry},
  year = {1987},
  volume = {16},
  pages = {205-226}
}

@ARTICLE{Eisenman:1980,
  author = {Eisenman, G. and Enos, B. and Hagglund, J. and Sandbloom, J},
  title = {Gramicidin as an example of a single-filing ion channel},
  journal = {Ann. N.Y. Acad. Sci.},
  year = {1980},
  volume = {339},
  pages = {8-20}
}

@ARTICLE{elad2003bis,
  author = {Elad, A. and Kimmel, R.},
  title = {{On bending invariant signatures for surfaces}},
  journal = {IEEE Trans. on PAMI},
  year = {2003},
  volume = {25},
  pages = {1285--1295},
  number = {10}
}

@ARTICLE{Elcock:1999,
  author = {Elcock, A. H. and Gabdoulline, R. R. and Wade, R. C. and McCammon,
	J. A.},
  title = {Computer simulation of protein-protein association kinetics: Acetylcholinesterase-fasciculin},
  journal = {Journal of Molecular Biology},
  year = {1999},
  volume = {291},
  pages = {149-162},
  number = {1},
  abstract = {Computer simulations were performed to investigate the role of electrostatic
	interactions in promoting fast association of acetylcholinesterase
	with its peptidic inhibitor, the neurotoxin fasciculin. The encounter
	of the two macromolecules was simulated with the technique of Brownian
	dynamics (BD), using atomically detailed structures, and association
	rate constants were calculated for the wild-type and a number of
	mutant proteins. In a first set of simulations, the ordering of the
	experimental rate constants for the mutant proteins was correctly
	reproduced, although the absolute values of the rate constants were
	overestimated by a factor of around 30. Rigorous calculations of
	the full electrostatic interaction energy between the two proteins
	indicate that this overestimation of association rates results at
	least in part from approximations made in the description of interaction
	energetics in the BD simulations. In particular, the initial BD simulations
	neglect the unfavourable electrostatic desolvation effects that result
	from the exclusion of high dielectric solvent that accompanies the
	approach of the two low dielectric proteins. This electrostatic desolvation
	component is so large that the overall contribution of electrostatics
	to the binding energy of the complex is unlikely to be strongly favourable.
	Nevertheless, electrostatic interactions are still responsible for
	increased association rates, because even if they are unfavourable
	in the fully formed complex, they are still favourable at intermediate
	protein-protein separation distances. It therefore appears possible
	for electrostatic interactions to promote the kinetics of binding
	even if they do not make a strongly favourable contribution to the
	thermodynamics of binding. When an approximate description of these
	electrostatic desolvation effects is included in a second set of
	BD simulations, the relative ordering of the mutant proteins is again
	correctly reproduced, but now association rate constants that are
	much closer in magnitude to the experimental values are obtained.
	Inclusion of electrostatic desolvation effects also improves reproduction
	of the experimental ionic strength dependence of the wild-type association
	rate.},
  address = {Univ Calif San Diego La Jolla, CA USA 92093 Elcock, AH aelcock{\char64}chemcca10.ucsd.edu
	Dept Chem \& Biochem Univ Calif San Diego La Jolla, CA USA 92093
	Dept Chem \& Biochem Univ Calif San Diego La Jolla, CA USA 92093
	Dept Pharmacol European Mol Biol Lab Heidelberg Germany D-69117},
  annote = {Computer simulation of protein-protein association kinetics: Acetylcholinesterase-fasciculin;
	AUG 6},
  bdsk-url-1 = {http://dx.doi.org/10.1006/jmbi.1999.2919},
  date-added = {2008-09-01 13:55:21 -0500},
  date-modified = {2008-09-01 13:55:21 -0500},
  journal1 = {J Mol Biol},
  keywords = {Acetylcholinesterase; NerveAgents; Diffusion; Electrostatics},
  read = {Yes},
  ty = {JOUR},
  url = {http://dx.doi.org/10.1006/jmbi.1999.2919}
}

@ARTICLE{McCammon:1997,
  author = {Elcock, A. H. and McCammon, J. A. },
  title = {A continuum solvation model for studying protein hydration thermodynamics
	at high temperatures},
  journal = {J. Phys. Chem. B},
  year = {1997},
  volume = {101},
  pages = {9624-9634}
}

@ARTICLE{ETKSD07,
  author = {Sharif Elcott and Yiying Tong and Eva Kanso and Peter Schr{\"o}der
	and Mathieu Desbrun},
  title = {Stable, Circulation-Preserving, Simplicial Fluids},
  journal = {ACM Trans. on Graphics},
  year = {2007},
  volume = {26},
  pages = {4},
  number = {1},
  month = jan
}

@ARTICLE{MEAD,
  author = {Engels, M. and Gerwert, K. and Bashford, D.},
  title = {Computational studies on bacteriorhodopsin: Conformation and proton
	transfer energetics},
  journal = {Biophys. Chem.},
  year = {1995},
  volume = {56},
  pages = {95}
}

@ARTICLE{EngquistOsher,
  author = {Bjorn Engquist and Stanley Osher},
  title = {{One-Sided Difference Schemes and Transonic Flow}},
  journal = {PNAS},
  year = {1980},
  volume = {77},
  pages = {3071--3074},
  number = {6}
}

@ARTICLE{Enkvist00325,
  author = {Enkvist, C. and Zhang, Y. K. and Yang, W. T.},
  title = {Density functional study of a weakly hydrogen-bonded benzene-ammonia
	complex: The importance of the exchange functional},
  journal = {International Journal of Quantum Chemistry},
  year = {2000},
  volume = {79},
  pages = {325-329},
  number = {5},
  month = {Sep},
  abstract = {Density functional theory calculations on the benzene-ammonia complex
	have been performed. The benzene-ammonia complex is weakly hydrogen
	bonded, and crucial for obtaining good agreement with experimental
	results is the choice of the exchange functional used, as in the
	case of van der Waals interactions. It is found that the behavior
	of the exchange functional in the region where the density is small
	and the density gradient large plays an important role in describing
	the weak hydrogen-bonding interaction. Calculations show that generalized
	gradient approximation functionals, which behave properly in this
	region, have achieved an accuracy similar to the second-order Moller-Plesset
	(MP2) method for the benzene-ammonia complex. (C) 2000 John Wiley
	& Sons, Inc.},
  endnotereftype = {Journal Article},
  issn = {0020-7608},
  shorttitle = {Density functional study of a weakly hydrogen-bonded benzene-ammonia
	complex: The importance of the exchange functional},
  url = {<Go to ISI>://000088848700006}
}

@ARTICLE{PLSM,
  author = {D. Enright and R. Fedkiw, J. Ferziger and I. Mitchell},
  title = {{A Hybrid Particle Level Set Method for Improved Interface Capturing}},
  journal = {J. Computational Physics},
  year = {2002},
  volume = {183},
  pages = {83-116}
}

@ARTICLE{Erickson:2006,
  author = {Erickson, D. and Rockwood, T. and Emery, T. and Scherer, A. and Psaltis,
	D. },
  title = {Nanofluidic tuning of photonic crystal circuits },
  journal = {Optical Letters },
  year = {2006},
  volume = {31},
  pages = { 59-61 },
  number = { }
}

@ARTICLE{Evans:1992,
  author = {Evans, L. C. and Soner, H. M. and Souganidis, P. E.},
  title = {Phase transitions and generalized motion by mean curvature},
  journal = {Comm. Pure Appl. Math.},
  year = {1992},
  volume = {45},
  pages = {1097-1123},
  annote = {Phase transitions and generalized motion by mean curvature},
  date-added = {2008-09-19 10:28:56 -0500},
  date-modified = {2008-09-19 10:28:56 -0500},
  ty = {JOUR}
}

@ARTICLE{Evans:1991,
  author = {Evans, L. C. and Spruck, J.},
  title = {Motion of level sets by mean curvature},
  journal = {J. Diff. Geom.},
  year = {1991},
  volume = {33},
  pages = {635-681},
  annote = {Motion of level sets by mean curvature},
  date-added = {2008-09-19 10:28:56 -0500},
  date-modified = {2008-09-19 10:28:56 -0500},
  ty = {JOUR}
}

@ARTICLE{Ewing:1999,
  author = { Ewing, R. E. and Li, Z. L. and Lin, T. and Lin, Y. P.},
  title = {The immersed finite volume element methods for the elliptic interface
	problems},
  journal = {Mathematics and Computers in Simulation},
  year = {1999},
  volume = {50},
  pages = {63-76}
}

@ARTICLE{Fadlun:2000,
  author = {Fadlun, E. A. and Verzicco, R. and Orlandi, P. and Mohd-Yusof, J.},
  title = {Combined Immersed-Boundary Finite-Difference Methods for Three-Dimensional
	Complex Flow Simulations},
  journal = {J. Comput. Phys.},
  year = {2000},
  volume = {161},
  pages = {35--60},
  number = {1},
  abstract = { A second-order accurate, highly efficient method is developed for
	simulating unsteady three-dimensional incompressible flows in complex
	geometries. This is achieved by using boundary body forces that allow
	the imposition of the boundary conditions on a given surface not
	coinciding with the computational grid. The governing equations,
	therefore, can be discretized and solved on a regular mesh thus retaining
	the advantages and the efficiency of the standard solution procedures.
	Two different forcings are tested showing that while the quality
	of the results is essentially the same in both cases, the efficiency
	of the calculation strongly depends on the particular expression.
	A major issue is the interpolation of the forcing over the grid that
	determines the accuracy of the scheme; this ranges from zeroth-order
	for the most commonly used interpolations up to second-order for
	an ad hoc velocity interpolation. The present scheme has been used
	to simulate several flows whose results have been validated by experiments
	and other results available in the literature. Finally in the last
	example we show the flow inside an IC piston/cylinder assembly at
	high Reynolds number; to our knowledge this is the first example
	in which the immersed boundary technique is applied to a full three-dimensional
	complex flow with moving boundaries and with a Reynolds number high
	enough to require a subgrid-scale turbulence model.},
  bdsk-url-1 = {http://www.sciencedirect.com/science/article/B6WHY-45FC8JY-4M/2/6b24ae68ad18e0ba9af4096f2e8a3117},
  date-added = {2008-09-14 15:46:53 -0500},
  date-modified = {2008-09-14 15:46:53 -0500},
  doi = {10.1006/jcph.2000.6484 },
  keywords = {Mathematics; FluidMechanics},
  ty = {JOUR},
  url = {http://www.sciencedirect.com/science/article/B6WHY-45FC8JY-4M/2/6b24ae68ad18e0ba9af4096f2e8a3117}
}

@ARTICLE{Falco:2005,
  author = {de Falco, Carlo and Gatti, E. and Lcacaita, A. L. and Sacco, R.},
  title = {Quantum-corrected drift-diffusion models for transport in semiconductor
	devices},
  journal = {J. Comput. Phys.},
  year = {2005},
  volume = {204},
  pages = {533-561}
}

@ARTICLE{Falco:2009,
  author = {de Falco, Carlo and Jerome, J. W. and Sacco, R.},
  title = {Quantum-corrected drift-diffusion models: Solution fixed point map
	and finite element approximation},
  journal = {J. Comput. Phys.},
  year = {2009},
  volume = {204},
  pages = {533-561}
}

@ARTICLE{Degond:2002,
  author = {de Falco, Carlo and Jerome, J. W. and Sacco, R.},
  title = {{A coupled Schr\"{o}dinger drift-diffusion model for quantum semiconductor
	devices simulations}},
  journal = {J. Comput. Phys.},
  year = {1964},
  volume = {181},
  pages = {222-259}
}

@ARTICLE{Gummel:1964,
  author = {de Falco, Carlo and Jerome, J. W. and Sacco, R.},
  title = {A self-consitent iterative scheme for the one-dimensional steady-state
	transistor calculations },
  journal = {IEEE Trans. Ele. Dev.},
  year = {1964},
  volume = {11},
  pages = {455-465}
}

@ARTICLE{Fan:2004,
  author = {Fan, H. and Mark, A. E.},
  title = {{Refinement of homology-based protein structures by molecular dynamics
	simulation techniques}},
  journal = {Protein Sci},
  year = {2004},
  volume = {13},
  pages = {211-220},
  number = {1}
}

@ARTICLE{Fan:2005a,
  author = {Fan, H. and Mark, A. E. and Zhu, J. and Honig, B.},
  title = {Comparative study of generalized Born models: Protein dynamics},
  journal = {Proceedings of the National Academy of Sciences of the United States
	of America},
  year = {2005},
  volume = {102},
  pages = {6760-4},
  number = {19},
  abstract = {In this work, we compare the results of molecular dynamics simulations
	involving the application of three generalized Born (GB) models to
	10 different proteins. The three GB models, the Still, HCT, and modified
	analytical generalized Born models, were implemented in the computationally
	efficient GROMACS package. The performance of each model was assessed
	from the backbone rms deviation from the native structure, the number
	of native hydrogen bonds retained in the simulation, and the experimental
	and calculated radius of gyration. Analysis of variance (ANOVA) was
	used to analyze the results of the simulations. The rms deviation
	measure was found to be unable to distinguish the quality of the
	results obtained with the three different GB models, whereas the
	number of native hydrogen bonds and radius of gyration yielded a
	statistically meaningful discrimination among models. Our results
	suggest that, of the three, modified analytical generalized Born
	yields the best agreement between calculated and experimentally derived
	structures. More generally, our study highlights the need both to
	evaluate the effects of different variables on the results of simulations
	and to verify that the results of molecular dynamics simulations
	are statistically meaningful.},
  annote = {Comparative study of generalized Born models: Protein dynamics},
  bdsk-url-1 = {http://dx.doi.org/10.1073/pnas.0408857102},
  date-added = {2008-06-29 08:38:59 -0500},
  date-modified = {2008-06-29 08:38:59 -0500},
  keywords = {Solvation},
  ty = {JOUR},
  url = {http://dx.doi.org/10.1073/pnas.0408857102}
}

@ARTICLE{Farajian:2007,
  author = {Farajian, A. A. and Belosludov, R. V. and Mizuseki, H. and Kawazoe,
	Y. and Hashizume, T. and Yakobson, B. I.},
  title = {Gate-induced switching and negative differential resistance in a
	single-molecule transistor: Emergence of fixed and shifting states
	with molecular length },
  journal = { JOURNAL OF CHEMICAL PHYSICS },
  year = {2007},
  volume = {127},
  number = {024901 }
}

@ARTICLE{Fauquet:2005,
  author = {Fauquet, C. M. and Stanley, J.},
  title = {Revising the way we conceive and name viruses below the species level:
	A review of geminivirus taxonomy calls for new standardized isolate
	descriptors },
  journal = {Archives of Virology },
  year = {2005},
  volume = {150},
  pages = {2151 - 2179},
  annote = {Revising the way we conceive and name viruses below the species level:
	A review of geminivirus taxonomy calls for new standardized isolate
	descriptors},
  date-added = {2009-03-10 },
  date-modified = {2009-03-10},
  ty = {JOUR}
}

@ARTICLE{coarea,
  author = {H. Federer},
  title = {{Curvature Measures}},
  journal = {Trans. Amer. Math. Soc.},
  year = {1959},
  volume = {93},
  pages = {418--491}
}

@INPROCEEDINGS{FedkiwStamJensen01,
  author = {Ronald Fedkiw and Jos Stam and Henrik Wann Jensen},
  title = {{Visual Simulation of Smoke}},
  booktitle = {Proc. ACM SIGGRAPH},
  year = {2001},
  pages = {15--22}
}

@ARTICLE{Fedkiw:1999,
  author = {Fedkiw, R. P. and Aslam, T. and Merriman, B. and Osher, S.},
  title = {A non-oscillatory {Eulerian} approach to interfaces in multimaterial
	flows (the ghost fluid method)},
  journal = {J. Comput. Phys. },
  year = {1999},
  volume = {152},
  pages = {457-492},
  annote = {A non-oscillatory {Eulerian} approach to interfaces in multimaterial
	flows (the ghost fluid method)},
  date-added = {2008-09-19 10:28:56 -0500},
  date-modified = {2008-09-19 10:28:56 -0500},
  ty = {JOUR}
}

@ARTICLE{Fedorov:2009,
  author = {Fedorov, M. V. and Goodman, J. M. and Schumm, S. },
  title = {To Switch or Not To Switch: The Effects of Potassium and Sodium Ions
	on $\alpha$-Poly-l-glutamate Conformations in Aqueous Solutions
	
	},
  journal = {J. Am. Chem. Soc.},
  year = {2009},
  volume = {131},
  pages = {10854-0856}
}

@ARTICLE{Fedorov:2007a,
  author = {Fedorov, M. V. and Kornyshev, A. A.},
  title = {Unravelling the solvent response to neutral and charged solutes},
  journal = {Molecular Physics},
  year = {2007},
  volume = {105},
  pages = {1-16},
  number = {1},
  abstract = {In this article we discuss the effects of solute-water interactions
	with focus on a set of old standing questions. How strong is the
	nonlinear response of water polarization to charged solute? How strong
	is the asymmetry of the response between cations and anions of similar
	size? What is the role of the finite size of the solute? How 'positive'
	or 'negative' hydration manifest itself in the dielectric response?
	Can non-local electrostatics, based on the bulk value of the solvent
	dielectric function, be used to describe the electric field of an
	ion and its hydration? Are experimental data on hydration energies
	compatible with the hypothesis of the over-screening effect in the
	bulk solvent response? The answers rest on a crude but analytically
	viable model of water (modified SPC/E); in no way final, they are
	intended to provoke future, more sophisticated studies, based on
	ab initio quantum molecular dynamic simulations and new experiments.},
  annote = {Unravelling the solvent response to neutral and charged solutes},
  bdsk-file-1 = {YnBsaXN0MDDUAQIDBAUGCQpYJHZlcnNpb25UJHRvcFkkYXJjaGl2ZXJYJG9iamVjdHMSAAGGoNE
	HCFRyb290gAFfEA9OU0tleWVkQXJjaGl2ZXKoCwwXGBkdJCVVJG51bGzTDQ4PEBEUViRjbGFzc1
	dOUy5rZXlzWk5TLm9iamVjdHOAB6ISE4ACgAOiFRaABIAGWWFsaWFzRGF0YVxyZWxhdGl2ZVBhd
	GjSDRobHFdOUy5kYXRhgAVPEQHSAAAAAAHSAAIAAAxNYWNpbnRvc2ggSEQAAAAAAAAAAAAAAAAA
	AADD4v5NSCsAAAAZYksZMjAwNy1GZWRvcm92S29ybnlzaGV2LnBkZgAAAAAAAAAAAAAAAAAAAAA
	AAAAAAAAAAAAAAAAAAAAAAAAAAAAAABlibsIJgjoAAAAAAAAAAAAEAAQAAAkgAAAAAAAAAAAAAA
	AAAAAAB0FyY2hpdmUAABAACAAAw+NSrQAAABEACAAAwgnWmgAAAAEAFAAZYksAGWIDAAqkKAAKp
	BEAAHrcAAIAT01hY2ludG9zaCBIRDpVc2VyczpiYWtlcjpEb2N1bWVudHM6UmVmZXJlbmNlczpB
	cmNoaXZlOjIwMDctRmVkb3Jvdktvcm55c2hldi5wZGYAAA4ANAAZADIAMAAwADcALQBGAGUAZAB
	vAHIAbwB2AEsAbwByAG4AeQBzAGgAZQB2AC4AcABkAGYADwAaAAwATQBhAGMAaQBuAHQAbwBzAG
	gAIABIAEQAEgBCVXNlcnMvYmFrZXIvRG9jdW1lbnRzL1JlZmVyZW5jZXMvQXJjaGl2ZS8yMDA3L
	UZlZG9yb3ZLb3JueXNoZXYucGRmABMAAS8AABUAAgAM//8AANIeHyAhWCRjbGFzc2VzWiRjbGFz
	c25hbWWjISIjXU5TTXV0YWJsZURhdGFWTlNEYXRhWE5TT2JqZWN0XxBCLi4vLi4vLi4vLi4vRG9
	jdW1lbnRzL1JlZmVyZW5jZXMvQXJjaGl2ZS8yMDA3LUZlZG9yb3ZLb3JueXNoZXYucGRm0h4fJi
	eiJyNcTlNEaWN0aW9uYXJ5AAgAEQAaAB8AKQAyADcAOgA/AEEAUwBcAGIAaQBwAHgAgwCFAIgAi
	gCMAI8AkQCTAJ0AqgCvALcAuQKPApQCnQKoAqwCugLBAsoDDwMUAxcAAAAAAAACAQAAAAAAAAAo
	AAAAAAAAAAAAAAAAAAADJA==},
  bdsk-url-1 = {http://dx.doi.org/10.1080/00268970601110316},
  date-added = {2008-09-01 14:05:13 -0500},
  date-modified = {2008-09-01 14:05:13 -0500},
  keywords = {Solvation; StatisticalMechanics},
  read = {Yes},
  ty = {JOUR},
  url = {http://dx.doi.org/10.1080/00268970601110316}
}

@ARTICLE{Feig:2004b,
  author = {Feig, M. and Brooks {III}, C. L.},
  title = {Recent advances in the development and application of implicit solvent
	models in biomolecule simulations},
  journal = {Curr Opin Struct Biol.},
  year = {2004},
  volume = {14},
  pages = {217 - 224},
  annote = {FeigCOSB; A recent review of implicit solvent methods with a GB-specific
	focus that is complementary to the current article.},
  ty = {JOUR},
  url = {http://dx.doi.org/10.1016/j.sbi.2004.03.009}
}

@ARTICLE{Feig:2002,
  author = {Feig, M. and Brooks, C. L. 3rd.},
  title = {{Evaluating CASP4 predictions with physical energy functions.}},
  journal = {Proteins},
  year = {2002},
  volume = {49},
  pages = {232-245},
  number = {2}
}

@ARTICLE{Feig:2004c,
  author = {Feig, M. and Im, W. and Brooks {III}, C. L.},
  title = {Implicit solvation based on generalized {Born} theory in different
	dielectric environments},
  journal = {Journal of Chemical Physics},
  year = {2004},
  volume = {120},
  pages = {903-911},
  number = {2},
  abstract = {In this paper we are investigating the effect of the dielectric environment
	on atomic Born radii used in generalized Born (GB) methods. Motivated
	by the Kirkwood expression for the reaction field of a single off-center
	charge in a spherical cavity, we are proposing extended formalisms
	for the calculation of Born radii as a function of external and internal
	dielectric constants. We demonstrate that reaction field energies
	calculated from environmentally dependent Born radii lead to much
	improved agreement with PoissonÃ¢Â€Â“Boltzmann solutions
	for low dielectric external environments, such as biological membranes
	or organic solvent, compared to previous methods where the calculation
	of Born radii does not depend on the environment. We also examine
	how this new approach can be applied for the calculation of transfer
	free energies from vacuum to a given external dielectric for a system
	with an internal dielectric larger than one. This has not been possible
	with standard GB theory but is relevant when scoring minimized or
	average structures with implicit solvent.Ã‚Â??004 American Institute
	of Physics.},
  annote = {Implicit solvation based on generalized Born theory in different
	dielectric environments},
  bdsk-url-1 = {http://ojps.aip.org/journals/doc/JCPSA6-ft/vol_120/iss_2/903_1.html},
  date-added = {2008-06-29 08:42:10 -0500},
  date-modified = {2008-06-29 08:42:10 -0500},
  keywords = {Electrostatics},
  ty = {JOUR},
  url = {http://ojps.aip.org/journals/doc/JCPSA6-ft/vol_120/iss_2/903_1.html}
}

@ARTICLE{Feig:2004a,
  author = {Feig, M. and Onufriev, A. and Lee, M. S. and Im, W. and Case, D.
	A. and Brooks, C. L. , III},
  title = {Performance comparison of generalized {Born} and {Poisson} methods
	in the calculation of electrostatic solvation energies for protein
	structures},
  journal = {Journal of Computational Chemistry},
  year = {2004},
  volume = {25},
  pages = {265-284},
  number = {2},
  abstract = {This study compares generalized Born (GB) and Poisson (PB) methods
	for calculating electrostatic solvation energies of proteins. A large
	set of GB and PB implementations from our own laboratories as well
	as others is applied to a series of protein structure test sets for
	evaluating the performance of these methods. The test sets cover
	a significant range of native protein structures of varying size,
	fold topology, and amino acid composition as well as nonnative extended
	and misfolded structures that may be found during structure prediction
	and folding/unfolding studies. We find that the methods tested here
	span a wide range from highly accurate and computationally demanding
	PB-based methods to somewhat less accurate but more affordable GB-based
	approaches and a few fast, approximate PB solvers. Compared with
	PB solvation energies, the latest, most accurate GB implementations
	were found to achieve errors of 1{\%} for relative solvation energies
	between different proteins and 0.4{\%} between different conformations
	of the same protein. This compares to accurate PB solvers that produce
	results with deviations of less than 0.25{\%} between each other
	for both native and nonnative structures. The performance of the
	best GB methods is discussed in more detail for the application for
	force field-based minimizations or molecular dynamics simulations.
	Ã‚Â??003 Wiley Periodicals, Inc. J Comput Chem 25: 265-284,
	2004},
  annote = {Performance comparison of generalized born and Poisson methods in
	the calculation of electrostatic solvation energies for protein structures;
	**; A side-by-side comparison of the accuracy and efficiency of several
	GB and PB implementations. While one can argue about the usefulness
	of the efficiency benchmarks (particularly since our code rated more
	slowly), the paper is a very useful guide to the {\tt{}"{}}state
	of the art{\tt{}"{}} in GB and PB methods.},
  bdsk-url-1 = {http://www3.interscience.wiley.com/cgi-bin/fulltext/106566437/HTMLSTART},
  date-added = {2008-06-29 08:43:04 -0500},
  date-modified = {2008-06-29 08:43:04 -0500},
  keywords = {Electrostatics},
  ty = {JOUR},
  url = {http://www3.interscience.wiley.com/cgi-bin/fulltext/106566437/HTMLSTART}
}

@ARTICLE{Feig:2000,
  author = {Feig, M. and Rotkiewicz, P. and Kolinski, A. and Skolnick, J. and
	Brooks, C.L. 3rd.},
  title = {{Accurate reconstruction of all-atom protein representations from
	side-chain-based low-resolution models}},
  journal = {Proteins},
  year = {2000},
  volume = {41},
  pages = {86-97},
  number = {1}
}

@ARTICLE{feldmar1996raa,
  author = {Feldmar, J. and Ayache, N.},
  title = {{Rigid, affine and locally affine registration of free-form surfaces}},
  journal = {International Journal of Computer Vision},
  year = {1996},
  volume = {18},
  pages = {99--119},
  number = {2}
}

@ARTICLE{Felts:2002,
  author = {Felts, A. K. and Gallicchio, E. and Wallqvist, A. and Levy, R. M.},
  title = {{Distinguishing native conformations of proteins from decoys with
	an effective free energy estimator based on the OPLS all-atom force
	field and the Surface Generalized Born solvent model}},
  journal = {Proteins},
  year = {2002},
  volume = {48},
  pages = {404-422},
  number = {2}
}

@ARTICLE{Felts:2004,
  author = {Felts, A. K. and Harano, Y. and Gallicchio, E. and Levy, R. M.},
  title = {{Free energy surfaces of beta-hairpin and alpha-helical peptides
	generated by replica exchange molecular dynamics with the AGBNP implicit
	solvent model}},
  journal = {Proteins},
  year = {2004},
  volume = {56},
  pages = {310-321},
  number = {2}
}

@ARTICLE{Feng049458,
  author = {Feng, H. S. and Bian, J. and Li, L. M. and Yang, W. T.},
  title = {An efficient method for constructing nonorthogonal localized molecular
	orbitals},
  journal = {Journal of Chemical Physics},
  year = {2004},
  volume = {120},
  pages = {9458-9466},
  number = {20},
  month = {May},
  abstract = {A new method for constructing nonorthogonal localized molecular orbitals
	(NOLMOs) is presented. The set of highly localized NOLMOs is obtained
	by minimization of the spread functional starting from an initial
	set of canonical orthogonal molecular orbitals. To enhance the stability
	and efficiency, the centroids of the NOLMOs are constrained to be
	those of the corresponding orthogonal localized molecular orbitals
	(OLMOs), which are obtained with the Boys criterion in advance. In
	particular, these centroid constraints make the optimization for
	each NOLMO independent of the others, which is an attractive feature
	for application to large systems. The minimization with the constraints
	incorporated through the multiplier-penalty function method is stable
	and efficient in convergence. While exhibiting the classical bonding
	pattern in chemistry and sharing a spatial distribution similar to
	that of the corresponding OLMOs, the obtained NOLMOs are more compact
	than the corresponding OLMOs with about 10%-28% reduction in the
	value of the spread functional and devoid of the troublesome "orthogonalization
	tails." (C) 2004 American Institute of Physics.},
  endnotereftype = {Journal Article},
  issn = {0021-9606},
  shorttitle = {An efficient method for constructing nonorthogonal localized molecular
	orbitals},
  url = {<Go to ISI>://000221268300005}
}

@ARTICLE{Feng:2004a,
  author = {Feng, X. and Prohl, A. },
  title = {Analysis of a fully discrete finite element method for the phase
	field model and approximation of its sharp interface limits},
  journal = {Mathematics of Computation},
  year = {2004},
  volume = {73},
  pages = {541--567},
  abstract = {We propose and analyze a fully discrete finite element scheme for
	the phase field model describing the solidification process in materials
	science. The primary goal of this paper is to establish some useful
	a priori error estimates for the proposed numerical method, in particular,
	by focusing on the dependence of the error bounds on the parameter
	, known as the measure of the interface thickness. Optimal order
	error bounds are shown for the fully discrete scheme under some reasonable
	constraints on the mesh size and the time step size . In particular,
	it is shown that all error bounds depend on only in some lower polynomial
	order for small . The cruxes of the analysis are to establish stability
	estimates for the discrete solutions, to use a spectrum estimate
	result of Chen, and to establish a discrete counterpart of it for
	a linearized phase field operator to handle the nonlinear effect.
	Finally, as a nontrivial byproduct, the error estimates are used
	to establish convergence of the solution of the fully discrete scheme
	to solutions of the sharp interface limits of the phase field model
	under different scaling in its coefficients. The sharp interface
	limits include the classical Stefan problem, the generalized Stefan
	problems with surface tension and surface kinetics, the motion by
	mean curvature flow, and the Hele-Shaw model.},
  bdsk-url-1 = {http://www.ams.org/mcom/2004-73-246/S0025-5718-03-01588-6/home.html},
  date-added = {2008-06-30 09:48:29 -0500},
  date-modified = {2008-06-30 09:48:29 -0500},
  keywords = {mathematics},
  posted-at = {2008-06-30 15:48:01},
  priority = {0},
  url = {http://www.ams.org/mcom/2004-73-246/S0025-5718-03-01588-6/home.html}
}


@BOOK{Fermini:2008,
  title = {Ion Channels},
  publisher = {Springer-Verlag},
  year = {2008},
  author = {Fermini, B. and Priest, B. T. }
}

@ARTICLE{Ferrier:2006,
  author = {Ferrier, M. and Clerc, R. and Ghibaudo, G. and Boeuf, F. and Skotnicki,
	T. },
  title = {{Analytical model for quantization on strained and unstrained bulk
	nMOSFET and its impact on quasi-ballistic current} },
  journal = {Solid- State Electrons},
  year = {2006},
  volume = {50},
  pages = {69-77 },
  annote = {Analytical model for quantization on strained and unstrained bulk
	nMOSFET and its impact on quasi-ballistic current },
  date-added = {2008-11-25 10:28:56 -0500},
  date-modified = {2008-11-25 10:28:56 -0500},
  ty = {JOUR}
}

@ARTICLE{Fetrow:1998,
  author = {Fetrow, J. S. and Skolnick, J.},
  title = {{Method for prediction of protein function from sequence using the
	sequence-to-structure-to-function paradigm with application to glutaredoxins/thioredoxins
	and T1 ribonucleases}},
  journal = {J Mol Biol},
  year = {1998},
  volume = {281},
  pages = {949-968},
  number = {5}
}

@ARTICLE{Fiedler73,
  author = {Miroslav Fiedler},
  title = {Algebraic Connectivity of Graphs},
  journal = {Czechoslovak Mathematical Journal},
  year = {1973},
  volume = {23},
  pages = {298--305},
  number = {98}
}

@ARTICLE{Fiori:2008,
  author = {Fiori, G. and Di Pascoli, S. and Lannaccone, G. },
  title = {Three-dimensional simulations of quantum confinement and random dopants
	effects in nanoscale nMOSFETs},
  journal = {J. Comput. Theor. Nanoscience},
  year = {2008},
  volume = {5},
  pages = {1115-1119 },
  annote = {Three-dimensional simulations of quantum confinement and random dopants
	effects in nanoscale nMOSFETs},
  date-added = {2008-11-25 10:28:56 -0500},
  date-modified = {2008-11-25 10:28:56 -0500},
  ty = {JOUR}
}

@ARTICLE{Fiori:2007,
  author = {Fiori, G. and Lannaccone, G. },
  title = {Three-dimensional simulation of one-dimensional transport in silicon
	nanowire transistors },
  journal = {IEEE T Nanotechnology},
  year = {2007},
  volume = {6},
  pages = {524-529 },
  annote = {Three-dimensional simulation of one-dimensional transport in silicon
	nanowire transistors },
  date-added = {2008-11-25 10:28:56 -0500},
  date-modified = {2008-11-25 10:28:56 -0500},
  ty = {JOUR}
}

@PROCEEDINGS{FCS07,
  title = {{Out of core MLS reconstruction}},
  year = {2007},
  author = {Fiorin, Valentino and Cignoni, Paolo and Scopigno, Roberto},
  journal = {The Ninth IASTED International Conference on Computer Graphics an
	Imaging - CGIM 2007},
  page = {27--34},
  timestamp = {2009.03.26}
}

@ARTICLE{Fischetti:1999,
  author = {Fischetti, M. V.},
  title = {Master-equation approach to the study of electronic transport in
	small semiconductor devices},
  journal = {Phys. Rev. B},
  year = {1999},
  volume = {59},
  pages = {4901-4917},
  annote = {Master-equation approach to the study of electronic transport in
	small semiconductor devices },
  date-added = {2008-11-25 10:28:56 -0500}
}

@ARTICLE{Fixel:2007,
  author = {Fixel, D. A. and Hitchon, W. N. G.},
  title = {Convective scheme solution of the Boltzmann transport equation for
	nanoscale semiconductor devices },
  journal = {J. Comput. Phys.},
  year = {2007},
  volume = {227},
  pages = {1387-1410},
  annote = {Convective scheme solution of the Boltzmann transport equation for
	nanoscale semiconductor devices },
  date-added = {2008-11-25 10:28:56 -0500},
  date-modified = {2008-11-25 10:28:56 -0500},
  ty = {JOUR}
}

@ARTICLE{Fixman:1979,
  author = {Fixman, M.},
  title = {The {{Poisson-Boltzmann}} equation and its application to polyelectrolytes},
  journal = {Journal of Chemical Physics},
  year = {1979},
  volume = {70},
  pages = {4995-5005},
  number = {11},
  abstract = {The validity of the PoissonÃ¢Â€Â“Boltzmann (PB) equation is
	reconsidered on the basis of functional expansion techniques supplemented
	by the mean spherical approximation. In the application of greatest
	interest a strong Coulomb potential originating in an external source,
	such as a polyelectrolyte molecule, acts on a salt solution of small
	mobile ions. Where the local charge density of mobile ions is high,
	substantial errors may occur in the PB approximation that relates
	charge density to mean potential. However, the solution to the PB
	equation is nevertheless a good approximation in the indicated application
	because a quite small percentage change in the electrostatic potential
	can compensate large errors in the Boltzmann distribution. An application
	to DNA illustrates this compensation, and also its impending failure
	at bulk salt concentrations in excess of 0.1M. A two phase (or condensation)
	model is derived as an approximation to the PB equation and retains
	fair accuracy even at substantial salt concentrations, where the
	limiting laws lose theoretical validity.},
  annote = {The PoissonÃ¢Â€Â“Boltzmann equation and its application to
	polyelectrolytes},
  bdsk-url-1 = {http://dx.doi.org/10.1063/1.437340},
  date-added = {2008-06-29 08:43:53 -0500},
  date-modified = {2008-06-29 08:53:50 -0500},
  keywords = {Electrostatics; Statistical_mechanics},
  ty = {JOUR},
  url = {http://dx.doi.org/10.1063/1.437340}
}

@ARTICLE{Fleury:2009,
  author = {Fleury, V.},
  title = {Clarifying tetrapod embryogenesis, a physicist?s point of view},
  journal = {Eur. Phys. J. Appl. Phys.},
  year = {2009},
  volume = {45},
  number = {30101 }
}

@ARTICLE{Floriani2003,
  author = {Floriani, Leila De and Hui, Annie},
  title = {{A scalable data structure for three-dimensional non-manifold objects}},
  journal = {Proceedings of the 2003 Eurographics/ACM},
  year = {2003},
  pages = {72--82},
  file = {:C\:/Dropbox/Dropbox/Paper/10.1.1.90.3688.pdf:pdf},
  owner = {doubletony},
  timestamp = {2012.04.26},
  url = {http://dl.acm.org/citation.cfm?id=882380}
}

@ARTICLE{Fogelson:2001,
  author = {Aaron L. Fogelson and James P. Keener},
  title = {Immersed Interface Methods for Neumann and Related Problems in Two
	and Three Dimensions},
  journal = {SIAM Journal on Scientific Computing},
  year = {2001},
  volume = {22},
  pages = {1630-1654},
  number = {5},
  abstract = {We develop and apply a finite-difference method to discretize the
	Laplacian operator with Neumann boundary conditions on an irregular
	domain using a regular Cartesian grid. The method is an extension
	of the immersed interface method developed by LeVeque and Li [SIAM
	J. Numer. Anal., 31 (1994) 1019--1044]. With careful selection of
	stencils, the method is second order accurate and produces a matrix
	that is stable (diagonally semidominant). The method is illustrated
	on several two-dimensional problems and one three-dimensional problem.},
  bdsk-url-1 = {http://link.aip.org/link/?SCE/22/1630/1},
  bdsk-url-2 = {http://dx.doi.org/10.1137/S1064827597327541},
  date-added = {2008-09-14 15:32:12 -0500},
  date-modified = {2008-09-14 15:32:12 -0500},
  doi = {10.1137/S1064827597327541},
  keywords = {Mathematics},
  publisher = {SIAM},
  url = {http://link.aip.org/link/?SCE/22/1630/1}
}

@ARTICLE{Fogolari:1997,
  author = {Fogolari, F. and Briggs, J. M. },
  title = {On the variational approach to {P}oisson{-}{B}oltzmann free energies},
  journal = {Chemical Physics Letters},
  year = {1997},
  volume = {281},
  pages = {135-139}
}

@ARTICLE{Fogolari:2003,
  author = {Fogolari, F. and Brigo, A. and Molinari, H.},
  title = {Protocol for MM/PBSA Molecular Dynamics Simulations of Proteins},
  journal = {Biophysical Journal},
  year = {2003},
  volume = {85},
  pages = {159-166},
  number = {1},
  abstract = {Continuum solvent models have been employed in past years for understanding
	processes such as protein folding or biomolecular association. In
	the last decade, several attempts have been made to merge atomic
	detail molecular dynamics simulations with solvent continuum models.
	Among continuum models, the {Poisson-Boltzmann} solvent accessible
	surface area model is one of the oldest and most fundamental. Notwithstanding
	its wide usage for simulation of biomolecular electrostatic potential,
	the {Poisson-Boltzmann} equation has been very seldom used to obtain
	solvation forces for molecular dynamics simulation. We propose here
	a fast and reliable methodology to implement continuum forces in
	standard molecular mechanics and dynamics algorithms. Results for
	a totally unrestrained 1 ns molecular dynamics simulation of a small
	protein are quantitatively similar to results obtained by explicit
	solvent molecular dynamics simulations.},
  annote = {Protocol for MM/PBSA Molecular Dynamics Simulations of Proteins;
	*; A very readable introduction to PB methods together with some
	modifications to accelerate solution of the PB in a molecular dynamics
	setting.},
  bdsk-url-1 = {http://www.biophysj.org/cgi/content/full/85/1/159},
  date-added = {2008-06-29 08:46:47 -0500},
  date-modified = {2008-06-29 08:46:47 -0500},
  keywords = {Electrostatics; Solvation},
  ty = {JOUR},
  url = {http://www.biophysj.org/cgi/content/full/85/1/159}
}

@ARTICLE{Fogolari:2002,
  author = {Fogolari, F. and Brigo, A. and Molinari, H.},
  title = {The {{Poisson-Boltzmann}} equation for biomolecular electrostatics:
	a tool for structural biology},
  journal = {Journal of Molecular Recognition},
  year = {2002},
  volume = {15},
  pages = {377-92},
  number = {6},
  abstract = {Electrostatics plays a fundamental role in virtually all processes
	involving biomolecules in solution. The {Poisson-Boltzmann} equation
	constitutes one of the most fundamental approaches to treat electrostatic
	effects in solution. The theoretical basis of the {Poisson-Boltzmann}
	equation is reviewed and a wide range of applications is presented,lecules
	in solution, the computation of the free energy of association and
	its salt dependence, the study of pKa shifts and the combination
	with classical molecular mechanics and dynamics. Theoretical results
	may be used for rationalizing or predicting experimental results,
	or for suggesting working hypotheses. An ever-increasing body of
	successful applications proves that the {Poisson-Boltzmann} equation
	is a useful tool for structural biology and complementary to other
	established experimental and theoretical methodologies.},
  annote = {The {Poisson-Boltzmann} equation for biomolecular electrostatics:
	a tool for structural biology; *; A good review of PB methods; up-to-date
	as of 2002.},
  bdsk-url-1 = {http://dx.doi.org/10.1002/jmr.577},
  date-added = {2008-09-01 14:12:06 -0500},
  date-modified = {2008-09-01 14:12:06 -0500},
  keywords = {Electrostatics},
  ty = {JOUR},
  url = {http://dx.doi.org/10.1002/jmr.577}
}

@BOOK{Fornberg,
  title = {A Practical Guide to Pseudospectral Methods},
  publisher = {Cambridge University Press, Cambridge},
  year = {1996},
  author = {Fornberg, B.}
}

@ARTICLE{Forsman:2004,
  author = {Forsman, J.},
  title = {A Simple Correlation-Corrected {{Poisson-Boltzmann}} Theory},
  journal = {Journal of Physical Chemistry B},
  year = {2004},
  volume = {108},
  pages = {9236-45},
  number = {26},
  abstract = {A simple approach is used to introduce effects of ion-ion correlations
	into the {Poisson-Boltzmann} theory. The mean-field character of
	the theory is retained and correlations are approximated by an effective
	interaction potential, which differs from the Coulombic at short
	range. In particular, the severe overestimation of the average interaction
	energy between ions of like charge inherent in the original {Poisson-Boltzmann}
	theory, is accounted for by this effective potential. We show that
	important phenomena due to ion-ion correlations, such as net attraction
	between surfaces of like charge and charge reversal in double layer
	systems, are qualitatively and semiquantitatively reproduced by this
	correlation-corrected theory, which contains no adjustable parameter.
	The response of net surface interactions to the addition of salt
	is also captured by the theory and satisfactory quantitative agreement
	is found with simulation results, even at molar concentrations of
	divalent salt and in the presence of highly charged surfaces. The
	mean-field theory is furthermore able to qualitatively predict the
	way in which bulk salt properties such as the osmotic coefficient
	and the excess chemical potential depend on the salt concentration.
	The quantitative performance is poorer than for electric double layer
	systems, but there is still a substantial improvement relative to
	the ordinary {Poisson-Boltzmann} theory.},
  annote = {A Simple Correlation-Corrected {Poisson-Boltzmann} Theory},
  bdsk-url-1 = {http://dx.doi.org/10.1021/jp049571u},
  date-added = {2008-06-29 08:54:18 -0500},
  date-modified = {2008-06-29 08:54:18 -0500},
  keywords = {Electrostatics},
  ty = {JOUR},
  url = {http://dx.doi.org/10.1021/jp049571u}
}

@ARTICLE{Forsten:1994,
  author = {Forsten, K. E. and Kozack, R. E. and Lauffenburger, D. A. and Subramaniam,
	S.},
  title = {Numerical Solution of the Nonlinear {{Poisson-Boltzmann}} Equation
	for a Membrane-Electrolyte System},
  journal = {Journal of Physical Chemistry},
  year = {1994},
  volume = {98},
  pages = {5580-6},
  number = {21},
  bdsk-url-1 = {http://dx.doi.org/10.1021/j100072a028},
  date-added = {2008-06-29 14:45:42 -0500},
  date-modified = {2008-06-29 14:45:42 -0500},
  doi = {10.1021/j100072a028},
  keywords = {electrostatics; biomembranes; Solvation},
  url = {http://dx.doi.org/10.1021%2Fj100072a028}
}

@INPROCEEDINGS{Foster:2001:PAO,
  author = {Nick Foster and Ronald Fedkiw},
  title = {{Practical Animation of Liquids}},
  booktitle = {ACM SIGGRAPH},
  year = {2001},
  pages = {23--30},
  month = aug
}


%  author = {Fotin, A. and Cheng, Y. and Sliz, P. and Grigorieff, N. and Harrison, S. C. and Kirchhausen, T. and Walz, T.},
@ARTICLE{Fotin2004,
  author = {Fotin, A. and Cheng, Y. and Sliz, P. and Grigorieff, N. and Harrison et al, S. C.},
  title = {Molecular model for a complete clathrin lattice from electron cryomicroscopy.},
  journal = {Nature},
  year = {2004},
  volume = {432},
  pages = {573-9--},
  number = {7017},
  month = dec,
  abstract = {Clathrin-coated vesicles are important vehicles of membrane traffic
	in cells. We report the structure of a clathrin lattice at subnanometre
	resolution, obtained from electron cryomicroscopy of coats assembled
	in vitro. We trace most of the 1,675-residue clathrin heavy chain
	by fitting known crystal structures of two segments, and homology
	models of the rest, into the electron microscopy density map. We
	also define the position of the central helical segment of the light
	chain. A helical tripod, the carboxy-terminal parts of three heavy
	chains, projects inward from the vertex of each three-legged clathrin
	triskelion, linking that vertex to 'ankles' of triskelions centred
	two vertices away. Analysis of coats with distinct diameters shows
	an invariant pattern of contacts in the neighbourhood of each vertex,
	with more variable interactions along the extended parts of the triskelion
	'legs'. These invariant local interactions appear to stabilize the
	lattice, allowing assembly and uncoating to be controlled by events
	at a few specific sites.},
  address = {Biophysics Graduate Program, Department of Cell Biology, Harvard
	Medical School, 240 Longwood Avenue, Boston, Massachusetts 02115,
	USA.},
  comment = {Research Support, Non-U.S. Gov't,Research Support, U.S. Gov't, P.H.S.,},
  keywords = {Animals, Cattle, Clathrin, Cryoelectron Microscopy, Crystallography,
	X-Ray, Models, Molecular, Protein Structure, Quaternary},
  owner = {SeanLab},
  timestamp = {2012.05.23},
  url = {http://ukpmc.ac.uk/abstract/MED/15502812}
}

@ARTICLE{Franco:2006,
  author = {Franco, A. A. and Schott, P. and Jallut, C. and Maschke, B.},
  title = {A dynamic mechanistic model of an electrochemical interface},
  journal = {Journal of The Electrochemical Society},
  year = {2006},
  volume = {153},
  pages = {A1053-A1061 }
}

@ARTICLE{Francois:2003,
  author = {Francois, M. and Shyy, W.},
  title = {Computations of drop dynamics with the immersed boundary method,
	part 2: Drop impact and heat transfer},
  journal = {Numer. Heat Trans. Part B-Fund.},
  year = {2003},
  volume = {44},
  annote = {Computations of drop dynamics with the immersed boundary method,
	part 2: Drop impact and heat transfer},
  date-added = {2008-09-19 10:28:56 -0500},
  date-modified = {2008-09-19 10:28:56 -0500},
  ty = {JOUR}
}

@ARTICLE{Francois:2004,
  author = {Francois, M and Uzgoren, E. and Jackson, J. and Shyy, W.},
  title = {Multigrid computations with the immersed boundary technique for multiphase
	flows},
  journal = {Int. J. Numer. Meth. Heat Fluid Flow },
  year = {2004},
  volume = {14},
  pages = {98-115},
  annote = {Multigrid computations with the immersed boundary technique for multiphase
	flows},
  date-added = {2008-09-19 10:28:56 -0500},
  date-modified = {2008-09-19 10:28:56 -0500},
  ty = {JOUR}
}

@ARTICLE{Frank:1998,
  author = {Frank, D. J. and Taur, Y. and Wong, H. S. P.},
  title = {{Generalized scale length for two-dimensional effects in MOSFETs}},
  journal = {IEEE Electron Dev. Lett.},
  year = {1998},
  volume = {10},
  pages = {385-387}
}

@ARTICLE{FSD07,
  author = {Ilja Friedel and Peter Schr{\"o}der and Mathieu Desbrun},
  title = {Unconstrained Spherical Parameterization},
  journal = {Journal of Graphics Tools},
  year = {2007},
  volume = {12},
  pages = {17--26},
  number = {1}
}

@ARTICLE{Fries:1985,
  author = {Fries, P. H. and Patey, G. N.},
  title = {The solution of the hypernetted-chain approximation for fluids of
	nonspherical particles. A general method with application to dipolar
	hard spheres},
  journal = {Journal of Chemical Physics},
  year = {1985},
  volume = {82},
  pages = {429 - 440}
}

@INPROCEEDINGS{ADF,
  author = {S. Frisken and R. Perry and A. Rockwood and T. Jones},
  title = {{Adaptively Sampled Distance Fields: A General Representation of
	Shape for Computer Graphics}},
  booktitle = {ACM SIGGRAPH Proc.},
  year = {2000},
  pages = {249--254}
}

@MISC{LSM-FVM2,
  author = {P. Frolkovic and K. Mikula},
  title = {{High-resolution Flux-based Level Set Method}},
  howpublished = {{Preprint 2005-12}},
  year = {2005},
  note = {{Department of Mathematics and Descriptive Geometry, Slovak University
	of Technology, Bratislava}}
}

@MISC{LSM-FVM,
  author = {P. Frolkovic and K. Mikula},
  title = {{Flux-based Level Set Method: A Finite Volume Method for Evolving
	Interfaces}},
  howpublished = {{Preprint 15}},
  month = sep,
  year = {2003},
  note = {{Interdisziplin{\"a}res Zentrum f{\"u}r Wissenschaftliches Rechnen}}
}

@ARTICLE{Frydel:2011,
  author = {Frydel, D.},
  title = {Polarizable Poisson-Boltzmann equation: The study of polarizability
	effects on the structure of a double layer},
  journal = {J. Chem. Phys.},
  year = {2011},
  volume = {134},
  pages = {234704}
}

@ARTICLE{JPFu:2007,
  author = {Fu, J. P. and Schoch, R. B. and Stevens, A. L. and Tannenbaum, S.
	R. and Han, J. Y. },
  title = {A patterned anisotropic nanofluidic sieving structure for continuous-flow
	separation of DNA and proteins },
  journal = {Nature Nanotechnology },
  year = {2007},
  volume = {2},
  pages = { 121-128 },
  number = { }
}

@ARTICLE{Fujimoto0854102,
  author = {Fujimoto, K. and Yang, W. T.},
  title = {Density-fragment interaction approach for quantum-mechanical/molecular-mechanical
	calculations with application to the excited states of a Mg2+-sensitive
	dye},
  journal = {Journal of Chemical Physics},
  year = {2008},
  volume = {129},
  pages = {054102},
  number = {5},
  month = {Aug},
  abstract = {A density-fragment interaction (DFI) approach for large-scale calculations
	is proposed. The DFI scheme describes electron density interaction
	between many quantum-mechanical (QM) fragments, which overcomes errors
	in electrostatic interactions with the fixed point-charge description
	in the conventional quantum-mechanical/molecular-mechanical (QM/MM)
	method. A self-consistent method, which is a mean-field treatment
	of the QM fragment interactions, was adopted to include equally the
	electron density interactions between the QM fragments. As a result,
	this method enables the evaluation of the polarization effects of
	the solvent and the protein surroundings. This method was combined
	with not only density functional theory (DFT) but also time-dependent
	DFT. In order to evaluate the solvent polarization effects in the
	DFI-QM/MM method, we have applied it to the excited states of the
	magnesium-sensitive dye, KMG-20. The DFI-QM/MM method succeeds in
	including solvent polarization effects and predicting accurately
	the spectral shift caused by Mg2+ binding. (C) 2008 American Institute
	of Physics.},
  endnotereftype = {Journal Article},
  issn = {0021-9606},
  shorttitle = {Density-fragment interaction approach for quantum-mechanical/molecular-mechanical
	calculations with application to the excited states of a Mg2+-sensitive
	dye},
  url = {<Go to ISI>://000258336100002}
}

@ARTICLE{Gabashvili:2007,
  author = {Gabashvili, I. S. and Sokolowski, B. H. A and Morton, C. C. and Giersch,
	A. B. S. },
  title = {Ion channel gene expression in the inner ear},
  journal = {J Assoc Res Otolaryngol.},
  year = {2007},
  volume = {8},
  pages = {305-328},
  number = {3}
}

@ARTICLE{Gabdoulline:1996,
  author = {Gabdoulline, R.R. and Wade, R.C.},
  title = {Analytically defined surfaces to analyze molecular interaction properties},
  journal = {Journal of Molecular Graphics},
  year = {1996},
  volume = {14},
  pages = {341-353.},
  number = {6}
}

@ARTICLE{Gabdoulline:1998,
  author = {Gabdoulline, R. R. and Wade, R. C.},
  title = {Brownian dynamics simulation of protein-protein diffusional encounter},
  journal = {Methods-a Companion to Methods in Enzymology},
  year = {1998},
  volume = {14},
  pages = {329-341},
  number = {3},
  abstract = {Protein association events are ubiquitous in biological systems. Some
	protein associations and subsequent responses are diffusion controlledin
	vivo.Hence, it is important to be able to compute bimolecular diffusional
	association rates for proteins. The Brownian dynamics simulation
	methodology may be used to simulate proteinÃ¢Â€Â“protein
	encounter, compute association rates, and examine their dependence
	on protein mutation and the nature of the physical environment (e.g.,
	as a function of ionic strength or viscosity). Here, the theory for
	Brownian dynamics simulations is described, and important methodological
	aspects, particularly pertaining to the correct modeling of electrostatic
	forces and definition of encounter complex formation, are highlighted.
	To illustrate application of the method, simulations of the diffusional
	encounter of the extracellular ribonuclease, barnase, and its intracellular
	inhibitor, barstar, are described. This shows how experimental rates
	for a series of mutants and the dependence of rates on ionic strength
	can be reproduced well by Brownian dynamics simulations. Potential
	future uses of the Brownian dynamics method for investigating proteinÃ¢Â€Â“protein
	association are discussed.},
  address = {EUROPEAN MOL BIOL LAB HEIDELBERG GERMANY D-69117 Wade, RC STRUCT
	BIOL PROGRAMME, MEYERHOFSTR 1 European mol biol lab heidelberg germany
	d-69117 struct biol programme},
  annote = {Brownian dynamics simulation of protein-protein diffusional encounter;
	MAR},
  bdsk-url-1 = {http://dx.doi.org/10.1006/meth.1998.0588},
  date-added = {2008-09-01 13:54:58 -0500},
  date-modified = {2008-09-01 13:54:58 -0500},
  journal1 = {Methods},
  keywords = {Diffusion; Electrostatics},
  read = {Yes},
  ty = {JOUR},
  url = {http://dx.doi.org/10.1006/meth.1998.0588}
}

@ARTICLE{gage-hamilton:86,
  author = {Gage, M. and Hamilton, R.S.},
  title = {The Heat Equation Shrinking Convex Plane Curves},
  journal = {Journal of Diff. Geo.},
  year = {1986},
  volume = {23},
  pages = {69--96}
}

@ARTICLE{Galler:2007,
  author = {Galler, M. and Schurrer, F. },
  title = {Mathematical properties of a kinetic transport model for carriers
	and phonons in semiconductors },
  journal = {Zeitschrift fur Angewandte Mathematik und Physik},
  year = {2007},
  volume = {58},
  pages = {907 - 925},
  annote = {Mathematical properties of a kinetic transport },
  date-added = {2008-11-25 10:28:56 -0500},
  date-modified = {2008-11-25 10:28:56 -0500},
  ty = {JOUR}
}

@ARTICLE{Galler:2005,
  author = {Galler, M. and Schurrer, F. },
  title = {A deterministic solver for the transport of the AlGaN/GaN 2D electron
	gas including hot-phonon and degeneracy effects },
  journal = {Jounal of Computational Physics},
  year = {2005},
  volume = {210},
  pages = {519-534},
  annote = {A deterministic solver for the transport },
  date-added = {2008-11-25 10:28:56 -0500},
  date-modified = {2008-11-25 10:28:56 -0500},
  ty = {JOUR}
}

@ARTICLE{Gallicchio:2000,
  author = {Gallicchio, E. and Kubo, M. M. and Levy, R. M.},
  title = {Enthalpy-Entropy and Cavity Decomposition of Alkane Hydration Free
	Energies: Numerical Results and Implications for Theories of Hydrophobic
	Solvation},
  journal = {Journal of Physical Chemistry B},
  year = {2000},
  volume = {104},
  pages = {6271-6285},
  number = {26}
}

@ARTICLE{Gallicchio:2004,
  author = {Gallicchio, E. and Levy, R. M.},
  title = {{AGBNP}: An analytic implicit solvent model suitable for molecular
	dynamics simulations and high-resolution modeling},
  journal = {Journal of Computational Chemistry},
  year = {2004},
  volume = {25},
  pages = {479-499},
  number = {4},
  abstract = {We have developed an implicit solvent effective potential (AGBNP)
	that is suitable for molecular dynamics simulations and high-resolution
	modeling. It is based on a novel implementation of the pairwise descreening
	Generalized Born model for the electrostatic component and a new
	nonpolar hydration free energy estimator. The nonpolar term consists
	of an estimator for the solute-solvent {van der Waals} dispersion
	energy designed to mimic the continuum solvent solute-solvent {van
	der waals} interaction energy, in addition to a surface area term
	corresponding to the work of cavity formation. AGBNP makes use of
	a new parameter-free algorithm to calculate the scaling coefficients
	used in the pairwise descreening scheme to take into account atomic
	overlaps. The same algorithm is also used to calculate atomic surface
	areas. We show that excellent agreement is achieved for the GB self-energies
	and surface areas in comparison to accurate, but much more expensive,
	numerical evaluations. The parameter-free approach used in AGBNP
	and the sensitivity of the AGBNP model with respect to large and
	small conformational changes makes the model suitable for high-resolution
	modeling of protein loops and receptor sites as well as high-resolution
	prediction of the structure and thermodynamics of protein-ligand
	complexes. We present illustrative results for these kinds of benchmarks.
	The model is fully analytical with first derivatives and is computationally
	efficient. It has been incorporated into the IMPACT molecular simulation
	program.},
  annote = {{AGBNP}: An analytic implicit solvent model suitable for molecular
	dynamics simulations and high-resolution modeling; LevyGallicchio2;
	A very promising formulation of GB together with a novel description
	of apolar energetics; shows sensitivity to both large and small conformational
	changes which makes it a promising method for a variety of molecular
	simulations.},
  bdsk-url-1 = {http://www3.interscience.wiley.com/cgi-bin/abstract/106599641/ABSTRACT},
  date-added = {2008-08-29 15:50:55 -0500},
  date-modified = {2008-08-29 15:50:55 -0500},
  keywords = {Electrostatics},
  ty = {JOUR},
  url = {http://www3.interscience.wiley.com/cgi-bin/abstract/106599641/ABSTRACT}
}

@ARTICLE{Gallicchio:2002,
  author = {Gallicchio, E. and Zhang, L. Y. and Levy, R. M.},
  title = {The {SGB/NP} hydration free energy model based on the surface generalized
	{Born} solvent reaction field and novel nonpolar hydration free energy
	estimators},
  journal = {Journal of Computational Chemistry},
  year = {2002},
  volume = {23},
  pages = {517-29},
  number = {5},
  abstract = {The development and parameterization of a solvent potential of mean
	force designed to reproduce the hydration thermodynamics of small
	molecules and macromolecules aimed toward applications in conformation
	prediction and ligand binding free energy prediction is presented.
	The model, named SGB/NP, is based on a parameterization of the Surface
	Generalized Born continuum dielectric electrostatic model using explicit
	solvent free energy perturbation calculations and a newly developed
	nonpolar hydration free energy estimator motivated by the results
	of explicit solvent simulations of the thermodynamics of hydration
	of hydrocarbons. The nonpolar model contains, in addition to the
	more commonly used solvent accessible surface area term, a component
	corresponding to the attractive solute-solvent interactions. This
	term is found to be important to improve the accuracy of the model,
	particularly for cyclic and hydrogen bonding compounds. The model
	is parameterized against the experimental hydration free energies
	of a set of small organic molecules. The model reproduces the experimental
	hydration free energies of small organic molecules with an accuracy
	comparable or superior to similar models employing more computationally
	demanding estimators and/or a more extensive set of parameters},
  annote = {The SGB/NP hydration free energy model based on the surface generalized
	{Born} solvent reaction field and novel nonpolar hydration free energy
	estimators; LevyGallicchio},
  bdsk-url-1 = {http://dx.doi.org/10.1002/jcc.10045},
  date-added = {2008-08-29 15:50:55 -0500},
  date-modified = {2008-08-29 15:50:55 -0500},
  keywords = {Solvation; Electrostatics},
  ty = {JOUR},
  url = {http://dx.doi.org/10.1002/jcc.10045}
}

@ARTICLE{Gallo:2002,
  author = {Gallo, K. A. and Johnson, G. L. },
  title = {Mixed-lineage kinase control of JNK and p38 MAPK pathways.},
  journal = {Nat Rev Mol Cell Biol},
  year = {2002},
  volume = {3},
  pages = {663--672},
  number = {9},
  abstract = {Mixed-lineage kinases (MLKs) are serine/threonine protein kinases
	that regulate signalling by the c-Jun amino-terminal kinase (JNK)
	and p38 mitogen-activated-protein kinase (MAPK) pathways. MLKs are
	represented in the genomes of both Caenorhabditis elegans and Drosophila
	melanogaster. The Drosophila MLK Slipper regulates JNK to control
	dorsal closure during embryonic morphogenesis. In mammalian cells,
	MLKs are implicated in the control of apoptosis and are potential
	drug targets for many neurodegenerative diseases.},
  address = {Department of Physiology, Michigan State University, East Lansing,
	Michigan 48824, USA. gallok@msu.edu},
  bdsk-url-1 = {http://dx.doi.org/10.1038/nrm906},
  date-added = {2008-06-30 21:52:39 -0400},
  date-modified = {2008-06-30 21:52:39 -0400},
  doi = {10.1038/nrm906},
  issn = {1471-0072},
  keywords = {misc},
  posted-at = {2008-07-01 02:52:04},
  priority = {0},
  url = {http://dx.doi.org/10.1038/nrm906}
}

@ARTICLE{Garcia-Garcia:2003,
  author = {Garcia-Garcia, C. and Draper, D. E.},
  title = {Electrostatic Interactions in a Peptide-RNA Complex},
  journal = {Journal of Molecular Biology},
  year = {2003},
  volume = {331},
  pages = {75-88},
  number = {1},
  abstract = {Parallel experimental measurements and theoretical calculations have
	been used to investigate the energetics of electrostatic interactions
	in the complex formed between a 22 residue, -helical peptide from
	the N protein of phage and its cognate 19 nucleotide box B RNA hairpin.
	Salt-dependent free energies were measured for both peptide folding
	from coil to helix and peptide binding to RNA, and from these the
	saltdependence of binding pre-folded, helical peptide to RNA was
	determined ((GÃ-\,^{\circ}$dock)/log{$[$}KCl{$]$}=5.98(Ã-\pm$0.21)
	kcal/mol). (A folding transition taking place in the RNA hairpin
	loop was shown to have a negligible dependence on salt concentration.)
	The non-linear PoissonÃ¢Â€Â“Boltzmann equation was used to
	calculate the same salt dependence of the binding free energy as
	5.87(Ã-\pm\$0.22) kcal/mol, in excellent agreement with the measured
	value. Close agreement between experimental measurements and calculations
	was also obtained for two variant peptides in which either a basic
	or acidic residue was replaced with an uncharged residue, and for
	an RNA variant with a deletion of a single loop nucleotide. The calculations
	suggest that the strength of electrostatic interactions between a
	peptide residue and RNA varies considerably with environment, but
	that all 12 positive and negative N peptide charges contribute significantly
	to the electrostatic free energy of RNA binding, even at distances
	up to 11 Ãƒ from backbone phosphate groups. Calculations also show
	that the net release of ions that accompanies complex formation originates
	from rearrangements of both peptide and RNA ion atmospheres, and
	includes accumulation of ions in some regions of the complex as well
	as displacement of cations and anions from the ion atmospheres of
	the RNA and peptide, respectively.},
  annote = {Electrostatic Interactions in a PeptideÃ¢Â€Â“RNA Complex},
  bdsk-url-1 = {http://dx.doi.org/10.1016/S0022-2836(03)00615-6},
  date-added = {2008-09-16 15:38:31 -0500},
  date-modified = {2008-09-16 15:38:31 -0500},
  keywords = {Electrostatics; NucleicAcids},
  ty = {JOUR},
  url = {http://dx.doi.org/10.1016/S0022-2836(03)00615-6}
}

@ARTICLE{garland97,
  author = {Garland, M. and Heckbert, P.S.},
  title = {{Surface simplification using quadric error metrics}},
  journal = {ACM SIGGRAPH},
  year = {1997},
  pages = {209-216}
}

@ARTICLE{GMSCD,
  author = {Garnier, E. and Mossi, M. and Sagaut, P. and Comet, P. and Deville,
	M.},
  title = {On the use of shock-capturing scheme for large-eddy simulation},
  journal = {J. Comput. Phys.},
  year = {2001},
  volume = {153},
  pages = {273-311}
}

@ARTICLE{eric01,
  author = {Garnier, E. and Sagaut, P. and Deville, M.},
  title = {A class of explicit {ENO} filters with application to unsteady flows},
  journal = {J. Comput. Phys.},
  year = {2001},
  volume = {170},
  pages = {184-204}
}

@ARTICLE{gatzke2005cml,
  author = {Gatzke, T. and Grimm, C. and Garland, M. and Zelinka, S.},
  title = {{Curvature maps for local shape comparison}},
  journal = {Proc. Shape Modeling International},
  year = {2005}
}

@ARTICLE{SAMPL:2010,
  author = {Geballe, T. M. and Skillman, A. G. and Nicholls, A. and Guthrie,
	J. P. and Taylor, J. P. },
  title = {The SAMPL2 blind prediction challenge: introduction and overview},
  journal = {Journal of Computer-Aided Molecular Design},
  year = {2010},
  volume = {24},
  pages = {259 -279}
}

@INPROCEEDINGS{gelfand-mitra-etal:05,
  author = {Gelfand, N. and Mitra, N.J. and Guibas, L.J. and Pottmann, H.},
  title = {Robust Global Registration},
  booktitle = {Symp. on Geo. Processing},
  year = {2005},
  pages = {197--206}
}

@ARTICLE{Geng:2011,
  author = {Geng, W. and Wei, G. W. },
  title = {Multiscale molecular dynamics using the matched interface and boundary
	method},
  journal = {J Comput. Phys.},
  year = {2011},
  volume = {230},
  pages = {435-457},
  number = {2}
}

@ARTICLE{Geng:2007a,
  author = {Geng, Weihua and Yu, Sining and Wei, G. W.},
  title = {Treatment of charge singularities in implicit solvent models},
  journal = {Journal of Chemical Physics},
  year = {2007},
  volume = {127},
  pages = {114106},
  annote = {Treatment of charge singularities in implicit solvent models},
  date-added = {2008-09-19 10:28:56 -0500},
  date-modified = {2008-09-19 10:28:56 -0500},
  ty = {JOUR}
}

@ARTICLE{Georgescu:2002,
  author = {Georgescu, R. E. and Alexov, E. G. and Gunner, M. R.},
  title = {Combining Conformational Flexibility and Continuum Electrostatics
	for Calculating {pKas} in Proteins},
  journal = {Biophysical Journal},
  year = {2002},
  volume = {83},
  pages = {1731-1748},
  number = {4},
  abstract = {Protein stability and function relies on residues being in their appropriate
	ionization states at physiological pH. In situ residue pKas also
	provides a sensitive measure of the local protein environment. Multiconformation
	continuum electrostatics (MCCE) combines continuum electrostatics
	and molecular mechanics force fields in Monte Carlo sampling to simultaneously
	calculate side chain ionization and conformation. The response of
	protein to charges is incorporated both in the protein dielectric
	constant (prot) of four and by explicit conformational changes. The
	pKa of 166 residues in 12 proteins was determined. The root mean
	square error is 0.83 pH units, and >90{\%} have errors of <1 pH units
	whereas only 3{\%} have errors >2 pH units. Similar results are found
	with crystal and solution structures, showing that the method's explicit
	conformational sampling reduces sensitivity to the initial structure.
	The outcome also changes little with protein dielectric constant
	(prot 4-20). Multiconformation continuum electrostatics titrations
	show coupling of conformational flexibility and changes in ionization
	state. Examples are provided where ionizable side chain position
	(protein G), Asn orientation (lysozyme), His tautomer distribution
	(RNase A), and phosphate ion binding (RNase A and H) change with
	pH. Disallowing these motions changes the calculated pKa.},
  annote = {Combining Conformational Flexibility and Continuum Electrostatics
	for Calculating pKas in Proteins; *; A description of state-of-the-art
	methods to using PB calculations to calculate pKa's of titratable
	residues in proteins while including a limited range of protein motions.
	Interestingly, unlike the work of Nielsen and McCammon (see reference),
	this paper finds that the inclusion of flexibility does improve the
	accuracy of the calculations.},
  bdsk-url-1 = {http://www.biophysj.org/cgi/content/abstract/83/4/1731},
  date-added = {2008-06-29 08:56:55 -0500},
  date-modified = {2008-06-29 08:56:55 -0500},
  keywords = {Electrostatics},
  ty = {JOUR},
  url = {http://www.biophysj.org/cgi/content/abstract/83/4/1731}
}

@INPROCEEDINGS{TopoPreserv,
  author = {T. Gerstner and R. Pajarola},
  title = {{Topology Preserving and Controlled Topology Simplifying Multiresolution
	Isosurface Extraction}},
  booktitle = {IEEE Visualization},
  year = {2000},
  pages = {259?266}
}

@ARTICLE{Getty05241401,
  author = {Getty, S. A. and Engtrakul, C. and Wang, L. and Liu, R. and Ke, S.
	H. and Baranger, H. U. and Yang, W. and Fuhrer, M. S. and Sita, L.
	R.},
  title = {Near-perfect conduction through a ferrocene-based molecular wire},
  journal = {Physical Review B},
  year = {2005},
  volume = {71},
  pages = {241401},
  number = {24},
  month = {Jun},
  abstract = {Here we describe the design, single-molecule transport measurements,
	and theoretical modeling of a ferrocene-based organometallic molecular
	wire, whose bias-dependent conductance shows a clear Lorentzian form
	with magnitude exceeding 70% of the conductance quantum G(0). We
	attribute this unprecedented level of single-molecule conductance
	to a manifestation of the low-lying molecular resonance and extended
	orbital network long predicted for a conjugated organic system. A
	similar-in-length, all-organic conjugated phenylethynyl oligomer
	molecular framework shows much lower conductance.},
  endnotereftype = {Journal Article},
  issn = {1098-0121},
  shorttitle = {Near-perfect conduction through a ferrocene-based molecular wire},
  url = {<Go to ISI>://000230276900017}
}

@ARTICLE{Giard:2010,
  author = {Giard, J. and Macq, B. },
  title = {Molecular Surface Mesh Generation by Filtering Electron Density Map},
  journal = {International Journal of Biomedical Imaging},
  year = {2010},
  volume = {2010},
  pages = {9 pages},
  number = {923780}
}

@ARTICLE{Gibou:2005,
  author = {Gibou, FrÃ©dÃ©ric and Fedkiw, Ronald},
  title = {A fourth order accurate discretization for the {Laplace} and heat
	equations on arbitrary domains, with applications to the {Stefan}
	problem},
  journal = {J. Comput. Phys.},
  year = {2005},
  volume = {202},
  pages = {577--601},
  number = {2},
  abstract = { In this paper, we first describe a fourth order accurate finite difference
	discretization for both the Laplace equation and the heat equation
	with {Dirichlet} boundary conditions on irregular domains. In the
	case of the heat equation we use an implicit discretization in time
	to avoid the stringent time step restrictions associated with requirements
	for explicit schemes. We then turn our focus to the Stefan problem
	and construct a third order accurate method that also includes an
	implicit time discretization. Multidimensional computational results
	are presented to demonstrate the order accuracy of these numerical
	methods.},
  bdsk-url-1 = {http://www.sciencedirect.com/science/article/B6WHY-4DCMFXM-1/2/f6af3d91fdae186e52a367f91843285f},
  date-added = {2008-09-14 15:32:12 -0500},
  date-modified = {2008-09-14 15:32:12 -0500},
  doi = {10.1016/j.jcp.2004.07.018 },
  keywords = {Mathematics; Diffusion},
  ty = {JOUR},
  url = {http://www.sciencedirect.com/science/article/B6WHY-4DCMFXM-1/2/f6af3d91fdae186e52a367f91843285f}
}

@ARTICLE{Gibson:1967,
  author = {Gibson, K. D. and Scheraga, H. A.},
  title = {Minimization of polypeptide energy. {I.} Preliminary structures of
	bovine pancreatic ribonuclease S-peptide.},
  journal = {Proceedings of the National Academy of Sciences of the United States
	of America},
  year = {1967},
  volume = {58},
  pages = {420-7},
  number = {2},
  annote = {Minimization of polypeptide energy. {I.} Preliminary structures of
	bovine pancreatic ribonuclease S-peptide.; GibsonScheraga; Includes
	volume-based solvation energy term.},
  bdsk-url-1 = {http://www.pubmedcentral.gov/pagerender.fcgi?artid=335651},
  date-added = {2008-09-16 15:28:14 -0500},
  date-modified = {2008-09-16 15:28:14 -0500},
  keywords = {Electrostatics; Solvation},
  ty = {JOUR},
  url = {http://www.pubmedcentral.gov/pagerender.fcgi?artid=335651}
}

@ARTICLE{GGilboa:2004,
  author = {Gilboa, G. and Sochen, N. and Zeevi, Y. Y.},
  title = {Image sharpening by flows based on triple well potentials},
  journal = {Journal of Mathematical Imaging and Vision},
  year = {2004},
  volume = {20},
  pages = {121-131},
  number = {1-2}
}

@ARTICLE{Gilboa:2004,
  author = {Gilboa, G. and Sochen, N. and Zeevi, Y. Y.},
  title = {Image sharpening by flows based on triple well potentials},
  journal = {Journal of Mathematical Imaging and Vision},
  year = {2004},
  volume = {20},
  pages = {121-131},
  annote = {Image sharpening by flows based on triple well potentials},
  date-added = {2008-09-19 10:28:56 -0500},
  date-modified = {2008-09-19 10:28:56 -0500},
  ty = {JOUR}
}

@ARTICLE{GGilboa:2002,
  author = {Gilboa, G. and Sochen, N. and Zeevi, Y. Y.},
  title = {Forward-and-backward diffusion processes for adaptive image enhancement
	and denoising},
  journal = {{IEEE} Transactions on Image Processing},
  year = {2002},
  volume = {11},
  pages = {689-703},
  number = {7}
}

@BOOK{Invariance,
  title = {Invariance theory, the heat equation, and the Atiyah-Singer index
	theorem},
  publisher = {Publish or Perish, Boston},
  year = {1984},
  author = {P. Gilkey}
}

@ARTICLE{Gillespie:2008,
  author = {Gillespie, D.},
  title = {{Energetics of divalent selectivity in a calcium channel: the ryanodine
	receptor case study}},
  journal = {Biophys. J.},
  year = {2008},
  volume = {94(4)},
  pages = {1169-84}
}

@ARTICLE{Gillespie:2002,
  author = {Gillespie, D. and Nonner, W. and Eisenberg, B. S. },
  title = {Coupling Poisson-Nernst-Planck and density functional theory
	to calculate ion flux },
  journal = {Journal of Physics: Condensed Matter},
  year = {2002},
  volume = {14},
  pages = {12129-12145 },
  number = {46}
}

@ARTICLE{DGillespie:2005,
  author = { Gillespie, D. and Valisko, M. and Boda, D. },
  title = { Density functional theory of the electrical double layer: the RFD
	functional
	
	},
  journal = { J. Phys.: Condens. Matter },
  year = {2005},
  volume = {17},
  pages = {6609 - 6626}
}

@ARTICLE{Gillespie:2005,
  author = {Gillespie, D. and Valisko, M. and Boda, D. },
  title = {Density functional theory of the electrical double layer: the {RFD
	functional}},
  journal = {Journal of Physics: Condensed Matter},
  year = {2005},
  volume = {17},
  pages = {6609-6626}
}

@ARTICLE{Gilson:1993,
  author = {Gilson, M. K. and Davis, M. E. and Luty, B. A. and McCammon, J. A.},
  title = {Computation of electrostatic forces on solvated molecules using the
	{Poisson-Boltzmann} equation},
  journal = {Journal of Physical Chemistry},
  year = {1993},
  volume = {97},
  pages = {3591-3600},
  number = {14},
  abstract = {Numerical solutions of the {Poisson-Boltzmann} equation (PBE) have
	found wide application in the computation of electrostatic energies
	of hydrated molecules, including biological macromolecules. However,
	solving the PBE for electrostatic forces has proved more difficult,
	largely because of the challenge of computing the pressures exerted
	by a high dielectric aqueous solvent on the solute surface. This
	paper describes an accurate method for computing these forces. We
	begin by presenting a novel derivation of the forces acting in a
	system governed by the PBE. The resulting expression contains three
	distinct terms: the effect of electric fields on 'fixed" atomic charges;
	the dielectric boundary pressure, which accounts for the tendency
	of the high dielectric solvent to displace the low dielectric solute
	wherever an electric field exists; and the ionic boundary pressure,
	which accounts for the tendency of the dissolved electrolyte to move
	into regions of nonzero electrostatic potential. Techniques for extracting
	each of these three force contributions from finite difference solutions
	of the PBE for a solvated molecule are then described. Tests of the
	methods against both analytic and numeric results demonstrate their
	accuracy. Finally, the electrostatic forces acting on the two members
	of a salt bridge in the enzyme triose phosphate isomerase are analyzed.
	The dielectric boundary pressures are found to make substantial contributions
	to the atomic forces. In fact, their neglect leads to the unphysical
	situation of a significant net electrostatic force on the system.
	In contrast, the ionic boundary forces are usually extremely weak
	a t physiologic ionic strength.},
  address = {Univ houston,dept chem houston, tx usa 77204},
  annote = {Computation of electrostatic forces on solvated molecules using the
	{Poisson-Boltzmann} equation; APR 8},
  bdsk-url-1 = {http://pubs.acs.org/cgi-bin/sample.cgi/jpchax/1993/97/i14/pdf/j100116a025.pdf},
  date-added = {2008-06-29 08:57:48 -0500},
  date-modified = {2008-06-29 08:57:48 -0500},
  journal1 = {J Phys Chem},
  keywords = {Electrostatics},
  ty = {JOUR},
  url = {http://pubs.acs.org/cgi-bin/sample.cgi/jpchax/1993/97/i14/pdf/j100116a025.pdf}
}

@ARTICLE{Gilson:1987,
  author = {Gilson, M. K. and Sharp, K. and Honig, B.},
  title = {Calculating the Electrostatic Potential of Molecules in Solution:
	Method and error assessment},
  journal = {J. Comp. Chem.},
  year = {1987},
  volume = {9},
  pages = {327-335}
}

@ARTICLE{Ginalski:2003,
  author = {Ginalski, K. and Rychlewski, L.},
  title = {{Protein structure prediction of CASP5 comparative modeling and fold
	recognition targets using consensus alignment approach and 3D assessment}},
  journal = {Proteins},
  year = {2003},
  volume = {53},
  pages = {410-417},
  number = {Suppl 6}
}

@ARTICLE{Giraud:2003,
  author = {Giraud, G. and Gordon, C. M. and Dunkin, I. R. and and Wynne, K.},
  title = {The effects of anion and cation substitution on the ultrafast solvent
	dynamics of ionic liquids: A time-resolved optical Kerr-effect spectroscopic
	study},
  journal = {J. Chem. Phys.},
  year = {2003},
  volume = {119},
  pages = {464-477}
}

@ARTICLE{Glickenstein,
  author = {David Glickenstein},
  title = {A Monotonicity Property for Weighted Delaunay Triangulations},
  journal = {Journal Discrete and Computational Geometry (to appear)},
  year = {2007},
  pages = {DOI 10.1007/s00454-007-9009-y}
}

@ARTICLE{ConservFront,
  author = {James Glimm and Xiao Lin Li and Yingjie Liu and Ning Zhao},
  title = {{Conservative Front Tracking and Level Set Algorithms}},
  journal = {PNAS},
  year = {2001},
  volume = {98},
  pages = {14198--14201},
  number = {25}
}

@ARTICLE{Glowinski:1994,
  author = { Glowinski, R. and Pan, Tsorng-Whay and Periaux, Jacques},
  title = { A fictitious domain method for {Dirichlet} problem and applications
	
	},
  journal = {Computer Methods in Applied Mechanics and Engineering},
  year = {1994},
  volume = {111},
  pages = {283-303}
}

@ARTICLE{Gnanakaran:2003,
  author = {Gnanakaran, S. and Garcia, A. E.},
  title = {{Folding of a highly conserved diverging turn motif from the SH3
	domain}},
  journal = {Biophys J},
  year = {2003},
  volume = {84},
  pages = {1548-1562},
  number = {3}
}

@ARTICLE{Goedecker:1999,
  author = {Goedecker, S.},
  title = {Linear scaling electronic structure methods},
  journal = {Rev. Mod. Phys.},
  year = {1999},
  volume = {71},
  pages = {1085- 1123}
}

@ARTICLE{Gogonea:1994,
  author = {Gogonea, V. and E. Osawa, E.},
  title = {Implementation of solvent effect in molecular mechanics. 1. Model
	development and analytical algorithm for the solvent -Accessible
	surface area},
  journal = {Supramol. Chem.},
  year = {1994},
  volume = {3},
  pages = {303-317}
}

@ARTICLE{Gogonea:1999,
  author = {Gogonea, V. and Merz, K. M.},
  title = {Fully Quantum Mechanical Description of Proteins in Solution. Combining
	Linear Scaling Quantum Mechanical Methodologies with the Poisson-Boltzmann
	Equation},
  journal = {J. Phys. Chem. A},
  year = {1999},
  volume = {103},
  pages = {5171-5188}
}

@ARTICLE{Gogonea,
  author = {Gogonea, V. and Osawa, E. },
  title = {Implementation of Solvent Effect in Molecular Mechanics. 1. Model
	Development and Analytical Algorithm for the Solvent -Accessible
	Surface Area},
  journal = {Supramol. Chem.},
  year = {1994},
  volume = {3},
  pages = {303-317}
}

@ARTICLE{Gohlke:2004,
  author = {Gohlke, H. and Case, D. A.},
  title = {Converging free energy estimates: {MM-PB(GB)SA} studies on the protein-protein
	complex Ras-Raf},
  journal = {Journal of Computational Chemistry},
  year = {2004},
  volume = {25},
  pages = {238-250},
  number = {2},
  abstract = {Estimating protein-protein interaction energies is a very challenging
	task for current simulation protocols. Here, absolute binding free
	energies are reported for the complex H-Ras/C-Raf1 using the MM-PB(GB)SA
	approach, testing the internal consistency and model dependence of
	the results. Averaging gas-phase energies (MM), solvation free energies
	as determined by Generalized Born models (GB/SA), and entropic contributions
	calculated by normal mode analysis for snapshots obtained from 10
	ns explicit-solvent molecular dynamics in general results in an overestimation
	of the binding affinity when a solvent-accessible surface area-dependent
	model is used to estimate the nonpolar solvation contribution. Applying
	the sum of a cavity solvation free energy and explicitly modeled
	solute-solvent {van der waals} interaction energies instead provides
	less negative estimates for the nonpolar solvation contribution.
	When the polar contribution to the solvation free energy is determined
	by solving the {Poisson-Boltzmann} equation (PB) instead, the calculated
	binding affinity strongly depends on the atomic radii set chosen.
	For three GB models investigated, different absolute deviations from
	PB energies were found for the unbound proteins and the complex.
	As an alternative to normal-mode calculations, quasiharmonic analyses
	have been performed to estimate entropic contributions due to changes
	of solute flexibility upon binding. However, such entropy estimates
	do not converge after 10 ns of simulation time, indicating that sampling
	issues may limit the applicability of this approach. Finally, binding
	free energies estimated from snapshots of the unbound proteins extracted
	from the complex trajectory result in an underestimate of binding
	affinity. This points to the need to exercise caution in applying
	the computationally cheaper one-trajectory-alternative to systems
	where there may be significant changes in flexibility and structure
	due to binding. The best estimate for the binding free energy of
	Ras-Raf obtained in this study of -8.3 kcal mol-1 is in good agreement
	with the experimental result of -9.6 kcal mol-1, however, further
	probing the transferability of the applied protocol that led to this
	result is necessary. Ã‚Â??003 Wiley Periodicals, Inc. J Comput
	Chem 2: 238-250, 2003},
  annote = {Converging free energy estimates: MM-PB(GB)SA studies on the protein-protein
	complex Ras-Raf},
  bdsk-url-1 = {http://www3.interscience.wiley.com/cgi-bin/abstract/106566382/ABSTRACT},
  date-added = {2008-06-29 09:00:17 -0500},
  date-modified = {2008-06-29 09:00:17 -0500},
  keywords = {Electrostatics; Solvation},
  ty = {JOUR},
  url = {http://www3.interscience.wiley.com/cgi-bin/abstract/106566382/ABSTRACT}
}

@ARTICLE{Goj042845,
  author = {Goj, L. A. and Cisneros, G. A. and Yang, W. T. and Widenhoefer, R.
	A.},
  title = {Dramatic effect of homoallylic substitution on the rate of palladium-catalyzed
	diene cycloisomerization (vol 687, pg 498, 2003)},
  journal = {Journal of Organometallic Chemistry},
  year = {2004},
  volume = {689},
  pages = {2845-2845},
  number = {17},
  month = {Sep},
  endnotereftype = {Journal Article},
  issn = {0022-328X},
  shorttitle = {Dramatic effect of homoallylic substitution on the rate of palladium-catalyzed
	diene cycloisomerization (vol 687, pg 498, 2003)},
  url = {<Go to ISI>://000223387200013}
}

@ARTICLE{Goj03498,
  author = {Goj, L. A. and Cisneros, G. A. and Yang, W. T. and Widenhoefer, R.
	A.},
  title = {Dramatic effect of homoallylic substitution on the rate of palladium-catalyzed
	diene cycloisomerization},
  journal = {Journal of Organometallic Chemistry},
  year = {2003},
  volume = {687},
  pages = {498-507},
  number = {2},
  month = {Dec},
  abstract = {Cycloisomerization of 4,4-bis(acetoxymethyl)-1,6-heptadiene (5) catalyzed
	by [(phen)Pd(Me)CNCH3](+) [BAr4](-) [Ar = 3,5-C6H3(CF3)(2)] (2) to
	form predominantly 3,3-bis(acetoxymethyl)-1,5-dimethylcyclopentene
	(6) was similar to400 times faster than was the cycloisomerization
	of dimethyl diallylmalonate (1) under identical conditions. Mechanistic
	studies performed in conjunction with density functional theory calculations
	attribute the large rate acceleration of the cycloisomerization of
	5 relative to the cycloisomerization of 1 to the formation of a stable
	oxo chelate complex as an intermediate in the cycloisomerization
	of 1, but not in the cycloisomerization of 5. (C) 2003 Published
	by Elsevier B.V.},
  endnotereftype = {Journal Article},
  issn = {0022-328X},
  shorttitle = {Dramatic effect of homoallylic substitution on the rate of palladium-catalyzed
	diene cycloisomerization},
  url = {<Go to ISI>://000187223300035}
}

@MISC{arpack,
  author = {Francisco M. Gomes and Danny C. Sorensen},
  title = {{ARPACK}++: A {C}++ implementation of {ARPACK} eigenvalue package.}
}

@ARTICLE{Gomes:2001,
  author = {Gomes, J. and Faugeras, O. D.},
  title = {Using the Vector Distance Functions to Evolve Manifolds of Arbitrary
	Codimension},
  journal = {Lecture Notes in Computer Science},
  year = {2001},
  volume = {2106},
  pages = {1-13},
  bdsk-url-1 = {http://portal.acm.org/citation.cfm?id=715383&dl=GUIDE&coll=GUIDE},
  date-added = {2008-06-30 20:55:28 -0400},
  date-modified = {2008-06-30 20:56:16 -0400},
  url = {http://portal.acm.org/citation.cfm?id=715383&dl=GUIDE&coll=GUIDE}
}

@ARTICLE{Gong:2009,
  author = { Gong, H. P. and Freed, K. F. },
  title = { Langevin-Debye model for nonlinear electrostatic screening of solvated
	ions },
  journal = {Physical Review Letters},
  year = {2009},
  volume = {102},
  pages = {057603}
}

@ARTICLE{Gordon:2009,
  author = {Gordon, D. and Krishnamurthy, V. and Chung, S.H.},
  title = {Generalized Langevin models of molecular dynamics simulations with
	applications to ion channels},
  journal = {J. Chem. Phys.},
  year = {2009},
  volume = {131},
  pages = { },
  number = {134102}
}

@ARTICLE{Gorenflo:2001,
  author = {Gorenflo,R. and Mainardi,F. and Scalas,E. and Raberto,M. },
  title = {Fractional calculus and continuous-time Finance.III,The diffusion
	limit.Mathematical Finance(Konstanz, 2000)},
  journal = {Trends in Math., Birkhuser, Basel},
  year = {2001},
  volume = { },
  pages = {171 ?C18},
  number = { }
}

@ARTICLE{GoHuZh10,
  author = {Goroshin, R. and Q. Huynh, Q. and Zhou, H.M.},
  title = {Approximate Solution to Several Visibility Optimization Problems},
  journal = {Communications in Mathematical Sciences},
  year = {submitted 2010},
  number = { }
}

@ARTICLE{gottlieb01,
  author = {Gottlieb, D. and Hesthaven, J. S. },
  title = {Spectral methods for hyperbolic problems},
  journal = {J. Comput. Appl. Math.},
  year = {2001},
  volume = {128},
  pages = {83-131}
}

@ARTICLE{gottlieb81,
  author = {Gottlieb, D. and Lustman, L. and Orszag, S. A.},
  title = {Spectral Calculations of One-Dimensional Inviscid Compressible Flow},
  journal = {SIAM J. Sci. Stat. Comput.},
  year = {1981},
  volume = {2},
  pages = {296-310}
}

@ARTICLE{gottlieb92,
  author = {Gottlieb, D. and Shu, C. -W. and Solomonoff, A. and Vandeven, H.},
  title = {On the {{Gibbs}} phenomenon {{I}}},
  journal = {J. Comput. Appl. Math.},
  year = {1992},
  volume = {43},
  pages = {81-98}
}

@ARTICLE{gottliebtadmor84,
  author = {Gottlieb, D. and Tadmor, E.},
  title = {Recovering pointwise values of discontinuous data within spectral
	accuracy},
  journal = {Progress and Supercomputing in Computational Fluid Dynamics, Earll
	M. Murman and Saul S. Abarbanel eds.,Birkh{\"a}user},
  year = {1985},
  pages = {357-375}
}

@ARTICLE{Gouda:2003,
  author = {Gouda, H. and Kuntz, I. D. and Case, D. A. and Kollman, P. A.},
  title = {Free energy calculations for theophylline binding to an {RNA} aptamer:
	Comparison of {MM-PBSA} and thermodynamic integration methods},
  journal = {Biopolymers},
  year = {2003},
  volume = {68},
  pages = {16-34},
  number = {1},
  abstract = {We have applied the molecular mechanics {Poisson-Boltzmann} surface
	area (MM-PBSA) method (J. Srinivasan, T. E. Cheatham, P. Cieplak,
	P. A. Kollman, and D. A. Case, Journal of the American Chemical Society,
	1998, Vol. 120, pp. 9401-9409) to study the interaction of an RNA
	aptamer with theophylline and its analogs. The MM-PBSA free energy
	analysis provides a reasonable absolute binding free energy for the
	RNA aptamer-theophylline complex formation. Energetic analysis reveals
	that the {van der waals} interaction and the nonpolar contribution
	to solvation provide the basis for the favorable absolute free energy
	of complex. This trend is similar to other protein-ligand interactions
	studied previously. The MM-PBSA method also ranks the relative binding
	energies of five theophylline analogs approximately correctly, but
	not as well as the more conventional thermodynamic integration calculations,
	which were carried out to convert theophylline into its analogs.
	The comparison of MM-PBSA with TI suggests that the MM-PBSA method
	has some difficulties with the first-solvation-shell energetics.},
  annote = {Free energy calculations for theophylline binding to an RNA aptamer:
	Comparison of MM-PBSA and thermodynamic integration methods; *; Uses
	the MM/PBSA method to study ligand binding to RNA to demonstrate
	that the implicit solvent method isn't performing as well as the
	explicit solvent technique, presumably due to important interactions
	mediated by discrete water in the first hydration shell.},
  bdsk-url-1 = {http://www3.interscience.wiley.com/cgi-bin/abstract/101519811/ABSTRACT},
  date-added = {2008-06-29 09:01:11 -0500},
  date-modified = {2008-06-29 09:01:11 -0500},
  keywords = {Electrostatics; Solvation; molecular\_dynamics; nucleic\_acids},
  ty = {JOUR},
  url = {http://www3.interscience.wiley.com/cgi-bin/abstract/101519811/ABSTRACT}
}

@ARTICLE{Graf:2004,
  author = {Graf, Peter and Kurnikova, Maria G. and Coalson, Rob D. and Nitzan,
	Abraham},
  title = {Comparison of Dynamic Lattice {Monte Carlo} Simulations and the Dielectric
	Self-Energy {Poisson-Nernst-Planck} Continuum Theory for Model Ion
	Channels},
  journal = {J. Phys. Chem. B},
  year = {2004},
  volume = {108},
  pages = {2006-2015},
  month = { }
}

@ARTICLE{Sonar,
  author = {Grahs, T. and Sonar, T.},
  title = {Entropy-controlled artificial anisotropic diffusion for the numerical
	solution of conservation laws based on algorithms from image processing},
  journal = {J. Vis. Commun. Image R.},
  year = {2002},
  volume = {13},
  pages = {176-194}
}

@ARTICLE{Zap,
  author = {Grant, J. Andrew and Pickup, Barry T. and Nicholls, Anthony},
  title = {A smooth permittivity function for {{Poisson-Boltzmann}} solvation
	methods},
  journal = {Journal of Computational Chemistry},
  year = {2001},
  volume = {22},
  pages = {608-640},
  number = {6},
  abstract = {This work introduces a continuous smooth permittivity function into
	{Poisson-Boltzmann} techniques for continuum approaches to modeling
	the solvation of small molecules and proteins. The permittivity function
	is derived using a Gaussian method to describe volume exclusion.
	The new method allows a rigorous determination of solvent forces
	within a grid-based technology. The generality of approach is demonstrated
	by considering a range of applications for small molecules and macromolecules.
	We also present a very complete statistical analysis of grid errors,
	and show that the accuracy of our Gaussian-based method is improved
	over standard techniques. The method has been implemented in a new
	code called ZAP, which is freely available to academic institutions.{$[$}1{$]$}
	Ã‚Â??001 John Wiley \& Sons, Inc. J Comput Chem 22: 608-640,
	2001},
  annote = {A smooth permittivity function for {Poisson-Boltzmann} solvation
	methods},
  bdsk-url-1 = {http://www3.interscience.wiley.com/cgi-bin/abstract/78003217/ABSTRACT},
  date-added = {2008-06-29 09:01:44 -0500},
  date-modified = {2008-06-29 09:01:44 -0500},
  keywords = {Electrostatics},
  ty = {JOUR},
  url = {http://www3.interscience.wiley.com/cgi-bin/abstract/78003217/ABSTRACT}
}

@ARTICLE{Grant:2007,
  author = {Grant, J. A. and Pickup, B. T. and Sykes, M. T. and Kitchen, C. A.
	and Nicholls, A.},
  title = {The {Gaussian Generalized Born} model: application to small molecules},
  journal = {Physical Chemistry Chemical Physics},
  year = {2007},
  volume = {9},
  pages = {4913-22},
  abstract = {This work presents a Generalized Born model for the computation of
	the electrostatic component of solvation energies which is based
	on volume integration. An analytic masking function is introduced
	to remove Coulombic singularities. This approach leads to analytic
	formulae for the computation of Born radii, which are differentiable
	to arbitrary order, and computationally straightforward to implement.},
  bdsk-url-1 = {http://dx.doi.org/10.1039/b707574j},
  date-added = {2008-09-15 10:03:26 -0500},
  date-modified = {2008-09-15 10:03:26 -0500},
  keywords = {Solvation; Electrostatics},
  url = {http://dx.doi.org/10.1039/b707574j}
}

@ARTICLE{Grant:1995,
  author = {Grant, J. and Pickup, B.},
  title = {A Gaussian description of molecular shape},
  journal = {Journal of Physical Chemistry},
  year = {1995},
  volume = {99},
  pages = {3503-3510}
}

@ARTICLE{Graziano:2006,
  author = {Graziano, G.},
  title = {Scaled Particle Theory Study of the Length Scale Dependence of Cavity
	Thermodynamics in Different Liquids},
  journal = {Journal of Physical Chemistry B},
  year = {2006},
  volume = {110},
  pages = {11421-6},
  number = {23},
  abstract = {It has been noted that the work of cavity creation in water exhibits
	a crossover behavior, in that its cavity size dependence changes
	from volume dependence for small cavities to area dependence for
	larger cavities {$[$}Lum, K.; Chandler, D.; Weeks, J. D. J. Phys.
	Chem. B 1999, 103, 4570{$]$}. It is shown here that this behavior
	can be reproduced using the scaled particle theory in a straightforward
	manner for six different liquids (water, methanol, ethanol, benzene,
	cyclohexane, and carbon tetrachloride). It has also been suggested
	that the crossover is due to a change in the physical mechanism of
	the process, from one entropy-dominated to another enthalpy-dominated.
	However, the crossover behavior can be produced using the scaled
	particle theory without invoking any change in any physical mechanism.
	Also, the crossover occurs at a length scale of the size of the liquid
	molecules, as has been pointed out by others. This is the length
	regime where the work of cavity creation bears little relation to
	the bulk liquid surface tension. In addition, it is pointed out that
	cavity creation can always be considered as a purely entropy-driven
	process, which is usually accompanied by another process with compensating
	enthalpy and entropy changes.},
  annote = {Scaled Particle Theory Study of the Length Scale Dependence of Cavity
	Thermodynamics in Different Liquids},
  bdsk-url-1 = {http://dx.doi.org/10.1021/jp0571269},
  date-added = {2008-09-17 09:14:02 -0500},
  date-modified = {2008-09-17 09:14:02 -0500},
  keywords = {StatisticalMechanics; Solvation},
  ty = {JOUR},
  url = {http://dx.doi.org/10.1021/jp0571269}
}

@ARTICLE{Greer:2004,
  author = {Greer, J. B. and Bertozzi, A. L.},
  title = {H-1 solutions of a class of fourth order nonlinear equations for
	image processing},
  journal = {Discrete and Continuous Dynamical Systems},
  year = {2004},
  volume = {10},
  pages = {349-366},
  annote = {H-1 solutions of a class of fourth order nonlinear equations for
	image processing},
  date-added = {2008-09-19 10:28:56 -0500},
  date-modified = {2008-09-19 10:28:56 -0500},
  ty = {JOUR}
}

@ARTICLE{Greer:2004b,
  author = {Greer, J. B. and Bertozzi, A. L.},
  title = {Traveling wave solutions of fourth order PDEs for image processingl},
  journal = {SIAM Journal on Mathematics Analysis},
  year = {2004},
  volume = {36},
  pages = {38-68},
  annote = {Traveling wave solutions of fourth order PDEs for image processing},
  date-added = {2008-09-19 10:28:56 -0500},
  date-modified = {2008-09-19 10:28:56 -0500},
  ty = {JOUR}
}

@ARTICLE{JGreer:2004a,
  author = {Greer, J. B. and Bertozzi, A. L.},
  title = {H-1 solutions of a class of fourth order nonlinear equations for
	image processing},
  journal = {Discrete and Continuous Dynamical Systems},
  year = {2004},
  volume = {10},
  pages = {349-366},
  number = {1-2}
}

@ARTICLE{JGreer:2004b,
  author = {Greer, J. B. and Bertozzi, A. L.},
  title = {Traveling wave solutions of fourth order {{PDE}}s for image processing},
  journal = {{SIAM} Journal on Mathematical Analysis},
  year = {2004},
  volume = {36},
  pages = {38-68},
  number = {1}
}

@ARTICLE{Gregersen:2009,
  author = {Gregersen, M. M. and Okkels, F. and Bazant, M. Z. and Bruus, H},
  title = {Topology and shape optimization of induced-charge electro-osmotic
	micropumps},
  journal = {New Journal of Physics},
  year = {2009},
  volume = {11},
  pages = {075019.}
}

@ARTICLE{Griffith:2005,
  author = {Griffith, B. E. and Peskin, C. S.},
  title = {On the order of accuracy of the immersed boundary method: Higher
	order convergence rates for sufficiently smooth problems},
  journal = {J. Comput. Phys. },
  year = {2005},
  volume = {208},
  pages = {75-105},
  annote = {On the order of accuracy of the immersed boundary method: Higher
	order convergence rates for sufficiently smooth problems},
  date-added = {2008-09-19 10:28:56 -0500},
  date-modified = {2008-09-19 10:28:56 -0500},
  ty = {JOUR}
}

@ARTICLE{Grigoryev:2009,
  author = {Grigoryev, S. A. and Arya, G. and Correll, S. and Woodcock, C. L.
	and Schlick, T.},
  title = {Evidence for heteromorphic chromatin fibers from analysis of nucleosome
	interactions},
  journal = {Proc. Nat. Acad. Sci. USA},
  year = {2009},
  volume = {106},
  pages = { 13317 - 13322}
}

@MISC{DDGCourse,
  author = {Eitan Grinspun},
  title = {Discrete Differential Geometry: an applied introduction},
  year = {2006},
  note = {ACM SIGGRAPH Course}
}

@INPROCEEDINGS{EitanShells,
  author = {Eitan Grinspun and Anil~N. Hirani and Mathieu Desbrun and Peter Schr\"{o}der},
  title = {Discrete shells},
  booktitle = {ACM SIGGRAPH Symp. on Computer Animation},
  year = {2003},
  pages = {62--67}
}

@BOOK{Grisvard:1985,
  title = { Elliptic Problems in Nonsmooth Domains},
  publisher = {Pitman Advanced Pub. Program},
  year = {1985},
  author = {Grisvard, P. }
}

@ARTICLE{Grochowski:2008,
  author = {Grochowski, P. and Trylska, J},
  title = {Continuum Molecular Electrostatics, Salt Effects, and Counterion
	Binding??A Review of the Poisson?CBoltzmann Theory and Its
	Modifications},
  journal = {Biopolymers},
  year = {2008},
  volume = {89},
  pages = {93-113.},
  number = {2}
}

@ARTICLE{Grochowski:2007,
  author = {Grochowski, P. and Trylska, Joanna},
  title = {Continuum molecular electrostatics, salt effects and counterion binding.
	A review of the {{Poisson-Boltzmann}} theory and its modifications.},
  journal = {Biopolymers},
  year = {2007},
  volume = {89},
  pages = {93-113},
  number = {2},
  abstract = {This work is a review of the {Poisson-Boltzmann} (PB) continuum electrostatics
	theory and its modifications with a focus on salt effects and counterion
	binding. The PB model is one of the mesoscopic theories which describes
	the electrostatic potential and equilibrium distribution of mobile
	ions around molecules in solution. It serves as a tool to describe
	electrostatic properties of molecules, counterion association, electrostatic
	contributions to solvation and molecular binding free energies. We
	focus on general formulations which can be applied to large molecules
	of arbitrary shape in all-atomic representation, including highly
	charged biomolecules such as nucleic acids. These molecules present
	a challenge for theoretical description because the conventional
	PB model may become insufficient in those cases. We discuss the conventional
	PB equation, the corresponding functionals of the electrostatic free
	energy, including a connection to DFT, simple empirical extensions
	to this model accounting for finite size of ions, the modified PB
	theory including ionic correlations and fluctuations, the cell model
	and supplementary methods allowing to incorporate site-bound ions
	in the PB calculations. Â© 2007 Wiley Periodicals, Inc. Biopolymers,
	2007},
  address = {Interdisciplinary Centre for Mathematical and Computational Modelling,
	University of Warsaw, 02-106 Warsaw, Poland},
  bdsk-url-1 = {http://dx.doi.org/10.1002/bip.20877},
  bdsk-url-2 = {http://dx.doi.org/10.1002/bip.20877},
  date-added = {2008-09-01 14:03:06 -0500},
  date-modified = {2008-09-01 14:03:06 -0500},
  doi = {10.1002/bip.20877},
  keywords = {Electrostatics, Solvation, StatisticalMechanics; BeyondMeanField},
  priority = {0},
  url = {http://dx.doi.org/10.1002/bip.20877}
}

@ARTICLE{Grosberg:2002,
  author = {Grosberg, A.Y. and Nguyen, T.T. and Shklovskii, B.I.},
  title = {Colloquium:The physics of charge inversion in chemical and biological
	systems},
  journal = {Reviews of Modern Physics},
  year = {2002},
  volume = {74},
  pages = {329-345.},
  number = {2}
}

@INPROCEEDINGS{Eigenmeshes,
  author = {Markus Gross and Andreas Hubeli},
  title = {Eigenmeshes},
  booktitle = {ETH CS Technical Report 338},
  year = {2000},
  url = {ftp://ftp.inf.ethz.ch/pub/publications/tech-reports/3xx/338.pdf}
}

@ARTICLE{Gross:2002,
  author = {Gross, W. J. and Vasileska, D. and Ferry, D. K.},
  title = {Three-dimensional simulations of ultrasmall metal-oxide-semiconductor
	field-effect transistors: The role of the discrete impurities on
	the device terminal characteristics},
  journal = {Journal of Applied Physics},
  year = {2002},
  volume = {91},
  pages = {3737-3740},
  number = {6}
}

@ARTICLE{Gross:2000,
  author = {Gross, W. J. and Vasileska, D. and Ferry, D. K.},
  title = {{Ultrasmall MOSFETs: The Importance of the Full Coulomb Interaction
	on Device Characteristics}},
  journal = {IEEE Transactions on Electron Devices},
  year = {2000},
  volume = {47},
  pages = {1831-1837},
  number = {10}
}

@ARTICLE{Gross:1999,
  author = {Gross, W. J. and Vasileska, D. and Ferry, D. K.},
  title = {A Novel Approach for Introducing the Electron-Electron and Electron-Impurity
	Interations in Partical-Based Simulations},
  journal = {IEEE Electron Device Letters},
  year = {1999},
  volume = {20},
  pages = {463-465},
  number = {9}
}

@ARTICLE{guwei,
  author = {Gu, Y. and Wei, G. W.},
  title = {Conjugated filter approach for shock capturing},
  journal = {Commun. Numer. Meth. Engng.},
  year = {2003},
  volume = {19},
  pages = {99-110}
}

@ARTICLE{YGu:2003,
  author = {Gu, Y. and Zhou, Y. C. and Wei, G. W. },
  title = {Conjugate filters with spectral-like resolution for {2D} incompressible
	flows },
  journal = {Computers and Fluids },
  year = {2003},
  volume = {33},
  pages = {777- 794},
  number = { }
}

@ARTICLE{SGGuan:2003,
  author = { Guan, S. G. and Zhou, Y. C. and Wei, G. W. and Lai, C. H. },
  title = { Controlling flow turbulence },
  journal = {Chaos },
  year = {2003},
  volume = {13},
  pages = {64-70},
  number = { }
}

@ARTICLE{Guen05,
  author = {Eran Guendelman and Andrew Selle and Frank Losasso and Ronald Fedkiw},
  title = {{Coupling Water and Smoke to Thin Deformable and Rigid Shell}},
  journal = {ACM Trans. Graph.},
  year = {2005},
  volume = {24},
  pages = {973--981},
  number = {3}
}

@ARTICLE{Guibas1985,
  author = {Guibas, Leonidas and Stolfi, Jorge},
  title = {Primitives for the manipulation of general subdivisions and the computation
	of Voronoi},
  journal = {ACM Trans. Graph.},
  year = {1985},
  volume = {4},
  pages = {74--123},
  number = {2},
  month = apr,
  acmid = {282923},
  address = {New York, NY, USA},
  doi = {10.1145/282918.282923},
  issn = {0730-0301},
  issue_date = {April 1985},
  keywords = {Euler operators, Voronoi and Delaunay diagrams, closest point, computational
	topology, convex hull, geometric primitives, nearest neighbours,
	planar graphs, point location, representation of polynedra, trianglations},
  numpages = {50},
  publisher = {ACM},
  url = {http://doi.acm.org/10.1145/282918.282923}
}

@ARTICLE{vanGunsteren:1996,
  author = {van Gunsteren, W. F. and Billeter, S.R. and Eising, A. A. and Hunenberger,
	P. H. and Kruger, P. and Mark, A. E. and Scott, W. R. P. and Tironi,
	I. G.},
  title = {{Biomolecular Simulation: The GROMOS96 Manual and User Guide (vdf
	Hochschulverlag AG an der ETH zurich and BIOMOS b.v.: zurich, Groningen,
	1996.)}},
  journal = { },
  year = { },
  volume = { },
  pages = { }
}

@ARTICLE{Gurau:2009,
  author = {Gurau, V. and Mann, J. A.},
  title = {A Critical Overview of Computational Fluid Dynamics Multiphase Models
	for Proton Exchange Membrane Fuel Cells},
  journal = {SIAM J. Appl. Math.},
  year = {2009},
  volume = {70},
  pages = {410-454}
}

@INPROCEEDINGS{guskov02hybrid,
  author = {I. Guskov and A. Khodakovsky and P. oder and W. Sweldens},
  title = {Hybrid Meshes: Multiresolution using Regular and Irregular Refinement},
  booktitle = {Proceedings of the Eighteenth Annual Symposium on Computational Geometry},
  year = {2002},
  pages = {264--272},
  url = {citeseer.ist.psu.edu/guskov02hybrid.html}
}

@INPROCEEDINGS{Guskov,
  author = {Igor Guskov and Wim Sweldens and Peter Schr\"{o}der},
  title = {Multiresolution signal processing for meshes},
  booktitle = {SIGGRAPH '99: Proceedings of the 26th annual conference on Computer
	graphics and interactive techniques},
  year = {1999},
  pages = {325--334}
}

@ARTICLE{Guyer:2004,
  author = {Guyer, J.E. and Boettinger, W.J. and Warren, J.A.},
  title = {Phase field modeling of electrochemistry. I. Equilibrium},
  journal = {Phys. Rev. E},
  year = {2004},
  volume = {69},
  pages = {021603.}
}

@INPROCEEDINGS{Guyomarch:2004,
  author = {Guyomarch, G. and Lee, C. O.},
  title = {A discontinuous Galerkin method for elliptic interface problems with
	application to electroporation},
  booktitle = {AISTDAM Research Report},
  year = {2004},
  pages = {04--14}
}

@ARTICLE{Hache:1988,
  author = {Hache, F. and Ricard, D. and Flytzanis, C. and Kreibig, U},
  title = {The optical kerr effect in small metal particles and metal colloids:
	The case of gold },
  journal = {Appl. Phys. A },
  year = {1988},
  volume = {47},
  pages = {437- 457}
}

@BOOK{Hacker:2009,
  title = {Pharmacology: Principles and Practice},
  publisher = {Academic Press},
  year = {2009},
  author = {Hacker, M. and Messer, W. and Bachmann, K. },
  address = { },
  date-added = { },
  date-modified = { },
  keywords = { },
  ty = {THES}
}

@ARTICLE{Hadd:1999,
  author = {Hadd, A. G. and Jacobson, S. C. and Ramsey, J. M.},
  title = {Microfluidic assays of acetylcholinesterase inhibitors},
  journal = {Analytical Chemistry },
  year = {1999},
  volume = {71},
  pages = {5206-5212}
}

@ARTICLE{Hadley:2002,
  author = {Hadley, G. R.},
  title = {High-accuracy finite-difference equations for dielectric waveguide
	analysis I: uniform regions and dielectric interfaces},
  journal = {Journal of Lightwave Technology },
  year = {2002},
  volume = {20},
  pages = {1210-1218},
  annote = {High-accuracy finite-difference equations for dielectric waveguide
	analysis I: uniform regions and dielectric interfaces},
  date-added = {2008-09-19 10:28:56 -0500},
  date-modified = {2008-09-19 10:28:56 -0500},
  ty = {JOUR}
}

@ARTICLE{Han:2004,
  author = {Han, B.C. and Van der Ven, A. and Morgan, D and Ceder, G.},
  title = {Electrochemical modeling of intercalation processes with phase field
	models},
  journal = {Electrochimica Acta},
  year = {2004},
  volume = {49},
  pages = {4691-4699.}
}

@ARTICLE{HanJ:2008,
  author = {Han, J. and Fu, J. P. , and Schoch, R. B. },
  title = {Molecular Sieving Using Nanofilters: Past, Present and Future},
  journal = {Lab Chip},
  year = {2008},
  volume = {8},
  pages = {23-33},
  number = {1}
}

@ARTICLE{Han:2005,
  author = {Han, Z. Y. and Goldsman, N. and Lin, C. K.},
  title = {{Incorporation of quantum corrections to semiclassical two-dimensional
	device modeling with the Wigner-Boltzmann equation} },
  journal = {Solid-State Electronics},
  year = {2005},
  volume = {49},
  pages = {145-154 },
  annote = {Incorporation of quantum corrections to semiclassical two-dimensional
	device modeling with the Wigner-Boltzmann equation },
  date-added = {2008-11-25 10:28:56 -0500},
  date-modified = {2008-11-25 10:28:56 -0500},
  ty = {JOUR}
}

@ARTICLE{Hansbo:2002,
  author = {Hansbo, A. and Hansbo, P.},
  title = { An unfitted finite element method},
  journal = {Comput. Methods Appl. Mech. Engng},
  year = {2002},
  volume = {191},
  pages = {5537-5552}
}

@ARTICLE{Hansmann:1997,
  author = {Hansmann, U. H. E.},
  title = {{Parallel tempering algorithm for conformational studies of biological
	molecules}},
  journal = {Chem Phys Lett},
  year = {1997},
  volume = {281},
  pages = {140-150}
}

@ARTICLE{Harari:2010,
  author = {Harari, I. and Dolbow, J.},
  title = {Analysis of an efficient finite element method for embedded interface
	problems
	
	},
  journal = { Comput. Math. },
  year = {2010},
  volume = {46},
  pages = {205-211}
}

@ARTICLE{Harbola:2008,
  author = {Harbola, U. and Mukamel, S.},
  title = {{Superoperator nonequilibrium Green's function theory of many-body
	systems; applications to charge transfer and transport in open junctions}},
  journal = {Physics Report - Review Section of Physics Letters},
  year = {2008},
  volume = {465},
  pages = {191-222 },
  annote = {Superoperator nonequilibrium Green's function theory of many-body
	systems; applications to charge transfer and transport in open junctions},
  date-added = {2008-11-25 10:28:56 -0500},
  date-modified = {2008-11-25 10:28:56 -0500},
  ty = {JOUR}
}

@ARTICLE{Harms:2008,
  author = {Harms, Michael J. and Schlessman, Jamie L. and Chimenti, Michael
	S. and Sue, Gloria R. and Damjanovic, Ana and Garcia-Moreno},
  title = {A buried lysine that titrates with a normal {pKa} : Role of conformational
	flexibility at the protein-water interface as a determinant of {pKa}
	values},
  journal = {Protein Science},
  year = {2008},
  volume = {17},
  pages = {833--845},
  number = {5},
  abstract = {Previously we reported that Lys, Asp, and Glu residues at positions
	66 and 92 in staphylococcal nuclease (SNase) titrate with pKa values
	shifted by up to 5 pKa units in the direction that promotes the neutral
	state. In contrast, the internal Lys-38 in SNase titrates with a
	normal pKa . The crystal structure of the L38K variant shows that
	the side chain of Lys-38 is buried. The ionizable moiety is [~]7
	A from solvent and ion paired with Glu-122. This suggests that the
	pKa value of Lys-38 is normal because the energetic penalty for dehydration
	is offset by a favorable Coulomb interaction. However, the pKa of
	Lys-38 was also normal when Glu-122 was replaced with Gln or with
	Ala. Continuum electrostatics calculations were unable to reproduce
	the pKa of Lys-38 unless the protein was treated with an artificially
	high dielectric constant, consistent with structural reorganization
	being responsible for the normal pKa value of Lys-38. This reorganization
	must be local because circular dichroism and NMR spectroscopy indicate
	that the L38K protein is native-like under all conditions studied.
	In molecular dynamics simulations, the ion pair between Lys-38 and
	Glu-122 is unstable. The simulations show that a minor rearrangement
	of a loop is sufficient to allow penetration of water to the amino
	moiety of Lys-38. This illustrates both the important roles of local
	flexibility and water penetration as determinants of pKa values of
	ionizable groups buried near the protein-water interface, and the
	challenges faced by structure-based pKa calculations in reproducing
	these effects. 10.1110/ps.073397708},
  bdsk-url-1 = {http://dx.doi.org/10.1110/ps.073397708},
  date-added = {2008-09-16 15:43:36 -0500},
  date-modified = {2008-09-16 15:43:36 -0500},
  doi = {10.1110/ps.073397708},
  keywords = {Electrostatics, pKa, Solvation},
  posted-at = {2008-06-05 11:59:31},
  priority = {0},
  url = {http://dx.doi.org/10.1110/ps.073397708}
}

@article{bas2008very,
  title={Very fast prediction and rationalization of pKa values for protein--ligand complexes},
  author={Bas, Delphine C and Rogers, David M and Jensen, Jan H},
  journal={Proteins: Structure, Function, and Bioinformatics},
  volume={73},
  number={3},
  pages={765--783},
  year={2008},
  publisher={Wiley Online Library}
}

@incollection{yang2017spider2,
  title={Spider2: A package to predict secondary structure, accessible surface area, and main-chain torsional angles by deep neural networks},
  author={Yang, Yuedong and Heffernan, Rhys and Paliwal, Kuldip and Lyons, James and Dehzangi, Abdollah and Sharma, Alok and Wang, Jihua and Sattar, Abdul and Zhou, Yaoqi},
  booktitle={Prediction of protein secondary structure},
  pages={55--63},
  year={2017},
  publisher={Springer}
}

@ARTICLE{harten,
  author = {Harten, A. and Engquist, B. and Osher, S. and Chakravarthy, S.},
  title = {Uniform high-order accurate essentially non-oscillatory schemes,
	{III}},
  journal = {J. Comput. Phys.},
  year = {1997},
  volume = {131},
  pages = {3-47}
}

@ARTICLE{Hasegawa03838,
  author = {Hasegawa, J. Y. and Ishida, M. and Nakatsuji, H. and Lu, Z. Y. and
	Liu, H. Y. and Yang, W. T.},
  title = {Energetics of the electron transfer from bacteriopheophytin to ubiquinone
	in the photosynthetic reaction center of Rhodopseudomonas viridis:
	Theoretical study},
  journal = {Journal of Physical Chemistry B},
  year = {2003},
  volume = {107},
  pages = {838-847},
  number = {3},
  month = {Jan},
  abstract = {The energetics of electron transfer in the photosynthetic reaction
	center of Rhodopseudomonas viridis was studied using the density
	functional theory (DFT). By examining the basis set-dependence and
	the accuracy of the DFT for calculating adiabatic electron affinity,
	single-point calculations with 6-31+G(d) basis sets, at the geometry
	optimized with 6-31G(d) basis sets, were found to be almost independent
	of the basis set. In gas-phase calculations, bacteriopheophytin (H)
	had the greatest electron affinity among the three chromophores:
	H, menaquinone (MQ), and ubiquinone (UQ). However, the order of the
	electron affinity was reversed to be UQ > MQ > H by including residues
	that interacted with the chromophores through hydrogen bonding. Based
	on the QM/MM optimized geometries, cluster models for the binding
	sites were constructed. The computed reaction energy was comparable
	to values obtained experimentally. The reaction energy can be decomposed
	into a vertical electron affinity term and a relaxation energy term
	using a driving force analysis. The most important term was the vertical
	electron affinity of the chromophores. Based on optimization, there
	was little structural reorganization. The present results indicate
	that, with regard to the energetics of electron transfer, local interactions
	between the chromophores and proteins play a decisive role by tuning
	the electron affinity of the chromophores, whereas the effects of
	distant residues are of secondary importance.},
  endnotereftype = {Journal Article},
  issn = {1520-6106},
  shorttitle = {Energetics of the electron transfer from bacteriopheophytin to ubiquinone
	in the photosynthetic reaction center of Rhodopseudomonas viridis:
	Theoretical study},
  url = {<Go to ISI>://000180545300027}
}

@ARTICLE{He:2007,
  author = {He, Qing and Duan, Ye and Miles, J. and Takahashi, N.},
  title = {A Context-Sensitive Active Contour for 2D Corpus Callosum Segmentation},
  journal = {International Journal of Biomedical Imaging},
  year = {2007},
  volume = {2007},
  pages = {24826}
}

@ARTICLE{XHe:2010,
  author = { He, Xiaoming and Lin, Tao and Lin, Yanping},
  title = {Interior penalty bilinear {IFE } discontinuous {Galerkin} methods
	for elliptic equations with discontinuous coefficient},
  journal = {Journal of System Science and Complexity},
  year = {2010},
  volume = {23},
  pages = {467-483}
}

@ARTICLE{YHe:2009,
  author = {He, Y. and Gillespie, D. and Boda, D. and Vlassiouk, I. and Eisenberg,
	B. S. and Siwy, Z. S.},
  title = {Tuning Transport Properties of Nanofluidic Devices with Local Charge
	Inversion },
  journal = {Journal of the American Chemical Society },
  year = {2009},
  volume = {131},
  pages = { 5194-5202 }
}

@ARTICLE{Heaton-Burgess0736403,
  author = {Heaton-Burgess, T. and Ayers, P. and Yang, W. T.},
  title = {Spin-potential functional formalism for current-carrying noncollinear
	magnetic systems},
  journal = {Physical Review Letters},
  year = {2007},
  volume = {98},
  pages = {36403},
  number = {3},
  month = {Jan},
  abstract = {We develop a formalism dual to spin-current-density functional theory
	(CDFT) where minimization with respect to the scalar and vector spin
	potentials is used. In this way we circumvent the issues surrounding
	the nonuniqueness of the mapping between spin potentials and ground-state
	wave functions, and the v representability issue of current-density
	functionals. The approach applied within the Kohn-Sham formalism
	provides the foundations for the optimized effective potential method
	for CDFT.},
  endnotereftype = {Journal Article},
  issn = {0031-9007},
  shorttitle = {Spin-potential functional formalism for current-carrying noncollinear
	magnetic systems},
  url = {<Go to ISI>://000243587200041}
}

@ARTICLE{Heaton-Burgess07256401,
  author = {Heaton-Burgess, T. and Bulat, F. A. and Yang, W. T.},
  title = {Optimized effective potentials in finite basis sets},
  journal = {Physical Review Letters},
  year = {2007},
  volume = {98},
  pages = {256401},
  number = {25},
  month = {Jun},
  abstract = {The finite basis optimized effective potential (OEP) method within
	density functional theory is examined as an ill-posed problem. It
	is shown that the generation of nonphysical potentials is a controllable
	manifestation of the use of unbalanced, and thus unsuitable, basis
	sets. A modified functional incorporating a regularizing smoothness
	measure of the OEP is introduced. This provides a condition on balanced
	basis sets for the potential, as well as a method to determine the
	most appropriate OEP and energy from calculations performed with
	any finite basis set.},
  endnotereftype = {Journal Article},
  issn = {0031-9007},
  shorttitle = {Optimized effective potentials in finite basis sets},
  url = {<Go to ISI>://000247469400036}
}

@ARTICLE{Heaton-Burgess08114702,
  author = {Heaton-Burgess, T. and Cohen, A. J. and Yang, W. T. and Davidson,
	E. R.},
  title = {Size extensivity of the direct optimized effective potential method},
  journal = {Journal of Chemical Physics},
  year = {2008},
  volume = {128},
  pages = {114702},
  number = {11},
  month = {Mar},
  abstract = {We investigate the size extensivity of the direct optimized effective
	potential procedure of Yang and Wu [Phys. Rev. Lett. 89, 143002 (2002)].
	The choice of reference potential within the finite basis construction
	of the local Kohn-Sham potential can lead to a method that is not
	size extensive. Such a situation is encountered when one employs
	the Fermi-Amaldi potential, which is often used to enforce the correct
	asymptotic behavior of the exact exchange-correlation potential.
	The size extensivity error with the Fermi-Amaldi reference potential
	is shown to behave linearly with the number of electrons in the limit
	of an infinite number of well separated monomers. In practice, the
	error tends to be rather small and rapidly approaches the limiting
	linear behavior. Moreover, with a flexible enough potential basis
	set, the error can be decreased significantly. We also consider one
	possible reference potential, constructed from the van Leeuwen-Baerends
	potential, which provides a size extensive implementation while also
	enforcing the correct asymptotic behavior.},
  endnotereftype = {Journal Article},
  issn = {0021-9606},
  shorttitle = {Size extensivity of the direct optimized effective potential method},
  url = {<Go to ISI>://000254292500052}
}

@ARTICLE{Heaton-Burgess08194102,
  author = {Heaton-Burgess, T. and Yang, W. T.},
  title = {Optimized effective potentials from arbitrary basis sets},
  journal = {Journal of Chemical Physics},
  year = {2008},
  volume = {129},
  pages = {194102},
  number = {19},
  month = {Nov},
  abstract = {We investigate the use of a regularized optimized effective potential
	(OEP) energy functional and L-curve procedure [T. Heaton-Burgess,
	F. A. Bulat, and W. Yang, Phys. Rev. Lett. 98, 256401 (2007)] for
	determining physically meaningful OEPs from arbitrary combinations
	of finite orbital and potential basis sets. The important issue of
	the manner in which the optimal regularization parameter is determined
	from the L-curve perspective is reconsidered with the introduction
	of a rigorous measure of the quality of the potential generated-that
	being, the extent to which the Ghosh-Parr exchange energy virial
	relation is satisfied along the L-curve. This approach yields nearly
	identical potentials to our previous work employing a minimum derivative
	condition, however, gives rise to slightly lower exact-exchange total
	energies. We observe that the ground-state energy and orbital energies
	obtained from this approach, either with balanced or unbalanced basis
	sets, yield meaningful potentials and energies which are in good
	comparison to other (a priori balanced) finite basis OEP calculations
	and experimental ionization potentials. As such, we believe that
	the regularized OEP functional approach provides a computationally
	robust method to address the numerical stability issues of this often
	ill-posed problem.},
  endnotereftype = {Journal Article},
  issn = {0021-9606},
  shorttitle = {Optimized effective potentials from arbitrary basis sets},
  url = {<Go to ISI>://000261141300002}
}

@ARTICLE{Helfrich:1973,
  author = {Helfrich, W.},
  title = {Elastic Properties of Lipid Bilayers: Theory and Possible Experiments},
  journal = {Zeitschrift f\"{u}r Naturforschung Teil C},
  year = {1973},
  volume = {28},
  pages = {693 - 703}
}

@ARTICLE{Hellrung:2012,
  author = {Hellrung Jr., J. L. and Wang, L. M. and Sifakis, E. and Teran, J.
	M. },
  title = { A second order virtual node method for elliptic problems with interfaces
	and irregular domains in three dimensions
	
	},
  journal = { Journal of Computational Physics },
  year = {2012},
  volume = {231},
  pages = {2015-2048}
}

@ARTICLE{Hemsath:2005,
  author = {Hemsath, Lars and Dvorsky, Radovan and Fiegen, Dennis and Carlier,
	Marie-France and Ahmadian, Mohammad R. },
  title = {An Electrostatic Steering Mechanism of Cdc42 Recognition by Wiskott-Aldrich
	Syndrome Proteins},
  journal = {Molecular Cell},
  year = {2005},
  volume = {20},
  pages = {313--324},
  number = {2},
  abstract = {Summary The specific and rapid formation of protein complexes is essential
	for diverse cellular processes such as remodeling of actin filaments
	in response to the interaction between Rho GTPases and the Wiskott-Aldrich
	syndrome proteins (WASp and N-WASp). Although Cdc42, TC10, and other
	members of the Rho family have been implicated in binding to and
	activating the WAS proteins, the exact nature of such a protein-protein
	recognition process has remained obscure. Here, we describe a mechanism
	that ensures rapid and selective long-range Cdc42-WASp recognition.
	The crystal structure of TC10, together with mutational and bioinformatic
	analyses, proved that the basic region of WASp and two unique glutamates
	in Cdc42 generate favorable electrostatic steering forces that control
	the accelerated WASp-Cdc42 association reaction. This process is
	a prerequisite for WASp activation and a critical step in temporal
	regulation and integration of WASp-mediated cellular responses.},
  bdsk-url-1 = {http://dx.doi.org/10.1016/j.molcel.2005.08.036},
  date-added = {2008-06-30 21:55:46 -0400},
  date-modified = {2008-06-30 21:55:46 -0400},
  doi = {10.1016/j.molcel.2005.08.036},
  keywords = {diffusion, electrostatics, kinetics, protein-protein\_interactions},
  posted-at = {2008-07-01 02:55:16},
  priority = {0},
  url = {http://dx.doi.org/10.1016/j.molcel.2005.08.036}
}

@ARTICLE{MappedWENO,
  author = {A. K. Henrick and T. D. Aslam and J. M. Powers},
  title = {{Mapped Weighted Essentially Non- Oscillatory Schemes: Achieving
	optimal order near critical points}},
  journal = {J. Comp. Phys.},
  year = {2005},
  volume = {207},
  pages = {542--567}
}

@ARTICLE{Hesthaven:2003,
  author = {Hesthaven, J. S.},
  title = {High-order accurate methods in time-domain computational electromagnetics.
	A review},
  journal = {Advances in Imaging and Electron Physics },
  year = {2003},
  volume = {127},
  pages = {59-123},
  annote = {High-order accurate methods in time-domain computational electromagnetics.
	A review},
  date-added = {2008-09-19 10:28:56 -0500},
  date-modified = {2008-09-19 10:28:56 -0500},
  ty = {JOUR}
}

@ARTICLE{LagrangianLSM,
  author = {Simone E. Hieber and Petros Koumoutsakos},
  title = {{A Lagrangian particle level set method}},
  journal = {J. Comput. Phys.},
  year = {2005},
  volume = {210},
  pages = {342--367},
  number = {1}
}

@ARTICLE{Hildebrandt:2007,
  author = {Hildebrandt, A. and Blossey, R. and Rjasanow, S. and Kohlbacher,
	O. and Lenhof, H.},
  title = {Electrostatic potentials of proteins in water: a structured continuum
	approach},
  journal = {Bioinformatics},
  year = {2007},
  volume = {23},
  pages = {E99- E103},
  number = {2}
}

@ARTICLE{Hill,
  author = {Hill, D. J. and Pullin, D. I.},
  title = {Hybrid tuned center-difference-{WENO} method for large eddy simulations
	in the presence of strong shocks},
  journal = {J. Comput. Phys.},
  year = {2004},
  volume = {194},
  number = {435-450}
}

@ARTICLE{Pullin,
  author = {D. J. Hill and D. I. Pullin},
  title = {{Hybrid Tuned Center-Difference-WENO Method for Large Eddy Simulations
	in the Presence of Strong Shocks}},
  journal = {J. Comput. Phys.},
  year = {2004},
  volume = {194},
  pages = {435--450},
  number = {2}
}

@BOOK{Hille:1992,
  title = {Ionic Channels of Excitable Membranes},
  publisher = {Sunderland, MA: Sinauer Associates},
  year = {1992},
  author = {Hille, Bertil},
  address = { },
  date-added = { },
  date-modified = { },
  keywords = { },
  ty = {THES}
}

@ARTICLE{Hiptmair:2010,
  author = {Hiptmair, R. and Li, J. and Zou, J.},
  title = {Convergence analysis of finite element methods for {H(div;Omega)}-elliptic
	interface problems
	
	
	},
  journal = {J. Numer. Math.},
  year = {2010},
  volume = {18},
  pages = {187-218}
}

@PHDTHESIS{hirani:03,
  author = {Hirani, A.N.},
  title = {Discrete Exterior Calculus},
  school = {Caltech},
  year = {2003}
}

@ARTICLE{Hochberg:1978,
  author = {Hochberg, K.J.},
  title = {Signed measure on path space related to Wiener measure},
  journal = {The Annals of Probability},
  year = {1978},
  volume = {6},
  pages = {433-458},
  number = { 99}
}


%  author = {Hodgkinson, J. L.  and Horsley, A. and Stabat, D. and Simon, M. and Johnson, S. and da Fonseca, P. C. and Morris, E. P. and Wall, J. S. and Lea, S. M. and	Blocker, A. J.},
@ARTICLE{Hodgkinson2009,
  author = {Hodgkinson, J. L.  and Horsley, A. and Stabat, D. and Simon, M. and Johnson et al, S.},
  title = {Three-dimensional reconstruction of the Shigella T3SS transmembrane
	regions reveals 12-fold symmetry and novel features throughout.},
  journal = {Nat Struct Mol Biol},
  year = {2009},
  volume = {16},
  pages = {477-85--},
  number = {5},
  month = may,
  abstract = {Type III secretion systems (T3SSs) mediate bacterial protein translocation
	into eukaryotic cells, a process essential for virulence of many
	Gram-negative pathogens. They are composed of a cytoplasmic secretion
	machinery and a base that bridges both bacterial membranes, into
	which a hollow, external needle is embedded. When isolated, the latter
	two parts are termed the 'needle complex'. An incomplete understanding
	of the structure of the needle complex has hampered studies of T3SS
	function. To estimate the stoichiometry of its components, we measured
	the mass of its subdomains by scanning transmission electron microscopy
	(STEM). We determined subunit symmetries by analysis of top and side
	views within negatively stained samples in low-dose transmission
	electron microscopy (TEM). Application of 12-fold symmetry allowed
	generation of a 21-25-A resolution, three-dimensional reconstruction
	of the needle complex base, revealing many new features and permitting
	tentative docking of the crystal structure of EscJ, an inner membrane
	component.},
  address = {Sir William Dunn School of Pathology, University of Oxford, UK.},
  comment = {Research Support, Non-U.S. Gov't,Research Support, U.S. Gov't, Non-P.H.S.,Research
	Support, N.I.H., Extramural,},
  keywords = {Bacterial Proteins, Cell Membrane, Crystallography, X-Ray, Membrane
	Proteins, Microscopy, Electron, Scanning Transmission, Models, Molecular,
	Protein Structure, Secondary, Secretin, Shigella flexneri},
  owner = {SeanLab},
  timestamp = {2012.05.23},
  url = {http://ukpmc.ac.uk/abstract/MED/19396171}
}

@ARTICLE{Hohenberg:1964,
  author = {Hohenberg, P. and Kohn, W.},
  title = {Inhomogeneous electron gas},
  journal = {Phys. Rev.},
  year = {1964},
  volume = {136},
  pages = {B864-871},
  annote = {Inhomogeneous electron gas},
  date-added = {2008-11-25 10:28:56 -0500},
  date-modified = {2008-11-25 10:28:56 -0500},
  ty = {JOUR}
}

@ARTICLE{Hollerbach:2002,
  author = {Hollerbach, Uwe and Chen, DuanPin and Eisenberg, B. S. },
  title = {Two- and Three-Dimensional {Poisson-Nernst-Planck} Simulations of
	Current Flow Through {Gramicidin A}},
  journal = {Journal of Scientific Computing},
  year = {2002},
  volume = {16},
  pages = {373-409},
  number = {4},
  month = {Decemeber}
}

@BOOK{Holm:2001,
  title = {Electrostatic effects in soft matter and biophysics; NATO Science
	Series},
  publisher = {Kluwer Academic Publishers},
  year = {2001},
  author = {Holm, Christian and Kekicheff, Patrick and Podgornik, Rudolf},
  address = {Boston},
  address1 = {46},
  annote = {Electrostatic effects in soft matter and biophysics},
  date-added = {2008-09-01 14:00:49 -0500},
  date-modified = {2008-09-01 14:00:49 -0500},
  isbn = {1-4020-0196-5},
  keywords = {Electrostatics},
  ty = {BOOK}
}

@ARTICLE{Holst:2001,
  author = {Holst, M.},
  title = {Adaptive numerical treatment of elliptic systems on manifolds},
  journal = {Advances in Computational Mathematics},
  year = {2001},
  volume = {15},
  pages = {139-191},
  number = {1-4},
  abstract = {Adaptive multilevel finite element methods are developed and analyzed
	for certain elliptic systems arising in geometric analysis and general
	relativity. This class of nonlinear elliptic systems of tensor equations
	on manifolds is first reviewed, and then adaptive multilevel finite
	element methods for approximating solutions to this class of problems
	are considered in some detail. Two a posteriori error indicators
	are derived, based on local residuals and on global linearized adjoint
	or dual problems. The design of Manifold Code (MC) is then discussed;
	MC is an adaptive Multilevel finite element software package for
	2- and 3-manifolds developed over several years at Caltech and UC
	San Diego. It employs a posteriori error estimation, adaptive simplex
	subdivision, unstructured algebraic multilevel methods, global inexact
	Newton methods, and numerical continuation methods for the numerical
	solution of nonlinear covariant elliptic systems on 2- and 3-manifolds.
	Some of the more interesting features of MC are described in detail,
	including some new ideas for topology and geometry representation
	in simplex meshes, and an unusual partition of unity-based method
	for exploiting parallel computers. A short example is then given
	which involves the Hamiltonian and momentum constraints in the Einstein
	equations, a representative nonlinear 4-component covariant elliptic
	system on a Riemannian 3-manifold which arises in general relativity.
	A number of operator proper-ties and solvability results recently
	established in {$[$}55{$]$} are first summarized, making possible
	two quasi-optimal a priori error estimates for Galerkin approximations
	which are then derived. These two results complete the theoretical
	framework for effective use of adaptive multilevel finite element
	methods. A sample calculation using the MC software is then presented
	more detailed examples using MC for this application may be found
	in {$[$}26{$]$}.},
  address = {Univ Calif San Diego, Dept Math, La Jolla, CA 92093 USA},
  annote = {Adaptive numerical treatment of elliptic systems on manifolds; ISI:000174392100007;
	Kluwer Academic Publ; Times Cited: 0 Article English Cited References
	Count: 95 531aj},
  bdsk-url-1 = {http://dx.doi.org/10.1023/A:1014246117321},
  date-added = {2008-09-16 15:14:46 -0500},
  date-modified = {2008-09-16 15:14:46 -0500},
  journal1 = {Adv Comput Math},
  keywords = {Mathematics; Software},
  ty = {JOUR},
  url = {http://dx.doi.org/10.1023/A:1014246117321}
}

@PHDTHESIS{Holst:1994,
  author = {Holst, Michael},
  title = {The {Poisson-Boltzmann} equation: Analysis and multilevel numerical
	solution.},
  school = {California Institute of Technology},
  year = {1994},
  number = { }
}

@ARTICLE{Holst:2000,
  author = {Holst, M. and Baker, N. and Wang, F.},
  title = {Adaptive multilevel finite element solution of the {{Poisson-Boltzmann}}
	equation {I}. Algorithms and examples},
  journal = {Journal of Computational Chemistry},
  year = {2000},
  volume = {21},
  pages = {1319-1342},
  number = {15},
  abstract = {This article is the first of two articles on the adaptive multilevel
	finite element treatment of the nonlinear {Poisson-Boltzmann} equation
	(PBE), a nonlinear eliptic equation arising in biomolecular modeling.
	Fast and accurate numerical solution of the PBE is usually difficult
	to accomplish, due to the presence of discontinuous coefficients,
	delta functions, three spatial dimensions, unbounded domain, and
	rapid (exponential) nonlinearity. In this first article, we explain
	how adaptive multilevel finite element methods can be used to obtain
	extremely accurate solutions to the PBE with very modest computational
	resources, and we present some illustrative examples using two well-known
	test problems. The PBE is first discretized with piece-wise linear
	finite elements over a very coarse simplex triangulation of the domain.
	The resulting nonlinear algebraic equations are solved with global
	inexact Newton methods, which we have described in an article appearing
	previously in this journal. A posteriori error estimates are then
	computed from this discrete solution, which then drives a simplex
	subdivision algorithm for performing adaptive mesh refinement. The
	discretize-solve-estimate-refine procedure is then repeated, until
	a nearly uniform solution quality is obtained. The sequence of unstructured
	meshes is used to apply multilevel methods in conjunction with global
	inexact Newton methods, so that the cost of solving the nonlinear
	algebraic equations at each step approaches optimal O(N) linear complexity.
	All of the numerical procedures are implemented in MANIFOLD CODE
	(MC), a computer program designed and built by the first author over
	several years at Caltech and UC San Diego. MC is designed to solve
	a very general class of nonlinear elliptic equations on complicated
	domains in two and three dimensions. We describe some of the key
	features of MC, and give a detailed analysis of its performance for
	two model PBE problems, with comparisons to the alternative methods.
	It is shown that the best available uniform mesh-based finite difference
	or box-method algorithms, including multilevel methods, require substantially
	more time to reach a target PBE solution accuracy than the adaptive
	multilevel methods in MC. In the second article, we develop an error
	estimator based on geometric solvent accessibility, and present a
	series of detailed numerical experiments for several complex biomolecules.
	Ã‚Â??000 John Wiley \& Sons, Inc. J Comput Chem 21: 1319-1342,
	2000},
  address = {Univ Calif San Diego La Jolla, CA USA 92093 Holst, M mholst{\char64}math.ucsd.edu
	Dept Math Univ Calif San Diego La Jolla, CA USA 92093 Dept Math Univ
	Calif San Diego La Jolla, CA USA 92093 Dept Chem Univ Calif San Diego
	La Jolla, CA USA 92093 Dept Math, Sci Computat Grp Univ Calif Irvine
	Irvine, CA USA 92697 Dept Math},
  annote = {Adaptive multilevel finite element solution of the {Poisson-Boltzmann}
	equation I. Algorithms and examples; HolstEtal2000},
  bdsk-file-1 = {YnBsaXN0MDDUAQIDBAUGCQpYJHZlcnNpb25UJHRvcFkkYXJjaGl2ZXJYJG9iamVjdHMSAAGGoNE
	HCFRyb290gAFfEA9OU0tleWVkQXJjaGl2ZXKoCwwXGBkdJCVVJG51bGzTDQ4PEBEUViRjbGFzc1
	dOUy5rZXlzWk5TLm9iamVjdHOAB6ISE4ACgAOiFRaABIAGWWFsaWFzRGF0YVxyZWxhdGl2ZVBhd
	GjSDRobHFdOUy5kYXRhgAVPEQHKAAAAAAHKAAIAAAxNYWNpbnRvc2ggSEQAAAAAAAAAAAAAAAAA
	AADD4v5NSCsAAAAZYksXMjAwMC1Ib2xzdEJha2VyV2FuZy5wZGYAAAAAAAAAAAAAAAAAAAAAAAA
	AAAAAAAAAAAAAAAAAAAAAAAAAAAAAABlii8NHN1xQREYgcHJ2dwAEAAQAAAkgAAAAAAAAAAAAAA
	AAAAAAB0FyY2hpdmUAABAACAAAw+NSrQAAABEACAAAw0d9rAAAAAEAFAAZYksAGWIDAAqkKAAKp
	BEAAHrcAAIATU1hY2ludG9zaCBIRDpVc2VyczpiYWtlcjpEb2N1bWVudHM6UmVmZXJlbmNlczpB
	cmNoaXZlOjIwMDAtSG9sc3RCYWtlcldhbmcucGRmAAAOADAAFwAyADAAMAAwAC0ASABvAGwAcwB
	0AEIAYQBrAGUAcgBXAGEAbgBnAC4AcABkAGYADwAaAAwATQBhAGMAaQBuAHQAbwBzAGgAIABIAE
	QAEgBAVXNlcnMvYmFrZXIvRG9jdW1lbnRzL1JlZmVyZW5jZXMvQXJjaGl2ZS8yMDAwLUhvbHN0Q
	mFrZXJXYW5nLnBkZgATAAEvAAAVAAIADP//AADSHh8gIVgkY2xhc3Nlc1okY2xhc3NuYW1loyEi
	I11OU011dGFibGVEYXRhVk5TRGF0YVhOU09iamVjdF8QQC4uLy4uLy4uLy4uL0RvY3VtZW50cy9
	SZWZlcmVuY2VzL0FyY2hpdmUvMjAwMC1Ib2xzdEJha2VyV2FuZy5wZGbSHh8mJ6InI1xOU0RpY3
	Rpb25hcnkACAARABoAHwApADIANwA6AD8AQQBTAFwAYgBpAHAAeACDAIUAiACKAIwAjwCRAJMAn
	QCqAK8AtwC5AocCjAKVAqACpAKyArkCwgMFAwoDDQAAAAAAAAIBAAAAAAAAACgAAAAAAAAAAAAA
	AAAAAAMa},
  bdsk-url-1 = {http://www3.interscience.wiley.com/cgi-bin/abstract/73503240/ABSTRACT},
  date-added = {2008-06-28 10:32:58 -0500},
  date-modified = {2008-06-28 10:32:58 -0500},
  journal1 = {J Comput Chem},
  keywords = {Electrostatics; Mathematics},
  ty = {JOUR},
  url = {http://www3.interscience.wiley.com/cgi-bin/abstract/73503240/ABSTRACT}
}

@ARTICLE{Holst:1993a,
  author = {Holst, M. and Saied, F.},
  title = {Multigrid solution of the {{Poisson-Boltzmann}} equation},
  journal = {Journal of Computational Chemistry},
  year = {1993},
  volume = {14},
  pages = {105-13},
  number = {1},
  abstract = {A multigrid method is presented for the numerical solution of the
	linearized {Poisson-Boltzmann} equation arising in molecular biophysics.
	The equation is discretized with the finite volume method, and the
	numerical solution of the discrete equations is accomplished with
	multiple grid techniques originally developed for two-dimensional
	interface problems occurring in reactor physics. A detailed analysis
	of the resulting method is presented for several computer architectures,
	including comparisons to diagonally scaled CG, ICCG, vectorized ICCG
	and MICCG, and to SOR provided with an optimal relaxation parameter.
	The authors' results indicate that the multigrid method is superior
	to the preconditioned CG methods and SOR and that the advantage of
	multigrid grows with the problem size.},
  annote = {Multigrid solution of the {Poisson-Boltzmann} equation; Article},
  date-added = {2008-06-29 09:04:28 -0500},
  date-modified = {2008-06-29 09:04:28 -0500},
  journal1 = {J. Comput. Chem. (USA)},
  keywords = {Electrostatics; Mathematics},
  ty = {JOUR}
}

@BOOK{Holst:1993,
  title = {Multilevel Methods for the {Poisson-Boltzmann} Equation},
  publisher = {University of Illinois at Urbana-Champaign, Numerical Computing Group},
  year = {1993},
  author = {Holst, Michael J.},
  address = {Urbana-Champaign},
  date-added = {2008-06-29 09:03:26 -0500},
  date-modified = {2008-06-29 09:03:26 -0500},
  keywords = {Electrostatics; Mathematics},
  ty = {THES}
}

@ARTICLE{Holst:1995,
  author = {Holst, M. J. and Saied, F.},
  title = {Numerical solution of the nonlinear {{Poisson-Boltzmann}} equation:
	developing more robust and efficient methods},
  journal = {Journal of Computational Chemistry},
  year = {1995},
  volume = {16},
  pages = {337-64},
  number = {3},
  abstract = {We present a robust and efficient numerical method for solution of
	the nonlinear {Poisson-Boltzmann} equation arising in molecular biophysics.
	The equation is discretized with the box method, and solution of
	the discrete equations is accomplished with a global inexact-Newton
	method, combined with linear multilevel techniques we have described
	in an article appearing previously in this journal. A detailed analysis
	of the resulting method is presented, with comparisons to other methods
	that have been proposed in the literature, including the classical
	nonlinear multigrid method, the nonlinear conjugate gradient method,
	and nonlinear relaxation methods such as successive overrelaxation.
	Both theoretical and numerical evidence suggests that this method
	will converge in the case of molecules for which many of the existing
	methods will not. In addition, for problems which the other methods
	are able to solve, numerical experiments show that the new method
	is substantially more efficient, and the superiority of this method
	grows with the problem size. The method is easy to implement once
	a linear multilevel solver is available and can also easily be used
	in conjunction with linear methods other than multigrid.},
  annote = {Numerical solution of the nonlinear {Poisson-Boltzmann} equation:
	developing more robust and efficient methods; Article},
  date-added = {2008-09-16 15:14:15 -0500},
  date-modified = {2008-09-16 15:14:15 -0500},
  journal1 = {J. Comput. Chem. (USA)},
  keywords = {Electrostatics; Mathematics},
  ty = {JOUR}
}

@ARTICLE{Hong:2004,
  author = {Hong, C. and Milor, L. and Lin, M. Z.},
  title = {Analysis of the layout impact on electric fields in interconnect
	structures using finite element method},
  journal = { MICROELECTRONICS RELIABILITY },
  year = {2004},
  volume = {44},
  pages = {1867-1871 }
}

@ARTICLE{DiscontFluids,
  author = {Jeong-Mo Hong and Chang-Hun Kim},
  title = {Discontinuous fluids},
  journal = {ACM Trans. Graph.},
  year = {2005},
  volume = {24},
  pages = {915--920},
  number = {3}
}

@INPROCEEDINGS{BubblesVOF,
  author = {Jeong-Mo Hong and Chang-Hun Kim},
  title = {{Animation of Bubbles in Liquid}},
  booktitle = {Proc. of Eurographics},
  year = {2003},
  pages = {253--262}
}

@ARTICLE{Honig:1995a,
  author = {Honig, B. and Nicholls, A.},
  title = {Classical electrostatics in biology and chemistry},
  journal = {Science},
  year = {1995},
  volume = {268},
  pages = {1144-9},
  number = {5214},
  abstract = {A major revival in the use of classical electrostatics as an approach
	to the study of charged and polar molecules in aqueous solution has
	been made possible through the development of fast numerical and
	computational methods to solve the {Poisson-Boltzmann} equation for
	solute molecules that have complex shapes and charge distributions.
	Graphical visualization of the calculated electrostatic potentials
	generated by proteins and nucleic acids has revealed insights into
	the role of electrostatic interactions in a wide range of biological
	phenomena. Classical electrostatics has also proved to be successful
	quantitative tool yielding accurate descriptions of electrical potentials,
	diffusion limited processes, pH-dependent properties of proteins,
	ionic strength-dependent phenomena, and the solvation free energies
	of organic molecules.},
  address = {Department of Biochemistry and Molecular Biophysics, Columbia University,
	New York, NY 10032, USA.},
  annote = {May 26; Classical electrostatics in biology and chemistry; 7761829;
	0036-8075 Journal Article Review Review, Academic},
  bdsk-url-1 = {http://www.ncbi.nlm.nih.gov/entrez/query.fcgi?cmd=Retrieve&db=PubMed&dopt=Citation&list_uids=7761829},
  date-added = {2008-06-29 13:04:36 -0500},
  date-modified = {2008-06-29 13:04:36 -0500},
  keywords = {Electrostatics},
  ty = {JOUR},
  url = {http://www.ncbi.nlm.nih.gov/entrez/query.fcgi?cmd=Retrieve&db=PubMed&dopt=Citation&list_uids=7761829}
}

@ARTICLE{Hopp:2009,
  author = {Hopp, K. A. and Weber, K. M. and Bellissimo, D. B. and Pietz, B.
	C. and Denomme, G. A. and Curtis, B. R. and Johnson, S. T.},
  title = {Expanded Use of Nanofluidic PCR Assay for Red Cell and Platelet Antigen
	Genotyping to Predict Phenotype },
  journal = {TRANSFUSION },
  year = {2009},
  volume = {49},
  pages = {134A-134A }
}

@ARTICLE{Hori07581,
  author = {Hori, T. and Takahashi, H. and Furukawa, S. I. and Nakano, M. and
	Yang, W. T.},
  title = {Computational study on the relative acidity of acetic acid by the
	QM/MM method combined with the theory of energy representation},
  journal = {Journal of Physical Chemistry B},
  year = {2007},
  volume = {111},
  pages = {581-588},
  number = {3},
  month = {Jan},
  abstract = {We have applied the quantum mechanical/molecular mechanical (QM/MM)
	method combined with the theory of energy representation (ER) to
	study the acidity of acetic acid in aqueous solution. We have focused
	our attention on the relative acidity Delta pK(a) of the molecule
	with respect to water solvent to circumvent the ambiguity of the
	solvation free energies of the molecular species referred to as proton.
	The value of Delta pK(a) for the acetic acid has been computed as
	-11.5 when we adopt the free energy change in the gas phase obtained
	by the B3LYP functional, which is in excellent agreement with the
	experimental value of -11.0. It has been demonstrated that the QM/MM-ER
	approach recentlyanic molecules.},
  endnotereftype = {Journal Article},
  issn = {1520-6106},
  shorttitle = {Computational study on the relative acidity of acetic acid by the
	QM/MM method combined with the theory of energy representation},
  url = {<Go to ISI>://000243535900014}
}

@ARTICLE{Hori:2006,
  author = {Hori, Takumi and Takahashi, Hideaki and Nakano, Masayoshi and Nitta,
	Tomoshige and Yang, Weitao },
  title = {A QM/MM study combined with the theory of energy representation:
	Solvation free energies for anti/syn acetic acids in aqueous solution},
  journal = {Chemical Physics Letters},
  year = {2006},
  volume = {419},
  pages = {240--244},
  number = {1-3},
  abstract = {The solvation free energies for acetic acids in the anti/syn conformations
	in water solution have been computed by the novel QM/MM approach
	combined with the theory of energy representation (QM/MM-ER). To
	examine the accuracy of the methodology, we have compared the results
	with those given by experiments and other theoretical calculations.
	The solvation free energies computed by the QM/MM-ER approach are
	in reasonable agreement with corresponding experimental values. The
	free energy difference between the anti and syn conformers also agrees
	well with the results of AM1/TIP3P or RISM-SCF calculations.},
  bdsk-url-1 = {http://dx.doi.org/10.1016/j.cplett.2005.11.096},
  date-added = {2008-06-30 06:06:07 -0500},
  date-modified = {2008-06-30 06:06:07 -0500},
  doi = {10.1016/j.cplett.2005.11.096},
  keywords = {quantum\_mechanics, solvation},
  posted-at = {2008-06-30 12:05:32},
  priority = {0},
  url = {http://dx.doi.org/10.1016/j.cplett.2005.11.096}
}

@ARTICLE{Hori06240,
  author = {Hori, T. and Takahashi, H. and Nakano, M. and Nitta, T. and Yang,
	W. T.},
  journal = {Chemical Physics Letters},
  volume = {419},
  pages = {240-244},
  number = {1-3},
  month = {Feb},
  abstract = {The solvation free energies for acetic acids in the anti/syn conformations
	in water solution have been computed by the novel QM/MM approach
	combined with the theory of energy representation (QM/MM-ER). To
	examine the accuracy of the methodology, we have compared the results
	with those given by experiments and other theoretical calculations.
	The solvation free energies computed by the QM/MM-ER approach are
	in reasonable agreement with corresponding experimental values. The
	free energy difference between the anti and syn conformers also agrees
	well with the results of AM1/TIP3P or RISM-SCF calculations. (c)
	2005 Elsevier B.V. All rights reserved.},
  endnotereftype = {Journal Article},
  issn = {0009-2614},
  shorttitle = {A QM/MM study combined with the theory of energy representation: Solvation
	free energies for anti/syn acetic acids in aqueous solution},
  url = {<Go to ISI>://000235438900047}
}

@ARTICLE{Horikis:2006,
  author = {Horikis, T. P. and Kath, W. L.},
  title = {Modal analysis of circular Bragg fibers with arbitrary index profiles},
  journal = {Optics Lett. },
  year = {2006},
  volume = {31},
  pages = {3417-3419},
  annote = {Modal analysis of circular Bragg fibers with arbitrary index profiles},
  date-added = {2008-09-19 10:28:56 -0500},
  date-modified = {2008-09-19 10:28:56 -0500},
  ty = {JOUR}
}

@ARTICLE{Hormann2006MVC,
  author = {K. Hormann and M. S. Floater},
  title = {Mean Value Coordinates for Arbitrary Planar Polygons},
  journal = {ACM Transactions on Graphics},
  year = {2006},
  month = {mar}
}

@ARTICLE{Hou:2005a,
  author = {Hou, Songming and Liu, Xu-Dong},
  title = {A numerical method for solving variable coefficient elliptic equation
	with interfaces},
  journal = {J. Comput. Phys.},
  year = {2005},
  volume = {202},
  pages = {411--445},
  number = {2},
  abstract = { A new 2nd order accurate numerical method on non-body-fitting grids
	is proposed for solving the variable coefficient elliptic equation
	in disjoint subdomains [Omega]Â± separated by interfaces [Gamma].
	The variable coefficients, the source term, and hence the solution
	itself and its derivatives may be discontinuous across the interfaces.
	Jump conditions in solution and its co-normal derivative at interface
	are prescribed. Instead of smooth, the interfaces are only required
	to be Lipschitz continuous as submanifold. A weak formulation is
	developed, the existence, uniqueness and regularity of the solutions
	are studied. The numerical method is derived by discretizing the
	weak formulation. The method is different from traditional finite
	element methods. Extensive numerical experiments are presented and
	show that the method is 2nd order accurate in solution and 1st order
	accurate in its gradient in L[infinity] norm if the interface is
	C2 and solutions are C2 on the closures of the subdomains. The method
	can handle the problems when the solutions and/or the interfaces
	are weaker than C2. For example, u [set membership, variant] H2([Omega]Â±),
	[Gamma] is Lipschitz continuous and their singularities coincide,
	see Example 18 in Section 4. The accuracies of the method under various
	circumstances are listed in Table 19.},
  bdsk-url-1 = {http://www.sciencedirect.com/science/article/B6WHY-4DFK6WG-1/2/039f78dafd77c69584b8460e68036c0c},
  date-added = {2008-09-14 15:32:12 -0500},
  date-modified = {2008-09-14 15:32:12 -0500},
  doi = {10.1016/j.jcp.2004.07.016 },
  keywords = {Mathematics},
  ty = {JOUR},
  url = {http://www.sciencedirect.com/science/article/B6WHY-4DFK6WG-1/2/039f78dafd77c69584b8460e68036c0c}
}

@ARTICLE{Hou:2010,
  author = {Hou, S. M. and Wang, W. and Wang, L. Q.},
  title = {Numerical method for solving matrix coefficient elliptic equation
	with sharp-edged interfaces},
  journal = {J. Comput. Phys.},
  year = {2010},
  volume = {229},
  pages = { 7162 -7179}
}

@ARTICLE{Hou:1997,
  author = {Hou, T. Y. and Li, Z. L. and Osher, S. and Zhao, H. K.},
  title = {A Hybrid Method for Moving Interface Problems with Application to
	the Hele?Shaw Flow},
  journal = {J. Comput. Phys.},
  year = {1997},
  volume = {134},
  pages = {236--252},
  number = {2},
  abstract = { In this paper, a hybrid approach which combines theimmersed interface
	methodwith thelevel set approachis presented. The fast version of
	the immersed interface method is used to solve the differential equations
	whose solutions and their derivatives may be discontinuous across
	the interfaces due to the discontinuity of the coefficients or/and
	singular sources along the interfaces. The moving interfaces then
	are updated using the newly developed fast level set formulation
	which involves computation only inside some small tubes containing
	the interfaces. This method combines the advantage of the two approaches
	and gives a second-order {Eulerian} discretization for interface
	problems. Several key steps in the implementation are addressed in
	detail. This new approach is then applied to {Hele-Shaw} flow, an
	unstable flow involving two fluids with very different viscosity.},
  bdsk-url-1 = {http://www.sciencedirect.com/science/article/B6WHY-45SJ858-4/2/986431c3be9c2d4811362a8cd88c638e},
  date-added = {2008-09-14 15:32:12 -0500},
  date-modified = {2008-09-14 15:32:12 -0500},
  doi = {10.1006/jcph.1997.5689 },
  keywords = {Mathematics},
  ty = {JOUR},
  url = {http://www.sciencedirect.com/science/article/B6WHY-45SJ858-4/2/986431c3be9c2d4811362a8cd88c638e}
}

@ARTICLE{XYHou:2008,
  author = {Hou, X. Y. and Huang, R. and Chen, G. and Liu, S. and Zhang, X. and
	Yu, B. and Wang, Y. Y.},
  title = {A novel 10-nm physical gate length double-gate junction field effect
	transistor},
  journal = {CHINESE PHYSICS B },
  year = {2008},
  volume = {17},
  pages = {685-689}
}

@ARTICLE{HRLE,
  author = {B. Houston and M. Nielsen and C. Batty and O. Nilsson and K. Museth},
  title = {{Hierarchical RLE Level Set: A Compact and Versatile Deformable Surface
	Representation}},
  journal = {ACM Trans. on Graphics},
  year = {2006},
  volume = {25},
  pages = {151--175},
  number = {1}
}

@ARTICLE{Hsieh:2004,
  author = {Hsieh, M.J. and Luo, R.},
  title = {{Physical scoring function based on AMBER force field and Poisson-Boltzmann
	implicit solvent for protein structure prediction}},
  journal = {Proteins},
  year = {2004},
  volume = {56},
  pages = {475-486},
  number = {3}
}

@ARTICLE{Hu0814493,
  author = {Hu, H. and Boone, A. and Yang, W. T.},
  title = {Mechanism of OMP Decarboxylation in Orotidine 5 '-Monophosphate Decarboxylase},
  journal = {Journal of the American Chemical Society},
  year = {2008},
  volume = {130},
  pages = {14493-14503},
  number = {44},
  month = {Nov},
  abstract = {Despite extensive experimental and theoretical studies, the detailed
	catalytic mechanism of orotidine 5'-monophosphate decarboxylase (ODCase)
	remains controversial. In particular simulation studies using high
	level quantum mechanics have failed to reproduce experimental activation
	free energy. One common feature of many previous simulations is that
	there is a water molecule in the vicinity of the leaving CO2 group
	whose presence was only observed in the inhibitor bound complex of
	ODCase/BMP. Various roles have even been proposed for this water
	molecule from the perspective of stabilizing the transition state
	and/or intermediate state. We hypothesize that this water molecule
	is not present in the active ODCase/OMP complex. Based on QM/MM minimum
	free energy path simulations with accurate density functional methods,
	we show here that in the absence of this water molecule the enzyme
	functions through a simple direct decarboxylation mechanism. Analysis
	of the interactions in the active site indicates multiple factors
	contributing to the catalysis, including the fine-tuned electrostatic
	environment of the active site and multiple hydrogen-bonding interactions.
	To understand better the interactions between the enzyme and the
	inhibitor BMP molecule, simulations were also carried out to determine
	the binding free energy of this special water molecule in the ODCase/BMP
	complex. The results indicate that the water molecule in the active
	site plays a significant role in the binding of BMP by contributing
	similar to -3 kcal/mol to the binding free energy of the complex.
	Therefore, the complex of BMP plus a water molecule, instead of the
	BMP molecule alone, better represents the tight binding transition
	state analogue of ODCase. Our simulation results support the direct
	decarboxylation mechanism and highlight the importance of proper
	recognition of protein bound water molecules in the protein-ligand
	binding and the enzyme catalysis.},
  endnotereftype = {Journal Article},
  issn = {0002-7863},
  shorttitle = {Mechanism of OMP Decarboxylation in Orotidine 5 '-Monophosphate Decarboxylase},
  url = {<Go to ISI>://000260533400062}
}

@ARTICLE{Hu:2003,
  author = {Hu, H. and Elstner, M. and Hermans, J.},
  title = {{Comparison of a QM/MM force field and molecular mechanics force
	fields in simulations of alanine and glycine "dipeptides" (Ace-Ala-Nme
	and Ace-Gly-Nme) in water in relation to the problem of modeling
	the unfolded peptide backbone in solution}},
  journal = {Proteins},
  year = {2003},
  volume = {50},
  pages = {451-463},
  number = {3}
}

@ARTICLE{Hu075685,
  author = {Hu, H. and Lu, Z. Y. and Elstner, M. and Hermans, J. and Yang, W.
	T.},
  title = {Simulating water with the self-consistent-charge density functional
	tight binding method: From molecular clusters to the liquid state},
  journal = {Journal of Physical Chemistry A},
  year = {2007},
  volume = {111},
  pages = {5685-5691},
  number = {26},
  month = {Jul},
  abstract = {The recently developed self-consistent-charge density functional tight
	binding (SCCDFTB) method provides an accurate and inexpensive quantum
	mechanical solution to many molecular systems of interests. To examine
	the performance of the SCCDFTB method on (liquid) water, the most
	fundamental yet indispensable molecule in biological systems, we
	report here the simulation results of water in sizes ranging from
	molecular clusters to the liquid state. The latter simulation was
	achieved through the use of the linear scaling divide-and-conquer
	approach. The results of liquid water simulation indicate that the
	SCCDFTB method can describe the structural and energetics of liquid
	water in qualitative agreement with experiments, and the results
	for water clusters suggest potential future improvements of the SCCDFTB
	method.},
  endnotereftype = {Journal Article},
  issn = {1089-5639},
  shorttitle = {Simulating water with the self-consistent-charge density functional
	tight binding method: From molecular clusters to the liquid state},
  url = {<Go to ISI>://000247573600013}
}

@ARTICLE{Hu:2007,
  author = {Hu, H. and Lu, Z. Y. and Elstner, M. and Hermans, J. and Yang, W.
	T.},
  title = {Simulating water with the self-consistent-charge density functional
	tight binding method: From molecular clusters to the liquid state},
  journal = {Journal of Physical Chemistry A},
  year = {2007},
  volume = {111},
  pages = {5685-5691},
  annote = {Simulating water with the self-consistent-charge density functional
	tight binding method: From molecular clusters to the liquid state},
  date-added = {2008-09-19 10:28:56 -0500},
  date-modified = {2008-09-19 10:28:56 -0500},
  ty = {JOUR}
}

@ARTICLE{Hu0834105,
  author = {Hu, H. and Lu, Z. Y. and Parks, J. M. and Burger, S. K. and Yang,
	W. T.},
  title = {Quantum mechanics/molecular mechanics minimum free-energy path for
	accurate reaction energetics in solution and enzymes: Sequential
	sampling and optimization on the potential of mean force surface},
  journal = {Journal of Chemical Physics},
  year = {2008},
  volume = {128},
  pages = {034105},
  number = {3},
  month = {Jan},
  abstract = {To accurately determine the reaction path and its energetics for enzymatic
	and solution-phase reactions, we present a sequential sampling and
	optimization approach that greatly enhances the efficiency of the
	ab initio quantum mechanics/molecular mechanics minimum free-energy
	path (QM/MM-MFEP) method. In the QM/MM-MFEP method, the thermodynamics
	of a complex reaction system is described by the potential of mean
	force (PMF) surface of the quantum mechanical (QM) subsystem with
	a small number of degrees of freedom, somewhat like describing a
	reaction process in the gas phase. The main computational cost of
	the QM/MM-MFEP method comes from the statistical sampling of conformations
	of the molecular mechanical (MM) subsystem required for the calculation
	of the QM PMF and its gradient. In our new sequential sampling and
	optimization approach, we aim to reduce the amount of MM sampling
	while still retaining the accuracy of the results by first carrying
	out MM phase-space sampling and then optimizing the QM subsystem
	in the fixed-size ensemble of MM conformations. The resulting QM
	optimized structures are then used to obtain more accurate sampling
	of the MM subsystem. This process of sequential MM sampling and QM
	optimization is iterated until convergence. The use of a fixed-size,
	finite MM conformational ensemble enables the precise evaluation
	of the QM potential of mean force and its gradient within the ensemble,
	thus circumventing the challenges associated with statistical averaging
	and significantly speeding up the convergence of the optimization
	process. To further improve the accuracy of the QM/MM-MFEP method,
	the reaction path potential method developed by Lu and Yang [Z. Lu
	and W. Yang, J. Chem. Phys. 121, 89 (2004)] is employed to describe
	the QM/MM electrostatic interactions in an approximate yet accurate
	way with a computational cost that is comparable to classical MM
	simulations. The new method was successfully applied to two example
	reaction processes, the classical S(N)2 reaction of Cl-+CH3Cl in
	solution and the second proton transfer step of the reaction catalyzed
	by the enzyme 4-oxalocrotonate tautomerase. The activation free energies
	calculated with this new sequential sampling and optimization approach
	to the QM/MM-MFEP method agree well with results from other simulation
	approaches such as the umbrella sampling technique with direct QM/MM
	dynamics sampling, demonstrating the accuracy of the iterative QM/MM-MFEP
	method. (c) 2008 American Institute of Physics.},
  endnotereftype = {Journal Article},
  issn = {0021-9606},
  shorttitle = {Quantum mechanics/molecular mechanics minimum free-energy path for
	accurate reaction energetics in solution and enzymes: Sequential
	sampling and optimization on the potential of mean force surface},
  url = {<Go to ISI>://000252471100005}
}

@ARTICLE{HaoHu:2007,
  author = {Hu, H and Lu, Z. Y. and Yang, W. T.},
  title = {Fitting Molecular Electrostatic Potentials from Quantum Mechanical
	Calculations},
  journal = {Journal of Chemical Theory and Computation},
  year = {2007},
  volume = {3},
  pages = {1004 -- 1013}
}

@ARTICLE{Hu071004,
  author = {Hu, H. and Lu, Z. Y. and Yang, W. T.},
  title = {Fitting molecular electrostatic potentials from quantum mechanical
	calculations},
  journal = {Journal of Chemical Theory and Computation},
  year = {2007},
  volume = {3},
  pages = {1004-1013},
  number = {3},
  month = {May-Jun},
  abstract = {We develop here a new method to fit the molecular electrostatic potentials
	obtained in quantum mechanical calculations to a set of classical
	electrostatic multipoles, usually point charges located at atomic
	positions. We define an object function of fitting as an integration
	of the difference of electrostatic potentials in the entire 3-dimensional
	physical space. The object function is thus rotationally invariant
	with respect to the molecular orientation and varies smoothly with
	respect to molecular geometric fluctuations. Compared with commonly
	employed methods such as the Merz-Singh-Kollman and CHELPG schemes,
	this new method, while possessing comparable accuracy, shows greatly
	improved numerical stability with respect to the molecular positions
	and geometries. The method can be used in the fitting of electrostatic
	potentials for the molecular mechanics force fields and also can
	be applied to the calculation of electrostatic polarizabilites of
	molecular or atomic systems.},
  endnotereftype = {Journal Article},
  issn = {1549-9618},
  shorttitle = {Fitting molecular electrostatic potentials from quantum mechanical
	calculations},
  url = {<Go to ISI>://000246282600037}
}

@ARTICLE{Hu07390,
  author = {Hu, H. and Lu, Z. Y. and Yang, W. T.},
  title = {QM/MM minimum free-energy path: Methodology and application to triosephosphate
	isomerase},
  journal = {Journal of Chemical Theory and Computation},
  year = {2007},
  volume = {3},
  pages = {390-406},
  number = {2},
  month = {Mar-Apr},
  abstract = {Structural and energetic changes are two important characteristic
	properties of a chemical reaction process. In the condensed phase,
	studying these two properties is very challenging because of the
	great computational cost associated with the quantum mechanical calculations
	and phase space sampling. Although the combined quantum mechanics/molecular
	mechanics (QM/MM) approach significantly reduces the amount of the
	quantum mechanical calculations and facilitates the simulation of
	solution-phase and enzyme-catalyzed reactions, the required quantum
	mechanical calculations remain quite expensive and extensive sampling
	can be achieved routinely only with semiempirical quantum mechanical
	methods. QM/MM simulations with ab initio QM methods, therefore,
	are often restricted to narrow regions of the potential energy surface
	such as the reactant, product and transition state, or the minimum-energy
	path. Such ab initio QM/MM calculations have previously been performed
	with the QM/MM-free energy (QM/MM-FE) method of Zhang et al. (J.
	Chem. Phys. 2000, 112, 3483-3492) to generate the free-energy profile
	along the reaction coordinate using free-energy perturbation calculations
	at fixed structures of the QM subsystems. Results obtained with the
	QM/MM-FE method depend on the determination of the minimum-energy
	reaction path, which is based on local conformations of the protein/solvent
	environment and can be difficult to obtain in practice. To overcome
	the difficulties associated with the QM/MM-FE method and to further
	enhance the sampling of the MM environment conformations, we develop
	here a new method to determine the QM/MM minimum free-energy path
	(QM/MM-MFEP) for chemical-reaction processes in solution and in enzymes.
	Within the QM/MM framework, we express the free energy of the system
	as a function of the QM conformation, thus leading to a simplified
	potential of mean force (PMF) description for the thermodynamics
	of the system. The free-energy difference between two QM conformations
	is evaluated by the QM/MM free-energy perturbation method. The free-energy
	gradients with respect to the QM degrees of freedom are calculated
	from molecular dynamics simulations at given QM conformations. With
	the free energy and free-energy gradients in hand, we further implement
	chain-of-conformation optimization algorithms in the search for the
	reaction path on the free-energy surface without specifying a reaction
	coordinate. This method thus efficiently provides a unique minimum
	free-energy path for solution and enzyme reactions, with structural
	and energetic properties being determined simultaneously. To further
	incorporate the dynamic contributions of the QM subsystem into the
	simulations, we develop the reaction path potential of Lu, et al.
	(J. Chem. Phys. 2004, 121, 89-100) for the minimum free-energy path.
	The combination of the methods developed here presents a comprehensive
	and accurate treatment for the simulation of reaction processes in
	solution and in enzymes with ab initio QM/MM methods. The method
	has been demonstrated on the first step of the reaction of the enzyme
	triosephosphate isomerase with good agreement with previous studies.},
  endnotereftype = {Journal Article},
  issn = {1549-9618},
  shorttitle = {QM/MM minimum free-energy path: Methodology and application to triosephosphate
	isomerase},
  url = {<Go to ISI>://000244855300008}
}

@ARTICLE{HaoHu:2009,
  author = {Hu, H. and Yang, W. T.},
  title = {Development and application of ab initio QM/MM methods for mechanistic
	simulation of reactions in solution and in enzymes},
  journal = {J Mole. Struc. Theochem.},
  year = {2009},
  volume = {898},
  pages = {17 -- 30}
}

@ARTICLE{Hu0917,
  author = {Hu, H. and Yang, W. T.},
  title = {Development and application of ab initio QM/MM methods for mechanistic
	simulation of reactions in solution and in enzymes},
  journal = {Journal of Molecular Structure-Theochem},
  year = {2009},
  volume = {898},
  pages = {17-30},
  number = {1-3},
  month = {Mar},
  abstract = {Determining the free energies and mechanisms of chemical reactions
	in solution and enzymes is a major challenge. For such complex reaction
	processes, combined quantum mechanics/molecular mechanics (QM/MM)
	method is the most effective simulation method to provide an accurate
	and efficient theoretical description of the molecular system. The
	computational costs of ab initio QM methods, however, have limited
	the application of ab initio QM/MM methods. Recent advances in ab
	initio QM/MM methods allowed accurate simulation of the free energies
	for reactions in solution and in enzymes and thus paved the way for
	broader applications of the ab initio QM/MM methods. We review here
	the theoretical developments and applications of the ab initio QM/MM
	methods, focusing on the determination of reaction path and the free
	energies of the reaction processes in solution and enzymes. (C) 2008
	Elsevier B.V. All rights reserved.},
  endnotereftype = {Journal Article},
  isinote = {Sp. Iss. SI},
  issn = {0166-1280},
  shorttitle = {Development and application of ab initio QM/MM methods for mechanistic
	simulation of reactions in solution and in enzymes},
  url = {<Go to ISI>://000264947700004 }
}

@ARTICLE{HaoHu:2008,
  author = {Hu, H. and Yang, W. T.},
  title = {Free energies of chemical reactions in solution and in enzymes with
	ab initio quantum mechanics/molecular mechanics methods},
  journal = {Annual Rev. Phys. Chem.},
  year = {2008},
  volume = {59},
  pages = {573 -- 601}
}

@ARTICLE{Hu08573,
  author = {Hu, H. and Yang, W. T.},
  title = {Free energies of chemical reactions in solution and in enzymes with
	ab initio quantum mechanics/molecular mechanics methods},
  journal = {Annual Review of Physical Chemistry},
  year = {2008},
  volume = {59},
  pages = {573-601},
  abstract = {Combined quantum mechanics/molecular mechanics (QM/AW) methods provide
	an accurate and efficient energetic description of complex chemical
	and biological systems, leading to significant advances in the understanding
	of chemical reactions in solution and in enzymes. Here we review
	progress in QA/MM methodology and applications, focusing on ab initio
	QM-based approaches. Ab initio QM/MM methods capitalize on the accuracy
	and reliability of the associated quantum-mechanical approaches,
	however, at a much higher computational cost compared with semiempirical
	quantum-mechanical approaches. Thus reaction-path and activation
	free-energy calculations based on ab initio QM/MM methods encounter
	unique challenges in simulation timescales and phase-space sampling.
	This review features recent developments overcoming these challenges
	and enabling accurate free-energy determination for reaction processes
	in solution and in enzymes, along with applications.},
  endnotereftype = {Journal Article},
  issn = {0066-426X},
  shorttitle = {Free energies of chemical reactions in solution and in enzymes with
	ab initio quantum mechanics/molecular mechanics methods},
  url = {<Go to ISI>://000255723500023}
}

@ARTICLE{Hu0541102,
  author = {Hu, H. and Yang, W. T.},
  title = {Dual-topology/dual-coordinate free-energy simulation using QM/MM
	force field},
  journal = {Journal of Chemical Physics},
  year = {2005},
  volume = {123},
  pages = {41102},
  number = {4},
  month = {Jul},
  abstract = {We have developed a dual-topology/dual-coordinate free-energy simulation
	method for use with a QM/MM force field. By combining two parallel
	processes into one alchemical process, we are able to compute the
	double free-energy difference (Delta Delta F) within a single simulation,
	which eliminates half of the expensive quantum-mechanical simulation
	in general. The method has been tested in computing the solvation
	free-energy differences of several molecular pairs and shows close
	agreement with experimental results. (C) 2005 American Institute
	of Physics.},
  endnotereftype = {Journal Article},
  issn = {0021-9606},
  shorttitle = {Dual-topology/dual-coordinate free-energy simulation using QM/MM force
	field},
  url = {<Go to ISI>://000230991800002}
}

@ARTICLE{LHu:2012b,
  author = {Hu, Langhua and Wei, G. W.},
  title = {Nonlinear Poisson equation for heterogeneous media},
  journal = { Biophys. J.},
  year = {2012}
}

@ARTICLE{Hu:2011a,
  author = {Hu, Langhua and Zheng,Qiong and Yang,Siyang and Wei,Guo-Wei},
  title = {PDE transform for hyperbolic conservation laws},
  journal = {submitted},
  year = {2011}
}

@ARTICLE{LHu:2011a,
  author = {Hu, Langhua and Zheng, Qiong and Yang, Siyang and Wei, Guo-Wei},
  title = {PDE transform for hyperbolic conservation laws},
  journal = {submitted},
  year = {2011}
}

@ARTICLE{Hu0864102,
  author = {Hu, X. Q. and Beratan, D. N. and Yang, W. T.},
  title = {A gradient-directed Monte Carlo approach to molecular design},
  journal = {Journal of Chemical Physics},
  year = {2008},
  volume = {129},
  pages = {064102},
  number = {6},
  month = {Aug},
  abstract = {The recently developed linear combination of atomic potentials (LCAP)
	approach [M. Wang , J. Am. Chem. Soc. 128, 3228 (2006)] allows continuous
	optimization in a discrete chemical space, and thus is useful in
	the design of molecules for targeted properties. To address further
	challenges arising from the rugged, continuous property surfaces
	in the LCAP approach, we develop a gradient-directed Monte Carlo
	(GDMC) strategy as an augmentation to the original LCAP optimization
	method. The GDMC method retains the power of exploring molecular
	space by utilizing local gradient information computed from the LCAP
	approach to jump between discrete molecular structures. It also allows
	random MC moves to overcome barriers between local optima on property
	surfaces. The combined GDMC-LCAP approach is demonstrated here for
	optimizing nonlinear optical properties in a class of donor-acceptor
	substituted benzene and porphyrin frameworks. Specifically, one molecule
	with four nitrogen atoms in the porphyrin ring was found to have
	a larger first hyperpolarizability than structures with the conventional
	porphyrin motif. (C) 2008 American Institute of Physics.},
  endnotereftype = {Journal Article},
  issn = {0021-9606},
  shorttitle = {A gradient-directed Monte Carlo approach to molecular design},
  url = {<Go to ISI>://000258490600003}
}

@ARTICLE{Huang:2001a,
  author = {Huang, D. M. and Geissler, P. L. and Chandler, D. },
  title = {Scaling of Hydrophobic Solvation Free Energies},
  journal = {Journal of Physical Chemistry B},
  year = {2001},
  volume = {105},
  pages = {6704--6709},
  number = {28},
  abstract = {Abstract: We have calculated the free energy of solvation for hard
	sphere solutes, as large as 20 \r{A} in diameter, in two simple-point-charge
	models of water. These results were obtained using umbrella sampling
	of ensembles with fixed, ambient temperature and pressure. For the
	same water models, we have also calculated the surface tension of
	a liquid-vapor interface at room temperature. Analogous calculations
	were carried out for three thermodynamic states of the Lennard-Jones
	(LJ) fluid near liquid-vapor coexistence. For both water and the
	LJ fluid at the conditions we have simulated, extrapolation of our
	results suggests that the planar interface between coexisting liquid
	and vapor phases has the same surface tension as the planar limit
	of hard sphere solvation. We expect this correspondence to be a general
	result for fluids at thermodynamic states close to phase coexistence,
	as measured by the difference in chemical potential between bulk
	liquid and vapor phases, and far from the critical point. The solvation
	free energies we have computed for water and the LJ fluid cross over
	at microscopic solute sizes from a dependence on solute volume to
	an approximate dependence on solute surface area, as predicted by
	Lum et al. [J. Phys. Chem. B 1999, 103, 4570].},
  address = {Department of Chemistry, University of California at Berkeley, California
	94720},
  bdsk-url-1 = {http://dx.doi.org/10.1021/jp0104029},
  date-added = {2008-06-30 06:08:30 -0500},
  date-modified = {2008-06-30 06:08:30 -0500},
  doi = {10.1021/jp0104029},
  keywords = {nonpolar, solvation, statistical\_mechanics},
  posted-at = {2008-06-30 12:07:43},
  priority = {0},
  url = {http://dx.doi.org/10.1021/jp0104029}
}

@ARTICLE{Huang:1999b,
  author = {Huang, H. and Li, Z. L.},
  title = {Convergence analysis of the immersed interface method},
  journal = {IMA Journal of Numerical Analysis},
  year = {1999},
  volume = {19},
  pages = {583-608},
  number = {4},
  abstract = {A rigorous error analysis is given for the immersed interface method
	(IIM) applied to elliptic problems with discontinuities and singularities.
	The finite difference scheme using IIM is shown to satisfy the conditions
	of a maximum principle for a certain class of problems. Comparison
	functions are constructed to obtain error bounds for some of the
	approximate solutions. The asymptotic error expansion provides further
	useful insights and details of the behaviour and convergence properties
	of IIM, which leads to a sharper estimate of the error bound. Second-order
	convergence of IIM is indicated by the analysis. Numerical examples
	are also given to support the analytical results.},
  date-added = {2008-09-14 15:32:12 -0500},
  date-modified = {2008-09-14 15:32:12 -0500},
  keywords = {Mathematics}
}


@ARTICLE{Hua98,
  author = {Huang, N. and Shen , Z. and Long, S.R. and Wu, N.C. and Shih, H.H.
	and Zheng, Q. and Yen, N.C. and Tung, C.C. and Liu, H.H.},
  title = { The empirical mode decomposition and the {Hilbert} spectrum for
	nonlinear nonstationary time series analysi},
  journal = {Proceedings of Royal Society of London A},
  year = {1998},
  volume = {454},
  pages = {903-995},
  number = { }
}

@ARTICLE{weizhang:2008,
  author = {Huang, W. and Ma, J. T. and Russell, R. D. },
  title = {{A study of moving mesh PDE methods for numerical simulation of blowup
	in reaction diffusion equations}},
  journal = {J. Comput. Phys.},
  year = {2008},
  volume = {227},
  pages = {6532-6552}
}

@ARTICLE{weizhang:1994,
  author = {Huang, W. and Ren, Y. and Russell, R. D.},
  title = {{Moving mesh partial differential equations (MMPDES) based on the
	equidistribution principle}},
  journal = {SIAM J.Numer.Anal.},
  year = {1994},
  volume = {31},
  pages = {709--730}
}

@ARTICLE{weizhang:1999,
  author = {Huang,W and Russell, R. D.},
  title = {{Moving mesh strategy based on a gradient flow equation for two-dimensional
	problems}},
  journal = {SIAM J.Numer.Anal.},
  year = {1999},
  volume = {20},
  pages = {998--1015}
}

@ARTICLE{Hubbard:2006,
  author = {Hubbard, R. E., editor},
  title = {{Structure-Based Drug Discovery}},
  journal = {First edition ed: Royal Society of Chemistry},
  year = {2006}
}

@ARTICLE{Huber:2009,
  author = {Huber, D. E. and Markel, M. L. and Pennathur, S. and Patel, K. D.},
  title = {Oligonucleotide hybridization and free-solution electrokinetic separation
	in a nanofluidic device },
  journal = {Lab on a Chip },
  year = {2009},
  volume = {9},
  pages = {2933-2940}
}

@ARTICLE{Huiskens:1987,
  author = {Huiskens, G.},
  title = {The volume preserving mean curvature flow},
  journal = {J. Reine. Angew. Math.},
  year = {1987},
  volume = {382},
  pages = {35-48},
  annote = {The volume preserving mean curvature flow},
  date-added = {2008-09-19 10:28:56 -0500},
  date-modified = {2008-09-19 10:28:56 -0500},
  ty = {JOUR}
}

@ARTICLE{Hummer:1996a,
  author = {Hummer, G. and Garde, S. and Garc\'{i}a, A. E. and Pohorille, A.
	and Pratt, L. R.},
  title = {An information theory model of hydrophobic interactions},
  journal = {Proceedings of the National Academy of Sciences of the United States
	of America},
  year = {1996},
  volume = {93},
  pages = {8951-8955},
  number = {17},
  abstract = {A molecular model of poorly understood hydrophobic effects is heuristically
	developed using the methods of information theory. Because primitive
	hydrophobic effects can be tied to the probability of observing a
	molecular-sized cavity in the solvent, the probability distribution
	of the number of solvent centers in a cavity volume is modeled on
	the basis of the two moments available from the density and radial
	distribution of oxygen atoms in liquid water. The modeled distribution
	then yields the probability that no solvent centers are found in
	the cavity volume. This model is shown to account quantitatively
	for the central hydrophobic phenomena of cavity formation and association
	of inert gas solutes. The connection of information theory to statistical
	thermodynamics provides a basis for clarification of hydrophobic
	effects. The simplicity and flexibility of the approach suggest that
	it should permit applications to conformational equilibria of nonpolar
	solutes and hydrophobic residues in biopolymers.},
  annote = {An information theory model of hydrophobic interactions},
  bdsk-url-1 = {http://www.pnas.org/cgi/content/abstract/93/17/8951},
  date-added = {2008-06-29 13:07:35 -0500},
  date-modified = {2008-06-29 13:07:35 -0500},
  keywords = {Solvation},
  ty = {JOUR},
  url = {http://www.pnas.org/cgi/content/abstract/93/17/8951}
}

@ARTICLE{VMD,
  author = {Humphrey, W. and Dalke, A. and Schulten, K.},
  title = {{VMD} -- Visual Molecular Dynamics},
  journal = {Journal of Molecular Graphics},
  year = {1996},
  volume = {14},
  pages = {33-38},
  number = {1},
  abstract = {VMD is a molecular graphics program designed for the display and analysis
	of molecular assemblies, in particular biopolymers such as proteins
	and nucleic acids. VMD can simultaneously display any number of structures
	using a wide variety of rendering styles and coloring methods. Molecules
	are displayed as one or more {\tt{}"{}}representations,{\tt{}"{}}
	in which each representation embodies a particular rendering method
	and coloring scheme for a selected subset of atoms. The atoms displayed
	in each representation are chosen using an extensive atom selection
	syntax, which includes Boolean operators and regular expressions.
	VMD provides a complete graphical user interface for program control,
	as well as a text interface using the Tcl embeddable parser to allow
	for complex scripts with variable substitution, control loops, and
	function calls. Full session logging is supported, which produces
	a VMD command script for later playback. High-resolution raster images
	of displayed molecules may be produced by generating input scripts
	for use by a number of photorealistic image-rendering applications.
	VMD has also been expressly designed with the ability to animate
	molecular dynamics (MD) simulation trajectories, imported either
	from files or from a direct connection to a running MD simulation.
	VMD is the visualization component of MDScope, a set of tools for
	interactive problem solving in structural biology, which also includes
	the parallel MD program NAMD, and the MDCOMM software used to connect
	the visualization and simulation programs. VMD is written in C++,
	using an object-oriented design; the program, including source code
	and extensive documentation, is freely available via anonymous ftp
	and through the World Wide Web.},
  annote = {VMD -- Visual Molecular Dynamics},
  bdsk-url-1 = {http://dx.doi.org/10.1016/0263-7855(96)00018-5},
  date-added = {2008-09-17 09:17:32 -0500},
  date-modified = {2008-09-17 09:17:32 -0500},
  keywords = {Software},
  ty = {JOUR},
  url = {http://dx.doi.org/10.1016/0263-7855(96)00018-5}
}

@ARTICLE{Hunter:2002,
  author = {Hunter, John K. and Li, Z. L. and Zhao, Hongkai},
  title = {Reactive Autophobic Spreading of Drops},
  journal = {J. Comput. Phys.},
  year = {2002},
  volume = {183},
  pages = {335--366},
  number = {2},
  abstract = { We use a lubrication theory approximation to formulate a model for
	the reactive spreading of drops that deposit an autophobic monolayer
	of surfactant on a surface. The model consists of a Poisson equation
	on a moving domain with boundary conditions that depend on the history
	of the domain motion. We develop a numerical algorithm for solving
	the model, using the immersed interface method and the level-set
	method. Numerical solutions for traveling drops are qualitatively
	similar to experimental observations of reactive autophobic spreading.},
  bdsk-url-1 = {http://www.sciencedirect.com/science/article/B6WHY-47K6R7G-F/2/7ab80c20baeff48d68148534dc2dce9a},
  date-added = {2008-09-14 15:32:12 -0500},
  date-modified = {2008-09-14 15:32:12 -0500},
  doi = {10.1006/jcph.2002.7168 },
  keywords = {Diffusion; Solvation; Mathematics},
  ty = {JOUR},
  url = {http://www.sciencedirect.com/science/article/B6WHY-47K6R7G-F/2/7ab80c20baeff48d68148534dc2dce9a}
}

@ARTICLE{Husowitz:2007,
  author = {Husowitz, B. and Talanquer, V. },
  title = {Solvent density inhomogeneities and solvation free energies in supercritical
	diatomic fluids: A density functional approach},
  journal = {The Journal of Chemical Physics},
  year = {2007},
  volume = {126},
  pages = {054508},
  number = {5},
  abstract = {View this record in Web of Science},
  bdsk-url-1 = {http://link.aip.org/link/?JCPSA6/126/054508/1},
  date-added = {2008-06-29 14:29:51 -0500},
  date-modified = {2008-06-29 14:29:51 -0500},
  doi = {10.1063/1.2432327},
  keywords = {solvation, statistical\_mechanics},
  posted-at = {2008-06-29 20:27:58},
  priority = {0},
  publisher = {AIP},
  url = {http://link.aip.org/link/?JCPSA6/126/054508/1}
}

@ARTICLE{hussaini84,
  author = {Hussaini, M. Y. and Kopriva, D. A. and Salas, M. D. and Zang, T.
	A.},
  title = {Spectral methods for the Euler equation: Part {I - Fourier} methods
	and shock-capturing},
  journal = {AIAA J.},
  year = {1985},
  volume = {23},
  pages = {64-70},
  number = {No. 1}
}

@ARTICLE{Hwang:2007,
  author = { Hwang, H. and Schatz, G. C. and Ratner, M. A. },
  title = {Incorporation of Inhomogeneous Ion Diffusion Coefficients into Kinetic
	Lattice Grand Canonical {Monte Carlo} Simulations and Application
	to Ion Current Calculations in a Simple Model Ion Channel},
  journal = {J. Phys. Chem. A},
  year = {2007},
  volume = {111},
  pages = {12506-12512},
  number = {49}
}

@ARTICLE{Hwang:2006,
  author = { Hwang, H. and Schatz, G. C. and Ratner, M. A.},
  title = {Ion current calculations based on three dimensional {Poisson-Nernst-Planck}
	theory for a cyclic peptide nanotube },
  journal = {Journal of Physical Chemistry B},
  year = {2006},
  volume = {110},
  pages = {6999-7008}
}

@ARTICLE{Hyon:2010,
  author = {Hyon, YunKyong and Eisenberg, Bob and Liu, Chun},
  title = {{A mathematical model of the hard sphere repulsion in ionic solutions}},
  journal = {Communications in Mathematical Sciences},
  year = {2010},
  volume = {9},
  pages = {459-475}
}

@ARTICLE{Hyon:2011,
  author = {Hyon, Y. and Eisenberg, B. S. and Liu, Chun},
  title = {A Mathematical model for the hard sphere repulsion in ionic solution},
  journal = {Commun. Math. Sci. },
  year = {2011},
  volume = {9},
  pages = {459 - 475}
}

@ARTICLE{Iaccarino:2003,
  author = {Iaccarino, G. and Verzicco, R.},
  title = {Immersed boundary technique for turbulent flow simulations},
  journal = {Appl. Mech. Rev. },
  year = {2003},
  volume = {56},
  pages = {331-347},
  annote = {Immersed boundary technique for turbulent flow simulations},
  date-added = {2008-09-19 10:28:56 -0500},
  date-modified = {2008-09-19 10:28:56 -0500},
  ty = {JOUR}
}

@BOOK{Ikezu:2008,
  title = {Neuroimmune Pharmacology},
  publisher = {Springer},
  year = {2008},
  author = { Ikezu, T. and Gendelman, H. E. }
}

@ARTICLE{CHARMM-PB,
  author = {Im, W. and Beglov, D. and Roux, B.},
  title = {Continuum solvation model: electrostatic forces from numerical solutions
	to the {{Poisson-Boltzmann}} equation},
  journal = {Computer Physics Communications},
  year = {1998},
  volume = {111},
  pages = {59-75},
  number = {1-3},
  abstract = {A rigorous formulation of the solvation forces (first derivatives)
	associated with the electrostatic free energy calculated from numerical
	solutions of the linearized {Poisson-Boltzmann} equation on a discrete
	grid is described. The solvation forces are obtained from the formal
	solution of the linearized {Poisson-Boltzmann} equation written in
	terms of the Green function. An intermediate region for the solute-solvent
	dielectric boundary is introduced to yield a continuous solvation
	free energy and accurate solvation forces. A series of numerical
	tests show that the calculated forces agree extremely well with finite-difference
	derivatives of the solvation free energy. To gain a maximum efficiency,
	the nonpolar contribution to the free energy is expressed in terms
	of the discretized grid used for the electrostatic problem. The current
	treatment of solvation forces can be used to introduce the influence
	of a continuum solvation model in molecular mechanics calculations
	of large biological systems.},
  annote = {Continuum solvation model: electrostatic forces from numerical solutions
	to the {Poisson-Boltzmann} equation; IBR},
  bdsk-url-1 = {http://dx.doi.org/10.1016/S0010-4655(98)00016-2},
  date-added = {2008-06-29 13:08:53 -0500},
  date-modified = {2008-06-29 13:08:53 -0500},
  keywords = {Electrostatics; molecular\_simulation},
  ty = {JOUR},
  url = {http://dx.doi.org/10.1016/S0010-4655(98)00016-2}
}

@ARTICLE{Im:2002,
  author = {Im, W. and Roux, B. },
  title = {Ion Permeation and Selectivity of OmpF Porin:A Theoretical Study
	Based on Molecular Dynamics, {Brownian} Dynamics, and Continuum Electrodiffusion
	Theory},
  journal = {J. Mol. Biol.},
  year = {2002},
  volume = {322},
  pages = {851-869},
  number = { }
}

@ARTICLE{Improta:2006,
  author = {Improta, R. and Barone, V. and Scalmani, G. and Frisch, M. J.},
  title = {A state-specific polarizable continuum model time dependent density
	functional theory method for excited state calculations in solution},
  journal = {Journal of Chemical Physics},
  year = {2006},
  volume = {125},
  pages = {054103}
}

@ARTICLE{Ishikuro:1998,
  author = {Ishikuro, H. and Hiramoto, T.},
  title = {Hopping transport in multiple-dot silicon single electron MOSFET
	},
  journal = {Solid-State Electronics},
  year = {1998},
  volume = {42},
  pages = {1425-1428},
  annote = {Hopping transport in multiple-dot silicon single electron MOSFET
	},
  date-added = {2008-11-25 10:28:56 -0500},
  date-modified = {2008-11-25 10:28:56 -0500},
  ty = {JOUR}
}

@ARTICLE{Iwamoto:2006,
  author = {Iwamoto, M. and Liu, F. and Ou-Yang, Z. C.},
  title = {Shape and stability of two-dimensional lipid domains with dipole-dipole
	interactions },
  journal = {J. Chem. Phys.},
  year = {2006},
  volume = {125},
  pages = {224701}
}

@ARTICLE{Jackson,
  author = {Jackson, R.M. and Sternberg, M.J. },
  title = {DNA binding and bending by HMG boxes: Energetic determinants of specificity},
  journal = {J. Mol. Biol.},
  year = {1995},
  volume = {250},
  pages = {258-275}
}

@ARTICLE{Jackson:1995,
  author = {Jackson, Richard M. and Sternberg, Michael J. },
  title = {A Continuum Model for Protein-Protein Interactions: Application to
	the Docking Problem},
  journal = {Journal of Molecular Biology},
  year = {1995},
  volume = {250},
  pages = {258--275},
  number = {2},
  abstract = {The prediction of protein-protein interactions in solution is a major
	goal of theoretical structural biology. Here, we implement a continuum
	description of the thermodynamic processes involved. The model differs
	considerably from previous models in its use of ` molecular surface''
	area to describe the hydrophobic component to the free energy of
	conformational change in solution. We have applied this model to
	a data set of alternative docked conformations of protein-protein
	complexes which were generated independently of this work. It was
	found previously that commonly used energy evaluation techniques
	fail to distinguish between near-native and certain non-native complexes
	in this data set. Here, we found that an energy function that takes
	into account (1) total electrostatic free energy, (2) hydrophobic
	free energy and (3) loss in side-chain conformational energy was
	able to reliably discriminate between near-native and non-native
	configurations but only when molecular surface is used as a descriptor
	of the hydrophobic effect. It is shown that the molecular surface
	and the more conventional surface descriptor ` solvent accessible
	surface'' give very different quantitative measures of hydrophobicity.
	In terms of the contribution of different energy components to the
	free energy of complex formation it was found that loss in side-chain
	conformational entropy is a second order effect. Electrostatic interaction
	energy (which is commonly used to score docked conformations) was
	a poor indicator of complementarity when starting from unbound conformations.
	It was found that electrostatic desolvation energy and the hydrophobic
	contribution (based on a molecular surface area descriptor) are much
	less sensitive to local fluctuations in atomic structure than point-to-point
	interaction energies and thus may be more suited for use as a scoring
	function when docking unbound conformations, where atomic complementarity
	is much less apparent. Whilst a combined energy function was able
	to distinguish near-native from non-native energy function was able
	to distinguish near-native from non-native conformations in the six
	systems studied here, it remains to be determined to what extent
	more sizeable conformational changes would influence the results.f2},
  bdsk-url-1 = {http://dx.doi.org/10.1006/jmbi.1995.0375},
  date-added = {2008-06-30 09:37:58 -0500},
  date-modified = {2008-06-30 09:37:58 -0500},
  doi = {10.1006/jmbi.1995.0375},
  keywords = {electrostatics, protein-protein\_interactions, solvation},
  posted-at = {2008-06-30 15:37:33},
  priority = {0},
  url = {http://dx.doi.org/10.1006/jmbi.1995.0375}
}

@BOOK{Jacoboni:1989,
  title = {{The Monte Carlo Method for Semiconductor Device Simulation }},
  publisher = {New York: Springer-Verlag},
  year = {1989},
  author = {Jacoboni, C. and Lugli, P.}
}

@ARTICLE{JaTsZh08,
  author = {Jain, S. and Tsiotras, P. and Zhou, H. M.},
  title = {Adaptive Multiresolution Mesh Refinement for the Solution of Evolution
	PDE's},
  journal = {SIAM J. Sci. Comput.},
  year = {2008},
  volume = {31},
  pages = {1221-1248}
}

@INPROCEEDINGS{ShapeMatching,
  author = {Varun Jain and Hao Zhang},
  title = {Shape-Based Retrieval of Articulated 3D Models Using Spectral Embeddings},
  booktitle = {Proc. IEEE Geometric Modeling and Processing (GMP)},
  year = {2006},
  pages = {295--308}
}

@ARTICLE{Jakalian:2000,
  author = {Jakalian, Araz and Bush, Bruce L. and Jack, David B. and Bayly, Christopher
	I. },
  title = {Fast, efficient generation of high-quality atomic charges. AM1-BCC
	model: I. Method},
  journal = {Journal of Computational Chemistry},
  year = {2000},
  volume = {21},
  pages = {132--146},
  number = {2},
  abstract = {The AM1-BCC method quickly and efficiently generates high-quality
	atomic charges for use in condensed-phase simulations. The underlying
	features of the electron distribution including formal charge and
	delocalization are first captured by AM1 atomic charges for the individual
	molecule. Bond charge corrections (BCCs), which have been parameterized
	against the HF/6-31G* electrostatic potential (ESP) of a training
	set of compounds containing relevant functional groups, are then
	added using a formalism identical to the consensus BCI (bond charge
	increment) approach. As a proof of the concept, we fit BCCs simultaneously
	to 45 compounds including O-, N-, and S-containing functionalities,
	aromatics, and heteroaromatics, using only 41 BCC parameters. AM1-BCC
	yields charge sets of comparable quality to HF/6-31G* ESP-derived
	charges in a fraction of the time while reducing instabilities in
	the atomic charges compared to direct ESP-fit methods. We then apply
	the BCC parameters to a small ldquotest setrdquo consisting of aspirin,
	d-glucose, and eryodictyol; the AM1-BCC model again provides atomic
	charges of quality comparable with HF/6-31G* RESP charges, as judged
	by an increase of only 0.01 to 0.02 atomic units in the root-mean-square
	(RMS) error in ESP. Based on these encouraging results, we intend
	to parameterize the AM1-BCC model to provide a consistent charge
	model for any organic or biological molecule. Â© 2000 John Wiley
	\& Sons, Inc. J Comput Chem 21: 132-146, 2000},
  address = {Department of Chemistry and Biochemistry, Concordia University, Montr\'{e}al,
	Qu\'{e}bec, Canada; Merck Research Laboratories, Department of Molecular
	Design and Diversity, Rahway, New Jersey, USA; Merck Frosst Canada,
	Inc., PO Box 1005, Pointe-Claire-Dorval, Qu\'{e}bec H9R 4P8, Canada},
  bdsk-url-1 = {http://dx.doi.org/10.1002/(SICI)1096-987X(20000130)21:2%5C%3C132::AID-JCC5%5C%3E3.0.CO;2-P},
  bdsk-url-2 = {http://dx.doi.org/10.1002/(SICI)1096-987X(20000130)21:2%3C132::AID-JCC5%3E3.0.CO;2-P},
  date-added = {2008-06-30 21:49:44 -0400},
  date-modified = {2008-06-30 21:49:44 -0400},
  doi = {10.1002/(SICI)1096-987X(20000130)21:2<132::AID-JCC5>3.0.CO;2-P},
  keywords = {electrostatics, molecular\_dynamics, molecular\_simulation, quantum\_mechanics},
  posted-at = {2008-07-01 02:49:19},
  priority = {0},
  url = {http://dx.doi.org/10.1002/(SICI)1096-987X(20000130)21:2\%3C132::AID-JCC5\%3E3.0.CO;2-P}
}

@ARTICLE{Jakalian:2002,
  author = {Jakalian, A. and Jack, D. B. and Bayly, C. I. },
  title = {Fast, efficient generation of high-quality atomic charges. {AM1-BCC}
	model: {II}. Parameterization and validation.},
  journal = {Journal of Computational Chemistry},
  year = {2002},
  volume = {23},
  pages = {1623--1641},
  number = {16},
  abstract = {We present the first global parameterization and validation of a novel
	charge model, called AM1-BCC, which quickly and efficiently generates
	high-quality atomic charges for computer simulations of organic molecules
	in polar media. The goal of the charge model is to produce atomic
	charges that emulate the HF/6-31G* electrostatic potential (ESP)
	of a molecule. Underlying electronic structure features, including
	formal charge and electron delocalization, are first captured by
	AM1 population charges; simple additive bond charge corrections (BCCs)
	are then applied to these AM1 atomic charges to produce the AM1-BCC
	charges. The parameterization of BCCs was carried out by fitting
	to the HF/6-31G* ESP of a training set of >2700 molecules. Most organic
	functional groups and their combinations were sampled, as well as
	an extensive variety of cyclic and fused bicyclic heteroaryl systems.
	The resulting BCC parameters allow the AM1-BCC charging scheme to
	handle virtually all types of organic compounds listed in The Merck
	Index and the NCI Database. Validation of the model was done through
	comparisons of hydrogen-bonded dimer energies and relative free energies
	of solvation using AM1-BCC charges in conjunction with the 1994 Cornell
	et al. forcefield for AMBER.(13) Homo- and hetero-dimer hydrogen-bond
	energies of a diverse set of organic molecules were reproduced to
	within 0.95 kcal/mol RMS deviation from the ab initio values, and
	for DNA dimers the energies were within 0.9 kcal/mol RMS deviation
	from ab initio values. The calculated relative free energies of solvation
	for a diverse set of monofunctional isosteres were reproduced to
	within 0.69 kcal/mol of experiment. In all these validation tests,
	AMBER with the AM1-BCC charge model maintained a correlation coefficient
	above 0.96. Thus, the parameters presented here for use with the
	AM1-BCC method present a fast, accurate, and robust alternative to
	HF/6-31G* ESP-fit charges for general use with the AMBER force field
	in computer simulations involving organic small molecules.},
  address = {Boehringer Ingelheim (Canada) Ltd Research and Development, 2100
	Rue Cunard, Laval, Quebec, Canada, H7S 2G5.},
  bdsk-url-1 = {http://dx.doi.org/10.1002/jcc.10128},
  date-added = {2008-06-30 21:46:45 -0400},
  date-modified = {2008-06-30 21:46:45 -0400},
  doi = {10.1002/jcc.10128},
  issn = {0192-8651},
  keywords = {electrostatics, molecular\_dynamics, molecular\_simulation, quantum\_mechanics},
  posted-at = {2008-07-01 02:46:11},
  priority = {0},
  url = {http://dx.doi.org/10.1002/jcc.10128}
}

@ARTICLE{courantNodal,
  author = {D. Jakobson and N. Nadirashvili and J. Toth},
  title = {Geometric Properties of Eigenfunctions},
  journal = {Russian Math Surveys},
  year = {2001},
  volume = {56},
  pages = {1085--1106},
  number = {6}
}

@ARTICLE{DyRT,
  author = {Doug James and Dinesh Pai},
  title = {DyRT: Dynamic Response Textures for Real Time Deformation Simulation
	With Graphics Hardware},
  journal = {ACM Transactions on Graphics (SIGGRAPH 2002)},
  year = {2002},
  volume = {21},
  pages = {582 - 585},
  number = {3},
  month = {July},
  note = {MPEG Video available at: http://www.cs.cmu.edu/~djames/movies/dyrt.mpg}
}

@ARTICLE{Jaramillo:2005,
  author = {Jaramillo, A. and Wodak, S. J.},
  title = {{Computational protein design is a challenge for implicit solvation
	models}},
  journal = {Biophys J},
  year = {2005},
  volume = {88},
  pages = {156-171},
  number = {1}
}

@ARTICLE{Jauch:2007,
  author = {Jauch, R. and Yeo, H.C. and Kolatkar, P. R. and Clarke, N. D.},
  title = {{Assessment of CASP7 structure predictions for template free targets}},
  journal = {Proteins},
  year = {2007},
  volume = {69},
  pages = {57-67},
  number = {S8}
}

@ARTICLE{Jayaram:1998,
  author = {Jayaram, B. and Sprous, D. and Beveridge, D. L. },
  title = {Solvation Free Energy of Biomacromolecules: Parameters for a Modified
	Generalized {Born} Model Consistent with the {AMBER} Force Field},
  journal = {Journal of Physical Chemistry B},
  year = {1998},
  volume = {102},
  pages = {9571--9576},
  number = {47},
  abstract = {Abstract: The generalized Born (GB) model provides rapid estimates
	of the electrostatic free energies of solvation for diverse molecules
	and molecular ions. This method is expected to be of considerable
	utility for studies of solvation in macromolecular and biological
	systems. Calculations on biological molecules are typically based
	on empirical energy functions, each of which have their own prescriptions
	for determining net atomic charges. For maximum compatibility, GB
	parameters tailored to specific force fields are required. The development
	of parameters compatible with the AMBER force field is described.
	The method is used to estimate free energies of A and B form structures
	of DNA obtained from molecular dynamics simulations. The results
	provide an account of the conformational preferences of right-handed
	DNA in solution.},
  address = {Department of Chemistry, Wesleyan University, Middletown, Connecticut
	06459},
  bdsk-url-1 = {http://dx.doi.org/10.1021/jp982007x},
  date-added = {2008-06-30 06:10:59 -0500},
  date-modified = {2008-06-30 06:10:59 -0500},
  doi = {10.1021/jp982007x},
  keywords = {generalized\_born, molecular\_simulation, solvation},
  posted-at = {2008-06-30 12:10:27},
  priority = {0},
  url = {http://dx.doi.org/10.1021/jp982007x}
}

@BOOK{Jerome:1995,
  title = {{Analysis of Charge Transport. Mathematical Theory and Approximation
	of Semiconductor Models.}},
  publisher = {New York: Springer-Verlag},
  year = {1995},
  author = {Jerome, J.W.}
}

@ARTICLE{Jia:2008,
  author = {Jia, Z. and Aranson, I. and Karpeev, D. and Bates, P.W.},
  title = {Simulation Studies of Self-Organization of Microtubules and Molecular
	Motors},
  journal = {Phys. Rev. E},
  year = {2008},
  volume = {77},
  pages = { 051905},
  annote = {Simulation Studies of Self-Organization of Microtubules and Molecular
	Motors},
  date-added = {2008-09-19 10:28:56 -0500},
  date-modified = {2008-09-19 10:28:56 -0500},
  ty = {JOUR}
}

@ARTICLE{S-WENO,
  author = {Jiang, G. S. and Shu, C. W.},
  title = {Efficient Implementation of Weighted {ENO} Schemes},
  journal = {J. Comp. Phys.},
  year = {1996},
  volume = {126},
  pages = {202--228},
  number = {1}
}

@ARTICLE{shu96,
  author = {Jiang, G. S. and Shu, C. W.},
  title = {Efficient Implementation of Weighted {ENO} Schemes},
  journal = {J. Comp. Phys.},
  year = {1996},
  volume = {126},
  pages = {202--228},
  number = {1}
}

@ARTICLE{Jiang0326806,
  author = {Jiang, H. and Baranger, H. U. and Yang, W.},
  title = {Spin and conductance-peak-spacing distributions in large quantum
	dots: A density-functional theory study},
  journal = {Physical Review Letters},
  year = {2003},
  volume = {90},
  pages = {26806},
  number = {2},
  month = {Jan},
  abstract = {We use spin-density-functional theory to study the spacing between
	conductance peaks and the ground-state spin of 2D model quantum dots
	with up to 200 electrons. Distributions for different ranges of electron
	number are obtained in both symmetric and asymmetric potentials.
	The even/odd effect is pronounced for small symmetric dots but vanishes
	for large asymmetric ones, suggesting substantially stronger interaction
	effects than expected. The fraction of high-spin ground states is
	remarkably large.},
  endnotereftype = {Journal Article},
  issn = {0031-9007},
  shorttitle = {Spin and conductance-peak-spacing distributions in large quantum dots:
	A density-functional theory study},
  url = {<Go to ISI>://000180444200042}
}

@ARTICLE{Jiang03165337,
  author = {Jiang, H. and Baranger, H. U. and Yang, W. T.},
  title = {Density-functional theory simulation of large quantum dots},
  journal = {Physical Review B},
  year = {2003},
  volume = {68},
  pages = {165337},
  number = {16},
  month = {Oct},
  abstract = {Kohn-Sham spin-density functional theory provides an efficient and
	accurate model to study electron-electron interaction effects in
	quantum dots, but its application to large systems is a challenge.
	Here an efficient method for the simulation of quantum dots using
	density-function theory is developed; it includes the particle-in-the-box
	representation of the Kohn-Sham orbitals, an efficient conjugate-gradient
	method to directly minimize the total energy, a Fourier convolution
	approach for the calculation of the Hartree potential, and a simplified
	multigrid technique to accelerate the convergence. We test the methodology
	in a two-dimensional model system and show that numerical studies
	of large quantum dots with several hundred electrons become computationally
	affordable. In the noninteracting limit, the classical dynamics of
	the system we study can be continuously varied from integrable to
	fully chaotic. The qualitative difference in the noninteracting classical
	dynamics has an effect on the quantum properties of the interacting
	system: integrable classical dynamics leads to higher-spin states
	and a broader distribution of spacing between Coulomb blockade peaks.},
  endnotereftype = {Journal Article},
  issn = {1098-0121},
  shorttitle = {Density-functional theory simulation of large quantum dots},
  url = {<Go to ISI>://000186571800068}
}

@ARTICLE{Jiang0585313,
  author = {Jiang, H. and Ullmo, D. and Yang, W. T. and Baranger, H. U.},
  title = {Scrambling and gate-induced fluctuations in realistic quantum dots},
  journal = {Physical Review B},
  year = {2005},
  volume = {71},
  pages = {85313},
  number = {8},
  month = {Feb},
  abstract = {We evaluate the magnitude of two important mesoscopic effects using
	a realistic model of typical quantum dots. "Scrambling" and "gate
	effect" are defined as the change in the single-particle spectrum
	due to added electrons or gate-induced shape deformation, respectively.
	These two effects are investigated systematically in both the self-consistent
	Kohn-Sham (KS) theory and a Fermi liquidlike Strutinsky approach.
	We find that the,genuine scrambling effect is small because the potential
	here is smooth. In the KS theory, a key point is the implicit inclusion
	of residual interactions in the spectrum; these dominate and make
	scrambling appear larger. Finally, the gate effect is comparable
	in the two cases and, while small, is able to cause gate-induced
	spin transitions.},
  endnotereftype = {Journal Article},
  issn = {1098-0121},
  shorttitle = {Scrambling and gate-induced fluctuations in realistic quantum dots},
  url = {<Go to ISI>://000228065300055}
}

@ARTICLE{Jiang04235326,
  author = {Jiang, H. and Ullmo, D. and Yang, W. T. and Baranger, H. U.},
  title = {Electron-electron interactions in isolated and realistic quantum
	dots: A density functional theory study},
  journal = {Physical Review B},
  year = {2004},
  volume = {69},
  pages = {235326},
  number = {23},
  month = {Jun},
  abstract = {We use Kohn-Sham spin-density-functional theory to study the statistics
	of ground-state spin and the spacing between conductance peaks in
	the Coulomb blockade regime for both two-dimensional isolated and
	realistic quantum dots. We make a systematic investigation of the
	effects of electron-electron interaction strength and electron number
	on both the peak spacing and spin distributions. A direct comparison
	between the distributions from isolated and realistic dots shows
	that, despite the difference in the boundary conditions and confining
	potential, the statistical properties are qualitatively the same.
	Strong even/odd pairing in the peak spacing distribution is observed
	only in the weak e-e interaction regime and vanishes for moderate
	interactions. The probability of high spin ground states increases
	for stronger e-e interaction and seems to saturate around r(s)similar
	to4. The saturated value is larger than previous theoretical predictions.
	Both spin and conductance peak spacing distributions show substantial
	variation as the electron number increases, not saturating until
	Nsimilar to150. To interpret our numerical results, we analyze the
	spin distribution in the even N case using a simple two-level model.},
  endnotereftype = {Journal Article},
  issn = {1098-0121},
  shorttitle = {Electron-electron interactions in isolated and realistic quantum dots:
	A density functional theory study},
  url = {<Go to ISI>://000222531400079}
}

@ARTICLE{Jiang042030,
  author = {Jiang, H. and Yang, W. T.},
  title = {Conjugate-gradient optimization method for orbital-free density functional
	calculations},
  journal = {Journal of Chemical Physics},
  year = {2004},
  volume = {121},
  pages = {2030-2036},
  number = {5},
  month = {Aug},
  abstract = {Orbital-free density functional theory as an extension of traditional
	Thomas-Fermi theory has attracted a lot of interest in the past decade
	because of developments in both more accurate kinetic energy functionals
	and highly efficient numerical methodology. In this paper, we developed
	a conjugate-gradient method for the numerical solution of spin-dependent
	extended Thomas-Fermi equation by incorporating techniques previously
	used in Kohn-Sham calculations. The key ingredient of the method
	is an approximate line-search scheme and a collective treatment of
	two spin densities in the case of spin-dependent extended Thomas-Fermi
	problem. Test calculations for a quartic two-dimensional quantum
	dot system and a three-dimensional sodium cluster Na-216 with a local
	pseudopotential demonstrate that the method is accurate and efficient.
	(C) 2004 American Institute of Physics.},
  endnotereftype = {Journal Article},
  issn = {0021-9606},
  shorttitle = {Conjugate-gradient optimization method for orbital-free density functional
	calculations},
  url = {<Go to ISI>://000222680900004}
}

@ARTICLE{Jiang:2008,
  author = {Jiang, H. Y. and Shao, S. H. and Cai, W. and Zhang, P. W.},
  title = {{Boundary treatments in non-equilibrium Green's function (NEGF) methods
	for quantum transport in nano-MOSFETs} },
  journal = {J Comput. Physics},
  year = {2008},
  volume = {227},
  pages = {6553-6573 },
  annote = {Boundary treatments in non-equilibrium Green's function (NEGF) methods
	for quantum transport in nano-MOSFETs },
  date-added = {2008-11-25 10:28:56 -0500},
  date-modified = {2008-11-25 10:28:56 -0500},
  ty = {JOUR}
}

@ARTICLE{Jiang:2008a,
  author = {Jiang, X.W. and Deng, H. X. and Luo, J. W. and Li, S. S. and Wang,
	L. W.},
  title = {{A fully three-dimensional atomistic quantum mechanical study on
	random dopant-induced effects in 25-nm MOSFETs} },
  journal = {IEEE T Electron Devices},
  year = {2008},
  volume = {55},
  pages = {1720-1726 },
  annote = {A fully three-dimensional atomistic quantum mechanical study on random
	dopant-induced effects in 25-nm MOSFETs },
  date-added = {2008-11-25 10:28:56 -0500},
  date-modified = {2008-11-25 10:28:56 -0500},
  ty = {JOUR}
}

@ARTICLE{Jiang:2009,
  author = {Jiang, Y. H. and Cai, Wei},
  title = {Effect of Boundary Treatments on Quantum Transport Current in the
	Green's Function and Wigner Distribution Methods for a Nano-scale
	DG-MOSFET},
  journal = {J. Comput. Phys.},
  year = {Submitted, 2009}
}

@ARTICLE{FaceOffset,
  author = {Xiangmin Jiao},
  title = {{Face offsetting: A unified approach for explicit moving interfaces}},
  journal = {J. Comput. Phys.},
  year = {2005},
  volume = {210},
  pages = {342--367},
  number = {1}
}

@ARTICLE{Jimenez:2007,
  author = {Jimenez, D. and L. Wang, L. and Wang, Y.},
  title = {On PCM quantization errors and the white noise hypothesis},
  journal = {SIAM J. Math Analysis},
  year = {2007},
  volume = {38},
  pages = {2042 - 2056}
}

@ARTICLE{RicciFlow,
  author = {Miao Jin and Feng Luo and Xianfeng David Gu},
  title = {Computing general geometric structures on surfaces using Ricci flow},
  journal = {Comput. Aided Des.},
  year = {2007},
  volume = {39},
  pages = {663--675},
  number = {8},
  address = {Newton, MA, USA},
  doi = {http://dx.doi.org/10.1016/j.cad.2007.05.006},
  issn = {0010-4485},
  publisher = {Butterworth-Heinemann}
}

@ARTICLE{jin96,
  author = {Jin, S. and Levermore, C. D.},
  title = {Numerical schemes for hyperbolic conservation laws with stiff relaxation
	terms},
  journal = {J. Comput. Phys.},
  year = {1996},
  volume = {126},
  pages = {449-467}
}

@ARTICLE{Jin:2006,
  author = {Jin, S. and Park, Y. J. and Min, H. S.},
  title = {A three-dimensional simulation of quantum transport in silicon nanowire
	transistor in the presence of electron - phonon interactions},
  journal = {J. Appl. Phys.},
  year = {2006},
  volume = {99},
  pages = {123719-10},
  annote = {A three-dimensional simulation of quantum transport in silicon nanowire
	transistor in the presence of electron - phonon interactions},
  date-added = {2008-11-25 10:28:56 -0500},
  date-modified = {2008-11-25 10:28:56 -0500},
  ty = {JOUR}
}

@ARTICLE{Jin:2002,
  author = {Jin, Shi and Wang, Xuelei},
  title = {Robust Numerical Simulation of Porosity Evolution in Chemical Vapor
	Infiltration: {II}. Two-Dimensional Anisotropic Fronts},
  journal = {J. Comput. Phys.},
  year = {2002},
  volume = {179},
  pages = {557--577},
  number = {2},
  abstract = { A mathematical model is developed to study formation and evolution
	of pores during the chemical vapor infiltration (CVI) process. In
	this model the evolving fiber-gas interface is described by a level-set
	function with growth rate determined by the vapor precursor concentration
	and the local geometry. The vapor precursor, solely driven by diffusion,
	is described by a boundary value problem of the Laplace equation.
	We then numerically solve this model using the immersed interface
	method and a fast searching method developed by the authors for pore
	detection. This model is able to numerically advance the fiber-gas
	interface and automatically handle fiber merging and pore formation.
	Numerical experiments are conducted to validate this model and the
	corresponding numerical algorithm.},
  bdsk-url-1 = {http://www.sciencedirect.com/science/article/B6WHY-463X8CK-B/2/bc4a8a1783d2c23ea12938103941115d},
  date-added = {2008-09-14 15:32:12 -0500},
  date-modified = {2008-09-14 15:32:12 -0500},
  doi = {10.1006/jcph.2002.707},
  keywords = {Misc; Mathematics; Diffusion},
  ty = {JOUR},
  url = {http://www.sciencedirect.com/science/article/B6WHY-463X8CK-B/2/bc4a8a1783d2c23ea12938103941115d}
}

@ARTICLE{ZJin:2010,
  author = {Jin, Z. M. and Yang, X. P.},
  title = {{Strong solutions for the generalized Perona-Malik equation for image
	restoration}},
  journal = {Nonlinear Analysis-Theory Methods and Applications},
  year = {2010},
  volume = {73},
  pages = {1077-1084},
  number = {4}
}

@ARTICLE{ZMJin:2010,
  author = {Jin, Z. M. and Yang, X. P.},
  title = {Strong solutions for the generalized Perona-Malik equation for image
	restoration},
  journal = {Nonlinear Analysis-Theory Methods and Applications},
  year = {2010},
  volume = {73},
  pages = {1077-1084}
}

@ARTICLE{Jinnouchi:2008,
  author = {Jinnouchi, R. and Anderson, A. B.},
  title = {Electronic structure calculations of liquid-solid interfaces: Combination
	of density functional theory and modified {Poisson-Boltzmann} theory},
  journal = { PHYSICAL REVIEW B },
  year = {2008},
  volume = {77},
  pages = {245417 }
}

@ARTICLE{Jo:2008,
  author = {Jo, S. and Vargyas, M. and Vasko-Szedlar, J. and Roux, B. and Im,
	W.},
  title = {PBEQ-Solver for online visualization of electrostatic potential of
	biomolecules},
  journal = {Nucleic Acids Research},
  year = {2008},
  volume = {36},
  pages = {W270 -W275}
}

@ARTICLE{Jogai:2003,
  author = {Jogai, B. },
  title = {Influence of surface states on the two-dimensional electron gas in
	AlGaN/GaN heterojunction field-effect transistors },
  journal = {J. Applied Physics},
  year = {2003},
  volume = {93},
  pages = {1631-1635 },
  annote = {Influence of surface states on the two-dimensional electron gas in
	AlGaN/GaN heterojunction field-effect transistors },
  date-added = {2008-11-25 10:28:56 -0500},
  date-modified = {2008-11-25 10:28:56 -0500},
  ty = {JOUR}
}

@ARTICLE{Johansen:1998,
  author = {Johansen, Hans and Colella, Phillip},
  title = {A {Cartesian} Grid Embedded Boundary Method for {Poisson}'s Equation
	on Irregular Domains},
  journal = {J. Comput. Phys.},
  year = {1998},
  volume = {147},
  pages = {60--85},
  number = {1},
  abstract = { We present a numerical method for solving Poisson's equation, with
	variable coefficients and {Dirichlet} boundary conditions, on two-dimensional
	regions. The approach uses a finite-volume discretization, which
	embeds the domain in a regular Cartesian grid. We treat the solution
	as a cell-centered quantity, even when those centers are outside
	the domain. Cells that contain a portion of the domain boundary use
	conservative differencing of second-order accurate fluxes on each
	cell volume. The calculation of the boundary flux ensures that the
	conditioning of the matrix is relatively unaffected by small cell
	volumes. This allows us to use multigrid iterations with a simple
	point relaxation strategy. We have combined this with an adaptive
	mesh refinement (AMR) procedure. We provide evidence that the algorithm
	is second-order accurate on various exact solutions and compare the
	adaptive and nonadaptive calculations.},
  bdsk-url-1 = {http://www.sciencedirect.com/science/article/B6WHY-45J58SM-S/2/b657bd207093d513f78ea2e7d1e94600},
  date-added = {2008-09-14 15:32:12 -0500},
  date-modified = {2008-09-14 15:32:12 -0500},
  doi = {10.1006/jcph.1998.5965 },
  keywords = {Electrostatics; Mathematics},
  ty = {JOUR},
  url = {http://www.sciencedirect.com/science/article/B6WHY-45J58SM-S/2/b657bd207093d513f78ea2e7d1e94600}
}

@ARTICLE{Johansen,
  author = {Johansen, S. T. and Wu, J. Y. and Shyy, W.},
  title = {Filter-based unsteady RANS computations},
  journal = {Int. J. Heat Fluid Flow},
  year = {2004},
  volume = {25},
  pages = {10-21}
}

@ARTICLE{SpinImages99,
  author = {Johnson, AE and Hebert, M.},
  title = {{Using spin images for efficient object recognition in cluttered
	3Dscenes}},
  journal = {IEEE Trans. on PAMI},
  year = {1999},
  volume = {21},
  pages = {433-449},
  number = {5}
}

@ARTICLE{Johnson08204112,
  author = {Johnson, E. R. and Mori-Sanchez, P. and Cohen, A. J. and Yang, W.
	T.},
  title = {Delocalization errors in density functionals and implications for
	main-group thermochemistry},
  journal = {Journal of Chemical Physics},
  year = {2008},
  volume = {129},
  pages = {204112},
  number = {20},
  month = {Nov},
  abstract = {The difficulty of approximate density functionals in describing the
	energetics of Diels-Alder reactions and dimerization of aluminum
	complexes is analyzed. Both of these reaction classes involve formation
	of cyclic or bicyclic products, which are found to be underbound
	by the majority of functionals considered. We present a consistent
	view of these results from the perspective of delocalization error.
	This error causes approximate functionals to give too low energy
	for delocalized densities or too high energy for localized densities,
	as in the cyclic and bicyclic reaction products. This interpretation
	allows us to understand better a wide range of errors in main-group
	thermochemistry obtained with popular density functionals. In general,
	functionals with minimal delocalization error should be used for
	theoretical studies of reactions where there is a loss of extended
	conjugation or formation of highly branched, cyclic, and cagelike
	molecules.},
  endnotereftype = {Journal Article},
  issn = {0021-9606},
  shorttitle = {Delocalization errors in density functionals and implications for
	main-group thermochemistry},
  url = {<Go to ISI>://000261212200015}
}

@ARTICLE{Jones:1999,
  author = {Jones, D. T.},
  title = {{Protein secondary structure prediction based on position-specific
	scoring matrices}},
  journal = {J Mol Biol},
  year = {1999},
  volume = {292},
  pages = {195-202}
}

@ARTICLE{JDD03,
  author = {Thouis R. Jones and Fr{\'e}do Durand and Mathieu Desbrun},
  title = {Non-iterative, Feature-Preserving Mesh Smoothing},
  journal = {ACM Trans. on Graphics (SIGGRAPH)},
  year = {2003},
  volume = {22},
  pages = {943--949},
  number = {3},
  month = jun
}

@ARTICLE{Jorgensen:1996,
  author = {Jorgensen, W. L. and Maxwell, D. S. and Tirado-Rives, J.},
  title = {{Development and Testing of the OPLS All-Atom Force Field on Conformational
	Energetics and Properties of Organic Liquids}},
  journal = {J Am Chem Soc},
  year = {1996},
  volume = {118},
  pages = {11225-11236}
}

@INPROCEEDINGS{JTDP03,
  author = {Pushkar Joshi and Wen Tien and Mathieu Desbrun and Fred Pighin},
  title = {Learning Controls for Blendshape-based Realistic Facial Animation},
  booktitle = {EG/SIGGRAPH Symposium on Computer Animation},
  year = {2003},
  pages = {187--192},
  month = Jun
}

@ARTICLE{Ju2002,
  author = {Ju, Tao and Losasso, Frank and Schaefer, Scott and Warren, Joe},
  title = {Dual contouring of hermite data},
  journal = {ACM Trans. Graph. (SIGGRAPH)},
  year = {2002},
  volume = {21},
  pages = {339--346},
  number = {3},
  month = jul,
  acmid = {566586},
  address = {New York, NY, USA},
  doi = {10.1145/566654.566586},
  issn = {0730-0301},
  issue_date = {July 2002},
  keywords = {contouring, crack prevention, implicit functions, polyhedral simplification,
	quadratic error functions},
  numpages = {8},
  publisher = {ACM},
  url = {http://doi.acm.org/10.1145/566654.566586}
}

@INPROCEEDINGS{JSWD05,
  author = {Tao Ju and Scott Schaefer and Joe Warren and Mathieu Desbrun},
  title = {A Geometric Construction of Coordinates for Convex Polyhedra using
	Polar Duals},
  booktitle = {EG/ACM SIGGRAPH Symposium of Geometry Processing},
  year = {2005},
  pages = {181--186},
  month = Jul
}

@ARTICLE{Juffer:1991,
  author = {Juffer, A. and Botta E. and van Keulen, B. and van der Ploeg, A.
	and Berendsen, H.},
  title = {The electric potential of a macromolecule in a solvent: a fundamental
	approach},
  journal = {J. Comput. Phys.},
  year = {1991},
  volume = {97},
  pages = {144-171}
}

@ARTICLE{Jumarie:2006,
  author = {Jumarie, G.},
  title = { Modified Riemann-Liouville derivative and fractional Taylor series
	of nondifferentiable functions Further results},
  journal = { Computers and Mathematics with Applications},
  year = {2006},
  volume = {51},
  pages = {1367-1376},
  number = { }
}

@MISC{AreaMin3,
  author = {Youngjean Jung and Kevin T. Chu and Salvatore Torquato},
  title = {{A Variational Level Set Approach for Surface Area Minimization of
	Triply Periodic Surfaces}},
  note = {ArXiv:math.OC/0606345}
}

@ARTICLE{Jung:2009,
  author = {Jung, Y. W. and Lu, B. Z. and Mascagni, M.},
  title = {A computational study of ion conductance in the {KcsA K+} channel
	using a {Nernst-Planck} model with explicit resident ions},
  journal = {J. Chem. Phys.},
  year = {2009},
  volume = {131},
  pages = { },
  number = {215101}
}

@BOOK{Kadanoff:1962,
  title = {Quantum Statistical Mechanics},
  year = {1962},
  author = {Kadanoff, L.P. and Byam, G.},
  pages = {907-925},
  annote = {Quantum Statistical Mechanics},
	publisher ={W.A. Benjamin, Inc. },
  date-added = {2008-11-25 10:28:56 -0500},
  date-modified = {2008-11-25 10:28:56 -0500},
  ty = {BOOK}
}

@ARTICLE{Kafafy:2005,
  author = {Kafafy, R. and Lin, T. and Lin, Y. and Wang, J.},
  title = {Three-dimensional immersed finite element methods for electric field
	simulation in composite materials},
  journal = {Int. J. Numer. Methods Engng. },
  year = {2005},
  volume = {64},
  pages = {940-972},
  annote = {Three-dimensional immersed finite element methods for electric field
	simulation in composite materials},
  date-added = {2008-09-19 10:28:56 -0500},
  date-modified = {2008-09-19 10:28:56 -0500},
  ty = {JOUR}
}

@ARTICLE{QC,
  author = {Kalberer and Felix and Nieser and Matthias and Polthier and Konrad},
  title = {QuadCover - Surface Parameterization using Branched Coverings},
  journal = {Computer Graphics Forum},
  year = {2007},
  volume = {26},
  pages = {375--384},
  number = {3},
  month = {September},
  doi = {10.1111/j.1467-8659.2007.01060.x},
  issn = {0167-7055},
  publisher = {Blackwell Publishing},
  url = {http://dx.doi.org/10.1111/j.1467-8659.2007.01060.x}
}

@ARTICLE{Kamerlin:2009,
  author = {Kamerlin, S. C. L. and Haranczyk, M. and Warshel, A.},
  title = {Progress in ab initio QM/MM free-energy simulations of electrostatic
	energies in proteins: Accelerated QM/MM studies of pK(a), redox reactions
	and solvation free energies},
  journal = {Journal of Phys. Chem. B},
  year = {2009},
  volume = {113},
  pages = {1253-1272}
}

@ARTICLE{Kamholz:1999,
  author = {Kamholz, A. E. and Weigl, B. H. and Finlayson, B. A. and Yager, P.},
  title = {Quantitative analysis of molecular interaction in a microfluidic
	channel: The T-sensor},
  journal = {Analytical Chemistry},
  year = {1999},
  volume = {71},
  pages = {5340-5347}
}

@INPROCEEDINGS{Kandilarov:2003,
  author = {Juri D. Kandilarov},
  title = {Immersed Interface Method for a Reaction-Diffusion Equation with
	a Moving Own Concentrated Source},
  booktitle = {NMA '02: Revised Papers from the 5th International Conference on
	Numerical Methods and Applications},
  year = {2003},
  pages = {506--513},
  address = {London, UK},
  publisher = {Springer-Verlag},
  date-added = {2008-09-14 15:32:12 -0500},
  date-modified = {2008-09-14 15:32:12 -0500},
  isbn = {3-540-00608-7},
  keywords = {Diffusion; Mathematics}
}

@ARTICLE{Kanduc:2009,
  author = {Kanduc, M. and Naji, M. A. and Jho, Y. S. and Pincus, P. A. and Podgornik,
	R.},
  title = {The role of multipoles in counterion-mediated interactions between
	charged surfaces: strong and weak coupling},
  journal = {Journal of Physics: Condensed Matter},
  year = {2009},
  volume = {21},
  pages = {424103}
}

@ARTICLE{KATYMD07,
  author = {Eva Kanso and Marino Arroyo and Yiying Tong and Arash Yavari and
	Jerrold E. Marsden and Mathieu Desbrun},
  title = {On the Geometric Character of Stress in Continuum Mechanics},
  journal = {Z. angew. Math. Phys.},
  year = {2007},
  volume = {58},
  pages = {1--14}
}

@ARTICLE{Kao:2005,
  author = { Kao, Chiu-Yen and Osher, Stanley and Yablonovitch, Eli},
  title = {Maximizing Band Gaps in Two Dimensional Photonic Crystals by Using
	Level Set Methods},
  journal = { Applied Physics B: Lasers and Optics},
  year = {2005},
  volume = {81},
  pages = {235-244}
}

@INPROCEEDINGS{GotsmanCompression1,
  author = {Zachi Karni and Craig Gotsman},
  title = {Spectral compression of mesh geometry},
  booktitle = {Proceedings of ACM SIGGRAPH},
  year = {2000},
  pages = {279--286}
}

@BOOK{Karniadakis:2005,
  title = {Microflows and nanoflows : fundamentals and simulation},
  publisher = {Springer},
  year = {2005},
  author = {Karniadakis, G. and Besk{\"o}k, A. and Aluru, Narayana Rao}
}

@ARTICLE{Karnik:2005,
  author = {Karnik, R. and Castelino, K. and Fan, R. and Yang, P. and Majumdar,
	A. },
  title = {Effects of biological reactions and modifications on conductance
	of nanofluidic channels },
  journal = {Nano Letters},
  year = {2005},
  volume = {5},
  pages = { 1638-1642 },
  number = { }
}

@ARTICLE{Karnik:2007,
  author = {Karnik, R. and Duan, C. H. and Castelino, K. and Daiguji, H. and
	Majumdar, A. },
  title = {Rectification of ionic current in a nanofluidic diode },
  journal = {Nnao Letters },
  year = {2007},
  volume = {7},
  pages = { 547-551 },
  number = { }
}

@ARTICLE{Karnik:2005b,
  author = {Karnik, R. and Fan, R. and Yue, M. and Li, D. Y. and Yang, P. D.
	and Majumdar, A. },
  title = {Electrostatic control of ions and molecules in nanofluidic transistors
	},
  journal = {Nano Letters},
  year = {2005},
  volume = {5},
  pages = { 943-948 },
  number = { }
}

@ARTICLE{Karplus:1998,
  author = {Karplus, K. and Barrett, C. and Hughey, R.},
  title = {{Hidden Markov models for detecting remote protein homologies}},
  journal = {Bioinformatics},
  year = {1998},
  volume = {14},
  pages = {846-856}
}

@ARTICLE{Kass88,
  author = {M. Kass and A. Witkin and D. Terzopoulos},
  title = {Snakes: Active Contour Models},
  journal = {Int. Journal of Computer Vision},
  year = {1988},
  volume = {1},
  pages = {321-331},
  number = {4}
}

@ARTICLE{Kato:2006,
  author = {Kato, M. and Pisliakov, A. V. and Warshel, A.},
  title = {The barrier for proton transport in aquaporins as a challenge for
	electrostatic models: The role of protein relaxation in mutational
	calculations},
  journal = {Proteins},
  year = {2006},
  volume = {64},
  pages = {829-44},
  number = {4},
  abstract = {The origin of the barrier for proton transport through the aquaporin
	channel is a problem of general interest. It is becoming increasingly
	clear that this barrier is not attributable to the orientation of
	the water molecules across the channel but rather to the electrostatic
	penalty for moving the proton charge to the center of the channel.
	However, the reason for the high electrostatic barrier is still rather
	controversial. It has been argued by some workers that the barrier
	is due to the so-called NPA motif and/or to the helix macrodipole
	or to other specific elements. However, our works indicated that
	the main reason for the high barrier is the loss of the generalized
	solvation upon moving the proton charge from the bulk to the center
	of the channel and that this does not reflect a specific repulsive
	electrostatic interaction but the absence of sufficient electrostatic
	stabilization. At this stage it seems that the elucidation and clarification
	of the origin of the electrostatic barrier can serve as an instructive
	test case for electrostatic models. Thus, we reexamine the free-energy
	surface for proton transport in aquaporins using the microscopic
	free-energy perturbation/umbrella sampling (FEP/US) and the empirical
	valence bond/umbrella sampling (EVB/US) methods as well as the semimacroscopic
	protein dipole Langevin dipole model in its linear response approximation
	version (the PDLD/S-LRA). These extensive studies help to clarify
	the nature of the barrier and to establish the reduced solvation
	effect as the primary source of this barrier. That is, it is found
	that the barrier is associated with the loss of the generalized solvation
	energy (which includes of course all electrostatic effects) upon
	moving the proton charge from the bulk solvent to the center of the
	channel. It is also demonstrated that the residues in the NPA region
	and the helix dipole cannot be considered as the main reasons for
	the electrostatic barrier. Furthermore, our microscopic and semimacroscopic
	studies clarify the problems with incomplete alternative calculations,
	illustrating that the effects of various electrostatic elements are
	drastically overestimated by macroscopic calculations that use a
	low dielectric constant and do not consider the protein reorganization.
	Similarly, it is pointed out that microscopic potential of mean force
	calculations that do not evaluate the electrostatic barrier relative
	to the bulk water cannot be used to establish the origin of the electrostatic
	barrier. The relationship between the present study and calculations
	of pKas in protein interiors is clarified, pointing out that approaches
	that are applied to study the aquaporin barrier should be validated
	by pKas calculations. Such calculations also help to clarify the
	crucial role of solvation energies in establishing the barrier in
	aquaporins.},
  annote = {The barrier for proton transport in aquaporins as a challenge for
	electrostatic models: The role of protein relaxation in mutational
	calculations},
  bdsk-url-1 = {http://dx.doi.org/10.1002/prot.21012},
  date-added = {2008-09-01 13:56:44 -0500},
  date-modified = {2008-09-01 13:56:44 -0500},
  keywords = {Electrostatics; Solvation; pKa},
  ty = {JOUR},
  url = {http://dx.doi.org/10.1002/prot.21012}
}

@INPROCEEDINGS{Kazhdan06,
  author = {Michael Kazhdan and M. Bolitho and Hugues Hoppe},
  title = {{Poisson Surface Reconstruction}},
  booktitle = {Symposium on Geometry Processing},
  year = {2006},
  pages = {61--70}
}

@ARTICLE{Ke07144107,
  author = {Ke, S. H. and Baranger, H. U. and Yang, W.},
  title = {Electron transport through single conjugated organic molecules: Basis
	set effects in ab initio calculations},
  journal = {Journal of Chemical Physics},
  year = {2007},
  volume = {127},
  pages = {144107},
  number = {14},
  month = {Oct},
  abstract = {We investigate electron transport through single conjugated molecules-including
	benzenedithiol, oligophenylene ethynylenes of different lengths,
	and a ferrocene-containing molecule sandwiched between two gold electrodes
	with different contact structures-by using a single-particle Green
	function method combined with density functional theory calculation.
	We focus on the effect of the basis set in the ab initio calculation.
	It is shown that the position of the Fermi energy in the transport
	gap is sensitive to the molecule-lead charge transfer which is affected
	by the size of basis set. This can dramatically change, by orders
	of magnitude, the conductance for long molecules, though the effect
	is only minor for short ones. A resonance around the Fermi energy
	tends to pin the position of the Fermi energy and suppress this effect.
	The result is discussed in comparison with experimental data. (c)
	2007 American Institute of Physics.},
  endnotereftype = {Journal Article},
  issn = {0021-9606},
  shorttitle = {Electron transport through single conjugated organic molecules: Basis
	set effects in ab initio calculations},
  url = {<Go to ISI>://000250140800012}
}

@ARTICLE{Ke07146802,
  author = {Ke, S. H. and Baranger, H. U. and Yang, W. T.},
  title = {Contact transparency of nanotube-molecule-nanotube junctions},
  journal = {Physical Review Letters, gle-walled carbon nanotubes is investigated
	using a single-particle Green's function method which combines a
	Landauer approach with ab initio density functional theory. We find
	that the overall conjugation required for good contact transparency
	is broken by connecting through a six-member ring on the tube. Full
	conjugation achieved by an all-carbon contact through a five-member
	ring leads to near perfect contact transparency for different conjugated
	molecular bridges.},
  year = {2007},
  month = {Oct},
  endnotereftype = {Journal Article},
  issn = {0031-9007},
  shorttitle = {Contact transparency of nanotube-molecule-nanotube junctions},
  url = {<Go to ISI>://000249974000050}
}

@ARTICLE{Ke07201102,
  author = {Ke, S. H. and Baranger, H. U. and Yang, W. T.},
  title = {Role of the exchange-correlation potential in ab initio electron
	transport calculations},
  journal = {Journal of Chemical Physics},
  year = {2007},
  volume = {126},
  pages = {201102},
  number = {20},
  month = {May},
  abstract = {The effect of the exchange-correlation potential in ab initio electron
	transport calculations is investigated by constructing optimized
	effective potentials using different energy functionals or the electron
	density from second-order perturbation theory. The authors calculate
	electron transmission through two atomic chain systems, one with
	charge transfer and one without. Dramatic effects are caused by two
	factors: changes in the energy gap and the self-interaction error.
	The error in conductance caused by the former is about one order
	of magnitude while that caused by the latter ranges from several
	times to two orders of magnitude, depending on the coupling strength
	and charge transfer. The implications for accurate quantum transport
	calculations are discussed. (c) 2007 American Institute of Physics.},
  endnotereftype = {Journal Article},
  issn = {0021-9606},
  shorttitle = {Role of the exchange-correlation potential in ab initio electron transport
	calculations},
  url = {<Go to ISI>://000246891700002}
}

@ARTICLE{Ke06819,
  author = {Ke, S. H. and Baranger, H. U. and Yang, W. T.},
  title = {Development of ab initio calculation for electron transport and the
	effects of lead and contact structures in molecular electronics},
  journal = {Journal of Computational and Theoretical Nanoscience},
  year = {2006},
  volume = {3},
  pages = {819-823},
  number = {5},
  month = {Oct},
  abstract = {A fully self-consistent method combining density functional theory
	(DFT) and nonequilibrium Green function approach for calculating
	electron transport through molecular devices is reviewed. It uses
	periodic boundary conditions for DFT and treats the leads and molecule
	of a device system on the same footing. Also reviewed is its application
	for the molecular conductance of Au-benzenedithiol-Au systems. Two
	important issues in molecular electronics are discussed: (1) quantum
	confinement effects in thin electrodes (leads) and (2) effects of
	local atomic configuration around the contacts. Quantum-confinement-induced
	waveguide effect causes large oscillations in the transmission function.
	Single or double apex Au atoms at each contact lead to a significant
	conductance resonance, which is quite similar to increasing the molecule-lead
	separation.},
  endnotereftype = {Journal Article},
  issn = {1546-1955},
  shorttitle = {Development of ab initio calculation for electron transport and the
	effects of lead and contact structures in molecular electronics},
  url = {<Go to ISI>://000241685400022}
}

@ARTICLE{Ke05113401,
  author = {Ke, S. H. and Baranger, H. U. and Yang, W. T.},
  title = {Electron transport through molecules: Gate-induced polarization and
	potential shift},
  journal = {Physical Review B},
  year = {2005},
  volume = {71},
  pages = {113401},
  number = {11},
  month = {Mar},
  abstract = {We analyze the effect of a gate on the conductance of molecules by
	separately evaluating the gate-induced polarization and the potential
	shift of the molecule relative to the leads. The calculations use
	ab initio density functional theory combined with a Green function
	method for electron transport. For a general view, we study several
	systems: (1) atomic chains of C or Al sandwiched between Al electrodes,
	(2) a benzene molecule between Au leads, and (3) (9,0) and (5,5)
	carbon nanotubes. We find that the polarization effect is small because
	of screening, while the effect of the potential shift is significant,
	providing a mechanism for single-molecule transistors.},
  endnotereftype = {Journal Article},
  issn = {1098-0121},
  shorttitle = {Electron transport through molecules: Gate-induced polarization and
	potential shift},
  url = {<Go to ISI>://000228065500027}
}

@ARTICLE{Ke05114701,
  author = {Ke, S. H. and Baranger, H. U. and Yang, W. T.},
  title = {Models of electrodes and contacts in molecular electronics},
  journal = {Journal of Chemical Physics},
  year = {2005},
  volume = {123},
  pages = {114701},
  number = {11},
  month = {Sep},
  abstract = {Bridging the difference in atomic structure between experiments and
	theoretical calculations and exploring quantum confinement effects
	in thin electrodes (leads) are both important issues in molecular
	electronics. To address these issues, we report here, by using Au-benzenedithiol-Au
	as a model system, systematic investigations of different models
	for the leads and the lead-molecule contacts: leads with different
	cross sections, leads consisting of infinite surfaces, and surface
	leads with a local nanowire or atomic chain of different lengths.
	The method adopted is a nonequilibrium Green's-function approach
	combined with density-functional theory calculations for the electronic
	structure and transport, in which the leads and molecule are treated
	on the same footing. It is shown that leads with a small cross section
	will lead to large oscillations in the transmission function T(E),
	which depend significantly on the lead structure (orientation) because
	of quantum waveguide effects. This oscillation slowly decays as the
	lead width increases, with the average approaching the limit given
	by infinite surface leads. Local nanowire structures around the contacts
	induce moderate fluctuations in T(E), while a Au atomic chain (including
	a single Au apex atom) at each contact leads to a significant conductance
	resonance. (c) 2005 American Institute of Physics.},
  endnotereftype = {Journal Article},
  issn = {0021-9606},
  shorttitle = {Models of electrodes and contacts in molecular electronics},
  url = {<Go to ISI>://000232033800036}
}

@ARTICLE{Ke0574704,
  author = {Ke, S. H. and Baranger, H. U. and Yang, W. T.},
  title = {Contact atomic structure and electron transport through molecules},
  journal = {Journal of Chemical Physics},
  year = {2005},
  volume = {122},
  pages = {74704},
  number = {7},
  month = {Feb},
  abstract = {Using benzene sandwiched between two Au leads as a model system, we
	investigate from first principles the change in molecular conductance
	caused by different atomic structures around the metal-molecule contact.
	Our motivation is the variable situations that may arise in break
	junction experiments; our approach is a combined density functional
	theory and Green function technique. We focus on effects caused by
	(1) the presence of an additional Au atom at the contact and (2)
	possible changes in the molecule-lead separation. The effects of
	contact atomic relaxation and two different lead orientations are
	fully considered. We find that the presence of an additional Au atom
	at each of the two contacts will increase the equilibrium conductance
	by up to two orders of magnitude regardless of either the lead orientation
	or different group-VI anchoring atoms. This is due to a resonance
	peak near the Fermi energy from the lowest energy unoccupied molecular
	orbital. In the nonequilibrium properties, the resonance peak manifests
	itself in a negative differential conductance. We find that the dependence
	of the equilibrium conductance on the molecule-lead separation can
	be quite subtle: either very weak or very strong depending on the
	separation regime. (C) 2005 American Institute of Physics.},
  endnotereftype = {Journal Article},
  issn = {0021-9606},
  shorttitle = {Contact atomic structure and electron transport through molecules},
  url = {<Go to ISI>://000227140000051}
}

@ARTICLE{Ke0415897,
  author = {Ke, S. H. and Baranger, H. U. and Yang, W. T.},
  title = {Molecular conductance: Chemical trends of anchoring groups},
  journal = {Journal of the American Chemical Society},
  year = {2004},
  volume = {126},
  pages = {15897-15904},
  number = {48},
  month = {Dec},
  abstract = {Combining density functional theory calculations for molecular electronic
	structure with a Green function method for electron transport, we
	calculate from first principles the molecular conductance of benzene
	connected to two Au leads through different anchoring atoms-S, Se,
	and Te. The relaxed atomic structure of the contact, different lead
	orientations, and different adsorption sites are fully considered.
	We find that the molecule-lead coupling, electron transfer, and conductance
	all depend strongly on the adsorption site, lead orientation, and
	local contact atomic configuration. For flat contacts the conductance
	decreases as the atomic number of the anchoring atom increases, regardless
	of the adsorption site, lead orientation, or bias. For small bias
	this chemical trend is, however, dependent on the contact atomic
	configuration: an additional Au atom at the contact with the (111)
	lead changes the best anchoring atom from S to Se, although for large
	bias the original chemical trend is recovered.},
  endnotereftype = {Journal Article},
  issn = {0002-7863},
  shorttitle = {Molecular conductance: Chemical trends of anchoring groups},
  url = {<Go to ISI>://000225505700043}
}

@ARTICLE{Ke0485410,
  author = {Ke, S. H. and Baranger, H. U. and Yang, W. T.},
  title = {Electron transport through molecules: Self-consistent and non-self-consistent
	approaches},
  journal = {Physical Review B},
  year = {2004},
  volume = {70},
  pages = {85410},
  number = {8},
  month = {Aug},
  abstract = {A self-consistent method for calculating electron transport through
	a molecular device is developed. It is based on density functional
	theory electronic structure calculations under periodic boundary
	conditions and implemented in the framework of the nonequilibrium
	Green function approach. To avoid the substantial computational cost
	in finding the I-V characteristic of large systems, we also develop
	an approximate but much more efficient non-self-consistent method.
	Here the change in effective potential in the device region caused
	by a bias is approximated by the main features of the voltage drop.
	As applications, the I-V curves of a carbon chain and an aluminum
	chain sandwiched between two aluminum electrodes are calculated-two
	systems in which the voltage drops very differently. By comparing
	to the self-consistent results, we show that this non-self-consistent
	approach works well and can give quantitatively good results.},
  endnotereftype = {Journal Article},
  issn = {1098-0121},
  shorttitle = {Electron transport through molecules: Self-consistent and non-self-consistent
	approaches},
  url = {<Go to ISI>://000223716700084}
}

@ARTICLE{Ke03116803,
  author = {Ke, S. H. and Baranger, H. U. and Yang, W. T.},
  title = {Addition energies of fullerenes and carbon nanotubes as quantum dots:
	The role of symmetry},
  journal = {Physical Review Letters},
  year = {2003},
  volume = {91},
  pages = {116803},
  number = {11},
  month = {Sep},
  abstract = {Using density-functional theory calculations, we investigate the addition
	energy (AE) of quantum dots formed of fullerenes or closed single-wall
	carbon nanotubes. We focus on the connection between symmetry and
	oscillations in the AE spectrum. In the highly symmetric fullerenes
	the oscillation period is large because of the large level degeneracy
	and Hund's rule. For long nanotubes, the AE oscillation is fourfold.
	Adding defects destroys the spatial symmetry of the tubes, leaving
	only spin degeneracy; correspondingly, the fourfold behavior is destroyed,
	leaving an even/odd behavior which is quite robust. We use our symmetry
	results to explain recent experiments.},
  endnotereftype = {Journal Article},
  issn = {0031-9007},
  shorttitle = {Addition energies of fullerenes and carbon nanotubes as quantum dots:
	The role of symmetry},
  url = {<Go to ISI>://000185288000047}
}

@ARTICLE{Ke083257,
  author = {Ke, S. H. and Yang, W. T. and Baranger, H. U.},
  title = {Quantum-Interference-Controlled Molecular Electronics},
  journal = {Nano Letters},
  year = {2008},
  volume = {8},
  pages = {3257-3261},
  number = {10},
  month = {Oct},
  abstract = {Quantum interference in coherent transport through single molecular
	rings may provide a mechanism to control the current in molecular
	electronics. We investigate its applicability, using a single-particle
	Green function method combined with ab initio electronic structure
	calculations. We find that the quantum interference effect (QIE)
	is strongly dependent on the interaction between molecular pi-states
	and contact sigma-states. It is masked by sigma tunneling in small
	molecular rings with Au leads, such as benzene, due to strong pi-sigma
	hybridization, while it is preserved in large rings, such as [18]annulene,
	which then could be used to realize quantum interference effect (QIE)
	transistors.},
  endnotereftype = {Journal Article},
  issn = {1530-6984},
  shorttitle = {Quantum-Interference-Controlled Molecular Electronics},
  url = {<Go to ISI>://000259906800033}
}

@ARTICLE{Ke06181102,
  author = {Ke, S. H. and Yang, W. T. and Baranger, H. U.},
  title = {Nanotube-metal junctions: 2-and 3-terminal electrical transport},
  journal = {Journal of Chemical Physics},
  year = {2006},
  volume = {124},
  pages = {181102},
  number = {18},
  month = {May},
  abstract = {We address the quality of electrical contact between carbon nanotubes
	and metallic electrodes by performing first-principles calculations
	for the electron transmission through ideal 2- and 3-terminal junctions,
	thus revealing the physical limit of tube-metal conduction. The structural
	model constructed involves surrounding the tube by the metal atoms
	of the electrode as in most experiments; we consider metallic (5,5)
	and n-doped semiconducting (10,0) tubes surrounded by Au or Pd. In
	the case of metallic tubes, the contact conductance is shown to approach
	the ideal 4e(2)/h in the limit of large contact area. For three-terminals,
	the division of flux among the different transmission channels depends
	strongly on the metal material. A Pd electrode has nearly perfect
	tube-electrode transmission and therefore turns off the straight
	transport along the tube. Our results are in good agreement with
	some recent experimental reports and clarify a fundamental discrepancy
	between theory and experiment. (c) 2006 American Institute of Physics.},
  endnotereftype = {Journal Article},
  issn = {0021-9606},
  shorttitle = {Nanotube-metal junctions: 2-and 3-terminal electrical transport},
  url = {<Go to ISI>://000237477800002}
}

@ARTICLE{Ke091011,
  author = {Ke, S. H. and Yang, W. T. and Curtarolo, S. and Baranger, H. U.},
  title = {Thermopower of Molecular Junctions: An ab Initio Study},
  journal = {Nano Letters},
  year = {2009},
  volume = {9},
  pages = {1011-1014},
  number = {3}
}

@ARTICLE{Keinan07176,
  author = {Keinan, S. and Hu, X. Q. and Beratan, D. N. and Yang, W. T.},
  title = {Designing molecules with optimal properties using the linear combination
	of atomic potentials approach in an AM1 semiempirical framework},
  journal = {Journal of Physical Chemistry A},
  year = {2007},
  volume = {111},
  pages = {176-181},
  number = {1},
  month = {Jan},
  abstract = {The linear combination of atomic potentials (LCAP) approach is implemented
	in the AM1 semiempirical framework and is used to design molecular
	structures with optimized properties. The optimization procedure
	uses property derivative information to search molecular space and
	thus avoid direct enumeration and evaluation of each molecule in
	a library. Two tests are described: the optimization of first hyperpolarizabilities
	of substituted aromatics and the optimization of a figure of merit
	for n-type organic semiconductors.},
  endnotereftype = {Journal Article},
  issn = {1089-5639},
  shorttitle = {Designing molecules with optimal properties using the linear combination
	of atomic potentials approach in an AM1 semiempirical framework},
  url = {<Go to ISI>://000243229000023}
}

@ARTICLE{Keinan083256,
  author = {Keinan, S. and Paquette, W. D. and Skoko, J. J. and Beratan, D. N.
	and Yang, W. T. and Shinde, S. and Johnston, P. A. and Lazo, J. S.
	and Wipf, P.},
  title = {Computational design, synthesis and biological evaluation of para-quinone-based
	inhibitors for redox regulation of the dual-specificity phosphatase
	Cdc25B},
  journal = {Organic \& Biomolecular Chemistry},
  year = {2008},
  volume = {6},
  pages = {3256-3263},
  number = {18},
  month = {Sep},
  abstract = {Quinoid inhibitors of Cdc25B were designed based oil the Linear Combination
	of Atomic potentials (LCAP) methodology. In contrast to it published
	hypothesis. the biological activities and hydrogen peroxide generation
	in reducing media of three synthetic models did not correlate with
	the (quinone half-wave potential, E-1/2.},
  endnotereftype = {Journal Article},
  issn = {1477-0520},
  shorttitle = {Computational design, synthesis and biological evaluation of para-quinone-based
	inhibitors for redox regulation of the dual-specificity phosphatase
	Cdc25B},
  url = {<Go to ISI>://000259407800005}
}

@ARTICLE{Keinan0812203,
  author = {Keinan, S. and Therien, M. J. and Beratan, D. N. and Yang, W. T.},
  title = {Molecular Design of Porphyrin-Based Nonlinear Optical Materials},
  journal = {Journal of Physical Chemistry A},
  year = {2008},
  volume = {112},
  pages = {12203-12207},
  number = {47},
  month = {Nov},
  abstract = {Nonlinear optical chromophores containing (porphyrinato)Zn(II), proquinoid,
	and (terpyridyl)metal(II) building blocks were optimized in a library
	containing similar to 10(6) structures using the linear combination
	of atomic potentials (LCAP) methodology. We report here the library
	design and molecular property optimizations. Two basic structural
	types of large beta(0) chromophores were examined: linear and T-shaped
	motifs. These T-shaped geometries suggest a promising NLO chromophoric
	architecture for experimental investigation and further support the
	value of performing LCAP searches in large chemical spaces.},
  endnotereftype = {Journal Article},
  issn = {1089-5639},
  shorttitle = {Molecular Design of Porphyrin-Based Nonlinear Optical Materials},
  url = {<Go to ISI>://000261056300033}
}

@ARTICLE{Khan:2004,
  author = {Khan, H. R. and Vasileska, D. and Ahmed, S. S.},
  title = {{Modeling of FinFet: 3D MC Simulation Using FMM and Unintentional
	Doping Effects on Device Operation}},
  journal = {Journal of Computational Electronics},
  year = {2004},
  volume = {3},
  pages = {337-340}
}

@ARTICLE{khan:2005,
  author = {Khan, T. and Vasileska, D. and Thornton, T. J.},
  title = {Effect of interface roughness on silicon-on-insulator-metal-semiconductor
	field-effect transistor mobility and the device low-power high-frequence
	operation},
  journal = {J. Vac. Sci. Technol. B},
  year = {2005},
  volume = {23},
  pages = {1782-1784},
  number = {4}
}

@INPROCEEDINGS{KWTKMSD06,
  author = {Liliya Kharevych and Weiwei and Yiying Tong and Eva Kanso and Jerrold
	E. Marsden and Peter Schr{\"o}der and Mathieu Desbrun},
  title = {Geometric, Variational Integrators for Computer Animation},
  booktitle = {ACM/EG Symposium on Computer Animation},
  year = {2006},
  pages = {43--51},
  month = Jul
}

@ARTICLE{KADS02,
  author = {Andrei Khodakovsky and Pierre Alliez and Mathieu Desbrun and Peter
	Schr{\"o}der},
  title = {Near-Optimal Connectivity Encoding of 2-Manifold Polygon Meshes},
  journal = {Graphical Models},
  year = {2002},
  volume = {64},
  pages = {147--168},
  number = {3--4}
}

@INPROCEEDINGS{Khodakovsky,
  author = {Andrei Khodakovsky and Peter Schr\"{o}der and Wim Sweldens},
  title = {Progressive Geometry Compression},
  booktitle = {ACM SIGGRAPH},
  year = {2000},
  pages = {271--278}
}

@INPROCEEDINGS{kmp_shape_space_sig_07,
  author = {Martin Kilian and N. J. Mitra and H. Pottmann},
  title = {Geometric Modeling in Shape Space},
  booktitle = {ACM Transactions on Graphics (SIGGRAPH)},
  year = {2007}
}

@ARTICLE{Kilic2:2007,
  author = {Kilic, M. S. and Bazant, M. Z. and Ajdari, A. },
  title = {Steric effects in the dynamics of electrolytes at large applied voltages.
	{II}. Modified Poisson-Nernst-Planck Equations},
  journal = {Phys. Rev. E },
  year = {2007},
  volume = {75},
  pages = {  },
  number = {021503}
}

@ARTICLE{Kilic:2007,
  author = {Kilic, M. S. and Bazant, M. Z. and Ajdari, A. },
  title = {Steric effects in the dynamics of electrolytes at large applied voltages.
	{I}. Double-layer charging},
  journal = {Phys. Rev. E },
  year = {2007},
  volume = {75},
  pages = {16 pages },
  number = {021502}
}

@ARTICLE{Kim:2008a,
  author = {Kim, B. and Kwon, W. and Baek, C. and Jin, S. and Song, Y. and Kim,
	D. M.},
  title = {{Three-Dimensional Simulation of Dopant-Fluctuation-Induced Threshold
	Voltage Dispersion in Nonplanar MOS Structures Targeting Flash EEPROM
	Transistors}},
  journal = {IEEE T Electron Devices},
  year = {2008},
  volume = {55},
  pages = {1456-1463},
  annote = {Three-Dimensional Simulation of Dopant-Fluctuation-Induced Threshold
	Voltage Dispersion in Nonplanar MOS Structures Targeting Flash EEPROM
	Transistors },
  date-added = {2008-11-25 10:28:56 -0500},
  date-modified = {2008-11-25 10:28:56 -0500},
  ty = {JOUR}
}

@ARTICLE{BYKim:2009,
  author = {Kim, B. Y. and Yang, J. and Gong, M. J. and Flachsbart, B. R. and
	Shannon, M. A. and Bohn, P. W. and Sweedler, J. V. },
  title = {Multidimensional Separation of Chiral Amino Acid Mixtures in a Multilayered
	Three-Dimensional Hybrid Microfluidic/Nanofluidic Device },
  journal = {J. Anal. Chem. },
  year = {2009},
  volume = {81},
  pages = { 2715-2722 }
}

@ARTICLE{Kim:2004,
  author = {Kim, K. and Kwon, O. and Seo, J. and Won, T. and Birner, S. and Trellakis,
	A. },
  title = {{Nanoscale device modeling and simulation: Fin field-effect transistor
	(FinFET)} },
  journal = {Japanese Journal of Applied Physics Part 1 - Regular Papers Short
	Notes \& Review Papers},
  year = {2004},
  volume = {43},
  pages = {3784-3789},
  annote = {Nanoscale device modeling and simulation: Fin field-effect transistor
	(FinFET) },
  date-added = {2008-11-25 10:28:56 -0500},
  date-modified = {2008-11-25 10:28:56 -0500},
  ty = {JOUR}
}

@INPROCEEDINGS{KKSD02,
  author = {Laehyun Kim and Anna Kyrikou and Gaurav Sukhatme and Mathieu Desbrun},
  title = {An Implicit-based Haptic Rendering Technique},
  booktitle = {IEEE/RSJ IROS Conference},
  year = {2002},
  volume = {3},
  pages = {2943--2948},
  month = sep
}

@ARTICLE{KSD04,
  author = {Laehyun Kim and Gaurav Sukhatme and Mathieu Desbrun},
  title = {A Haptic Rendering Technique Based on Hybrid Surface Representation},
  journal = {IEEE Computer and Graphics Applications (Special Issue: Haptic Rendering
	Beyond Visual Computing)},
  year = {2004},
  volume = {24},
  pages = {66--75},
  number = {2}
}

@INPROCEEDINGS{KSD03,
  author = {Laehyun Kim and Gaurav Sukhatme and Mathieu Desbrun},
  title = {Haptic Editing for Decoration and Material Properties},
  booktitle = {IEEE Symposium on Haptic Interfaces},
  year = {2003},
  pages = {213--220},
  month = jun
}

@ARTICLE{KimSJ:2010,
  author = {Kim, S. J. and Ko, S. H. and Kang, K. H. and Han, J. },
  title = {Direct seawater desalination by ion concentration polarization},
  journal = {Nature Nanotechnology},
  year = {2010},
  volume = {5},
  pages = {297-301}
}

@ARTICLE{SJKim:2009,
  author = {Kim, S. J. and Li, L. D. and Han, J. Y.},
  title = {Amplified Electrokinetic Response by Concentration Polarization near
	Nanofluidic Channel },
  journal = {LANGMUIR },
  year = {2009},
  volume = {25},
  pages = { 7759-7765 }
}

@ARTICLE{SJKim:2007,
  author = {Kim, S. J. and Wang, Y. C. and Lee, J. H. and Jang, H. and Han, J.
	Y. },
  title = {Concentration polarization and nonlinear electrokinetic flow near
	a nanofluidic channel },
  journal = {Phys. Rev Lett. },
  year = {2007},
  volume = {99},
  pages = { },
  number = { 044501 }
}

@ARTICLE{Kirk2006,
  author = {Kirk, Benjamin S. and Peterson, John W. and Stogner, Roy H. and Carey,
	Graham F.},
  title = {libMesh: a C++ library for parallel adaptive mesh refinement/coarsening
	simulations},
  journal = {Eng. with Comput.},
  year = {2006},
  volume = {22},
  pages = {237--254},
  number = {3},
  month = dec,
  acmid = {1230693},
  address = {London, UK, UK},
  doi = {10.1007/s00366-006-0049-3},
  issn = {0177-0667},
  issue_date = {December 2006},
  keywords = {Adaptive mesh refinement, Finite elements, Parallel computing},
  numpages = {18},
  publisher = {Springer-Verlag},
  url = {http://dx.doi.org/10.1007/s00366-006-0049-3}
}

@ARTICLE{Kirkwood:1934,
  author = {Kirkwood, J. G.},
  title = {Theory of solution of molecules containing widely separated charges
	with special application to Zwitterions},
  journal = {J. Comput. Phys.},
  year = {1934},
  volume = {7},
  pages = {351 - 361}
}

@ARTICLE{Kiselev:2011,
  author = {Kiselev, Y. V. and Leda, M. and Lobanov, A. I. and Marenduzzo, D.
	and Goryachev, A. B.},
  title = {Lateral dynamics of charged lipids and peripheral proteins in spatially
	heterogeneous membranes: Comparison of continuous and Monte Carlo
	approaches},
  journal = {J. Chem. Phys. },
  year = {2011},
  volume = {135},
  number = {155103}
}

@BOOK{Kittel:1980,
  title = {Thermal physics},
  publisher = {Macmillan},
  year = {2010},
  author = {Kittel, C. and Kroemer, H.},
  address = { },
  date-added = { },
  date-modified = { },
  keywords = { },
  ty = {THES}
}

@ARTICLE{Klapper:1986,
  author = {Klapper, I. and Hagstrom, R. and Fine, R. and Sharp, K. and Honig,
	B.},
  title = {Focussing of Electric Fields in the Active Site of Cu-Zn Superoxide
	Dismutase: Effects of Ionic Strength and Amino Acid Modification},
  journal = {Protein},
  year = {1986},
  volume = {1},
  pages = {47 - 59}
}

@ARTICLE{ShapeSpace,
  author = {Eric Klassen and Anuj Srivastava and Washington Mio and Shantanu
	H. Joshi},
  title = {Analysis of Planar Shapes using Geodesic Paths on Shape Spaces},
  journal = {IEEE Trans. on PAMI},
  year = {2004},
  volume = {26},
  pages = {372-383},
  number = {3}
}

@ARTICLE{Klebe:2006,
  author = {Klebe, G.},
  title = {{Virtual ligand screening: strategies, perspectives and limitations}},
  journal = {Drug Discov Today},
  year = {2006},
  volume = {11},
  pages = {580-594},
  number = {13-14}
}

@ARTICLE{Klicic:2002,
  author = {Klicic, J. J. and Friesner, R. A. and Liu, S. Y. and Guida, W. C.},
  title = {Accurate prediction of acidity constants in aqueous solution via
	density functional theory and self-consistent reaction field methods},
  journal = {J. Phys. Chem. A},
  year = {2002},
  volume = {106},
  pages = {1327--1335 }
}

@ARTICLE{james06,
  author = {Bryan M. Klingner and Bryan E. Feldman and Nuttapong Chentanez and
	James F. O'Brien},
  title = {{Fluid Animation with Dynamic Meshes}},
  journal = {ACM Trans. Graph. (SIGGRAPH)},
  year = {2006},
  month = aug
}

@ARTICLE{Knap:2001,
  author = {Knap, J. and Ortiz, M.},
  title = {Spanning the continuum to quantum length scales in a dynamic simulation
	of brittle fracture},
  journal = {J. Mech. Phys. Solids},
  year = {2001},
  volume = {49},
  pages = {1899 - 1923}
}

@ARTICLE{Leif2000,
  author = {Leif Kobbelt},
  title = {Discrete Fairing and Variational Subdivision for Freeform Surface
	Design},
  journal = {The Visual Computer},
  year = {2000},
  volume = {16},
  pages = {142-158},
  number = {3-4}
}

@INPROCEEDINGS{Kobbelt2001,
  author = {Kobbelt, Leif P. and Botsch, Mario and Schwanecke, Ulrich and Seidel,
	Hans-Peter},
  title = {Feature sensitive surface extraction from volume data},
  booktitle = {Proceedings of the 28th annual conference on Computer graphics and
	interactive techniques},
  year = {2001},
  series = {SIGGRAPH '01},
  pages = {57--66},
  address = {New York, NY, USA},
  publisher = {ACM},
  acmid = {383265},
  doi = {10.1145/383259.383265},
  isbn = {1-58113-374-X},
  numpages = {10},
  url = {http://doi.acm.org/10.1145/383259.383265}
}

@INPROCEEDINGS{KDMS07,
  author = {Marin Kobilarov and Mathieu Desbrun and Jerrold E. Marsden and Gaurav
	S. Sukhatme},
  title = {A Discrete Geometric Optimal Control Framework for Systems with Symmetries},
  booktitle = {Robotics: Science and Systems},
  year = {2007},
  pages = {(unknown)},
  month = Jun
}

@ARTICLE{Koehl:2006,
  author = {Koehl, P.},
  title = {Electrostatics calculations: latest methodological advances},
  journal = {Current Opinion in Structural Biology},
  year = {2006},
  volume = {16},
  pages = {142-51},
  number = {2},
  abstract = {Electrostatics plays a major role in the stabilization and function
	of biomolecules; as such, it remains a major focus of theoretical
	and computational studies of macromolecules. Electrostatic interactions
	are long range, and strongly dependent on the solvent and ions surrounding
	the biomolecule under study. During the past year, progress has been
	reported in the treatment of electrostatics in explicit and implicit
	solvent models. Interesting new developments of explicit solvent
	models include more efficient Ewald summation methods, as well as
	alternative approaches based on reaction field theory, periodic images
	and Euler summations. Implicit solvent models remain divided into
	those that solve the PoissonÃ¢Â€Â“Boltzmann equation numerically
	and those based on the generalized Born formalism. Both approaches
	are now included in molecular dynamics simulations and their accuracies
	may be assessed by direct comparison against experimental data. It
	is worth mentioning the recent development of web interfaces that
	facilitate access to and usage of existing tools for computing electrostatic
	interactions.},
  annote = {Electrostatics calculations: latest methodological advances},
  bdsk-url-1 = {http://dx.doi.org/10.1016/j.sbi.2006.03.001},
  date-added = {2008-09-01 13:57:34 -0500},
  date-modified = {2008-09-01 13:57:34 -0500},
  keywords = {Electrostatics},
  ty = {JOUR},
  url = {http://dx.doi.org/10.1016/j.sbi.2006.03.001}
}


@ARTICLE{Koehl:2009b,
  author = {Koehl, P. and Orland, H. and Delarue, M.},
  title = {Computing ion solvation free energies using the dipolar Poisson model},
  journal = {J. Phys. Chem. B},
  year = {2009},
  volume = {113},
  pages = {5694 -5698}
}

@ARTICLE{Kohn:1965,
  author = {Kohn, W. and Sham, L. J.},
  title = {Self-Consistent Equations Including Exchange and Correlation Effects},
  journal = {Phys. Rev.},
  year = {1965},
  volume = {140},
  pages = {A1133- A1138 }
}

@ARTICLE{Kohn:1965,
  author = {Kohn, W. and Sham, L. J.},
  title = {Self-Consistent Equations Including Exchange and Correlation Effects},
  journal = {Phys. Rev.},
  year = {1965},
  volume = {140},
  pages = {A1133- A1138 }
}

@ARTICLE{Kollman:2000,
  author = {Kollman, P. A. and Massova, I. and Reyes, C. and Kuhn, B. and Huo,
	S. and Chong, L. and Lee, M. and Lee, T. and Duan, Y. and Wang, W.
	and Donini, O. and Cieplak, P. and Srinivasan, J. and Case, D. A.
	and Cheatham, T. E. , III},
  title = {Calculating structures and free energies of complex molecules: combining
	molecular mechanics and continuum models},
  journal = {Accounts of Chemical Research},
  year = {2000},
  volume = {33},
  pages = {889-97},
  number = {12},
  abstract = {A historical perspective on the application of molecular dynamics
	(MD) to biological macromolecules is presented. Recent developments
	combining state-of-the-art force fields with continuum solvation
	calculations have allowed us to reach the fourth era of MD applications
	in which one can often derive both accurate structure and accurate
	relative free energies from molecular dynamics trajectories. We illustrate
	such applications on nucleic acid duplexes, RNA hairpins, protein
	folding trajectories, and protein-ligand, protein-protein, and protein-nucleic
	acid interactions.},
  address = {Department of Pharmaceutical Chemistry, University of California,
	San Francisco, California 94143, USA.},
  annote = {Dec; Calculating structures and free energies of complex molecules:
	combining molecular mechanics and continuum models; 11123888},
  bdsk-url-1 = {http://dx.doi.org/10.1021/ar000033j},
  date-added = {2008-06-29 13:10:46 -0500},
  date-modified = {2008-06-29 13:10:46 -0500},
  keywords = {molecular\_dynamics},
  ty = {JOUR},
  url = {http://dx.doi.org/10.1021/ar000033j}
}

@ARTICLE{Kolpakov:2007,
  author = {Kolpakov, A. and Tagantsev, A. K. and Berlyand, L. and Kanareykin,
	A.},
  title = {Nonlinear dielectric response of periodic composite materials},
  journal = {J Electroceram},
  year = {2007},
  volume = {18},
  pages = {129-137}
}

@ARTICLE{Konecny:2006,
  author = {Konecny, R. and Trylska, J. and Tama, F. and Zhang, D. and Baker,
	N. A. and Brooks, C. L. , {III} and McCammon, J. A.},
  title = {Electrostatic properties of cowpea chlorotic mottle virus and cucumber
	mosaic virus capsids},
  journal = {Biopolymers},
  year = {2006},
  volume = {82},
  pages = {106-20},
  number = {2},
  abstract = {Electrostatic properties of cowpea chlorotic mottle virus (CCMV) and
	cucumber mosaic virus (CMV) were investigated using numerical solutions
	to the {Poisson-Boltzmann} equation. Experimentally, it has been
	shown that CCMV particles swell in the absence of divalent cations
	when the pH is raised from 5 to 7. CMV, although structurally homologous,
	does not undergo this transition. An analysis of the calculated electrostatic
	potential confirms that a strong electrostatic repulsion at the calcium
	binding sites in the CCMV capsid is most likely the driving force
	for the capsid swelling process during the release of calcium. The
	binding interaction between the encapsulated genome material (RNA)
	inside of the capsid and the inner capsid shell is weakened during
	the swelling transition. This probably aids in the RNA release process,
	but it is unlikely that the RNA is released through capsid openings
	due to unfavorable electrostatic interaction between the RNA and
	capsid inner shell residues at these openings. Calculations of the
	calcium binding energies show that Ca2+ can bind both to the native
	and swollen forms of the CCMV virion. Favorable binding to the swollen
	form suggests that Ca2+ ions can induce the capsid contraction and
	stabilize the native form.},
  annote = {Electrostatic properties of cowpea chlorotic mottle virus and cucumber
	mosaic virus capsids; KonecnyEtal2006},
  bdsk-file-1 = {YnBsaXN0MDDUAQIDBAUGCQpYJHZlcnNpb25UJHRvcFkkYXJjaGl2ZXJYJG9iamVjdHMSAAGGoNE
	HCFRyb290gAFfEA9OU0tleWVkQXJjaGl2ZXKoCwwXGBkdJCVVJG51bGzTDQ4PEBEUViRjbGFzc1
	dOUy5rZXlzWk5TLm9iamVjdHOAB6ISE4ACgAOiFRaABIAGWWFsaWFzRGF0YVxyZWxhdGl2ZVBhd
	GjSDRobHFdOUy5kYXRhgAVPEQImAAAAAAImAAIAAAxNYWNpbnRvc2ggSEQAAAAAAAAAAAAAAAAA
	AADD4v5NSCsAAAAZYksfMjAwNi1Lb25lY255VHJ5bHNrYVQjMTk2MjhFLnBkZgAAAAAAAAAAAAA
	AAAAAAAAAAAAAAAAAAAAAAAAAAAAAABlijsNHOMNQREYgcHJ2dwAEAAQAAAkgAAAAAAAAAAAAAA
	AAAAAAB0FyY2hpdmUAABAACAAAw+NSrQAAABEACAAAw0d/EwAAAAEAFAAZYksAGWIDAAqkKAAKp
	BEAAHrcAAIAVU1hY2ludG9zaCBIRDpVc2VyczpiYWtlcjpEb2N1bWVudHM6UmVmZXJlbmNlczpB
	cmNoaXZlOjIwMDYtS29uZWNueVRyeWxza2FUIzE5NjI4RS5wZGYAAA4AaAAzADIAMAAwADYALQB
	LAG8AbgBlAGMAbgB5AFQAcgB5AGwAcwBrAGEAVABhAG0AYQBaAGgAYQBuAGcAQgBhAGsAZQByAE
	IAcgBvAG8AawBzAE0AYwBDAGEAbQBtAG8AbgAuAHAAZABmAA8AGgAMAE0AYQBjAGkAbgB0AG8Ac
	wBoACAASABEABIAXFVzZXJzL2Jha2VyL0RvY3VtZW50cy9SZWZlcmVuY2VzL0FyY2hpdmUvMjAw
	Ni1Lb25lY255VHJ5bHNrYVRhbWFaaGFuZ0Jha2VyQnJvb2tzTWNDYW1tb24ucGRmABMAAS8AABU
	AAgAM//8AANIeHyAhWCRjbGFzc2VzWiRjbGFzc25hbWWjISIjXU5TTXV0YWJsZURhdGFWTlNEYX
	RhWE5TT2JqZWN0XxBcLi4vLi4vLi4vLi4vRG9jdW1lbnRzL1JlZmVyZW5jZXMvQXJjaGl2ZS8yM
	DA2LUtvbmVjbnlUcnlsc2thVGFtYVpoYW5nQmFrZXJCcm9va3NNY0NhbW1vbi5wZGbSHh8mJ6In
	I1xOU0RpY3Rpb25hcnkACAARABoAHwApADIANwA6AD8AQQBTAFwAYgBpAHAAeACDAIUAiACKAIw
	AjwCRAJMAnQCqAK8AtwC5AuMC6ALxAvwDAAMOAxUDHgN9A4IDhQAAAAAAAAIBAAAAAAAAACgAAA
	AAAAAAAAAAAAAAAAOS},
  bdsk-url-1 = {http://dx.doi.org/10.1002/bip.20409},
  date-added = {2008-09-16 15:49:49 -0500},
  date-modified = {2008-09-16 15:49:49 -0500},
  keywords = {Electrostatics; NucleicAcids},
  ty = {JOUR},
  url = {http://dx.doi.org/10.1002/bip.20409}
}

@INPROCEEDINGS{ACE,
  author = {Yehuda Koren and Liran Carmel and David Harel},
  title = {ACE: A Fast Multiscale Eigenvectors Computation for Drawing Huge
	Graphs},
  booktitle = {IEEE Symposium on Information Visualization},
  year = {2002},
  pages = {137}
}

@ARTICLE{Kornyshev:2003,
  author = {Kornyshev, A. A. and Kuznetsov, A. M. and Spohr, E. and Ulstrup,
	J. },
  title = {{Kinetics of Proton Transport in Water }},
  journal = {Journal of Physical Chemistry},
  year = {2003},
  volume = {107},
  pages = {3351-3366}
}

@ARTICLE{Kornyshev:1998,
  author = {Kornyshev, A. A. and Sutmann, G. },
  title = {Nonlocal nonlinear static dielectric response of polar liquids},
  journal = {Journal of Electroanalytical Chemistry},
  year = {1998},
  volume = {450},
  pages = {143-156}
}

@ARTICLE{Kornyshev:1997,
  author = {Kornyshev, A. A. and Sutmann, G.},
  title = {Nonlocal dielectric saturation in liquid water},
  journal = {Physical Review Letters},
  year = {1997},
  volume = {79},
  pages = {3435-3438}
}

@ARTICLE{Kortemme:2003,
  author = {Kortemme, T. and Morozov, A. V. and Baker, D.},
  title = {{An orientation-dependent hydrogen bonding potential improves prediction
	of specificity and structure for proteins and protein-protein complexes}},
  journal = {J Mol Biol},
  year = {2003},
  volume = {326},
  pages = {1239-1259},
  number = {4}
}


%  author = {Kostyuchenko, V. A. and Leiman, P. G. and Chipman, P. R. and Kanamaru, S. and	van Raaij, M. J. and Arisaka, F. and Mesyanzhinov, V. V. and Rossmann, M. G.},
@ARTICLE{Kostyuchenko2003,
  author = {Kostyuchenko, V. A. and Leiman, P. G. and Chipman, P. R. and Kanamaru, S. and	van Raaij et al, M. J.},
  title = {Three-dimensional structure of bacteriophage T4 baseplate.},
  journal = {Nat Struct Biol},
  year = {2003},
  volume = {10},
  pages = {688-93--},
  number = {9},
  month = sep,
  __markedentry = {[SeanLab]},
  abstract = {The baseplate of bacteriophage T4 is a multiprotein molecular machine
	that controls host cell recognition, attachment, tail sheath contraction
	and viral DNA ejection. We report here the three-dimensional structure
	of the baseplate-tail tube complex determined to a resolution of
	12 A by cryoelectron microscopy. The baseplate has a six-fold symmetric,
	dome-like structure approximately 520 A in diameter and approximately
	270 A long, assembled around a central hub. A 940 A-long and 96 A-diameter
	tail tube, coaxial with the hub, is connected to the top of the baseplate.
	At the center of the dome is a needle-like structure that was previously
	identified as a cell puncturing device. We have identified the locations
	of six proteins with known atomic structures, and established the
	position and shape of several other baseplate proteins. The baseplate
	structure suggests a mechanism of baseplate triggering and structural
	transition during the initial stages of T4 infection.},
  address = {Shemyakin-Ovchinnikov Institute of Bioorganic Chemistry of Russian
	Academy of Sciences, 16/10 Miklukho-Maklaya Str., 117997 Moscow,
	Russia.},
  comment = {Research Support, Non-U.S. Gov't,Research Support, U.S. Gov't, Non-P.H.S.,},
  keywords = {Bacteriophage T4, Cryoelectron Microscopy, Image Processing, Computer-Assisted,
	Microscopy, Electron, Models, Molecular, Protein Structure, Tertiary},
  owner = {SeanLab},
  timestamp = {2012.05.23},
  url = {http://ukpmc.ac.uk/abstract/MED/12923574}
}

@MISC{PLIC-MCM,
  author = {D. Kothe and W. Rider and S. Mosso and J. Brock and J. Hochstein},
  title = {{Volume Tracking of Interfaces having Surface Tension in $2$ and
	$3D$}},
  howpublished = {Technical Report AIAA 96--0859},
  year = {1996}
}

@ARTICLE{kraevoy2005tbm,
  author = {Kraevoy, V. and Sheffer, A.},
  title = {{Template-based mesh completion}},
  journal = {Eurographics Symposium on Geometry Processing},
  year = {2005},
  pages = {13--22}
}

@ARTICLE{krasny,
  author = {Krasny, R.},
  title = {A study of singularity formation in a vortex sheet by the point vortex
	approximation},
  journal = {J. Fluid Mech.},
  year = {1986},
  volume = {167},
  pages = { 65-93}
}

@ARTICLE{Krishtalik:2000,
  author = {Krishtalik, L. I},
  title = {The mechanism of the proton transfer: {An} outline },
  journal = {Biochimica Et Biophysical Acta-Bioenergetics},
  year = {2000},
  volume = {1458},
  pages = {6-27},
  number = { }
}

@ARTICLE{Kucukural:2009,
  author = {Kucukural, A. and Szilagyi, A. and Sezerman, O. and Zhang, Y.},
  title = {{Protein Homology Analysis for Function Prediction with Parallel
	Sub-Graph Isomorphism}},
  journal = {In: Lodhi H, Yamanishi Y, editors. Chemoinformatics: Advances in
	Chemoinformatics and Computational Methods: IGI global},
  year = {2009},
  pages = {129-144}
}

@ARTICLE{Kuhn:1992,
  author = {Kuhn, Leslie A. and Siani, Michael A. and Pique, Michael E. and Fisher,
	Cindy L. and Getzoff, Elizabeth D. and Tainer, John A. },
  title = {The interdependence of protein surface topography and bound water
	molecules revealed by surface accessibility and fractal density measures},
  journal = {Journal of Molecular Biology},
  year = {1992},
  volume = {228},
  pages = {13--22},
  number = {1},
  abstract = {To characterize water binding to proteins, which is fundamental to
	protein folding, stability and activity, the relationships of 10,837
	bound water positions to protein surface shape and residue type were
	analyzed in 56 high-resolution crystallographic structures. Fractal
	atomic density and accessibility algorithms provided an objective
	characterization of deep grooves in solvent-accessible protein surfaces.
	These deep grooves consistently had approximately the diameter of
	one water molecule, suggesting that deep grooves are formed by the
	interactions between protein atoms and bound water molecules. Protein
	surface topography dominates the chemistry and extent of water binding.
	Protein surface area within grooves bound three times as many water
	molecules as non-groove surface; grooves accounted for one-quarter
	of the total surface area yet bound half the water molecules. Moreover,
	only within grooves did bound water molecules discriminate between
	different side-chains. In grooves, main-chain surface was as hydrated
	as that of the most hydrophilic side-chains, Asp and Glu, whereas
	outside grooves all main and side-chains bound water to a similar,
	and much decreased, extent. This identification of the interdependence
	of protein surface shape and hydration has general implications for
	modelling and prediction of protein surface shape, recognition, local
	folding and solvent binding.},
  bdsk-url-1 = {http://dx.doi.org/10.1016/0022-2836(92)90487-5},
  date-added = {2008-06-30 09:26:27 -0500},
  date-modified = {2008-06-30 09:26:27 -0500},
  doi = {10.1016/0022-2836(92)90487-5},
  keywords = {bioinformatics, solvation, structure},
  posted-at = {2008-06-30 15:25:55},
  priority = {0},
  url = {http://dx.doi.org/10.1016/0022-2836(92)90487-5}
}

@ARTICLE{Kuhn,
  author = {Kuhn, L.A. and Siani, M. A. and Pique, M. E. and Fisher, C. L. and
	Getzoff, E. D. and Tainer, J. A. },
  title = {The interdependence of protein surface topography and bound water
	molecules revealed by surface accessibility and fractal density measures},
  journal = {J. Mol. Biol.},
  year = {1992},
  volume = {228},
  pages = {13-22}
}

@ARTICLE{Kurganov,
  author = {Kurganov, A. and Levy, D.},
  title = {A third-order semidiscrete central scheme for conservation laws and
	convention diffusion equations},
  journal = {SIAM J. Sci. Comput.},
  year = {2000},
  volume = {22},
  pages = {1461-1488}
}

@ARTICLE{Kurnikova:1999,
  author = { Kurnikova, M. G. and Coalson, R. D. and Graf, P. and Nitzan, A.
	},
  title = {A Lattice Relaxation Algorithm for {Three-Dimensional} {Poisson-Nernst-Planck}
	Theory with Application to Ion Transport through the {Gramicidin
	A} Channel},
  journal = {Biophysical Journal},
  year = {1999},
  volume = {76},
  pages = {642-656},
  number = { }
}

@ARTICLE{Kuyucak:2001,
  author = {Kuyucak, Serdar and Andersen, Olaf. Sparre and Chung, Shin-Ho },
  title = {Models of permeation in ion channels},
  journal = {Rep. Prog. Phys},
  year = {2001},
  volume = {64},
  pages = {1427-1472}
}

@ARTICLE{Kyte:1982,
  author = {Kyte, J. and Doolittle, R. F.},
  title = {{A simple method for displaying the hydropathic character of a protein}},
  journal = {J Mol Biol},
  year = {1982},
  volume = {157},
  pages = {105-132}
}

@ARTICLE{Labelle2007,
  author = {Labelle, Fran\c{c}ois and Shewchuk, Jonathan Richard},
  title = {Isosurface stuffing: fast tetrahedral meshes with good dihedral angles},
  journal = {ACM Trans. Graph. (SIGGRAPH)},
  year = {2007},
  volume = {26},
  number = {3},
  month = jul,
  acmid = {1276448},
  address = {New York, NY, USA},
  articleno = {57},
  doi = {10.1145/1276377.1276448},
  issn = {0730-0301},
  issue_date = {July 2007},
  keywords = {dihedral angle, isosurface, tetrahedral mesh generation},
  publisher = {ACM},
  url = {http://doi.acm.org/10.1145/1276377.1276448}
}

@ARTICLE{lafon92,
  author = {Lafon, F. and Osher, S.},
  title = {High order filtering methods for approximating hyperbolic systems
	of conservation laws},
  journal = {J. Comput. Phys.},
  year = {1992},
  volume = {172},
  pages = {574-591}
}

@ARTICLE{Lagally:2001,
  author = {Lagally, E. T. and Medintz, I. and Mathies, R. A.},
  title = {Single-molecule DNA amplification and analysis in an integrated microfluidic
	device},
  journal = {Analytical Chemistry},
  year = {2001},
  volume = {73},
  pages = {565-570}
}

@ARTICLE{Lai:2000,
  author = {Lai, M. C. and Peskin, C. S.},
  title = {An immersed boundary method with formal second-order accuracy and
	reduced numerical viscosity},
  journal = {J. Comput. Phys. },
  year = {2000},
  volume = {160},
  pages = {705-719},
  annote = {An immersed boundary method with formal second-order accuracy and
	reduced numerical viscosity},
  date-added = {2008-09-19 10:28:56 -0500},
  date-modified = {2008-09-19 10:28:56 -0500},
  ty = {JOUR}
}

@ARTICLE{Lake:1997,
  author = {Lake, R. and Klimeck, G. and Bowen, R. C. and Jovanovic, D.},
  title = {Single and multiband modeling of quantum electron transport through
	layered semiconductor devices },
  journal = {Journal of Applied Physics},
  year = {1997},
  volume = {81},
  pages = {7845-7869},
  annote = {Single and multiband modeling of quantum electron transport through
	layered semiconductor devices },
  date-added = {2008-11-25 10:28:56 -0500},
  date-modified = {2008-11-25 10:28:56 -0500},
  ty = {JOUR}
}

@INCOLLECTION{Lamm:2003,
  author = {Lamm, G.},
  title = {The {{Poisson-Boltzmann}} Equation},
  booktitle = {Reviews in Computational Chemistry},
  publisher = {John Wiley and Sons, Inc.},
  year = {2003},
  editor = {Lipkowitz, K. B. and Larter, R. and Cundari, T. R.},
  pages = {147-366},
  address = {Hoboken, N.J.},
  address1 = {19},
  annote = {The {Poisson-Boltzmann} Equation; LammRCC},
  date-added = {2008-09-15 10:04:43 -0500},
  date-modified = {2008-09-15 10:04:43 -0500},
  keywords = {Electrostatics},
  ty = {CHAP}
}

@BOOK{google,
  title = {Google's PageRank and Beyond: The Science of Search Engine Rankings},
  publisher = {Princeton University Press},
  year = {2006},
  author = {Amy N. Langville and Carl D. Meyer}
}

@ARTICLE{Lapidus:2007,
  author = {Lapidus, L. J. and Yao, S. and McGarrity, K. and Hertzog, D. and
	Tubman, E. and Bakajin, O.},
  title = {Protein Hydrophobic Collapse and Early Folding Steps Observed in
	a Microfluidic Mixer},
  journal = {Biophys. J. },
  year = {2007},
  volume = {93},
  pages = {218 - 224}
}

@ARTICLE{Larini:2010,
  author = {Larini, L and Lu, L.Y. and Voth, G. A.},
  title = {The multiscale coarse-graining method. VI. Implementation of three-body
	coarse-grained potentials},
  journal = {Journal of Chemical Physics},
  year = {2010},
  volume = {132},
  number = {164107}
}

@ARTICLE{Lawson:2008,
  author = { Lawson, C. L. and Dutta, S. and Westbrook, J. D. and Henrick, K.
	and Berman, H. M. },
  title = {Representation of viruses in the remediated PDB archive},
  journal = {Acta Crystallographica Section D- Biological Crystalography},
  year = {2008},
  volume = {64},
  pages = {874 - 882},
  annote = {Representation of viruses in the remediated PDB archive },
  date-added = {2009-03-10 },
  date-modified = {2009-03-10},
  ty = {JOUR}
}

@ARTICLE{Layton:2009,
  author = {Layton, A. T.},
  title = {Using integral equations and the immersed interface method to solve
	immersed boundary problems with stiff forces },
  journal = { Comput. Fluids.},
  year = {2009},
  volume = {38},
  pages = { 266-272}
}

@ARTICLE{Lazaridis:1999(a),
  author = {Lazaridis, T. and Karplus, M.},
  title = {{Discrimination of the native from misfolded protein models with
	an energy function including implicit solvation}},
  journal = {J Mol Biol},
  year = {1999},
  volume = {288},
  pages = {477-487},
  number = {3}
}

@ARTICLE{Lazaridis:1999(b),
  author = {Lazaridis, T. and Karplus, M.},
  title = {{Effective energy function for proteins in solution}},
  journal = {Proteins},
  year = {1999},
  volume = {35},
  pages = {133-152},
  number = {2}
}

@ARTICLE{Lebard:2008,
  author = {Lebard, David N. and Matyushov, Dmitry V. },
  title = {Redox entropy of plastocyanin: Developing a microscopic view of mesoscopic
	polar solvation},
  journal = {The Journal of Chemical Physics},
  year = {2008},
  volume = {128},
  pages = {155106},
  number = {15},
  abstract = {View this record in Web of Science},
  bdsk-url-1 = {http://dx.doi.org/10.1063/1.2904879},
  date-added = {2008-06-29 13:12:19 -0500},
  date-modified = {2008-06-29 13:12:19 -0500},
  doi = {10.1063/1.2904879},
  keywords = {molecular\_simulation, multiscale, solvation},
  posted-at = {2008-05-22 12:03:41},
  priority = {0},
  publisher = {AIP}
}

@ARTICLE{Lee:1971,
  author = {Lee, B. and Richards, F. M.},
  title = {The interpretation of protein structures: estimation of static accessibility},
  journal = {J Mol Biol},
  year = {1971},
  volume = {55},
  pages = {379-400},
  number = {3},
  annote = {Feb 14; The interpretation of protein structures: estimation of static
	accessibility; 5551392; LeeRichards},
  bdsk-url-1 = {http://www.ncbi.nlm.nih.gov/entrez/query.fcgi?cmd=Retrieve&db=PubMed&dopt=Citation&list_uids=5551392},
  date-added = {2008-06-29 13:13:28 -0500},
  date-modified = {2008-06-29 13:13:28 -0500},
  keywords = {Electrostatics; Misc},
  ty = {JOUR},
  url = {http://www.ncbi.nlm.nih.gov/entrez/query.fcgi?cmd=Retrieve&db=PubMed&dopt=Citation&list_uids=5551392}
}

@ARTICLE{LeRoZh10,
  author = {Lee, C.Y. and Rozovskii, B.L. and Zhou, H. M.},
  title = {Randomization of Forcing in Large Systems of PDE for Improvement
	of Energy Estimates},
  journal = {Multiscale Modeling and Simulation },
  year = {2010},
  volume = {8},
  number = { }
}

@ARTICLE{Lee932971,
  author = {Lee, C. T. and Fitzgerald, G. and Yang, W. T.},
  title = {Nonlocal Density Functional Calculations - Comparison of 2 Implementation
	Schemes},
  journal = {Journal of Chemical Physics},
  year = {1993},
  volume = {98},
  pages = {2971-2974},
  number = {4},
  month = {Feb},
  abstract = {We have carried out nonlocal density-functional calculations of bond
	dissociation and isomerization energies of several polyatomic molecules
	in two schemes. In the first scheme, the nonlocal energy functional
	is incorporated into the optimization of both the electronic and
	nuclear degrees of freedom. In the second scheme, the nonlocal energy
	functional is only included in a non-self-consistent fashion in which
	we just use the molecular geometry and electron density determined
	by the corresponding local density calculations. Our study reveals
	that the differences of the energies are very small between these
	two schemes.},
  endnotereftype = {Journal Article},
  issn = {0021-9606},
  shorttitle = {Nonlocal Density Functional Calculations - Comparison of 2 Implementation
	Schemes},
  url = {<Go to ISI>://A1993KP93800048}
}

@ARTICLE{Lee922408,
  author = {Lee, C. T. and Yang, W. T.},
  title = {The Divide-and-Conquer Density-Functional Approach - Molecular Internal-Rotation
	and Density of States},
  journal = {Journal of Chemical Physics},
  year = {1992},
  volume = {96},
  pages = {2408-2411},
  number = {3},
  month = {Feb},
  endnotereftype = {Journal Article},
  issn = {0021-9606},
  shorttitle = {The Divide-and-Conquer Density-Functional Approach - Molecular Internal-Rotation
	and Density of States},
  url = {<Go to ISI>://A1992HC61000082}
}

@ARTICLE{Lee88305,
  author = {Lee, C. T. and Yang, W. T. and Parr, R. G.},
  title = {Local Softness and Chemical-Reactivity in the Molecules Co, Scn-
	and H2co},
  journal = {Theochem-Journal of Molecular Structure},
  year = {1988},
  volume = {40},
  pages = {305-313},
  month = {Jan},
  endnotereftype = {Journal Article},
  issn = {0166-1280},
  shorttitle = {Local Softness and Chemical-Reactivity in the Molecules Co, Scn- and
	H2co},
  url = {<Go to ISI>://A1988M178000023}
}

@ARTICLE{Lee88785,
  author = {Lee, C. T. and Yang, W. T. and Parr, R. G.},
  title = {Development of the Colle-Salvetti Correlation-Energy Formula into
	a Functional of the Electron-Density},
  journal = {Physical Review B},
  year = {1988},
  volume = {37},
  pages = {785-789},
  number = {2},
  month = {Jan},
  endnotereftype = {Journal Article},
  isinote = {ISI Document Delivery No.: L9762 Times Cited: 16425 Cited Reference
	Count: 16},
  issn = {0163-1829},
  shorttitle = {Development of the Colle-Salvetti Correlation-Energy Formula into
	a Functional of the Electron-Density},
  url = {<Go to ISI>://A1988L976200011}
}

@ARTICLE{Lee:1988,
  author = { Lee, C. T. and Yang, W. T. and Parr, R. G. },
  title = {Development of the Colle-Salvetti correlation-energy formula into
	a functional of the electron-density},
  journal = {Physical Review B},
  year = {1988},
  volume = {37},
  pages = {785 -- 789}
}

@ARTICLE{GBLee:2001,
  author = {Lee, G. B. and Chen, S. H. and Huang, G. R. and Sung, W. C. and Lin,
	Y. H.},
  title = {Microfabricated plastic chips by hot embossing methods and their
	applications for DNA separation and detection},
  journal = {Sensors and Actuators B-Chemical},
  year = {2001},
  volume = {75},
  pages = {142-148}
}

@INPROCEEDINGS{LAD02,
  author = {Haeyoung Lee and Pierre Alliez and Mathieu Desbrun},
  title = {Angle Analyzer: A Triangle-Quad Mesh Codec},
  booktitle = {Eurographics Conference},
  year = {2002},
  volume = {21},
  pages = {383--392},
  month = Sep
}

@INPROCEEDINGS{Compression,
  author = {H. Lee and M. Desbrun and P. Schr{\"o}der},
  title = {Progressive Encoding of Complex Isosurfaces},
  booktitle = {Proc. of ACM SIGGRAPH},
  year = {2003},
  pages = {471--476}
}

@ARTICLE{LDS03,
  author = {Haeyoung Lee and Mathieu Desbrun and Peter Schr{\"o}der},
  title = {Progressive Encoding of Complex Isosurfaces},
  journal = {ACM Trans. on Graphics (SIGGRAPH)},
  year = {2003},
  volume = {22},
  pages = {471--476},
  number = {3},
  month = jun
}

@ARTICLE{Lee084200,
  author = {Lee, H. and Kim, K. W. and Park, J. and Kim, H. and Kim, S. and Kim,
	D. and Hu, X. Q. and Yang, W. T. and Hong, J. Y.},
  title = {A general strategy for construction of both 2,6-cis- and 2,6-trans-disubstituted
	tetrahydropyrans: Substrate-controlled asymmetric total synthesis
	of (+)-scanlonenyne},
  journal = {Angewandte Chemie-International Edition},
  year = {2008},
  volume = {47},
  pages = {4200-4203},
  number = {22},
  endnotereftype = {Journal Article},
  issn = {1433-7851},
  shorttitle = {A general strategy for construction of both 2,6-cis- and 2,6-trans-disubstituted
	tetrahydropyrans: Substrate-controlled asymmetric total synthesis
	of (+)-scanlonenyne},
  url = {<Go to ISI>://000256261900032}
}

@INPROCEEDINGS{LKMD01,
  author = {Haeyoung Lee and Laeyhun Kim and Mark Meyer and Mathieu Desbrun},
  title = {Meshes on Fire},
  booktitle = {Eurographics Workshop on Animation and Simulation},
  year = {2001},
  month = sep
}

@ARTICLE{LTD05,
  author = {Haeyoung Lee and Yiying Tong and Mathieu Desbrun},
  title = {Geodesics-based One-to-One Parameterization of 3D Triangle Meshes},
  journal = {IEEE Multimedia},
  year = {2005},
  volume = {12},
  pages = {27--33},
  number = {1},
  month = jan
}

@ARTICLE{Lee:2009,
  author = {Lee, J. and Wu, S. and Zhang, Y.},
  title = {{Ab initio protein structure prediction}},
  journal = {From Protein Structure to Function with Bioinformatics},
  year = {2009},
  volume = {1},
  pages = {3-25}
}

@ARTICLE{Lee:2003a,
  author = {Long Lee and Randall J. LeVeque},
  title = {An Immersed Interface Method for Incompressible Navier--Stokes Equations},
  journal = {SIAM Journal on Scientific Computing},
  year = {2003},
  volume = {25},
  pages = {832-856},
  number = {3},
  abstract = {The method developed in this paper is motivated by Peskin's immersed
	boundary (IB) method, and allows one to model the motion of flexible
	membranes or other structures immersed in viscous incompressible
	fluid using a fluid solver on a fixed Cartesian grid. The IB method
	uses a set of discrete delta functions to spread the entire singular
	force exerted by the immersed boundary to the nearby fluid grid points.
	Our method instead incorporates part of this force into jump conditions
	for the pressure, avoiding discrete dipole terms that adversely affect
	the accuracy near the immersed boundary. This has been implemented
	for the two-dimensional incompressible Navier--Stokes equations using
	a high-resolution finite-volume method for the advective terms and
	a projection method to enforce incompressibility. In the projection
	step, the correct jump in pressure is imposed in the course of solving
	the Poisson problem. This gives sharp resolution of the pressure
	across the interface and also gives better volume conservation than
	the traditional IB method. Comparisons between this method and the
	IB method are presented for several test problems. Numerical studies
	of the convergence and order of accuracy are included. },
  bdsk-url-1 = {http://link.aip.org/link/?SCE/25/832/1},
  bdsk-url-2 = {http://dx.doi.org/10.1137/S1064827502414060},
  date-added = {2008-09-14 15:32:12 -0500},
  date-modified = {2008-09-14 15:32:12 -0500},
  doi = {10.1137/S1064827502414060},
  keywords = {Mathematics; FluidMechanics},
  publisher = {SIAM},
  url = {http://link.aip.org/link/?SCE/25/832/1}
}

@ARTICLE{Lee:2004,
  author = {Lee, M. C. and Duan, Y.},
  title = {{Distinguish protein decoys by using a scoring function based on
	a new AMBER force field, short molecular dynamics simulations, and
	the generalized born solvent model}},
  journal = {Proteins},
  year = {2004},
  volume = {55},
  pages = {620-634},
  number = {3}
}

@ARTICLE{Lee:2001,
  author = {Lee, M. R. and Tsai, J. and Baker, D. and Kollman, P. A.},
  title = {{Molecular dynamics in the endgame of protein structure prediction}},
  journal = {J Mol Biol},
  year = {2001},
  volume = {313},
  pages = {417-430},
  number = {2}
}

@ARTICLE{Lee:2004a,
  author = {Lee, M. S. and Salsbury, F. R. , Jr. and Olson, M. A.},
  title = {An efficient hybrid explicit/implicit solvent method for biomolecular
	simulations},
  journal = {Journal of Computational Chemistry},
  year = {2004},
  volume = {25},
  pages = {1967-78},
  number = {16},
  abstract = {We present a new hybrid explicit/implicit solvent method for dynamics
	simulations of macromolecular systems. The method models explicitly
	the hydration of the solute by either a layer or sphere of water
	molecules, and the generalized Born (GB) theory is used to treat
	the bulk continuum solvent outside the explicit simulation volume.
	To reduce the computational cost, we implemented a multigrid method
	for evaluating the pairwise electrostatic and GB terms. It is shown
	that for typical ion and protein simulations our method achieves
	similar equilibrium and dynamical observables as the conventional
	particle mesh Ewald (PME) method. Simulation timings are reported,
	which indicate that the hybrid method is much faster than PME, primarily
	due to a significant reduction in the number of explicit water molecules
	required to model hydration effects.},
  annote = {An efficient hybrid explicit/implicit solvent method for biomolecular
	simulations},
  bdsk-url-1 = {http://dx.doi.org/10.1002/jcc.20119},
  date-added = {2008-09-15 10:07:46 -0500},
  date-modified = {2008-09-15 10:07:46 -0500},
  keywords = {Solvation; Electrostatics; MolecularSimulation; Multiscale},
  ty = {JOUR},
  url = {http://dx.doi.org/10.1002/jcc.20119}
}

@ARTICLE{LLM,
  author = {Lee, S. and Lele, S. K. and Moin, P.},
  title = {Interaction of isotropic turbulence with shock waves: Effect of shock
	strength},
  journal = {J. Fluid Mech.},
  year = {1997},
  volume = {340},
  pages = {225-247}
}

@ARTICLE{LeZhBa10,
  author = {Lee, S. and Zhou, H. M. and Baldwin, D.},
  title = {A Numerical Study of Void Nucleation and Growth in a Flip Chip Assembly
	Process},
  journal = { Modelling and Simulation in Materials Science and Engineering},
  year = {2010},
  volume = {18},
  number = {065005 }
}

@ARTICLE{Lee98259,
  author = {Lee, T. S. and Lewis, J. P. and Yang, W. T.},
  title = {Linear-scaling quantum mechanical calculations of biological molecules:
	The divide-and-conquer approach},
  journal = {Computational Materials Science},
  year = {1998},
  volume = {12},
  pages = {259-277},
  number = {3},
  month = {Oct},
  abstract = {The divide-and-conquer technique for linear-scaling quantum mechanical
	calculations is reviewed. The method divides a large system into
	many subsystems, determines the density matrix of each subsystem
	separately, and sums the corresponding subsystem contributions to
	obtain the total density matrix and the energy of the system. There
	is a uniform chemical potential to allow transfer of electrons between
	subsystems and to insure the normalization of the electron density.
	The implementation of the method for semiempirical quantum chemistry
	Hamiltonians is described. The review describes the application to
	the study of the catalytic mechanisms of cytidine deaminase, an enzyme
	which accelerates the rate of hydrolytic deamination of cytidine
	to uridine. The linear-scaling quantum mechanical calculations determined
	the active species of the ground-state complex and the structure
	of the reaction transition-state analog complex. (C) 1998 Elsevier
	Science B.V. All rights reserved.},
  endnotereftype = {Journal Article},
  issn = {0927-0256},
  shorttitle = {Linear-scaling quantum mechanical calculations of biological molecules:
	The divide-and-conquer approach},
  url = {<Go to ISI>://000077608200006}
}

@ARTICLE{TSLee:1998,
  author = { Lee, T. S. and Lewis, J. P. and Yang, W. T.},
  title = {Linear-scaling quantum mechanical calculations of biological molecules:
	The divide-and-conquer approach},
  journal = {Comput. Mater. Science},
  year = {1998},
  volume = {12},
  pages = {259 -- 277}
}

@ARTICLE{Lee98397,
  author = {Lee, T. S. and Yang, W. T.},
  title = {Frozen density matrix approach for electronic structure calculations},
  journal = {International Journal of Quantum Chemistry},
  year = {1998},
  volume = {69},
  pages = {397-404},
  number = {3},
  month = {Aug},
  abstract = {A frozen density matrix approach for determining local geometry changes
	of large molecules is proposed based on the density matrix divide-and-conquer
	method. This approach divides a large molecule into a small active
	part and the rest as the frozen part. After a single-point self-consistent
	field (SCF) calculation for the whole molecule, only the local molecular
	orbitals of the active part and its neighbor are updated when the
	geometry of the active part changes. The updated density matrix is
	calculated from the new local molecular orbitals of the active part
	and the stored local molecular orbitals of the frozen part. The electron
	transfer between the active and the frozen part is allowed via a
	common and variable chemical potential. The preliminary tests using
	semiempirical quantum chemical methods show this approach predicts
	the local geometry change well. The error in geometric parameters
	is less than 0.002 Angstrom and less than 0.5 degrees for bond length
	and bond angle, respectively. (C) 1998 John Wiley & Sons, Inc.},
  endnotereftype = {Journal Article},
  issn = {0020-7608},
  shorttitle = {Frozen density matrix approach for electronic structure calculations},
  url = {<Go to ISI>://000075006800016}
}

@ARTICLE{Lee:1996,
  author = {Lee, Tai S. and York, Darrin M. and Yang, Weitao },
  title = {Linear-scaling semiempirical quantum calculations for macromolecules},
  journal = {The Journal of Chemical Physics},
  year = {1996},
  volume = {105},
  pages = {2744--2750},
  number = {7},
  bdsk-url-1 = {http://link.aip.org/link/?JCPSA6/105/2744/1},
  date-added = {2008-06-30 06:13:53 -0500},
  date-modified = {2008-06-30 06:13:53 -0500},
  doi = {10.1063/1.472136},
  keywords = {quantum\_mechanics, solvation}
}

@ARTICLE{Lee962744,
  author = {Lee, T. S. and York, D. M. and Yang, W. T.},
  title = {Linear-scaling semiempirical quantum calculations for macromolecules},
  journal = {Journal of Chemical Physics},
  year = {1996},
  volume = {105},
  pages = {2744-2750},
  number = {7},
  month = {Aug},
  abstract = {A linear-scaling method to carry out semiempirical quantum mechanical
	calculations for large systems has been developed based on the density
	matrix version of the divide-and-conquer approach. The method has
	been tested and demonstrated to be accurate and efficient. With this
	implementation, semiempirical quantum mechanical calculations are
	made possible for large molecules over 9000 atoms on a typical workstation.
	For biological macromolecules, solvent effects are included with
	a dielectric continuum model. (C) 1996 American Institute of Physics.},
  endnotereftype = {Journal Article},
  issn = {0021-9606},
  shorttitle = {Linear-scaling semiempirical quantum calculations for macromolecules},
  url = {<Go to ISI>://A1996VB45200023}
}

@ARTICLE{Lee957549,
  author = {Lee, T. S. and York, D. M. and Yang, W. T.},
  title = {A New Definition of Atomic Charges Based on a Variational Principle
	for the Electrostatic Potential-Energy},
  journal = {Journal of Chemical Physics},
  year = {1995},
  volume = {102},
  pages = {7549-7556},
  number = {19},
  month = {May},
  endnotereftype = {Journal Article},
  issn = {0021-9606},
  shorttitle = {A New Definition of Atomic Charges Based on a Variational Principle
	for the Electrostatic Potential-Energy},
  url = {<Go to ISI>://A1995QX77300029}
}

@ARTICLE{Leitch:2007,
  author = {Leitch, S. and Bradley, M. J. and Rowe, J. L. and Chivers, P. T.
	and Maroney, M. J.},
  title = {Nickel-Specific Response in the Transcriptional Regulator, Escherichia
	coli {NikR}},
  journal = {Journal of the American Chemical Society},
  year = {in press},
  abstract = {Studies of the transcriptional repression of the Ni-specific permease
	encoded by the Pnik operon by Escherichia coli NikR using a LacZ
	reporter assay establish that the NikR response is specific to nickel
	in vivo. Toward understanding this metal ion-specific response, X-ray
	absorption spectroscopy (XAS) analysis of various M-NikR complexes
	(M = Co(II), Ni(II), Cu(II), Cu(I), and Zn(II)) was used to show
	that each high-affinity binding site metal adopts a unique structure,
	with Ni(II) and Cu(II) being the only two metal ions to feature planar
	four-coordinate complexes. The results are consistent with an allosteric
	mechanism whereby the geometry and ligand selection of the metal
	present in the high-affinity site induce a unique conformation in
	NikR that subsequently influences DNA binding. The influence of the
	high-affinity metal on protein structure was examined using hydrogen/deuterium
	(H/D) exchange detected by liquid chromatography-electrospray ionization
	mass spectrometry (LC-ESI-MS). Each NikR complex gives rise to differing
	amounts of H/D exchange; Zn(II)- and Co(II)-NikR are most like apo-NikR,
	while the exchange time course is substantially different for Ni(II)
	and to a lesser extent for Cu(II). In addition to the high-affinity
	metal binding site, {E. coli} NikR has a low-affinity metal-binding
	site that affects DNA binding affinity. We have characterized this
	low-affinity site using XAS in heterobimetallic complexes of NikR.
	When Cu(II) occupies the high-affinity site and Ni(II) occupies the
	low-affinity site, the Ni K-edge XAS spectra show that the Ni site
	is composed of six N/O-donors. A similar low-affinity site structure
	is found for the NikR complex when Co(II) occupies the low-affinity
	site and Ni(II) occupies the high-affinity site, except that one
	of the Co(II) ligands is a chloride derived from the buffer.},
  bdsk-url-1 = {http://dx.doi.org/10.1021/ja068505y},
  date-added = {2008-09-16 15:46:13 -0500},
  date-modified = {2008-09-16 15:46:13 -0500},
  keywords = {Metalloregulation},
  url = {http://dx.doi.org/10.1021/ja068505y}
}

@INPROCEEDINGS{LCS,
  author = {P.F.J. Lermusiaux and F. Lekien},
  title = {Dynamics and Lagrangian Coherent Structures in the Ocean and their
	Uncertainty},
  booktitle = {Dynamical Systems Methods in Fluid Dynamics},
  year = {2005},
  editor = {J.E. Marsden and J. Scheurle (Eds)},
  series = {Mathematisches Forschungsinstitut Oberwolfach 531},
  pages = {19--20}
}

@ARTICLE{Lether:2000,
  author = {Lether, F. G.},
  title = {Analytical Expansion and Numerical Approximation of the Fermi-Dirac
	Integrals of order -1/2 and 1/2},
  journal = {J. Sci. Comput.},
  year = {2000},
  volume = {4},
  pages = {479-497}
}

@ARTICLE{LeVeque96,
  author = {Randall J. LeVeque},
  title = {{High-Resolution Conservative Algorithms for Advection in Incompressible
	Flow}},
  journal = {J. Numer. Anal.},
  year = {1996},
  volume = {33},
  pages = {627--665}
}

@ARTICLE{LeVeque:1994,
  author = {LeVeque, R. J. and Li, Z. L.},
  title = {The immersed interface method for elliptic equations with discontinuous
	coefficients and singular sources},
  journal = {SIAM J. Numer. Anal. },
  year = {1994},
  volume = {31},
  pages = {1019-1044},
  annote = {The immersed interface method for elliptic equations with discontinuous
	coefficients and singular sources},
  date-added = {2008-09-19 10:28:56 -0500},
  date-modified = {2008-09-19 10:28:56 -0500},
  ty = {JOUR}
}

@ARTICLE{leveque,
  author = {LeVeque, R. J. and Pelanti, M.},
  title = {A class of approximate Riemann solvers and their relation to relaxation
	schemes},
  journal = {J. Comput. Phys.},
  year = {2001},
  volume = {172},
  pages = {574-591}
}

@ARTICLE{Levin:2002,
  author = {Levin, Y.},
  title = {Electrostatic correlations: from plasma to biology},
  journal = {Rep. Prog. Phys.},
  year = {2002},
  volume = {65},
  pages = {1577-1632.}
}

@ARTICLE{Levitt:1999,
  author = {Levitt, D. G. },
  title = {Modeling of Ion Channels},
  journal = {J. Gen. Physiol.},
  year = {1999},
  volume = {113},
  pages = {789-794},
  number = { 6}
}

@ARTICLE{Levitt:1986,
  author = {Levitt, D. G. },
  title = {Interpretation of Biological ION Channel Flux Data--Reaction-Rate
	versus Continuum Theory},
  journal = {Annual Review of Biophysics and Biophysical Chemistry},
  year = {1986},
  volume = {15},
  pages = {29-57},
  number = { }
}

@ARTICLE{Levitt:1995,
  author = {Levitt, M. and Hirshberg, M. and Sharon, R. and Daggett, V.},
  title = {{Potential-Energy Function and Parameters for Simulations of the
	Molecular-Dynamics of Proteins and Nucleic-Acids in Solution}},
  journal = {Computer Physics Communications},
  year = {1995},
  volume = {91},
  pages = {215-231},
  number = {1-3}
}

@INPROCEEDINGS{Levy06,
  author = {Bruno Levy},
  title = {{Laplace-Beltrami }Eigenfunctions: {Towards} an Algorithm that Understands
	Geometry},
  booktitle = {IEEE Shape Modeling and Applications (invited talk)},
  year = {2006},
  page = {13}
}

@ARTICLE{TriangleCentralWENO,
  author = {D. Levy and S. Nayak and C.W. Shu and Y.T. Zhang},
  title = {{Central WENO Schemes for Hamilton-Jacobi Equations on Triangular
	Meshes}},
  journal = {J. Sci. Comput.},
  year = {2005},
  volume = {27},
  pages = {532--552}
}

@ARTICLE{Levy852334,
  author = {Levy, M. and Yang, W. and Parr, R. G.},
  title = {A New Functional with Homogeneous Coordinate Scaling in Density Functional
	Theory - F[P,Lambda]},
  journal = {Journal of Chemical Physics},
  year = {1985},
  volume = {83},
  pages = {2334-2336},
  number = {5},
  endnotereftype = {Journal Article},
  issn = {0021-9606},
  shorttitle = {A New Functional with Homogeneous Coordinate Scaling in Density Functional
	Theory - F[P,Lambda]},
  url = {<Go to ISI>://A1985AQG3700039}
}

@ARTICLE{Levy:2003,
  author = {Levy, R. M. and Zhang, L. Y. and Gallicchio, E. and Felts, A. K.},
  title = {On the nonpolar hydration free energy of proteins: surface area and
	continuum solvent models for the solute-solvent interaction energy},
  journal = {Journal of the American Chemical Society},
  year = {2003},
  volume = {125},
  pages = {9523-9530},
  number = {31},
  abstract = {Implicit solvent hydration free energy models are an important component
	of most modern computational methods aimed at protein structure prediction,
	binding affinity prediction, and modeling of conformational equilibria.
	The nonpolar component of the hydration free energy, consisting of
	a repulsive cavity term and an attractive {van der waals} solute-solvent
	interaction term, is often modeled using estimators based on the
	solvent exposed solute surface area. In this paper, we analyze the
	accuracy of linear surface area models for predicting the {van der
	waals} solute-solvent interaction energies of native and non-native
	protein conformations, peptides and small molecules, and the desolvation
	penalty of protein-protein and protein-ligand binding complexes.
	The target values are obtained from explicit solvent simulations
	and from a continuum solvent {van der waals} interaction energy model.
	The results indicate that the standard surface area model, while
	useful on a coarse-grained scale, may not be accurate or transferable
	enough for high resolution modeling studies of protein folding and
	binding. The continuum model constructed in the course of this study
	provides one path for the development of a computationally efficient
	implicit solvent nonpolar hydration free energy estimator suitable
	for high-resolution structural and thermodynamic modeling of biological
	macromolecules.},
  annote = {On the nonpolar hydration free energy of proteins: surface area and
	continuum solvent models for the solute-solvent interaction energy;
	LevyGallicchio1},
  bdsk-url-1 = {http://dx.doi.org/10.1021/ja029833a},
  date-added = {2008-08-29 15:50:55 -0500},
  date-modified = {2008-08-29 15:50:55 -0500},
  keywords = {Solvation},
  ty = {JOUR},
  url = {http://dx.doi.org/10.1021/ja029833a}
}

@ARTICLE{Lewiner03efficientimplementation,
  author = {Thomas Lewiner and Helio Lopes and Antonio Wilson Vieira and Geovan
	Tavares},
  title = {Efficient implementation of Marching Cubes' cases with topological
	guarantees},
  journal = {Journal of Graphics Tools},
  year = {2003},
  volume = {8},
  pages = {2003}
}

@ARTICLE{Lewis985407,
  author = {Lewis, J. P. and Carter, C. W. and Hermans, J. and Pan, W. and Lee,
	T. S. and Yang, W. T.},
  title = {Active species for the ground-state complex of cytidine deaminase:
	A linear-scaling quantum mechanical investigation},
  journal = {Journal of the American Chemical Society},
  year = {1998},
  volume = {120},
  pages = {5407-5410},
  number = {22},
  month = {Jun},
  abstract = {We present results of large-scale (1330 atoms) linear-scaling quantum
	mechanical serniempirical (PM3) simulations done to optimize geometries
	surrounding the active site within the enzyme cytidine deaminase.
	We make a strong prediction about the structure of the active site
	for the active species, based on the energetics of the calculated
	structures and comparisons to X-ray crystallographic data. The lowest
	energy structure indicates that Zn-OH- is the active species formed
	prior to nucleophilic attack of the ligand, that the active species
	of Glu-104 is with O-epsilon 2 protonated and hydrogen-bonded with
	N-3 Of the ligand, and that the C-4 and OH- atoms are significantly
	closer than is permitted by their van der Waals radii. In addition,
	we predict structures corresponding to the low-pH and high-pH states
	in the active site of the enzyme.},
  endnotereftype = {Journal Article},
  issn = {0002-7863},
  shorttitle = {Active species for the ground-state complex of cytidine deaminase:
	A linear-scaling quantum mechanical investigation},
  url = {<Go to ISI>://000074213800006}
}

@ARTICLE{Lewis99242,
  author = {Lewis, J. P. and Liu, S. B. and Lee, T. S. and Yang, W. T.},
  title = {A linear-scaling quantum mechanical investigation of cytidine deaminase},
  journal = {J. Comput. Phys.},
  year = {1999},
  volume = {151},
  pages = {242-263},
  number = {1},
  month = {May},
  abstract = {We describe the divide-and-conquer technique for linear-scaling semiempirical
	quantum mechanical calculations. This method has been successfully
	applied to study cytidine deaminase. Large-scale simulations were
	performed for optimizing geometries surrounding the active site of
	the enzyme and obtaining related energetics. The results of the minimizations
	provide a significant complement to experimental efforts and aid
	in the understanding of the enzymatic profile of cytidine deaminase.
	More specifically, we present our predictions about the structure
	of the active species and the structure of the active site for low
	pH. Finally, we present our results for the structure of the zinc
	ion coordination for different substrates which represent points
	along the reaction profile. In particular, we find that our results
	for the Zn-S-gamma 132 and the Zn-S-gamma 129 bondlengths yield similar
	trends compared to x-ray crystallography data as the enzyme structure
	changes from the ground-state to the transition-state analog and
	from the transition-state analog to the product. (C) 1999 Academic
	Press.},
  endnotereftype = {Journal Article},
  issn = {0021-9991},
  shorttitle = {A linear-scaling quantum mechanical investigation of cytidine deaminase},
  url = {<Go to ISI>://000080181500011}
}

@ARTICLE{Libo:2010,
  author = {Li, B. and Lu, B. Z. and Wang, Z. M. and McCammon, J. A.},
  title = {Solutions to a reduced {P}oisson{-}{N}ernst{-P}lanck system and determination
	of reaction rates},
  journal = {Physica A},
  year = {2010},
  volume = {389},
  pages = {1329-1345},
  number = {7}
}

@ARTICLE{VarLevelSet,
  author = {Chunming Li and Chenyang Xu and Changfeng Gui and Martin D. Fox},
  title = {{Level Set Evolution Without Re-initialization: A New Variational
	Formulation}},
  journal = {Proc. of IEEE CVPR},
  year = {2005},
  volume = {1},
  pages = {430--436}
}

@ARTICLE{Li:2006k,
  author = {Li, G. and Aluru, N. R.},
  title = {A Lagrangian approach for quantum-mechanical electrostatic analysis
	of deformable silicon nanostructures },
  journal = {Engineering Analysis with Boundary Element },
  year = {2006},
  volume = {30},
  pages = {925-939 },
  annote = {A Lagrangian approach for quantum-mechanical electrostatic analysis
	of deformable silicon nanostructures },
  date-added = {2008-11-25 10:28:56 -0500},
  date-modified = {2008-11-25 10:28:56 -0500},
  ty = {JOUR}
}

@ARTICLE{Li:2004k,
  author = {Li, G. and Aluru, N. R.},
  title = {Hybrid techniques for electrostatic analysis of nanoelectromechanical
	systems },
  journal = {J. Applied Physics},
  year = {2004},
  volume = {96},
  pages = {2221-2231 },
  annote = {Hybrid techniques for electrostatic analysis of nanoelectromechanical
	systems },
  date-added = {2008-11-25 10:28:56 -0500},
  date-modified = {2008-11-25 10:28:56 -0500},
  ty = {JOUR}
}

@ARTICLE{PROPKA,
  author = {Li, H. and Robertson, A. D. and Jensen, J. H.},
  title = {Very fast empirical prediction and rationalization of protein pKa
	values},
  journal = {Proteins},
  year = {2005},
  volume = {61},
  pages = {704-21},
  number = {4},
  abstract = {A very fast empirical method is presented for structure-based protein
	pKa prediction and rationalization. The desolvation effects and intra-protein
	interactions, which cause variations in pKa values of protein ionizable
	groups, are empirically related to the positions and chemical nature
	of the groups proximate to the pKa sites. A computer program is written
	to automatically predict pKa values based on these empirical relationships
	within a couple of seconds. Unusual pKa values at buried active sites,
	which are among the most interesting protein pKa values, are predicted
	very well with the empirical method. A test on 233 carboxyl, 12 cysteine,
	45 histidine, and 24 lysine pKa values in various proteins shows
	a root-mean-square deviation (RMSD) of 0.89 from experimental values.
	Removal of the 29 pKa values that are upper or lower limits results
	in an RMSD = 0.79 for the remaining 285 pKa values.},
  annote = {Very fast empirical prediction and rationalization of protein pKa
	values.
	
	
	 PROPKA},
  bdsk-file-1 = {YnBsaXN0MDDUAQIDBAUGCQpYJHZlcnNpb25UJHRvcFkkYXJjaGl2ZXJYJG9iamVjdHMSAAGGoNE
	HCFRyb290gAFfEA9OU0tleWVkQXJjaGl2ZXKoCwwXGBkdJCVVJG51bGzTDQ4PEBEUViRjbGFzc1
	dOUy5rZXlzWk5TLm9iamVjdHOAB6ISE4ACgAOiFRaABIAGWWFsaWFzRGF0YVxyZWxhdGl2ZVBhd
	GjSDRobHFdOUy5kYXRhgAVPEQHWAAAAAAHWAAIAAAxNYWNpbnRvc2ggSEQAAAAAAAAAAAAAAAAA
	AADD4v5NSCsAAAAZYksaMjAwNS1MaVJvYmVydHNvbkplbnNlbi5wZGYAAAAAAAAAAAAAAAAAAAA
	AAAAAAAAAAAAAAAAAAAAAAAAAAAAAABkGoMHuQL8AAAAAAAAAAAAEAAQAAAkgAAAAAAAAAAAAAA
	AAAAAAB0FyY2hpdmUAABAACAAAw+NSrQAAABEACAAAwe6VHwAAAAEAFAAZYksAGWIDAAqkKAAKp
	BEAAHrcAAIAUE1hY2ludG9zaCBIRDpVc2VyczpiYWtlcjpEb2N1bWVudHM6UmVmZXJlbmNlczpB
	cmNoaXZlOjIwMDUtTGlSb2JlcnRzb25KZW5zZW4ucGRmAA4ANgAaADIAMAAwADUALQBMAGkAUgB
	vAGIAZQByAHQAcwBvAG4ASgBlAG4AcwBlAG4ALgBwAGQAZgAPABoADABNAGEAYwBpAG4AdABvAH
	MAaAAgAEgARAASAENVc2Vycy9iYWtlci9Eb2N1bWVudHMvUmVmZXJlbmNlcy9BcmNoaXZlLzIwM
	DUtTGlSb2JlcnRzb25KZW5zZW4ucGRmAAATAAEvAAAVAAIADP//AADSHh8gIVgkY2xhc3Nlc1ok
	Y2xhc3NuYW1loyEiI11OU011dGFibGVEYXRhVk5TRGF0YVhOU09iamVjdF8QQy4uLy4uLy4uLy4
	uL0RvY3VtZW50cy9SZWZlcmVuY2VzL0FyY2hpdmUvMjAwNS1MaVJvYmVydHNvbkplbnNlbi5wZGAAAA
	AAAAACgAAAAAAAAAAAAAAAAAAAMp},
  bdsk-url-1 = {http://dx.doi.org/10.1002/prot.20660},
  date-added = {2008-09-01 13:53:42 -0500},
  date-modified = {2008-09-01 13:53:48 -0500},
  keywords = {Solvation; Electrostatics},
  local-url = {internal-pdf://fulltext-1677901824/fulltext.pdf},
  ty = {JOUR},
  url = {http://dx.doi.org/10.1002/prot.20660}
}

@ARTICLE{Li:2004e,
  author = {Li, H. and Robertson, A. D. and Jensen, J. H.},
  title = {The determinants of carboxyl {pKa} values in turkey ovomucoid third
	domain},
  journal = {Proteins},
  year = {2004},
  volume = {55},
  pages = {689-704},
  number = {3},
  abstract = {A computational methodology for protein pKa predictions, based on
	ab initio quantum mechanical treatment of part of the protein and
	linear {Poisson-Boltzmann} equation treatment of the bulk solvent,
	is presented. The method is used to predict and interpret the pKa
	values of the five carboxyl residues (Asp7, Glu10, Glu19, Asp27,
	and Glu43) in the serine protease inhibitor turkey ovomucoid third
	domain. All the predicted pKa values are within 0.5 pH units of experiment,
	with a root-mean-square deviation of 0.31 pH units. We show that
	the decreased pKa values observed for some of the residues are primarily
	due to hydrogen bonds to the carboxyl oxygens. Hydrogen bonds involving
	amide protons are shown to be particularly important, and the effect
	of hydrogen bonding is shown to be nonadditive. Hydrophobic effects
	are also shown to be important in raising the pKa. Interactions with
	charged residues are shown to have relatively little effect on the
	carboxyl pKa values in this protein, in general agreement with experiment},
  annote = {The determinants of carboxyl pKa values in turkey ovomucoid third
	domain},
  bdsk-url-1 = {http://dx.doi.org/10.1002/prot.20032},
  date-added = {2008-09-01 13:54:02 -0500},
  date-modified = {2008-09-01 13:54:02 -0500},
  keywords = {Solvation; Electrostatics},
  ty = {JOUR},
  url = {http://dx.doi.org/10.1002/prot.20032}
}

@ARTICLE{Li:1996,
  author = {Li, J. and Fisher, C. L. and Chen, J. L. and Bashford, D. and Noodleman,
	L.},
  title = {Calculation of Redox Potentials and {pKa} Values of Hydrated Transition
	Metal Cations by a Combined Density Functional and Continuum Dielectric
	Theory},
  journal = {Inorganic Chemistry},
  year = {1996},
  volume = {35},
  pages = {4694-702},
  number = {16},
  abstract = {Density functional and continuum dielectric theories have been combined
	to calculate molecular properties such as hydration enthalpies, redox
	potentials, and absolute pKa values of transition metal cations in
	solution. The discrete cluster model, which is treated explicitly
	by density functional theory, includes six waters in the first hydration
	shell and another twelve waters in the second shell. The solvent
	reaction field is obtained from a finite-difference solution to the
	{Poisson-Boltzmann} equation and is coupled to the nonlocal density
	functional calculation in a self-consistent way. The calculated hydration
	enthalpies are 409, 1073, 431, and 1046 kcal/mol for Mn2+, Mn3+,
	Fe2+, and Fe3+, respectively, comparing fairly well to the experimental
	measurements of 440, 1087, 465, and 1060 kcal/mol. The calculated
	redox potentials for the Mn2+/Mn3+ and Fe2+/Fe3+ pairs are 1.59 and
	1.06 V, respectively, in good agreement with the experimental values
	of 1.56 and 0.77 V. The computed absolute pKa values, 14.0, -6.5,
	9.0, and -4.0 for Mn2+, Mn3+, Fe2+, and Fe3+, respectively, deviate
	significantly from the experimental results of 10.6, 0.1, 9.5, and
	2.2 but show the proper behavior with changes in oxidation state
	and metal type. The calculated redox potentials and pKa values appear
	to converge toward the experimental data with increasing size of
	the cluster models. For such highly charged cations, the second hydration
	shell in the cluster model is indispensable, since this buffer shell
	retains strong hydrogen bonds and electron transfer between the inner
	and outer shells as well as the solute-solvent dispersion interaction.},
  annote = {Calculation of Redox Potentials and pKa Values of Hydrated Transition
	Metal Cations by a Combined Density Functional and Continuum Dielectric
	Theory},
  bdsk-url-1 = {http://pubs.acs.org/cgi-bin/abstract.cgi/inocaj/1996/35/i16/abs/ic951428f.html},
  date-added = {2008-09-01 13:51:43 -0500},
  date-modified = {2008-09-01 13:51:43 -0500},
  keywords = {Solvation; Electrostatics},
  ty = {JOUR},
  url = {http://pubs.acs.org/cgi-bin/abstract.cgi/inocaj/1996/35/i16/abs/ic951428f.html}
}

@ARTICLE{LiangLi:2010,
  author = {Li, L. and Ismagilov, R. F.},
  title = {Protein Crystallization Using Microfluidic Technologies Based on
	Valves, Droplets, and SlipChip
	
	},
  journal = {Annual Review of Biophysics},
  year = {2010},
  volume = {39}
}

@ARTICLE{Yau,
  author = {P. Li and S. T. Yau},
  title = {Estimate of Eigenvalues of a Compact Riemannian Manifold},
  journal = {Proceedings of the Symposium in Pure Mathematics},
  year = {1980},
  volume = {36},
  pages = {205?235}
}

@ARTICLE{RLig:2002,
  author = {Li, R. and Tang, T. and Zhang, P.},
  title = {{A moving mesh finite element algorithm for singular problems in
	two and three space dimensions}},
  journal = {J. Comput. Phys.},
  year = {2002},
  volume = {177},
  pages = {365--393}
}

@ARTICLE{RLi:2001,
  author = {Li, R. and Tang, T. and Zhang, P.},
  title = {{Moving mesh methods in multiple dimensions based on harmonic maps}},
  journal = {J. Comput. Phys.},
  year = {2001},
  volume = {170},
  pages = {562--588}
}

@ARTICLE{X.Li:2005,
  author = {Li, X. and E, W. N.},
  title = {Multiscale modeling for dynamics of solids at finite temperature},
  journal = {J. Mech. Phys. Solids},
  year = {2005},
  volume = {53},
  pages = {1650 - 1685}
}

@ARTICLE{Li:2004f,
  author = {Li, X. -Y. and Fu, K. -X.},
  title = {Continuous medium theory for nonequilibrium solvation: I. How to
	correctly evaluate solvation free energy of nonequilibrium},
  journal = {Journal of Computational Chemistry},
  year = {2004},
  volume = {25},
  pages = {500-509},
  number = {4},
  abstract = {Considering the influences of electrostatic potential upon the change
	of solute charge distribution and upon the change at the same time,
	a more reasonable integral formula of dG = (1/2) V ( + )dV is used
	to calculate the change of the electrostatic free energy in charging
	the solute-solvent system to a nonequilibrium state, instead of the
	one of dG = V dV used before. This modification improves the expressions
	of electrostatic free energy and solvation free energy, in which
	no quantity of the intermediate equilibrium state is explicitly involved.
	Detailed investigation reveals that the solvation free energy of
	nonequilibrium only contains the interaction energy between the field
	due to the solute charge in vacuum, and the dielectric polarization
	at the nonequilibrium state. The solvent reorganization energies
	of forward and backward electron transfer reactions have been redefined
	because the derivations lead to a remarkable feature that these quantities
	are direction-dependent, unlike the theoretical models developed
	before. The deductions are given in the electric field-displacement
	form. Relevant discussions on the reliability of theoretical models
	suggested in this work have also been presented Ã‚Â??004 Wiley
	Periodicals, Inc. J Comput Chem 25: 500-509, 2004},
  annote = {Continuous medium theory for nonequilibrium solvation: I. How to
	correctly evaluate solvation free energy of nonequilibrium},
  bdsk-url-1 = {http://www3.interscience.wiley.com/cgi-bin/abstract/106599639/ABSTRACT},
  date-added = {2008-06-29 13:14:40 -0500},
  date-modified = {2008-06-29 13:14:40 -0500},
  keywords = {Electrostatics; Solvation},
  ty = {JOUR},
  url = {http://www3.interscience.wiley.com/cgi-bin/abstract/106599639/ABSTRACT}
}

@ARTICLE{Li:2009(b),
  author = {Li, Y. and Roy, A. and Zhang, Y.},
  title = {{HAAD: A quick algorithm for accurate prediction of hydrogen atoms
	in protein structures}},
  journal = {PLoS One},
  year = {2009},
  volume = {4},
  pages = {e6701},
  number = {8}
}

@ARTICLE{Li:1996a,
  author = {Li, Y. and Santosa, F.},
  title = {A computational algorithm for minimizing total variation in image
	restoration},
  journal = {IEEE Transactions on Image Processing},
  year = {1996},
  volume = {5},
  pages = {987-95},
  number = {6},
  date-added = {2008-09-16 14:53:34 -0500},
  date-modified = {2008-09-16 14:54:20 -0500}
}

@ARTICLE{Li:2009(a),
  author = {Li, Y. and Zhang, Y.},
  title = {{REMO: A new protocol to refine full atomic protein models from C-alpha
	traces by optimizing hydrogen-bonding networks}},
  journal = {Proteins},
  year = {2009},
  volume = {76},
  pages = {665-676},
  number = {3}
}

@ARTICLE{Li:2001a,
  author = {Zhilin Li AND Sharon R. Lubkin},
  title = {Numerical analysis of interfacial two-dimensional Stokes flow with
	discontinuous viscosity and variable surface tension},
  journal = {International Journal for Numerical Methods in Fluids},
  year = {2001},
  volume = {37},
  pages = {525-540},
  number = {5},
  abstract = {A fluid model of the incompressible Stokes equations in two space
	dimensions is used to simulate the motion of a droplet boundary separating
	two fluids with unequal viscosity and variable surface tension. Our
	theoretical analysis leads to decoupled jump conditions that are
	used in constructing the numerical algorithm. Numerical results agree
	with others in the literature and include some new findings that
	may apply to processes similar to cell cleavage. The method developed
	here accurately preserves area for our test problems. Some interesting
	observations are obtained with different choices of the parameters.
	Copyright Â© 2001 John Wiley & Sons, Ltd.},
  bdsk-url-1 = {http://dx.doi.org/10.1002/fld.185},
  date = {2001 %@ 1097-0363 %+ Center for Research in Scientific Computation
	and Department of Mathematics, North Carolina State University, Raleigh,
	NC, U.S.A.; Biomathematics Program, North Carolina State University,
	Raleigh, NC, U.S.A.},
  date-added = {2008-09-14 15:32:12 -0500},
  date-modified = {2008-09-14 15:32:12 -0500},
  doi = {10.1002/fld.185},
  keywords = {Mathematics; FluidMechanics},
  refer1 = {10.1002/fld.185},
  url = {http://dx.doi.org/10.1002/fld.185}
}

@ARTICLE{Li08345225,
  author = {Li, Z. and Wang, C. Y. and Zhang, X. and Ke, S. H. and Yang, W. T.},
  title = {Transport properties of an armchair carbon nanotube with a double
	vacancy under stretching},
  journal = {Journal of Physics-Condensed Matter},
  year = {2008},
  volume = {20},
  pages = {345225},
  number = {34},
  month = {Aug},
  abstract = {Structural properties of metallic single-walled carbon nanotubes with
	a double vacancy under stretching are studied by using a multiscale
	hybrid energy density method. Based on the optimized structure, the
	single-particle Green function method is then used to investigate
	the transport property. It is found that a reconstruction of the
	structure occurs with an increase of the imposed axial force, which
	alters the transmission function around the Fermi energy and will
	reduce the current. This reconstruction cannot be found by running
	a molecular dynamics simulation without a quantum description.},
  endnotereftype = {Journal Article},
  issn = {0953-8984},
  shorttitle = {Transport properties of an armchair carbon nanotube with a double
	vacancy under stretching},
  url = {<Go to ISI>://000258317600028}
}

@ARTICLE{Li:2003a,
  author = {Zhilin Li and Wei-Cheng Wang and I-Liang Chern and Ming-Chih Lai},
  title = {New Formulations for Interface Problems in Polar Coordinates},
  journal = {SIAM Journal on Scientific Computing},
  year = {2003},
  volume = {25},
  pages = {224-245},
  number = {1},
  abstract = {In this paper, numerical methods are proposed for some interface problems
	in polar or Cartesian coordinates. The new methods are based on a
	formulation that transforms the interface problem with a nonsmooth
	or discontinuous solution into a problem with a smooth solution.
	The new formulation leads to a simple second order finite difference
	scheme for the partial differential equation and a new interpolation
	scheme for the normal derivative of the solution. In conjunction
	with the fast immersed interface method, a fast solver has been developed
	for the interface problems with a piecewise constant but a discontinuous
	coefficient using the new formulation in a polar coordinate system.},
  bdsk-url-1 = {http://link.aip.org/link/?SCE/25/224/1},
  bdsk-url-2 = {http://dx.doi.org/10.1137/S106482750139618X},
  date-added = {2008-09-14 15:32:12 -0500},
  date-modified = {2008-09-14 15:32:12 -0500},
  doi = {10.1137/S106482750139618X},
  keywords = {Mathematics},
  publisher = {SIAM},
  url = {http://link.aip.org/link/?SCE/25/224/1}
}

@ARTICLE{Li:2001,
  author = {Li, Z. L. and Ito, K.},
  title = {Maximum principle preserving schemes for interface problems with
	discontinuous coefficients},
  journal = {SIAM J. Sci. Comput. },
  year = {2001},
  volume = {23},
  pages = {339-361},
  annote = {Maximum principle preserving schemes for interface problems with
	discontinuous coefficients},
  date-added = {2008-09-19 10:28:56 -0500},
  date-modified = {2008-09-19 10:28:56 -0500},
  ty = {JOUR}
}

@ARTICLE{Li:2003,
  author = {Li, Z. L. and Lin, T. and Wu, X. H.},
  title = {New {Cartesian} grid methods for interface problems using the finite
	element formulation},
  journal = {Numerische Mathematik },
  year = {2003},
  volume = {96},
  pages = {61-98},
  annote = {New {Cartesian} grid methods for interface problems using the finite
	element formulation},
  date-added = {2008-09-19 10:28:56 -0500},
  date-modified = {2008-09-19 10:28:56 -0500},
  ty = {JOUR}
}

@ARTICLE{Liang:1997,
  author = {Liang, J. and Subranmaniam, S. },
  title = {Computation of molecular electrostatics with boundary element methods},
  journal = {Biophys. J.},
  year = {1997},
  volume = {73},
  pages = {1830--1841}
}

@ARTICLE{XGLiang:2007,
  author = {Liang, X. G. and Morton, K. J. and Austin, R. H. and Chou, S. Y.
	},
  title = {Single sub-20 nm wide, centimeter-long nanofluidic channel fabricated
	by novel nanoimprint Mold fabrication and direct imprinting },
  journal = { Nano Letters },
  year = {2007},
  volume = {7},
  pages = { 3774-3780 },
  number = { }
}

@ARTICLE{Liao:1992,
  author = {Liao, G. and Anderson, D.},
  title = {{A new approach to grid generation}},
  journal = {Appl. Anal.},
  year = {1992},
  volume = {44},
  pages = {285--298}
}

@ARTICLE{Liao:2000,
  author = {Liao, G. and Liu, F. and Pena, G. C. de la and Peng, D. and Osher,
	S.},
  title = {{Level-set-based deformation methods for adaptive grids}},
  journal = {J. Comput. Phys.},
  year = {2000},
  volume = {159},
  pages = {103--122}
}

@ARTICLE{LiCata,
  author = {LiCata , V.J. and Allewell, N.M. },
  title = {Functionally linked hydration changes in Escherichia coli aspartate
	transcarbamylase and its catalytic subunit},
  journal = {Biochemistry},
  year = {1997},
  volume = {36},
  pages = {10161-10167}
}

@ARTICLE{Licata:1997,
  author = {Licata, V. J. and Allewell, N. M. },
  title = {Functionally Linked Hydration Changes in Escherichia coli Aspartate
	Transcarbamylase and Its Catalytic Subunit},
  journal = {Biochemistry},
  year = {1997},
  volume = {36},
  pages = {10161--10167},
  number = {33},
  abstract = {Abstract: Aspartate transcarbamylase (ATCase) is a highly regulated,
	dodecameric enzyme that catalyzes the first committed step in pyrimidine
	biosynthesis. Upon ligation, ATCase undergoes a conformational transition
	from a low-activity T-state to a high-activity R-state. This transition
	involves major changes in the molecular architecture, including structural
	rearrangements of several intersubunit interfaces and a 12 \r{A}
	expansion of the molecule along its 3-fold axis. Solute-induced osmotic
	stress experiments report that ~208 solvent waters are taken up by
	ATCase as it binds substrate. Solvent-accessible surface area calculations
	conducted on the T and R conformers of ATCase agree very well with
	this result, predicting that ~189 waters are taken up during this
	conformational change. Both osmotic stress measurements and surface
	area calculations on the catalytic trimer of ATCase predict water
	release upon ligation of the trimer. Specific aspects of the application
	of osmotic stress to ATCase are also discussed, including solute
	size effects, and an assessment of potential alternative explanations
	for these results.},
  address = {Department of Biochemistry, University of Minnesota, 1479 Gortner
	Avenue, St. Paul, Minnesota 55108},
  bdsk-url-1 = {http://dx.doi.org/10.1021/bi970669r},
  date-added = {2008-06-30 09:40:02 -0500},
  date-modified = {2008-06-30 09:40:02 -0500},
  doi = {10.1021/bi970669r},
  keywords = {solvation, structure},
  posted-at = {2008-06-30 15:39:24},
  priority = {0},
  url = {http://dx.doi.org/10.1021/bi970669r}
}

@BOOK{Lide:1995,
  title = {CRC Handbook of Chemistry and Physics},
  publisher = {CRC:Boca Raton, FL},
  year = {1995},
  author = {Lide, D. R.},
  volume = {75}
}

@ARTICLE{Lieberman-Aiden:2009,
  author = {Lieberman-Aiden, E. and van Berkum, N.L. and Williams, L. and Imakaev,
	M. and Ragoczy, T. and Telling, A. and Amit, I. and Lajoie, B. R.
	and Sabo, P.J. and Dorschner, M.O. and Sandstrom, R. and Bernstein,
	B. and Bender, M.A. and Groudine, M. and Gnirke, A. and Stamatoyannopoulos,
	J. and Mirny, L.A. and Lander, E.S. and Dekker, J.},
  title = {Comprehensive Mapping of Long-Range Interactions Reveals Folding
	Principles of the Human Genome},
  journal = {SCIENCE },
  year = {2009},
  volume = {326},
  pages = {289-293 },
  number = { }
}

@ARTICLE{Lienhardt1994,
  author = {Lienhardt, Pascal},
  title = {{N-dimensional generalized combinatorial maps and cellular quasi-manifolds}},
  journal = {International Journal on Computational Geometry and Applications},
  year = {1994},
  volume = {4},
  pages = {275--324},
  owner = {doubletony},
  timestamp = {2012.04.26}
}

@ARTICLE{Lienhardt1991,
  author = {Lienhardt, Pascal},
  title = {{Topological models for boundary representation : a comparison with
	n-dimensional generalized maps}},
  journal = {Computer-Aided Design},
  year = {1991},
  volume = {23},
  pages = {59--82},
  number = {1},
  doi = {10.1016/0010-4485(91)90082-8},
  file = {:C\:/Dropbox/Dropbox/Paper/1-s2.0-001044859190100B-main.pdf:pdf},
  issn = {00104485},
  owner = {doubletony},
  publisher = {Elsevier},
  timestamp = {2012.04.26},
  url = {http://linkinghub.elsevier.com/retrieve/pii/0010448591900828}
}

@ARTICLE{Liesen:2004,
  author = {Liesen, J. and Tichy, P.},
  title = {Convergence analysis of {Krylov} subspace methods},
  journal = {CGAMM-Mitteilungen},
  year = {2004},
  volume = {27},
  pages = {153-173}
}

@ARTICLE{Lim:2005,
  author = {Lim, C. W. and Li, Z. R. and Xiang, Y. and Wei, G. W. and Wang, C.
	M.},
  title = {On the missing modes when using the exact frequency relationship
	between {Kirchhoff} and {Mindlin} plates},
  journal = {Advances in Vibration Engineering},
  year = {2005},
  volume = {4},
  pages = {221-48},
  date-added = {2008-06-30 22:00:52 -0400},
  date-modified = {2008-06-30 22:01:36 -0400},
  keywords = {mathematics}
}

@ARTICLE{Lin:2003,
  author = {Lin, J. H. and Perryman, A. L. and Schames, J. R. and McCammon, J.
	A. },
  title = {The relaxed complex method: Accommodating receptor flexibility for
	drug design with an improved scoring scheme.},
  journal = {Biopolymers},
  year = {2003},
  volume = {68},
  pages = {47--62},
  number = {1},
  abstract = {An extension of the new computational methodology for drug design,
	the "relaxed complex" method (J.-H. Lin, A. L. Perryman, J. R. Schames,
	and J. A. McCammon, Journal of the American Chemical Society, 2002,
	vol. 24, pp. 5632-5633), which accommodates receptor flexibility,
	is described. This relaxed complex method recognizes that ligand
	may bind to conformations that occur only rarely in the dynamics
	of the receptor. We have shown that the ligand-enzyme binding modes
	are very sensitive to the enzyme conformations, and our approach
	is capable of finding the best ligand enzyme complexes. Rapid docking
	serves as an efficient initial filtering method to screen a myriad
	of docking modes to a limited set, and it is then followed by more
	accurate scoring with the MM/PBSA (Molecular Mechanics/Poisson Boltzmann
	Surface Area) approach to find the best ligand-receptor complexes.
	The MM/PBSA scorings consistently indicate that the calculated binding
	modes that are most similar to those observed in the x-ray crystallographic
	complexes are the ones with the lowest free energies.},
  address = {Howard Hughes Medical Institute, Department of Chemistry, University
	of California at San Diego, 9500 Gilman Dr. La Jolla, CA 92093-0365,
	USA. jlin@mccammon.ucsd.edu},
  bdsk-url-1 = {http://dx.doi.org/10.1002/bip.10218},
  bdsk-url-2 = {http://dx.doi.org/10.1002/bip.10218},
  date-added = {2008-09-16 15:37:31 -0500},
  date-modified = {2008-09-16 15:37:31 -0500},
  doi = {10.1002/bip.10218},
  issn = {0006-3525},
  keywords = {Electrostatics, Protein-ligandInteractions, Solvation},
  posted-at = {2008-04-16 13:47:44},
  priority = {0},
  url = {http://dx.doi.org/10.1002/bip.10218}
}

@ARTICLE{Lin:2002,
  author = {Lin, Jung-Hsin and Baker, Nathan Andrew and McCammon, J. Andrew},
  title = {Bridging the implicit and explicit solvent approaches for membrane
	electrostatics},
  journal = {Biophysical Journal},
  year = {2002},
  volume = {83},
  pages = {1374-1379},
  number = {3},
  abstract = {Conformations of a zwitterionic bilayer were sampled from a molecular
	dynamics simulation and their electrostatic properties analyzed by
	solution of the Poisson equation. These traditionally implicit electrostatic
	calculations were performed in the presence of varying amounts of
	explicit solvent to assess the magnitude of error introduced by a
	uniform dielectric description of water surrounding the bilayer.
	It was observed that membrane dipole potential calculations in the
	presence of explicit water were significantly different than wholly
	implicit solvent calculations with the calculated dipole potential
	converging to a reasonable value when four or more hydration layers
	were included explicitly.},
  annote = {Bridging the implicit and explicit solvent approaches for membrane
	electrostatics; LinEtal2002; A discussion of the importance of the
	heterogeneity of discrete water surrounding a biomembrane and the
	failure of simple implicit solvent models to correctly reproduce
	the membrane dipole potential.},
  bdsk-file-1 = {YnBsaXN0MDDUAQIDBAUGCQpYJHZlcnNpb25UJHRvcFkkYXJjaGl2ZXJYJG9iamVjdHMSAAGGoNE
	HCFRyb290gAFfEA9OU0tleWVkQXJjaGl2ZXKoCwwXGBkdJCVVJG51bGzTDQ4PEBEUViRjbGFzc1
	dOUy5rZXlzWk5TLm9iamVjdHOAB6ISE4ACgAOiFRaABIAGWWFsaWFzRGF0YVxyZWxhdGl2ZVBhd
	GjSDRobHFdOUy5kYXRhgAVPEQHSAAAAAAHSAAIAAAxNYWNpbnRvc2ggSEQAAAAAAAAAAAAAAAAA
	AADD4v5NSCsAAAAZYksZMjAwMi1MaW5CYWtlck1jQ2FtbW9uLnBkZgAAAAAAAAAAAAAAAAAAAAA
	AAAAAAAAAAAAAAAAAAAAAAAAAAAAAABliWsM6C1RQREYgcHJ2dwAEAAQAAAkgAAAAAAAAAAAAAA
	AAAAAAB0FyY2hpdmUAABAACAAAw+NSrQAAABEACAAAwzpRpAAAAAEAFAAZYksAGWIDAAqkKAAKp
	BEAAHrcAAIAT01hY2ludG9zaCBIRDpVc2VyczpiYWtlcjpEb2N1bWVudHM6UmVmZXJlbmNlczpB
	cmNoaXZlOjIwMDItTGluQmFrZXJNY0NhbW1vbi5wZGYAAA4ANAAZADIAMAAwADIALQBMAGkAbgB
	CAGEAawBlAHIATQBjAEMAYQBtAG0AbwBuAC4AcABkAGYADwAaAAwATQBhAGMAaQBuAHQAbwBzAG
	gAIABIAEQAEgBCVXNlcnMvYmFrZXIvRG9jdW1lbnRzL1JlZmVyZW5jZXMvQXJjaGl2ZS8yMDAyL
	UxpbkJha2VyTWNDYW1tb24ucGRmABMAAS8AABUAAgAM//8AANIeHyAhWCRjbGFzc2VzWiRjbGFz
	c25hbWWjISIjXU5TTXV0YWJsZURhdGFWTlNEYXRhWE5TT2JqZWN0XxBCLi4vLi4vLi4vLi4vRG9
	jdW1lbnRzL1JlZmVyZW5jZXMvQXJjaGl2ZS8yMDAyLUxpbkJha2VyTWNDYW1tb24ucGRm0h4fJi
	eiJyNcTlNEaWN0aW9uYXJ5AAgAEQAaAB8AKQAyADcAOgA/AEEAUwBcAGIAaQBwAHgAgwCFAIgAi
	gCMAI8AkQCTAJ0AqgCvALcAuQKPApQCnQKoAqwCugLBAsoDDwMUAxcAAAAAAAACAQAAAAAAAAAo
	AAAAAAAAAAAAAAAAAAADJA==},
  bdsk-url-1 = {http://www.biophysj.org/cgi/content/abstract/83/3/1374},
  date-added = {2008-09-17 09:22:40 -0500},
  date-modified = {2008-09-17 09:22:40 -0500},
  keywords = {Biomembranes; Solvation; Electrostatics},
  ty = {JOUR},
  url = {http://www.biophysj.org/cgi/content/abstract/83/3/1374}
}

@ARTICLE{Lin:2009,
  author = { Lin, L. and Wang, Y. and Zhou, H.},
  title = {An alternative approach to empirical mode decomposition},
  journal = {IEEE Trans. Signal Processing},
  year = {submitted, 2009}
}

@ARTICLE{LLin:2009,
  author = {Lin, L. and Wang, Y. and Zhou, H.},
  title = {{Iterative filtering as an alternative algorithm for empirical mode
	decomposition}},
  journal = {Advances in Adaptive Data Analysis},
  year = {2009},
  volume = {1},
  pages = {543--560},
  number = {4}
}

@ARTICLE{LWZ09,
  author = {Lin, L. and Wang, Y. and Zhou, H.},
  title = { Iterative filtering as an alternative algorithm for empirical mode
	decomposition},
  journal = {Advances in Adaptive Data Analysis},
  year = {2009},
  volume = {1},
  pages = {543--560},
  number = { }
}

@ARTICLE{LiWaZh09,
  author = {Lin, L. and Wang, Y. and Zhou, H. M.},
  title = {Iterative Filters As An Alternative Algorithm for Empirical Mode
	Decomposition},
  journal = {Advances in Adaptive Data Analysis (AADA)},
  year = {2009},
  volume = {1}
}

@ARTICLE{Lin062981,
  author = {Lin, P. and Yang, W. T. and Pedersen, L. C. and Negishi, M. and Pedersen,
	L. G.},
  title = {Searching for the minimum energy path in the sulfuryl transfer reaction
	catalyzed by human estrogen sulfotransferase: Role of enzyme dynamics},
  journal = {International Journal of Quantum Chemistry},
  year = {2006},
  volume = {106},
  pages = {2981-2998},
  number = {14},
  month = {Nov},
  abstract = {The enzymatic transfer of a sulfuryl group from the ubiquitous biological
	source of sulfate X-phosphoadenosine 5'-phosphosulfate (PAPS) to
	estrogen is investigated by the pseudo-bond quantum mechanical/molecular
	mechanical method (QM/MM) method. Calculations of the reaction path
	are performed starting with models based on two crystal structures,
	which differ in information about the cofactor and substrates. In
	addition, a subsequent relaxation of the enzyme was performed with
	the found transition state frozen, followed by redetermination of
	the path. An activation barrier of 22 kcal/mol is estimated. The
	reaction mechanism features a proton transfer from the estrogen to
	a catalytic histidine followed by the rate determining SO, transfer.
	The mechanism found is largely dissociative. (C) 2006 Wiley Periodicals,
	Inc.},
  endnotereftype = {Journal Article},
  issn = {0020-7608},
  shorttitle = {Searching for the minimum energy path in the sulfuryl transfer reaction
	catalyzed by human estrogen sulfotransferase: Role of enzyme dynamics},
  url = {<Go to ISI>://000241276800019}
}

@ARTICLE{Linnick:2005,
  author = {Linnick, Mark N. and Fasel, Hermann F.},
  title = {A high-order immersed interface method for simulating unsteady incompressible
	flows on irregular domains},
  journal = {J. Comput. Phys.},
  year = {2005},
  volume = {204},
  pages = {157--192},
  number = {1},
  abstract = { Immersed boundary methods and immersed interface methods are becoming
	increasingly popular for the computation of unsteady flows around
	complex geometries using a Cartesian grid. While good results, both
	qualitative and quantitative, have been obtained, most of the methods
	rely on low-order corrections to account for the immersed boundary.
	The objective of the present work is to present, as an alternative,
	a high-order modified immersed interface method for the 2D, unsteady,
	incompressible Navier-Stokes equations in stream function-vorticity
	formulation. The method employs an explicit fourth-order Runge-Kutta
	time integration scheme, fourth-order compact finite-differences
	for computation of spatial derivatives, and a nine-point, fourth-order
	compact discretization of the Poisson equation for computation of
	the stream function. Corrections to the finite difference schemes
	are used to maintain high formal accuracy at the immersed boundary,
	as confirmed by analytical tests. To validate the method in its application
	to incompressible flows, several physically relevant test cases are
	computed, including uniform flow past a circular cylinder and Tollmien-Schlichting
	waves in a boundary layer.},
  bdsk-url-1 = {http://www.sciencedirect.com/science/article/B6WHY-4DS6T02-4/2/dac26eb90a07caf629d9adaf57093f36},
  date-added = {2008-09-14 15:32:12 -0500},
  date-modified = {2008-09-14 15:32:12 -0500},
  doi = {10.1016/j.jcp.2004.09.017 },
  keywords = {Mathematics; FluidMechanics},
  ty = {JOUR},
  url = {http://www.sciencedirect.com/science/article/B6WHY-4DS6T02-4/2/dac26eb90a07caf629d9adaf57093f36}
}

@ARTICLE{Little9953,
  author = {Little, S. B. and Rabinowitz, J. R. and Wei, P. and Yang, W. T.},
  title = {A comparison of calculated and experimental geometries for crowded
	polycyclic aromatic hydrocarbons and their metabolites},
  journal = {Polycyclic Aromatic Compounds},
  year = {1999},
  volume = {14},
  pages = {53-61},
  abstract = {It has become useful to consider the subclass of PAHs with a crowded
	bay region because of similar biological activity within the subclass.
	Crowding in the bay region of a polycyclic aromatic hydrocarbon results
	in a twisted molecular geometry. The purpose of this study is to
	help gauge the utility of various computational methods for determining
	the molecular geometry of molecules in this subclass and their metabolites.
	The results from serm-empirical methods AM1 and PM3, ab initio Hartree-Fock
	methods and density functional methods will be compared to experimentally
	determined geometries for crowded PAHs. It will be seen that excellent
	geometries for all local minimum energy structures are obtained from
	semi-empirical methods. More exact and computationally extensive
	methods yield equivalent or somewhat better results only with good
	basis sets. However, methods disagree on the relative energies of
	the isomers of diol-epoxides.},
  endnotereftype = {Journal Article},
  issn = {1040-6638},
  shorttitle = {A comparison of calculated and experimental geometries for crowded
	polycyclic aromatic hydrocarbons and their metabolites},
  url = {<Go to ISI>://000086076000007}
}

@ARTICLE{Liu:1998,
  author = {Liu, F. and Ji, S. and Liao, G.},
  title = {{An adaptive grid method and its application to steady Euler flow
	calculations}},
  journal = {SIAM J.Sci.Comput.},
  year = {1998},
  volume = {20},
  pages = {811--825}
}

@ARTICLE{Liu01484,
  author = {Liu, H. Y. and Elstner, M. and Kaxiras, E. and Frauenheim, T. and
	Hermans, J. and Yang, W. T.},
  title = {Quantum mechanics simulation of protein dynamics on long timescale},
  journal = {Proteins-Structure Function and Genetics},
  year = {2001},
  volume = {44},
  pages = {484-489},
  number = {4},
  month = {Sep},
  abstract = {Protein structure and dynamics are the keys to a wide range of problems
	in biology. In principle, both can be fully understood by using quantum
	mechanics as the ultimate tool to unveil the molecular interactions
	involved. Indeed, quantum mechanics of atoms and molecules have come
	to play a central role in chemistry and physics. In practice, however,
	direct application of quantum mechanics to protein systems has been
	prohibited by the large molecular size of proteins. As a consequence,
	there is no general quantum mechanical treatment that not only exceeds
	the accuracy of state-of-the-art empirical models for proteins but
	also maintains the efficiency needed for extensive sampling in the
	conformational space, a requirement mandated by the complexity of
	protein systems. Here we show that, given recent developments in
	methods, a general quantum mechanical-based treatment can be constructed.
	We report a molecular dynamics simulation of a protein, crambin,
	in solution for 350 ps in which we combine a semiempirical quantum-mechanical
	description of the entire protein with a description of the surrounding
	solvent, and solvent-protein interactions based on a molecular mechanics
	force field. Comparison with a recent very high-resolution crystal
	structure of crambin (Jelsch et al., Proc Natl Acad Sci USA 2000;102:2246-2251)
	shows that geometrical detail is better reproduced in this simulation
	than when several alternate molecular mechanics force fields are
	used to describe the entire system of protein and solvent, even though
	the structure is no less flexible. Individual atomic charges deviate
	in both directions from "canonical" values, and some charge transfer
	is found between the N and C-termini. The capability of simulating
	protein dynamics on and beyond the few hundred ps timescale with
	a demonstrably accurate quantum mechanical model will bring new opportunities
	to extend our understanding of a range of basic processes in biology
	such as molecular recognition and enzyme catalysis. Proteins 2001;44:484-489.
	(C) 2001 Wiley-Liss, Inc.},
  endnotereftype = {Journal Article},
  issn = {0887-3585},
  shorttitle = {Quantum mechanics simulation of protein dynamics on long timescale},
  url = {<Go to ISI>://000170477600010}
}

@ARTICLE{Liu:2001,
  author = {Liu, H. Y. and Elstner, M. and Kaxiras, E. and Frauenheim, T. and
	Hermans, J. and Yang, W. T.},
  title = {Quantum mechanics simulation of protein dynamics on long timescale},
  journal = {Proteins-Structure Function and Genetics},
  year = {2001},
  volume = {44},
  pages = {484-489},
  annote = {Quantum mechanics simulation of protein dynamics on long timescale},
  date-added = {2008-09-19 10:28:56 -0500},
  date-modified = {2008-09-19 10:28:56 -0500},
  ty = {JOUR}
}

@ARTICLE{Liu04697,
  author = {Liu, H. Y. and Lu, Z. Y. and Cisneros, G. A. and Yang, W. T.},
  title = {Parallel iterative reaction path optimization in ab initio quantum
	mechanical/molecular mechanical modeling of enzyme reactions},
  journal = {Journal of Chemical Physics},
  year = {2004},
  volume = {121},
  pages = {697-706},
  number = {2},
  month = {Jul},
  abstract = {The determination of reaction paths for enzyme systems remains a great
	challenge for current computational methods. In this paper we present
	an efficient method for the determination of minimum energy reaction
	paths with the ab initio quantum mechanical/molecular mechanical
	approach. Our method is based on an adaptation of the path optimization
	procedure by Ayala and Schlegel for small molecules in gas phase,
	the iterative quantum mechanical/molecular mechanical (QM/MM) optimization
	method developed earlier in our laboratory and the introduction of
	a new metric defining the distance between different structures in
	the configuration space. In this method we represent the reaction
	path by a discrete set of structures. For each structure we partition
	the atoms into a core set that usually includes the QM subsystem
	and an environment set that usually includes the MM subsystem. These
	two sets are optimized iteratively: the core set is optimized to
	approximate the reaction path while the environment set is optimized
	to the corresponding energy minimum. In the optimization of the core
	set of atoms for the reaction path, we introduce a new metric to
	define the distances between the points on the reaction path, which
	excludes the soft degrees of freedom from the environment set and
	includes extra weights on coordinates describing chemical changes.
	Because the reaction path is represented by discrete structures and
	the optimization for each can be performed individually with very
	limited coupling, our method can be executed in a natural and efficient
	parallelization, with each processor handling one of the structures.
	We demonstrate the applicability and efficiency of our method by
	testing it on two systems previously studied by our group, triosephosphate
	isomerase and 4-oxalocrotonate tautomerase. In both cases the minimum
	energy paths for both enzymes agree with the previously reported
	paths. (C) 2004 American Institute of Physics.},
  endnotereftype = {Journal Article},
  issn = {0021-9606},
  shorttitle = {Parallel iterative reaction path optimization in ab initio quantum
	mechanical/molecular mechanical modeling of enzyme reactions},
  url = {<Go to ISI>://000222265600011}
}

@ARTICLE{Liu006560,
  author = {Liu, H. Y. and Zhang, Y. K. and Yang, W. T.},
  title = {How is the active site of enolase organized to catalyze two different
	reaction steps?},
  journal = {Journal of the American Chemical Society},
  year = {2000},
  volume = {122},
  pages = {6560-6570},
  number = {28},
  month = {Jul},
  abstract = {Using a combined ab initio quantum mechanical/molecular mechanical
	approach developed in our laboratory, we obtained the reaction paths
	and free energy barriers for the two steps of the reaction catalyzed
	by enolase. In the first step, the alpha-proton of the substrate,
	2-phospho-D-glycerate (PGA), is removed by Lys345, resulting in an
	enolic intermediate. In the second step, the beta-hydroxyl group
	leaves the enolic intermediate with the assistance of a general acid,
	Glu211. The calculated free energies of activation are 13.1 and 9.4
	kcaI mol(-1) for the first and the second step, respectively. The
	barrier heights are consistent with the reaction rates measured from
	experiments. The calculations indicate that the electrostatic interactions
	between the substrate and two divalent metal cations at the active
	site strongly favor the first step. However, the same metal cations
	strongly disfavor the second step because the change in charge of
	the substrate is of an opposite sign compared with that in the first
	step. We conclude that the enzyme environment (excluding Lys345,
	Glu211, and the metal cations) forms an essential part of the reaction
	mechanism. It counterbalances the disfavoring effects of the metal
	cations in the second step without interfering with the first step
	despite the reversed charge changes of the substrate in the two steps.
	This capability of the enzyme originates from the three-dimensional
	organization of polar and charged groups in the active site of enolase,
	as indicated by correlations between the three-dimensional structure
	and energetic analyses based on our calculations. To achieve overall
	catalytic efficiency, the structure of the enolase active site takes
	advantage of the fact that the charge reorganization procedures accompanying
	the two reaction steps take place in two different directions in
	space.},
  endnotereftype = {Journal Article},
  issn = {0002-7863},
  shorttitle = {How is the active site of enolase organized to catalyze two different
	reaction steps?},
  url = {<Go to ISI>://000088320700004}
}

@ARTICLE{JGLiu:2000,
  author = {Liu, J. G. and Shu, C. W.},
  title = {A high-order discontinuous Galerkin method for {2D} incompressible
	flows },
  journal = {Journal of Comput. Phys.},
  year = {2000},
  volume = {160},
  pages = {577 - 596}
}

@ARTICLE{Liu066274,
  author = {Liu, R. and Ke, S. H. and Baranger, H. U. and Yang, W. T.},
  title = {Negative differential resistance and hysteresis through an organometallic
	molecule from molecular-level crossing},
  journal = {Journal of the American Chemical Society},
  year = {2006},
  volume = {128},
  pages = {6274-6275},
  number = {19},
  month = {May},
  endnotereftype = {Journal Article},
  issn = {0002-7863},
  shorttitle = {Negative differential resistance and hysteresis through an organometallic
	molecule from molecular-level crossing},
  url = {<Go to ISI>://000237590400003}
}

@ARTICLE{Liu051959,
  author = {Liu, R. and Ke, S. H. and Baranger, H. U. and Yang, W. T.},
  title = {Organometallic spintronics: Dicobaltocene switch},
  journal = {Nano Letters},
  year = {2005},
  volume = {5},
  pages = {1959-1962},
  number = {10},
  month = {Oct},
  abstract = {A single-molecule spintronic switch and spin valve using two cobaltocene
	moieties is proposed. Spin-dependent transport through a lead-molecule-lead
	junction has been calculated using first-principles density functional
	and nonequilibrium Green function methods. We find that the antiparallel
	(singlet) configuration of the cobaltocene spins blocks electron
	transport near the Fermi energy, while the spin parallel (triplet)
	configuration enables much higher current. The energy difference
	between the antiparallel and parallel states depends on the insulating
	spacer separating the two cobaltocenes, allowing switching through
	the application of a moderate magnetic field.},
  endnotereftype = {Journal Article},
  issn = {1530-6984},
  shorttitle = {Organometallic spintronics: Dicobaltocene switch},
  url = {<Go to ISI>://000232623700019}
}

@ARTICLE{Liu0544703,
  author = {Liu, R. and Ke, S. H. and Baranger, H. U. and Yang, W. T.},
  title = {Intermolecular effect in molecular electronics},
  journal = {Journal of Chemical Physics},
  year = {2005},
  volume = {122},
  pages = {44703},
  number = {4},
  month = {Jan},
  abstract = {We investigate the effects of lateral interactions on the conductance
	of two molecules connected in parallel to semi-infinite leads. The
	method we use combines a Green function approach to quantum transport
	with density functional theory for the electronic properties. The
	system, modeled after a self-assembled monolayer, consists of benzylmercaptane
	molecules sandwiched between gold electrodes. We find that the conductance
	increases when intermolecular interaction comes into play. The source
	of this increase is the indirect interaction through the gold substrate
	rather than direct molecule-molecule interaction. A striking resonance
	is produced only 0.3 eV above the Fermi energy. (C) 2005 American
	Institute of Physics.},
  endnotereftype = {Journal Article},
  issn = {0021-9606},
  shorttitle = {Intermolecular effect in molecular electronics},
  url = {<Go to ISI>://000226807000054}
}

@ARTICLE{Liu07141104,
  author = {Liu, R. and Ke, S. H. and Yang, W. and Baranger, H. U.},
  title = {Cobaltocene as a spin filter},
  journal = {Journal of Chemical Physics},
  year = {2007},
  volume = {127},
  pages = {141104},
  number = {14},
  month = {Oct},
  abstract = {In the context of investigating organic molecules for molecular electronics,
	doping molecular wires with transition metal atoms provides additional
	means of controlling their transport behavior. The incorporation
	of transition metal atoms may generate spin dependence because the
	conduction channels of only one spin component align with the chemical
	potential of the leads, resulting in a spin polarized electric current.
	The possibility to create such a spin polarized current is investigated
	here with the organometallic moiety cobaltocene. According to our
	calculations, cobaltocene contacted with gold electrodes acts as
	a robust spin filter: Applying a voltage less than 0.2 V causes the
	current of one spin component crossing the molecular bridge to be
	two orders of magnitude larger than the other. We address the key
	issue of sensitivity to molecule-lead geometry by showing that a
	weak barrier generated by CH2 groups between the cobaltocene and
	the leads is crucial in reducing the sensitivity to the contact geometry
	while only reducing the current modestly. These results suggest cobaltocene
	as a robust basic building block for molecular spintronics. (c) 2007
	American Institute of Physics.},
  endnotereftype = {Journal Article},
  issn = {0021-9606},
  shorttitle = {Cobaltocene as a spin filter},
  url = {<Go to ISI>://000250140800004}
}

@ARTICLE{Liu0624718,
  author = {Liu, R. and Ke, S. H. and Yang, W. T. and Baranger, H. U.},
  title = {Organometallic molecular rectification},
  journal = {Journal of Chemical Physics},
  year = {2006},
  volume = {124},
  pages = {24718},
  number = {2},
  month = {Jan},
  abstract = {We study the rectification of current through a single molecule with
	an intrinsic spatial asymmetry. The molecule contains a cobaltocene
	moiety in order to take advantage of its relatively localized and
	high-energy d states. A rectifier with large voltage range, high
	current, and low threshold can be realized. The evolution of molecular
	orbitals under both forward and reverse biases is captured in a self-consistent
	nonequilibrium Green function plus density functional theory description.
	Our calculations demonstrate the plausibility of making excellent
	molecular diodes by using metallocenes, pointing to a fruitful class
	of molecules. (c) 2006 American Institute of Physics.},
  endnotereftype = {Journal Article},
  issn = {0021-9606},
  shorttitle = {Organometallic molecular rectification},
  url = {<Go to ISI>://000234607700078}
}

@ARTICLE{Liu001634,
  author = {Liu, S. B. and Perez-Jorda, J. M. and Yang, W. T.},
  title = {Nonorthogonal localized molecular orbitals in electronic structure
	theory},
  journal = {Journal of Chemical Physics},
  year = {2000},
  volume = {112},
  pages = {1634-1644},
  number = {4},
  month = {Jan},
  abstract = {The concept of nonorthogonal localized molecular orbital (NOLMO) is
	investigated in this paper. Given a set of the commonly used canonical
	molecular orbitals, a direct minimization algorithm is proposed to
	obtain both the orthogonal localized molecular orbitals (OLMO) and
	NOLMO by using the Boys criterion and conjugate gradient minimization.
	To avoid the multiple-minimum problem, the absolute energy minimization
	principle of Yang is employed to obtain initial guesses. Contrary
	to the early conclusion drawn by Lipscomb and co-workers who claimed
	that OLMOs and the corresponding NOLMOs are more or less the same,
	we found that NOLMOs are about 10%-30% more localized than OLMOs.
	More importantly, the so-called "delocalization tail" that plagues
	OLMOs is not present in NOLMOs, showing that NOLMOs are more compact
	and less oscillatory and capable of providing greater transferability
	in describing the electronic structure of molecules. We also found
	that main lobes of NOLMOs are slightly larger in size than those
	of OLMOs because of the normalization requirement. These features
	establish NOLMOs to be valuable as building blocks in electronic
	structure theory and for the understanding of chemical bonding. They
	show the promise for the utilization of NOLMOs-the most localized
	possible-in the linear scaling approaches of the electronic structure
	theory for molecules and solids. (C) 2000 American Institute of Physics.
	[S0021-9606(00)30204-5].},
  endnotereftype = {Journal Article},
  issn = {0021-9606},
  shorttitle = {Nonorthogonal localized molecular orbitals in electronic structure
	theory},
  url = {<Go to ISI>://000084776000002}
}

@ARTICLE{Liu:2006,
  author = {Liu, W. K. and Liu, Y. and Farrell, D. and Zhang, L. and Wang, X.
	and Fukui, Y. and Patankar, N. and Zhang, Y. and Bajaj, C. and Chen,
	X. and Hsu, H.},
  title = {Immersed finite element method and its applications to biological
	systems},
  journal = {Computer Methods in Applied Mechanics and Engineering },
  year = {2006},
  volume = {195},
  pages = {1722-1749},
  annote = {Immersed finite element method and its applications to biological
	systemsn},
  date-added = {2008-09-19 10:28:56 -0500},
  date-modified = {2008-09-19 10:28:56 -0500},
  ty = {JOUR}
}

@ARTICLE{LiuWS:2005,
  author = { Liu, W. S. },
  title = {Geometric singular perturbation approach to steady-state {Poisson-Nernst-Planck}
	systems},
  journal = {SIAM J. Appl. Math.},
  year = {2005},
  volume = {65},
  pages = {754-766 },
  number = {3 }
}

@ARTICLE{WENO,
  author = {X.D. Liu and S. Osher and T. Chan},
  title = {{Weighted Essentially Non-oscillatory Schemes}},
  journal = {J. Sci. Comput.},
  year = {1996},
  volume = {126},
  pages = {202--212}
}

@ARTICLE{Liu:2000,
  author = {Liu, X. D. and Fedkiw, R. P. and Kang, M.},
  title = {A boundary condition capturing method for {Poisson}'s equation on
	irregular domains},
  journal = {J. Comput. Phys.},
  year = {2000},
  volume = {160},
  pages = {151-178},
  date-added = {2008-09-19 10:28:56 -0500},
  date-modified = {2008-09-19 10:28:56 -0500},
  ty = {JOUR}
}

@ARTICLE{LiuTad,
  author = {Liu, X. -D. and Tadmor, E.},
  title = {Third order non-oscillatory central scheme for hyperbolic conservation
	laws},
  journal = {Numer. Math.},
  year = {1998},
  volume = {79},
  pages = {397-425}
}

@ARTICLE{Liu2005,
  author = {Liu, Yuanxin and Snoeyink, Jack},
  title = {{A Comparison of Five Implementations of 3D Delaunay Tessellation}},
  journal = {Combinatorial and Computational Geometry},
  year = {2005},
  volume = {52},
  pages = {435--453},
  file = {:C\:/Dropbox/Dropbox/Paper/23liu.pdf:pdf},
  owner = {doubletony},
  timestamp = {2012.04.26},
  url = {http://books.google.com/books?hl=en&amp;lr=&amp;id=iibCrkwJ2ysC&amp;oi=fnd&amp;pg=PA439&amp;dq=A+Comparison+of+Five+Implementations+of+3D+Delaunay+Tessellation&amp;ots=G8uiTW2iw0&amp;sig=0MlhLJxPpS6L_s-UuJV3cuhZMlc}
}

@ARTICLE{Livesay:2003,
  author = {Livesay, D. R. and Jambeck, P. and Rojnuckarin, A. and Subramaniam,
	S.},
  title = {Conservation of Electrostatic Properties within Enzyme Families and
	Superfamilies},
  journal = {Biochemistry},
  year = {2003},
  volume = {42},
  pages = {3464-3473},
  number = {12},
  abstract = {Electrostatic interactions play a key role in enzyme catalytic function.
	At long range, electrostatics steer the incoming ligand/substrate
	to the active site, and at short distances, electrostatics provide
	the specific local interactions for catalysis. In cases in which
	electrostatics determine enzyme function, orthologs should share
	the electrostatic properties to maintain function. Often, electrostatic
	potential maps are employed to depict how conserved surface electrostatics
	preserve function. We expand on previous efforts to explain conservation
	of function, using novel electrostatic sequence and structure analyses
	of four enzyme families and one enzyme superfamily. We show that
	the spatial charge distribution is conserved within each family and
	superfamily. Conversely, phylogenetic analysis of key electrostatic
	residues provide the evolutionary origins of functionality.},
  address = {Department of Chemistry, University of Illinois, Urbana, Illinois
	61820, USA, Departments of Bioengineering and Chemistry and Biochemistry,
	University of California at San Diego, San Diego, California 92093-0412,
	USA, and Department of Chemical Engineering, University of Wisconsin,
	Madison, Wisconsin 53706, USA.},
  annote = {Apr 1; Conservation of Electrostatic Properties within Enzyme Families
	and Superfamilies; 12653550; 0006-2960 Journal article},
  bdsk-file-1 = {YnBsaXN0MDDUAQIDBAUGCQpYJHZlcnNpb25UJHRvcFkkYXJjaGl2ZXJYJG9iamVjdHMSAAGGoNE
	HCFRyb290gAFfEA9OU0tleWVkQXJjaGl2ZXKoCwwXGBkdJCVVJG51bGzTDQ4PEBEUViRjbGFzc1
	dOUy5rZXlzWk5TLm9iamVjdHOAB6ISE4ACgAOiFRaABIAGWWFsaWFzRGF0YVxyZWxhdGl2ZVBhd
	GjSDRobHFdOUy5kYXRhgAVPEQIUAAAAAAIUAAIAAAxNYWNpbnRvc2ggSEQAAAAAAAAAAAAAAAAA
	AADD4v5NSCsAAAAZYksfMjAwMy1MaXZlc2F5SmFtYmVja1IjMTk2Mjc4LnBkZgAAAAAAAAAAAAA
	AAAAAAAAAAAAAAAAAAAAAAAAAAAAAABlieL8eZZUAAAAAAAAAAAAEAAQAAAkgAAAAAAAAAAAAAA
	AAAAAAB0FyY2hpdmUAABAACAAAw+NSrQAAABEACAAAvx6r5QAAAAEAFAAZYksAGWIDAAqkKAAKp
	BEAAHrcAAIAVU1hY2ludG9zaCBIRDpVc2VyczpiYWtlcjpEb2N1bWVudHM6UmVmZXJlbmNlczpB
	cmNoaXZlOjIwMDMtTGl2ZXNheUphbWJlY2tSIzE5NjI3OC5wZGYAAA4AXAAtADIAMAAwADMALQB
	MAGkAdgBlAHMAYQB5AEoAYQBtAGIAZQBjAGsAUgBvAGoAbgB1AGMAawBhAHIAaQBuAFMAdQBiAH
	IAYQBtAGEAbgBpAGEAbQAuAHAAZABmAA8AGgAMAE0AYQBjAGkAbgB0AG8AcwBoACAASABEABIAV
	lVzZXJzL2Jha2VyL0RvY3VtZW50cy9SZWZlcmVuY2VzL0FyY2hpdmUvMjAwMy1MaXZlc2F5SmFt
	YmVja1Jvam51Y2thcmluU3VicmFtYW5pYW0ucGRmABMAAS8AABUAAgAM//8AANIeHyAhWCRjbGF
	zc2VzWiRjbGFzc25hbWWjISIjXU5TTXV0YWJsZURhdGFWTlNEYXRhWE5TT2JqZWN0XxBWLi4vLi
	4vLi4vLi4vRG9jdW1lbnRzL1JlZmVyZW5jZXMvQXJjaGl2ZS8yMDAzLUxpdmVzYXlKYW1iZWNrU
	m9qbnVja2FyaW5TdWJyYW1hbmlhbS5wZGbSHh8mJ6InI1xOU0RpY3Rpb25hcnkACAARABoAHwAp
	ADIANwA6AD8AQQBTAFwAYgBpAHAAeACDAIUAiACKAIwAjwCRAJMAnQCqAK8AtwC5AtEC1gLfAuo
	C7gL8AwMDDANlA2oDbQAAAAAAAAIBAAAAAAAAACgAAAAAAAAAAAAAAAAAAAN6},
  bdsk-url-1 = {http://dx.doi.org/10.1021/bi026918f},
  date-added = {2008-09-15 10:05:07 -0500},
  date-modified = {2008-09-15 10:05:07 -0500},
  keywords = {Electrostatics; Bioinformatics},
  ty = {JOUR},
  url = {http://dx.doi.org/10.1021/bi026918f}
}

@ARTICLE{Livingstone:1991,
  author = {Livingstone, J. R. and Spolar, R. S. and Record Jr, M. T.},
  title = {Contribution to the thermodynamics of protein folding from the reduction
	in water-accessible nonpolar surface area},
  journal = {Biochemistry},
  year = {1991},
  volume = {30},
  pages = {4237-44},
  number = {17},
  abstract = {Protein folding and the transfer of hydrocarbons from a dilute aqueous
	solution to the pure liquid phase are thermodynamically similar in
	that both processes remove nonpolar surface from water and both are
	accompanied by anomalously large negative heat capacity changes.
	On the basis of a limited set of published surface areas, we previously
	proposed that heat capacity changes (delta C degrees p) for the transfer
	of hydrocarbons from water to the pure liquid phase and for the folding
	of globular proteins exhibit the same proportionality to the reduction
	in water-accessible nonpolar surface area (delta Anp) {$[$}Spolar,
	R.S., Ha, J.H., \& Record, M.T., Jr. (1989) Proc. Natl. Acad. Sci.
	U.S.A. 86, 8382-8385{$]$}. The consequence of this proposal is that
	the experimental delta C degrees p for protein folding can be used
	to obtain estimates of delta Anp and of the contribution to the stability
	of the folded state from removal of a nonpolar surface from water.
	In this paper, a rigorous molecular surface area algorithm {$[$}Richmond,
	T.J. (1984) J. Mol. Biol. 178, 63-89{$]$} is applied to obtain self-consistent
	values of the water-accessible nonpolar surface areas of the native
	and completely denatured states of the entire set of globular proteins
	for which both crystal structures and delta C degrees p of folding
	have been determined and for the set of liquid and liquefiable hydrocarbons
	for which delta C degrees p of transfer are known. Both processes
	(hydrocarbon transfer and protein folding) exhibit the same direct
	proportionality between delta C degrees p and delta Anp. We conclude
	that the large negative heat capacity changes observed in protein
	folding and other self-assembly processes involving proteins provide
	a quantitative measure of the reduction in the water-accessible nonpolar
	surface area and of the contribution of the hydrophobic effect to
	the stability of the native state and to protein assembly.},
  annote = {Contribution to the thermodynamics of protein folding from the reduction
	in water-accessible nonpolar surface area},
  bdsk-url-1 = {http://pubs.acs.org/cgi-bin/sample.cgi/bichaw/1991/30/i17/pdf/bi00231a019.pdf},
  date-added = {2008-06-30 06:52:53 -0500},
  date-modified = {2008-06-30 06:52:53 -0500},
  keywords = {Solvation; Protein_folding},
  ty = {JOUR},
  url = {http://pubs.acs.org/cgi-bin/sample.cgi/bichaw/1991/30/i17/pdf/bi00231a019.pdf}
}

@ARTICLE{Liwo:1999,
  author = {Liwo, A. and Lee, J. and Ripoll, D.R. and Pillardy, J. and Scheraga,
	H.A.},
  title = {{Protein structure prediction by global optimization of a potential
	energy function}},
  journal = {Proc Natl Acad Sci USA},
  year = {1999},
  volume = {96},
  pages = {5482-5485},
  number = {10}
}

@ARTICLE{Lombard:2003,
  author = {Bruno Lombard and Jo\"{e}l Piraux},
  title = {How to Incorporate the Spring-Mass Conditions in Finite-Difference
	Schemes},
  journal = {SIAM Journal on Scientific Computing},
  year = {2003},
  volume = {24},
  pages = {1379-1407},
  number = {4},
  abstract = {The spring-mass conditions are an efficient way to model imperfect
	contacts between elastic media. These conditions link together the
	limit values of the elastic stress and of the elastic displacement
	on both sides of interfaces. To insert these spring-mass conditions
	in classical finite-difference schemes, we use an interface method,
	the explicit simplified interface method (ESIM). This insertion is
	automatic for a wide class of schemes. The interfaces do not need
	to coincide with the uniform Cartesian grid. The local truncation
	error analysis and numerical experiments show that the ESIM maintains,
	with interfaces, properties of the schemes in homogeneous medium.},
  bdsk-url-1 = {http://link.aip.org/link/?SCE/24/1379/1},
  bdsk-url-2 = {http://dx.doi.org/10.1137/S1064827501385931},
  date-added = {2008-09-14 15:32:12 -0500},
  date-modified = {2008-09-14 15:32:12 -0500},
  doi = {10.1137/S1064827501385931},
  keywords = {Mathematics; Mechanics},
  publisher = {SIAM},
  url = {http://link.aip.org/link/?SCE/24/1379/1}
}

@TECHREPORT{LD03,
  author = {Santiago Lombeyda and Mathieu Desbrun},
  title = {Interactive Extraction of High-Frequency Aesthetically-Coherent Colormaps},
  institution = {Caltech},
  year = {2003}
}

@ARTICLE{Lorensen:1987,
  author = {Lorensen, W. E. and Cline, H. E.},
  title = {Marching cubes: a high resolution 3D surface reconstruction algorithm},
  journal = {Computer Graphics },
  year = {1987},
  volume = {21},
  pages = {163-169}
}

@ARTICLE{Lorenzen:2007,
  author = {Lorenzen, S. and Zhang, Y.},
  title = {{Monte Carlo refinement of rigid-body protein docking structures
	with backbone displacement and side-chain optimization}},
  journal = {Protein Science},
  year = {2007},
  volume = {16},
  pages = {2716-2725}
}

@ARTICLE{Losasso04,
  author = {Frank Losasso and Fr{\'{e}}d{\'{e}}ric Gibou and Ronald Fedkiw},
  title = {{Simulating Water and Smoke with an Octree Data Structure}},
  journal = {ACM Trans. Graph.},
  year = {2004},
  volume = {23},
  pages = {457--462},
  number = {3},
  month = aug
}

@ARTICLE{Loughnane:1999,
  author = {Loughnane, B. J. and Scodinu, A. and Farrer, R. A. and Fourkas, J.
	T. and Mohanty, U. },
  title = {Exponential intermolecular dynamics in optical Kerr effect spectroscopy
	of small-molecule liquids },
  journal = {J. Chem. Phys.},
  year = {1999},
  volume = {111},
  pages = {2686-2694}
}

@ARTICLE{Loussier:2008,
  author = {Loussier, X. and Munteanu, D. and Autran, J. L. and Tintori, O.},
  title = {{Impact of Geometrical and Electrical Parameters on Speed Performance
	Characteristics in Ultimate Double-Gate Metal-Oxide-Semiconductor
	Field-Effect Transistors} },
  journal = {Japanese J Applied Physics},
  year = {2008},
  volume = {47},
  pages = {3390-3395},
  annote = {Impact of Geometrical and Electrical Parameters on Speed Performance
	Characteristics in Ultimate Double-Gate Metal-Oxide-Semiconductor
	Field-Effect Transistors },
  date-added = {2008-11-25 10:28:56 -0500},
  date-modified = {2008-11-25 10:28:56 -0500},
  ty = {JOUR}
}

@ARTICLE{Lu:2002,
  author = {Lu, B. Z. and Chen, W. Z. and Wang, C. X. and Xu, X. J.},
  title = {Protein molecular dynamics with electrostatic force entirely determined
	by a single {Poisson-Boltzmann} calculation},
  journal = {Proteins},
  year = {2002},
  volume = {48},
  pages = {497-504},
  number = {3},
  abstract = {The electrostatic force including the intramolecular Coulombic interactions
	and the electrostatic contribution of solvation effect were entirely
	calculated by using the finite difference {Poisson-Boltzmann} method
	(FDPB), which was incorporated into the GROMOS96 force field to complete
	a new finite difference stochastic dynamics procedure (FDSD). Simulations
	were performed on an insulin dimer. Different relative dielectric
	constants were successively assigned to the protein interior; a value
	of 17 was selected as optimal for our system. The simulation data
	were analyzed and compared with those obtained from 500-ps molecular
	dynamics (MD) simulation with explicit water and a 500-ps conventional
	stochastic dynamics (SD) simulation without the mean solvent force.
	The results indicate that the FDSD method with GROMOS96 force field
	is suitable to study the dynamics and structure of proteins in solution
	if used with the optimal protein dielectric constant.},
  address = {Department of Astronomy and Applied Physics, University of Science
	and Technology of China, Hefei, China.},
  annote = {Aug 15; Protein molecular dynamics with electrostatic force entirely
	determined by a single {Poisson-Boltzmann} calculation; 12112674},
  bdsk-url-1 = {http://www3.interscience.wiley.com/cgi-bin/abstract/94518072/ABSTRACT},
  date-added = {2008-06-29 14:18:57 -0500},
  date-modified = {2008-06-29 14:18:57 -0500},
  keywords = {Electrostatics; molecular\_simulation},
  ty = {JOUR},
  url = {http://www3.interscience.wiley.com/cgi-bin/abstract/94518072/ABSTRACT}
}

@ARTICLE{LuBZ:2010,
  author = {Lu, B.-Z. and Holst, M. J. and McCammon, J. A. and Zhou, Y. C. },
  title = {Poisson-Nernst-Planck equations for simulating biomolecular diffusion-reaction
	processes I: Finite element solutions},
  journal = {J. of Comput. Phys.},
  year = {2010},
  volume = {229},
  pages = {6979 - 6994},
  number = {19}
}

@ARTICLE{Lu:2001,
  author = {Lu, H. and Skolnick, J.},
  title = {{A distance-dependent atomic knowledge-based potential for improved
	protein structure selection}},
  journal = {Proteins},
  year = {2001},
  volume = {44},
  pages = {223-232},
  number = {3}
}

@ARTICLE{Lu9411421,
  author = {Lu, J. P. and Yang, W. T.},
  title = {The Shape of Large Single-Shell and Multiple-Shell Fullerenes},
  journal = {Physical Review B},
  year = {1994},
  volume = {49},
  pages = {11421-11424},
  number = {16},
  month = {Apr},
  abstract = {The morphology of multiple-shell fullerenes is investigated by ab
	initio calculations using Yang's O(N) method. It is found that for
	large single-shell fullerenes with I(h) symmetry, the spherical morphology
	has lower energy than that of polyhedron. The formation energy per
	atom follows a simple scaling law. Including an estimate of intershell
	van de Waals interactions leads to the conclusion that spherical
	multiple-shell fullerenes are likely the most stable structure of
	large carbon clusters. These results are in good agreement with recent
	experiments.},
  endnotereftype = {Journal Article},
  issn = {0163-1829},
  shorttitle = {The Shape of Large Single-Shell and Multiple-Shell Fullerenes},
  url = {<Go to ISI>://A1994NK06300070}
}

@ARTICLE{Lu:2003,
  author = {Lu, Q. and Luo, R.},
  title = {A {{Poisson-Boltzmann}} dynamics method with nonperiodic boundary
	condition},
  journal = {Journal of Chemical Physics},
  year = {2003},
  volume = {119},
  pages = {11035-11047},
  number = {21},
  abstract = {We have developed a well-behaved and efficient finite difference PoissonÃ¢Â€Â“Boltzmann
	dynamics method with a nonperiodic boundary condition. This is made
	possible, in part, by a rather fine grid spacing used for the finite
	difference treatment of the reaction field interaction. The stability
	is also made possible by a new dielectric model that is smooth both
	over time and over space, an important issue in the application of
	implicit solvents. In addition, the electrostatic focusing technique
	facilitates the use of an accurate yet efficient nonperiodic boundary
	condition: boundary grid potentials computed by the sum of potentials
	from individual grid charges. Finally, the particleÃ¢Â€Â“particle
	particleÃ¢Â€Â“mesh technique is adopted in the computation
	of the Coulombic interaction to balance accuracy and efficiency in
	simulations of large biomolecules. Preliminary testing shows that
	the nonperiodic PoissonÃ¢Â€Â“Boltzmann dynamics method is
	numerically stable in trajectories at least 4 ns long. The new model
	is also fairly efficient: it is comparable to that of the pairwise
	generalized Born solvent model, making it a strong candidate for
	dynamics simulations of biomolecules in dilute aqueous solutions.
	Note that the current treatment of total electrostatic interactions
	is with no cutoff, which is important for simulations of biomolecules.
	Rigorous treatment of the DebyeÃ¢Â€Â“HÃƒÂ¼ckel screening
	is also possible within the PoissonÃ¢Â€Â“Boltzmann framework:
	its importance is demonstrated by a simulation of a highly charged
	protein.},
  annote = {A {Poisson-Boltzmann} dynamics method with nonperiodic boundary condition;
	LuoPB1; A complete method for describing the implementation of PB
	forces in a molecular dynamics setting using a smooth dielectric
	function. Although this was not reviewed by Feig et al. in their
	comparison of PB solvers, the authors report that this implementation
	is also very fast and comparable in efficiency with GB.},
  bdsk-url-1 = {http://dx.doi.org/10.1063/1.1622376},
  date-added = {2008-06-29 14:19:30 -0500},
  date-modified = {2008-06-29 14:19:30 -0500},
  keywords = {Electrostatics},
  ty = {JOUR},
  url = {http://dx.doi.org/10.1063/1.1622376}
}

@INCOLLECTION{Lu021606,
  author = {Lu, Zhenyu and Liu, Haiyan and Elstner, Marcus and Yang, W. T.},
  title = {Parameterization of COSMO Solvent Model for Self-Consistent Charge
	Density-Functional Based Tight-Binding Calculations},
  booktitle = {Reviews In Modern Quantum Chemistry: A Celebration Of The Contributions
	Of R. G. PARR},
  publisher = {World Scientific},
  year = {2002},
  editor = {K.D.Sen},
  pages = {1606--1614},
  address = {Singapore},
  endnotereftype = {Book Section},
  shorttitle = {Parameterization of COSMO Solvent Model for Self-Consistent Charge
	Density-Functional Based Tight-Binding Calculations}
}

@ARTICLE{Lu06L57,
  author = {Lu, Z. Y. and Hu, H. and Yang, W. T. and Marszaleky, P. E.},
  title = {Simulating force-induced conformational transitions in polysaccharides
	with the SMD replica exchange method},
  journal = {Biophysical Journal},
  year = {2006},
  volume = {91},
  pages = {L57-L59},
  number = {6},
  month = {Sep},
  abstract = {Conventional steered molecular dynamics (SMD) simulations do not readily
	reproduce equilibrium conditions of atomic force microscopy (AFM)
	stretch and release measurements of polysaccharides undergoing force-induced
	conformational transitions because of the gap between the timescales
	of computer simulations (similar to 1 mu s) and AFM measurements
	(similar to 1 s). To circumvent this limitation, we propose using
	the replica exchange method ( REM) to enhance sampling during SMD
	simulations. By applying REM SMD to a small polysaccharide system
	and comparing the results with those from AFM stretching experiments,
	we demonstrate that REM SMD reproduces the experimental results not
	only qualitatively but quantitatively, approaching near equilibrium
	conditions of AFM measurements. As tested in this work, hysteresis
	and computational time of REM SMD simulations of short polysaccharide
	chains are significantly reduced as compared to regular SMD simulations,
	making REM SMD an attractive tool for studying forced-induced conformational
	transitions of small biopolymer systems.},
  endnotereftype = {Journal Article},
  issn = {0006-3495},
  shorttitle = {Simulating force-induced conformational transitions in polysaccharides
	with the SMD replica exchange method},
  url = {<Go to ISI>://000240130500001}
}

@ARTICLE{Lu049033,
  author = {Lu, Z. Y. and Nowak, W. and Lee, G. R. and Marszalek, P. E. and Yang,
	W. T.},
  title = {Elastic properties of single amylose chains in water: A quantum mechanical
	and AFM study},
  journal = {Journal of the American Chemical Society},
  year = {2004},
  volume = {126},
  pages = {9033-9041},
  number = {29},
  month = {Jul},
  abstract = {Recent single-molecule atomic force microscopy (AFM) experiments have
	revealed that some polysaccharides display large deviations from
	force-extension relationships of other polymers which typically behave
	as simple entropic springs. However, the mechanism of these deviations
	has not been fully elucidated. Here we report the use of novel quantum
	mechanical methodologies, the divide-and-conquer linear scaling approach
	and the self-consistent charge density functional-based tight binding
	(SCC-DFTB) method, to unravel the mechanism of the extensibility
	of the polysaccharide amylose, which in water displays particularly
	large deviations from the simple entropic elasticity. We studied
	the deformations of maltose, a building block of amylose, both in
	a vacuum and in solution. To simulate the deformations in solution,
	the TIP3P molecular mechanical model is used to model the solvent
	water, and the SCC-DFTB method is used to model the solute. The interactions
	between the solute and water are treated by the combined quantum
	mechanical and molecular mechanical approach. We find that water
	significantly affects the mechanical properties of maltose. Furthermore,
	we performed two nanosecond-scale steered molecular dynamics simulations
	for single amylose chains composed of 10 glucopyranose rings in solution.
	Our SCC-DFTB/MM simulations reproduce the experimentally measured
	force-extension curve, and we find that the force-induced chair-to-boat
	transitions of glucopyranose rings are responsible for the characteristic
	plateau in the force-extension curve of amylose. In addition, we
	performed single-molecule AFM measurements on carboxymethyl amylose,
	and we found that, in contrast to the results of an earlier work
	by others, these side groups do not significantly affect amylose
	elasticity. By combining our experimental and modeling results, we
	conclude that the nonentropic elastic behavior of amylose is governed
	by the mechanics of pyranose rings themselves and their force-induced
	conformational transitions.},
  endnotereftype = {Journal Article},
  issn = {0002-7863},
  shorttitle = {Elastic properties of single amylose chains in water: A quantum mechanical
	and AFM study},
  url = {<Go to ISI>://000222855300043}
}

@ARTICLE{Lu0489,
  author = {Lu, Z. Y. and Yang, W. T.},
  title = {Reaction path potential for complex systems derived from combined
	ab initio quantum mechanical and molecular mechanical calculations},
  journal = {Journal of Chemical Physics},
  year = {2004},
  volume = {121},
  pages = {89-100},
  number = {1},
  month = {Jul},
  abstract = {Combined ab initio quantum mechanical and molecular mechanical calculations
	have been widely used for modeling chemical reactions in complex
	systems such as enzymes, with most applications being based on the
	determination of a minimum energy path connecting the reactant through
	the transition state to the product in the enzyme environment. However,
	statistical mechanics sampling and reaction dynamics calculations
	with a combined ab initio quantum mechanical (QM) and molecular mechanical
	(MM) potential are still not feasible because of the computational
	costs associated mainly with the ab initio quantum mechanical calculations
	for the QM subsystem. To address this issue, a reaction path potential
	energy surface is developed here for statistical mechanics and dynamics
	simulation of chemical reactions in enzymes and other complex systems.
	The reaction path potential follows the ideas from the reaction path
	Hamiltonian of Miller, Handy and Adams for gas phase chemical reactions
	but is designed specifically for large systems that are described
	with combined ab initio quantum mechanical and molecular mechanical
	methods. The reaction path potential is an analytical energy expression
	of the combined quantum mechanical and molecular mechanical potential
	energy along the minimum energy path. An expansion around the minimum
	energy path is made in both the nuclear and the electronic degrees
	of freedom for the QM subsystem internal energy, while the energy
	of the subsystem described with MM remains unchanged from that in
	the combined quantum mechanical and molecular mechanical expression
	and the electrostatic interaction between the QM and MM subsystems
	is described as the interaction of the MM charges with the QM charges.
	The QM charges are polarizable in response to the changes in both
	the MM and the QM degrees of freedom through a new response kernel
	developed in the present work. The input data for constructing the
	reaction path potential are energies, vibrational frequencies, and
	electron density response properties of the QM subsystem along the
	minimum energy path, all of which can be obtained from the combined
	quantum mechanical and molecular mechanical calculations. Once constructed,
	it costs much less for its evaluation. Thus, the reaction path potential
	provides a potential energy surface for rigorous statistical mechanics
	and reaction dynamics calculations of complex systems. As an example,
	the method is applied to the statistical mechanical calculations
	for the potential of mean force of the chemical reaction in triosephosphate
	isomerase. (C) 2004 American Institute of Physics.},
  endnotereftype = {Journal Article},
  issn = {0021-9606},
  shorttitle = {Reaction path potential for complex systems derived from combined
	ab initio quantum mechanical and molecular mechanical calculations},
  url = {<Go to ISI>://000222112100010}
}

@ARTICLE{Lum:1999,
  author = {Lum, K. and Chandler, D. and Weeks, J. D.},
  title = {Hydrophobicity at small and large length scales},
  journal = {Journal of Physical Chemistry B},
  year = {1999},
  volume = {103},
  pages = {4570-7},
  number = {22},
  abstract = {We develop a unified and generally applicable theory of solvation
	of small and large apolar species in water. In the former, hydrogen
	bonding of water is hindered yet persists near the solutes. In the
	latter, hydrogen bonding is depleted, leading to drying of extended
	apolar surfaces, large forces of attraction, and hysteresis on mesoscopic
	length scales. The crossover occurs on nanometer length scales, when
	the local concentration of apolar units is sufficiently high, or
	when an apolar surface is sufficiently large. Our theory for the
	crossover has implications concerning the stability of protein assemblies
	and protein folding.},
  annote = {Hydrophobicity at small and large length scales; LCW},
  bdsk-url-1 = {http://dx.doi.org/10.1021/jp984327m},
  date-added = {2008-06-29 15:11:31 -0500},
  date-modified = {2008-06-29 15:11:31 -0500},
  keywords = {Solvation; Statistical_mechanics},
  ty = {JOUR},
  url = {http://dx.doi.org/10.1021/jp984327m}
}

@ARTICLE{Lundstrom:2005,
  author = {Lundstrom, K. and Chiu, M., editors.},
  title = {{G Protein-Coupled Receptors in Drug Discovery}},
  journal = {First edition ed: Taylor and Francis},
  year = {2005}
}

@ARTICLE{AMBER-PB,
  author = {Luo, R. and David, L. and Gilson, M. K.},
  title = {Accelerated {{Poisson-Boltzmann}} calculations for static and dynamic
	systems},
  journal = {Journal of Computational Chemistry},
  year = {2002},
  volume = {23},
  pages = {1244-53},
  number = {13},
  abstract = {We report here an efficient implementation of the finite difference
	{Poisson-Boltzmann} solvent model based on the Modified Incomplete
	Cholsky Conjugate Gradient algorithm, which gives rather impressive
	performance for both static and dynamic systems. This is achieved
	by implementing the algorithm with Eisenstat's two optimizations,
	utilizing the electrostatic update in simulations, and applying prudent
	approximations, including: relaxing the convergence criterion, not
	updating {Poisson-Boltzmann}-related forces every step, and using
	electrostatic focusing. It is also possible to markedly accelerate
	the supporting routines that are used to set up the calculations
	and to obtain energies and forces. The resulting finite difference
	{Poisson-Boltzmann} method delivers efficiency comparable to the
	distance-dependent dielectric model for a system tested, HIV Protease,
	making it a strong candidate for solution-phase molecular dynamics
	simulations. Further, the finite difference method includes all intrasolute
	electrostatic interactions, whereas the distance dependent dielectric
	calculations use a 15-A cutoff. The speed of our numerical finite
	difference method is comparable to that of the pair-wise Generalized
	Born approximation to the {Poisson-Boltzmann} method.},
  address = {Department of Molecular Biology and Biochemistry, University of California,
	Irvine, California 92697-3900, USA.},
  annote = {Oct; Accelerated {Poisson-Boltzmann} calculations for static and
	dynamic systems; 12210150; LuoPB; A discussion of several straightforward
	modifications of PB solvers in order to provide significant acceleration
	of the solution and thereby enable the use of PB forces in molecular
	dynamics simulations.},
  bdsk-url-1 = {http://www3.interscience.wiley.com/cgi-bin/abstract/96516852/ABSTRACT},
  date-added = {2008-06-29 14:47:19 -0500},
  date-modified = {2008-06-29 14:47:19 -0500},
  keywords = {Electrostatics},
  ty = {JOUR},
  url = {http://www3.interscience.wiley.com/cgi-bin/abstract/96516852/ABSTRACT}
}

@ARTICLE{Luscombe:1992,
  author = {Luscombe, J. H. and Bouchard, A. M. and Luban, M.},
  title = {{Electron confinement in quantum nanostructure - Self-consistent
	Poisson-Schr\"{o}dinger theory}},
  journal = {Physical Review B},
  year = {1992},
  volume = {46},
  pages = {10262-10268 },
  annote = {Electron confinement in quantum nanostructure - Self-consistent Poisson-Schrodinger
	theory},
  date-added = {2008-11-25 10:28:56 -0500},
  date-modified = {2008-11-25 10:28:56 -0500},
  ty = {JOUR}
}

@ARTICLE{Luty:1992b,
  author = {Luty, B. A. and Davis, M. E. and McCammon, J. A.},
  title = {Solving the finite-difference non-linear {{Poisson-Boltzmann}} equation},
  journal = {Journal of Computational Chemistry},
  year = {1992},
  volume = {13},
  pages = {1114-1118},
  annote = {Solving the finite-difference non-linear {{Poisson-Boltzmann}} equation},
  date-added = {2008-09-16 15:33:12 -0500},
  date-modified = {2008-09-16 15:33:12 -0500},
  keywords = {Electrostatics},
  ty = {JOUR}
}

@ARTICLE{Lysaker:2003,
  author = {Lysaker, M. and Lundervold, A. and Tai, X. C.},
  title = {Noise removal using fourth-order partial differential equation with
	application to medical magnetic resonance images in space and time},
  journal = {IEEE Trans. Imag. Proc.},
  year = {2003},
  volume = {12},
  pages = {1579-1590},
  annote = {Noise removal using fourth-order partial differential equation with
	application to medical magnetic resonance images in space and time},
  date-added = {2008-09-19 10:28:56 -0500},
  date-modified = {2008-09-19 10:28:56 -0500},
  ty = {JOUR}
}

@ARTICLE{MLysaker:2003,
  author = {Lysaker, M. and Lundervold, A. and Tai, X. C.},
  title = {Noise removal using fourth-order partial differential equation with
	application to medical magnetic resonance images in space and time},
  journal = {{IEEE} Transactions on Image Processing},
  year = {2003},
  volume = {12},
  pages = {1579-1590},
  number = {12}
}

@ARTICLE{MacDermaid:2007,
  author = {MacDermaid, C. M. and Kaminski, G. A.},
  title = {Electrostatic Polarization Is Crucial for Reproducing {pKa} shifts
	of Carboxylic Residues in Turkey Ovomucoid Third Domain},
  journal = {Journal of Physical Chemistry B},
  year = {2007},
  volume = {111},
  pages = {9036-44},
  number = {30},
  abstract = {We have computed pKa shifts for carboxylic residues of the serine
	protease inhibitor turkey ovomucoid third domain (residues Asp7,
	Glu10, Glu19, Asp27, and Glu43). Both polarizable and nonpolarizable
	empirical force fields were employed. Hydration was represented by
	the surface generalized Born and {Poisson-Boltzmann} continuum model.
	The calculations were carried out in the most physically straightforward
	fashion, by directly comparing energies of the protonated and deprotonated
	protein forms, without any additional parameter fitting or adjustment.
	Our studies have demonstrated that (i) the {Poisson-Boltzmann} solvation
	model is more than adequate in reproducing pKa shifts, most likely
	due to its intrinsically many-body formalism; (ii) explicit treatment
	of electrostatic polarization included in our polarizable force field
	(PFF) calculations appears to be crucial in reproducing the acidity
	constant shifts. The average error of the PFF results was found to
	be as low as 0.58 pKa units, with the best fixed-charges average
	deviation being 3.28 units. Therefore, the pKa shifts phenomena and
	the governing electrostatics are clearly many-body controlled in
	their intrinsic nature; (iii) our results confirm previously reported
	conclusions that pKa shifts for protein residues are controlled by
	the immediate environment of the residues in question, as opposed
	to long-range interactions in proteins. We are confident that our
	confirmation of the importance of explicit inclusion of polarization
	in empirical force fields for protein studies will be useful far
	beyond the immediate goal of accurate calculation of acidity constants.},
  bdsk-url-1 = {http://dx.doi.org/10.1021/jp071284d},
  date-added = {2008-09-01 13:52:12 -0500},
  date-modified = {2008-09-01 13:52:12 -0500},
  keywords = {pKa; Electrostatics; Solvation},
  url = {http://dx.doi.org/10.1021/jp071284d}
}

@ARTICLE{CHARMM22,
  author = {MacKerell, A. D. , Jr. and Bashford, D. and Bellot, M. and Dunbrack,
	R. L. , Jr. and Evanseck, J. D. and Field, M. J. and Fischer, S.
	and Gao, J. and Guo, H. and Ha, S. and Joseph-McCarthy, D. and Kuchnir,
	L. and Kuczera, K. and Lau, F. T. K. and Mattos, C. and Michnick,
	S. and Ngo, T. and Nguyen, D. T. and Prodhom, B. and Reiher, W. E.
	, {III} and Roux, B. and Schlenkrich, M. and Smith, J. C. and Stote,
	R. and Straub, J. and Watanabe, M. and Wiorkiewicz-Kuczera, J. and
	Yin, D. and Karplus, M.},
  title = {All-Atom Empirical Potential for Molecular Modeling and Dynamics
	Studies of Proteins},
  journal = {Journal of Physical Chemistry B},
  year = {1998},
  volume = {102},
  pages = {3586-3616},
  number = {18},
  abstract = {New protein parameters are reported for the all-atom empirical energy
	function in the CHARMM program. The parameter evaluation was based
	on a self-consistent approach designed to achieve a balance between
	the internal (bonding) and interaction (nonbonding) terms of the
	force field and among the solvent-solvent, solvent-solute, and solute-solute
	interactions. Optimization of the internal parameters used experimental
	gas-phase geometries, vibrational spectra, and torsional energy surfaces
	supplemented with ab initio results. The peptide backbone bonding
	parameters were optimized with respect to data for N-methylacetamide
	and the alanine dipeptide. The interaction parameters, particularly
	the atomic charges, were determined by fitting ab initio interaction
	energies and geometries of complexes between water and model compounds
	that represented the backbone and the various side chains. In addition,
	dipole moments, experimental heats and free energies of vaporization,
	solvation and sublimation, molecular volumes, and crystal pressures
	and structures were used in the optimization. The resulting protein
	parameters were tested by applying them to noncyclic tripeptide crystals,
	cyclic peptide crystals, and the proteins crambin, bovine pancreatic
	trypsin inhibitor, and carbonmonoxy myoglobin in vacuo and in crystals.
	A detailed analysis of the relationship between the alanine dipeptide
	potential energy surface and calculated protein , angles was made
	and used in optimizing the peptide group torsional parameters. The
	results demonstrate that use of ab initio structural and energetic
	data by themselves are not sufficient to obtain an adequate backbone
	representation for peptides and proteins in solution and in crystals.
	Extensive comparisons between molecular dynamics simulations and
	experimental data for polypeptides and proteins were performed for
	both structural and dynamic properties. Energy minimization and dynamics
	simulations for crystals demonstrate that the latter are needed to
	obtain meaningful comparisons with experimental crystal structures.
	The presented parameters, in combination with the previously published
	CHARMM all-atom parameters for nucleic acids and lipids, provide
	a consistent set for condensed-phase simulations of a wide variety
	of molecules of biological interest.},
  annote = {All-Atom Empirical Potential for Molecular Modeling and Dynamics
	Studies of Proteins},
  bdsk-url-1 = {http://dx.doi.org/10.1021/jp973084f},
  date-added = {2008-06-30 11:39:34 -0500},
  date-modified = {2008-06-30 11:39:41 -0500},
  keywords = {molecular\_dynamics},
  ty = {JOUR},
  url = {http://dx.doi.org/10.1021/jp973084f}
}

@ARTICLE{MacKerell:1998,
  author = {MacKerell, Jr. A. D. and Bashford, D. and Bellott, M. and Dunbrack,
	J. R. L. and Evanseck, J.D. and Field, M.J. and Fischer, S. and Gao,
	J. and Guo, H. and Ha, S. and Joseph-McCarthy, S. and Kuchnir, L.
	and Kuczera, K. and Lau, F.T.K. and Mattos, C. and Michnick, S. and
	Ngo, T. and Nguyen, D.T. and Prodhom, B. and Reiher, I. W. E. and
	Roux, B. and Schlenkrich, M. and Smith, J.C. and Stote, R. and Straub,
	J. and Watanabe, M. and Wi-rkiewicz-Kuczera, J. and Yin, D.
	and Karplus, M.},
  title = {{All-Atom Empirical Potential for Molecular Modeling and Dynamics
	Studies of Proteins}},
  journal = {J Phys Chem B},
  year = {1998},
  volume = {102},
  pages = {3586-3616},
  number = {18}
}

@ARTICLE{Macounova:2000,
  author = {Macounova, K. and Cabrera, C. R. and Holl, M. R. and Yager, P.},
  title = {Generation of natural pH gradients in microfluidic channels for use
	in isoelectric focusing},
  journal = {Analytical Chemistry },
  year = {2000},
  volume = {72},
  pages = {3745-3751}
}

@ARTICLE{UHBD,
  author = {Madura, J. D. and Briggs, J. M. and Wade, R. C. and Davis, M. E.
	and Luty, B. A. and Ilin, A. and Antosiewicz, J. and Gilson, M. K.
	and Bagheri, B. and Scott, L. R. and McCammon, J. A.},
  title = {Electrostatics and diffusion of molecules in solution - simulations
	with the {University of Houston Brownian Dynamics} program},
  journal = {Computer Physics Communications},
  year = {1995},
  volume = {91},
  pages = {57-95},
  number = {1-3},
  abstract = {This paper is a follow-up to the initial communication (Comput. Phys.
	Commun. 62 (1991) 187Ã¢Â€Â-97) on the Brownian Dynamics/Electrostatics
	program UHBD developed at the University of Houston. The program
	is now capable of computing pKas of ionizable groups in proteins,
	performing Brownian dynamics simulations with a flexible substrate
	and target, and molecular mechanics/dynamics calculations using a
	continuum solvent. These new capabilities and other features are
	discussed along with selected applications which illustrate the capabilities
	of the current version of UHBD.},
  address = {Univ so alabama,dept chem mobile, al usa 36688 Univ calif san diego,dept
	chem \& biochem san diego, ca usa 92093 Univ calif san diego,dept
	pharmacol san diego, ca usa 92093 European molec biol lab d-69012
	heidelberg germany Bristol myers squibb pharmaceut res inst princeton,
	nj usa 08543 Eth zurich,phys chem lab ch-8092 zurich switzerland
	Univ houston,dept math houston, tx usa 77204 Nist,ctr adv res biotechnol
	rockville, md usa 20850},
  annote = {Electrostatics and diffusion of molecules in solution - simulations
	with the University of Houston Brownian Dynamics program; SEP},
  bdsk-url-1 = {http://dx.doi.org/10.1016/0010-4655(95)00043-F},
  date-added = {2008-09-01 13:54:40 -0500},
  date-modified = {2008-09-01 13:54:40 -0500},
  journal1 = {Comput Phys Commun},
  keywords = {Diffusion},
  ty = {JOUR},
  url = {http://dx.doi.org/10.1016/0010-4655(95)00043-F}
}

@ARTICLE{Mainardi:2000,
  author = { Mainardi, F. and Gorenflo, R. },
  title = { On { Mittag-Leffler-type} functions in fractional evolution processes
	
	},
  journal = { Journal of Computational and Applied Mathematics },
  year = {2000},
  volume = {118},
  pages = {283 - 299}
}

@ARTICLE{osher78,
  author = {Majda, A. and McDonough, J. and Osher, S.},
  title = {The Fourier method for nonsmooth initial data},
  journal = {Math. Comput.},
  year = {1978},
  volume = {32},
  pages = {1041-1081}
}

@ARTICLE{Majles:2011,
  author = { Majles Ara, M. H. and Mousavi, S. H. and Mousavi, Z. and Zakerhamidi,
	M. S. },
  title = {Investigation of the Kerr effect and third-order susceptibility constants
	in a nematic liquid crystal },
  journal = {Journal of Molecular Liquids},
  year = {2011},
  volume = {161},
  pages = {41 - 43}
}

@ARTICLE{Majumdara:2008,
  author = {Majumdara, K. and Bhat, N.},
  title = {Band structure effects in ultra-thin-body double-gate field effect
	transistor: A fullband analysis },
  journal = {J Applied Physics},
  year = {2008},
  volume = {103},
  pages = {114503},
  annote = {Band structure effects in ultra-thin-body double-gate field effect
	transistor: A fullband analysis },
  date-added = {2008-11-25 10:28:56 -0500},
  date-modified = {2008-11-25 10:28:56 -0500},
  ty = {JOUR}
}

@ARTICLE{Mamonov:2003,
  author = {Mamonov, Artem B. and Coalson, Rob D. and Nitzan, Abraham and Kurnikova,
	Maria G. },
  title = {The Role of the Dielectric Barrier in Narrow Biological Channels:
	A Novel Composite Approach to Modeling Single-Channel Currents},
  journal = {Biophysical Journal},
  year = {2003},
  volume = {84},
  pages = {3646-3661},
  month = {June}
}

@ARTICLE{Mamonov:2006,
  author = {Mamonov, A. B. and Kurnikova, M. G. and Coalson, R. D. },
  title = {Diffusion constant of {K$^+$ inside Gramicidin A}: a comparative study
	of four computational methods},
  journal = {Biophys Chem},
  year = {2006},
  volume = {124},
  pages = {268-78}
}

@ARTICLE{Manciu:2003,
  author = {Manciu, M. and Ruckenstein, E.},
  title = {On the Chemical Free Energy of the Electrical Double Layer},
  journal = {Langmuir},
  year = {2003},
  volume = {19},
  pages = {1114 - 1120},
  number = {4}
}

@ARTICLE{Marenich:2008,
  author = {Marenich, Aleksandr V. and Cramer, Christopher J. and Truhlar, Donald
	G.},
  title = {Perspective on Foundations of Solvation Modeling: The Electrostatic
	Contribution to the Free Energy of Solvation},
  journal = {Journal of Chemical Theory and Computation},
  year = {2008},
  volume = {4},
  pages = {877-887},
  number = {6},
  abstract = {no abstract},
  affiliation = {Department of Chemistry and Supercomputing Institute, University of
	Minnesota, Minneapolis, Minnesota 55455-0431},
  bdsk-url-1 = {http://pubs3.acs.org/acs/journals/doilookup?in_doi=10.1021/ct800029c},
  date-added = {2008-09-03 13:18:36 -0500},
  date-modified = {2008-09-03 13:18:36 -0500},
  doi = {10.1021/ct800029c},
  keywords = {Solvation; Electrostatics; Review},
  url = {http://pubs3.acs.org/acs/journals/doilookup?in_doi=10.1021/ct800029c}
}

@BOOK{Markowich:1986,
  title = {The Stationary Semiconductor Device Equations},
  publisher = {Springer-Verlag},
  year = {1986},
  author = {Markowich, P. }
}

@ARTICLE{Marrink:2007,
  author = {Marrink, S. J. and Risselada, H. J. and Yefimov, S. and Tieleman,
	D. P. and de Vries, A. H.},
  title = {The {MARTINI} Force Field: Coarse Grained Model for Biomolecular
	Simulations},
  journal = {J. Phys. Chem. B},
  year = {submitted, 2010},
  volume = {111},
  number = {7812 - 7824}
}

@ARTICLE{Marrink:2007,
  author = {Marrink, S. J. and Risselada, H. J. and Yefimov, S. and Tieleman,
	D. P. and de Vries, A. H.},
  title = {The {MARTINI} Force Field: Coarse Grained Model for Biomolecular
	Simulations},
  journal = {J. Phys. Chem. B},
  year = {submitted, 2010},
  volume = {111},
  number = {7812 - 7824}
}

@MISC{MarsdenComm,
  author = {Jerrold E. Marsden},
  howpublished = {Private Communication},
  year = {2007}
}

@ARTICLE{Martinez:2007,
  author = { Martinez, A. and Barker, J. R. and Svizhenko, A. and Anantram, M.
	P. and Asenov, A.},
  title = {The impact of random dopant aggregation in source and drain on the
	performance of ballisitic {DG} {Nano-MOSFETs}: {A NEGF} study},
  journal = {IEEE TRansactions on Nanotechnology},
  year = {2007},
  volume = {6},
  pages = {438-445}
}

@ARTICLE{Marx:2000,
  author = {Marx, D. and Hutter, J. },
  title = {Ab Initio Molecular Dynamics: Theory and Implementation},
  journal = {Modern Methods and Algorithms of Quantum Chemistry, J. Grotendorst
	(Ed.), John von Neumann Institute for Computing, J$\ddot{u}$lich,
	NIC Series},
  year = {2000},
  volume = {3},
  pages = {329-477}
}

@ARTICLE{Massova:1999,
  author = {Massova, I. and Kollman, P. A.},
  title = {{Computational Alanine Scanning To Probe Protein-Protein Interactions:
	A Novel Approach To Evaluate Binding Free Energies}},
  journal = {Journal of the American Chemical Society},
  year = {1999},
  volume = {121},
  pages = {8133-43},
  number = {36},
  abstract = {Noncovalent interactions are important in many physiological processes
	of complexation which involve all components of the living cells.
	Here we report an approach to computationally study the interaction
	free energies in protein-protein complexes which allows from a single
	simulation an estimate of the individual contribution of each residue
	to the binding. We developed this new technique-computational alanine
	scanning-and applied it to study the interactions of the oncoprotein
	Mdm2 to the N-terminal stretch of tumor suppressor protein p53. Excellent
	agreement has been found between the calculated and experimental
	data. This residue mutation methodology could prove to be a useful
	general design tool for molecules-nucleotides, peptides, lipids,
	or any other organic compound-optimized for interactions or stability,
	since one can qualitatively estimate the free energy consequences
	of many mutations from a single molecular dynamics trajectory.},
  annote = {Computational Alanine Scanning To Probe Protein-Protein Interactions:
	A Novel Approach To Evaluate Binding Free Energies; MM/PBSA},
  bdsk-url-1 = {http://dx.doi.org/10.1021/ja990935j},
  date-added = {2008-09-01 13:51:02 -0500},
  date-modified = {2008-09-01 13:51:02 -0500},
  keywords = {Electrostatics; MolecularDynamics},
  ty = {JOUR},
  url = {http://dx.doi.org/10.1021/ja990935j}
}

@ARTICLE{Mathur:2009,
  author = {Mathur, S. R. and Murthy, J. Y. },
  title = {A multigrid method for the {Poisson-Nernst-Planck} equations},
  journal = {SIAM J. Appl. Math.},
  year = {2009},
  volume = {52},
  pages = {4031-4039},
  number = {17-18}
}

@ARTICLE{Matousek:2007,
  author = {Matousek, William M. and Ciani, Barbara and Fitch, Carolyn A. and
	Garcia-Moreno, Bertrand E. and Kammerer, Richard A. and Alexandrescu,
	Andrei T.},
  title = {Electrostatic Contributions to the Stability of the {GCN4} Leucine
	Zipper Structure},
  journal = {Journal of Molecular Biology},
  year = {2007},
  volume = {374},
  pages = {206-19},
  number = {1},
  abstract = {Ion pairs are ubiquitous in X-ray structures of coiled coils, and
	mutagenesis of charged residues can result in large stability losses.
	By contrast, pKa values determined by NMR in solution often predict
	only small contributions to stability from charge interactions. To
	help reconcile these results we used triple-resonance NMR to determine
	pKa values for all groups that ionize between pH 1 and 13 in the
	33-residue leucine zipper fragment, GCN4p. In addition to the native
	state we also determined comprehensive pKa values for two models
	of the GCN4p denatured state: the protein in 6 M urea, and unfolded
	peptide fragments of the protein in water. Only residues that form
	ion pairs in multiple X-ray structures of GCN4p gave large pKa differences
	between the native and denatured states. Moreover, electrostatic
	contributions to stability were not equivalent for oppositely charged
	partners in ion pairs, suggesting that the interactions between a
	charge and its environment are as important as those within the ion
	pair. The pH dependence of protein stability calculated from NMR-derived
	pKa values agreed with the stability profile measured from equilibrium
	urea-unfolding experiments as a function of pH. The stability profile
	was also reproduced with structure-based continuum electrostatic
	calculations, although contributions to stability were overestimated
	at the extremes of pH. We consider potential sources of errors in
	the calculations, and how pKa predictions could be improved. Our
	results show that although hydrophobic packing and hydrogen bonding
	have dominant roles, electrostatic interactions also make significant
	contributions to the stability of the coiled coil.},
  bdsk-url-1 = {http://www.sciencedirect.com/science/article/B6WK7-4PMT358-2/2/ac0795cf40f8edbeacbf905f1bde28c4},
  bdsk-url-2 = {http://dx.doi.org/10.1016/j.jmb.2007.09.007},
  date-added = {2008-09-01 13:53:29 -0500},
  date-modified = {2008-09-01 13:53:29 -0500},
  doi = {10.1016/j.jmb.2007.09.007},
  keywords = {Electrostatics; pKa; Solvation},
  priority = {0},
  url = {http://www.sciencedirect.com/science/article/B6WK7-4PMT358-2/2/ac0795cf40f8edbeacbf905f1bde28c4}
}

@ARTICLE{Mayo:1984,
  author = {Mayo, A.},
  title = {The fast solution of {Poisson}'s and the biharmonic equations on
	irregular regions},
  journal = {SIAM J. Numer. Anal. },
  year = {1984},
  volume = {21},
  pages = {285-299},
  annote = {The fast solution of {Poisson}'s and the biharmonic equations on
	irregular regions},
  date-added = {2008-09-19 10:28:56 -0500},
  date-modified = {2008-09-19 10:28:56 -0500},
  ty = {JOUR}
}

@ARTICLE{Mayo:2007,
  author = {Mayo, M. and Greenbaum, A.},
  title = {Fourth order accurate evaluation of integrals in potential theory
	on exterior 3D regions},
  journal = {J. Comput. Phys. },
  year = {2007},
  volume = {220},
  pages = {900-914},
  annote = {Fourth order accurate evaluation of integrals in potential theory
	on exterior 3D regions},
  date-added = {2008-09-19 10:28:56 -0500},
  date-modified = {2008-09-19 10:28:56 -0500},
  ty = {JOUR}
}

@ARTICLE{mcinerney1996dmm,
  author = {McInerney, T. and Terzopoulos, D.},
  title = {{Deformable models in medical image analysis}},
  journal = {Mathematical methods in biomedical image analysis},
  year = {1996},
  pages = {171--180}
}

@ARTICLE{McKenney:1995,
  author = {McKenney, A. and Greengard, L. and Mayo, A.},
  title = {A fast {Poisson} solver for complex geometries},
  journal = {J. Comput. Phys. },
  year = {1995},
  volume = {118},
  pages = {348-355},
  annote = {A fast {Poisson} solver for complex geometries},
  date-added = {2008-09-19 10:28:56 -0500},
  date-modified = {2008-09-19 10:28:56 -0500},
  ty = {JOUR}
}

@INPROCEEDINGS{MLD05,
  author = {Alexander McKenzie and Santiago Lombeyda and Mathieu Desbrun},
  title = {Vector Field Analysis and Visualization through Variational Clustering},
  booktitle = {EG/IEEE VGTC Symposium on Visualization},
  year = {2005},
  pages = {1--7},
  month = Jun
}

@ARTICLE{McKenzie,
  author = {McKenzie, J. F. and Westphal, K. O.},
  title = {Interaction of linear waves with oblique shock waves.},
  journal = {Physics of Fluids},
  year = {1968},
  volume = {11},
  pages = {2350--2362}
}

@ARTICLE{McKimm-Breschkin:2000,
  author = {McKimm-Breschkin, J. L.},
  title = {Resistance of influenza viruses to neuraminidase inhibitors - a review
	},
  journal = {Journal of Infection },
  year = {2000},
  volume = {47},
  pages = {1 - 17},
  annote = {Resistance of influenza viruses to neuraminidase inhibitors - a review
	},
  date-added = {2009-03-10 },
  date-modified = {2009-03-10},
  ty = {JOUR}
}



@ARTICLE{Alhadeff:2014,
  author = {Alhadeff, R. and   Assa, D. and   Astrahan, P and  Krugliak, M. and  Arkin, I. T.},
  title = {Computational and experimental analysis of drug binding to the Influenza {M2} channel
	},
  journal = { Biochimica et Biophysica Acta (BBA) - Biomembranes  },
  year = {2000},
  volume = {1838},
  pages = {1068-1073},
}



@ARTICLE{McKinnon:2003,
  author = {McKinnon, W. R.},
  title = {{Fokker-Planck approach to extending the one-flux method of carrier
	transport in semiconductors to variable energies} },
  journal = {J. Applied Phys.},
  year = {2003},
  volume = {94},
  pages = {4986-4994},
  annote = {Fokker-Planck approach to extending the one-flux method of carrier
	transport in semiconductors to variable energies },
  date-added = {2008-11-25 10:28:56 -0500},
  date-modified = {2008-11-25 10:28:56 -0500},
  ty = {JOUR}
}

@ARTICLE{McNamara2004,
  author = {Antoine McNamara and Adrien Treuille and Zoran Popovic and Jos Stam},
  title = {{Fluid Control Using the Adjoint Method}},
  journal = {ACM Trans. Graph.},
  year = {2004},
  volume = {23},
  pages = {449--456},
  number = {3},
  month = aug
}

@ARTICLE{Meerschaert:WorldScientific,
  author = {Meerschaert, M.M.},
  title = {Fractional Calculus, Anomalous Diffusion, and Probability},
  journal = {Fractional Dynamics, R. Metzler and J. Klafter, Eds., World Scientific,
	Singapore},
  year = {2012},
  volume = { },
  pages = {265-284},
  number = { }
}

@ARTICLE{Meerschaert:2002,
  author = {Meerschaert,M.M and Benson, D. and ScheXer,H.P. and Baeumer,B. },
  title = {Stochastic solution of space-time fractional diffusion equations},
  journal = {Phys.Rev.E},
  year = {2002},
  volume = {65},
  pages = { 1103?C1106},
  number = { }
}

@ARTICLE{Meerschaert:2004,
  author = {Meerschaert,M.M. and Tadjeran,C. },
  title = {Finite difference approximations for fractional advection-dispersion
	flow equations},
  journal = {Journal of Computational and Applied Mathematics},
  year = {2004},
  volume = {172},
  pages = {65-77},
  number = {1}
}

@ARTICLE{Mei:2006,
  author = {Mei, Y. and Ji, C. G. and Zhang, J. Z. H.},
  title = {A new quantum method for electrostatic solvation energy of protein},
  journal = {J. Chem. Phys.},
  year = {2006},
  volume = {125},
  number = {094906}
}

@ARTICLE{Mennucci:1997,
  author = {Mennucci, B. and Cances, E. and Tomasi, J.},
  title = {Evaluation of solvent effects in isotropic and anisotropic dielectrics
	and in ionic solutions with a unified integral equation method: theoretical
	bases, computational implementation, and numerical applications},
  journal = {J. Phys. Chem. B},
  year = {1997},
  volume = {101},
  pages = {10506 - 10517}
}

@ARTICLE{MDDB01,
  author = {Mark Meyer and Gilles Debunne and Mathieu Desbrun and Alan H. Barr},
  title = {Interactive Animation of Cloth-like Objects for Virtual Reality},
  journal = {Jounal of Visualization and Computer Animation},
  year = {2001},
  pages = {1--12},
  month = {May},
  numero = {12(1)}
}

@INPROCEEDINGS{meyer-desbrun-etal:02,
  author = {Meyer, M. and Desbrun, M. and Schr\"oder, P. and Barr, A.H.},
  title = {Discrete Differential-Geometry Operators for 2-Manifolds},
  booktitle = {Proc. of Int. Workshop on Vis. and Math.},
  year = {2002},
  pages = {52--58}
}

@INPROCEEDINGS{MDSB02,
  author = {Mark Meyer and Mathieu Desbrun and Peter Schr{\"o}der and Alan H.
	Barr},
  title = {Discrete Differential-Geometry Operators for Triangulated 2-Manifolds},
  booktitle = {{V}isualization and {M}athematics III},
  year = {2003},
  editor = {Hans-Christian Hege and Konrad Polthier},
  pages = {35--57},
  publisher = {Springer-Verlag}
}

@ARTICLE{MLBD02,
  author = {Mark Meyer and Haeyoung Lee and Alan H. Barr and Mathieu Desbrun},
  title = {Generalized Barycentric Coordinates for Arbitrary N-gons},
  journal = {Jounal of Graphics Tools},
  year = {2002},
  volume = {7},
  pages = {13--22},
  number = {1}
}

@MISC{michor-mumford:05,
  author = {Michor, P.W. and Mumford, D.},
  title = {Riemannian Geometries of Space of Plane Curves},
  year = {2005},
  note = {Preprint}
}

@INPROCEEDINGS{CLSVOF-SCA,
  author = {V. Mihalef and D. Metaxas and M. Sussman and M.Y. Hussaini},
  title = {{Animation and Control of Breaking Waves}},
  booktitle = {EG/ACM SIGGRAPH Symp. on Comput. Anim.},
  year = {2004},
  pages = {315--324}
}

@INPROCEEDINGS{Boiling,
  author = {V. Mihalef and B. Unlusu and D. Metaxas and M. Sussman and M.Y. Hussaini},
  title = {{Physics-based Boiling Simulation}},
  booktitle = {EG/ACM SIGGRAPH Symp. on Comput. Anim.},
  year = {2006},
  pages = {317--324}
}

@ARTICLE{Mikula:2004,
  author = {Mikula, Karol and Sevcovic, Daniel },
  title = {A direct method for solving an anisotropic mean curvature flow of
	plane curves with an external force},
  journal = {Mathematical Methods in the Applied Sciences},
  year = {2004},
  volume = {27},
  pages = {1545--1565},
  number = {13},
  abstract = {A new method for solution of the evolution of plane curves satisfying
	the geometric equation v=beta(x,k,nu), where v is the normal velocity,
	k and nu are the curvature and tangential angle of a plane curve
	Gamma sub \&Ropf;2 at the point xisinGamma, is proposed. We derive
	a governing system of partial differential equations for the curvature,
	tangential angle, local length and position vector of an evolving
	family of plane curves and prove local in time existence of a classical
	solution. These equations include a non-trivial tangential velocity
	functional governing a uniform redistribution of grid points and
	thus preventing numerically computed solutions from forming various
	instabilities. We discretize the governing system of equations in
	order to find a numerical solution for 2D anisotropic interface motions
	and image segmentation problems. Copyright Â© 2004 John Wiley \&
	Sons, Ltd.},
  address = {Department of Mathematics, Slovak University of Technology, Radlinsk\'{e}ho
	11, 813 68 Bratislava, Slovak Republic; Institute of Applied Mathematics,
	Faculty of Mathematics, Physics \& Informatics, Comenius University,
	842 48 Bratislava, Slovak Republic},
  bdsk-url-1 = {http://dx.doi.org/10.1002/mma.514},
  date-added = {2008-06-30 21:04:10 -0400},
  date-modified = {2008-06-30 21:04:10 -0400},
  doi = {10.1002/mma.514},
  keywords = {mathematics},
  posted-at = {2008-07-01 02:01:56},
  priority = {0},
  url = {http://dx.doi.org/10.1002/mma.514}
}

@ARTICLE{Miller:1996,
  author = {Miller, J. L. and Kollman, P. A. },
  title = {Solvation Free Energies of the Nucleic Acid Bases},
  journal = {Journal of Physical Chemistry},
  year = {1996},
  volume = {100},
  pages = {8587--8594},
  number = {20},
  abstract = {Abstract: We present free energy perturbation calculations on the
	solvation free energies of the N-methylated nucleic acid bases adenine,
	guanine, cytosine, thymine, and uracil. This work demonstrates the
	importance of using thermodynamic cycles, a careful study of convergence,
	and the use of both single and dual perturbation topologies. We find
	that the calculated solvation free energies of 9-methyladenine and
	1-methylthymine are close to available experimental data. Additionally,
	we predict the solvation free energies for 9-methylguanine, 1-methylcytosine,
	and 1-methyluracil. The topologies used in these perturbations can
	be directly applied to free energy studies of higher order nucleic
	acid structures.},
  address = {Department of Pharmaceutical Chemistry, University of California-San
	Francisco, San Francisco, California 94143},
  bdsk-url-1 = {http://dx.doi.org/10.1021/jp9605358},
  date-added = {2008-06-30 06:15:51 -0500},
  date-modified = {2008-06-30 06:15:51 -0500},
  doi = {10.1021/jp9605358},
  keywords = {molecular\_simulation, nucleic\_acids, solvation},
  posted-at = {2008-06-30 12:15:23},
  priority = {0},
  url = {http://dx.doi.org/10.1021/jp9605358}
}

@ARTICLE{Miller:1981,
  author = {Miller, K.},
  title = {{Moving finite elements {II}}},
  journal = {SIAM J.Numer.Anal.},
  year = {1981},
  volume = {18},
  pages = {1033--1057}
}

@ARTICLE{Miller:1998,
  author = {Miller, W. H.},
  title = {Spiers Memorial Lecture - Quantum and semiclassical theory of chemical
	reaction rates},
  journal = {FARADAY DISCUSSIONS},
  year = {1998},
  volume = {110},
  pages = {1--21}
}

@ARTICLE{Mitchell:1976,
  author = {Mitchell, P},
  title = {Vectorial chemistry and the molecular mechanics of chemiosmotic coupling:
	power transmission by proticity},
  journal = {Biochem Soc Trans},
  year = {1976},
  volume = {4},
  pages = {399 - 430}
}

@ARTICLE{mitra-gelfand-etal:04,
  author = {Mitra, N.J. and Gelfand, N. and Pottmann, H. and Guibas, L.},
  title = {Registration of Point Cloud Data from a Geometric Optimization Perspective},
  journal = {Symp. on Geometry Processing},
  year = {2004},
  pages = {23--32}
}

@INPROCEEDINGS{MGP07,
  author = {Mitra, Niloy J. and Guibas, Leonidas J. and Pauly, Mark },
  title = {Symmetrization},
  booktitle = {SIGGRAPH '07: ACM SIGGRAPH 2007 papers},
  year = {2007},
  address = {New York, NY, USA},
  publisher = {ACM},
  abstract = {We present a symmetrization algorithm for geometric objects. Our algorithm
	enhances approximate symmetries of a model while minimally altering
	its shape. Symmetrizing deformations are formulated as an optimization
	process that couples the spatial domain with a transformation configuration
	space, where symmetries can be expressed more naturally and compactly
	as parametrized point-pair mappings. We derive closed-form solution
	for the optimal symmetry transformations, given a set of corresponding
	sample pairs. The resulting optimal displacement vectors are used
	to drive a constrained deformation model that pulls the shape towards
	symmetry. We show how our algorithm successfully symmetrizes both
	the geometry and the discretization of complex 2D and 3D shapes and
	discuss various applications of such symmetrizing deformations.},
  citeulike-article-id = {3824535},
  doi = {10.1145/1275808.1276456},
  keywords = {similarity, symmetry},
  location = {San Diego, California},
  owner = {Yiying},
  posted-at = {2008-12-26 16:09:08},
  priority = {2},
  timestamp = {2009.03.28},
  url = {http://dx.doi.org/10.1145/1275808.1276456}
}

@ARTICLE{MGP06,
  author = {Mitra, Niloy J. and Guibas, Leonidas J. and Pauly, Mark },
  title = {Partial and approximate symmetry detection for 3D geometry},
  journal = {ACM Trans. Graph.},
  year = {2006},
  volume = {25},
  pages = {560--568},
  number = {3},
  abstract = {"Symmetry is a complexity-reducing concept [...]; seek it every-where."
	- Alan J. PerlisMany natural and man-made objects exhibit significant
	symmetries or contain repeated substructures. This paper presents
	a new algorithm that processes geometric models and efficiently discovers
	and extracts a compact representation of their Euclidean symmetries.
	These symmetries can be partial, approximate, or both. The method
	is based on matching simple local shape signatures in pairs and using
	these matches to accumulate evidence for symmetries in an appropriate
	transformation space. A clustering stage extracts potential significant
	symmetries of the object, followed by a verification step. Based
	on a statistical sampling analysis, we provide theoretical guarantees
	on the success rate of our algorithm. The extracted symmetry graph
	representation captures important high-level information about the
	structure of a geometric model which in turn enables a large set
	of further processing operations, including shape compression, segmentation,
	consistent editing, symmetrization, indexing for retrieval, etc.},
  address = {New York, NY, USA},
  citeulike-article-id = {3391164},
  doi = {10.1145/1141911.1141924},
  issn = {0730-0301},
  keywords = {similarity, symmetry},
  owner = {Yiying},
  posted-at = {2008-10-09 17:45:09},
  priority = {5},
  publisher = {ACM},
  timestamp = {2009.03.28},
  url = {http://dx.doi.org/10.1145/1141911.1141924}
}

@ARTICLE{Mittal:2005,
  author = {Mittal, M. and Iaccarino, G.},
  title = {Immersed boundary methods},
  journal = {Annu. Rev. Fluid Mech. },
  year = {2005},
  volume = {37},
  pages = {236-261},
  annote = {Immersed boundary methods},
  date-added = {2008-09-19 10:28:56 -0500},
  date-modified = {2008-09-19 10:28:56 -0500},
  ty = {JOUR}
}

@ARTICLE{Mobley:2008,
  author = {Mobley, D. L. and Dill, K. A. and Chodera, J. D. },
  title = {Treating Entropy and Conformational Changes in Implicit Solvent Simulations
	of Small Molecules},
  journal = {Journal of Physical Chemistry B},
  year = {2008},
  volume = {112},
  pages = {938--946},
  number = {3},
  abstract = {Abstract: Implicit solvent models are increasingly popular for estimating
	aqueous solvation (hydration) free energies in molecular simulations
	and other applications. In many cases, parameters for these models
	are derived to reproduce experimental values for small molecule hydration
	free energies. Often, these hydration free energies are computed
	for a single solute conformation, neglecting solute conformational
	changes upon solvation. Here, we incorporate these effects using
	alchemical free energy methods. We find significant errors when hydration
	free energies are estimated using only a single solute conformation,
	even for relatively small, simple, rigid solutes. For example, we
	find conformational entropy (TS) changes of up to 2.3 kcal/mol upon
	hydration. Interestingly, these changes in conformational entropy
	correlate poorly (R2 = 0.03) with the number of rotatable bonds.
	The present study illustrates that implicit solvent modeling can
	be improved by eliminating the approximation that solutes are rigid.},
  address = {Department of Chemistry, Stanford University, Stanford, California
	94305},
  bdsk-url-1 = {http://dx.doi.org/10.1021/jp0764384},
  bdsk-url-2 = {http://dx.doi.org/10.1021/jp0764384},
  date-added = {2008-09-16 15:40:09 -0500},
  date-modified = {2008-09-16 15:40:09 -0500},
  doi = {10.1021/jp0764384},
  keywords = {Electrostatics, Nonpolar, Solvation},
  priority = {0},
  url = {http://dx.doi.org/10.1021/jp0764384}
}

@ARTICLE{Mohan:1992,
  author = {Mohan, V. and Davis, M. E. and McCammon, J. A. and Pettitt, B. M.},
  title = {Continuum model calculations of solvation free energies: accurate
	evaluation of electrostatic contributions},
  journal = {Journal of Physical Chemistry},
  year = {1992},
  volume = {96},
  pages = {6428-31},
  number = {15},
  bdsk-url-1 = {http://dx.doi.org/10.1021/j100194a060},
  date-added = {2008-06-30 06:18:31 -0500},
  date-modified = {2008-06-30 06:18:31 -0500},
  doi = {10.1021/j100194a060},
  keywords = {solvation; electrostatics},
  url = {http://dx.doi.org/10.1021%2Fj100194a060}
}

@ARTICLE{Momany:1978,
  author = {Momany, F. A.},
  title = {Determination of Partial Atomic Charges from Ab Initio Molecular
	Electrostatic Potentials. Application to Formamide, Methanol, and
	Formic Acid},
  journal = {J. Phys. Chem.},
  year = {1978},
  volume = {82},
  pages = { 592-601}
}

@ARTICLE{Mongan:2007,
  author = {Mongan, J. and Simmerling, C. and McCammon, J. A. and Case, D. A.
	and Onufriev, A.},
  title = {Generalized {Born} Model with a Simple, Robust Molecular Volume Correction},
  journal = {Journal of Chemical Theory and Computation},
  year = {2007},
  volume = {3},
  pages = {159-69},
  number = {1},
  abstract = {Generalized Born (GB) models provide a computationally efficient means
	of representing the electrostatic effects of solvent and are widely
	used, especially in molecular dynamics (MD). A class of particularly
	fast GB models is based on integration over an interior volume approximated
	as a pairwise union of atom spheres-effectively, the interior is
	defined by a {van der Waals} rather than Lee-Richards molecular surface.
	The approximation is computationally efficient but, if uncorrected,
	allows for high dielectric (water) regions smaller than a water molecule
	between atoms, leading to decreased accuracy. Here, an earlier pairwise
	GB model is extended by a simple analytic correction term that largely
	alleviates the problem by correctly describing the solvent-excluded
	volume of each pair of atoms. The correction term introduces a free
	energy barrier to the separation of nonbonded atoms. This free energy
	barrier is seen in explicit solvent and Lee-Richards molecular surface
	implicit solvent calculations but has been absent from earlier pairwise
	GB models. When used in MD, the correction term yields protein hydrogen
	bond length distributions and polypeptide conformational ensembles
	that are in better agreement with explicit solvent results than earlier
	pairwise models. The robustness and simplicity of the correction
	preserves the efficiency of the pairwise GB models while making them
	a better approximation to reality.},
  annote = {Generalized Born Model with a Simple, Robust Molecular Volume Correction},
  bdsk-url-1 = {http://dx.doi.org/10.1021/ct600085e},
  date-added = {2008-09-15 10:03:03 -0500},
  date-modified = {2008-09-15 10:03:03 -0500},
  keywords = {Solvation; Electrostatics},
  ty = {JOUR},
  url = {http://dx.doi.org/10.1021/ct600085e}
}

@ARTICLE{Montani1994,
  author = {Montani, Claudio and Scateni, Riccardo and Scopigno, Roberto},
  title = {{A modified look-up table for implicit disambiguation of Marching
	Cubes}},
  journal = {The Visual Computer},
  year = {1994},
  volume = {10},
  pages = {353--355},
  number = {6},
  month = jun,
  doi = {10.1007/BF01900830},
  file = {:C\:/Users/yiying/Desktop/SVN/geometrycode/references/Montani, Scateni, Scopigno - 1994 - A modified look-up table for implicit disambiguation of Marching Cubes.pdf:pdf},
  issn = {0178-2789},
  keywords = {face reconstruction - look-up,marching cubes algorithms triangula-,tables,volume
	visualization - sur-},
  url = {http://www.springerlink.com/index/10.1007/BF01900830}
}

@INPROCEEDINGS{MoretonSequin92,
  author = {Henri Moreton and Carlo S{\'e}quin},
  title = {Functional Optimization for Fair Surface Design},
  booktitle = {ACM SIGGRAPH},
  year = {1992},
  pages = {167--176}
}

@ARTICLE{Morgenthal:2007,
  author = {Morgenthal, G. and Walther, J. H.},
  title = {An immersed interface method for the Vortex-In-Cell algorithm},
  journal = {Computers \& Structures},
  year = {2007},
  volume = {85},
  pages = {712--726},
  number = {11-14},
  abstract = { The paper presents a two-dimensional immersed interface technique
	for the Vortex-In-Cell (VIC) method for simulation of flows past
	bodies of complex geometry. The particle-mesh VIC algorithm is augmented
	by a local particle-particle correction term in a Particle-Particle
	Particle-Mesh (P3M) context to resolve sub-grid scales incurred by
	the presence of the immersed interface. The particle-particle correction
	furthermore allows to disjoin mesh and particle resolution by explicitly
	resolving sub-grid scales on the particles. This P3M algorithm uses
	an influence matrix technique to annihilate the anisotropic sub-grid
	scales and adds an exact particle-particle correction term. Free-space
	boundary conditions are satisfied through the use of modified Green's
	functions in the solution of the Poisson equation for the streamfunction.
	The concept is extended such as to provide exact velocity predictions
	on the mesh with free-space boundary conditions. The random walk
	technique is employed for the diffusion in order to relax the need
	for a remeshing of the computational elements close to solid boundaries.
	A novel partial remeshing technique is introduced which only performs
	remeshing of the vortex elements which are located sufficiently distant
	from the immersed interfaces, thus maintaining a sufficient spatial
	representation of the vorticity field. Convergence of the present
	P3M algorithm is demonstrated for a circular patch of vorticity.
	The immersed interface technique is applied to the flow past a circular
	cylinder at a Reynolds number of 3000 and the convergence of the
	method is demonstrated by a systematic refinement of the spatial
	parameters. Finally, the flow past a cactus-like geometry is considered
	to demonstrate the efficient handling of complex bluff body geometries.
	The simulations offer an insight into physically interesting flow
	behavior involving a temporarily negative total drag force on the
	section.},
  bdsk-url-1 = {http://www.sciencedirect.com/science/article/B6V28-4N7RD1M-1/2/3f0d6f1d09bb1d71c9f1c95f52a569ae},
  booktitle = {Fourth MIT Conference on Computational Fluid and Solid Mechanics},
  date-added = {2008-09-14 15:32:12 -0500},
  date-modified = {2008-09-14 15:32:12 -0500},
  doi = {10.1016/j.compstruc.2007.01.020 },
  keywords = {Mathematics; FluidMechanics},
  ty = {JOUR},
  url = {http://www.sciencedirect.com/science/article/B6V28-4N7RD1M-1/2/3f0d6f1d09bb1d71c9f1c95f52a569ae}
}

@ARTICLE{Mori-Sanchez09066403,
  author = {Mori-Sanchez, P. and Cohen, A. J. and Yang, W. T.},
  title = {Discontinuous Nature of the Exchange-Correlation Functional in Strongly
	Correlated Systems},
  journal = {Physical Review Letters},
  year = {2009},
  volume = {102},
  pages = {066403},
  number = {6},
  month = {Feb},
  abstract = {Standard approximations for the exchange-correlation functional have
	been found to give big errors for the linearity condition of fractional
	charges, leading to delocalization error, and the constancy condition
	of fractional spins, leading to static correlation error. These two
	conditions are now unified and extended to states with both fractional
	charge and fractional spin to give a much more stringent condition:
	the exact energy functional is a plane, linear along the fractional
	charge coordinate and constant along the fractional spin coordinate
	with a line of discontinuity at the integer. Violation of this condition
	underlies the failure of all known approximate functionals to describe
	the gaps in strongly correlated systems. It is shown that explicitly
	discontinuous functionals of the density or orbitals that go beyond
	these currently used smooth approximations is the key for the application
	of density functional theory to strongly correlated systems.},
  endnotereftype = {Journal Article},
  issn = {0031-9007},
  shorttitle = {Discontinuous Nature of the Exchange-Correlation Functional in Strongly
	Correlated Systems},
  url = {<Go to ISI>://000263389500047 }
}

@ARTICLE{Mori-Sanchez08146401,
  author = {Mori-Sanchez, P. and Cohen, A. J. and Yang, W. T.},
  title = {Localization and delocalization errors in density functional theory
	and implications for band-gap prediction},
  journal = {Physical Review Letters},
  year = {2008},
  volume = {100},
  pages = {146401},
  number = {14},
  month = {Apr},
  abstract = {The band-gap problem and other systematic failures of approximate
	exchange-correlation functionals are explained from an analysis of
	total energy for fractional charges. The deviation from the correct
	intrinsic linear behavior in finite systems leads to delocalization
	and localization errors in large and bulk systems. Functionals whose
	energy is convex for fractional charges such as the local density
	approximation display an incorrect apparent linearity in the bulk
	limit, due to the delocalization error. Concave functionals also
	have an incorrect apparent linearity in the bulk calculation, due
	to the localization error and imposed symmetry. This resolves an
	apparent paradox and identifies the physical nature of the error
	to be addressed to obtain accurate band gaps from density functional
	theory.},
  endnotereftype = {Journal Article},
  issn = {0031-9007},
  shorttitle = {Localization and delocalization errors in density functional theory
	and implications for band-gap prediction},
  url = {<Go to ISI>://000254940900050}
}

@ARTICLE{Mori-Sanchez06201102,
  author = {Mori-Sanchez, P. and Cohen, A. J. and Yang, W. T.},
  title = {Many-electron self-interaction error in approximate density functionals},
  journal = {Journal of Chemical Physics},
  year = {2006},
  volume = {125},
  pages = {201102},
  number = {20},
  month = {Nov},
  abstract = {One of the most important challenges in density functional theory
	(DFT) is the proper description of fractional charge systems relating
	to the self-interaction error (SIE). Traditionally, the SIE has been
	formulated as a one-electron problem, which has been addressed in
	several recent functionals. However, these recent one-electron SIE-free
	functionals, while greatly improving the description of thermochemistry
	and reaction barriers in general, still exhibit many of the difficulties
	associated with SIE. Thus we emphasize the need to surpass this limit
	and shed light on the many-electron SIE. After identifying the sufficient
	condition for functionals to be free from SIE, we focus on the symptoms
	and investigate the performance of most popular functionals. We show
	that these functionals suffer from many-electron SIE. Finally, we
	give a SIE classification of density functionals. (c) 2006 American
	Institute of Physics.},
  endnotereftype = {Journal Article},
  issn = {0021-9606},
  shorttitle = {Many-electron self-interaction error in approximate density functionals},
  url = {<Go to ISI>://000242408100002}
}

@ARTICLE{Mori-Sanchez0691102,
  author = {Mori-Sanchez, P. and Cohen, A. J. and Yang, W. T.},
  title = {Self-interaction-free exchange-correlation functional for thermochemistry
	and kinetics},
  journal = {Journal of Chemical Physics},
  year = {2006},
  volume = {124},
  pages = {91102},
  number = {9},
  month = {Mar},
  abstract = {We develop a self-interaction-free exchange-correlation functional
	which is very accurate for thermochemistry and kinetics. This is
	achieved by theoretical construction of the functional form and nonlinear
	fitting. We define a simple interpolation of the adiabatic connection
	that uses exact exchange, generalized gradient approximation (GGA)
	and meta-GGA functionals. The performance is optimized by fitting
	a small number of empirical parameters. Overall the new functional
	improves significantly upon hybrids and meta-GGAs while correctly
	describing one-electron systems. The mean absolute error on a large
	set of reaction barriers is reduced to 1.99 kcal/mol. (c) 2006 American
	Institute of Physics.},
  endnotereftype = {Journal Article},
  issn = {0021-9606},
  shorttitle = {Self-interaction-free exchange-correlation functional for thermochemistry
	and kinetics},
  url = {<Go to ISI>://000235828300002}
}

@ARTICLE{Mori-Sanchez0562204,
  author = {Mori-Sanchez, P. and Wu, Q. and Yang, W. T.},
  title = {Orbital-dependent correlation energy in density-functional theory
	based on a second-order perturbation approach: Success and failure},
  journal = {Journal of Chemical Physics},
  year = {2005},
  volume = {123},
  pages = {62204},
  number = {6},
  month = {Aug},
  abstract = {We have developed a second-order perturbation theory (PT) energy functional
	within density-functional theory (DFT). Based on PT with the Kohn-Sham
	(KS) determinant as a reference, this new ab initio exchange-correlation
	functional includes an exact exchange (EXX) energy in the first order
	and a correlation energy including all single and double excitations
	from the KS reference in the second order. The explicit dependence
	of the exchange and correlation energy on the KS orbitals in the
	functional fits well into our direct minimization approach for the
	optimized effective potential, which is a very efficient method to
	perform fully self-consistent calculations for any orbital-dependent
	functionals. To investigate the quality of the correlation functional,
	we have applied the method to selected atoms and molecules. For two-electron
	atoms and small molecules described with small basis sets, this new
	method provides excellent results, improving both second-order Moller-Plesset
	expression and any conventional DFT results significantly. For larger
	systems, however, it performs poorly, converging to very low unphysical
	total energies. The failure of PT based energy functionals is analyzed,
	and its origin is traced back to near degeneracy problems due to
	the orbital- and eigenvalue-dependent algebraic structure of the
	correlation functional. The failure emerges in the self-consistent
	approach but not in perturbative post-EXX calculations, emphasizing
	the crucial importance of self-consistency in testing new orbital-dependent
	energy functionals. (C) 2005 American Institute of Physics.},
  endnotereftype = {Journal Article},
  issn = {0021-9606},
  shorttitle = {Orbital-dependent correlation energy in density-functional theory
	based on a second-order perturbation approach: Success and failure},
  url = {<Go to ISI>://000231310500006}
}

@ARTICLE{Mori-Sanchez0311001,
  author = {Mori-Sanchez, P. and Wu, Q. and Yang, W. T.},
  title = {Accurate polymer polarizabilities with exact exchange density-functional
	theory},
  journal = {Journal of Chemical Physics},
  year = {2003},
  volume = {119},
  pages = {11001-11004},
  number = {21},
  month = {Dec},
  abstract = {The long-standing problem of the large overestimation of polymer polarizabilities
	in density-functional theory is reexamined and largely solved using
	an exact exchange method. We have built an accurate optimized effective
	potential as the sum of a fixed potential and a linear combination
	of basis sets based on our direct optimization method. This effective
	potential properly develops a linear counteracting depolarization
	field, and it significantly improves recent results from approximate
	optimized potentials. The controversial case of hydrogen chains is
	now correctly described and the failure of the local density approach
	is attributed to the large self-interaction error in systems with
	a non-integer number of electrons. (C) 2003 American Institute of
	Physics.},
  endnotereftype = {Journal Article},
  issn = {0021-9606},
  shorttitle = {Accurate polymer polarizabilities with exact exchange density-functional
	theory},
  url = {<Go to ISI>://000186492900001}
}

@ARTICLE{Morrison90819,
  author = {Morrison, R. C. and Yang, W. T. and Parr, R. G. and Lee, C. T.},
  title = {Approximate Density-Matrices and Wigner Distribution-Functions from
	Density, Kinetic-Energy Density, and Idempotency Constraints},
  journal = {International Journal of Quantum Chemistry},
  year = {1990},
  volume = {38},
  pages = {819-830},
  number = {6},
  month = {Dec},
  endnotereftype = {Journal Article},
  isinote = {ISI Document Delivery No.: EL087 Times Cited: 2 Cited Reference Count:
	28},
  issn = {0020-7608},
  shorttitle = {Approximate Density-Matrices and Wigner Distribution-Functions from
	Density, Kinetic-Energy Density, and Idempotency Constraints},
  url = {<Go to ISI>://A1990EL08700004}
}

@ARTICLE{Moult:2007,
  author = {Moult, J. and Fidelis, K. and Kryshtafovych, A. and Rost, B. and
	Hubbard, T. and Tramontano, A.},
  title = {{Critical assessment of methods of protein structure prediction-Round
	VII.}},
  journal = {Proteins},
  year = {2007},
  volume = {69},
  pages = {3-9},
  number = {Suppl 8}
}

@ARTICLE{Moult:2005,
  author = {Moult, J. and Fidelis, K. and Rost, B. and Hubbard, T. and Tramontano,
	A.},
  title = {{Critical assessment of methods of protein structure prediction (CASP)--round
	6}},
  journal = {Proteins},
  year = {2005},
  volume = {61},
  pages = {3-7},
  number = {Suppl 7}
}

@ARTICLE{Moult:2003,
  author = {Moult, J. and Fidelis, K. and Zemla, A. and Hubbard, T.},
  title = {{Critical assessment of methods of protein structure prediction (CASP)-round
	V}},
  journal = {Proteins},
  year = {2003},
  volume = {53},
  pages = {334-339},
  number = {Suppl 6}
}

@ARTICLE{Moy:2000,
  author = {Moy, B. Corry, Ben and Kuyucak, Serdar and Chung, Shin-Ho},
  title = {Tests of continuum theories as models of ion channels. {I}. {Poisson-Boltzmann}
	theory versus {Brownian dynamics}},
  journal = {Biophys. J.},
  year = {2000},
  volume = {78},
  pages = {2349-2363},
  number = { }
}

@ARTICLE{LMu:2011a,
  author = {Mu, L. and Wang, J. and Wang, Y. and Ye, X.},
  title = {A Computational Study of the Weak {Galerkin} Method for Second-Order
	Elliptic Equations},
  journal = {arXiv:1111.0618v1},
  year = {2011}
}

@ARTICLE{LMu:2013a,
  author = {Mu, L. and Wang, J. and Wei, G. W. and Ye, X. and Zhao, S.},
  title = {Weak { Galerkin} method for second order elliptic interface problems},
  journal = {Journal of Computational Physics},
  year = {2013},
	volume = {250},
  pages = {106 - 125},
}

@ARTICLE{LMu:2011b,
  author = {Mu, L. and Wang, J. and Ye, X. and Zhao, S.},
  title = {A Numerical Study on the Weak {Galerkin} Method for the {Helmholtz}
	Equation with Large Wave Numbers},
  journal = {arXiv:1111.0671v1},
  year = {2011}
}

@ARTICLE{Mu:2003,
  author = {Mu, Y. and Kosov, D. S. and Stock, G.},
  title = {{Conformational Dynamics of Trialanine in Water. 2. Comparison of
	AMBER, CHARMM, GROMOS, and OPLS Force Fields to NMR and Infrared
	Experiments}},
  journal = {J Phys Chem B},
  year = {2003},
  volume = {107},
  pages = {5064-5073}
}

@ARTICLE{Mu:2007,
  author = {Mu, Yuguang and Yang, Ye and Xu, Weixin},
  title = {Hybrid Hamiltonian replica exchange molecular dynamics simulation
	method employing the {Poisson--Boltzmann} model},
  journal = {Journal of Chemical Physics},
  year = {2007},
  volume = {127},
  number = {8},
  abstract = {A hybrid Hamiltonian replica exchange molecular dynamics simulation
	scheme based on explicit water model hybrided with Poisson\&ndash;Boltzmann
	model is brought out. In this method the motions of atoms are governed
	by potential energy obtained from explicit water model. However,
	the exchanges between different replicas under different temperatures
	are controlled by the solvation energies of the solute calculated
	using the Poisson\&ndash;Boltzmann model. In order to get the correct
	canonical ensembles, the {van der Waals} radii, which are used to
	define the dielectric boundary, have to be optimized. The conformational
	spaces of three distinct pentapeptides, Met-enkephalin, alanine 5,
	and glycine 5, are explored. We find that with the optimized radii
	the structural ensembles are nearly identical to those obtained by
	standard replica exchange simulations while the number of replica
	needed is reduced greatly.
	
	 \&copy;2007 American Institute of Physics},
  bdsk-url-1 = {http://dx.doi.org/10.1063/1.2772264},
  bdsk-url-2 = {http://dx.doi.org/10.1063/1.2772264},
  date-added = {2008-09-16 14:25:52 -0500},
  date-modified = {2008-09-16 14:25:52 -0500},
  doi = {10.1063/1.2772264},
  keywords = {Electrostatics; Multiscale; Solvation},
  priority = {0},
  publisher = {AIP},
  url = {http://dx.doi.org/10.1063/1.2772264}
}

%  author = {Muench, S. P. and Huss, M. and Song, C. F. and Phillips, C. and Wieczorek,	H. and Trinick, J. and Harrison, M. A.},
@ARTICLE{Muench2009,
  author = {Muench, S. P. and Huss, M. and Song, C. F. and Phillips, C. and Wieczorek et al,	H. },
  title = {Cryo-electron microscopy of the vacuolar ATPase motor reveals its
	mechanical and regulatory complexity.},
  journal = {J Mol Biol},
  year = {2009},
  volume = {386},
  pages = {989-99--},
  number = {4},
  month = mar,
  abstract = {The vacuolar H+-ATPase (V-ATPase) is an ATP-driven rotary molecular
	motor that is a transmembrane proton pump in all eukaryotic cells.
	Although its activity is fundamental to many physiological processes,
	our understanding of the structure and mechanism of the V-ATPase
	is poor. Using cryo-electron microscopy of the tobacco hornworm (Manduca
	sexta) enzyme, we have calculated the first 3D reconstruction of
	the intact pump in its native state. The resolution of 16.5 A is
	significantly higher than that of previous cryo-electron microscopy
	models of either V-ATPase or the related F1F0-ATPase. A network of
	four stalk structures connecting the V1 catalytic domain and the
	V0 membrane domain is now fully resolved, demonstrating substantially
	greater complexity than that found in the F-ATPase. Three peripheral
	stator stalks connect these domains to a horizontal collar that partly
	encircles the region between V1 and V0. The fourth stalk is a central
	axle that connects to V0 but makes minimal contact with V1. Several
	subunit crystal structures can be fit accurately into the reconstruction.
	The model thus provides new insights into the organisation of key
	components involved in mechanical coupling between the domains and
	regulation of activity.},
  address = {Institute of Membrane and Systems Biology, Faculty of Biological
	Sciences, University of Leeds, LS2 9JT, UK.},
  comment = {Research Support, Non-U.S. Gov't,},
  keywords = {Animals, Catalytic Domain, Cryoelectron Microscopy, Image Processing,
	Computer-Assisted, Manduca, Models, Molecular, Molecular Motor Proteins,
	Protein Subunits, Vacuolar Proton-Translocating ATPases},
  owner = {SeanLab},
  timestamp = {2012.05.23},
  url = {http://ukpmc.ac.uk/abstract/MED/19244615}
}

@ARTICLE{Mukherjee:2010(a),
  author = {Mukherjee, S. and Szilagyi, A. and Roy, A. and Zhang, Y.},
  title = {{Genome-wide protein structure prediction}},
  journal = {In: Kolniski A, editor. Multiscale approaches to protein modeling:
	structure prediction, dynamics, thermodynamics and macromolecular
	assemblies},
  year = {2010},
  pages = {810-842}
}

@ARTICLE{Mukherjee:2010(b),
  author = {Mukherjee, S. and Wu, S. and Zhang, Y.},
  title = {{Protein-protein complex structure predictions by multimeric threading
	and template recombination}},
  journal = {Proc Natl Acad Sci USA},
  year = {2010:Submitted.}
}

@ARTICLE{sloan91,
  author = {Mulholland, L. S. and Sloan, D. M.},
  title = {he effect of filtering on the pseudospectral solution of evolutionary
	partial differential equation},
  journal = {J. Comput. Phys.},
  year = {1991},
  volume = {96},
  pages = {369-390 }
}

@ARTICLE{MCPT09,
  author = {Patrick Mullen and Keenan Crane and Dmitry Pavlov and Yiying Tong
	and Mathieu Desbrun},
  title = {Energy-Preserving Integrators for Fluid Animation},
  journal = {ACM Trans. on Graph. (SIGGRAPH)},
  year = {submitted}
}

@ARTICLE{MMPT09,
  author = {P. Mullen and A. McKenzie and D. Pavlov and Y. Tong and E. Kanso
	and J. E. Marsden and M. Desbrun},
  title = {Discrete Lie Advection of Differential $k$-Forms},
  journal = {Foundations of Computational Mathematics},
  year = {submitted}
}

@ARTICLE{MMTD07,
  author = {Patrick Mullen and Alexander McKenzie and Yiying Tong and Mathieu
	Desbrun},
  title = {A Variational Approach to Eulerian Geometry Processing},
  journal = {ACM Trans. on Graphics (SIGGRAPH)},
  year = {2007},
  pages = {66},
  month = jul
}

@ARTICLE{MTAD08,
  author = {Patrick Mullen and Yiying Tong and Pierre Alliez and Mathieu Desbrun},
  title = {Spectral Conformal Parameterization},
  journal = {Computer Graphics Forum (Symposium of Geometry Processing)},
  year = {2008},
  month = Jul
}

@ARTICLE{Mulliken:1955,
  author = { Mulliken, R. S.},
  title = {Electronic population analysis on LCAOMO [linear combination of atomic
	orbital-molecular orbital] molecular wave functions},
  journal = {I. J. Chem. Phys.},
  year = {1955},
  volume = {23},
  pages = {1833-1840}
}

@ARTICLE{Mumford:1989,
  author = {David Mumford and Jayant Shah},
  title = {Optimal approximations by piecewise smooth functions and associated
	variational problems},
  journal = {Communications on Pure and Applied Mathematics},
  year = {1989},
  volume = {42},
  pages = {577-685},
  number = {5},
  abstract = {No Abstract.},
  bdsk-url-1 = {http://dx.doi.org/10.1002/cpa.3160420503},
  date = {1989 %@ 1097-0312 %+ Harvard University; Northeastern University},
  date-added = {2008-09-16 14:43:24 -0500},
  date-modified = {2008-09-16 14:43:24 -0500},
  doi = {10.1002/cpa.3160420503},
  keywords = {Mathematics},
  refer1 = {10.1002/cpa.3160420503},
  url = {http://dx.doi.org/10.1002/cpa.3160420503}
}

@ARTICLE{Murdoch1997,
  author = {Murdoch, P},
  title = {{The spatial twist continuum: A connectivity based method for representing
	all-hexahedral finite element meshes}},
  journal = {Finite Elements in Analysis and Design},
  year = {1997},
  volume = {28},
  pages = {137--149},
  number = {2},
  doi = {10.1016/S0168-874X(97)81956-7},
  issn = {0168874X},
  url = {http://linkinghub.elsevier.com/retrieve/pii/S0168874X97819567}
}

@ARTICLE{LSSEO,
  author = {Museth, K. and Breen, D. and Whitaker, R. and Barr, A.},
  title = {{Level Set Surface Editing Operators}},
  journal = {ACM Trans. on Graphics},
  year = {2002},
  volume = {21},
  pages = {330--338},
  number = {3}
}

@BOOK{Museth:LSM:2002,
  title = {Level set surface editing operators},
  year = {2002},
  author = {Museth, K. and Breen, D. E. and Whitaker, R. T. and Barr, A. H. },
  volume = {21},
  number = {3},
  pages = {330--338},
  booktitle = {ACM Trans. on Graphics (SIGGRAPH)}
}

@ARTICLE{Nadler:2003,
  author = {Nadler, Boza and Hollerbach, Uwe and Eisenberg, B. S.},
  title = {Dielectric boundary force and its crucial role in {Gramicidin}},
  journal = {Physical Review E},
  year = {2003},
  volume = {68},
  pages = {1-9},
  number = { }
}

@ARTICLE{DiffusionMaps,
  author = {B. Nadler and S. Lafon and R.R. Coifman and I.G. Kevrekidis},
  title = {Diffusion Maps, Spectral Clustering and Reaction Coordinate of Dynamical
	Systems},
  year = {2006},
  volume = {21},
  pages = {113--127},
  booktitle = {Applied and Computational Harmonic Analysis--Special issue on Diffusion
	Maps and Wavelets}
}

@ARTICLE{Nagle:1978,
  author = {Nagle, J. F. and Morowitz, H. J.},
  title = {Molecular Mechanisms for Proton Transport in Membranes},
  journal = {Proc. Natl. Acad. Sci. U.S.A},
  year = {1978},
  volume = {1458},
  pages = {298-302},
  number = {72 }
}

@ARTICLE{Natori:1994,
  author = {Natori, K.},
  title = {Ballistic metal-oxide-semiconductor field effect transistor},
  journal = {J. Appl. Phys.},
  year = {1994},
  pages = {4879-4890},
  annote = {Ballistic metal-oxide-semiconductor field effect transistor},
  date-added = {2008-11-25 10:28:56 -0500},
  date-modified = {2008-11-25 10:28:56 -0500},
  ty = {JOUR}
}

@ARTICLE{Neidigh:2002,
  author = {Neidigh, J. W. and Fesinmeyer, R. M. and Andersen, N. H. },
  title = {Designing a 20-residue protein},
  journal = {Nat. Struct. Biol.},
  year = {2002},
  volume = {9},
  pages = {425-430},
  number = { }
}

@ARTICLE{Neria:1996,
  author = {Neria, E. and Fischer, S. and Karplus, M.},
  title = {{Simulation of activation free energies in molecular systems}},
  journal = {J Chem Phys},
  year = {1996},
  volume = {105},
  pages = {1902-1921},
  number = {5}
}

@ARTICLE{Tadmor,
  author = {Nessyahu, H. and Tadmor, E.},
  title = { Non-oscillation central differencing for hyperbolic conservation
	laws},
  journal = {J. Comput. Phys.},
  year = {1990},
  volume = {87},
  pages = {408-463}
}

@ARTICLE{Netz:2000a,
  author = {Netz, R. R. and Orland, H.},
  title = {Beyond {{Poisson-Boltzmann}}: Fluctuation effects and correlation
	functions},
  journal = {European Physical Journal E},
  year = {2000},
  volume = {1},
  pages = {203-14},
  number = {2-3},
  abstract = {We formulate the exact non-linear field theory for a fluctuating counter-ion
	distribution in the presence of a fixed, arbitrary charge distribution.
	The {Poisson-Boltzmann} equation is obtained as the saddle-point
	of the field-theoretic action, and the effects of counter-ion fluctuations
	are included by a loop-wise expansion around this saddle point. The
	Poisson equation is obeyed at each order in this loop expansion.
	We explicitly give the expansion of the Gibbs potential up to two
	loops. We then apply our field-theoretic formalism to the case of
	a single impenetrable wall with counter ions only (in the absence
	of salt ions). We obtain the fluctuation corrections to the electrostatic
	potential and the counter-ion density to one-loop order without further
	approximations. The relative importance of fluctuation corrections
	is controlled by a single parameter, which is proportional to the
	cube of the counter-ion valency and to the surface charge density.
	The effective interactions and correlation functions between charged
	particles close to the charged wall are obtained on the one-loop
	level.},
  bdsk-url-1 = {http://dx.doi.org/10.1007/s101890050023},
  date-added = {2008-09-01 14:00:31 -0500},
  date-modified = {2008-09-01 14:00:31 -0500},
  keywords = {Electrostatics; StatisticalMechanics; BeyondMeanField},
  url = {http://dx.doi.org/10.1007/s101890050023}
}

@ARTICLE{Newman:1999,
  author = {Newman, M. E. J. and Barkema, G. T.},
  title = {{Monte Carlo Methods in Statistical Physics}},
  journal = {Clarendon Press, Oxford},
  year = {1999}
}

@INPROCEEDINGS{eigenmultigridsolver,
  author = {Klaus Neymeyr},
  title = {Solving Mesh Eigenproblems with Multigrid Efficiency},
  booktitle = {Numerical Methods for Scientific Computing: Variational Problems
	and Applications},
  year = {2003},
  editor = {Y. Kuznetsov and P. Neittaanmaki and O. Pironneau}
}

@ARTICLE{Ngo:2008,
  author = {Ngo, Jacky C. and Huang, Mingdong and Roth, David A. and Furie, Barbara
	C. and Furie, Bruce },
  title = {Crystal Structure of Human Factor {VIII}: Implications for the Formation
	of the Factor {IXa}-Factor {VIIIa} Complex},
  journal = {Structure},
  year = {2008},
  volume = {16},
  pages = {597--606},
  number = {4},
  abstract = {Summary Factor VIII is a procofactor that plays a critical role in
	blood coagulation, and is missing or defective in hemophilia A. We
	determined the X-ray crystal structure of B domain-deleted human
	factor VIII. This protein is composed of five globular domains and
	contains one Ca2+ and two Cu2+ ions. The three homologous A domains
	form a triangular heterotrimer where the A1 and A3 domains serve
	as the base and interact with the C2 and C1 domains, respectively.
	The structurally homologous C1 and C2 domains reveal membrane binding
	features. Based on biochemical studies, a model of the factor IXa-factor
	VIIIa complex was constructed by in silico docking. Factor IXa wraps
	across the side of factor VIII, and an extended interface spans the
	factor VIII heavy and light chains. This model provides insight into
	the activation of factor VIII and the interaction of factor VIIIa
	with factor IXa on the membrane surface.},
  bdsk-url-1 = {http://dx.doi.org/10.1016/j.str.2008.03.001},
  bdsk-url-2 = {http://dx.doi.org/10.1016/j.str.2008.03.001},
  date-added = {2008-09-15 09:57:13 -0500},
  date-modified = {2008-09-15 09:57:13 -0500},
  doi = {10.1016/j.str.2008.03.001},
  keywords = {APBS, Structure},
  posted-at = {2008-04-18 13:40:34},
  priority = {0},
  url = {http://dx.doi.org/10.1016/j.str.2008.03.001}
}

@ARTICLE{Ni965732,
  author = {Ni, H. H. and York, D. M. and Bartolotti, L. and Wells, R. L. and
	Yang, W. T.},
  title = {Density-functional study of the geometries, stabilities, and bond
	energies of group {III-V} (13-15) four-membered-ring compounds},
  journal = {Journal of the American Chemical Society},
  year = {1996},
  volume = {118},
  pages = {5732-5736},
  number = {24},
  month = {Jun},
  abstract = {A theoretical investigation has been carried out on several group
	III-V (13-15) four-membered-ring compounds which, if experimentally
	attainable, are potentially useful as precursors to nanocrystalline
	electronic and semiconductor materials. Four-membered-ring compounds
	considered in this study have core structures of the following form:
	MEM'E' and MEMX (M, M' = In, Ga, Al; E, E' = P, As; X = Cl, Br).
	Equilibrium geometries, binding energies, and bond energies were
	determined based on local density approximation (LDA) and gradient-corrected
	density-functional methods. Optimized ring geometries obtained with
	LDA agree closely with single-crystal X-ray crystallographic structures
	of known compounds with the same four-membered-ring cores. The following
	trends in bond energies are observed: M-Cl much greater than M-P
	> M-As much greater than M-Br (M = In, Ga, Al), and Al-Y > Ga-Y >
	In-Y (Y = P, As, Cl, Br). Although only one M-Br-containing mixed-bridge
	four-membered-ring compound has been reported and no such Al-Cl-containing
	mixed-bridge species have yet been synthesized, our calculations
	suggest that compounds containing these two ring systems are stable.},
  endnotereftype = {Journal Article},
  issn = {0002-7863},
  shorttitle = {Density-functional study of the geometries, stabilities, and bond
	energies of group III-V (13-15) four-membered-ring compounds},
  url = {<Go to ISI>://A1996UR83900026}
}

@ARTICLE{Nicholls:2008,
  author = {Nicholls, Anthony and Mobley, David L. and Guthrie, Peter J. and
	Chodera, John D. and Pande, Vijay S. },
  title = {Predicting Small-Molecule Solvation Free Energies: An Informal Blind
	Test for Computational Chemistry},
  journal = {Journal of Medicinal Chemistry},
  year = {2008},
  volume = {51},
  pages = {769-79},
  number = {4},
  abstract = {Abstract: Experimental data on the transfer of small molecules between
	vacuum and water are relatively sparse. This makes it difficult to
	assess whether computational methods are truly predictive of this
	important quantity or merely good at explaining what has been seen.
	To explore this, a prospective test was performed of two different
	methods for estimating solvation free energies: an implicit solvent
	approach based on the PoissonBoltzmann equation and an explicit
	solvent approach using alchemical free energy calculations. For a
	set of 17 small molecules, root mean square errors from experiment
	were between 1.3 and 2.6 kcal/mol, with the explicit solvent free
	energy approach yielding somewhat greater accuracy but at greater
	computational expense. Insights from outliers and suggestions for
	future prospective challenges of this kind are presented.},
  address = {OpenEye Scientific Software, Inc., Santa Fe, New Mexico 87508, Department
	of Pharmaceutical Chemistry, University of California, San Francisco,
	California 94143, Department of Chemistry, University of Western
	Ontario, London, Ontario, Canada N6A 5B7, and Department of Chemistry,
	Stanford University, Stanford, California 94305},
  bdsk-url-1 = {http://dx.doi.org/10.1021%5C/jm070549%5C+},
  bdsk-url-2 = {http://dx.doi.org/10.1021/jm070549+},
  date-added = {2008-06-29 15:02:22 -0500},
  date-modified = {2008-06-29 15:02:22 -0500},
  doi = {10.1021/jm070549+},
  keywords = {electrostatics, nonpolar, solvation},
  priority = {0},
  url = {http://dx.doi.org/10.1021\%2Fjm070549\%2B}
}

@ARTICLE{Nielsen:1999,
  author = {Nielsen, J. E. and Andersen, K. V. and Honig, B. and Hooft, R. W.
	W. and Klebe, G. and Vriend, G. and Wade, R. C.},
  title = {Improving macromolecular electrostatics calculations},
  journal = {Protein Engineering},
  year = {1999},
  volume = {12},
  pages = {657-662},
  number = {8},
  abstract = {Electrostatic interactions play a key role in many aspects of protein
	engineering. Consequently, much effort has been put into the design
	of software for calculating electrostatic fields around macromolecules.
	We show that optimization of hydrogen bonding networks can improve
	both the results of pKa calculations and the results of electrostatic
	calculations performed by commonly used programs such as DelPhi.
	Further optimization can often be achieved by flipping the side chains
	of asparagine, histidine and glutamine around their 2, 2 and 3 torsion
	angles, respectively, when this improves the local hydrogen bonding
	network. These optimizations are applied to some well characterized
	proteins: BPTI, hen egg white lysozyme and superoxide dismutase.
	A search for flipped residues in the PDB revealed that significant
	improvements in electrostatic calculations in or near the active
	site of enzymes can be expected for about one quarter of all enzymes
	in the PDB.},
  address = {European Mol Biol Lab Heidelberg Germany D-69117 Vriend, G Vriend,
	G vriend@embl-heidelberg.de European Mol Biol Lab Heidelberg Germany
	D-69117 Novo Nordisk AS Bagsvaerd Denmark DK-2880 Columbia Univ New
	York, NY USA 10032 Nonius BV Delft Netherlands Univ Marburg Marburg
	Germany D-35032},
  annote = {Improving macromolecular electrostatics calculations; AUG},
  bdsk-url-1 = {http://protein.oupjournals.org/cgi/content/full/12/8/657},
  date-added = {2008-09-01 13:52:47 -0500},
  date-modified = {2008-09-01 13:52:47 -0500},
  journal1 = {Protein Eng},
  keywords = {Electrostatics},
  ty = {JOUR},
  url = {http://protein.oupjournals.org/cgi/content/full/12/8/657}
}

@ARTICLE{Nielsen:2003a,
  author = {Nielsen, J. E. and McCammon, J. A.},
  title = {On the evaluation and optimization of protein X-ray structures for
	pKa calculations},
  journal = {Protein Sci},
  year = {2003},
  volume = {12},
  pages = {313-26},
  number = {2},
  abstract = {The calculation of the physical properties of a protein from its X-ray
	structure is of importance in virtually every aspect of modern biology.
	Although computational algorithms have been developed for calculating
	everything from the dynamics of a protein to its binding specificity,
	only limited information is available on the ability of these methods
	to give accurate results when used with a particular X-ray structure.
	We examine the ability of a pKa calculation algorithm to predict
	the proton-donating residue in the catalytic mechanism of hen egg
	white lysozyme. We examine the correlation between the ability of
	the pKa calculation method to obtain the correct result and the overall
	characteristics of 41 X-ray structures such as crystallization conditions,
	resolution, and the output of structure validation software. We furthermore
	examine the ability of energy minimizations (EM), molecular dynamics
	(MD) simulations, and structure-perturbation methods to optimize
	the X-ray structures such that these give correct results with the
	pKa calculation algorithm. We propose a set of criteria for identifying
	the proton donor in a catalytic mechanism, and demonstrate that the
	application of these criteria give highly accurate prediction results
	when using unmodified X-ray structures. More specifically, we are
	able to successfully identify the proton donor in 85{\%} of the X-ray
	structures when excluding structures with crystal contacts near the
	active site. Neither the use of the overall characteristics of the
	X-ray structures nor the optimization of the structure by EM, MD,
	or other methods improves the results of the pKa calculation algorithm.
	We discuss these results and their implications for the design of
	structure-based energy calculation algorithms in general.},
  address = {Howard Hughes Medical Institute and Department of Chemistry and Biochemistry,
	Department of Pharmacology, University of California, San Diego,
	La Jolla, California 92093, USA.},
  annote = {Feb; On the evaluation and optimization of protein X-ray structures
	for pKa calculations; 12538895; *; A description of state-of-the-art
	methods to using PB calculations to calculate pKa's of titratable
	residues in proteins. Interestingly, unlike the work of Georgescu
	et al. (see reference), Nielsen and McCammon find that the inclusion
	of flexibility does not improve the accuracy of the calculations.},
  bdsk-url-1 = {http://www.ncbi.nlm.nih.gov/entrez/query.fcgi?cmd=Retrieve&db=PubMed&dopt=Citation&list_uids=12538895},
  date-added = {2008-06-29 15:07:59 -0500},
  date-modified = {2008-06-29 15:07:59 -0500},
  keywords = {Electrostatics},
  ty = {JOUR},
  url = {http://www.ncbi.nlm.nih.gov/entrez/query.fcgi?cmd=Retrieve&db=PubMed&dopt=Citation&list_uids=12538895}
}

@ARTICLE{Nielsen:2001,
  author = {Nielsen, J. E. and Vriend, G.},
  title = {Optimizing the hydrogen-bond network in {{Poisson-Boltzmann}} equation-based
	{pK(a)} calculations},
  journal = {Proteins},
  year = {2001},
  volume = {43},
  pages = {403-412},
  number = {4},
  abstract = {pKa calculation methods that are based on finite difference solutions
	to the {Poisson-Boltzmann} equation (FDPB) require that energy calculations
	be performed for a large number of different protonation states of
	the protein. Normally, the differences between these protonation
	states are modeled by changing the charges on a few atoms, sometimes
	the differences are modeled by adding or removing hydrogens, and
	in a few cases the positions of these hydrogens are optimized locally.
	We present an FDPB-based pKa calculation method in which the hydrogen-bond
	network is globally optimized for every single protonation state
	used. This global optimization gives a significant improvement in
	the accuracy of calculated pKa values, especially for buried residues.
	It is also shown that large errors in calculated pKa values are often
	due to structural artifacts induced by crystal packing. Optimization
	of the force fields and parameters used in pKa calculations should
	therefore be performed with X-ray structures that are corrected for
	crystal artifacts. Proteins 2001;43:403-412. Ã‚Â??001 Wiley-Liss,
	Inc.},
  address = {European Mol Biol Lab Heidelberg Germany D-69117 Nielsen, JE nielsen{\char64}embl-heidelberg.de
	Meyerhofstr 1 European Mol Biol Lab Heidelberg Germany D-69117},
  annote = {Optimizing the hydrogen-bond network in {Poisson-Boltzmann} equation-based
	pK(a) calculations; JUN 1},
  bdsk-file-1 = {YnBsaXN0MDDUAQIDBAUGCQpYJHZlcnNpb25UJHRvcFkkYXJjaGl2ZXJYJG9iamVjdHMSAAGGoNE
	HCFRyb290gAFfEA9OU0tleWVkQXJjaGl2ZXKoCwwXGBkdJCVVJG51bGzTDQ4PEBEUViRjbGFzc1
	dOUy5rZXlzWk5TLm9iamVjdHOAB6ISE4ACgAOiFRaABIAGWWFsaWFzRGF0YVxyZWxhdGl2ZVBhd
	GjSDRobHFdOUy5kYXRhgAVPEQHGAAAAAAHGAAIAAAxNYWNpbnRvc2ggSEQAAAAAAAAAAAAAAAAA
	AADD4v5NSCsAAAAZYksWMjAwMS1OaWVsc2VuVnJpZW5kLnBkZgAAAAAAAAAAAAAAAAAAAAAAAAA
	AAAAAAAAAAAAAAAAAAAAAAAAAAAAAABlipMQP6GUAAAAAAAAAAAAEAAQAAAkgAAAAAAAAAAAAAA
	AAAAAAB0FyY2hpdmUAABAACAAAw+NSrQAAABEACAAAxBAutQAAAAEAFAAZYksAGWIDAAqkKAAKp
	BEAAHrcAAIATE1hY2ludG9zaCBIRDpVc2VyczpiYWtlcjpEb2N1bWVudHM6UmVmZXJlbmNlczpB
	cmNoaXZlOjIwMDEtTmllbHNlblZyaWVuZC5wZGYADgAuABYAMgAwADAAMQAtAE4AaQBlAGwAcwB
	lAG4AVgByAGkAZQBuAGQALgBwAGQAZgAPABoADABNAGEAYwBpAG4AdABvAHMAaAAgAEgARAASAD
	9Vc2Vycy9iYWtlci9Eb2N1bWVudHMvUmVmZXJlbmNlcy9BcmNoaXZlLzIwMDEtTmllbHNlblZya
	WVuZC5wZGYAABMAAS8AABUAAgAM//8AANIeHyAhWCRjbGFzc2VzWiRjbGFzc25hbWWjISIjXU5T
	TXV0YWJsZURhdGFWTlNEYXRhWE5TT2JqZWN0XxA/Li4vLi4vLi4vLi4vRG9jdW1lbnRzL1JlZmV
	yZW5jZXMvQXJjaGl2ZS8yMDAxLU5pZWxzZW5WcmllbmQucGRm0h4fJieiJyNcTlNEaWN0aW9uYX
	J5AAgAEQAaAB8AKQAyADcAOgA/AEEAUwBcAGIAaQBwAHgAgwCFAIgAigCMAI8AkQCTAJ0AqgCvA
	LcAuQKDAogCkQKcAqACrgK1Ar4DAAMFAwgAAAAAAAACAQAAAAAAAAAoAAAAAAAAAAAAAAAAAAAD
	FQ==},
  bdsk-url-1 = {http://www3.interscience.wiley.com/cgi-bin/abstract/78505732/ABSTRACT},
  date-added = {2008-09-01 13:51:58 -0500},
  date-modified = {2008-09-01 13:51:58 -0500},
  journal1 = {Protein-Struct Funct Genet},
  keywords = {Electrostatics},
  ty = {JOUR},
  url = {http://www3.interscience.wiley.com/cgi-bin/abstract/78505732/ABSTRACT}
}

@ARTICLE{Nilges:1991,
  author = {Nilges, M. and Brunger, A. T.},
  title = {{Automated modeling of coiled coils: application to the GCN4 dimerization
	region}},
  journal = {Protein Eng},
  year = {1991},
  volume = {4},
  pages = {649-659},
  number = {6}
}

@ARTICLE{Nina:1997,
  author = {Nina, M. and Beglov, D. and Roux, B. },
  title = {Atomic radii for continuum electrostatics calculations based on molecular
	dynamics free energy simulations},
  journal = {J. Phys. Chem. B},
  year = {1997},
  volume = {101},
  pages = {5239-5248},
  number = { }
}

@ARTICLE{Nina:1999,
  author = {Nina, M. and Im, W. and Roux, B.},
  title = {Optimized atomic radii for protein continuum electrostatics solvation
	forces},
  journal = {Biophysical Chemistry},
  year = {1999},
  volume = {78},
  pages = {89-96},
  number = {1-2},
  abstract = {Recently, we presented a Green's function approach for the calculation
	of analytic continuum electrostatic solvation forces based on numerical
	solutions of the finite-difference Poisson-Botzmann (FDPB) equation
	{$[$}Im et al., Comp. Phys. Comm. 111(1998) 59{$]$}. In this treatment
	the analytic forces were explicitly defined as the first derivative
	of the FDPB continuum electrostatic free energy with respect to the
	coordinates of the solute atoms. A smooth intermediate region for
	the solute-solvent dielectric boundary needed to be introduced to
	avoid abrupt discontinuous variations in the solvation free energy
	and forces as a function of the atomic positions. In the present
	paper we extend the set of optimized radii, which was previously
	parametrized from molecular dynamics free energy simulations of the
	20 standard amino acids with explicit solvent molecules {$[$}Nina
	et al., J. Phys. Chem. 101 (1997) 5239{$]$}, to yield accurate solvation
	free energy by taking the influence of the smoothed dielectric region
	into account. (C) 1999 Elsevier Science B.V. All rights reserved.},
  address = {Roux, B. Univ Montreal, Dept Phys \& chem, CP 6128,Succ,Ctr Ville,
	Montreal, PQ H3C 3J7, Canada Univ Montreal, Dept Phys \& chem, Montreal,
	PQ H3C 3J7, Canada},
  annote = {APR 5; Optimized atomic radii for protein continuum electrostatics
	solvation forces; ISI:000080041100007},
  bdsk-url-1 = {http://dx.doi.org/10.1016/S0301-4622(98)00236-1},
  date-added = {2008-09-16 14:31:07 -0500},
  date-modified = {2008-09-16 14:31:07 -0500},
  journal1 = {Biophys Chem},
  keywords = {Electrostatics; MolecularDynamics},
  ty = {JOUR},
  url = {http://dx.doi.org/10.1016/S0301-4622(98)00236-1}
}

@ARTICLE{zien98,
  author = {Nithiarasu, P. and Zienkiewicz, O. C. and Sai, B. V. K. S. and Morgan,
	K. and Codina, R. and Vazquez, M.},
  title = {Shock capturing viscosities for the general fluid mechanics algorithm},
  journal = {Int. J. Numer. Meth. Fluids},
  year = {1998},
  volume = {28},
  pages = {1325-1353}
}

@ARTICLE{Noble:2005,
  author = {le Noble, F. and Fleury, V. and Pries, A. and Corvol, P. and Eichmann,
	A. and Reneman, R. S.},
  title = {Control of arterial branching morphogenesis in embryogenesis: go
	with the flow},
  journal = {Eur. Phys. J. Appl. Phys.},
  year = {2005},
  volume = {65},
  pages = {619-628 },
  number = { }
}

@ARTICLE{Nottale:2008,
  author = {Nottale, L. and Auffray, C.},
  title = {Scale relativity theory and integrative systems biology: 2 Macroscopic
	quantum-type mechanics },
  journal = {Prog. Biophy. Mole. Biol.},
  year = {2008},
  volume = {97},
  pages = {115-157}
}

@INPROCEEDINGS{obrien:2001:SSP,
  author = {James F. O'Brien and Perry R. Cook and Georg Essl},
  title = {Synthesizing sounds from physically based motion},
  booktitle = {Proceedings of ACM SIGGRAPH 2001},
  year = {2001},
  pages = {529--536},
  month = aug
}

@ARTICLE{Oevermann:2006,
  author = {Oevermann, M. and Klein, R.},
  title = {A Cartesian grid finite volume method for elliptic equations with
	variable coefficients and embedded interfaces},
  journal = {J. Comput. Phys. },
  year = {2006},
  volume = {219},
  pages = {749-769},
  annote = {A Cartesian grid finite volume method for elliptic equations with
	variable coefficients and embedded interfaces},
  date-added = {2008-09-19 10:28:56 -0500},
  date-modified = {2008-09-19 10:28:56 -0500},
  ty = {JOUR}
}

@ARTICLE{YJOh:2009,
  author = {Oh, Y. J. and Garcia, A. L. and Petsev, D. N. and Lopez, G. P. and
	Brueck, S. R. J. and Ivory, C. F. and Han, S. M. },
  title = {Effect of wall-molecule interactions on electrokinetic transport
	of charged molecules in nanofluidic channels during FET flow control},
  journal = { Lab on a Chip },
  year = {2009},
  volume = {9},
  pages = {1601-1608 }
}

@ARTICLE{Okur:2006,
  author = {Okur, A. and Wickstrom, L. and Layten, M. and Geney, R. and Song,
	K. and Hornak, V. and Simmerling, C. },
  title = {Improved Efficiency of Replica Exchange Simulations through Use of
	a Hybrid Explicit/Implicit Solvation Model},
  journal = {Journal of Chemical Theory and Computation},
  year = {2006},
  volume = {2},
  pages = {420--433},
  number = {2},
  abstract = {Abstract: The use of parallel tempering or replica exchange molecular
	dynamics (REMD) simulations has facilitated the exploration of free
	energy landscapes for complex molecular systems, but application
	to large systems is hampered by the scaling of the number of required
	replicas with increasing system size. Use of continuum solvent models
	reduces system size and replica requirements, but these have been
	shown to provide poor results in many cases, including overstabilization
	of ion pairs and secondary structure bias. Hybrid explicit/continuum
	solvent models can overcome some of these problems through an explicit
	representation of water molecules in the first solvation shells,
	but these methods typically require restraints on the solvent molecules
	and show artifacts in water properties due to the solvation interface.
	We propose an REMD variant in which the simulations are performed
	with a fully explicit solvent, but the calculation of exchange probability
	is carried out using a hybrid model, with the solvation shells calculated
	on the fly during the fully solvated simulation. The resulting reduction
	in the perceived system size in the REMD exchange calculation provides
	a dramatic decrease in the computational cost of REMD, while maintaining
	a very good agreement with results obtained from the standard explicit
	solvent REMD. We applied several standard and hybrid REMD methods
	with different solvent models to alanine polymers of 1, 3, and 10
	residues, obtaining ensembles that were essentially independent of
	the initial conformation, even with explicit solvation. Use of only
	a continuum model without a shell of explicit water provided poor
	results for Ala3 and Ala10, with a significant bias in favor of the
	-helix. Likewise, using only the solvation shells and no continuum
	model resulted in ensembles that differed significantly from the
	standard explicit solvent data. Ensembles obtained from hybrid REMD
	are in very close agreement with explicit solvent data, predominantly
	populating polyproline II conformations. Inclusion of a second shell
	of explicit solvent was found to be unnecessary for these peptides.},
  address = {Department of Chemistry, Graduate Program in Biochemistry and Structural
	Biology, Graduate Program in Molecular and Cellular Biology, and
	Center for Structural Biology, Stony Brook University, Stony Brook,
	New York 11794, and Computational Science Center, Brookhaven National
	Laboratory, Upton, New York 11973},
  bdsk-url-1 = {http://dx.doi.org/10.1021/ct050196z},
  bdsk-url-2 = {http://dx.doi.org/10.1021/ct050196z},
  date-added = {2008-09-15 10:08:43 -0500},
  date-modified = {2008-09-15 10:08:43 -0500},
  doi = {10.1021/ct050196z},
  keywords = {MolecularDynamics, MolecularSimulation, Solvation},
  priority = {0},
  url = {http://dx.doi.org/10.1021/ct050196z}
}

@ARTICLE{Olsson1,
  author = {Elin Olsson and Gunilla Kreiss},
  title = {{A Conservative Level Set Method for Two Phase Flow}},
  journal = {J. Comput. Phys.},
  year = {2005},
  volume = {210},
  pages = {225--246},
  number = {1}
}

@ARTICLE{Onufriev:2000,
  author = {Onufriev, A. and Bashford, D. and Case, D. A.},
  title = {Modification of the generalized {Born} model suitable for macromolecules},
  journal = {Journal of Physical Chemistry B},
  year = {2000},
  volume = {104},
  pages = {3712-3720},
  number = {15},
  abstract = {The analytic generalized Born approximation is an efficient electrostatic
	model that describes molecules in solution. Here it is modified to
	permit a more accurate description of large macromolecules, while
	its established performance on small compounds is nearly unaffected.
	The modified model is also adapted to describe molecules with an
	interior dielectric constant not equal to unity. The model is tested
	by computations of pK shifts for a number of titratable residues
	in lysozyme, myoglobin, and bacteriorhodopsin. In general, except
	for some deeply buried residues of bacteriorhodopsin, the results
	show reasonable agreement with both experimental data and calculations
	based on numerical solution of the {Poisson-Boltzmann} equation.
	A very close agreement between the two models is obtained in an application
	to the prediction of the pK shifts associated with conformational
	change. The calculations based on this version of the generalized
	Born approximation are much faster than finite difference solutions
	of the {Poisson-Boltzmann} equation, which makes the present method
	useful for a variety of other applications where computational time
	is a critical factor. The model may also be integrated into molecular
	dynamics programs to replace explicit solvent simulations which are
	particularly time-consuming for large molecules.},
  address = {Scripps Clin \& Res Inst La Jolla, CA USA 92037 Case, DA Dept Mol
	Biol Case, DA case@scripps.edu Scripps Clin \& Res Inst La Jolla,
	CA USA 92037 Dept Mol Biol},
  annote = {Modification of the generalized Born model suitable for macromolecules;
	APR 20},
  bdsk-url-1 = {http://dx.doi.org/10.1021/jp994072s},
  date-added = {2008-09-01 13:59:03 -0500},
  date-modified = {2008-09-01 13:59:03 -0500},
  journal1 = {J Phys Chem B},
  keywords = {Electrostatics; Solvation},
  ty = {JOUR},
  url = {http://dx.doi.org/10.1021/jp994072s}
}

@ARTICLE{Onufriev:2002,
  author = {Onufriev, A. and Case, D. A. and Bashford, D.},
  title = {Effective {Born} radii in the generalized {Born} approximation: the
	importance of being perfect},
  journal = {Journal of Computational Chemistry},
  year = {2002},
  volume = {23},
  pages = {1297-304},
  number = {14},
  abstract = {Generalized Born (GB) models provide, for many applications, an accurate
	and computationally facile estimate of the electrostatic contribution
	to aqueous solvation. The GB models involve two main types of approximations
	relative to the Poisson equation (PE) theory on which they are based.
	First, the self-energy contributions of individual atoms are estimated
	and expressed as {\tt{}"{}}effective Born radii.{\tt{}"{}} Next,
	the atom-pair contributions are estimated by an analytical function
	f(GB) that depends upon the effective Born radii and interatomic
	distance of the atom pairs. Here, the relative impacts of these approximations
	are investigated by calculating {\tt{}"{}}perfect{\tt{}"{}} effective
	Born radii from PE theory, and enquiring as to how well the atom-pairwise
	energy terms from a GB model using these perfect radii in the standard
	f(GB) function duplicate the equivalent terms from PE theory. In
	tests on several biological macromolecules, the use of these perfect
	radii greatly increases the accuracy of the atom-pair terms; that
	is, the standard form of f(GB) performs quite well. The remaining
	small error has a systematic and a random component. The latter cannot
	be removed without significantly increasing the complexity of the
	GB model, but an alternative choice of f(GB) can reduce the systematic
	part. A molecular dynamics simulation using a perfect-radii GB model
	compares favorably with simulations using conventional GB, even though
	the radii remain fixed in the former. These results quantify, for
	the GB field, the importance of getting the effective Born radii
	right; indeed, with perfect radii, the GB model gives a very good
	approximation to the underlying PE theory for a variety of biomacromolecular
	types and conformations.},
  address = {Department of Molecular Biology, The Scripps Research Institute,
	10550 N. Torrey Pines Rd., La Jolla, California 92037, USA.},
  annote = {Nov 15; Effective Born radii in the generalized Born approximation:
	the importance of being perfect; 12214312; OnufrievPerfect; A systematic
	comparison of generalized Born and Poisson treatments presented to
	assess various GB functional forms.},
  bdsk-url-1 = {http://dx.doi.org/10.1002/jcc.10126},
  date-added = {2008-09-01 14:00:11 -0500},
  date-modified = {2008-09-01 14:00:11 -0500},
  keywords = {Electrostatics},
  ty = {JOUR},
  url = {http://dx.doi.org/10.1002/jcc.10126}
}

@ARTICLE{Ordejon:2000,
  author = {Ordejon, P.},
  title = { Linear Scaling ab initio Calculations in Nanoscale Materials with	SIESTA},
  journal = {Phys. Stat. Sol.},
  year = {2000},
  volume = {217},
  pages = {335}
}

@ARTICLE{Ordejon:1996,
  author = {Ordejon, P. and Artacho, E. and Soler, J. M.},
  title = {Self-consistent order-N density-functional calculations for very
	large systems},
  journal = {Phys. Rev. B},
  year = {1996},
  volume = {53},
  pages = {10441-10444}
}


@ARTICLE{Orozco:2000,
  author = {Orozco, M. and Luque, F. J.},
  title = {Theoretical Methods for the Description of the Solvent Effect in
	Biomolecular Systems},
  journal = {Chem. Rev.},
  year = {2000},
  volume = {100},
  pages = {4187-4225}
}

@INPROCEEDINGS{Ortega:1999,
  author = {Ortega, J. M. },
  booktitle = {Numerical Analysis: A second course},
  year = {1999},
  publisher = {Academic Press, NY}
}

@ARTICLE{Osher:1993,
  author = {Osher, Stanley },
  title = {A Level Set Formulation for the Solution of the {Dirichlet} Problem
	for Hamilton--Jacobi Equations},
  journal = {SIAM Journal on Mathematical Analysis},
  year = {1993},
  volume = {24},
  pages = {1145--1152},
  number = {5},
  abstract = {A level set formulation for the solution of the Hamilton Jacobi equation
	$F(x,y,u,u_x ,u_y ) = 0$ is presented, where $u$ is prescribed on
	a set of closed bounded noncharacteristic curves. A time dependent
	Hamilton--Jacobi equation is derived such that the zero level set
	at various time t of this solution is precisely the set of points
	$(x,y)$ for which $u(x,y) = t$. This gives a fast and simple numerical
	method for generating the viscosity solution to $F = 0$. The level
	set capturing idea was first introduced by Osher and Sethian [J.
	Comput. Phys., 79 (1988), pp. 12--49], and the observation that this
	is useful for an important computer vision problem of this type was
	then made by Kimmel and Bruckstein in [Technion (Israel) Computer
	Science Report, CIS #9209, 1992] following Bruckstein [Comput. Vision
	Graphics Image Process, 44 (1988), pp. 139--154]. Finally, it is
	noted that an extension to many space dimensions is immediate.},
  bdsk-url-1 = {http://dx.doi.org/10.1137/0524066},
  date-added = {2008-06-30 21:27:34 -0400},
  date-modified = {2008-06-30 21:27:34 -0400},
  doi = {10.1137/0524066},
  keywords = {mathematics},
  posted-at = {2008-07-01 02:26:27},
  priority = {0},
  publisher = {SIAM},
  url = {http://dx.doi.org/10.1137/0524066}
}

@BOOK{OsherFedkiwBook,
  title = {Level Set Methods and Dynamic Implicit Surfaces},
  publisher = {Springer-Verlag},
  year = {2003},
  author = {Stanley Osher and Ronald Fedkiw},
  volume = {153},
  series = {Applied Mathematical Sciences},
  address = {New York}
}

@ARTICLE{Osher:2001,
  author = {Osher, Stanley and Fedkiw, Ronald P. },
  title = {Level Set Methods: An Overview and Some Recent Results},
  journal = {J. Comput. Phys.},
  year = {2001},
  volume = {169},
  pages = {463--502},
  number = {2},
  abstract = {The level set method was devised by S. Osher and J. A. Sethian (1988,
	J. Comput. Phys.79, 12-49) as a simple and versatile method for computing
	and analyzing the motion of an interface [Gamma] in two or three
	dimensions. [Gamma] bounds a (possibly multiply connected) region
	[Omega]. The goal is to compute and analyze the subsequent motion
	of [Gamma] under a velocity field v. This velocity can depend on
	position, time, the geometry of the interface, and the external physics.
	The interface is captured for later time as the zero level set of
	a smooth (at least Lipschitz continuous) function [phi] (x, t); i.e.,
	[Gamma](t)={x[phi](x, t)=0}. [phi] is positive inside [Omega], negative
	outside [Omega], and is zero on [Gamma](t). Topological merging and
	breaking are well defined and easily performed. In this review article
	we discuss recent variants and extensions, including the motion of
	curves in three dimensions, the dynamic surface extension method,
	fast methods for steady state problems, diffusion generated motion,
	and the variational level set approach. We also give a user's guide
	to the level set dictionary and technology and couple the method
	to a wide variety of problems involving external physics, such as
	compressible and incompressible (possibly reacting) flow, Stefan
	problems, kinetic crystal growth, epitaxial growth of thin films,
	vortex-dominated flows, and extensions to multiphase motion. We conclude
	with a discussion of applications to computer vision and image processing.},
  bdsk-url-1 = {http://dx.doi.org/10.1006/jcph.2000.6636},
  date-added = {2008-06-30 21:08:49 -0400},
  date-modified = {2008-06-30 21:08:49 -0400},
  doi = {10.1006/jcph.2000.6636},
  keywords = {mathematics},
  posted-at = {2008-07-01 02:08:08},
  priority = {0},
  url = {http://dx.doi.org/10.1006/jcph.2000.6636}
}

@ARTICLE{Osher:1990,
  author = {Stanley Osher and Leonid I. Rudin},
  title = {Feature-Oriented Image Enhancement Using Shock Filters},
  journal = {SIAM Journal on Numerical Analysis},
  year = {1990},
  volume = {27},
  pages = {919-940},
  number = {4},
  abstract = {Shock filters for image enhancement are developed. The filters use
	new nonlinear time dependent partial differential equations and their
	discretizations. The evolution of the initial image $u_0 (x,y)$ as
	$t \to \infty $ into a steady state solution $u_\infty (x,y)$ through
	$u(x,y,t)$, $t > 0$, is the filtering process. The partial differential
	equations have solutions which satisfy a maximum principle. Moreover
	the total variation of the solution for any fixed $t > 0$ is the
	same as that of the initial data. The processed image is piecewise
	smooth, nonoscillatory, and the jumps occur across zeros of an elliptic
	operator (edge detector). The algorithm is relatively fast and easy
	to program. Â©1990 Society for Industrial and Applied Mathematics},
  bdsk-url-1 = {http://link.aip.org/link/?SNA/27/919/1},
  bdsk-url-2 = {http://dx.doi.org/10.1137/0727053},
  date-added = {2008-09-16 14:56:54 -0500},
  date-modified = {2008-09-16 14:56:54 -0500},
  doi = {10.1137/0727053},
  keywords = {Mathematics; Visualization},
  publisher = {SIAM},
  url = {http://link.aip.org/link/?SNA/27/919/1}
}

@ARTICLE{osher-sethian:88,
  author = {Osher, S. and Sethian, J.A.},
  title = {Fronts Propagating with Curvature-Dependent Speed: Algorithms Based
	on {H}amilton--{J}acobi Formulations},
  journal = {J. Comput. Phys.},
  year = {1988},
  volume = {79},
  pages = {12--49},
  number = {1}
}

@ARTICLE{SOsher:1988,
  author = {Osher, S. and Sethian, J.A.},
  title = {{Fronts propagating with curvature-dependent speed: algorithms based
	on Hamilton-Jacobi formulations}},
  journal = {Journal of computational physics},
  year = {1988},
  volume = {79},
  pages = {12--49},
  number = {1},
  issn = {0021-9991},
  publisher = {Elsevier}
}

@ARTICLE{OsherSethian,
  author = {Stanley Osher and James E. Sethian},
  title = {{Fronts Propagating with Curvature-dependent Speed: Algorithms based
	on the Hamilton{-}Jacobi Formulation}},
  journal = {J. Comput. Phys.},
  year = {1988},
  volume = {79},
  pages = {12-49}
}

@ARTICLE{Oster:1985,
  author = {Oster, G. F. and Murray, J. D. and Maini, P. K. },
  title = {A model for chondrogenic condensations in the developing limb: the
	role of extracellular matrix and cell tractions},
  journal = { J. Embryol. Exper. Morph},
  year = {1985},
  volume = {89},
  pages = {93 - 112 },
  number = { }
}

@ARTICLE{Ou-Yang:1989,
  author = {Ou-Yang, Z. C. and Helfrich, W.},
  title = {Bending energy of vesicle membranes: General expressions for the
	first, second, and third variation of the shape energy and applications
	to spheres and cylinders},
  journal = {Phys. Rev. A},
  year = {1989},
  volume = {39},
  pages = {5280 - 5288}
}

@ARTICLE{Paci:2002,
  author = {Paci, E. and Vendruscolo, M. and Karplus, M.},
  title = {Validity of Go Models: Comparison with a Solvent-Shielded Empirical
	Energy Decomposition},
  journal = {Biophys J },
  year = {2002},
  volume = {83},
  pages = {3032-038},
  number = { }
}

@ARTICLE{Page:2006c,
  author = {Page, Christopher S. and Bates, Paul A. },
  title = {Can {MM-PBSA} calculations predict the specificities of protein kinase
	inhibitors?},
  journal = {Journal of Computational Chemistry},
  year = {2006},
  volume = {27},
  pages = {1990--2007},
  number = {16},
  abstract = {An application of the Molecular mechanics {Poisson-Boltzmann} surface
	area (MM-PBSA) protocol to the prediction of protein kinase inhibitor
	selectivity is presented. Six different inhibitors are placed in
	equivalent orientations in each of six different receptors. Fully
	solvated molecular dynamics is then run for 1 ns on each of the 36
	complexes, and the resulting trajectories scored, using the implicit
	solvent model. The results show some correlation with experimentally-determined
	specificities; anomalies may be attributed to a variety of causes,
	including difficulties in quantifying induced fit penalties and variabilities
	in normal modes calculations. Decomposing interaction energies on
	a per-residue basis yields more useful insights into the natures
	of the binding modes and suggests that the real value of such calculations
	lies in understanding interactions rather than outright prediction.
	Â© 2006 Wiley Periodicals, Inc. J Comput Chem, 2007},
  address = {Biomolecular Modelling Laboratory, Cancer Research UK London Research
	Institute, 44 Lincoln's Inn Fields, London, GB-WC2A 3PX, United Kingdom},
  bdsk-url-1 = {http://dx.doi.org/10.1002/jcc.20534},
  bdsk-url-2 = {http://dx.doi.org/10.1002/jcc.20534},
  date-added = {2008-09-01 13:50:28 -0500},
  date-modified = {2008-09-01 13:50:28 -0500},
  doi = {10.1002/jcc.20534},
  keywords = {Electrostatics, Protein-ligandInteractions, Solvation},
  posted-at = {2008-04-16 13:54:18},
  priority = {0},
  url = {http://dx.doi.org/10.1002/jcc.20534}
}

@ARTICLE{Pal:2005,
  author = {Pal, D. and Eisenberg, D.},
  title = {{Inference of protein function from protein structure}},
  journal = {Structure},
  year = {2005},
  volume = {13},
  pages = {121-130},
  number = {1}
}

@INPROCEEDINGS{Nrosy,
  author = {Jonathan Palacios and Eugene Zhang},
  title = {Rotational symmetry field design on surfaces},
  booktitle = {SIGGRAPH '07: ACM SIGGRAPH 2007 papers},
  year = {2007},
  pages = {55},
  address = {New York, NY, USA},
  publisher = {ACM},
  doi = {http://doi.acm.org/10.1145/1275808.1276446},
  location = {San Diego, California}
}

@ARTICLE{Palmer:2010b,
  author = {Palmer, D. S. and Frolov, A. I. and Ratkova, E. L. and Fedorov, M.
	V. },
  title = {Towards a universal method for calculating hydration free energies:
	a 3D reference interaction site model with partial molar volume correction},
  journal = { Journal of Physics: Condensed Matter },
  year = {2010},
  volume = {22},
  number = {492101}
}

@ARTICLE{Palmer:2010,
  author = {Palmer, D. S. and Sergiievskyi, V. P. and Jensen, F. and Fedorov,
	M. V. },
  title = {Accurate calculations of the hydration free energies of druglike
	molecules using the reference interaction site model
	
	},
  journal = {J. Chem. Phys.},
  year = {2010},
  volume = {133},
  number = {044104}
}

@ARTICLE{Pan981101,
  author = {Pan, W. and Lee, T. S. and Yang, W. T.},
  title = {Parallel implementation of divide-and-conquer semiempirical quantum
	chemistry calculations},
  journal = {Journal of Computational Chemistry},
  year = {1998},
  volume = {19},
  pages = {1101-1109},
  number = {9},
  month = {Jul},
  abstract = {We have implemented a parallel divide-and-conquer method for semiempirical
	quantum mechanical calculations. The standard message passing library,
	the message passing interface (MPI), was used. In this parallel version,
	the memory needed to store the Fock and density matrix elements is
	distributed among the processors. This memory distribution solves
	the problem of demanding requirement of memory for very large molecules.
	While the parallel calculation for construction of matrix elements
	is straightforward, the parallel calculation of Fock matrix diagonalization
	is achieved via the divide-and-conquer method. Geometry optimization
	is also implemented with parallel gradient calculations. The code
	has been tested on a Gray T3E parallel computer, and impressive speedup
	of calculations has been achieved. Our results indicate that the
	divide-and-conquer method is efficient for parallel implementation.
	(C) 1998 John Wiley & Sons, Inc.},
  endnotereftype = {Journal Article},
  issn = {0192-8651},
  shorttitle = {Parallel implementation of divide-and-conquer semiempirical quantum
	chemistry calculations},
  url = {<Go to ISI>://000074229900010}
}

@ARTICLE{Pan973981,
  author = {Pan, W. and Zhu, T. H. and Yang, W. T.},
  title = {First-principles study of the structural and electronic properties
	of ethylene adsorption on Si(100)-(2x1) surface},
  journal = {Journal of Chemical Physics},
  year = {1997},
  volume = {107},
  pages = {3981-3985},
  number = {10},
  month = {Sep},
  abstract = {We present a first-principles density-functional study for ethylene
	adsorption on the Si(100)-(2x1) surface. Ethylene is di-a bonded
	to the surface Si dimers with the adsorption energy of 1.81 eV. The
	dimer-maintained adsorption structure is found to be more stable
	than the dimer-cleaved one by 0.91 eV. Our calculations on the post-exposure
	of the ethylene-saturated surface to atomic hydrogen demonstrate
	the formation of Si-H bonds, the cleavage of the Si dimer bonds,
	and the minor changes for the chemisorbed ethylene, which is in good
	agreement with the recent experimental observations. (C) 1997 American
	Institute of Physics.},
  endnotereftype = {Journal Article},
  issn = {0021-9606},
  shorttitle = {First-principles study of the structural and electronic properties
	of ethylene adsorption on Si(100)-(2x1) surface},
  url = {<Go to ISI>://A1997XV75600027}
}

@ARTICLE{Papazyan:1997,
  author = {Papazyan, A. and Warshel, A.},
  title = {A stringent test of the cavity concept in continuum dielectrics},
  journal = {J. Chem. Phys.},
  year = {1997},
  volume = {107},
  pages = {7975- 7978}
}

@ARTICLE{PP08,
  author = {Park,, Cheong Hee and Park,, Haesun},
  title = {A comparison of generalized linear discriminant analysis algorithms},
  journal = {Pattern Recogn.},
  year = {2008},
  volume = {41},
  pages = {1083--1097},
  number = {3},
  address = {New York, NY, USA},
  doi = {http://dx.doi.org/10.1016/j.patcog.2007.07.022},
  issn = {0031-3203},
  owner = {Yiying},
  publisher = {Elsevier Science Inc.},
  timestamp = {2009.03.28}
}

@ARTICLE{Park:2009,
  author = {Park, H. M. and Choi, Y. J. },
  title = {Electroosmotic flow driven by oscillating zeta potentials: Comparison
	of the Poisson{-}Boltzmann model, the Debye{-}H{$\ddot{u}$}kel model
	and the Nernst{-}Planck model},
  journal = {International Journal of Heat and Mass Transfer},
  year = {2009},
  volume = {52},
  pages = {4279-4295},
  number = {19-20}
}

@ARTICLE{Park:2007,
  author = {Park, H. M. and Lee, J. S. and Kim, T. W. },
  title = {Comparison of the Nernst{-}Planck model and the Poisson{-}Boltzmann
	model for electroosmotic flows in microchannels},
  journal = {Journal of Colloid and Interface Science},
  year = {2007},
  volume = {315},
  pages = {731-739 },
  number = {2}
}

@ARTICLE{Park:2002,
  author = {Park, J. T. and Colinge, J. P.},
  title = {{Multiple-gate SOI MOSFETs: Device design guidelines}},
  journal = {IEEE Trans. Electron Devices},
  year = {2002},
  volume = {49},
  pages = {2222-2229},
  annote = {Multiple-gate SOI MOSFETs: Device design guidelines},
  date-added = {2008-11-25 10:28:56 -0500},
  date-modified = {2008-11-25 10:28:56 -0500},
  ty = {JOUR}
}

@ARTICLE{jhpark:1997,
  author = {Park, J.-H. and Jerome, J. W.},
  title = {Qualitative Properties of Steady-State Poisson-Nernst-Planck Systems:
	Mathematical Study},
  journal = {SIAM J. APPL. MATH.},
  year = {1997},
  volume = {57},
  pages = {609 - 630},
  number = {3}
}

@ARTICLE{MeshIntersect,
  author = {Sang C. Park},
  title = {{Triangular Mesh Intersection}},
  journal = {The Visual Computer},
  year = {2004},
  volume = {20},
  pages = {448--456},
  number = {7}
}

@ARTICLE{SMPark:2009,
  author = {Park, S. M. and Huh, Y. S. and Craighead, H. G. and Erickson, D.},
  title = {A method for nanofluidic device prototyping using elastomeric collapse
	},
  journal = {PNAS},
  year = {2009},
  volume = {106},
  pages = {15549-15554 }
}

@ARTICLE{Parks08154106,
  author = {Parks, J. M. and Hu, H. and Cohen, A. J. and Yang, W. T.},
  title = {A pseudobond parametrization for improved electrostatics in quantum
	mechanical/molecular mechanical simulations of enzymes},
  journal = {Journal of Chemical Physics},
  year = {2008},
  volume = {129},
  pages = {154106},
  number = {15},
  month = {Oct},
  abstract = {The pseudobond method is used in quantum mechanical/molecular mechanical
	(QM/MM) simulations in which a covalent bond connects the quantum
	mechanical and classical subsystems. In this method, the molecular
	mechanical boundary atom is replaced by a special quantum mechanical
	atom with one free valence that forms a bond with the rest of the
	quantum mechanical subsystem. This boundary atom is modified through
	the use of a parametrized effective core potential and basis set.
	The pseudobond is designed to reproduce the properties of the covalent
	bond that it has replaced, while invoking as small a perturbation
	as possible on the system. Following the work of Zhang [J. Chem.
	Phys. 122, 024114 (2005)], we have developed new pseudobond parameters
	for use in the simulation of enzymatic systems. Our parameters yield
	improved electrostatics and deprotonation energies, while at the
	same time maintaining accurate geometries. We provide parameters
	for C-ps(sp(3))-C(sp(3)), C-ps(sp(3))-C(sp(2),carbonyl), and C-ps(sp(3))-N(sp(3))
	pseudobonds, which allow the interface between the quantum mechanical
	and molecular mechanical subsystems to be constructed at either the
	C-alpha-C-beta bond of a given amino acid residue or along the peptide
	backbone. In addition, we demonstrate the efficiency of our parametrization
	method by generating residue-specific pseudobond parameters for a
	single amino acid. Such an approach may enable higher accuracy than
	general purpose parameters for specific QM/MM applications. (C) 2008
	American Institute of Physics. [DOI: 10.1063/1.2994288]},
  endnotereftype = {Journal Article},
  issn = {0021-9606},
  shorttitle = {A pseudobond parametrization for improved electrostatics in quantum
	mechanical/molecular mechanical simulations of enzymes},
  url = {<Go to ISI>://000260280600006}
}

@ARTICLE{Parks095217,
  author = {Parks, J. M. and Hu, H. and Rudolph, J. and Yang, W. T.},
  title = {Mechanism of Cdc25B Phosphatase with the Small Molecule Substrate
	p-Nitrophenyl Phosphate from QM/MM-MFEP Calculations},
  journal = {Journal of Physical Chemistry B},
  year = {2009},
  volume = {113},
  pages = {5217-5224},
  number = {15},
  month = {Apr},
  abstract = {Cdc25B is a dual-specificity phosphatase that catalyzes the dephosphorylation
	of the Cdk2/CycA protein complex. This enzyme is an important regulator
	of the human cell cycle and has been identified as a potential anticancer
	target. In general, protein tyrosine phosphatases are thought to
	bind the dianionic form of the phosphate and employ general acid
	catalysis via the Asp residue in the highly conserved WPD-loop. However,
	the Cdc25 phosphatases form a special subfamily based on their distinct
	differences from other protein tyrosine phosphatases. Although Cdc25B
	contains the (H/V)CX5R catalytic motif present in all other protein
	tyrosine phosphatases, it lacks an analogous catalytic acid residue.
	No crystallographic data currently exist for the complex of Cdc25B
	with Cdk2/CycA, so in addition to its natural protein substrate,
	experimental and theoretical studies are often carried out with small
	molecule substrates. In an effort to gain understanding of the dephosphorylation
	mechanism of Cdc25B with a commonly used small molecule substrate,
	we have performed simulations of the rate-limiting step of the reaction
	catalyzed by Cdc25B with the substrate p-nitrophenyl phosphate using
	the recently developed QM/MM Minimum Free Energy Path method (Hu
	et al. J. Chem. Phys. 2008, 034105). We have simulated the first
	step of the reaction with both the monoanionic and the dianionic
	forms of the substrate, and our calculations favor a mechanism involving
	the monoanionic form. Thus, Cdc25 may employ a unique dephosphorylation
	mechanism among protein tyrosine phosphatases, at least in the case
	of the small molecule substrate p-nitrophenyl phosphate.},
  endnotereftype = {Journal Article},
  issn = {1520-6106},
  shorttitle = {Mechanism of Cdc25B Phosphatase with the Small Molecule Substrate
	p-Nitrophenyl Phosphate from QM/MM-MFEP Calculations},
  url = {<Go to ISI>://000265030500033 }
}

@ARTICLE{Parks083168,
  author = {Parks, J. M. and Kondru, R. K. and Hu, H. and Beratan, D. N. and
	Yang, W. T.},
  title = {Hepatitis C virus NS5B polymerase: QM/MM calculations show the important
	role of the internal energy in ligand binding},
  journal = {Journal of Physical Chemistry B},
  year = {2008},
  volume = {112},
  pages = {3168-3176},
  number = {10},
  month = {Mar},
  abstract = {The inter- and intramolecular interactions that determine the experimentally
	observed binding mode of the ligand(2Z)-2-(benzoylamino)-3-[4-(2-bromophenoxy)phenyl]-2-propenoate
	in complex with hepatitis C virus NS5B polymerase have been studied
	using QM/MM calculations. DFT-based QM/MM optimizations were performed
	on a number of ligand conformers in the protein-ligand complex. Using
	these initial poses, our aim is 2-fold. First, we identify the minimum
	energy pose. Second, we dissect the energetic contributions to this
	pose using QM/MM methods. The study reveals the critical importance
	of internal energy for the proper energy ranking of the docked poses.
	Using this protocol, we successfully identified three poses that
	have low RMSD with respect to the crystallographic structure from
	among the top 20 initially docked poses. We show that the most important
	energetic component contributing to binding for this particular protein-ligand
	system is the conformational (i.e., QM internal) energy.},
  endnotereftype = {Journal Article},
  issn = {1520-6106},
  shorttitle = {Hepatitis C virus NS5B polymerase: QM/MM calculations show the important
	role of the internal energy in ligand binding},
  url = {<Go to ISI>://000253784700054}
}

@BOOK{Parr:1989,
  title = {Density Functional Theory of Atoms and Molecules},
  year = {1989},
  author = {Parr, R. and Yang, W.},
  annote = {Density Functional Theory of Atoms and Molecules},
  bdsk-url-1 = {Oxford University Press, New York},
  date-added = {2008-11-25 10:28:56 -0500},
  date-modified = {2008-11-25 10:28:56 -0500},
  ty = {BOOK}
}

@BOOK{Parr89,
  title = {Density-Functional Theory of Atoms and Molecules},
  publisher = {Oxford University Press},
  year = {1989},
  author = {Parr, R. G. and Yang, W.},
  address = {New York},
  endnotereftype = {Book},
  shorttitle = {Density-Functional Theory of Atoms and Molecules}
}

@ARTICLE{Parr95701,
  author = {Parr, R. G. and Yang, W. T.},
  title = {Density-Functional Theory of the Electronic-Structure of Molecules},
  journal = {Annual Review of Physical Chemistry},
  year = {1995},
  volume = {46},
  pages = {701-728},
  abstract = {Recent fundamental advances in the density-functional theory of electronic
	structure are summarized. Emphasis is given to four aspects of the
	subject: (a) tests of functionals, (b) new methods for determining
	accurate exchange-correlation functionals, (c) linear scaling methods,
	and (d) developments in the description of chemical reactivity.},
  endnotereftype = {Journal Article},
  issn = {0066-426X},
  shorttitle = {Density-Functional Theory of the Electronic-Structure of Molecules},
  url = {<Go to ISI>://A1995TF48600025}
}

@ARTICLE{Parr844049,
  author = {Parr, R. G. and Yang, W. T.},
  title = {Density Functional-Approach to the Frontier-Electron Theory of Chemical-Reactivity},
  journal = {Journal of the American Chemical Society},
  year = {1984},
  volume = {106},
  pages = {4049-4050},
  number = {14},
  endnotereftype = {Journal Article},
  isinote = {ISI Document Delivery No.: SZ328 Times Cited: 518 Cited Reference
	Count: 8},
  issn = {0002-7863},
  shorttitle = {Density Functional-Approach to the Frontier-Electron Theory of Chemical-Reactivity},
  url = {<Go to ISI>://A1984SZ32800036}
}

@ARTICLE{Parr:1984,
  author = {Parr, R. G. and Yang, W. T.},
  title = {Density functional-approach to the frontier-electron theory of chemical-reactivity},
  journal = {J. Amer. Chem. Soc.},
  year = {1984},
  volume = {106},
  pages = {4049 -- 4050}
}

@ARTICLE{Partenskii:1994,
  author = {Partenskii, M. B. and Dormann, V. and Jordan, P. C.},
  title = {Influence of a channel-forming peptide on energy barriers to ion
	permeation, viewed from a continuum dielectric perspective.},
  journal = {Biophysical Journal},
  year = {2002},
  volume = {67},
  pages = {1429-1438},
  month = { }
}

@ARTICLE{Patnaik:2002,
  author = {Patnaik, B. S. V. and Wei, G. W. },
  title = { Controlling wake turbulence },
  journal = {Physical Review Letters },
  year = {2002},
  volume = {88},
  number = { 054502 }
}

@ARTICLE{Patrick:2011a,
  author = { Patrick Guidotti and Kate Longo },
  title = { Well-posedness for a class of fourth order diffusions for image
	processing
	
	},
  journal = { NODEA-Nonlinear Differential Equations and Applications },
  year = {2011},
  volume = {18},
  pages = {407-425}
}

@ARTICLE{Patrick:2011b,
  author = { Patrick Guidotti and Kate Longo },
  title = { Two Enhanced Fourth Order Diffusion Models for Image Denoising
	
	},
  journal = { Journal of Mathematical Imaging and Vision },
  year = {2011},
  volume = {40},
  pages = {188-198}
}

@ARTICLE{pauly2005ebs,
  author = {Pauly, M. and Mitra, N.J. and Giesen, J. and Gross, M. and Guibas,
	L.J.},
  title = {{Example-based 3D scan completion}},
  journal = {Symposium on Geometry Processing},
  year = {2005},
  pages = {23--32}
}

@ARTICLE{Paxton:1997,
  author = {Paxton, B. and Newman, J. },
  title = { Modeling of nickel/metal hydride batteries
	
	},
  journal = { Journal of the Electrochemical Society },
  year = {1997},
  volume = {144},
  pages = {3818-3831}
}

@ARTICLE{Peet891746,
  author = {Peet, A. C. and Yang, W. T.},
  title = {The Collocation Method for Calculating Vibrational Bound-States of
	Molecular-Systems - with Application to Ar-Hcl},
  journal = {Journal of Chemical Physics},
  year = {1989},
  volume = {90},
  pages = {1746-1751},
  number = {3},
  month = {Feb},
  endnotereftype = {Journal Article},
  isinote = {ISI Document Delivery No.: T0188 Times Cited: 52 Cited Reference Count:
	25},
  issn = {0021-9606},
  shorttitle = {The Collocation Method for Calculating Vibrational Bound-States of
	Molecular-Systems - with Application to Ar-Hcl},
  url = {<Go to ISI>://A1989T018800055}
}

@ARTICLE{Peet896598,
  author = {Peet, A. C. and Yang, W. T.},
  title = {An Adapted Form of the Collocation Method for Calculating Energy-Levels
	of Rotating Atom Diatom Complexes},
  journal = {Journal of Chemical Physics},
  year = {1989},
  volume = {91},
  pages = {6598-6603},
  number = {11},
  month = {Dec},
  endnotereftype = {Journal Article},
  issn = {0021-9606},
  shorttitle = {An Adapted Form of the Collocation Method for Calculating Energy-Levels
	of Rotating Atom Diatom Complexes},
  url = {<Go to ISI>://A1989CB98400005}
}

@ARTICLE{Penfold:1990,
  author = {Penfold, R. and Nordholm, S. and JÃ¶nsson, B. and Woodward, C.
	E.},
  title = {A simple analysis of ion-ion correlation in polyelectrolyte solutions},
  journal = {Journal of Chemical Physics},
  year = {1990},
  volume = {92},
  pages = {1915-1922},
  number = {3},
  abstract = {In the PoissonÃ¢Â€Â“Boltzmann theory of macroion screening
	in electrolyte solutions the chief simplifying assumption is the
	neglect of correlations within the ionic atmosphere. Using a generalized
	{van der Waals} density functional analysis incorporating ionÃ¢Â€Â“ion
	correlation in a local approximation we obtain a simple correlation
	corrected PoissonÃ¢Â€Â“Boltzmann theory. For point charges
	in the salt free case, this local correlation approximation leads
	to asymptotic instability (a ``structuring catastrophe'') though
	the correction is well behaved to low orders in perturbation theory.
	Results in zeroth order and in a zeroth order field approximation
	are compared with an extended series of Monte Carlo simulations within
	a cell model (and a planar electrode model). An excellent agreement
	is found over a wide range of coupling strengths.},
  annote = {A simple analysis of ionÃ¢Â€Â“ion correlation in polyelectrolyte
	solutions},
  bdsk-url-1 = {http://dx.doi.org/10.1063/1.458022},
  date-added = {2008-09-01 14:06:35 -0500},
  date-modified = {2008-09-01 14:06:35 -0500},
  keywords = {Electrostatics},
  ty = {JOUR},
  url = {http://dx.doi.org/10.1063/1.458022}
}

@ARTICLE{peng04pkz,
  author = {Jianbo Peng and Daniel Kristjansson and Denis Zorin},
  title = {Interactive modeling of topologically complex geometric detail},
  journal = {ACM Trans. Graph.},
  year = {2004},
  volume = {23},
  pages = {635--643},
  number = {3}
}

@ARTICLE{Perez-Jorda9871,
  author = {Perez-Jorda, J. M. and Yang, W. T.},
  title = {On the scaling of multipole methods for particle-particle interactions},
  journal = {Chemical Physics Letters},
  year = {1998},
  volume = {282},
  pages = {71-78},
  number = {1},
  month = {Jan},
  abstract = {Then is some controversy regarding the scaling of the fast multipole
	method (FMM). it has recently been proven by Aluru that the FMM is
	not a linear scaling method, but an O(N log(4) N) method. Aluru's
	proof cannot be applied to typical computational chemistry calculations
	where the required precision is smaller than the machine accuracy.
	In this Letter, we deal with this kind of situation and give a rigorous
	bound to the scaling and a statistical estimate. We also perform
	numerical tests. Our results agree with Aluru's proof. The scaling
	of other methods that use multipoles is also discussed. (C) 1998
	Elsevier Science B.V.},
  endnotereftype = {Journal Article},
  issn = {0009-2614},
  shorttitle = {On the scaling of multipole methods for particle-particle interactions},
  url = {<Go to ISI>://000072327200011}
}

@ARTICLE{PerezJorda971218,
  author = {PerezJorda, J. M. and Yang, W. T.},
  title = {Fast evaluation of the Coulomb energy for electron densities},
  journal = {Journal of Chemical Physics},
  year = {1997},
  volume = {107},
  pages = {1218-1226},
  number = {4},
  month = {Jul},
  abstract = {The evaluation of the Coulomb interaction of the electron density
	with itself dominates the cost of a density-functional theory calculation,
	due to its quadratic scaling with the size of the system. A similar
	problem is found in simulations of systems of particles, where the
	cost is dominated by the particle-particle interactions, Recently,
	we have presented a simple method for the particle-particle problem
	[J. M. Perez-Jorda and W. Yang, Chem. Phys. Lett. 247, 484 (1995)].
	In this paper, our scheme is generalized to densities, in particular
	for calculations with Gaussian basis functions. Near linear scaling
	is observed for molecules with about 400 first-row atoms. CPU time
	savings of up to one order of magnitude are observed for these molecules.
	The method distinguishes between localized and diffuse distributions
	in a much simpler way than in other proposed approaches. (C) 1997
	American Institute of Physics.},
  endnotereftype = {Journal Article},
  issn = {0021-9606},
  shorttitle = {Fast evaluation of the Coulomb energy for electron densities},
  url = {<Go to ISI>://A1997XL40200021}
}

@ARTICLE{PerezJorda968003,
  author = {PerezJorda, J. M. and Yang, W. T.},
  title = {A concise redefinition of the solid spherical harmonics and its use
	in fast multipole methods},
  journal = {Journal of Chemical Physics},
  year = {1996},
  volume = {104},
  pages = {8003-8006},
  number = {20},
  month = {May},
  abstract = {Several fast algorithms for the approximation of particle-particle
	interactions by means of multipole expansions in spherical harmonics
	have appeared recently. In this letter we present a redefinition
	of the solid spherical harmonics that is real and gives simple expressions
	for the evaluation of the functions and their derivatives. Application
	to the recursive bisection method [J. M. Perez-Jorda and W. Yang,
	Chem. Phys. Lett. 247, 484 (1995)] greatly improves its performance.
	(C) 1996 American Institute of Physics.},
  endnotereftype = {Journal Article},
  issn = {0021-9606},
  shorttitle = {A concise redefinition of the solid spherical harmonics and its use
	in fast multipole methods},
  url = {<Go to ISI>://A1996UL12500022}
}

@ARTICLE{Perezjorda95469,
  author = {Perezjorda, J. M. and Yang, W. T.},
  title = {An Algorithm for 3d Numerical-Integration That Scales Linearly with
	the Size of the Molecule},
  journal = {Chemical Physics Letters},
  year = {1995},
  volume = {241},
  pages = {469-476},
  number = {4},
  month = {Jul},
  abstract = {The cost of numerical integration in density-functional theory scales
	as the cube of the size of the molecule: it is proportional to the
	number of grid points and to the square of the number of basis functions.
	We describe a scheme that makes this cost independent of the number
	of basis functions, thus yielding an algorithm that scales linearly
	with the size of the molecule. The error introduced by the present
	scheme can be made as small as desired by lowering a threshold tau.
	The method can be applied to any quadrature rule and local basis
	set.},
  endnotereftype = {Journal Article},
  issn = {0009-2614},
  shorttitle = {An Algorithm for 3d Numerical-Integration That Scales Linearly with
	the Size of the Molecule},
  url = {<Go to ISI>://A1995RL96600033}
}

@ARTICLE{PerezJorda95484,
  author = {PerezJorda, J. M. and Yang, W. T.},
  title = {A simple O(N log N) algorithm for the rapid evaluation of particle-particle
	interactions},
  journal = {Chemical Physics Letters},
  year = {1995},
  volume = {247},
  pages = {484-490},
  number = {4-6},
  month = {Dec},
  abstract = {Exact simulations of huge systems of charged particles are impossible
	in practice, because their cost is proportional to N-2, where N is
	the number of particles. We present an approximate and simple O(N
	lap N) algorithm based upon the idea of recursive bisection of the
	set of particles. A small fraction of the particle-particle interactions
	is evaluated exactly by direct summation, while the rest is approximated
	via multipole expansions. Our algorithm is easy to program (in particular,
	in parallel, which is trivial), and it is well suited for systems
	with a non-uniform distribution of particles. For uniform systems,
	its accuracy and execution time are comparable to other fast methods
	such as tree codes and the fast multipole method.},
  endnotereftype = {Journal Article},
  issn = {0009-2614},
  shorttitle = {A simple O(N log N) algorithm for the rapid evaluation of particle-particle
	interactions},
  url = {<Go to ISI>://A1995TN29100026}
}

@ARTICLE{AMBER,
  author = {Perlman, D. A. and Case, D. A. and Caldwell, J. W. and Ross, W. S.
	and Cheatham, T. E. and Debolt, S. and Ferguson, D. and Seibel, G.
	and Kollman, P.},
  title = {AMBER, a package of computer programs for applying molecular mechanics,
	normal mode analysis, molecular dynamics and free energy calculations
	to simulate the structural and energetic properties of molecules},
  journal = {Comp. Phys. Commun.},
  year = {1995},
  volume = {91},
  pages = {1-41},
  month = { }
}

@ARTICLE{PPerona:1990,
  author = {Perona, P. and Malik, J.},
  title = {Scale-space and edge-detection using anisotropic diffusion},
  journal = {{IEEE} Transactions on Pattern Analysis and Machine Intelligence},
  year = {1990},
  volume = {12},
  pages = {629-639},
  number = {7}
}

@ARTICLE{Peskin:1989,
  author = {Peskin, C. P. and McQueen, D. M.},
  title = {A 3-dimensional computational method for blood-flow in the heart.
	1. Immersed elastic fibers in a viscous incompressible fluid},
  journal = {J. Comput. Phys.},
  year = {1989},
  volume = {81},
  pages = {372-405},
  annote = {A 3-dimensional computational method for blood-flow in the heart.
	1. Immersed elastic fibers in a viscous incompressible fluid},
  date-added = {2008-09-19 10:28:56 -0500},
  date-modified = {2008-09-19 10:28:56 -0500},
  ty = {JOUR}
}

@ARTICLE{Peskin:1981,
  author = {Peskin, C. S.},
  title = {Lectures on mathematical aspects of physiology},
  journal = {Lectures in Appl. Math. },
  year = {1981},
  volume = {19},
  pages = {69-107},
  annote = {Lectures on mathematical aspects of physiology},
  date-added = {2008-09-19 10:28:56 -0500},
  date-modified = {2008-09-19 10:28:56 -0500},
  ty = {JOUR}
}

@ARTICLE{Peskin:1977,
  author = {Peskin, C. S.},
  title = {Numerical analysis of blood flow in the heart},
  journal = {J. Comput. Phys.},
  year = {1977},
  volume = {25},
  pages = {220-52},
  number = {3},
  abstract = {The flow pattern of blood in the heart is intimately connected with
	the performance of the heart valves.^This paper extends previous
	work on the solution of the Navier-Stokes equations in the presence
	of moving immersed boundaries which interact with the fluid.^The
	boundary representation now includes the muscular heart wall.^The
	fixed topology of the boundary representation is exploited in the
	solution of the nonlinear equations which implicitly define the boundary
	forces.^An improved numerical representation of the sigma-function
	is introduced.^A fast Laplace-solver is used.^The results of calculations
	with a natural valve and with a prosthetic valve are presented.},
  date-added = {2008-09-14 15:46:53 -0500},
  date-modified = {2008-09-14 15:46:53 -0500},
  keywords = {Mathematics; FluidMechanics}
}

@ARTICLE{GRASP2,
  author = {Petrey, D. and Honig, B.},
  title = {{GRASP2}: Visualization, Surface Properties, and Electrostatics of
	Macromolecular Structures and Sequences},
  journal = {Methods in Enzymology},
  year = {2003},
  volume = {374},
  pages = {492-509},
  bdsk-url-1 = {http://dx.doi.org/10.1016/S0076-6879(03)74021-X},
  date-added = {2008-09-01 13:55:42 -0500},
  date-modified = {2008-09-01 13:55:42 -0500},
  doi = {http://dx.doi.org/10.1016/S0076-6879(03)74021-X},
  keywords = {Electrostatics, Software, Visualization}
}

@ARTICLE{Pierotti:1976,
  author = {Pierotti, R. A.},
  title = {A scaled particle theory of aqueous and nonaqeous solutions},
  journal = {Chemical Reviews},
  year = {1976},
  volume = {76},
  pages = {717-726},
  number = {6},
  abstract = {The increasing trend on the part of chemists to endeavor to interpret
	the thermodynamic behavior of chemical systems in fluid media in
	terms of molecular parameters and intermolecular interactions has
	resulted in a need for new statistical thermodynamic approaches to
	fluids and fluid mixtures. While a number of such approaches have
	been developed, a particularly useful and intuitively attractive
	approach which yields important insight into the nature of such fluids
	is the scaled particle theory.Ã¢Â€Â™-1Ã-\,^{\circ}$ Although
	this theory was originally developed as a formal statistical mechanical
	theory of dense hard-sphere fluids, it became apparent that it provided
	relations which were relevant to the behavior of real fluids. The
	present article is not a review of the formalism of the scaled particle
	theory, but rather is an effort to select those aspects of the theory
	which make it important in understanding qualitatively and semiquantitatively
	the important contributions to the thermodynamic properties of nonaqueous
	and aqueous solutions. These solution properties have always been
	of interest to physical chemists, but in recent years there has been
	an unprecedented interest in solution thermodynamics by physical
	organic chemists, by inorganic chemists, by electrochemists, and,
	most notably, by biochemists. This interest stems in part from the
	importance of solvent effects on reaction rates and mechanisms, on
	the nature of ionic interactions in electrolyte solutions, and on
	the nature of hydrophobic interactions and the conformational properties
	of proteins and other biologically important molecules. Particular
	emphasis will be placed on the nature of dilute solutions, that is,
	on solutions in which the solubility of a substance is directly proportional
	to either the pressure or activity of the substance. These solutions
	The increasing trend on the part of chemists to endeavor to interpret
	the thermodynamic behavior of chemical systems in fluid media in
	terms of molecular parameters and intermolecular interactions has
	resulted in a need for new statistical thermodynamic approaches to
	fluids and fluid mixtures. While a number of such approaches have
	been developed, a particularly useful and intuitively attractive
	approach which yields important insight into the nature of such fluids
	is the scaled particle theory.Ã¢Â€Â™-1Ã-\,^{\circ}$ Although
	this theory was originally developed as a formal statistical mechanical
	theory of dense hard-sphere fluids, it became apparent that it provided
	relations which were relevant to the behavior of real fluids. The
	present article is not a review of the formalism of the scaled particle
	theory, but rather is an effort to select those aspects of the theory
	which make it important in understanding qualitatively and semiquantitatively
	the important contributions to the thermodynamic properties of nonaqueous
	and aqueous solutions. These solution properties have always been
	of interest to physical chemists, but in recent years there has been
	an unprecedented interest in solution thermodynamics by physical
	organic chemists, by inorganic chemists, by electrochemists, and,
	most notably, by biochemists. This interest stems in part from the
	importance of solvent effects on reaction rates and mechanisms, on
	the nature of ionic interactions in electrolyte solutions, and on
	the nature of hydrophobic interactions and the conformational properties
	of proteins and other biologically important molecules. Particular
	emphasis will be placed on the nature of dilute solutions, that is,
	on solutions in which the solubility of a substance is directly proportional
	to either the pressure or activity of the substance. These solutions
	the deviations from HenryÃ¢Â€Â™s law are made, then molecular
	information can be obtained involving not only the solute-solvent
	interaction but also the interaction between two or more solute molecules.},
  annote = {A scaled particle theory of aqueous and nonaqeous solutions; PierrotiSPT},
  bdsk-url-1 = {http://pubs.acs.org/cgi-bin/sample.cgi/chreay/1976/76/i06/pdf/cr60304a002.pdf},
  date-added = {2008-09-17 09:14:02 -0500},
  date-modified = {2008-09-17 09:14:02 -0500},
  keywords = {Solvation},
  ty = {JOUR},
  url = {http://pubs.acs.org/cgi-bin/sample.cgi/chreay/1976/76/i06/pdf/cr60304a002.pdf}
}

@ARTICLE{pighin1999rfa,
  author = {Pighin, F. and Szeliski, R. and Salesin, D.},
  title = {{Resynthesizing facial animation through 3d model-based tracking}},
  journal = {Proceedings, International Conference on Computer Vision},
  year = {1999}
}

@ARTICLE{Pinkall,
  author = {Ulrich Pinkall and Konrad Polthier},
  title = {Computing Discrete Minimal Surfaces and their Conjugates},
  journal = {Experimental Mathematics},
  year = {1993},
  volume = {2(1)},
  pages = {15--36}
}

@ARTICLE{pinkall-polthier:93,
  author = {Pinkall, U. and Polthier, K.},
  title = {Computing Discrete Minimal Surfaces and Their Conjugates},
  journal = {Experimental Mathematics},
  year = {1993},
  volume = {2},
  pages = {15--36},
  number = {1}
}

@ARTICLE{Piasani:2008,
  author = {Pisani, L. and Siciliano, G.},
  title = {{Note on a Schr\"{o}dinger-Poisson system in a bounded domain}},
  journal = {App. Math. Lett.},
  year = {2008},
  volume = {21},
  pages = {521-528}
}

@ARTICLE{planitz2005cfs,
  author = {Planitz, BM and Maeder, AJ and Williams, JA},
  title = {{The correspondence framework for 3D surface matching algorithms}},
  journal = {Computer Vision and Image Understanding},
  year = {2005},
  volume = {97},
  pages = {347-383},
  number = {3},
  publisher = {Elsevier Science Inc. New York, NY, USA}
}

@ARTICLE{Polizzi:2005,
  author = {Polizzi, E. and Ben Abdallah, N.},
  title = {Subband decomposition approach for the simulation of quantum electron
	transport in nanostructures},
  journal = {J. Comput. Phys.},
  year = {2005},
  volume = {202},
  pages = {150-180},
  annote = {Subband decomposition approach for the simulation of quantum electron
	transport in nanostructures},
  date-added = {2008-11-25 10:28:56 -0500},
  date-modified = {2008-11-25 10:28:56 -0500},
  ty = {JOUR}
}

@ARTICLE{Roux2:2002,
  author = { Pomes, Regis and Roux, Benoit },
  title = {Molecular Mechanism of {H$^{+}$} Conduction in the Single-File Water
	Chain of the {Gramicidin} Channel},
  journal = {Biophysical Journal},
  year = {2002},
  volume = {82},
  pages = {2304-2316}
}

@ARTICLE{Roux:1996,
  author = {Pomes, Regis and Roux, Benoit },
  title = {{Structure and Dynamics of a Proton Wire: A Theoretical Study of
	{H$^{+}$} Translocation along the Single-File Water Chain in the
	{Gramicidin A} Channel}},
  journal = {Biophysical Journal},
  year = {2002},
  volume = {71},
  pages = {19-39}
}

@ARTICLE{Pomes1:1996,
  author = {Pomes, Regis and Roux, Benoit },
  title = {Theoretical Study of {H$^{+}$} Translocation along a Model Proton
	Wire},
  journal = {J. Phys. Chem},
  year = {1996},
  volume = {100},
  pages = {2519-2527}
}

@ARTICLE{Ponder:2003a,
  author = {Ponder, J. W. and Case, D. A.},
  title = {Force fields for protein simulations},
  journal = {Advances in Protein Chemistry},
  year = {2003},
  volume = {66},
  pages = {27-85},
  annote = {Force fields for protein simulations},
  bdsk-url-1 = {http://dx.doi.org/10.1016/S0065-3233(03)66002-X},
  date-added = {2008-09-03 13:20:24 -0500},
  date-modified = {2008-09-03 13:20:24 -0500},
  keywords = {MolecularSimulation},
  ty = {JOUR},
  url = {http://dx.doi.org/10.1016/S0065-3233(03)66002-X}
}

@ARTICLE{Pongsaksawad:2007,
  author = {Pongsaksawad, W. and Adam, C.P. and Dussault, D.},
  title = {Phase-Field Modeling of Transport-Limited Electrolysis in Solid and
	Liquid States},
  journal = {Journal of The Electrochemical Society},
  year = {2007},
  volume = {154},
  pages = {F122-F133.},
  number = {6}
}

@ARTICLE{Prabhu:2008,
  author = {Prabhu, N. V. and Panda, M. and Yang, Q. Y. and Sharp, K. A.},
  title = {Explicit ion, implicit water solvation for molecular dynamics of
	nucleic acids and highly charged molecules},
  journal = {J. Comput. Chem.},
  year = {2008},
  volume = {29},
  pages = {1113--1130}
}

@ARTICLE{Prabhu:2004,
  author = {Prabhu, N. V. and Zhu, P. and Sharp, K. A.},
  title = {Implementation and testing of stable, fast implicit solvation in
	molecular dynamics using the smooth-permittivity finite difference
	{{Poisson-Boltzmann}} method},
  journal = {Journal of Computational Chemistry},
  year = {2004},
  volume = {25},
  pages = {2049-2064},
  number = {16},
  abstract = {A fast stable finite difference {Poisson-Boltzmann} (FDPB) model for
	implicit solvation in molecular dynamics simulations was developed
	using the smooth permittivity FDPB method implemented in the OpenEye
	ZAP libraries. This was interfaced with two widely used molecular
	dynamics packages, AMBER and CHARMM. Using the CHARMM-ZAP software
	combination, the implicit solvent model was tested on eight proteins
	differing in size, structure, and cofactors: calmodulin, horseradish
	peroxidase (with and without substrate analogue bound), lipid carrier
	protein, flavodoxin, ubiquitin, cytochrome c, and a de novo designed
	3-helix bundle. The stability and accuracy of the implicit solvent
	simulations was assessed by examining root-mean-squared deviations
	from crystal structure. This measure was compared with that of a
	standard explicit water solvent model. In addition we compared experimental
	and calculated NMR order parameters to obtain a residue level assessment
	of the accuracy of MD-ZAP for simulating dynamic quantities. Overall,
	the agreement of the implicit solvent model with experiment was as
	good as that of explicit water simulations. The implicit solvent
	method was up to eight times faster than the explicit water simulations,
	and approximately four times slower than a vacuum simulation (i.e.,
	with no solvent treatment).},
  annote = {Implementation and testing of stable, fast implicit solvation in
	molecular dynamics using the smooth-permittivity finite difference
	{Poisson-Boltzmann} method; **; A demonstration of the efficiency
	and accuracy (in terms of MD stability) of the ZAP PB solver.},
  bdsk-url-1 = {http://dx.doi.org/10.1002/jcc.20138},
  date-added = {2008-06-29 14:48:36 -0500},
  date-modified = {2008-06-29 14:48:36 -0500},
  keywords = {molecular\_dynamics; Electrostatics},
  ty = {JOUR},
  url = {http://dx.doi.org/10.1002/jcc.20138}
}

@BOOK{NumRecipes,
  title = {Numerical Recipes in C: The Art of Scientific Computing},
  publisher = {Cambridge University Press},
  year = {1992},
  author = {William H. Press and Brian P. Flannery and Saul A. Teukolsky and
	William T. Vetterling},
  edition = {2nd}
}

@ARTICLE{Promislow:2009,
  author = {Promislow, K. and Wetton, B.},
  title = {{PEM} fuel cells: {A mathematical overview}},
  journal = {SIAM J Appl. Math.},
  year = {2009},
  volume = {70},
  pages = {369-409}
}

@ARTICLE{DrumShape,
  author = {M. H. Protter},
  title = {Can one hear the shape of a drum? revisited},
  journal = {SIAM Rev.},
  year = {1987},
  volume = {29},
  pages = {185--197},
  number = {2}
}

@ARTICLE{PuckettProj,
  author = {Elbridge Gerry Puckett and Ann S. Almgren and John B. Bell and Daniel
	L. Marcus and William J. Rider},
  title = {A High-order Projection Method for Tracking Fluid Interfaces in Variable
	Density Incompressible Flows},
  journal = {J. Comput. Phys.},
  year = {1997},
  volume = {130},
  pages = {269--282},
  number = {2}
}

@BOOK{Purves:2001,
  title = {Neuroscience, 2nd edition},
  publisher = {Sunderland, MA: Sinauer Associates},
  year = {2001},
  author = {Purves, D. and Augustine, G. J. and Fitzpatrick, D. and Katz, L.
	C. and LaMantia, A. S. and McNamara, J. O. and Williams, S. M. },
  address = { },
  date-added = { },
  date-modified = { },
  keywords = { },
  ty = {THES}
}

@ARTICLE{JQiu:2011,
  author = {Qiu, J. M. and Shu, C. W.},
  title = {Conservative high order semi-Lagrangian finite difference {WENO}
	methods for advection in incompressible flow},
  journal = {Journal of Computational Physics},
  year = {2011},
  volume = {230},
  pages = {863 - 889}
}

@ARTICLE{JQiu:2011,
  author = {Qiu, J. M. and Shu, C. W.},
  title = {Conservative high order semi-Lagrangian finite difference {WENO}
	methods for advection in incompressible flow},
  journal = {Journal of Computational Physics},
  year = {2011},
  volume = {230},
  pages = {863 - 889}
}

@ARTICLE{qiu,
  author = {Qiu, J. -X. and Shu, C. -W.},
  title = {On the construction, comparison, and local characteristic decomposition
	for high order central {WENO} schemes},
  journal = {J. Comput. Phys.},
  year = {2002},
  volume = {183},
  pages = {187-209}
}

@ARTICLE{Quina:1995,
  author = {Quina, F. H. and Alonso, E. O. and Farah, J. P. S.},
  title = {Incorporation of nonionic solutes into aqueous micelles: a linear
	solvation free energy relationship analysis},
  journal = {Journal of Physical Chemistry},
  year = {1995},
  volume = {99},
  pages = {11708-14},
  date-added = {2008-06-30 06:22:35 -0500},
  date-modified = {2008-06-30 06:22:35 -0500},
  keywords = {solvation; biomembranes}
}

@ARTICLE{Raberto:2002,
  author = {Raberto,M. and Scalas,E. and Mainardi,F.},
  title = {Waiting-times and returns in high-frequency Financial data: an empirical
	study},
  journal = {Physica A},
  year = {2002},
  volume = {314},
  pages = {749?C755},
  number = { }
}

@ARTICLE{Rajamani:2005,
  author = {Rajamani, S. and Truskett, T. M. and Garde, S.},
  title = {Hydrophobic hydration from small to large lengthscales: Understanding
	and manipulating the crossover},
  journal = {Proceedings of the National Academy of Sciences of the United States
	of America},
  year = {2005},
  volume = {102},
  pages = {9475-80},
  number = {27},
  abstract = {Small and large hydrophobic solutes exhibit remarkably different hydration
	thermodynamics. Small solutes are accommodated in water with minor
	perturbations to water structure, and their hydration is captured
	accurately by theories that describe density fluctuations in pure
	water. In contrast, hydration of large solutes is accompanied by
	dewetting of their surfaces and requires a macroscopic thermodynamic
	description. A unified theoretical description of these lengthscale
	dependencies was presented by Lum, Chandler, and Weeks {$[$}(1999)
	J. Phys. Chem. B 103, 4570Ã¢Â€Â-577{$]$}. Here, we use molecular
	simulations to study lengthscale-dependent hydrophobic hydration
	under various thermodynamic conditions. We show that the hydration
	of small and large solutes displays disparate dependencies on thermodynamic
	variables, including pressure, temperature, and additive concentration.
	Understanding these dependencies allows manipulation of the small-to-large
	crossover lengthscale, which is nanoscopic under ambient conditions.
	Specifically, applying hydrostatic tension or adding ethanol decreases
	the crossover length to molecular sizes, making it accessible to
	atomistic simulations. With detailed temperature-dependent studies,
	we further demonstrate that hydration thermodynamics changes gradually
	from entropic to enthalpic near the crossover. The nanoscopic lengthscale
	of the crossover and its sensitivity to thermodynamic variables imply
	that quantitative modeling of biomolecular self-assembly in aqueous
	solutions requires elements of both molecular and macroscopic hydration
	physics. We also show that the small-to-large crossover is directly
	related to the Egelstaff-Widom lengthscale, the product of surface
	tension and isothermal compressibility, which is another fundamental
	lengthscale in liquids.},
  annote = {Hydrophobic hydration from small to large lengthscales: Understanding
	and manipulating the crossover; RajTrusGard05},
  bdsk-url-1 = {http://dx.doi.org/10.1073/pnas.0504089102},
  date-added = {2008-09-16 15:27:32 -0500},
  date-modified = {2008-09-16 15:27:32 -0500},
  keywords = {Solvation},
  ty = {JOUR},
  url = {http://dx.doi.org/10.1073/pnas.0504089102}
}

@ARTICLE{Ramiere:2008,
  author = { Ramiere, I.},
  title = {Convergence analysis of the $Q_1$-finite element method for elliptic
	problems with non-boundary-fitted meshes},
  journal = {Int. J. Numer. Meth. Engng},
  year = {2008},
  volume = {75},
  pages = {1007-1052}
}

@ARTICLE{Ramirez:2005,
  author = {Ramirez, R. and Borgis, D. },
  title = {Density functional theory of solvation and its relation to implicit
	solvent models},
  journal = {Journal of physical chemistry. B.},
  year = {2005},
  volume = {109},
  pages = {6754-63},
  number = {14}
}

@ARTICLE{Raschke,
  author = {Raschke, T.M. and Tsai, J. and Levitt, M. },
  title = {Quantification of the hydrophobic interaction by simulations of the
	aggregation of small hydrophobic solutes in water},
  journal = {Proc. Natl. Acad. Sci. USA},
  year = {2001},
  volume = {98},
  pages = {5965-5969}
}

@ARTICLE{Ratkova:2010,
  author = {Ratkova, E. L. and Chuev, G. N. and Sergiievskyi, V. P. and Fedorov,
	M. V.},
  title = {An Accurate Prediction of Hydration Free Energies by Combination
	of Molecular Integral Equations Theory with Structural Descriptors
	
	},
  journal = {J. Phys. Chem. B},
  year = {2010},
  volume = {114},
  pages = {12068-2079},
  number = {37}
}

@INBOOK{Raviart-Thomas,
  pages = {292-315},
  title = {{A mixed finite element method for 2-nd order elliptic problems}},
  publisher = { Springer:Berlin},
  year = {1977},
  author = {Raviart, P. A. and Thomas, J. M.},
  volume = {606},
  series = {Mathematical Aspects of Finite Element Methods. Lecture Notes in
	Mathematics Series, A. Dold and B. Eckmann (Eds.)}
}

@ARTICLE{Rawat:2003,
  author = {Rawat, S. S. and Viard, M. and Gallo, S. A. and Rein, A. and Blumenthal,
	R. and Puri, A.},
  title = {Modulation of entry of enveloped viruses by cholesterol and sphingolipids
	(Review)},
  journal = {Molecular Membrane Biology },
  year = {2003},
  volume = {20},
  pages = {243-254},
  annote = { Modulation of entry of enveloped viruses by cholesterol and sphingolipids
	(Review)},
  date-added = {2009-03-10 },
  date-modified = {2009-03-10},
  ty = {JOUR}
}

@ARTICLE{PGP,
  author = {Nicolas Ray and Wan Chiu Li and Bruno L\'{e}vy and Alla Sheffer and
	Pierre Alliez},
  title = {Periodic global parameterization},
  journal = {ACM Trans. Graph.},
  year = {2006},
  volume = {25},
  pages = {1460--1485},
  number = {4},
  address = {New York, NY, USA},
  doi = {http://doi.acm.org/10.1145/1183287.1183297},
  issn = {0730-0301},
  publisher = {ACM}
}

@ARTICLE{Reddy:2007,
  author = {Reddy, M. R. and Singh, U. C. and Erion, M. D.},
  title = {Ab initio quantum mechanics-based free energy perturbation method
	for calculating relative solvation free energies},
  journal = {Journal of Computational Chemistry},
  year = {2007},
  volume = {28},
  pages = {491-4},
  number = {2},
  abstract = {A free energy perturbation (FEP) method was developed that uses ab
	initio quantum mechanics (QM) for treating the solute molecules and
	molecular mechanics (MM) for treating the surroundings. Like our
	earlier results using AM1 semi empirical QMs, the ab initio QM/MM-based
	FEP method was shown to accurately calculate relative solvation free
	energies for a diverse set of small molecules that differ significantly
	in structure, aromaticity, hydrogen bonding potential, and electron
	density. Accuracy was similar to or better than conventional FEP
	methods. The QM/MM-based methods eliminate the need for time-consuming
	development of MM force field parameters, which are frequently required
	for drug-like molecules containing structural motifs not adequately
	described by MM. Future automation of the method and parallelization
	of the code for Linux 128/256/512 clusters is expected to enhance
	the speed and increase its use for drug design and lead optimization.
	Â© 2006 Wiley Periodicals, Inc. J Comput Chem 28: 491-494, 2007},
  bdsk-url-1 = {http://www3.interscience.wiley.com/journal/114027045/abstract},
  bdsk-url-2 = {http://dx.doi.org/10.1002/jcc.20510},
  date-added = {2008-06-29 14:35:53 -0500},
  date-modified = {2008-06-29 14:37:08 -0500},
  doi = {10.1002/jcc.20510},
  url = {http://www3.interscience.wiley.com/journal/114027045/abstract}
}

@ARTICLE{Reed:1988,
  author = {Reed, A. E. and Curtiss, L. A. and Weinhold, F.},
  title = {Intermolecular interactions from a natural bond orbital, donor-acceptor
	viewpoint},
  journal = {Chem. Rev.},
  year = {1988},
  volume = {88},
  pages = {899-926}
}

@ARTICLE{Ren:2003,
  author = { Ren, P.Y. and Ponder J.W.},
  title = {Polarizable atomic multipole water model for molecular mechanics
	simulation},
  journal = {Journal of Physical Chmeistry B},
  year = {2003},
  volume = {107},
  pages = {5933-5947}
}


@ARTICLE{Ren:2003c,
  author = { Ren, Z. and Venugopal, R. and Goasquen, S. and Datta, S. and Lundstrom,
	M. S. },
  title = {{NanoMOS 2.5: A two-dimensional simulator for quantum transport in
	double-gate MOSFETs}},
  journal = {IEEE Trans. Elec. Dev.},
  year = {2003},
  volume = {50},
  pages = {1914 - 1925}
}

@INPROCEEDINGS{LaplaceSpectra,
  author = {Martin Reuter and Franz-Erich Wolter and Niklas Peinecke},
  title = {Laplace-Spectra as Fingerprints for Shape Matching},
  booktitle = {Proceedings of the ACM symposium on Solid and Physical Modeling},
  year = {2005},
  pages = {101--106}
}

@ARTICLE{ribner85,
  author = {Ribner, H. S.},
  title = {Cylindrical sound wave generated by shock-vortex interaction},
  journal = {AIAA Journal},
  year = {1985},
  volume = {23},
  pages = {1708-1715},
  number = {11}
}

@ARTICLE{Rice:1965,
  author = {Rice, C. L. and Whitehead, R.},
  title = {Electrokinetic Flow in a Narrow Cylindrical Capillary},
  journal = {Journal of Physical Chemistry },
  year = {1965},
  volume = {69},
  pages = {4017-4024}
}

@ARTICLE{Richards:1977,
  author = {Richards, F. M. },
  title = {Areas, Volumes, Packing, and Protein Structure},
  journal = {Annual Review of Biophysics and Bioengineering},
  year = {1977},
  volume = {6},
  pages = {151--176},
  number = {1},
  bdsk-url-1 = {http://arjournals.annualreviews.org/doi/abs/10.1146/annurev.bb.06.060177.001055},
  bdsk-url-2 = {http://dx.doi.org/10.1146/annurev.bb.06.060177.001055},
  date-added = {2008-06-30 06:40:24 -0500},
  date-modified = {2008-06-30 06:40:24 -0500},
  doi = {10.1146/annurev.bb.06.060177.001055},
  keywords = {electrostatics, solvation, structure},
  posted-at = {2008-06-30 12:39:51},
  priority = {0},
  url = {http://arjournals.annualreviews.org/doi/abs/10.1146/annurev.bb.06.060177.001055}
}

@ARTICLE{Riehn:2005,
  author = {Riehn, R. and Lu, M. C. and Wang, Y. M. and Lim, S. F. and Cox, E.
	C. and Austin, R. H. },
  title = {Restriction mapping in nanofluidic devices },
  journal = {PNAS},
  year = {2005},
  volume = {102},
  pages = { 10012-10016 },
  number = { }
}

@ARTICLE{Robertson:2008,
  author = {Robertson, J. and Hall, D.A.},
  title = {Nonlinear dielectric properties of particulate barium titanate-polymer
	composites},
  journal = {Journal of Physics D: Applied Physices},
  year = {2008},
  volume = {41},
  pages = {115407-115414}
}

@ARTICLE{Robins99,
  author = {V. Robins},
  title = {Toward computing homology from finite approximations},
  journal = {Topology Proceedings},
  year = {1999},
  volume = {24},
  pages = {503-532},
  owner = {Yiying},
  timestamp = {2010.03.29}
}

@ARTICLE{Rocchia:2001,
  author = { Rocchia, W. and Alexov, E. and Honig, B.},
  title = {Extending the applicability of the nonlinear Poisson-Boltzmann equation:
	Multiple dielectric constants and multivalent ions},
  journal = {J. Phys. Chem.},
  year = {2001},
  volume = {105},
  pages = {6507-6514}
}




@ARTICLE{Rocchia:2002,
  author = { Rocchia, W. and Sridharan, S. and Nicholls, A. and Alexov, E and
	Chiabrera, A and Honig, B.},
  title = {{Rapid grid-based construction of the molecular surface and the use
	of induced surface charge to calculate reaction field energies: Applications
	to the molecular systems and geometric objects}},
  journal = {Journal of Computational Chemistry},
  year = {2002},
  volume = {23},
  pages = {128 - 137}
}


@ARTICLE{JLChen:1994,
  author = {Chen, J. L. and  Noodleman, Louis and Case, D. A. and  Bashford, D.},
  title = {Incorporating solvation effects into density-functional electronic-structure calculations
},
  journal = {J. Phys. Chem.},
  year = {1994},
  volume = {98},
  pages = { 11059-11068}
}

@ARTICLE{Romano:2007,
  author = {Romano, V.},
  title = {2D numerical simulation of the MEP energy-transport model with a
	finite difference scheme },
  journal = {J. Comput. Phys.},
  year = {2007},
  volume = {221},
  pages = {439-468},
  annote = {2D numerical simulation of the MEP energy-transport model with a
	finite difference scheme },
  date-added = {2008-11-25 10:28:56 -0500},
  date-modified = {2008-11-25 10:28:56 -0500},
  ty = {JOUR}
}

@ARTICLE{Rosenfeld:1988,
  author = {Rosenfeld, Y.},
  title = {Scaled field particle theory of the structure and the thermodynamics
	of isotropic hard particle fluids},
  journal = {Journal of Chemical Physics},
  year = {1988},
  volume = {89},
  pages = {4272-87},
  number = {7},
  abstract = {The pair structure and the thermodynamics of isotropic fluids composed
	of hard particles of different shapes and concentrations are considered
	by a new approach which (i) unifies the diagramatic PercusÃ¢Â€Â“Yevick
	theory and the geometric scaled particle theory, and (ii) leads to
	analytic accurate approximations for the direct correlation functions
	and cavity distribution functions. The scaled-particle interpolation
	idea of Reiss et al. is achieved diagramatically, approximating the
	full expansion of the direct correlation functions by appropriately
	renormalized low order graphs, in which the size of the field particle
	(``black circle'') is scaled. It is shown that the lowest order scaled
	field particle approximation, involving only pair excluded volumes
	as variables, and pair overlap volumes as functions, contains the
	exact solution of the PercusÃ¢Â€Â“Yevick integral equation
	for the general hard sphere mixture in D dimensions. An exact geometric
	relation obeyed by the excluded volume (covolume) of two fused convex
	bodies and another single convex body, is used to show that the scaled
	field particle theory is equivalent to thescaled particle expansion
	of the chemical potential in terms of the fundamental measures of
	the hard particles. This is in contrast to the conventional scaled
	particle Taylor series expansion in powers of the linear scale of
	the solute particle. The first order scaled field particle approximation
	and the ``fundamental measure'' scaled particle theory become identical
	when the fluid mixture contains only convex particles. For a D-dimensional
	(D=odd) hard spheres fluid mixture our new analysis enables to obtain
	the complete exact solution of the PercusÃ¢Â€Â“Yevick integral
	equation for the structure directly from its compressibility equation
	of state. This leads to the derivation of simple, analytic, geometric
	approximations for the direct correlation functions and cavity distribution
	functions of the general isotropic hard particle fluid, conformal
	to those for the hard sphere fluid mixture.},
  annote = {Scaled field particle theory of the structure and the thermodynamics
	of isotropic hard particle fluids},
  bdsk-url-1 = {http://dx.doi.org/10.1063/1.454810},
  date-added = {2008-09-17 09:14:02 -0500},
  date-modified = {2008-09-17 09:14:02 -0500},
  keywords = {Solvation; StatisticalMechanics},
  ty = {JOUR},
  url = {http://dx.doi.org/10.1063/1.454810}
}

@ARTICLE{Roth:2010,
  author = { Roth, R.},
  title = { Fundamental measure theory for hard-sphere mixtures: a review
	
	},
  journal = { J. Phys.: Condens. Matter },
  year = {2010},
  volume = {22},
  pages = {063102}
}

@ARTICLE{Roux1:2002,
  author = {Roux, Benoit },
  title = {Computational Studies of the {Gramicidin} Channel},
  journal = {Acc. Chem. Res.},
  year = {2002},
  volume = {35},
  pages = {366-375}
}

@ARTICLE{Roux:1997,
  author = {Roux, Benoit },
  title = {Influence of the Membrane Potential on the Free Energy of an Intrinsic
	Protein},
  journal = {Biophysical Journal},
  year = {1997},
  volume = {73},
  pages = {2980-2989},
  month = {December}
}

@ARTICLE{Roux:2004,
  author = {Roux, Benoit and Allen, Toby and Berneche, Simon and Im, Wonpil },
  title = {Theoretical and computational models of biological ionchannels},
  journal = {Quarterly Reviews of Biophysics},
  year = {2004},
  volume = {7},
  pages = {1-103},
  number = {1}
}

@ARTICLE{Roux:1999,
  author = {Roux, B. and Simonson, T.},
  title = {Implicit solvent models},
  journal = {Biophysical Chemistry},
  year = {1999},
  volume = {78},
  pages = {1-20},
  number = {1-2},
  abstract = {Implicit solvent models for biomolecular simulations are reviewed
	and their underlying statistical mechanical basis is discussed. The
	fundamental quantity that implicit models seek to approximate is
	the solute potential of mean force, which determines the statistical
	weight of solute conformations, and which is obtained by averaging
	over the solvent degrees of freedom. It is possible to express the
	total free energy as the reversible work performed in two successive
	steps. First, the solute is inserted in the solvent with zero atomic
	partial charges; second, the atomic partial charges of the solute
	are switched from zero to their full values. Consequently, the total
	solvation free energy corresponds to a sum of non-polar and electrostatic
	contributions. These two contributions are often approximated by
	simple geometrical models (such as solvent exposed area models) and
	by macroscopic continuum electrostatics, respectively. One powerful
	route is to approximate the average solvent density distribution
	around the solute, i.e. the soluteÃ¢Â€Â“solvent density correlation
	functions, as in statistical mechanical integral equations. Recent
	progress with semi-analytical approximations makes continuum electrostatics
	treatments very efficient. Still more efficient are fully empirical,
	knowledge-based models, whose relation to explicit solvent treatments
	is not fully resolved, however. Continuum models that treat both
	solute and solvent as dielectric continua are also discussed, and
	the relation between the solute fluctuations and its macroscopic
	dielectric constant(s) clarified.},
  address = {Univ Montreal Montreal, PQ Canada H3C 3J7 Roux, B Dept Phys, CP 6128,Succursale,Ctr
	Ville Univ Montreal Montreal, PQ Canada H3C 3J7 Dept Phys Univ Montreal
	Montreal, PQ Canada H3C 3J7 Dept Chim IGBMC Strasbourg France F-67404
	CNRS, Lab Biol Struct},
  annote = {Implicit solvent models; RouxSimonson},
  bdsk-url-1 = {http://dx.doi.org/10.1016/S0301-4622(98)00226-9},
  date-added = {2008-06-29 14:49:35 -0500},
  date-modified = {2008-06-29 14:49:35 -0500},
  journal1 = {Biophys Chem},
  keywords = {Electrostatics; Solvation},
  read = {Yes},
  url = {http://dx.doi.org/10.1016/S0301-4622(98)00226-9}
}

@ARTICLE{Rouy:867,
  author = {Elisabeth Rouy and Agnes Tourin},
  title = {A Viscosity Solutions Approach to Shape-From-Shading},
  journal = {SIAM J. on Num.l Analysis},
  year = {1992},
  volume = {29},
  pages = {867--884},
  number = {3}
}

@ARTICLE{LLE,
  author = {Sam Roweis and Lawrence Saul},
  title = {Nonlinear dimensionality reduction by locally linear embedding},
  journal = {Science},
  year = {2000},
  volume = {290},
  pages = {2323--2326},
  number = {5500}
}

@ARTICLE{Rowlinson:1979,
  author = {Rowlinson, J.S.},
  title = {Translation of {J}. {D}. van der {Waals}' ``The Thermodynamic Theory
	of Capillarity Under the Hypothesis of a Continuous Variation of
	Density ''},
  journal = {Journal of Statistical Physics},
  year = {1979},
  volume = {20},
  pages = {197-200.},
  number = {2}
}

@ARTICLE{Roy:2010(b),
  author = {Roy, A. and Kucukural, A. and Mukherjee, S. and Hefty, P. S. and
	Zhang, Y.},
  title = {{Large scale benchmarking of protein function prediction using modeled
	predicted protein structures}},
  journal = {J Mol Biol},
  year = {2010:Submitted}
}

@ARTICLE{Roy:2010(a),
  author = {Roy, A. and Kucukural, A. and Zhang, Y.},
  title = {{I-TASSER: a unified platform for automated protein structure and
	function prediction}},
  journal = {Nat Protoc},
  year = {2010},
  volume = {5},
  pages = {725-738},
  number = {4}
}

@ARTICLE{Roy:2009,
  author = {Roy, A. and Wu, S. and Zhang, Y.},
  title = {{Composite approaches to protein tertiary structure prediction: A
	case-study by I-TASSER}},
  journal = {In: Rangwala H, Karypis G, editors. Protein Structure Prediction:
	Method and Algorithms},
  year = {2009},
  pages = {243-264}
}

@BOOK{Rubinstein:1990,
  title = {{Electro-diffusion of ions.}},
  publisher = {Philadelphia: SIAM.},
  year = {1990},
  author = {Rubinstein, I}
}


@INPROCEEDINGS{Rudin:1992,
  author = {Rudin, Leonid I. and Osher, Stanley and Fatemi, Emad },
  title = {Nonlinear total variation based noise removal algorithms},
  booktitle = {Proceedings of the eleventh annual international conference of the
	Center for Nonlinear Studies on Experimental mathematics : computational
	issues in nonlinear science},
  year = {1992},
  pages = {259--268},
  address = {Amsterdam, The Netherlands, The Netherlands},
  publisher = {Elsevier North-Holland, Inc.},
  bdsk-url-1 = {http://portal.acm.org/citation.cfm?id=142312},
  bdsk-url-2 = {http://dx.doi.org/10.1016/0167-2789(92)90242-F},
  date-added = {2008-06-30 21:22:09 -0400},
  date-modified = {2008-06-30 21:22:09 -0400},
  doi = {10.1016/0167-2789(92)90242-F},
  issn = {0167-2789},
  keywords = {mathematics},
  posted-at = {2008-07-01 02:21:35},
  priority = {2},
  url = {http://portal.acm.org/citation.cfm?id=142312}
}

@ARTICLE{rusinkiewicz2001evi,
  author = {Rusinkiewicz, S. and Levoy, M.},
  title = {{Efficient variants of the ICP algorithm}},
  journal = {Proc. 3DIM},
  year = {2001},
  pages = {145--152}
}

@ARTICLE{Rzepiela:2010,
  author = {Rzepiela, A.J. and Schafer, L.V. and Goga, N. and Risselada, H.J.
	and De Vries, A.H. and Marrink, S.J.},
  title = {Software News and Update Reconstruction of Atomistic Details from
	Coarse-Grained Structures},
  journal = {Journal of Computational Chemistry},
  year = {2010},
  volume = {31},
  pages = {1333-1343 }
}

@ARTICLE{Sabatelli:2002,
  author = {Sabatelli,L. and Keating,S. and Dudley,J. and Richmond,P.},
  title = {Waiting time distributions in Financial markets},
  journal = {Eur.Phys.J.B},
  year = {2002},
  volume = {27},
  pages = {273?C275},
  number = { }
}

@ARTICLE{Saito:2002,
  author = {Saito, T. and Saraya, T. and Inukai, T. and Majimi, H. and Nangumo,
	T. and Hiramoto, T.},
  title = {Suppression of short channel effect in triangular parallel wire channel
	MOSFETs},
  journal = {IEICE Trans. Electron},
  year = {2002},
  volume = {E85C},
  pages = {1073 - 1080},
  annote = {Suppression of short channel effect in triangular parallel wire channel
	MOSFETs},
  date-added = {2008-11-25 10:28:56 -0500},
  date-modified = {2008-11-25 10:28:56 -0500},
  ty = {JOUR}
}

@ARTICLE{Sakurai:2001,
  author = {Sakurai, Kazumasa and Oobatake, Motohisa and Goto, Yuji},
  title = {Salt-dependent monomer - dimer equilibrium of bovine $\beta$ -lactoglobulin
	at pH 3},
  journal = {Protein Sci},
  year = {2001},
  volume = {10},
  pages = {2325-2335},
  number = { }
}

@ARTICLE{Samudrala:1998,
  author = {Samudrala, R. and Moult, J.},
  title = {{An all-atom distance-dependent conditional probability discriminatory
	function for protein structure prediction}},
  journal = {J Mol Biol},
  year = {1998},
  volume = {275},
  pages = {895-916},
  number = {5}
}

@ARTICLE{PMV,
  author = {Sanner, Michel F.},
  title = {Python: a programming language for software integration and development},
  journal = {J. Mol. Graphics Mod.},
  year = {1999},
  volume = {17},
  pages = {57-61},
  annote = {Python: a programming language for software integration and development},
  date-added = {2008-09-17 09:19:18 -0500},
  date-modified = {2008-09-17 09:19:18 -0500},
  keywords = {Software},
  ty = {JOUR}
}

@ARTICLE{Sanner:1996,
  author = {Sanner, M. F. and Olson, A. J. and Spehner, J. C.},
  title = {Reduced surface: An efficient way to compute molecular surfaces },
  journal = {Biopolymers},
  year = {1996},
  volume = {38},
  pages = {305-320},
  annote = {Reduced surface: An efficient way to compute molecular surfaces },
  date-added = {2008-09-17 09:19:18 -0500},
  date-modified = {2008-09-17 09:19:18 -0500},
  keywords = {Software},
  ty = {JOUR}
}

@ARTICLE{Sansom:1996,
  author = {Sansom, Msp and Kerr, Id and Breed, J and Sankararamakrishnan, R
	},
  title = {Water in channel-like cavities: structure and dynamics},
  journal = {Biophys J},
  year = {1996},
  volume = {70},
  pages = {693-702}
}

@ARTICLE{Sapiro:1996,
  author = {Sapiro, G. and Ringach, D. L. },
  title = {Anisotropic diffusion of multivalued images with applications to
	color filtering},
  journal = {Image Processing, IEEE Transactions on},
  year = {1996},
  volume = {5},
  pages = {1582--1586},
  number = {11},
  abstract = {A general framework for anisotropic diffusion of multivalued images
	is presented. We propose an evolution equation where, at each point
	in time, the directions and magnitudes of the maximal and minimal
	rate of change in the vector-image are first evaluated. These are
	given by eigenvectors and eigenvalues of the first fundamental form
	in the given image metric. Then, the image diffuses via a system
	of coupled differential equations in the direction of minimal change.
	The diffusion \&ldquo;strength\&rdquo; is controlled by a function
	that measures the degree of dissimilarity between the eigenvalues.
	We apply the proposed framework to the filtering of color images
	represented in CIE-L*a*b* space},
  bdsk-url-1 = {http://ieeexplore.ieee.org/xpls/abs%5C_all.jsp?arnumber=541429},
  booktitle = {Image Processing, IEEE Transactions on},
  date-added = {2008-09-16 15:02:39 -0500},
  date-modified = {2008-09-16 15:02:44 -0500},
  keywords = {colour, segmentation},
  posted-at = {2007-11-12 11:04:03},
  priority = {0},
  url = {http://ieeexplore.ieee.org/xpls/abs\_all.jsp?arnumber=541429}
}

@ARTICLE{Sapp:2009,
  author = {Sapp, M. and Day, P.M.},
  title = {Structure, attachment and entry of polyoma- and papillomaviruses},
  journal = {Rirology},
  year = {2009},
  volume = {384},
  pages = {400-409},
  annote = {Structure, attachment and entry of polyoma- and papillomaviruses},
  date-added = {2009-03-10 },
  date-modified = {2009-03-10},
  ty = {JOUR}
}

@ARTICLE{Saraniti:2006,
  author = {Saraniti, Marco and Aboud, Shela and Eisenberg, B. S.},
  title = {The Simulation of Ionic Charge Transport in Biological Ion Channels:
	an Introduction to Numerical Methods},
  journal = {Reviews in Computational Chemistry},
  year = {2006},
  volume = {22},
  pages = {229-294}
}

@ARTICLE{Sarti:2002,
  author = {Sarti, A. and Malladi, R. and Sethian, J. A. },
  title = {Subjective Surfaces: A Geometric Model for Boundary Completion},
  journal = {International Journal of Computer Vision},
  year = {2002},
  volume = {46},
  pages = {201--221},
  number = {3},
  abstract = {We present a geometric model and a computational method for segmentation
	of images with missing boundaries. In many situations, the human
	visual system fills in missing gaps in edges and boundaries, building
	and completing information that is not present. Boundary completion
	presents a considerable challenge in computer vision, since most
	algorithms attempt to exploit existing data. A large body of work
	concerns completion models, which postulate how to construct missing
	data; these models are often trained and specific to particular images.
	In this paper, we take the following, alternative perspective: we
	consider a given reference point within the image, and then develop
	an algorithm which tries to build missing information on the basis
	of the given point of view and the available information as boundary
	data to the algorithm. Starting from this point of view, a surface
	is constructed. It is then evolved with the mean curvature flow in
	the metric induced by the image until a piecewise constant solution
	is reached. We test the computational model on modal completion,
	amodal completion, and texture segmentation. We extend the geometric
	model and the algorithm to 3D in order to extract shapes from low
	signal/noise ratio ultrasound image volumes. Results in 3D echocardiography
	and 3D fetal echography are also presented.},
  bdsk-url-1 = {http://dx.doi.org/10.1023/A:1014028906229},
  date-added = {2008-06-30 21:11:03 -0400},
  date-modified = {2008-06-30 21:11:03 -0400},
  doi = {10.1023/A:1014028906229},
  keywords = {mathematics},
  posted-at = {2008-07-01 02:10:29},
  priority = {0},
  url = {http://dx.doi.org/10.1023/A:1014028906229}
}

@ARTICLE{Savelyev:2007,
  author = {Savelyev, A. and Papoian, G. A.},
  title = {Inter-{DNA} Electrostatics from Explicit Solvent Molecular Dynamics
	Simulations},
  journal = {Journal of the American Chemical Society},
  year = {2007},
  volume = {129},
  pages = {6060-1},
  number = {19},
  abstract = {Electrostatic repulsion between two DNA molecules, computed from explicit
	water-free energy simulations, is screened stronger by Na+ counterions
	than K+ counterions. An effective electrostatic potential was constructed
	for a coarse-grained model, where each base pair is represented by
	a bead.},
  bdsk-url-1 = {http://dx.doi.org/10.1021/ja070207t},
  date-added = {2008-09-01 14:05:48 -0500},
  date-modified = {2008-09-01 14:05:48 -0500},
  keywords = {Electrostatics; NucleicAcids},
  url = {http://dx.doi.org/10.1021/ja070207t}
}

@ARTICLE{SaxenaGH:2009,
  author = {Saxena, R. and Gelb, A. and Mittelmann, H.},
  title = {A high order method for determining the edges in the gradient of
	a function},
  journal = {Commun. Comput. Phys.},
  year = {2009},
  volume = {5},
  pages = {694-711 },
  annote = {A high order method for determining the edges in the gradient of
	a function},
  date-added = {2008-11-25 10:28:56 -0500},
  date-modified = {2008-11-25 10:28:56 -0500},
  ty = {JOUR}
}

@ARTICLE{Sbert:2003,
  author = {Sbert, Catalina and Sol\'{e}, Andreas F. },
  title = {3D Curves Reconstruction Based on Deformable Models},
  journal = {Journal of Mathematical Imaging and Vision},
  year = {2003},
  volume = {18},
  pages = {211--223},
  number = {3},
  abstract = {We present a new method, based on curve evolution, for the reconstruction
	of a 3D curve from two different projections. It is based on the
	minimization of an energy functional. Following the work on geodesic
	active contours by Caselles et al. (in Int. Conf. on Pattern Recognition,
	1996, Vol. 43, pp. 693--737), we then transform the problem of minimizing
	the functional into a problem of geodesic computation in a Riemann
	space. The Euler-Lagrange equation of this new functional is derived
	and its associated PDE is solved using the level set formulation,
	giving the existence and uniqueness results. We apply the model to
	the reconstruction of a vessel from a biplane angiography.},
  bdsk-url-1 = {http://dx.doi.org/10.1023/A:1022821409482},
  date-added = {2008-06-30 21:12:52 -0400},
  date-modified = {2008-06-30 21:12:52 -0400},
  doi = {10.1023/A:1022821409482},
  keywords = {mathematics},
  posted-at = {2008-07-01 02:12:19},
  priority = {0},
  url = {http://dx.doi.org/10.1023/A:1022821409482}
}

@ARTICLE{Scaldaferri:2007,
  author = {Scaldaferri, S. and Curatola, G. and Iannaccone, G.},
  title = {{Direct solution of the Boltzmann transport equation and Poisson-Schr\"{o}dinger
	equation for nanoscale MOSFETs }},
  journal = {IEEE T. Electron Devices},
  year = {2007},
  volume = {54},
  pages = {2901-2909 },
  annote = {Direct solution of the boltzmann transport equation and poisson-schrodinger
	equation for nanoscale MOSFETs },
  date-added = {2008-11-25 10:28:56 -0500},
  date-modified = {2008-11-25 10:28:56 -0500},
  ty = {JOUR}
}

@ARTICLE{LSVOF,
  author = {Ruben Scardovelli and Stephane Zaleski},
  title = {{Interface Reconstruction with Least-Square Fit and Split Eulerian-Lagrangian
	Advection}},
  journal = {Int. J. Numer. Meth. Fluids},
  year = {2003},
  volume = {41},
  pages = {251--274}
}

@ARTICLE{netgen,
  author = {Sch\"{o}berl, Joachim},
  title = {NETGEN - An Advancing Front 2D/3D Mesh Generator Based on Abstract
	Rules},
  journal = {Comput and Vis in Science},
  year = {1997},
  volume = {1},
  pages = {41--52},
  number = {1}
}

@ARTICLE{Schaefer:1996,
  author = {Schaefer, M. and Karplus, M.},
  title = {A comprehensive analytical treatment of continuum electrostatics},
  journal = {Journal of Physical Chemistry},
  year = {1996},
  volume = {100},
  pages = {1578-1599},
  number = {5},
  abstract = {An analytical treatment of the continuum model for electrostatic solvation
	is presented and shown to be in good agreement with numerical finite-difference
	continuum calculations for the same system. Because the analytic
	method, called ACE, is relatively fast and yields a pairwise potential
	from which gradients and second derivatives can be obtained, its
	use with molecular mechanics/molecular dynamics programs will be
	possible. For calculating the self-energies of molecules in aqueous
	solution, a new analytic method is introduced. It is based on a continuum
	electrostatics model in which charges are defined as Gaussian charge
	distributions, rather than point charges, and in which the solute
	interior is described by a continuous density function. The self-energy
	potential is a pairwise energy function which only depends on charges,
	interatomic distances, and the effective, solvent-inaccessible volumes
	of the atoms. The potential is derived by integrating the energy
	density of the electric field and termed the integrated field (IF)
	method. A combination of the analytic self-energy potential with
	the generalized Born equation for charge-charge interactions,(1-3)
	termed analytic continuum electrostatics (ACE) potential, makes possible
	an analytic treatment of the electrostatic contribution to solvation.
	The focusing of field lines is included. The TF method is applied
	to the calculation of self-energies of all charges on a series of
	small organic compounds and the protein bovine pancreatic trypsin
	inhibitor (BPTI). The agreement with self-energies as calculated
	using a finite-difference program is excellent for small molecules
	and satisfactory for BPTI. Application of the combined ACE potential
	to the calculation of solvation energies of small compounds shows
	good agreement with results of finite-difference calculations. The
	potential on a plane through the protein superoxide dismutase using
	ACE and a finite-difference program is in good agreement. For the
	calculation of the solvation energies of small molecules (20 atoms),
	ACE is more than 3 orders of magnitude faster than the program UHBD91
	which was used for all numerical continuum electrostatics calculations;
	for BPTI, the speedup is more than 2 orders of magnitude.},
  address = {Schaefer, M. Harvard Univ,Dept Chem,12 Oxford St,Cambridge,Ma 02138
	Univ Louis Pasteur Strasbourg 1,Inst Le Bel,Lab Chim Biophys,F-67000
	Strasbourg,France},
  annote = {FEB 1; A comprehensive analytical treatment of continuum electrostatics;
	ISI:A1996TT53300022; ACE; Times Cited: 90 Review English Cited References
	Count: 121 Tt533},
  bdsk-url-1 = {http://dx.doi.org/10.1021/jp9521621},
  date-added = {2008-09-01 13:57:48 -0500},
  date-modified = {2008-09-01 13:57:48 -0500},
  journal1 = {J Phys Chem-Us},
  keywords = {Electrostatics; Solvation},
  ty = {JOUR},
  url = {http://dx.doi.org/10.1021/jp9521621}
}

@ARTICLE{Schmitt:1999,
  author = {Schmitt, Udo W. and Voth, Gregory A.},
  title = {{The computer simulation of proton transport in water}},
  journal = {Journal of Chemical Physics},
  year = {1999},
  volume = {111},
  pages = {9361-9381}
}

@ARTICLE{Schnell:2008,
  author = {Schnell,Jason R. and Chou, James J.},
  title = {Structure and mechanism of the {M2} proton channel of {influenza
	A} virus},
  journal = {Nature},
  year = {2008},
  volume = {451},
  pages = {591-596},
  month = {January}
}

@ARTICLE{Schnieders:2007b,
  author = {Schnieders, M.J. and Ponder J.W.},
  title = {Polarizable atomic multipole solutes in a generalized Kirkwood continuum},
  journal = {Journal of Chemical Theory and Computation},
  year = {2007},
  volume = {3},
  pages = {2083-2097}
}

@ARTICLE{Schnieders:2007,
  author = {Schnieders, M. J. and Baker, N. A. and Ren, P. and Ponder, J. W.},
  title = {Polarizable atomic multipole solutes in a {{Poisson-Boltzmann}} continuum},
  journal = {Journal of Chemical Physics},
  year = {2007},
  volume = {126},
  pages = {124114},
  abstract = {Modeling the change in the electrostatics of organic molecules upon
	moving from vacuum into solvent, due to polarization, has long been
	an interesting problem. In vacuum, experimental values for the dipole
	moments and polarizabilities of small, rigid molecules are known
	to high accuracy; however, it has generally been difficult to determine
	these quantities for a polar molecule in water. A theoretical approach
	introduced by Onsager [J. Am. Chem. Soc. 58, 1486 (1936)] used vacuum
	properties of small molecules, including polarizability, dipole moment,
	and size, to predict experimentally known permittivities of neat
	liquids via the Poisson equation. Since this important advance in
	understanding the condensed phase, a large number of computational
	methods have been developed to study solutes embedded in a continuum
	via numerical solutions to the {Poisson-Boltzmann} equation. Only
	recently have the classical force fields used for studying biomolecules
	begun to include explicit polarization in their functional forms.
	Here the authors describe the theory underlying a newly developed
	polarizable multipole {Poisson-Boltzmann} (PMPB) continuum electrostatics
	model, which builds on the atomic multipole optimized energetics
	for biomolecular applications (AMOEBA) force field. As an application
	of the PMPB methodology, results are presented for several small
	folded proteins studied by molecular dynamics in explicit water as
	well as embedded in the PMPB continuum. The dipole moment of each
	protein increased on average by a factor of 1.27 in explicit AMOEBA
	water and 1.26 in continuum solvent. The essentially identical electrostatic
	response in both models suggests that PMPB electrostatics offers
	an efficient alternative to sampling explicit solvent molecules for
	a variety of interesting applications, including binding energies,
	conformational analysis, and pKa prediction. Introduction of 150
	mM salt lowered the electrostatic solvation energy between 2 and
	13 kcal/mole, depending on the formal charge of the protein, but
	had only a small influence on dipole moments},
  bdsk-file-1 = {YnBsaXN0MDDUAQIDBAUGCQpYJHZlcnNpb25UJHRvcFkkYXJjaGl2ZXJYJG9iamVjdHMSAAGGoNE
	HCFRyb290gAFfEA9OU0tleWVkQXJjaGl2ZXKoCwwXGBkdJCVVJG51bGzTDQ4PEBEUViRjbGFzc1
	dOUy5rZXlzWk5TLm9iamVjdHOAB6ISE4ACgAOiFRaABIAGWWFsaWFzRGF0YVxyZWxhdGl2ZVBhd
	GjSDRobHFdOUy5kYXRhgAVPEQHwAAAAAAHwAAIAAAxNYWNpbnRvc2ggSEQAAAAAAAAAAAAAAAAA
	AADD4v5NSCsAAAAZYksfMjAwNy1TY2huaWVkZXJzQmFrZXIjMTk2Mjk3LnBkZgAAAAAAAAAAAAA
	AAAAAAAAAAAAAAAAAAAAAAAAAAAAAABlil8Iy8fgAAAAAAAAAAAAEAAQAAAkgAAAAAAAAAAAAAA
	AAAAAAB0FyY2hpdmUAABAACAAAw+NSrQAAABEACAAAwjM4SAAAAAEAFAAZYksAGWIDAAqkKAAKp
	BEAAHrcAAIAVU1hY2ludG9zaCBIRDpVc2VyczpiYWtlcjpEb2N1bWVudHM6UmVmZXJlbmNlczpB
	cmNoaXZlOjIwMDctU2NobmllZGVyc0Jha2VyIzE5NjI5Ny5wZGYAAA4ARAAhADIAMAAwADcALQB
	TAGMAaABuAGkAZQBkAGUAcgBzAEIAYQBrAGUAcgBSAGUAbgBQAG8AbgBkAGUAcgAuAHAAZABmAA
	8AGgAMAE0AYQBjAGkAbgB0AG8AcwBoACAASABEABIASlVzZXJzL2Jha2VyL0RvY3VtZW50cy9SZ
	WZlcmVuY2VzL0FyY2hpdmUvMjAwNy1TY2huaWVkZXJzQmFrZXJSZW5Qb25kZXIucGRmABMAAS8A
	ABUAAgAM//8AANIeHyAhWCRjbGFzc2VzWiRjbGFzc25hbWWjISIjXU5TTXV0YWJsZURhdGFWTlN
	EYXRhWE5TT2JqZWN0XxBKLi4vLi4vLi4vLi4vRG9jdW1lbnRzL1JlZmVyZW5jZXMvQXJjaGl2ZS
	8yMDA3LVNjaG5pZWRlcnNCYWtlclJlblBvbmRlci5wZGbSHh8mJ6InI1xOU0RpY3Rpb25hcnkAC
	AARABoAHwApADIANwA6AD8AQQBTAFwAYgBpAHAAeACDAIUAiACKAIwAjwCRAJMAnQCqAK8AtwC5
	Aq0CsgK7AsYCygLYAt8C6AM1AzoDPQAAAAAAAAIBAAAAAAAAACgAAAAAAAAAAAAAAAAAAANK},
  bdsk-url-1 = {http://dx.doi.org/10.1063/1.2714528},
  date-added = {2008-09-17 09:22:18 -0500},
  date-modified = {2008-09-17 09:22:18 -0500},
  keywords = {Electrostatics; Solvation},
  read = {Yes},
  url = {http://dx.doi.org/10.1063/1.2714528}
}

@ARTICLE{schreiner2004ism,
  author = {Schreiner, J. and Asirvatham, A. and Praun, E. and Hoppe, H.},
  title = {{Inter-surface mapping}},
  journal = {ACM Transactions on Graphics (TOG)},
  year = {2004},
  volume = {23},
  pages = {870-877},
  number = {3},
  publisher = {ACM Press New York, NY, USA}
}

@INBOOK{PeterGeoMeasure,
  pages = {8--12},
  title = {{What Can We Measure}},
  publisher = {ACM SIGGRAPH Course Lecture Notes},
  year = {2006},
  author = {P. Schr{\"o}der},
  series = {Discrete Differential Geometry, E. Grinspun, P. Schr{\"o}der, M.
	Desbrun (Eds.)}
}

@ARTICLE{Schulz:2002,
  author = {Schulz, Martin and Steinebach, Gerd},
  title = {Two-dimensional modelling of the river {Rhine}},
  journal = {Journal of Computational and Applied Mathematics},
  year = {2002},
  volume = {145},
  pages = {11--20},
  number = {1},
  abstract = { The system for operational water level forecast and prediction of
	(fortunately not daily) pollutant transport for the river Rhine is
	in daily use. This model is based on the Saint-Venant or one-dimensional
	shallow water equations. The model is augmented by additional terms
	and equations to model the effect of dead zones and the transport
	of soluble components. The next step is to move towards two-dimensional
	models. An important problem that arises is that the domain of the
	fluid is not fixed by the given data, but depends on the water level
	and is therefore part of the solution of the model. Even worse, depending
	on the topography of the river bed, even the topology of the fluid
	domain may change, as islands may appear at low water and get flooded
	at high water situations.},
  bdsk-url-1 = {http://www.sciencedirect.com/science/article/B6TYH-4475Y60-3/2/2dde189a99039cd454328f210e524f4d},
  date-added = {2008-09-14 15:32:12 -0500},
  date-modified = {2008-09-14 15:32:12 -0500},
  doi = {10.1016/S0377-0427(01)00532-5 },
  keywords = {Mathematics; FluidMechanics},
  ty = {JOUR},
  url = {http://www.sciencedirect.com/science/article/B6TYH-4475Y60-3/2/2dde189a99039cd454328f210e524f4d}
}

@ARTICLE{Schumaker:2000,
  author = {Schumaker, Mark F. and Pomes, Regis and Roux, Benoit },
  title = {A Combined Molecular Dynamics and Diffusion Model of Single Proton
	Conduction through {Gramicidin}},
  journal = {Biophysical Journal},
  year = {2000},
  volume = {79},
  pages = {2840-2857},
  month = {December}
}

@ARTICLE{Schuss:2001,
  author = {Schuss, Z. and Nadler, B. and Eisenberg, B. S. },
  title = {{Derivation of Poisson and Nernst-Planck equations in a bath and
	channel from a molecular model}},
  journal = {Phys. Rev. E Stat Nonlin Soft Matter Phys},
  year = {2001},
  volume = {64},
  pages = {036116}
}

@ARTICLE{Schwede:2006,
  author = {Schwede, T.},
  title = {{Assessment of Template Based Modeling at CASP7, in{Assessment talk
	given at CASP7 conference. Asilomar Conference Center, Pacific Grove,
	CA}}},
  year = {2006}
}

@ARTICLE{Schwinger:1961,
  author = {Schwinger, J.},
  title = {Brownian motion of a quantum oscillator},
  journal = {J. Math. Phys.},
  year = {1961},
  volume = {2},
  pages = {407-432},
  annote = {Brownian motion of a quantum oscillator},
  date-added = {2008-11-25 10:28:56 -0500},
  date-modified = {2008-11-25 10:28:56 -0500},
  ty = {JOUR}
}

@ARTICLE{Sciubba:2004,
  author = {Sciubba, Enrico},
  title = {Flow Exergy as a Lagrangian for the {{Navier-Stokes}} Equations for
	Incompressible Flow},
  journal = {Int. J. Thermodynamics},
  year = {2004},
  volume = {7},
  pages = {115-122}
}

@ARTICLE{Selle05,
  author = {Andrew Selle and Nick Rasmussen and Ronald Fedkiw},
  title = {{A Vortex Particle Method for Smoke, Water and Explosions}},
  journal = {ACM Trans. Graph.},
  year = {2005},
  volume = {24},
  pages = {910--914},
  number = {3},
  month = aug
}

@ARTICLE{Sept:1999,
  author = {Sept, D. and Elcock, A. H. and McCammon, J. A.},
  title = {Computer simulations of actin polymerization can explain the barbed-pointed
	end asymmetry},
  journal = {Journal of Molecular Biology},
  year = {1999},
  volume = {294},
  pages = {1181-1189},
  number = {5},
  abstract = {Computer simulations of actin polymerization were performed to investigate
	the role of electrostatic interactions in determining polymerization
	rates. Atomically detailed models of actin monomers and filaments
	were used in conjunction with a Brownian dynamics method. The simulations
	were able to reproduce the measured barbed end association rates
	over a range of ionic strengths and predicted a slower growing pointed
	end, in agreement with experiment. Similar simulations neglecting
	electrostatic interactions indicate that configurational and entropic
	factors may actually favor polymerization at the pointed end, but
	electrostatic interactions remove this trend. This result would indicate
	that polymerization at the pointed end is not only limited by diffusion,
	but faces electrostatic forces that oppose binding. The binding of
	the actin depolymerizing factor (ADF) and G-actin complex to the
	end of a filament was also simulated. In this case, electrostatic
	steering effects lead to an increase in the simulated association
	rate. Together, the results indicate that simulations provide a realistic
	description of both polymerization and the binding of more complex
	structures to actin filaments.},
  address = {Univ Calif San Diego La Jolla, CA USA 92093 Sept, D dsept{\char64}ucsd.edu
	Dept Chem \& Biochem Univ Calif San Diego La Jolla, CA USA 92093
	Dept Chem \& Biochem Univ Calif San Diego La Jolla, CA USA 92093
	Dept Pharmacol},
  annote = {Computer simulations of actin polymerization can explain the barbed-pointed
	end asymmetry; DEC 17},
  bdsk-url-1 = {http://dx.doi.org/10.1006/jmbi.1999.3332},
  date-added = {2008-09-01 13:55:30 -0500},
  date-modified = {2008-09-01 13:55:30 -0500},
  journal1 = {J Mol Biol},
  keywords = {Diffusion; Electrostatics},
  ty = {JOUR},
  url = {http://dx.doi.org/10.1006/jmbi.1999.3332}
}

@ARTICLE{Sept:2001,
  author = {Sept, D. and McCammon, J. A.},
  title = {Thermodynamics and kinetics of actin filament nucleation},
  journal = {Biophysical Journal},
  year = {2001},
  volume = {81},
  pages = {667-674},
  number = {2},
  abstract = {We have performed computer simulations and free energy calculations
	to determine the thermodynamics and kinetics of actin nucleation
	and thus identify a probable nucleation pathway and critical nucleus
	size. The binding free energies of structures along the nucleation
	pathway are found through a combination of electrostatic calculations
	and estimates of the entropic and surface area contributions. The
	association kinetics for the formation of each structure are determined
	through a series of Brownian dynamics simulations. The combination
	of the binding free energies and the association rate constants determines
	the dissociation rate constants, allowing for a complete characterization
	of the nucleation and polymerization kinetics. The results indicate
	that the trimer is the size of the critical nucleus, and the rate
	constants produce polymerization plots that agree very well with
	experimental results over a range of actin monomer concentrations.},
  address = {Washington Univ St Louis, MO USA 63130 Sept, D dsept{\char64}biomed.wustl.edu
	Dept Biomed Engn, Campus Box 1097 Washington Univ St Louis, MO USA
	63130 Dept Biomed Engn Washington Univ St Louis, MO USA 63130 Ctr
	Computat BIol Univ Calif San Diego La Jolla, CA USA 92093 Howard
	Hughes Med Inst, Dept Chem \& Biochem Univ Calif San Diego La Jolla,
	CA USA 92093 Dept Pharmacol},
  annote = {Thermodynamics and kinetics of actin filament nucleation; AUG},
  bdsk-url-1 = {http://www.biophysj.org/cgi/content/abstract/81/2/667},
  date-added = {2008-09-01 14:02:00 -0500},
  date-modified = {2008-09-01 14:02:00 -0500},
  journal1 = {Biophys J},
  keywords = {Electrostatics; Diffusion},
  ty = {JOUR},
  url = {http://www.biophysj.org/cgi/content/abstract/81/2/667}
}

@INPROCEEDINGS{Serna2011,
  author = {Serna, S Pena and Stork, A and Fellner, D W},
  title = {{Considerations toward a Dynamic Mesh Data Structure}},
  booktitle = {SIGRAD Conference},
  year = {2011},
  pages = {83--90},
  file = {:C\:/Dropbox/Dropbox/Paper/ecp11065012.pdf:pdf},
  owner = {doubletony},
  timestamp = {2012.04.26}
}

@ARTICLE{Sethian:2001,
  author = {Sethian, J. A. },
  title = {Evolution, Implementation, and Application of Level Set and Fast
	Marching Methods for Advancing Fronts},
  journal = {J. Comput. Phys.},
  year = {2001},
  volume = {169},
  pages = {503--555},
  number = {2},
  abstract = {A variety of numerical techniques are available for tracking moving
	interfaces. In this review, we concentrate on techniques that result
	from the link between the partial differential equations that describe
	moving interfaces and numerical schemes designed for approximating
	the solutions to hyperbolic conservation laws. This link gives rise
	to computational techniques for tracking moving interfaces in two
	and three space dimensions under complex speed laws. We discuss the
	evolution of these techniques, the fundamental numerical approximations,
	involved, implementation details, and applications. In particular,
	we review some work on three aspects of materials sciences: semiconductor
	process simulations, seismic processing, and optimal structural topology
	design.},
  bdsk-url-1 = {http://dx.doi.org/10.1006/jcph.2000.6657},
  date-added = {2008-06-30 21:15:39 -0400},
  date-modified = {2008-06-30 21:15:39 -0400},
  doi = {10.1006/jcph.2000.6657},
  keywords = {mathematics},
  posted-at = {2008-07-01 02:15:08},
  priority = {0},
  url = {http://dx.doi.org/10.1006/jcph.2000.6657}
}

@BOOK{SethianBook,
  title = {Level Set Methods and Fast Marching Methods},
  publisher = {Cambridge University Press},
  year = {1999},
  author = {Sethian, J. A.},
  volume = {3},
  series = {Monographs on Appl. Comput. Math.},
  address = {Cambridge},
  edition = {2nd}
}

@ARTICLE{Shadden,
  author = {S.C. Shadden and F. Lekien and J.E. Marsden},
  title = {Definition and Properties of Lagrangian Coherent Structures from
	Finite-Time Lyapunov Exponents in Two-Dimensional Aperiodic Flows},
  journal = {Physica D},
  year = {2005},
  volume = {212},
  pages = {271?304},
  number = {3-4}
}

@ARTICLE{Sham:1998,
  author = {Sham, Y. Y. and Muegge, I. and Warshel, A.},
  title = {The effect of protein relaxation on charge-charge interactions and
	dielectric constants of proteins},
  journal = {Biophysical Journal},
  year = {1998},
  volume = {74},
  pages = {1744-1753},
  number = {4},
  abstract = {The effect of the reorganization of the protein polar groups on charge-charge
	interaction and the corresponding effective dielectric constant (eff)
	is examined by the semimicroscopic version of the Protein Dipole
	Langevin Dipoles (PDLD/S) method within the framework of the Linear
	Response Approximation (LRA). This is done by evaluating the interactions
	between ionized residues in the reaction center of Rhodobacter sphaeroides,
	while taking into account the protein reorganization energy. It is
	found that an explicit consideration of the protein relaxation leads
	to a significant increase in eff and that semimicroscopic models
	that do not take this relaxation into account force one to use a
	large value for the so-called {\tt{}"{}}protein dielectric constant,{\tt{}"{}}
	p, of the {Poisson-Boltzmann} model or for the corresponding in in
	the PDLD/S model. An additional increase in eff is expected from
	the reorganization of ionized residues and from changes in the degree
	of water penetration. This finding provides further support for the
	idea that in (or p) represents contributions that are not considered
	explicitly. The present study also provides a systematic illustration
	of the nature of eff, supporting our previously reported view that
	charge-charge interactions correspond to a large value of this {\tt{}"{}}dielectric
	constant,{\tt{}"{}} even in protein interiors. It is also pointed
	out that eff for the interaction between ionizable groups in proteins
	is very different from the effective dielectric constant, 'eff, that
	determines the free energy of ion pairs in proteins ('eff reflects
	the effect of preoriented protein dipoles). Finally, the problems
	associated with the search for a general in are discussed. It is
	clarified that the in that reproduces the effect of protein relaxation
	on charge-charge interaction is not equal to the in that reproduces
	the corresponding effect upon formation of individual charges. This
	reflects fundamental inconsistencies in attempts to cast microscopic
	concepts in a macroscopic model. Thus one should either use a large
	in for charge-charge interactions and a small in for charge-dipole
	interactions or consider the protein relaxation microscopically.},
  address = {UNIV SO CALIF LOS ANGELES, CA USA 90089 Warshel, A DEPT CHEM Univ
	so calif los angeles, ca usa 90089 dept chem},
  annote = {The effect of protein relaxation on charge-charge interactions and
	dielectric constants of proteins; APR},
  bdsk-url-1 = {http://www.biophysj.org/cgi/content/full/74/4/1744%20http://www.biophysj.org},
  date-added = {2008-09-01 13:58:09 -0500},
  date-modified = {2008-09-01 13:58:09 -0500},
  journal1 = {Biophys J},
  keywords = {Electrostatics},
  ty = {JOUR},
  url = {http://www.biophysj.org/cgi/content/full/74/4/1744 http://www.biophysj.org}
}

@ARTICLE{Shao:2006,
  author = {Shao, S. H. and Cai, W. and Tang, H. Z.},
  title = {Accurate calculation of Green's function of the Schrodinger equation
	in a block layered potential },
  journal = {J Comput. Physics},
  year = {2006},
  volume = {219},
  pages = {733-748},
  annote = {Accurate calculation of Green's function of the Schrodinger equation
	in a block layered potential },
  date-added = {2008-11-25 10:28:56 -0500},
  date-modified = {2008-11-25 10:28:56 -0500},
  ty = {JOUR}
}

@ARTICLE{Sharp:1990,
  author = {Sharp, K. A. and Honig, B.},
  title = {Calculating Total Electrostatic Energies with the Nonlinear {Poisson-Boltzmann}
	Equation},
  journal = {Journal of Physical Chemistry},
  year = {1990},
  volume = {94},
  pages = {7684-7692},
  address = {Columbia univ, dept biochem \& molec biophys,630 w 168th st new york,
	NY USA 10032},
  keywords = {Electrostatics},
  ty = {JOUR}
}

@ARTICLE{Sharp:1990a,
  author = {Sharp, K. A. and Honig, B.},
  title = {Electrostatic Interactions in Macromolecules - Theory and Applications},
  journal = {Annual Review of Biophysics and Biophysical Chemistry},
  year = {1990},
  volume = {19},
  pages = {301-332},
  address = {Columbia univ,dept biochem \& molec biophys,630 w 168th st new york,
	ny usa 10032},
  annote = {Electrostatic Interactions in Macromolecules - Theory and Applications},
  date-added = {2008-06-29 14:51:04 -0500},
  date-modified = {2008-06-29 14:51:04 -0500},
  journal1 = {Ann R Biop},
  keywords = {Electrostatics},
  ty = {JOUR}
}

@INPROCEEDINGS{sheffer2004pcm,
  author = {Sheffer, A. and Kraevoy, V.},
  title = {{Pyramid coordinates for morphing and deformation}},
  booktitle = {Int. Symp. on 3D Data Processing, Visualization and Transmission},
  year = {2004},
  pages = {68-75}
}

@ARTICLE{Shen:2006,
  author = {Shen, M. Y. and Sali, A.},
  title = {{Statistical potential for assessment and prediction of protein structures}},
  journal = {Protein Sci},
  year = {2006},
  volume = {15},
  pages = {2507-2524},
  number = {11}
}

@ARTICLE{Shepherd:2006,
  author = {Shepherd, C. M. and Borelli, I. A. and Lander, G. and Natarajan,
	P. and Siddavanahalli1, V. and Bajaj, C. and Johnson, J. E. and Brooks
	{III}, C. L. and Reddy, V. S.},
  title = {VIPERdb: a relational database for structural virology},
  journal = {Nucleic Acids Research},
  year = {2006},
  volume = {34},
  pages = {D386 - D389},
  annote = {VIPERdb: a relational database for structural virology},
  date-added = {2009-03-10 },
  date-modified = {2009-03-10},
  ty = {JOUR}
}

@ARTICLE{Shepherd:2010,
  author = {Shepherd, Lynsey M. S. and Morrison, Carole A. },
  title = {{Simulating Proton Transport through a Simplified Model for Trans-Membrane
	Proteins}},
  journal = {Journal of Physical Chemistry},
  year = {2010},
  volume = {114},
  pages = {7047-7055}
}

@PHDTHESIS{Shewchuk1997,
  author = {Jonathan Richard Shewchuk},
  title = {Delaunay {R}efinement {M}esh {G}eneration},
  school = {School of Computer Science, Carnegie Mellon University},
  year = {1997},
  address = {Pittsburgh, Pennsylvania},
  month = may,
  note = {Available as Technical Report CMU-CS-97-137}
}

@ARTICLE{DShi:2011,
  author = { Shi, D. and Xiao, X. R. and Huang, X. S.},
  title = { Modeling Stresses in the Separators in a Pouch Lithium-Ion Cell
	
	},
  journal = { Journal Power Sources },
  year = {2011},
  volume = {196},
  pages = {8129 - 8139}
}

@ARTICLE{Shi:2001,
  author = {Shi, J. and Blundell, T.L. and Mizuguchi, K.},
  title = {{FUGUE: sequence-structure homology recognition using environment-specific
	substitution tables and structure-dependent gap penalties}},
  journal = {J Mol Biol},
  year = {2001},
  volume = {310},
  pages = {243-257},
  number = {1}
}

@ARTICLE{Malik,
  author = {Jianbo Shi and Jitendra Malik},
  title = {Normalized Cuts and Image Segmentation},
  journal = {IEEE Trans. Pattern Anal. Mach. Intell.},
  year = {2000},
  volume = {22},
  pages = {888--905},
  number = {8}
}

@ARTICLE{SZTDBG08,
  author = {Xiaohan Shi and Kun Zhou and Yiying Tong and Mathieu Desbrun and
	Hujun Bao and Baining Guo},
  title = {Example-Based Dynamic Skinning in Real Time},
  journal = {ACM Trans. on Graphics (SIGGRAPH)},
  year = {2008},
  month = aug,
  owner = {yiying},
  timestamp = {2009.03.23}
}

@ARTICLE{SZTDBG07,
  author = {Xiaohan Shi and Kun Zhou and Yiying Tong and Mathieu Desbrun and
	Hujun Bao and Baining Guo},
  title = {Mesh Puppetry: Cascading Optimization of Mesh Deformation with Inverse
	Kinematics},
  journal = {ACM Trans. on Graphics (SIGGRAPH)},
  year = {2007},
  pages = {81},
  month = jul
}

@ARTICLE{Shibuta:2007,
  author = {Shibuta, Y. and Okajima, Y. and Suzuki, T.},
  title = {Phase-field modeling for electrodeposition process},
  journal = {Science and Technology of Advanced Materials},
  year = {2007},
  volume = {8},
  pages = {511-518.}
}

@ARTICLE{Shieh:2006,
  author = {Shieh, Shih F. and Wang, Yiqian and Wei, Guowei and Lai, Choy H.
	},
  title = {Mathematical analysis of the wavelet method of chaos control},
  journal = {Journal of Mathematical Physics},
  year = {2006},
  volume = {47},
  pages = {082701},
  number = {8},
  abstract = {View This Record in Scopus},
  bdsk-url-1 = {http://link.aip.org/link/?JMP/47/082701},
  date-added = {2008-06-30 22:03:52 -0400},
  date-modified = {2008-06-30 22:03:52 -0400},
  doi = {10.1063/1.2203229},
  keywords = {mathematics},
  posted-at = {2008-07-01 03:02:57},
  priority = {0},
  publisher = {AIP},
  url = {http://link.aip.org/link/?JMP/47/082701}
}

@ARTICLE{Shingleton:2008,
  author = {Shingleton, A. W. and Mirth, C. and Bates, P. W.},
  title = {Developmental Model of Static Allometry in Holometabolous Insects},
  journal = {Proc. Royal Soc. B.},
  year = {in press, 2008},
  annote = {Developmental Model of Static Allometry in Holometabolous Insects},
  date-added = {2008-09-19 10:28:56 -0500},
  date-modified = {2008-09-19 10:28:56 -0500},
  ty = {JOUR}
}

@ARTICLE{Showalter:2004,
  author = {Showalter, S. A. and Baker, N. A. and Tang, C. and Hall, K. B.},
  title = {Iron responsive element {RNA} flexibility described by {NMR} and
	isotropic reorientational eigenmode dynamics},
  journal = {Journal of Biomolecular NMR},
  year = {2004},
  volume = {32},
  pages = {179-93},
  number = {3},
  abstract = {The first example of the application of reorientational eigenmode
	dynamics (RED) to RNA is shown here for the small and floppy Iron
	Responsive Element (IRE) RNA hairpin. Order parameters calculated
	for bases and riboses from a 12 ns molecular dynamics trajectory
	are compared to experimentally determined order parameters from 13C-1H
	NMR relaxation experiments, and shown to be in qualitative agreement.
	Given the small size of the IRE hairpin and its very flexible loop,
	isotropic RED (iRED) was also used to analyze the trajectory in order
	to describe its dynamic motions. iRED analysis shows that the global
	and internal dynamics of the IRE are not rigorously separable, which
	will result in inaccurate experimental order parameters. In addition,
	the iRED analysis described the many correlated motions that comprise
	the dynamics of the IRE RNA. The combined use of NMR relaxation,
	RED, and iRED provide a uniquely detailed description of IRE RNA
	dynamics.},
  annote = {Iron responsive element RNA flexibility described by NMR and isotropic
	reorientational eigenmode dynamics; ShowalterEtal2004},
  bdsk-file-1 = {YnBsaXN0MDDUAQIDBAUGCQpYJHZlcnNpb25UJHRvcFkkYXJjaGl2ZXJYJG9iamVjdHMSAAGGoNE
	HCFRyb290gAFfEA9OU0tleWVkQXJjaGl2ZXKoCwwXGBkdJCVVJG51bGzTDQ4PEBEUViRjbGFzc1
	dOUy5rZXlzWk5TLm9iamVjdHOAB6ISE4ACgAOiFRaABIAGWWFsaWFzRGF0YVxyZWxhdGl2ZVBhd
	GjSDRobHFdOUy5kYXRhgAVPEQHqAAAAAAHqAAIAAAxNYWNpbnRvc2ggSEQAAAAAAAAAAAAAAAAA
	AADD4v5NSCsAAAAZYksfMjAwNC1TaG93YWx0ZXJCYWtlclRhbmdIYWxsLnBkZgAAAAAAAAAAAAA
	AAAAAAAAAAAAAAAAAAAAAAAAAAAAAABliicM6CetQREYgcHJ2dwAEAAQAAAkgAAAAAAAAAAAAAA
	AAAAAAB0FyY2hpdmUAABAACAAAw+NSrQAAABEACAAAwzpQOwAAAAEAFAAZYksAGWIDAAqkKAAKp
	BEAAHrcAAIAVU1hY2ludG9zaCBIRDpVc2VyczpiYWtlcjpEb2N1bWVudHM6UmVmZXJlbmNlczpB
	cmNoaXZlOjIwMDQtU2hvd2FsdGVyQmFrZXJUYW5nSGFsbC5wZGYAAA4AQAAfADIAMAAwADQALQB
	TAGgAbwB3AGEAbAB0AGUAcgBCAGEAawBlAHIAVABhAG4AZwBIAGEAbABsAC4AcABkAGYADwAaAA
	wATQBhAGMAaQBuAHQAbwBzAGgAIABIAEQAEgBIVXNlcnMvYmFrZXIvRG9jdW1lbnRzL1JlZmVyZ
	W5jZXMvQXJjaGl2ZS8yMDA0LVNob3dhbHRlckJha2VyVGFuZ0hhbGwucGRmABMAAS8AABUAAgAM
	//8AANIeHyAhWCRjbGFzc2VzWiRjbGFzc25hbWWjISIjXU5TTXV0YWJsZURhdGFWTlNEYXRhWE5
	TT2JqZWN0XxBILi4vLi4vLi4vLi4vRG9jdW1lbnRzL1JlZmVyZW5jZXMvQXJjaGl2ZS8yMDA0LV
	Nob3dhbHRlckJha2VyVGFuZ0hhbGwucGRm0h4fJieiJyNcTlNEaWN0aW9uYXJ5AAgAEQAaAB8AK
	QAyADcAOgA/AEEAUwBcAGIAaQBwAHgAgwCFAIgAigCMAI8AkQCTAJ0AqgCvALcAuQKnAqwCtQLA
	AsQC0gLZAuIDLQMyAzUAAAAAAAACAQAAAAAAAAAoAAAAAAAAAAAAAAAAAAADQg==},
  bdsk-url-1 = {http://dx.doi.org/10.1007/s10858-005-7948-2},
  date-added = {2008-09-16 15:50:38 -0500},
  date-modified = {2008-09-16 15:50:38 -0500},
  keywords = {MolecularDynamics; QuasiharmonicModels; NucleicAcids},
  ty = {JOUR},
  url = {http://dx.doi.org/10.1007/s10858-005-7948-2}
}

@ARTICLE{ENO,
  author = {C.W. Shu and S. Osher},
  title = {{Efficient Implementation of Essentially non-Oscillatory Shock Capturing
	Schemes}},
  journal = {J. Sci. Comput.},
  year = {1988},
  volume = {77},
  pages = {439--471}
}

@ARTICLE{tetgen,
  author = {Si, Hang},
  title = {Constrained Delaunay tetrahedral mesh generation and refinement},
  journal = {Finite Elem. Anal. Des.},
  year = {2010},
  volume = {46},
  pages = {33--46},
  month = {January},
  acmid = {1660230},
  address = {Amsterdam, The Netherlands, The Netherlands},
  doi = {10.1016/j.finel.2009.06.017},
  issn = {0168-874X},
  issue = {1-2},
  numpages = {14},
  publisher = {Elsevier Science Publishers B. V.},
  url = {http://dl.acm.org/citation.cfm?id=1660153.1660230}
}

@INPROCEEDINGS{Sieger2011,
  author = {Sieger, Daniel and Botsch, Mario},
  title = {{Design , Implementation , and Evaluation of the Surface mesh Data
	Structure}},
  booktitle = {International Meshing Roundtable},
  year = {2011},
  pages = {533--550},
  file = {:C\:/Dropbox/Dropbox/Paper/imr11.pdf:pdf},
  owner = {doubletony},
  timestamp = {2012.04.26}
}

@ARTICLE{Sigfridsson:1998,
  author = {Sigfridsson, E. and Ryde, U. },
  title = {Comparison of Methods for Deriving Atomic Charges from the Electrostatic
	Potential and Moments},
  journal = {J. Comput. Chem.},
  year = {1998},
  volume = {19},
  pages = {377-395},
  number = {4}
}

@ARTICLE{Silva:2004,
  author = {Silva, H. and Tiwari, S.},
  title = { A nano-scale memory and transistor based on back-side trapping },
  journal = { IEEE Transactions on Nanotechnology},
  year = {2004},
  volume = {3},
  pages = {264 - 269 }
}

@ARTICLE{Simakov:2010,
  author = {Simakov, N. A. and Kurnikova, M. G. },
  title = {Soft Wall Ion Channel in Continuum Representation with Application
	to Modeling Ion Currents in $\alpha${-}Hemolysin},
  journal = {J. Phys. Chem. B},
  year = {2010},
  volume = {114},
  pages = {15180?C15190},
  number = {46}
}

@ARTICLE{Simmonett:2005,
  author = {Simmonett, A. C. and Gilbert, A. T. B. and Gill, P. M. W.},
  title = {An optimal point-charge model for molecular electrostatic potentials},
  journal = {Mol. Phys.},
  year = {2005},
  volume = {103},
  pages = {2789-2793}
}

@ARTICLE{Simonett:2001,
  author = {Simonett, G.},
  title = {The Willmore flow for near spheres},
  journal = {Differential and Integral Equations},
  year = {2001},
  volume = {14},
  pages = {1005-1014},
  annote = {The Willmore flow for near spheres},
  date-added = {2008-09-19 10:28:56 -0500},
  date-modified = {2008-09-19 10:28:56 -0500},
  ty = {JOUR}
}

@ARTICLE{Simons:1997,
  author = {Simons, K. T. and Kooperberg, C. and Huang, E. and Baker, D.},
  title = {{Assembly of protein tertiary structures from fragments with similar
	local sequences using simulated annealing and Bayesian scoring functions}},
  journal = {J Mol Biol},
  year = {1997},
  volume = {268},
  pages = {209-225},
  number = {1}
}

@ARTICLE{Simonson:2003,
  author = {Simonson, T.},
  title = {Electrostatics and dynamics of proteins},
  journal = {Reports on Progress in Physics},
  year = {2003},
  volume = {66},
  pages = {737-87},
  number = {5},
  abstract = {Proteins are the working chemists of living cells. They are complex
	macromolecules, which display a rich and sometimes counterintuitive
	behaviour on many length- and timescales. They contain charged and
	polar groups, and electrostatic interactions control important aspects
	of their structure and function. Experiments and computer simulations
	have been used intensively to probe their electrostatic and dielectric
	properties. A simple framework to rationalize the results is continuum
	electrostatics, even though proteins are smaller than the usual,
	macroscopic length scales of continuum theory. We discuss selected
	topics, including protein structure, dynamics, and solvation; the
	dielectric response of proteins at large (macromolecular) and small
	(atomic) length scales, and the physical and numerical basis of current
	continuum models of proteins and protein solvation.},
  annote = {Electrostatics and dynamics of proteins; {Poisson-Boltzmann}, dielectric,
	forces},
  bdsk-url-1 = {http://dx.doi.org/10.1088/0034-4885/66/5/202},
  date-added = {2008-09-01 14:12:27 -0500},
  date-modified = {2008-09-01 14:12:27 -0500},
  keywords = {Electrostatics},
  ty = {JOUR},
  url = {http://dx.doi.org/10.1088/0034-4885/66/5/202}
}

@ARTICLE{Simonson:2001,
  author = {Simonson, T.},
  title = {Macromolecular electrostatics: continuum models and their growing
	pains},
  journal = {Current Opinion in Structural Biology},
  year = {2001},
  volume = {11},
  pages = {243-252},
  number = {2},
  abstract = {Theoretical understanding of macromolecular electrostatics has advanced
	substantially over the past year. Continuum models have given promising
	results for calculating proteinÃ¢Â€Â“ligand binding free
	energy differences, as well as pKas and redox properties, particularly
	with explicit treatment of multiple conformers. Generalized Born
	and other techniques have led to the first molecular dynamics simulations
	of proteins and RNA with continuum solvent. Continuum and microscopic
	descriptions of dielectric relaxation have been critically compared.},
  annote = {Macromolecular electrostatics: continuum models and their growing
	pains},
  bdsk-url-1 = {http://dx.doi.org/10.1016/S0959-440X(00)00197-4},
  date-added = {2008-09-01 13:59:41 -0500},
  date-modified = {2008-09-01 13:59:41 -0500},
  keywords = {Electrostatics; Solvation},
  ty = {JOUR},
  url = {http://dx.doi.org/10.1016/S0959-440X(00)00197-4}
}

@ARTICLE{Simonson:1994,
  author = {Simonson, T. and Brunger, A. T.},
  title = {Solvation free energies estimated from macroscopic continuum theory:
	an accuracy assessment},
  journal = {Journal of Physical Chemistry},
  year = {1994},
  volume = {98},
  pages = {4683-4694},
  number = {17},
  abstract = {The solvation thermodynamics of a set of small organic molecules is
	studied using a simple continuum model. Transfer from vapor or cyclohexane
	to water is decomposed into three steps: first the atomic partial
	charges of the solute are removed, then it is transferred into aqueous
	solution, and then its partial charges are restored. The electrostatic
	steps are treated using continuum electrostatics; the hydrophobic
	transfer step is treated using atomic Ã¢Â€Âœsolvation parametersÃ¢Â€Â?
	or Ã¢Â€Âœsurface tensionsÃ¢Â€Â?. Vapor-to-water transfer
	free energies of 35 neutral compounds were estimated, including analogues
	of 17 amino acid side chains. Variants of the model were tested,
	using from one to three atom types, each with its own surface tension.
	With a single surface tension, taken from literature data on linear
	alkanes, the data were reproduced with a root-mean-square (rms) error
	of 1.3 kcal/mol. Using up to three atom types did not improve the
	fit significantly. A model with up to eight atom types, but no electrostatic
	term, behaved no better. The model was also applied to cyclohexane-to-water
	transfer of the 17 amino acid side chain analogues considered above.
	Using a single, adjustable, atomic surface tension, the data were
	fit with an rms error of 1.2 kcal/mol, giving a microscopic surface
	tension of 19 f 6 cal/(mol A2), in agreement with experimental estimates
	for n-alkanes. Models with up to three atom types did not behave
	significantly better. Thus parametrized, the model was used to calculate
	the potential of mean force between two N-methylacetamide molecules
	in solvents of dielectric constant 80, mimicking water, and 2.2,
	mimicking carbon tetrachloride.},
  annote = {Solvation free energies estimated from macroscopic continuum theory:
	an accuracy assessment},
  bdsk-url-1 = {http://pubs.acs.org/cgi-bin/sample.cgi/jpchax/1994/98/i17/pdf/j100068a033.pdf},
  date-added = {2008-06-29 15:04:41 -0500},
  date-modified = {2008-06-29 15:04:41 -0500},
  keywords = {Electrostatics; Solvation},
  ty = {JOUR},
  url = {http://pubs.acs.org/cgi-bin/sample.cgi/jpchax/1994/98/i17/pdf/j100068a033.pdf}
}

@ARTICLE{Singer:2008,
  author = {Singer, A. and Gillespie, D. and Norbury ,J. and Eisenberg, R. S.},
  title = {Singular perturbation analysis of the steady state {Poisson-Nernst-Planck}
	system: Applications to ion channels},
  journal = {European Journal of Applied Mathematics},
  year = {2008},
  volume = {19},
  pages = {541-560}
}

@ARTICLE{GKSingh:2008,
  author = {Singh, G. K. and Ceder, G. and Bazant, M. Z.},
  title = {Intercalation dynamics in rechargeable battery materials: General
	theory and phase-transformation waves in {LiFePO4}},
  journal = {Electrochimica Acta},
  year = {2008},
  volume = {53},
  pages = {7599-7613.}
}

@ARTICLE{Singh:1984,
  author = { Singh, U. C. and Kollman, P. A.},
  title = {An approach to computing electrostatic charges for molecules},
  journal = { J. Comput. Chem.},
  year = {1984},
  volume = {5},
  pages = {129-1453}
}

@ARTICLE{Sitkoff:1996,
  author = {Sitkoff, D. and Ben-Tal, N. and Honig, B.},
  title = {Calculation of Alkane to Water Solvation Free Energies Using Continuum
	Solvent Models
	
	},
  journal = {J. Phys. Chem.},
  year = {1996},
  volume = {100},
  pages = {2744 - 2752 }
}

@ARTICLE{PARSE,
  author = {Sitkoff, D. and Sharp, K. A. and Honig, B.},
  title = {Accurate Calculation of Hydration Free Energies Using Macroscopic
	Solvent Models},
  journal = {Journal of Physical Chemistry},
  year = {1994},
  volume = {98},
  pages = {1978-1988},
  number = {7},
  abstract = {A method and parametrization scheme which allow fast and accurate
	calculations of hydration free energies are described. The solute
	is treated as a polarizable cavity of a shape defined by the molecular
	surface, containing point charges at the location of atomic nuclei.
	Electrostatic contributions to solvation are derived from finite
	difference solutions of the Poisson equation (FDPB method). Nonpolar
	(cavity/{van der waals}) energies are added as a surface area dependent
	term, with a single surface tension coefficient (7) derived from
	hydrocarbon solubility in water. Atomic charges and radii are obtained
	by modifying existing force-field or quantum mechanically-derived
	values, by fitting to experimental solvation energies of small organic
	molecules. A new, simple parameter set (parameters for solvation
	energy, PARSE) is developed specifically for the FDPB/y method, by
	choosing atomic charges and radii which reproduce the estimated contributions
	to solvation of simple functional groups. The PARSE parameters reproduce
	hydration free energies for a test set of 67 molecules with an average
	error of 0.4 kcal/mol. For amino acid side chain and peptide backbone
	analogs the average error is only 0.1 kcal/mol.},
  address = {Columbia univ,dept biochem \& molec biophys,630 w 168th st new york,
	ny usa 10032 Columbia univ,dept biochem \& molec biophys new york,
	ny usa 10032 Columbia univ,ctr biomolec simulat new york, ny usa
	10032 Univ penn,dept biochem \& biophys philadelphia, pa usa 19104},
  annote = {Accurate Calculation of Hydration Free Energies Using Macroscopic
	Solvent Models},
  bdsk-url-1 = {http://pubs.acs.org/cgi-bin/sample.cgi/jpchax/1994/98/i07/pdf/j100058a043.pdf},
  date-added = {2008-06-29 15:03:10 -0500},
  date-modified = {2008-06-29 15:03:10 -0500},
  journal1 = {J Phys Chem},
  keywords = {Electrostatics; Solvation},
  ty = {JOUR},
  url = {http://pubs.acs.org/cgi-bin/sample.cgi/jpchax/1994/98/i07/pdf/j100058a043.pdf}
}

@ARTICLE{Skolnick:2000,
  author = {Skolnick, J. and Fetrow, J. S. and Kolinski, A.},
  title = {{Structural genomics and its importance for gene function analysis}},
  journal = {Nat Biotechnol},
  year = {2000},
  volume = {18},
  pages = {283-287},
  number = {3}
}

@ARTICLE{Skolnick:1997,
  author = {Skolnick, J. and Jaroszewski, L. and Kolinski, A. and Godzik, A.},
  title = {{Derivation and testing of pair potentials for protein folding. When
	is the quasichemical approximation correct?}},
  journal = {Protein Science},
  year = {1997},
  volume = {6},
  pages = {676-688}
}

@ARTICLE{Skolnick:2004,
  author = {Skolnick, J. and Kihara, D. and Zhang, Y.},
  title = {{Development and large scale benchmark testing of the $PROSPECTOR_3$
	threading algorithm}},
  journal = {Proteins},
  year = {2004},
  volume = {56},
  pages = {502-518},
  number = {3}
}

@ARTICLE{Slater:1951,
  author = {Slater, J. C. },
  title = {A simplification of the {Hartree-Fock} method},
  journal = {Phys. Rev.},
  year = { 1951},
  volume = {81},
  pages = {385-390},
  annote = {A simplification of the {Hartree-Fock} method},
  date-added = {2008-11-25 10:28:56 -0500},
  date-modified = {2008-11-25 10:28:56 -0500},
  ty = {JOUR}
}

@ARTICLE{Smereka:2006,
  author = {Smereka, Peter },
  title = {The numerical approximation of a delta function with application
	to level set methods},
  journal = {J. Comput. Phys.},
  year = {2006},
  volume = {211},
  pages = {77--90},
  number = {1},
  abstract = {It is shown that a discrete delta function can be constructed using
	a technique developed by Anita Mayo [The fast solution of Poisson's
	and the biharmonic equations on irregular regions, SIAM J. Sci. Comput.
	21 (1984) 285-299] for the numerical solution of elliptic equations
	with discontinuous source terms. This delta function is concentrated
	on the zero level set of a continuous function. In two space dimensions,
	this corresponds to a line and a surface in three space dimensions.
	Delta functions that are first and second order accurate are formulated
	in both two and three dimensions in terms of a level set function.
	The numerical implementation of these delta functions achieves the
	expected order of accuracy.},
  bdsk-url-1 = {http://dx.doi.org/10.1016/j.jcp.2005.05.005},
  bdsk-url-2 = {http://dx.doi.org/10.1016/j.jcp.2005.05.005},
  date-added = {2008-06-30 11:44:03 -0500},
  date-modified = {2008-06-30 11:44:03 -0500},
  doi = {10.1016/j.jcp.2005.05.005},
  keywords = {mathematics},
  priority = {0},
  url = {http://dx.doi.org/10.1016/j.jcp.2005.05.005}
}

@ARTICLE{Smereka:2003,
  author = {Smereka, Peter},
  title = {Semi-Implicit Level Set Methods for Curvature and Surface Diffusion
	Motion},
  journal = {Journal of Scientific Computing},
  year = {2003},
  volume = {19},
  pages = {439--456},
  number = {1},
  abstract = {In this paper we introduce semi-implicit methods for evolving interfaces
	by mean curvature flow and surface diffusion using level set methods.},
  bdsk-url-1 = {http://dx.doi.org/10.1023/A:1025324613450},
  date-added = {2008-09-16 14:41:31 -0500},
  date-modified = {2008-09-16 14:41:31 -0500},
  doi = {10.1023/A:1025324613450},
  ty = {JOUR},
  url = {http://dx.doi.org/10.1023/A:1025324613450}
}

@ARTICLE{Smith:2001,
  author = {Smith, A. and Hall, C.K.},
  title = {Alpha-Helix Formation: Discontinuous Molecular Dynamics on an Intermediate-Resolution
	Protein Model},
  journal = {Proteins},
  year = {2001},
  volume = {44},
  pages = {344-60},
  number = { }
}

@ARTICLE{Smith:2005,
  author = {Smith, G. R. and Sternberg, M. J. and Bates, P. A.},
  title = {{The relationship between the flexibility of proteins and their conformational
	states on forming protein-protein complexes with an application to
	protein-protein docking}},
  journal = {J Mol Biol},
  year = {2005},
  volume = {347},
  pages = {1077-1101},
  number = {5}
}

@ARTICLE{Snider:1960,
  author = {Snider, R. F.},
  title = {Quantum-Mechanical Modified Boltzmann Equation for Degenerate Internal
	States },
  journal = {J. Chem. Phys.},
  year = {1960},
  volume = {32},
  pages = {1051-1060},
  annote = {Quantum-Mechanical Modified Boltzmann Equation for Degenerate Internal
	States },
  date-added = {2008-11-25 10:28:56 -0500},
  date-modified = {2008-11-25 10:28:56 -0500},
  ty = {JOUR}
}

@ARTICLE{Snider:1996a,
  author = {Snider, R. F. and Wei, G. W. and Muga, J. G.},
  title = {Moderately dense gas quantum kinetic theory: Transport coefficient
	expressions },
  journal = {J. Chem. Phys. },
  year = {1996},
  volume = {105},
  pages = {3066-3078 },
  annote = {Moderately dense gas quantum kinetic theory: Transport coefficient
	expressions},
  date-added = {2008-11-25 10:28:56 -0500},
  date-modified = {2008-11-25 10:28:56 -0500},
  ty = {JOUR}
}

@ARTICLE{Snider:1996b,
  author = {Snider, R. F. and Wei, G. W. and Muga, J. G.},
  title = {Moderately dense gas quantum kinetic theory: Aspects of pair correlations},
  journal = {J. Chem. Phys. },
  year = {1996},
  volume = {105},
  pages = {3057-3065 },
  annote = {Moderately dense gas quantum kinetic theory: Aspects of pair correlations},
  date-added = {2008-11-25 10:28:56 -0500},
  date-modified = {2008-11-25 10:28:56 -0500},
  ty = {JOUR}
}

@ARTICLE{Sochen:1998,
  author = {Sochen, N. and Kimmel, R. and Malladi, R. },
  title = {A general framework for low level vision},
  journal = {Image Processing, IEEE Transactions on},
  year = {1998},
  volume = {7},
  pages = {310--318},
  number = {3},
  abstract = {We introduce a new geometrical framework based on which natural flows
	for image scale space and enhancement are presented. We consider
	intensity images as surfaces in the (x,I) space. The image is, thereby,
	a two-dimensional (2-D) surface in three-dimensional (3-D) space
	for gray-level images, and 2-D surfaces in five dimensions for color
	images. The new formulation unifies many classical schemes and algorithms
	via a simple scaling of the intensity contrast, and results in new
	and efficient schemes. Extensions to multidimensional signals become
	natural and lead to powerful denoising and scale space algorithms},
  bdsk-url-1 = {http://dx.doi.org/10.1109/83.661181},
  date-added = {2008-06-30 21:17:53 -0400},
  date-modified = {2008-06-30 21:17:53 -0400},
  doi = {10.1109/83.661181},
  keywords = {mathematics},
  posted-at = {2008-07-01 02:17:06},
  priority = {0},
  url = {http://dx.doi.org/10.1109/83.661181}
}

@ARTICLE{Soding:2005,
  author = {Soding, J.},
  title = {{Protein homology detection by HMM-HMM comparison}},
  journal = {Bioinformatics (Oxford, England)},
  year = {2005},
  volume = {21},
  pages = {951-960},
  number = {7}
}

@ARTICLE{Sohn0516563,
  author = {Sohn, R. and Parks, J. M. and Buhrman, G. and Brown, P. and Kristjansdottir,
	K. and Safi, A. and Edelsbrunner, H. and Yang, W. T. and Rudolph,
	J.},
  title = {Experimental validation of the docking orientation of Cdc25 with
	its Cdk2-CycA protein substrate},
  journal = {Biochemistry},
  year = {2005},
  volume = {44},
  pages = {16563-16573},
  number = {50},
  month = {Dec},
  abstract = {Cdc25 phosphatases are key activators of the eukaryotic cell cycle
	and compelling anticancer targets because their overexpression has
	been associated with numerous cancers. However, drug discovery targeting
	these phosphatases has been hampered by the lack of structural information
	about how Cdc25s interact with their native protein substrates, the
	cyclin-dependent kinases. Herein, we predict a docked orientation
	for Cdc25B with its Cdk2-pTpY-CycA protein substrate by a rigid-body
	docking method and refine the docked models with full-scale molecular
	dynamics simulations and minimization. We validate the stable ensemble
	structure experimentally by a variety of in vitro and in vivo techniques.
	Specifically, we compare our model with a crystal structure of the
	substrate-trapping mutant of Cdc25B. We identify and validate in
	vivo a novel hot-spot residue on Cdc25B (Arg492) that plays a central
	role in protein substrate recognition. We identify a hot-spot residue
	on the Substrate Cdk2 (Asp206) and confirm its interaction with hot-spot
	residues on Cdc25 using hot-spot swapping and double mutant cycles
	to derive interaction energies. Our experimentally validated model
	is consistent with previous studies of Cdk2 and its interaction partners
	and initiates the opportunity for drug discovery of inhibitors that
	target the remote binding sites of this protein-protein interaction.},
  endnotereftype = {Journal Article},
  issn = {0006-2960},
  shorttitle = {Experimental validation of the docking orientation of Cdc25 with its
	Cdk2-CycA protein substrate},
  url = {<Go to ISI>://000234036300019}
}

@ARTICLE{Soler:2002,
  author = {Soler, J. M.},
  title = {The SIESTA method for ab initio order-N materials simulation},
  journal = {J. Phys.: Condens. Matter},
  year = {2002},
  volume = {14},
  pages = {2745- 2779}
}

@ARTICLE{HSoltanianzadeh:1995,
  author = {Soltanianzadeh, H. and Windham, J. P. and Yagle, A. E.},
  title = { A multidimensional nonlinear edge-preserving filter for magnetic-resonace
	image-restoration },
  journal = {{IEEE} Transactions on Image Processing},
  year = {1995},
  volume = {4},
  pages = {147-161},
  number = {2}
}

@ARTICLE{Somarelli:2010,
  author = {Somarelli, J. A. and Mesa, A. and Roy, A. and Zhang, Y. and Herrera,
	R.J.},
  title = {{A three-dimensional model of the U1 small nuclear ribonucleoprotein
	particle}},
  journal = {Entomological Research},
  year = {2010},
  volume = {40},
  pages = {104-112},
  number = {2}
}

@ARTICLE{Sondergaard:2008,
  author = {Sondergaard, Chresten R. and Mcintosh, Lawrence P. and Pollastri,
	Gianluca and Nielsen, Jens E.},
  title = {Determination of electrostatic interaction energies and protonation
	state populations in enzyme active sites},
  journal = {Journal of Molecular Biology},
  year = {2008},
  volume = {376},
  pages = {269-87},
  number = {1},
  abstract = {The pH-dependence of the NMR chemical shift for titratable groups
	in proteins often deviate from a standard Henderson--Hasselbalch
	(HH) titration curve. A non-HH dependence of the chemical shift for
	a given residue can arise from a single-site, non-HH titrational
	event for that residue, or if the chemical shift of the group is
	influenced by additional titrational events occurring in other residues.
	We show that simultaneous fits of several non-HH NMR titration curves
	of interacting protein residues to a statistical mechanical model
	can be used to distinguish between these two cases. From fitting
	of non-HH titrations, we can extract electrostatic interaction energies
	between protein residues. Furthermore, by performing simultaneous
	fits of NMR titration curves and enzymatic pH-activity profiles,
	we can gain information on the identity and populations of the catalytically
	competent protonation states in enzymes. We apply the global fitting
	of titrational events (GloFTE) method to experimental data on five
	enzyme systems and on a single non-enzyme system, and show that the
	extracted electrostatic interaction energies and effective dielectric
	constants for a subset of these systems agree excellently with experimentally
	determined values as well as with theoretical calculations. In the
	case of reduced Escherichia coli thioredoxin we use GloFTE analysis
	to distinguish between two possible interpretations of the NMR titration
	curves of the active site residues. We also show that for the strongly
	coupled system of titratable groups in the active site of the Bacillus
	circulans xylanase (BCX) N35D mutant, GloFTE fits of a single titration
	curve and an enzymatic pH-activity profile can give a full description
	of the energetics of the titrational events in the enzyme's active
	site. Using only the X-ray crystallographic structure of the enzyme
	and the electrostatic interaction energies extracted from such a
	GloFTE fit, we can uniquely identify the three catalytic groups in
	this system. This raises the prospect of completely characterising
	active site titrational events from a single unassigned NMR titration
	curve and an enzymatic pH-activity profile.},
  bdsk-file-1 = {YnBsaXN0MDDUAQIDBAUGCQpYJHZlcnNpb25UJHRvcFkkYXJjaGl2ZXJYJG9iamVjdHMSAAGGoNE
	HCFRyb290gAFfEA9OU0tleWVkQXJjaGl2ZXKoCwwXGBkdJCVVJG51bGzTDQ4PEBEUViRjbGFzc1
	dOUy5rZXlzWk5TLm9iamVjdHOAB6ISE4ACgAOiFRaABIAGWWFsaWFzRGF0YVxyZWxhdGl2ZVBhd
	GjSDRobHFdOUy5kYXRhgAVPEQISAAAAAAISAAIAAAxNYWNpbnRvc2ggSEQAAAAAAAAAAAAAAAAA
	AADD4v5NSCsAAAAZYksfMjAwOC1Tb25kZXJnYWFyZE1jaW4jMTk2MkFGLnBkZgAAAAAAAAAAAAA
	AAAAAAAAAAAAAAAAAAAAAAAAAAAAAABlir8P6iLVQREYgcHJ2dwAEAAQAAAkgAAAAAAAAAAAAAA
	AAAAAAB0FyY2hpdmUAABAACAAAw+NSrQAAABEACAAAw/rPBQAAAAEAFAAZYksAGWIDAAqkKAAKp
	BEAAHrcAAIAVU1hY2ludG9zaCBIRDpVc2VyczpiYWtlcjpEb2N1bWVudHM6UmVmZXJlbmNlczpB
	cmNoaXZlOjIwMDgtU29uZGVyZ2FhcmRNY2luIzE5NjJBRi5wZGYAAA4AWgAsADIAMAAwADgALQB
	TAG8AbgBkAGUAcgBnAGEAYQByAGQATQBjAGkAbgB0AG8AcwBoAFAAbwBsAGwAYQBzAHQAcgBpAE
	4AaQBlAGwAcwBlAG4ALgBwAGQAZgAPABoADABNAGEAYwBpAG4AdABvAHMAaAAgAEgARAASAFVVc
	2Vycy9iYWtlci9Eb2N1bWVudHMvUmVmZXJlbmNlcy9BcmNoaXZlLzIwMDgtU29uZGVyZ2FhcmRN
	Y2ludG9zaFBvbGxhc3RyaU5pZWxzZW4ucGRmAAATAAEvAAAVAAIADP//AADSHh8gIVgkY2xhc3N
	lc1okY2xhc3NuYW1loyEiI11OU011dGFibGVEYXRhVk5TRGF0YVhOU09iamVjdF8QVS4uLy4uLy
	4uLy4uL0RvY3VtZW50cy9SZWZlcmVuY2VzL0FyY2hpdmUvMjAwOC1Tb25kZXJnYWFyZE1jaW50b
	3NoUG9sbGFzdHJpTmllbHNlbi5wZGbSHh8mJ6InI1xOU0RpY3Rpb25hcnkACAARABoAHwApADIA
	NwA6AD8AQQBTAFwAYgBpAHAAeACDAIUAiACKAIwAjwCRAJMAnQCqAK8AtwC5As8C1ALdAugC7AL
	6AwEDCgNiA2cDagAAAAAAAAIBAAAAAAAAACgAAAAAAAAAAAAAAAAAAAN3},
  bdsk-url-1 = {http://www.sciencedirect.com/science/article/B6WK7-4PT29CB-4/2/317c0c23ba0375ea494d6df43b31f74f},
  bdsk-url-2 = {http://dx.doi.org/10.1016/j.jmb.2007.09.070},
  date-added = {2008-09-16 15:42:52 -0500},
  date-modified = {2008-09-16 15:42:52 -0500},
  doi = {10.1016/j.jmb.2007.09.070},
  keywords = {Solvation, pKa, Electrostatics},
  priority = {0},
  url = {http://www.sciencedirect.com/science/article/B6WK7-4PT29CB-4/2/317c0c23ba0375ea494d6df43b31f74f}
}

@ARTICLE{JSong:2009,
  author = {Song, J. and Yu, B. and Yuan, Y. and Taur, Y.},
  title = {A Review on Compact Modeling of Multiple-Gate MOSFETs},
  journal = {IEEE TRANSACTIONS ON CIRCUITS AND SYSTEMS I-REGULAR PAPERS },
  year = {2009},
  volume = {56},
  pages = {1858-1869}
}

@ARTICLE{Song:2009,
  author = {Song, J. H. and Evans, R. and Lin, Y. Y. and Hsu, B. N. and Fair,
	R. B.},
  title = {A scaling model for electrowetting-on-dielectric microfluidic actuators},
  journal = {Microfluid Nanofluid},
  year = {2009},
  volume = {7},
  pages = {75 - 89},
  number = { }
}

@ARTICLE{Song:1999,
  author = { Song, J. Y. and Wang, Y. Y. and Wan, C. C. },
  title = { Review of gel-type polymer electrolytes for lithium-ion batteries
	
	},
  journal = { Journal of Power Sources },
  year = {1999},
  volume = {77},
  pages = {183-197}
}

@ARTICLE{Song:2005a,
  author = {Song, Y. and Guallar, V. and Baker, N. A.},
  title = {Molecular Dynamics Simulations of Salicylate Effects on the Micro-
	and Mesoscopic Properties of a Dipalmitoylphosphatidylcholine Bilayer},
  journal = {Biochemistry},
  year = {2005},
  volume = {44},
  pages = {13425-38},
  number = {41},
  abstract = {Salicylate, an amphiphilic molecule and a popular member of the nonsteroidal
	anti-inflammatory drug family, is known to affect hearing through
	reduction of the electromechanical coupling in the outer hair cells
	of the ear. This reduction of electromotility by salicylate has been
	widely studied, but the molecular mechanism of the phenomenon is
	still unknown. In this study, we investigated one aspect of salicylate's
	action, namely the perturbation of electrical and mechanical membrane
	properties by salicylate in the absence of cytoskeletal or membrane-bound
	motor proteins such as prestin. In particular, we simulated the interaction
	of salicylate with a dipalmitoylphosphatidylcholine (DPPC) bilayer
	via atomically detailed molecular dynamics simulations to observe
	the effect of salicylate on the microscopic and mesoscopic properties
	of the bilayer. The results demonstrate that salicylate interacts
	with the bilayer by associating at the water-DPPC interface in a
	nearly perpendicular orientation and penetrating more deeply into
	the bilayer than either sodium or chloride. This association has
	several affects on the membrane properties. First, binding of salicylate
	to the membrane displaces chloride from the bilayer-water interface.
	Second, salicylate influences the electrostatic potential and dielectric
	properties of the bilayer, with significant changes at the water-lipid
	bilayer interface. Third, salicylate association results in structural
	changes, including decreased headgroup area per lipid and increased
	lipid tail order. However, salicylate does not significantly alter
	the mechanical properties of the DPPC bilayer; bulk compressibility,
	area compressibility, and bending modulus were only perturbed by
	small, statistically insignificant amounts by the presence of salicylate.
	The observations from these simulations are in qualitative agreement
	with experimental data and support the conclusion that salicylate
	influences the electrical but not the mechanical properties of DPPC
	membranes.},
  annote = {Molecular Dynamics Simulations of Salicylate Effects on the Micro-
	and Mesoscopic Properties of a Dipalmitoylphosphatidylcholine Bilayer;
	SongEtal2005},
  bdsk-file-1 = {YnBsaXN0MDDUAQIDBAUGCQpYJHZlcnNpb25UJHRvcFkkYXJjaGl2ZXJYJG9iamVjdHMSAAGGoNE
	HCFRyb290gAFfEA9OU0tleWVkQXJjaGl2ZXKoCwwXGBkdJCVVJG51bGzTDQ4PEBEUViRjbGFzc1
	dOUy5rZXlzWk5TLm9iamVjdHOAB6ISE4ACgAOiFRaABIAGWWFsaWFzRGF0YVxyZWxhdGl2ZVBhd
	GjSDRobHFdOUy5kYXRhgAVPEQHSAAAAAAHSAAIAAAxNYWNpbnRvc2ggSEQAAAAAAAAAAAAAAAAA
	AADD4v5NSCsAAAAZYksZMjAwNS1Tb25nR3VhbGxhckJha2VyLnBkZgAAAAAAAAAAAAAAAAAAAAA
	AAAAAAAAAAAAAAAAAAAAAAAAAAAAAABliecKAp6YAAAAAAAAAAAAEAAQAAAkgAAAAAAAAAAAAAA
	AAAAAAB0FyY2hpdmUAABAACAAAw+NSrQAAABEACAAAwoDt9gAAAAEAFAAZYksAGWIDAAqkKAAKp
	BEAAHrcAAIAT01hY2ludG9zaCBIRDpVc2VyczpiYWtlcjpEb2N1bWVudHM6UmVmZXJlbmNlczpB
	cmNoaXZlOjIwMDUtU29uZ0d1YWxsYXJCYWtlci5wZGYAAA4ANAAZADIAMAAwADUALQBTAG8AbgB
	nAEcAdQBhAGwAbABhAHIAQgBhAGsAZQByAC4AcABkAGYADwAaAAwATQBhAGMAaQBuAHQAbwBzAG
	gAIABIAEQAEgBCVXNlcnMvYmFrZXIvRG9jdW1lbnRzL1JlZmVyZW5jZXMvQXJjaGl2ZS8yMDA1L
	VNvbmdHdWFsbGFyQmFrZXIucGRmABMAAS8AABUAAgAM//8AANIeHyAhWCRjbGFzc2VzWiRjbGFz
	c25hbWWjISIjXU5TTXV0YWJsZURhdGFWTlNEYXRhWE5TT2JqZWN0XxBCLi4vLi4vLi4vLi4vRG9
	jdW1lbnRzL1JlZmVyZW5jZXMvQXJjaGl2ZS8yMDA1LVNvbmdHdWFsbGFyQmFrZXIucGRm0h4fJi
	eiJyNcTlNEaWN0aW9uYXJ5AAgAEQAaAB8AKQAyADcAOgA/AEEAUwBcAGIAaQBwAHgAgwCFAIgAi
	gCMAI8AkQCTAJ0AqgCvALcAuQKPApQCnQKoAqwCugLBAsoDDwMUAxcAAAAAAAACAQAAAAAAAAAo
	AAAAAAAAAAAAAAAAAAADJA==},
  bdsk-url-1 = {http://dx.doi.org/10.1021/bi0506829},
  date-added = {2008-09-16 15:51:08 -0500},
  date-modified = {2008-09-16 15:51:08 -0500},
  keywords = {Biomembranes},
  ty = {JOUR},
  url = {http://dx.doi.org/10.1021/bi0506829}
}

@ARTICLE{Song:2004b,
  author = {Song, Y. and Zhang, Y. and Bajaj, C. L. and Baker, N. A.},
  title = {Continuum Diffusion Reaction Rate Calculations of Wild-Type and Mutant
	Mouse Acetylcholinesterase: Adaptive Finite Element Analysis},
  journal = {Biophysical Journal},
  year = {2004},
  volume = {87},
  pages = {1558-66},
  number = {3},
  abstract = {As described previously, continuum models, such as the Smoluchowski
	equation, offer a scalable framework for studying diffusion in biomolecular
	systems. This work presents new developments in the efficient solution
	of the continuum diffusion equation. Specifically, we present methods
	for adaptively refining finite element solutions of the Smoluchowski
	equation based on a posteriori error estimates. We also describe
	new, molecular-surface-based models, for diffusional reaction boundary
	criteria and compare results obtained from these models with the
	traditional spherical criteria. The new methods are validated by
	comparison of the calculated reaction rates with experimental values
	for wild-type and mutant forms of mouse acetylcholinesterase. The
	results show good agreement with experiment and help to define optimal
	reactive boundary conditions.},
  annote = {Continuum Diffusion Reaction Rate Calculations of Wild-Type and Mutant
	Mouse Acetylcholinesterase: Adaptive Finite Element Analysis; SongEtal2004a},
  bdsk-file-1 = {YnBsaXN0MDDUAQIDBAUGCQpYJHZlcnNpb25UJHRvcFkkYXJjaGl2ZXJYJG9iamVjdHMSAAGGoNE
	HCFRyb290gAFfEA9OU0tleWVkQXJjaGl2ZXKoCwwXGBkdJCVVJG51bGzTDQ4PEBEUViRjbGFzc1
	dOUy5rZXlzWk5TLm9iamVjdHOAB6ISE4ACgAOiFRaABIAGWWFsaWFzRGF0YVxyZWxhdGl2ZVBhd
	GjSDRobHFdOUy5kYXRhgAVPEQHeAAAAAAHeAAIAAAxNYWNpbnRvc2ggSEQAAAAAAAAAAAAAAAAA
	AADD4v5NSCsAAAAZYkscMjAwNC1Tb25nWmhhbmdCYWphakJha2VyLnBkZgAAAAAAAAAAAAAAAAA
	AAAAAAAAAAAAAAAAAAAAAAAAAAAAAABliW8KApm8AAAAAAAAAAAAEAAQAAAkgAAAAAAAAAAAAAA
	AAAAAAB0FyY2hpdmUAABAACAAAw+NSrQAAABEACAAAwoDsvwAAAAEAFAAZYksAGWIDAAqkKAAKp
	BEAAHrcAAIAUk1hY2ludG9zaCBIRDpVc2VyczpiYWtlcjpEb2N1bWVudHM6UmVmZXJlbmNlczpB
	cmNoaXZlOjIwMDQtU29uZ1poYW5nQmFqYWpCYWtlci5wZGYADgA6ABwAMgAwADAANAAtAFMAbwB
	uAGcAWgBoAGEAbgBnAEIAYQBqAGEAagBCAGEAawBlAHIALgBwAGQAZgAPABoADABNAGEAYwBpAG
	4AdABvAHMAaAAgAEgARAASAEVVc2Vycy9iYWtlci9Eb2N1bWVudHMvUmVmZXJlbmNlcy9BcmNoa
	XZlLzIwMDQtU29uZ1poYW5nQmFqYWpCYWtlci5wZGYAABMAAS8AABUAAgAM//8AANIeHyAhWCRj
	bGFzc2VzWiRjbGFzc25hbWWjISIjXU5TTXV0YWJsZURhdGFWTlNEYXRhWE5TT2JqZWN0XxBFLi4
	vLi4vLi4vLi4vRG9jdW1lbnRzL1JlZmVyZW5jZXMvQXJjaGl2ZS8yMDA0LVNvbmdaaGFuZ0Jham
	FqQmFrZXIucGRm0h4fJieiJyNcTlNEaWN0aW9uYXJ5AAgAEQAaAB8AKQAyADcAOgA/AEEAUwBcA
	GIAaQBwAHgAgwCFAIgAigCMAI8AkQCTAJ0AqgCvALcAuQKbAqACqQK0ArgCxgLNAtYDHgMjAyYA
	AAAAAAACAQAAAAAAAAAoAAAAAAAAAAAAAAAAAAADMw==},
  bdsk-url-1 = {http://www.biophysj.org/cgi/content/abstract/87/3/1558},
  date-added = {2008-09-01 14:02:28 -0500},
  date-modified = {2008-09-01 14:02:28 -0500},
  keywords = {Diffusion; Acetylcholinesterase; Mathematics},
  ty = {JOUR},
  url = {http://www.biophysj.org/cgi/content/abstract/87/3/1558}
}

@ARTICLE{Song:2004,
  author = {Song, Y. and Zhang, Y. and Shen, T. and Bajaj, C. L. and McCammon,
	J. A. and Baker, N. A.},
  title = {Finite element solution of the steady-state {Smoluchowksi} equation
	for rate constant calculations},
  journal = {Biophysical Journal},
  year = {2004},
  volume = {86},
  pages = {2017-2029},
  number = {4},
  abstract = {This paper describes the development and implementation of algorithms
	to study diffusion in biomolecular systems using continuum mechanics
	equations. Specifically, finite element methods have been developed
	to solve the steady-state Smoluchowksi equation to calulate ligand
	binding rate constants for large biomolecules. The resulting software
	has been validated and applied to mouse acetylcholinesterase. Rates
	for inhibitor binding to mAChE were calculated at various ionic strengths
	with several different reaction criteria. The calculated rates were
	compared with experimental data and show very good agreement when
	the correct reaction criterion is used. Additionally, these finite
	element methods require significantly less computional resources
	than existing particle-based Brownian dynamics methods.},
  annote = {Finite element solution of the steady-state Smoluchowksi equation
	for rate constant calculations; SongEtal2004b},
  bdsk-file-1 = {YnBsaXN0MDDUAQIDBAUGCQpYJHZlcnNpb25UJHRvcFkkYXJjaGl2ZXJYJG9iamVjdHMSAAGGoNE
	HCFRyb290gAFfEA9OU0tleWVkQXJjaGl2ZXKoCwwXGBkdJCVVJG51bGzTDQ4PEBEUViRjbGFzc1
	dOUy5rZXlzWk5TLm9iamVjdHOAB6ISE4ACgAOiFRaABIAGWWFsaWFzRGF0YVxyZWxhdGl2ZVBhd
	GjSDRobHFdOUy5kYXRhgAVPEQIGAAAAAAIGAAIAAAxNYWNpbnRvc2ggSEQAAAAAAAAAAAAAAAAA
	AADD4v5NSCsAAAAZYksfMjAwNC1Tb25nWmhhbmdTaGVuQmEjMTk2MjYwLnBkZgAAAAAAAAAAAAA
	AAAAAAAAAAAAAAAAAAAAAAAAAAAAAABliYMM6Cp1QREYgcHJ2dwAEAAQAAAkgAAAAAAAAAAAAAA
	AAAAAAB0FyY2hpdmUAABAACAAAw+NSrQAAABEACAAAwzpQ7QAAAAEAFAAZYksAGWIDAAqkKAAKp
	BEAAHrcAAIAVU1hY2ludG9zaCBIRDpVc2VyczpiYWtlcjpEb2N1bWVudHM6UmVmZXJlbmNlczpB
	cmNoaXZlOjIwMDQtU29uZ1poYW5nU2hlbkJhIzE5NjI2MC5wZGYAAA4AUgAoADIAMAAwADQALQB
	TAG8AbgBnAFoAaABhAG4AZwBTAGgAZQBuAEIAYQBqAGEAagBNAGMAQwBhAG0AbQBvAG4AQgBhAG
	sAZQByAC4AcABkAGYADwAaAAwATQBhAGMAaQBuAHQAbwBzAGgAIABIAEQAEgBRVXNlcnMvYmFrZ
	XIvRG9jdW1lbnRzL1JlZmVyZW5jZXMvQXJjaGl2ZS8yMDA0LVNvbmdaaGFuZ1NoZW5CYWphak1j
	Q2FtbW9uQmFrZXIucGRmAAATAAEvAAAVAAIADP//AADSHh8gIVgkY2xhc3Nlc1okY2xhc3NuYW1
	loyEiI11OU011dGFibGVEYXRhVk5TRGF0YVhOU09iamVjdF8QUS4uLy4uLy4uLy4uL0RvY3VtZW
	50cy9SZWZlcmVuY2VzL0FyY2hpdmUvMjAwNC1Tb25nWmhhbmdTaGVuQmFqYWpNY0NhbW1vbkJha
	2VyLnBkZtIeHyYnoicjXE5TRGljdGlvbmFyeQAIABEAGgAfACkAMgA3ADoAPwBBAFMAXABiAGkA
	cAB4AIMAhQCIAIoAjACPAJEAkwCdAKoArwC3ALkCwwLIAtEC3ALgAu4C9QL+A1IDVwNaAAAAAAA
	AAgEAAAAAAAAAKAAAAAAAAAAAAAAAAAAAA2c=},
  bdsk-url-1 = {http://www.biophysj.org/cgi/content/abstract/86/4/2017},
  date-added = {2008-09-01 14:02:28 -0500},
  date-modified = {2008-09-01 14:02:28 -0500},
  keywords = {Diffusion; Acetylcholinesterase},
  ty = {JOUR},
  url = {http://www.biophysj.org/cgi/content/abstract/86/4/2017}
}

@ARTICLE{Spolar:1989,
  author = {Spolar, R. S. and Ha, J. H. and Record Jr, M. T.},
  title = {Hydrophobic effect in protein folding and other noncovalent processes
	involving proteins},
  journal = {Proceedings of the National Academy of Sciences of the United States
	of America},
  year = {1989},
  volume = {86},
  pages = {8382-8385},
  number = {21},
  abstract = {Large negative standard heat capacity changes (delta CP degree much
	less than 0) are the hallmark of processes that remove nonpolar surface
	from water, including the transfer of nonpolar solutes from water
	to a nonaqueous phase and the folding, aggregation/association, and
	ligand-binding reactions of proteins {$[$}Sturtevant, J. M. (1977)
	Proc. Natl. Acad. Sci. USA 74, 2236-2240{$]$}. More recently, Baldwin
	{$[$}Baldwin, R. L. (1986) Proc. Natl. Acad. Sci. USA 83, 8069-8072{$]$}
	proposed that the delta CP degree of protein folding could be used
	to quantify the contribution of the burial of nonpolar surface (the
	hydrophobic effect) to the stability of a globular protein. We demonstrate
	that identical correlations between the delta CP degree and the change
	in water-accessible nonpolar surface area (delta Anp) are obtained
	for both the transfer of nonpolar solutes from water to the pure
	liquid phase and the folding of small globular proteins: delta CP
	degree/delta Anp = -(0.28 +/- 0.05) (where delta Anp is expressed
	in A2 and delta CP degree is expressed in cal.mol-1.K-1; 1 cal =
	4.184 J). The fact that these correlations are identical validates
	the proposals by both Sturtevant and Baldwin that the hydrophobic
	effect is in general the dominant contributor to delta CP degree
	and provides a straightforward means of estimating the contribution
	of the hydrophobic driving force (delta Ghyd degree) to the standard
	free energy change of a noncovalent process characterized by a large
	negative delta CP degree in the physiological temperature range:
	delta Ghyd degree congruent to (80 +/- 10)delta CP degree.},
  annote = {Hydrophobic effect in protein folding and other noncovalent processes
	involving proteins.; SpolarRecord},
  bdsk-url-1 = {http://www.pubmedcentral.nih.gov/articlerender.fcgi?tool=pubmed&pubmedid=2813394},
  date-added = {2008-06-30 06:52:53 -0500},
  date-modified = {2008-06-30 06:52:53 -0500},
  keywords = {Solvation}
}

@ARTICLE{Spolar,
  author = {Spolar, R. S. and Record Jr., M. T. },
  title = {Coupling of local folding to site{-}specific binding of proteins
	to DNA},
  journal = {Science},
  year = {1994},
  volume = {263},
  pages = {777--784}
}

@INCOLLECTION{SD06,
  author = {Ari Stern and Mathieu Desbrun},
  title = {Discrete Geometric Mechanics for Variational Integrators},
  booktitle = {ACM SIGGRAPH'06 Course Notes on Discrete Differential Geometry},
  publisher = {ACM Press},
  year = {2006}
}

@ARTICLE{Stillinger:1973,
  author = {Stillinger, F. H.},
  title = {Structure in Aqueous Solutions of Nonpolar Solutes from the Standpoint
	of Scaled-Particle Theory},
  journal = {J. Solution Chem.},
  year = {1973},
  volume = {2},
  pages = {141 -- 158}
}

@INPROCEEDINGS{stoll:td:2006,
  author = {Stoll, Carsten and Karni, Zachi and R{\"o}ssl, Christian and Yamauchi,
	Hitoshi and Seidel, Hans-Peter},
  title = {Template Deformation for Point Cloud Fitting},
  booktitle = {Symposium on Point-Based Graphics},
  year = {2006},
  pages = {27--35}
}

@ARTICLE{Stone:1985,
  author = {Stone, A. J. and Alderton, M.},
  title = {Distributed multipole analysis methods and applications},
  journal = {Mol. Phys.},
  year = {1985},
  volume = {56},
  pages = {1047-1064}
}

@ARTICLE{Straaten:2005,
  author = {van der Straaten, T. A. and Kathawala, G. and Trellakis, A. and Eisenberg,
	B. S. and Ravaioli, U},
  title = {{BioMOCA:} a {Boltzmann} transport {Monte Carlo} model for ion channel
	simulation},
  journal = {Molecular Simulation},
  year = {2005},
  volume = {31},
  pages = {151-157},
  number = {2}
}

@ARTICLE{Su:2004,
  author = {Su, Y. and Gallicchio, E.},
  title = {The non-polar solvent potential of mean force for the dimerization
	of alanine dipeptide: the role of solute-solvent {van der Waals}
	interactions},
  journal = {Biophysical Chemistry},
  year = {2004},
  volume = {109},
  pages = {251-260},
  number = {2},
  abstract = {The non-polar component of the potential of mean force of dimerization
	of alanine dipeptide has been calculated in explicit solvent by free
	energy perturbation. We observe that the calculated PMF is inconsistent
	with a non-polar hydration free energy model based solely on the
	solute surface area. The non-linear behavior of the soluteÃ¢Â€Â“solvent
	{van der Waals} energy is primarily responsible for the non-linear
	dependence of the potential of mean force with respect to the surface
	area. The calculated potential of mean force is reproduced by an
	implicit solvent model based on a solvent continuum model for the
	soluteÃ¢Â€Â“solvent {van der Waals} interaction energy and
	the surface area for the work of forming the solute cavity.},
  annote = {The non-polar solvent potential of mean force for the dimerization
	of alanine dipeptide: the role of solute-solvent {van der Waals}
	interactions; SuGallicchio2004},
  bdsk-url-1 = {http://dx.doi.org/10.1016/j.bpc.2003.11.007},
  date-added = {2008-08-29 15:51:14 -0500},
  date-modified = {2008-08-29 15:51:14 -0500},
  keywords = {Solvation},
  ty = {JOUR},
  url = {http://dx.doi.org/10.1016/j.bpc.2003.11.007}
}

@ARTICLE{Summa:2007,
  author = {Summa, C. M. and Levitt, M.},
  title = {{Near-native structure refinement using in vacuo energy minimization}},
  journal = {Proc Natl Acad Sci USA},
  year = {2007},
  volume = {104},
  pages = {3177-3182},
  number = {9}
}

@ARTICLE{Sun:2006d,
  author = {Sun, Yuhui and Wu, P. R. and Wei, G. W. and G. Wang, G.},
  title = {Evolution operator based single-step method for image processing},
  journal = {Int. J. Biomed. Imaging},
  year = {2006},
  volume = {83847},
  pages = {1 -- 27}
}

@ARTICLE{YHSun:2006,
  author = {Sun, Y.H. and Zhou, Y. C. and Li, S. G. and Wei, G. W.},
  title = {A windowed Fourier spectral scheme for hyperbolic conservation laws},
  journal = {J. Comput. Phys.},
  year = {2006},
  volume = {214},
  pages = {466 - 490}
}

@ARTICLE{Sun:2006,
  author = {Sun, Yuhui and Zhou, Y. C. and Li, Shu-Guang and Wei, G. W. },
  title = {A windowed {Fourier} pseudospectral method for hyperbolic conservation
	laws},
  journal = {J. Comput. Phys.},
  year = {2006},
  volume = {214},
  pages = {466--490},
  number = {2},
  abstract = {A class of local spectral wavelet filters, discrete singular convolution
	(DSC) filters, is utilized to facilitate the Fourier pseudospectral
	method for the solution of hyperbolic conservation law systems. The
	DSC lowpass filters are adaptively implemented directly in the Fourier
	domain (i.e., windowed Fourier pseudospectral method), while a physical
	domain algorithm is also given to enable the treatment of some special
	boundary conditions. By adjusting the effective wavenumber region
	of the DSC filter, Gibbs oscillations can be removed effectively
	while the high resolution feature of the spectral method can be retained
	for a wide class of problems with various boundary conditions. The
	utility and effectiveness of the present approach are validated by
	extensive numerical experiments. The proposed method could operate
	at a resolution as high as only five points per wavelength (PPW)
	for the interaction of shocks and physical high frequency waves,
	which is some of the best for this class of problems. This high resolution,
	together with the low complexity of the fast Fourier transform (FFT),
	endows the proposed method considerable potential for solving large
	scale problems in hyperbolic conservation laws.},
  bdsk-url-1 = {http://dx.doi.org/10.1016/j.jcp.2005.09.027},
  date-added = {2008-06-30 22:06:24 -0400},
  date-modified = {2008-06-30 22:06:24 -0400},
  doi = {10.1016/j.jcp.2005.09.027},
  keywords = {mathematics},
  posted-at = {2008-07-01 03:06:00},
  priority = {0},
  url = {http://dx.doi.org/10.1016/j.jcp.2005.09.027}
}

@ARTICLE{Sun-wei:2006,
  author = {Sun, Y. H. and Wu, P. R. and Wei, G. W. and Wang, G.},
  title = {Evolution operator based single-step method for image processing},
  journal = {Int. J. Biomed. Imaging},
  year = {2006},
  volume = {83847},
  pages = {1-27 },
  annote = {Evolution operator based single-step method for image processing},
  date-added = {2008-11-25 10:28:56 -0500},
  date-modified = {2008-11-25 10:28:56 -0500},
  ty = {JOUR}
}

@ARTICLE{YSun:2006a,
  author = {Sun, Y. H. and Wu, P. R. and Wei, G. W. and Wang, G.},
  title = {Evolution-Operator-Based Single-Step Method for Image Processing},
  journal = {Int. J. Biomed. Imaging},
  year = {2006},
  volume = {83847},
  pages = {1--27}
}

@ARTICLE{YSun:2006b,
  author = {Sun, Y. H. and Wu, P. R. and Wei, G. W. and Wang, G.},
  title = {Evolution-Operator-Based single-step method for image processing},
  journal = {Int. J. Biomed. Imaging},
  year = {2006},
  volume = {83847},
  pages = {1}
}

@ARTICLE{Sun:2006a,
  author = {Sun, Y. H. and Zhou, Y. C. and Li, S. G. and Wei, G. W. },
  title = {A windowed Fourier pseudospectral method for hyperbolic conservation
	laws},
  journal = {J. Comput. Phys.},
  year = {2006},
  volume = {214},
  pages = {466-490}
}

@ARTICLE{SobolevContours,
  author = {G. Sundaramoorthi and A. Yezzi and A. C. G. Mennucci},
  title = {Sobolev Active Contours},
  journal = {IJCV},
  year = {2007},
  volume = {73},
  pages = {345--366},
  number = {3}
}

@ARTICLE{SobolevContours,
  author = {G. Sundaramoorthi and A. Yezzi and A. C. G. Mennucci},
  title = {Sobolev Active Contours},
  journal = {IJCV, \emph{to appear}},
  year = {2006}
}

@ARTICLE{LSM-VOF,
  author = {Mark Sussman and Elbridge G. Puckett},
  title = {{A Coupled Level Set and Volume-Of-Fluid method for Computing 3D
	and Axisymmetric Incompressible Two-phase Flows}},
  journal = {J. Comput. Phys.},
  year = {2000},
  volume = {162},
  pages = {301--337},
  number = {2}
}

@ARTICLE{Svizhenko:2002,
  author = {Svizhenko, A. and Anantram, M. and Govindan, T. R. and Biegel, B.
	and Venugopal, R.},
  title = {Two-dimensional quantum mechanical modeling of nanotransistors},
  journal = {J Applied Phys.},
  year = {2002},
  volume = {91},
  pages = {2343- 2354},
  annote = {Two-dimensional quantum mechanical modeling of nanotransistors},
  date-added = {2008-11-25 10:28:56 -0500},
  date-modified = {2008-11-25 10:28:56 -0500},
  ty = {JOUR}
}

@ARTICLE{Swanson:2004,
  author = {Swanson, J. M. J. and Henchman, R. H. and McCammon, J. A.},
  title = {Revisiting Free Energy Calculations: A Theoretical Connection to
	{MM/PBSA} and Direct Calculation of the Association Free Energy},
  journal = {Biophysical Journal},
  year = {2004},
  volume = {86},
  pages = {67-74},
  number = {1},
  abstract = {The prediction of absolute ligand-receptor binding affinities is essential
	in a wide range of biophysical queries, from the study of protein-protein
	interactions to structure-based drug design. End-point free energy
	methods, such as the Molecular Mechanics {Poisson-Boltzmann} Surface
	Area (MM/PBSA) model, have received much attention and widespread
	application in recent literature. These methods benefit from computational
	efficiency as only the initial and final states of the system are
	evaluated, yet there remains a need for strengthening their theoretical
	foundation. Here a clear connection between statistical thermodynamics
	and end-point free energy models is presented. The importance of
	the association free energy, arising from one molecule's loss of
	translational and rotational freedom from the standard state concentration,
	is addressed. A novel method for calculating this quantity directly
	from a molecular dynamics simulation is described. The challenges
	of accounting for changes in the protein conformation and its fluctuations
	from separate simulations are discussed. A simple first-order approximation
	of the configuration integral is presented to lay the groundwork
	for future efforts. This model has been applied to FKBP12, a small
	immunophilin that has been widely studied in the drug industry for
	its potential immunosuppressive and neuroregenerative effects.},
  annote = {Revisiting Free Energy Calculations: A Theoretical Connection to
	MM/PBSA and Direct Calculation of the Association Free Energy; SwansonMMPBSA;
	An analysis of MM/PBSA in the context of statistical mechanics together
	with a discussion of the application of the theory to molecular dynamics
	simulations.},
  bdsk-url-1 = {http://www.biophysj.org/cgi/content/full/86/1/67},
  date-added = {2008-06-29 15:06:55 -0500},
  date-modified = {2008-06-29 15:06:55 -0500},
  keywords = {Electrostatics; molecular\_dynamics},
  ty = {JOUR},
  url = {http://www.biophysj.org/cgi/content/full/86/1/67}
}

@ARTICLE{Swanson:2005a,
  author = {Swanson, J. M. J. and Mongan, J. and McCammon, J. A.},
  title = {Limitations of Atom-Centered Dielectric Functions in Implicit Solvent
	Models},
  journal = {Journal of Physical Chemistry B},
  year = {2005},
  volume = {109},
  pages = {14769-72},
  number = {31},
  abstract = {Many recent advances in {Poisson-Boltzmann} and generalized Born implicit
	solvent models have used atom-centered polynomial or Gaussian functions
	to define the boundary separating low and high dielectric regions.
	In contrast to the Lee and Richards molecular surface, atom-centered
	surfaces result in interatomic crevices and buried pockets of high
	dielectric which are too small for a solvent molecule to occupy.
	We show that these interstitial high dielectric regions are of significant
	magnitude in globular proteins, that they artificially increase solvation
	energies, and that they distort the free energy surface of nonbonded
	interactions. These results suggest that implicit solvent dielectric
	functions must exclude interstitial high dielectric regions in order
	to yield physically meaningful results.},
  annote = {Limitations of Atom-Centered Dielectric Functions in Implicit Solvent
	Models},
  bdsk-url-1 = {http://dx.doi.org/10.1021/jp052883s},
  date-added = {2008-06-30 11:28:47 -0500},
  date-modified = {2008-06-30 11:28:47 -0500},
  keywords = {Electrostatics},
  ty = {JOUR},
  url = {http://dx.doi.org/10.1021/jp052883s}
}

@ARTICLE{Swanson:2007,
  author = {Swanson, J. M. J. and Wagoner, J. A. and Baker, N. A. and McCammon,
	J. A.},
  title = {Optimizing the Poisson Dielectric Bounday with Explicit Solvent Forces
	and Energies: Lessons Learned with Atom-Centered Dielectric Functions},
  journal = {Journal of Chemical Theory and Computation},
  year = {2007},
  volume = {3},
  pages = {170-83},
  number = {1},
  abstract = {Accurate implicit solvent models require parameters that have been
	optimized in a system- or atom-specific manner on the basis of experimental
	data or more rigorous explicit solvent simulations. Models based
	on the Poisson or {Poisson-Boltzmann} equation are particularly sensitive
	to the nature and location of the boundary which separates the low
	dielectric solute from the high dielectric solvent. Here, we present
	a novel method for optimizing the solute radii, which define the
	dielectric boundary, on the basis of forces and energies from explicit
	solvent simulations. We use this method to optimize radii for protein
	systems defined by AMBER ff99 partial charges and a spline-smoothed
	solute surface. The spline-smoothed surface is an atom-centered dielectric
	function that enables stable and efficient force calculations. We
	explore the relative performance of radii optimized with forces alone
	and those optimized with forces and energies. We show that our radii
	reproduce the explicit solvent forces and energies more accurately
	than four other parameter sets commonly used in conjunction with
	the AMBER force field, each of which has been appropriately scaled
	for spline-smoothed surfaces. Finally, we demonstrate that spline-smoothed
	surfaces show surprising accuracy for small, compact systems but
	may have limitations for highly solvated protein systems. The optimization
	method presented here is efficient and applicable to any system with
	explicit solvent parameters. It can be used to determine the optimal
	continuum parameters when experimental solvation energies are unavailable
	and the computational costs of explicit solvent charging free energies
	are prohibitive.},
  annote = {Optimizing the Poisson Dielectric Bounday with Explicit Solvent Forces
	and Energies: Lessons Learned with Atom-Centered Dielectric Functions},
  bdsk-file-1 = {YnBsaXN0MDDUAQIDBAUGCQpYJHZlcnNpb25UJHRvcFkkYXJjaGl2ZXJYJG9iamVjdHMSAAGGoNE
	HCFRyb290gAFfEA9OU0tleWVkQXJjaGl2ZXKoCwwXGBkdJCVVJG51bGzTDQ4PEBEUViRjbGFzc1
	dOUy5rZXlzWk5TLm9iamVjdHOAB6ISE4ACgAOiFRaABIAGWWFsaWFzRGF0YVxyZWxhdGl2ZVBhd
	GjSDRobHFdOUy5kYXRhgAVPEQH6AAAAAAH6AAIAAAxNYWNpbnRvc2ggSEQAAAAAAAAAAAAAAAAA
	AADD4v5NSCsAAAAZYksfMjAwNy1Td2Fuc29uV2Fnb25lckIjMTk2MjdGLnBkZgAAAAAAAAAAAAA
	AAAAAAAAAAAAAAAAAAAAAAAAAAAAAABlif8HI3m4AAAAAAAAAAAAEAAQAAAkgAAAAAAAAAAAAAA
	AAAAAAB0FyY2hpdmUAABAACAAAw+NSrQAAABEACAAAwckyzgAAAAEAFAAZYksAGWIDAAqkKAAKp
	BEAAHrcAAIAVU1hY2ludG9zaCBIRDpVc2VyczpiYWtlcjpEb2N1bWVudHM6UmVmZXJlbmNlczpB
	cmNoaXZlOjIwMDctU3dhbnNvbldhZ29uZXJCIzE5NjI3Ri5wZGYAAA4ASgAkADIAMAAwADcALQB
	TAHcAYQBuAHMAbwBuAFcAYQBnAG8AbgBlAHIAQgBhAGsAZQByAE0AYwBDAGEAbQBtAG8AbgAuAH
	AAZABmAA8AGgAMAE0AYQBjAGkAbgB0AG8AcwBoACAASABEABIATVVzZXJzL2Jha2VyL0RvY3VtZ
	W50cy9SZWZlcmVuY2VzL0FyY2hpdmUvMjAwNy1Td2Fuc29uV2Fnb25lckJha2VyTWNDYW1tb24u
	cGRmAAATAAEvAAAVAAIADP//AADSHh8gIVgkY2xhc3Nlc1okY2xhc3NuYW1loyEiI11OU011dGF
	ibGVEYXRhVk5TRGF0YVhOU09iamVjdF8QTS4uLy4uLy4uLy4uL0RvY3VtZW50cy9SZWZlcmVuY2
	VzL0FyY2hpdmUvMjAwNy1Td2Fuc29uV2Fnb25lckJha2VyTWNDYW1tb24ucGRm0h4fJieiJyNcT
	lNEaWN0aW9uYXJ5AAgAEQAaAB8AKQAyADcAOgA/AEEAUwBcAGIAaQBwAHgAgwCFAIgAigCMAI8A
	kQCTAJ0AqgCvALcAuQK3ArwCxQLQAtQC4gLpAvIDQgNHA0oAAAAAAAACAQAAAAAAAAAoAAAAAAA
	AAAAAAAAAAAADVw==},
  bdsk-url-1 = {http://dx.doi.org/10.1021/ct600216k},
  date-added = {2008-06-30 11:29:41 -0500},
  date-modified = {2008-06-30 11:29:41 -0500},
  keywords = {Electrostatics; Solvation},
  ty = {JOUR},
  url = {http://dx.doi.org/10.1021/ct600216k}
}

@ARTICLE{Swendsen:1986,
  author = {Swendsen, R. H. and Wang, J. S.},
  title = {{Replica Monte Carlo simulation of spin glasses}},
  journal = {Physical Review Letters},
  year = {1986},
  volume = {57},
  pages = {2607-2609},
  number = {21}
}

@ARTICLE{Szeliskit:1992,
  author = {Szeliskit, R. and Tonnesen, D.},
  title = {Surface Modeling with Oriented Particle Systems},
  journal = {Computer Graphics},
  year = {1992},
  volume = {26},
  pages = {185-194}
}

@ARTICLE{tadmor89,
  author = {Tadmor, E.},
  title = {Convergence of spectral methods for nonlinear conservation laws},
  journal = {SIAM J. Numer. Anal.},
  year = {1989},
  volume = {26},
  pages = {30-44}
}

@ARTICLE{Tadmor:1996,
  author = {Tadmor, E. B. and Ortiz, M. and Phillips, R.},
  title = {Quasicontinuum analysis of defects in crystals},
  journal = {Phil. Mag. A},
  year = {1996},
  volume = {76},
  pages = {1529 - 1564}
}

@ARTICLE{Tagantsev:2003,
  author = {Tagantsev, A. K. and Sherman, V. O. and Astafiev, K. F. and Venkatesh,
	J. and Setter, N.},
  title = {Ferroelectric Materials for Microwave Tunable Applications},
  journal = {Journal of Electroceramics},
  year = {2003},
  volume = {11},
  pages = {5-66}
}

@ARTICLE{Takano:2005,
  author = {Takano, Y. and Houk, K. N. },
  title = {Benchmarking the Conductor-like Polarizable Continuum Model (CPCM)
	for Aqueous Solvation Free Energies of Neutral and Ionic Organic
	Molecules},
  journal = {Journal of Chemical Theory and Computation},
  year = {2005},
  volume = {1},
  pages = {70--77},
  number = {1},
  abstract = {Abstract: The conductor-like polarizable continuum model (CPCM) using
	several cavity models is applied to compute aqueous solvation free
	energies for a number of organic molecules (30 neutral molecules,
	21 anions, and 19 cations). The calculated solvation free energies
	are compared to the available experimental data from the viewpoint
	of cavity models, computational methods, calculation time, and aqueous
	pKa values. The HF/6-31+G(d)//HF/6-31+G(d) and the HF/6-31+G(d)//B3LYP/6-31+G(d)
	with the UAKS cavities, in which radii are optimized with PBE0/6-31G(d),
	provide aqueous solvation effects in best agreement with available
	experimental data. The mean absolute deviations from experiment are
	2.6 kcal/mol. The MP2/6-31++G(d,p)//HF/6-31+G(d) with the CPCM-UAKS(HF/6-31+G(d))
	calculation is also performed for the base-catalyzed hydrolysis of
	methyl acetate in water.},
  address = {Department of Chemistry and Biochemistry, University of California,
	Los Angeles, 607 Charles E. Young Drive East, Los Angeles, California
	90095-1569},
  bdsk-url-1 = {http://dx.doi.org/10.1021/ct049977a},
  date-added = {2008-06-30 06:24:31 -0500},
  date-modified = {2008-06-30 06:24:31 -0500},
  doi = {10.1021/ct049977a},
  keywords = {quantum\_mechanics, solvation},
  posted-at = {2008-06-30 12:23:59},
  priority = {0},
  url = {http://dx.doi.org/10.1021/ct049977a}
}

@ARTICLE{Takayama:2008,
  author = {Takayama, Yuki and Castaneda, Carlos A. and Chimenti, Michael and
	Garcia-Moreno, Bertrand and Iwahara, Junji},
  title = {Direct Evidence for Deprotonation of a Lysine Side Chain Buried in
	the Hydrophobic Core of a Protein},
  journal = {Journal of the American Chemical Society},
  year = {2008},
  volume = {130},
  pages = {6714-6715},
  number = {21},
  abstract = {Abstract: We report direct evidence for deprotonation of a lysine
	side chain buried in the hydrophobic core of a protein, demonstrating
	heteronuclear 1H15N NMR data on the Lys-66 side chain amine (Nâˆ
	group in the Ã®-PHS/V66K variant of staphylococcal nuclease. Previous
	crystallographic study has shown that the Lys-66 Nâˆ?group is completely
	buried in the hydrophobic core. On the basis of double and triple
	resonance experiments, we found that the 1Hâˆ?and 15Nâˆ?chemical
	shifts at pH 8.0 and 6 âˆžC for the buried lysine are 0.81 and
	23.3 ppm, respectively, which are too abnormal to correspond to the
	protonated (NH3+) state. Further investigations using a model system
	suggested that the abnormal 1H and 15N chemical shifts represent
	the deprotonated (NH2) state of the Lys-66 Nâˆ?group. More straightforward
	evidence for the deprotonation was obtained with 2D F1-1H-coupled
	1H15N heteronuclear correlation experiments. Observed 15N multiplets
	clearly indicated that the spin system for the Lys-66 Nâˆ?group
	is AX2 (NH2) rather than AX3 (NH3+). Interestingly, although the
	amine group is buried in the hydrophobic core, the hydrogen exchange
	between water and the Lys-66 Nâˆ?group was found to be relatively
	rapid (93 s1 at 1 âˆžC), which suggests the presence of a dynamic
	process such as local unfolding or water penetration. The partial
	self-decoupling effect on 15Nâˆ?multiplets due to the rapid hydrogen
	exchange is also discussed.},
  affiliation = {Department of Biochemistry and Molecular Biology, Sealy Center for
	Structural Biology and Molecular Biophysics, University of Texas
	Medical Branch, Galveston, Texas 77555-0647, and Department of Biophysics,
	Johns Hopkins University, Baltimore, Maryland 21218},
  bdsk-url-1 = {http://pubs3.acs.org/acs/journals/doilookup?in_doi=10.1021/ja801731g},
  date-added = {2008-09-16 15:43:14 -0500},
  date-modified = {2008-09-16 15:43:14 -0500},
  doi = {10.1021/ja801731g },
  issn = {0002-7863},
  keywords = {Solvation; Electrostatics; pKa},
  url = {http://pubs3.acs.org/acs/journals/doilookup?in_doi=10.1021/ja801731g}
}

@ARTICLE{CIP,
  author = {H. Takewaki and A. Nishiguchi and T. Yabe},
  title = {{The Cubic-interpolated Pseudo-particle (CIP) Method for Solving
	Hyperbolic-type Equations}},
  journal = {J. Comput. Phys.},
  year = {1985},
  volume = {61},
  pages = {261-268}
}

@ARTICLE{Tan:2007b,
  author = {Tan, C. and Tan, Y. H. and Luo, R.},
  title = {Implicit Nonpolar Solvent Models},
  journal = {Journal of Physical Chemistry B},
  year = {2007},
  volume = {111},
  pages = {12263--74},
  number = {42},
  abstract = {Abstract: We have systematically analyzed a new nonpolar solvent model
	that separates nonpolar solvation free energy into repulsive and
	attractive components. Our analysis shows that either molecular surfaces
	or volumes can be used to correlate with repulsive free energies
	of tested molecules in explicit solvent with correlation coefficients
	higher than 0.99. In addition, the attractive free energies in explicit
	solvent can also be reproduced with the new model with a correlation
	coefficient higher than 0.999. Given each component optimized, the
	new nonpolar solvent model is found to reproduce monomer nonpolar
	solvation free energies in explicit solvent very well. However, the
	overall accuracy of the nonpolar solvation free energies is lower
	than that of each component. In the more challenging dimer test cases,
	the agreement of the new model with explicit solvent is less impressive.
	Nevertheless, it is found that the new model works reasonably well
	for reproducing the relative nonpolar free energy landscapes near
	the global minimum of the dimer complexes.},
  address = {Department of Molecular Biology and Biochemistry, University of California,
	Irvine, California 92697-3900},
  bdsk-url-1 = {http://dx.doi.org/10.1021/jp073399n},
  bdsk-url-2 = {http://dx.doi.org/10.1021/jp073399n},
  date-added = {2008-06-30 06:25:13 -0500},
  date-modified = {2008-06-30 06:25:13 -0500},
  doi = {10.1021/jp073399n},
  keywords = {solvation, nonpolar},
  priority = {0},
  url = {http://dx.doi.org/10.1021/jp073399n}
}

@ARTICLE{Tan:2006d,
  author = {Tan, C. and Yang, L. and Luo, R. },
  title = {How Well Does {{Poisson-Boltzmann}} Implicit Solvent Agree with Explicit
	Solvent? {A} Quantitative Analysis},
  journal = {Journal of Physical Chemistry B},
  year = {2006},
  volume = {110},
  pages = {18680--18687},
  number = {37},
  abstract = {Abstract: We have quantitatively studied the performance of a finite-difference
	{Poisson-Boltzmann} implicit solvent with respect to the TIP3P explicit
	solvent in a range of systems of biochemical interest. An overall
	agreement was found between the tested implicit and explicit solvents
	for hydrogen-bonding/salt-bridging dimers and peptide monomers and
	dimers of different conformations and different lengths. These comparative
	analyses also indicate a good transferability of empirically optimized
	parameters for the implicit solvent from small training molecules
	to large testing peptides. However, deviations between the two tested
	solvents are also apparent. Specifically, a consistent deviation
	was observed when hydrogen-bonding or salt-bridging dimers are within
	4-6 \r{A}. The deviation reaches a maximum at about 5.5 \r{A}, the
	so-called water-bridging distance. The tested implicit solvent, even
	with optimized parameters, cannot capture the subtle fluctuation
	in the distance-dependent reaction field energy profiles, although
	smoothed profiles can still be obtained and are in overall agreement
	with those in the explicit solvent. Interestingly, the same mechanism
	underlining the above discrepancy is also responsible for the larger
	deviations of certain peptide conformations, such as parallel -strand
	dimers. It is likely that the observed discrepancy may cause improper
	conformational distributions in simulations with the implicit solvent
	when hydrogen-bonding or salt-bridging interactions are crucial,
	such as secondary structure populations in proteins. Validation of
	the implicit solvent with optimized parameters in dynamics simulations
	will be the next step to study the influences of the observed discrepancy
	at biological conditions.},
  address = {Department of Molecular Biology and Biochemistry, University of California,
	Irvine, California 92697-3900},
  bdsk-url-1 = {http://dx.doi.org/10.1021/jp063479b},
  bdsk-url-2 = {http://dx.doi.org/10.1021/jp063479b},
  date-added = {2008-09-01 13:54:13 -0500},
  date-modified = {2008-09-01 13:54:13 -0500},
  doi = {10.1021/jp063479b},
  keywords = {Electrostatics, MolecularSimulation, Solvation},
  posted-at = {2008-04-18 11:27:21},
  priority = {2},
  url = {http://dx.doi.org/10.1021/jp063479b}
}

@ARTICLE{Tan:2006c,
  author = {Tan, Jian J. and Chen, Wei Z. and Wang, Cun X. },
  title = {Investigating interactions between {HIV-1 gp41} and inhibitors by
	molecular dynamics simulation and {MM-PBSA/GBSA} calculations},
  journal = {Journal of Molecular Structure: Theochem.},
  year = {2006},
  volume = {766},
  pages = {77--82},
  number = {2-3},
  abstract = {An approved peptidic HIV-1 fusion inhibitor, T-20, has shown significant
	promises in clinical applications. However, T-20 must be injected
	twice daily and is too expensive. Consequently, it is necessary to
	research oral small molecule HIV-1 fusion inhibitors. In an effort
	to understand the molecular mechanism of the small molecule inhibitors
	binding to gp41, we have carried out docking studies, explicit solvent
	molecular dynamics simulations, and binding free energy calculations.
	The results of calculated binding free energy are in agreement with
	the experimental data. Further analysis of the binding free energy
	components reveals the dominant contributions to hydrophobic interactions.
	These results could be used to design more effective HIV-1 inhibitors
	targeted to the hydrophobic pocket of HIV-1 gp41.},
  bdsk-url-1 = {http://dx.doi.org/10.1016/j.theochem.2006.02.022},
  bdsk-url-2 = {http://dx.doi.org/10.1016/j.theochem.2006.02.022},
  date-added = {2008-09-01 13:50:42 -0500},
  date-modified = {2008-09-01 13:50:42 -0500},
  doi = {10.1016/j.theochem.2006.02.022},
  keywords = {Electrostatics, Protein-ligandInteractions, Solvation},
  posted-at = {2008-04-16 14:11:48},
  priority = {0},
  url = {http://dx.doi.org/10.1016/j.theochem.2006.02.022}
}

@ARTICLE{Tan:2005,
  author = {Tan, Z. -J. and Chen, S. -J.},
  title = {Electrostatic correlations and fluctuations for ion binding to a
	finite length polyelectrolyte},
  journal = {Journal of Chemical Physics},
  year = {2005},
  volume = {122},
  pages = {044903},
  abstract = {A statistical mechanical model is presented which explicitly accounts
	for the fluctuations, the electrostatic, and the excluded volume
	correlations for ions bound to a polyelectrolyte such as DNA. The
	method can be employed to treat a wide range of ionic conditions
	including multivalent ions. The microscopic framework of the theory
	permits the use of realistic finite length and grooved structural
	model for the polyelectrolyte and modeling of the finite size of
	the bound ions. Test against Monte Carlo simulations suggests that
	the theory can give accurate predictions for the ion distribution
	and the thermodynamic properties. For multivalent ions, the theory
	makes improved predictions as compared with the mean-field approach.
	Moreover, for long polyelectrolyte and dilute salt concentration,
	the theory predicts ion binding properties that agree with the counterion
	condensation theory.},
  annote = {Electrostatic correlations and fluctuations for ion binding to a
	finite length polyelectrolyte},
  bdsk-url-1 = {http://dx.doi.org/10.1063/1.1842059},
  date-added = {2008-09-01 13:58:37 -0500},
  date-modified = {2008-09-01 13:58:37 -0500},
  keywords = {Electrostatics; StatisticalMechanics; BeyondMeanField},
  ty = {JOUR},
  url = {http://dx.doi.org/10.1063/1.1842059}
}

@ARTICLE{Tanaka:2001,
  author = {Tanaka, M. and Grosberg, A. Y.},
  title = {Giant charge inversion of a macroion due to multivalent counterions
	and monovalent coions: Molecular dynamics study},
  journal = {Journal of Chemical Physics},
  year = {2001},
  volume = {115},
  pages = {567-574},
  number = {1},
  abstract = {We report molecular dynamics simulation of the (overall neutral) system
	consisting of an immobile macroion surrounded by the electrolyte
	of multivalent counterions and monovalent coions. In a short time
	(< a few nanoseconds), counterions adsorb on the macroion surface
	in the amount much exceeding neutralization requirement, thus effectively
	inverting the sign of the macroion charge. We find two conditions
	necessary for charge inversion, namely, counterions must be multivalently
	charged and Coulomb interactions must be strong enough compared to
	thermal energy. On the other hand, coion condensation on the multivalent
	counterions similar to Bjerrum pairing is the major factor restricting
	the amount of charge inversion. Depending on parameters, we observe
	inverted charge up to about 200{\%} the original charge of the macroion
	in absolute value. The inverted charge scales as \~{}z1/2 when z<1
	and crosses over to \~{}z for z>1, where = z(A0/rs)2, rs is the Debye
	screening length in the electrolyte and A0 is the distance between
	adsorbed counterions under neutralizing conditions. These findings
	are consistent with the theory of {\tt{}"{}}giant charge inversion{\tt{}"{}}
	{$[$}Phys. Rev. Lett. 85, 1568 (2000){$]$}.},
  annote = {Giant charge inversion of a macroion due to multivalent counterions
	and monovalent coions: Molecular dynamics study},
  bdsk-url-1 = {http://dx.doi.org/10.1063/1.1377033},
  date-added = {2008-09-01 14:05:29 -0500},
  date-modified = {2008-09-01 14:05:29 -0500},
  keywords = {Electrostatics},
  ty = {JOUR},
  url = {http://dx.doi.org/10.1063/1.1377033}
}

@ARTICLE{Tang:2007,
  author = {Tang, C. L. and Alexov, E. and Pyle, A. M. and Honig, B.},
  title = {Calculation of {pKa}s in {RNA}: On the Structural Origins and Functional
	Roles of Protonated Nucleotides},
  journal = {Journal of Molecular Biology},
  year = {2007},
  volume = {366},
  pages = {1475-96},
  number = {5},
  abstract = {pKa calculations based on the PoissonÃ¢Â€Â“Boltzmann equation
	have been widely used to study proteins and, more recently, DNA.
	However, much less attention has been paid to the calculation of
	pKa shifts in RNA. There is accumulating evidence that protonated
	nucleotides can stabilize RNA structure and participate in enzyme
	catalysis within ribozymes. Here, we calculate the pKa shifts of
	nucleotides in RNA structures using numerical solutions to the PoissonÃ¢Â€Â“Boltzmann
	equation. We find that significant shifts are predicted for several
	nucleotides in two catalytic RNAs, the hairpin ribozyme and the hepatitis
	delta virus ribozyme, and that the shifts are likely to be related
	to their functions. We explore how different structural environments
	shift the pKas of nucleotides from their solution values. RNA structures
	appear to use two basic strategies to shift pKas: (a) the formation
	of compact structural motifs with structurally-conserved, electrostatic
	interactions; and (b) the arrangement of the phosphodiester backbone
	to focus negative electrostatic potential in specific regions.},
  annote = {Calculation of pKas in RNA: On the Structural Origins and Functional
	Roles of Protonated Nucleotides; PARSE},
  bdsk-url-1 = {http://dx.doi.org/10.1016/j.jmb.2006.12.001},
  date-added = {2008-09-03 13:27:56 -0500},
  date-modified = {2008-09-03 13:27:56 -0500},
  keywords = {NucleicAcids; Solvation; Electrostatics; pKa},
  read = {Yes},
  ty = {JOUR},
  url = {http://dx.doi.org/10.1016/j.jmb.2006.12.001}
}

@ARTICLE{Huazhong:2003,
  author = {Tang, H. and Tang, T.},
  title = {{Adaptive mesh methods for one-and two-dimensional hyperbolic conservation
	laws}},
  journal = {J. Comput. Phys.},
  year = {2001},
  volume = {41},
  pages = {487--515}
}

@ARTICLE{Tang:2006,
  author = {Tang, S. and Hou, T. Y. and Liu, W. K.},
  title = {A pseudo-spectral multiscale method: interfacial conditions and coarse
	grid equations},
  journal = {J. Comput. Phys.},
  year = {2006},
  volume = {213},
  pages = {57 - 85}
}

@ARTICLE{Tang:2005,
  author = {Tang, T. },
  title = {{Moving mesh methods for computational fluid dynamics}},
  journal = {Contemporary Mathematics},
  year = {2005},
  volume = {383}
}

@ARTICLE{Tannor:1994,
  author = {Tannor, D. J. and Marten, B. and Murphy, R. and Friesner, R. A. and
	Sitkoff, D. and Nicholls, A. and Ringnalda, M. and Goddard, W. A.
	and Honig, B.},
  title = {Accurate First Principles Calcualtion of Molecular Charge Distribution
	and Solvation Energies from Ab Initio Quantum Mechanics and Continuum
	Dielectric Theory},
  journal = {J. Am. Chem. Soc.},
  year = {1994},
  volume = {116},
  pages = {11875 - 11882}
}

@ARTICLE{SurfaceProcessing,
  author = {T. Tasdizen and R. Whitaker and P. Burchard and S. Osher},
  title = {{Geometric Surface Processing via Normal Maps}},
  journal = {ACM Trans. on Graphics},
  year = {2003},
  volume = {2},
  pages = {1012--1033},
  number = {4}
}

@ARTICLE{TTasdizen:2003,
  author = {Tasdizen, T. and Whitaker, R. and Burchard, P. and Osher, S.},
  title = {Geometric surface processing via normal maps},
  journal = {Acm Transactions on Graphics},
  year = {2003},
  volume = {22},
  pages = {1012-1033},
  number = {4}
}

@INPROCEEDINGS{Taubin95,
  author = {Gabriel Taubin},
  title = {A signal processing approach to fair surface design},
  booktitle = {ACM SIGGRAPH},
  year = {1995},
  pages = {351--358}
}

@INPROCEEDINGS{Taubin:1995:ASP,
  author = {Gabriel Taubin},
  title = {A Signal Processing Approach to Fair Surface Design},
  booktitle = {Proc. of SIGGRAPH},
  year = {1995},
  pages = {351--358},
  month = aug
}

@ARTICLE{Tautges1996,
  author = {Tautges, T J and Blacker, T and Mitchell, S A},
  title = {{The Whisker Weaving Algorithm: a Connectivity-Based Method for Constructing
	All-Hexahedral Finite Element Meshes}},
  journal = {International Journal for Numerical Methods in Engineering},
  year = {1996},
  volume = {39},
  pages = {3327--3349},
  number = {19},
  doi = {10.1002/(SICI)1097-0207(19961015)39:19<3327::AID-NME2>3.0.CO;2-H},
  issn = {00295981},
  url = {http://doi.wiley.com/10.1002/%28SICI%291097-0207%2819961015%2939%3A19%3C3327%3A%3AAID-NME2%3E3.0.CO%3B2-H}
}

@ARTICLE{Tawa:1998,
  author = {Tawa, G. J. and Topol, I. A. and Burt, S. K. and Caldwell, R. A.
	and Rashin, A. A. },
  title = {Calculation of the aqueous solvation free energy of the proton},
  journal = {The Journal of Chemical Physics},
  year = {1998},
  volume = {109},
  pages = {4852--4863},
  number = {12},
  abstract = {View This Record in Scopus},
  bdsk-url-1 = {http://link.aip.org/link/?JCPSA6/109/4852/1},
  date-added = {2008-06-30 06:27:53 -0500},
  date-modified = {2008-06-30 06:27:53 -0500},
  keywords = {electrostatics, pka, solvation},
  posted-at = {2008-06-30 12:27:13},
  priority = {0},
  publisher = {AIP},
  url = {http://link.aip.org/link/?JCPSA6/109/4852/1}
}

@ARTICLE{Taylor:2000,
  author = {Taylor, W.R.},
  title = {A deeply knotted protein structure and how it might fold},
  journal = {NATURE},
  year = {2000},
  volume = {406},
  pages = {916-919 },
  number = { }
}

@ARTICLE{sagaut00,
  author = {Tenaud, C. and Garnier, E. and Sagaut, P.},
  title = {Evaluation of some high-order shock capturing schemes for direct
	numerical simulation of unsteady two-dimensional free flows},
  journal = {Int. J. Numer. Meth. Fluids},
  year = {2000},
  volume = {33},
  pages = {249-278}
}

@ARTICLE{Terekhova:2010,
  author = {Terekhova, I. V. and Romanova, A. O. and Kumeev, R. S. and Fedorov,
	M. V. },
  title = {Selective Na+/K+ Effects on the Formation of $\alpha$-Cyclodextrin
	Complexes with Aromatic Carboxylic Acids: Competition for the Guest
	
	},
  journal = {J. Phys. Chem. B},
  year = {2010},
  volume = {114},
  pages = {12607-2613},
  number = {37}
}

@ARTICLE{Thompson:1974,
  author = {Thompson, J. F. and Thames, F. C. and Mastin, C. W.},
  title = {{Automatic numerical generation of body-fitted curvilinear coordinate
	system for field containing any number of arbitrary two-dimensional
	bodies}},
  journal = {J. Comput. Phys.},
  year = {1974},
  volume = {15},
  pages = {299--319}
}

@BOOK{Thompson:1985,
  title = {Numerical Grid Generation},
  publisher = {North-Holland},
  year = {1985},
  author = {Thompson, J. F. and Warsi, Z. U. A. and Mastin, C. W.},
  address = {New York}
}

@ARTICLE{Tieleman:2001,
  author = {Tieleman, D. P. and Biggin, P. C. and Smith , G. R. and Sansom, M.
	S. P. },
  title = {Simulation approaches to ion channel structure?Cfunction relationships},
  journal = {Quarterly Reviews of Biophysics},
  year = {2001},
  volume = {34},
  pages = {473-561},
  number = {04}
}

@ARTICLE{Till:2008,
  author = {Till, Mirco S. and Essigke, Timm and Becker, Torsten and Ullmann,
	G. Matthias },
  title = {Simulating the Proton Transfer in {Gramicidin A} by a Sequential
	Dynamical {Monte Carlo} Method},
  journal = {J. Phys. Chem},
  year = {2008},
  volume = {112},
  pages = {13401-13410}
}

@ARTICLE{Tjong:2007a,
  author = {Tjong, H. and Zhou, H. -X.},
  title = {GBr6: A Parameterization-Free, Accurate, Analytical Generalized {Born}
	Method},
  journal = {Journal of Physical Chemistry B},
  year = {in press},
  abstract = {The {Poisson-Boltzmann} (PB) equation is widely used for modeling
	electrostatic effects and solvation for macromolecules. The generalized
	Born (GB) model has been developed to mimic PB results at substantial
	lower computational cost. Here, we report an analytical GB method
	that reproduces PB results with high accuracy. The analytical approach
	builds on previous work of Gallicchio and Levy (J. Comput. Chem.
	2004, 25, 479), and incorporates an improvement, proposed by Grycuk
	(J. Chem. Phys. 2003, 119, 4817), of the Coulomb-field approximation
	used in most GB methods. Tested against PB results, our GB method
	has an average unsigned relative error of only 0.6{\%} for a representative
	set of 55 proteins and of 0.4{\%} and 0.3{\%}, respectively, for
	folded and unfolded conformations of cytochrome b562 sampled in molecular
	dynamics simulations. The dependencies of the electrostatic solvation
	free energy on solute and solvent dielectric constants and on salt
	concentration are fully accounted for in our method.},
  annote = {GBr6: A Parameterization-Free, Accurate, Analytical Generalized Born
	Method},
  bdsk-url-1 = {http://dx.doi.org/10.1021/jp066284c},
  date-added = {2008-08-29 15:50:55 -0500},
  date-modified = {2008-08-29 15:50:55 -0500},
  keywords = {Electrostatics; Solvation},
  read = {Yes},
  ty = {JOUR},
  url = {http://dx.doi.org/10.1021/jp066284c}
}

@ARTICLE{Tjong:2007b,
  author = {Tjong, H. and Zhou, H. -X.},
  title = {{GBr6NL}: A generalized {Born} method for accurately reproducing
	solvation energy of the nonlinear {{Poisson-Boltzmann}} equation},
  journal = {Journal of Chemical Physics},
  year = {2007},
  volume = {126},
  pages = {195102},
  abstract = {The nonlinear {Poisson-Boltzmann} (NLPB) equation can provide accurate
	modeling of electrostatic effects for nucleic acids and highly charged
	proteins. Generalized Born methods have been developed to mimic the
	linearized {Poisson-Boltzmann} (LPB) equation at substantially reduced
	cost. The computer time for solving the NLPB equation is ~fivefold
	longer than for the LPB equation, thus presenting an even greater
	obstacle. Here we present the first generalized Born method, GBr6NL,
	for mimicking the NLPB equation. GBr6NL is adapted from GBr6, a generalized
	Born method recently developed to reproduce the solvation energy
	of the LPB equation [Tjong and Zhou, J. Phys. Chem. B 111, 3055 (2007)].
	Salt effects predicted by GBr6NL on 55 proteins overall deviate from
	NLPB counterparts by 0.5 kcal/mol from ionic strengths from 10 to
	1000 mM, which is ~10% of the average magnitudes of the salt effects.
	GBr6NL predictions for the salts effects on the electrostatic interaction
	energies of two protein:RNA complexes are very promising},
  bdsk-url-1 = {http://dx.doi.org/10.1063/1.2735322},
  date-added = {2008-09-01 14:01:26 -0500},
  date-modified = {2008-09-01 14:01:26 -0500},
  keywords = {Solvation; Electrostatics},
  url = {http://dx.doi.org/10.1063/1.2735322}
}

@ARTICLE{Tomasi:2005,
  author = { Tomasi, Jacopo and Mennucci, Benedetta and Cammi, Roberto},
  title = {Quantum mechanical continuum solvation models},
  journal = {Chem. Rev.},
  year = {2005},
  volume = {105},
  pages = {2999--3093}
}

@ARTICLE{Tomasi:1994,
  author = {Tomasi, J. and Persico, M.},
  title = {Molecular Interactions in Solution: An Overview of Methods Based
	on Continuous Distributions of the Solvent},
  journal = {Chem. Rev.},
  year = {1994},
  volume = {94},
  pages = {2027-2094}
}

@INPROCEEDINGS{TACD06,
  author = {Yiying Tong and Pierre Alliez and David Cohen-Steiner and Mathieu
	Desbrun},
  title = {Designing Quadrangulations with Discrete Harmonic Forms},
  booktitle = {ACM/EG Symposium on Geometry Processing},
  year = {2006},
  pages = {201--210},
  month = Jul
}

@ARTICLE{TLHD03,
  author = {Yiying Tong and Santiago Lombeyda and Anil Hirani and Mathieu Desbrun},
  title = {Discrete Multiscale Vector Field Decomposition},
  journal = {ACM Trans. on Graphics (SIGGRAPH)},
  year = {2003},
  volume = {22},
  pages = {445--452},
  number = {3},
  month = jun
}

@ARTICLE{Tornberg:2004,
  author = {Tornberg, Anna-Karin and Engquist, BjÃ¶rn},
  title = {Numerical approximations of singular source terms in differential
	equations},
  journal = {J. Comput. Phys.},
  year = {2004},
  volume = {200},
  pages = {462--488},
  number = {2},
  abstract = { Singular terms in differential equations pose severe challenges for
	numerical approximations on regular grids. Regularization of the
	singularities is a very useful technique for their representation
	on the grid. We analyze such techniques for the practically preferred
	case of narrow support of the regularizations, extending our earlier
	results for wider support. The analysis also generalizes existing
	theory for one dimensional problems to multi-dimensions. New high
	order multi-dimensional techniques for differential equations and
	numerical quadrature are introduced based on the analysis and numerical
	results are presented. We also show that the common use of distance
	functions in level-set methods to extend one dimensional regularization
	to higher dimensions may produce O(1) errors.},
  bdsk-url-1 = {http://www.sciencedirect.com/science/article/B6WHY-4CKNKH3-3/2/33dd215487ffd168edaf9a816a35c0f1},
  date-added = {2008-09-14 15:32:12 -0500},
  date-modified = {2008-09-14 15:32:12 -0500},
  doi = {10.1016/j.jcp.2004.04.011 },
  keywords = {Mathematics},
  ty = {JOUR},
  url = {http://www.sciencedirect.com/science/article/B6WHY-4CKNKH3-3/2/33dd215487ffd168edaf9a816a35c0f1}
}

@ARTICLE{toro98,
  author = {Toro, E. F. and Millington, R. C. and Titarev, V. A. },
  title = {DER: arbitrary-order non-oscillatory advection scheme},
  journal = {{\it Proc. 8th International Conference on Non-linear Hyperbolic
	Problems}, Magdeburg, Germany, March},
  year = {2000}
}

@ARTICLE{Tournois2009,
  author = {Tournois, Jane and Wormser, Camille and Alliez, Pierre and Desbrun,
	Mathieu},
  title = {Interleaving Delaunay refinement and optimization for practical isotropic
	tetrahedron mesh generation},
  journal = {ACM Trans. Graph. (SIGGRAPH)},
  year = {2009},
  volume = {28},
  pages = {75:1--75:9},
  number = {3},
  month = jul,
  acmid = {1531381},
  address = {New York, NY, USA},
  articleno = {75},
  doi = {10.1145/1531326.1531381},
  issn = {0730-0301},
  issue_date = {August 2009},
  keywords = {Delaunay refinement, graded meshing, isotropic meshing, mesh generation,
	mesh optimization},
  numpages = {9},
  publisher = {ACM},
  url = {http://doi.acm.org/10.1145/1531326.1531381}
}

@ARTICLE{Tozzini:2005,
  author = {Tozzini, V.},
  title = {Coarse-grained models for proteins},
  journal = {Current Opinion in Structural Biology },
  year = {2005},
  volume = {15},
  pages = {144-150},
  annote = {Coarse-grained models for proteins},
  date-added = {2009-03-10 },
  date-modified = {2009-03-10},
  ty = {JOUR}
}

@BOOK{Trefethen,
  title = {Spectral Methods in Matlab},
  publisher = {Oxford University, Oxford, England},
  year = {2000},
  author = {Trefethen, L. N.}
}

@ARTICLE{Trellakis:1997,
  author = {Trellakis, A. and Galick, A. T. and Pacelli, A. and Ravaioli, U.},
  title = {{Iteration scheme for the solution of the two-dimensional Schr\"{o}dinger-Poisson
	equations in quantum structures}},
  journal = {J. Appl. Phys.},
  year = {1997},
  volume = {81},
  pages = {7880-7884},
  annote = {Iteration scheme for the solution of the two-dimensional Schrodinger-Poisson
	equations in quantum structures},
  date-added = {2008-11-25 10:28:56 -0500},
  date-modified = {2008-11-25 10:28:56 -0500},
  ty = {JOUR}
}

@ARTICLE{Tsui:2001,
  author = {Tsui, V. and Case, D. A.},
  title = {Calculations of the Absolute Free Energies of Binding between {RNA}
	and Metal Ions Using Molecular Dynamics Simulations and Continuum
	Electrostatics},
  journal = {Journal of Physical Chemistry B},
  year = {2001},
  volume = {105},
  pages = {11314-11325},
  number = {45},
  abstract = {The calculation of binding free energies between highly charged species
	is a major challenge for free energy simulations. In this study,
	we applied a combination of molecular dynamics simulations and continuum
	electrostatics, along with normal-mode analysis, to compute the absolute
	free energies of binding between cobalt (III) hexammine and two RNA
	fragments for which NMR structures have been determined. The predicted
	affinities, using the finite-difference {Poisson-Boltzmann} method
	with a solute dielectric constant of 1 to treat solvation, were overall
	underestimated relative to the experimental values. However, internal
	consistency in the calculated energies was maintained between the
	different trajectories, and the structures in the simulations gave
	excellent agreement with NMR data. Various models for obtaining the
	electrostatic contributions were analyzed, including the effects
	of solute dielectric constants and {van der Waals} radii, linear
	and nonlinear salt contributions, as well as results from generalized
	Born versus finite-difference {Poisson-Boltzmann} models. These provide
	insight into the strengths and limitations in the current methods
	and force fields for free energy calculations.},
  annote = {Calculations of the Absolute Free Energies of Binding between RNA
	and Metal Ions Using Molecular Dynamics Simulations and Continuum
	Electrostatics},
  bdsk-url-1 = {http://dx.doi.org/10.1021/jp011923z},
  date-added = {2008-09-01 14:01:14 -0500},
  date-modified = {2008-09-01 14:01:14 -0500},
  keywords = {Electrostatics; NucleicAcids},
  ty = {JOUR},
  url = {http://dx.doi.org/10.1021/jp011923z}
}

@ARTICLE{Tsui:2000,
  author = {Tsui, V. and Case, D. A.},
  title = {Molecular dynamics simulations of nucleic acids with a generalized
	{Born} solvation model},
  journal = {Journal of the American Chemical Society},
  year = {2000},
  volume = {122},
  pages = {2489-2498},
  number = {11},
  abstract = {A generalized Born (GB) model has been applied to molecular dynamics
	simulations of the A- and B-forms of a duplex DNA d(CCAACGTTGG)2
	and the corresponding duplex RNA r(CCAACGUUGG)2, resulting in good
	agreement with simulations using explicit water solvent in terms
	of both structure and energetics. In particular, the A B energy differences
	derived from GB trajectories for both DNA and RNA closely match those
	obtained earlier using explicit water simulations and finite-difference
	{Poisson-Boltzmann} calculations. A GB simulation starting from A-form
	DNA converges to B-DNA within 20 ps, more than 20 times faster than
	the transition from A- to B-DNA in explicit solvent simulations.
	For B-form d(CCAACGTTGG)2, fluctuations about the mean are highly
	correlated between GB and explicit water simulations, being slightly
	larger in the former, and the essential subspaces found from principal
	component analysis overlap to a high degree. Hence, for many purposes
	this parametrization offers an alternative to more expensive explicit
	water simulations for studies of nucleic acid energetics and structure.},
  address = {Scripps Clin \& Res Inst La Jolla, CA USA 92037 Case, DA Dept Mol
	Biol Scripps Clin \& Res Inst La Jolla, CA USA 92037 Dept Mol Biol},
  annote = {Molecular dynamics simulations of nucleic acids with a generalized
	Born solvation model; MAR 22},
  bdsk-url-1 = {http://dx.doi.org/10.1021/ja9939385},
  date-added = {2008-09-01 13:59:26 -0500},
  date-modified = {2008-09-01 13:59:26 -0500},
  journal1 = {J Amer Chem Soc},
  keywords = {MolecularSimulation; Electrostatics},
  ty = {JOUR},
  url = {http://dx.doi.org/10.1021/ja9939385}
}

@ARTICLE{Tully-Smith:1970,
  author = {Tully-Smith, D. M. and Reiss, H.},
  title = {Further Development of Scaled Particle Theory of Rigid Sphere Fluids},
  journal = {Journal of Chemical Physics},
  year = {1970},
  volume = {53},
  pages = {4015-25},
  number = {10},
  abstract = {A new approach to the scaled particle theory of fluids is developed
	which is based on detailed consideration of the reversible work required
	to create a fixed spherical cavity of radius r in a rigid sphere
	fluid. The new results depend only on the mechanical concept of work
	and the classical virial theorem. A cycle greatly facilitates the
	necessary detailed analysis. A new integral equation for G(r), the
	primary function in scaled particle theory, culminates the new results.
	Approximation schemes may be employed relatively easily in this integral
	equation. The series approximation [dformula G(r) [equals sign] [summation][sub
	n [equals sign] 0][sup [infinity]]G[sub n](r[sup -1])[sup n],] which
	is asymptotically correct as r --> [infinity], is discussed. A new
	set of exact conditions on the coefficients Gn in this asymptotic
	expansion, the most striking of which is G3 [equivalent] 0 in three
	dimensions, is derived. These exact conditions relate to surface
	properties. The infinity and integral exact conditions on G(r) are
	shown to be truly independent. The jump condition on the second derivative
	of G(r) is incorporated successfully for the first time with other
	exact conditions in the derivation of two new expressions for G(a),
	both of which give rise to equations of state. One of these expressions
	yields the best virial coefficients thus far obtained for a rigid
	sphere system from any analytic equation of state not based on cluster
	expansions. The new approach and results are easily generalized to
	arbitrary dimension. Future work will center on attempts to extend
	the new integral equation for G(r), on possible extensions of the
	present method to real fluids, and on studies of the nature of the
	asymptotic series approximation scheme},
  annote = {Further Development of Scaled Particle Theory of Rigid Sphere Fluids},
  bdsk-file-1 = {YnBsaXN0MDDUAQIDBAUGCQpYJHZlcnNpb25UJHRvcFkkYXJjaGl2ZXJYJG9iamVjdHMSAAGGoNE
	HCFRyb290gAFfEA9OU0tleWVkQXJjaGl2ZXKoCwwXGBkdJCVVJG51bGzTDQ4PEBEUViRjbGFzc1
	dOUy5rZXlzWk5TLm9iamVjdHOAB6ISE4ACgAOiFRaABIAGWWFsaWFzRGF0YVxyZWxhdGl2ZVBhd
	GjSDRobHFdOUy5kYXRhgAVPEQHSAAAAAAHSAAIAAAxNYWNpbnRvc2ggSEQAAAAAAAAAAAAAAAAA
	AADD4v5NSCsAAAAZYksZMTk3MC1UdWxseS1TbWl0aFJlaXNzLnBkZgAAAAAAAAAAAAAAAAAAAAA
	AAAAAAAAAAAAAAAAAAAAAAAAAAAAAABkGvMD73KwAAAAAAAAAAAAEAAQAAAkgAAAAAAAAAAAAAA
	AAAAAAB0FyY2hpdmUAABAACAAAw+NSrQAAABEACAAAwPwi/AAAAAEAFAAZYksAGWIDAAqkKAAKp
	BEAAHrcAAIAT01hY2ludG9zaCBIRDpVc2VyczpiYWtlcjpEb2N1bWVudHM6UmVmZXJlbmNlczpB
	cmNoaXZlOjE5NzAtVHVsbHktU21pdGhSZWlzcy5wZGYAAA4ANAAZADEAOQA3ADAALQBUAHUAbAB
	sAHkALQBTAG0AaQB0AGgAUgBlAGkAcwBzAC4AcABkAGYADwAaAAwATQBhAGMAaQBuAHQAbwBzAG
	gAIABIAEQAEgBCVXNlcnMvYmFrZXIvRG9jdW1lbnRzL1JlZmVyZW5jZXMvQXJjaGl2ZS8xOTcwL
	VR1bGx5LVNtaXRoUmVpc3MucGRmABMAAS8AABUAAgAM//8AANIeHyAhWCRjbGFzc2VzWiRjbGFz
	c25hbWWjISIjXU5TTXV0YWJsZURhdGFWTlNEYXRhWE5TT2JqZWN0XxBCLi4vLi4vLi4vLi4vRG9
	jdW1lbnRzL1JlZmVyZW5jZXMvQXJjaGl2ZS8xOTcwLVR1bGx5LVNtaXRoUmVpc3MucGRm0h4fJi
	eiJyNcTlNEaWN0aW9uYXJ5AAgAEQAaAB8AKQAyADcAOgA/AEEAUwBcAGIAaQBwAHgAgwCFAIgAi
	gCMAI8AkQCTAJ0AqgCvALcAuQKPApQCnQKoAqwCugLBAsoDDwMUAxcAAAAAAAACAQAAAAAAAAAo
	AAAAAAAAAAAAAAAAAAADJA==},
  bdsk-url-1 = {http://dx.doi.org/10.1063/1.1673873},
  date-added = {2008-09-17 09:14:02 -0500},
  date-modified = {2008-09-17 09:14:02 -0500},
  keywords = {Solvation; StatisticalMechanics},
  ty = {JOUR},
  url = {http://dx.doi.org/10.1063/1.1673873}
}

@ARTICLE{Turner:2002,
  author = {Turner, S. W. P. and Cabodi, M. and Craighead, H. G. },
  title = {Confinement-induced entropic recoil of single DNA molecules in a
	nanofluidic structure },
  journal = {Phys. Rev. Lett. },
  year = {2002},
  volume = {88},
  number = { 128103 }
}

@ARTICLE{Tyagi:2010,
  author = {Tyagi, S. and Suzen, M. and Sega, M. and Barbosa, M. and Kantorovich,
	S .S. and Holm, C. },
  title = {{An iterative, fast, linear-scaling method for computing induced
	charges on arbitrary dielectric boundaries}},
  journal = {J Chem Phys },
  year = {2010},
  volume = {132(15)},
  pages = {154112-9.}
}

@ARTICLE{Tynan-Connolly:2007,
  author = {Tynan-Connolly, B. M. and Nielsen, J. E.},
  title = {Redesigning protein {pKa} values},
  journal = {Protein Science},
  year = {2007},
  volume = {16},
  pages = {239-49},
  number = {2},
  abstract = {The ability to re-engineer enzymatic pH-activity profiles is of importance
	for industrial applications of enzymes. We theoretically explore
	the feasibility of re-engineering enzymatic pH-activity profiles
	by changing active site pKa values using point mutations. We calculate
	the maximum achievable pKa values for 141 target titratable groups
	in seven enzymes by introducing conservative net-charge altering
	point mutations. We examine the importance of the number of mutations
	introduced, their distance from the target titratable group, and
	the characteristics of the target group itself. The results show
	that multiple mutations at 10Ãƒ can change pKa values up to two
	units, but that the introduction of a requirement to keep other pKa
	values constant reduces the magnitude of the achievable pKa. The
	algorithm presented shows a good correlation with existing experimental
	data and is available for download and via a web server at http://enzyme.ucd.ie/pKD.},
  annote = {Redesigning protein pKa values},
  bdsk-url-1 = {http://dx.doi.org/10.1110/ps.062538707},
  date-added = {2008-09-16 15:42:42 -0500},
  date-modified = {2008-09-16 15:42:42 -0500},
  keywords = {Solvation; pKa; ProteinEngineering; Electrostatics},
  ty = {JOUR},
  url = {http://dx.doi.org/10.1110/ps.062538707}
}

@ARTICLE{Tynan-Connolly:2006,
  author = {Tynan-Connolly, B. M. and Nielsen, J. E.},
  title = {{pKD}: re-designing protein {pKa} values},
  journal = {Nucleic Acids Research},
  year = {2006},
  volume = {34},
  pages = {W48-W51},
  abstract = {The pKa values in proteins govern the pH-dependence of protein stability
	and enzymatic activity. A large number of mutagenesis experiments
	have been carried out in the last three decades to re-engineer the
	pH-activity and pH-stability profile of enzymes and proteins. We
	have developed the pKD webserver (http://polymerase.ucd.ie/pKa{\_}Design),
	which predicts sets of point mutations that will change the pKa values
	of a set of target residues in a given direction, thus allowing for
	targeted re-design of the pH-dependent characteristics of proteins.
	The server provides the user with an interactive experience for re-designing
	pKa values by pre-calculating pKa values from all feasible point
	mutations. Design solutions are found in less than 10 min for a typical
	design job for a medium-sized protein. Mutant pKa values calculated
	by the pKD web server are in close agreement with those produced
	by comparing results from full-fledged pKa calculation methods.},
  annote = {pKD: re-designing protein pKa values},
  bdsk-url-1 = {http://dx.doi.org/10.1093/nar/gkl192},
  date-added = {2008-09-16 15:42:27 -0500},
  date-modified = {2008-09-16 15:42:27 -0500},
  keywords = {Solvation; Electrostatics; pKa},
  ty = {JOUR},
  url = {http://dx.doi.org/10.1093/nar/gkl192}
}

@ARTICLE{Ullmo05201310,
  author = {Ullmo, D. and Jiang, H. and Yang, W. T. and Baranger, H. U.},
  title = {Interactions and broken time-reversal symmetry in chaotic quantum
	dots},
  journal = {Physical Review B},
  year = {2005},
  volume = {71},
  pages = {201310},
  number = {20},
  month = {May},
  abstract = {When treating interactions in quantum dots within a random-phase-
	approximation (RPA)-like approach, time-reversal symmetry plays an
	important role as higher-order terms-the Cooper series-need to be
	included when this symmetry is present. Here we consider model quantum
	dots in a magnetic field weak enough to leave the dynamics of the
	dot chaotic, but strong enough to break time-reversal symmetry. The
	ground-state spin and addition energy for dots containing 120-200
	electrons are found using local spin-density-functional theory, and
	we compare the corresponding distributions with those derived from
	an RPA-like treatment of the interactions. The agreement between
	the two approaches is very good, significantly better than for analogous
	calculations in the presence of time-reversal-symmetry. This demonstrates
	that the discrepancies between the two approaches in the time-reversal
	symmetric case indeed originate from the Cooper channel, indicating
	that these higher order terms might not be properly taken into account
	in the spin-density-functional calculations.},
  endnotereftype = {Journal Article},
  issn = {1098-0121},
  shorttitle = {Interactions and broken time-reversal symmetry in chaotic quantum
	dots},
  url = {<Go to ISI>://000230244300012}
}

@ARTICLE{Ullmo04205309,
  author = {Ullmo, D. and Jiang, H. and Yang, W. T. and Baranger, H. U.},
  title = {Landau Fermi-liquid picture of spin density functional theory: Strutinsky
	approach to quantum dots},
  journal = {Physical Review B},
  year = {2004},
  volume = {70},
  pages = {205309},
  number = {20},
  month = {Nov},
  abstract = {We analyze the ground-state energy and spin of quantum dots obtained
	from spin density functional theory (SDFT) calculations. First, we
	introduce a Strutinsky-type approximation, in which quantum interference
	is treated as a correction to a smooth Thomas-Fermi description.
	For large irregular dots, we find that the second-order Strutinsky
	expressions have an accuracy of about 5% of a mean level spacing
	compared to the full SDFT and capture all the qualitative features.
	Second, we perform a random matrix-theory/random-plane wave analysis
	of the Strutinsky SDFT expressions. The results are statistically
	similar to the SDFT quantum dot statistics. Finally, we note that
	the second-order Strutinsky approximation provides, in essence, a
	Landau Fermi-liquid picture of spin density functional theory. For
	instance, the leading term in the spin channel is simply the familiar
	exchange constant. A direct comparison between SDFT and the perturbation
	theory derived "universal Hamiltonian" is thus made possible.},
  endnotereftype = {Journal Article},
  issn = {1098-0121},
  shorttitle = {Landau Fermi-liquid picture of spin density functional theory: Strutinsky
	approach to quantum dots},
  url = {<Go to ISI>://000225478600074}
}

@ARTICLE{Urbic:2006,
  author = {Urbic, T. and Vlachy, V. and Dill, K.A.},
  title = {{Confined Water: A Mercedes-Benz Model Study}},
  journal = {Journal of Physical Chemistry},
  year = {2006},
  volume = {110},
  pages = {4963 - 4970}
}

@ARTICLE{Valentini:2009,
  author = {Valentini, P. and Schwartzentruber, T. E.},
  title = {Large-scale molecular dynamics simulations of normal shock waves
	in dilute argon
	
	},
  journal = {Phys. Fluids},
  year = {2009},
  volume = {21},
  pages = { },
  number = { 066101 }
}

@INPROCEEDINGS{Levy07,
  author = {Bruno Vallet and Bruno Levy},
  title = {Spectral Geometry Processing with Manifold Harmonics},
  booktitle = {Tech Report},
  year = {2007}
}

@ARTICLE{Vande-Voorde:2004,
  author = {Vande Voorde, J. John and Vierendeels, Jan and Dick, Erik},
  title = {Flow simulations in rotary volumetric pumps and compressors with
	the fictitious domain method},
  journal = {Journal of Computational and Applied Mathematics},
  year = {2004},
  volume = {168},
  pages = {491--499},
  number = {1-2},
  abstract = { The fictitious domain (FD) method is an interesting method of flow
	calculation for domains where mesh generation is not straightforward.
	This method has been reported in literature to be able to simulate
	flow in relatively open domains with incompressible fluids. In this
	paper a FD technique is tested for flow calculations inside closed
	geometries and for compressible flow. The computational fluid dynamics
	code FLUENT, versions 5.4 and 6.0, has been extended with user-defined
	functions and has been used for the analysis of incompressible flow
	in a lobe pump and the analysis of compressible flow in a tooth compressor.
	The results show that the FD method can be made to work for incompressible
	flow, although further development is necessary for compressible
	flow.},
  bdsk-url-1 = {http://www.sciencedirect.com/science/article/B6TYH-4C6TJV0-1/2/ed7cdd729f04acc25e2ba89dfc2f3f72},
  booktitle = {Selected Papers from the Second International Conference on Advanced
	Computational Methods in Engineering (ACOMEN 2002)},
  date-added = {2008-09-14 15:32:12 -0500},
  date-modified = {2008-09-14 15:32:12 -0500},
  doi = {10.1016/j.cam.2003.04.007 },
  keywords = {Mathematics; FluidMechanics},
  ty = {JOUR},
  url = {http://www.sciencedirect.com/science/article/B6TYH-4C6TJV0-1/2/ed7cdd729f04acc25e2ba89dfc2f3f72}
}

@ARTICLE{vandeven91,
  author = {Vandeven, H.},
  title = {Family of spectral filters for discontinuous problems},
  journal = {J. Sci. Comput.},
  year = {1991},
  volume = {6},
  pages = {159-192}
}

@ARTICLE{Varga:2007,
  author = {Varga, K. and Pantelides, S. T. },
  title = {Quantum transport in molecules and nanotube devices},
  journal = {PHYSICAL REVIEW LETTERS},
  year = {2007},
  volume = {98},
  number = { 076804}
}

@ARTICLE{Vath:1999,
  author = {Vath, P. and Zimmt, M. B. and Matyushov, D. V. and Voth, G. A.},
  title = {A Failure of Continuum Theory: Temperature Dependence of the Solvent
	Reorganization Energy of Electron Transfer in Highly Polar Solvents},
  journal = {J. Phys. Chem. B},
  year = {1999},
  volume = {103},
  pages = {9130- 9140}
}

@ARTICLE{Venturi:1989,
  author = {Venturi, F. and Smith, R.K. and Sangiorgi, E. C. and Pinto, M. R.
	and Ricco, B.},
  title = {A general purpose device simulator coupling {Poisson} and {Monte
	Carlo} transport with applications to deep submicron {MOSFETs}},
  journal = {IEEE Trans. Computer-Aided Design},
  year = {1989},
  volume = {8},
  pages = {360}
}

@ARTICLE{Venugopal:2002,
  author = {Venugopal, R. and Ren, Z. and Datta, S. and Lundstrom, M. S.},
  title = {Simulating quantum transport in nanoscale transitors: Real versus
	mode-space approaches},
  journal = {J. App. Phys.},
  year = {2002},
  volume = {92},
  pages = {3730-3739}
}

@ARTICLE{Vieth:1994,
  author = {Vieth, M. and Kolinski, A. and Brooks, C. L. 3rd, and Skolnick, J.},
  title = {{Prediction of the folding pathways and structure of the GCN4 leucine
	zipper}},
  journal = {J Mol Biol},
  year = {1994},
  volume = {237},
  pages = {361-367},
  number = {4}
}

@ARTICLE{Vince1983,
  author = {Vince, A},
  title = {{Combinatorial maps}},
  journal = {Journal of Combinatorial Theory Series B},
  year = {1983},
  volume = {34},
  pages = {1--21},
  number = {1},
  doi = {10.1016/0095-8956(83)90002-3},
  file = {:C\:/Dropbox/Dropbox/Paper/Combinatorial maps.pdf:pdf},
  issn = {00958956},
  owner = {doubletony},
  publisher = {Citeseer},
  timestamp = {2012.04.26},
  url = {http://linkinghub.elsevier.com/retrieve/pii/0095895683900023}
}

@ARTICLE{ISIM,
  author = {Vitalis, A. and Baker, N. A. and McCammon, J. A.},
  title = {{ISIM}: A Program for Grand Canonical {Monte Carlo} Simulations of
	the Ionic Environment of Biomolecules},
  journal = {Molecular Simulation},
  year = {2004},
  volume = {30},
  pages = {45-61},
  number = {1},
  annote = {ISIM: A Program for Grand Canonical Monte Carlo Simulations of the
	Ionic Environment of Biomolecules; ISIM},
  bdsk-file-1 = {YnBsaXN0MDDUAQIDBAUGCQpYJHZlcnNpb25UJHRvcFkkYXJjaGl2ZXJYJG9iamVjdHMSAAGGoNE
	HCFRyb290gAFfEA9OU0tleWVkQXJjaGl2ZXKoCwwXGBkdJCVVJG51bGzTDQ4PEBEUViRjbGFzc1
	dOUy5rZXlzWk5TLm9iamVjdHOAB6ISE4ACgAOiFRaABIAGWWFsaWFzRGF0YVxyZWxhdGl2ZVBhd
	GjSDRobHFdOUy5kYXRhgAVPEQHiAAAAAAHiAAIAAAxNYWNpbnRvc2ggSEQAAAAAAAAAAAAAAAAA
	AADD4v5NSCsAAAAZYksdMjAwNC1WaXRhbGlzQmFrZXJNY0NhbW1vbi5wZGYAAAAAAAAAAAAAAAA
	AAAAAAAAAAAAAAAAAAAAAAAAAAAAAABliasM6CthQREYgcHJ2dwAEAAQAAAkgAAAAAAAAAAAAAA
	AAAAAAB0FyY2hpdmUAABAACAAAw+NSrQAAABEACAAAwzpRKAAAAAEAFAAZYksAGWIDAAqkKAAKp
	BEAAHrcAAIAU01hY2ludG9zaCBIRDpVc2VyczpiYWtlcjpEb2N1bWVudHM6UmVmZXJlbmNlczpB
	cmNoaXZlOjIwMDQtVml0YWxpc0Jha2VyTWNDYW1tb24ucGRmAAAOADwAHQAyADAAMAA0AC0AVgB
	pAHQAYQBsAGkAcwBCAGEAawBlAHIATQBjAEMAYQBtAG0AbwBuAC4AcABkAGYADwAaAAwATQBhAG
	MAaQBuAHQAbwBzAGgAIABIAEQAEgBGVXNlcnMvYmFrZXIvRG9jdW1lbnRzL1JlZmVyZW5jZXMvQ
	XJjaGl2ZS8yMDA0LVZpdGFsaXNCYWtlck1jQ2FtbW9uLnBkZgATAAEvAAAVAAIADP//AADSHh8g
	IVgkY2xhc3Nlc1okY2xhc3NuYW1loyEiI11OU011dGFibGVEYXRhVk5TRGF0YVhOU09iamVjdF8
	QRi4uLy4uLy4uLy4uL0RvY3VtZW50cy9SZWZlcmVuY2VzL0FyY2hpdmUvMjAwNC1WaXRhbGlzQm
	FrZXJNY0NhbW1vbi5wZGbSHh8mJ6InI1xOU0RpY3Rpb25hcnkACAARABoAHwApADIANwA6AD8AQ
	QBTAFwAYgBpAHAAeACDAIUAiACKAIwAjwCRAJMAnQCqAK8AtwC5Ap8CpAKtArgCvALKAtEC2gMj
	AygDKwAAAAAAAAIBAAAAAAAAACgAAAAAAAAAAAAAAAAAAAM4},
  bdsk-url-1 = {http://dx.doi.org/10.1080/08927020310001597862},
  date-added = {2008-09-01 14:06:52 -0500},
  date-modified = {2008-09-01 14:06:52 -0500},
  keywords = {Electrostatics; StatisticalMechanics; MolecularDynamics; Software;
	BeyondMeanField},
  ty = {JOUR},
  url = {http://dx.doi.org/10.1080/08927020310001597862}
}

@ARTICLE{Absinth,
  author = {Vitalis, A. and Pappu, R. V.},
  title = {{ABSINTH:} A new continuum solvation model for simulations of polypeptides
	in aqueous solutions},
  journal = {Journal of Computational Chemistry},
  year = {2009},
  volume = {30},
  pages = {673-99},
  number = {5},
  date-added = {2008-09-01 13:57:58 -0500},
  date-modified = {2008-09-01 13:57:58 -0500}
}

@ARTICLE{Vlachy:1999,
  author = {Vlachy, V.},
  title = {Ionic effects beyond Poisson-Boltzmann theory},
  journal = {Annu. Rev. Phys. Chem.},
  year = {1999},
  volume = {50},
  pages = {145-165.}
}

@ARTICLE{Vlassiouk:2009,
  author = {Vlassiouk, I. and Kozel, T. R. and Siwy, Z. S.},
  title = {Biosensing with Nanofluidic Diodes },
  journal = {Journal of the American Chemical Society },
  year = {2009},
  volume = {131},
  pages = {8211-8220}
}

@ARTICLE{Vlassiouk:2008,
  author = {Vlassiouk, I. and Smirnov, S. and Siwy, Z.},
  title = {Ionic selectivity of single nanochannels },
  journal = {Nano Letters},
  year = {2008},
  volume = {8},
  pages = {1978-1985 }
}

@ARTICLE{Vlassiouk:2008b,
  author = {Vlassiouk, I. and Smirnov, S. and Siwy, Z.},
  title = {Nanofluidic ionic diodes. Comparison of analytical and numerical
	solutions },
  journal = {ACS Nano },
  year = {2008},
  volume = {2},
  pages = { 1589-1602 }
}

@ARTICLE{Vorobjev:1997,
  author = {Vorobjev, Y. N. and Scheraga, H. A.},
  title = {A fast adaptive multigrid boundary element method for macromolecular
	electrostatic computations in a solvent},
  journal = {Journal of Computational Chemistry},
  year = {1997},
  volume = {18},
  pages = {569-583},
  number = {4},
  abstract = {A fast multigrid boundary element (MBE) method for solving the Poisson
	equation for macromolecular electrostatic calculations in a solvent
	is developed. To convert the integral equation of the BE method into
	a numerical linear equation of low dimensions, the MBE method uses
	an adaptive tesselation of the molecular surface by BEs with nonregular
	size. The size of the BEs increases in three successive levels as
	the uniformity of the electrostatic field on the molecular surface
	increases. The MBE method provides a high degree of consistency,
	good accuracy, and stability when the sizes of the BEs are varied.
	The computational complexity of the unrestricted MBE method scales
	as O(Nat), where Nat is the number of atoms in the macromolecule.
	The MBE method is ideally suited for parallel computations and for
	an integrated algorithm for calculations of solvation free energy
	and free energy of ionization, which are coupled with the conformation
	of a solute molecule. The current version of the 3-level MBE method
	is used to calculate the free energy of transfer from a vacuum to
	an aqueous solution and the free energy of the equilibrium state
	of ionization of a 17-residue peptide in a given conformation at
	a given pH in 400 s of CPU time on one node of the IBM SP2 supercomputer.},
  annote = {A fast adaptive multigrid boundary element method for macromolecular
	electrostatic computations in a solvent},
  bdsk-url-1 = {http://www3.interscience.wiley.com/cgi-bin/abstract/48486/ABSTRACT},
  date-added = {2008-06-29 14:51:59 -0500},
  date-modified = {2008-06-29 14:51:59 -0500},
  keywords = {Electrostatics},
  ty = {JOUR},
  url = {http://www3.interscience.wiley.com/cgi-bin/abstract/48486/ABSTRACT}
}

@BOOK{BrainMappingBook,
  title = {Brain Mapping: The Methods},
  publisher = {Academic Press},
  year = {2002},
  author = {Toga A. W. and Mazziotta J. C.\},
  edition = {Second},
  isbn = {0126930198}
}

@ARTICLE{Wade:2001,
  author = {Wade, R. C. and Gabdoulline, R. R. and De Rienzo, F.},
  title = {Protein interaction property similarity analysis},
  journal = {International Journal of Quantum Chemistry},
  year = {2001},
  volume = {83},
  pages = {122-127},
  number = {3-4},
  abstract = {We describe how similarity indices may be applied to semiquantitatively
	compare the molecular interaction fields, such as electrostatic and
	hydrophobic potentials, of proteins. We then review ways in which
	this approach has been used to investigate protein interaction properties
	in diverse applications ranging from in-depth comparison of pairs
	of proteins to large-scale analysis of hundreds of modeled protein
	structures.},
  address = {European Mol Biol Lab Heidelberg Germany D-69012 Wade, RC rebecca.wade{\char64}eml.villa-basch.de
	Meyerhofstr 1 European Mol Biol Lab Heidelberg Germany D-69012 European
	Media Lab Heidelberg Germany D-69118 Univ Modena \& Reggio Emilia
	Modena Italy I-41100 Dipartimento Chim},
  annote = {Protein interaction property similarity analysis; JUN 5},
  bdsk-url-1 = {http://www3.interscience.wiley.com/cgi-bin/abstract/80002581/ABSTRACT},
  date-added = {2008-09-15 10:06:52 -0500},
  date-modified = {2008-09-15 10:06:52 -0500},
  journal1 = {Int J Quantum Chem},
  keywords = {Electrostatics; Bioinformatics},
  read = {Yes},
  ty = {JOUR},
  url = {http://www3.interscience.wiley.com/cgi-bin/abstract/80002581/ABSTRACT}
}

@ARTICLE{Wagoner:2006,
  author = {Wagoner, J. A. and Baker, N. A.},
  title = {Assessing implicit models for nonpolar mean solvation forces: the
	importance of dispersion and volume terms},
  journal = {Proceedings of the National Academy of Sciences of the United States
	of America},
  year = {2006},
  volume = {103},
  pages = {8331-6},
  number = {22},
  abstract = {Continuum solvation models provide appealing alternatives to explicit
	solvent methods because of their ability to reproduce solvation effects
	while alleviating the need for expensive sampling. Our previous work
	has demonstrated that {Poisson-Boltzmann} methods are capable of
	faithfully reproducing polar explicit solvent forces for dilute protein
	systems; however, the popular solvent-accessible surface area model
	was shown to be incapable of accurately describing nonpolar solvation
	forces at atomic-length scales. Therefore, alternate continuum methods
	are needed to reproduce nonpolar interactions at the atomic scale.
	In the present work, we address this issue by supplementing the solvent-accessible
	surface area model with additional volume and dispersion integral
	terms suggested by scaled particle models and Weeks-Chandler-Andersen
	theory, respectively. This more complete nonpolar implicit solvent
	model shows very good agreement with explicit solvent results and
	suggests that, although often overlooked, the inclusion of appropriate
	dispersion and volume terms are essential for an accurate implicit
	solvent description of atomic-scale nonpolar forces.},
  annote = {Assessing implicit models for nonpolar mean solvation forces: the
	importance of dispersion and volume terms; WagonerNonpolar},
  bdsk-file-1 = {YnBsaXN0MDDUAQIDBAUGCQpYJHZlcnNpb25UJHRvcFkkYXJjaGl2ZXJYJG9iamVjdHMSAAGGoNE
	HCFRyb290gAFfEA9OU0tleWVkQXJjaGl2ZXKoCwwXGBkdJCVVJG51bGzTDQ4PEBEUViRjbGFzc1
	dOUy5rZXlzWk5TLm9iamVjdHOAB6ISE4ACgAOiFRaABIAGWWFsaWFzRGF0YVxyZWxhdGl2ZVBhd
	GjSDRobHFdOUy5kYXRhgAVPEQHCAAAAAAHCAAIAAAxNYWNpbnRvc2ggSEQAAAAAAAAAAAAAAAAA
	AADD4v5NSCsAAAAZYksVMjAwNi1XYWdvbmVyQmFrZXIucGRmAAAAAAAAAAAAAAAAAAAAAAAAAAA
	AAAAAAAAAAAAAAAAAAAAAAAAAAAAAABlib8KAogYAAAAAAAAAAAAEAAQAAAkgAAAAAAAAAAAAAA
	AAAAAAB0FyY2hpdmUAABAACAAAw+NSrQAAABEACAAAwoDoVgAAAAEAFAAZYksAGWIDAAqkKAAKp
	BEAAHrcAAIAS01hY2ludG9zaCBIRDpVc2VyczpiYWtlcjpEb2N1bWVudHM6UmVmZXJlbmNlczpB
	cmNoaXZlOjIwMDYtV2Fnb25lckJha2VyLnBkZgAADgAsABUAMgAwADAANgAtAFcAYQBnAG8AbgB
	lAHIAQgBhAGsAZQByAC4AcABkAGYADwAaAAwATQBhAGMAaQBuAHQAbwBzAGgAIABIAEQAEgA+VX
	NlcnMvYmFrZXIvRG9jdW1lbnRzL1JlZmVyZW5jZXMvQXJjaGl2ZS8yMDA2LVdhZ29uZXJCYWtlc
	i5wZGYAEwABLwAAFQACAAz//wAA0h4fICFYJGNsYXNzZXNaJGNsYXNzbmFtZaMhIiNdTlNNdXRh
	YmxlRGF0YVZOU0RhdGFYTlNPYmplY3RfED4uLi8uLi8uLi8uLi9Eb2N1bWVudHMvUmVmZXJlbmN
	lcy9BcmNoaXZlLzIwMDYtV2Fnb25lckJha2VyLnBkZtIeHyYnoicjXE5TRGljdGlvbmFyeQAIAB
	EAGgAfACkAMgA3ADoAPwBBAFMAXABiAGkAcAB4AIMAhQCIAIoAjACPAJEAkwCdAKoArwC3ALkCf
	wKEAo0CmAKcAqoCsQK6AvsDAAMDAAAAAAAAAgEAAAAAAAAAKAAAAAAAAAAAAAAAAAAAAxA=},
  bdsk-url-1 = {http://dx.doi.org/10.1073/pnas.0600118103},
  date-added = {2008-06-30 06:28:44 -0500},
  date-modified = {2008-06-30 06:28:44 -0500},
  keywords = {Solvation; nonpolar},
  ty = {JOUR},
  url = {http://dx.doi.org/10.1073/pnas.0600118103}
}

@ARTICLE{Wagoner:2004,
  author = {Wagoner, J. and Baker, N. A.},
  title = {Solvation forces on biomolecular structures: A comparison of explicit
	solvent and {Poisson-Boltzmann} models},
  journal = {Journal of Computational Chemistry},
  year = {2004},
  volume = {25},
  pages = {1623-9},
  number = {13},
  abstract = {Continuum electrostatics methods have become increasingly popular
	due to their ability to provide approximate descriptions of solvation
	energies and forces without expensive sampling required by explicit
	solvent models. In particular, the {Poisson-Boltzmann} equation (PBE)
	provides electrostatic potentials, solvation energies, and forces
	by modeling the solvent as a featureless, dielectric material, and
	the mobile ions as a continuous distribution of charge. Polar solvation
	forces and energies obtained from the PBE are often supplemented
	with simple solvent-accessible surface area (SASA) models of nonpolar
	solvation. Given the recent development of methods that enable the
	use of PBE and SASA forces in molecular dynamics simulations, it
	is important to determine the ability of these implicit solvent models
	to accurately reproduce the solvation forces of more detailed explicit
	solvent simulations. In this article, we compare PBE and SASA solvation
	forces with explicit solvent forces for several snapshots from eight
	trajectories of static conformations of intestinal fatty acid binding
	protein. The results from this comparison show that current implementations
	of the PBE are capable of generating polar solvation forces that
	correlate well with explicit solvent forces but systematically overestimate
	the magnitude of the interaction. However, SASA-based nonpolar forces
	are found to have no significant correlation with nonpolar explicit
	solvent forces. Nevertheless, due to the small magnitude of the nonpolar
	forces in the current system, a good correlation is still obtained
	for total solvation forces. The good correlation of implicit solvent
	forces with more detailed explicit solvent models is encouraging
	and implies that the systematic errors identified in these models
	could be corrected by appropriate parameterization of the force fields.},
  annote = {Solvation forces on biomolecular structures: A comparison of explicit
	solvent and {Poisson-Boltzmann} models; WagonerPolar; Compares PB/SA
	calculations to explicit solvent simulations and observes strong
	correlation between implicit and explicit solvent polar forces but
	poor agreement for apolar forces.},
  bdsk-file-1 = {YnBsaXN0MDDUAQIDBAUGCQpYJHZlcnNpb25UJHRvcFkkYXJjaGl2ZXJYJG9iamVjdHMSAAGGoNE
	HCFRyb290gAFfEA9OU0tleWVkQXJjaGl2ZXKoCwwXGBkdJCVVJG51bGzTDQ4PEBEUViRjbGFzc1
	dOUy5rZXlzWk5TLm9iamVjdHOAB6ISE4ACgAOiFRaABIAGWWFsaWFzRGF0YVxyZWxhdGl2ZVBhd
	GjSDRobHFdOUy5kYXRhgAVPEQHCAAAAAAHCAAIAAAxNYWNpbnRvc2ggSEQAAAAAAAAAAAAAAAAA
	AADD4v5NSCsAAAAZYksVMjAwNC1XYWdvbmVyQmFrZXIucGRmAAAAAAAAAAAAAAAAAAAAAAAAAAA
	AAAAAAAAAAAAAAAAAAAAAAAAAAAAAABliisNCATxQREYgcHJ2dwAEAAQAAAkgAAAAAAAAAAAAAA
	AAAAAAB0FyY2hpdmUAABAACAAAw+NSrQAAABEACAAAw0JHjAAAAAEAFAAZYksAGWIDAAqkKAAKp
	BEAAHrcAAIAS01hY2ludG9zaCBIRDpVc2VyczpiYWtlcjpEb2N1bWVudHM6UmVmZXJlbmNlczpB
	cmNoaXZlOjIwMDQtV2Fnb25lckJha2VyLnBkZgAADgAsABUAMgAwADAANAAtAFcAYQBnAG8AbgB
	lAHIAQgBhAGsAZQByAC4AcABkAGYADwAaAAwATQBhAGMAaQBuAHQAbwBzAGgAIABIAEQAEgA+VX
	NlcnMvYmFrZXIvRG9jdW1lbnRzL1JlZmVyZW5jZXMvQXJjaGl2ZS8yMDA0LVdhZ29uZXJCYWtlc
	i5wZGYAEwABLwAAFQACAAz//wAA0h4fICFYJGNsYXNzZXNaJGNsYXNzbmFtZaMhIiNdTlNNdXRh
	YmxlRGF0YVZOU0RhdGFYTlNPYmplY3RfED4uLi8uLi8uLi8uLi9Eb2N1bWVudHMvUmVmZXJlbmN
	lcy9BcmNoaXZlLzIwMDQtV2Fnb25lckJha2VyLnBkZtIeHyYnoicjXE5TRGljdGlvbmFyeQAIAB
	EAGgAfACkAMgA3ADoAPwBBAFMAXABiAGkAcAB4AIMAhQCIAIoAjACPAJEAkwCdAKoArwC3ALkCf
	wKEAo0CmAKcAqoCsQK6AvsDAAMDAAAAAAAAAgEAAAAAAAAAKAAAAAAAAAAAAAAAAAAAAxA=},
  bdsk-url-1 = {http://dx.doi.org/10.1002/jcc.20089},
  date-added = {2008-06-30 11:32:28 -0500},
  date-modified = {2008-06-30 11:32:28 -0500},
  keywords = {Electrostatics; Solvation; molecular\_dynamics},
  ty = {JOUR},
  url = {http://dx.doi.org/10.1002/jcc.20089}
}

@ARTICLE{Waldmann:1957,
  author = {Waldmann, L.},
  title = {{Die Boltzmann-Gleichung fur Gase mit rotierenden Molekulen}},
  journal = {Z. Naturforsch. Teil A},
  year = {1957},
  volume = {12},
  pages = {660-662},
  annote = { },
  date-added = {2008-11-25 10:28:56 -0500},
  date-modified = {2008-11-25 10:28:56 -0500},
  ty = {JOUR}
}

@ARTICLE{Wallis:1995,
  author = {Wallis, Russel and Moore, Geoffrey R. and James, Richard and Kleanthous,
	Colin},
  title = {{Protein-Protein Interactions in Colicin E9 DNase-Immunity Protein
	Complexes. 1. Diffusion-Controlled Association and Femtomolar Binding
	for the Cognate Complex}},
  journal = {Biochemistry},
  year = {1995},
  volume = {34},
  pages = {13743-13750},
  number = { }
}

@ARTICLE{Wallquist:1995,
  author = {Wallquist, A. and Berne, B. J.},
  title = {Computer-simulation of hydrophobic hydration forces stacked plates
	at short-range},
  journal = {Journal of Physical Chemistry},
  year = {1995},
  volume = {99},
  pages = {2893-2899}
}

@ARTICLE{DCWan:2002,
  author = {Wan, D. C. and Patnaik, B. S. V. and Wei, G. W.},
  title = {Discrete singularconvolution-finite subdomain method forthe solution
	of incompressible viscous flows},
  journal = {J. Comput. Phys.},
  year = {2002},
  volume = {180},
  pages = {229 - 255}
}

@ARTICLE{WPWjcp02,
  author = {Wan, D. C. and Patnaik, B. S. V. and Wei, G. W. },
  title = {Discrete singular convolution-finite subdomain method for the solution
	of incompressible viscous flows},
  journal = {J. Comput. Phys.},
  year = {2002},
  volume = {180},
  pages = {229-255}
}

@ARTICLE{wan:2007(a),
  author = {Wan, D. C. and Turek, S.},
  title = {{An efficient multigrid-FEM method for the simulation of solid-liquid
	two phase flows}},
  journal = {J. Computational and Applied Mathematics},
  year = {2007},
  volume = {203},
  pages = {561--580}
}

@ARTICLE{wan:2007(b),
  author = {Wan, D. C. and Turek, S.},
  title = {{Fictitious boundary and moving mesh methods for the numerical simulation
	of rigid particulate flows}},
  journal = {J. Comput. Phys.},
  year = {2007},
  volume = {222},
  pages = {28--56}
}

@ARTICLE{CWWang:2007,
  author = { Wang, C. W. and Sastrya, A. M. },
  title = { Mesoscale Modeling of a Li-Ion Polymer Cell
	
	},
  journal = { Journal of The Electrochemical Society },
  year = {2007},
  volume = {154},
  pages = {A1035-A1047}
}

@ARTICLE{DWang:2010,
  author = { Wang, D. A. and Li, R. and Yan, N. N.},
  title = {An Edge-Based Anisotropic Mesh Refinement Algorithm and its Application
	to Interface Problems
	
	},
  journal = { Commun. Comput. Phys. },
  year = {2010},
  volume = {8},
  pages = {511-540}
}

@ARTICLE{Wang:2006,
  author = {Wang, G. and Shen, H. and Cong, W. and Zhao, S. and Wei, G. W.},
  title = {Temperature modulated bioluminescence tomography},
  journal = {Optics Express},
  year = {2006},
  volume = {14},
  pages = {7852-7871},
  annote = {Temperature modulated bioluminescence tomography},
  date-added = {2008-09-19 10:28:56 -0500},
  date-modified = {2008-09-19 10:28:56 -0500},
  ty = {JOUR}
}

@ARTICLE{Wang2005,
  author = {Wang, HW and Nogales, E},
  title = {Nucleotide-dependent bending flexibility of tubulin regulates microtubule
	assembly.},
  journal = {Nature},
  year = {2005},
  volume = {435},
  pages = {911-5--},
  number = {7044},
  month = jun,
  abstract = {The atomic structure of tubulin in a polymerized, straight protofilament
	is clearly distinct from that in a curved conformation bound to a
	cellular depolymerizer. The nucleotide contents are identical, and
	in both cases the conformation of the GTP-containing, intra-dimer
	interface is indistinguishable from the GDP-containing, inter-dimer
	contact. Here we present two structures corresponding to the start
	and end points in the microtubule polymerization and hydrolysis cycles
	that illustrate the consequences of nucleotide state on longitudinal
	and lateral assembly. In the absence of depolymerizers, GDP-bound
	tubulin shows distinctive intra-dimer and inter-dimer interactions
	and thus distinguishes the GTP and GDP interfaces. A cold-stable
	tubulin polymer with the non-hydrolysable GTP analogue GMPCPP, containing
	semi-conserved lateral interactions, supports a model in which the
	straightening of longitudinal interfaces happens sequentially, starting
	with a conformational change after GTP binding that straightens the
	dimer enough for the formation of lateral contacts into a non-tubular
	intermediate. Closure into a microtubule does not require GTP hydrolysis.},
  address = {Howard Hughes Medical Institute, University of California Berkeley,
	Berkeley, California 94720-3200, USA.},
  comment = {Research Support, Non-U.S. Gov't,Research Support, U.S. Gov't, Non-P.H.S.,Research
	Support, N.I.H., Extramural,Research Support, U.S. Gov't, P.H.S.,},
  keywords = {Cryoelectron Microscopy, Dimerization, Guanosine Diphosphate, Guanosine
	Triphosphate, Hydrolysis, Microtubules, Models, Molecular, Pliability,
	Protein Conformation, Tubulin},
  owner = {SeanLab},
  timestamp = {2012.05.23},
  url = {http://ukpmc.ac.uk/abstract/MED/15959508}
}

@ARTICLE{JWang:2009,
  author = {Wang, J. and Lin, M. and Crenshaw, A. and Hutchinson, A. and Hicks,
	B. and Yeager, M. and Berndt, S. and Huang, W. Y. and Hayes, R. B.
	and Chanock, S. J. and Jones, R. C. and Ramakrishnan, R.},
  title = {High-throughput single nucleotide polymorphism genotyping using nanofluidic
	Dynamic Arrays},
  journal = {BMC Genomics},
  year = {2009},
  volume = {10},
  number = {561}
}

@ARTICLE{JWang:2004,
  author = {Wang, J. and Polizzi, E. and Lundstrom, M.},
  title = {A three-dimensional quantum simulation of silicon nanowire transistors
	with the effective-mass approximation},
  journal = {J. Appl. Phys.},
  year = {2004},
  volume = {96},
  pages = { 2192--203},
  annote = {A three-dimensional quantum simulation of silicon nanowire transistors
	with the effective-mass approximation},
  date-added = {2008-11-25 10:28:56 -0500},
  date-modified = {2008-11-25 10:28:56 -0500},
  ty = {JOUR}
}

@ARTICLE{JWang:2010,
  author = {Wang, J. and Wang, L.},
  title = {{Sparse supervised dimension reduction in high dimensional classification}},
  journal = {Electronic Journal of Statistics},
  year = {2010},
  volume = {4},
  pages = {914 - 931}
}

@ARTICLE{Wang:2004b,
  author = {Wang, J. and Wolf, R. M. and Caldwell, J. W. and Kollman, P. A. and
	Case, D. A.},
  title = {Development and testing of a general {AMBER} force field},
  journal = {Journal of Computational Chemistry},
  year = {2004},
  volume = {25},
  pages = {1157-74},
  number = {9},
  abstract = {We describe here a general Amber force field (GAFF) for organic molecules.
	GAFF is designed to be compatible with existing Amber force fields
	for proteins and nucleic acids, and has parameters for most organic
	and pharmaceutical molecules that are composed of H, C, N, O, S,
	P, and halogens. It uses a simple functional form and a limited number
	of atom types, but incorporates both empirical and heuristic models
	to estimate force constants and partial atomic charges. The performance
	of GAFF in test cases is encouraging. In test I, 74 crystallographic
	structures were compared to GAFF minimized structures, with a root-mean-square
	displacement of 0.26 Ã- which is comparable to that of the Tripos
	5.2 force field (0.25 Ã- and better than those of MMFF 94 and
	CHARMm (0.47 and 0.44 Ã- respectively). In test II, gas phase
	minimizations were performed on 22 nucleic acid base pairs, and the
	minimized structures and intermolecular energies were compared to
	MP2/6-31G* results. The RMS of displacements and relative energies
	were 0.25 Ã-and 1.2 kcal/mol, respectively. These data are comparable
	to results from Parm99/RESP (0.16 Ã-and 1.18 kcal/mol, respectively),
	which were parameterized to these base pairs. Test III looked at
	the relative energies of 71 conformational pairs that were used in
	development of the Parm99 force field. The RMS error in relative
	energies (compared to experiment) is about 0.5 kcal/mol. GAFF can
	be applied to wide range of molecules in an automatic fashion, making
	it suitable for rational drug design and database searching.},
  bdsk-url-1 = {http://dx.doi.org/10.1002/jcc.20035},
  date-added = {2008-06-30 11:40:43 -0500},
  date-modified = {2008-06-30 11:40:43 -0500},
  keywords = {molecular\_dynamics; molecular\_simulation},
  url = {http://dx.doi.org/10.1002/jcc.20035}
}

@ARTICLE{JPWang:2011,
  author = { Wang, J. P. and Ye, X.},
  title = {A weak {Galerkin} finite element method for second-order elliptic
	problems},
  journal = { arXiv:1104.2897v1},
  year = {2011}
}

@ARTICLE{WWTDS06,
  author = {Ke Wang and Weiwei and Yiying Tong and Mathieu Desbrun and Peter
	Schr{\"o}der},
  title = {Edge Subdivision Schemes and the Construction of Smooth Vector Fields},
  journal = {ACM Trans. on Graphics (SIGGRAPH)},
  year = {2006},
  volume = {25},
  pages = {1041--1048},
  number = {3},
  month = jul
}

@ARTICLE{LWang:2010a,
  author = {Wang, L. and Li, H. and Huang, J.},
  title = {{Variable selection for the Cox model with time-varying regression
	coefficients}},
  year = {2010}
}

@ARTICLE{LWang:2010b,
  author = {Wang, L. and Luan, Y., and Li, H.},
  title = {{Boosting For high-dimensional linear models with group variables}},
  year = {2010}
}

@ARTICLE{MingliangWang:2007,
  author = {Wang, M.L. and Wong, C. F. and Liu, J. H. and Zhang, P. X.},
  title = {Efficient quantum mechanical calculation of solvation free energies
	based on density functional theory, numerical atomic orbitals and
	{Poisson-Boltzmann} equation},
  journal = {Chemical Physics Letters},
  year = {2007},
  volume = {442},
  pages = {464--467}
}

@ARTICLE{Wang063228,
  author = {Wang, M. L. and Hu, X. Q. and Beratan, D. N. and Yang, W. T.},
  title = {Designing molecules by optimizing potentials},
  journal = {Journal of the American Chemical Society},
  year = {2006},
  volume = {128},
  pages = {3228-3232},
  number = {10},
  month = {Mar},
  abstract = {The astronomical number of accessible discrete chemical structures
	makes rational molecular design extremely challenging. We formulate
	the design of molecules with specific tailored properties as performing
	a continuous optimization in the space of electron-nuclear attraction
	potentials. The optimization is facilitated by using a linear combination
	of atomic potentials (LCAP), a general framework that creates a continuous
	property landscape from an otherwise unlinked set of discrete molecular-property
	values. A demonstration of this approach is given for the optimization
	of molecular electronic polarizability and hyperpolarizability. We
	show that the optimal structures can be determined without enumerating
	and separately evaluating the characteristics of the combinatorial
	number of possible structures, a process that would be much slower.
	The LCAP approach may be used with quantum or classical Hamiltonians,
	suggesting possible applications to drug design and new materials
	discovery.},
  endnotereftype = {Journal Article},
  issn = {0002-7863},
  shorttitle = {Designing molecules by optimizing potentials},
  url = {<Go to ISI>://000236035100037}
}

@ARTICLE{Wang06124516,
  author = {Wang, M. L. and Lu, Z. Y. and Yang, W. T.},
  title = {Nuclear quantum effects on an enzyme-catalyzed reaction with reaction
	path potential: Proton transfer in triosephosphate isomerase},
  journal = {Journal of Chemical Physics},
  year = {2006},
  volume = {124},
  pages = {124516},
  number = {12},
  month = {Mar},
  abstract = {Nuclear quantum mechanical effects have been examined for the proton
	transfer reaction catalyzed by triosephosphate isomerase, with the
	normal mode centroid path integral molecular dynamics based on the
	potential energy surface from the recently developed reaction path
	potential method. In the simulation, the primary and secondary hydrogens
	and the C and O atoms involving bond forming and bond breaking were
	treated quantum mechanically, while all other atoms were dealt classical
	mechanically. The quantum mechanical activation free energy and the
	primary kinetic isotope effects were examined. Because of the quantum
	mechanical effects in the proton transfer, the activation free energy
	was reduced by 2.3 kcal/mol in comparison with the classical one,
	which accelerates the rate of proton transfer by a factor of 47.5.
	The primary kinetic isotope effects of k(H)/k(D) and k(H)/k(T) were
	estimated to be 4.65 and 9.97, respectively, which are in agreement
	with the experimental value of 4 +/- 0.3 and 9. The corresponding
	Swain-Schadd exponent was predicted to be 3.01, less than the semiclassical
	limit value of 3.34, indicating that the quantum mechanical effects
	mainly arise from quantum vibrational motion rather than tunneling.
	The reaction path potential, in conjunction with the normal mode
	centroid molecular dynamics, is shown to be an efficient computational
	tool for investigating the quantum effects on enzymatic reactions
	involving proton transfer. (c) 2006 American Institute of Physics.},
  endnotereftype = {Journal Article},
  issn = {0021-9606},
  shorttitle = {Nuclear quantum effects on an enzyme-catalyzed reaction with reaction
	path potential: Proton transfer in triosephosphate isomerase},
  url = {<Go to ISI>://000236464000053}
}

@ARTICLE{Wang04101,
  author = {Wang, M. L. and Lu, Z. Y. and Yang, W. T.},
  title = {Transmission coefficient calculation for proton transfer in triosephosphate
	isomerase based on the reaction path potential method},
  journal = {Journal of Chemical Physics},
  year = {2004},
  volume = {121},
  pages = {101-107},
  number = {1},
  month = {Jul},
  abstract = {A global potential energy surface has been constructed through interpolation
	of our recently developed reaction path potential for chemical reactions
	in enzymes which is derived from combined ab initio quantum mechanical
	and molecular mechanical calculations. It has been implemented for
	the activated molecular dynamics simulations of the initial proton
	transfer reaction catalyzed by triosephosphate isomerase. To examine
	the dynamical effects on the rate constants of the enzymatic reaction,
	the classical transmission coefficient kappa(t) is evaluated to be
	0.47 with the reactive flux approach, demonstrating considerable
	deviations from transition state theory. In addition, the fluctuations
	of protein environments have small effects on the barrier recrossing,
	and the transmission coefficient kappa(t) strongly depends on the
	fluctuations of atoms near the active site of the enzyme. (C) 2004
	American Institute of Physics.},
  endnotereftype = {Journal Article},
  issn = {0021-9606},
  shorttitle = {Transmission coefficient calculation for proton transfer in triosephosphate
	isomerase based on the reaction path potential method},
  url = {<Go to ISI>://000222112100011}
}

@ARTICLE{MLWang:2006,
  author = {Wang, M. L. and Wong, C. F.},
  title = {Calculation of Solvation Free Energy from Quantum Mechanical Charge
	Density and Continuum Dielectric Theory},
  journal = {J. Phys. Chem. A},
  year = {2006},
  volume = {110},
  pages = {4873-4879}
}


@ARTICLE{MLWang:2007,
  author = {Wang, M. L. and Wong, C. F. and Liu, J. H. and Zhang, P. X.},
  title = {Efficient quantum mechanical calculation of solvation free energies
	based on density functional theory, numerical atomic orbitals and
	Poisson-Boltzmann equation},
  journal = {Chemical Physics Letters},
  year = {2007},
  volume = {442},
  pages = {464- 467}
}

@ARTICLE{Wang0710252,
  author = {Wang, W. and Qiao, J. and Wang, L. D. and Duan, L. A. and Zhang,
	D. Q. and Yang, W. T. and Qiu, Y.},
  title = {Synthesis, structures, and optical properties of cadmium iodide/phenethylamine
	hybrid materials with controlled structures and emissions},
  journal = {Inorganic Chemistry},
  year = {2007},
  volume = {46},
  pages = {10252-10260},
  number = {24},
  month = {Nov},
  abstract = {new type of organic-inorganic hybrid materials based on cadmium iodide
	(Cdl(2)) and phenethylamine (PEA) has been synthesized and characterized.
	The reaction of Cdl(2) with PEA in a 1:2 molar ratio yields a four-coordinate
	hybrid material Cdl(2)(PEA)(2) (1) with extended 1D (Cdl(2))(n) chains,
	while the reaction of Cdl(2) with PEA in a 1:4 molar ratio produces
	a six-coordinate hybrid material Cdl(2)(PEA)(4) (2) with a discrete
	linear structure of Cdl(2) moiety. By introducing a trace amount
	of Na2S to the reaction for Cdl(2)(PEA)(2), we obtained a new compound
	[Cdl(2)(PEA)(2)]-(CdS)(0.038) (3) with uniformly doped US nanoparticles.
	Steady and transient photoluminescence studies reveal that compounds
	1 and 2 exhibit bright blue (465 nm) and green (512 nm) fluorescent
	emissions in solid state at room temperature, respectively, while
	compound 3 gives a broad and complex emission ranging from 450 to
	700 nm. Theoretical studies of electronic structures were carried
	out using density functional theory in order to gain a good understanding
	of the luminescent behaviors of these hybrid materials.},
  endnotereftype = {Journal Article},
  issn = {0020-1669},
  shorttitle = {Synthesis, structures, and optical properties of cadmium iodide/phenethylamine
	hybrid materials with controlled structures and emissions},
  url = {<Go to ISI>://000251109500028}
}

@ARTICLE{WWang:2009,
  author = {Wang, W. and Shu, C. W.},
  title = {The WKB Local Discontinuous Galerkin Method for the Simulation of
	Schrodinger Equation in a Resonant Tunneling Diode},
  journal = {Journal of Scientific Computing},
  year = {2009},
  volume = {40},
  pages = {360 - 374}
}

@ARTICLE{XWang:2009,
  author = { Wang, X. Sheldon and Zhang, L. T. and Liu Wing Kam},
  title = {On computational issues of immersed finite element methods},
  journal = {Journal of Computational Physics},
  year = {2009},
  volume = {228},
  pages = {2535-2551}
}

@ARTICLE{Wang:2002y,
  author = {Wang, Y. },
  title = {Spectral Sets, tiling and wavelets},
  journal = {Duke Math.},
  year = {2002},
  volume = {114},
  pages = {43 - 57}
}

@ARTICLE{Wang:1995y,
  author = {Wang, Y.},
  title = {Existence and regularity of solutions to a variational problem of
	Mumford and Shah: a constructive approach},
  journal = {SIAM J. Optimization},
  year = {1995},
  volume = {5},
  pages = {892 - 913}
}

@ARTICLE{YWang:2009,
  author = {Wang, Y. and Pant, K. and Chen, Z. J. and Wang, G. R. and Diffey,
	W. F. and Ashley, P. and Sundaram, S.},
  title = {Numerical analysis of electrokinetic transport in micro-nanofluidic
	interconnect preconcentrator in hydrodynamic flow },
  journal = { Microfluid. and Nanofluid.},
  year = {2009},
  volume = {7},
  pages = {683-696}
}

@ARTICLE{YWang:2010c,
  author = {Wang, Y. and Wu, Q.},
  title = {{Sparse PCA by Iterative Elimination Algorithm}},
  journal = {Preprint},
  year = {2010}
}

@ARTICLE{YWang:2012a,
  author = {Wang, Y. and Wei, G. W. and Yang, Si-Yang},
  title = {{Iterative filtering decomposition based on local spectral evolution
	kernel}},
  journal = {Journal of Scientific Computing},
  year = {2012},
  volume = {50},
  pages = {629-664}
}

@ARTICLE{YWang:2012b,
  author = {Wang, Y. and Wei, G. W. and Yang, Si-Yang},
  title = {{Mode decomposition evolution equations}},
  journal = {Journal of Scientific Computing},
  year = {2012},
  volume = {50},
  pages = {495-518}
}


@ARTICLE{YWang:2011c,
  author = {Wang, Y. and Wei, G. W. and Yang, Si-Yang},
  title = {Partial differential equation transform -- {Variational formulation
	and Fourier analysis}},
  journal = {International Journal for Numerical Methods in Biomedical Engineering
	},
  year = { 2011},
  volume = {27},
  pages = {1996-2020}
}

@ARTICLE{YWang:2012d,
  author = {Wang, Y. and Wei, G. W. and Yang, Si-Yang},
  title = {Selective extraction of entangled textures via adaptive PDE transform},
  journal = {International Journal in Biomedical Imaging },
  year = {2012},
  volume = {2012},
  pages = {Article ID 958142}
}


@ARTICLE{Wang:1998y,
  author = {Wang, Y. and Zhou, G.},
  title = {On the use of high order ambiguity functions for multicomponent polynomial
	phase signals},
  journal = {Signal Processing},
  year = {1998},
  volume = {65},
  pages = {283-296}
}

@ARTICLE{YWang:2010d,
  author = {Wang, Y. and Zhou, H.},
  title = {MULTISCALE TOTAL VARIATIONAL ALGGORITHMS FOR DENOISING NATURAL COLOR
	PHOTOS IN DIGITAL PHOTOGRAPHY},
  journal = {Preprint}
}

@ARTICLE{YWang:2010e,
  author = {Wang, Y. and Zhou, H.},
  title = {MULTISCALE TOTAL VARIATIONAL ALGGORITHMS FOR DENOISING NATURAL COLOR
	PHOTOS IN DIGITAL PHOTOGRAPHY}
}

@ARTICLE{Wang:2006y,
  author = {Wang, Y. and Zhou, H.},
  title = {Total VariationWavelet Based Medical Image Denoising},
  journal = {Int. J. Biomedical Imaging},
  year = {2006},
  volume = {2006},
  pages = {1-6}
}

@ARTICLE{WanZho06,
  author = {Wang, Y. and Zhou, H. M.},
  title = {A Total Variation Wavelet Algorithm for Medical Image Denoising},
  journal = {International Journal on Biomedical Imaging},
  year = {2006},
  volume = {2006},
  number = {89095 }
}

@ARTICLE{YangWang:2006,
  author = {Wang, Yang and Zhou, H. M.},
  title = {A Total Variation Wavelet Algorithm for Medical Image Denoising},
  journal = {International Journal of Biomedical Imaging},
  year = {2006},
  volume = {2006},
  pages = {89095}
}

@ARTICLE{YCWang:2005,
  author = {Wang, Y. C. and Stevens, A. L. and Han, J. Y. },
  title = {Million-fold preconcentration of proteins and peptides by nanofluidic
	filter },
  journal = {Analyitcal Chemistry },
  year = {2005},
  volume = {77},
  pages = {4293-4299 },
  number = { }
}

@ARTICLE{WSHD05,
  author = {Joe Warren and Scott Schaefer and Anil Hirani and Mathieu Desbrun},
  title = {Barycentric Coordinates for Convex Sets},
  journal = {Advances in Computational Mathematics},
  year = {2007},
  volume = {DOI 10.1007/s10444-005-9008-6},
  number = {to appear}
}

@ARTICLE{Warshel:1991,
  author = {Warshel, A. and {\AA}qvist, L.},
  title = {Electrostatic energy and macromolecular function},
  journal = {Annu. Rev. Biophys. Biophys. Chem.},
  year = {1991},
  volume = {20},
  pages = {267-98}
}

@ARTICLE{Warshel:1998,
  author = {Warshel, A. and Papazyan, A.},
  title = {Electrostatic effects in macromolecules: fundamental concepts and
	practical modeling},
  journal = {Current Opinion in Structural Biology},
  year = {1998},
  volume = {8},
  pages = {211-7},
  number = {2},
  abstract = {The past few years have seen an exponential growth in the calculations
	of electrostatic energies of macromolecules and an increased recognition
	of the crucial role of electrostatic effects. This review considers
	the current state of the field. Focus is placed on calculations of
	pKas, redox potentials and binding energies in macromolecules and
	clarification of the fact that the value of the dielectric Ã¢Â€Â˜constantÃ¢Â€Â™of
	a protein depends on its definition and that small dielectric constants
	should not be used in describing chargeÃ¢Â€Â-charge interactions
	by current continuum models.},
  annote = {Electrostatic effects in macromolecules: fundamental concepts and
	practical modeling},
  bdsk-url-1 = {http://dx.doi.org/10.1016/S0959-440X(98)80041-9},
  date-added = {2008-09-01 13:56:59 -0500},
  date-modified = {2008-09-01 13:56:59 -0500},
  keywords = {Electrostatics},
  ty = {JOUR},
  url = {http://dx.doi.org/10.1016/S0959-440X(98)80041-9}
}

@ARTICLE{Warshel:2006,
  author = {Warshel, A. and Sharma, P. K. and Kato, M. and Parson, W. W.},
  title = {Modeling electrostatic effects in proteins},
  journal = {Biochimica et Biophysica Acta (BBA) - Proteins \& Proteomics},
  year = {2006},
  volume = {1764},
  pages = {1647-76},
  number = {11},
  abstract = {Electrostatic energies provide what is perhaps the most effective
	tool for structureÃ¢Â€Â“function correlation of biological
	molecules. This review considers the current state of simulations
	of electrostatic energies in macromolecules as well as the early
	developments of this field. We focus on the relationship between
	microscopic and macroscopic models, considering the convergence problems
	of the microscopic models and the fact that the dielectric Ã¢Â€Â˜constantsÃ¢Â€Â™in
	semimacroscopic models depend on the definition and the specific
	treatment. The advances and the challenges in the field are illustrated
	considering a wide range of functional properties including pKa's,
	redox potentials, ion and proton channels, enzyme catalysis, ligand
	binding and protein stability. We conclude by pointing out that,
	despite the current problems and the significant misunderstandings
	in the field, there is an overall progress that should lead eventually
	to quantitative descriptions of electrostatic effects in proteins
	and thus to quantitative descriptions of the function of proteins.},
  annote = {Modeling electrostatic effects in proteins},
  bdsk-file-1 = {YnBsaXN0MDDUAQIDBAUGCQpYJHZlcnNpb25UJHRvcFkkYXJjaGl2ZXJYJG9iamVjdHMSAAGGoNE
	HCFRyb290gAFfEA9OU0tleWVkQXJjaGl2ZXKoCwwXGBkdJCVVJG51bGzTDQ4PEBEUViRjbGFzc1
	dOUy5rZXlzWk5TLm9iamVjdHOAB6ISE4ACgAOiFRaABIAGWWFsaWFzRGF0YVxyZWxhdGl2ZVBhd
	GjSDRobHFdOUy5kYXRhgAVPEQHuAAAAAAHuAAIAAAxNYWNpbnRvc2ggSEQAAAAAAAAAAAAAAAAA
	AADD4v5NSCsAAAAZYksfMjAwNi1XYXJzaGVsU2hhcm1hS2EjMTk2MkFCLnBkZgAAAAAAAAAAAAA
	AAAAAAAAAAAAAAAAAAAAAAAAAAAAAABliq8N1anUAAAAAAAAAAAAEAAQAAAkgAAAAAAAAAAAAAA
	AAAAAAB0FyY2hpdmUAABAACAAAw+NSrQAAABEACAAAw3W+1QAAAAEAFAAZYksAGWIDAAqkKAAKp
	BEAAHrcAAIAVU1hY2ludG9zaCBIRDpVc2VyczpiYWtlcjpEb2N1bWVudHM6UmVmZXJlbmNlczpB
	cmNoaXZlOjIwMDYtV2Fyc2hlbFNoYXJtYUthIzE5NjJBQi5wZGYAAA4AQgAgADIAMAAwADYALQB
	XAGEAcgBzAGgAZQBsAFMAaABhAHIAbQBhAEsAYQB0AG8AUABhAHIAcwBvAG4ALgBwAGQAZgAPAB
	oADABNAGEAYwBpAG4AdABvAHMAaAAgAEgARAASAElVc2Vycy9iYWtlci9Eb2N1bWVudHMvUmVmZ
	XJlbmNlcy9BcmNoaXZlLzIwMDYtV2Fyc2hlbFNoYXJtYUthdG9QYXJzb24ucGRmAAATAAEvAAAV
	AAIADP//AADSHh8gIVgkY2xhc3Nlc1okY2xhc3NuYW1loyEiI11OU011dGFibGVEYXRhVk5TRGF
	0YVhOU09iamVjdF8QSS4uLy4uLy4uLy4uL0RvY3VtZW50cy9SZWZlcmVuY2VzL0FyY2hpdmUvMj
	AwNi1XYXJzaGVsU2hhcm1hS2F0b1BhcnNvbi5wZGbSHh8mJ6InI1xOU0RpY3Rpb25hcnkACAARA
	BoAHwApADIANwA6AD8AQQBTAFwAYgBpAHAAeACDAIUAiACKAIwAjwCRAJMAnQCqAK8AtwC5AqsC
	sAK5AsQCyALWAt0C5gMyAzcDOgAAAAAAAAIBAAAAAAAAACgAAAAAAAAAAAAAAAAAAANH},
  bdsk-url-1 = {http://dx.doi.org/10.1016/j.bbapap.2006.08.007},
  date-added = {2008-09-01 13:56:38 -0500},
  date-modified = {2008-09-01 13:56:38 -0500},
  keywords = {Electrostatics; Solvation},
  ty = {JOUR},
  url = {http://dx.doi.org/10.1016/j.bbapap.2006.08.007}
}

@ARTICLE{Warsi:1990,
  author = {Warsi, Z. U. A. and Dvinsky, J. F.},
  title = {{Application of variational methods in the fixed and adaptive grid
	generation}},
  journal = {J. Comput. Phys.},
  year = {1990},
  volume = {19},
  pages = {31--41}
}

@ARTICLE{Warwicker:2004,
  author = {Warwicker, J.},
  title = {Improved {pKa} calculations through flexibility based sampling of
	a water-dominated interaction scheme},
  journal = {Protein Science},
  year = {2004},
  volume = {13},
  pages = {2793-805},
  number = {10},
  abstract = {Ionizable groups play critical roles in biological processes. Computation
	of pKas is complicated by model approximations and multiple conformations.
	Calculated and experimental pKas are compared for relatively inflexible
	active-site side chains, to develop an empirical model for hydration
	entropy changes upon charge burial. The modification is found to
	be generally small, but large for cysteine, consistent with small
	molecule ionization data and with partial charge distributions in
	ionized and neutral forms. The hydration model predicts significant
	entropic contributions for ionizable residue burial, demonstrated
	for components in the pyruvate dehydrogenase complex. Conformational
	relaxation in a pH-titration is estimated with a mean-field assessment
	of maximal side chain solvent accessibility. All ionizable residues
	interact within a low protein dielectric finite difference (FD) scheme,
	and more flexible groups also access water-mediated Debye-HÃƒÂ¼ckel
	(DH) interactions. The DH method tends to match overall pH-dependent
	stability, while FD can be more accurate for active-site groups.
	Tolerance for side chain rotamer packing is varied, defining access
	to DH interactions, and the best fit with experimental pKas obtained.
	The new (FD/DH) method provides a fast computational framework for
	making the distinction between buried and solvent-accessible groups
	that has been qualitatively apparent from previous work, and pKa
	calculations are significantly improved for a mixed set of ionizable
	residues. Its effectiveness is also demonstrated with computation
	of the pH-dependence of electrostatic energy, recovering favorable
	contributions to folded state stability and, in relation to structural
	genomics, with substantial improvement (reduction of false positives)
	in active-site identification by electrostatic strain.},
  annote = {Improved pKa calculations through flexibility based sampling of a
	water-dominated interaction scheme},
  bdsk-url-1 = {http://dx.doi.org/10.1110/ps.04785604},
  date-added = {2008-06-29 15:08:53 -0500},
  date-modified = {2008-06-29 15:08:53 -0500},
  keywords = {Electrostatics; Solvation},
  ty = {JOUR},
  url = {http://dx.doi.org/10.1110/ps.04785604}
}

@ARTICLE{Warwicker:1982,
  author = {Warwicker, J. and Watson, H. C.},
  title = {Calculation of the electric potential in the active site cleft due
	to alpha-helix dipoles},
  journal = {Journal of Molecular Biology},
  year = {1982},
  volume = {157},
  pages = {671-9},
  number = {4},
  annote = {Jun 5; Calculation of the electric potential in the active site cleft
	due to alpha-helix dipoles},
  bdsk-file-1 = {YnBsaXN0MDDUAQIDBAUGCQpYJHZlcnNpb25UJHRvcFkkYXJjaGl2ZXJYJG9iamVjdHMSAAGGoNE
	HCFRyb290gAFfEA9OU0tleWVkQXJjaGl2ZXKoCwwXGBkdJCVVJG51bGzTDQ4PEBEUViRjbGFzc1
	dOUy5rZXlzWk5TLm9iamVjdHOAB6ISE4ACgAOiFRaABIAGWWFsaWFzRGF0YVxyZWxhdGl2ZVBhd
	GjSDRobHFdOUy5kYXRhgAVPEQHOAAAAAAHOAAIAAAxNYWNpbnRvc2ggSEQAAAAAAAAAAAAAAAAA
	AADD4v5NSCsAAAAZYksYMTk4Mi1XYXJ3aWNrZXJXYXRzb24ucGRmAAAAAAAAAAAAAAAAAAAAAAA
	AAAAAAAAAAAAAAAAAAAAAAAAAAAAAADEe98QrVyFQREYgcHJ2dwAEAAQAAAkgAAAAAAAAAAAAAA
	AAAAAAB0FyY2hpdmUAABAACAAAw+NSrQAAABEACAAAxCudcQAAAAEAFAAZYksAGWIDAAqkKAAKp
	BEAAHrcAAIATk1hY2ludG9zaCBIRDpVc2VyczpiYWtlcjpEb2N1bWVudHM6UmVmZXJlbmNlczpB
	cmNoaXZlOjE5ODItV2Fyd2lja2VyV2F0c29uLnBkZgAOADIAGAAxADkAOAAyAC0AVwBhAHIAdwB
	pAGMAawBlAHIAVwBhAHQAcwBvAG4ALgBwAGQAZgAPABoADABNAGEAYwBpAG4AdABvAHMAaAAgAE
	gARAASAEFVc2Vycy9iYWtlci9Eb2N1bWVudHMvUmVmZXJlbmNlcy9BcmNoaXZlLzE5ODItV2Fyd
	2lja2VyV2F0c29uLnBkZgAAEwABLwAAFQACAAz//wAA0h4fICFYJGNsYXNzZXNaJGNsYXNzbmFt
	ZaMhIiNdTlNNdXRhYmxlRGF0YVZOU0RhdGFYTlNPYmplY3RfEEEuLi8uLi8uLi8uLi9Eb2N1bWV
	udHMvUmVmZXJlbmNlcy9BcmNoaXZlLzE5ODItV2Fyd2lja2VyV2F0c29uLnBkZtIeHyYnoicjXE
	5TRGljdGlvbmFyeQAIABEAGgAfACkAMgA3ADoAPwBBAFMAXABiAGkAcAB4AIMAhQCIAIoAjACPA
	JEAkwCdAKoArwC3ALkCiwKQApkCpAKoArYCvQLGAwoDDwMSAAAAAAAAAgEAAAAAAAAAKAAAAAAA
	AAAAAAAAAAAAAx8=},
  bdsk-url-1 = {http://cholla.wustl.edu/baker/papers/WarwickerJ_WatsonHC_1982.pdf},
  date-added = {2008-06-29 14:56:24 -0500},
  date-modified = {2008-06-29 14:56:24 -0500},
  keywords = {Electrostatics},
  ty = {JOUR},
  url = {http://cholla.wustl.edu/baker/papers/WarwickerJ_WatsonHC_1982.pdf}
}

@ARTICLE{Weber:2004,
  author = {Weber, A. Z. and Newman, J. },
  title = { Modeling Transport in Polymer-Electrolyte Fuel Cells
	
	},
  journal = { Chemical Reviews },
  year = {2004},
  volume = {104},
  pages = {4679-4726}
}

@INPROCEEDINGS{SparseLSM,
  author = {Martin Weber and Andrew Blake and Roberto Cipolla},
  title = {{Sparse Finite Elements For Geodesic Contours With Level-Sets}},
  booktitle = {Proc. of ECCV},
  year = {2004},
  pages = {391--404}
}

@ARTICLE{Weber:2008,
  author = {Weber, T. P. and Stilianakis, N. I.},
  title = {Inactivation of {influenza A} viruses in the environment and modes
	of transmission: {A critical review}},
  journal = {Journal of Infection },
  year = {2008},
  volume = {57},
  pages = {361 - 373},
  annote = {Inactivation of {influenza A} viruses in the environment and modes
	of transmission: {A} critical review},
  date-added = {2009-03-10 },
  date-modified = {2009-03-10},
  ty = {JOUR}
}

@ARTICLE{Weeks:1971,
  author = {Weeks, J. D. and Chandler, D. and Andersen, H. C.},
  title = {Role of Repulsive Forces in Determining the Equilibrium Structure
	of Simple Liquids},
  journal = {Journal of Chemical Physics},
  year = {1971},
  volume = {54},
  pages = {5237-47},
  number = {12},
  abstract = {The different roles the attractive and repulsive forces play in forming
	the equilibrium structure of a Lennard-Jones liquid are discussed.
	It is found that the effects of these forces are most easily separated
	by considering the structure factor (or equivalently, the Fourier
	transform of the pair-correlation function) rather than the pair-correlation
	function itself. At intermediate and large wave vectors, the repulsive
	forces dominate the quantitative behavior of the liquid structure
	factor. The attractions are manifested primarily in the small wave
	vector part of the structure factor; but this effect decreases as
	the density increases and is almost negligible at reduced densities
	higher than 0.65. These conclusions are established by considering
	the structure factor of a hypothetical reference system in which
	the intermolecular forces are entirely repulsive and identical to
	the repulsive forces in a Lennard-Jones fluid. This reference system
	structure factor is calculated with the aid of a simple but accurate
	approximation described herein. The conclusions lead to a very simple
	prescription for calculating the radial distribution function of
	dense liquids which is more accurate than that obtained by any previously
	reported theory. The thermodynamic ramifications of the conclusions
	are presented in the form of calculations of the free energy, the
	internal energy (from the energy equation), and the pressure (from
	the virial equation). The implications of our conclusions to perturbation
	theories for liquids and to the interpretation of x-ray scattering
	experiments are discussed.},
  annote = {Role of Repulsive Forces in Determining the Equilibrium Structure
	of Simple Liquids; WCA},
  bdsk-url-1 = {http://dx.doi.org/10.1063/1.1674820},
  date-added = {2008-06-30 11:43:16 -0500},
  date-modified = {2008-06-30 11:43:16 -0500},
  keywords = {Statistical_mechanics},
  ty = {JOUR},
  url = {http://dx.doi.org/10.1063/1.1674820}
}

@ARTICLE{Wei:2009,
  author = {Wei, G. W.},
  title = {Differential geometry based multiscale models},
  journal = {Bulletin of Mathematical Biology},
  year = {2010},
  volume = {72},
  pages = {1562 - 1622}
}

@ARTICLE{Wei:2002b,
  author = {Wei, G. W.},
  title = {Oscillation reduction by anisotropic diffusions},
  journal = {Comput. Phys. Commun.},
  year = {2002},
  volume = {144},
  pages = {417-342},
  date-added = {2008-09-16 15:08:35 -0500},
  date-modified = {2008-09-16 15:09:09 -0500}
}

@ARTICLE{Wei:2002d,
  author = {Wei, G. W.},
  title = {Synchronization of single-side locally averaged adaptive coupling
	and its application to shock capturing},
  journal = {Phys.  Rev.  Lett. },
  year = {2002},
  volume = {86},
  pages = {3542-3545},
  number = { }
}


@ARTICLE{Wei:2002e,
  author = {Wei, G. W. and Zhan, Meng and Lai, C. H.},
  title = {Tailoring    wavelets  for  chaos  control},
  journal = {Phys.  Rev.  Lett. },
  year = {2002},
  volume = {89},
  pages = {284103},
  number = { }
}


@ARTICLE{Weicpc02,
  author = {Wei, G. W.},
  title = {Oscillation reduction by anisotropic diffusions},
  journal = {Comput. Phys. Commun.},
  year = {2002},
  volume = {144},
  pages = {317-342}
}

@ARTICLE{Wei:2001a,
  author = {Wei, G. W.},
  title = {Vibration analysis by discrete singular convolution},
  journal = {J. Sound Vibration},
  year = {2001},
  volume = {244},
  pages = {535 - 553}
}

@ARTICLE{Wei:2001b,
  author = {Wei, G. W.},
  title = {A new algorithm forsolving some mechanical problems},
  journal = {Comput. Methods Appl. Mech. Engng.},
  year = {2001},
  volume = {190},
  pages = {2017 - 2030 }
}


@ARTICLE{JCPWei:1999,
  author = {Wei, G. W..},
  title = {Discrete singular convolution for the solution of the {Fokker-Planck}
	equations},
  journal = {J. Chem. Phys.},
  year = {1999},
  volume = {110},
  pages = { 8930- 8942},
  number = { }
}

@ARTICLE{Wei:1999,
  author = {Wei, G. W.},
  title = {Generalized { Perona-Malik} equation for Image Restoration},
  journal = {IEEE Signal Processing Lett.},
  year = {1999},
  volume = {6},
  pages = {165-167 },
  annote = {Generalized Perona-Malik equation for Image Restoration},
  date-added = {2008-11-25 10:28:56 -0500},
  date-modified = {2008-11-25 10:28:56 -0500},
  ty = {JOUR}
}

@ARTICLE{Weijcp99,
  author = {Wei, G. W.},
  title = {Discrete singular convolution for the solution of the {Fokker-Planck}
	equations},
  journal = {J. Chem. Phys.},
  year = {1999},
  volume = {110},
  pages = {8930-8942}
}

@ARTICLE{Wei:1997a,
  author = {Wei, G. W. and Alavi, S. and Snider, R. F.},
  title = {Equal reaction rates for all recombination pathways},
  journal = {J. Chem. Phys. },
  year = {1997},
  volume = {106},
  pages = {1463-1466 },
  annote = {Equal reaction rates for all recombination pathways},
  date-added = {2008-11-25 10:28:56 -0500},
  date-modified = {2008-11-25 10:28:56 -0500},
  ty = {JOUR}
}

@ARTICLE{Wei:1998a,
  author = {Wei, G. W. and Althorpe, S. and Kouri, D. J. and Hoffman, D. K. },
  title = {Lagrange-distributed approximating-functional approach to wave-packet
	propagation: Application to the time-independent wave-packet reactant-product
	decoupling method},
  journal = {Phys. Rev. A },
  year = {1998},
  volume = {57},
  pages = {3309-3316 },
  annote = {Lagrange-distributed approximating-functional approach },
  date-added = {2008-11-25 10:28:56 -0500},
  date-modified = {2008-11-25 10:28:56 -0500},
  ty = {JOUR}
}

@ARTICLE{Wei:1998b,
  author = {Wei, G. W. and Althorpe, S. and Kouri, D. J. and Hoffman, D. K. },
  title = {An application of distributed approximating functional-wavelets to
	reactive scattering},
  journal = {J. Chem. Phys. },
  year = {1998},
  volume = {108},
  pages = {7065-7069 },
  annote = {An application of distributed approximating functional-wavelets to
	reactive scattering},
  date-added = {2008-11-25 10:28:56 -0500},
  date-modified = {2008-11-25 10:28:56 -0500},
  ty = {JOUR}
}

@ARTICLE{weigu,
  author = {Wei, G. W. and Gu, Y.},
  title = {Conjugated filter approach for solving {Burgers'} equation},
  journal = {J. Comput. Appl. Math.},
  year = {2002},
  volume = {149},
  pages = {439-456}
}

@ARTICLE{Wei:2002a,
  author = {Wei, G. W. and Jia, Y. Q.},
  title = {Synchronization-based image edge detection},
  journal = {Europhysics Letters},
  year = {2002},
  volume = {59},
  pages = {814-819},
  number = {6}
}

@ARTICLE{Wei:1996,
  author = {Wei, G. W. and Snider, R. F.},
  title = {Discrete basis representation of Ursell operators },
  journal = {Phys. Rev. E},
  year = {1996},
  volume = {54},
  pages = {2414-2418},
  annote = {Discrete basis representation of Ursell operators},
  date-added = {2008-11-25 10:28:56 -0500},
  date-modified = {2008-11-25 10:28:56 -0500},
  ty = {JOUR}
}

@ARTICLE{Wei:1995,
  author = {Wei, G. W. and Snider, R. F.},
  title = {Correlated state evaluation of the second virial coefficient},
  journal = {Phys. Rev. A},
  year = {1995},
  volume = {52},
  pages = {2925-2936 },
  annote = {Correlated state evaluation of the second virial coefficient},
  date-added = {2008-11-25 10:28:56 -0500},
  date-modified = {2008-11-25 10:28:56 -0500},
  ty = {JOUR}
}

@ARTICLE{Weisurface:2005,
  author = {Wei, G. W. and Sun, Y. H. and Zhou, Y.C. and Feig, M.},
  title = {Molecular multiresolution surfaces},
  journal = {arXiv:math-ph/0511001v1},
  year = {2005},
  date-added = {2008-09-19 10:28:56 -0500},
  date-modified = {2008-09-19 10:28:56 -0500},
  ty = {JOUR}
}

@ARTICLE{Wei:2005,
  author = {Wei, G. W. and Sun, Y. H. and Zhou, Y. C. and Feig, M.},
  title = {Molecular multiresolution surfaces},
  journal = {arXiv:math-ph/0511001v1},
  year = {2005},
  pages = {1 - 11},
  annote = {Molecular multiresolution surfaces},
  date-added = {2009-03-10 },
  date-modified = {2009-03-10},
  ty = {JOUR}
}

@ARTICLE{Wei:2002f,
  author = {Wei, G. W. and Zhao, Y. B. and Xiang, Y.},
  title = {Discrete singular convolution and its application to the analysis
	of plates with internal supports, {I} Theory and algorithm},
  journal = {Int. J. Numer. Methods Engng.},
  year = {2002},
  volume = {55},
  pages = {913 - 946}
}

@ARTICLE{WZXijnme02,
  author = {Wei, G. W. and Zhao, Y. B. and Xiang, Y.},
  title = {Discrete singular convolution and its application to the analysis
	of plates with internal supports, {I} Theory and algorithm},
  journal = {Int. J. Numer. Meth. Engng.},
  year = {2002},
  volume = {55},
  pages = {913-946}
}


@ARTICLE{Wei957224,
  author = {Wei, P. and Yang, W. T.},
  title = {Structure and Stability of Molybdenum Carbide Clusters (Moc4)(N)
	(N=1 to 4) and Their Anions},
  journal = {Physical Review B},
  year = {1995},
  volume = {51},
  pages = {7224-7230},
  number = {11},
  month = {Mar},
  endnotereftype = {Journal Article},
  issn = {1098-0121},
  shorttitle = {Structure and Stability of Molybdenum Carbide Clusters (Moc4)(N) (N=1
	to 4) and Their Anions},
  url = {<Go to ISI>://A1995QP77400054}
}

@ARTICLE{Weigl:1997,
  author = {Weigl, B. H. and Yager, P.},
  title = {Silicon-microfabricated diffusion-based optical chemical sensor},
  journal = {Sensors and Actuators B-Chemical },
  year = {1997},
  volume = {39},
  pages = {452-457}
}

@ARTICLE{Weiner:1986,
  author = {Weiner, S. J. and Kollman, P. A. and Nguyem, D. T. and Case, D. A.},
  title = {{An all atom force-field for simulations of proteins and nucleic-acids}},
  journal = {J Comp Chem},
  year = {1986},
  volume = {7},
  pages = {230-252},
  number = {2}
}

@ARTICLE{Weinzinger:2005,
  author = {Weinzinger, Philip and Hannongbua, Sup and Wolschann, Pete },
  title = {Molecular mechanics {PBSA} ligand binding energy and interaction
	of Efavirenz derivatives with {HIV-1} reverse transcriptase},
  journal = {Journal of Enzyme Inhibition and Medicinal Chemistry},
  year = {2005},
  volume = {20},
  pages = {129--134},
  number = {2},
  bdsk-file-1 = {YnBsaXN0MDDUAQIDBAUGCQpYJHZlcnNpb25UJHRvcFkkYXJjaGl2ZXJYJG9iamVjdHMSAAGGoNE
	HCFRyb290gAFfEA9OU0tleWVkQXJjaGl2ZXKoCwwXGBkdJCVVJG51bGzTDQ4PEBEUViRjbGFzc1
	dOUy5rZXlzWk5TLm9iamVjdHOAB6ISE4ACgAOiFRaABIAGWWFsaWFzRGF0YVxyZWxhdGl2ZVBhd
	GjSDRobHFdOUy5kYXRhgAVPEQIAAAAAAAIAAAIAAAxNYWNpbnRvc2ggSEQAAAAAAAAAAAAAAAAA
	AADD4v5NSCsAAAAZYksfMjAwNS1XZWluemluZ2VySGFubm8jMzE3NzcwLnBkZgAAAAAAAAAAAAA
	AAAAAAAAAAAAAAAAAAAAAAAAAAAAAADF3cMQrwoQAAAAAAAAAAAAEAAQAAAkgAAAAAAAAAAAAAA
	AAAAAAB0FyY2hpdmUAABAACAAAw+NSrQAAABEACAAAxCwI1AAAAAEAFAAZYksAGWIDAAqkKAAKp
	BEAAHrcAAIAVU1hY2ludG9zaCBIRDpVc2VyczpiYWtlcjpEb2N1bWVudHM6UmVmZXJlbmNlczpB
	cmNoaXZlOjIwMDUtV2Vpbnppbmdlckhhbm5vIzMxNzc3MC5wZGYAAA4ATgAmADIAMAAwADUALQB
	XAGUAaQBuAHoAaQBuAGcAZQByAEgAYQBuAG4AbwBuAGcAYgB1AGEAVwBvAGwAcwBjAGgAYQBuAG
	4ALgBwAGQAZgAPABoADABNAGEAYwBpAG4AdABvAHMAaAAgAEgARAASAE9Vc2Vycy9iYWtlci9Eb
	2N1bWVudHMvUmVmZXJlbmNlcy9BcmNoaXZlLzIwMDUtV2Vpbnppbmdlckhhbm5vbmdidWFXb2xz
	Y2hhbm4ucGRmAAATAAEvAAAVAAIADP//AADSHh8gIVgkY2xhc3Nlc1okY2xhc3NuYW1loyEiI11
	OU011dGFibGVEYXRhVk5TRGF0YVhOU09iamVjdF8QTy4uLy4uLy4uLy4uL0RvY3VtZW50cy9SZW
	ZlcmVuY2VzL0FyY2hpdmUvMjAwNS1XZWluemluZ2VySGFubm9uZ2J1YVdvbHNjaGFubi5wZGbSH
	h8mJ6InI1xOU0RpY3Rpb25hcnkACAARABoAHwApADIANwA6AD8AQQBTAFwAYgBpAHAAeACDAIUA
	iACKAIwAjwCRAJMAnQCqAK8AtwC5Ar0CwgLLAtYC2gLoAu8C+ANKA08DUgAAAAAAAAIBAAAAAAA
	AACgAAAAAAAAAAAAAAAAAAANf},
  bdsk-url-1 = {http://dx.doi.org/10.1080/14756360400020520},
  bdsk-url-2 = {http://dx.doi.org/10.1080/14756360400020520},
  date-added = {2008-09-01 13:50:14 -0500},
  date-modified = {2008-09-01 13:50:14 -0500},
  doi = {10.1080/14756360400020520},
  issn = {1475-6366},
  keywords = {Electrostatics, Protein-ligandInteractions, Solvation},
  posted-at = {2008-04-16 13:43:25},
  priority = {2},
  publisher = {Taylor and Francis Ltd},
  url = {http://dx.doi.org/10.1080/14756360400020520}
}

@ARTICLE{Whitten:2005,
  author = {Whitten, S. T. and GarcÃ­a-Moreno E. , B.},
  title = {Local conformational fluctuations can modulate the coupling between
	proton binding and global structural transitions in proteins},
  journal = {Proceedings of the National Academy of Sciences of the United States
	of America},
  year = {2005},
  volume = {102},
  pages = {4282-7},
  number = {12},
  abstract = {Local conformational fluctuations in proteins can affect the coupling
	between ligand binding and global structural transitions. This finding
	was established by monitoring quantitatively how the population distribution
	in the ensemble of microstates of staphylococcal nuclease was affected
	by proton binding. Analysis of acid unfolding and proton-binding
	data with an ensemble-based model suggests that local fluctuations:
	(i) can be effective modulators of ligand-binding affinities, (ii)
	are important determinants of the cooperativity of ligand-driven
	global structural transitions, and (iii) are well represented thermodynamically
	as local unfolding processes. These studies illustrate how an ensemble-based
	description of proteins can be used to describe quantitatively the
	interdependence of local conformational fluctuations, ligand-binding
	processes, and global structural transitions. This level of understanding
	of the relationship between conformation, energy, and dynamics is
	required for a detailed mechanistic understanding of allostery, cooperativity,
	and other complex functional and regulatory properties of macromolecules.},
  annote = {Local conformational fluctuations can modulate the coupling between
	proton binding and global structural transitions in proteins},
  bdsk-url-1 = {http://dx.doi.org/10.1073/pnas.0407499102},
  date-added = {2008-09-16 15:43:19 -0500},
  date-modified = {2008-09-16 15:43:19 -0500},
  keywords = {Solvation; Electrostatics},
  ty = {JOUR},
  url = {http://dx.doi.org/10.1073/pnas.0407499102}
}

@ARTICLE{Wiegmann:2000,
  author = {Andreas Wiegmann and Kenneth P. Bube},
  title = {The Explicit-Jump Immersed Interface Method: Finite Difference Methods
	for {PDEs} with Piecewise Smooth Solutions},
  journal = {SIAM Journal on Numerical Analysis},
  year = {2000},
  volume = {37},
  pages = {827-862},
  number = {3},
  abstract = {Many boundary value problems (BVPs) or initial BVPs have nonsmooth
	solutions, with jumps along lower-dimensional interfaces. The explicit-jump
	immersed interface method (EJIIM) was developed following Li's fast
	iterative immersed interface method (FIIIM), recognizing that the
	foundation for the efficient solution of many such problems is a
	good solver for elliptic BVPs. EJIIM generalizes the class of problems
	for which FIIIM is applicable. It handles interfaces between constant
	and variable coefficients and extends the immersed interface method
	(IIM) to BVPs on irregular domains with Neumann and {Dirichlet} boundary
	conditions. Proofs of second order convergence for a one-dimensional
	(1D) problem with piecewise constant coefficients and for two-dimensional
	(2D) problems with singular sources are given. Other problems are
	reduced to the singular sources case, with additional equations determining
	the source strengths. The advantages of EJIIM are high quality of
	solutions even on coarse grids and easy adaptation to many problems
	with complicated geometries, while still maintaining the efficiency
	of the FIIIM.},
  bdsk-url-1 = {http://link.aip.org/link/?SNA/37/827/1},
  bdsk-url-2 = {http://dx.doi.org/10.1137/S0036142997328664},
  date-added = {2008-09-14 15:32:12 -0500},
  date-modified = {2008-09-14 15:32:12 -0500},
  doi = {10.1137/S0036142997328664},
  keywords = {elliptic boundary value problems; immersed interface method; Cartesian
	grid; nonsmooth solutions; irregular domain; interface; singular
	source; discontinuous coefficients; finite difference methods},
  publisher = {SIAM},
  url = {http://link.aip.org/link/?SNA/37/827/1}
}

@BOOK{Willmore:1997,
  title = {Riemannian Geometry},
  publisher = {Oxford University Press, USA},
  year = {1997},
  author = {Willmore, T. J. },
  abstract = {Recent developments in the field of differential geometry have been
	so extensive that a new book with particular emphasis on current
	work in Riemannian geometry is clearly necessary. This new text brilliantly
	serves that purpose and includes an elementary account of twistor
	spaces that will interest both applied mathematicians and physicists.
	It presents recent developments in the theory of harmonic spaces,
	commutative spaces, and mean- value theorems previously only available
	in the source literature. The final chapter provides the only account
	available in book form of manifolds known as `Willmore surfaces',
	illustrated by a series of computer-generated pictures. This book
	is sure to be welcomed by researchers, teachers, and students interested
	in the latest developments in differential geometry.},
  bdsk-url-1 = {http://www.amazon.ca/exec/obidos/redirect?tag=citeulike09-20%5C&amp;path=ASIN/0198514921},
  date-added = {2008-06-30 09:46:09 -0500},
  date-modified = {2008-06-30 09:46:09 -0500},
  howpublished = {Paperback},
  isbn = {0198514921},
  keywords = {mathematics},
  posted-at = {2008-06-30 15:45:33},
  priority = {2},
  url = {http://www.amazon.ca/exec/obidos/redirect?tag=citeulike09-20\&amp;path=ASIN/0198514921}
}

@ARTICLE{Wilson:2010,
  author = {Wilson, J.R. and Cronin, J.S. and Duong, A.T. and Rukes, S. and Chen,
	H.Y. and Thornton, K. and Mumm, D.R. and Barnett, S.},
  title = {{Effect of composition of $({\rm La}_{0.8}{\rm Sr}_{0.2}{\rm Mn}_{O3}-{\rm
	Y}_{2}{\rm O}_{3}-{\rm stabilized}~~ {\rm ZrO}_{2})$ cathodes: Correlating
	three-dimensional microstructure and polarization resistance}},
  journal = {Journal of Power Sources},
  year = {2010},
  volume = {195},
  pages = {1829-1840.}
}

@ARTICLE{Wilson:1992,
  author = {Wilson, K.P. and Malcolm, B.A. and Matthews, B.W.},
  title = {Structural and thermodynamic analysis of compensating mutations within
	the core of chicken egg white lysozyme},
  journal = {J. Biol. Chem.},
  year = {1992},
  volume = {267},
  pages = {10842 - 10849},
  number = { }
}

@ARTICLE{Winslow:1967,
  author = {Winslow, A. M.},
  title = {{Numerical solution of the quasilinear Poisson equation in a nonuniform
	triangle mesh}},
  journal = {J. Comput. Phys.},
  year = {1967},
  volume = {2},
  pages = {149--172}
}

@ARTICLE{TWitelski:2003,
  author = {Witelski, T. P. and Bowen, M.},
  title = {{ADI schemes for higher-order nonlinear diffusion equations}},
  journal = {Applied Numerical Mathematics},
  year = {2003},
  volume = {45},
  pages = {331-351},
  number = {2-3}
}

@ARTICLE{AWitkin:1984,
  author = {Witkin, A.},
  title = {Scale-space filtering: A new approach to multi-scale description},
  journal = {Proceedings of {IEEE} International Conference on Acoustic Speech
	Signal Processing},
  year = {1984},
  volume = {9},
  pages = {150-153}
}

@BOOK{Wolfgang:2002,
  title = {Differential Geometry: Curves-Surface-Manifolds},
  publisher = {American Mathematical Society},
  year = {2002},
  author = {Wolfgang, K.}
}

@ARTICLE{Wong:2001,
  author = {Wong, C. F. and Hunenberger, P. H. and Akamine, P. and Narayana,
	N. and Diller, T. and McCammon, J. A. and Taylor, S. and Xuong, N.
	H.},
  title = {Computational analysis of PKA-balanol interactions},
  journal = {J Med Chem},
  year = {2001},
  volume = {44},
  pages = {1530-9},
  number = {10},
  abstract = {Protein kinases are important targets for designing therapeutic drugs.
	This paper illustrates a computational approach to extend the usefulness
	of a single protein-inhibitor structure in aiding the design of protein
	kinase inhibitors. Using the complex structure of the catalytic subunit
	of PKA (cPKA) and balanol as a guide, we have analyzed and compared
	the distribution of amino acid types near the protein-ligand interface
	for nearly 400 kinases. This analysis has identified a number of
	sites that are more variable in amino acid types among the kinases
	analyzed, and these are useful sites to consider in designing specific
	protein kinase inhibitors. On the other hand, we have found kinases
	whose protein-ligand interfaces are similar to that of the cPKA-balanol
	complex and balanol can be a useful lead compound for developing
	effective inhibitors for these kinases. Generally, this approach
	can help us discover new drug targets for an existing class of compounds
	that have already been well characterized pharmacologically. The
	relative significance of the charge/polarity of residues at the protein-ligand
	interface has been quantified by carrying out computational sensitivity
	analysis in which the charge/polarity of an atom or functional group
	was turned off/on, and the resulting effects on binding affinity
	have been examined. The binding affinity was estimated by using an
	implicit-solvent model in which the electrostatic contributions were
	obtained by solving the Poisson equation and the hydrophobic effects
	were accounted for by using surface-area dependent terms. The same
	sensitivity analysis approach was applied to the ligand balanol to
	develop a pharmacophoric model for searching new drug leads from
	small-molecule libraries. To help evaluate the binding affinity of
	designed inhibitors before they are made, we have developed a semiempirical
	approach to improve the predictive reliability of the implicit-solvent
	binding model.},
  address = {Department of Pharmacology, Howard Hughes Medical Institute, School
	of Medicine, University of California at San Diego, La Jolla, California
	92093, USA. c4wong{\char64}ucsd.edu},
  annote = {May 10; Computational analysis of PKA-balanol interactions; 11334563;
	21233423 0022-2623 Journal Article},
  bdsk-url-1 = {http://dx.doi.org/10.1021/jm000443d},
  date-added = {2008-09-16 15:36:36 -0500},
  date-modified = {2008-09-16 15:36:36 -0500},
  keywords = {Misc; BiologicalSystems; Electrostatics},
  ty = {JOUR},
  url = {http://dx.doi.org/10.1021/jm000443d}
}

@ARTICLE{Wong:2006,
  author = {Wong, C. J. and Rice, R. L. Baker, N. A. and Ju, T. and Lohman, T.
	M.},
  title = {Probing {3'-ssDNA} loop formation in {E. coli} {RecBCD/RecBC-DNA}
	complexes using non-natural {DNA}: a model for {\tt{}"{}}Chi{\tt{}"{}}
	recognition complexes},
  journal = {Journal of Molecular Biology},
  year = {2006},
  volume = {362},
  pages = {26-43},
  number = {1},
  abstract = {The equilibrium binding of {E. coli} RecBC and RecBCD helicases to
	duplex DNA ends containing varying lengths of polyethylene glycol
	(PEG) spacers within pre-formed 3'-single-stranded (ss) DNA ((dT){\_}n)
	tails were studied. These studies were designed to test a previous
	proposal that the 3'-(dT){\_}n tail can be looped out upon binding
	RecBC and RecBCD for 3'-ssDNA tails with n {$\backslash$}geq 6 nucleotides.
	Equilibrium binding of protein to unlabeled DNA substrates with ends
	containing PEG-substituted 3'-ssDNA tails was examined by competition
	with a Cy3-labeled reference DNA which undergoes a Cy3 fluorescence
	enhancement upon protein binding. We find that the binding affinities
	of both RecBC and RecBCD for a DNA end are unaffected upon substituting
	PEG for the ssDNA between the sixth and the final two nucleotides
	of the 3'-(dT){\_}n tail. However, placing PEG at the end of the
	3'-(dT){\_}n tail increases the binding affinities to their maximum
	values (i.e. the same as binding constants for RecBC or RecBCD to
	a DNA end with only a 3'-(dT){\_}6 tail). Equilibrium binding studies
	of a RecBC mutant containing a nuclease domain deletion, RecB\^{}{\{}{$\backslash$}Delta
	nuc{\}}C\^{}1 suggest that looping of the 3'-tail (when n {$\backslash$}geq
	6 nucleotides) occurs even in the absence of the RecB nuclease domain,
	the nuclease domain stabilizes such loop formation. Computer modeling
	of the RecBCD-DNA complexes suggests that the loop in the 3'-ssDNA
	tail may form at the RecB/RecC interface. Based on these results
	we suggest a model for how a loop in the 3'-ssDNA tail might form
	upon encounter of a {\tt{}"{}}Chi{\tt{}"{}} recognition sequence
	during unwinding of DNA by the RecBCD helicase.},
  annote = {Probing 3'-ssDNA loop formation in {E. coli} RecBCD/RecBC-DNA complexes
	using non-natural DNA: a model for {\tt{}"{}}Chi{\tt{}"{}} recognition
	complexes},
  bdsk-file-1 = {YnBsaXN0MDDUAQIDBAUGCQpYJHZlcnNpb25UJHRvcFkkYXJjaGl2ZXJYJG9iamVjdHMSAAGGoNE
	HCFRyb290gAFfEA9OU0tleWVkQXJjaGl2ZXKoCwwXGBkdJCVVJG51bGzTDQ4PEBEUViRjbGFzc1
	dOUy5rZXlzWk5TLm9iamVjdHOAB6ISE4ACgAOiFRaABIAGWWFsaWFzRGF0YVxyZWxhdGl2ZVBhd
	GjSDRobHFdOUy5kYXRhgAVPEQHSAAAAAAHSAAIAAAxNYWNpbnRvc2ggSEQAAAAAAAAAAAAAAAAA
	AADD4v5NSCsAAAAZYksZMjAwNi1Xb25nUmljZUp1TG9obWFuLnBkZgAAAAAAAAAAAAAAAAAAAAA
	AAAAAAAAAAAAAAAAAAAAAAAAAAAAAABlircKAqUMAAAAAAAAAAAAEAAQAAAkgAAAAAAAAAAAAAA
	AAAAAAB0FyY2hpdmUAABAACAAAw+NSrQAAABEACAAAwoDvkwAAAAEAFAAZYksAGWIDAAqkKAAKp
	BEAAHrcAAIAT01hY2ludG9zaCBIRDpVc2VyczpiYWtlcjpEb2N1bWVudHM6UmVmZXJlbmNlczpB
	cmNoaXZlOjIwMDYtV29uZ1JpY2VKdUxvaG1hbi5wZGYAAA4ANAAZADIAMAAwADYALQBXAG8AbgB
	nAFIAaQBjAGUASgB1AEwAbwBoAG0AYQBuAC4AcABkAGYADwAaAAwATQBhAGMAaQBuAHQAbwBzAG
	gAIABIAEQAEgBCVXNlcnMvYmFrZXIvRG9jdW1lbnRzL1JlZmVyZW5jZXMvQXJjaGl2ZS8yMDA2L
	VdvbmdSaWNlSnVMb2htYW4ucGRmABMAAS8AABUAAgAM//8AANIeHyAhWCRjbGFzc2VzWiRjbGFz
	c25hbWWjISIjXU5TTXV0YWJsZURhdGFWTlNEYXRhWE5TT2JqZWN0XxBCLi4vLi4vLi4vLi4vRG9
	jdW1lbnRzL1JlZmVyZW5jZXMvQXJjaGl2ZS8yMDA2LVdvbmdSaWNlSnVMb2htYW4ucGRm0h4fJi
	eiJyNcTlNEaWN0aW9uYXJ5AAgAEQAaAB8AKQAyADcAOgA/AEEAUwBcAGIAaQBwAHgAgwCFAIgAi
	gCMAI8AkQCTAJ0AqgCvALcAuQKPApQCnQKoAqwCugLBAsoDDwMUAxcAAAAAAAACAQAAAAAAAAAo
	AAAAAAAAAAAAAAAAAAADJA==},
  bdsk-url-1 = {http://dx.doi.org/10.1016/j.jmb.2006.07.016},
  date-added = {2008-09-16 15:50:17 -0500},
  date-modified = {2008-09-16 15:50:17 -0500},
  keywords = {NucleicAcids; Protein-nucleicAcidInteractions},
  ty = {JOUR},
  url = {http://dx.doi.org/10.1016/j.jmb.2006.07.016}
}

@ARTICLE{Wong:1998,
  author = {Wong, H. S. P. and Tuar, Y. and Frank, D. J.},
  title = {Microelectronics reliability},
  journal = {SIAM J. Appl. Math.},
  year = {1998},
  volume = {38},
  pages = {1447-1456}
}

@ARTICLE{WHDS04,
  author = {Zo{\"e} Wood and Hugues Hoppe and Mathieu Desbrun and Peter Schr{\"o}der},
  title = {Removing Excess Topology From Isosurfaces},
  journal = {ACM Trans. on Graphics},
  year = {2004},
  volume = {23},
  pages = {190--203},
  number = {2}
}

@ARTICLE{Zoe,
  author = {Z. Wood and H. Hoppe and M. Desbrun and P. Schr{\"o}der},
  title = {Removing excess topology from isosurfaces},
  journal = {ACM Trans. Graph.},
  year = {2004},
  volume = {23},
  pages = {190--208},
  number = {2}
}

@INPROCEEDINGS{WDSB00,
  author = {Zo{\"e} J. Wood and Mathieu Desbrun and Peter Schr{\"o}der and David
	Breen},
  title = {Semi-Regular Mesh Extraction from Volumes},
  booktitle = {IEEE Visualization Conference},
  year = {2000},
  pages = {275--282}
}

@ARTICLE{Wroblewska:2007,
  author = {Wroblewska, L. and Skolnick, J.},
  title = {{Can a physics-based, all-atom potential find a protein's native
	structure among misfolded structures? I. Large scale AMBER benchmarking.}},
  journal = {J Comput Chem},
  year = {2007},
  volume = {28},
  pages = {2059-2066},
  number = {12}
}

@ARTICLE{Wu:2011,
  author = {Wu, C. L. and Li, Z. L. and Lai, M. C.},
  title = {Adaptive mesh refinement for elliptic interface problems using the
	non-conforming immerse finite element method},
  journal = {International Journal of Numerical Analysis and Modeling},
  year = {2011},
  volume = {8},
  pages = {466--483}
}

@ARTICLE{DPWu:2009,
  author = {Wu, D. P. and Steckl, A. J.},
  title = {High speed nanofluidic protein accumulator },
  journal = { Lab on a Chip },
  year = {2009},
  volume = {9},
  pages = { 1890-1896}
}

@ARTICLE{Wu032978,
  author = {Wu, Q. and Ayers, P. W. and Yang, W. T.},
  title = {Density-functional theory calculations with correct long-range potentials},
  journal = {Journal of Chemical Physics},
  year = {2003},
  volume = {119},
  pages = {2978-2990},
  number = {6},
  month = {Aug},
  abstract = {A variational method for forcing the exchange-correlation potential
	in density-functional theory (DFT) to have the correct asymptotic
	decay is developed. The resulting exchange-correlation potentials
	are much improved while the total energies remain essentially the
	same, compared with conventional density-functional theory calculations.
	The highest occupied orbital energies from the asymptotically corrected
	exchange-correlation potentials are found to provide significantly
	more accurate approximations to the ionization potential (for a neutral
	molecule) and the electron affinity (for an anion) than those from
	conventional calculations, although the results are usually inferior
	to direct methods by computing energy differences. Extending recent
	results from exchange-only DFT, we show that exact exchange-correlation
	potential is nonuniform asymptotically. Correcting the asymptotic
	decay of approximate exchange-correlation potentials towards the
	exact functional form binds the highest occupied orbitals for atomic
	and molecular anions, which supports the use of DFT calculations
	for negatively charged molecular species. With this technique, even
	hybrid functionals have local exchange-correlation potentials, effectively
	removing the largest objection to including these functionals in
	the panoply of Kohn-Sham DFT methods. (C) 2003 American Institute
	of Physics.},
  endnotereftype = {Journal Article},
  issn = {0021-9606},
  shorttitle = {Density-functional theory calculations with correct long-range potentials},
  url = {<Go to ISI>://000184350300006}
}

@ARTICLE{Wu05134111,
  author = {Wu, Q. and Cohen, A. J. and Yang, W. T.},
  title = {Analytic energy gradients of the optimized effective potential method},
  journal = {Journal of Chemical Physics},
  year = {2005},
  volume = {123},
  pages = {134111},
  number = {13},
  month = {Oct},
  abstract = {The analytic energy gradients of the optimized effective potential
	(OEP) method in density-functional theory are developed. Their implementation
	in the direct optimization approach of Yang and Wu [Phys. Rev. Lett.
	89, 143002 (2002)] and Wu and Yang [J. Theor. Comput. Chem. 2, 627
	(2003)] are carried out and the validity is confirmed by comparison
	with corresponding gradients calculated via numerical finite difference.
	These gradients are then used to perform geometry optimizations on
	a test set of molecules. It is found that exchange-only OEP (EXX)
	molecular geometries are very close to the Hartree-Fock results and
	that the difference between the B3LYP and OEP-B3LYP results is negligible.
	When the energy is expressed in terms of a functional of Kohn-Sham
	orbitals, or in terms of a Kohn-Sham potential, the OEP becomes the
	only way to perform density-functional calculations and the present
	development in the OEP method should play an important role in the
	applications of orbital or potential functionals. (c) 2005 American
	Institute of Physics.},
  endnotereftype = {Journal Article},
  issn = {0021-9606},
  shorttitle = {Analytic energy gradients of the optimized effective potential method},
  url = {<Go to ISI>://000232442500013}
}

@ARTICLE{Wu05711,
  author = {Wu, Q. and Cohen, A. J. and Yang, W. T.},
  title = {Excitation energies from time-dependent density functional theory
	with accurate exchange-correlation potentials},
  journal = {Molecular Physics},
  year = {2005},
  volume = {103},
  pages = {711-717},
  number = {6-8},
  month = {Mar-Apr},
  abstract = {We have applied two Of Our recently developed methods for calculating
	accurate Kohn-Sham potentials, namely direct optimization of non-interacting
	kinetic energy of a known electron density and the asymptotic correction
	of approximate exchange-correlation potentials, to the calculation
	of excitation energies within time-dependent density functional theory.
	Our asymptotic correction method is found not to be adequate in improving
	Rydberg state results, probably because the potential is still affected
	by the approximate energy functional due to the variational nature
	of the method. However, Kohn-Sham potentials calculated from coupled
	Cluster singles and doubles densities give excellent results for
	the He and Be atoms, and consistently Much improved results for molecules.},
  endnotereftype = {Journal Article},
  issn = {0026-8976},
  shorttitle = {Excitation energies from time-dependent density functional theory
	with accurate exchange-correlation potentials},
  url = {<Go to ISI>://000228583300001}
}

@ARTICLE{Wu032498,
  author = {Wu, Q. and Yang, W. T.},
  title = {A direct optimization method for calculating density functionals
	and exchange-correlation potentials from electron densities},
  journal = {Journal of Chemical Physics},
  year = {2003},
  volume = {118},
  pages = {2498-2509},
  number = {6},
  month = {Feb},
  abstract = {A direct optimization method is developed for the computation of the
	Kohn-Sham kinetic energy density functional T-s from a given electron
	density and the exchange-correlation potential v(xc) if this density
	is from a ground state. The method is based on the construction of
	a variational functional of the one-electron potential. This functional
	is derived from the conventional Levy constrained-search formulation
	and is shown to be closely related to the Lieb functional construction.
	The one-electron potential is expanded in terms of some fixed terms
	plus a linear expansion in a basis set. The determination of the
	Kohn-Sham kinetic energy for an input density is then turned into
	the maximization of this functional of potential. The analytic first
	and second derivatives of the variational functional with respect
	to the linear basis set expansion coefficients and also the nonlinear
	parameters in the basis set are derived. This enables very efficient
	iterative optimization of the potential and hence the calculation
	of T-s and v(xc). The efficiency and accuracy of the method is shown
	in the numerical implementation for atomic and molecular calculations
	with Gaussian basis set expansions both for molecular orbitals and
	for one-electron potentials. Finally, this direct optimization method
	is extended to general density functionals and the analytic derivatives
	are also developed for use in optimization methods. (C) 2003 American
	Institute of Physics.},
  endnotereftype = {Journal Article},
  issn = {0021-9606},
  shorttitle = {A direct optimization method for calculating density functionals and
	exchange-correlation potentials from electron densities},
  url = {<Go to ISI>://000180564800008}
}

@ARTICLE{Wu03627,
  author = {Wu, Q. and Yang, W. T.},
  title = {Algebraic equation and iterative optimization for the optimized effective
	potential in density functional theory},
  journal = {Journal of Theoretical \& Computational Chemistry},
  year = {2003},
  volume = {2},
  pages = {627-638},
  number = {4},
  month = {Dec},
  abstract = {We further develop our recent direct method for the optimized effective
	potential (OEP) in density functional theory (DFT) [Yang and Wu,
	Phys. Rev. Lett. 89, 143002 (2002)]. First, we show that the stationary
	condition in our optimization approach leads to a proper nonlinear
	algebraic equation for the OEP in a finite basis set, which differs
	from other finite basis set approaches. Then by constructing an approximate
	second derivative matrix of the energy functional in conjunction
	with the use of the Newton method, we significantly accelerate the
	convergence of the iterative optimization for OEP. Enhancement of
	the method is made in using the Tikhonov regularization method for
	the inversion of the second derivative matrix when it is singular
	or nearly singular and the direct inversion in the iterative space.
	It is shown that under a fixed stepsize condition, the optimization
	approach is equivalent to the self-consistent solution to the nonlinear
	algebraic equation for OEP. Because the approximate second derivatives
	are easy to compute and the iteration numbers are small now, the
	computation costs of OEP become comparable to that of regular DFT
	calculations as shown by calculations of some molecules, small and
	larger ones. We show how to find balanced results between energies
	and potentials when choosing a basis set for potentials.},
  endnotereftype = {Journal Article},
  issn = {0219-6336},
  shorttitle = {Algebraic equation and iterative optimization for the optimized effective
	potential in density functional theory},
  url = {<Go to ISI>://000220867400015}
}

@ARTICLE{Wu02515,
  author = {Wu, Q. and Yang, W. T.},
  title = {Empirical correction to density functional theory for van der Waals
	interactions},
  journal = {Journal of Chemical Physics},
  year = {2002},
  volume = {116},
  pages = {515-524},
  number = {2},
  month = {Jan},
  abstract = {An empirical method has been designed to account for the van der Waals
	interactions in practical molecular calculations with density functional
	theory. For each atom pair separated at a distance R, the method
	adds to the density functional electronic structure calculations
	an additional attraction energy E-vdW=-f(d)(R)C6R-6, where f(d)(R)
	is the damping function which equals to one at large value of R and
	zero at small value of R. The coefficients C-6 for pair interactions
	between hydrogen, carbon, nitrogen, and oxygen atoms have been developed
	in this work by a least-square fitting to the molecular C-6 coefficients
	obtained from the dipole oscillator strength distribution method
	by Meath and co-workers. Two forms of the damping functions have
	been studied, with one dropping to zero at short distances much faster
	than the other. Four density functionals have been examined: Becke's
	three parameter hybrid functional with the Lee-Yang-Parr correlation
	functional, Becke's 1988 exchange functional with the LYP correlation
	functional, Becke's 1988 exchange functional with Perdew and Wang's
	1991 (PW91) correlation functional, and PW91 exchange and correlation
	functional. The method has been applied to three systems where the
	van der Waals attractions are known to be important: rare-gas diatomic
	molecules, stacking of base pairs and polyalanines' conformation
	stabilities. The results show that this empirical method, with the
	damping function dropping to zero smoothly, provides a significant
	correction to both of the Becke's hybrid functional and the PW91
	exchange and correlation functional. Results are comparable to the
	corresponding second-order Moller-Plesset calculations in many cases.
	(C) 2002 American Institute of Physics.},
  endnotereftype = {Journal Article},
  issn = {0021-9606},
  shorttitle = {Empirical correction to density functional theory for van der Waals
	interactions},
  url = {<Go to ISI>://000172926700007}
}

@ARTICLE{Wu:2007(a),
  author = {Wu, S. and Skolnick, J. and Zhang, Y.},
  title = {{Ab initio modeling of small proteins by iterative TASSER simulations}},
  journal = {BMC Biol},
  year = {2007},
  volume = {5},
  pages = {17}
}

@ARTICLE{Wu:2010(a),
  author = {Wu, S. and Szilagyi, A. and Zhang, Y.},
  title = {{Improving protein structure prediction using multiple sequence-based
	contact predictions}},
  year = {2010:Submitted}
}

@ARTICLE{Wu:2009,
  author = {Wu, S. and Zhang, Y.},
  title = {{Protein structure prediction.}},
  journal = {In: Edwards D, Hansen D, Stajich J, editors. Bioinformatics: Tools
	and Applications: Springer-London},
  year = {2009. p in press}
}

@ARTICLE{Wu:2010(b),
  author = {Wu, S. and Zhang, Y.},
  title = {{Recognizing protein substructure similarity using segmental threading}},
  journal = {Structure},
  year = {2010},
  volume = {18},
  pages = {858-867},
  number = {7}
}

@ARTICLE{Wu:2008(a),
  author = {Wu, S. T. and Zhang, Y.},
  title = {{MUSTER: Improving Protein Sequence Profile-Profile Alignments by
	Using Multiple Sources of Structure Information}},
  journal = {Proteins},
  year = {2008},
  volume = {72},
  pages = {547-556},
  number = {2}
}

@ARTICLE{Wu:2008(b),
  author = {Wu, S. and Zhang, Y.},
  title = {{MUSTER: Improving protein sequence profile-profile alignments by
	using multiple sources of structure information}},
  journal = {Proteins},
  year = {2008},
  volume = {72},
  pages = {547-556},
  number = {2}
}

@ARTICLE{Wu:2008(c),
  author = {Wu, S. and Zhang, Y.},
  title = {{A comprehensive assessment of sequence-based and template-based
	methods for protein contact prediction}},
  journal = {Bioinformatics},
  year = {2008},
  volume = {24},
  pages = {924-931},
  number = {7}
}

@ARTICLE{Wu:2008(d),
  author = {Wu, S. and Zhang, Y.},
  title = {{ANGLOR: a composite machine-learning algorithm for protein backbone
	torsion angle prediction}},
  journal = {PLoS ONE},
  year = {2008},
  volume = {3},
  pages = {e3400},
  number = {10}
}

@ARTICLE{Wu:2007(b),
  author = {Wu, S. T. and Zhang, Y.},
  title = {{LOMETS: A local meta-threading-server for protein structure prediction}},
  journal = {Nucl Acids Res},
  year = {2007},
  volume = {35},
  pages = {3375-3382}
}

@ARTICLE{Wu:2007(c),
  author = {Wu, S. T. and Skolnick, J. and Zhang, Y.},
  title = {{Ab initio modeling of small proteins by iterative TASSER simulations}},
  journal = {BMC Biology},
  year = {2007},
  volume = {5},
  pages = {17}
}



@ARTICLE{Xiang2006,
  author = {Xiang, Y and Morais, MC and Battisti, AJ and Grimes, S and Jardine,
	PJ and Anderson, DL and Rossmann, MG},
  title = {Structural changes of bacteriophage phi29 upon DNA packaging and
	release.},
  journal = {EMBO J},
  year = {2006},
  volume = {25},
  pages = {5229-39--},
  number = {21},
  month = nov,
  abstract = {Cryo-electron microscopy three-dimensional reconstructions have been
	made of mature and of emptied bacteriophage phi29 particles without
	making symmetry assumptions. Comparisons of these structures with
	each other and with the phi29 prohead indicate how conformational
	changes might initiate successive steps of assembly and infection.
	The 12 adsorption capable 'appendages' were found to have a structure
	homologous to the bacteriophage P22 tailspikes. Two of the appendages
	are extended radially outwards, away from the long axis of the virus,
	whereas the others are around and parallel to the phage axis. The
	appendage orientations are correlated with the symmetry-mismatched
	positions of the five-fold related head fibers, suggesting a mechanism
	for partial cell wall digestion upon rotation of the head about the
	tail when initiating infection. The narrow end of the head-tail connector
	is expanded in the mature virus. Gene product 3, bound to the 5'
	ends of the genome, appears to be positioned within the expanded
	connector, which may potentiate the release of DNA-packaging machine
	components, creating a binding site for attachment of the tail.},
  address = {Department of Biological Sciences, Purdue University, West Lafayette,
	IN 47907-2054, USA.},
  comment = {Research Support, Non-U.S. Gov't,Research Support, U.S. Gov't, Non-P.H.S.,Research
	Support, N.I.H., Extramural,Comparative Study,},
  keywords = {Bacillus Phages, Cryoelectron Microscopy, DNA Packaging, DNA, Viral,
	Genome, Viral, Models, Biological, Viral Proteins, Virus Assembly},
  owner = {SeanLab},
  timestamp = {2012.05.23},
  url = {http://ukpmc.ac.uk/abstract/MED/17053784}
}

@ARTICLE{Xiao082814,
  author = {Xiao, D. Q. and Bulat, F. A. and Yang, W. T. and Beratan, D. N.},
  title = {A donor-nanotube paradigm for nonlinear optical materials},
  journal = {Nano Letters},
  year = {2008},
  volume = {8},
  pages = {2814-2818},
  number = {9},
  month = {Sep},
  abstract = {Studies of the nonlinear electronic response of donor/acceptor substituted
	nanotubes suggest a behavior that is both surprising and qualitatively
	distinct from that in conventional conjugated organic species. We
	find that the carbon nanotubes serve as both electronic bridges and
	acceptors, leading to a donor-nanotube paradigm for the effective
	design of large first hyperpolarizabilities. We also find that tuning
	the donor orientation, relative to the nanotube, can significantly
	enhance the first hyperpolarizability.},
  endnotereftype = {Journal Article},
  issn = {1530-6984},
  shorttitle = {A donor-nanotube paradigm for nonlinear optical materials},
  url = {<Go to ISI>://000259140200036}
}

@ARTICLE{Xiao0844106,
  author = {Xiao, D. Q. and Yang, W. T. and Beratan, D. N.},
  title = {Inverse molecular design in a tight-binding framework},
  journal = {Journal of Chemical Physics},
  year = {2008},
  volume = {129},
  pages = {044106},
  number = {4},
  month = {Jul},
  abstract = {The number of chemical species of modest molecular weight that can
	be accessed with known synthetic methods is astronomical. An open
	challenge is to explore this space in a manner that will enable the
	discovery of molecular species and materials with optimized properties.
	Recently, an inverse molecular design strategy, the linear combination
	of atomic potentials (LCAP) approach [J. Am. Chem. Soc. 128, 3228
	(2006)] was developed to optimize electronic polarizabilities and
	first hyperpolarizabilities. Here, using a simple tight-binding (TB)
	approach, we show that continuous optimization can be carried out
	on the LCAP surface successfully to explore vast chemical libraries
	of 10(2) to 10(16) extended aromatic compounds. We show that the
	TB-LCAP optimization is not only effective in locating globally optimal
	structures based on their electronic polarizabilities and first hyperpolarizabilities,
	but also is straightforwardly extended to optimize transition dipole
	moments and HOMO-LUMO energy gaps. This approach finds optimal structures
	among 10(4) candidates with about 40 individual molecular property
	calculations. As such, for structurally similar molecular candidates,
	the TB-LCAP approach may provide an effective means to identify structures
	with optimal properties. (C) 2008 American Institute of Physics.},
  endnotereftype = {Journal Article},
  issn = {0021-9606},
  shorttitle = {Inverse molecular design in a tight-binding framework},
  url = {<Go to ISI>://000258171500011}
}

@ARTICLE{Xie:2007,
  author = { Xie, D. and Zhou, S. Z.},
  title = {A new minimization protocol for solving nonlinear {{Poisson-Boltzmann}}
	mortar finite element equation},
  journal = {BIT NUMERICAL MATHEMATICS},
  year = {2007},
  volume = {47},
  pages = {853-871 }
}

@ARTICLE{Xie048039,
  author = {Xie, L. and Liu, H. Y. and Yang, W. T.},
  title = {Adapting the nudged elastic band method for determining minimum-energy
	paths of chemical reactions in enzymes},
  journal = {Journal of Chemical Physics},
  year = {2004},
  volume = {120},
  pages = {8039-8052},
  number = {17},
  month = {May},
  abstract = {Optimization of reaction paths for enzymatic systems is a challenging
	problem because such systems have a very large number of degrees
	of freedom and many of these degrees are flexible. To meet this challenge,
	an efficient, robust and general approach is presented based on the
	well-known nudged elastic band reaction path optimization method
	with the following extensions: (1) soft spectator degrees of freedom
	are excluded from path definitions by using only inter-atomic distances
	corresponding to forming/breaking bonds in a reaction; (2) a general
	transformation of the distances is defined to treat multistep reactions
	without knowing the partitioning of steps in advance; (3) a multistage
	strategy, in which path optimizations are carried out for reference
	systems with gradually decreasing rigidity, is developed to maximize
	the opportunity of obtaining continuously changing environments along
	the path. We demonstrate the applicability of the approach using
	the acylation reaction of type A beta-lactamase as an example. The
	reaction mechanism investigated involves four elementary reaction
	steps, eight forming/breaking bonds. We obtained a continuous minimum
	energy path without any assumption on reaction coordinates, or on
	the possible sequence or the concertedness of chemical events. We
	expect our approach to have general applicability in the modeling
	of enzymatic reactions with quantum mechanical/molecular mechanical
	models. (C) 2004 American Institute of Physics.},
  endnotereftype = {Journal Article},
  issn = {0021-9606},
  shorttitle = {Adapting the nudged elastic band method for determining minimum-energy
	paths of chemical reactions in enzymes},
  url = {<Go to ISI>://000221084500026}
}

@ARTICLE{Xu:2009,
  author = {Xu, D. and Zhang, Y.},
  title = {{Generating triangulated macromolecular surfaces by Euclidean Distance
	Transform}},
  journal = {PLoS One},
  year = {2009},
  volume = {4},
  pages = {e8140},
  number = {12}
}

@ARTICLE{Xu:DSM:2006,
  author = {Guoliang Xu and Qing Pan and Chandrajit L. Bajaj},
  title = {Discrete Surface Modeling Using Partial Differential Equations},
  journal = {Computer Aided Geometric Design},
  year = {2006},
  volume = {23},
  pages = {125--145},
  number = {2}
}

@ARTICLE{Xu:2010(a),
  author = {Xu, J. and Han, D. and Han, B. and Wang, Y. and Zhang, H. and Han,
	L. and Chen, Y. and Ji, Z. Y. Z.},
  title = {{Investigation of Cytokine Activities by Genome Wide Identification
	of Novel Cytokine-Receptor interactions}},
  year = {2010:Submitted}
}

@ARTICLE{Xu:2010(b),
  author = {Xu, J. and Zhang, Y.},
  title = {{How significant is a protein structure similarity with TM-score
	= 0.5 ?}},
  journal = {Bioinformatics},
  year = {2010},
  volume = {26},
  pages = {889-895},
  number = {7}
}

@ARTICLE{Xu01,
  author = {Xu, K.},
  title = {A gas-kinetic {BGK} scheme for the {Navier-Stokes} equations and
	its connection with artificial dissipation and {Godunov} method},
  journal = {J. Comput. Phys.},
  year = {2001},
  volume = {171},
  pages = {289-335}
}

@ARTICLE{MXu:2007,
  author = {Xu, M. and Zhou, S. L.},
  title = {Existence and uniqueness of weak solutions for a fourth-order nonlinear
	parabolic equation},
  journal = {Journal of Mathematical Analysis and Applications},
  year = {2007},
  volume = {325},
  pages = {636-654},
  number = {1},
  abstract = {In this paper we establish the existence and uniqueness of weak solutions
	for the initial-boundary value problem of a fourth-order nonlinear
	parabolic equation. (c) 2006 Elsevier Inc. All rights reserved.}
}

@ARTICLE{Xu:2000,
  author = {Xu, Y. and Xu, D.},
  title = {{Protein threading using PROSPECT: design and evaluation}},
  journal = {Proteins},
  year = {2000},
  volume = {40},
  pages = {343-354},
  number = {3}
}

@ARTICLE{Xue87258,
  author = {Xue, W. and Yang, W.T.},
  title = {Application of a Scaled Particle Theory to Polar Solute System and
	Calculation of the Salt Effect Constant},
  journal = {Acta Physico-Chimica Sinica},
  year = {1987},
  volume = {3},
  pages = {258},
  endnotereftype = {Journal Article},
  shorttitle = {Application of a Scaled Particle Theory to Polar Solute System and
	Calculation of the Salt Effect Constant}
}

@ARTICLE{Wang:2008y,
  author = {Wang Y.},
  title = {Sigma-delta quantization and the travelling salesman problem},
  journal = {Advances in Computational Math.},
  year = {2008},
  volume = {28},
  pages = {101 - 118}
}

@ARTICLE{RXYan:2009,
  author = {Yan, R. X. and Liang, W. J. and Fan, R. and Yang, P. D. },
  title = {Nanofluidic Diodes Based on Nanotube Heterojunctions},
  journal = {Nano Letters },
  year = {2009},
  volume = {9},
  pages = { 3820-3825 }
}

@ARTICLE{SYan:2007,
  author = {Yan, S. H. and Liang Zhang, L. and Cukier, R. I. and Bu, Y. X.},
  title = {Exploration on regulating factors for proton transfer along hydrogen-bonded
	water chains },
  journal = {Chem. Phys. Chem.},
  year = {2007},
  volume = {8},
  pages = {944-954}
}

@ARTICLE{Yang:1993a,
  author = {Yang, A. S. and Gunner, M. R. and Sampogna, R. and Sharp, K. and
	Honig, B.},
  title = {On the Calculation of {pK(a)s} in proteins},
  journal = {Proteins-Structure Function and Genetics},
  year = {1993},
  volume = {15},
  pages = {252-265},
  number = {3},
  address = {Columbia univ coll phys \& surg,dept biochem \& molec biophys,630
	w 168th st new york, ny usa 10032},
  annote = {On the Calculation of Pk(a)S in Proteins; MAR},
  date-added = {2008-09-01 13:53:00 -0500},
  date-modified = {2008-09-01 13:53:00 -0500},
  journal1 = {Protein-Struct Funct Genet},
  keywords = {Electrostatics; pKa},
  ty = {JOUR}
}

@ARTICLE{SYYang:2002,
  author = {Yang, S. Y. and Zhou, Y. C. and Wei, G. W.},
  title = {Comparison of the discrete singular convolution algorithm and the
	Fourier pseudospectral methods for solving partial differential equations},
  journal = {Comput. Phys. Commun.},
  year = {2002},
  volume = {143},
  pages = {113 -135}
}

@ARTICLE{yangsy,
  author = {Yang, S. Y. and Zhou, Y. C. and Wei, G. W.},
  title = {Comparison of the discrete singular convolution algorithm and the
	Fourier pseudospectral method for solving partial differential equations},
  journal = {Comput. Phys. Commun.},
  year = {2002},
  volume = {143},
  pages = {113--135}
}

@ARTICLE{Yang863320,
  author = {Yang, W. and Harriman, J. E.},
  title = {Analysis of the Kinetic-Energy Functional in Density Functional Theory},
  journal = {Journal of Chemical Physics},
  year = {1986},
  volume = {84},
  pages = {3320-3323},
  number = {6},
  month = {Mar},
  endnotereftype = {Journal Article},
  issn = {0021-9606},
  shorttitle = {Analysis of the Kinetic-Energy Functional in Density Functional Theory},
  url = {<Go to ISI>://A1986A369700051}
}

@ARTICLE{Yang855412,
  author = {Yang, W. and Lee, C. and Ghosh, S. K.},
  title = {Molecular Softness as the Average of Atomic Softnesses - Companion
	Principle to the Geometric Mean Principle for Electronegativity Equalization},
  journal = {Journal of Physical Chemistry},
  year = {1985},
  volume = {89},
  pages = {5412-5414},
  number = {25},
  endnotereftype = {Journal Article},
  issn = {0022-3654},
  shorttitle = {Molecular Softness as the Average of Atomic Softnesses - Companion
	Principle to the Geometric Mean Principle for Electronegativity Equalization},
  url = {<Go to ISI>://A1985AVP2500019}
}

@ARTICLE{Yang865708,
  author = {Yang, W. and Mortier, W. J.},
  title = {The Use of Global and Local Molecular-Parameters for the Analysis
	of the Gas-Phase Basicity of Amines},
  journal = {Journal of the American Chemical Society},
  year = {1986},
  volume = {108},
  pages = {5708-5711},
  number = {19},
  month = {Sep},
  endnotereftype = {Journal Article},
  issn = {0002-7863},
  shorttitle = {The Use of Global and Local Molecular-Parameters for the Analysis
	of the Gas-Phase Basicity of Amines},
  url = {<Go to ISI>://A1986E058400008}
}

@ARTICLE{Yang842862,
  author = {Yang, W. and Parr, R. G. and Pucci, R.},
  title = {Electron-Density, Kohn-Sham Frontier Orbitals, and Fukui Functions},
  journal = {Journal of Chemical Physics},
  year = {1984},
  volume = {81},
  pages = {2862-2863},
  number = {6},
  endnotereftype = {Journal Article},
  issn = {0021-9606},
  shorttitle = {Electron-Density, Kohn-Sham Frontier Orbitals, and Fukui Functions},
  url = {<Go to ISI>://A1984TJ82200048}
}

@ARTICLE{Yang87191,
  author = {Yang, W. and Parr, R. G. and Uytterhoeven, L.},
  title = {New Relation between Hardness and Compressibility of Minerals},
  journal = {Physics and Chemistry of Minerals},
  year = {1987},
  volume = {15},
  pages = {191-195},
  number = {2},
  endnotereftype = {Journal Article},
  issn = {0342-1791},
  shorttitle = {New Relation between Hardness and Compressibility of Minerals},
  url = {<Go to ISI>://A1987L016700012}
}

@ARTICLE{Yang90522,
  author = {Yang, W. and Peet, A. C.},
  title = {A Method for Calculating Vibrational Bound-States - Iterative Solution
	of the Collocation Equations Constructed from Localized Basis-Sets},
  journal = {Journal of Chemical Physics},
  year = {1990},
  volume = {92},
  pages = {522-526},
  number = {1},
  month = {Jan},
  endnotereftype = {Journal Article},
  issn = {0021-9606},
  shorttitle = {A Method for Calculating Vibrational Bound-States - Iterative Solution
	of the Collocation Equations Constructed from Localized Basis-Sets},
  url = {<Go to ISI>://A1990CH55200060}
}

@ARTICLE{Yang897537,
  author = {Yang, W. and Peet, A. C. and Miller, W. H.},
  title = {A Collocation Approach for Quantum Scattering Based on the S-Matrix
	Version of the Kohn Variational Principle},
  journal = {Journal of Chemical Physics},
  year = {1989},
  volume = {91},
  pages = {7537-7542},
  number = {12},
  month = {Dec},
  endnotereftype = {Journal Article},
  issn = {0021-9606},
  shorttitle = {A Collocation Approach for Quantum Scattering Based on the S-Matrix
	Version of the Kohn Variational Principle},
  url = {<Go to ISI>://A1989CD88000024}
}

@INCOLLECTION{Yang93367,
  author = {Yang, W. T.},
  title = {Density-functional theory of large systems: a divide-and-conquer
	approach},
  booktitle = {Condensed-Matter Theories. Vol 8},
  publisher = {Plenum Press},
  year = {1993},
  editor = {Blum, L. and Malik, F. B.},
  pages = {367-372},
  address = {Berlin},
  endnotereftype = {Book Section},
  shorttitle = {Density-functional theory of large systems: a divide-and-conquer approach}
}

@INCOLLECTION{Yang87499,
  author = {Yang, W. T.},
  title = {Some Remarks on Scaling Relations in Density-Functional Theory},
  booktitle = {Density Matrices and Density-Functionals},
  publisher = {D. Reidel Publishing Company},
  year = {1987},
  editor = {Erdahl, R. and V. H. Smith, Jr.},
  pages = {499--506},
  address = {Dordrecht, Holland},
  endnotereftype = {Book Section},
  shorttitle = {Some Remarks on Scaling Relations in Density-Functional Theory}
}

@INCOLLECTION{Yang90293,
  author = {Yang, W. T.},
  title = {Integral Formulation of Density-Functional Theory},
  booktitle = {Density Functional Theory of Many-Fermion Systems},
  year = {1990},
  editor = {Trickey, Samuel B.},
  volume = {21},
  pages = {293},
  note = {Invited paper},
  endnotereftype = {Book Section},
  shorttitle = {Integral Formulation of Density-Functional Theory}
}

@ARTICLE{Yang9810107,
  author = {Yang, W. T.},
  title = {Generalized adiabatic connection in density functional theory},
  journal = {Journal of Chemical Physics},
  year = {1998},
  volume = {109},
  pages = {10107-10110},
  number = {23},
  month = {Dec},
  abstract = {A generalized adiabatic connection is developed for density functional
	theory. The method extends the well-known adiabatic connection formula
	and provides a general link between the Kohn-Sham and the physical
	system. When the complimentary error function is used as a special
	case, the expression for the exchange-correlation functional does
	not have the 1/r(12) Coulomb component. The exact contributions from
	the physical system and the noninteracting system are established:
	The physical system limit has a dominant contribution, while the
	noninteracting system limit has no contribution. (C) 1998 Americnn
	Instifrrte of Physics. [S0021-9606(98)30647-9].},
  endnotereftype = {Journal Article},
  issn = {0021-9606},
  shorttitle = {Generalized adiabatic connection in density functional theory},
  url = {<Go to ISI>://000077469200001}
}

@ARTICLE{Yang979294,
  author = {Yang, W. T.},
  title = {Absolute-energy-minimum principles for linear-scaling electronic-structure
	calculations},
  journal = {Physical Review B},
  year = {1997},
  volume = {56},
  pages = {9294-9297},
  number = {15},
  month = {Oct},
  abstract = {Two absolute energy minimum principles are developed for first-principle
	linear-scaling electronic structure calculations. One is with a normalization
	constraint and the other without any constraint. The density matrix
	is represented by a set of nonorthogonal localized orbitals and an
	auxiliary matrix which at the minimum becomes a generalized inverse
	of the overlap matrix of the localized orbitals. The number of localized
	orbitals is allowed to exceed the number of occupied orbitals. Comparison
	with other variational principles is made and numerical tests presented.},
  endnotereftype = {Journal Article},
  issn = {0163-1829},
  shorttitle = {Absolute-energy-minimum principles for linear-scaling electronic-structure
	calculations},
  url = {<Go to ISI>://A1997YC39100030}
}

@ARTICLE{Yang92461,
  author = {Yang, W. T.},
  title = {Electron-Density as the Basic Variable - a Divide-and-Conquer Approach
	to the Abinitio Computation of Large Molecules},
  journal = {Theochem-Journal of Molecular Structure},
  year = {1992},
  volume = {87},
  pages = {461-479},
  month = {Mar},
  abstract = {A recently developed approach for calculations of ground states of
	many-electron systems is described. The method is based on density-functional
	theory. It uses the electron density as the basic computational variable
	and does not invoke molecular orbitals. A divide-and-conquer strategy
	is employed: a large system is first divided into subsystems in the
	physical space, then the densities of subsystems are calculated separately,
	and finally the total energy and the electron density are obtained
	as the sums of subsystem contributions. Various molecular calculations
	are presented to show that the new method is capable of describing
	electronic structure with accuracy comparable to the Kohn-Sham orbital
	approach. The method is expected to enable efficient first-principle
	calculations of large molecules beyond the reach of conventional
	approaches. Analysis is presented to address the physics underlying
	the method, the relation of the method to the traditional Thomas-Fermi-type
	theory, the effect of molecular symmetry, the scaling of computational
	effort, and the suitability for parallel computation.},
  endnotereftype = {Journal Article},
  issn = {0166-1280},
  shorttitle = {Electron-Density as the Basic Variable - a Divide-and-Conquer Approach
	to the Abinitio Computation of Large Molecules},
  url = {<Go to ISI>://A1992HM94900024}
}

@ARTICLE{WeitaoYang:1991,
  author = {Yang, W. T.},
  title = {Direct calculation of electron density in density-functional theory},
  journal = {Physical Review Letters},
  year = {1991},
  volume = {66},
  pages = {1438 -- 1441}
}

@ARTICLE{Yang911208,
  author = {Yang, W. T.},
  title = {A Local Projection Method for the Linear Combination of Atomic Orbital
	Implementation of Density-Functional Theory},
  journal = {Journal of Chemical Physics},
  year = {1991},
  volume = {94},
  pages = {1208-1214},
  number = {2},
  month = {Jan},
  abstract = {A local projection method is proposed for obtaining the solution of
	the Kohn-Sham equation within the density-functional theory of molecules.
	The method uses the conventional linear combination of atomic orbitals
	as the approximate orbitals. However, it does not require multicenter
	integration in the construction of algebraic eigenvalue equations,
	and thus significantly reduces the corresponding computational effort.
	The method is tested on the self-consistent calculations of nitrogen
	molecules, N2, with basis sets of various accuracies and found to
	give results which are as accurate as the conventional approach.
	It is also shown that the local projection method can be applied
	to the non-self-consistent calculation scheme and provides a most
	efficient method for carrying out this type of electronic structure
	calculations.},
  endnotereftype = {Journal Article},
  issn = {0021-9606},
  shorttitle = {A Local Projection Method for the Linear Combination of Atomic Orbital
	Implementation of Density-Functional Theory},
  url = {<Go to ISI>://A1991EU59200043}
}

@ARTICLE{Yang911438,
  author = {Yang, W. T.},
  title = {Direct Calculation of Electron-Density in Density-Functional Theory},
  journal = {Physical Review Letters},
  year = {1991},
  volume = {66},
  pages = {1438-1441},
  number = {11},
  month = {Mar},
  abstract = {A new approach for the study of ground states of many-electron systems
	is developed via direct calculation of the density in density-functional
	theory. Not using the Kohn-Sham equations, the method divides a system
	into subsystems in physical space and determines the density for
	each subsystem. The method is demonstrated with calculations for
	the nitrogen molecule, which is divided into two atomic subsystems.
	We expect this approach to enable calculations for large molecules
	beyond the reach of conventional methods.},
  endnotereftype = {Journal Article},
  issn = {0031-9007},
  shorttitle = {Direct Calculation of Electron-Density in Density-Functional Theory},
  url = {<Go to ISI>://A1991FB93700015}
}

@ARTICLE{Yang917823,
  author = {Yang, W. T.},
  title = {Direct Calculation of Electron-Density in Density-Functional Theory
	- Implementation for Benzene and a Tetrapeptide},
  journal = {Physical Review A},
  year = {1991},
  volume = {44},
  pages = {7823-7826},
  number = {11},
  month = {Dec},
  abstract = {A recently developed approach for the direct calculation of electron
	density is implemented for polyatomic molecules: benzene and a tetrapeptide
	with four glycine residues. The method uses the density as the basic
	variable, divides a system into subsystems, and determines the density
	for each subsystem. It is found that the method is capable of describing
	the electronic structure with accuracy comparable to the Kohn-Sham
	method. This substantiates the hope for ab initio calculations of
	large systems beyond the reach of conventional methods.},
  endnotereftype = {Journal Article},
  issn = {1050-2947},
  shorttitle = {Direct Calculation of Electron-Density in Density-Functional Theory
	- Implementation for Benzene and a Tetrapeptide},
  url = {<Go to ISI>://A1991GU88200088}
}

@ARTICLE{Yang885494,
  author = {Yang, W. T.},
  title = {Abinitio Approach for Many-Electron Systems without Invoking Orbitals
	- an Integral Formulation of Density-Functional Theory},
  journal = {Physical Review A},
  year = {1988},
  volume = {38},
  pages = {5494-5503},
  number = {11},
  month = {Dec},
  endnotereftype = {Journal Article},
  isinote = {ISI Document Delivery No.: R2342 Times Cited: 13 Cited Reference Count:
	47},
  issn = {1050-2947},
  shorttitle = {Abinitio Approach for Many-Electron Systems without Invoking Orbitals
	- an Integral Formulation of Density-Functional Theory},
  url = {<Go to ISI>://A1988R234200004}
}

@ARTICLE{Yang885504,
  author = {Yang, W. T.},
  title = {Thermal-Properties of Many-Electron Systems - an Integral Formulation
	of Density-Functional Theory},
  journal = {Physical Review A},
  year = {1988},
  volume = {38},
  pages = {5504-5511},
  number = {11},
  month = {Dec},
  endnotereftype = {Journal Article},
  isinote = {ISI Document Delivery No.: R2342 Times Cited: 8 Cited Reference Count:
	20},
  issn = {1050-2947},
  shorttitle = {Thermal-Properties of Many-Electron Systems - an Integral Formulation
	of Density-Functional Theory},
  url = {<Go to ISI>://A1988R234200005}
}

@ARTICLE{Yang885512,
  author = {Yang, W. T.},
  title = {Dynamic Linear Response of Many-Electron Systems - an Integral Formulation
	of Density-Functional Theory},
  journal = {Physical Review A},
  year = {1988},
  volume = {38},
  pages = {5512-5519},
  number = {11},
  month = {Dec},
  endnotereftype = {Journal Article},
  isinote = {ISI Document Delivery No.: R2342 Times Cited: 11 Cited Reference Count:
	45},
  issn = {1050-2947},
  shorttitle = {Dynamic Linear Response of Many-Electron Systems - an Integral Formulation
	of Density-Functional Theory},
  url = {<Go to ISI>://A1988R234200006}
}

@ARTICLE{Yang871569,
  author = {Yang, W. T.},
  title = {Abinitio Approach for Many-Electron Systems without Invoking Orbitals
	- an Integral Formulation of Density-Functional Theory},
  journal = {Physical Review Letters},
  year = {1987},
  volume = {59},
  pages = {1569-1572},
  number = {14},
  month = {Oct},
  endnotereftype = {Journal Article},
  issn = {0031-9007},
  shorttitle = {Abinitio Approach for Many-Electron Systems without Invoking Orbitals
	- an Integral Formulation of Density-Functional Theory},
  url = {<Go to ISI>://A1987K210800022}
}

@ARTICLE{Yang864575,
  author = {Yang, W. T.},
  title = {Gradient Correction in Thomas-Fermi Theory},
  journal = {Physical Review A},
  year = {1986},
  volume = {34},
  pages = {4575-4585},
  number = {6},
  month = {Dec},
  endnotereftype = {Journal Article},
  isinote = {ISI Document Delivery No.: E9451 Times Cited: 68 Cited Reference Count:
	61},
  issn = {1050-2947},
  shorttitle = {Gradient Correction in Thomas-Fermi Theory},
  url = {<Go to ISI>://A1986E945100006}
}

@ARTICLE{Yang04146404,
  author = {Yang, W. T. and Ayers, P. W. and Wu, Q.},
  title = {Potential functionals: Dual to density functionals and solution to
	the upsilon-representability problem},
  journal = {Physical Review Letters},
  year = {2004},
  volume = {92},
  pages = {146404},
  number = {14},
  month = {Apr},
  abstract = {A functional of external potentials and its variational principle
	for the ground-state energy is constructed. This potential functional
	formulation is dual to the density functional approach and provides
	a solution to the v-representability problem in the original Hohenberg-Kohn
	theory. A second potential functional for Kohn-Sham noninteracting
	systems establishes the foundation for the optimized effective potential
	approach and results in efficient approaches for ensemble Kohn-Sham
	calculations.},
  endnotereftype = {Journal Article},
  issn = {0031-9007},
  shorttitle = {Potential functionals: Dual to density functionals and solution to
	the upsilon-representability problem},
  url = {<Go to ISI>://000221037500045}
}

@ARTICLE{Yang955674,
  author = {Yang, W. T. and Lee, T. S.},
  title = {A Density-Matrix Divide-and-Conquer Approach for Electronic-Structure
	Calculations of Large Molecules},
  journal = {Journal of Chemical Physics},
  year = {1995},
  volume = {103},
  pages = {5674-5678},
  number = {13},
  month = {Oct},
  abstract = {A density matrix divide-and-conquer method is proposed for electronic
	structure calculation of large molecules. It is based on partition
	of density matrix and thus applicable to both density-functional
	and Hartree-Fock method. Compared to the original formulation with
	electron density, the present method is more efficient and as accurate.
	(C) 1995 American Institute of Physics.},
  endnotereftype = {Journal Article},
  issn = {0021-9606},
  shorttitle = {A Density-Matrix Divide-and-Conquer Approach for Electronic-Structure
	Calculations of Large Molecules},
  url = {<Go to ISI>://A1995RW88100049}
}

@ARTICLE{Yang:1995,
  author = { Yang, W. T. and Lee, T. S.},
  title = {A density matrix divide and conquer approach for electronic structure
	calculations of large molecules},
  journal = {J. Chem. Phys.},
  year = {1995},
  volume = {103},
  pages = {5674-5678 },
  annote = {A density matrix divide and conquer approach for electronic structure
	calculations of large molecules},
  date-added = {2008-09-19 10:28:56 -0500},
  date-modified = {2008-09-19 10:28:56 -0500},
  ty = {JOUR}
}

@ARTICLE{Yang98227,
  author = {Yang, W. T. and Levy, Mel and Trickey, S.},
  title = {Special issue: Symposium on density functional and applications (Part
	{{I}} of II) - Introduction},
  journal = {International Journal of Quantum Chemistry: Symposium},
  year = {1998},
  volume = {69},
  pages = {227--227},
  endnotereftype = {Journal Article},
  shorttitle = {Special issue: Symposium on density functional and applications (Part
	{{I}} of II) - Introduction}
}

@ARTICLE{Yang893504,
  author = {Yang, W. T. and Miller, W. H.},
  title = {Block Lanczos Approach Combined with Matrix Continued-Fraction for
	the S-Matrix Kohn Variational Principle in Quantum Scattering},
  journal = {Journal of Chemical Physics},
  year = {1989},
  volume = {91},
  pages = {3504-3508},
  number = {6},
  month = {Sep},
  endnotereftype = {Journal Article},
  issn = {0021-9606},
  shorttitle = {Block Lanczos Approach Combined with Matrix Continued-Fraction for
	the S-Matrix Kohn Variational Principle in Quantum Scattering},
  url = {<Go to ISI>://A1989AP35500025}
}

@ARTICLE{Yang856723,
  author = {Yang, W. T. and Parr, R. G.},
  title = {Hardness, Softness, and the Fukui Function in the Electronic Theory
	of Metals and Catalysis},
  journal = {Proceedings of the National Academy of Sciences of the United States
	of America},
  year = {1985},
  volume = {82},
  pages = {6723-6726},
  number = {20},
  endnotereftype = {Journal Article},
  isinote = {ISI Document Delivery No.: ATC60 Times Cited: 354 Cited Reference
	Count: 20},
  issn = {0027-8424},
  shorttitle = {Hardness, Softness, and the Fukui Function in the Electronic Theory
	of Metals and Catalysis},
  url = {<Go to ISI>://A1985ATC6000001}
}

@ARTICLE{Yang864586,
  author = {Yang, W. T. and Parr, R. G. and Lee, C. T.},
  title = {Various Functionals for the Kinetic-Energy Density of an Atom or
	Molecule},
  journal = {Physical Review A},
  year = {1986},
  volume = {34},
  pages = {4586-4590},
  number = {6},
  month = {Dec},
  endnotereftype = {Journal Article},
  isinote = {ISI Document Delivery No.: E9451 Times Cited: 21 Cited Reference Count:
	30},
  issn = {1050-2947},
  shorttitle = {Various Functionals for the Kinetic-Energy Density of an Atom or Molecule},
  url = {<Go to ISI>://A1986E945100007}
}

@ARTICLE{Yang8898,
  author = {Yang, W. T. and Peet, A. C.},
  title = {The Collocation Method for Bound Solutions of the Schrodinger-Equation},
  journal = {Chemical Physics Letters},
  year = {1988},
  volume = {153},
  pages = {98-104},
  number = {1},
  month = {Dec},
  endnotereftype = {Journal Article},
  issn = {0009-2614},
  shorttitle = {The Collocation Method for Bound Solutions of the Schrodinger-Equation},
  url = {<Go to ISI>://A1988R312600018}
}

@INCOLLECTION{Yang981496,
  author = {Yang, W. T. and P{\'e}, rez-Jord 'a Jos 'e M.},
  title = {Linear Scaling Methods for Electronic Structure Calculations},
  booktitle = {Encyclopedia of Computational Chemistry},
  publisher = {John Wiley \& Sons},
  year = {1998},
  editor = {Schleyer, P. v R.},
  pages = {1496--1513},
  address = {New York},
  endnotereftype = {Book Section},
  shorttitle = {Linear Scaling Methods for Electronic Structure Calculations}
}

@ARTICLE{Yang02143002,
  author = {Yang, W. T. and Wu, Q.},
  title = {Direct method for optimized effective potentials in density-functional
	theory},
  journal = {Physical Review Letters},
  year = {2002},
  volume = {89},
  pages = {143002},
  number = {14},
  month = {Sep},
  abstract = {The conventional optimized effective potential method is based on
	a difficult-to-solve integral equation. In the new method, this potential
	is constructed as a sum of a fixed potential and a linear combination
	of basis functions. The energy derivatives with respect to the coefficients
	of the linear combination are obtained. This enables calculations
	by optimization methods. Accurate atomic and molecular calculations
	with Gaussian basis sets are presented for exact exchange functionals.
	This efficient and accurate method for the optimized effective potential
	should play an important role in the development and application
	of density functionals.},
  endnotereftype = {Journal Article},
  issn = {0031-9007},
  shorttitle = {Direct method for optimized effective potentials in density-functional
	theory},
  url = {<Go to ISI>://000178087200012}
}

@ARTICLE{Yang005172,
  author = {Yang, W. T. and Zhang, Y. K. and Ayers, P. W.},
  title = {Degenerate ground states and a fractional number of electrons in
	density and reduced density matrix functional theory},
  journal = {Physical Review Letters},
  year = {2000},
  volume = {84},
  pages = {5172-5175},
  number = {22},
  month = {May},
  abstract = {For a linear combination of electron densities of degenerate ground
	states, it is shown that the value of any energy functional is the
	ground state energy, if the energy functional is exact for ground
	state densities, size consistent, and translational invariant. The
	corresponding functional of kinetic and inter action energy is the
	linear combination of the functionals of the degenerate densities.
	Without invoking ensembles, it is shown that the energy functional
	of fractional number electrons is a series of straight lines interpolating
	its values at integers. These results underscore the importance of
	grand canonical ensemble formulation in density functional theory.},
  endnotereftype = {Journal Article},
  issn = {0031-9007},
  shorttitle = {Degenerate ground states and a fractional number of electrons in density
	and reduced density matrix functional theory},
  url = {<Go to ISI>://000087266300036}
}

@INCOLLECTION{Yang94177,
  author = {Yang, W. T. and Zhou, Zhongxiang},
  title = {Electronic Structure of Solid-State Systems via the Divide-and-Conquer
	Method},
  booktitle = {Electronic Functional Theory of Molecules, Clusters, and Solids},
  publisher = {Kluwer Academic Publishers},
  year = {1994},
  editor = {Ellis, D. E.},
  pages = {177-188},
  address = {Dordrecht},
  endnotereftype = {Book Section},
  shorttitle = {Electronic Structure of Solid-State Systems via the Divide-and-Conquer
	Method}
}

@ARTICLE{Yasuda:2008,
  author = {Yasuda, S. and Yamamoto, R.},
  title = {A model for hybrid simulations of molecular dynamics and computational
	fluid dynamics
	
	},
  journal = {Phys. Fluids},
  year = {2008},
  volume = {20},
  pages = { },
  number = {113101}
}

@ARTICLE{Yee,
  author = {Yee, H. C. and Sandham, N. D. and Djomehri, M. J.},
  title = {Low-dissipative high-order shock-capturing methods using characteristic-based
	filters},
  journal = {J. Comput. Phys.},
  year = {1999},
  volume = {150},
  pages = {199--238}
}

@INPROCEEDINGS{yezzi-mennucci:05,
  author = {Yezzi, A.J. and Mennucci, A.},
  title = {Conformal Metrics and True "Gradient Flows" for Curves},
  booktitle = {International Conference on Computer Vision},
  year = {2005},
  pages = {913--919}
}

@ARTICLE{Yoda:2004(a),
  author = {Yoda, T. and Sugita, Y. and Okamoto, Y.},
  title = {{Secondary-structure preferences of force fields for proteins evaluated
	by generalized-ensemble simulations}},
  journal = {Chemical Physics},
  year = {2004},
  volume = {307},
  pages = {269-283},
  number = {2-3}
}

@ARTICLE{Yoda:2004(b),
  author = {Yoda, T. and Sugita, Y. and Okamoto, Y.},
  title = {{Comparisons of force fields for proteins by generalized-ensemble
	simulations}},
  journal = {Chemical Physics Letters},
  year = {2004},
  volume = {386},
  pages = {460-467},
  number = {4-6}
}

@ARTICLE{York948526,
  author = {York, D. and Lu, J. P. and Yang, W. T.},
  title = {Density-Functional Calculations of the Structure and Stability of
	C240},
  journal = {Physical Review B},
  year = {1994},
  volume = {49},
  pages = {8526-8528},
  number = {12},
  month = {Mar},
  abstract = {Density-functional calculations have been performed to determine optimized
	geometries and energies Of C240 using the divide-and-conquer method.
	Six initial geometries were considered, resulting in convergence
	to two optimized configurations. The formation energies of the optimized
	structures are separated by approximately 0.07 eV/carbon atom. The
	lower-energy structure is highly spherical in agreement with preliminary
	studies and experimental observations. The higher-energy structure
	is polyhedrally faceted. The results support the conclusion that
	the most stable form of large carbon clusters is that of dense spherical
	caged structures.},
  endnotereftype = {Journal Article},
  issn = {0163-1829},
  shorttitle = {Density-Functional Calculations of the Structure and Stability of
	C240},
  url = {<Go to ISI>://A1994NG11600085}
}

@ARTICLE{York943298,
  author = {York, D. and Yang, W. T.},
  title = {The Fast Fourier-Poisson Method for Calculating Ewald Sums},
  journal = {Journal of Chemical Physics},
  year = {1994},
  volume = {101},
  pages = {3298-3300},
  number = {4},
  month = {Aug},
  abstract = {The conventional Ewald expression for the electrostatic energy and
	forces is recast in a form that can be evaluated to high accuracy
	in order N log(N) steps using fast Fourier transforms. The fast Fourier
	Poisson method does not rely on interpolation approaches or Taylor/multipole
	expansions, and can be easily integrated with conventional molecular
	dynamics algorithms.},
  endnotereftype = {Journal Article},
  issn = {0021-9606},
  shorttitle = {The Fast Fourier-Poisson Method for Calculating Ewald Sums},
  url = {<Go to ISI>://A1994PA00900071}
}

@ARTICLE{York985011,
  author = {York, D. M. and Lee, T. S. and Yang, W. T.},
  title = {Quantum mechanical treatment of biological macromolecules in solution
	using linear-scaling electronic structure methods},
  journal = {Physical Review Letters},
  year = {1998},
  volume = {80},
  pages = {5011-5014},
  number = {22},
  month = {Jun},
  abstract = {A linear-scaling self-consistent field method for calculation of the
	electronic structure of biological macromolecules in solution is
	presented. The method is applied at the semiempirical Hartree-Fock
	level to the determination of heats of formation, solvation free
	energies, and density of electronic states for several protein and
	DNA systems.},
  endnotereftype = {Journal Article},
  issn = {0031-9007},
  shorttitle = {Quantum mechanical treatment of biological macromolecules in solution
	using linear-scaling electronic structure methods},
  url = {<Go to ISI>://000073915100045}
}

@ARTICLE{York9610940,
  author = {York, D. M. and Lee, T. S. and Yang, W. T.},
  title = {Quantum mechanical study of aqueous polarization effects on biological
	macromolecules},
  journal = {Journal of the American Chemical Society},
  year = {1996},
  volume = {118},
  pages = {10940-10941},
  number = {44},
  month = {Nov},
  endnotereftype = {Journal Article},
  issn = {0002-7863},
  shorttitle = {Quantum mechanical study of aqueous polarization effects on biological
	macromolecules},
  url = {<Go to ISI>://A1996VR41900052}
}

@ARTICLE{York96297,
  author = {York, D. M. and Lee, T. S. and Yang, W. T.},
  title = {Parameterization and efficient implementation of a solvent model
	for linear-scaling semiempirical quantum mechanical calculations
	of biological macromolecules},
  journal = {Chemical Physics Letters},
  year = {1996},
  volume = {263},
  pages = {297-304},
  number = {1-2},
  month = {Dec},
  abstract = {A method is developed to include solvation effects in linear-scaling
	semiempirical quantum calculations. Favorable molecules is achieved
	using a preconditioned conjugate gradient technique in conjunction
	with a linear-scaling recursive bisection method for evaluation of
	electrostatic interactions. The method requires approximately 30%
	computational overhead relative to gas-phase calculations. Effective
	atomic radii for biological macromolecules are derived from fitting
	to experimental and theoretical solvation energies for small molecules
	homologous to amino- and nucleic acid residues.},
  endnotereftype = {Journal Article},
  issn = {0009-2614},
  shorttitle = {Parameterization and efficient implementation of a solvent model for
	linear-scaling semiempirical quantum mechanical calculations of biological
	macromolecules},
  url = {<Go to ISI>://A1996VW24400047}
}

@ARTICLE{York96159,
  author = {York, D. M. and Yang, W. T.},
  title = {A chemical potential equalization method for molecular simulations},
  journal = {Journal of Chemical Physics},
  year = {1996},
  volume = {104},
  pages = {159-172},
  number = {1},
  month = {Jan},
  abstract = {A formulation of the chemical potential (electronegativity)equalization
	principle is presented from the perspective of density-functional
	theory. The resulting equations provide a linear-response framework
	for describing the redistribution of electrons upon perturbation
	by an applied field. The method has two main advantages over existing
	electronegativity equalization and charge equilibration methods that
	allow extension to accurate molecular dynamics simulations. Firstly,
	the expansion of the energy is taken about the molecular ground state
	instead of the neutral atom ground states; hence, in the absence
	of an external field, the molecular charge distribution can be represented
	by static point charges and dipoles obtained from fitting to high-level
	ab initio calculations without modification. Secondly, in the presence
	of applied fields or interactions with other molecules, the density
	response can be modeled accurately using basis functions. Inclusion
	of basis functions with dipolar or higher order multipolar character
	allows molecules or chemical groups to have correct Ideal anisotropic
	polarizabilities. A modified semiempirical form of the hardness matrix
	has been introduced that can be evaluated efficiently using Gaussians,
	and requires only one parameter per basis function. Applications
	at two basis-set levels demonstrate the method can accurately reproduce
	induced dipole moments and estimated chemical potentials obtained
	from density-functional calculations for a variety of molecules.
	Inclusion of basis functions beyond the conventional spherical-atom
	type is essential in some instances. The present formulation provides
	the foundation for a promising semi-empirical model for polarization
	and charge transfer in molecular simulations. (C) 1996 American Institute
	of Physics.},
  endnotereftype = {Journal Article},
  issn = {0021-9606},
  shorttitle = {A chemical potential equalization method for molecular simulations},
  url = {<Go to ISI>://A1996TN53000019}
}

@ARTICLE{York955001,
  author = {York, D. M. and Yang, W. T. and Lee, H. and Darden, T. and Pedersen,
	L. G.},
  title = {Toward the Accurate Modeling of DNA - the Importance of Long-Range
	Electrostatics},
  journal = {Journal of the American Chemical Society},
  year = {1995},
  volume = {117},
  pages = {5001-5002},
  number = {17},
  month = {May},
  endnotereftype = {Journal Article},
  issn = {0002-7863},
  shorttitle = {Toward the Accurate Modeling of DNA - the Importance of Long-Range
	Electrostatics},
  url = {<Go to ISI>://A1995QW14000034}
}

@ARTICLE{YYou:2002,
  author = {You, Y.L. and Kaveh, M.},
  title = {{Fourth-order partial differential equations for noise removal}},
  journal = {{IEEE} Transactions on Image Processing},
  year = {2002},
  volume = {9},
  pages = {1723--1730},
  number = {10},
  issn = {1057-7149},
  publisher = {{IEEE}}
}

@ARTICLE{ShapeSpace2,
  author = {Laurent Younes},
  title = {Optimal Matching Between Shapes via Elastic Deformations},
  journal = {Image \& Vision Comp.},
  year = {1999},
  volume = {17},
  pages = {381-389},
  number = {5}
}

@ARTICLE{BinYu:2002,
  author = {Yu, Bin and Chang, L. and Ahmed, S. and Wang, H. H. and Bell, S.
	and Yang, C.Y. and Tabery, C. and Ho, C. and Xiang, Q. and King,
	T.J. and Bokor, J. and Hu, C.M. and Lin, M.R. and Kyser, D.},
  title = {FinFET scaling to 10 nm gate length},
  journal = {IEDM Tech. Dig.},
  year = {2002},
  pages = {251-254}
}

@ARTICLE{BinYu:1997,
  author = {Yu, B. and Wann, C. H. J. and Nowak, E. D. and Noda, K. and Hu, C.
	M.},
  title = {Short-channel effect improved by lateral channel-engineering in deep-submicronmeter
	MOSFET's},
  journal = {IEEE TRANSACTIONS ON ELECTRON DEVICES },
  year = {1997},
  volume = {44},
  pages = {627-634}
}

@ARTICLE{Yu,
  author = {Yu, S. N. and Zhao, S. and Wei, G. W.},
  title = { Local spectral time splitting method for first and second order
	partial differential equations},
  journal = {J. Comput. Phys.},
  year = {2005},
  volume = {206},
  pages = {727--780}
}

@ARTICLE{Yuthesis:2007,
  author = {Yu, S. N.},
  title = {Matched Interface and Boundary ({MIB}) Method for Geometric Singularities
	and Its Application to Molecular Biology and Structural Analysis},
  year = {2007},
  note = {Dissertation of Michigan State University}
}

@ARTICLE{Yu:2007,
  author = {Yu, S. N. and Geng, W. H. and Wei, G. W.},
  title = {Treatment of geometric singularities in implicit solvent models},
  journal = {Journal of Chemical Physics},
  year = {2007},
  volume = {126},
  pages = {244108},
  abstract = {Geometric singularities, such as cusps and self-intersecting surfaces,
	are major obstacles to the accuracy, convergence, and stability of
	the numerical solution of the {Poisson-Boltzmann} (PB) equation.
	In earlier work, an interface technique based PB solver was developed
	using the matched interface and boundary {(MIB)} method, which explicitly
	enforces the flux jump condition at the solvent-solute interfaces
	and leads to highly accurate biomolecular electrostatics in continuum
	electric environments. However, such a PB solver, denoted as {MIBPB}-I,
	cannot maintain the designed second order convergence whenever there
	are geometric singularities, such as cusps and self-intersecting
	surfaces. Moreover, the matrix of the {MIBPB}-I is not optimally
	symmetrical, resulting in the convergence difficulty. The present
	work presents a new interface method based PB solver, denoted as
	{MIBPB}-II, to address the aforementioned problems. The present MIBPB-II
	solver is systematical and robust in treating geometric singularities
	and delivers second order convergence for arbitrarily complex molecular
	surfaces of proteins. A new procedure is introduced to make the MIBPB-II
	matrix optimally symmetrical and diagonally dominant. The MIBPB-II
	solver is extensively validated by the molecular surfaces of few-atom
	systems and a set of 24 proteins. Converged electrostatic potentials
	and solvation free energies are obtained at a coarse grid spacing
	of 0.5 Ã-and are considerably more accurate than those obtained
	by the PBEQ and the APBS at finer grid spacings.},
  bdsk-url-1 = {http://dx.doi.org/10.1063/1.2743020},
  date-added = {2008-06-30 11:38:02 -0500},
  date-modified = {2008-06-30 11:38:02 -0500},
  keywords = {Solvation; Mathematics},
  url = {http://dx.doi.org/10.1063/1.2743020}
}

@ARTICLE{Yu:2007a,
  author = {Yu, S. N. and Wei, G. W.},
  title = {Three-dimensional matched interface and boundary {(MIB)} method for
	treating geometric singularities},
  journal = {J. Comput. Phys.},
  year = {2007},
  volume = {227},
  pages = {602-632},
  abstract = {Thispaperreportsthethree-dimensional (3D)generalizationof ourprevious2Dhigher-ordermatched
	interfaceandboundary{(MIB)} methodfor solvingellipticequations withdiscontinuous
	coefficients and non-smoothinterfaces. NewMIBalgorithmsthatmakeuseof
	twosetsof interfacejumpconditionsare proposedtoremovethecriticalacuteangleconstraintofourearlierMIBschemefortreatinginterfaceswith
	sharpgeometricsingularities, suchassharpedges, sharpwedgesandsharptips.
	Theresulting3DMIB schemesareof second-orderaccuracyforarbitrarilycomplexinterfaceswithsharpgeometricsingularities,
	of fourth-orderaccuracyforcomplexinterfaceswithmoderategeometricsingularities,
	andof sixth-order accuracyforcurvedsmoothinterfaces. Asystematical
	procedureisintroducedtomaketheMIBmatrix optimallysymmetricandbandedbyappropriatelychoosingauxiliarygridpoints.
	Consequently, thenew MIBlinearalgebraicequationscanbesolvedwithfewernumberof
	iterations. TheproposedMIBmethod makes useof Cartesiangrids, standardfinitedifferenceschemes,
	lowest-order interfacejumpconditions andfictitiousvalues. Theinterfacejumpconditionsareenforcedateachintersectingpointoftheinterface
	andmeshlinestoovercomethestaircasephenomenainfinitedifferenceapproximation.
	Whileapairof fictitiousvaluesaredeterminedalongameshatatime, aniterativeprocedureisproposedtodetermineall
	therequiredfictitiousvaluesforhigher-orderschemesbyrepeatedlyusingthelowestorderjumpconditions.
	Avarietyof MIBtechniquesaredevelopedtoovercomegeometricconstraints.
	Theessential strategyof theMIBmethodistolocallyreducea2Dora3Dinterfaceprobleminto1D-likeones.
	TheproposedMIB methodisextensivelyvalidatedintermsof theorderof accuracy,
	thespeedof convergence, thenumber of iterationsandCPUtime. Numerical
	experimentsarecarriedouttocomplexinterfaces, includingthe molecularsurfacesof
	aprotein, amissileinterface, andvanderWaalssurfacesof intersectingspheres.},
  bdsk-url-2 = {http://dx.doi.org/10.1016/j.jcp.2007.08.003},
  date-added = {2008-06-30 11:34:20 -0500},
  date-modified = {2008-06-30 11:34:20 -0500},
  doi = {10.1016/j.jcp.2007.08.003},
  keywords = {electrostatics; mathematics},
  url = {http://www.sciencedirect.com/science/article/B6WHY-4PF1WN4-1/2/a142bb0596d6f227a0537b4790d00bcf}
}


@ARTICLE{SNYu:2009,
  author = {Yu, S. N. and Xiang, Y. and Wei, G. W.},
  title = {Matched interface and boundary (MIB) method for the vibration analysis
	of plates },
  journal = { Commun. Numer. Methods Engng},
  year = {2009},
  volume = {25},
  pages = {923-950}
}

@ARTICLE{Yu:2005b,
  author = {Yu, S. N. and Zhao, Shan and Wei, G. W. },
  title = {Local spectral time splitting method for first- and second-order
	partial differential equations},
  journal = {J. Comput. Phys.},
  year = {2005},
  volume = {206},
  pages = {727--780},
  number = {2},
  abstract = {A family of local spectral evolution kernels (LSEKs) are derived for
	analytically integrating a class of partial differential equations
	(PDEs)The LSEK can solve the above PDEs with x-independent coefficients
	in a single step. They are utilized in operator splitting schemes
	to arrive at a local spectral time-splitting (LSTS) method for solving
	more general linear and/or nonlinear PDEs. Like previous local spectral
	methods, this new method is of controllable accuracy in both spatial
	and temporal discretizations, and it can be of spectral accuracy
	in space and arbitrarily high-order accuracy in time. Its complexity
	scales as O(N) at a fixed level of accuracy. It is explicit, time
	transverse invariant, unconditionally stable for many problems whose
	two split parts are both analytically integrable. It adopts uniform
	grid meshes. The proposed method is extensively validated in terms
	of accuracy, stability, efficiency, robustness and reliability by
	the Fokker-Planck equation, the Black-Scholes equation, the heat
	equation, the plane wave propagation, the Zakharov system, and a
	linear harmonic oscillator. Numerical applications are considered
	to Fisher's equation, the generalized nonlinear Schr\"{o}dinger equation,
	the Bose-Einstein condensates, and the Schr\"{o}dinger equation in
	the semi-classical regime. Numerical results compare well with those
	in the literature.},
  bdsk-url-1 = {http://dx.doi.org/10.1016/j.jcp.2005.01.010},
  date-added = {2008-06-30 22:11:23 -0400},
  date-modified = {2008-06-30 22:11:23 -0400},
  doi = {10.1016/j.jcp.2005.01.010},
  keywords = {kinetics, mathematics, molecular\_dynamics},
  posted-at = {2008-07-01 03:10:54},
  priority = {0},
  url = {http://dx.doi.org/10.1016/j.jcp.2005.01.010}
}

@ARTICLE{Yu:2007c,
  author = {Yu, S. N. and Zhou, Y. C. and Wei, G. W. },
  title = {Matched interface and boundary ({MIB}) method for elliptic problems
	with sharp-edged interfaces},
  journal = {J. Comput. Phys.},
  year = {2007},
  volume = {224},
  pages = {729--756},
  number = {2},
  abstract = {Elliptic problems with sharp-edged interfaces, thin-layered interfaces
	and interfaces that intersect with geometric boundary, are notoriously
	challenging to existing numerical methods, particularly when the
	solution is highly oscillatory. This work generalizes the matched
	interface and boundary {(MIB)} method previously designed for solving
	elliptic problems with curved interfaces to the aforementioned problems.
	We classify these problems into five distinct topological relations
	involving the interfaces and the Cartesian mesh lines. Flexible strategies
	are developed to systematically extends the computational domains
	near the interface so that the standard central finite difference
	scheme can be applied without the loss of accuracy. Fictitious values
	on the extended domains are determined by enforcing the physical
	jump conditions on the interface according to the local topology
	of the irregular point. The concepts of primary and secondary fictitious
	values are introduced to deal with sharp-edged interfaces. For corner
	singularity or tip singularity, an appropriate polynomial is multiplied
	to the solution to remove the singularity. Extensive numerical experiments
	confirm the designed second order convergence of the proposed method.},
  bdsk-url-1 = {http://dx.doi.org/10.1016/j.jcp.2006.10.030},
  date-added = {2008-06-30 21:31:42 -0400},
  date-modified = {2008-06-30 21:31:42 -0400},
  doi = {10.1016/j.jcp.2006.10.030},
  keywords = {electrostatics, mathematics, solvation},
  posted-at = {2008-07-01 02:31:14},
  priority = {0},
  url = {http://dx.doi.org/10.1016/j.jcp.2006.10.030}
}

@ARTICLE{Yu:2008g,
  author = {Yu, Z. Y. and Bajaj, C.},
  title = {Computational approaches for automatic structural analysis of large
	biomolecular complexes},
  journal = {IEEE/ACM Trans Comput Biol Bioinform },
  year = {2008},
  volume = {5},
  pages = {568-582 },
  annote = {Computational approaches for automatic structural analysis of large
	biomolecular complexes},
  date-added = {2009-03-10 },
  date-modified = {2009-03-10},
  ty = {JOUR}
}

@ARTICLE{Yu:2005g,
  author = {Yu, Z. Y. and Bajaj, C.},
  title = {Automatic ultrastructure segmentation of reconstructed cryoEM maps
	of icosahedral viruses},
  journal = {IEEE Trans Image Process},
  year = {2005},
  volume = {14},
  pages = {1324-1337 },
  annote = {Automatic ultrastructure segmentation of reconstructed cryoEM maps
	of icosahedral viruses},
  date-added = {2009-03-10 },
  date-modified = {2009-03-10},
  ty = {JOUR}
}

@ARTICLE{ZYu:2008,
  author = {Yu, Z. Y. and Holst, M. and Cheng, Y. and McCammon, J. A. },
  title = {Feature-Preserving Adaptive Mesh Generation for Molecular Shape Modeling
	and Simulation
	},
  journal = { Journal of Molecular Graphics and Modeling },
  year = {2008},
  volume = {26},
  pages = {1370-1380}
}

   %author = {Yu, Z. and Holst, M. and  Hayashi, T. and Bajaj, C. L. and Ellisman, M. H. and McCammon, J. A. and Hoshijima, M.},
@ARTICLE{ZYu:2008b,
   author = {Yu, Z. and Holst, M. and  Hayashi, T. and Bajaj, C. L. and Ellisman, M. H. and McCammon, J. A. and Hoshijima, M.},
   title = {Three-Dimensional Geometric Modeling of Membrane-bound Organelles in Ventricular Myocytes: Bridging the Gap between Microscopic Imaging and Mathematical Simulation},
  journal = { Journal of Structural Biology },
  year = {2008},
  volume = {164},
  pages = {304-313}
}


@ARTICLE{Zacharias:2003,
  author = {Zacharias, M.},
  title = {Continuum Solvent Modeling of Nonpolar Solvation: Improvement by
	Separating Surface Area Dependent Cavity and Dispersion Contributions},
  journal = {Journal of Physical Chemistry A},
  year = {2003},
  volume = {107},
  pages = {3000-3004},
  number = {16},
  abstract = {Continuum models are frequently used to calculate hydration properties
	of organic and biomolecules and to estimate its dependence on conformation
	and association. Often a single surface tension parameter has been
	used to estimate nonpolar solvation contributions from the solvent
	accessible surface of a molecule. The assumption of a uniform surface
	tension parameter is based on the observation that for linear alkanes
	free energies of hydration (vacuum to water transfer free energies)
	increase (approximately) linearly with the solvent accessible surface
	area (SAS). However, this correlation for example does not hold for
	the vacuum to water transfer of cyclic alkanes. The transfer of a
	nonpolar solute from vacuum to water can be formally split into a
	contribution due to cavity formation which involves a redistribution
	and reordering of water molecules and changes in water-water interaction
	and second {van der Waals} (dispersion) interactions between solute
	and water. In the present study, the solute solvent dispersion contribution
	has been calculated using a surface integral continuum approach (Floris,
	F.; Tomasi, J. J. Comput. Chem. 1989, 10, 616-627). Combined with
	a cavity contribution that has been assumed to be proportional to
	the solvent accessible surface area calculated hydration free energies
	for linear, branched and cyclic alkanes are in significantly better
	agreement with experiment than using a pure SAS model. In addition,
	the calculated changes of hydration free energies upon alkane conformational
	changes agree much better with results of explicit solvent simulations
	compared to a model that employs a single surface tension parameter.},
  annote = {Continuum Solvent Modeling of Nonpolar Solvation: Improvement by
	Separating Surface Area Dependent Cavity and Dispersion Contributions;
	ZachariasIntegral; This article discusses the importance of including
	dispersion ({van der Waals}) interactions in addition to the cavity-related
	surface area terms. The author develops a new apolar hydration model
	based on this argument and shows that it generates much better agreement
	with explicit solvent simulations.},
  bdsk-url-1 = {http://dx.doi.org/10.1021/jp027598c},
  date-added = {2008-08-29 15:52:06 -0500},
  date-modified = {2008-08-29 15:52:06 -0500},
  keywords = {Electrostatics; Solvation; Nonpolar},
  ty = {JOUR},
  url = {http://dx.doi.org/10.1021/jp027598c}
}

@ARTICLE{Zagrovic:2002,
  author = {Zagrovic, B. and Snow, C. D. and Shirts, M. R. and Pande, V. S.},
  title = {{Simulation of folding of a small alpha-helical protein in atomistic
	detail using worldwide-distributed computing}},
  journal = {J Mol Biol},
  year = {2002},
  volume = {323},
  pages = {927-937},
  number = {5}
}

@ARTICLE{Zaslavsky:1994,
  author = {Zaslavsky,G.},
  title = {Fractional kinetic equation for Hamiltonian chaos.Chaotic advection,
	tracer dynamics and turbulent dispersion},
  journal = {Phys.D},
  year = {1994},
  volume = {76},
  pages = {110?C122},
  number = { }
}

@ARTICLE{Zauhar:1985,
  author = {Zauhar, R. J. and Morgan, R. S.},
  title = {A new method for computing the macromolecular electric potential},
  journal = {Journal of Molecular Biology},
  year = {1985},
  volume = {186},
  pages = {815-20},
  number = {4},
  abstract = {A general methodology is developed for the rigorous computation of
	the electrostatic potential for a protein of arbitrary shape, assuming
	the presence of linear dielectric media. The theory proceeds by considering
	the distribution of induced polarization charge at the dielectric
	interface, rather than by attempting a direct solution of Poisson's
	equation (as in the finite-difference approach of Warwicker \& Watson).
	The method is applied to a study of two-dimensional model proteins,
	where it is shown that the presence of a cleft is associated with
	a region of relatively high potential in the solvent medium. The
	results of a preliminary calculation in three dimensions for the
	protein lysozyme are also discussed; again, a region of enhanced
	potential is observed near the cleft at the active site. Our computational
	evidence supports the suggestion of Warwicker \& Watson that clefts
	are associated with important electrostatic effects.},
  annote = {Dec 20; A new method for computing the macromolecular electric potential;
	4093987; 0022-2836 Journal Article},
  bdsk-url-1 = {http://www.ncbi.nlm.nih.gov/entrez/query.fcgi?cmd=Retrieve&db=PubMed&dopt=Citation&list_uids=4093987},
  date-added = {2008-06-29 14:53:04 -0500},
  date-modified = {2008-06-29 14:53:04 -0500},
  keywords = {Electrostatics},
  ty = {JOUR},
  url = {http://www.ncbi.nlm.nih.gov/entrez/query.fcgi?cmd=Retrieve&db=PubMed&dopt=Citation&list_uids=4093987}
}

@ARTICLE{zelinka2004sbs,
  author = {Zelinka, S. and Garland, M.},
  title = {{Similarity-based surface modelling using geodesic fans}},
  journal = {Symposium on Geometry Processing},
  year = {2004},
  pages = {204-213}
}

@ARTICLE{Zeng2008x,
  author = {Zeng, X. and Hu, H. and Zhou, H. X. and Marszalek, P. E. and Yang,
	W. T.},
  title = {Direct Calculations of the Potential of Mean Force for Polysaccharides
	with the Replica-Exchange Enhanced Umbrella Sampling Approach},
  year = {2009},
  note = {in preparation}
}

@ARTICLE{Zeng08124510,
  author = {Zeng, X. C. and Hu, H. and Hu, X. Q. and Cohen, A. J. and Yang, W.
	T.},
  title = {Ab initio quantum mechanical/molecular mechanical simulation of electron
	transfer process: Fractional electron approach},
  journal = {Journal of Chemical Physics},
  year = {2008},
  volume = {128},
  pages = {124510},
  number = {12},
  month = {Mar},
  abstract = {Electron transfer (ET) reactions are one of the most important processes
	in chemistry and biology. Because of the quantum nature of the processes
	and the complicated roles of the solvent, theoretical study of ET
	processes is challenging. To simulate ET processes at the electronic
	level, we have developed an efficient density functional theory (DFT)
	quantum mechanical (QM)/molecular mechanical (MM) approach that uses
	the fractional number of electrons as the order parameter to calculate
	the redox free energy of ET reactions in solution. We applied this
	method to study the ET reactions of the aqueous metal complexes Fe(H2O)(6)(2+/3+)
	and Ru(H2O)(6)(2+/3+). The calculated oxidation potentials, 5.82
	eV for Fe(II/III) and 5.14 eV for Ru(II/III), agree well with the
	experimental data, 5.50 and 4.96 eV, for iron and ruthenium, respectively.
	Furthermore, we have constructed the diabatic free energy surfaces
	from histogram analysis based on the molecular dynamics trajectories.
	The resulting reorganization energy and the diabatic activation energy
	also show good agreement with experimental data. Our calculations
	show that using the fractional number of electrons (FNE) as the order
	parameter in the thermodynamic integration process leads to efficient
	sampling and validate the ab initio QM/MM approach in the calculation
	of redox free energies. (C) 2008 American Institute of Physics.},
  endnotereftype = {Journal Article},
  issn = {0021-9606},
  shorttitle = {Ab initio quantum mechanical/molecular mechanical simulation of electron
	transfer process: Fractional electron approach},
  url = {<Go to ISI>://000254537200047}
}

@ARTICLE{Zhang:2004,
  author = {Zhang, D. and Konecny, R. and Baker, N. A. and McCammon, J. A.},
  title = {Electrostatic interaction between {RNA} and protein capsid in cowpea
	chlorotic mottle virus simulated by a coarse-grain {RNA} model and
	a {Monte Carlo} approach},
  journal = {Biopolymers},
  year = {2004},
  volume = {75},
  pages = {325-37},
  number = {4},
  abstract = {Although many viruses have been crystallized and the protein capsid
	structures have been determined by x-ray crystallography, the nucleic
	acids often cannot be resolved. This is especially true for RNA viruses.
	The lack of information about the conformation of DNA/RNA greatly
	hinders our understanding of the assembly mechanism of various viruses.
	Here we combine a coarse-grain model and a Monte Carlo method to
	simulate the distribution of viral RNA inside the capsid of cowpea
	chlorotic mottle virus. Our results show that there is very strong
	interaction between the N-terminal residues of the capsid proteins,
	which are highly positive charged, and the viral RNA. Without these
	residues, the binding energy disfavors the binding of RNA by the
	capsid. The RNA forms a shell close to the capsid with the highest
	densities associated with the capsid dimers. These high-density regions
	are connected to each other in the shape of a continuous net of triangles.
	The overall icosahedral shape of the net overlaps with the capsid
	subunit icosahedral organization. Medium density of RNA is found
	under the pentamers of the capsid. These findings are consistent
	with experimental observations.},
  annote = {Electrostatic interaction between RNA and protein capsid in cowpea
	chlorotic mottle virus simulated by a coarse-grain RNA model and
	a Monte Carlo approach; ZhangEtal2004},
  bdsk-file-1 = {YnBsaXN0MDDUAQIDBAUGCQpYJHZlcnNpb25UJHRvcFkkYXJjaGl2ZXJYJG9iamVjdHMSAAGGoNE
	HCFRyb290gAFfEA9OU0tleWVkQXJjaGl2ZXKoCwwXGBkdJCVVJG51bGzTDQ4PEBEUViRjbGFzc1
	dOUy5rZXlzWk5TLm9iamVjdHOAB6ISE4ACgAOiFRaABIAGWWFsaWFzRGF0YVxyZWxhdGl2ZVBhd
	GjSDRobHFdOUy5kYXRhgAVPEQH0AAAAAAH0AAIAAAxNYWNpbnRvc2ggSEQAAAAAAAAAAAAAAAAA
	AADD4v5NSCsAAAAZYksfMjAwNC1aaGFuZ0tvbmVjbnlCYWsjMTk2MjhELnBkZgAAAAAAAAAAAAA
	AAAAAAAAAAAAAAAAAAAAAAAAAAAAAABlijcNHOFpQREYgcHJ2dwAEAAQAAAkgAAAAAAAAAAAAAA
	AAAAAAB0FyY2hpdmUAABAACAAAw+NSrQAAABEACAAAw0d+qgAAAAEAFAAZYksAGWIDAAqkKAAKp
	BEAAHrcAAIAVU1hY2ludG9zaCBIRDpVc2VyczpiYWtlcjpEb2N1bWVudHM6UmVmZXJlbmNlczpB
	cmNoaXZlOjIwMDQtWmhhbmdLb25lY255QmFrIzE5NjI4RC5wZGYAAA4ARgAiADIAMAAwADQALQB
	aAGgAYQBuAGcASwBvAG4AZQBjAG4AeQBCAGEAawBlAHIATQBjAEMAYQBtAG0AbwBuAC4AcABkAG
	YADwAaAAwATQBhAGMAaQBuAHQAbwBzAGgAIABIAEQAEgBLVXNlcnMvYmFrZXIvRG9jdW1lbnRzL
	1JlZmVyZW5jZXMvQXJjaGl2ZS8yMDA0LVpoYW5nS29uZWNueUJha2VyTWNDYW1tb24ucGRmAAAT
	AAEvAAAVAAIADP//AADSHh8gIVgkY2xhc3Nlc1okY2xhc3NuYW1loyEiI11OU011dGFibGVEYXR
	hVk5TRGF0YVhOU09iamVjdF8QSy4uLy4uLy4uLy4uL0RvY3VtZW50cy9SZWZlcmVuY2VzL0FyY2
	hpdmUvMjAwNC1aaGFuZ0tvbmVjbnlCYWtlck1jQ2FtbW9uLnBkZtIeHyYnoicjXE5TRGljdGlvb
	mFyeQAIABEAGgAfACkAMgA3ADoAPwBBAFMAXABiAGkAcAB4AIMAhQCIAIoAjACPAJEAkwCdAKoA
	rwC3ALkCsQK2Ar8CygLOAtwC4wLsAzoDPwNCAAAAAAAAAgEAAAAAAAAAKAAAAAAAAAAAAAAAAAA
	AA08=},
  bdsk-url-1 = {http://dx.doi.org/10.1002/bip.20120},
  date-added = {2008-09-16 15:49:49 -0500},
  date-modified = {2008-09-16 15:49:49 -0500},
  keywords = {Electrostatics; MolecularSimulation},
  ty = {JOUR},
  url = {http://dx.doi.org/10.1002/bip.20120}
}

@ARTICLE{Zhang:2005,
  author = {Zhang, D. and Suen, J. and Zhang, Y. and Radic, Z. and Taylor, P.
	and Holst, M. and Bajaj, C. and Baker, N. A. and McCammon, J. A.},
  title = {Tetrameric Mouse Acetylcholinesterase: Continuum Diffusion Rate Calculations
	by Solving the Steady-State {Smoluchowski} Equation Using Finite
	Element Methods},
  journal = {Biophysical Journal},
  year = {2005},
  volume = {88},
  pages = {1659-65},
  number = {3}
}

@ARTICLE{wei:1997,
  author = {Zhang, D. S. and Wei, G. W. and Kouri, D. J. and Hoffman, D. K.},
  title = {{{{Burgers}}' equation with high Reynolds number}},
  journal = {Phys. Fluids},
  year = {1997},
  volume = {6},
  pages = {1853--1855}
}

@INPROCEEDINGS{zhang_EG,
  author = {Hao Zhang and Oliver van Kaick and Ramsay Dyer},
  title = {Spectral Methods for Mesh Processing and Analysis},
  booktitle = {Proc. of Eurographics State-of-the-art Report},
  year = {2007},
  pages = {1--22}
}

@ARTICLE{Zhang:2004d,
  author = {Zhang, Hua and Wu, Wei and Du, Yan and Santos, Sarah J. and Conrad,
	Susan E. and Watson, Jack T. and Grammatikakis, Nicholas and Gallo,
	Kathleen A. },
  title = {Hsp90/p50cdc37 Is Required for Mixed-lineage Kinase (MLK) 3 Signaling},
  journal = {Journal of Biological Chemistry},
  year = {2004},
  volume = {279},
  pages = {19457--19463},
  number = {19},
  abstract = {Mixed-lineage kinase 3 (MLK3) is a mitogen-activated protein kinase
	(MAPK) kinase kinase that activates MAPK pathways, including the
	c-Jun NH2-terminal kinase (JNK) and p38 pathways. MLK3 and its family
	members have been implicated in JNK-mediated apoptosis. A survey
	of human cell lines revealed high levels of MLK3 in breast cancer
	cells. To learn more about MLK3 regulation and its signaling pathways
	in breast cancer cells, we engineered the estrogen-responsive human
	breast cancer cell line, MCF-7, to stably, inducibly express FLAG
	epitope-tagged MLK3. FLAG{middle dot}MLK3 complexes were isolated
	by affinity purification, and associated proteins were identified
	by in-gel trypsin digestion followed by liquid chromatography/tandem
	mass spectrometry. Among the proteins identified were heat shock
	protein 90{alpha},{beta} (Hsp90) and its kinase-specific co-chaperone
	p50cdc37. We show that endogenous MLK3 complexes with Hsp90 and p50cdc37.
	Further experiments demonstrate that MLK3 associates with Hsp90/p50cdc37
	through its catalytic domain in an activity-independent manner. Upon
	treatment of MCF-7 cells with geldanamycin, an ansamycin antibiotic
	that inhibits Hsp90 function, MLK3 levels decrease dramatically.
	Furthermore, tumor necrosis factor {alpha}-induced activation of
	MLK3 and JNK in MCF-7 cells is blocked by geldanamycin treatment.
	Our finding that geldanamycin treatment does not affect the cellular
	levels of the downstream signaling components, MAPK kinase 4, MAPK
	kinase 7, and JNK, suggests that Hsp90/p50cdc37 regulates JNK signaling
	at the MAPK kinase kinase level. Previously identified Hsp90/p50cdc37
	clients include oncoprotein kinases and protein kinases that promote
	cellular proliferation and survival. Our findings reveal that Hsp90/p50cdc37
	also regulates protein kinases involved in apoptotic signaling. 10.1074/jbc.M311377200},
  bdsk-url-1 = {http://dx.doi.org/10.1074/jbc.M311377200},
  date-added = {2008-06-30 21:59:13 -0400},
  date-modified = {2008-06-30 21:59:13 -0400},
  doi = {10.1074/jbc.M311377200},
  keywords = {misc},
  posted-at = {2008-07-01 02:58:43},
  priority = {0},
  url = {http://dx.doi.org/10.1074/jbc.M311377200}
}

@ARTICLE{Zhang:2010,
  author = {Zhang, J. and Zhang, Y.},
  title = {{A Novel Side-chain Orientation Dependent Potential Derived from
	Random-Walk Reference State for Protein Fold Selection and Structure
	Prediction}},
  year = {2010},
  volume = {5},
  pages = {e15386},
  number = {10}
}

@ARTICLE{Zhang:2006f,
  author = {Zhang, L. and Xiang, Y. and Wei, G. W. },
  title = {Local adaptive differential quadrature for free vibration analysis
	of cylindrical shells with various boundary conditions},
  journal = {International Journal of Mechanical Sciences},
  year = {2006},
  volume = {48},
  pages = {1126--1138},
  number = {10},
  abstract = {This paper presents the formulation and numerical analysis of circular
	cylindrical shells by the local adaptive differential quadrature
	method (LaDQM), which employs both localized interpolating basis
	functions and exterior grid points for boundary treatments. The governing
	equations of motion are formulated using the Goldenveizer-Novozhilov
	shell theory. Appropriate management of exterior grid points is presented
	to couple the discretized boundary conditions with the governing
	differential equations instead of using the interior points. The
	use of compactly supported interpolating basis functions leads to
	banded and well-conditioned matrices, and thus, enables large-scale
	computations. The treatment of boundary conditions with exterior
	grid points avoids spurious eigenvalues. Detailed formulations are
	presented for the treatment of various shell boundary conditions.
	Convergence and comparison studies against existing solutions in
	the literature are carried out to examine the efficiency and reliability
	of the present approach. It is found that accurate natural frequencies
	can be obtained by using a small number of grid points with exterior
	points to accommodate the boundary conditions.},
  bdsk-url-1 = {http://dx.doi.org/10.1016/j.ijmecsci.2006.05.005},
  date-added = {2008-06-30 22:13:12 -0400},
  date-modified = {2008-06-30 22:13:12 -0400},
  doi = {10.1016/j.ijmecsci.2006.05.005},
  keywords = {mathematics},
  posted-at = {2008-07-01 03:12:45},
  priority = {0},
  url = {http://dx.doi.org/10.1016/j.ijmecsci.2006.05.005}
}

@ARTICLE{Zhang069387,
  author = {Zhang, Q. M. and Lu, Z. Y. and Hu, H. and Yang, W. T. and Marszalek,
	P. E.},
  title = {Direct detection of the formation of V-amylose helix by single molecule
	force spectroscopy},
  journal = {Journal of the American Chemical Society},
  year = {2006},
  volume = {128},
  pages = {9387-9393},
  number = {29},
  month = {Jul},
  abstract = {An important polysaccharide, amylose crystallizes as a regular single
	left-handed helix from a propanol, butanol, or iodine solution. However,
	its solution structure remains elusive because amylose does not form
	molecular solutions in these solvents, and standard spectroscopic
	techniques cannot be exploited to determine its structure. Using
	AFM, we forced individual amylose chains adsorbed to a surface to
	enter these poor solvents and carried out stretch-release measurements
	on them in solution. In this manner, we directly captured the formation
	of individual amylose helices induced by butanol and iodine. With
	an accuracy approaching that of X-ray diffraction on amylose crystals,
	we determined that the pitch of the helix in solution is 1.3 angstrom/ring.
	We also directly measured the force driving the formation of the
	helix in solution to be 50 pN. SMD simulations in explicit butanol
	reproduced the AFM-measured force-extension curves and revealed that
	the long plateau feature is caused by the rupture of O(2)(n)-O(6)(n+6)
	and O(3)(n)-O(6)(n+6) hydrogen bonds and by the unwinding of the
	helix. We also found that amylose helices formed in iodine solution
	are more compliant and hysteretic as compared to helices in butanol,
	which extend/relax reversibly. In iodine solution, the formation
	of the helix is inhibited by force and limited by the slow kinetics
	of the amylose-iodine complex. By forcing individual molecules into
	poor solvents and performing force spectroscopy measurements in solution,
	our AFM approach uniquely supplements X-ray diffraction and NMR methods
	for investigating solution conformations of insoluble biopolymers.},
  endnotereftype = {Journal Article},
  issn = {0002-7863},
  shorttitle = {Direct detection of the formation of V-amylose helix by single molecule
	force spectroscopy},
  url = {<Go to ISI>://000239120700052}
}

@PHDTHESIS{Zhang-2006-RWM,
  author = {Song Zhang},
  title = {Revealing White Matter Fiber Structure with Diffusion Imaging},
  school = {Brown University},
  year = {2006},
  month = {August},
  added-by = {Daniel Acevedo},
  date-added = {Thu September 21 0:45:17 2006},
  project = {brain},
  theme = {medicine}
}

@ARTICLE{Zhang:2009(a),
  author = {Zhang, Y.},
  title = {{I-TASSER: Fully automated protein structure prediction in CASP8}},
  journal = {Proteins},
  year = {2009},
  volume = {77},
  pages = {100-113},
  number = {S9}
}

@ARTICLE{Zhang:2009(b),
  author = {Zhang, Y.},
  title = {{Protein structure prediction: when is it useful?}},
  journal = {Curr Opin Struct Biol},
  year = {2009},
  volume = {19},
  pages = {145-155},
  number = {2}
}

@ARTICLE{Zhang:2008(a),
  author = {Zhang, Y.},
  title = {{I-TASSER server for protein 3D structure prediction}},
  journal = {BMC Bioinformatics},
  year = {2008},
  volume = {9},
  pages = {40}
}

@ARTICLE{Zhang:2008(b),
  author = {Zhang, Y.},
  title = {{Progress and challenges in protein structure prediction}},
  journal = {Curr Opin Struct Biol},
  year = {2008},
  volume = {18},
  pages = {342-348},
  number = {3}
}

@ARTICLE{Zhang:2007(a),
  author = {Zhang, Y.},
  title = {{Template-based modeling and free modeling by I-TASSER in CASP7}},
  journal = {Proteins},
  year = {2007},
  volume = {69},
  pages = {108-117},
  number = {S8}
}

@ARTICLE{Zhang:2007(b),
  author = {Zhang, Y.},
  title = {{Template-based modeling and free modeling by I-TASSER in CASP7}},
  journal = {Proteins},
  year = {2007},
  volume = {69},
  pages = {108-117},
  number = {Suppl S8}
}

@ARTICLE{Zhang:2005(a),
  author = {Zhang, Y. and Arakaki, A. and Skolnick, J.},
  title = {{TASSER: An automated method for the prediction of protein tertiary
	structures in CASP6}},
  journal = {Proteins},
  year = {2005},
  volume = {61},
  pages = {91-98},
  number = {Suppl 7}
}

@ARTICLE{YZhang:2009,
  author = {Zhang, Yongjie and Bajaj, Chandrajit and Xu, Guoliang},
  title = {Surface smoothing and quality improvement of quadrilateral/hexahedral
	meshes with geometric flow},
  journal = {Communications in Numerical Methods in Engineering},
  year = {2009},
  volume = {25},
  pages = {1-18}
}

@ARTICLE{YZhang:2006,
  author = {Zhang, Y. and Hubner, I. A. and Arakaki, A. K. and Shakhnovich, E.
	and Skolnick, J.},
  title = {{ On the origin and completeness of highly likely single domain protein
	structures}},
  journal = {Proc. Natl. Acad. Sci. USA},
  year = {2006},
  volume = {103},
  pages = {2605-2610}
}

@ARTICLE{Zhang:2006,
  author = {Zhang, Y. and Hubner, I. and Arakaki, A. and Shakhnovich, E. and
	Skolnick, J.},
  title = {{On the origin and completeness of highly likely single domain protein
	structures}},
  journal = {Proc Natl Acad Sci USA},
  year = {2006},
  volume = {103},
  pages = {2605-2610}
}

@ARTICLE{Zhang:2002,
  author = {Zhang, Y. and Kihara, D. and Skolnick, J.},
  title = {{Local energy landscape flattening: Parallel hyperbolic Monte Carlo
	sampling of protein folding}},
  journal = {Proteins},
  year = {2002},
  volume = {48},
  pages = {192-201}
}

@ARTICLE{Zhang:2003,
  author = {Zhang, Y. and Kolinski, A. and Skolnick, J.},
  title = {{TOUCHSTONE II: A new approach to ab initio protein structure prediction}},
  journal = {Biophys J},
  year = {2003},
  volume = {85},
  pages = {1145-1164}
}

@INCOLLECTION{Zhang02332,
  author = {Zhang, Yingkai and Liu, Haiyan and Yang, W. T.},
  title = {Ab Initio QM/MM and Free Energy Calculations of Enzyme Reactions},
  booktitle = {Computational Methods for Macromolecules--Challenges and Applications,
	Springer Verlag's Lecture Notes Series in Computational Science and
	Engineering},
  publisher = {Springer},
  year = {2002},
  editor = {Schlick, T. and  Gan, H. H.},
  pages = {332--354},
  address = {New York},
  endnotereftype = {Book Section},
  shorttitle = {Ab Initio QM/MM and Free Energy Calculations of Enzyme Reactions}
}

@ARTICLE{TriangleWENO,
  author = {Y.T. Zhang and C.W. Shu},
  title = {{High-Order WENO Schemes for Hamilton-Jacobi Equations on Triangular
	Meshes}},
  journal = {J. Sci. Comput.},
  year = {2003},
  volume = {24},
  pages = {1005--1030}
}

@ARTICLE{YZhang:2005a,
  author = {Zhang, Y. and Skolnick, J.},
  title = {{The protein structure prediction problem could be solved using the
	current PDB library}},
  journal = {Proc. Natl. Acad. Sci. USA},
  year = {2005},
  volume = {102},
  pages = {1029-1034}
}

@ARTICLE{YZhang:2005b,
  author = {Zhang, Y. and Skolnick, J.},
  title = {{ TM-align: a protein structure alignment algorithm based on the
	TM-score}},
  journal = {Nucleic. Acids Res.},
  year = {2005},
  volume = {33},
  pages = {2302-230}
}

@ARTICLE{Zhang:2005(b),
  author = {Zhang, Y. and Skolnick, J.},
  title = {{The protein structure prediction problem could be solved using the
	current PDB library}},
  journal = {Proc Natl Acad Sci USA},
  year = {2005},
  volume = {102},
  pages = {1029-1034}
}

@ARTICLE{Zhang:2005(c),
  author = {Zhang, Y. and Skolnick, J.},
  title = {{TM-align: a protein structure alignment algorithm based on the TM-score}},
  journal = {Nucleic Acids Res},
  year = {2005},
  volume = {33},
  pages = {2302-2309},
  number = {7}
}

@ARTICLE{YZhang:2004,
  author = {Zhang, Y. and Skolnick, J.},
  title = {{ Scoring function for automated assessment of protein structure
	template quality}},
  journal = {Proteins},
  year = {2004},
  volume = {57},
  pages = {702-710}
}

@ARTICLE{Zhang:2004(a),
  author = {Zhang, Y. and Skolnick, J.},
  title = {{Automated structure prediction of weakly homologous proteins on
	a genomic scale}},
  journal = {Proc Natl Acad Sci USA},
  year = {2004},
  volume = {101},
  pages = {7594-7599}
}

@ARTICLE{Zhang:2004(b),
  author = {Zhang, Y. and Skolnick, J.},
  title = {{Tertiary structure predictions on a comprehensive benchmark of medium
	to large size proteins}},
  journal = {Biophys J},
  year = {2004},
  volume = {87},
  pages = {2647-2655}
}

@ARTICLE{Zhang:2004(c),
  author = {Zhang, Y. and Skolnick, J.},
  title = {{SPICKER: A clustering approach to identify near-native protein folds}},
  journal = {J Comput Chem},
  year = {2004},
  volume = {25},
  pages = {865-871},
  number = {6}
}

@ARTICLE{Zhang:2006c,
  author = {Zhang, Y. and Xu, G. and Bajaj, C.},
  title = {Quality meshing of implicit solvation models of biomolecular structures},
  journal = {Computer Aided Geometric Design},
  year = {2006},
  volume = {23},
  pages = {510-30},
  number = {6},
  abstract = {This paper describes a comprehensive approach to construct quality
	meshes for implicit solvation models of biomolecular structures starting
	from atomic resolution data in the Protein Data Bank (PDB). First,
	a smooth volumetric electron density map is constructed from atomic
	data using weighted Gaussian isotropic kernel functions and a two-level
	clustering technique. This enables the selection of a smooth implicit
	solvation surface approximation to the LeeÃ¢Â€Â“Richards
	molecular surface. Next, a modified dual contouring method is used
	to extract triangular meshes for the surface, and tetrahedral meshes
	for the volume inside or outside the molecule within a bounding sphere/box
	of influence. Finally, geometric flow techniques are used to improve
	the surface and volume mesh quality. Several examples are presented,
	including generated meshes for biomolecules that have been successfully
	used in finite element simulations involving solvation energetics
	and binding rate constants.},
  annote = {Quality meshing of implicit solvation models of biomolecular structures},
  bdsk-url-1 = {http://dx.doi.org/10.1016/j.cagd.2006.01.008},
  date-added = {2008-06-30 11:27:16 -0500},
  date-modified = {2008-06-30 11:27:16 -0500},
  keywords = {Mathematics; Electrostatics; Diffusion},
  ty = {JOUR},
  url = {http://dx.doi.org/10.1016/j.cagd.2006.01.008}
}

@ARTICLE{YZhang:2009a,
  author = {Zhang, Y. and Yu, H. and Qin, J. H. and Lin, B. C.},
  title = {A microfluidic DNA computing processor for gene expression analysis
	and gene drug synthesisn},
  journal = {Biomicrofluidics},
  year = {2009},
  volume = {3},
  number = {044105 }
}

@ARTICLE{Zhang9946,
  author = {Zhang, Y. K. and Lee, T. S. and Yang, W. T.},
  title = {A pseudobond approach to combining quantum mechanical and molecular
	mechanical methods},
  journal = {Journal of Chemical Physics},
  year = {1999},
  volume = {110},
  pages = {46-54},
  number = {1},
  month = {Jan},
  abstract = {A major challenge for combined quantum mechanical and molecular mechanical
	methods (QM/MM) to study large molecules is how to treat the QM/MM
	boundary that bisects some covalent bonds. Here a pseudobond approach
	has been developed to solve this problem for ab initio QM/MM calculations:
	a one-foe-valence atom with an effective core potential is constructed
	to replace the boundary atom of the environment part and to form
	a pseudobond with the boundary atom of the active part. This pseudobond,
	which is described only by the QM method, is designed to mimic the
	original bond with similar bond length and strength, and similar
	effects on the rest of the active part. With this pseudobond approach,
	some well-known deficiencies of the link atom approach have been
	circumvented and a well-defined potential energy surface of the whole
	QM/MM system has been provided. The construction of the effective
	core potential for the pseudobond is independent of the molecular
	mechanical force field and the same effective core potential is applicable
	to both Hartree-Fock and density functional methods. Tests on a series
	of molecules yield very good structural, electronic, and energetic
	results in comparison with the corresponding full ab initio quantum
	mechanical calculations. (C) 1999 American Institute of Physics.
	[S0021-9606(99)30201-4].},
  endnotereftype = {Journal Article},
  issn = {0021-9606},
  shorttitle = {A pseudobond approach to combining quantum mechanical and molecular
	mechanical methods},
  url = {<Go to ISI>://000077697900010}
}

@ARTICLE{Zhang003483,
  author = {Zhang, Y. K. and Liu, H. Y. and Yang, W. T.},
  title = {Free energy calculation on enzyme reactions with an efficient iterative
	procedure to determine minimum energy paths on a combined ab initio
	QM/MM potential energy surface},
  journal = {Journal of Chemical Physics},
  year = {2000},
  volume = {112},
  pages = {3483-3492},
  number = {8},
  month = {Feb},
  abstract = {A new practical approach to studying enzyme reactions by combining
	ab initio QM/MM calculations with free energy perturbation is presented.
	An efficient iterative optimization procedure has been developed
	to determine optimized structures and minimum energy paths for a
	system with thousands of atoms on the ab initio QM/MM potential:
	the small QM sub-system is optimized using a quasi-Newton minimizer
	in redundant internal coordinates with ab initio QM/MM calculations,
	while the large MM sub-system is minimized by the truncated Newton
	method in Cartesian coordinates with only molecular mechanical calculations.
	The above two optimization procedures are performed iteratively until
	they converge. With the determined minimum energy paths, free energy
	perturbation calculations are carried out to determine the change
	in free energy along the reaction coordinate. Critical to the success
	of the iterative optimization procedure and the free energy calculations
	is the smooth connection between the QM and MM regions provided by
	a recently proposed pseudobond QM/MM approach [J. Chem. Phys. 110,
	46 (1999)]. The methods have been demonstrated by studying the initial
	proton transfer step in the reaction catalyzed by the enzyme triosephosphate
	isomerase (TIM). (C) 2000 American Institute of Physics. [S0021-9606(00)30708-5].},
  endnotereftype = {Journal Article},
  issn = {0021-9606},
  shorttitle = {Free energy calculation on enzyme reactions with an efficient iterative
	procedure to determine minimum energy paths on a combined ab initio
	QM/MM potential energy surface},
  url = {<Go to ISI>://000085345300003}
}

@ARTICLE{Zhang977921,
  author = {Zhang, Y. K. and Pan, W. and Yang, W. T.},
  title = {Describing van der Waals Interaction in diatomic molecules with generalized
	gradient approximations: The role of the exchange functional},
  journal = {Journal of Chemical Physics},
  year = {1997},
  volume = {107},
  pages = {7921-7925},
  number = {19},
  month = {Nov},
  abstract = {Generalized gradient approximations have been used to calculate the
	potential energy curves for six rare gas diatomic molecules. Several
	generalized gradient approximations are found to provide a good description
	of binding in these diatomic molecules and show a significant improvement
	over the local density approximation in the prediction of bond lengths
	and dissociation energies. It is shown here that the behavior of
	an exchange functional in the region of small density and large density
	gradient plays a very important role in the ability of the functional
	to describe this type of van der Waals attraction. (C) 1997 American
	Institute of Physics.},
  endnotereftype = {Journal Article},
  issn = {0021-9606},
  shorttitle = {Describing van der Waals Interaction in diatomic molecules with generalized
	gradient approximations: The role of the exchange functional},
  url = {<Go to ISI>://A1997YG65500035}
}

@ARTICLE{Zhang00346,
  author = {Zhang, Y. K. and Yang, W. T.},
  title = {Perspective on "Density-functional theory for fractional particle
	number: derivative discontinuities of the energy" Perdew JP, Parr
	RG, Levy M, Balduz JL Jr},
  journal = {Theoretical Chemistry Accounts},
  year = {2000},
  volume = {103},
  pages = {346-348},
  number = {3-4},
  month = {Feb},
  abstract = {This paper provides an overview of the title paper by Perdew, Parr,
	Levy and Balduz [Phys Rev Lett 49:1691 (1982)]. The title paper extended
	density functional theory to fractional electron number by an ensemble
	approach and proved that the energy is a series of straight lines
	interpolating its values at integer numbers of electrons, it also
	established that the highest-occupied exact Kohn-Sham orbital energy
	is the negative of the ionization energy, and showed that the exchange-correlation
	potential jumps by a constant as the number of electrons increases
	by an integer. These results are fundamental and continue to inspire
	developments in density functional theory.},
  endnotereftype = {Journal Article},
  issn = {1432-881X},
  shorttitle = {Perspective on "Density-functional theory for fractional particle
	number: derivative discontinuities of the energy" Perdew JP, Parr
	RG, Levy M, Balduz JL Jr},
  url = {<Go to ISI>://000085419900057}
}

@ARTICLE{Zhang982604,
  author = {Zhang, Y. K. and Yang, W. T.},
  title = {A challenge for density functionals: Self-interaction error increases
	for systems with a noninteger number of electrons},
  journal = {Journal of Chemical Physics},
  year = {1998},
  volume = {109},
  pages = {2604-2608},
  number = {7},
  month = {Aug},
  abstract = {The difficulty of widely used density functionals in describing the
	dissociation behavior of some homonuclear and heteronuclear diatomic
	radicals is analyzed. It is shown that the self-interaction error
	of these functionals accounts for the problem-it is much larger for
	a system with a noninteger number of electrons than a system with
	an integer number of electrons. We find the condition for the erroneous
	dissociation behavior described by approximate density functionals:
	when the ionization energy of one dissociation partner differs from
	the electron affinity of the other partner by a small amount, the
	self-interaction error will lead to wrong dissociation limit. Systems
	with a noninteger number of electrons and hence the large amount
	of self-interaction error in approximate density functionals arise
	also in the transition states of some chemical reactions and in some
	charge-transfer complexes. In the course of analysis, we derive a
	scaling relation necessary for an exchange-correlation functional
	to be self-interaction free. (C) 1998 American Institute of Physics.},
  endnotereftype = {Journal Article},
  issn = {0021-9606},
  shorttitle = {A challenge for density functionals: Self-interaction error increases
	for systems with a noninteger number of electrons},
  url = {<Go to ISI>://000075271100004}
}

@ARTICLE{Zhang98890,
  author = {Zhang, Y. K. and Yang, W. T.},
  title = {Comment on "Generalized gradient approximation made simple"},
  journal = {Physical Review Letters},
  year = {1998},
  volume = {80},
  pages = {890-890},
  number = {4},
  month = {Jan},
  endnotereftype = {Journal Article},
  issn = {0031-9007},
  shorttitle = {Comment on "Generalized gradient approximation made simple"},
  url = {<Go to ISI>://000071717100066}
}

@ARTICLE{Zhao:2011,
  author = {Zhao, D. X. and Yu, L. and Gong, L. D. and Liu, C. and Yang, Z. Z.
	},
  title = {Calculating solvation energies by means of a fluctuating charge model
	combined with continuum solvent model},
  journal = {J. Chem. Phys.},
  year = {2011},
  volume = {134},
  pages = {194115},
  abstract = {provide a polarizable charge protocol for the GB method}
}

@ARTICLE{Zhao959598,
  author = {Zhao, Q. S. and Yang, W. T.},
  title = {Analytical Energy Gradients and Geometry Optimization in the Divide-and-Conquer
	Method for Large Molecules},
  journal = {Journal of Chemical Physics},
  year = {1995},
  volume = {102},
  pages = {9598-9603},
  number = {24},
  month = {Jun},
  endnotereftype = {Journal Article},
  issn = {0021-9606},
  shorttitle = {Analytical Energy Gradients and Geometry Optimization in the Divide-and-Conquer
	Method for Large Molecules},
  url = {<Go to ISI>://A1995RD33200018}
}


@ARTICLE{SZhao:2011a,
  author = {Zhao, Shan},
  title = {Pseudo-time-coupled nonlinear models for biomolecular surface representation
	and solvation analysis},
  journal = {International Journal for Numerical Methods in Biomedical Engineering
	},
  year = {2011},
  volume = {27},
  pages = {1964-1981}
}

@ARTICLE{SZhao:2014a,
  author = {Zhao, Shan},
  title = {Operator splitting ADI schemes for pseudo-time coupled nonlinear solvation simulations},
  journal = {Journal of Computational Physics
	},
  year = {2014},
  volume = {257},
  pages = {1000 - 1021}
}

@ARTICLE{SZhao:2014b,
  author = {Zhao, Shan and Wei, G. W.},
  title = {A  unified    discontinuous   { Galerkin}    framework  for    time    integration},
  journal = {Mathematical Methods in the Applied Sciences
	},
  year = {2014},
  volume = {37},
  pages = {1042 - 1071}
}


@ARTICLE{SZhao:2010a,
  author = {Zhao, S.},
  title = {High order matched interface and boundary methods for the {Helmholtz}
	equation in media with arbitrarily curved interfaces},
  journal = {J. Comput. Phys.},
  year = {2010},
  volume = {229},
  pages = {3155-3170}
}

@ARTICLE{SZhao:2010b,
  author = {Zhao, Shan },
  title = {A fourth order finite difference method for waveguides with curved
	perfectly conducting boundaries },
  journal = {Computer Methods in Applied Mechanics and Engineering},
  year = {2010},
  volume = {199},
  pages = { 2655-2662}
}

@ARTICLE{ZhaoShan:2009,
  author = { Zhao, S.},
  title = {High order vectorial analysis of waveguides with curved dielectric
	interfaces},
  journal = {IEEE Microwave and Wireless Components Letters},
  year = {2009},
  volume = {19},
  pages = {266 - 268}
}

@ARTICLE{Zhaoshan:2009b,
  author = {Zhao, Shan},
  title = {High order vectorial analysis of waveguides with curved dielectric
	interfaces},
  journal = {IEEE Microwave and Wireless Components Letters},
  year = {2009},
  volume = {19},
  pages = {266 - 268}
}

@ARTICLE{SZhao:2008a,
  author = {Zhao, S.},
  title = {Full-vectorial matched interface and boundary ({MIB}) method for
	the modal analysis of dielectric waveguides},
  journal = {IEEE/OSA Journal of Lighwave Technology},
  year = {2008},
  volume = {26},
  pages = {2251-2259}
}

@ARTICLE{SZhao:2007,
  author = {Zhao, S.},
  title = {On the spurious solutions in the high-order finite difference methods},
  journal = {Computer Methods in Applied Mechanics and Engineering},
  year = {2007},
  volume = {196},
  pages = {5031-5046}
}

@ARTICLE{ShanZhao:2009,
  author = {Zhao, Shan and Wei, G. W.},
  title = {Matched interface and boundary {(MIB)} for the implementation of
	boundary conditions in high order central finite differences },
  journal = {International Journal for Numerical Methods in Engineering},
  year = {2009},
  volume = {77},
  pages = { 1690-1730}
}

@ARTICLE{Zhao:2008,
  author = {Zhao, S. and Wei, G. W. },
  title = {Matched interface and boundary ({MIB}) for the implementation of
	boundary conditions in high order central finite differences},
  journal = {Int. J. Numer. Meth. Engng.},
  year = {2009},
  volume = {77},
  pages = {1690 - 1730},
  annote = {Matched interface and boundary ({MIB}) for the implementation of
	boundary conditions in high order central finite differencesy},
  date-added = {2008-09-19 10:28:56 -0500},
  date-modified = {2008-09-19 10:28:56 -0500},
  ty = {JOUR}
}

@ARTICLE{Zhaoshan:2009a,
  author = {Zhao, Shan and Wei, G. W.},
  title = {Matched interface and boundary ({MIB}) for the implementation of
	boundary conditions in high-order central finite differences},
  journal = {Int. J. Numer. Meth. Engng.},
  year = {2009},
  volume = {77},
  pages = {1690 - 1730}
}

@ARTICLE{Zhao:2004,
  author = {Zhao, Shan and Wei, G. W. },
  title = {High-order {FDTD} methods via derivative matching for {Maxwell's}
	equations with material interfaces},
  journal = {J. Comput. Phys.},
  year = {2004},
  volume = {200},
  pages = {60--103},
  number = {1},
  abstract = {This paper introduces a series of novel hierarchical implicit derivative
	matching methods to restore the accuracy of high-order finite-difference
	time-domain ({FDTD}) schemes of computational electromagnetics (CEM)
	with material interfaces in one (1D) and two spatial dimensions (2D).
	By making use of fictitious points, systematic approaches are proposed
	to locally enforce the physical jump conditions at material interfaces
	in a preprocessing stage, to arbitrarily high orders of accuracy
	in principle. While often limited by numerical instability, orders
	up to 16 and 12 are achieved, respectively, in 1D and 2D. Detailed
	stability analyses are presented for the present approach to examine
	the upper limit in constructing embedded {FDTD} methods. As natural
	generalizations of the high-order {FDTD} schemes, the proposed derivative
	matching methods automatically reduce to the standard {FDTD} schemes
	when the material interfaces are absent. An interesting feature of
	the present approach is that it encompasses a variety of schemes
	of different orders in a single code. Another feature of the present
	approach is that it can be robustly implemented with other high accuracy
	time-domain approaches, such as the multiresolution time-domain method
	and the local spectral time-domain method, to cope with material
	interfaces. Numerical experiments on both 1D and 2D problems are
	carried out to test the convergence, examine the stability, access
	the efficiency, and explore the limitation of the proposed methods.
	It is found that operating at their best capacity, the proposed high-order
	schemes could be over 2000 times more efficient than their fourth-order
	versions in 2D. In conclusion, the present work indicates that the
	proposed hierarchical derivative matching methods might lead to practical
	high-order schemes for numerical solution of time-domain {Maxwell's}
	equations with material interfaces.},
  bdsk-url-1 = {http://dx.doi.org/10.1016/j.jcp.2004.03.008},
  date-added = {2008-06-30 21:35:12 -0400},
  date-modified = {2008-06-30 21:35:12 -0400},
  doi = {10.1016/j.jcp.2004.03.008},
  keywords = {electrostatics, mathematics},
  posted-at = {2008-07-01 02:33:13},
  priority = {0},
  url = {http://dx.doi.org/10.1016/j.jcp.2004.03.008}
}

@ARTICLE{Zhao:2005a,
  author = {Zhao, S. and Wei, G. W. and Xiang, Y. },
  title = {DSC analysis of free-edged beams by an iteratively matched boundary
	method},
  journal = {Journal of Sound and Vibration},
  year = {2005},
  volume = {284},
  pages = {487--493},
  number = {1-2},
  abstract = {This communication introduces a novel scheme for the treatment of
	free edge supports in the analysis of beams by using the discrete
	singular convolution (DSC) algorithm. Accommodating free edges has
	been a challenging issue in the DSC analysis of beams, plates, and
	shells. An iteratively matched boundary (IMB) method is proposed
	to overcome the difficulty. Numerical experiments are carried out
	to demonstrate that the proposed IMB method works very well in dealing
	with arbitrary combinations of beam edge supports.},
  bdsk-url-1 = {http://dx.doi.org/10.1016/j.jsv.2004.08.037},
  date-added = {2008-06-30 22:14:45 -0400},
  date-modified = {2008-06-30 22:14:45 -0400},
  doi = {10.1016/j.jsv.2004.08.037},
  keywords = {mathematics},
  posted-at = {2008-07-01 03:14:17},
  priority = {0},
  url = {http://dx.doi.org/10.1016/j.jsv.2004.08.037}
}

@ARTICLE{SLZhao:2011,
  author = {Zhao, S. L. and Ramirez, R. and Vuilleumier, R. and Borgis, D.},
  title = {Molecular density functional theory of solvation: from polar solvents
	to water},
  journal = {Journal of chemical physics},
  year = {2011},
  volume = {134},
  pages = {194102},
  number = {19}
}

@ARTICLE{QZheng:2011a,
  author = {Zheng, Qiong and Chen, Duan and Wei, G. W.},
  title = {Second-order {Poisson-Nernst-Planck} solver for ion transport },
  journal = {Journal of Comput. Phys.},
  year = {2011},
  volume = {230},
  pages = {5239 - 5262}
}


@ARTICLE{QZheng:2011b,
  author = {Zheng, Qiong and Wei, G. W.},
  title = {{Poisson-Boltzmann-Nernst-Planck model}},
  journal = {Journal of Chemical Physics},
  year = {2011},
  volume = {134},
  pages = {194101}
}

@ARTICLE{QZheng:2012,
  author = {Zheng, Q. and Yang, S. Y. and Wei, G. W.},
  title = {{ Molecular surface generation using PDE transform}},
  year = {2012},
  journal = {International Journal for Numerical Methods in Biomedical Engineering},
  volume = {28},
  pages = {291-316}
}

@ARTICLE{SZheng:2010,
  author = {Zheng, S. and Wang, L. and Yang, L.},
  title = {{Global estimation for longitudinal data via local linear estimator}},
  year = {2010}
}

@INPROCEEDINGS{Bubbles,
  author = {Wen Zheng and Jun-Hai Yong and Jean-Claude Paul},
  title = {{Simulations of Bubbles}},
  booktitle = {EG/ACM SIGGRAPH Symp. on Comput. Anim.},
  year = {2006},
  pages = {325-333}
}

@ARTICLE{Zheng:2005,
  author = {Zheng, Y. and Rivas, C. and Lake, R. and Alam, K. T. and Boykin,
	B. and Klimeck, G.},
  title = {Electronic properties of silicon nanowires},
  journal = {IEEE Trans. Electron Devices},
  year = {2005},
  volume = {52},
  pages = {1097-1103},
  annote = {Electronic properties of silicon nanowires},
  date-added = {2008-11-25 10:28:56 -0500},
  date-modified = {2008-11-25 10:28:56 -0500},
  ty = {JOUR}
}

@ARTICLE{ZhiZheng:2003,
  author = {Zheng, Zhi and Hansford, D. J. and Conlisk, A. T.},
  title = { Effect of multivalent ions on electroosmotic flow in micro- and
	nanochannels},
  journal = {Electrophoresis},
  year = {2003},
  volume = {24},
  pages = {3006 - 3017}
}

@ARTICLE{Zhou:2005,
  author = {Zhou, H. and Zhou, Y.},
  title = {{Fold recognition by combining sequence profiles derived from evolution
	and from depth-dependent structural alignment of fragments}},
  journal = {Proteins},
  year = {2005},
  volume = {58},
  pages = {321-328},
  number = {2}
}

@ARTICLE{Zhou:2004,
  author = {Zhou, H. and Zhou, Y.},
  title = {{Single-body residue-level knowledge-based energy score combined
	with sequence-profile and secondary structure information for fold
	recognition}},
  journal = {Proteins},
  year = {2004},
  volume = {55},
  pages = {1005-1013},
  number = {4}
}

@ARTICLE{Zhou:2002,
  author = {Zhou, H. and Zhou, Y.},
  title = {{Distance-scaled, finite ideal-gas reference state improves structure-derived
	potentials of mean force for structure selection and stability prediction}},
  journal = {Protein Sci},
  year = {2002},
  volume = {11},
  pages = {2714-2726},
  number = {11}
}

@ARTICLE{ZHWTDGS06,
  author = {K. Zhou and X. Huang and X. Wang and Y. Tong and M. Desbrun and B.
	Guo and H.-Y. Sheum},
  title = {Mesh Quilting For Geometric Texture Synthesis},
  journal = {ACM Trans. on Graphics (SIGGRAPH)},
  year = {2006},
  volume = {25},
  pages = {690--697},
  number = {3},
  month = jul
}

@ARTICLE{ZWTDGS05,
  author = {Kun Zhou and Xi Wang and Yiying Tong and Mathieu Desbrun and Baining
	Guo and H.-Y. Shum},
  title = {TextureMontage: Seamless Texturing of Surfaces From Multiple Images},
  journal = {ACM Trans. on Graphics (SIGGRAPH)},
  year = {2005},
  volume = {24},
  pages = {1148--1155},
  number = {3},
  month = jul
}

@ARTICLE{Zhou:2003,
  author = {Zhou, R.},
  title = {{Free energy landscape of protein folding in water: explicit vs.
	implicit solvent}},
  journal = {Proteins},
  year = {2003},
  volume = {53},
  pages = {148-161},
  number = {2}
}

@ARTICLE{Zhou:2011,
  author = { Zhou, Shenggao and Wang, Zhongming and Li, Bo},
  title = {{Mean-field description of ionic size effects with non-uniform ionic
	sizes: A numerical approach}},
  journal = {Phys. Rev. E},
  year = {2011},
  volume = {84},
  pages = {021901}
}

@ARTICLE{Zhou:2008b,
  author = {Zhou, Y. C. and Feig, M. and Wei, G. W.},
  title = {Highly accurate biomolecular electrostatics in continuum dielectric
	environments},
  journal = {Journal of Computational Chemistry},
  year = {2008},
  volume = {29},
  pages = {87-97}
}

@ARTICLE{YCZhou:2003c,
  author = { Zhou, Y. C. and Gu, Y. and Wei, G. W. },
  title = {Shock-capturing with natural high frequency oscillations },
  journal = {Int. J. Numer. Methods in Fluid },
  year = {2003},
  volume = {41},
  pages = {1319-1338}
}

@ARTICLE{zhou,
  author = {Zhou, Y. C. and Gu, Y. and Wei, G. W.},
  title = {Shock-capturing with natural high frequency oscillations},
  journal = {Int. J. Numer. Methods Fluid},
  year = {2003},
  volume = {41},
  pages = {1319--1338}
}

@ARTICLE{Zhou:2008d,
  author = {Zhou, Y. C. and Holst, M. J. and McCammon, J. A.},
  title = {A nonlinear elasticity model of macromolecular conformational change
	induced by electrostatic forces },
  journal = {Journal of Mathematical Analysis and Applications},
  year = {2008},
  volume = {340},
  pages = {135-164}
}

@ARTICLE{YCZhou:2012a,
  author = { Zhou, Y. C. and Liu, J. G. and Harry, D. L. },
  title = { A matched interface and boundary method for solving multi-flow Navier-Stokes
	equations with applications to geodynamics
	
	},
  journal = { Journal of Computational Physics },
  year = {2012},
  volume = {231},
  pages = {223-242}
}

@ARTICLE{YCZhou:2008,
  author = {Zhou, Y. C. and Lu, B. Z. and Huber, G. A. and Holst, M. J. and McCammon,
	J. A.},
  title = {Continuum simulations of acetylcholine consumption by acetylcholinesterase:
	A {Poisson-Nernst-Planck} approach},
  journal = {J. Phys. Chem. B},
  year = {2008},
  volume = {112},
  pages = {270 - 275}
}

@ARTICLE{YCZhou:2003b,
  author = {Zhou, Y. C. and Patnaik, B. S. V. and Wan, D. C. and Wei, G. W. },
  title = {DSC solution for flow in a staggered double lid drivencavity },
  journal = {Int. J. Numer. Methods in Engng. },
  year = {2003},
  volume = {57},
  pages = { 211-234},
  number = { }
}

@ARTICLE{Zhou:2006d,
  author = {Zhou, Y. C. and Wei, G. W. },
  title = {On the fictitious-domain and interpolation formulations of the matched
	interface and boundary ({MIB}) method},
  journal = {J. Comput. Phys.},
  year = {2006},
  volume = {219},
  pages = {228--246},
  number = {1},
  abstract = {This work overcomes the difficulty of dealing with large curvatures
	in a high order matched interface and boundary {(MIB)} method proposed
	for solving elliptic interface problems. The MIB method smoothly
	extends the solution across the interface so that standard high order
	central finite difference schemes can be used without the loss of
	accuracy. One feature of the MIB is that it disassociates the discretization
	of the elliptic equation from the enforcement of interface jump conditions.
	The other is to make iterative use of only the lowest order jump
	conditions to determine the fictitious values on extended domains.
	It is of arbitrarily high order in convergence, in principle. However,
	its applicability was hindered by the lack of sufficiently many grid
	points to determine all the fictitious values required for high order
	schemes at the location where the curvature of the interface is relatively
	large. We remove this obstacle by introducing a new concept, the
	disassociation between the discretization and the domain extension.
	We show that the improved MIB method is robust for handling general
	irregular interfaces by extensive numerical experiments on the Poisson
	equation and the Helmholtz equation. To better understand the MIB
	method and other potential high order interface schemes, we propose
	an alternative interpolation formulation of the MIB method and show
	that the new formulation is essentially equivalent to the improved
	one.},
  bdsk-url-1 = {http://dx.doi.org/10.1016/j.jcp.2006.03.027},
  date-added = {2008-06-30 21:40:36 -0400},
  date-modified = {2008-06-30 21:40:36 -0400},
  doi = {10.1016/j.jcp.2006.03.027},
  keywords = {electrostatics, mathematics},
  posted-at = {2008-07-01 02:39:39},
  priority = {0},
  url = {http://dx.doi.org/10.1016/j.jcp.2006.03.027}
}

@ARTICLE{YCZhou:2003,
  author = { Zhou, Y. C. and Wei, G. W.},
  title = {High-resolution conjugate filters for the simulation of flows},
  journal = {J. Comput. Phys.},
  year = {2003},
  volume = {189},
  pages = {150 - 179}
}

@ARTICLE{ZhoWeijcp,
  author = {Zhou, Y. C. and Wei, G. W. },
  title = {High resolution conjugate filters for the simulation of flows},
  journal = {J. Comput. Phys.},
  year = {2003},
  volume = {189},
  pages = {159--179}
}

@ARTICLE{Zhou:2006c,
  author = {Zhou, Y. C. and Zhao, Shan and Feig, Michael and Wei, G. W. },
  title = {High order matched interface and boundary method for elliptic equations
	with discontinuous coefficients and singular sources},
  journal = {J. Comput. Phys.},
  year = {2006},
  volume = {213},
  pages = {1--30},
  number = {1},
  abstract = {This paper introduces a novel high order interface scheme, the matched
	interface and boundary {(MIB)} method, for solving elliptic equations
	with discontinuous coefficients and singular sources on Cartesian
	grids. By appropriate use of auxiliary line and/or fictitious points,
	physical jump conditions are enforced at the interface. Unlike other
	existing interface schemes, the proposed method disassociates the
	enforcement of physical jump conditions from the discretization of
	the differential equation under study. To construct higher order
	interface schemes, the proposed MIB method bypasses the major challenge
	of implementing high order jump conditions by repeatedly enforcing
	the lowest order jump conditions. The proposed MIB method is of arbitrarily
	high order, in principle. In treating straight, regular interfaces
	we construct MIB schemes up to 16th-order. For more general elliptic
	problems with curved, irregular interfaces and boundary, up to 6th-order
	MIB schemes have been demonstrated. By employing the standard high-order
	finite difference schemes to discretize the Laplacian, the present
	MIB method automatically reduces to the standard central difference
	scheme when the interface is absent. The immersed interface method
	(IIM) is regenerated for a comparison study of the proposed method.
	The robustness of the MIB method is verified against the large magnitude
	of the jump discontinuity across the interface. The nature of high
	efficiency and low memory requirement of the MIB method is extensively
	validated via solving various elliptic immersed interface problems
	in two- and three-dimensions.},
  bdsk-url-1 = {http://dx.doi.org/10.1016/j.jcp.2005.07.022},
  date-added = {2008-06-30 21:37:49 -0400},
  date-modified = {2008-06-30 21:37:49 -0400},
  doi = {10.1016/j.jcp.2005.07.022},
  keywords = {electrostatics, mathematics},
  posted-at = {2008-07-01 02:37:16},
  priority = {0},
  url = {http://dx.doi.org/10.1016/j.jcp.2005.07.022}
}

@ARTICLE{Zhou:1996a,
  author = {Zhou, Z. and Payne, P. and Vasquez, M. and Kuhn, N. and Levitt, M.},
  title = {Finite-difference solution of the {{Poisson-Boltzmann}} equation:
	complete elimination of self-energy},
  journal = {Journal of Computational Chemistry},
  year = {1996},
  volume = {17},
  pages = {1344-1351},
  abstract = {A new procedure to solve the {Poisson-Boltzmann} equation is proposed
	and shown to be efficient. The electrostatic potential due to the
	reaction field is calculated directly. Self-interactions among the
	charges are completely eliminated. Therefore, the reference calculation
	to cancel out the self-energy is not needed. Ã‚Â??996 by John
	Wiley \& Sons, Inc.},
  annote = {Finite-difference solution of the {Poisson-Boltzmann} equation: complete
	elimination of self-energy},
  bdsk-url-1 = {http://www3.interscience.wiley.com/cgi-bin/abstract/65965/ABSTRACT},
  date-added = {2008-09-17 09:07:27 -0500},
  date-modified = {2008-09-17 09:07:27 -0500},
  keywords = {Electrostatics; Solvation; Mathematics},
  ty = {JOUR},
  url = {http://www3.interscience.wiley.com/cgi-bin/abstract/65965/ABSTRACT}
}

@ARTICLE{Zhu:2005,
  author = {Zhu, J. and Alexov, E. and Honig, B.},
  title = {Comparative Study of Generalized {Born} Models: {Born} Radii and
	Peptide Folding},
  journal = {Journal of Physical Chemistry B},
  year = {2005},
  volume = {109},
  pages = {3008-22},
  number = {7},
  abstract = {In this study, we have implemented four analytical generalized Born
	(GB) models and investigated their performance in conjunction with
	the GROMOS96 force field. The four models include that of Still and
	co-workers, the HCT model of Cramer, Truhlar, and co-workers, a modified
	form of the AGB model of Levy and co-workers, and the GBMV2 model
	of Brooks and co-workers. The models were coded independently and
	implemented in the GROMOS software package and in TINKER. They were
	compared in terms of their ability to reproduce the results of {Poisson-Boltzmann}
	(PB) calculations and in their performance in the ab initio peptide
	folding of two peptides, one that forms a -hairpin in solution and
	one that forms an -helix. In agreement with previous work, the GBMV2
	model is most successful in reproducing PB results while the other
	models tend to underestimate the effective Born radii of buried atoms.
	In contrast, stochastic dynamics simulations on the folding of the
	two peptides, the C-terminus -hairpin of the B1 domain of protein
	G and the alanine-based -helical peptide 3K(I), suggest that the
	simpler GB models are more effective in sampling conformational space.
	Indeed, the Still model used in conjunction with the GROMOS96 force
	field is able to fold the hairpin peptide to a native-like structure
	without the benefit of enhanced sampling techniques. This is due
	in part to the properties of the united-atom GROMOS96 force field
	which appears to be more flexible, and hence to sample more efficiently,
	than force fields such as OPLSAA. Our results suggest a general strategy
	which involves using different combinations of force fields and solvent
	models in different applications, for example, using GROMOS96 and
	a simple GB model in sampling and OPLSAA and a more accurate GB model
	in refinement. The fact that various methods have been implemented
	in a unified way should facilitate the testing and subsequent use
	of different methods to evaluate conformational free energies in
	different applications. Our results also bear on some general issues
	involved in peptide folding and structure prediction which are addressed
	in the Discussion.},
  annote = {Comparative Study of Generalized Born Models: Born Radii and Peptide
	Folding; HonigGBCompare},
  bdsk-url-1 = {http://dx.doi.org/10.1021/jp046307s},
  date-added = {2008-09-15 10:02:30 -0500},
  date-modified = {2008-09-15 10:02:30 -0500},
  keywords = {Electrostatics},
  ty = {JOUR},
  url = {http://dx.doi.org/10.1021/jp046307s}
}

@ARTICLE{Zhu934814,
  author = {Zhu, T. H. and Lee, C. T. and Yang, W. T.},
  title = {Examination of Several Exchange-Correlation Energy Functionals by
	Accurate Self-Consistent Atomic Calculations},
  journal = {Journal of Chemical Physics},
  year = {1993},
  volume = {98},
  pages = {4814-4821},
  number = {6},
  month = {Mar},
  abstract = {Several local and nonlocal exchange-correlation functionals are tested
	through accurate Kohn-Sham self-consistent calculations for six nobel
	gas atoms and three isoelectronic series (with two, four, and ten
	electrons and atomic numbers up to 20). The calculated exchange,
	correlation, and total energies have been compared with those from
	accurate Hartree-Fock calculations and accurate estimates of correlation
	energies available recently. Improvements over local-density approximation
	are found for all the tested nonlocal exchange-correlation functionals.
	In particular, nonlocal correlation energy functionals are shown
	to perform significantly better than the local approximations when
	both are used in conjunction with the nonlocal Becke's exchange energy
	functional. However, in most cases, all the functionals fail to predict
	the correct trends of exchange and correlation energies as the atomic
	charge increases.},
  endnotereftype = {Journal Article},
  issn = {0021-9606},
  shorttitle = {Examination of Several Exchange-Correlation Energy Functionals by
	Accurate Self-Consistent Atomic Calculations},
  url = {<Go to ISI>://A1993KU22200051}
}

@ARTICLE{Zhu972,
  author = {Zhu, T. H. and Pan, W. and Yang, W. T.},
  title = {Divide-and-conquer calculations for clean surfaces and surface adsorption},
  journal = {Theoretical Chemistry Accounts},
  year = {1997},
  volume = {96},
  pages = {2-6},
  number = {1},
  month = {Apr},
  abstract = {The divide-and-conquer density-functional approach is implemented
	for electronic structure calculations of clean surfaces and surface
	adsorption. The method divides a semi-infinite solid-state system
	into subsystems and determines each subsystem density separately.
	We have applied the method to study two low index Li surfaces and
	the chemisorption of a monolayer of atomic hydrogen on the Li(100)
	surface. Surface and adsorption energies converge well with respect
	to the number of buffer atoms and surface layers. Our converged energies
	are in very good agreement with accurate theoretical and available
	experimental results.},
  endnotereftype = {Journal Article},
  issn = {1432-881X},
  shorttitle = {Divide-and-conquer calculations for clean surfaces and surface adsorption},
  url = {<Go to ISI>://A1997XF32500001}
}

@ARTICLE{Zhu9612713,
  author = {Zhu, T. H. and Pan, W. and Yang, W. T.},
  title = {Structure of solid-state systems from embedded-cluster calculations:
	A divide-and-conquer approach},
  journal = {Physical Review B},
  year = {1996},
  volume = {53},
  pages = {12713-12724},
  number = {19},
  month = {May},
  abstract = {The first-principles divide-and-conquer density-functional approach
	has been extended to solid-state systems. The method has the following
	features. (1) It divides a periodic solid-state system into equivalent
	primitive cells and further divides each cell into subsystems. The
	electron density of each subsystem is determined through the local
	representation of the one-electron Hamiltonian and used to form the
	total density per primitive cell. The method calculates the electronic
	structure of solids without involving the reciprocal space and its
	associated band structure. (2) It uses numerical atomic orbitals
	as basis functions with great variational flexibility. The Hamiltonian
	and other matrix elements are evaluated by numerical integration
	without any shape approximation to the effective one-electron potential.
	(3) This method, based on real space partition, can be applied to
	extended solid-state systems without translational symmetry, such
	as defects and surface chemisorption. As the first step, we have
	applied and tested the method to the electronic structure calculations
	of various crystalline solids: metallic lithium and copper, ionic
	sodium chloride, and covalent diamond and silicon. The self-consistently
	computed cohesive energies, structural properties, and density of
	states are in good agreement with those from the local-density approximation
	band-structure calculations and experimental results.},
  endnotereftype = {Journal Article},
  issn = {1098-0121},
  shorttitle = {Structure of solid-state systems from embedded-cluster calculations:
	A divide-and-conquer approach},
  url = {<Go to ISI>://A1996UM47800039}
}

@ARTICLE{Zhu94613,
  author = {Zhu, T. H. and Yang, W. T.},
  title = {Structure of the Ammonia Dimer Studied by Density-Functional Theory},
  journal = {International Journal of Quantum Chemistry},
  year = {1994},
  volume = {49},
  pages = {613-623},
  number = {5},
  month = {Feb},
  abstract = {Self-consistent Kohn-Sham density functional calculations have been
	carried out to study the structure of the ammonia dimer. The local-density
	approximation yields unusually large binding energy and short internitrogen
	distance compared with the experimental and more accurate theoretical
	data. The results from the Becke-Perdew gradient-corrected functionals
	are generally in good agreement with those at the SCF MP2 level when
	the geometry is fully optimized with various large basis sets. With
	our best estimation, the staggered quasi-linear structure (C-s) is
	0.6 kcal/mol lower in energy than the symmetric cyclic one (C-2h)
	The hydrogen-bonded N-H bond in the staggered quasi-linear structure
	is found to be 0.008 Angstrom longer than the N-H bond in ammonia.
	In our calculations, we could not find the minima on the energy surface
	corresponding to the two asymmetric cyclic structures suggested by
	microwave spectra and coupled pair functional calculations. (C) 1994
	John Wiley & Sons, Inc.},
  endnotereftype = {Journal Article},
  issn = {0020-7608},
  shorttitle = {Structure of the Ammonia Dimer Studied by Density-Functional Theory},
  url = {<Go to ISI>://A1994MU69800006}
}

@INPROCEEDINGS{Zhukov,
  author = {L. Zhukov and A. H. Barr},
  title = {Heart-muscle fiber reconstruction from diffusion tensor {MRI}},
  booktitle = {IEEE Visualization},
  year = {2003},
  pages = {597--602}
}

@BOOK{AMR,
  title = {{Manifolds, Tensor Analysis, and Applications}},
  publisher = {Applied Mathematical Sciences Vol. 75, Springer},
  year = {1988},
  editor = {R. Abraham and J.E. Marsden and T. Ratiu}
}

@BOOK{Uversky:2007,
  title = {Methods in Protein Structure and Stability Analysis: Conformational
	Stability, Size, Shape and Surface of Protein Molecules},
  publisher = {Nova sicence publishers inc.},
  year = {2007},
  editor = {Uversky V.N. and Permyakov E.A.}
}

@MISC{CGoGN,
  title = {{Combinatorial and Geometric modeling with Generic N-dimensional
	Maps}},
  howpublished = {\url{http://cgogn.u-strasbg.fr/Wiki/index.php/CGoGN}},
  year = {2012},
  key = {CGoGN}
}

@MISC{OpenVolumeMesh,
  title = {{OpenVolumeMesh - A Generic and Versatile Index-Based Data Structure
	for Polytopal Meshes}},
  howpublished = {\url{http://www.openvolumemesh.org/}},
  year = {2012},
  key = {OpenVolumeMesh}
}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% KELIN XIA added begin:


@INPROCEEDINGS{Fernandez:2007,
  AUTHOR =       {Fernandez, J. J. and Li, S. and Lucic, V.},
  TITLE =        {Three-Dimensional Anisotropic Noise Reduction with Automated Parameter Tuning: Application to Electron Cryotomography},
  booktitle =    {Current Topics in Artificial Intelligence},
  YEAR =         {2007},
  volume =       {4788},
  number =       {},
  pages =        {60-69}
}





%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%the above papers are related to denoise method

@INPROCEEDINGS{Volkmann:2010,
  AUTHOR =       {Volkmann, N.},
  TITLE =        {Methods for segmentation and interpretation of electron tomographic reconstructions},
  booktitle =    {Methods Enzymol},
  YEAR =         {2010},
  volume =       {483},
  number =       {},
  pages =        {31-46}
}

@ARTICLE{Leis:2009,
  AUTHOR =       {Leis, A. and Rockel, B. and Andrees, L. and Baumeister, W.},
  TITLE =        {Visualizing cells at the nanoscale},
  JOURNAL =      {Trends Biochem. Sci.},
  YEAR =         {2009},
  volume =       {34},
  number =       {},
  pages =        {60?C70}
}

@ARTICLE{Nickell:2006,
  AUTHOR =       {Nickell, S. and Kofler, C. and Leis, A. P. and Baumeister, W.},
  TITLE =        {A visual approach to proteomics},
  JOURNAL =      {Nat. Rev. Mol. Cell Biol.},
  YEAR =         {2006},
  volume =       {7},
  number =       {},
  pages =        {225-230}
}

@ARTICLE{Robinson:2007,
  AUTHOR =       {Robinson, C. V. and Sali, A. and Baumeister, W.},
  TITLE =        {The molecular sociology of the cell},
  JOURNAL =      {Nature},
  YEAR =         {2007},
  volume =       {450},
  number =       {},
  pages =        {973?C982}
}

@INPROCEEDINGS{Tocheva:2010,
  AUTHOR =       {Tocheva, E. I. and Li, Z. and Jensen, G. J.},
  TITLE =        {Electron cryotomography},
  booktitle =    {Cold Spring Harb. Perspect. Biol.},
  YEAR =         {2010},
  volume =       {2},
  pages =        {A003442}
}

@ARTICLE{Noske:2008,
  AUTHOR =       {Noske, A. B. and Costin, A. J. and Morgan, G. P. and Marsh, B. J.},
  TITLE =        {Expedited approaches to whole cell electron tomography and organelle mark-up in situ in high-pressure frozen pancreatic islets},
  JOURNAL =      {J. Struct. Biol.},
  YEAR =         {2008},
  volume =       {161},
  number =       {},
  pages =        {298?C313}
}

@ARTICLE{Pierson:2010,
  AUTHOR =       {Pierson, J. and Fernandez, J. J. and Bos, E. and Amini, S. and Gnaegi, H. and Vos, M.and Bel, B. and Adolfsen, F. and Carrascosa, J. L. and Peters, P. J.},
  TITLE =        {Improving the technique of vitreous cryosectioning for cryo-electron tomography: Electrostatic charging for section attachment and implementation of an anti-contamination glove box},
  JOURNAL =      {J. Struct. Biol.},
  YEAR =         {2010},
  volume =       {169},
  number =       {},
  pages =        {219?C225}
}

@ARTICLE{Salje:2009,
  AUTHOR =       {Salje, J. and Zuber, B. and and Lowe, J.},
  TITLE =        {Electron cryomicroscopy of E. coli reveals filament bundles involved in plasmid DNA segregation},
  JOURNAL =      {Science},
  YEAR =         {2009},
  volume =       {323},
  number =       {},
  pages =        {509?C512}
}

@ARTICLE{Hsieh:2006,
  AUTHOR =       {Hsieh, C. E. and Leith, A. and Mannella, C. A. and Frank, J. and Marko, M.},
  TITLE =        {Towards highresolution three-dimensional imaging of native mammalian tissue: Electron tomography of frozen-hydrated rat liver sections},
  JOURNAL =      {J. Struct. Biol.},
  YEAR =         {2006},
  volume =       {153},
  number =       {},
  pages =        {1-13}
}

@ARTICLE{Gruska:2008,
  AUTHOR =       {Gruska, M. and Medalia, O. and Baumeister, W. and Leis, A.},
  TITLE =        {Electron tomography of vitreous sections from cultured mammalian cells},
  JOURNAL =      {J. Struct. Biol.},
  YEAR =         {2008},
  volume =       {161},
  number =       {},
  pages =        {384?C392}
}

@ARTICLE{Al-Amoudi:2007,
  AUTHOR =       {Al-Amoudi, A. and Diez, D. C. and Betts, M. J. and Frangakis, A. S.},
  TITLE =        {The molecular architecture of cadherins in native epidermal desmosomes},
  JOURNAL =      {Nature},
  YEAR =         {2007},
  volume =       {450},
  number =       {},
  pages =        {832?C837}
}

@ARTICLE{Bajaj:2003,
  AUTHOR =       {Bajaj, C. and Yu, Z. Y. and Auer, M.},
  TITLE =        {Volumetric feature extraction and visualization of tomographic molecular imaging},
  JOURNAL =      {J. Struct. Biol.},
  YEAR =         {2003},
  volume =       {144},
  number =       {},
  pages =        {132?C143}
}

@ARTICLE{Sandberg:2007,
  AUTHOR =       {Sandberg, K.},
  TITLE =        {Methods for image segmentation in cellular tomography},
  JOURNAL =      {Methods Cell Biol.},
  YEAR =         {2007},
  volume =       {79},

  number =       {},
  pages =        {769?C798}
}

@INPROCEEDINGS{Lizier:2008,
  author = {M.A.S. Lizier and J.F. Shepherd and L.G. Nonato and J. Comba and
	C.T. Silva},
  title = {Comparing Techniques for Tetrahedral Mesh Generation},
  booktitle = {Inaugural International Conference of the Engineering Mechanics Institute},
  year = {2008},
  owner = {lgn},
  timestamp = {2008.03.27}
}

@article{Koenderink:1992,
author = {Koenderink, Jan J and van Doorn, Andrea J},
doi = {10.1016/0262-8856(92)90076-F},
issn = {02628856},
journal = {Image and Vision Computing},
month = oct,
number = {8},
pages = {557--564},
title = {{Surface shape and curvature scales}},
url = {http://linkinghub.elsevier.com/retrieve/pii/026288569290076F},
volume = {10},
year = {1992}
}

@article{Xu:2004,
 author = {Xu, Guoliang},
 title = {Convergence of discrete {Laplace-Beltrami} operators over surfaces},
 journal = {Comput. Math. Appl.},
 issue_date = {August, 2004},
 volume = {48},
 number = {3-4},
 month = aug,
 year = {2004},
 issn = {0898-1221},
 pages = {347--360},
 numpages = {14},
 url = {http://dx.doi.org/10.1016/j.camwa.2004.05.001},
 doi = {10.1016/j.camwa.2004.05.001},
 acmid = {1665805},
 publisher = {Pergamon Press, Inc.},
 address = {Tarrytown, NY, USA},
 keywords = {Convergence, Laplace-Beltrami operator, Surface triangulation},
}

@article{Xu:2006,
 author = {Xu, Guoliang},
 title = {Convergence analysis of a discretization scheme for Gaussian curvature over triangular surfaces},
 journal = {Comput. Aided Geom. Des.},
 issue_date = {February 2006},
 volume = {23},
 number = {2},
 month = feb,
 year = {2006},
 issn = {0167-8396},
 pages = {193--207},
 numpages = {15},
 url = {http://dx.doi.org/10.1016/j.cagd.2005.07.002},
 doi = {10.1016/j.cagd.2005.07.002},
 acmid = {1133953},
 publisher = {Elsevier Science Publishers B. V.},
 address = {Amsterdam, The Netherlands, The Netherlands},
 keywords = {Gaussian curvature, convergence, parallelogram criterion, surface triangulation},
}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% KELIN XIA added end:

@ARTICLE{Cabani:1981,
  author = {Cabani, S. and Gianni, P. and Mollica, V and Lepori, L},
  title = {{Group Contributions to the Thermodynamic Properties of Non-Ionic Organic Solutes in Dilute Aqueous Solution}},
  journal = {Journal of Solution Chemistry},
  year = {1981},
  volume = {10},
  number={8},
  pages = {563--595}
}

@ARTICLE{Veenstra:1992,
  author = {Veenstra, D. and Ferguson, D. and Kollman, P.},
  month = {},
  year = {1992},
  title = {{How transferable are hydrogen parameters in molecular mechanics calculations?}},
  note = {},
  journal = {Journal of Computational Chemistry},
  volume = {13},
  number = {8},
  pages = {971-978}
}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%papers zhan add from 6/22 for the revision of apolar paper

%For the comment saying What is the connection of this method with methods developed in the 70's-90's to address %the structure of liquids at interfaces, including RISM (and their many corrections RISM-X, RISM3D, etc), MSA,
%Perkus-Yevick, density functional theory of liquids, HNC, Ornstein-Zernike, etc, etc, etc.

% RISM: the reference interaction site model
@Article{Ishizuka:2008,
  title={An integral equation theory for inhomogeneous molecular fluids: The reference interaction site model approach},
  author={Ishizuka, R. and Chong, S. H. and Hirata, F.},
  journal={Journal of Chemical Physics},
  volume={128},
  number={3},
  pages={34504--34504},
  year={2008},
  publisher={[New York, etc.]: American Institute of Physics.}
}

@Article{Hsu:1978,
  title={RISM calculation of the structure of liquid acetonitrile},
  author={Hsu, C. S. and Chandler, D.},
  journal={Molecular Physics},
  volume={36},
  number={1},
  pages={215--224},
  year={1978},
  publisher={Taylor \& Francis}
}
%RISM3D

@Article{Kovalenko:1999,
  title={Self-consistent description of a metal--water interface by the Kohn--Sham density functional
  theory and the three-dimensional reference interaction site model},
  author={Kovalenko, A. and Hirata, F.},
  journal={The Journal of chemical physics},
  volume={110},
  pages={10095},
  year={1999}
}

% MSA (mean spherical approximation):http://www.sklogwiki.org/SklogWiki/index.php/Mean_spherical_approximation

@Article{Lebowitz:1966,
  title={Mean spherical model for lattice gases with extended hard cores and continuum fluids},
  author={Lebowitz, J. L. and Percus, J. K.},
  journal={Physical Review},
  volume={144},
  number={1},
  pages={251},
  year={1966},
  publisher={APS}
}

@Article{Triolo:1976,
  title={Simple electrolytes in the mean spherical approximation},
  author={Triolo, R. and Grigera, J. R. and Blum, L.},
  journal={The Journal of Physical Chemistry},
  volume={80},
  number={17},
  pages={1858--1861},
  year={1976},
  publisher={ACS Publications}
}

%Perkus-Yevick: a closure relation for solving the OZ equation

@Article{Percus:1958,
  title={Analysis of classical statistical mechanics by means of collective coordinates},
  author={Percus, J. K. and Yevick, G. J.},
  journal={Physical Review},
  volume={110},
  number={1},
  pages={1},
  year={1958},
  publisher={APS}
}

@Article{Wertheim:1963,
  title={Exact solution of the Percus-Yevick integral equation for hard spheres},
  author={Wertheim, M. S.},
  journal={Physical Review Letters},
  volume={10},
  number={8},
  pages={321--323},
  year={1963},
  publisher={APS}
}

%density functional theory of liquids

@Article{Donley:1994,
  title={A density functional theory for pair correlation functions in molecular liquids},
  author={Donley, J. P. and Curro, J. G. and McCoy, J. D.},
  journal={The Journal of chemical physics},
  volume={101},
  pages={3205},
  year={1994}
}

@BOOK{Parr:1994,
  title={Density-functional theory of atoms and molecules},
  author={Parr, R. G. and Yang, W.},
  volume={16},
  year={1994},
  publisher={Oxford University Press, USA}
}

%HNC (Hypernetted-chain equation:  a closure relation to solve the Ornstein-Zernike equation
      %commonly applied in statistical mechanics and fluid theory, More details can be seen from
      %wiki: Classical-map hypernetted-chain method )

@Article{Van:1959,
  title={New method for the calculation of the pair correlation function. I},
  author={Van Leeuwen, J. M. J. and Groeneveld, J. and De Boer, J.},
  journal={Physica},
  volume={25},
  number={7-12},
  pages={792--808},
  year={1959},
  publisher={Elsevier}
}

%Ornstein-Zernike: is an integral equation for defining the direct correlation function. It basically describes
%how the correlation between two molecules can be calculated. Its applications can mainly be found in fluid theory.
%Percus-Yevick approximation, a closure relation for solving the OZ equation
%Hypernetted-chain equation, a closure relation for solving the OZ equation

@INPROCEEDINGS{Ornstein:1914,
  title={Accidental deviations of density and opalescence at the critical point of a single substance},
  author={Ornstein, L. S. and Zernike, F.},
  booktitle={Proc. Akad. Sci.(Amsterdam)},
  volume={17},
  pages={793},
  year={1914}
}

@Article{Percus:1964,
  title={The Equilibrium Theory of Classical Fluids},
  author={Percus, J. K. and Frisch, H. L. and Lebowitz, J. L.},
  journal={Editors: Frisch, HL, Lebowitz, JL, Editorial Benjamin},
  pages={1133},
  year={1964}
}

% The following cited paper for comment 5
%More recent papers that attempt at relating old and new liquid theories with focus on the interfaces, are,
%e.g., P. Koehl, H. Orland, and M. Delarue, Phys. Rev. Lett. 102, 087801 (2009) (this paper discusses
%liquid structure at the interface, but with less emphasis on the dielectric response) and S. A. Hassan, J.
%Phys. Chem. B 111, 227 (2007) (which focuses on the dielectric response at the interfaces, with less
%emphasis on the structure; the author discusses at length the physics of polar solvation). The authors
%should make an effort to put their method in context with these and other papers, and discuss the
%connection with both dielectric theory and theory of liquid structure. Many other papers can be found in
%the extensive literature that addresses these topics with more or less theoretical rigor (e.g., A. Rubinstein
%and S. Sherman, Biopolymers 87, 149 (2007)); yet all of them are perfectly aware of the serious problem
%one faces when modeling interfaces.

@Article{Koehl:2009,
  title={Beyond Poisson-Boltzmann: Modeling Biomolecule-Water and Water-Water Interactions},
  author={Koehl, P. and Orland, H. and Delarue, M.},
  journal={Physical review letters},
  volume={102},
  number={8},
  pages={087801},
  year={2009},
  publisher={NIH Public Access}
}

@Article{Hassan:2007,
  title={Liquid-structure forces and electrostatic modulation of biomolecular interactions in solution},
  author={Hassan, S. A.},
  journal={The Journal of Physical Chemistry B},
  volume={111},
  number={1},
  pages={227--241},
  year={2007},
  publisher={ACS Publications}
}


@Article{Rubinstein:2007,
  title={Evaluation of the influence of the internal aqueous solvent structure on electrostatic interactions at the protein-solvent interface by nonlocal continuum electrostatic approach},
  author={Rubinstein, A. and Sherman, S.},
  journal={Biopolymers},
  volume={87},
  number={2-3},
  pages={149--164},
  year={2007},
  publisher={Wiley Online Library}
}

%dielectric response of the liquid
@Article{Madden:1984,
  title={A consistent molecular treatment of dielectric phenomena},
  author={Madden, P. and Kivelson, D.},
  journal={Advances in chemical physics},
  pages={467--566},
  year={1984},
  publisher={Wiley Online Library}
}


@ARTICLE{Wei:2012,
  author = {Wei, Guo-Wei and Zheng, Qiong and Chen, Zhan and Xia, Kelin},
  month = {},
  year = {2012},
  title = {Variational multiscale models for charge transport},
  note = {},
  journal = {SIAM Review},
  volume = {54},
  number = {4},
  pages = {699 - 754}
}



@ARTICLE{Wei:2013,
  author = {Wei, Guo-Wei  },
  month = {},
  year = {2013},
  title = {Multiscale, multiphysics and multidomain models {I: Basic} theory},
  note = {},
  journal = {Journal of Theoretical and Computational Chemistry},
  volume = {12},
  number = {8},
  pages = {1341006 }
}
%%%%%%%%%%%%%%%% End Zhan Chen %%%%%%%%%%%%5


@ARTICLE{Decherchi:2013,
  author = {  Decherchi, S. and  Colmenares, J. and  Catalano, C. E. and  Spagnuolo, M. and  Alexov, E. and  Rocchia, W.  },
  title = {Between Algorithm and Model: {Different} Molecular Surface Definitions for the {Poisson-Boltzmann} Based Electrostatic Characterization of Biomolecules in Solution},
  journal = {Communications in Computational Physics},
  year = {2002},
  volume = {13},
  pages = {61-89}
}

@ARTICLE{MXChen:2012,
  author = {Chen, Minxin and Tu, Bin and  Lu, Benzhuo  },
  title = {Triangulated manifold meshing method preserving molecular surface topology},
  journal = { J. Mole. Graph. Model. },
  year = {2012},
  volume = {38},
  pages = {411-418 }
}

@ARTICLE{XFeng:2012a,
  author = {Feng, Xin and Xia, Kelin and Tong, Yiying and Wei, Guo-Wei},
  month = {},
  year = { 2012},
  title = {Geometric modeling of subcellular structures, organelles and large multiprotein complexes},
  note = {},
  journal = {International  Journal  for Numerical    Methods  in   Biomedical    Engineering},
  volume = {28},
  pages = { 1198-1223}
}








@ARTICLE{Cipriano:2009,
  author = {Cipriano, G.  and Phillips Jr., G. N. and  Gleicher, M.},
  month = {},
  year = {2009},
  title = {Multi-Scale Surface Descriptors},
  note = {},
  journal = {IEEE Transactions on Visualization and Computer Graphics },
  volume = {15},
  number = {},
  pages = {1201-1208}
}


@ARTICLE{Sazonov:2012,
  author = {Sazonov, Igor and Nithiarasu, Perumal},
  month = {},
  year = {2012},
  title = {Semi-automatic surface and volume mesh generation for subject-specific biomedical geometries},
  note = {},
  journal = {International Journal for Numerical Methods in Biomedical Engineering},
  volume = {28},
  number = {},
  pages = {133-157}
}


@ARTICLE{Marchandise:2010,
  author = {Marchandise, E and Compere, G and  Willemet, M and  Bricteux, G and  Geuzaine, C and  Remacle, J. F.},
  month = {},
  year = {2010},
  title = {Quality meshing based on STL triangulations for biomedical simulations},
  note = {},
  journal = {International Journal for Numerical Methods in Biomedical Engineering},
  volume = {26},
  number = {},
  pages = {876-889}
}




@ARTICLE{d'Otreppe:2012,
  author = {d'Otreppe, Vinciane and  Boman, Romain and Ponthot, Jean-Philippe},
  month = {},
  year = {2012},
  title = {Generating smooth surface meshes from multi-region medical images},
  note = {},
  journal = {International Journal for Numerical Methods in Biomedical Engineering},
  volume = {28},
  number = {},
  pages = {642-660}
}



@ARTICLE{SZhao:2011,
  author = {Zhao, Shan},
  month = {},
  year = {2012},
  title = { Pseudo-time-coupled nonlinear models for biomolecular surface representation and solvation analysis},
  note = {},
  journal = {International Journal for Numerical Methods in Biomedical Engineering},
  volume = {27},
  number = {},
  pages = {1964- 1981}
}


@ARTICLE{JLiang:2012,
  author = {Liang, Jie and Naveed, H. and Jimenez-Morales, D. and Adamian, L. and  Lin, Meishan},
  month = {},
  year = {2012},
  title = {Computational Studies of Membrane Proteins: {Models} and Predictions for Biological Understanding},
  note = {},
  journal = {Biochimica et Biophysica Acta (BBA) - Biomembranes},
  volume = {1818},
  number = {},
  pages = {927- 941 }
}



@ARTICLE{QWang:2012,
  author = {Wang, Qi and Zhang, Tianyu},
  month = {},
  year = {2012},
  title = {Kinetic Theory for biofilms},
  note = {},
  journal = {Discrete and Continuous Dynamical Systems-Series B},
  volume = {17},
  number = {},
  pages = {1027-1059}
}


@ARTICLE{Scott2010,
  author = {Scott, L. R.},
  title = {Nonstandard dielectric response},
  journal = {UChicago CS technical report},
  year = {2010},
  volume = {},
  pages = {}
}


@ARTICLE{DXXie2012,
  author = {Xie, D. and Jiang, Y. and  Brune, P. and  Scott, L. R.},
  title = {A fast solver for a nonlocal dielectric continuum model},
  journal = {SIAM Journal on Scientific Computing},
  year = {2012},
  volume = {34},
  pages = {B107 -B126}
}


@ARTICLE{LHHu:2012,
  author = {Hu, L. H. and Wei, G. W. },
  title = {Nonlinear    Poisson    equation   for    heterogeneous  media},
  journal = { Biophysical Journal},
  year = {2012},
  volume = {103},
  pages = {758 - 766}
}

@ARTICLE{LHHu:2014,
  author = {Hu, L. H. and Yang, S. Y. and  Wei, G. W. },
  title = {Simulation of inviscid compressible flows using PDE transform},
  journal = { Commun. Comput. Phys.},
  year = {2014},
  volume = {16},
  pages = {1201 - 1238}
}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%Kelin Xia


@ARTICLE{Du:1999,
  author = {Du, Q. and Faber, V. and Gunzburger, M },
  month = {},
  year = {1999},
  title = { Centroidal Voronoi tessellations: Applications and algorithms},
  note = {},
  journal = {SIAM Review},
  volume = {41},
  number = {4},
  pages = {637-676}
}

@ARTICLE{Ju:2002,
  author = {Ju, L. L. and Du, Q. and Gunzburger, M },
  month = {},
  year = {2002},
  title = { Probabilistic methods for centroidal Voronoi tessellations and their parallel implementations},
  note = {},
  journal = {Parallel Computing},
  volume = {28},
  number = {},
  pages = {1477?C1500}
}

@ARTICLE{Wan:2011,
  author = {Wan, M. and Wang, Y. and Wang, D. S.},
  month = {},
  year = {2011},
  title = { Variational surface reconstruction based on Delaunay triangulation and graph cut},
  note = {},
  journal = {Int. J. Numer. Meth. Engng},
  volume = {85},
  number = {},
  pages = {206?C229}
}


@ARTICLE{George:1991,
  author = {George, P. L. and Hecht, F. and Saltel, E. },
  month = {},
  year = {1991},
  title = { Automatic mesh generator with specified boundary},
  note = {},
  journal = {Computer Methods in Applied Mechanics and Engineering},
  volume = {92},
  number = {},
  pages = {269- 288}
}

@ARTICLE{Weatherill:1994,
  author = {Weatherill, N. P. and Hassan, O.},
  month = {},
  year = {1994},
  title = { Efficient three-dimensional Delaunay triangulation with automatic point creation and imposed boundary constraints},
  note = {},
  journal = {Int. J. Numer. Meth. Engng},
  volume = {37},
  number = {},
  pages = {2005-2039}
}

@ARTICLE{Sazonov:2011,
  author = {Sazonov, I. and Yeo, S. Y. and Bevan, L. T. and Xie, X. H. and Loon, R. V. and Nithiarasu, P.},
  month = {},
  year = {2011},
  title = { Modelling pipeline for subject-specific arterial blood flow??A review},
  note = {},
  journal = {International Journal for Numerical Methods in Biomedical Engineering},
  volume = {27},
  number = {},
  pages = {1868-1910}
}

@ARTICLE{Saksono:2012,
  author = {Saksono, P. H. and Nithiarasu, P. and Sazonov, I.},
  month = {},
  year = {2012},
  title = { Numerical prediction of heat transfer patterns in a subject-specific human upper airway},
  note = {},
  journal = {Journal of Heat Transfer},
  volume = {134},
  number = {031022},
  pages = {1-9}
}

@ARTICLE{Koltun:1965,
  author = {Koltun, W. L.},
  month = {},
  year = {1965},
  title = {  Precision space-filling atomic models},
  note = {},
  journal = {Biopolymers},
  volume = {3},
  number = {},
  pages = {667-679}
}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%The above is added by Kelin Xia


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% KELIN XIA added begin:
@ARTICLE{Fernandez:2009,
  AUTHOR =       {Fernandez,J.J.},
  TITLE =        {TOMOBFLOW: feature-preserving noise filtering for electron tomography},
  JOURNAL =      {BMC Bioinformatics},
  YEAR =         {2009},
  volume =       {178},
  number =       {},
  pages =        {1-10}
}

@INPROCEEDINGS{Fernandez:2007,
  AUTHOR =       {Fernandez,J.J. and Li, S. and Lucic, V.},
  TITLE =        {Three-Dimensional Anisotropic Noise Reduction with Automated Parameter Tuning: Application to Electron Cryotomography},
  booktitle =    {Current Topics in Artificial Intelligence},
  YEAR =         {2007},
  volume =       {4788},
  number =       {},
  pages =        {60-69}
}

@ARTICLE{Stoschek:1997,
  AUTHOR =       {Stoschek, A. and Hegerl, R.},
  TITLE =        {Denoising of electron tomographic reconstructions using multiscale transformations},
  JOURNAL =      {J. Struct. Biol.},
  YEAR =         {1997},
  volume =       {120},
  number =       {},
  pages =        {257?C265}
}


@ARTICLE{Frangakis:2001,
  AUTHOR =       {Frangakis, A. S. and Hegerl, R.},
  TITLE =        {Noise reduction in electron tomographic reconstructions using nonlinear anisotropic diffusion},
  JOURNAL =      {J. Struct. Biol.},
  YEAR =         {2001},
  volume =       {135},
  number =       {},
  pages =        {239?C250}
}

@ARTICLE{Fernandez:2003,
  AUTHOR =       {Fernandez, J. J. and Li, S.},
  TITLE =        {An improved algorithm for anisotropic nonlinear diffusion for denoising cryo-tomograms},
  JOURNAL =      {J. Struct. Biol.},
  YEAR =         {2003},
  volume =       {144},
  number =       {},
  pages =        {152?C161}
}

@ARTICLE{Tomasi:1998,
  AUTHOR =       {Tomasi, C. and Manduchi, R.},
  TITLE =        {Bilateral filtering for gray and color images},
  JOURNAL =      {Proc. ICCV},
  YEAR =         {1998},
  volume =       {98},
  number =       {},
  pages =        {839?C846}
}

@ARTICLE{Jiang:2003,
  AUTHOR =       {Jiang, W. and Baker, M. L.and Wu, Q. and Bajaj, C. and Chiu, W.},
  TITLE =        {Applications of a bilateral denoising filter in biological electron microscopy},
  JOURNAL =      {J. Struct. Biol.},
  YEAR =         {2003},
  volume =       {144},
  number =       {},
  pages =        {114 - 122}
}

@ARTICLE{Pantelic:2006,
  AUTHOR =       {Pantelic, R. S. and Rothnagel, R.and Huang, C. Y. and Muller, D. and Woolford, D. and Landsberg, M. J. and McDowall, A. and Pailthorpe, B. and Young, P. R. and Banks, J. and Hankamer, B. and Ericksson, G.},
  TITLE =        {The discriminative bilateral filter: An enhanced denoising filter for electron microscopy data},
  JOURNAL =      {J. Struct. Biol.},
  YEAR =         {2006},
  volume =       {155},
  number =       {},
  pages =        {395?C408}
}

@ARTICLE{vanderHeide:2007,
  AUTHOR =       {van der Heide, P. and Xu, X. P. and Marsh, B. J. and Hanein, D. and Volkmann, N.},
  TITLE =        {Efficient automatic noise reduction of electron tomographic reconstructions based on iterative median filtering},
  JOURNAL =      {J. Struct. Biol.},
  YEAR =         {2007},
  volume =       {158},
  number =       {},
  pages =        {196?C204}
}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%the above papers are related to denoise method



@ARTICLE{Noske:2008,
  AUTHOR =       {Noske, A. B. and Costin, A. J. and Morgan, G. P. and Marsh, B. J.},
  TITLE =        {Expedited approaches to whole cell electron tomography and organelle mark-up in situ in high-pressure frozen pancreatic islets},
  JOURNAL =      {J. Struct. Biol.},
  YEAR =         {2008},
  volume =       {161},
  number =       {},
  pages =        {298?C313}
}

@ARTICLE{Pierson:2010,
  AUTHOR =       {Pierson, J. and Fernandez, J. J. and Bos, E. and Amini, S. and Gnaegi, H. and Vos, M.and Bel, B. and Adolfsen, F. and Carrascosa, J. L. and Peters, P. J.},
  TITLE =        {Improving the technique of vitreous cryosectioning for cryo-electron tomography: Electrostatic charging for section attachment and implementation of an anti-contamination glove box},
  JOURNAL =      {J. Struct. Biol.},
  YEAR =         {2010},
  volume =       {169},
  number =       {},
  pages =        {219?C225}
}

@ARTICLE{Salje:2009,
  AUTHOR =       {Salje, J. and Zuber, B. and and Lowe, J.},
  TITLE =        {Electron cryomicroscopy of E. coli reveals filament bundles involved in plasmid DNA segregation},
  JOURNAL =      {Science},
  YEAR =         {2009},
  volume =       {323},
  number =       {},
  pages =        {509?C512}
}

@ARTICLE{Hsieh:2006,
  AUTHOR =       {Hsieh, C. E. and Leith, A. and Mannella, C. A. and Frank, J. and Marko, M.},
  TITLE =        {Towards highresolution three-dimensional imaging of native mammalian tissue: Electron tomography of frozen-hydrated rat liver sections},
  JOURNAL =      {J. Struct. Biol.},
  YEAR =         {2006},
  volume =       {153},
  number =       {},
  pages =        {1-13}
}

@ARTICLE{Gruska:2008,
  AUTHOR =       {Gruska, M. and Medalia, O. and Baumeister, W. and Leis, A.},
  TITLE =        {Electron tomography of vitreous sections from cultured mammalian cells},
  JOURNAL =      {J. Struct. Biol.},
  YEAR =         {2008},
  volume =       {161},
  number =       {},
  pages =        {384-392}
}

@ARTICLE{Al-Amoudi:2007,
  AUTHOR =       {Al-Amoudi, A. and Diez, D. C. and Betts, M. J. and Frangakis, A. S.},
  TITLE =        {The molecular architecture of cadherins in native epidermal desmosomes},
  JOURNAL =      {Nature},
  YEAR =         {2007},
  volume =       {450},
  number =       {},
  pages =        {832?C837}
}

@ARTICLE{Bajaj:2003,
  AUTHOR =       {Bajaj, C. and Yu, Z. Y. and Auer, M.},
  TITLE =        {Volumetric feature extraction and visualization of tomographic molecular imaging},
  JOURNAL =      {J. Struct. Biol.},
  YEAR =         {2003},
  volume =       {144},
  number =       {},
  pages =        {132-143}
}

@ARTICLE{Sandberg:2007,
  AUTHOR =       {Sandberg, K.},
  TITLE =        {Methods for image segmentation in cellular tomography},
  JOURNAL =      {Methods Cell Biol.},
  YEAR =         {2007},
  volume =       {79},
  number =       {},
  pages =        {769-798}
}

@ARTICLE{Kindlmann:2003,
  AUTHOR = {Kindlmann, G. and Whitaker, R. and Tasdizen, T. and M{\"o}ller, T.},
  TITLE  = {Curvature-based transfer functions for direct volume rendering: methods and applications},
  JOURNAL = {Proc. IEEE Visualization},
  YEAR = {2003},
  volume = {},
  pages = {},
  number = {}
}


@ARTICLE{Soldea:2006,
  AUTHOR = {Soldea, O. and Elber, G. and Rivlin, E. },
  TITLE = {Global segmentation and curvature analysis of volumetric data sets using trivariate B-spline functions},
  JOURNAL = {IEEE Trans. on PAMI},
  YEAR = {2006},
  volume = {28},
  pages = {265 - 278},
  number = {2}
}




%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% KELIN XIA added end:
%%% Wei ---



@ARTICLE{Kuo:2010,
  author = { Kuo, Y. L.; Cleghorn, W. L. },
  title = { Curvature- and displacement-based finite element analyses of flexible slider crank mechanisms },
  year = {2010},
  journal = {International Journal for Numerical Methods in Biomedical Engineering},
  volume = {26 },
  pages = {1228-1245}
}

@ARTICLE{KLow:2012,
  author = {Low, K. and van Loon, R. and Sazonov, I. and Bevan, R. L. T.  and  Nithiarasu, P. },
  title = {An improved baseline model for a human arterial network to study
the impact of aneurysms on pressure-flow waveforms},
  year = {2012},
  journal = {International Journal for Numerical Methods in Biomedical Engineering},
  volume = {},
  pages = {}
}



@ARTICLE{Younes:2010,
  author = { Younes, A.  and Fahs, M. and   Ackerer, P. },
  title = { An efficient geometric approach to solve the slope limiting problem with the Discontinuous Galerkin method on unstructured triangles },
  year = {2010},
  journal = {International Journal for Numerical Methods in Biomedical Engineering},
  volume = {26},
  pages = {1824-1835}
}


@ARTICLE{Scott:2010,
  author = { Scott, M. H. and Hamutcuoglu, O. M. },
  title = { Analytical sensitivity of interpolatory quadrature in force-based frame elements  },
  year = {2010},
  journal = {International Journal for Numerical Methods in Biomedical Engineering},
  volume = {26},
  pages = {1586-1595}
}


@ARTICLE{Xiao:2010,
  author = {  Xiao, Y. X. and Shu, S. and Zhang, P. and Tan, M. },
  title = {  An algebraic multigrid method for isotropic linear elasticity problems on anisotropic meshes  },
  year = {2010},
  journal = {International Journal for Numerical Methods in Biomedical Engineering},
  volume = {26},
  pages = {534 - 553}
}



@ARTICLE{Salo:2012,
  author = { Salo, Zoryana and Beek, Maarten and Whyne, Cari Marisa },
  title = {   Evaluation of mesh morphing and mapping techniques in patient specific modelling of the human pelvis   },
  year = {2012},
  journal = {International Journal for Numerical Methods in Biomedical Engineering},
  volume = {28},
  pages = {904 - 913}
}


@ARTICLE{Qian:2011,
  author = { Qian, Jing and  Lu, Jia },
  title = {    Point-cloud method for image-based biomechanical stress analysis  },
  year = {2011},
  journal = {International Journal for Numerical Methods in Biomedical Engineering},
  volume = {27},
  pages = {1493 - 1506}
}


@ARTICLE{Pan:2011,
  author = {Pan, Wenke and Wheel, Marcus },
  title = { A finite-volume method for solids with a rotational degrees of freedom based on the 6-node triangle },
  year = {2011},
  journal = {International Journal for Numerical Methods in Biomedical Engineering},
  volume = {27},
  pages = {1411 - 1426}
}



@ARTICLE{Mohapatra:2011,
  author = { Mohapatra, Jugal and Natesan, Srinivasan },
  title = { Uniformly convergent numerical method for singularly perturbed differential-difference equation using grid equidistribution },
  year = {2011},
  journal = {International Journal for Numerical Methods in Biomedical Engineering},
  volume = {27},
  pages = {1427 - 1445}
}



@ARTICLE{Miki:2011,
  author = {  Miki, T. and  Imai, Y. and  Ishikawa, T. and  Wada, S. and  Aoki, T. and  Yamaguchi, T.},
  title = {A fourth-order Cartesian local mesh refinement method for the computational fluid dynamics of physiological flow in multi-generation branched vessels },
  year = {2011},
  journal = {International Journal for Numerical Methods in Biomedical Engineering},
  volume = {27},
  pages = {424-435}
}

@ARTICLE{Ko:2010,
  author = { Ko, J. H. and   Park, S. H. and  Park, H. C. and    Byun, D.},
  title = { Finite macro-element-based volume grid deformation for large moving boundary problems  },
  year = {2010},
  journal = {International Journal for Numerical Methods in Biomedical Engineering},
  volume = {26},
  pages = {1656-1673}
}

@ARTICLE{Yamakawa:2010,
  author = {Yamakawa, Soji and Shimada, Kenji  },
  title = { 88-Element solution to Schneiders' pyramid hex-meshing problem  },
  year = {2010},
  journal = {International Journal for Numerical Methods in Biomedical Engineering},
  volume = {26},
  pages = {1700-1712}
}




@ARTICLE{Phongthanapanich:2010,
  author = {Phongthanapanich, S. and Dechaumphai, P.},
  title = {   Finite volume method for convection-diffusion-reaction equation on triangular meshes   },
  year = {2010},
  journal = {International Journal for Numerical Methods in Biomedical Engineering},
  volume = {26},
  pages = {716-727 }
}





@ARTICLE{Lv:2010,
  author = {Lv, Guixia and Shen, Longjun and Shen, Zhijun},
  title = { Numerical methods for energy flux of temperature diffusion equation on unstructured meshes  },
  year = {2010},
  journal = {International Journal for Numerical Methods in Biomedical Engineering},
  volume = {26},
  pages = {646-665}
}

@ARTICLE{Botti:2010,
  author = {Botti, Lorenzo and Piccinelli, Marina and Ene-Iordache, Bogdan and Remuzzi, Andrea and  Antiga, Luca},
  title = { An adaptive mesh refinement solver for large-scale simulation of biological flows   },
  year = {2010},
  journal = {International Journal for Numerical Methods in Biomedical Engineering},
  volume = {26},
  pages = {86-100}
}

@ARTICLE{Tsai:2012,
  author = {Tsai, Kunyu and Ma, Jianwei and Ye, Datian and Wu, Jian},
  title = {  Curvelet processing of MRI for local image enhancement   },
  year = {2012},
  journal = {International Journal for Numerical Methods in Biomedical Engineering},
  volume = {28},
  pages = {661-677}
 }

@ARTICLE{MPan:2011,
  author = {Pan, Mei-sen and Tang, Jing-tian and Rong, Qiu-sheng and Zhang, Fen},
  title = {  Medical image registration using modified iterative closest points   },
  year = {2011},
  journal = {International Journal for Numerical Methods in Biomedical Engineering},
  volume = {27},
  pages = {1150-1166}
  }

@ARTICLE{Radaelli:2010,
  author = {Radaelli, A. G. and Peiro, J.},
  title = {   On the segmentation of vascular geometries from medical images   },
  year = {2010},
  journal = {International Journal for Numerical Methods in Biomedical Engineering},
  volume = {26},
  pages = {3-34 }
  }



@ARTICLE{Twarock:2008,
  author = {Twarock, R. and  Jonoska, N.},
  title = {  Blueprints for dodecahedral DNA cages   },
  year = {2008},
  journal = {Journal of Physics A: Mathematical and Theoretical},
  volume = {41},
  pages = { 304043 -304057}
  }


@ARTICLE{Jonoska:2012,
  author = {Jonoska, N. and Twarock, R. },
  title = {A Note on Genome Organisation in RNA Viruses with Icosahedral Symmetry    },
  year = {submitted 2012},
  journal = {J. Theor. Biol.},
  volume = {},
  pages = {}
  }



	
	

@ARTICLE{Hughes:2012,
  author = { Hughes, J. M. and  Mao, D. and  Rockmore, D. N. and  Wang, Y. and  Wu, Q.  },
  title = {Empirical Mode Decomposition Analysis for Visual Stylometry  },
  year = { 2012},
  journal = { IEEE T.   Pattern Analysis Machine Intelligence},
  volume = {34},
  pages = {2147-2157}
  }


@ARTICLE{JLi:2012,
  author = {  Li, J. and  Yao, L. and    Hendriks, E.  and  Wang, J. Z.    },
  title = {Rhythmic Brushstrokes Distinguish van Gogh from His Contemporaries: Findings via Automated Brushstroke Extraction  },
  year = { 2012},
  journal = { IEEE T.   Pattern Analysis Machine Intelligence},
  volume = {34},
  pages = {1159-1176}
  }



@ARTICLE{Sawant:2011,
  author = {  Sawant, N. and   Li, J. and  Wang, J. Z.    },
  title = {Automatic image semantic interpretation using social action and tagging data },
  year = { 2011},
  journal = { MULTIMEDIA TOOLS AND APPLICATIONS},
  volume = {51},
  pages = {213-246}
  }



@ARTICLE{Lee:2012,
  author = { Lee, H. and   Li, J. and  Wang, J. Z.    },
  title = { Variable Selection for Clustering by Separability Based on Ridgelines },
  year = { 2012},
  journal = {JOURNAL OF COMPUTATIONAL AND GRAPHICAL STATISTICS},
  volume = {21},
  pages = {315-337}
  }


@ARTICLE{Darnell:2008,
  author = { Darnell, S. J. and LeGault, L. and  Mitchell, J. C.  },
  title = {  KFC Server: interactive forecasting of protein interaction hot spots },
  year = { 2008},
  journal = {NUCLEIC ACIDS RESEARCH },
  volume = {36},
  pages = {W265-W269 }
  }


@ARTICLE{Demerdash:2009,
  author = { Demerdash, O. N. A. and Daily, M. D. and Mitchell, J. C. },
  title = { Structure-Based Predictive Models for Allosteric Hot Spots },
  year = { 2009},
  journal = {PLOS Computational Biology },
  volume = {5},
  pages = {e1000531}
  }


@article{NHuang:1996,
   author = {Huang, N. E. and Long, S. R. and Shen, Z.},
   title = {The mechanism for frequency downshift in nonlinear wave evolution},
   journal = {Advances in Applied Mechanics, Vol 32},
   volume = {32},
   pages = {59},
   year = {1996}
}

@article{NHuang:1998,
   author = {Huang, N. E. and Shen, Z. and Long, S. R. and Wu, M. L. C. and Shih, H. H. and Zheng, Q. N. and Yen, N. C. and Tung, C. C. and Liu, H. H.},
   title = {{The empirical mode decomposition and the {Hilbert} spectrum for nonlinear and non-stationary time series analysis}},
   journal = {Proceedings of the Royal Society of London Series a-Mathematical Physical and Engineering Sciences},
   volume = {454},
   number = {1971},
   pages = {903-995},
   year = {1998}
}

@article{NHuang:1999,
   author = {Huang, N. E. and Shen, Z. and Long, S. R.},
   title = {{A new view of nonlinear water waves: The {Hilbert} spectrum}},
   journal = {Annual Review of Fluid Mechanics},
   volume = {31},
   pages = {417-457},
   year = {1999}
}

@article{QChen:2006,
   author = {Chen, Q. H. and Huang, N. and Riemenschneider, S. and Xu, Y. S.},
   title = {A {B}-spline approach for empirical mode decompositions},
   journal = {Advances in Computational Mathematics},
   volume = {24},
   number = {1-4},
   pages = {171-195},
   year = {2006}
}


@article{GRilling:2007,
   author = {Rilling, G. and Flandrin, P. and Goncalves, P. and Lilly, J. M.},
   title = {Bivariate empirical mode decomposition},
   journal = {{IEEE} Signal Processing Letters},
   volume = {14},
   pages = {936-939},
   year = {2007}
}


@ARTICLE{YTang:2010,
author = {Tang, Ya-Wen and Tai, Cheng-Chi and Su, Ching-Chau and Chen, Chien-Yi and Chen, Jiann-Fuh},
year = {2010},
title = {A correlated empirical mode decomposition method for partial discharge signal denoising},
journal = {Measure. Science Tech.},
volume = {21},
number = {},
pages = {085106}
}

@BOOK{IDaubechies:1992,
author = {Daubechies, I.},
title = {Ten Lectures on Wavelets},
publisher = {{SIAM}, Philadelphia},
year = {1992}
}


@article{FMeyer:1997,
   author = {Meyer, F. G. and Coifman, R. R.},
   title = {Brushlets: A tool for directional image analysis and image compression},
   journal = {Applied and Computational Harmonic Analysis},
   volume = {4},
   number = {2},
   pages = {147-187},
   year = {1997}
}

@article{YChen:1995,
   author = {Chen, Y. M. and Li, J. Y. and Lin, F. H.},
   title = {PARTIAL REGULARITY FOR WEAK HEAT FLOWS INTO SPHERES},
   journal = {Communications on Pure and Applied Mathematics},
   volume = {48},
   number = {4},
   pages = {429-448},
   year = {1995}
}

@article{MFarge:1992,
   author = {Farge, M.},
   title = {WAVELET TRANSFORMS AND THEIR APPLICATIONS TO TURBULENCE},
   journal = {Annual Review of Fluid Mechanics},
   volume = {24},
   pages = {395-457},
   year = {1992}
}

@article{GSpedding:1993a,
   author = {Spedding, G. R. and Browand, F. K. and Huang, N. E. and Long, S. R.},
   title = {A 2-D COMPLEX WAVELET ANALYSIS OF AN UNSTEADY WIND-GENERATED SURFACE-WAVE FIELD},
   journal = {Dynamics of Atmospheres and Oceans},
   volume = {20},
   number = {1-2},
   pages = {55-77},
   year = {1993}
}


@article{GWei:2000,
  title={Wavelets generated by using discrete singular convolution kernels},
  author={Wei, G. W.},
  journal={Journal of Physics A: Mathematical and General},
  volume={33},
  pages={8577 -- 8596},
  year={2000},
  publisher={IOP Publishing}
}

@article{JJin:1999,
   author = {Jin, J. H. and Shi, J. J.},
   title = {Feature-preserving data compression of stamping tonnage information using wavelets},
   journal = {Technometrics},
   volume = {41},
   number = {4},
   pages = {327-339},
   year = {1999}
}

@article{SGuan:2002,
  title={{A wavelet method for the characterization of spatiotemporal patterns}},
  author={Guan, S. and Lai, C.H. and Wei, GW},
  journal={Physica D: Nonlinear Phenomena},
  volume={163},
  number={1-2},
  pages={49--79},
  issn={0167-2789},
  year={2002},
  publisher={Elsevier}
}

@book{YChan:1995,
  title={{Wavelet basics}},
  author={Chan, YT},
  isbn={0792395360},
  year={1995},
  publisher={Springer}
}


@article{JLi:2008,
  title={ Real-time computerized annotation of pictures},
  author={Li, J. and  Wang, J. Z. },
  journal={IEEE T.   Pattern Analysis Machine Intelligence},
  volume={30},
  number={},
  pages={ 985 - 1002 },
  issn={},
  year={2008},
  publisher={}
}


@ARTICLE{Namhee:2012,
  author = {Kim, N. and Schlick, T. },
  title = {A New Toolkit for Modeling RNA from a Pseudo-Torsional Space: Commentary on “Discrete RNA libraries from pseudo-torsional space- by Humphris-Narayanan and Pyle },
  year = {2012},
  journal = {Journal of Molecular Biology},
  volume = {421},
  pages = {1-5}
  }

@ARTICLE{Joseph:2011,
  author = {Izzo,J. and Kim, N. and Elmetwaly S. and Schlick, T. },
  title = {RAG: An update to the RNA-As-Graphs resource },
  year = {2011},
  journal = {BMC Bioinformatics},
  volume = {12},
  pages = {1-17}
  }
%-----------------------------------------

@ARTICLE{Ren:2013,
  author = {Ren, P. and   Chun, J. and    Thomas, D. G. and   Schnieders, M. J. and Marucho, M.  and  Zhang, J.  and  Baker, N. A.   },
  title = { Biomolecular electrostatics and solvation: a computational perspective },
  year = {2013},
  journal = {Quart. Rev. Biophys.},
  volume = { },
  pages = { }
  }


@ARTICLE{Rosenfeld:1993,
  author = { Rosenfeld, Y.  },
  title = {  Free energy model for inhomogeneous fluid mixtures: Yukawa charged hard spheres, general interactions, and plasmas },
  year = {1993},
  journal = {J. Chem. Phys.},
  volume = {98 },
  pages = { 8126-8148}
  }


@ARTICLE{Rosenfeld:1997,
  author = { Rosenfeld, Y. and  Schmidt, M. and Lowen, H. and Tarazona, P.  },
  title = {  Fundamental-Measure Free-Energy Density Functional for Hard Spheres: Dimensional Crossover and Freezing },
  year = {1997},
  journal = {Phys. Rev. E },
  volume = {55},
  pages = { 4245-4263}
  }


@ARTICLE{Hoye:1978,
  author = { Hoye, J. S. and Blum, L.   },
  title = { Mean Spherical Model for Asymmetric Electrolytes - Thermodynamics and Pair Correlation-Function },
  year = {1978},
  journal = { Mol. Phys.  },
  volume = {35},
  pages = { 299-300}
  }



@ARTICLE{Gillespie:2003,
  author = { Gillespie, D. and  Nonner, W. and  Eisenberg, R.S.  },
  title = {  Density functional theory of charged, hard-sphere fluids },
  year = {2003},
  journal = { Phys. Rev. E},
  volume = {68 },
  pages = {  031503}
  }

@ARTICLE{Knepley:2010,
  author = {Knepley, M.G. and  Karpeev, D. A. and  Davidovits,  S. and  Eisenberg, R. S. and  Gillespie, D.},
  title = {   An efficient algorithm for classical density functional theory in three dimensions: Ionic solutions },
  year = {2010},
  journal = {J. Chem.   Phys.  },
  volume = {132 },
  pages = {  124101}
  }



@ARTICLE{Patra:1999,
  author = { Patra, C. N.  and   Yethiraj, A.},
  title = {   Density Functional Theory for the Distribution of Small Ions around Polyions},
  year = {1999},
  journal = {J.     Phys. Chem. B  },
  volume = {101},
  pages = {6080-6087}
  }


@ARTICLE{Patra:2000,
  author = { Patra, C. N.  and   Yethiraj, A.},
  title = {  Density Functional Theory for the Nonspecific Binding of Salt to Polyelectrolytes: Thermodynamic Properties},
  year = {2000},
  journal = {Biophys. J. },
  volume = {78},
  pages = {699-706}
  }

@ARTICLE{KWang:2004,
  author = { Wang, K. and Yu, Y.-X. and  and Gao, G.-H. },
  title = {   Density functional study on the structures and thermodynamic properties of small ions around polyanionic DNA},
  year = {2004},
  journal = { Phys. Rev. E },
  volume = {70},
  pages = {011912}
  }


@ARTICLE{Thomas:2013,
  author = { Thomas, D.G. and Chun, J. and  Chen, Z. and Wei, G. W.  and Baker, N. A.  },
  title = {   Parameterization of a Geometric Flow Implicit Solvation Model},
  year = {2013},
  journal = { J. Comput. Chem. },
  volume = {24},
  pages = {687-695}
  }



@ARTICLE{Schneck:2012,
  author = { Schneck, E. and  Sedlmeier, F. and  Netz, R. R. },
  title = {  Hydration repulsion between biomembranes results from an interplay of dehydration and depolarization},
  year = {2012},
  journal = {PNAS},
  volume = {109},
  pages = { 14405-14409}
  }



@ARTICLE{Kirmizialtin:2012,
  author = {  Kirmizialtin, S. and  Pabit, S. A. and  Meisburger, S. P. and Pollack, L. and Elber, R.  },
  title = { RNA and Its Ionic Cloud: Solution Scattering Experiments and Atomically Detailed Simulations},
  year = {2012},
  journal = { Biophysical J.},
  volume = {102},
  pages = { 819-828}
  }




@ARTICLE{Mukhopadhyay:2012,
  author = { Mukhopadhyay, A. and Fenley, A. T.  and Tolokh, I. S. and  Onufriev, A. V.  },
  title = {  Charge Hydration Asymmetry: The Basic Principle and How to Use it to Test and Improve Waster Models},
  year = {2012},
  journal = { J. Phys. Chem. B},
  volume = {116},
  pages = { 9776-9783}
  }




@ARTICLE{Yoo:2012,
  author = { Yoo, J. and  Aksimentiev, A. },
  title = { Competitive binding of cations to duplex DNA revealed through molecular dynamics simulations},
  year = {2005},
  journal = { J. Phys. Chem. B},
  volume = {116},
  pages = { 12946 - 12954}
  }


@ARTICLE{JZWu:2007,
  author = { Wu, J. Z. and  Li, Z. D. },
  title = { Density-Functional Theory for Complex Fluids},
  year = {2007},
  journal = { Annu. Rev. Phys. Chem.},
  volume = {58},
  pages = { 85-112}
  }



@ARTICLE{YXYu:2004,
  author = { Yu, Y. X.  and  Wu, J. Z. and Gao, G. H. },
  title = { Density-functional theory of spherical electric double layers
and $\zeta$ potentials of colloidal particles in restricted-primitive-model
electrolyte solutions},
  year = {2004},
  journal = {J. Chem. Phys. },
  volume = {120},
  pages = { 7223-7233}
  }


@ARTICLE{Waisman:1972,
  author = {   Waisman, E. and  Lebowitz, J. L. },
  title = { Mean Spherical Model Integral Equation for Charged Hard Spheres
{I.} Method of Solution},
  year = {1972},
  journal = {J. Chem. Phys. },
  volume = {56},
  pages = { 3086-3093}
  }



@ARTICLE{Zerah:1986,
  author = {  Zerah, G. and  Hansen, J. P. },
  title = { Self-consistent integral equations for fluid pair distribution functions: Another
attempt},
  year = {1984},
  journal = {J. Chem. Phys. },
  volume = {84},
  pages = { 2336-2043}
  }


@ARTICLE{Sushko:2010,
  author = { Sushko,  M. L. and  Liu, J.},
  title = { Structural Rearrangements in Self-Assembled Surfactant Layers at Surfaces},
  year = {2010},
  journal = {J. Phys. Chem.  B},
  volume = {114},
  pages = { 3847-3854}
  }


@ARTICLE{Sushko:2011,
  author = { Sushko,  M. L. and  Liu, J.},
  title = { Surfactant Two-Dimensional Self-Assembly under Confinement},
  year = {2011},
  journal = {J. Phys. Chem.  B},
  volume = {115},
  pages = { 4322-4328}
  }






@ARTICLE{Sushko:2009,
  author = { Sushko,  M. L.  },
  title = { Nanomechanics of organic/inorganic interfaces: a theoretical insight},
  year = {2009},
  journal = {Faraday Discussions},
  volume = {143},
  pages = { 63-80}
  }







@ARTICLE{Sushko:2008,
  author = { Sushko,  M. L.  and  Harding, J. H. and Shluger, A. L. and  McKendry, R. A. and Watari, M.},
  title = { Physics of Nanomechanical Biosensing on Cantilever Arrays},
  year = {2008},
  journal = {Advanced Materials},
  volume = { 20},
  pages = { 3848-3853}
  }


@ARTICLE{Sushko:2010b,
  author = { Sushko,  M. L.  and   Rosso,  K. M. and  Liu, J.},
  title = { Size effects on Li$^+$/electron conductivity in TiO$_2$ nanoparticles},
  year = {2010},
  journal = {Journal of Physical Chemistry Letters},
  volume = { 1},
  pages = { 1967-1972}
  }



@ARTICLE{Sushko:2010c,
  author = { Sushko,  M. L.  and   Rosso,  K. M. and  Liu, J.},
  title = { The Mechanism of Li$^+$/Electron Conductivity in Rutile and Anatase TiO$_2$},
  year = {2010},
  journal = {Journal of Physical Chemistry C},
  volume = { 114},
  pages = { 20277-20283}
  }



@ARTICLE{DPCao:2005,
  author = { Cao, D. P. and Wu, J. Z. },
  title = { Microstructure of block copolymers near selective surfaces: Theoretical predictions and configurational-bias Monte Carlo simulation},
  year = {2005},
  journal = {Macromolecules},
  volume = {38},
  pages = { 971-978}
  }


@ARTICLE{XYYu:2002,
  author = { Yu, X. Y. and Wu, J. Z. },
  title = { Structures of hard-sphere fluids from a modified fundamental-measure theory},
  year = {2002},
  journal = { Journal of Chemical Physics},
  volume = {117},
  pages = { 10156-10164}
  }



@ARTICLE{Blum:1975,
  author = {  Blum, L. },
  title = { Mean Spherical Model for Asymmetric Electrolytes. 1. Method of Solution},
  year = {1975},
  journal = {Molecular Physics },
  volume = {30},
  pages = { 1529-1535}
  }



@ARTICLE{Chandler:1973,
  author = {  Chandler, D. },
  title = { Derivation of an integral equation for pair correlation functions in molecular fluids},
  year = {1973},
  journal = {J. Chem. Phys. },
  volume = {59},
  pages = { 2742-2746 }
  }

@ARTICLE{ZGuo:2013,
  author = {  Guo, Z. and Li, B. and Dzubiella, J. and  Cheng, Li-Tien and McCammon, J. A. and Che, J.},
  title = { Evaluation of Hydration Free Energy by Level-Set Variational Implicit-Solvent Model with Coulomb-Field Approximation
},
  year = {accepted 2013},
  journal = {J. Chem. Theory Comput.},
  volume = {},
  pages = {}
  }


@ARTICLE{Grossfield:2003,
  author = {  Grossfield, A. and Ren, P. Y. and Ponder, J. W.},
  title = {  Ion solvation thermodynamics from simulation with a polarizable force field
},
  year = { 2003},
  journal = {J. Amer. Chem. Soc.},
  volume = {125},
  pages = {15671-15682}
  }


@ARTICLE{Ponder:2010,
  author = {   Ponder, J. W.  and Wu, C. J. and  Ren, P. Y. and Pande, V. S.  and Chodera, J. D.  and  Schnieders, M. J.  and  Haque, I.  and Mobley, D. L.  and  Lambrecht, D. S. and  DiStasio, R. A. and Head-Gordon, M. and  Clark, G. N. I. and  Johnson, M. E.  and  Head-Gordon, T. },
  title = {  Current Status of the AMOEBA Polarizable Force Field },
  year = { 2010},
  journal = {J. Phys. Chem. B},
  volume = {114},
  pages = { 2549 - 2564}
}



@ARTICLE{Beglov:1997,
  author = { Beglov, D and  Roux, B.},
  title = {  An integral equation to describe the solvation of polar molecules in liquid water },
  year = {1997},
  journal = {J. Phys. Chem. B},
  volume = {101},
  pages = { 7821-7826}
}


@ARTICLE{Pettitt:1982,
  author = {    Pettitt, B. M.  and   Rossky, P. R.},
  title = {  Integral equation predictions of liquid state structure for waterlike intermolecular potentials  },
  year = {1982},
  journal = {J. Chem. Phys.},
  volume = {77},
  pages = { 1451-1457}
}



@ARTICLE{HChen:2012,
  author = { Chen, H. and Meisburger, S. P. and  Pabit, S. A.  and  Sutton, J. L. and  Webb, W. W. and Pollack, L.},
  title = {  Ionic strength-dependent persistence lengths of single-stranded RNA and DNA },
  year = {2012},
  journal = {PNAS},
  volume = {109},
  pages = { 799-804}
}


@ARTICLE{Pabit:2009,
  author = { Pabit, S. A. and Qiu, X. Y. and  Lamb, J. S. and  Li, L. and  Meisburger, S. P. and   Pollack, L.},
  title = {   Both helix topology and counterion distribution contribute to the more effective charge screening in dsRNA compared with dsDNA},
  year = {2009},
  journal = {Nucleic Acids Research},
  volume = {37},
  pages = { 3887-3896}
}






@ARTICLE{Shkel:2004,
  author = {  Shkel, I. A; Record, M. T. },
  title = {  Effect of the number of nucleic acid oligomer charges on the salt dependence of stability (Delta G degrees(37)) and melting temperature (T-m): NLPB analysis of experimental data},
  year = {2004},
  journal = { Biochemistry},
  volume = {43},
  pages = { 7090-7101}
}




@ARTICLE{Mengistu:2008,
  author = {  Mengistu, D.  H. and  May, Sylvio},
  title = {   Nonlinear Poisson-Boltzmann model of charged lipid membranes: Accounting for the presence of zwitterionic lipidsa},
  year = {2008},
  journal = { J. Chem. Phys. },
  volume = {129},
  pages = { 121105 }
}




@ARTICLE{GHHou:2012,
  author = { Hou, G. H. and  Zhu, X.  and Elstner, M. and Cui, Q. },
  title = {  A Modified QM/MM Hamiltonian with the Self-Consistent-Charge Density-Functional-Tight-Binding Theory for Highly Charged QM Regions},
  year = {2012},
  journal = { J. Chem. Theory and Comput.},
  volume = {8},
  pages = {4293-4304 }
}



@ARTICLE{Kireeva:2012,
  author = {  Kireeva, M. L.  and Opron, K.  and  Seibold, S. A.  and  Domecq, C.  and  Cukier, R. I. and Coulombe, B.   and  Kashlev, M.   and Burton, Z. F. },
  title = { Molecular dynamics and mutational analysis of the catalytic and translocation cycle of RNA polymerase},
  year = {2012},
  journal = { BMC Biophysics},
  volume = {5},
  pages = {11 }
}




@ARTICLE{Diehla:1999,
  author = {    Diehla, A. and      Tamashirob, M. N. and Barbosac,    M. C.  and  Levinc, Y. },
  title = { Density-functional theory for attraction between like-charged plates},
  year = {1999},
  journal = {Physica A: Statistical Mechanics and its Applications},
  volume = {274},
  pages = {433?445}
}



@ARTICLE{GNi:2008,
  AUTHOR =       {Ni, Guoxi and Jiang, Song and Xu, Kun  },
  TITLE =        {A DGBGK scheme based on WENO limiters for viscous and inviscid flows},
  JOURNAL =      {J. Comput. Phys.},
  YEAR =         {2008},
  volume =       {227},
  number =       {},
  pages =        {5799-5815}
}



@ARTICLE{JLi:2011,
  AUTHOR =       {Li, Jiequan; Li, Qibing; Xu, Kun  },
  TITLE =        { Comparison of the generalized Riemann solver and the gas-kinetic scheme for inviscid compressible flow simulations},
  JOURNAL =      {J. Comput. Phys.},
  YEAR =         {2011},
  volume =       {230},
  number =       {},
  pages =        {5080-5099}
}

%#############################!!!!!!!!!!!!!add by KELIN

@ARTICLE{Lorensen1987,
  author = {Lorensen, W. E. and Cline, H. E. },
  title = {Marching cubes: A high resolution 3D surface construction algorithm   },
  year = {1987},
  journal = {COMPUTER GRAPHICS},
  volume = {21},
  pages = {163-169}
  }

@ARTICLE{Heiden:1993,
  author = {Heiden, W. and Moeckel, G. and Brickmann, J. },
  title = {A new approach to analysis and display of local lipophilicity/hydrophilicity mapped on molecular surfaces },
  year = {1993},
  journal = {Journal of Computer-Aided Molecular Design},
  volume = {7},
  pages = {503-514}
  }

@ARTICLE{LGong:2010,
  author = {Gong, L. D. and Yang, Z. Z. },
  title = {Investigation of the molecular surface area and volume: Defined and calculated by the molecular face theory},
  year = {2010},
  journal = {Journal of Computational Chemistry},
  volume = {31},
  pages = {2098-2108}
  }

@ARTICLE{Federer:1959,
  author = {Federer, H. },
  title = {{Curvature Measures}},
  journal = {Trans. Amer. Math. Soc.},
  year = {1959},
  volume = {93},
  pages = {418--491}
}

	

@ARTICLE{WYChen:2010,
  author = {Chen, Wenyu and  Zheng, Jianmin and Cai, Yiyu},
  title = {Kernel modeling for molecular surfaces using a uniform solution},
  journal = {Computer Aided Design   },
  year = {2010},
  volume = {42},
  pages = {267--278}
}

 Title:
Author(s):
Source: JOURNAL OF COMPUTATIONAL CHEMISTRY  Volume: 19   Issue: 11   Pages:    DOI: 10.1002/(SICI)1096-987X(199808)19:11<1268::AID-JCC6>3.0.CO;2-I   Published: AUG 1998


@ARTICLE{SLChan:1998,
  author = {Chan, S. L. and  Purisima, E. O.},
  title = {Molecular surface generation using marching tetrahedra},
  journal = {J. Computat. Chem. },
  year = {1998},
  volume = {11},
  pages = {1268-1277}
}


@ARTICLE{Perkins:1998,
  author = {Perkins, T. D. J. and  Mills, J. E. J. and  Dean, P. M.},
  title = {Molecular surface-volume and property matching to superpose flexible dissimilar molecules},
  journal = {J. Computer-Aided Molecular Design   },
  year = {1998},
  volume = {9},
  pages = {479-490}
}


@ARTICLE{Max:1988,
  author = {Max, N. L. and Getzoff,  E. D.},
  title = {Spherical Harmonic Molecular-surfaces },
  journal = {IEEE Computer Graphics and Applications   },
  year = {1988},
  volume = {8},
  pages = {42-50}
}


@ARTICLE{MCWu:1996,
  author = {Wu, M. C. and Liu, C. R.},
  title = {Analysis on machined feature recognition techniques based on B-rep },
  journal = { Computer-Aided  Design   },
  year = {1996},
  volume = {28},
  pages = {603-616}
}


@ARTICLE{MXChen:2011,
  author = {Chen, Minxin and  Lu, Benzhuo},
  title = {TMSmesh: A Robust Method for Molecular Surface Mesh Generation Using a Trace Technique},
  journal = { J Chem. Theory and Comput. },
  year = {2011},
  volume = {7},
  pages = {203-212}
}



@ARTICLE{Burger:2012,
  author = {Burger, M. and Schlake, B. and Wolfram, M. T.},
  title = { Nonlinear Poisson-Nernst-Planck equations for ion flux through confined geometries},
  journal = { Nonlinearity },
  year = {2012},
  volume = {25},
  pages = { 961-990}
}


@ARTICLE{JKim:2012,
  author = {Kim, Junseok},
  title = { Phase-Field Models for Multi-Component Fluid Flows},
  journal = {Commun. Comput. Phys. },
  year = {2012},
  volume = {12},
  pages = {613-661}
}


@ARTICLE{JWu:2011,
  author = {Wu, J. and  Xia, Z. and  Shen, H. J. and Li, G. H. and Ren, P. Y.},
  title = { Gay-Berne and Electrostatic Multipole based Coarse Grained Model and Application with Polyalanine in Implicit Solvent},
  journal = {J. Chem. Phys. },
  year = {2011},
  volume = {135},
  pages = {155104}
}


@ARTICLE{JWang:2011,
  author = {Wang, J and Zhu, W and Li, G. H. and  Hansmann, U. H. E. },
  title = {  Velocity-scaling optimized replica exchange molecular dynamics of proteins in a hybrid explicit /implicit solvent },
  journal = {J. Chem. Phys. },
  year = {2011},
  volume = {135},
  pages = {084115}
}




@ARTICLE{ZFu:2011,
  author = { Fu, Z. and Li, X. and and Merz, K. M., Jr. },
  title = { Accurate Assessment of the Strain Energy in a Protein-Bound Drug Using {QM/MM} X-ray Refinement and Converged Quantum Chemistry },
  journal = {J. Comput. Chem.   },
  year = {2011},
  volume = {32},
  pages = {2587-2597}
}





%%%%%%%%%%%%%%%%%%%%%%% normal mode analysis----KELIN XIA added 2013###############

@ARTICLE{Go:1983,
  AUTHOR =       {Go, N. and  Noguti, T. and Nishikawa, T. },
  TITLE =        {Dynamics of a small globular protein in terms of low-frequency vibrational modes},
  JOURNAL =      {Proc. Natl. Acad. Sci. },
  YEAR =         {1983},
  volume =       {80},
  number =       {},
  pages =        {3696 - 3700}
}


@ARTICLE{Tasumi:1982,
  AUTHOR =       {Tasumi, M. and Takenchi, H. and Ataka, S. and Dwidedi, A. M. and  Krimm, S.},
  TITLE =        {Normal vibrations of proteins: Glucagon},
  JOURNAL =      {Biopolymers},
  YEAR =         {1982},
  volume =       {21},
  number =       {},
  pages =        {711 - 714}
}



@ARTICLE{Tirion:1996,
  AUTHOR =       { Tirion, M. M.},
  TITLE =        { Large amplitude elastic motions in proteins from a
single-parameter, atomic analysis.},
  JOURNAL =      { Phys. Rev. Lett.},
  YEAR =         {1996},
  volume =       {77},
  number =       {},
  pages =        {1905 - 1908}
}


@ARTICLE{Flory:1976,
  AUTHOR =       { Flory, P. J. },
  TITLE =        { Statistical thermodynamics of random networks.},
  JOURNAL =      { Proc. Roy. Soc. Lond. A,},
  YEAR =         {1976},
  volume =       {351},
  number =       {},
  pages =        {351  -  378}
}


@ARTICLE{Bahar:1997,
  AUTHOR =       { Bahar, I. and Atilgan, A. R. and Erman, B. },
  TITLE =        {Direct evaluation of thermal fluctuations in proteins using a single-parameter harmonic potential. },
  JOURNAL =      {Folding and Design},
  YEAR =         {1997},
  volume =       {2},
  number =       {},
  pages =        {173 - 181}
}

@ARTICLE{Bahar:1998,
  AUTHOR =       {Bahar, I. and Atilgan, A. R. and Demirel, M. C. and Erman, B. },
  TITLE =        { Vibrational dynamics of proteins: Significance of slow and fast modes in relation to function and stability.},
  JOURNAL =      { Phys. Rev. Lett},
  YEAR =         {1998},
  volume =       {80},
  number =       {},
  pages =        {2733  -  2736}
}

@ARTICLE{Atilgan:2001,
  AUTHOR =       {Atilgan, A. R. and Durrell, S. R. and Jernigan, R. L. and Demirel, M. C. and Keskin, O. and Bahar, I.},
  TITLE =        { Anisotropy of fluctuation dynamics of proteins with an elastic network model.},
  JOURNAL =      {Biophys. J.},
  YEAR =         {2001},
  volume =       {80},
  number =       {},
  pages =        {505  -  515}
}

@ARTICLE{Hinsen:1998,
  AUTHOR =       {Hinsen, K.},
  TITLE =        { Analysis of domain motions by approximate normal mode calculations.},
  JOURNAL =      {Proteins},
  YEAR =         {1998},
  volume =       {33},
  number =       {},
  pages =        {417 - 429}
}

@ARTICLE{Tama:2001,
  AUTHOR =       { Tama, F. and Sanejouand, Y. H.},
  TITLE =        { Conformational change of proteins arising from normal mode calculations.},
  JOURNAL =      {Protein Eng.},
  YEAR =         {2001},
  volume =       {14},
  number =       {},
  pages =        {1 - 6}
}

@ARTICLE{LiGH:2002,
  AUTHOR =       { Li, G. H. and Cui, Q. },
  TITLE =        {A coarse-grained normal mode approach for macromolecules: an efficient implementation and application to {Ca(2+)-ATPase}.},
  JOURNAL =      {Bipohys. J.},
  YEAR =         {2002},
  volume =       {83},
  number =       {},
  pages =        { 2457 - 2474}
}

%%%%%%%%%%%%%%%%%%  application in biological systems

%%%%%% Lysozyme

@ARTICLE{Levitt:1985,
AUTHOR =         {Levitt, M.  and  Sander,  C. and Stern,  P. S.},
  TITLE =        {Protein normal-mode dynamics: Trypsin inhibitor, crambin, ribonuclease and lysozyme.},
  JOURNAL =      {J. Mol. Biol.},
  YEAR =         {1985},
  volume =       {181},
  number =       {3},
  pages =        {423 - 447},
}

@ARTICLE{Brooks:1985,
AUTHOR =         { Brooks, B. R. and Karplus, M.},
  TITLE =        {Normal modes for specific motions of macromolecules: application to the hinge-bending mode of lysozyme.},
  JOURNAL =      {Proc. Natl. Acad. Sci.},
  YEAR =         {1985},
  volume =       {82},
  number =       {15},
  pages =        {4995 - 4999},
}

%

@ARTICLE{CXu:2003,
AUTHOR =         { Xu, C. and Tobi, D. and Bahar, I. },
  TITLE =        { Allosteric changes in protein structure computed by a simple mechanical model: hemoglobin T <--> R2 transition.},
  JOURNAL =      {J. Mol. Biol.},
  YEAR =         {2003},
  volume =       {333},
  number =       {},
  pages =        {153 - 168},
}

%F1-ATPrase
@ARTICLE{WZheng:2003,
AUTHOR =         {Zheng, W. J. and Doniach, S. },
  TITLE =        {A comparative study of motor-protein motions by using a simple elastic-network model},
  JOURNAL =      {Proc. Natl. Acad. Sci. USA.},
  YEAR =         {2003},
  volume =       {100},
  number =       {23},
  pages =        {13253 - 13258},
}

@ARTICLE{QCui:2004,
AUTHOR =         {Cui, Q. and Li, G. J. and Ma, J. and Karplus, M. },
  TITLE =       { A normal mode analysis of structural plasticity in the biomolecular motor F(1)-ATPase},
  JOURNAL =      {J. Mol. Biol.},
  YEAR =         {2004},
  volume =       {340},
  number =       {2},
  pages =        {345 - 372},
}

%%%%    chaperonin GroEL
@ARTICLE{Keskin:2002,
AUTHOR =         { Keskin, O. and Bahar, I. and Flatow, D. and Covell, D. G. and Jernigan, R. L. },
  TITLE =       { Molecular mechanisms of chaperonin GroEL-GroES function.},
  JOURNAL =      { Biochem.},
  YEAR =         {2002},
  volume =       {41},
  number =       {},
  pages =        {491  -  501},
}

@ARTICLE{WZheng:2007,
AUTHOR =         {Zheng, W. and Brooks, B. R. and Thirumalai, D. },
  TITLE =       {Allosteric transitions in the chaperonin {GroEL} are captured by a dominant normal mode that is most robust to sequence variations.},
  JOURNAL =      { Biophys. J.},
  YEAR =         {2007},
  volume =       {93},
  number =       {},
  pages =        {2289 - 2299},
}

%%%%%%%%%%%% Viral Capsids

@ARTICLE{Rader:2005,
AUTHOR =        {Rader, A. J. and Vlad, D. H. and Bahar, I.},
  TITLE =       { Maturation dynamics of bacteriophage HK97 capsid.},
  JOURNAL =      {Structure},
  YEAR =         {2005},
  volume =       {13},
  number =       {},
  pages =        {413 - 421},
}

@ARTICLE{Tama:2005,
AUTHOR =        { Tama, F. and Brooks III, C. K.},
  TITLE =       { Diversity and identity of mechanical properties of icosahedral viral capsids studied with elastic network normal mode analysis.},
  JOURNAL =      {J. Mol. Biol.},
  YEAR =         {2005},
  volume =       {345},
  number =       {},
  pages =        {299 - 314},
}

%%%%%%%%%%%%%%  ribosome

@ARTICLE{Tama:2003,
AUTHOR =        { Tama, F. and Valle, M. and Frank, J. and Brooks III, C. K. },
  TITLE =       { Dynamic reorganization of the functionally active ribosome explored by normal mode analysis and cryo-electron microscopy.},
  JOURNAL =      {Proc. Natl Acad. Sci.},
  YEAR =         {2003},
  volume =       {100},
  number =       {16},
  pages =        {9319 - 9323},
}

@ARTICLE{YWang:2004,
AUTHOR =        {Wang, Y.  and Rader, A. J. and Bahar, I. and Jernigan, R. L. },
  TITLE =       {Global ribosome motions revealed with elastic network model.},
  JOURNAL =      {J. Struct. Biol.},
  YEAR =         {2004},
  volume =       {147},
  number =       {},
  pages =        {302 - 314},
}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% crystal structure


@ARTICLE{Kundu:2002,
AUTHOR =         { Kundu, S. and Melton, J. S. and  Sorensen, D. C. and Phillips, Jr. G. N. },
  TITLE =        {Dynamics of proteins in crystals: comparison of experiment with simple models. },
  JOURNAL =      { Biophys. J. },
  YEAR =         {2002},
  volume =       {83},
  number =       {},
  pages =        {723  -  732},
}

@ARTICLE{Kondrashov:2007,
AUTHOR =         {Kondrashov, D. A. and Van Wynsberghe, A. W. and Bannen, R. M.  and Cui, Q. and Phillips, Jr. G. N. },
  TITLE =        {Protein structural variation in computational models and crystallographic data. },
  JOURNAL =      { Structure },
  YEAR =         {2007},
  volume =       {15},
  number =       {},
  pages =        {169  -  177},
}

@ARTICLE{Hinsen:2008,
AUTHOR =         {Hinsen, K.  },
  TITLE =        { Structural flexibility in proteins: impact of the crystal environment. },
  JOURNAL =      { Bioinformatics},
  YEAR =         {2008},
  volume =       {24},
  number =       {},
  pages =        {521  -  528},
}

@ARTICLE{GSong:2007,
AUTHOR =         {Song, G. and Jernigan, R. L. },
  TITLE =        { vGNM: a better model for understanding the dynamics of proteins in crystals. },
  JOURNAL =      { J. Mol. Biol.},
  YEAR =         {2007},
  volume =       {369},
  number =       {3},
  pages =        {880 - 893},
}

%%%%%%%%%%%%%%%%%%%%%%%%% review paper

@ARTICLE{JMa:2005,
AUTHOR =        {Ma, J. P.},
  TITLE =       { Usefulness and limitations of normal mode analysis in modeling dynamics of biomolecular complexes.},
  JOURNAL =      { Structure},
  YEAR =         {2005},
  volume =       {13},
  number =       {},
  pages =        {373 - 180},
}

@ARTICLE{LWYang:2008,
AUTHOR =        {Yang, L. W. and Chng, C. P.},
  TITLE =       {Coarse-grained models reveal functional dynamics--{I}. Elastic network models--theories, comparisons and perspectives.},
  JOURNAL =      {Bioinformatics and Biology Insights},
  YEAR =         {2008},
  volume =       {2},
  number =       {},
  pages =        {25 - 45},
}


@ARTICLE{Skjaven:2009,
AUTHOR =        {Skjaerven, L. and Hollup, S. M. and Reuter, N.},
  TITLE =       {Normal mode analysis for proteins},
  JOURNAL =      {Journal of Molecular Structure: Theochem.},
  YEAR =         {2009},
  volume =       {898},
  number =       {},
  pages =        {42 - 48},
}


@BOOK{QCui:2010,
  title = {Normal mode analysis: theory and applications to biological and chemical systems},
  publisher = {Chapman and Hall/CRC},
  year = {2010},
  author = {Cui, Q. and Bahar, I.}
}

%%%%%%%%%%%%%%%%% Chaos



@ARTICLE{Lorenz:1963,
AUTHOR =        {Lorenz, E. N.},
  TITLE =       {Deterministic nonperiodic flow},
  JOURNAL =      {Journal of the Atmospheric Sciences},
  YEAR =         {1963},
  volume =       {20},
  number =       {},
  pages =        {130- 141 },
}



@ARTICLE{Pecora:1997,
AUTHOR =        {Pecora, L. M. and   Carroll, T. L. and Johnson, G. A. and Mar, D. J.},
  TITLE =       {Fundamentals of synchronization in chaotic systems, concepts and applications},
  JOURNAL =      {Chaos},
  YEAR =         {1997},
  volume =       {7},
  number =       {},
  pages =        {520- 543 },
}


@ARTICLE{GHu:1998,
AUTHOR =        {Hu, G. and  Yang, J. H. and  Liu, W. J.},
  TITLE =       {Instability and controllability of linearly coupled oscillators: Eigenvalue analysis},
  JOURNAL =      {Phys. Rev. E},
  YEAR =         {1998},
  volume =       {58},
  number =       {},
  pages =        {4440- 4453 },
}



@ARTICLE{Ott:1990,
AUTHOR =        {Ott, E. and  Grebogi, C.   and   Yorke, J. A.},
  TITLE =       {Controlling chaos},
  JOURNAL =      {Phys. Rev. Lett.},
  YEAR =         {1990},
  volume =       {64},
  number =       {},
  pages =        {1196 - 1199},
}



@ARTICLE{Pecora:1990,
AUTHOR =        {Pecora, L. M.    and Carroll, T. L.},
  TITLE =       {Synchronization in chaotic systems},
  JOURNAL =      {Phys. Rev. Lett.},
  YEAR =         {1990},
  volume =       {64},
  number =       {},
  pages =        {821-824 },
}


@ARTICLE{Chiti:2006,
AUTHOR =        {Chiti, F.  and Dobson, C. M.},
  TITLE =       {Protein Misfolding, Functional Amyloid, and Human Disease},
  JOURNAL =      {Annu. Rev. Biochem.},
  YEAR =         {2006},
  volume =       {75},
  number =       {},
  pages =        {333 - 366 },
}



@ARTICLE{Mahadevan:2007,
AUTHOR =        {  Mahadevan, T. S. and Garofalini, S. H.},
  TITLE =       {Dissociative Water Potential for Molecular Dynamics Simulations},
  JOURNAL =      {J. Phys. Chem.},
  YEAR =         {2007},
  volume =       {8919},
  number =       {},
  pages =        {8919 - 8927},
}


@ARTICLE{Uversky:2008,
AUTHOR =        {  Uversky, V. and  Dunker, A. K.},
  TITLE =       { Controlled chaos},
  JOURNAL =      {Sceince},
  YEAR =         {2008},
  volume =       {322},
  number =       {},
  pages =        {1340 - 1341},
}


@ARTICLE{Watts:1998,
AUTHOR =        {  Watts, D. J.  and Strogatz, S. H.},
  TITLE =       { Collective dynamics of 'small-world' networks},
  JOURNAL =      {Nature},
  YEAR =         {1998},
  volume =       {393},
  number =       {},
  pages =        {440 -442},
}



@ARTICLE{Fischer:1894,
AUTHOR =        {  Fischer, E.},
  TITLE =       { Einfluss der Configuration auf die Wirkung den},
  JOURNAL =      {Enzyme  Ber. Dtsch. Chem. Ges.},
  YEAR =         {1894},
  volume =       {27},
  number =       {},
  pages =        {2985 - 2993},
}




@ARTICLE{Anfinsen:1973,
AUTHOR =        {  Anfinsen,  C. B.},
  TITLE =       { Einfluss der Configuration auf die Wirkung den},
  JOURNAL =      {Science},
  YEAR =         {1973},
  volume =       {181},
  number =       {},
  pages =        {223 - 230},
}


@ARTICLE{NGo:1983,
AUTHOR =         {Go,   N.},
  TITLE =        { Theoretical studies of protein folding},
  JOURNAL =      {Annu Rev Biophys Bioeng.},
  YEAR =         {1983},
  volume =       {12},
  number =       {},
  pages =        {183 - 210},
}


@ARTICLE{Schroder:2005,
AUTHOR =        { Schroder, M and   Kaufman, R. J.},
  TITLE =       { The mammalian unfolded protein response},
  JOURNAL =      {Annual Review of Biochemistry},
  YEAR =         {2005},
  volume =       {74},
  number =       {},
  pages =        {739 - 789},
}



@ARTICLE{Onuchic:1997,
AUTHOR =        {Onuchic, J. N. and   Luthey-Schulten, Z. and    Wolynes, P. G.},
  TITLE =       { Theory of protein folding: The energy landscape perspective},
  JOURNAL =      {Annu. Rev. Phys. Chem},
  YEAR =         {1997},
  volume =       {48},
  number =       {},
  pages =        {545-600},
}



@ARTICLE{White:1999,
AUTHOR =        {White, S. H. and Wimley, W. C.},
  TITLE =       { Membrane protein folding and stability: Physical principles},
  JOURNAL =      {Annual Review of Biophysics and Biomolecular Structure},
  YEAR =         {1999},
  volume =       {28},
  number =       {},
  pages =        {319-365 },
}



@ARTICLE{Ashwin:2003,
AUTHOR =        {Ashwin, P.},
  TITLE =       {  Nonlinear dynamics - Synchronization from chaos},
  JOURNAL =      {Nature},
  YEAR =         {2003},
  volume =       {422},
  number =       {},
  pages =        {384-385 },
}




@ARTICLE{Bryngelson:1995,
AUTHOR =        {Bryngelson, J. D. and   Onuchic, J. N. and  Socci,  N. D. and  Wolynes,   P. G.},
  TITLE =       {  Funnels, pathways, and the energy landscape of protein folding: A synthesis},
  JOURNAL =      {Proteins: Structure, Function, and Bioinformatics},
  YEAR =         {1995},
  volume =       {21},
  number =       {},
  pages =        {167 -195   },
}


@ARTICLE{Dill:1997,
AUTHOR =        {Dill, K. A.  and   Chan, H. S.},
  TITLE =       {  From Levinthal to pathways to funnels},
  JOURNAL =      {Nature Structural Biology},
  YEAR =         {1997},
  volume =       {4},
  number =       {},
  pages =        {10 -19   },
}

@INPROCEEDINGS{Levinthal:1969,
  author = {Levinthal, C.},
  title = {How to Fold Graciously},
  booktitle = {Mossbauer Spectroscopy in Biological Systems: Proceedings of a meeting held at Allerton House, Monticello, Illinois, J.T.P. DeBrunner and E. Munck eds., University of Illinois Press},
  year = {1969},
  pages = {22-24},
  month = {}
}


@ARTICLE{Poincare:1890,
  author = {Poincar\'{e}, J. H.},
  title =  {Sur le probl?me des trois corps et les \'{e}quations de la dynamique. Divergence des s?ries de M. Lindstedt},
  JOURNAL ={Acta Mathematica},
  year =   {1890},
  volume = {13},
  pages =  {A3-A270},
  month = {}
}



@ARTICLE{Boccaletti:2000,
  author = {Boccaletti, S. and  Grebogi, C. and    Lai, Y. C.  and  Mancini, H. and Maza, D.},
  title =  {The control of chaos: {Theory} and applications},
  JOURNAL ={Physics Reports},
  year =   {2000},
  volume = {329},
  pages =  {103-197},
  month = {}
}




@ARTICLE{Tucker:2002,
  author = {Tucker, Warwick},
  title =  {A Rigorous ODE Solver and Smale's 14th Problem},
  JOURNAL ={Foundations of Computational Mathematics},
  year =   {2002},
  volume = {2},
  pages =  {53?117},
  month = {}
}


@ARTICLE{Dudko:2006,
  author = {Dudko, O. K. and  Hummer, G. and   Szabo, A. },
  title =  {Intrinsic rates and activation free energies from single-molecule pulling experiments},
  JOURNAL ={ Phys. Rev. Lett.},
  year =   {2006},
  volume = {96},
  pages =  {108101},
  month = {}
}



@ARTICLE{Paci:2000,
  author = {Paci, E. and  Karplus, M. },
  title =  {Unfolding proteins by external forces and temperature: The importance of topology and energetics},
  JOURNAL ={ Proceedings of the National Academy of Sciences},
  year =   {2000},
  volume = {97},
  pages =  {6521 - 6526},
  month = {}
}


@ARTICLE{Rubin:1985,
  author = {Rubin, B. },
  title =  {Macromolecule backbone models},
  JOURNAL ={ Methods in Enzymology},
  year =   {1985},
  volume = {115},
  pages =  {391-397},
  month = {}
}



@ARTICLE{Braxenthaler:1997,
  author = {Braxenthaler, M. and  Unger, R. and  Auerbach, D. and    Given, J. A. and    Moult, J. },
  title =  {Chaos in protein dynamics},
  JOURNAL ={ Proteins},
  year =   {1997},
  volume = {29},
  pages =  {417 -425  },
  month = {}
}




@ARTICLE{Karplus:1985,
  author = {Karplus,  P. A. and  Schulz, G. E. },
  title =  { Prediction of chain flexibility in proteins - a tool for the selection of peptide antigens},
  JOURNAL ={Naturwissenschaften},
  year =   {1985},
  volume = {72},
  pages =  {212 -213  },
  month = {}
}

@ARTICLE{Vihinen:1994,
  author = {Vihinen, M. and Torkkila, E. and  Riikonen, P. },
  title =  {Accuracy of protein flexibility predictions},
  JOURNAL ={Proteins},
  year =   {1994},
  volume = {19},
  pages =  {141 -149  },
  month = {}
}


@ARTICLE{Vihinen:1987,
  author = {Vihinen, M.  },
  title =  {Relationship of protein flexibility to thermostability},
  JOURNAL ={Protein Eng.},
  year =   {1987},
  volume = {1},
  pages =  {477-480  },
  month = {}
}


@ARTICLE{Parthasarathy:2000,
  author = {Parthasarathy, S. and  Murthy, M. R. N.  },
  title =  { Protein thermal stability: insights from atomic displacement parameters (B values)},
  JOURNAL ={Protein Eng.},
  year =   {2000},
  volume = {13},
  pages =  {9 -13  },
  month = {}
}




@ARTICLE{Carugo:1998,
  author = {Carugo, O. and  Argos, P.  },
  title =  { Accessibility to internal cavities and ligand binding sites monitored by protein crystallographic thermal factors},
  JOURNAL ={Proteins},
  year =   {1998},
  volume = {31},
  pages =  {201 -213  },
  month = {}
}




@ARTICLE{Yuan:2003,
  author = {Yuan, Z. and  Zhao, J. and Wang, Z. X.   },
  title =  { Flexibility analysis of enzyme active sites by crystallographic temperature factor},
  JOURNAL ={Protein Eng.},
  year =   {2003},
  volume = {16},
  pages =  {109 -114  },
  month = {}
}



@ARTICLE{Mohan:2003,
  author = {Mohan, S. and  Sinha, N. and  Smith-Gill, J.  },
  title =  { Modeling the binding sites of anti-hen egg white lysozyme antibodies HyHEL-8 and HyHEL-26: an insight into the molecular basis of antibody cross-reactivity and
specificity},
  JOURNAL ={Biophys J.},
  year =   {2003},
  volume = {85},
  pages =  {3221 - 3236  },
  month = {}
}

@ARTICLE{Carugo:1997,
  author = {Carugo, O. and  Argos, P.  },
  title =  {  Correlation between side chain mobility and conformation in protein structures},
  JOURNAL ={Protein Eng.},
  year =   {1997},
  volume = {10},
  pages =  {777 - 787  },
  month = {}
}

@ARTICLE{Eyal:2003,
  author = {Eyal, E. and  Najmanovich,  R. and  Edelman, M. and  Sobolev, V.  },
  title =  { Protein side chain rearrangement in regions of point mutations},
  JOURNAL ={Proteins},
  year =   {2003},
  volume = {50},
  pages =  {272 - 282  },
  month = {}
}

 @ARTICLE{Altman:1994,
  author = {Altman, R. and  Hughes,  C. and  Zhao,  D. and  Jardetsky, O.  },
  title =  { Compositional characteristics of relatively disordered regions in proteins},
  JOURNAL ={Prot. Pept. Lett.},
  year =   {1994},
  volume = {1},
  pages =  {120 - 127 },
  month = {}
}

 @ARTICLE{Radivojac:2004,
  author = { Radivojac, P. and  Obradovic,  Z. and  Smith, D. K. and  Zhu, G. and  Vucetic, S. and  Brown, C. J. and
Lawson, J. D. and  Dunker,  A. K.  },
  title =  { Protein flexibility and intrinsic disorder},
  JOURNAL ={Protein Sci.},
  year =   {2004},
  volume = {13},
  pages =  {71 - 80 },
  month = {}
}



 @ARTICLE{JKPark:2013,
  author = { Park, J. K. and Jernigan, Robert and  Wu, Zhijun  },
  title =  { Coarse Grained Normal Mode Analysis vs. Refined Gaussian Network Model for Protein Residue-Level Structural Fluctuations},
  JOURNAL ={ Bulletin of Mathematical Biology},
  year =   {2013},
  volume = {75},
  pages =  {124 -160 },
  month = {}
}


 @ARTICLE{Marsh:2012,
  author = {  Marsh, J. A. and    Teichmann, S. A. and   Forman-Kay, J. D. },
  title =  {Probing the diverse landscape of protein flexibility and binding},
  JOURNAL ={Current Opinion in Structural Biology},
  year =   {2012},
  volume = {22},
  pages =  {643?650 },
  month = {}
}

 @ARTICLE{HouSM:2013,
  author = { Hou, S. M.  and  Song, P.  and Wang, L. Q. and Zhao, H. K.  },
  title =  {A weak formulation for solving elliptic interface problems
without body fitted grid},
  JOURNAL ={J. Comput. Phys. },
  year =   {2013},
  volume = {249},
  pages =  {80-95 },
  month = {}
}

 @ARTICLE{DuanChen:2010b,
  author = {Chen, D.  and Guo, W. W. },
  title =  {Modeling and simulation of electronic structure, material interface and
random doping in nano-electronic devices},
  JOURNAL ={J. Comput. Phys. },
  year =   {2010},
  volume = {229},
  pages =  {4431-4460 },
  month = {}
}


@ARTICLE{Antonny:2013,
Author = {Antonny, Bruno},
Title = {{Mechanisms of Membrane Curvature Sensing}},
Journal = {{Annual Review of Biochemistry}},
Year = {{2011}},
Volume = {{80}},
Pages = {{101-123}},
}

@article{Habermann:2004,
Author = {Habermann, B},
Title = {{The BAR-domain family of proteins: a case of bending and binding? The
   membrane bending and GTPase-binding functions of proteins from the
   BAR-domain family}},
Journal = {{EMBO Reports}},
Year = {{2004}},
Volume = {{5}},
Number = {{3}},
Pages = {{250-255}},
}

 @article{Peter:2004,
Author = {Peter, BJ and Kent, HM and Mills, IG and Vallis, Y and Butler, PJG and
   Evans, PR and McMahon, HT},
Title = {{BAR domains as sensors of membrane curvature: The amphiphysin BAR
   structure}},
Journal = {{Science}},
Year = {{2004}},
Volume = {{303}},
Number = {{5657}},
Pages = {{495-499}},
Month = {{JAN 23}},
}

@article{McMahon:2005,
Author = {McMahon, HT and Gallop, JL},
Title = {{Membrane curvature and mechanisms of dynamic cell membrane remodelling}},
Journal = {{Nature}},
Year = {{2005}},
Volume = {{438}},
Number = {{7068}},
Pages = {{590-596}},
Month = {{DEC 1}},
}

@article{Sept:2010,
Author = {Sept, David and MacKintosh, Fred C.},
Title = {{Microtubule Elasticity: Connecting All-Atom Simulations with Continuum
   Mechanics}},
Journal = {{Physical Review Letters}},
Year = {{2010}},
Volume = {{104}},
Number = {{1}},
Month = {{Jan 8}},
}



@article{Janosi:1998,
Author = {Janosi, IM and Chretien, D and Flyvbjerg, H},
Title = {{Modeling elastic properties of microtubule tips and walls}},
Journal = {{European Biophysics Journal with Biophysics Letters}},
Year = {{1998}},
Volume = {{27}},
Number = {{5}},
Pages = {{501-513}},
}

@article{Villa:2004,
Author = {Villa, E and Balaeff, A and Mahadevan, L and Schulten, K},
Title = {{Multiscale method for simulating protein-DNA complexes}},
Journal = {{Multiscale Modeling \& Simulation}},
Year = {{2004}},
Volume = {{2}},
Number = {{4}},
Pages = {{527-553}},
}




@article{Brown:2012,
Author = {Brown, Michael F.},
Title = {{Curvature Forces in Membrane Lipid-Protein Interactions}},
Journal = {{Biochemistry}},
Year = {{2012}},
Volume = {{51}},
Number = {{49}},
Pages = {{9782-9795}},
Month = {{DEC 11}},
}

@article{Frauenfelder:1991,
Author = {Frauenfelder, H. and Slihar, S. G. and Wolynes, P. G.
},
Title = {{ The energy landsapes and motion of proteins
}},
Journal = {{Science}},
Year = {{1991}},
Volume = {{254}},
Number = {{5038}},
Pages = {{1598-1603}},
Month = {{DEC 13}},
}

@article{ZYuan:2005,
Author = {Yuan, Z and Bailey, TL and Teasdale, RD},
Title = {{Prediction of protein B-factor profiles}},
Journal = {{Proteins-Structure Function and Bioinformatics}},
Year = {{2005}},
Volume = {{58}},
Number = {{4}},
Pages = {{905-912}},
Month = {{MAR 1}},
}



@article{XYPan:2009,
Author = {Pan, Xiao-Yong and Shen, Hong-Bin},
Title = {{Robust Prediction of B-Factor Profile from Sequence Using Two-Stage SVR
   Based on Random Forest Feature Selection}},
Journal = {{Protein and Peptide Letters}},
Year = {{2009}},
Volume = {{16}},
Number = {{12}},
Pages = {{1447-1454}},
}

@article{LYang:2009,
Author = {Yang, Lei and Song, Guang and Jernigan, Robert L.},
Title = {{Protein elastic network models and the ranges of cooperativity}},
Journal = {{Proceedings of the National Academy of Sciences of the United States of America }},
Year = {{2009}},
Volume = {{106}},
Number = {{30}},
Pages = {{12347-12352}},
Month = {{JUL 28}},
}

@article{Renka:1988,
Author = {Renka, R. J.},
Title = {{Multivariate interpolation of large sets of scattered data}},
Journal = {{ACM Transactions on Mathematical Software}},
Year = {{1988}},
Volume = {{14}},
Number = {{2}},
Pages = {{139-148}},
Month = {{JUN}},
}

@article{Thacker:2010,
Author = {Thacker, William I. and Zhang, Jingwei and Watson, Layne T. and Birch,
   Jeffrey B. and Iyer, Manjula A. and Berry, Michael W.},
Title = {{Algorithm 905: SHEPPACK: Modified Shepard Algorithm for Interpolation of
   Scattered Multivariate Data}},
Journal = {{ACM Transactions on Mathematical Software}},
Year = {{2010}},
Volume = {{37}},
Number = {{3}},
Month = {{SEP}},
}

@article{Demerdash:2012,
Author = {Demerdash, Omar N. A. and Mitchell, Julie C.},
Title = {{Density-cluster NMA: A new protein decomposition technique for
   coarse-grained normal mode analysis}},
Journal = {{Proteins:Structure Function and Bioinformatics}},
Year = {{2012}},
Volume = {{80}},
Number = {{7}},
Pages = {{1766-1779}},
Month = {{JUL}},
}

@article{Jacobs:2001,
Author = {Jacobs, D. J. and Rader, A. J. and Kuhn, L. A. and Thorpe, M. F.},
Title = {{Protein flexibility predictions using graph theory}},
Journal = {{Proteins-Structure, Function, and Genetics}},
Year = {{2001}},
Volume = {{44}},
Number = {{2}},
Pages = {{150-165}},
Month = {{AUG 1}},
}

@article{Livesay:2004,
Author = {Livesay, D. R. and Dallakyan, S. and Wood, G. G. and Jacobs, D. J. },
Title = {{A flexible approach for understanding protein stability}},
Journal = {{FEBS Letters}},
Year = {{2004}},
Volume = {{576}},
Pages = {{468-476}},
}


!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!  steered molecular dynamics

@article{Gao:2002,
Author = {Gao, M. and Craig, D. and Vogel, V. and Schulten, K.},
Title = {Identifying unfolding intermediates of $FN-III_{10}$ by steered molecular dynamics},
Journal = {J. Mol. Biol.},
Year = {2002},
Volume = {323},
Number = {},
Pages = {939-950},
}

@article{Hui:1998,
Author = {Hui, L. and Isralewitz, B. and Krammer, A. and Vogel, V. and Schulten, K.},
Title = {Unfolding of Titin Immunoglobulin Domains by Steered Molecular Dynamics Simulation},
Journal = {Biophysical Journal},
Year = {1998},
Volume = {75},
Number = {},
Pages = {662-671},
}


@article{Isralewitz:2001,
Author = {Isralewitz, B. and Gao, M. and Schulten, K.},
Title = {Steered molecular dynamics and mechanical functions of proteins},
Journal = {Curr Opin Struct Biol},
Year = {2001},
Volume = {11},
Number = {2},
Pages = {224-230},
}

@article{Srivastava:2013,
Author = {Srivastava, A. and Granek, R.},
Title = {Cooperativity in thermal and force-induced protein unfolding: integration of crack propagation and network elasticity models},
Journal = { Phys. Rev. Lett.},
Year = {2013},
Volume = {110},
Number = {138101},
Pages = {1-5},
}


@article{Janin:2013,
Author = {Janin, J.  and Sternberg,  M. J.},
Title = {Protein flexibility, not disorder, is intrinsic to molecular recognition},
Journal = {F1000 Biology Reports},
Year = {2013},
Volume = {5(2)},
Number = {},
Pages = {1-7},
}




@article{Gulick:2003,
Author = {Gulick, A. M. and V. J. Starai and A. R. Horswill and K. M. Homick and J. C.Escalante-Semerena},
Title = {The 1.75 A crystal structure of acetyl-CoA synthetase bound to adenosine-59-propylphosphate and coenzyme A.},
Journal = {Biochemistry },
Year = {2003},
Volume = {},
Number = {},
Pages = {},
}

@article{Szarecka:2007,
Author = {Szarecka, A and Xu, Y and Tang, P},
Title = {Dynamics of Firefly Luciferase Inhibition by General Anesthetics: Gaussian and Anisotropic Network Analyses},
Journal = {Biophysical Journal },
Year = {2007},
Volume = {93},
Number = {},
Pages = {1895-1905},
}




@article{Paci:1999,
Author = {Paci, E. and Karplus, M.},
Title = {Forced unfolding of fibronectin type 3 modules: an analysis by biased molecular dynamics simulations},
Journal = { J. Mol. Biol.},
Year = {1999},
Volume = {288},
Number = {},
Pages = {441-459},
}







@article{McCammon:1977,
Author = {McCammon, J. A. and Gelin, B. R. and Karplus, M.},
Title = {Dynamics of    folded proteins},
Journal = {Nature },
Year = {1977},
Volume = {267},
Number = {},
Pages = {585-590},
}


@article{Gibbons:2000,
  title={The structure of the central stalk in bovine F1-ATPase at 2.4 {\AA} resolution},
  author={Gibbons, Clyde and Montgomery, Martin G and Leslie, Andrew GW and Walker, John E},
  journal={Nature Structural \& Molecular Biology},
  volume={7},
  number={11},
  pages={1055--1061},
  year={2000},
  publisher={Nature Publishing Group}
}

@article{Rastogi:1999,
  title={Structural changes linked to proton translocation by subunit c of the ATP synthase},
  author={Rastogi, Vinit K and Girvin, Mark E},
  journal={Nature},
  volume={402},
  number={6759},
  pages={263--268},
  year={1999},
  publisher={Nature Publishing Group}
}

@article{Rayment:1993,
  title={Three-dimensional structure of myosin subfragment-1: a molecular motor},
  author={Rayment, Ivan and Rypniewski, Wojciech R and Schmidt-Base, Karen and Smith, Robert and Tomchick, Diana R and Benning, Matthew M and Winkelmann, Donald A and Wesenberg, Gary and Holden, Hazel M},
  journal={Science},
  volume={261},
  number={5117},
  pages={50--58},
  year={1993},
  publisher={American Association for the Advancement of Science}
}

@article{peskin:2000,
  title={Protein flexibility and the correlation ratchet},
  author={Peskin, Charles S and You, Dwight and Elston, Timothy C},
  journal={SIAM Journal on Applied Mathematics},
  volume={61},
  number={3},
  pages={776--791},
  year={2000},
  publisher={SIAM}
}

@article{duselder:2012,
  title={Neck-Linker Length Dependence of Processive Kinesin-5 Motility},
  author={D{\"u}selder, Andr{\'e} and Thiede, Christina and Schmidt, Christoph F and Lak{\"a}mper, Stefan},
  journal={Journal of molecular biology},
  year={2012},
  publisher={Elsevier}
}

@article{kull:1996,
  title={Crystal structure of the kinesin motor domain reveals a structural similarity to myosin},
  author={Kull, F Jon and Sablin, Elena P and Lau, Rebecca and Fletterick, Robert J and Vale, Ronald D},
  journal={Nature},
  volume={380},
  number={6574},
  pages={550},
  year={1996},
  publisher={NIH Public Access}
}

@article{sablin:1998,
  title={Direction determination in the minus-end-directed kinesin motor ncd},
  author={Sablin, Elena P and Case, Ryan B and Dai, Shirleko C and Hart, Cynthia L and Ruby, Aaron and Vale, Ronald D and Fletterick, Robert J},
  journal={Nature},
  volume={395},
  number={6704},
  pages={813--816},
  year={1998},
  publisher={Nature Publishing Group}
}

@article{brunnbauer:2012,
  title={Torque generation of kinesin motors is governed by the stability of the neck domain},
  author={Brunnbauer, Melanie and Dombi, Renate and Ho, Thi-Hieu and Schliwa, Manfred and Rief, Matthias and {\"O}kten, Zeynep},
  journal={Molecular Cell},
  volume={46},
  number={2},
  pages={147--158},
  year={2012},
  publisher={Elsevier}
}

@article{bormuth2012,
  title={The highly processive kinesin-8, Kip3, switches microtubule protofilaments with a bias toward the left},
  author={Bormuth, Volker and Nitzsche, Bert and Ruhnow, Felix and Mitra, Aniruddha and Storch, Marko and Rammner, Burkhard and Howard, Jonathon and Diez, Stefan},
  journal={Biophysical Journal},
  volume={103},
  number={1},
  pages={L4--L6},
  year={2012},
  publisher={Elsevier}
}

@article{sindelar2002,
  title={Two conformations in the human kinesin power stroke defined by X-ray crystallography and EPR spectroscopy},
  author={Sindelar, Charles V and Budny, Mary Jane and Rice, Sarah and Naber, Nariman and Fletterick, Robert and Cooke, Roger},
  journal={Nature Structural \& Molecular Biology},
  volume={9},
  number={11},
  pages={844--848},
  year={2002},
  publisher={Nature Publishing Group}
}

@article{sancho2006,
  title={Kinesin as an electrostatic machine},
  author={Sancho, JM and Tsironis, GP and others},
  journal={Journal of biological physics},
  volume={32},
  number={5},
  pages={455--463},
  year={2006},
  publisher={Springer}
}

@article{shastry:2010,
  title={Neck linker length determines the degree of processivity in kinesin-1 and kinesin-2 motors.},
  author={Shastry, Shankar and Hancock, William},
  journal={Current biology : {CB}},
  volume={20},
  number={10},
  pages={939-943},
  year={2010}
}

@article{valesearching2000,
  title={Searching for kinesin's mechanical amplifier.},
  author={Vale, R and Case, R and Sablin, E and Hart, C and Fletterick, R},
  journal={Philosophical transactions of the Royal Society of London. Series B, Biological sciences},
  volume={355},
  number={1396},
  pages={449-457},
  year={2000}
}

@article{caserole2000,
  title={Role of the kinesin neck linker and catalytic core in microtubule-based motility.},
  author={Case, R and Rice, S and Hart, C and Ly, B and Vale, R},
  journal={Current biology : {CB}},
  volume={10},
  number={3},
  pages={157-160},
  year={2000}
  }


  @article{grant2011,
  title={Electrostatically biased binding of kinesin to microtubules.},
  author={Grant, Barry and Gheorghe, Dana and Zheng, Wenjun and Alonso, Maria and Huber, Gary and Dlugosz, Maciej and {McCammon,} J and Cross, Robert},
  journal={{PLoS} biology},
  volume={9},
  number={11},
  year={2011}
}

@article{okada2000,
  title={Mechanism of the single-headed processivity: Diffusional anchoring between the K-loop of kinesin and the C terminus of tubulin},
  author={Y. Okada},
  journal={Proceedings of the National Academy of Sciences},
  volume={97},
  year={2000},
  doi={10.1073/pnas.97.2.640},
  url={http://dx.doi.org/10.1073/pnas.97.2.640}
}

@article{Yang:2006,
  title={{oGNM:} online computation of structural dynamics using the Gaussian Network Model.},
  author={Yang, {Lee-Wei} and Rader, A and Liu, Xiong and Jursa, Cristopher and Chen, Shann and Karimi, Hassan and Bahar, Ivet},
  journal={Nucleic acids research},
  volume={34},
  number={Web Server issue},
  pages={W24-W31},
  year={2006},
  abstract={An assessment of the equilibrium dynamics of biomolecular systems, and in particular their most cooperative fluctuations accessible under native state conditions, is a first step towards understanding molecular mechanisms relevant to biological function. We present a web-based system, {oGNM} that enables users to calculate online the shape and dispersion of normal modes of motion for proteins, oligonucleotides and their complexes, or associated biological units, using the Gaussian Network Model {(GNM).} Computations with the new engine are 5-6 orders of magnitude faster than those using conventional normal mode analyses. Two cases studies illustrate the utility of {oGNM.} The first shows that the thermal fluctuations predicted for 1250 non-homologous proteins correlate well with X-ray crystallographic data over a broad range [7.3-15 A] of inter-residue interaction cutoff distances and the correlations improve with increasing observation temperatures. The second study, focused on 64 oligonucleotides and oligonucleotide-protein complexes, shows that good agreement with experiments is achieved by representing each nucleotide by three {GNM} nodes (as opposed to one-node-per-residue in proteins) along with uniform interaction ranges for all components of the complexes. These results open the way to a rapid assessment of the dynamics of {DNA/RNA-containing} complexes. The server can be accessed at {http://ignm.ccbb.pitt.edu/GNM\_Online\_Calculation.htm.}},
  doi={10.1093/nar/gkl084},
  url={http://dx.doi.org/10.1093/nar/gkl084}
}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
Flexibility 3
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


@article{hingeprot,
  title={{HingeProt:} automated prediction of hinges in protein structures.},
  author={Emekli, Ugur and {Schneidman-Duhovny,} Dina and Wolfson, Haim and Nussinov, Ruth and Haliloglu, Turkan},
  journal={Proteins},
  volume={70},
  number={4},
  pages={1219-1227},
  year={2008},
  abstract={Proteins are highly flexible molecules. Prediction of molecular flexibility aids in the comprehension and prediction of protein function and in providing details of functional mechanisms. The ability to predict the locations, directions, and extent of molecular movements can assist in fitting atomic resolution structures to low-resolution {EM} density maps and in predicting the complex structures of interacting molecules (docking). There are several types of molecular movements. In this work, we focus on the prediction of hinge movements. Given a single protein structure, the method automatically divides it into the rigid parts and the hinge regions connecting them. The method employs the Elastic Network Model, which is very efficient and was validated against a large data set of proteins. The output can be used in applications such as flexible protein-protein and protein-ligand docking, flexible docking of protein structures into {cryo-EM} maps, and refinement of low-resolution {EM} structures. The web server of {HingeProt} provides convenient visualization of the results and is available with two mirror sites at {http://www.prc.boun.edu.tr/appserv/prc/HingeProt3} and {http://bioinfo3d.cs.tau.ac.il/HingeProt/.}},
  doi={10.1002/prot.21613},
  url={http://dx.doi.org/10.1002/prot.21613}
}

@article{stonehinge,
  title={{StoneHinge:} Hinge prediction by network analysis of individual protein structures},
  author={Keating, Kevin S and Flores, Samuel C and Gerstein, Mark B and Kuhn, Leslie A},
  journal={Protein Science},
  volume={18},
  number={2},
  pages={359-371},
  year={2009},
  publisher={Wiley Online Library},
  doi={10.1002/pro.38},
  url={http://dx.doi.org/10.1002/pro.38}
}

@article{flexprot,
  title={{FlexProt:} alignment of flexible protein structures without a predefinition of hinge regions},
  author={Shatsky, Maxim and Nussinov, Ruth and Wolfson, Haim J},
  journal={Journal of Computational Biology},
  volume={11},
  number={1},
  pages={83-8106},
  year={2004},
  publisher={Mary Ann Liebert, Inc.},
  doi={10.1089/106652704773416902},
  url={http://dx.doi.org/10.1089/106652704773416902}
}

@article{flexoracle,
  title={{FlexOracle:} predicting flexible hinges by identification of stable domains},
  author={Flores, Samuel and Gerstein, Mark},
  journal={{BMC} bioinformatics},
  volume={8},
  number={1},
  year={2007},
  publisher={{BioMed} Central Ltd},
  doi={10.1186/1471-2105-8-215},
  url={http://dx.doi.org/10.1186/1471-2105-8-215}
}

@article{hingeatlas,
  title={Hinge Atlas: relating protein sequence to sites of structural flexibility.},
  author={Flores, Samuel and Lu, Long and Yang, Julie and Carriero, Nicholas and Gerstein, Mark},
  journal={{BMC} bioinformatics},
  volume={8},
  year={2007},
  abstract={Relating features of protein sequences to structural hinges is important for identifying domain boundaries, understanding structure-function relationships, and designing flexibility into proteins. Efforts in this field have been hampered by the lack of a proper dataset for studying characteristics of hinges.},
  doi={10.1186/1471-2105-8-167},
  url={http://dx.doi.org/10.1186/1471-2105-8-167}
}



@article{Gerek:2010,
  title={ A flexible docking scheme to explore the binding selectivity of PDZ domains},
  author={Gerek, Z. Nevin and Ozkan, S. Banu},
  journal={Protein Science},
  volume={19},
  year={2010},
   pages={914-928},
}


@article{vonderLieth:1996,
  title={ A bond flexibility index derived from the constitution of molecules},
  author={von der Lieth, C. W. and Stumpf-Nothof, K. and Prior, U. },
  journal={Journal of Chemical Information and Computer Science},
  volume={36},
  year={1996},
   pages={711--716},
}

@article{WFTian:2014,
  title={ A fast {ADI} algorithm for geometric flow equations in biomolecular surface generations},
  author={Tian, W. F. and Zhao, Shan},
  journal={International Journal for Numerical Methods in Biomedical Engineering},
  volume={30},
  year={2014},
   pages={490-516},
}



@article{Gaus:2011,
  title={ DFTB3: Extension of the Self-Consistent-Charge Density-Functional Tight-Binding Method (SCC-DFTB)},
  author={Gaus, M. and  Cui, Q. and   Elstner, M. },
  journal={ournal of Chemmical Theory and Computation   },
  volume={7},
  year={2011},
   pages={931-948},
}



@article{Daily:2013,
  title={Origin of parameter degeneracy and molecular shape relationships in geometric-flow calculations of solvation free energies},
  author={Daily, M. and  Chun, J. and Heredia-Langner, A. and  Wei, G. W. and  Baker, N. A.},
  journal={Journal of Chemical Physics, },
  volume={139},
  year={2013},
   pages={204108},
}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% Nanofluidic references by Jin Park %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%Daiguji
@article{daiguji2004ion,
  title={Ion transport in nanofluidic channels},
  author={Daiguji, Hirofumi and Yang, Peidong and Majumdar, Arun},
  journal={Nano Letters},
  volume={4},
  number={1},
  pages={137--142},
  year={2004},
  publisher={ACS Publications}
}
@article{daiguji2010ion,
  title={Ion transport in nanofluidic channels},
  author={Daiguji, H.},
  journal={Chemical Society Reviews},
  volume={39},
  number={3},
  pages={901--911},
  year={2010},
  publisher={Royal Society of Chemistry}
}
@article{daiguji2005nanofluidic,
  title={Nanofluidic diode and bipolar transistor},
  author={Daiguji, Hirofumi and Oka, Yukiko and Shirono, Katsuhiro},
  journal={Nano Letters},
  volume={5},
  number={11},
  pages={2274--2280},
  year={2005},
  publisher={ACS Publications}
}

%Sparreboom
@article{sparreboom2009principles,
  title={Principles and applications of nanofluidic transport},
  author={Sparreboom, W. and Van Den Berg, A. and Eijkel, JCT},
  journal={Nature nanotechnology},
  volume={4},
  number={11},
  pages={713--720},
  year={2009},
  publisher={Nature Publishing Group}
}

%Eijkel
@article{eijkel2005nanofluidics,
  title={Nanofluidics: what is it and what can we expect from it?},
  author={Eijkel, Jan CT and Berg, Albert van den},
  journal={Microfluidics and Nanofluidics},
  volume={1},
  number={3},
  pages={249--267},
  year={2005},
  publisher={Springer}
}

%Radak
@article{radak2008modeling,
  title={Modeling Ion Channels Using Poisson--Nernst--Planck Theory as an Integrated Approach To Introducing Nanotechnology Concepts: The PNP Cyclic Peptide Ion Channel Model},
  author={Radak, Brian and Hwang, Hyonseok and Schatz, George C},
  journal={Journal of Chemical Education},
  volume={85},
  number={5},
  pages={744},
  year={2008},
  publisher={ACS Publications}
}

%Di Ventra
@book{di2004introduction,
  title={Introduction to nanoscale science and technology},
  author={Di Ventra, Massimiliano and Evoy, Stephane and Heflin Jr, James R},
  volume={6},
  year={2004},
  publisher={Springer}
}

%Schoch
@article{schoch2008transport,
  title={Transport phenomena in nanofluidics},
  author={Schoch, Reto B and Han, Jongyoon and Renaud, Philippe},
  journal={Reviews of Modern Physics},
  volume={80},
  number={3},
  pages={839},
  year={2008},
  publisher={APS}
}

%zhou
@article{zhou2011transport,
  title={Transport and Sensing in Nanofluidic Devices},
  author={Zhou, Kaimeng and Perry, John M and Jacobson, Stephen C},
  journal={Annual Review of Analytical Chemistry},
  volume={4},
  pages={321--341},
  year={2011},
  publisher={Annual Reviews}
}


@article{vlassiouk2008nanofluidic,
  title={Nanofluidic ionic diodes. Comparison of analytical and numerical solutions},
  author={Vlassiouk, Ivan and Smirnov, Sergei and Siwy, Zuzanna},
  journal={ACS Nano},
  volume={2},
  number={8},
  pages={1589--1602},
  year={2008},
  publisher={ACS Publications}
}

@article{siwy2010engineered,
  title={Engineered voltage-responsive nanopores},
  author={Siwy, Zuzanna S and Howorka, Stefan},
  journal={Chemical Society Reviews},
  volume={39},
  number={3},
  pages={1115--1132},
  year={2010},
  publisher={Royal Society of Chemistry}
}

% Coalson
@article{coalson2005poisson,
  title={{Poisson-Nernst-Planck } theory approach to the calculation of current through biological ion channels},
  author={Coalson, R. D. and Kurnikova, M. G.},
  journal={NanoBioscience, IEEE Transactions on},
  volume={4},
  number={1},
  pages={81--93},
  year={2005},
  publisher={IEEE}
}

% Eisenberg
@article{hollerbach2001two,
  title={Two- and three-dimensional {Poisson--Nernst--Planck} simulations of current flow through {Gramicidin A}},
  author={Hollerbach, U. and Chen, D. P. and Eisenberg, R. S.},
  journal={Journal of Scientific Computing},
  volume={16},
  number={4},
  pages={373--409},
  year={2001},
  publisher={Springer}
}

% Cardenas
@article{cardenas2000three,
  title={Three-dimensional Poisson-Nernst-Planck theory studies: influence of membrane electrostatics on {Gramicidin A} channel conductance},
  author={Cardenas, Alfredo E and Coalson, Rob D and Kurnikova, Maria G},
  journal={Biophysical Journal},
  volume={79},
  number={1},
  pages={80--93},
  year={2000},
  publisher={Elsevier}
}

%%%% Matched interface and boundary method

@article{geng2011multiscale,
  title={Multiscale molecular dynamics using the matched interface and boundary method},
  author={Geng, Weihua and Wei, G. W.},
  journal={Journal of computational physics},
  volume={230},
  number={2},
  pages={435--457},
  year={2011},
  publisher={Elsevier}
}

% Yu
@article{yu2007matched,
  title={Matched interface and boundary {(MIB)} method for elliptic problems with sharp-edged interfaces},
  author={Yu, S. N. and Zhou, Y. and Wei, G. W.},
  journal={Journal of Computational Physics},
  volume={224},
  number={2},
  pages={729--756},
  year={2007},
  publisher={Elsevier}
}

@article{yu2007three,
  title={Three-dimensional matched interface and boundary (MIB) method for treating geometric singularities},
  author={Yu, Sining and Wei, GW},
  journal={Journal of Computational Physics},
  volume={227},
  number={1},
  pages={602--632},
  year={2007},
  publisher={Elsevier}
}


% Zhou
@article{zhou2006high,
  title={High order matched interface and boundary method for elliptic   equations with discontinuous coefficients and singular sources},
  author={Zhou, Y. C. and Zhao, S. and Feig, M. and Wei, G. W.},
  journal={Journal of Computational Physics},
  volume={213},
  number={1},
  pages={1--30},
  year={2006},
  publisher={Elsevier}
}

% Zheng
@article{zheng2011second,
  title={Second-order {Poisson Nernst-Planck} solver for ion transport},
  author={Zheng, Q. and Chen, D. and Wei, G. W.},
  journal={Journal of computational physics},
  year={2011},
  volume={230},
  pages={5239--5262}
}
@article{zheng2011poisson,
  title={Poisson--Boltzmann--Nernst--Planck model},
  author={Zheng, Qiong and Wei, Guo-Wei},
  journal={The Journal of chemical physics},
  volume={134},
  pages={194101},
  year={2011}
}

% Zhen
@article{yuan2007electrokinetic,
  title={Electrokinetic transport and separations in fluidic nanochannels},
  author={Yuan, Zhen and Garcia, Anthony L and Lopez, Gabriel P and Petsev, Dimiter N},
  journal={Electrophoresis},
  volume={28},
  number={4},
  pages={595--610},
  year={2007},
  publisher={Wiley Online Library}
}

% Karnik
@article{karnik2007rectification,
  title={Rectification of ionic current in a nanofluidic diode},
  author={Karnik, Rohit and Duan, Chuanhua and Castelino, Kenneth and Daiguji, Hirofumi and Majumdar, Arun},
  journal={Nano letters},
  volume={7},
  number={3},
  pages={547--551},
  year={2007},
  publisher={ACS Publications}
}

% Pu
@article{pu2004ion,
  title={Ion-enrichment and ion-depletion effect of nanochannel structures},
  author={Pu, Qiaosheng and Yun, Jongsin and Temkin, Henryk and Liu, Shaorong},
  journal={Nano Letters},
  volume={4},
  number={6},
  pages={1099--1103},
  year={2004},
  publisher={ACS Publications}
}

% Cheng
@article{cheng2010nanofluidic,
  title={Nanofluidic diodes},
  author={Cheng, Li-Jing and Guo, L Jay},
  journal={Chemical Society Reviews},
  volume={39},
  number={3},
  pages={923--938},
  year={2010},
  publisher={Royal Society of Chemistry}
}

% Mukhopadhyay
@article{mukhopadhyay2006does,
  title={What does nanofluidics have to offer?},
  author={Mukhopadhyay, Rajendrani},
  journal={Analytical Chemistry},
  volume={78},
  number={21},
  pages={7379--7382},
  year={2006},
  publisher={ACS Publications}
}

% Abgrall
@article{abgrall2008nanofluidic,
  title={Nanofluidic devices and their applications},
  author={Abgrall, Patrick and Nguyen, Nam Trung},
  journal={Analytical Chemistry},
  volume={80},
  number={7},
  pages={2326--2341},
  year={2008},
  publisher={ACS Publications}
}

% Modi
@article{modi2012computational,
  title={Computational modeling of ion transport through nanopores},
  author={Modi, Niraj and Winterhalter, Mathias and Kleinekath{\"o}fer, Ulrich},
  journal={Nanoscale},
  volume={4},
  number={20},
  pages={6166--6180},
  year={2012},
  publisher={Royal Society of Chemistry}
}

% Cervera
@article{cervera2005poisson,
  title={A {Poisson/Nernst-Planck} model for ionic transport through synthetic conical nanopores},
  author={Cervera, J and Schiedt, B and Ramirez, P},
  journal={EPL (Europhysics Letters)},
  volume={71},
  number={1},
  pages={35},
  year={2005},
  publisher={IOP Publishing}
}

% Li
@article{li1998brownian,
  title={Brownian dynamics study of ion transport in the vestibule of membrane channels},
  author={Li, Siu Cheung and Hoyles, Matthew and Kuyucak, Serdar and Chung, Shin-Ho},
  journal={Biophysical Journal},
  volume={74},
  number={1},
  pages={37--47},
  year={1998},
  publisher={Elsevier}
}

% Roux
@article{roux2004theoretical,
  title={Theoretical and computational models of biological ion channels},
  author={Roux, B. and Allen, T. and Berneche, S. and Im, W.},
  journal={Quarterly Reviews of Biophysics},
  volume={37},
  number={01},
  pages={15--103},
  year={2004},
  publisher={Cambridge Univ Press}
}

% Zhou
@article{zhou2008highly,
  title={Highly accurate biomolecular electrostatics in continuum dielectric environments},
  author={Zhou, YC and Feig, Michael and Wei, GW},
  journal={Journal of Computational Chemistry},
  volume={29},
  number={1},
  pages={87--97},
  year={2008},
  publisher={Wiley Online Library}
}

% Branton
@article{branton2008potential,
  title={The potential and challenges of nanopore sequencing},
  author={Branton, Daniel and Deamer, David W and Marziali, Andre and Bayley, Hagan and Benner, Steven A and Butler, Thomas and Di Ventra, Massimiliano and Garaj, Slaven and Hibbs, Andrew and Huang, Xiaohua and others},
  journal={Nature Biotechnology},
  volume={26},
  number={10},
  pages={1146--1153},
  year={2008},
  publisher={Nature Publishing Group}
}

% Perry
@article{perry2010ion,
  title={Ion transport in nanofluidic funnels},
  author={Perry, John M and Zhou, Kaimeng and Harms, Zachary D and Jacobson, Stephen C},
  journal={ACS Nano},
  volume={4},
  number={7},
  pages={3897--3902},
  year={2010},
  publisher={ACS Publications}
}

% Li
@article{li2003dna,
  title={DNA molecules and configurations in a solid-state nanopore microscope},
  author={Li, Jiali and Gershow, Marc and Stein, Derek and Brandin, Eric and Golovchenko, JA},
  journal={Nature Materials},
  volume={2},
  number={9},
  pages={611--615},
  year={2003},
  publisher={Nature Publishing Group}
}

% Stein
@article{stein2004surface,
  title={Surface-charge-governed ion transport in nanofluidic channels},
  author={Stein, Derek and Kruithof, Maarten and Dekker, Cees},
  journal={Physical Review Letters},
  volume={93},
  number={3},
  pages={035901},
  year={2004},
  publisher={APS}
}

% Wei
@article{wei2010differential,
  title={Differential geometry based multiscale models},
  author={Wei, Guo-Wei},
  journal={Bulletin of mathematical biology},
  volume={72},
  number={6},
  pages={1562--1622},
  year={2010},
  publisher={Springer}
}

% Holst
@phdthesis{holst1994poisson,
  title={The Poisson-Boltzmann Equation: Analysis and Multilevel Numerical Solution},
  author={Holst, Michael J},
  year={1994},
  school={Numerical Computing Group, University of Illinois at Urbana-Champaign}
}

% Corry
@article{corry2000tests,
  title={Tests of continuum theories as models of ion channels. II. Poisson--Nernst--Planck theory versus Brownian dynamics},
  author={Corry, Ben and Kuyucak, Serdar and Chung, Shin-Ho},
  journal={Biophysical Journal},
  volume={78},
  number={5},
  pages={2364--2381},
  year={2000},
  publisher={Elsevier}
}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%  End of  Nanofluidic references by Jin Park %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

@article{Busath:1998,
  title={Noncontact Dipole Effects on Channel Permeation. I. Experiments with (5F-Indole)Trp$^{13}$ {Gramicidin A} Channels},
  author={   Busath,  D. D.  and
     Thulin, C. D.  and
          Hendershot, R. W. and
     Phillips, L. R.  and
     Maughan, P. and
     Cole, C. D. and
     Bingham, N. C. and
      Morrison, S. and
     Baird, L. C. and
     Hendershot, R. J. and
     Cotten, M  and    Cross, T. A. },
  journal={Biophysical Journal},
  volume={75},
  number={},
  pages={2830--2844},
  year={1998},
  publisher={Elsevier}
}



@article{Ward:2012,
  title={Microfluidic-packaged CMOS chemiresistor detector for micro-scale gas chromatograph},
  author={Ward, N. and  Mu, X. and  Serrano, G. and  Covington, E. and  Kurdak, C. and  Zellers, E. T. and  Mason, A. J. and  Li, W.   },
  journal={Micro \& Nano Letters},
  volume={7},
  year={2012},
   pages={721--724},
}


@article{JPFu:2009,
  title={Continuous-flow bioseparation using microfabricated anisotropic nanofluidic
sieving structures},
  author={Fu, J. P.  and  Mao, P. and  Han, J. Y.     },
  journal={Nature Protocols },
  volume={4},
  year={2009},
   pages={1681--1698},
}



@article{Zhou2013Variational,
    abstract = {The synthetic host cucurbit[7]uril ({CB}[7]) binds aromatic guests or metal complexes with ultrahigh affinity compared with that typically displayed in protein?ligand binding. Due to its small size, {CB}[7] serves as an ideal receptor?ligand system for developing computational methods for molecular recognition. Here, we apply the recently developed variational implicit-solvent model ({VISM}), numerically evaluated by the level-set method, to study hydration effects in the high-affinity binding of the B2 bicyclo[2.2.2]octane derivative to {CB}[7]. For the unbound host, we find that the host cavity favors the hydrated state over the dry state due to electrostatic effects. For the guest binding, we find reasonable agreement to experimental binding affinities. Dissection of the individual {VISM} free-energy contributions shows that the major driving forces are water-mediated hydrophobic interactions and the intrinsic (vacuum) host?guest van der Waals interactions. These findings are in line with recent experiments and molecular dynamics simulations with explicit solvent. It is expected that the level-set {VISM}, with further refinement on the electrostatic descriptions, can efficiently predict molecular binding and recognition in a wide range of future applications. The synthetic host cucurbit[7]uril ({CB}[7]) binds aromatic guests or metal complexes with ultrahigh affinity compared with that typically displayed in protein?ligand binding. Due to its small size, {CB}[7] serves as an ideal receptor?ligand system for developing computational methods for molecular recognition. Here, we apply the recently developed variational implicit-solvent model ({VISM}), numerically evaluated by the level-set method, to study hydration effects in the high-affinity binding of the B2 bicyclo[2.2.2]octane derivative to {CB}[7]. For the unbound host, we find that the host cavity favors the hydrated state over the dry state due to electrostatic effects. For the guest binding, we find reasonable agreement to experimental binding affinities. Dissection of the individual {VISM} free-energy contributions shows that the major driving forces are water-mediated hydrophobic interactions and the intrinsic (vacuum) host?guest van der Waals interactions. These findings are in line with recent experiments and molecular dynamics simulations with explicit solvent. It is expected that the level-set {VISM}, with further refinement on the electrostatic descriptions, can efficiently predict molecular binding and recognition in a wide range of future applications.},
    author = {Zhou, Shenggao and Rogers, Kathleen E. and de Oliveira, C\'{e}sar A. and Baron, Riccardo and Cheng, Li-Tien and Dzubiella, Joachim and Li, Bo and McCammon, J. Andrew},
    day = {1},
    doi = {10.1021/ct400232m},
    journal = {J. Chem. Theory Comput.},
    keywords = {electrostatics, geometric\_flow, host-guest, nonpolar, solvation},
    month = aug,
    number = {9},
    pages = {4195--4204},
    priority = {2},
    publisher = {American Chemical Society},
    title = {Variational {Implicit-Solvent} Modeling of {Host-Guest} Binding: A Case Study on Cucurbit[7]uril|},
    url = {http://dx.doi.org/10.1021/ct400232m},
    volume = {9},
    year = {2013}
}


@article{DzubiellaHansen:2003,
    abstract = {We examine the effective force between two nanometer scale solutes in water by Molecular Dynamics simulations. Macroscopic considerations predict a strong reduction of the hydrophobic attraction between solutes when the latter are charged. This is confirmed by the simulations which point to a surprising constancy of the effective force between oppositely charged solutes at contact, while like charged solutes lead to significantly different behavior between positive and negative pairs. The latter exhibit the phenomenon of  ” like-charge attraction” previously observed in some colloidal dispersions. {\copyright} 2003 American Institute of Physics.},
    author = {Dzubiella, J. and Hansen, J. P.},
    doi = {10.1063/1.1632902},
    issn = {0021-9606},
    journal = {The Journal of Chemical Physics},
    keywords = {colloids, molecular\_dynamics, nanoparticles, nonpolar, solvation},
    number = {23},
    pages = {12049--12052},
    priority = {2},
    publisher = {AIP},
    title = {Reduction of the hydrophobic attraction between charged solutes in water},
    url = {http://dx.doi.org/10.1063/1.1632902},
    volume = {119},
    year = {2003}
}

@article{DzubiellaHansen:2004,
    abstract = {The solvation of charged, nanometer-sized spherical solutes in water, and the effective, solvent-induced force between two such solutes are investigated by constant temperature and pressure molecular dynamics simulations of model solutes carrying various chargepatterns. The results for neutral solutes agree well with earlier findings, and with predictions of simple macroscopic considerations: substantial hydrophobic attraction may be traced back to strong depletion ( ” drying”) of the solvent between the solutes. This hydrophobic attraction is strongly reduced when the solutes are uniformly charged, and the total force becomes repulsive at sufficiently high charge; there is a significant asymmetry between anionic and cationic solute pairs, the latter experiencing a lesser hydrophobic attraction. The situation becomes more complex when the solutes carry discrete (rather than uniform) chargepatterns. Due to antagonistic effects of the resulting hydrophilic and hydrophobic  ” patches” on the solvent molecules, water is once more significantly depleted around the solutes, and the effective interaction reverts to being mainly attractive, despite the direct electrostatic repulsion between solutes. Examination of a highly coarse-grained configurational probability density shows that the relative orientation of the two solutes is very different in explicit solvent, compared to the prediction of the crude implicit solvent representation. The present study strongly suggests that a realistic modeling of the charge distribution on the surface of globular proteins, as well as the molecular treatment of water, are essential prerequisites for any reliable study of protein aggregation.},
    author = {Dzubiella, J. and Hansen, J.-P.},
    day = {03},
    doi = {10.1063/1.1783274},
    issn = {0021-9606},
    journal = {The Journal of Chemical Physics},
    keywords = {electrostatics, geometric\_flow, nonpolar, solvation},
    month = sep,
    number = {11},
    pages = {5514--5530},
    priority = {2},
    title = {Competition of hydrophobic and Coulombic interactions between nanosized solutes},
    url = {http://dx.doi.org/10.1063/1.1783274},
    volume = {121},
    year = {2004}
}

@article{Li2013Variational,
    abstract = {
                Central in a variational implicit-solvent description of biomolecular solvation is an effective free-energy functional of the solute atomic positions and the solute-solvent interface (i.e., the dielectric boundary). The free-energy functional couples together the solute molecular mechanical interaction energy, the solute-solvent interfacial energy, the solute-solvent van der Waals interaction energy, and the electrostatic energy. In recent years, the sharp-interface version of the variational implicit-solvent model has been developed and used for numerical computations of molecular solvation. In this work, we propose a diffuse-interface version of the variational implicit-solvent model with solute molecular mechanics. We also analyze both the sharp-interface and diffuse-interface models. We prove the existence of free-energy minimizers and obtain their bounds. We also prove the convergence of the diffuse-interface model to the sharp-interface model in the sense of G-convergence. We further discuss properties of sharp-interface free-energy minimizers, the boundary conditions and the coupling of the {Poisson-Boltzmann} equation in the diffuse-interface model, and the convergence of forces from diffuse-interface to sharp-interface descriptions. Our analysis relies on the previous works on the problem of minimizing surface areas and on our observations on the coupling between solute molecular mechanical interactions with the continuum solvent. Our studies justify rigorously the self consistency of the proposed diffuse-interface variational models of implicit solvation.
            },
    author = {Li, Bo and Zhao, Yanxiang},
    doi = {10.1137/120883426},
    issn = {0036-1399},
    journal = {SIAM journal on applied mathematics},
    keywords = {electrostatics, geometric\_flow, nonpolar, review, solvation},
    number = {1},
    pages = {1--23},
    pmcid = {PMC3778507},
    pmid = {24058213},
    posted-at = {2014-02-16 00:42:45},
    priority = {2},
    title = {Variational Implicit Solvation with Solute Molecular Mechanics: From {Diffuse-Interface} to {Sharp-Interface} Models.},
    url = {http://dx.doi.org/10.1137/120883426},
    volume = {73},
    year = {2013}
}

@article{Setny:2009,
    abstract = {We report on a combined atomistic molecular dynamics simulation and implicit solvent analysis of a generic hydrophobic pocket-ligand (host-guest) system. The approaching ligand induces complex wetting-dewetting transitions in the weakly solvated pocket. The transitions lead to bimodal solvent fluctuations which govern magnitude and range of the pocket-ligand attraction. A recently developed implicit water model, based on the minimization of a geometric functional, captures the sensitive aqueous interface response to the concave-convex pocket-ligand configuration semiquantitatively.},
    author = {Setny, P. and Wang, Z. and Cheng, L. T. and Li, B. and McCammon, J. A. and Dzubiella, J.},
    day = {16},
    doi = {10.1103/physrevlett.103.187801},
    eprint = {0911.2970},
    journal = {Physical Review Letters},
    keywords = {geometric\_flow, ligand-protein\_interactions, nonpolar, solvation},
    month = oct,
    number = {18},
    pages = {187801+},
    posted-at = {2011-07-30 00:15:25},
    priority = {0},
    publisher = {American Physical Society},
    title = {{Dewetting-Controlled} Binding of Ligands to Hydrophobic Pockets},
    url = {http://dx.doi.org/10.1103/physrevlett.103.187801},
    volume = {103},
    year = {2009}
}


@article{Cheng2009Interfaces,
    abstract = {A model nanometer-sized hydrophobic receptor-ligand system in aqueous solution is studied by the recently developed level-set variational implicit solvent model ({VISM}). This approach is compared to all-atom computer simulations. The simulations reveal complex hydration effects within the (concave) receptor pocket, sensitive to the distance of the (convex) approaching ligand. The ligand induces and controls an intermittent switching between dry and wet states of the hosting pocket, which determines the range and magnitude of the pocket-ligand attraction. In the level-set {VISM}, a geometric free-energy functional of all possible solute-solvent interfaces coupled to the local dispersion potential is minimized numerically. This approach captures the distinct metastable states that correspond to topologically different solute-solvent interfaces, and thereby reproduces the bimodal hydration behavior observed in the all-atom simulation. Geometrical singularities formed during the interface relaxation are found to contribute significantly to the energy barrier between different metastable states. While the hydration phenomena can thus be explained by capillary effects, the explicit inclusion of dispersion and curvature corrections seems to be essential for a quantitative description of hydrophobically confined systems on nanoscales. This study may shed more light onto the tight connection between geometric and energetic aspects of biomolecular hydration and may represent a valuable step toward the proper interpretation of experimental receptor-ligand binding rates.},
    author = {Cheng, Li-Tien and Wang, Zhongming and Setny, Piotr and Dzubiella, Joachim and Li, Bo and McCammon, J. Andrew},
    day = {09},
    doi = {10.1063/1.3242274},
    issn = {0021-9606},
    journal = {The Journal of Chemical Physics},
    keywords = {electrostatics, geometric\_flow, geometry, ligand-protein\_interactions, nonpolar, solvation},
    month = oct,
    number = {14},
    pages = {144102+},
    pmid = {19831428},
    posted-at = {2011-04-30 02:43:06},
    priority = {0},
    publisher = {AIP},
    title = {Interfaces and hydrophobic interactions in receptor-ligand systems: A level-set variational implicit solvent approach},
    url = {http://dx.doi.org/10.1063/1.3242274},
    volume = {131},
    year = {2009}
}

@ARTICLE{BTu:2013,
  author = { Tu, B. and  Chen, M. X. and Xie, Y. and  Zhang, L. B. and  Eisenberg, B. and Lu, B. Z. },
  title = {  A Parallel Finite Element Simulator for Ion Transport through Three-Dimensional Ion Channel Systems
},
  year = {2013},
  journal = { J. Comput. Chem. },
  volume = {34},
  pages = {2065-2078 }
}



%%%%%%%%%%%%%%%%% Added by KELIN XIA ----11/27/2013


@article{Becker:2009,
  title={A Nitsche extended finite element method for incompressible elasticity with discontinuous modulus of elasticity},
  author={Becker, R. and   Burman, E. and Hansbo, P.},
  journal={Comput. Methods Appl. Mech. Engrg.},
  volume={198},
  year={2009},
   pages={3352--3360},
}

@PHDTHESIS{Mergheim:2006,
  author = {Mergheim, J.},
  title = {Computational Modeling of Strong and Weak Discontinuities},
  school = {Technical University of Kaiserslautern},
  year = {2006}
}

%%%%   XFEM and related
@article{Fries:2010,
  title={The extended/generalized finite element method: An overview of the method and its applications},
  author={Fries, T.  P. and Belyschko, T.},
  journal={Int. J. Numer. Meth. Engng.},
  volume={84},
  year={2010},
   pages={253--304},
}

@article{Sukumar:2001,
  title={Modeling holes and inclusions by level sets in the extended finite-element method},
  author={Sukumar, N. and  Chopp, D. L. and  Moes, N. and Belytschko, T.},
  journal={Comput. Methods Appl. Mech. Engrg.},
  volume={190},
  year={2001},
   pages={6180--6200},
}

@article{Stolarska:2001,
  title={Modelling crack growth by level sets in the extended finite element method},
  author={Stolarska, M. and Chopp, D. L. and Moes, N. and  Belytschko, T.},
  journal={Int. J. Numer. Meth. Engng},
  volume={51},
  year={2001},
   pages={943--960},
}

%%%%  lin tao and li zhilin.

@article{LinT:2012,
  title={Linear and bilinear immersed finite elements for planar elasticity interface problems},
  author={Lin, T. and Zhang, X.},
  journal={Journal of Computational and Applied Mathematics},
  volume={236},
  year={2012},
   pages={4681--4699},
}

@article{LinT:2013,
  title={A locking-free immersed finite element method for planar elasticity interface problems},
  author={Lin, T. and  Sheen, D. W. and Zhang, X.},
  journal={Journal of Comput. Phys.},
  volume={247},
  year={2013},
   pages={228--247},
}

@article{YangXZ:2003,
  title={The Immersed Interface Method for Elasticity Problems with Interface},
  author={Yang, X. Z. and Li, B. and Li, Z. L.},
  journal={Dyn. Contin. Discrete Impuls. Syst. Ser. A Math. Anal.},
  volume={10},
  year={2003},
   pages={783--808},
}

@article{LiZL:2005,
  title={An Immersed FEM for Elasticity Equations with Interfaces},
  author={Li, Z. L. and Yang, X. Z.},
  journal={AMS  Contemporary Mathematics},
  volume={383},
  year={2005},
   pages={285--298},
}

@article{XieH:2011,
  title={A finite element method for elasticity interface problems with locally modified triangulations},
  author={Xie, H. and Li, Z. L. and Qiao, Z. H.},
  journal={ International Journal of Numerical Analysis and Modeling},
  volume={8},
  year={2011},
   pages={189--200},
}

@article{HouSM:2012,
  title={A numerical method for solving elasticity equations with sharp-edged interfaces},
  author={Hou, S. and Li, Z. and  Wang, L. and Wang, W.},
  journal={ Commun. Comput. Phys.},
  volume={12},
  year={2012},
   pages={595--612},
}

%%%%%%%% xu zhiliang and wang xiaodong

@INPROCEEDINGS{XuZL:2003,
  author = { Xu, Z. L. and  Glimm,  J. and Li, X. L. },
  title = {Front Tracking Algorithm Using Adaptively Refined Meshes},
  booktitle = {Adaptive Mesh Refinement - Theory and Applications, the Lecture Notes in Computational Science and Engineering},
  year = {2003},
  pages = {83--89},
  month = {September}
}

@article{WangXS:2009,
  title={On computational issues of immersed ?nite element methods},
  author={Wang, X. S and  Zhang, L. T. and Liu, W. K.},
  journal={Journal of Comput. Phys.},
  volume={228},
  year={2009},
   pages={2535--2551},
}

%%%%%%%% BOOKS

@BOOK{Shearer:1999,
  title = { Introduction to seismology},
  publisher = {Cambridge University Press},
  year = {1999},
  author = {Shearer, P. M.}
}

@BOOK{Dvorak:2013,
  title = { Micromechanics of composite materials},
  publisher = {Springer},
  year = {2013},
  author = {Dvorak, G.}
}

@BOOK{Anandarajah:2010,
  title = { Computational Methods in Elasticity and Plasticity:Solids and Porous Media},
  publisher = {Springer},
  year = {2010},
  author = {Anandarajah, A.}
}

%%%%%%%%Eshelby

@article{Eshelby:1956,
  title={The continuum theory of lattice defects},
  author={Eshelby, J. D.},
  journal={Progress in solid state physics},
  volume={3},
  year={1956},
   pages={79--144},
}

@article{Eshelby:1957,
  title={The determination of the elastic field of an ellipsoidal inclusion, and related problems.},
  author={Eshelby, J. D.},
  journal={Proceedings of the Royal Society London A,},
  volume={241},
  year={1957},
   pages={376--396},
}

@article{Mathiesen:2008,
  title={Elasticity with arbitrarily shaped inhomogeneity.},
  author={Mathiesen, J. and Procaccia, I. and Regev, I. },
  journal={Physical Review E,},
  volume={77},
  year={2008},
   pages={026606},
}

@article{fonberg:1998,
  title={Calculation of weights in finite difference formulas.},
  author={B. Fornberg},
  journal={SIAM Rev},
  volume={40},
  year={1998},
   pages={685--691},
}
%%%%%%%%%%%%%%%%%%%%%%%%%%  END KELIN XIA





%%%%%%%%%%%%%%%%%%%%%% Kelin Xia added
@article{ZhangBL:1992a,
  title={The geometry of small fullerene cages:  {C$_{20}$} to  {C$_{70}$}},
  author={ Zhang, B. L. and Wang, C. Z. and   Ho, K. M. and  Xu, C. H. and Chan, C. T. },
  journal={The Journal of Chemical Physics},
  volume={97},
 number={5007},
  year={1992},
}

@article{ZhangBL:1992b,
  title={Systematic study of structures and stabilities of fullerens},
  author={ Zhang, B. L. and  Xu, C. H. and Wang, C. Z.  and Chan, C. T. and  Ho, K. M. },
  journal={ Physical Review B},
  volume={46},
 number={11},
  year={1992},
}

@article{Fowler:1996,
  title={Energetics of fullerenes with heptagonal rings},
  author={ Fowler, P. W. and Heine, T. and Mitchell, D. and Orlandi, G. and Schmidt, R. and Seifert, G. and Zerbetto, F. },
  journal={ J. Chem. Soc. Faraday Trans.},
  volume={92},
 number={12},
  year={1996},
}

@article{Murry:1994,
  title={Theoretical studies of fullerene annealing and fragmentation},
  author={Murry, R. L. and Strout, D. L. and Scuseria, G. E.},
  journal={International Journal of Mass Spectrometry and Ion Processes},
  volume={138},
 number={113-131},
  year={1994},
}

@article{Kroto:1985,
  title={{C$_{60}$}:Buckminster fullerene},
  author={Kroto, H. W. and Heath, J. R. and Obrien, S. C. and Curl, R. F. and Smalley, R. E.},
  journal={Nature},
  volume={318},
 number={162-163},
  year={1985},
}

@article{Kratschmer:1990,
  title={Solid {C$_{60}$}: a new form of carbon},
  author={Kratschmer,W. and  Lamb, L. D. and Fostiropoulos, K. and Huffman, D.R.},
  journal={Nature},
  volume={347},
 number={354-358},
  year={1990},
}

@article{Fowler:1988,
  title={Systematics of bonding in non-icosahedral carbon clusters},
  author={Fowler, P. W. and Cremona, J. E. and Steer, J. I.},
  journal={Theor. Chim. Acta},
  volume={73},
 number={1-26},
  year={1988},
}

@article{Manolopoulos:1991,
  title={Theoretical studies of the fullerenes: {C$_{34}$} to {C$_{70}$}},
  author={Manolopoulos, D. E. and May, J. C. and Down, S. E.},
  journal={Chemical Physics Letters},
  volume={181},
 number={105-111},
  year={1991},
}

@article{Fowler:1991,
  title={The higher fullerenes: a candidate for the structure of {C$_{78}$}},
  author={Fowler, P. W. and Batten, R. C. and Manolopoulos, D. E.},
  journal={J. Chem. Soc. Faraday Trans.},
  volume={87},
 number={3103-3104},
  year={1991},
}


@BOOK{Fowler:1995,
  title = {An atlas of fullerenes},
  publisher = {Clarendon press, Oxford},
  year = {1995},
  author = {Fowler, P. W. and Manolopoulos, D. E.}
}

@INPROCEEDINGS{Coxeter:1971,
  author = {Coxeter, H. S.},
  title = {Virus macromolecules and geodesic domes},
  booktitle = {A spectrum of mathematics},
  year = {1971},
  pages = {98-107},
 publisher={Auckland University Press, Auckland},
}

@BOOK{Streitwieser:1961,
  title = {Molecular orbital theory for organic chemists},
  publisher = {Wiley, New York},
  year = {1961},
  author = {Streitwieser, A.},
}

@ARTICLE{Raghavachari:1992,
   author = {Raghavachari, K.},
    title = {Ground state of {C$_{84}$}: two almost isoenergetic isomers},
  journal = {Chemical Physics Letters},
     year = 1992,
    pages = {397-400},
      doi = {10.1016/0009-2614(92)85162-4},
}

@article{Fowler:1994,
  title={Competing factors in fullerene stability},
  author={Fowler, P. W. and Austin, S. J. and Manolopoulos, D. E.},
  journal={Physics and Chemistry of the Fullerenes},
  volume={443},
 number={41-62},
  year={1994},
}

@BOOK{Schlegel:1883,
  title={Theorie der Homogen Zusammengesetzten Raumgebilde},
  author={Schlegel, V.},
  publisher = {Dresden, Druck von E. Blochmann und Sohn},
  year = {1883},
}

@article{Ballone:1990,
  title={Simulated annealing of carbon clusters},
  author={Ballone, P. and Milani, P.},
  journal={Physical Review B},
  volume={42},
 number={3201-3204},
  year={1990},
}

@article{Chelikowsky:1991,
  title = {Nucleation of {C$_{60}$} clusters},
  author = {Chelikowsky, J. R.},
  journal = {Phys. Rev. Lett.},
  volume = {67},
  issue = {21},
  pages = {2970--2973},
  year = {1991},
  month = {Nov},
  publisher = {American Physical Society},
}

@article {ChangYF:2005,
author = {Chang, Y. F. and Zhang, J. P. and Sun, H. and Hong, B. and An, Z. and Wang, R. S.},
title = {Geometry and stability of fullerene    cages: {C$_{24}$ to C$_{70}$}},
journal = {International Journal of Quantum Chemistry},
volume = {105},
number = {2},
publisher = {Wiley Subscription Services, Inc., A Wiley Company},
issn = {1097-461X},
url = {http://dx.doi.org/10.1002/qua.20691},
doi = {10.1002/qua.20691},
pages = {142--147},
keywords = {fullerenes, geometry, stability, DFT},
year = {2005},
}

%%%%%%%%%%%%%%%%% persistent homology

@article{Edelsbrunner:2002,
  title = {Topological persistence and simplification},
  author = {Edelsbrunner, H. and Letscher, D. and Zomorodian, A.},
  journal = {Discrete Comput. Geom.},
  volume = {28},
  issue = {4},
  pages = {511-533},
  year = {2002},
}

@article{Zomorodian:2005,
  title = {Computing {P}ersistent {H}omology},
  author = {Zomorodian, A. and Carlsson, G.},
  journal = {Discrete Comput. Geom.},
  volume = {33},
  issue = {2},
  pages = {249-274},
  year = {2005},
}

@article{Ghrist:2008,
  title = {Barcodes: {The} persistent topology of data},
  author = {Ghrist, R.},
  journal = {Bull. Amer. Math. Soc.},
  volume = {45},
  pages = {61-75},
  year = {2008},
}

@BOOK{Kaczynski:2004,
  title = {Computational homology},
  publisher = {Springer-Verlag},
  year = {2004},
  author = {Kaczynski, T. and Mischaikow, K. and Mrozek, M.}
}

@article{Mischaikow:1999,
  title = {Construction of symbolic dynamics from experimental time series},
  author = {Mischaikow, K. and Mrozek, M and Reiss, J. and Szymczak, A.},
  journal = { Physical Review Letters},
  volume = {82},
  pages = {1144-1147},
  year = {1999},
}

@article{Edelsbrunner:1994,
  title = {Three-dimensional alpha shapes},
  author = {Edelsbrunner, H. and Mucke, E. P.},
  journal = { Physical Review Letters},
  volume = {13},
  pages = {43-72},
  year = {1994},
}

@article{Carlsson:2008,
title={On the local behavior of spaces of natural images},
keywords={Topology; Natural images; Manifold; Filtration; Klein bottle; Persistent homology},
author={Carlsson, G. and Ishkhanov, T. and Silva, V. and Zomorodian, A.},
journal={International Journal of Computer Vision},
volume={76},
number={1},
pages={1-12},
year={2008},
}

@article{Carlsson:2009,
title={Topology and data},
author={Carlsson, G.},
journal={Am. Math. Soc},
volume={46},
number={2},
pages={255-308},
year={2009},
}

@article{YaoY:2009,
title={Topological methods for exploring low-density states in biomolecular folding pathways},
author={Yao, Y. and Sun, J. and Huang, X. H. and Bowman, G. R. and Singh, G. and Lesnick, M. and Guibas, L. J. and Pande, V. S. and Carlsson, G.},
journal={The Journal of Chemical Physics},
volume={130},
pages= {144115},
year={2009},
}

@article{:/content/aip/journal/jcp/130/14/10.1063/1.3103496,
   author = {Yao, Yuan and Sun, Jian and Huang, Xuhui and Bowman, Gregory R. and Singh, Gurjeet and Lesnick, Michael and Guibas, Leonidas J. and Pande, Vijay S. and Carlsson, Gunnar},
   title = {Topological methods for exploring low-density states in biomolecular folding pathways},
   journal = {The Journal of Chemical Physics},
   year = {2009},
   volume = {130},
   number = {14},
   url = {http://scitation.aip.org/content/aip/journal/jcp/130/14/10.1063/1.3103496},
   doi = {http://dx.doi.org/10.1063/1.3103496}
}


@article{Kasson:2007,
  title = {Persistent voids a new structural metric for membrane fusion},
  author = {Kasson, P. M. and Zomorodian, A. and Park, S. and Singhal, N. and Guibas, L. J. and Pande, V. S.},
  journal = {Bioinformatics},
  volume = {23},
  pages = {1753-1759},
  year = {2007},
}

@article{Gameiro:2013,
title={Topological measurement of protein compressibility via persistence diagrams},
author={Gameiro, M. and Hiraoka, Y. and Izumi, S. and Kramar, M. and Mischaikow, K. and Nanda, V.},
journal={preprint},
year = {2013},
}

@ARTICLE{Pachauri:2011,
author={Pachauri, D. and Hinrichs, C. and Chung, M.K. and Johnson, S.C. and Singh, V.},
journal={Medical Imaging, IEEE Transactions on},
title={Topology-Based Kernels With Application to Inference Problems in Alzheimer's Disease},
year={2011},
month={Oct},
volume={30},
number={10},
pages={1760-1770},
keywords={biomedical MRI;diseases;image classification;inference mechanisms;medical image processing;neurophysiology;regression analysis;support vector machines;Alzheimer's Disease Neuroimaging Initiative;Alzheimer's disease;SVM;automated inference;classification;cortical surfaces;cortical thickness measures;imaging data;inference problems;kernel based methods;kernel matrix specification;neuroimaging applications;neurological disorders;regression;scalar similarity measure;similarity matrix;statistical learning tools;support vector machine;topologically based attributed data;topology based kernels;Accuracy;Alzheimer's disease;Kernel;Neuroimaging;Surface treatment;Thickness measurement;Topology;Alzheimer's Disease Neuroimaging Initiative (ADNI);Alzheimer's disease;cortical thickness based kernels;topological persistence;Alzheimer Disease;Cerebral Cortex;Databases, Factual;Fourier Analysis;Humans;Image Processing, Computer-Assisted;Neuroimaging;ROC Curve;Regression Analysis;Support Vector Machines},
doi={10.1109/TMI.2011.2147327},
ISSN={0278-0062},}

@ARTICLE{LeeH:2012,
author={Lee, H and Kang, H. and Chung, M. K. and Kim, B. and Lee, D. S.},
journal={Medical Imaging, IEEE Transactions on},
title={Persistent Brain Network Homology From the Perspective of Dendrogram},
year={2012},
month={Dec},
volume={31},
number={12},
pages={2267-2277},
keywords={brain;medical disorders;positron emission tomography;Betti number;FDG-PET based functional brain network;Gromov-Hausdorff distance;Rips filtration;autism spectrum disorder children;barcode;novel multiscale framework;pediatric control subject;persistent brain network homology;persistent homology;single linkage dendrogram;Brain models;Correlation;Couplings;Measurement;Superluminescent diodes;Visualization;Barcode;Gromov-Hausdorff distance;functional brain network;persistent homology;rips complex;rips filtration;single linkage dendrogram;Attention Deficit Disorder with Hyperactivity;Brain Mapping;Case-Control Studies;Child;Child Development Disorders, Pervasive;Child, Preschool;Cluster Analysis;Female;Fluorodeoxyglucose F18;Humans;Image Processing, Computer-Assisted;Male;Neural Pathways;Positron-Emission Tomography;Radiopharmaceuticals},
doi={10.1109/TMI.2012.2219590},
ISSN={0278-0062},}

@INPROCEEDINGS{Silva:2005,
    author = {Silva, V. D. and Ghrist, R},
    title = {Blind swarms for coverage in 2-D},
    booktitle = {In Proceedings of Robotics: Science and Systems},
    year = {2005},
    pages = {01}
}

@article{Horak:2009,
  author={Horak, D. and Maletic, S and Rajkovic, M.},
  title={Persistent homology of complex networks},
  journal={Journal of Statistical Mechanics: Theory and Experiment},
  volume={2009},
  number={03},
  pages={P03034},
  url={http://stacks.iop.org/1742-5468/2009/i=03/a=P03034},
  year={2009},
  abstract={Long-lived topological features are distinguished from short-lived ones (considered as topological noise) in simplicial complexes constructed from complex networks. A new topological invariant, persistent homology, is determined and presented as a parameterized version of a Betti number. Complex networks with distinct degree distributions exhibit distinct persistent topological features. Persistent topological attributes, shown to be related to the robust quality of networks, also reflect the deficiency in certain connectivity properties of networks. Random networks, networks with exponential connectivity distribution and scale-free networks were considered for homological persistency analysis.}
}

@article{Dabaghian:2012,
    author = {Dabaghian,  Y.  and Memoli,  F.  and Frank, L. and Carlsson, G.},
    journal = {PLoS Comput Biol},
    publisher = {Public Library of Science},
    title = {A Topological Paradigm for Hippocampal Spatial Map Formation Using Persistent Homology},
    year = {2012},
    month = {08},
    volume = {8},
    url = {http://dx.doi.org/10.1371%2Fjournal.pcbi.1002581},
    pages = {e1002581},
    abstract = {<title>Author Summary</title><p>Our ability to navigate our environments relies on the ability of our brains to form an internal representation of the spaces we're in. The hippocampus plays a central role in forming this internal spatial map, and it is thought that the ensemble of active “place cells” (neurons that are sensitive to location) somehow encode metrical information about the environment, akin to a street map. Several considerations suggested to us, however, that the brain might be more interested in topological information—i.e., connectivity, containment, and adjacency, more akin to a subway map— so we employed new methods in computational topology to estimate how basic properties of neuronal firing affect the time required to form a hippocampal spatial map of three test environments. Our analysis suggests that, in order to encode topological information correctly and in a biologically reasonable amount of time, the hippocampal place cells must operate within certain parameters of neuronal activity that vary with both the geometric and topological properties of the environment. The interplay of these parameters forms a “learning region” in which changes in one parameter can successfully compensate for changes in the others; values beyond the limits of this region, however, impair map formation.</p>},
    number = {8},
    doi = {10.1371/journal.pcbi.1002581}
}

@article{Singh:2008,
author = {Singh, G. and Memoli, F. and Ishkhanov, T. and Sapiro, G. and Carlsson, G. and Ringach, D. L.},
title = {Topological analysis of population activity in visual cortex},
volume = {8},
number = {8},
year = {2008},
doi = {10.1167/8.8.11},
abstract ={Information in the cortex is thought to be represented by the joint activity of neurons. Here we describe how fundamental questions about neural representation can be cast in terms of the topological structure of population activity. A new method, based on the concept of persistent homology, is introduced and applied to the study of population activity in primary visual cortex (V1). We found that the topological structure of activity patterns when the cortex is spontaneously active is similar to those evoked by natural image stimulation and consistent with the topology of a two sphere. We discuss how this structure could emerge from the functional organization of orientation and spatial frequency maps and their mutual relationship. Our findings extend prior results on the relationship between spontaneous and evoked activity in V1 and illustrates how computational topology can help tackle elementary questions about the representation of information in the nervous system.},
URL = {http://www.journalofvision.org/content/8/8/11.abstract},
eprint = {http://www.journalofvision.org/content/8/8/11.full.pdf+html},
journal = {Journal of Vision} ,
}

@article{Mischaikow:2013,
year={2013},
issn={0179-5376},
journal={Discrete and Computational Geometry},
volume={50},
number={2},
doi={10.1007/s00454-013-9529-6},
title={Morse Theory for Filtrations and Efficient Computation of Persistent Homology},
url={http://dx.doi.org/10.1007/s00454-013-9529-6},
publisher={Springer US},
keywords={Computational topology; Discrete Morse theory; Persistent homology},
author={Mischaikow, K. and Nanda, V.},
pages={330-353},
language={English},
}

@book{Edelsbrunner:2010,
  title={Computational topology: an introduction},
  author={Edelsbrunner, H. and Harer, J.},
  year={2010},
  publisher={American Mathematical Soc.},
}

@article{Dey:2013,
year={2013},
issn={0179-5376},
journal={Discrete and Computational Geometry},
volume={49},
number={1},
doi={10.1007/s00454-012-9463-z},
title={Reeb Graphs: Approximation and Persistence},
url={http://dx.doi.org/10.1007/s00454-012-9463-z},
publisher={Springer-Verlag},
author={Dey, T. K. and Wang, Y. S.},
pages={46-73},
language={English}
}

@article{Dey:2008,
  author = {Dey, T. K. and Li, K. Y. and Sun, J. and David, C. S.},
  journal = {ACM Trans. Graph.},
  title = {Computing geometry aware handle and tunnel loops in 3D models.},
  volume = {27},
  year = {2008},
}

@misc{javaPlex,
    author = {Tausz, Andrew and Vejdemo-Johansson, Mikael and Adams, Henry},
    title = {JavaPlex: A research software package for persistent (co)homology},
    year = {2011},
    howpublished = "Software available at \url{http://code.google.com/p/javaplex}"
}

@misc{Perseus,
     author = {Vidit Nanda},
    title = {Perseus: the persistent homology software},
    howpublished = "Software available at \url{http://www.sas.upenn.edu/~vnanda/perseus}"
}

@misc{Dionysus,
    title = {Dionysus: the persistent homology software},
    howpublished = "Software available at \url{http://www.mrzv.org/software/dionysus}"
}


@ARTICLE{Munch:2013,
  author = {Munch, Elizabeth},
  title = {Applications of persistent homology to time varying systems},
  year = {2013},
  note = {Dissertation of Duke University}
}


@article{Hakon:1935,
  title={Volume, Shape and Roundness of Quartz Particles},
  author={ Hakon, Wadell},
  journal={Journal of Geology},
  volume={43},
  year={1935},
   pages={250--280},
}


@article{Feng:2013,
author = {Xin Feng and Yiying Tong},
title = {Choking Loops on Surfaces},
journal ={IEEE Transactions on Visualization and Computer Graphics},
volume = {19},
number = {8},
issn = {1298-1306},
year = {2013},
pages = {1298--1306},
doi = {http://doi.ieeecomputersociety.org/10.1109/TVCG.2013.9},
publisher = {IEEE Computer Society},
address = {Los Alamitos, CA, USA},
}

@article{Frosini:1999,
  title={Size theory as a topological tool for computer vision},
  author={Frosini, Patrizio and Landi, Claudia},
  journal={Pattern Recognition and Image Analysis},
  volume={9},
  number={4},
  pages={596--603},
  year={1999}
}

@inproceedings{Robins:1999,
  title={Towards computing homology from finite approximations},
  author={Robins, Vanessa},
  booktitle={Topology Proceedings},
  volume={24},
  number={},
  pages={503--532},
  year={1999}
}


@article{bubenik:2015,
  title={Statistical topological data analysis using persistence landscapes},
  author={Bubenik, P.},
  journal={The Journal of Machine Learning Research},
  volume={16},
  number={1},
  pages={77--102},
  year={2015}
}

@book{zomorodian2005topology,
  title={Topology for computing},
  author={Zomorodian, A. J.},
  volume={16},
  year={2005},
  publisher={Cambridge university press}
}


@book{munkres2018elements,
  title={Elements of algebraic topology},
  author={Munkres, J. R.},
  year={2018},
  publisher={CRC Press}
}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

@book{Allen:1987,
  title={Computer Simulation of Liquids},
  author={Allen, M. P. and Tildesley, D. J.},
  year={1987},
  publisher={ Oxford: Clarendon Press},
}


@article{Rossman:1974,
  title={Recognition of structural domains in globular proteins},
  author={Rossman, M. G. and  Liljas, A. },
  journal={ Journal of Molecular Biology},
  volume={85},
  number={},
  pages={177-181},
  year={1974}
}

@article{Bakan:2011,
  title={ProDy: Protein Dynamics Inferred from Theory and Experiments},
  author={Bakan, A and Meireles, L. M. and  Bahar, I.},
  journal={Bioinformatics},
  volume={27},
  number={},
  pages={1575 -1577},
  year={2011}
}


@article{CTWu:2013,
  title={Numerical modeling of composite solids using an immersed meshfree Galerkin method
},
  author={Wu, C. T. and  Guo, Y. and  Askari, E.},
  journal={Composites Part B: Engineering},
  volume={45},
  number={},
  pages={1397 - 1413},
  year={2013}
}

@article{YChang:2012,
  title={Adaptive Finite Element Method for Elasticity Interface Problems
},
  author={Chang, Y. Z. },
  journal={Journal of Computational Mathematics},
  volume={30},
  number={},
  pages={629 - 642},
  year={2012}
}

	
	
@article{YGong:2010,
  title={Immersed Interface Finite Element Methods for Elasticity Interface Problems with Non-Homogeneous Jump Conditions
},
  author={Gong, Y. and Li, Z. L.},
  journal={Numerical Mathematics -- Theoretical Methods and Applications},
  volume={3},
  number={},
  pages={23 - 39},
  year={2010}
}

	
	@article{Pinho:2013,
  title={ Automatic tracking of labeled red blood cells in microchannels},
  author={Pinho, D. and  Lima, R and  Pereira, A. I. and    Gayubo, F. },
  journal={International Journal for Numerical Methods in Biomedical Engineering},
  volume={29},
  year={2013},
   pages={ 977-987},
}



	@article{Isebe:2013,
  title={ Numerical simulation of particle dynamics in an orifice-electrode system. Application to counting and sizing by impedance measurement},
  author={Isebe, D. and  Nerin, P.  },
  journal={International Journal for Numerical Methods in Biomedical Engineering},
  volume={29},
  year={2013},
   pages={ 462-475}
}



@book{Hadwiger:1975,
  title={Vorlesungen \"{U}ber Inhalt, Oberfl\"{a}che und Isoperimetrie},
  author={Hadwiger, Hugo},
  year={1975},
  publisher={Springer},
}

@book{Hatcher:2001,
  title={Algebraic Topology},
  author={Allen Hatcher},
  year={2001},
  publisher={Cambridge University Press },
}


@article{Holec:2010,
  title={Curvature-induced excess surface energy of fullerenes: Density functional theory
and Monte Carlo simulations},
  author={Holec, David and   Hartmann, M. A. and Fischer, F. D. and Rammerstorfer, F. G. and Mayrhofer, P. H.  and  Paris, O. },
 journal={Phys. Rev. B},
  volume={81},
  year={2010},
   pages={235403}
}



@article{Guan:2014,
  title={Local curvature and stability of two-dimensional systems},
  author={Guan, J. and   Jin, Z. Q. and  Zhu, Z. and   Tom\'{a}nek, D.},
 journal={preprint},
  volume={},
  year={2014},
   pages={}
}



@article{BWang:2014a,
  title={Matched Interface and Boundary Method for Elasticity Interface Problems},
  author={ Wang, Bao and Xia K. L. and Wei, G. W.},
 journal={preprint},
  volume={},
  year={2014},
   pages={}
}


@article{BWang:2014d,
  title={ Superconvergent biomolecular electrostatic analysis by using a simplified MIBPB (SMIBPB) method},
  author={ Wang, Bao  and Wei, G. W.},
 journal={Journal of Computational Chemistry},
  volume={},
  year={submitted 2014},
   pages={}
}




%%%%%%%%%%%%%%%%%  Added by Kelin Xia
@article{YangLei:2009,
author = {Yang, L. and Song, G. and Jernigan, R. L.},
title = {Protein elastic network models and the ranges of cooperativity},
volume = {106},
number = {30},
pages = {12347-12352},
year = {2009},
doi = {10.1073/pnas.0902159106},
abstract ={Elastic network models (ENMs) are entropic models that have demonstrated in many previous studies their abilities to capture overall the important internal motions, with comparisons having been made against crystallographic B-factors and NMR conformational variabilities. ENMs have become an increasingly important tool and have been widely used to comprehend protein dynamics, function, and even conformational changes. However, reliance upon an arbitrary cutoff distance to delimit the range of interactions has presented a drawback for these models, because the optimal cutoff values can differ somewhat from protein to protein and can lead to quirks such as some shuffling in the order of the normal modes when applied to structures that differ only slightly. Here, we have replaced the requirement for a cutoff distance and introduced the more physical concept of inverse power dependence for the interactions, with a set of elastic network models that are parameter-free, with the distance cutoff removed. For small fluctuations about the native forms, the power dependence is the inverse square, but for larger deformations, the power dependence may become inverse 6th or 7th power. These models maintain and enhance the simplicity and generality of the original ENMs, and at the same time yield better predictions of crystallographic B-factors (both isotropic and anisotropic) and of the directions of conformational transitions. Thus, these parameter-free ENMs can be models of choice whenever elastic network models are used.},
URL = {http://www.pnas.org/content/106/30/12347.abstract},
eprint = {http://www.pnas.org/content/106/30/12347.full.pdf+html},
journal = {Proceedings of the National Academy of Sciences}
}


@article{ChangHW:2013,
  title={Persistent topology and metastable state in conformational dynamics},
  author={Chang, H. W. and Bacallado, S. and Pande, V. S. and Carlsson, G. E.},
 journal={PLos ONE},
  volume={8},
  number = {4},
  year={2013},
   pages={ e58699   }
}



@article{Mate:2014,
  title={A topological similarity measure for proteins },
  author={Mate, G. and  Hofmann, A. and  Wenzel, N. and  Heermann, D. W.},
 journal={Biochimica et Biophysica Acta (BBA) - Biomembranes},
  volume={1838},
  number = {},
  year={2014},
   pages={1180-1190}
}



@article{Biasotti:2008,
  title={Describing Shapes by Geometrical-Topological Properties of Real Functions  },
  author={Biasotti, S. and  De Floriani, L.  and  Falcidieno, B. and  Frosini, P. and  Giorgi, D. and  Landi, C. and  Papaleo, L. and  Spagnuolo, M.},
 journal={ACM Computing Surveys },
  volume={40},
  number = {4},
  year={2008},
   pages={12}
}

 @article{Zomorodian:2008,
  title={Localized homology},
  author={Zomorodian, A. and Carlsson, G.},
 journal={Computational Geometry - Theory and Applications},
  volume={41},
  number = {3},
  year={2008},
   pages={126-148}
}


 @article{Bendich:2010,
  title={Computing Robustness and Persistence for Images},
  author={Bendich, P. and  Edelsbrunner, H. and  Kerber, M.},
 journal={IEEE Transactions on Visualization and Computer Graphics },
  volume={16},
  number = {},
  year={2010},
   pages={1251-1260}
}



 @article{Bubenik:2007,
  title={A statistical approach to persistent homology},
  author={Bubenik, P. and  Kim, P. T.},
 journal={Homology, Homotopy and Applications  },
  volume={19},
  number = {},
  year={2007},
   pages={337-362}
}




 @article{Niyogi:2011,
  title={A Topological View of Unsupervised Learning from Noisy data},
  author={Niyogi, P. and  Smale, S. and Weinberger, S.},
 journal={SIAM Journal on Computing  },
  volume={40},
  number = {},
  year={2011},
   pages={ 646-663}
}


 @article{Frosini:2013,
  title={Persistent {Betti} numbers for a noise tolerant shape-based approach to image retrieval},
  author={Frosini, P. and Landi, C.},
 journal={Pattern Recognition Letters },
  volume={34},
  number ={8},
  year={2013},
   pages={863-872}
}


 @article{DiFabio:2011,
  title={A {Mayer-Vietoris} Formula for Persistent Homology with an Application to Shape Recognition in the Presence of Occlusions},
  author={Di Fabio, B. and  Landi, C.},
 journal={Foundations of Computational Mathematics  },
  volume={11},
  number = {},
  year={2011},
   pages={499-527}
}

@article{BeiWang:2011,
  title={Branching and Circular Features in High Dimensional Data},
  author={Wang, B. and  Summa, B. and  Pascucci, V. and Vejdemo-Johansson, M.},
 journal={IEEE Transactions on Visualization and Computer Graphics },
  volume={17},
  number = {},
  year={2011},
   pages={1902-1911}
}


@article{Rieck:2012,
  title={Multivariate Data Analysis Using Persistence-Based Filtering and Topological Signatures},
  author={Rieck, B. and  Mara, H. and Leitte, H.},
 journal={IEEE Transactions on Visualization and Computer Graphics },
  volume={18},
  number = {},
  year={2012},
   pages={2382-2391}
}


@article{XuLiu:2012,
  title={A fast algorithm for constructing topological structure in large data},
  author={Liu, X. and Xie, Z. and  Yi, D. Y.},
 journal={Homology, Homotopy and Applications },
  volume={14},
  number = {},
  year={2012},
   pages={221-238}
}


@article{Michaeli:2013,
  title={A Nitsche type method for stress fields calculation in dissimilar material with interface crack},
  author={Michaeli, Michael and Assous, Franck and  Golubchik, Anatoly},
 journal={Applied Numerical Mathematics },
  volume={67},
  number = {},
  year={2013},
   pages={187-203}
}



@article{Theillard:2013,
  title={A second-order sharp numerical method for solving the linear elasticity equations on irregular domains and adaptive grids - Application to shape optimization},
  author={Theillard, M and  Djodom, L. F. and  Vie, J. L.  and  Gibou, F. },
 journal={Journal of Computational Physics },
  volume={233},
  number = {},
  year={2013},
   pages={430--448}
}


@article{Boileau:2013,
  title={Flow-induced ATP release in patient-specific arterial geometries - a comparative study of computational models },
  author={Boileau, E. and  Bevan, R. L. T.  and  Sazonov, I.  and  Rees, M. I. and  Nithiarasu, P. },
 journal={International Journal for Numerical Methods in Engineering },
  volume={29},
  number = {},
  year={2013},
   pages={1038--1056}
}




@article{Sazonov:2012b,
  title={Modelling pipeline for subject-specific arterial blood flow -- A review  },
  author={  Sazonov, I. and  Yeo, S. Y. and  Bevan, R. L. T. and  Xie, X. H. and  van Loon, R. and  Nithiarasu, P. },
 journal={International Journal for Numerical Methods in Engineering },
  volume={28},
  number = {},
  year={2012},
   pages={ 1868-1910  }
}


@article{Mikhal:2013,
  title={Flow prediction in cerebral aneurysms based on geometry reconstruction from 3D rotational angiography },
  author={Mikhal, J and  Kroon, D. J. and Slump, C. H. and  Geurts, B. J.  },
 journal={International Journal for Numerical Methods in Engineering },
  volume={29},
  number = {},
  year={2013},
   pages={ 777-- 805 }
}




@article{Manzoni:2012,
  title={Model reduction techniques for fast blood flow simulation in parametrized geometries },
  author={ Manzoni, Andrea and  Quarteroni, Alfio and  Rozza, Gianluigi },
 journal={International Journal for Numerical Methods in Engineering },
  volume={28},
  number = {},
  year={2012},
   pages={ 604-625  }
}


@article{Ramalho:2012,
  title={Sensitivity to outflow boundary conditions and level of geometry description for a cerebral aneurysm   },
  author={Ramalho, S and  Moura, A and   Gambaruto, A. M. and  Sequeira, A.  },
 journal={International Journal for Numerical Methods in Engineering },
  volume={28},
  number = {},
  year={2012},
   pages={ 697-713}
}



@article{Sohn:2012,
  title={Axisymmetric multicomponent vesicles: A comparison of hydrodynamic and geometric models    },
  author={Sohn, J. S.  and  Li, S. W. and Li, X. F. and Lowengrub, J. S. },
 journal={International Journal for Numerical Methods in Engineering },
  volume={28},
  number = {},
  year={2012},
   pages={ 346--368}
}



@ARTICLE{SJLee:2012,
  author = {Lee, S. J.  and  Schlesinger, P. H. and  Wickline, S. A.  ND  Lanza, G. M.  and   Baker, N. A. },
  month = {},
  year = {2012},
  title = {Interaction of Melittin Peptides with Perfluorocarbon Nanoemulsion Particles},
  note = {},
  journal = {  Journal of Physical Chemistry B},
  volume = {115},
  number = {},
  pages = {15271-15279}
}




@ARTICLE{Pham:2014,
  author = {Pham, C. T. N. and  Thomas, D. G.  and Beiser, J. and  Mitchell, L. M. and  Huang, J. L. and   Senpan, A. and    Hu, G. and    Gordon, M. and   Baker, N. A.  and  Pan, D. and  and  Lanza, G. M. and   Hourcade, D. E. },
  month = {},
  year = {2014},
  title = {Application of a hemolysis assay for analysis of complement activation by Pham:2014,},
  note = {},
  journal = { NanoMedicine---Nanotechnology Biology and Medicine  },
  volume = {10},
  number = {},
  pages = {651-660}
}



@ARTICLE{Goel:2007,
  author = {Goel, T and  Patra, C. N.},
  month = {},
  year = {2007},
  title = {Structure of spherical electric double layers: A density functional approach},
  note = {},
  journal = {  Journal of Chemical Physics },
  volume = {127},
  number = {},
  pages = {034502}
}


@ARTICLE{Forsman:2009,
  author = {Forsman, J.},
  month = {},
  year = {2009},
  title = {Density functional theories of surface interactions in salt solutions},
  note = {},
  journal = {  Journal of Chemical Physics },
  volume = {130},
  number = {},
  pages = {064901}
}

@ARTICLE{Medasani:2014,
  author = {Medasani, B. and Ovanesyan, Z and  Thomas, D. G. and  Sushko, M. L. and Marucho1, M.},
  month = {},
  year = {2014},
  title = {Ionic asymmetry and solvent excluded volume effects on spherical electric
double layers: A density functional approach},
  note = {},
  journal = {  Journal of Chemical Physics },
  volume = {140},
  number = {},
  pages = {204510}
}

@ARTICLE{Diehl:1999,
  author = {Diehla, A. and  Tamashirob, M. N.  and  Barbosa, M. C. and Levin, Y.},
  month = {},
  year = {1999},
  title = {Density-functional theory for attraction between
like-charged plates},
  note = {},
  journal = {    Physica A },
  volume = {274},
  number = {},
  pages = {433--445}
}

@ARTICLE{Gillespie:2011,
  author = {Gillespie, D.},
  month = {},
  year = {2011},
  title = {Free-Energy Density Functional of Ions at a Dielectric Interface},
  note = {},
  journal = {J. Phys. Chem. Lett.   },
  volume = {2},
  number = {},
  pages = {1178--1182}
}

@ARTICLE{Frink:2012,
  author = {Frink, L. J. D. and   Frischknecht, A. L. and Heroux, M. A. and  Parks, M. L. and  Salinger, A. G. },
  month = {},
  year = {2012},
  title = {Toward Quantitative Coarse-Grained Models of Lipids with Fluids Density Functional Theory},
  note = {},
  journal = {J.  Chem. Theo. Comput.   },
  volume = {8},
  number = {},
  pages = {1393--1408}
}



@ARTICLE{Giambasu:2014,
  author = {Giambasu, G. M. and  Luchko, T. and Herschlag, D. and  York, D. M. and Case, D. A. },
  month = {},
  year = {2014},
  title = {Ion Counting from Explicit-Solvent Simulations and 3D-RISM
},
  note = {},
  journal = {Biophysical Journal  },
  volume = {106},
  number = {},
  pages = {883--894}
}


@ARTICLE{Bai:2007,
  author = {Bai, Y. and  Greenfeld, M. and Travers, K. J. and Chu, V. B. and Lipfert, J. and Doniach, S. and Herschlag, D. },
  month = {},
  year = {2007},
  title = {
Quantitative and comprehensive decomposition of the ion atmosphere around nucleic acids
},
  note = {},
  journal = {J. Am. Chem. Soc.},
  volume = {129},
  number = {},
  pages = {14981--14988}
}



@ARTICLE{Greenfeld:2009,
  author = {  Greenfeld, M.     and Herschlag, D. },
  month = {},
  year = {2007},
  title = {Probing nucleic acid-ion interactions with buffer exchange-atomic emission spectroscopy},
  note = {},
  journal = {Methods Enzymol.},
  volume = {469},
  number = {},
  pages = {375--389}
}



@ARTICLE{Doraiswamy:2013,
  author = { Doraiswamy, Harish and Natarajan, Vijay },
  month = {},
  year = {2013},
  title = {Computing Reeb Graphs as a Union of Contour Trees},
  note = {},
  journal = { IEEE Transactions on Visualization and Computer Graphics},
  volume = {19},
  number = {},
  pages = {249--262}
}



@article{Fujishiro:2000,
author = {Issei Fujishiro and Yuriko Takeshima and Taeko Azuma and Shigeo Takahashi},
title = {Volume Data Mining Using 3D Field Topology Analysis},
journal ={IEEE Computer Graphics and Applications},
volume = {20},
number = {5},
issn = {0272-1716},
year = {2000},
pages = {46-51},
doi = {http://doi.ieeecomputersociety.org/10.1109/38.865879},
publisher = {IEEE Computer Society},
address = {Los Alamitos, CA, USA},
}



@article{MTopf:2008,
author = {Maya Topf and  Keren Lasker and  Ben Webb and  Haim Wolfson and  Wah Chiuand Andrej Sali},
title = {Protein Structure Fitting and Refinement Guided by Cryo-EM Density},
journal ={Structure},
volume = {16},
year = {2008},
pages = {295-307},
}




@article{HWWang:2005,
author = {Wang, W. H. and Nogales, E.},
title = {Nucleotide-dependent bending flexibility of tubulin regulates microtubule assembly},
journal ={Nature},
volume = {435},
year = {2005},
pages = {911-915},
}




@article{EM3D:1999,
author = {Ress, D. and  Harlow, M. L. and  Schwarz, M. and  Marshall, R. M. and  McMahan, U. J.},
title = {Automatic acquisition of fiducial markers and alignment of images in tilt series for electron tomography},
journal ={J Electron Microsc (Tokyo) },
volume = {48},
year = {1999},
pages = {277-287},
}

@article{IMOD:1996,
author = {Kremer, J. R. and  Mastronarde, D. N. and  McIntosh, J. R.},
title = {Computer visualization of three-dimensional image data using {IMOD}},
journal ={J. Struct. Biol.},
volume = {116},
year = {1996},
pages = {71-76},
}



@article{PyTom:2012,
author = {Hrabe, T. and  Chen, Y. and  Pfeffer,  S. and  Cuellar, L.K. and  Mangold, A.V. and  Forster, F. },
title = {{PyTom}: a python-based toolbox for localization of macromolecules in cryo-electron tomograms and subtomogram analysis},
journal ={J. Struct. Biol.},
volume = {178},
year = {2012},
pages = {178-188},
}


@article{RAPTOR:2008,
author = {Amat, F. and  Moussavi,  F. and  Comolli, L. R. and  Elidan,  G. and  Downing, K. H. and  Horowitz, M. },
title = {Markov random field based automatic image alignment for electron tomography},
journal ={J. Struct. Biol.},
volume = {161},
year = {2008},
pages = {260-275},
}



@article{UCSFTomography:2007,
author = {Shawn Q. Zhenga and Bettina Keszthelyi and   Eric Branlunda and John M. Lyleb and  Michael B. Braunfelda and John W. Sedatb and   David A. Agarda },
title = {{UCSF tomography}: an integrated software suite for real-time electron microscopic tomographic data collection, alignment, and reconstruction},
journal ={J. Struct. Biol.},
volume = {157},
year = {2007},
pages = {138-147},
}


@article{UCSFChimera:2004,
author = {Pettersen, E. F. and  Goddard, T. D. and  Huang, C. C. and  Couch,  G. S. and  Greenblatt,  D. M. and  Meng, E. C. and  Ferrin,  T. E.},
title = {{UCSF Chimera}--a visualization system for exploratory research and analysis},
journal ={ J. Comput. Chem. },
volume = {25},
year = {2004},
pages = {1605-1612},
}



@article{Biswas:2012,
author = {Biswas, A. and  Si, D. and  Al Nasr, K. and  Ranjan, D. and  Zubair, M. and  He, J.},
title = {Improved Effeciency in {Cryo-EM} Secondary Structure Topology Determination from Inaccurate Data},
journal ={ Journal of Bioinformatics and Computational Biology },
volume = {10},
year = {2012},
pages = {1242006},
}

@article{Abeysinghe:2008,
author = {Abeysinghe, S. S.  and  Baker, M. and  Chiu, W. and Tao, J.},
title = {Segmentation-free skeletonization of grayscale volumes for shape
understanding},
journal ={ IEEE International Conference on Shape Modeling and Applications },
volume = {SMI Stony Brook, N.Y.},
year = {2012},
pages = {63-71},
}



@article{TJu:2007,
author = {Ju, T. and  Baker, M. L. and  Chiu, W.},
title = { Computing a family of skeletons of volumetric models for shape description},
journal ={ Computer-Aided Design },
volume = {39},
year = {2007},
pages = {352-360},
}


@article{MBaker:2006,
author = {Baker, M. L. and  Jiang, W. and  Wedemeyer,  W. J. and  Rixon,  F. J. and  Baker, D. and  Chiu, W.},
title = { Ab initio modeling of the herpesvirus VP26 core domain assessed by CryoEM density},
journal ={  PLoS Computational Biology  },
volume = {2},
year = {2006},
pages = { e146},
}


@article{Rohl:2004,
author = { Rohl, C. A. and  Strauss, C. E. and  Misura, K. M. and  Baker, D.},
title = { Protein structure prediction using {Rosetta}},
journal ={  Methods Enzymol  },
volume = {383},
year = {2004},
pages = {66-93},
}


@article{CWei:2013,
author = { Wei, Chenyu and  Pohorille, Andrew},
title = {Activation and Proton Transport Mechanism in Influenza A M2 Channel},
journal ={ Biophysical Journal },
volume = {105},
year = {2013},
pages = {2036-2045},
}


@article{Tran:2013,
author = {  Nhut Tran and  Linh Tran and Ly Le},
title = {Strategy in structure-based drug design for influenza A virus targeting {M2} channel proteins
},
journal ={ Medical Chemistry Research},
volume = {22},
year = {2013},
pages = {6078-6088},
}



@article{Opella:1999,
author = { Opella, S. J. and  Marassi, F. M. and Gesell, J. J. and   Valente, A. P. and  Kim, Y.  and  Oblatt-Montal, M. and  Montal, M. },
title = {Structures of the {M2} channel-lining segments from nicotinic acetylcholine and {NMDA receptors by NMR} spectroscopy
},
journal ={ Nature Structural Biology},
volume = {6},
year = {1999},
pages = {374-379},
}

@article{Smondyrev:2002,
author = { Smondyrev, A. M. and  Voth, G. A.},
title = {Molecular dynamics simulation of proton transport through the influenza A virus M2 channel

},
journal ={Biophysical Jopurnal },
volume = {83},
year = {2002},
pages = {1987-1996},
}

@ARTICLE{HTZB09,
  author = {Jin Huang and Yiying Tong and Kun Zhou and Hujun Bao and Mathieu
	Desbrun},
  title = {Interactive Shape Interpolation through Controllable Dynamic Deformation},
  journal = {IEEE Trans. on Visualization and Computer Graphics},
  year = {July 2011},
  volume = {17},
  pages = {983-992},
  number = {7},
}

@ARTICLE{HTWB11,
  author = {Jin Huang and Yiying Tong and Hongyu Wei and Hujun Bao},
  title = {Boundary Aligned Smooth 3D Cross-Frame Field},
  journal = {ACM Trans. on Graphics (SIGGRAPH Asia)},
  year = {Dec 2011},
  volume = {30},
  pages = {1--8},
  number = {6}
}

@article{Zhang2012,
author = {Yizhong Zhang and Huamin Wang and Shuai Wang and Yiying Tong and Kun Zhou},
title = {A Deformable Surface Model for Real-Time Water Drop Animation},
journal ={IEEE Transactions on Visualization and Computer Graphics},
volume = {18},
number = {8},
issn = {1077-2626},
year = {2012},
pages = {1281-1289},
doi = {http://doi.ieeecomputersociety.org/10.1109/TVCG.2011.141},
publisher = {IEEE Computer Society},
address = {Los Alamitos, CA, USA},
}

@article{Pan2012,
  author    = {Zherong Pan and
               Jin Huang and
               Yiying Tong and
               Hujun Bao},
  title     = {Wake Synthesis For Shallow Water Equation},
  journal   = {Comput. Graph. Forum (Pacific Graphics)},
  volume    = {31},
  number    = {7-1},
  year      = {2012},
  pages     = {2029-2036},
  ee        = {http://dx.doi.org/10.1111/j.1467-8659.2012.03195.x},
  bibsource = {DBLP, http://dblp.uni-trier.de}
}

@article{Wang2012,
journal = {Computer Graphics Forum},
title = {{Linear Surface Reconstruction from Discrete Fundamental Forms on Triangle Meshes}},
author = {Yuanzhen Wang and Beibei Liu and Yiying Tong },
pages = {2277-2287},
volume= {31},
number= {8},
year = {2012},
URL = {http://diglib.eg.org/EG/CGF/volume31/issue8/v31i8pp2277-2287.pdf},
DOI = {10.1111/j.1467-8659.2012.03153.x},
}

@article{Feng:2012a,
title = "Compact combinatorial maps: A volume mesh data structure",
journal = "Graphical Models",
volume = "28",
number = "12",
pages = "1198--1223",
year = "2013",
note = "",
issn = "1524-0703",
doi = "10.1016/j.gmod.2012.10.001",
url = "http://www.sciencedirect.com/science/article/pii/S1524070312000690",
author = "Xin Feng and Yuanzhen Wang and Yanlin Weng and Yiying Tong",
keywords = "3D mesh",
keywords = "Combinatorial maps",
keywords = "Cell complex",
keywords = "Half-face",
keywords = "Compact mesh data structure"
}

@inproceedings{FengWWT12,
  author    = {Xin Feng and
               Yuanzhen Wang and
               Yanlin Weng and
               Yiying Tong},
  title     = {Compact Combinatorial Maps in 3D},
  booktitle = {Computational Visual Media - First International Conference},
  year      = {2012},
  pages     = {194-201},
  ee        = {http://dx.doi.org/10.1007/978-3-642-34263-9_25},
  bibsource = {DBLP, http://dblp.uni-trier.de}
}

@article{Liu2013,
year={Sept 2013},
issn={1000-9000},
journal={Journal of Computer Science and Technology (CVM)},
volume={28},
number={5},
title={Orientation Field Guided Texture Synthesis},
publisher={Springer US},
author={Liu, Beibei and Weng, Yanlin and Wang, Jiannan and Tong, Yiying},
pages={827--835},
}

@ARTICLE{Pan2013,
  author = {Zherong Pan and Jin Huang and Yiying Tong and Changxi Zheng and Hujun Bao},
  title = {Interactive Localized Liquid Motion Editing},
  journal = {ACM Trans. on Graphics (SIGGRAPH Asia)},
  year = {Nov 2013},
  volume = {32},
  number = {6},
  pages = {184:1--184:10}
}

@article{Jiang2014,
author = {Tengfei Jiang and Jin Huang and Yuanzhen Wang and Yiying Tong and Hujun Bao},
title = {Frame Field Singularity Correction for Automatic Hexahedralization},
journal ={IEEE Transactions on Visualization and Computer Graphics},
volume = {20},
number = {8},
issn = {1077-2626},
year = {2014},
pages = {1189--1199},
doi = {http://doi.ieeecomputersociety.org/10.1109/TVCG.2013.250},
publisher = {IEEE Computer Society},
address = {Los Alamitos, CA, USA},
}

@article{huang2014ell,
  title={\&ell; 1-Based Construction of Polycube Maps from Complex Shapes},
  author={Huang, Jin and Jiang, Tengfei and Shi, Zeyun and Tong, Yiying and Bao, Hujun and Desbrun, Mathieu},
  journal={ACM Transactions on Graphics (TOG)},
  volume={33},
  number={3},
  pages={25},
  year={2014},
  publisher={ACM}
}



@INPROCEEDINGS{Krishnamoorthy:2007,
  author = {Bala Krishnamoorthy and  Scott Provan and  Alexander Tropsha},
  title = {A Topological Characterization of Protein Structure},
  booktitle = {Data Mining in Biomedicine, Springer Optimization and Its Applications},
  year = {2007},
  pages = {431-455}
}



@article{WSun:2009,
  author = { Sun, W.  and He, Jing},
  title = { Native Secondary Structure Topology has Near Minimum Contact Energy among All Possible Geometrically Constrained Topolgies},
  journal={Proteins: Structure, Function and Bioinformatics},
  volume={77},
  number={},
  pages={159-173},
  year={2009},
}




@article{YLu:2008,
  author = { Lu, Y. and  He, J.},
  title = {Deriving Topology and Sequence Alignment for Helix Skeleton in Low Resolution Protein Density Maps  },
  journal={Journal of Bionformatics and Computational Biology},
  volume={8},
  number={},
  pages={183-201},
  year={2008},
}



@article{Agarwal:2007,
  author = {Agarwal, P. K. and  Mustafa, N. H. and Wang, Y. S.},
  title = { Fast molecular shape matching using contact maps  },
  journal={ Journal of Computational Biology},
  volume={14},
  number={},
  pages={131-143},
  year={2007},
}





@article{Guibas:2007,
  author = { Guibas, L. J. and Wang, Y. S.},
  title = {Toward unsupervised segmentation of semi-rigid low-resolution molecular surfaces  },
  journal={Algorithica},
  volume={48},
  number={},
  pages={433-448},
  year={2007},
}

@article{Varadaraj:2012,
  author = {Ramesh Varadaraj and Cornelius Brons},
  title = {Molecular Origins of Crude Oil Interfacial Activity. Part 4: Oil-Water
Interface Elasticity and Crude Oil Asphaltene Films },
  journal={Energy \& Fuels},
  volume={26},
  number={},
  pages={7164-7169},
  year={2012},
}


@article{Petkov:2000,
  author = {Jordan T. Petkov and Theodor D. Gurkov and Bruce E. Campbell and Rajendra P. Borwankar},
  title = {Dilatational and Shear Elasticity of Gel-like Protein
Layers on Air/Water Interface },
  journal={Langmuir},
  volume={16},
  number={},
  pages={3703-3711},
  year={2000},
}


@article{Stirnemann:2012,
  author = {Guillaume Stirnemann and  David Giganti and  Julio M. Fernandez and  and B. J. Berne},
  title = {Elasticity, structure, and relaxation of extended proteins under force},
  journal={PNAS},
  volume={110},
  number={},
  pages={3847-3852},
  year={2012},
}


@article{Korenchenko:2008,
  author = {A. E. Korenchenko and V. P. Beskachko},
  title = {Determining the shear modulus of water in experiments with a floating disk },
  journal={Journal of Applied Mechanics and Technical Physics},
  volume={49},
  number={},
  pages={80-83},
  year={2008},
}

@article{Roos:2010,
  author = { Wouter H Roos and  Melissa M Gibbons and Anton Arkhipov and  Charlotte Uetrecht and  NR Watts and  PT Wingfield and  Alasdair C Steven and  Albert JR Heck and  Klaus Schulten and  William S Klug and Gijs JL Wuite},
  title = {Squeezing Protein Shells: How Continuum Elastic Models, Molecular Dynamics Simulations, and Experiments Coalesce at the Nanoscale },
  journal={ Biophysical Journal },
  volume={99},
  number={},
  pages={1175- 1181},
  year={2010},
}

@article{WeiJCP:1999,
  author = { Wei, G. W.},
  title = {Discrete singular convolution for the solution of the
        {Fokker-Planck} equations },
  journal={ J. Chem. Phys.},
  volume={110},
  number={},
  pages={8930-8942},
  year={1999},
}

@article{WeiJPA:2000,
  author = { Wei, G. W.},
  title = {A unified approach for the solution of the
        Fokker-Planck equations},
  journal={ J.  Phys. A, Mathematics and General},
  volume={33},
  number={},
  pages={4935-4953},
  year={2000},
}


@article{WeiCMAME:2001,
  author = { Wei, G. W.},
  title = {A new algorithm for solving some mechanical problems},
  journal={ Comput. Methods Appl. Mech. Engng.},
  volume={190},
  number={},
  pages={2017-2030},
  year={2001},
}

@article{WeiJSV:2001,
  author = { Wei, G. W.},
  title = {Vibration analysis by discrete singular convolution},
  journal={ J. Sound  Vibr.},
  volume={244},
  number={},
  pages={535-553 },
  year={2001},
}



@article{WeiES:2001,
  author = { Wei, G. W.},
  title = {Discrete  singular  convolution  for  beam  analysis},
  journal={ Engineering    Structures  },
  volume={23},
  number={},
  pages={1045-1053 },
  year={2001},
}


@article{WeiIJME:2001,
  author = { Wei, G. W. and Zhao, Y. B. and Xiang, Y. },
  title = {The  determination  of  the  natural  frequencies  of  rectangular  plates  with  mixed  boundary  conditions  by  discrete  singular    convolution},
  journal={ Int.  J.  Mech.  Sci.  },
  volume={43},
  number={},
  pages={1731-1746 },
  year={2001},
}

@article{WeiIJNME:2002,
  author = { Wei, G. W. and Zhao, Y. B. and Xiang, Y. },
  title = { Discrete  singular  convolution  and  its    application  to  the  analysis  of  plates  with  internal  supports,   { I  Theory } and  algorithm},
  journal={  Int.  J.    Numer.  Methods  Engng. },
  volume={55},
  number={},
  pages={ 913-946 },
  year={2002},
}
 	
@article{voth_memb,
	Author = {G. S. Ayton and S. Izvekov and W. G. Noid and G. A. Voth},
	Date-Added = {2009-04-26 01:14:22 -0500},
	Date-Modified = {2009-04-26 01:15:45 -0500},
	Journal = {Curr. Top. Membranes},
	Pages = {181-225},
	Title = {Multiscale simulation of membranes and membrane proteins: Connecting molecular interactions to mesoscopic behavior},
	Volume = {60},
	Year = {2008}}
	
	@article{bar_voth10rev,
	Author = {G. S. Ayton and G. A. Voth},
	Date-Added = {2011-07-11 11:28:11 -0500},
	Date-Modified = {2011-07-11 11:28:37 -0500},
	Journal = {Seminars in Cell \& Dev. Biol.},
	Pages = {357-362},
	Title = {Multiscale simulation of protein mediated membrane remodeling},
	Volume = {21},
	Year = {2010}}
	
	@article{deserno_rev09,
	Author = {M. Deserno},
	Date-Added = {2011-07-12 13:02:39 -0500},
	Date-Modified = {2011-07-12 13:03:33 -0500},
	Journal = {Macromol. Rapid Comm.},
	Pages = {752-771},
	Title = {Mesoscopic Membrane Physics: Concepts, Simulations, and Selected Applications},
	Volume = {30},
	Year = {2009}}
	
	@article{voth_cg_rev,
	Author = {G. S. Ayton and W. G. Noid and G. A. Voth},
	Date-Added = {2011-07-11 14:34:40 -0500},
	Date-Modified = {2011-07-11 14:34:40 -0500},
	Journal = {Curr. Opin. Struct. Biol.},
	Pages = {192-198},
	Title = {Multiscale modeling of biomolecular systems: in serial and in parallel},
	Volume = {17},
	Year = {2007}}
	
	
 @article{gbsw_mem,
	Author = {W. Im and M. Feig and C. L. Brooks},
	Date-Added = {2007-06-26 10:08:33 -0500},
	Date-Modified = {2007-06-26 10:08:33 -0500},
	Journal = {Biophys. J.},
	Pages = {2900-2918},
	Title = {An implicit membrane generalized born theory for the study of structure, stability, and interactions of membrane proteins},
	Volume = {85},
	Year = {2003}}

 @article{brown_rev08,
	Author = {F. L. H. Brown},
	Date-Added = {2011-09-06 22:21:47 +0000},
	Date-Modified = {2011-09-06 22:22:15 +0000},
	Journal = {Annu. Rev. Phys. Chem.},
	Pages = {685-712},
	Title = {Elastic Modeling of Biomembranes and Lipid Bilayers},
	Volume = {59},
	Year = {2008}}
	
	@article{marrink_rev09,
	Author = {S. J. Marrink and A. H. {de Vries} and D. P. Tieleman},
	Date-Added = {2011-07-11 14:28:56 -0500},
	Date-Modified = {2011-07-11 14:28:56 -0500},
	Journal = {Biochim. Biophys. Acta - Biomem.},
	Pages = {149-168},
	Title = {Lipids on the move: Simulations of membrane pores, domains, stalks and curves},
	Volume = {1788},
	Year = {2009}}
	
	@unpublished{BMW_ff,
	Author = {Z. Wu and Q. Cui and A. Yethiraj},
	Date-Added = {2011-07-11 13:42:18 -0500},
	Date-Modified = {2011-07-11 13:42:18 -0500},
	Note = {``A new coarse-grained force field for membrane-peptide simulations'', {\it J. Chem. Theo. Comp.} submitted},
	Title = {A new coarse-grained force field for membrane-peptide simulations}}

@article{klein_cg,
	Author = {W. Shinoda and R. DeVane and M. L. Klein},
	Date-Added = {2011-07-11 14:35:23 -0500},
	Date-Modified = {2011-07-11 14:35:23 -0500},
	Journal = {J. Phys. Chem. B},
	Pages = {6836-6849},
	Title = {Zwitterionic lipid assemblies: molecular dynamics sutdies of monolayers, bilayers and vesicles using a new coarse grain force field},
	Volume = {114},
	Year = {2010}}
	
	@article{grabe_mem,
	Author = {S. Choe and K. A. Hecht and M. Grabe},
	Date-Added = {2011-09-06 22:20:31 +0000},
	Date-Modified = {2011-09-06 22:21:04 +0000},
	Journal = {J. Gen. Physiol.},
	Pages = {563-573},
	Title = {A Continuum Method for Determining Membrane Protein Insertion Energies and the Problem of Charged Residues},
	Volume = {131},
	Year = {2008}}

@article{imm1_pore,
	Author = {M. Mihajlovic and T. Lazaridis},
	Date-Added = {2011-09-06 22:29:17 +0000},
	Date-Modified = {2011-09-06 22:30:19 +0000},
	Journal = {Biochim. Biophys. Acta - Biomem.},
	Pages = {1494-1502},
	Title = {Antimicrobial peptides bind more strongly to membrane pores},
	Volume = {1798},
	Year = {2010}}

@article{imm1_test,
	Author = {E. Hajjar and M. Milhajlovic and V. Witko-Sarsat and T. Lazaridis and N. Reuter},
	Date-Added = {2011-09-06 22:28:21 +0000},
	Date-Modified = {2011-09-06 22:29:16 +0000},
	Journal = {Proteins},
	Pages = {1655-1669},
	Title = {Computational prediction of the binding site of proteinase 3 to the plasma membrane},
	Volume = {71},
	Year = {2008}}

@article{imm1_anion,
	Author = {T. Lazaridis},
	Date-Added = {2011-09-06 22:27:43 +0000},
	Date-Modified = {2011-09-06 22:28:18 +0000},
	Journal = {Proteins},
	Pages = {518-527},
	Title = {Implicit solvent simulations of peptide interactions with anionic lipid membranes},
	Volume = {58},
	Year = {2005}}

@article{imm1,
	Author = {T. Lazaridis},
	Date-Added = {2011-09-06 22:26:04 +0000},
	Date-Modified = {2011-09-06 22:27:39 +0000},
	Journal = {Proteins},
	Pages = {176-192},
	Title = {Effective energy function for proteins in lipid membranes},
	Volume = {52},
	Year = {2003}}
	
	@article{imm1_shuo,
	Author = {M. Rajendram and S. Yang, S. and Q. Cui and D. B. Weibel},
	Date-Added = {2011-09-07 05:30:59 +0000},
	Date-Modified = {2011-09-07 05:35:02 +0000},
	Journal = {ms in preparation},
	Title = {RecA binds to cardiolipin enriched lipid membranes},
	Year = {2011}}
	@article{imm1_nadia,
	Author = {N. K. Sundlass and C. H. Eller and S. Yang and Q. Cui and R. T. Raines},
	Date-Added = {2011-09-07 05:33:35 +0000},
	Date-Modified = {2011-09-07 05:34:55 +0000},
	Journal = {ms in preparation},
	Title = {The Contribution of Electrostatics to the Binding of Pancreatic Ribonucleases to Membranes},
	Year = {2011}}
	
@article{Andersen:AnnuRevBiophysBiomolStruct:2007,
	Abstract = { },
	Author = {{A}ndersen, {O}. {S}. and {K}oeppe {I}i, {R}. {E}.},
	Date-Added = {2009-04-25 00:21:10 -0500},
	Date-Modified = {2009-04-25 00:21:10 -0500},
	Doi = {10.1146/annurev.biophys.36.040306.132643},
	Issn = {1056-8700},
	Journal = {{A}nnu {R}ev {B}iophys {B}iomol {S}truct},
	Pages = {107-30},
	Pmid = {17263662},
	Publicationstatus = {{P}ublished},
	Title = {{B}ilayer {T}hickness and {M}embrane {P}rotein {F}unction: {A}n {E}nergetic {P}erspective.},
	Us_Nlm_Id = {9211097},
	Uuid = {5401FA38-6DBE-4DAE-8AB3-C4D78A42B41A},
	Volume = {36},
	Year = {2007}
	}

@article{JLi:2014,
	Author = {Li, J and  Lu, K. N. and Bates, P. W.  },
	Journal = {Discrete and Continuous Dynamical Systems},
	Pages = {3639-3666},
	Title = {Invariant foliations for random dynamical systems },
	Volume = {34},
	Year = {2014}}
	
@article{Bates:2014,
	Author = { Bates, P. W. and Jin, J. Y.  },
	Journal = {Discrete and Continuous Dynamical Systems},
	Pages = {1-17},
	Title = {Global dynamics of boundary droplets },
	Volume = {34},
	Year = {2014}}

	
@article{Bates:2013a,
	Author = { Bates, P. W. and Lu, K. L. and Wang, B. X.  },
	Journal = {Journal of Mathematical Physics},
	Pages = {081505},
	Title = {Tempered random attractors for parabolic equations in weighted spaces},
	Volume = {54},
	Year = {2013}}
	
	
@article{Bates:2013b,
	Author = { Bates, P. W. and Liang, Y. and Shingleton, A. W.  },
	Journal = {Networks and Heterogeneous Media},
	Pages = {56-78},
	Title = {Growth regulation and the insulin signaling pathway},
	Volume = {8},
	Year = {2013}}
	
@article{Bates:2011,
	Author = { Bates, P. W. and Che, F. G. },
	Journal = {Nonlinear Analysis-Theory Methods and Applications},
	Pages = {7285-7295},
	Title = {Structure of principal eigenvectors and genetic diversity},
	Volume = {74},
	Year = {2011}}
	
	
@article{patti_gsbp,
	Author = {Schaefer, P. and Riccardi, D. and Cui, Q.},
	Date-Modified = {2006-01-09 23:14:40 -0600},
	Journal = {J. Chem. Phys.},
	Pages = {014905},
	Title = {{Reliable treatment of electrostatics in combined QM/MM simulation of macromolecules}},
	Volume = {123},
	Year = {2005}}
	
@article{demian_pka,
	Author = {D. Riccardi and P. Schaefer and Q. Cui},
	Date-Modified = {2006-01-09 23:13:02 -0600},
	Journal = {J. Phys. Chem. B},
	Pages = {17715-17733},
	Title = {{pK$_{a}$ calculations in solution and proteins with QM/MM free energy perturbation simulations}},
	Volume = {109},
	Year = {2005}}
	
	@article{riccardi_capka,
	Author = {D. Riccardi and Q. Cui},
	Date-Added = {2011-09-01 03:51:54 +0000},
	Date-Modified = {2011-09-01 03:51:54 +0000},
	Journal = {J. Phys. Chem. A},
	Pages = {5703-5711},
	Title = {p{K}$_{a}$ analysis for the zinc-bound water in {Human Carbonic Anhydrase II}: benchmark for ``multi-scale" {QM/MM} simulations and mechanistic implications},
	Volume = {111},
	Year = {2007}}
	
	
	@ARTICLE{Wei:1999a,
  author = {Wei, G. W.},
  title = {Generalized {Perona-Malik} equation for image restoration},
  journal = {IEEE Signal Processing Letters},
  year = {1999},
  volume = {6},
  pages = {165-7},
  number = {7},
  abstract = {This article introduces generalizations of the Perona-Malik (1990)
	equation. An edge enhancing functional is proposed for direct edge
	enhancement. A number of super diffusion operators is introduced
	for fast and effective smoothing. Statistical information is utilized
	for robust edge-stopping. Numerical integration is conducted by using
	a previously developed quasi-interpolating wavelet method. Computer
	experiments indicate that the present algorithm is very efficient
	for edge-detecting and noise-removing},
  bdsk-url-1 = {http://ieeexplore.ieee.org/xpls/abs_all.jsp?arnumber=769359},
  bdsk-url-2 = {http://dx.doi.org/10.1109/97.769359},
  date-added = {2008-09-16 15:06:30 -0500},
  date-modified = {2008-09-16 15:06:30 -0500},
  doi = {10.1109/97.769359},
  keywords = {Mathematics; Visualization},
  url = {http://ieeexplore.ieee.org/xpls/abs_all.jsp?arnumber=769359}
}


%%%%%%%%%% added by KELIN
%%microtubule related


@article{Alushin:2014,
  title={High-Resolution Microtubule Structures Reveal the Structural Transitions in $\alpha$$\beta$-Tubulin upon {GTP} Hydrolysis},
  author={Alushin, G. M. and Lander, G. C. and Kellogg, E. H. and Zhang, R. and Baker, D. and Nogales, E.},
  journal={Cell},
  volume={157},
  number={5},
  pages={1117--1129},
  year={2014},
  publisher={Elsevier}
}

@article{Nogales:2006,
  title={Structural intermediates in microtubule assembly and disassembly: how and why?},
  author={Nogales, E. and Wang, H. W.},
  journal={Current opinion in cell biology},
  volume={18},
  number={2},
  pages={179--184},
  year={2006},
  publisher={Elsevier}
}


@article{Topf:2008,
  title={Protein structure fitting and refinement guided by {Cryo-EM} density},
  author={Topf,  M. and Lasker, K. and Webb, B. and Wolfson, H. and Chiu, W. and Sali, A.},
  journal={Structure},
  volume={16},
  number={2},
  pages={295--307},
  year={2008},
  publisher={Elsevier}
}

@article{Pettersen:2004,
  title={{UCSF Chimera}--{A} visualization system for exploratory research and analysis},
  author={Pettersen,  E. F. and Goddard, T.  D. and Huang, C. C. and Couch, G. S. and Greenblatt, D. M. and Meng, E. C. and Ferrin, T. E.},
  journal={Journal of computational chemistry},
  volume={25},
  number={13},
  pages={1605--1612},
  year={2004},
  publisher={Wiley Online Library}
}

%%%%%%%%%% Persistent & denoising

@article{Bauer:2010,
  title={Total variation meets topological persistence: A first encounter},
  author={Bauer, U. and Sch{\"{o}}nlieb, C. B. and Wardetzky, M.},
  journal={AIP Conference Proceedings},
  volume={1281},
  number={1},
  pages={1022},
  year={2010}
}


@article{Gunther:2014,
  title={Fast and Memory-Efficient Topological Denoising of {2D and 3D} Scalar Fields},
  author={G{\"u}nther, D. and Jacobson, A. and Reininghaus, J. and Seidel, H. P. and Sorkine-Hornung, O. and Weinkauf, T.},
  journal={IEEE Transactions on Visualization and Computer Graphics},
  volume={20},
  pages={12},
  year={2014}
}

@incollection{Adler:2010,
  title={Persistent homology for random fields and complexes},
  author={Adler, R. J. and Bobrowski, O. and Borman, M. S. and Subag, E. and Weinberger, S.},
  booktitle={Borrowing Strength: Theory Powering Applications--A {Festschrift for Lawrence D. Brown}},
  volume={6},
  pages={124--143},
  year={2010},
  publisher={Institute of Mathematical Statistics}
}

@article{Kloke:2009,
  title={Topological de-noising: Strengthening the topological signal},
  author={Kloke, J. and Carlsson, G.},
  journal={arXiv preprint arXiv:0910.5947},
  year={2009}
}


@article{Fasy:2013,
  title={Statistical Inference For Persistent Homology: Confidence Sets For Persistence Diagrams},
  author={Fasy, B. T. and Lecci, F. and Rinaldo, A. and Wasserman, L. and Balakrishnan, S. and Singh, A.},
  journal={arXiv preprint arXiv:1303.7117},
  year={2013}
}

@inproceedings{DeSilva:2004,
  title={Topological estimation using witness complexes},
  author={De Silva, V. and Carlsson, G.},
  booktitle={Proceedings of the First Eurographics conference on Point-Based Graphics},
  pages={157--166},
  year={2004},
  organization={Eurographics Association}
}




@article{JKPark:2013a,
  title={ A molecular level  prototype for  mechanoelectrical  transducers in  mammalian   hair cells},
  author={Park, J. K. and Wei, G. W.},
  journal={Journal of Computational Neuroscience},
  volume={35},
  number={},
  pages={231-241},
  year={2014},
  publisher={ }
}

@article{XiChen:2008,
  title={ Gating mechanisms of mechanosensitive channels of large conductance, I: A continuum mechanics-based hierarchical framework},
  author={Chen, Xi and  Cui, Qiang and Tang, Yuye and Yoo, J. and Yethiraj, A.},
  journal={Biophysical Journal},
  volume={95},
  number={},
  pages={563-580},
  year={2008},
  publisher={ }
}

@article{YYTang:2008,
  title={Gating mechanisms of mechanosensitive channels of large conductance, II: Systematic study of conformational transitions
},
  author={ Tang, Yuye and Yoo, J. and Yethiraj, A. and  Cui, Qiang and  Chen, Xi },
  journal={Biophysical Journal},
  volume={95},
  number={},
  pages={581-596},
  year={2008},
  publisher={ }
}



@ARTICLE{BBWang:2013,
  author = {Wang, B. B. and  Feig, M. and Cukier, R. I. and  Burton, Z. F.},
  title = {{Computational simulation strategies for analysis of multisubunit RNA polymerases}},
  journal = {Chemical reviews},
  year = {2013},
	volume = {113},
  pages = {8546-8566}
}




@ARTICLE{Werner:2013,
  author = {Wang, B. B. and  Feig, M. and Cukier, R. I. and  Burton, Z. F.},
  title = {{Molecular mechanisms of transcription elongation in archaea}},
  journal = {Chemical reviews},
  year = {2013},
	volume = {113},
  pages = {8331-8349}
}



@ARTICLE{Burton:2014,
  author = {Burton, Z. F.},
  title = {{The Old and New Testaments of gene regulation: Evolution of multi-subunit RNA polymerases and co-evolution of eukaryote complexity with the RNAP II CTD}},
  journal = { Transcription },
  year = {2014},
	volume = {5},
  pages = {e28674}
}



@ARTICLE{Iyer:2003,
  author = {Iyer, L. M. and  Koonin, E. V. and  Aravind, L.},
  title = {{Evolutionary connection between the catalytic subunits of DNA-dependent RNA polymerases and eukaryotic RNA-dependent RNA polymerases and the origin of RNA polymerases}},
  journal = {BMC Structural Biology},
  year = {2003},
	volume = {3},
  pages = {1}
}




@ARTICLE{Lane:2010,
  author = {Lane, W. J. and  Darst, S. A.},
  title = {{Molecular evolution of multisubunit RNA polymerases: structural analysis}},
  journal = {Journal of molecular biology},
  year = {2010},
	volume = {395},
  pages = {686-704}
}



@ARTICLE{DWang:2006,
  author = {Wang, D. and  Bushnell,  D. A. and  Westover,  K. D. and  Kaplan,  C. D. and  Kornberg, R. D.},
  title = {{Structural basis of transcription: role of the trigger loop in substrate specificity and catalysis}},
  journal = {Cell},
  year = {2006},
	volume = {127},
  pages = {941-954}
}




@ARTICLE{Vassylyev:2007,
  author = {Vassylyev,  D. G. and  Vassylyeva,  M. N. and  Zhang, J. and  Palangat, M. and  Artsimovitch, I. and  Landick, R.},
  title = {{ Structural basis for substrate loading in bacterial RNA polymerase}},
  journal = {Nature},
  year = {2007},
	volume = {448},
  pages = {163-168}
}




@ARTICLE{Feig:2010,
  author = {Feig, M. and  Burton, Z. F.},
  title = {{ RNA polymerase II with open and closed trigger loops: active site dynamics and nucleic acid translocation}},
  journal = {Biophysical Journal},
  year = {2010},
	volume = {99},
  pages = {2577-2586}
}



@ARTICLE{Feig:2010b,
  author = {Feig, M. and  Burton, Z. F.},
  title = {{ RNA polymerase II flexibility during translocation from normal mode analysis}},
  journal = {Protein},
  year = {2010},
	volume = {78},
  pages = {434-446}
}




@ARTICLE{Medialkov:2013,
  author = {Nedialkov, Y. A. and  Opron, K. and  Assaf, F. and  Artsimovitch,  I. and  Kireeva, M. L. and  Kashlev, M. and Cukier, R. I.  and  Nudler, E and Burton, Z. F.},
  title = {{The RNA polymerase bridge helix YFI motif in catalysis, fidelity and translocation}},
  journal = {Biochimica et Biophysica Acta (BBA) - Gene Regulatory Mechanisms},
  year = {2013},
	volume = {1829},
  pages = {187-198}
}



@ARTICLE{Silva:2014,
  author = {Silva, D. A.  and Weiss, D. R. and  Avila, F. P. and    Da, L. T. and  Levitt, M. and    Wang, D.  and  Huang, X. H.},
  title = {{Millisecond dynamics of RNA polymerase II translocation at atomic resolution}},
  journal = {Proceedings of the National Academy of Sciences of the United States of America},
  year = {2014},
	volume = {111},
  pages = {7665-7670}
}



@ARTICLE{Kireeva:2013,
  author = {	Kireeva, M. L. and Kashlev, M. and  Burton Z. F.},
  title = {{RNA polymerase structure, function, regulation, dynamics, fidelity, and roles in gene expression}},
  journal = { Chemical Review},
  year = {2013},
	volume = {113},
  pages = {8325-8330}
}



@ARTICLE{Medialkov:2013b,
  author = {	Nedialkov, Y. A. and   Burton, Z. F.},
  title = {{Translocation and fidelity of Escherichia coli RNA polymerase}},
  journal = {Transcription},
  year = {2013},
	volume = {4},
  pages = {136-143}
}




@ARTICLE{Domecq:2010,
  author = {	Domecq, C and  Kireeva,  M. and  Archambault,  J. and  Kashlev,  M and  Coulombe, B.  and   Burton, Z. F.},
  title = {{Site-directed mutagenesis, purification and assay of Saccharomyces cerevisiae RNA polymerase II}},
  journal = {Protein Expression and Purification},
  year = {2010},
	volume = {69},
  pages = {83-90}
}


@ARTICLE{Medialkov:2012,
  author = {	Nedialkov, Y. A. and Nudler, E. and   Burton, Z. F.},
  title = {{RNA polymerase stalls in a post-translocated register and can hyper-translocate}},
  journal = {Transcription},
  year = {2012},
	volume = {3},
  pages = {260-269}
}



@ARTICLE{Kireeva:2009,
  author = {	Kireeva, M. L. and    Nedialkov, Y. A.  and  Gong, X. Q. and Zhang, C. F. and  Xiong, Y. L. and  Moon, W. and Burton, Z. F.  and Kashlev, M.   },
  title = {{RNA polymerase structure, function, regulation, dynamics, fidelity, and roles in gene expression}},
  journal = { Methods},
  year = {2009},
	volume = {48},
  pages = {333-345}
}




@ARTICLE{Batada:2004,
  author = {	Batada, N. N.  and  Westover, K. D. and  Bushnell, D. A.  and  Levitt, M  and  Kornberg, R. D.   },
  title = {{Diffusion of nucleoside triphosphates and role of the entry site to the RNA polymerase II active center}},
  journal = { Proceedings of the National Academy of Sciences of the United States of America},
  year = {2004},
	volume = {101},
  pages = {17361-17364}
}





@ARTICLE{LTDa:2013,
  author = {	Da, L. T. and  Avila, F. P. and Wang, D.  and X Huang, X.   },
  title = {{A two-state model for the dynamics of the pyrophosphate ion release in bacterial RNA polymerase}},
  journal = { PLoS Comput. Biol.},
  year = {2013},
	volume = {9},
  pages = {e1003020}
}



@ARTICLE{Johnson:2011,
  author = {Johnson, R. S. and  Strausbauch, M.  and  Carraway, J. K.    },
  title = {{Rapid pyrophosphate release from transcriptional elongation complexes appears to be coupled to a nucleotide-induced conformational change in E. coli core polymerase}},
  journal = {J. Mol. Biol.},
  year = {2011},
	volume = {412},
  pages = {849-861}
}




@ARTICLE{Kennedy:2011,
  author = {	Kennedy, S. R. and Erie,  D. A.   },
  title = {{Templated nucleoside triphosphate binding to a noncatalytic site on RNA polymerase regulates transcription}},
  journal = { Proceedings of the National Academy of Sciences of the United States of America},
  year = {2011},
	volume = {108},
  pages = {6079-6084}
}




@ARTICLE{HXZhou:2013,
  author = {	 Zhou, Huan Xiang and Cross, Timothy A.  },
  title = {{Modeling the membrane environment has implications for membrane protein structure and function: Influenza A M2 protein}},
  journal = {Protein Sciences },
  year = {2013},
	volume = {22},
  pages = {381-394}
}



@ARTICLE{Gilson:2007,
  author = {	 Gilson, M. K.  and Zhou, Huan Xiang  },
  title = {{  Calculation of protein-ligand binding affinities}},
  journal = { Annual Review of Biophysics and Biomolecular Structur},
  year = {2007},
	volume = {36},
  pages = {21-42}
}




@ARTICLE{MYLu:2005,
  author = {	 Lu, M. Y. and Ma, J. P.  },
  title = {{  The role of shape in determining molecular motions}},
  journal = { Biophysiccal Journal},
  year = {2005},
	volume = {89},
  pages = {2359-2401}
}




@ARTICLE{TWZang:2014,
  author = {	Zang, T. W. and  Yu, L. L. and Zhang, C    and Ma, J. P.  },
  title = {{ Parallel continuous simulated tempering and its applications in large-scale molecular simulations}},
  journal = {Journal of Chemical Physics},
  year = {2014},
	volume = {141},
  pages = {044113}
}



@ARTICLE{Cheatham:2000,
  author = {Cheatham, T. E. and  Kollman, P. A. },
  title = {{Molecular dynamics simulation of nucleic acids}},
  journal = {Annual Review of  Physical Chemistry},
  year = {2000},
	volume = {51},
  pages = {435-471}
}




@ARTICLE{Cheatham:2004,
  author = {Cheatham, T. E.   },
  title = {{Simulation and modeling of nucleic acid structure, dynamics and interactions}},
  journal = {Annual Review of  Physical Chemistry},
  year = {2004},
	volume = {14},
  pages = {360-367}
}

@ARTICLE{Harker:2010,
    author = {Shaun Harker and Konstantin Mischaikow and Marian Mrozek and Vidit N and Hubert Wagner and Mateusz Juda},
    title = {The Efficiency of a Homology Algorithm based on Discrete Morse Theory and Coreductions},
      journal = {Proceeding of the 3rd International Workshop on Computational Topology in Image
Context, Image A},
   year = {2010},
	volume = {},
  pages = {41-47}
}


@ARTICLE{Harker:2013,
  author = {Shaun Harker and  Konstantin Mischaikow and Marian Mrozek and  Vidit Nanda },
  title = {{Discrete Morse theoretic algorithms for computing homology of complexes
and maps}},
  journal = {Found. Comput. Math.},
  year = {2013},
	volume = {},
  pages = {doi:10.1007/s10208-013-9145-0}
}



@ARTICLE{Wagner:2012,
  author = {Wagner, C. and  Chen, C. and Vucini, E.},
  title = {{Efficient computation of persistent homology for cubical data}},
  journal = {Topological
Methods in Data Analysis and Visualization II},
  year = {2012},
	volume = {},
  pages = {Springer Heidelberg Dordrecht London New York}
}


@ARTICLE{Strombom:2007,
  author = {Strombom, D.},
  title = {{Persistent Homology in the cubical setting}},
  journal = {Master's Thesis, Lulea University of Technology},
  year = {2007},
	volume = {},
  pages = { }
}


@article{Qiao:2013,
  title={Structural architecture of the {CARMA1/Bcl10/MALT1} signalosome: nucleation-induced filamentous assembly},
  author={Qiao, Q. and Yang, C. H. and Zheng, C. and Font{\'a}n, L. and David, L. and Yu, X. and Bracken, C. and Rosen, M. and Melnick, A. and Egelman, E. H. and Wu, H.},
  journal={Molecular cell},
  volume={51},
  number={6},
  pages={766--779},
  year={2013},
  publisher={Elsevier}
}


@ARTICLE{BaoWang:2014,
  author = {Wang, Bao    and Wei, G. W. },
	 title = "{Objective-oriented Persistent Homology}",
  journal = {ArXiv e-prints},
archivePrefix = "arXiv",
   eprint = {1412.2368},
 primaryClass = "q-bio.BM",
 keywords = {Quantitative Biology - Biomolecules},
     year = 2014,
    month = dec,
   adsurl = {http://adsabs.harvard.edu/abs/2014arXiv1412.2368W},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{BaoWang:2016a,
  author = {Wang, B.  and Wei, G. W.  },
   title = {Object-oriented Persistent Homology},
  journal = { Journal of Computational Physics},
     year = {2016},
    volume={305},
  number={},
  pages={276-299},
}
	
	
%%%%%%%%%%%%%  multi-filtration
@article{Carlsson:2009theory,
  title={The theory of multidimensional persistence},
  author={Carlsson, G. and Zomorodian, A.},
  journal={Discrete Computational Geometry},
  volume={42},
  number={1},
  pages={71--93},
  year={2009},
  publisher={Springer}
}

@incollection{Carlsson:2009computing,
  title={Computing multidimensional persistence},
  author={Carlsson, G. and Singh, G. and Zomorodian, A.},
  booktitle={Algorithms and computation},
  pages={730--739},
  year={2009},
  publisher={Springer}
}

@inproceedings{Cohen:2006,
  title={Vines and vineyards by updating persistence in linear time},
  author={Cohen-Steiner, D. and Edelsbrunner, H. and Morozov, D.},
  booktitle={Proceedings of the twenty-second annual symposium on Computational geometry},
  pages={119--126},
  year={2006},
  organization={ACM}
}

@inproceedings{Cerri:2013,
  title={The persistence space in multidimensional persistent homology},
  author={Cerri, A. and Landi, C.},
  booktitle={Discrete Geometry for Computer Imagery},
  pages={180--191},
  year={2013},
  organization={Springer}
}


@article{Cerri:2013b,
  title={Betti numbers in multidimensional persistent homology are stable functions},
  author={Cerri, A. and Fabio, B. and Ferri, M. and Frosini, P. and Landi, C.},
  journal={Mathematical Methods in the Applied Sciences},
  volume={36},
  number={12},
  pages={1543--1557},
  year={2013},
  publisher={Wiley Online Library}
}

@article{verri1993use,
  title={On the use of size functions for shape analysis},
  author={Verri, A. and Uras, C. and Frosini, P. and Ferri, M.},
  journal={Biological cybernetics},
  volume={70},
  number={2},
  pages={99--107},
  year={1993},
  publisher={Springer}
}

@article{bergomi2019beyond,
  title={Beyond topological persistence: Starting from networks},
  author={Bergomi, M. G. and Ferri, M. and Vertechi, P. and Zuffi, L.},
  journal={arXiv preprint arXiv:1901.08051},
  year={2019}
}


@article{Alvarez-Garcia:2014,
author = {Alvarez-Garcia, Daniel and Barril, Xavier},
title = {Relationship between Protein Flexibility and Binding: Lessons for Structure-Based Drug Design},
journal = {Journal of Chemical Theory and Computation},
volume = {10},
number = {6},
pages = {2608-2614},
year = {2014},
doi = {10.1021/ct500182z},
 }


@article{Marsh:2014,
  title={Protein Flexibility Facilitates Quaternary Structure Assembly and Evolution},
  author={Marsh, J. A. and  Teichmann, S. A.},
  journal={PLoS Biol},
  volume={12},
  number={5},
  pages={e1001870},
  year={2014}
}


@article{ZBu:2011,
  title={Proteins MOVE! Protein dynamics and long-range allostery in cell signaling},
  author={Bu, Z. and  Callaway, D. J. },
  journal={Advances in Protein Chemistry and Structural Biology},
  volume={83},
  number={},
  pages={163-221},
  year={2011}
}

@article{Fraser:2009,
  title={Hidden alternative structures of proline isomerase essential for catalysis},
  author={Fraser, J. S.and  Clarkson, M. W. and  Degnan, S. C. and Erion, R. and  Kern, D. and Alber, T. },
  journal={Nature},
  volume={462},
  number={},
  pages={669-673},
  year={2009}
}



@article{Fischer:2014,
  title={Incorporation of protein flexibility and conformational energy penalties in docking screens to improve ligand discovery},
  author={Fischer, Marcus and  Coleman, Ryan G. and Fraser, James S. and Shoichet, Brian K. },
  journal={Nature Chemistry},
  volume={6},
  number={},
  pages={575-583},
  year={2014}
}


@article{Thorpe:2007,
  title={Comment on elastic network models and proteins},
  author={Thorpe, M. F. },
  journal={Physical Biology},
  volume={4},
  number={},
  pages={60-63},
  year={2007}
}

@article{Halle:2002,
  title={Flexibility and packing in proteins},
  author={Halle, B. },
  journal={ PNAS},
  volume={99},
  number={},
  pages={1274-1279},
  year={2002}
}


% Added for mFRI paper

@article{Shimomura1962,
  title={Extraction, purification and properties of aequorin, a bioluminescent protein from the luminous hydromedusan, Aequorea},
  author={Shimomura, Osamu and Johnson, Frank H and Saiga, Yo},
  journal={Journal of cellular and comparative physiology},
  volume={59},
  number={3},
  pages={223--239},
  year={1962},
  publisher={Wiley Online Library}
}

@article{Ai2006,
  title={Directed evolution of a monomeric, bright and photostable version of Clavularia cyan fluorescent protein: structural characterization and applications in fluorescence imaging},
  author={Ai, Hui-wang and Henderson, J and Remington, S and Campbell, R},
  journal={Biochem. J},
  volume={400},
  pages={531--540},
  year={2006}
}



@article{Matz1999,
  title={Fluorescent proteins from nonbioluminescent Anthozoa species},
  author={Matz, Mikhail V and Fradkov, Arkady F and Labas, Yulii A and Savitsky, Aleksandr P and Zaraisky, Andrey G and Markelov, Mikhail L and Lukyanov, Sergey A},
  journal={Nature biotechnology},
  volume={17},
  number={10},
  pages={969--973},
  year={1999},
  publisher={Nature Publishing Group}
}

@article{1V70,
  title={Crystal Structure of probable antibiotics synthesis protein from Thermus thermophilus HB8},
  author={Asada, Y and Kunishima, N},
  journal={To be Published},
  volume={PDB ID: 1V70},
  number={},
  pages={},
  year={},
  publisher={RIKEN Structural Genomics/Proteomics Initiative}
}

@article{Davies1996,
  title={The crystal structure of ribosomal protein L14 reveals an important organizational component of the translational apparatus},
  author={Davies, Christopher and White, Stephen W and Ramakrishnan, V},
  journal={Structure},
  volume={4},
  number={1},
  pages={55--66},
  year={1996},
  publisher={Elsevier}
}

@article{Kuhlbrandt:2014,
	author = {K{\"u}hlbrandt, Werner},
	title = {Cryo-EM enters a new era},
	volume = {3},
	year = {2014},
	doi = {10.7554/eLife.03678},
	publisher = {eLife Sciences Publications Limited},
	abstract = { },
	isbn = {2050-084X},
	journal = {eLife}
}



@article{Wriggers:1999,
	author = {Wriggers, W. and  Milligan, R. A. and  McCammon, J. A.
},
	title = {Situs: {A} package for docking crystal structures into low-resolution maps from electron microscopy},
	volume = {125},
	 pages={185--195},
	year = {1999},
	journal = {Journal of  Structure Biology}
}


@article{Warshel:1976,
	author = {Warshel, A. and  Levitt, M. },
	title = {Theoretical studies of enzymic reactions: Dielectric, electrostatic and steric stabilization of the carbonium ion in the reaction of lysozyme},
	volume = {103},
	 pages={227--249},
	year = {1976},
	journal = {Journal of Molecular Biology }
}


@article{Shimomura1962,
  title={Extraction, purification and properties of aequorin, a bioluminescent protein from the luminous hydromedusan, Aequorea},
  author={Shimomura, Osamu and Johnson, Frank H and Saiga, Yo},
  journal={Journal of cellular and comparative physiology},
  volume={59},
  number={3},
  pages={223--239},
  year={1962},
  publisher={Wiley Online Library}
}

@article{Ai2006,
  title={Directed evolution of a monomeric, bright and photostable version of Clavularia cyan fluorescent protein: structural characterization and applications in fluorescence imaging},
  author={Ai, Hui-wang and Henderson, J and Remington, S and Campbell, R},
  journal={Biochem. J},
  volume={400},
  pages={531--540},
  year={2006}
}



@article{Matz1999,
  title={Fluorescent proteins from nonbioluminescent Anthozoa species},
  author={Matz, Mikhail V and Fradkov, Arkady F and Labas, Yulii A and Savitsky, Aleksandr P and Zaraisky, Andrey G and Markelov, Mikhail L and Lukyanov, Sergey A},
  journal={Nature biotechnology},
  volume={17},
  number={10},
  pages={969--973},
  year={1999},
  publisher={Nature Publishing Group}
}

@article{1V70,
  title={Crystal Structure of probable antibiotics synthesis protein from Thermus thermophilus HB8},
  author={Asada, Y and Kunishima, N},
  journal={To be Published},
  volume={PDB ID: 1V70},
  number={},
  pages={},
  year={},
  publisher={RIKEN Structural Genomics/Proteomics Initiative}
}

@article{Davies1996,
  title={The crystal structure of ribosomal protein L14 reveals an important organizational component of the translational apparatus},
  author={Davies, Christopher and White, Stephen W and Ramakrishnan, V},
  journal={Structure},
  volume={4},
  number={1},
  pages={55--66},
  year={1996},
  publisher={Elsevier}
}


@article{Wang2006,
  title={Structural basis of transcription: role of the trigger loop in substrate specificity and catalysis},
  author={Wang, Dong and Bushnell, David A and Westover, Kenneth D and Kaplan, Craig D and Kornberg, Roger D},
  journal={Cell},
  volume={127},
  number={5},
  pages={941--954},
  year={2006},
  publisher={Elsevier}
}

@article{Feig2010rna,
  title={RNA polymerase II flexibility during translocation from normal mode analysis},
  author={Feig, Michael and Burton, Zachary F},
  journal={Proteins: Structure, Function, and Bioinformatics},
  volume={78},
  number={2},
  pages={434--446},
  year={2010},
  publisher={Wiley Online Library}
}

@article{Tama:2000,
  title={Building-block approach for determining low-frequency normal modes of macromolecules},
  author={Tama, F. and Gadea, F. X. and Marques, O. and Sanejouand, Y. H.},
  journal={Proteins: Structure, Function, and Bioinformatics},
  volume={41},
  number={1},
  pages={1--7},
  year={2000},
  publisher={Wiley Online Library}
}

@article{Iyer2003,
  title={Evolutionary connection between the catalytic subunits of DNA-dependent RNA polymerases and eukaryotic RNA-dependent RNA polymerases and the origin of RNA polymerases},
  author={Iyer, Lakshminarayan M and Koonin, Eugene V and Aravind, L},
  journal={BMC structural biology},
  volume={3},
  number={1},
  pages={1},
  year={2003},
  publisher={BioMed Central Ltd}
}

@article{Burton2014old,
  title={The Old and New Testaments of gene regulation: Evolution of multi-subunit RNA polymerases and co-evolution of eukaryote complexity with the RNAP II CTD},
  author={Burton, Zachary F},
  journal={Transcription},
  volume={5},
  number={3},
  year={2014},
  publisher={Taylor \& Francis}
	
	
}
@article{Feig2010rna2,
  title={RNA polymerase II with open and closed trigger loops: active site dynamics and nucleic acid translocation},
  author={Feig, Michael and Burton, Zachary F},
  journal={Biophysical journal},
  volume={99},
  number={8},
  pages={2577--2586},
  year={2010},
  publisher={Elsevier}
}

@article{van2004,
  title={Normal-mode analysis suggests protein flexibility modulation throughout RNA polymerase's functional cycle},
  author={Van Wynsberghe, Adam and Li, Guohui and Cui, Qiang},
  journal={Biochemistry},
  volume={43},
  number={41},
  pages={13083--13096},
  year={2004},
  publisher={ACS Publications}
}

@article{Opron:2015a,
  title={  Communication: Capturing protein multiscale thermal fluctuations},
  author={Opron, Kristopher and Xia, K. L. and  Wei, G. W. },
  journal={ Journal of Chemical Physics},
  volume={ 142},
  number={211101 },
  pages={ },
  year={ 2015}
}

@article{Opron:2015b,
  title={  Flexibility-rigidity index analysis of protein-nucleic acid complexes},
  author={Opron, Kristopher and Xia, K. L. and Burton, Z. and  Wei, G. W. },
  journal={ Nucleic Acids Research},
  volume={ },
  number={ },
  pages={ },
  year={submitted 2015}
}

@article{BBWang:2015,
  title={  Five checkpoints maintaining the fidelity of transcription by RNA polymerases in structural and energetic details},
  author={Wang, B. B. and Opron, K. and Burton, Z. F. and Cukier   R. I. and  Feig, M.},
  journal={ Nucleic acids research},
  volume={ 43},
  number={ },
  pages={ 1133-1146},
  year={2015}
}





@article{Nedialkov:2013,
  title={ The RNA polymerase bridge helix YFI motif in catalysis, fidelity and translocation},
  author={Nedialkov, Y. A. and Opron, K. and Assaf, F. and Artsimovitch, I. and Kireeva, M. L. and Kashlev, M. and Cukier, R.I. and Nudler, E. and and Burton, Z. F. },
  journal={BBA Gene Regulatory Mechanisms},
  volume={ 1829},
  number={ },
  pages={   187-198},
  year={2013}
}


@article{BBWang:2013b,
  title={ Energetic and Structural Details of the Trigger Loop Closing Transition in RNA Polymerase II},
  author={Wang, B. B. and Predeus, A. and  Burton, Z. F. and Feig, M. },
  journal={Biophysical J.},
  volume={ 105},
  number={ },
  pages={766-775},
  year={2013}
}



@article{Dipha,
  title={  Distributed computation of persistent homology  },
  author={Bauer, U. and Kerber, M. and Reininghaus, J. },
  journal={ Proceedings of the Sixteenth Workshop on Algorithm Engineering and Experiments (ALENEX)},
  volume={  },
  number={ },
  pages={ },
  year={2014}
}




@article{LXWang:2015,
  title={ A Mutation in the Intracellular Loop {III/IV } of Mosquito Sodium Channel Synergizes the Effect of Mutations in Helix {IIS6}  on Pyrethroid Resistance },
  author={Wang, L. X.  and  Nomura, Y. and    Du, Y. Z.   and  Liu, N. N.  and  Zhorov, B. S. and  Dong, K. },
  journal={Molecular Pharmacology },
  volume={87  },
  number={ },
  pages={421-429 },
  year={2015}
}

@article{Paramo:2014,
author = {Paramo, Teresa and East, Alexandra and Garzón, Diana and Ulmschneider, Martin B. and Bond, Peter J.},
title = {Efficient Characterization of Protein Cavities within Molecular Simulation Trajectories: trj\_cavity},
journal = {Journal of Chemical Theory and Computation},
volume = {10},
number = {5},
pages = {2151-2164},
year = {2014},
doi = {10.1021/ct401098b},
URL = {
        http://dx.doi.org/10.1021/ct401098b
},
eprint = {
        http://dx.doi.org/10.1021/ct401098b
}
}


%%%%%Kelin added
@article{CPLin:2008,
  title={Deriving protein dynamical properties from weighted protein contact number},
  author={Lin, C. P. and Huang, S. W. and Lai, Y. L. and Yen, S. C. and Shih, C. H.  and Lu, C. H. and Huang, C. C. and Hwang, J. K.},
  journal={Proteins: Structure, Function, and Bioinformatics},
  volume={72},
  number={3},
  pages={929--935},
  year={2008},
  publisher={Wiley Online Library}
}

@article{SWHuang:2008,
  title={Prediction of NMR order parameters in proteins using weighted protein contact-number model},
  author={Huang, S. W. and Shih, C. H. and Lin, C. P. and Hwang, J. K.},
  journal={Theoretical Chemistry Accounts},
  volume={121},
  number={3-4},
  pages={197--200},
  year={2008},
  publisher={Springer}
}

@article{DWLi:2009,
  title={All-atom contact model for understanding protein dynamics from crystallographic B-factors},
  author={Li, D. W. and Br{\"u}schweiler, R.},
  journal={Biophysical journal},
  volume={96},
  number={8},
  pages={3074--3081},
  year={2009},
  publisher={Elsevier}
}


@article{FLZhang:2002,
  title={Contact model for the prediction of NMR NH order parameters in globular proteins},
  author={Zhang, F. L. and Br{\"u}schweiler, R.},
  journal={Journal of the American Chemical Society},
  volume={124},
  number={43},
  pages={12654--12655},
  year={2002},
  publisher={ACS Publications}
}


@article{Mendoncca:2014,
  title={Inferring a weighted elastic network from partial unfolding with coarse-grained simulations},
  author={Mendon{\c{c}}a, M. R. and Rizzi, L. G. and Contessoto, V. and Leite, V. BP and Alves, N. A.},
  journal={Proteins: Structure, Function, and Bioinformatics},
  volume={82},
  number={1},
  pages={119--129},
  year={2014},
  publisher={Wiley Online Library}
}


@article{Lezon:2010,
  title={Using entropy maximization to understand the determinants of structural dynamics beyond native contact topology},
  author={Lezon, T. R. and Bahar, I.},
  journal={PLoS computational biology},
  volume={6},
  number={6},
  pages={1000816},
  year={2010},
  publisher={Public Library of Science}
}


@article{Krone:2012,
  title={Fast visualization of {Gaussian} density surfaces for molecular dynamics and particle system trajectories},
  author={Krone, M. and Stone, J. E. and Ertl, T. and Schulten, K.},
  journal={EuroVis-Short Papers},
  volume={2012},
  pages={67--71},
  year={2012}
}


@article{Zhang2010role,
  title={Role of the RNA polymerase trigger loop in catalysis and pausing},
  author={Zhang, Jinwei and Palangat, Murali and Landick, Robert},
  journal={Nature structural \& molecular biology},
  volume={17},
  number={1},
  pages={99--104},
  year={2010},
  publisher={Nature Publishing Group}
}

%%%%%%%%%%%%%%%%   added persistent entropy

@article{Chintakunta:2015,
  title={An entropy-based persistence barcode},
  author={Chintakunta, H. and Gentimis, T. and Gonzalez-Diaz, R. and Jimenez, M. J. and Krim, H.},
  journal={Pattern Recognition},
  volume={48},
  number={2},
  pages={391--401},
  year={2015},
  publisher={Elsevier}
}

@article{Merelli:2015topological,
  title={Topological characterization of complex systems: Using persistent entropy},
  author={Merelli, E. and Rucco, M. and Sloot, P. and Tesei, L.},
  journal={Entropy},
  volume={17},
  number={10},
  pages={6872--6892},
  year={2015},
  publisher={Multidisciplinary Digital Publishing Institute}
}

@incollection{Rucco:2016,
  title={Characterisation of the idiotypic immune network through persistent entropy},
  author={Rucco, M. and Castiglione, F. and Merelli, E. and Pettini, M.},
  booktitle={Proceedings of {ECCS} 2014},
  pages={117--128},
  year={2016},
  publisher={Springer}
}

@article{Rucco:2017new,
  title={A new topological entropy-based approach for measuring similarities among piecewise linear functions},
  author={Rucco, M. and Gonzalez-Diaz, R. and Jimenez, M. J. and Atienza, N. and Cristalli, C. and Concettoni, E. and Ferrante, A. and Merelli, E.},
  journal={Signal Processing},
  volume={134},
  pages={130--138},
  year={2017},
  publisher={Elsevier}
}


%%% conformational entropy


@INPROCEEDINGS{Korkut:2013,
  author = {Korkut, A. and Hendrickson, W. A.},
  title = {Stereochemistry of Polypeptide Conformation in {Coarse Grained} Analysis},
  booktitle = {Biomolecular Forms and Functions: A Celebration of 50 Years of the Ramachandran Map},
  year = {2013},
  pages = {136-147},
   publisher={World Scientific Publishing}
}


@article{Frederick:2007,
  title={Conformational entropy in molecular recognition by proteins},
  author={Frederick, K. K. and Marlow, M. S. and Valentine, K. G. and Wand, A. J.},
  journal={Nature},
  volume={448},
  number={7151},
  pages={325--329},
  year={2007},
  publisher={Nature Publishing Group}
}

@article{Marlow:2010role,
  title={The role of conformational entropy in molecular recognition by calmodulin},
  author={Marlow, M. S. and Dogan, J. and Frederick, K. K. and Valentine, K. G. and Wand, A. J.},
  journal={Nature chemical biology},
  volume={6},
  number={5},
  pages={352--358},
  year={2010},
  publisher={Nature Publishing Group}
}

@article{Zhang:2008RNA,
  title={Discrete state model and accurate estimation of loop entropy of RNA secondary structures},
  author={Zhang, J. and Lin, M. and Chen, R. and Wang, W. and Liang, J.},
  journal={The Journal of chemical physics},
  volume={128},
  number={12},
  pages={125107},
  year={2008}
}


@article{Stites:1995,
  title={Empirical evaluation of the influence of side chains on the conformational entropy of the polypeptide backbone},
  author={Stites, W. E. and Pranata, J.},
  journal={Proteins: Structure, Function, and Bioinformatics},
  volume={22},
  number={2},
  pages={132--140},
  year={1995},
  publisher={Wiley Online Library}
}


@article{Brady:1997entropy,
  title={Entropy in protein folding and in protein—protein interactions},
  author={Brady, G. P. and Sharp, K. A.},
  journal={Current opinion in structural biology},
  volume={7},
  number={2},
  pages={215--221},
  year={1997},
  publisher={Elsevier}
}

@article{Karplus:1981,
  title={Method for estimating the configurational entropy of macromolecules},
  author={Karplus, M. and Kushick, J. N.},
  journal={Macromolecules},
  volume={14},
  number={2},
  pages={325--332},
  year={1981},
  publisher={ACS Publications}
}

@article{Hagler:1979,
  title={Computer simulation of the conformational properties of oligopeptides. Comparison of theoretical methods and analysis of experimental results},
  author={Hagler, A. T. and Stern, P.S. and Sharon, R. and Becker, J. M. and Naider, F.},
  journal={Journal of the American Chemical Society},
  volume={101},
  number={23},
  pages={6842--6852},
  year={1979},
  publisher={ACS Publications}
}


@article{Levitt:1975computer,
  title={Computer simulation of protein folding},
  author={Levitt, M. and Warshel, A.},
  journal={Nature},
  volume={253},
  number={5494},
  pages={694--698},
  year={1975}
}

@article{Trbovic:2008,
  title={Protein side-chain dynamics and residual conformational entropy},
  author={Trbovic, N. and Cho, J.H. and Abel, R. and Friesner, R. A. and Rance, M. and Palmer III, A. G.},
  journal={Journal of the American Chemical Society},
  volume={131},
  number={2},
  pages={615--622},
  year={2008},
  publisher={ACS Publications}
}

@article{Sapienza:2010,
  title={Using {NMR} to study fast dynamics in proteins: methods and applications},
  author={Sapienza, P. J. and Lee, A. L.},
  journal={Current opinion in pharmacology},
  volume={10},
  number={6},
  pages={723--730},
  year={2010},
  publisher={Elsevier}
}


@article{Das:2013,
  title={Conformational contribution to thermodynamics of binding in protein-peptide complexes through microscopic simulation},
  author={Das, A. and Chakrabarti, J. and Ghosh, M.},
  journal={Biophysical journal},
  volume={104},
  number={6},
  pages={1274--1284},
  year={2013},
  publisher={Elsevier}
}


@article{Baron:2009,
  title={Absolute single-molecule entropies from quasi-harmonic analysis of microsecond molecular dynamics: correction terms and convergence properties},
  author={Baron, R. and Hünenberger, P. H and McCammon, J. A.},
  journal={Journal of chemical theory and computation},
  volume={5},
  number={12},
  pages={3150--3160},
  year={2009},
  publisher={ACS Publications}
}


@article{Thompson:2002,
  title={The backbone conformational entropy of protein folding: experimental measures from atomic force microscopy},
  author={Thompson, J. B. and Hansma, H. G. and Hansma, P. K. and Plaxco, K. W.},
  journal={Journal of Molecular biology},
  volume={322},
  number={3},
  pages={645--652},
  year={2002},
  publisher={Elsevier}
}

@article{Fitter:2003,
  title={A measure of conformational entropy change during thermal protein unfolding using neutron spectroscopy},
  author={Fitter, J.},
  journal={Biophysical journal},
  volume={84},
  number={6},
  pages={3924--3930},
  year={2003},
  publisher={Elsevier}
}

@article{Chang:2005,
  title={Evaluating the accuracy of the quasiharmonic approximation},
  author={Chang, C.E. and Chen, W. and Gilson, M. K.},
  journal={Journal of Chemical Theory and Computation},
  volume={1},
  number={5},
  pages={1017--1028},
  year={2005},
  publisher={ACS Publications}
}


@article{Brooks:1983harmonic,
  title={Harmonic dynamics of proteins: normal modes and fluctuations in bovine pancreatic trypsin inhibitor},
  author={Brooks, B. and Karplus, M.},
  journal={Proceedings of the National Academy of Sciences},
  volume={80},
  number={21},
  pages={6571--6575},
  year={1983},
  publisher={National Acad Sciences}
}


@article{Gromiha:2011,
  title={Scoring Function Based Approach for Locating Binding Sites and Understanding Recognition Mechanism of Protein- {DNA} Complexes},
  author={Gromiha, M. M. and Fukui, K.},
  journal={Journal of chemical information and modeling},
  volume={51},
  number={3},
  pages={721--729},
  year={2011},
  publisher={ACS Publications}
}


@article{Baruah:2015,
  title={Conformational entropy of intrinsically disordered proteins from amino acid triads},
  author={Baruah, A. and Rani, P. and Biswas, P.},
  journal={Scientific reports},
  volume={5},
  year={2015},
  publisher={Nature Publishing Group}
}


@article{Doig:1995side,
  title={Side-chain conformational entropy in protein folding},
  author={Doig, A. J. and Sternberg, M. J.E.},
  journal={Protein Science},
  volume={4},
  number={11},
  pages={2247--2251},
  year={1995},
  publisher={Wiley Online Library}
}

@article{Zhong:2006dihedral,
  title={Dihedral-angle information entropy as a gauge of secondary structure propensity},
  author={Zhong, S. and Moix, J. M. and Quirk, S. and Hernandez, R.},
  journal={Biophysical journal},
  volume={91},
  number={11},
  pages={4014--4023},
  year={2006},
  publisher={Elsevier}
}




@article{Bubenik:2015statistical,
  title={Statistical topological data analysis using persistence landscapes},
  author={Bubenik, P.},
  journal={Journal of Machine Learning Research},
  volume={16},
  number={1},
  pages={77--102},
  year={2015}
}


@article{Ghrist:2008barcodes,
  title={Barcodes: the persistent topology of data},
  author={Ghrist, R.},
  journal={Bulletin of the American Mathematical Society},
  volume={45},
  number={1},
  pages={61--75},
  year={2008}
}

@article{Gellman:1997,
  title={Introduction: molecular recognition},
  author={Gellman, S. H.},
  journal={Chemical reviews},
  volume={97},
  number={5},
  pages={1231--1232},
  year={1997},
  publisher={ACS Publications}
}

@article{Brooijmans:2003,
  title={Molecular recognition and docking algorithms},
  author={Brooijmans, N. and Kuntz, I. D.},
  journal={Annual review of biophysics and biomolecular structure},
  volume={32},
  number={1},
  pages={335--373},
  year={2003},
  publisher={Annual Reviews 4139 El Camino Way, PO Box 10139, Palo Alto, CA 94303-0139, USA}
}


@book{Munkres:1984,
  title={Elements of algebraic topology},
  author={Munkres, J. R.},
  volume={2},
  year={1984},
  publisher={Addison-Wesley Menlo Park}
}


@article{Chazal:2014persistence,
  title={Persistence stability for geometric complexes},
  author={Chazal, F. and De Silva, V. and Oudot, S.},
  journal={Geometriae Dedicata},
  volume={173},
  number={1},
  pages={193--214},
  year={2014},
  publisher={Springer}
}

@article{Carlsson:2014topological,
  title={Topological pattern recognition for point cloud data},
  author={Carlsson, G.},
  journal={Acta Numerica},
  volume={23},
  pages={289},
  year={2014},
  publisher={Cambridge University Press}
}

@article{Binchi:2014jholes,
  title={jHoles: A tool for understanding biological complex networks via clique weight rank persistent homology},
  author={Binchi, J. and Merelli, E. and Rucco, M. and Petri, G. and Vaccarino, F.},
  journal={Electronic Notes in Theoretical Computer Science},
  volume={306},
  pages={5--18},
  year={2014},
  publisher={Elsevier}
}



@article{SGZhou:2015,
  title={LS-VISM: A Software Package for Analysis of Biomolecular Solvation},
  author={Zhou, S. G. and  Cheng, L. T.  and  Sun, H.  and Che, J. W. and Dzubiella, J. and Li, B. and McCammon, J. A.
},
  journal={Journal of Computational Chemistry},
  volume={36},
  number={},
  pages={1047--1059},
  year={2015}
}



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%Added Bao Wang for binding energy paper
@ARTICLE{Harris:2013,
  author = {Harris, Robert C. and  Boschitsch, Aleander H. and Fenley, Marcia O.},
  title = {{Influence of Grid Spacing in Poisson-Boltzmann Equation Binding Energy Estimation}},
  journal = {Journal of Chemical Theory and Computation},
  year = {2013},
	volume = {9},
  pages = {3677-3685}
}


@ARTICLE{Harris:2015,
  author = {Harris, Robert C. and  Travis, Mackoy and Fenley, Marcia O.},
  title = {{Problems of Robustness in Poisson–Boltzmann Binding Free Energies}},
  journal = {Journal of Chemical Theory and Computation},
  year = {2015},
	volume = {11(2)},
  pages = {705-712}
}

@ARTICLE{ZhangZ:2011,
  author = {Zhang, Z. and  Witham, S. and Alexov, E.},
  title = {{On the role of electrostatics in protein-protein interactions}},
  journal = {Physical biology},
  year = {2011},
	volume = {8(3)},
  pages = {035001}
}

@ARTICLE{RenP:2012,
  author = {Ren, P. and Chun, J. and Thomas,  D. G. and Schnieders, M. J. and Marucho, M. and Zhang, J. and Baker, N. A.},
  title = {{Biomolecular electrostatics and solvation: a computational perspective}},
  journal = {Quarterly reviews of biophysics},
  year = {2012},
	volume = {45(04)},
  pages = {427-491}
}


@ARTICLE{Boehr:2009,
  author = {Boehr,  D. D. and Nussinov, R. and Wrigt, P. E.},
  title = {{The role of synamic conformational ensembles in biomolecular recognition}},
  journal = {Nature chemical biology},
  year = {2009},
	volume = {5(11)},
  pages = {789-796}
}


@ARTICLE{Onufriev:2013,
  author = {Onufriev,  A. V. and Alexov, E.},
  title = {{Protonation and pK changes in protein-ligand binding}},
  journal = {Quarterly reviews of biophysics},
  year = {2013},
	volume = {46(02)},
  pages = {181-219}
}




@ARTICLE{Delphi:2012,
  author = {Lin Li and Chuan Li and  Subhra Sarkar and Jie Zhang and Shawn Witham and Zhe Zhang and Lin Wang and  Nicholas Smith and Marharyta Petukh and Emil Alexov},
  title = {{Delphi}: a comprehensive suite for Delphi software and associated resources},
  journal = {BMC Biophysics},
  year = {2012},
  volume = {5:9},
  pages = {2046-1682}
}


@ARTICLE{Marcia:2011,
  author = {Boschitsch, A. H. and Fenley, M. O.},
  title = {{A Fast and Robust Poisson-Boltzmann Solver Based on Adaptive Cartesian Grids}},
  journal = {Journal of Chemical Theory and Computation},
  year = {2011},
  volume = {7},
  pages = {1524-1540}
}


@ARTICLE{LuoRayPBSA:2012,
  author = {Jun Wang and Qin Cai and Ye Xiang and Ray Luo},
  title = {{Reducing Grid Dependence in Finite Difference Poisson Boltzmann Calculations}},
  journal = {Journal of Chemical Theory and Computation},
  year = {2012},
  volume = {8},
  pages = {2741-2751}
}


@ARTICLE{LuBenzhuo:2013,
  author = {Benzhuo Lu and Xiaolin Cheng and Jingfang Huang and J. Andrew McCammon},
  title = {{AFMPB: An Adaptive Fast Multipole Poisson-Boltzmann Solver for Calculating Electrostatics in Biomolecular Systems}},
  journal = {Comput. Phys. Commun.},
  year = {2013},
  volume = {184},
  pages = {2618-2619}
}




@ARTICLE{Geng2013:1,
  author = {W. H. Geng and F. Jacob},
  title = {A GPU-accelerated direct-sum boundary integral Poisson-Boltzmann
solver},
  journal = {Comput. Phys. Commun.},
  year = {2013},
  volume = {184},
  pages = {1490 -1496}
}

@ARTICLE{Geng2013:2,
  author = {W. H. Geng},
  title = {Parallel higher-order boundary integral electrostatics computation on molecular surfaces
with curved triangulation},
  journal = {J. Comput. Phys.},
  year = {2013},
  volume = {241},
  pages = {253 -265}
}


@ARTICLE{Geng2013:3,
  author = {W. H. Geng and R. Krasny},
  title = {A treecode-accelerated boundary integral {Poisson-Boltzmann} solver for
continuum electrostatics of solvated biomolecules},
  journal = {J. Comput. Phys.},
  year = {2013},
  volume = {247},
  pages = {62-87}
}





@ARTICLE{LiLin:2014,
  author = {Lin Li and Chuan Li and Emil Alexov},
  title = {On the Modeling of Polar Component of Solvation Energy using Smooth Gaussian-Based Dielectric Function},
  journal = {Journal of Theoretical and Computational Chemistry},
  year = {2014},
  volume = {13},
  pages = {10.1142/S0219633614400021},
}








@ARTICLE{Jacopo:2005,
  author = {Jacopo Tomasi, Benedetta Mennucci and Roberto Cammi },
  title = {Quantum Mechanical Contunuum Solvation Models},
  journal = {Chem. Rev.},
  year = {2005},
  volume = {105},
  pages = {2999-3093}
}




@ARTICLE{GEPOL:1994,
  author = {J. L. Pascual-ahuir and E. Silla and I. Tuñon},
  title = {GEPOL: An improved description of molecular surfaces. III. A new algorithm for the computation of a solvent-excluding surface},
  journal = {Journal of Computational Chemistry},
  year = {1994},
  volume = {15},
  pages = {1127-1138}
}


@article{ZhanQM:2011,
  title={Differential geometry based solvation model. III. Quantum formulation},
  author={Zhan Chen and Guo-Wei Wei},
  journal={Journal of Chemical Physics},
  volume={135},
  number={194108},
  pages={},
  year={2011},
  publisher={}
}


@ARTICLE{YCZhouThesis,
    author =  {Zhou, Y. C. },
    title = { Matched interface and boundary (MIB) method and its applications to implicit solvent modeling of biomolecules},
      journal = {Ph.D. Thesis.},
   year = {2006},
	volume = {Michigan State University},
  pages = {}
}



@article{PCM:2005,
  title={Quantum Mechanical Continuum Solvent Models},
  author={Jacopo Tomasi and Benedetta Mennucci and Roberto Cammi},
  journal={Chem. Rev.},
  volume={105},
  pages={2999-3093},
  year={2005}
}

@article{PCM:1994,
  title={Molecular interactions in solution: an overview of methods based on continuous
distributions of the solvent},
  author={Jacopo Tomasi and Maurizio Persico},
  journal={Chem. Rev.},
  volume={94},
  pages={2027-2094},
  year={1994}
}

@article{PCM:1997,
  title={A new integral equation formalism for the polarizable continuum model: Theoretical background and applications
to isotropic dielectrics},
  author={E. Cances, B. Mennucci and J. Tomasi},
  journal={Jornal of Chemical Physics},
  volume={107},
  pages={3032},
  year={1997}
}


@article{Gilson:1988,
  title={Calculating the electrostatic potential of molecules in solution: Method and error assessment},
  author={Michael K. Gilson and Kim A. Sharp and Barry H. Honig},
  journal={Jornal of Computational Chemistry},
  volume={9},
  pages={327-335},
  year={1988}
}


@article{SESConnolly:1983,
  title={Solvent-Accessible Surfaces of Proteins and Nucleic Acids},
  author={Michael L. Cannolly},
  journal={Science},
  volume={221},
  number={4612},
  pages={709-713},
  year={1983}
}

@article{MIBPBSolvation:2015,
  title={Coarse Grid Poisson Boltzmann Solver without Loss of Accuracy},
  author={Bao Wang and Guo-Wei Wei},
  journal={Preprint},
  volume={},
  pages={},
  year={}
}


@article{SMIBPBSolvation:2015,
  title={An Accelerated MIBPB Solver via Posterior Interface Conditions
Matching},
  author={Bao Wang and Guo-Wei Wei},
  journal={Preprint},
  volume={},
  pages={},
  year={}
}

@article{RussianSolvation:2010,
  title={An Accurate Prediction of Hydration Free Energies by Combination of Molecular Integral Equations Theory with Structural Descriptors},
  author={Ekaterina L. Ratkova and Gennady N. Chuev and Volodmyr P. Sergiievskyi and Maxim V. Fedorov},
  journal={J. Phys. Chem. B},
  volume={114},
  pages={12068-12079},
  year={2010}
}



@article{SVM:2001,
  title={On the Algorithmic Implementation of Multi-class SVMs},
  author={K. Crammer and Y. Singer.},
  journal={JMLR},
  volume={},
  pages={},
  year={2001}
}



@article{SVM:2004,
  title={Support Vector Learning for Interdependent and Structured Output Spaces},
  author={ I. Tsochantaridis and T. Hofmann and T. Joachims and Y. Altun.},
  journal={ICML},
  volume={},
  pages={},
  year={2004}
}



@article{SVM:1999,
  title={Making Large-Scale SVM Learning Practical. Advances in Kernel Methods - Support Vector Learning},
  author={ B. Schölkopf and C. Burges and A. Smola.},
  journal={MIT Press},
  volume={},
  pages={},
  year={1999}
}




@article{Liblinear,
  title={LIBLINEAR: A library for large linear classification},
  author={R.-E. Fan and K.-W. Chang and C.-J. Hsieh and X.-R. Wang and and C.-J. Lin },
  journal={Journal of Machine Learning Research},
  volume={9},
  pages={1871-1874},
  year={2008}
}


@article{LibSVM,
  title={Working set selection using second order information for training SVM},
  author={R.-E. Fan, P.-H. Chen, and C.-J. Lin.},
  journal={Journal of Machine Learning Research},
  volume={6},
  pages={1889-1918},
  year={2005}
}


@article{SIESTA:2002,
  title={The SIESTA method for ab-initio order-N materials simulation},
  author={J. M. Soler and E. Artacho and J. D. Gale and A. García and J. Junquera and
P. Ordejón and D. Sánchez-Portal},
  journal={J. Phys.: Condens. Matt.},
  volume={14},
  pages={2745-2779},
  year={2002}
}


@article{Geosingularity:2007,
  title={Treatment  of  geometric  singularities  in  implicit  solvent  models},
  author={S.  N.  Yu and  W.  H.  Geng  and  G.W.  Wei.},
  journal={J. Chem.  Phys.},
  volume={126},
  pages={244108},
  year={2007}
}



@article{Nicholls:2008solvation,
  title={Predicting Small-Molecule Solvation Free Energies: An Informal Blind Test for Computational Chemistry},
  author={Anthony Nicholls and David L. Mobley and J. Peter Guthrie and John D. Chodera and Chridtopher I. Bayly and Matthew D. Cooper and Vijay S. Pande},
  journal={J. Med. Chem.},
  volume={51},
  pages={769-799},
  year={2008}
}


@article{David:2014solvation,
  title={Blind prediction of solvation free energies from the SAMPL4 challenge},
  author={David L. Mobley and Karisa L. Wymer and Nathan M. Lim and J. Peter Guthrie},
  journal={J. Comput Aided Mol Des},
  volume={28},
  pages={135-150},
  year={2014}
}


@article{Guthrie:2014solvation,
  title={SAMPL4, a blind challenge for computational solvation free energies: the compounds considered.},
  author={J. Peter Guthrie},
  journal={J. Comput Aided Mol Des},
  volume={28},
  pages={151-168},
  year={2014}
}


@article{Klamt:2014solvation,
  title={Prediction of free energies of hydration with COSMO-RS on the SAMPL4 data set},
  author={Jens Reinisch and Andreas Klamt},
  journal={J. Comput Aided Mol Des},
  volume={28},
  pages={169-173},
  year={2014}
}


@article{David:2012solvation,
  title={Alchemical prediction of hydration free energies for SAMPL},
  author={David L. Mobley and Shaui Liu and David S. Cerutti and William C. Swope and Julia E. Rice},
  journal={J. Comput Aided Mol Des.},
  volume={26},
  pages={551-562},
  year={2012}
}


@article{David:2010solvation,
  title={Predicting hydration free energies using all-atom molecular dynamics simulations and multiple starting conformations},
  author={Pavel V. Klimovich and David L. Mobley},
  journal={J. Comput Aided Mol Des.},
  volume={24},
  pages={307-316},
  year={2010}
}


@article{David:2009solvation,
  title={Predictions of Hydration Free Energies from all-Atom Molecular Dynamics Simulations},
  author={David L. Mobley and Christopher I. Bayly and Matthew D. Cooper and Ken A. Dill},
  journal={J. Phys. Chem. B.},
  volume={13},
  pages={4533-4537},
  year={2009}
}


@article{David:2019JCTCsolvation,
  title={Small Molecule Hydration Free Energies in Explicit Solvent: An Extensive Test of Fixed-Charge Atomistic Simulations},
  author={David L. Mobley and Christopher I. Bayly and Matthew D. Cooper and Michael R. Shirts and Ken A. Dill},
  journal={Journal of Chemical Theory and Computation},
  volume={5},
  pages={350-358},
  year={2009}
}



@article{David:2006JCTCsolvation,
  title={Estimation of Absolute Free Energies of Hydration Using Continuum Methods: Accuracy of Partial Charge Models and Optimization of Nonpolar Contributions},
  author={Robert C. Rizzo and Tiba Aynechi and David A. Case and Irwin D. Kuntz},
  journal={Journal of Chemical Theory and Computation},
  volume={2},
  pages={128-139},
  year={2006}
}


@article{David:2008JPCBsolvation,
  title={Treating Entropy and Conformational Changes in Implicit Solvent Simulations of Small Molecules},
  author={David L. Mobley and Ken A. Dill and John D. Chodera},
  journal={J. Phys. Chem. B.},
  volume={112},
  pages={938-946},
  year={2008}
}

@article{Wujianzhong:2014,
  title={Fast prediction of hydration free energies for SAMPL4 blind test from a classical density functional theory},
  author={J. Fu and Y. Liu and J. Wu},
  journal={The Journal of Computer-Aided Molecular Design},
  volume={28},
  pages={299-304},
  year={2014}
}


@article{Evans:1979,
  title={The nature of the liquid-vapor interface and other topics in the statistical mechanics of non-uniform, classical fluids},
  author={R. Evans},
  journal={Advance in physics},
  volume={28},
  pages={143-200},
  year={1979}
}


%%Nonaqueous solvent
@article{Chung:2003,
  title={Poisson-Boltzmann Continuum Solvation Models for Nonaqueous Solvents I. 1-Octanol},
  author={Insook Park and Yun Hee Jang and Sungu Hwang and Doo Soo Chung},
  journal={Chemistry Letters},
  volume={32},
  pages={4},
  year={2003}
}

@article{Honig:1996Nonaqueous,
  title={Calculation of Alkane to Water Solvation Free Energies Using Continuum Solvent Models},
  author={Doree Sitoff and Nir Ben-Tal and Barry Honig},
  journal={J. Phys. Chem.},
  volume={100},
  pages={2744-2752},
  year={1996}
}


@article{Liotard:1996Nonaqueous,
  title={Solvation Modeling in Aqueous and Nonaqueous Solvents},
  author={Joey W. Storer and David J. Giesen and Gregory D. Hawkins and Gillian C.Lynch,
Christopher J. Cramer and Donald G. Truhlar and Daniel A. Liotard},
  journal={Structure, Energetics, and Reactivity in Aqueous Solution: Characterization of Chemical
and Biological Systems},
  volume={},
  pages={24-29},
  year={1996}
}


%%%Truhlar solvation
@article{Truhlar:2008Solvation,
  title={A Universal Approach to Solvation Modeling},
  author={Christopher J. Cramer and Donald G. Truhlar},
  journal={Accounts of chemical research},
  volume={41},
  pages={760-768},
  year={2008}
}


@article{Truhlar:1998Solvation,
  title={Modeling Free Energies of Solvation and Transfer },
  author={D. J. Giesen and C. C. Chambers and G. D. Hawkins and C. J. Cramer and D. G. Truhlar},
  journal={Computational Thermochemistry},
  volume={},
  pages={285-300},
  year={1998}
}


@article{Truhlar:1998Solvation2,
  title={Universal Solvation Models },
  author={Gregory D. Hawkins and Tianhai Zhu and Jiabo Li and Candee C. Chanbers and David J. Giesen and  Daniel A. Liotard and Christopher J. Cramer and Donald G. Truhlar},
  journal={Combined Quantum Mechanical and Molecular Mechanical Methods},
  volume={},
  pages={201-219},
  year={1998}
}


@article{Truhlar:1999Solvationext,
  title={Extension of the platform of applicability of the SM5.42R universal solvation model },
  author={Jiabo Li and Tianhai Zhu and Gergory D. Hawkins and Paul Winget and Daniel A. Liotard and Christopher J. Cramer and Donald G. Truhlar},
  journal={Theoretical Chemistry Accounts},
  volume={103},
  pages={9-63},
  year={1999}
}


@article{Truhlar:2001Solvation,
  title={Solvation Thermodynamics and the Treatment of Equilibrium and Nonequilibrium Solvation Effects by
Models Based on Collective Solvent Coordinates},
  author={C. J. Cramer and D. G. Truhlar},
  journal={Free Energt Calculations in Rational Drug Design},
  volume={},
  pages={63-95},
  year={2001}
}



@article{Truhlar:2001Solvation2,
  title={Molecular-Scale Modeling of Reaction and Solvation},
  author={D. G. Truhlar},
  journal={First International conference on Foundations of Molecular Modeling and Simulation},
  volume={97},
  pages={71-83},
  year={2001}
}

@article{Truhlar:2006Solvation,
  title={SMx Continuum Models for Condensed Phases},
  author={Christopher J. Cramer and Donlad G. Truhlar},
  journal={Trends and Perspectives in Modern Computational Science},
  volume={6},
  pages={112-140},
  year={2006}
}

@article{Josefredo:2008Solvation,
  title={Transition State Theory and Chemical Reaction Dynamics in Solution},
  author={Donald G. Truhlar and Josefredo R. Pliego Jr},
  journal={Continuum Solvation Models in Chemical Physics},
  volume={},
  pages={338-365},
  year={2008}
}


@article{Truhlar:2008SolvationP,
  title={Perspective on Foundations of Solvation Modeling: The Electrostatic Contribution to the Free Energy of Solvation},
  author={Aleksandr V. Marenich and Christopher J. Cramer and Donald G. Truhlar},
  journal={J.Chem.Theory Comput},
  volume={4},
  pages={877-877},
  year={2008}
}


@article{Honig:1996Solvation,
  title={New Model for Calculation of Solvation Free Energies: Correction of Self-Consistent Reaction
Field Continuum Dielectric Theory for Short-Range Hydrogen-Bonding Effects},
  author={Bryan Marten and Kyungsun Kim and  Christian Cortis and Richard A. Friesner and Robert B. Murphy  and Murco N. Ringnalda and Doree Sitkoff  and Barry Honig },
  journal={J. Phys. Chem},
  volume={100},
  pages={11775-11788},
  year={1996}
}


@article{BaoWang:2015QMSolvation1,
  title={Coupling Physical and Statistical Models for Ab initio Solvatio Free Energy Calculation},
  author={Bao Wang and Guo-Wei Wei},
  journal={Preprint},
  volume={},
  pages={},
  year={}
}


@article{Yap:2011,
  title={PaDEL-Descriptor: An open source software to calculate molecular descriptors and fingerprints},
  author={Yap, C W},
  journal={Journal of Computational Chemistry.},
  volume={32(7)},
  pages={1466-1474},
  year={2011}
}


@article{RenxiaonWang:2007,
  title={Automatic Perception of Organic Molecules Based on Essential Structural Information},
  author={Yuan Zhao and Tiejun Cheng and Renxiao Wang},
  journal={J. Chem. Inf. Model.},
  volume={47},
  pages={1379-1385},
  year={2007}
}




@article{Kollman:2001Solvation,
  title={Solvation Model Based on Weighted Solvent ccessible surface Area},
  author={Junmei Wang and Wei Wang and Shuanghong Huo and Matthew Les and Peter A. Kollman},
  journal={J. Phys. Chem. B},
  volume={105},
  pages={5055-5067},
  year={2001}
}


@article{Truhlar:1999SolvationChemRev,
  title={Implicit solvation models: equilibria, structure, spectra, and dynamics},
  author={C. J. Cramer and D. G. Truhlar},
  journal={Chemical Reviews},
  volume={99(8)},
  pages={2161-2200},
  year={1999}
}


@misc{cvx,
  author       = {Michael Grant and Stephen Boyd},
  title        = {{CVX}: Matlab Software for Disciplined Convex Programming, version 2.1},
  howpublished = {\url{http://cvxr.com/cvx}},
  month        = {mar},
	 pages       = {513-520},
  year         = {2014}
}


@incollection{gb08,
  author    = {Michael Grant and Stephen Boyd},
  title     = {Graph implementations for nonsmooth convex programs},
  booktitle = {Recent Advances in Learning and Control},
  series    = {Lecture Notes in Control and Information Sciences},
  editor    = {V. Blondel and S. Boyd and H. Kimura},
  publisher = {Springer-Verlag Limited},
  pages     = {95--110},
  year      = 2008,
  note      = {\url{http://stanford.edu/~boyd/graph_dcp.html}}
}


@incollection{EMSL:2009,
  author    = {Trevor Hastie and Robert Tibshirani and Jerome Friedman},
  title = {The Elements of Statistical Learning: Data Mining, Inference, and Prediction},
	booktitle = {The Elements of Statistical Learning: Data Mining, Inference, and Prediction},
  series    = {Second Edition},
  editor    = {},
  publisher = {Springer},
  pages     = {},
  year      = 2009,
  note      = {}
}





@article{Mobley:2014,
    title     = {FreeSolv: a database of experimental and calculated hydration free energies, with input files},
  author    = {David L. Mobley and  J. Peter Guthrie },
  journal={Journal of Computer-Aided Molecular Design},
  volume={28},
  pages={ 711-720},
  year={2014}
}


@article{SJi:2012,
    title     = {{Poisson-Nernst-Planck systems for ion flow with Density Functional Theory for hard-sphere potential: I-V relations and critical potentials. Part I: Analysis}},
  author    = {S. Ji and Weishi Liu },
  journal={Journal of  Dynam. Differential Equations },
  volume={24},
  pages={ 955-983},
  year={2012}
}

@ARTICLE{Catterall:2012,
  author = {Catterall, W. A.},
  title = {{Voltage-gated sodium channels at 60: structure, function and pathophysiology}},
  journal = {J. Physiol.},
	volume = {590},
  year = {2012},
  pages = {2577-2589}
}



@ARTICLE{Dongetal:2014,
  author = {Dong, K. and  Du, Y. and  Rinkevich, F. D. and  Nomura, Y. and  Xu,  P. and  Wang, L. and  Silver,  K. and  and Zhorov, B. S. },
  title = {{Molecular biology of insect sodium channels and pyrethroid resistance}},
  journal = {Insect Biochem.},
	volume = {50},
  year = {2014},
  pages = {1-17}
}

@ARTICLE{Wangetal:2015,
  author = {Wang, L and Nomura, Y. and  Du, Y. and Liu, N. and Zhorov, B. S. and Dong, K. },
  title = {{A mutation in the intracellular loop III/IV of mosquito sodium channel synergizes the effect of mutations in helix IIS6 on pyrethroid resistance.}},
  journal = {Mol. Pharmacol.},
	volume = {106},
  year = {2015},
  pages = {93-100}
}


@ARTICLE{KDong:2007,
  author = {Dong, K.   },
  title = {{Insect sodium channels and insecticide resistance}},
  journal = {Invert. Neurosci. },
	volume = {7},
  year = {2007},
  pages = {17-30}
}



@ARTICLE{Duetal:2011,
  author = {Du, Y. and  Garden, D.P. and  Wang, L. and  Zhorov, B. S. and  Dong, K.},
  title = {{Identification of new batrachotoxin-sensing residues in segment IIIS6 of the sodium channel}},
  journal = {J. Biol. Chem.  },
	volume = {286},
  year = {2011},
  pages = {13151-13160}
}


@ARTICLE{Duetal:2013,
  author = {Du, Y. and  Nomura, Y. and  Satar, G. and  Hu, Z. and  Nauen, R. and  He, S. Y. and  Zhorov, B. S. and  Dong, K. },
  title = {{Molecular evidence for dual pyrethroid-receptor sites on a mosquito sodium channel}},
  journal = {Proc. Nat. Acad. Sci.  },
	volume = {110},
  year = {2013},
  pages = {11785-11790}
}

@ARTICLE{Duetal:2015,
  author = {Du, Y. and  Nomura, Y. and  Zhorov, B. S. and  Dong, K.  },
  title = {{Rotational Symmetry of two pyrethroid receptor sites in the mosquito sodium channel}},
  journal = {Mol. Pharmacol.  },
	volume = {},
  year = {in press 2015},
  pages = {}
}

@ARTICLE{Dongetal:2015,
  author = {Dong, K. and  Du, Y.  and  Rinkevich, F. and  Wang, L. and Xu, P. },
  title = {{The Drosophila sodium channel 1 (DSC1): The founding member of a new family of voltage-gated cation channels}},
  journal = {Pestic. Biochem. Physiol. },
	volume = {120},
  year = {2015},
  pages = {36-39}
}

@ARTICLE{LWang:2015,
  author = {Wang, L. and Du, Y. Z. and  Nomura, Y. and Dong K. },
  title = {{Distinct modulatory effects of TipE homologs 2-4 on Drosophila sodium channel splice variants}},
  journal =  {Insect Biochem. Mol. Biol.},
	volume = {60},
  year = {2015},
  pages = {26-32}
}

	
@ARTICLE{Rinkevich:2015,
  author = {Rinkevich,  F. D. and  Du, Y. and  Tolinski, J and  Ueda, A. and  Wu, C.-F. and Zhorov, B. S. and  Dong, K. },
  title = {{Distinct roles of the DmNav and DSC1 channels in the action of DDT and pyrethroids}},
  journal =  {Neurotoxicol.},
	volume = {47},
  year = {2015},
  pages = {99-106}
}

 @ARTICLE{LWang:2015b,
  author = {Wang, L. and  Nomura, Y. and  Du, Y. and  Liu, N. and Zhorov,  B. S. and Dong, K. },
  title = {{A mutation in the intracellular loop III/IV of mosquito sodium channel synergizes the effect of mutations in helix IIS6 on pyrethroid resistance}},
  journal =  {Mol. Pharmacol.},
	volume = {106},
  year = {2015},
  pages = {93-100}
}





@ARTICLE{Fengetal:1995,
  author = {Feng, G. and  Deak, P. T. and  Chopra, M. and Hall, L. M.     },
  title = {{Cloning and functional analysis of tipE, a novel membrane protein that enhances drosophila para sodium channel function}},
  journal = {Cell},
	volume = {82},
  year = {1995},
  pages = {1001-1011}
}


@ARTICLE{Oliveiraetal:2013,
  author = {Oliveira, E. E. and  Du, Y. and  Nomura, Y. and  Dong, K.    },
  title = {{A residue in the transmembrane segment 6 of domain I in insect and mammalian sodium channels regulate differential sensitivities to pyrethroid insecticides}},
  journal = {Neurotoxicology },
	volume = {38C},
  year = {2013},
  pages = {42-50}
}

@ARTICLE{Silveretal:2014,
  author = {Silver, K. S. and  Du, Y. and  Nomura, Y. and  Oliveira, E. E. and  Salgado, V. L. and  Zhorov, B. S. and  Dong, K.  },
  title = {{Voltage-gated sodium channels as insecticide target sites}},
  journal = {In “Target receptors in the control of insect pests.” Part II, ed. Ephraim Cohen, AIIP, UK: Academic Press},
	volume = {46},
  year = {2014},
  pages = {389-433}
}


@ARTICLE{Tanetal:2002,
  author = {Tan, J. and  Liu, Z. and  Nomura, Y. and  Goldin, A. L. and  Dong, K.  },
  title = {{Alternative splicing of an insect sodium channel gene generates pharmacologically distinct sodium channels}},
  journal = {J. Neurosci. },
	volume = {22},
  year = {2002},
  pages = {5300-5309}
}


@ARTICLE{Tanetal:2005,
  author = {Tan, J. and Liu, Z. and  Wang, R. and  Huang, Z. Y. and  Chen, A. C. and Gurevitz, M. and  Dong, K. },
  title = {{Identification of amino acid residues in the insect sodium channel critical for pyrethroid binding}},
  journal = {Mol. Pharmacol. },
	volume = {67},
  year = {2005},
  pages = {513-522}
}


@ARTICLE{Tatebayashi:1994,
  author = {Tatebayashi, H. and  Narahashi, T. },
  title = {{Differential mechanism of action of the pyrethroid tetramethrin on tetrodotoxin-sensitive and tetrodotoxin-resistant sodium channels}},
  journal = {J. Pharmacol. Exp. Ther. },
	volume = {270},
  year = {1994},
  pages = {595-603}
}


@ARTICLE{WWang:2003,
  author = {Wang, S. Y. and  Wang, G. K.},
  title = {{Voltage-gated sodium channels as primary targets of diverse lipid-soluble neurotoxins}},
  journal = {Cellular Signalling },
	volume = {15},
  year = {2003},
  pages = {151-159}
}


@ARTICLE{Warmkeetal:1997,
  author = {Warmke, J. W. and Reenan, R. A. G. and  Wang, P. Y. and  Qian, S. and  Arena, J. P. and  Wang, J. X. and  Wunderler, D. and  Liu, K. and  Kaczorowski, G. J. and  VanderPloeg, L. H. T. and  Ganetzky, B. and  Cohen, C. J.},
  title = {{Functional expression of Drosophila para sodium channels - Modulation by the membrane protein TipE and toxin pharmacology}},
  journal = {J. Gen. Physiol. },
	volume = {110},
  year = {1997},
  pages = {119-133}
}


@ARTICLE{Payandeh:2012,
  author = {Payandeh, J. and  Gamal El-Din, T. M. and  Scheuer, T. and  Zheng, N. and  Catterall, W. A.},
  title = {{Crystal structure of a voltage-gated sodium channel in two potentially inactivated states}},
  journal = {Nature },
	volume = {486},
  year = {2012},
  pages = {135-139}
}


	
	
@ARTICLE{Chowdhury:2014,
  author = {Sandipan Chowdhury and Benjamin M. Haehnel  and Baron Chanda},
  title = {{A self-consistent approach for determining pairwise interactions
that underlie channel activation}},
  journal = {J. Gen. Physiol. },
	volume = {144},
  year = {2014},
  pages = {441–455}
}

@ARTICLE{Chowdhury:2012,
  author = {Sandipan Chowdhury    and Baron Chanda},
  title = {{Thermodynamics of electromechanical coupling in voltage-gated
ion channels}},
  journal = {J. Gen. Physiol. },
	volume = {140},
  year = {2012},
  pages = {613–623}
}
	
@ARTICLE{Yarov-Yarovoy:2011,
  author = {Vladimir Yarov-Yarovoy and  Paul G. DeCaena and Ruth E. Westenbroeka and Chien-Yuan Pana and Todd Scheuera and David Bakerb and William A. Catteralla},
  title = {{Structural basis for gating charge movement in the
voltage sensor of a sodium channel}},
  journal = {Proc. Natl. Acad. Sci. USA },
	volume = {109},
  year = {2011},
  pages = {E93-E102}
}


@ARTICLE{Blunck:2012,
  author = {Rikard Blunck   and Zarah Batulan},
  title = {{Mechanism of electromechanical coupling in voltage-gated
potassium channels}},
  journal = {Frontiers in Pharmacology },
	volume = {3},
  year = {2012},
  pages = {Article 166}
}


@ARTICLE{Cestele:2006,
  author = {Sandrine Cestele and, Vladimir Yarov-Yarovoy and Yusheng Qu and François Sampieri and Todd
Scheuer  and William A. Catterall},
  title = {{Structure and Function of the Voltage Sensor of Sodium Channels
Probed by a $\beta$-Scorpion Toxin}},
  journal = {J. Biol. Chem. },
	volume = {281},
  year = {2006},
  pages = {21332-21344}
}


@ARTICLE{Jensen:2012,
  author = {Morten O. Jensen and Vishwanath Jogini and  David W. Borhani and Abba E. Leffler and
Ron O. Dror and David E. Shaw},
  title = {{Mechanism of Voltage Gating in Potassium Channels}},
  journal = {Science },
	volume = {336},
  year = {2012},
  pages = {229-232}
}


@ARTICLE{CJTsai:2013,
  author = {Tsai, C. J. and   Tani, K. and   Irie, K. and  Hiroaki, Y. and  Shimomura, T. and  Mcmillan, D. G. and   Cook, G. M. and   Schertler, G. and  Fujiyoshi, Y. and  Li, X. D.},
  title = {{Two alternative conformations of a voltage-gated sodium channel}},
  journal = { J. Mol. Biol.},
	volume = {425},
  year = {2013},
  pages = {4074-4088}
}



@ARTICLE{Boiteux:2014,
  author = {Céline Boiteuxa and Igor Vorobyovb and Robert J. Frenchc and Christopher Frenchd and Vladimir Yarov-Yarovoye and Toby W. Allena},
  title = {{Local anesthetic and antiepileptic drug access and
binding to a bacterial voltage-gated sodium channel}},
  journal = {Proc. Natl. Acad. Sci. USA},
	volume = {36},
  year = {2014},
  pages = {13057-13062}
}

@ARTICLE{Lacroix:2013,
  author = {Lacroix, J. J. and  Campos, F.V. and Frezza, L. and Bezanilla, F.},
  title = {{Molecular Bases for the Asynchronous Activation of Sodium and Potassium Channels Required for Nerve Impulse Generation}},
  journal = {Neuron },
	volume = {79},
  year = {2013},
  pages = {651-657}
}


@ARTICLE{Vargas:2012,
  author = {Vargas, E. and Yarov-Yarovoy V. and Khalili-Aragi, F. and  Catterall, W. A. and  Klein, M. L. and  Tarek, M. and  Lindahl, E. and Schulten, K. and Perozo, E. and  Bezanilla, F. and Roux, B.},
  title = {{Viewpoint: An emerging consensus on voltage-dependent gating from computational modeling and molecular dynamics simulations}},
  journal = {J. Gen. Physiol. },
	volume = {140},
  year = {2012},
  pages = {578-594}
}



@ARTICLE{Gutman:2005,
  author = {Gutman, G. A. and  Chandy, K. G. and  Grissmer,  S. and  Lazdunski, M. and  McKinnon, D. and  Pardo, L. A. and  Robertson,  G. A. and  Rudy,  B. and  Sanguinetti, M. C. and  Stuhmer, W. and  Wang, X.},
  title = {{International Union of Pharmacology. LIII. Nomenclature and molecular relationships of voltage-gated potassium channels}},
  journal = {Pharmacol Rev  },
	volume = {57},
  year = {2005},
  pages = {473-508}
}

@ARTICLE{SBLong:2005,
  author = {Long, S. B. and  Campbell,  E. B. and  Mackinnon, R. },
  title = {{Crystal structure of a mammalian voltage-dependent Shaker family K+ channel}},
  journal = {Science  },
	volume = {309},
  year = {2005},
  pages = {897-903}
}

@ARTICLE{Catteralletal:2003,
  author = {Catterall, W. A. and Goldin,  A. L. and Waxman, S. G. },
  title = {{International Union of Pharmacology. XXXIX. Compendium of voltage-gated ion channels: sodium channels}},
  journal = {Pharmacol Rev },
	volume = {55},
  year = {2003},
  pages = {575-578}
}


@ARTICLE{Catterall:2000,
  author = {Catterall, W. A. },
  title = {{Structure and regulation of voltage-gated Ca2+ channels}},
  journal = {Annu. Rev. Cell Dev. Biol. },
	volume = {16},
  year = {2000},
  pages = {521-555}
}


@ARTICLE{Catterall:2010,
  author = {Catterall, W. A. },
  title = {{
Ion Channel Voltage Sensors: Structure, Function, and Pathophysiology
}},
  journal = {Neuron},
	volume = {67},
  year = {2000},
  pages = {915-928}
}


@ARTICLE{McCuskeretal:2012,
  author = {McCusker, E. C. and Bagneris, C. and  Naylor, C. E. and  Cole, A. R. and  D'Avanzo, N. and  Nichols, C. G. and  Wallace, B. A. },
  title = {{ Structure of a bacterial voltage-gated sodium channel pore reveals mechanisms of opening and closing}},
  journal = {Nature Communications},
	volume = {3},
  year = {2012},
  pages = {1102}
}

@ARTICLE{Bagnerisetal:2013,
  author = {Bagneris, C. and  DeCaen, P. G. and Hall, B. A. and Naylor, C. E. and Clapham, D. E. and Kay, C. W. M. and    Wallace, B. A. },
  title = {{ Role of the C-terminal domain in the structure and function of tetrameric sodium channels}},
  journal = {Nature Communications},
	volume = {4},
  year = {2013},
  pages = {2465}
}

@ARTICLE{Shayaetal:2014,
  author = {Shaya, D. and   Findeisen, F.  and Abderemane-Ali, F. and Arrigoni, C. and  Wong, S. and  Nurva, S. R. and Loussouarn, G. and  Minor, D. L.},
  title = {Structure of a Prokaryotic Sodium Channel Pore Reveals Essential Gating Elements and an Outer Ion Binding Site Common to Eukaryotic Channels
},
  journal = {Journal of Molecular Biology},
	volume = {426},
  year = {2014},
  pages = {467-483}
}



@ARTICLE{Duetal:2009,
  author = {Du, Y. and Lee, J. E. and  Nomura, Y. and Zhang, T. and  Zhorov, B. S. and Dong, K. },
  title = {{Identification of a cluster of residues in transmembrane segment 6 of domain III of the cockroach sodium channel essential for the action of pyrethroid insecticides}},
  journal = {Biochem. J.  },
	volume = {419},
  year = {2009},
  pages = {377-385}
}

@ARTICLE{Chowdhury:2015,
  author = {Sandipan Chowdhury and  Benjamin M. Haehnel and Baron Chanda},
  title = {{A self-consistent approach for determining pairwise interactions
that underlie channel activation}},
  journal = {J. Gen. Physiol. },
	volume = { 144 },
  year = {2015},
  pages = {441-455}
}


@ARTICLE{Narahashi:2000,
  author = {Narahashi, T.},
  title = {{Neuroreceptors and ion channels as the basis for drug action: past, present, and future}},
  journal = {J. Pharmacol. Exp. Ther.  },
	volume = {294},
  year = {2000},
  pages = {1-26}
}


@ARTICLE{Groomeetal:1999,
  author = {Vijverberg, H. P. M. and  van der Zalm,  J. M. and van den Bercken, J.},
  title = {{Similar mode of
action of pyrethroids and DDT on sodium channel gating in myelinated nerves}},
  journal = {Nature},
	volume = {295},
  year = {1982},
  pages = {601-603}
}
	
	
@ARTICLE{Vijverbergetal:1982,
  author = {Vijverberg, H. P. M. and  van der Zalm,  J. M. and van den Bercken, J.},
  title = {{Similar mode of
action of pyrethroids and DDT on sodium channel gating in myelinated nerves}},
  journal = {Nature},
	volume = {295},
  year = {1982},
  pages = {601-603}
}

@ARTICLE{MSussman:1994,
  author = {M. Sussaman  and  P. Smereka and S. Osher},
  title = {{A level set approach for computing solutions to incompressible two-phase flow}},
  journal = {J. Comput. Phys.},
	volume = {114},
  year = {1994},
  pages = {146-154}
}


@ARTICLE{Overmann:2006,
  author = {M. Overmann and R. Klein},
  title = {{A Cartesian grid finite volume method for elliptic equations with variable coefficients and embedded interfaces}},
  journal = {J. Comput. Phys.},
	volume = {219},
  year = {2006},
  pages = {749–769}
}




@ARTICLE{Bastian:2009,
  author = {P. Bastian and C. Engwer},
  title = {{ An unfitted finite element method using discontinuous Galerkin}},
  journal = {Int. J. Numer. Meth. Engng.},
	volume = {79},
  year = {2009},
  pages = {1557-1576}
}

@article{AG98,
author = "V. I. Abkevich and A. M. Gutin and E. I. Shakhnovich",
title = "A protein engineering analysis of the transition state for protein folding: simulation in the lattice model",
journal = "Fold. Des.",
volume = 3,
pages = {183--194},
year = 1998
}

@article{AM06,
author = {Steward A. Adcock and J. Andrew McCammon},
title = "Molecular Dynamics: Survey of Methods for Simulating the Activity of Proteins",
journal = "Chem. Rev. ",
volume = 106,
number = 5,
pages = {1589--1615},
year = 2006
}

@InProceedings{Bajaj97thecontour,
  year = 	"1997",
  title =	"The Contour Spectrum",
  URL =  	"http://visinfo.zib.de/EVlib/Show?EVL-1997-134",
  author =	"Chandrajit L. Bajaj and Valerio Pascucci and Daniel R.
		 Schikore",
  keywords =	"Visualization, Scalar Data, User Interfaces,Real-time
		 Quantitative Query",
  booktitle =	"IEEE Visualization '97",
}

@inproceedings{BGW14,
  title="Measuring distance bewteen {R}eeb graphs",
  author="Ulrich Bauer and Xiaoyin Ge and Yusu Wang",
  booktitle="Proc. 30th Annu. Sympos. Comput. Geom. (SoCG)",
pages = {464--473},
  year={2014}
}

@inproceedings{BMW15,
author = "U. Bauer and E. Munch and Y. Wang",
title = "Strong equivalence of the interleaving and functional distortion metrics for {Reeb} graphs",
booktitle = "Proc. 31rd Annu. Sympos. Comput. Geom. (SoCG)",
pages = "461--475",
year = 2015
}

@article{BEJ09,
author = {Adam L. Beberg and Daniel L. Ensign and Guha Jayachandran and Siraj Khaliq and Vijay S. Pande},
title = {Folding\@home: Lessons from eight years of volunteer distributed computing},
journal ={Parallel and Distributed Processing Symposium, International},
volume = {0},
isbn = {978-1-4244-3751-1},
year = {2009},
pages = {1-8},
doi = {http://doi.ieeecomputersociety.org/10.1109/IPDPS.2009.5160922},
publisher = {IEEE Computer Society},
address = {Los Alamitos, CA, USA},
}

@article{BelkinLapMap2003,
  AUTHOR    = "M. Belkin and P. Niyogi",
  TITLE     = "Laplacian eigenmaps for dimensionality reduction and data representation",
  JOURNAL   = "Neural Comp",
  VOLUME    = "15",
  NUMBER    = "6",
  PAGES     = "1373-1396",
  YEAR      = "2003" }
	
	
@inproceedings{BQWZ12,
author = "M. Belkin and Q. Que and Y. Wang and X. Zhou",
title = "Toward understanding complex data: graph Laplacians on manifolds with singularities and boundaries",
booktitle = "Conf. Learning Theory (COLT)",
note = "to appear,",
year = 2012
}

@inproceedings{BCEHM07,
  author    = {Paul Bendich and
               David Cohen-Steiner and
               Herbert Edelsbrunner and
               John Harer and
               Dmitriy Morozov},
  title     = {Inferring Local Homology from Sampled Stratified Spaces},
  booktitle = {Proc. 48th IEEE Sympos. Found. Comput. Science},
  year      = {2007},
  pages     = {536-546},
}

@inproceedings{BWM12,
author = {P. Bendich and B. Wang and S. Mukherjee},
title = {Local homology transfer and stratification learning},
booktitle = {Proc. 23rd Ann. ACM-SIAM Sympos. Discrete Alg.},
year = 2012,
pages = {1355--1370}
}

@article{B12,
author = "R. B. Best",
title = "Atomistic molecular simulations of protein folding",
journal = "Curr. Opin. Struct. Biol.",
volume = 22,
number = 1,
pages = {52--61},
year = 2012
}

@phdthesis{Buchet14,
author = "M. Buchet",
title = "Topological inference from measures",
school = "Universit\'{e} Paris Sud -- Paris XI",
year =2014
}

@inproceedings{BCD15,
author = "M. Buchet and F. Chazal and T. K. Dey and F. Fan and S. Oudot and Y. Wang",
title = "Topological analysis of scalar fields with outliers",
booktitle = "Proc. 31rd Annu. Sympos. Comput. Geom. (SoCG)",
pages = "827--841",
year = 2015
}

@article{BDW10,
author = "O. Busaryev and T. K. Dey and Y. Wang",
title = "Tracking a generator by persistence",
journal = "Discrete Mathematics, Algorithms and Applications",
volume = 2,
number =4,
pages = {539--552},
year = 2010
}

@inproceedings{769927,
 author = {Carr, Hamish and Snoeyink, Jack},
 title = {Path seeds and flexible isosurfaces using topology for exploratory visualization},
 booktitle = {VISSYM '03: Proceedings of the symposium on Data visualisation 2003},
 year = {2003},
 isbn = {1-58113-698-6},
 pages = {49--58},
 location = {Grenoble, France},
 publisher = {Eurographics Association},
 address = {Aire-la-Ville, Switzerland, Switzerland},
 }

@Article{carr:tree,
  title =	"Computing contour trees in all dimensions",
  author =	"Hamish Carr and Jack Snoeyink and Ulrike Axen",
  journal =	"Comput. Geom",
  year = 	"2003",
  number =	"2",
  volume =	"24",
  bibdate =	"2003-11-20",
  bibsource =	"DBLP,
		 http://dblp.uni-trier.de/db/journals/comgeo/comgeo24.html#CarrSA03",
  pages =	"75--94",
}
@Article{CSA03,
  title =       "Computing contour trees in all dimensions",
  author =      "Hamish Carr and Jack Snoeyink and Ulrike Axen",
  journal =     "Comput. Geom",
  year =        "2003",
  number =      "2",
  volume =      "24",
  pages =       "75--94",
}

@INPROCEEDINGS{C98,
   author = {{Chandler}, D.},
    title = "{Finding transition pathways:. throwing ropes over rough mountain passes, in the dark}",
booktitle = {CLassical and Quantum Dynamics in Condensed Phase Simulations},
     year = 1998,
   editor = {{Berne}, B.~J. and {Ciccotti}, G. and {Coker}, D.~F.},
    pages = {51-66},
}

@article{COC04,
author = "L. L. Chavez and J. N. Onuchic and C. Clementi",
title = "Quantifying the roughness on the free energy landscape: {E}ntropic bottlenecks and protein folding rates",
journal = "J. Am. Chem. Soc.",
volume = 126,
pages = {8426--8432},
year = 2004
}

@article{CCM11,
author = "F. Chazal and D. Cohen-Steiner and Q. M{\'e}rigot",
title = "Geometric Inference for Probability Measures",
journal = "Foundations of Computational Mathematics",
year = 2011,
pages = {733--751},
volume = 11,
}

@inproceedings{CFL15,
author = "F. Chazal and B. T. Fasy and F. Lecci and B. Michel and A. Rinaldo and L. Wasserman",
title = "Subsampling methods for persistent homology",
booktitle = "Prof. Int. Conf. Machine Learning (ICML)",
note = "to appear",
year =2015
}

@inproceedings{CFL14,
author = "F. Chazal and B. T. Fasy and F. Lecci and A. Rinaldo and L. Wasserman",
title = "Stochastic convergence of persistence landscapes and sihouettes",
booktitle = "Proc. 30th. Sympos. Comput. Geom.",
year = 2014,
pages = "474--483"
}

@article{CLW06,
author = "S. S. Cho and Y. Levy and P. G. Wolynes",
title = "{P vs. Q: S}tructural Reaction Coordinates Capture Protein Folding on Smooth Landscapes",
journal = "Proc. Natl. Acad. Sci.",
volume = 103,
number = 3,
pages = {586--591},
year = 2006
}

@article{CJO01,
author= "C. Clementi and P. A. Jennings and J. N. Onuchic",
title = "Prediction of folding mechanism for circular-permuted proteins",
journal = "J. Mol. Biol.",
voume = 311,
pages = {879--890},
year = 2001
}

@article{DM06,
author = {P. Das and M. Moll and H. Stamati and L. E. Kavraki and C. Clementi},
title = "Low-dimensional, free-energy landscapes of protein-folding reactions by nonlinear dimensionality reduction",
journal = "Proc. Natl. Acad. Sci.",
volume = 103,
number = 26,
pages = {9885--9890},
year = 2006
}

@inproceedings{Dasgupta2008,
 author = {Dasgupta, Sanjoy and Freund, Yoav},
 title = {Random projection trees and low dimensional manifolds},
 booktitle = {Proceedings of the 40th annual ACM symposium on Theory of computing},
 series = {STOC '08},
 year = {2008},
 isbn = {978-1-60558-047-0},
 location = {Victoria, British Columbia, Canada},
 pages = {537--546},
 numpages = {10},
 acmid = {1374452},
 publisher = {ACM},
 address = {New York, NY, USA},
}

@inproceedings{DSW15,
author = "T. K. Dey and D. Shi and Y. Wang",
title = "Comparing graphs via persistence distortion",
booktitle = "Proc. 31rd Annu. Sympos. Comput. Geom. (SoCG)",
pages = "491--506",
year = 2015
}

@article{DSW11,
Author = {T. K. Dey and J. Sun and Y. Wang},
title = "Approximating Cycles in a Shortest Basis of the First Homology Group from Point Data",
journal = "Inverse Problems",
volume = 27,
pages = {124004},
year = 2011
}

@inproceedings{DW11,
author = "T. K. Dey and Y. Wang",
title = "Reeb graphs: Approximation and Persistence",
booktitle = "Proc. 26th Annu. ACM Sympos. Compu. Geom.",
pages = {226--235},
year = 2011
}

@article{DW13,
  author    = {Tamal K. Dey and
               Yusu Wang},
  title     = {Reeb Graphs: Approximation and Persistence},
  journal   = {Discrete Comput. Geom.},
  volume    = {49},
  number    = {1},
  year      = {2013},
  pages     = {46-73},
}

@article{DiFabio2014b,
  Title                    = {The edit distance for Reeb graphs of surfaces},
  Author                   = {Di Fabio, Barbara and Claudia Landi\},
  Journal                  = {arXiv: 1411.1544},
  Year                     = {2014},
}

@article{DLDS02,
author = "N. V. Dokholyan and L. Li and F. Ding and E. I. Shakhnovich",
title = "Topological determinants of protein folding",
journal = "Proc. Natl. Acad. Sci.",
volume = 99,
pages = {8637--8641},
year = 2002
}

@article{donoho2003hel,
  title={{Hessian eigenmaps: Locally linear embedding techniques for high-dimensional data}},
  author={D.L. Donoho and C. Grimes},
  journal={Proceedings of the National Academy of Sciences},
  volume={100},
  number={10},
  pages={5591-5596},
  year={2003}
}

@article{DP98,
author = "R. Du and Vijay S. Pande and Alexander Yu. Grosberg and Toyoichi Tanaka and Eudene S. Shakhnovich",
title = "On the transition coordinate for protein folding",
journal = "J. Chem. Phys.",
volume = 108,
number = 1,
pages = {334 -- 350},
year = 1998
}
@article{DM11,
author = {Jacob D. Durrant and J. Andrew McCammon},
title = "Molecular dynamics simulations and drug discovery",
journal = "BMC Biology",
volume = 9,
pages = {71--80},
year = 2011
}

@inproceedings{EBW15,
author = "J. Eldridge and M. Belkin and Y. Wang",
title = "Beyond {Hartigan} Consistency: Merge Distortion Metric for Hierarchical Clustering",
booktitle = "Intl. Conf. Learning Theory (COLT)",
note = "Best Student Paper award",
pages = "588--606",
year =2015
}

@article{FP11,
author = "A. L. Ferguson and A. Z. Panagiotopoulos and I. G. Kevrekidis and P. G. Debenedetti",
title = "Nonlinear dimensionality reduction in molecular simulation: The diffusionmap approach",
journal = "Chemical Physics Letters",
volume = 509,
page = {1 -- 11},
year = 2011
}

@incollection{GSBW11,
 title ={Data Skeletonization via Reeb Graphs},
 author="Xiaoyin Ge and Issam I. Safa and Mikhail Belkin and Yusu Wang",
 booktitle = {Advances in Neural Information Processing Systems (NIPS) 24},
 editor = {J. Shawe-Taylor and R.S. Zemel and P. Bartlett and F.C.N. Pereira and K.Q. Weinberger},
 pages = {837--845},
 year = {2011}
}

@InProceedings{Gold86,
  author =	"Christopher Gold and Sean Cormack",
  editor =	"Duane Marble",
  title =	"Spatially Ordered Networks and Topographic
		 Reconstruction",
  booktitle =	"Proceedings of the Second International Symposium on
		 Spatial Data Handling",
  pages =	"74--85",
  address =	"Seattle, Washington",
  year = 	"1986",
}

@article{HP14,
author = "W. Harvey and I. Park and O. {R\"{u}}bel and V. Pascucci and P.-T. Bremer and C. Li and Y. Wang",
title = "A collaborative visual analytics suite for protein folding research",
journal = "J. Mol. Graph. Modeling (JMGM)",
volume = 53,
pages = "59--71",
year = 2014
}

@article{HW10,
author = "W. Harvey and Y. Wang",
title = "Generating and exploring a collection of topological landscapes for visualization of scalar-valued functions",
journal = "Comput. Graph. Forum. (special issue from {\em Eurographics/IEEE Sympos. Visualization})",
note = "3rd Best Paper Award at IEEE EuroVis",
volume = 29,
number = 3,
year = 2010
}

@inproceedings{HWW10,
author = "W. Harvey and R. Wenger and Y. Wang",
title  = " A Randomized $O(m\log m)$ Time Algorithm for Computing {Reeb} Graph of Arbitrary Simplicial Complexes",
booktitle = "Proc. 25th Annu. ACM Sympos. Compu. Geom.",
pages = {267--276},
year = 2010
}

@INPROCEEDINGS{Indyk04low-distortionembeddings,
    author = {Piotr Indyk and Jiri Matousek},
    title = {Low-Distortion Embeddings of Finite Metric Spaces},
    booktitle = {in Handbook of Discrete and Computational Geometry},
    year = {2004},
    pages = {177--196},
    publisher = {CRC Press}
}

@inproceedings{Morozov2013,
  Title                    = {Interleaving Distance between Merge Trees},
  Author                   = {Dmitriy Morozov and Kenes Beketayev and Gunther Weber},
  Booktitle                = {Proceedings of TopoInVis},
  Year                     = {2013},
}

@InProceedings{pascucci01,
  title =	"On the topology of the level sets of a scalar field",
  author =	"Valerio Pascucci",
  year = 	"2001",
  bibdate =	"2002-11-11",
  bibsource =	"DBLP,
		 http://dblp.uni-trier.de/db/conf/cccg/cccg2001.html#Pascucci01",
  booktitle =	"CCCG",
  pages =	"141--144",
  URL =  	"http://compgeo.math.uwaterloo.ca/~cccg01/proceedings/long/pascucci-84239.ps.gz",
}

@article{PSCK07,
author = "E. Plaku and H. Stamati and C. Clementi and L. E. Kavraki",
title = "Fast and reliable analysis of molecular motion using proximity relations and dimensionality reduction",
journal = "Proteins: Structure, Function, and Bioinformatics",
volume = 67,
number = 4,
pages = {897--907},
year = 2007
}

@article{Reeb46,
	author = "Geoge Reeb",
	title = {Sur les points singuliers d'une forme de {Pfaff} compl\`{e}tement int\'{e}grable ou d'une fonction num\'{e}rique},
	journal = {Comptes Rendus Hebdomadaires des S\'{e}ances de l'Acad\'{e}mie des Sciences},
	volume = 222,
	pages = {847--849},
	year = 1946
}

@article{roweis2000ndr,
  title={{Nonlinear Dimensionality Reduction by Locally Linear Embedding}},
  author={S.T. Roweis and L.K. Saul},
  journal={Science},
  volume={290},
  number={5500},
  pages={2323},
  year={2000}
}

@article{SKL07,
author = {H. A. Scheraga and M. Khalili and A. Liwo},
title = {Protein-folding dynamics: overview of molecular simulation techniques},
journal = "Annu. Rev. Phys. Chem.",
volume = 58,
pages = {57--83},
year = 2007
}

@article{SB08,
author = {P. Sherwood and B. R. Brooks and M. S. Sansom},
title = {Multiscale methods for macromolecular simulations},
journal = "Curr. Opin. Struct. Biol.",
volume = 18,
number = 5,
pages = {630--640},
year = 2008
}

@article{ShigeoVis2009,
  title =	"Applying manifold learning to plotting approximate contour trees",
  author =	"Shigeo Takahashi and Issei Fujishiro and Masato Okada",
  publisher =	"IEEE Computer Society",
  journal = {IEEE Transactions on Visualization and Computer Graphics},
  volume = {15},
  number = {6},
  year = {2009},
}
@Article{journals/cgf/TakahashiISKU95,
  title =	"Algorithms for Extracting Correct Critical Points and
		 Constructing Topological Graphs from Discrete
		 Geographical Elevation Data",
  author =	"Shigeo Takahashi and Tetsuya Ikeda and Yoshihisa
		 Shinagawa and Tosiyasu L. Kunii and Minoru Ueda",
  journal =	"Comput. Graph. Forum",
  year = 	"1995",
  number =	"3",
  volume =	"14",
  bibdate =	"2003-11-21",
  bibsource =	"DBLP,
		 http://dblp.uni-trier.de/db/journals/cgf/cgf14.html#TakahashiISKU95",
  pages =	"181--192",
}

 @article{tenenbaum2000,
  title={{A Global Geometric Framework for Nonlinear Dimensionality Reduction}},
  author={J.B. Tenenbaum and V. and Silva and J.C. Langford},
  journal={Science},
  volume={290},
  number={5500},
  pages={2319},
  year={2000}
}

@inproceedings{WWW14,
  title={The {JS}-graph of Join and Split Trees},
  author="Suyi Wang and Yusu Wang and Rephael Wenger",
  booktitle="Proc. 30th Annu. Sympos. Comput. Geom. (SoCG)",
pages = {539--548},
  year={2014}
}

@article{timo:tl,
 author = {Weber, Gunther and Bremer, Peer-Timo and Pascucci, Valerio},
 title = {Topological Landscapes: A Terrain Metaphor for Scientific Data},
 journal = {IEEE Transactions on Visualization and Computer Graphics},
 volume = {13},
 number = {6},
 year = {2007},
 issn = {1077-2626},
 pages = {1416--1423},
 doi = {http://dx.doi.org/10.1109/TVCG.2007.70601},
 publisher = {IEEE Educational Activities Department},
 address = {Piscataway, NJ, USA},
 }

@article{1263272,
 author = {Weber, Gunther H. and Dillard, Scott E. and Carr, Hamish and Pascucci, Valerio and Hamann, Bernd},
 title = {Topology-Controlled Volume Rendering},
 journal = {IEEE Transactions on Visualization and Computer Graphics},
 volume = {13},
 number = {2},
 year = {2007},
 issn = {1077-2626},
 pages = {330--341},
 doi = {http://dx.doi.org/10.1109/TVCG.2007.47},
 publisher = {IEEE Educational Activities Department},
 address = {Piscataway, NJ, USA},
 }

@book{Wenger13
, author = "Rephael Wenger"
, title = "Isosurfaces: Geometry, Topology, and Algorithms"
, year = 2013
, publisher = "CRC Press"
, address = "Boca Raton, Florida"
}

@article{Z03,
author = "R. Zhou",
title = "Trp-case: {F}olding free energy landscape in explicit water",
journal = "Proc. Natl. Acad. Sci.",
volume = 100,
pages = {13280--13285},
year = 2003
}

@article{SOFW07,
        author = "A. Sacan and O. Ozturk and H. Ferhatosmanoglu and Y. Wang",
        title = "{LFM-Pro}: {A} tool for detecting significant local structural sites in proteins",
        journal = "Bioinformatics",
	volume = 23,
	number = 6,
	pages = {709--716},
        year = 2007
}

@article{AEHW06,
        author = "P. K. Agarwal and H. Edelsbrunner and J. Harer and Y. Wang",
        title = "Extreme Elevation on a 2-Manifold",
        journal = "Discrete and Computational Geometry (DCG)",
        volume = 36,
        number = 4,
        pages = {553--572},
        year = "2006"
}

@article{AHSW10,
author = "Pankaj K. Agarwal and Sariel Har-Peled and Micha Sharir and Yusu Wang",
title = "Hausdorff distance under translation for points and balls",
journal = "ACM Transactions on Algorithms",
volume = 6,
number = 4,
year = 2010
}
@Inproceedings{BBW09,
	author = "K. Buchin and M. Buchin and Y. Wang",
	title = "Partial Curve Matching under the Fr\'{e}chet{} Distance",
	booktitle = "Proc. 20th ACM-SIAM Sympos. Discrete Algorithms",
	pages = "645--654",
	year = {2009}
}

@inproceedings{CW13,
  title={Measuring similarity between curves on 2-manifolds via homotopy area},
  author={Dey, Tamal K and Fan, Fengtao and Wang, Yusu},
  booktitle="Proc. 29th Annu. Sympos. Comput. Geom. (SoCG)",
pages = {425--434},
  year={2013}
}

@article{SFOW08,
  author    = {Hong Sun and
               Hakan Ferhatosmanoglu and
               Motonori Ota and
               Yusu Wang},
  title     = {An enhanced partial order curve comparison algorithm and its application to analyzing protein folding trajectories},
  journal   = {BMC Bioinformatics},
  volume    = {9},
  year      = {2008}
}


@inproceedings{BSW08,
author = {Mikhail Belkin and Jian Sun and Yusu Wang},
title = {Discrete laplace operator on meshed surfaces},
booktitle = "Proc. 24th ACM Sympos. on Comput. Geom.",
year = {2008},
pages = {278--287}
}

@inproceedings{BSW09,
	author = "M. Belkin and J. Sun and Y. Wang",
	title = { Constructing {L}aplace Operator from Point Clouds in $\mathbb{R}^d$ },
	booktitle = "Proc. 20th ACM-SIAM Sympos. Discrete Algorithms",
	year = {2009},
	pages = {1031--1040}
}
@inproceedings{DRW10,
author = "T. K. Dey and P. Ranjan and Y. Wang",
title = "Convergence, Stability, and Discrete Approximation of {Laplace} Spectra",
booktitle = "Proc. 21st ACM-SIAM Sympos. Discrete Algorithms",
pages = {650--663},
year = 2010
}
@article{DRW12,
  author    = {Tamal K. Dey and
               Pawas Ranjan and
               Yusu Wang},
  title     = {Eigen deformation of 3D models},
  journal   = {The Visual Computer},
  volume    = {28},
  number    = {6-8},
  year      = {2012},
  pages     = {585-595}
}
@article{LSW09b,
	author = "C. Luo and I. Safa and Y. Wang",
	title = "Approximating Gradients for Meshes and  Point Clouds via Diffusion Metric",
	journal = "Comput. Graphics Forum",
	volume = 28,
	number = 5,
	pages = {1497--1508},
	year = 2009
}
@inproceedings{LSW09,
	author = "C. Luo and J. Sun and Y. Wang",
	title = "Integral estimation from point cloud in $d$-dimensional space: {A} geometric view",
	booktitle = "Proc. 25th ACM Sympos. on Comput. Geom.",
	pages = {116--124},
	year = 2009
}

@article{AMW07,
    author = "P. K. Agarwal and N. Mustafa and Y. Wang",
    title = "Efficient algorithms for contact-map overlap problem",
    journal = "J. Comput. Biology",
    volume = 14,
    number = 2,
    pages = {131--143},
    year = "2007"
}

@article{SSFW12,
author = "H. Sun and A. Sacan and H. Ferhatosmanoglu and Y. Wang",
title = "Smolign: {A} Spatial Motifs Based Multiple Protein Structures Alignment Method",
journal = "IEEE/ACM Trans. Comput. Bio. and Bioinfomatics",
volume = 9,
number = 1,
pages = {249--261},
year = 2012
}

@article{NWBPH06,
        author = "V. Natarajan and Y. Wang and T. Bremer and V. Pascucci and B. Hamann",
        title = "Segmenting Molecular Surfaces",
        journal = "Computer Aided Geometric Design (CAGD)",
        pages = {495--509},
        volumn = 23,
        year = 2006
}

@inproceedings{WABER05,
    author = "Y. Wang and P. K. Agarwal and P. Brown and H. Edelsbrunner and J. Rudolph",
    title = "Coarse and reliable geometric alignment for protein docking",
    booktitle = "Pac. Symp Biocomput",
    pages = {66--77},
    year = 2005
}


@incollection{NKWH07,
	author = "V. Natarajan and P. Koehl and Y. Wang and B. Hamann",
	title = "Visual Analysis of Biomolecular surfaces",
	booktitle = "Mathematical Methods for Visualization in Medicine and Life Science",
	editor = "L. Linsen and H. Hagen and B. Hamann",
	year = "2008",
	pages = "237--256",
	organization = "Mathematics and Visualization",
	publisher = "Springer Verlag"
}






@article{GW07,
  author    = {Leonidas J. Guibas and
               Yusu Wang},
  title     = {Toward Unsupervised Segmentation of Semi-Rigid Low-Resolution Molecular Surfaces},
  journal   = {Algorithmica},
  volume    = {48},
  number    = {4},
  year      = {2007},
  pages     = {433--438}
}

@incollection{harker:mischaikow:mrozek:nanda:wagner:juda:dlotko,
Author = {Harker, S. and Mischaikow, K. and Mrozek, M. and Nanda, V. and Wagner, H. and Juda, M. and Dlotko, P.},
Title = {The Efficiency of a Homology Algorithm based on Discrete Morse Theory and Coreductions},
Booktitle = {Proceedings of the 3rd International Workshop on Computational Topology in Image Context, Chipiona, Spain, November 2010},
Editor = {R. Gonzalez-Diaz and P. Real},
Year = {{2010}},
}

@article{harker:mischaikow:mrozek:nanda,
year={2013},
issn={1615-3375},
journal={Foundations of Computational Mathematics},
doi={10.1007/s10208-013-9145-0},
title={Discrete Morse Theoretic Algorithms for Computing Homology of Complexes and Maps},
url={http://dx.doi.org/10.1007/s10208-013-9145-0},
publisher={Springer-Verlag},
keywords={Computational homology; Discrete Morse theory; 55-04; 55N35; 57-04},
author={Harker, Shaun and Mischaikow, Konstantin and Mrozek, Marian and Nanda, Vidit},
pages={1-34},
language={English}
}

@article {mischaikow:nanda,
    AUTHOR = {Mischaikow, Konstantin and Nanda, Vidit},
     TITLE = {Morse theory for filtrations and efficient computation of
              persistent homology},
   JOURNAL = {Discrete Comput. Geom.},
  FJOURNAL = {Discrete \& Computational Geometry. An International Journal
              of Mathematics and Computer Science},
    VOLUME = {50},
      YEAR = {2013},
    NUMBER = {2},
     PAGES = {330--353},
      ISSN = {0179-5376},
   MRCLASS = {55N35 (57Rxx)},
  MRNUMBER = {3090522},
MRREVIEWER = {Massimo Ferri},
       DOI = {10.1007/s00454-013-9529-6},
       URL = {http://dx.doi.org.proxy.libraries.rutgers.edu/10.1007/s00454-013-9529-6},
}

@ARTICLE{harker:kokubu:mischaikow:pilarczyk,
   author = {{Harker}, S. and {Kokubu}, H. and {Mischaikow}, K. and {Pilarczyk}, P.
	},
    title = "{Inducing a map on homology from a correspondence}",
  journal = {ArXiv e-prints},
archivePrefix = "arXiv",
   eprint = {1411.7563},
 primaryClass = "math.AT",
 keywords = {Mathematics - Algebraic Topology, 55M99, 55-04},
     year = 2014,
    month = nov,
   adsurl = {http://adsabs.harvard.edu/abs/2014arXiv1411.7563H},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}
	@article { mischaikow:wanner:10,
    AUTHOR = {Mischaikow, Konstantin and Wanner, Thomas},
     TITLE = {Topology-guided sampling of nonhomogeneous random processes},
   JOURNAL = {Ann. Appl. Probab.},
  FJOURNAL = {The Annals of Applied Probability},
    VOLUME = {20},
      YEAR = {2010},
    NUMBER = {3},
     PAGES = {1068--1097},
      ISSN = {1050-5164},
   MRCLASS = {60G15 (60G17)},
  MRNUMBER = {2680558 (2011g:60068)},
       DOI = {10.1214/09-AAP652},
       URL = {http://dx.doi.org.proxy.libraries.rutgers.edu/10.1214/09-AAP652},
}

@article{ferry:mischaikow:nanda,
title ="Reconstructing functions from random samples",
journal ="Journal of Computational Dynamics",
volume ="1",
number ="2",
pages ="233-248",
year ="2014",
note =" ",
issn ="2158-2491",
doi ="10.3934/jcd.2014.1.233",
url ="http://aimsciences.org/journals/displayArticlesnew.jsp?paperID=10624",
author ="Steve  Ferry and Konstantin  Mischaikow and Vidit  Nanda",
keywords ="Homology",
keywords ="homotopy",
keywords ="nonlinear maps",
keywords ="topological inference",
}
@article {day:kalies:mischaikow:wanner,
    AUTHOR = {Day, Sarah and Kalies, William D. and Mischaikow, Konstantin
              and Wanner, Thomas},
     TITLE = {Probabilistic and numerical validation of homology
              computations for nodal domains},
   JOURNAL = {Electron. Res. Announc. Amer. Math. Soc.},
  FJOURNAL = {Electronic Research Announcements of the American Mathematical
              Society},
    VOLUME = {13},
      YEAR = {2007},
     PAGES = {60--73 (electronic)},
      ISSN = {1079-6762},
   MRCLASS = {65C99 (60G99)},
  MRNUMBER = {2320683 (2009b:65015)},
MRREVIEWER = {Volker Wihstutz},
       DOI = {10.1090/S1079-6762-07-00175-8},
       URL = {http://dx.doi.org.proxy.libraries.rutgers.edu/10.1090/S1079-6762-07-00175-8},
}

@article{ jaquette:kramar,
Author = {Jaquette, J. and Kramar, M.},
Title = {Rigorous Computation of Persistent Homology},
Journal = {{preprint}},
Year = {{2014}},
}
@article {kalies:mischaikow:vandervorst:14,
    AUTHOR = {Kalies, William and Mischaikow, Konstantin and Vandervorst Robert},
     TITLE = {Lattice Structures for Attractors {I}},
   JOURNAL = {Journal of Computational Dynamics},
  FJOURNAL = {Journal of Computational Dynamics},
    VOLUME = {1},
      YEAR = {2014},
    NUMBER = {2},
}
@ARTICLE{kalies:mischaikow:vandervorst:15,
   author = {{Kalies}, W.~D. and {Mischaikow}, K. and {Vandervorst}, R.~C.~A.~M.
	},
    title = "{Lattice Structures for Attractors {II}}",
  journal = {Found. Comput. Math.},
     year = 2015,
}

@article {arai:kalies:kokubu:mischaikow:oka:pilarczyk,
    AUTHOR = {Arai, Zin and Kalies, William and Kokubu, Hiroshi and
              Mischaikow, Konstantin and Oka, Hiroe and Pilarczyk, Pawe{\l}},
     TITLE = {A database schema for the analysis of global dynamics of
              multiparameter systems},
   JOURNAL = {SIAM J. Appl. Dyn. Syst.},
  FJOURNAL = {SIAM Journal on Applied Dynamical Systems},
    VOLUME = {8},
      YEAR = {2009},
    NUMBER = {3},
     PAGES = {757--789},
      ISSN = {1536-0040},
   MRCLASS = {37B35 (37N25 92-08)},
  MRNUMBER = {2533624 (2011c:37034)},
       DOI = {10.1137/080734935},
       URL = {http://dx.doi.org.proxy.libraries.rutgers.edu/10.1137/080734935},
}

@article{bush:gameiro:harker:kokubu:mischaikow:obayashi:pilarczyk,
Author = {Bush, Justin and Gameiro, Marcio and Harker, Shaun and Kokubu, Hiroshi
   and Mischaikow, Konstantin and Obayashi, Ippei and  Pilarczyk, Pawel },
Title = {{Combinatorial-topological framework for the analysis of global dynamics}},
Journal = {{CHAOS}},
Year = {{2012}},
Volume = {{22}},
Number = {{4}},
Month = {{DEC}},
Publisher = {{AMER INST PHYSICS}},
Type = {{Article}}
}

@article {arai:gameiro:gedeon:kokubu:mischaikow:oka,
AUTHOR = {Arai, Z. and Gameiro, M. and Gedeon, T. and Kokubu, H. and Mischaikow, K. and Oka, H.},
TITLE = {Graph-based topological approximation of saddle-node bifurcation in maps},
   JOURNAL = {RIMS Kokyuroku Beassatsu},
    VOLUME = {B31},
      YEAR = {2012},
    NUMBER = {},
PAGES = {225-241},
}

@article{newton,
Author = {Harker, S. and Bush, J and  Cowan, W. and Mischaikow, K.},
Title = {Conley-Morse Databases for the Angular Dynamics of Newton's Method on the Plane},
Journal = {{preprint}},
Year = {{2015}},
}

@article{sigmoidal,
Author = {Gedeon, T. and Harker, S.  and Kokubu, H. and Mischaikow, K. and Oka, H.},
Title = {Global Dynamics for Steep Sigmoidal Nonlinearities in Two Dimensions},
Journal = {{preprint}},
Year = {{2015}},
}

@article{ bush:mischaikow,
Author = {Bush, Justin and Mischaikow},
ISSN = {},
Journal = {Entropy},
Number = {},
Pages = {},
Title = {Combinatorial-topological framework for the analysis of global dynamics.},
Volume = {accepted},
Year = {2014},
}

@article {berg:lessard:mischaikow,
    AUTHOR = {van den Berg, Jan Bouwe and Lessard, Jean-Philippe and
              Mischaikow, Konstantin},
     TITLE = {Global smooth solution curves using rigorous branch following},
   JOURNAL = {Math. Comp.},
  FJOURNAL = {Mathematics of Computation},
    VOLUME = {79},
      YEAR = {2010},
    NUMBER = {271},
     PAGES = {1565--1584},
      ISSN = {0025-5718},
     CODEN = {MCMPAF},
   MRCLASS = {65Q20 (37M20)},
  MRNUMBER = {2630003 (2011i:65246)},
MRREVIEWER = {Brian L. Burrows},
       DOI = {10.1090/S0025-5718-10-02325-2},
       URL = {http://dx.doi.org.proxy.libraries.rutgers.edu/10.1090/S0025-5718-10-02325-2},
}

@article { berg:mirelesjames:lessard:mischaikow,
    AUTHOR = {van den Berg, Jan Bouwe and Mireles-James, Jason D. and
              Lessard, Jean-Philippe and Mischaikow, Konstantin},
     TITLE = {Rigorous numerics for symmetric connecting orbits: even
              homoclinics of the {G}ray-{S}cott equation},
   JOURNAL = {SIAM J. Math. Anal.},
  FJOURNAL = {SIAM Journal on Mathematical Analysis},
    VOLUME = {43},
      YEAR = {2011},
    NUMBER = {4},
     PAGES = {1557--1594},
      ISSN = {0036-1410},
     CODEN = {SJMAAH},
   MRCLASS = {34C37 (34C45 65P40)},
  MRNUMBER = {2821596 (2012g:34109)},
MRREVIEWER = {Jean Moulin-Ollagnier},
       DOI = {10.1137/100812008},
       URL = {http://dx.doi.org.proxy.libraries.rutgers.edu/10.1137/100812008},
}

@article{mirelesjames:mischaikow,
author={Mireles James,J.D. and Mischaikow,Konstantin},
year={2013},
title={Rigorous A Posteriori Computation of (Un)Stable Manifolds and Connecting Orbits for Analytic Maps},
journal={SIAM Journal on Applied Dynamical Systems},
volume={12},
number={2},
pages={957-1006}
}
@article{ode,
Author = {Gameiro, M. and  Kokubu, H. and  Mischaikow, K. and  Miyaji, T. and Pilarczyk, P.},
Title = {A study of rigorous ODE integrators for multi-scale set-oriented computations},
Journal = {{preprint}},
Year = {{2015}},
}
@article{mischaikow:mrozek:weilandt,
Author = {Mischaikow, K. and   Mrozek, M. and  Weilandt, F.},
Title = {Discrectization Strategies for Computing Conley Indices and Morse Decompositions of Flows},
Journal = {{preprint}},
Year = {{2015}},
}
@article{nature,
   AUTHOR = { Taylor, Dane and Klimm, Florian and Harrington, Heather A. and Kramar, Miroslav and Mischaikow, Konstantin and Porter, Mason A. and Mucha, Peter J.},
     TITLE = {Topological data analysis of contagion maps for examining spreading processes on networks},
   JOURNAL = {Nat Commun},
    VOLUME = {6},
      YEAR = {2015},
       URL = {http://dx.doi.org/10.1038/ncomms8723},
}
@article { protein,
    AUTHOR = {Gameiro, Marcio and Hiraoka, Yasuaki and Izumi, Shunsuke and
              Kramar, Miroslav and Mischaikow, Konstantin and Nanda, Vidit},
     TITLE = {A topological measurement of protein compressibility},
   JOURNAL = {Jpn. J. Ind. Appl. Math.},
  FJOURNAL = {Japan Journal of Industrial and Applied Mathematics},
    VOLUME = {32},
      YEAR = {2015},
    NUMBER = {1},
     PAGES = {1--17},
      ISSN = {0916-7005},
   MRCLASS = {92D20 (55N35 92E10)},
  MRNUMBER = {3318898},
       DOI = {10.1007/s13160-014-0153-5},
       URL = {http://dx.doi.org.proxy.libraries.rutgers.edu/10.1007/s13160-014-0153-5},
}
@article{epl12,
Author = {Kondic, L. and Goullet, A. and O'Hern, C. S. and Kramar, M. and
   Mischaikow, K. and Behringer, R. P.},
Title = {{Topology of force networks in compressed granular media}},
Journal = {{EPL}},
Year = {{2012}},
Volume = {{97}},
Number = {{5}},
Month = {{MAR}},
DOI = {{10.1209/0295-5075/97/54001}},
Article-Number = {{54001}},
ISSN = {{0295-5075}},
ResearcherID-Numbers = {{O'Hern, Corey/I-3459-2014}},
ORCID-Numbers = {{O'Hern, Corey/0000-0002-8272-5640}},
Unique-ID = {{ISI:000301952600014}},
}
@article{pre13,
Author = {Kramar, M. and Goullet, A. and Kondic, L. and Mischaikow, K.},
Title = {{Persistence of force networks in compressed granular media}},
Journal = {{PHYSICAL REVIEW E}},
Year = {{2013}},
Volume = {{87}},
Number = {{4}},
Month = {{APR 22}},
DOI = {{10.1103/PhysRevE.87.042207}},
Article-Number = {{042207}},
ISSN = {{1539-3755}},
Unique-ID = {{ISI:000317867300006}},
}

@article{pre14,
Author = {Kramar, Miroslav and Goullet, Arnaud and Kondic, Lou and Mischaikow,
   Konstantin},
Title = {{Evolution of force networks in dense particulate media}},
Journal = {{PHYSICAL REVIEW E}},
Year = {{2014}},
Volume = {{90}},
Number = {{5}},
Month = {{NOV 10}},
DOI = {{10.1103/PhysRevE.90.052203}},
Article-Number = {{052203}},
ISSN = {{1539-3755}},
EISSN = {{1550-2376}},
Unique-ID = {{ISI:000344918100004}},
}

@article{physicaD14,
Author = {Kramar, Miroslav and Goullet, Arnaud and Kondic, Lou and Mischaikow,
   Konstantin},
Title = {{Quantifying force networks in particulate systems}},
Journal = {{PHYSICA D-NONLINEAR PHENOMENA}},
Year = {{2014}},
Volume = {{283}},
Pages = {{37-55}},
Month = {{AUG 15}},
DOI = {{10.1016/j.physd.2014.05.009}},
ISSN = {{0167-2789}},
EISSN = {{1872-8022}},
Unique-ID = {{ISI:000340322100005}},
}

@ARTICLE{fluidP,
   author = {{Kramar}, M. and {Levanger}, R. and {Tithof}, J. and {Suri}, B. and
	{Xu}, M. and {Paul}, M. and {Schatz}, M.~F. and {Mischaikow}, K.
	},
    title = "{Analysis of Kolmogorov Flow and Rayleigh-B$\backslash$'enard Convection using Persistent Homology}",
  journal = {ArXiv e-prints},
archivePrefix = "arXiv",
   eprint = {1505.06168},
 primaryClass = "math.AT",
 keywords = {Mathematics - Algebraic Topology, Mathematics - Dynamical Systems, Physics - Fluid Dynamics},
     year = 2015,
    month = may,
   adsurl = {http://adsabs.harvard.edu/abs/2015arXiv150506168K},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@incollection {mischaikow:mrozek,
    AUTHOR = {Mischaikow, Konstantin and Mrozek, Marian},
     TITLE = {Conley index},
 BOOKTITLE = {Handbook of dynamical systems, {V}ol. 2},
     PAGES = {393--460},
 PUBLISHER = {North-Holland},
   ADDRESS = {Amsterdam},
      YEAR = {2002},
   MRCLASS = {37B30 (37C05 37C10 55M25)},
  MRNUMBER = {1901060 (2003g:37022)},
MRREVIEWER = {Octavian Cornea},
       DOI = {10.1016/S1874-575X(02)80030-3},
       URL = {http://dx.doi.org.proxy.libraries.rutgers.edu/10.1016/S1874-575X(02)80030-3},
}
@article {kalies:mischaikow:vandervorst:05,
    AUTHOR = {Kalies, W. D. and Mischaikow, K. and VanderVorst, R. C. A. M.},
     TITLE = {An algorithmic approach to chain recurrence},
   JOURNAL = {Found. Comput. Math.},
  FJOURNAL = {Foundations of Computational Mathematics. The Journal of the
              Society for the Foundations of Computational Mathematics},
    VOLUME = {5},
      YEAR = {2005},
    NUMBER = {4},
     PAGES = {409--449},
      ISSN = {1615-3375},
   MRCLASS = {37B35 (37B20 37B25 37B30 37C70 37M99)},
  MRNUMBER = {MR2189545 (2006i:37035)},
MRREVIEWER = {James S. Wiseman},
}

@book{kaczynski:mischaikow:mrozek:04,
    AUTHOR = {Kaczynski, Tomasz and Mischaikow, Konstantin and Mrozek,
              Marian},
     TITLE = {Computational Homology},
    SERIES = {Applied Mathematical Sciences},
    VOLUME = {157},
 PUBLISHER = {Springer-Verlag},
   ADDRESS = {New York},
      YEAR = {2004},
     PAGES = {xviii+480},
      ISBN = {0-387-40853-3},
   MRCLASS = {55-02 (37B30 55M20 55M25 68U10 94A08)},
  MRNUMBER = {2028588 (2005g:55001)},
MRREVIEWER = {Andrzej Kozlowski},
}

@article{BWang:2007d,
   AUTHOR = { Wang, B.  and Westerhoff, L. M. and    Merz Jr, K. M.},
     TITLE = {A Critical Assessment of the Performance of Protein-ligand Scoring Functions Based on NMR Chemical Shift Perturbations},
   JOURNAL = {J. Med. Chem.},
    VOLUME = {50},
      YEAR = {2007},
		PAGES = {5128 -5134}
}



@article{XHe:2009,
   AUTHOR = { He, X.  and  Wang, B.    and Merz Jr, K. M.},
     TITLE = {Protein NMR Chemical Shift Calculations Based on the Automated Fragmentation QM/MM Approach},
   JOURNAL = {  J. Phys. Chem. B.},
    VOLUME = {113},
      YEAR = {2009},
		PAGES = {10380-10388}
}


@article{Williams:2009,
   AUTHOR = {Williams, D. E.  and  Peters. M. B.  and  Wang, B.  and Roitberg, A. E.   and  Merz Jr, K. M.},
     TITLE = {AM1 parameters for the Prediction of 1H and 13C NMR Chemical Shifts in Proteins},
   JOURNAL = {  J. Phys. Chem. A.},
    VOLUME = {113},
      YEAR = {2009},
		PAGES = {11550-11559}
}

@article{Chakravorty:2013,
   AUTHOR = { Chakravorty, D. K.  and   Wang, B. and  Lee, C. W.  and Guerro, A. J.  and  Giedroc, D. P.  and Merz Jr, K. M.},
     TITLE = {Solution NMR refinement of a metal ion bound protein using metal ion inclusive restrained molecular dynamics methods},
   JOURNAL = { J. Biol. NMR},
    VOLUME = {56},
      YEAR = {2013},
		PAGES = {125-137}
}

@article{ZZheng:2013,
   AUTHOR = { Zheng, Z.  and Merz Jr, K. M.},
     TITLE = {Development of the Knowledge-based \& Empirical Combined Scoring Algorithm (KECSA) to Score Protein-Ligand Interactions},
   JOURNAL = {  J. Chem. Inf. Model.},
    VOLUME = {53},
      YEAR = {2013},
		PAGES = {1073-1083}
}

@article{BWang:2013d,
   AUTHOR = {Wang, B. and  He, X. and    Merz Jr, K. M.},
     TITLE = {A Quantum Mechanical Study of Vicinal J Spin-Spin Coupling Constants for the Protein Backbone},
   JOURNAL = { J. Chem. Theory and Comput.},
    VOLUME = {9},
      YEAR = {2013},
		PAGES = {4653-4659}
}

@article{ZZheng:2013d,
   AUTHOR = { Zheng, Z.  and   Ucisik,  M. N. and    Merz Jr, K. M.},
     TITLE = {The Movable Type Method Applied to Protein-Ligand Binding},
   JOURNAL = { J. Chem. Theory and Comput.},
    VOLUME = {9},
      YEAR = {2013},
		PAGES = {5526-5538}
}

	
@article{PLi:2013d,
   AUTHOR = { Li, P.  and Roberts,  B. P. and Chakravorty, D. K.  and   Merz Jr, K. M.},
     TITLE = {Rational Design of Particle Mesh Ewald Compatible Lennard-Jones Parameters for +2 Metal Cations in Explicit Solvent},
   JOURNAL = { J. Chem. Theory and Comput.},
    VOLUME = {9},
      YEAR = {2013},
		PAGES = {2733-2748}
}
	

@article{YMiao:2013d,
   AUTHOR = { Miao, Y. and    Merz Jr, K. M.},
     TITLE = {Acceleration of Electron Repulsion Integral Evaluation on Graphics Processing Units via Use of Recurrence Relations},
   JOURNAL = { J. Chem. Theory and Comput.},
    VOLUME = {9},
      YEAR = {2013},
		PAGES = {965-976}
}
	


@article{Merz:1989,
   AUTHOR = {    Merz Jr, K. M. and  Kollman,  Peter A.},
     TITLE = {Free energy perturbation simulations of the inhibition of thermolysin: prediction of the free energy of binding of a new inhibitor},
   JOURNAL = { J. Am. Chem. Soc.},
    VOLUME = {111},
      YEAR = {1989},
		PAGES = {5649-5658}
}


@article{BWang:2005d,
   AUTHOR = {Wang, B.  and  Merz Jr, K. M.},
     TITLE = {Validation of the Binding Site Structure of the Cellular Retinol-Binding Protein (CRBP) by Ligand NMR Chemical Shift Perturbations},
   JOURNAL = { J. Am. Chem. Soc.},
    VOLUME = {127},
      YEAR = {2005},
		PAGES = {5310-5311}
}

@article{Perea:2015a,
   AUTHOR = {Perea, J. A. and   Harer, J.},
     TITLE = {Sliding windows and persistence: An application of topological methods to signal analysis},
   JOURNAL = { Foundations of Computational Mathematics},
    VOLUME = {15},
      YEAR = {2015},
		PAGES = {799-838}
}

 @article{Perea:2015b,
   AUTHOR = {Perea, J. A. and Deckard, A. and  Haase, S. B. and   Harer, J.},
     TITLE = {SW1PerS: Sliding windows and 1-persistence scoring; discovering periodicity in gene expression time series data},
   JOURNAL = {BMC Bioinformatics},
    VOLUME = {16},
      YEAR = {2015},
		PAGES = {257}
}

	
 @article{Perea:2014,
   AUTHOR = {Perea, J. A. and    Carlsson, G.},
     TITLE = {A Klein-bottle-based dictionary for texture representation},
   JOURNAL = {International journal of computer vision},
    VOLUME = {107},
      YEAR = {2014},
		PAGES = {75-97}
}	


@article {Mischaikow:2002A,
AUTHOR = {Mischaikow, Konstantin},
TITLE = {Topological techniques for efficient rigorous
computation in
dynamics},
JOURNAL = {Acta Numer.},
FJOURNAL = {Acta Numerica},
VOLUME = {11},
YEAR = {2002},
PAGES = {435--477},
ISSN = {0962-4929},
MRCLASS = {37M99 (37B30)},
MRNUMBER = {2009377 (2004k:37184)},
MRREVIEWER = {Gary Froyland},
DOI = {10.1017/S0962492902000065},
URL = {http://dx.doi.org.proxy.libraries.rutgers.edu/
10.1017/S0962492902000065},
}
@article{Gameiro:2005b,
Author = {Gameiro, M and Mischaikow, K and Wanner, T},
Title = {{Evolution of pattern complexity in the Cahn-Hilliard
theory of phase
separation}},
Journal = {{ACTA MATERIALIA}},
Year = {{2005}},
Volume = {{53}},
Number = {{3}},
Pages = {{693-704}},
Month = {{FEB}},
DOI = {{10.1016/j.actamat.2004.10.022}},
ISSN = {{1359-6454}},
ResearcherID-Numbers = {{Gameiro, Marcio/F-1786-2011}},
Unique-ID = {{ISI:000226711600014}},
}
@article{Wilson:2009c,
Author = {Wilson, James R. and Gameiro, Marcio and Mischaikow,
Konstantin and
Kalies, William and Voorhees, Peter W. and Barnett, Scott
A.},
Title = {{Three-Dimensional Analysis of Solid Oxide Fuel Cell
Ni-YSZ Anode
Interconnectivity}},
Journal = {{MICROSCOPY AND MICROANALYSIS}},
Year = {{2009}},
Volume = {{15}},
Number = {{1}},
Pages = {{71-77}},
Month = {{FEB}},
DOI = {{10.1017/S1431927609090096}},
ISSN = {{1431-9276}},
ResearcherID-Numbers = {{Voorhees, Peter /B-6700-2009
Barnett, Scott/B-7502-2009
Gameiro, Marcio/F-1786-2011}},
Unique-ID = {{ISI:000262912700010}},
}
@article{Niethammer:2006d,
Author = {Niethammer, Marc and Kalies, William D. and
Mischaikow, Konstantin and
Tannenbaum, Allen},
Title = {{On the detection of simple points in higher dimensions
using cubical
homology}},
Journal = {{IEEE TRANSACTIONS ON IMAGE PROCESSING}},
Year = {{2006}},
Volume = {{15}},
Number = {{8}},
Pages = {{2462-2469}},
Month = {{AUG}},
DOI = {{10.1109/TIP.2006.877309}},
ISSN = {{1057-7149}},
Unique-ID = {{ISI:000239286900033}},
}
@article{Szymczak:2006e,
Author = {Szymczak, Andrzej and Stillman, Arthur and Tannenbaum,
Allen and
Mischaikow, Konstantin},
Title = {{Coronary vessel trees from 3D imagery: A topological
approach}},
Journal = {{MEDICAL IMAGE ANALYSIS}},
Year = {{2006}},
Volume = {{10}},
Number = {{4}},
Pages = {{548-559}},
Month = {{AUG}},
DOI = {{10.1016/j.media.2006.05.002}},
ISSN = {{1361-8415}},
Unique-ID = {{ISI:000240088500005}},
}
@inproceedings{Szymczak:2005f,
Author = {Szymczak, A and Tannenbaum, A and Mischaikow, K},
Editor = {{Fitzpatrick, JM and Reinhardt, JM}},
Title = {{Coronary vessel cores from 3D imagery: a topological
approach}},
Booktitle = {{Medical Imaging 2005: Image Processing, Pt 1-3}},
Series = {{PROCEEDINGS OF THE SOCIETY OF PHOTO-OPTICAL
INSTRUMENTATION ENGINEERS
(SPIE)}},
Year = {{2005}},
Volume = {{5747}},
Number = {{1-3}},
Pages = {{505-513}},
Note = {{Medical Imaging 2005 Conference, San Diego, CA, FEB
15-17, 2005}},
Organization = {{SPIE}},
DOI = {{10.1117/12.593837}},
ISSN = {{0277-786X}},
ISBN = {{0-8194-5721-3}},
Unique-ID = {{ISI:000230109600051}},
}
@inproceedings{Niethammer:2002g,
Author = {Niethammer, M and Stein, AN and Kalies, WD and
Pilarczyk, P and
Mischaikow, K and Tannenbaum, T},
Book-Group-Author = {{IEEE
IEEE}},
Title = {{Analysis of blood vessel topology by cubical
homology}},
Booktitle = {{2002 INTERNATIONAL CONFERENCE ON IMAGE PROCESSING,
VOL II, PROCEEDINGS}},
Year = {{2002}},
Pages = {{969-972}},
Note = {{IEEE International Conference on Image Processing,
ROCHESTER, NY, SEP
22-25, 2002}},
Organization = {{IEEE Signal Proc Soc}},
ISBN = {{0-7803-7622-6}},
Unique-ID = {{ISI:000185284000243}},
}
@inproceedings{Allili:2001h,
Author = {Allili, M and Mischaikow, K and Tannenbaum, A},
Book-Group-Author = {{IEEE
IEEE}},
Title = {{Cubical homology and the topological classification of
2D and 3D imagery}},
Booktitle = {{2001 INTERNATIONAL CONFERENCE ON IMAGE PROCESSING,
VOL II, PROCEEDINGS}},
Year = {{2001}},
Pages = {{173-176}},
Note = {{International Conference on Image Processing (ICIP
2001), THESSALONIKI,
GREECE, OCT 07-10, 2001}},
Organization = {{IEEE Signal Processing Soc; IEEE}},
ISBN = {{0-7803-6725-1}},
Unique-ID = {{ISI:000178044600045}},
}
@article{GChen:2008i,
Author = {Chen, Guoning and Mischaikow, Konstantin and Laramee,
Robert S. and
Zhang, Eugene},
Title = {{Efficient morse decompositions of vector fields}},
Journal = {{IEEE TRANSACTIONS ON VISUALIZATION AND COMPUTER
GRAPHICS}},
Year = {{2008}},
Volume = {{14}},
Number = {{4}},
Pages = {{848-862}},
Month = {{JUL-AUG}},
Note = {{9th Eurographics/IEEE VGTC Symposium on Visualization
(EuroVis `07),
Norrkoping, SWEDEN, MAY 23-25, 2007}},
DOI = {{10.1109/TVCG.2008.33}},
ISSN = {{1077-2626}},
Unique-ID = {{ISI:000255550600011}},
}
@article{GChen:2007j,
Author = {Chen, Guoning and Mischaikow, Konstantin and Laramee,
Robert S. and
Pilarczyk, Pawel and Zhang, Eugene},
Title = {{Vector field editing and periodic orbit extraction
using morse
decomposition}},
Journal = {{IEEE TRANSACTIONS ON VISUALIZATION AND COMPUTER
GRAPHICS}},
Year = {{2007}},
Volume = {{13}},
Number = {{4}},
Pages = {{769-785}},
Month = {{JUL-AUG}},
DOI = {{10.1109/TVCG.2007.1021}},
ISSN = {{1077-2626}},
Unique-ID = {{ISI:000247006000012}},
}
@article{EZhang:2006k,
Author = {Zhang, Eugene and Mischaikow, Konstantin and Turk,
Greg},
Title = {{Vector field design on surfaces}},
Journal = {{ACM TRANSACTIONS ON GRAPHICS}},
Year = {{2006}},
Volume = {{25}},
Number = {{4}},
Pages = {{1294-1326}},
Month = {{OCT}},
DOI = {{10.1145/1183287.1183290}},
ISSN = {{0730-0301}},
Unique-ID = {{ISI:000242553200003}},
}
@article{EZhang:2005l,
Author = {Zhang, E and Mischaikow, K and Turk, G},
Title = {{Feature-based surface parameterization and texture
mapping}},
Journal = {{ACM TRANSACTIONS ON GRAPHICS}},
Year = {{2005}},
Volume = {{24}},
Number = {{1}},
Pages = {{1-27}},
Month = {{JAN}},
DOI = {{10.1145/1037957.1037958}},
ISSN = {{0730-0301}},
Unique-ID = {{ISI:000225794000001}},
}

@article{Mischaikow:2007m,
Author = {Mischaikow, Konstantin and Wanner, Thomas},
Title = {{Probabilistic validation of homology computations for
nodal domains}},
Journal = {{ANNALS OF APPLIED PROBABILITY}},
Year = {{2007}},
Volume = {{17}},
Number = {{3}},
Pages = {{980-1018}},
Month = {{JUN}},
DOI = {{10.1214/105051607000000050}},
ISSN = {{1050-5164}},
Unique-ID = {{ISI:000247124100007}},
}





@article{Rader:2006,
  title={The {G}aussian network model: Theory and applications},
  author={Rader, A. J. and Chennubhotla, C. and Yang, L. W. and Bahar, I. and Cui, Q.},
  journal={Normal mode analysis: Theory and applications to biological and chemical systems},
  volume={9},
  pages={41--64},
  year={2006},
  publisher={Chapman \& Hall/CRC: Boca Raton, FL}
}


@article{Riccardi:2009,
  title={Application of elastic network models to proteins in the crystalline state},
  author={Riccardi, D. and Cui, Q. and Phillips, G. N.},
  journal={Biophysical journal},
  volume={96},
  number={2},
  pages={464--475},
  year={2009},
  publisher={Elsevier}
}


@article{Kundu:2004,
  title={Automatic domain decomposition of proteins by a {Gaussian} network model},
  author={Kundu, S. and Sorensen, D. C. and Phillips,  G. N. Jr.},
  journal={Proteins: Structure, Function, and Bioinformatics},
  volume={57},
  number={4},
  pages={725--733},
  year={2004},
  publisher={Wiley Online Library}
}

@article{Uyar:2014,
  title={Features of Large Hinge-Bending Conformational Transitions. Prediction of Closed Structure from Open State},
  author={Uyar, A. and Kantarci-Carsibasi, N. and Haliloglu, T. and Doruker, P.},
  journal={Biophysical Journal},
  volume={106},
  number={12},
  pages={2656--2666},
  year={2014},
  publisher={Elsevier}
}

@article{HYLi:2013,
  title={Analysis of Conformational Motions and Residue Fluctuations for Escherichia coli Ribose-Binding Protein Revealed with Elastic Network Models},
  author={Li, H. Y. and Cao, Z. X. and Zhao, L. L. and Wang, J. H.},
  journal={International Journal of Molecular Sciences},
  volume={14},
  number={5},
  pages={10552--10569},
  year={2013},
  publisher={Multidisciplinary Digital Publishing Institute}
}

	
@article{Leeetal:2009,
  title={Two Separate Interfaces between the Voltage
Sensor and Pore Are Required for the Function
of Voltage-Dependent {K$^+$ } Channels},
  author={Seok-Yong Lee and Anirban Banerjee and  Roderick MacKinnon},
  journal={Plos Biology},
  volume={7},
  number={5},
  pages={e1000047},
  year={2009},
  publisher={ }
}

@article{Fro90,
author= "Patrizio Frosini",
title = "A distance for similarity classes of submanifolds of a {Euclidean} space",
journal = "BUllentin of Australian Mathematical Society",
volume = 42,
number = 3,
pages = {407--416},
year = 1990
}
@article{BH11,
author = "Paul Bendich and John Harer",
title = "Persistent Intersection Homology",
journal = "Foundations of Computational Mathematics (FOCM)",
volume = 11,
number = 3,
year = 2011,
pages = {305--336},
}
@article{CEH09,
  author    = {David Cohen-Steiner and
               Herbert Edelsbrunner and
               John Harer},
  title     = {Extending Persistence Using Poincar{\'e} and Lefschetz
               Duality},
  journal   = {Foundations of Computational Mathematics},
  volume    = {9},
  number    = {1},
  year      = {2009},
  pages     = {79-103}
}

@article{CEH07,
  author    = {Cohen-Steiner D. and
               Edelsbrunner H.and
               Harer J.},
  title     = {Stability of Persistence Diagrams},
  journal   = {Discrete {\&} Computational Geometry},
  volume    = {37},
  number    = {1},
  year      = {2007},
  pages     = {103--120}
}

@inproceedings{CEHM09,
 author = {Cohen-Steiner, David and Edelsbrunner, Herbert and Harer, John and Morozov, Dmitriy},
 title = {Persistent Homology for Kernels, Images, and Cokernels},
 booktitle = {Proceedings of the Twentieth Annual ACM-SIAM Symposium on Discrete Algorithms},
 series = {SODA 09},
 year = {2009},
 pages = {1011--1020},
}

@article{cohen2010:lipschitz,
  title={Lipschitz functions have $L_p$-stable persistence},
  author={Cohen-Steiner, D. and Edelsbrunner, H. and Harer, J. and Mileyko, Y.},
  journal={Foundations of computational mathematics},
  volume={10},
  number={2},
  pages={127--139},
  year={2010},
  publisher={Springer}
}

@inproceedings{CCG09,
	author = "Fr{\'e}d{\'e}ric Chazal and David Cohen-Steiner and Marc Glisse and Leonidas J. Guibas and Steve Oudot",
	title = "Proximity of persistence modules and their diagrams",
	booktitle = "Proc. 25th ACM Sympos. on Comput. Geom.",
	pages = {237--246},
	year = 2009
}
@inproceedings{CGOS11,
 author = {Chazal, Fr{\'e}d{\'e}ric and Guibas, Leonidas J. and Oudot, Steve Y. and Skraba, Primoz},
 title = {Persistence-based clustering in riemannian manifolds},
 booktitle = {Proceedings of the 27th annual ACM symposium on Computational geometry},
 series = {SoCG '11},
 year = {2011},
 pages = {97--106},
}

@inproceedings{CSM09,
  author    = {Gunnar Carlsson and
               Vin de Silva and
               Dmitriy Morozov},
  title     = {Zigzag persistent homology and real-valued functions},
  booktitle = {Proc. 25th Annu. ACM Sympos. Comput. Geom.},
  year      = {2009},
  pages     = {247--256}
}


@article{SMV11,
author = {de Silva, V. and Morozov, D. and  Vejdemo-Johansson, M. },
  title     = {Persistent cohomology and circular coordinates},
journal = {Discrete and Comput. Geom.},
volume = 45,
pages = {737--759},
year = 2011
}

@article{zigzag,
  title={Zigzag persistence},
  author={Carlsson, Gunnar and De Silva, Vin},
  journal={Foundations of computational mathematics},
  volume={10},
  number={4},
  pages={367--405},
  year={2010},
  publisher={Springer-Verlag}
}

@inproceedings{OS13
, author = "Steve Y. Oudot and Donald R. Sheehy"
, title =  "{Z}igzag {Z}oology: {R}ips {Z}igzags for {H}omology {I}nference"
, booktitle = "Proc. 29th Annual Symposium on Computational Geometry"
, pages = "387--396"
, month = "June"
, year = "2013"
}

@article{CZOG05,
  title = "Persistence Barcodes for Shapes",
  author = "Carlsson, G. and Zomorodian, A. and Collins, A. and Guibas, L. J.",
  journal = "International Journal of Shape Modeling",
  year = 2005,
  volume = 11,
  number = 2,
  pages = "149--187",
 }
@misc{DFW13c,
author = "T. K. Dey and F. Fan and Y. Wang",
title = "Dimension detection with local homology",
note = "manuscript",
year = 2013
}
@inproceedings{DFW14,
  title={Computing topological persistence for simplicial maps},
  author={Dey, Tamal K and Fan, Fengtao and Wang, Yusu},
  booktitle="Proc. 30th Annu. Sympos. Comput. Geom. (SoCG)",
pages = {345--354},
  year={2014}
}

@inproceedings{AMR15,
author = "P. K. Agarwal and T. Molhave and M. Revsboek and I. Safa and Y. Wang and J. Yang",
title = "Maintaining contour trees of dynamic terrains",
booktitle = "Proc. 31rd Annu. Sympos. Comput. Geom. (SoCG)",
pages = "796--811",
year = 2015
}
@article{DL10,
author = "T. K. Dey and K. Li and C. Luo and P. Ranjan and I. Safa and Y. Wang",
title = "Persistent heat signature for pose-oblivious matching of incomplete models",
journal = "Comput. Graph. Forum. (special issue from {\em Sympos. Geom. Process.})",
volume = 29,
number = 5,
pages = "1545--1554",
year = 2010
}
@article{DFW13b,
  author    = {Tamal K. Dey and
               Fengtao Fan and
               Yusu Wang},
  title     = {An efficient computation of handle and tunnel loops via
               Reeb graphs},
  journal   = {ACM Trans. Graph.},
  volume    = {32},
  number    = {4},
  year      = {2013},
  pages     = {32},
}



@inproceedings{WWL15,
author = "Suyi Wang and Yusu Wang and Yanjie Li",
title = "Efficient map reconstruction and augmentation via topological methods",
booktitle = "23rd ACM SIGSPATIAL Intl. Conf. Adv. Geographic Info. Sys.",
note = "To appear",
year = 2015
}

@article{DMW15,
author = "Tamal Dey and Facundo M\'{e}moli and Yusu Wang",
title = "Multiscale mapper: {A} framework for topological summarization of data and maps",
journal = {arXiv:1504.03763},
year = 2015
}

@INPROCEEDINGS{mapper,
  author = {Gurjeet Singh and  M{\'e}moli, Facundo and Gunnar Carlsson },
  title = {{Topological Methods for the Analysis of High Dimensional Data Sets
	and 3D Object Recognition}},
  pages = {91-100},
booktitle = {Sympos. Point Based Graphics},
year = 2007
}
@article {Sousbie11a,
author = {Sousbie, T. and Pichon, C. and Kawahara, H.},
title = {The persistent cosmic web and its filamentary structure – II. Illustrations},
journal = {Monthly Notices of the Royal Astronomical Society},
volume = {414},
number = {1},
publisher = {Blackwell Publishing Ltd},
issn = {1365-2966},
url = {http://dx.doi.org/10.1111/j.1365-2966.2011.18395.x},
doi = {10.1111/j.1365-2966.2011.18395.x},
pages = {384--403},
keywords = {methods: data analysis, galaxies: formation, galaxies: kinematics and dynamics, cosmology: observations, dark matter, large-scale structure of Universe},
year = {2011},
}
@article{CSGO12,
  author    = {Fr{\'e}d{\'e}ric Chazal and
               Vin de Silva and
               Marc Glisse and
               Steve Oudot},
  title     = {The structure and stability of persistence modules},
  journal   = {CoRR},
  volume    = {abs/1207.3674},
  year      = {2012}
}
@article{CZ09,
  title = "The theory of multidimensional persistence",
  author = "Carlsson, G. and Zomorodian, A.",
  journal = "Discrete \& Computational Geometry",
  year = 2009,
  volume = 42,
  number = 1,
  pages = "71--93",
  doi = "doi:10.1007/s00454-009-9176-0",
}

@inproceedings{DFW13,
author = {T. K. Dey and F. Fan and Y. Wang},
title = "Graph induced complex for point data",
 booktitle = {Proc. 29th. Annu. Sympos. Comput. Geom. (SoCG)},
  year      = {2013},
  pages     = {107-116},
}
@inproceedings{AEHW04,
    author = "P. K. Agarwal and H. Edelsbrunner and J. Harer and Y. Wang",
    title = "Extreme elevation on a 2-manifold",
    booktitle = "Proc. 20th Sympos. Comput. Geom.",
    pages = {357--365},
    year = 2004
}
@techreport{Denali,
author = "J. Eldridge and M. Belkin and Y. Wang",
title = "{\it Denali}: {A} tool for visualizing scalar functions as landscape metaphors",
institution = "The Ohio State University",
note = {Tutorial and documentation of {\it Denali} can be found at: {\tt denali.cse.ohio-state.edu/}},
year = 2014
}

@inproceedings{BCCDW12,
  author    = {Oleksiy Busaryev and
               Sergio Cabello and
               Chao Chen and
               Tamal K. Dey and
               Yusu Wang},
  title     = {Annotating Simplices with a Homology Basis and Its Applications},
  booktitle = {SWAT},
  year      = {2012},
  pages     = {189-200}
}

@article{DG12,
author = "T. K. Dey and X. Ge and Q. Que and I. Safa and L. Wang and Y. Wang",
title = "Feature-preserving reconstruction of singular surfaces",
journal = "Computer Graphics Forum",
volume =31,
number = 5,
pages = {1787--1796},
year =2012
}

@article{deSilva2015,
author = "Vin de Silva and Elizabeth Munch and Amit Patel",
 Title                    = "Categorification of {Reeb} Graphs",
journal = "arXiv:1501.04147",
year = 2015
}



@phdthesis{LesnickThesis,
author = "Michael Lesnick",
title = "Multidimensional interleaving and applications to topological inference",
school = "Stanford University",
year = 2012
}
@inproceedings{Sheehy,
author = {D. Sheehy},
title = "Linear-size approximations to the {Vietoris-Rips} filtration",
 booktitle = {Proc. 28th. Annu. Sympos. Comput. Geom.},
  year      = {2012},
  pages     = {239-248},
}

@inproceedings{BCOS15,
  Title = {Efficient and Robust Persistent Homology for Measures},
  Author = {Micka\"{e}l Buchet and Fr\'{e}d\'{e}ric Chazal and Steve Y. Oudot and Donald Sheehy},
  Booktitle = {ACM-SIAM Symposium on Discrete Algorithms},
  Year = {2015}}

@article {Sousbie11b,
author = {Sousbie, T.},
title = {The persistent cosmic web and its filamentary structure – I. Theory and implementation},
journal = {Monthly Notices of the Royal Astronomical Society},
volume = {414},
number = {1},
publisher = {Blackwell Publishing Ltd},
issn = {1365-2966},
url = {http://dx.doi.org/10.1111/j.1365-2966.2011.18394.x},
doi = {10.1111/j.1365-2966.2011.18394.x},
pages = {350--383},
keywords = {methods: data analysis, methods: numerical, galaxies: formation, galaxies: kinematics and dynamics, cosmology: observations, large-scale structure of Universe},
year = {2011},
}


@article{NLC11,
author = "Monica Nicolau and Arnold J. Levine and Gunnar Carlsson",
title = {Topology based data analysis identifies a subgroup of breast cancers with a unique mutational profile and excellent survival},
journal = {Proc. Nat.  Acad. Sci. (PNAS)},
volume = 108,
issue = 17,
pages = {7265 --7270},
year = 2011,
}

@article{LS13,
title = "Extracting insights from the shape of complex data using topology",
author = "P. Y. Lum and  G. Singh and A. Lehman and  T. Ishkanov and M. Vejdemo-Johansson and M. Alagappan and J. Carlsson	 and G. Carlsson",	
journal= "Scientific Reports",
volume = 3,
number = 1236,
note= "doi:10.1038/srep01236",
year = 2013
}


@book{BVP15,
title = "Topological and statistical methods for complex data: {T}ackling large-scale, high-dimensional and multivariate data spaces",
editor = "Janine Bennett and Fabien Vivodtzev and Valerio Pascucci",
year = 2015,
series = "Mathematics and Visualization",
publisher= "Springer-Verlag Berlin Heidelberg",
}
@book{BHPP14,
title = "Topological methods in data analysis and visualization III: {T}heory, algorithms and applications",
editor="P. -T. Bremer and I. Hotz, V. Pascucci and R. Peikert",
year = 2014,
series = "Mathematics and Visualization",
publisher= "Springer International Publishing",
}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%Added by Z. Cang
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
@article{Lee:2007,
  title={Predicting protein function from sequence and structure},
  author={Lee, David and Redfern, Oliver and Orengo, Christine},
  journal={Nature Reviews Molecular Cell Biology},
  volume={8},
  number={12},
  pages={995--1005},
  year={2007},
  publisher={Nature Publishing Group}
}

@article{Laskowski:2005,
  title={ProFunc: a server for predicting protein function from 3D structure},
  author={Laskowski, Roman A and Watson, James D and Thornton, Janet M},
  journal={Nucleic Acids Research},
  volume={33},
  number={suppl 2},
  pages={W89--W93},
  year={2005},
  publisher={Oxford Univ Press}
}

@article{Roy:2010,
  title={I-TASSER: a unified platform for automated protein structure and function prediction},
  author={Roy, Ambrish and Kucukural, Alper and Zhang, Yang},
  journal={Nature protocols},
  volume={5},
  number={4},
  pages={725--738},
  year={2010},
  publisher={Nature Publishing Group}
}

@article{Haliloglu:1997,
  title={Gaussian dynamics of folded proteins},
  author={Haliloglu, Turkan and Bahar, Ivet and Erman, Burak},
  journal={Physical review letters},
  volume={79},
  number={16},
  pages={3090},
  year={1997},
  publisher={APS}
}

@article{Collins:2004,
  title={A barcode shape descriptor for curve point cloud data},
  author={Collins, A. and Zomorodian, A. and Carlsson, G. and Guibas, L. J.},
  journal={Computers and Graphics},
  volume={28},
  number={6},
  pages={881--894},
  year={2004},
  publisher={Elsevier}
}

@inproceedings{Javaplex:2014,
     author = {Tausz, Andrew and Vejdemo-Johansson, Mikael and Adams, Henry},
     title = {Java{P}lex: {A} research software package for persistent (co)homology},
     booktitle = {Proceedings of ICMS 2014},
     editor = {Hong, Han and Yap, Chee},
     series = {Lecture Notes in Computer Science 8592},
     year = {2014},
     pages = {129-136},
}

@article{Cortes:1995,
  title={Support-vector networks},
  author={Cortes, Corinna and Vapnik, Vladimir},
  journal={Machine learning},
  volume={20},
  number={3},
  pages={273--297},
  year={1995},
  publisher={Springer}
}

@article{Chang:2011,
 author = {Chang, Chih-Chung and Lin, Chih-Jen},
 title = {{LIBSVM}: A library for support vector machines},
 journal = {ACM Transactions on Intelligent Systems and Technology},
 volume = {2},
 issue = {3},
 year = {2011},
 pages = {27:1--27:27},
 note =	 {Software available at \url{http://www.csie.ntu.edu.tw/~cjlin/libsvm}}
}

@article{Fan:2005,
  title={Working set selection using second order information for training support vector machines},
  author={Fan, Rong-En and Chen, Pai-Hsuen and Lin, Chih-Jen},
  journal={The Journal of Machine Learning Research},
  volume={6},
  pages={1889--1918},
  year={2005},
  publisher={JMLR. org}
}

@article{Fox:2014,
  title={SCOPe: Structural Classification of Proteins-extended, integrating SCOP and ASTRAL data and classification of new structures},
  author={Fox, Naomi K and Brenner, Steven E and Chandonia, John-Marc},
  journal={Nucleic Acids Research},
  volume={42},
  number={D1},
  pages={D304--D309},
  year={2014},
  publisher={Oxford Univ Press}
}

@article{Fawcett:2006,
  title={An introduction to ROC analysis},
  author={Fawcett, Tom},
  journal={Pattern recognition letters},
  volume={27},
  number={8},
  pages={861--874},
  year={2006},
  publisher={Elsevier}
}

@article{Sonego:2007,
  title={A protein classification benchmark collection for machine learning},
  author={Sonego, Paolo and Pacurar, Mircea and Dhir, Somdutta and Kert{\'e}sz-Farkas, Attila and Kocsor, Andr{\'a}s and G{\'a}sp{\'a}ri, Zolt{\'a}n and Leunissen, Jack AM and Pongor, S{\'a}ndor},
  journal={Nucleic Acids Research},
  volume={35},
  number={suppl 1},
  pages={D232--D236},
  year={2007},
  publisher={Oxford Univ Press}
}

@article{Johnson:2008,
  title={NCBI BLAST: a better web interface},
  author={Johnson, Mark and Zaretskaya, Irena and Raytselis, Yan and Merezhuk, Yuri and McGinnis, Scott and Madden, Thomas L},
  journal={Nucleic Acids Research},
  volume={36},
  number={suppl 2},
  pages={W5--W9},
  year={2008},
  publisher={Oxford Univ Press}
}

@article{Li:2015,
  title={The EMBL-EBI bioinformatics web and programmatic tools framework},
  author={Li, Weizhong and Cowley, Andrew and Uludag, Mahmut and Gur, Tamer and McWilliam, Hamish and Squizzato, Silvano and Park, Young Mi and Buso, Nicola and Lopez, Rodrigo},
  journal={Nucleic Acids Research},
  pages={gkv279},
  year={2015},
  publisher={Oxford Univ Press}
}

@article{Henikoff:1992,
  title={Amino acid substitution matrices from protein blocks},
  author={Henikoff, Steven and Henikoff, Jorja G},
  journal={Proceedings of the National Academy of Sciences},
  volume={89},
  number={22},
  pages={10915--10919},
  year={1992},
  publisher={National Acad Sciences}
}

@article{Altschul:1993,
  title={A protein alignment scoring system sensitive at all evolutionary distances},
  author={Altschul, Stephen F},
  journal={Journal of molecular evolution},
  volume={36},
  number={3},
  pages={290--300},
  year={1993},
  publisher={Springer}
}
%PDB refs%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%M2 chimera channel
@article{Pielak:2011,
  title={Structural investigation of rimantadine inhibition of the AM2-BM2 chimera channel of influenza viruses},
  author={Pielak, Rafal M and Oxenoid, Kirill and Chou, James J},
  journal={Structure},
  volume={19},
  number={11},
  pages={1655--1663},
  year={2011},
  publisher={Elsevier}
}

@article{Bolton:1970,
  title={Three dimensional Fourier synthesis of horse deoxyhaemoglobin at 2.8 {\AA} resolution},
  author={Bolton, W and Perutz, MF},
  journal={Nature},
  volume={228},
  pages={551--552},
  year={1970}
}

%T-hemoglobin 2HHB
@article{Fermi:1984,
  title={The crystal structure of human deoxyhaemoglobin at 1.74 {\AA} resolution},
  author={Fermi, G and Perutz, MF and Shaanan, B and Fourme, R},
  journal={Journal of molecular biology},
  volume={175},
  number={2},
  pages={159--174},
  year={1984},
  publisher={Elsevier}
}

%M2 channel description
@article{Pielak:2011b,
  title={Influenza M2 proton channels},
  author={Pielak, Rafal M and Chou, James J},
  journal={Biochimica et Biophysica Acta (BBA)-Biomembranes},
  volume={1808},
  number={2},
  pages={522--529},
  year={2011},
  publisher={Elsevier}
}

@article{Dash:1997,
  title={Feature selection for classification},
  author={Dash, Manoranjan and Liu, Huan},
  journal={Intelligent data analysis},
  volume={1},
  number={1},
  pages={131--156},
  year={1997},
  publisher={Elsevier}
}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%End of refs by Z. Cang
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

@article{Stormo:1982,
  title={Use of the ‘Perceptron’ algorithm to distinguish translational initiation sites in E. coli},
  author={Stormo, Gary D and  Schneider, Thomas D. and  Gold, Larry and  Ehrenfeucht, Andrzej },
  journal={Nucleic Acids Research},
  volume={10},
  number={},
  pages={2997--3011},
  year={1982}
}


@article{Leslie:2004,
  title={ Mismatch string kernels for discriminative protein classification
},
  author={Leslie, C. S.  and  Eskin, E.  and Cohen, A. and    Weston, J. and  Noble, W. S.
 },
  journal={Bioinformtics},
  volume={20},
  number={},
  pages={467--476},
  year={2004}
}


@article{JLCheng:2006,
  title={ { DOMpro: Protein} domain prediction using profiles, secondary structure, relative solvent accessibility, and recursive neural networks
},
  author={Cheng, J. L. and Sweredoski, M. J.  and  Baldi, P.
 },
  journal={Data Mining and Knowledge Discovery},
  volume={13},
  number={},
  pages={1--10},
  year={2006}
}


@article{Meinicke:2015,
  title={{ UProC:} tools for ultra-fast protein domain classification},
  author={Meinicke, Peter
 },
  journal={Bioinformtics},
  volume={31},
  number={},
  pages={1382--1388},
  year={2015}
}


@article{Fernandez-Lozano:2014,
  title={Improving enzyme regulatory protein classification by means of SVM-RFE feature selection},
  author={Fernandez-Lozano, C. and  Fernandez-Blanco, E. and Dave, K. and  Pedreira, N. and  Gestal, M. and   Dorado, J. and  Munteanu, C. R. },
  journal={Molecular Biosystems},
  volume={10},
  number={},
  pages={1063--1071 },
  year={2014}
}


@article{Burges:1998,
  title={ A tutorial on Support Vector Machines for pattern recognition},
  author={ Burges, C. J. C. },
  journal={Data Mining and Knowledge Discovery},
  volume={2},
  number={},
  pages={121--167 },
  year={1998}
}


@article{CWHsu:2002,
  title={  A comparison of methods for multiclass support vector machines},
  author={ Hsu, C. W. and  Lin, C. J.  },
  journal={IEEE Transactions on Neural Networks},
  volume={13},
  number={},
  pages={415-442 },
  year={2002}
}


@article{McCulloch:1943,
  title={ A Logical Calculus of Ideas Immanent in Nervous Activity},
  author={ McCulloch, Warren and Pitts,   Walter  },
  journal={Bulletin of Mathematical Biophysics},
  volume={5},
  number={},
  pages={115-133 },
  year={1943}
}


@article{Hinton:2006,
  title={ A fast learning algorithm for deep belief nets
},
  author={ Hinton, Geoffrey E. and  Osindero, Simon and Teh, Yee-Whye },
  journal={Neural Computation  },
  volume={18},
  number={},
  pages={1527--1554 },
  year={2006}
}


@article{WeiWu:2013,
  title={An Efficient Multiple Protein Structure Comparison Method and its Application to Structure Clustering and Outlier Detection
},
  author={ Wu, Wei and  Srivastava, A. and Laborde, J. and  Zhang, J. F. },
  journal={IEEE, BIBM },
  volume={},
  number={},
  pages={69--73 },
  year={2013}
}

@article{Duncan:1993,
  title={Shape analysis of molecular surfaces
},
  author={Duncan, B. S. and  Olson, A. J.},
  journal={Biopolymers },
  volume={33},
  number={},
  pages={231-238 },
  year={1993}
}



@article{HCheng:2009,
  title={Quality mesh generation for molecular skin surfaces using restricted union of balls
},
  author={ Ho-Lun Cheng and  Xinwei Shi },
  journal={Computational Geometry },
  volume={42},
  number={},
  pages={ 196–206},
  year={2009}
}



@article{ Sridharan:1995,
  title={A fast molecular surfacing algorithm with applications to finite-difference electrostatic calculations
},
  author={ Sridharan, S. and R. Nicholls, A. and Honig, B.},
  journal={Biophys. J. },
  volume={68},
  number={},
  pages={220A},
  year={1995}
}



@article{Vorobjev:1997b,
  title={SIMS: Computation of a smooth invariant molecular surface
},
  author={ Sridharan, S. and R. Nicholls, A. and Honig, B.},
  journal={Biophys. J. },
  volume={73},
  number={},
  pages={722-732},
  year={1997}
}


@article{Ryu:2007,
  title={Molecular surfaces on proteins via beta shapes
},
  author={  Ryu, J. and Park, R. and Kim, D. S.},
  journal={Comput. Aided Des.},
  volume={73},
  number={},
  pages={1042- 1057},
  year={2007}
}

@ARTICLE{Krone:2009,
author={Krone, M. and Bidmon, K. and Ertl, T.},
journal={Visualization and Computer Graphics, IEEE Transactions on},
title={Interactive Visualization of Molecular Surface Dynamics},
year={2009},
month={Nov},
volume={15},
number={6},
pages={1391-1398},
doi={10.1109/TVCG.2009.157},
ISSN={1077-2626},}



%%%%%% Reference By Bao Wang Oct 2015 %%%%%%%%%%%%%%%%%%

@ARTICLE{Jenkins,
    author = {Kenneth Haugland},
    title = {Polynomial Equation Solver},
    journal = {http://www.codeproject.com/Articles/552678/Polynomial-Equation-Solver},
   year = {2013},
}
	
	
@article{ESES:2017,
Author = {Beibei Liu and Bao Wang and Rundong Zhao and Yiying Tong and Guo Wei Wei},
Title = {{ESES:  software for Eulerian solvent excluded surface}},
Journal = {Journal of Computational Chemistry},
Year = {2017},
  volume={38},
  number={},
  pages={}
}

@ARTICLE{VariationalFluid2010,
  author = {Dmitry Pavlov and Patrick Mullen and Yiying Tong and Eva Kanso and
	Jerrold E. Marsden and Mathieu Desbrun},
  title = {Structure-Preserving Discretization of Incompressible Fluids},
  journal = {Physica D: Nonlinear Phenomena},
  year = {March 2011},
  volume = {240},
  pages = {443-458},
  number = {6},
  owner = {Yiying},
  timestamp = {2010.11.07}
}
@article{de2014discrete,
  title={Discrete 2-Tensor Fields on Triangulations},
  author={de Goes, Fernando and Liu, Beibei and Budninskiy, Max and Tong, Yiying and Desbrun, Mathieu},
  journal={Computer Graphics Forum},
  volume={33},
  number={5},
  pages={13--24},
  year={2014}
}

@article{Solvationblind:2015,
Author = {Bao Wang and Zhixiong Zhao and Guo Wei Wei},
Title = {Hybrid Physical and Knowledge based Models for Blind Solvation Free Energy Prediction},
Journal = {{Preprint}},
Year = {2015},
}



@book{Harsen:book,
    AUTHOR = {J. P. Hansen and I. R. McDonald},
     TITLE = {Theory of Simple Liquids},
    SERIES = {Fourth Edition},
    VOLUME = {},
 PUBLISHER = {},
   ADDRESS = {},
      YEAR = {2000},
     PAGES = {},
      ISBN = {},
   MRCLASS = {},
  MRNUMBER = {},
MRREVIEWER = {},
}

@book{Hirata:book,
    AUTHOR = {F. Hirata},
     TITLE = {Molecular theory of solvation},
    SERIES = {},
    VOLUME = {},
 PUBLISHER = {Kluwer Academic Publishers, Dordrecht, Netherlands.},
   ADDRESS = {},
      YEAR = {2003},
     PAGES = {},
      ISBN = {},
   MRCLASS = {},
  MRNUMBER = {},
MRREVIEWER = {},
}

@article{LuoRayPB-VS-Explicitsolvent:2006,
  title={How Well Does Poisson-Boltzmann Implicit Solvent Agree with Explicit Solvent? A Quantitative Analysis},
  author={Tan, C. H. and Yang, L. J. and Luo, R.},
  journal={Journal of Physical Chemistry B},
  volume={110},
  number={},
  pages={18680-18687},
  year={2006}
}

@article{LuoRayPB-VS-Explicitsolvent:2010,
  title={Quantitative Analysis of Poisson-Boltzmann Implicit Solvent in Molecular Dynamics},
  author={Wang, J. and Tan, C. H. and  Chanco, E. and Luo, R.},
  journal = {Physical Chemistry Chemical Physics},
  volume={12},
  number={},
  pages={1194-1202},
  year={2010}
}


@article{Marcia:2011BiophysicalChemistry,
  title={Understanding the physical basis of the salt dependence of the electrostatic binding free energy of mutated charged ligand-nucleic acid complexes},
  author={Robert C. Harris and Johan H. Bredenberg and Alexander R. J. Silalahi and Alexander H. Boschitsch and Marcia O. Fenley},
  journal = {Biophysical Chemistry},
  volume={156},
  number={},
  pages={79-87},
  year={2011}
}



@ARTICLE{LiAnbang:2014,
  author = {Li Anbang},
  title = {Performance comparison of Poisson–Boltzmann equation solvers DelPhi and PBSA in calculation of electrostatic solvation energies},
  journal = {Journal of Theoretical and Computational Chemistry},
  year = {2014},
  volume = {13},
  pages = {1450040},
  number = {13}
}



@ARTICLE{LuoRay:2013force,
  author = {L. Xiao and Q. Cai and X. Ye and J. Wang and R. Luo},
  title = {{Electrostatics Forces in the Poisson-Boltzmann Systems}},
  journal = {Journal of Chemical Physics},
  year = {2013},
	volume = {139},
  pages = {094106}
}


@ARTICLE{PBSA:2009,
  author = {Q. Cai and M. J. Hsieh and J. Wang and R. Luo},
  title = {Performance of Nonlinear Finite-Difference {Poisson-Boltzmann} Solvers},
  journal = {Journal of Chemical Theory and Computation},
  year = {2009},
	volume = {6(1)},
  pages = {203-211}
}

@ARTICLE{PBSA:2008,
  author = {J. Wang and C. H. Tan and Y. H. Tan and Q. Lu and R. Luo},
  title = {{Poisson-Boltzmann solvents in molecular dynamics Simulations}},
  journal = {Communications in Computational Physics},
  year = {2008},
	volume = {3(5)},
  pages = {1010-1031}
}

@ARTICLE{IIMPB:2013,
  author = {C. Wang and J. Wang and Q. Cai and Z. Li and H. Zhao and R. Luo},
  title = {{Exploring Accurate Poisson-Boltzmann Methods for Biomolecular Simulations}},
  journal = {Comp Theo Chem},
  year = {2013},
	volume = {1022},
  pages = {34-44}
}

%%%%%% Duc added %%%%%%%%%%%%
@article{reyes2000structure,
  title={Structure and thermodynamics of {RNA-protein} binding: using molecular dynamics and free energy analyses to calculate the free energies of binding and conformational change},
  author={Reyes, Carolina M and Kollman, Peter A},
  journal={Journal of molecular biology},
  volume={297},
  number={5},
  pages={1145--1158},
  year={2000},
  publisher={Elsevier}
}

@article{shivakumar2010prediction,
  title={Prediction of absolute solvation free energies using molecular dynamics free energy perturbation and the {OPLS} force field},
  author={Shivakumar, Devleena and Williams, Joshua and Wu, Yujie and Damm, Wolfgang and Shelley, John and Sherman, Woody},
  journal={Journal of Chemical Theory and Computation},
  volume={6},
  number={5},
  pages={1509--1519},
  year={2010},
  publisher={ACS Publications}
}


@article{DDNguyen:2017a,
  title={Accurate, robust and reliable calculations of {Poisson-Boltzmann}   binding energies},
  author={Nguyen, Duc D and Wang, Bao and Wei, G. W.},
  journal={ Journal of  Computational Chemistry},
  volume={38},
  number={},
  pages={},
  year={2017},
  publisher={}
}
	
@article{DDNguyen:2016b,
  title={Generalized flexibility-rigidity index},
  author={Nguyen, Duc D and Xia, K. L. and Wei, G. W.},
  journal={Journal of Chemical Physics},
  volume={ 144 },
  number={},
  pages= {234106},
  year={ 2016},
  publisher={}
}

@article{DDNguyen:2016c,
  title={The impact of surface area, volume, curvature and Lennard-Jones potential to solvation modeling},
  author={Nguyen, Duc D  and Wei, G. W.},
  journal={Journal of Computational Chemistry},
  volume={},
  number={},
  pages={},
  year={submitted 2016},
  publisher={}
}

@article{BaoWang2015PB,
  title={{MIBPB: An} accurate and reliable software package for electrostatic analysis},
  author={Wang, Bao and Nguyen, Duc D and Zhao, Zhixiong and Cang, Zixuan and   Wei, Guo-Wei},
  journal={Preprint},
  volume={},
  number={},
  pages={},
  year={2015},
  publisher={}
}

%%%%%%%%%%% Jing He %%%%%%%%%%%%%%%%%%%%%%%%%%%%

@ARTICLE{Rossmann2000,
  author = {Rossmann, M.G.},
  title = {Fitting atomic models into electron-microscopy maps},
  journal = {Acta Crystallogr D Biol Crystallogr},
  year = {2000},
  volume = {56},
  pages = {627-635},
  number = {10}
}

@article{Topf2005191,
title = "Structural characterization of components of protein assemblies by comparative modeling and electron cryo-microscopy ",
journal = "Journal of Structural Biology ",
volume = "149",
number = "2",
pages = "191 - 203",
year = "2005",
note = "",
issn = "1047-8477",
doi = "http://dx.doi.org/10.1016/j.jsb.2004.11.004",
url = "http://www.sciencedirect.com/science/article/pii/S1047847704002175",
author = "Maya Topf and Matthew L. Baker and Bino John and Wah Chiu and Andrej Sali",
keywords = "Protein structure prediction",
keywords = "Comparative modeling",
keywords = "Electron cryo-microscopy",
keywords = "Fitting "
}

@article{Topf20061655,
title = "Refinement of Protein Structures by Iterative Comparative Modeling and CryoEM Density Fitting ",
journal = "Journal of Molecular Biology ",
volume = "357",
number = "5",
pages = "1655 - 1668",
year = "2006",
note = "",
issn = "0022-2836",
doi = "http://dx.doi.org/10.1016/j.jmb.2006.01.062",
url = "http://www.sciencedirect.com/science/article/pii/S0022283606001033",
author = "Maya Topf and Matthew L. Baker and Marc A. Marti-Renom and Wah Chiu and Andrej Sali",
keywords = "protein structure prediction",
keywords = "comparative modeling",
keywords = "homology modeling",
keywords = "cryo-electron-microscopy",
keywords = "density fitting "
}


@ARTICLE{Schroder2007,
  author = {Schröder, G. F. and Brunger, A. T. and Levitt, M.l},
  title = {Combining Efficient Conformational Sampling with a Deformable Elastic Network Model Facilitates Structure Refinement at Low Resolution},
  journal = {Structure },
  year = {2007},
  volume = {15},
  pages = {1630-1641},
  number = {12}
}

@ARTICLE{Wriggers2001,
  author = {Wriggers, W. and Birmanns, S.},
  title = {Using situs for flexible and rigid-body fitting of multiresolution single-molecule data},
  journal = {J Struct Biol},
  year = {2001},
  volume = {133},
  pages = {193-202},
  number = {2-3}
}

@ARTICLE{Trabuco2008,
  author = {Trabuco, L. G. and Villa, E. and Mitra, K. and Frank, J.},
  title = {Flexible Fitting of Atomic Structures into Electron Microscopy Maps Using Molecular Dynamics},
  journal = {Structure},
  year = {2008},
  volume = {16},
  pages = {673-683},
  number = {5}
}


@CONFERENCE{He2015,
  author = {He, J. and Zeil, S and Hallak, H and McKaig, K. and Kovacs, J. and Wriggers, W.},
  title = {Comparison of an atomic model and its cryo-EM image at the central axis of a helix},
  booktitle = {Proceeding of 2015 IEEE international Conference on Bioinformatics and Biomedicine},
  year = {2015},
  address = {Washington, D.C.},
  pages = {1253-1259},
  timestamp = {Nov. 9-12}
}

@ARTICLE{DalPalu2006,
  author = {Dal Palu, A. and He, J. and Pontelli, E. and Lu, Y.},
  title = {Identification of Alpha-Helices from Low Resolution Protein Density
	Maps},
  journal = {Proceeding of Computational Systems Bioinformatics Conference(CSB)},
  year = {2006},
  pages = {89-98}
}

@ARTICLE{Baker2012a,
  author = {Baker, Matthew L. and Baker, Mariah R. and Hryc, Corey F. and Ju,
	Tao and Chiu, Wah},
  title = {Gorgon and pathwalking: Macromolecular modeling tools for subnanometer
	resolution density maps},
  journal = {Biopolymers},
  year = {2012},
  volume = {97},
  pages = {655--668},
  number = {9},
  doi = {10.1002/bip.22065},
  issn = {1097-0282},
  keywords = {gorgon, pathwalking, cryo-em, computational modeling, macomolecular
	structure},
  publisher = {Wiley Subscription Services, Inc., A Wiley Company},
  url = {http://dx.doi.org/10.1002/bip.22065}
}


@ARTICLE{AlNasr2014,
  author = {Al Nasr, K. and Ranjan, D. and Zubair, M. and Chen, L. and He, J.},
  title = {Sovling the secondary structure matching problem in cryo-EM de novo modeling using a constrained K-shortest path graph algorithm},
  journal = {IEEE/ACM Trans Comput Biol Bioinform},
  year = {2014},
  volume = {11},
  pages = {419-429},
  number = {2}
}

@CONFERENCE{Si2013,
  author = {Si, D. and He, J.},
  title = {Beta-sheet Detection and Representation from Medium Resolution Cryo-EM
	Density Maps},
  booktitle = {Proceedings of ACM Conference on Bioinfor Comp Biol \& Biomed Inform},
  year = {2013},
  address = {Washington, D.C.},
  pages = {764-770},
  timestamp = {Sept 22-25}
}

@ARTICLE{Si2014,
  author = {Si, D. and He, J.},
  title = {Tracing Beta Strands Using StrandTwister from Cryo-EM Density Maps at Medium Resolutions},
  journal = {Structure},
  year = {2014},
  volume = {22},
  pages = {1665-1676},
  number = {11}
}

@article{Wriggers2015255,
title = "Numerical geometry of map and model assessment ",
journal = "Journal of Structural Biology ",
volume = "192",
number = "2",
pages = "255 - 261",
year = "2015",
issn = "1047-8477",
doi = "http://dx.doi.org/10.1016/j.jsb.2015.09.011",
url = "http://www.sciencedirect.com/science/article/pii/S1047847715300666",
author = "Willy Wriggers and Jing He",
keywords = "Cryo-electron microscopy",
keywords = "Protein structure",
keywords = "Fitting",
keywords = "Validation",
keywords = "Secondary structure "
}

@ARTICLE{He2004,
  author = {He, J. and Lu, Y. and Pontelli, E.},
  title = {A Parallel Algorithm for Helix Mapping between 3-{D} and 1-{D} Protein
	Structure using the Length Constraints},
  journal = {Lecture Notes in Computer Science},
  year = {2004},
  volume = {3358},
  pages = {746-756}
}

@CONFERENCE{Lu2007a,
  author = {Lu, Y. and He, J. and Strauss, CEM.},
  title = {Deriving Topology and Sequence Alignment for the Helix Skeleton in
	Low Resolution Protein Density Maps},
  booktitle = {Proceeding of Asia-Pacific Bioinformatics Conference},
  year = {2007},
  pages = {143-152},
  owner = {lchen},
  timestamp = {Jan 15-17}
}

@ARTICLE{Lu2007,
  author = {Lu, Y. and Strauss, C. E. M. and He, J.},
  title = {Incorporation of Constraints from Low Resolution Density Map in Ab
	Initio Structure Prediction Using Rosetta},
  journal = {Proceeding of 2007 IEEE international Conference on Bioinformatics
	and Biomedicine Workshops},
  year = {2007},
  pages = {p67-73}
}

@ARTICLE{Lu2008,
  author = {Lu, Y. and He, J. and Strauss, C. E.},
  title = {Deriving topology and sequence alignment for the helix skeleton in
	low-resolution protein density maps},
  journal = {J Bioinform Comput Biol},
  year = {2008},
  volume = {6},
  pages = {183-201},
  number = {1}
}

@ARTICLE{Sun2009a,
  author = {Sun, Weitao and He, Jing},
  title = {Reduction of the secondary structure topological space through direct
	estimation of the contact energy formed by the secondary structures},
  journal = {BMC Bioinformatics},
  year = {2009},
  volume = {10},
  pages = {1-11},
  number = {Suppl 1},
  doi = {10.1186/1471-2105-10-S1-S40},
  language = {English},
  publisher = {BioMed Central},
  url = {http://dx.doi.org/10.1186/1471-2105-10-S1-S40}
}

@ARTICLE{Sun2009,
  author = {Sun, W. and He, J.},
  title = {Native secondary structure topology has near minimum contact energy
	among all possible geometrically constrained topologies},
  journal = {Proteins},
  year = {2009},
  volume = {77},
  pages = {159-73},
  number = {1}
}

@ARTICLE{Sun2009b,
  author = {Sun, W. and He, J.},
  title = {Reduction of the secondary structure topological space through direct
	estimation of the contact energy formed by the secondary structures},
  journal = {BMC Bioinformatics},
  year = {2009},
  volume = {10 Suppl 1},
  pages = {S40}
}

@article {Sun2010,
author = {Sun, Weitao and He, Jing},
title = {Understanding on the residue contact network using the log-normal cluster model and the multilevel wheel diagram},
journal = {Biopolymers},
volume = {93},
number = {10},
pages = {904--916},
year = {2010}
}

@ARTICLE{AlNasr2009,
  author = {Al Nasr, K. and He, J.},
  title = {An effective convergence independent loop closure method using Forward-Backward
	Cyclic Coordinate Descent},
  journal = {International Journal of Data Mining and Bioinformatics },
  year = {2009},
  volume = {3},
  pages = {346-61},
  number = {3}
}

@Article{AlNasr2010,
author="Al Nasr, Kamal
and Sun, Weitao
and He, Jing",
title="Structure prediction for the helical skeletons detected from the low resolution protein density map",
journal="BMC Bioinformatics",
year="2010",
volume="11",
number="1",
pages="1--8"
}

@inproceedings{Nasr2014b,
 author = {Nasr, Kamal Al and He, Jing},
 title = {Construction of Protein Backbone Pieces Using Segment-based FBCCD and Cryo-EM Skeleton},
 booktitle = {Proceedings of the 5th ACM Conference on Bioinformatics, Computational Biology, and Health Informatics},
 series = {BCB '14},
 year = {2014},
 isbn = {978-1-4503-2894-4},
 location = {Newport Beach, California},
 pages = {711--716},
 numpages = {6},
 url = {http://doi.acm.org/10.1145/2649387.2660838},
 doi = {10.1145/2649387.2660838},
 acmid = {2660838},
 publisher = {ACM},
 address = {New York, NY, USA},
 keywords = {density, electron microscopy, graph, loop, modeling, protein, secondary structure, shortest paths, structure, topology, volume},
}


@incollection{AlNasr2015,
year={2015},
isbn={978-3-319-19047-1},
booktitle={Bioinformatics Research and Applications},
volume={9096},
series={Lecture Notes in Computer Science},
editor={Harrison, Robert and Li, Yaohang and Mandoiu, Ion},
doi={10.1007/978-3-319-19048-8_1},
title={Deriving Protein Backbone Using Traces Extracted from Density Maps at Medium Resolutions},
url={http://dx.doi.org/10.1007/978-3-319-19048-8_1},
publisher={Springer International Publishing},
keywords={Cryo-EM; Volume image; Skeletonization; Protein modeling; Loop modeling},
author={Nasr, KamalAl and He, Jing},
pages={1-11},
language={English}
}

@CONFERENCE{Si2014a,
author={Dong Si and Jing He},
booktitle={Engineering in Medicine and Biology Society (EMBC), 2014 36th Annual International Conference of the IEEE},
title={Combining image processing and modeling to generate traces of beta-strands from cryo-EM density images of beta-barrels},
year={2014},
pages={3941-3944},
month={Aug}
}

@inproceedings{Si2014c,
 author = {Si, Dong and He, Jing},
 title = {Orientations of Beta-strand Traces and Near Maximum Twist},
 booktitle = {Proceedings of the 5th ACM Conference on Bioinformatics, Computational Biology, and Health Informatics},
 series = {BCB '14},
 year = {2014},
 isbn = {978-1-4503-2894-4},
 location = {Newport Beach, California},
 pages = {690--694},
 numpages = {5},
 url = {http://doi.acm.org/10.1145/2649387.2660835},
 doi = {10.1145/2649387.2660835},
 acmid = {2660835},
 publisher = {ACM},
 address = {New York, NY, USA},
 keywords = {{\$\beta\$}-strand, electron microscopy, image, protein, secondary structure, twist},
}

@incollection{Biswas2015a,
year={2015},
isbn={978-3-319-19047-1},
booktitle={Bioinformatics Research and Applications},
volume={9096},
series={Lecture Notes in Computer Science},
editor={Harrison, Robert and Li, Yaohang and Mandoiu, Ion},
doi={10.1007/978-3-319-19048-8_6},
title={A Novel Computational Method for Deriving Protein Secondary Structure Topologies Using Cryo-EM Density Maps and Multiple Secondary Structure Predictions},
url={http://dx.doi.org/10.1007/978-3-319-19048-8_6},
publisher={Springer International Publishing},
author={Biswas, A. and Ranjan, D. and Zubair, M. and He, J.},
pages={60-71},
}

@Article{Biswas2015b,
author="Biswas, A. and Ranjan, D. and Zubai,r M. and He, J.",
title="A Dynamic Programming Algorithm for Finding the Optimal Placement of a Secondary Structure Topology in Cryo-EM Data",
journal="Journal of Comp Biol",
year="2015",
volume="22",
number="9",
pages="837-843"
}



%Added Bao Wang for solvation prediction paper
@incollection{SolvationTruhlarAndCramer:1994,
  author    = {Joey W. Storer and David J. Giesen and Gregory D. Hawkins and Gillian C. Lynch and Christopher J. Cramer and Donald G. Truhlar and Daniel A. Liotard},
  title = {Solvation Modeling in Aqueous and Nonaqueous Solvent, New techniques and a Reexamination of the Claisen Rearrangement},
	booktitle = {Structure, Energetics, and Reactivity in Aqueous Solution: Characterization of Chemical and Biological Systems},
  series    = {568},
  editor    = {C. J. Cramer and D. G. Truhlar},
  publisher = {American Chemical Society},
  pages     = {24-49},
  year      = 1994,
  note      = {}
}


@inproceedings{Daudel:1973,
  title={Quantum Theory of Chemical Reactivity},
  author={Daudel, R.},
  booktitle={Quantum Theory of Chemical Reactivity},
  pages={},
  year={1973},
  organization={}
}

@inproceedings{Reichardt:1990,
  title={Solvents and Solvent Effects in Organic Chemistry},
  author={Reichardt, C.},
  booktitle={Solvents and Solvent Effects in Organic Chemistry},
  publisher = {Wiley-VCH: New York},
  pages={},
  year={1990},
  organization={}
}


@inproceedings{Kreevoy:1986,
  title={In Investigation of Rates and Mechanisms of Reactions, Part I},
  author={Kreevoy, M.M. and Truhlar, D.G.},
  booktitle={In Investigation of Rates and Mechanisms of Reactions, Part I},
  series    = {},
  editor    = {C.F. Bernasconi},
  publisher = {Wiley: New York},
  pages     = {13},
  year      = 1986,
  note      = {}
}


@article{Marcia:2013BW,
    title     = {Influence of Grid Spacing in {Poisson-Boltzmann} Equation Binding Energy Estimation},
  author    = {Harris, Robert C. and  Boschitsch, Aleander H. and Fenley, Marcia O.},
  journal={Journal of Chemical Theory and Computation},
  volume={9},
  pages={3677-3685},
  year={2013}
}

@article{Warshel:1998BW,
    title     = {Electrostatic effects in macromolecules: fundamental concepts and practical modeling},
  author    = {Warshel,  A. and  Papazyan, A.},
  journal={Current Opinion in Structural Biology},
  volume={8(2)},
  pages={211-217},
  year={1998}
}



@inproceedings{Hirata:2003,
  title={Molecular Theory of Solvation},
  author={Hirata, F. },
  booktitle={Molecular Theory of Solvation},
  series    = {},
  editor    = {Hirata, F.},
  publisher = {Springer},
  pages     = {},
  year      = 2003,
  note      = {}
}

@article{Fedorov:2010,
    title     = {An Accurate Prediction of Hydration Free Energies by Combination of Molecular Integral Equations Theory with Structural Descriptors},
  author    = {Ekaterina L. Ratkova and Gennady N. Chuev and Volodynyr P. Sergiievskyi and Maxim V. Fedorov},
  journal={Journal of Physical Chemistry B},
  volume={114},
  pages={12068-12079},
  year={2010}
}

@article{Borgis:2005,
    title     = {Density Functional Theory of Solvation and Its Relation to Implicit Solvent Models},
  author    = {Rosa Ramirez and Daniel Borgis},
  journal={Journal of Physical Chemistry B},
  volume={109},
  pages={6754-6763},
  year={2005}
}


@article{BaoWang:2015cOptParm,
  title={Parameter optimization in differential geometry based solvation models},
  author={Bao Wang and   Guo-Wei Wei},
  journal={Jornal of Chemical Physics},
  volume={143},
  pages={134119},
  year={2015}
}

@article{SAMPL1:2009,
    title     = {A Blind Challenge for Computational Solvation Free Energies: Introduction and Overview},
  author    = {J. Peter Guthrie},
  journal={Journal of Physical Chemistry B},
  volume={113},
  pages={4501-4507},
  year={2009}
}


@ARTICLE{SAMPL3:2012,
  author = {Matthew T. Geballe and Guthrie,
	J. P.},
  title = {The {SAMPL3} blind prediction challenge: transfer energy overview},
  journal = {Journal of Computer-Aided Molecular Design},
  year = {2012},
  volume = {26},
  pages = {489 -496}
}





@article{Dill:2007data,
    title     = {Comparsion of charge models for fixed charge force fields: Small molecule hydration free energies in explicit solvent},
  author    = {Mobley, D. L. and Dumont, E., and Chodera, J. D. and Dill, K.},
  journal={Journal of Physical Chemistry B},
  volume={111(9)},
  pages={2242-2254},
  year={2007}
}



@article{BaoWang:MIBPBSolver,
    title     = {Accurate,  robust and  reliable  calculations of Poisson-Boltzmann solvation and binding energies},
  author= {Bao Wang  and Guo-Wei Wei},
  journal={Preprint},
  volume={},
  pages={},
  year={2016}
}


@article{Sherman:2010,
    title     = {Prediction of Absolute Solvation Fre Energies using Molecular Dynamics Free Energy Perturbation and the OPLS Force Field},
  author    = {Devleena Shlvakumar and Joshua Willams and Yujie Wu and Wolfgang Damm and John Shelly and Woody Sherman},
  journal={Journal of Chemical Theory and Computation},
  volume={6(5)},
  pages={1509-1519},
  year={2010}
}

@misc{g09,
author="M. J. Frisch and G. W. Trucks and H. B. Schlegel and G. E. Scuseria and M. A. Robb and J. R. Cheeseman and G. Scalmani and V. Barone and B. Mennucci and G. A. Petersson and H. Nakatsuji and M. Caricato and X. Li and H. P. Hratchian and A. F. Izmaylov and J. Bloino and G. Zheng and J. L. Sonnenberg and M. Hada and M. Ehara and K. Toyota and R. Fukuda and J. Hasegawa and M. Ishida and T. Nakajima and Y. Honda and O. Kitao and H. Nakai and T. Vreven and Montgomery, {Jr.}, J. A. and J. E. Peralta and F. Ogliaro and M. Bearpark and J. J. Heyd and E. Brothers and K. N. Kudin and V. N. Staroverov and R. Kobayashi and J. Normand and K. Raghavachari and A. Rendell and J. C. Burant and S. S. Iyengar and J. Tomasi and M. Cossi and N. Rega and J. M. Millam and M. Klene and J. E. Knox and J. B. Cross and V. Bakken and C. Adamo and J. Jaramillo and R. Gomperts and R. E. Stratmann and O. Yazyev and A. J. Austin and R. Cammi and C. Pomelli and J. W. Ochterski and R. L. Martin and K. Morokuma and V. G. Zakrzewski and G. A. Voth and P. Salvador and J. J. Dannenberg and S. Dapprich and A. D. Daniels and Ö. Farkas and J. B. Foresman and J. V. Ortiz and J. Cioslowski and D. J. Fox",
title="Gaussian~09 {R}evision {E}.01",
note="Gaussian Inc. Wallingford CT 2009"
}

@article{pybel,
    title     = {Integration of Structure-Activity Relationship and Artificial Intelligence Systems To Improve in Silico Prediction of Ames Test Mutagenicity},
  author    = {Paolo Mazzatorta and Liên-Anh Tran and Benoît Schilter and Martin Grigorov},
  journal={J. Chem. Inf. Model.},
  volume={47(1)},
  pages={34-38},
  year={2007}
}

@article{B3,
    title     = {Density-functional thermochemistry. III. The role of exact exchange},
  author    = {Becke, Axel D.},
  journal={Journal of Chemical Physics},
  volume={98(7)},
  pages={5648},
  year={1993}
}

@article{LYP,
    title     = {Development of the {Colle-Salvetti} correlation-energy formula into a functional of the electron density},
  author    = {Lee, Chengteh and Yang, Weitao and Parr, Robert G.},
  journal={Physical Review B},
  volume={37(2)},
  pages={785},
  year={1988}
}

@article{DMA:1981,
    title = {Distributed Multipole Analysis, or How to describe a molecular charge distribution},
	author = {A. J. Stone},
  journal = {Chemical Physics Letters},
     year = {1981},
	 volume={83(2)},
    pages = {233-239}
}

@article{Scheres:2012,
    title = {A Bayesian View on Cryo-{EM} Structure Determination},
	author =  {Sjors H. W. Scheres},
  journal = {Journal of Molecular Biology},
     year = {2012},
	 volume=   {415},
    pages = {406-418}
}
	
		
		
@article{Rees:2013,
    title = {{EMEN2:} an object oriented database and electronic lab notebook},
	author =  {Rees, I and  Langley, E. and  Chiu, W and Ludtke, S. J.},
  journal = {Microsc Microanal},
     year = {2013},
	 volume=   {19},
    pages = {1-10}
}
		
		
@article{XPeng:2013,
    title = {{Poisson-Boltzmann} calculations: van der {Waals} or molecular surface?},
	author =  {X. Pang and H.-X. Zhou},
  journal = {Commun. Comput. Phys.},
     year = {2013},
	 volume=   {13},
    pages = {1-12}
}
		
	

@BOOK{DasGupta2016,
  title = {Models and Algorithms for Biomolecules and Molecular Networks},
  publisher = {John Wiley \& Sons},
  year = {2016},
  author = {Bhaskar DasGupta and Jie Liang}
}
			


	@article{PMach:2011,
    title = { Geometric measures of large biomolecules: Surface, volume, and pockets},
	author =  {P. Mach and P. Koehl},
  journal = { J. Comp. Chem.},
     year = {2011},
	 volume=   {32},
    pages = {3023-3038}
}
	

	
	@article{XShi:2011,
    title = {Geometry and topology for modeling biomolecular surfaces},
	author =  {Shi, X. and  Koehl, P.},
  journal = {Far East J. Applied Math.},
     year = {2011},
	 volume=   {50},
    pages = {1-34}
}
	
@article{JLi:2013,
    title = {Measuring the shapes of macromolecules - and why it matters},
	author =  {Li, J. and  Mach, P. and  Koehl, P.},
  journal = {Comput Struct Biotechnol J.},
     year = {2013},
	 volume=   {8},
    pages = {e201309001}
}



%%%%%% Duc added on 02/26/16 %%%%%%%%%%%%

@article{ashbaugh1999universal,
  title={A ``universal'' surface area correlation for molecular hydrophobic phenomena},
  author={Ashbaugh, Henry S and Kaler, Eric W and Paulaitis, Michael E},
  journal={Journal of the American Chemical Society},
  volume={121},
  number={39},
  pages={9243--9244},
  year={1999},
  publisher={ACS Publications}
}

@article{chothia1974hydrophobic,
  title={Hydrophobic bonding and accessible surface area in proteins},
  author={Chothia, Cyrus},
  journal={Nature},
  volume={248},
  pages={338--339},
  year={1974}
}

@article{eisenberg1985solvation,
  title={Solvation energy in protein folding and binding.},
  author={Eisenberg, David and McLachlan, Andrew D},
  journal={Nature},
  volume={319},
  number={6050},
  pages={199--203},
  year={1985}
}

@article{sharp1991reconciling,
  title={Reconciling the magnitude of the microscopic and macroscopic hydrophobic effects},
  author={Sharp, Kim A and Nicholls, Anthony and Fine, Richard F and Honig, Barry},
  journal={Science},
  volume={252},
  number={5002},
  pages={106--109},
  year={1991},
  publisher={American Association for the Advancement of Science}
}

@article{wesson1992atomic,
  title={Atomic solvation parameters applied to molecular dynamics of proteins in solution},
  author={Wesson, Laura and Eisenberg, David},
  journal={Protein Science},
  volume={1},
  number={2},
  pages={227--235},
  year={1992},
  publisher={Wiley Online Library}
}

@article{massova2000combined,
  title={Combined molecular mechanical and continuum solvent approach {(MM-PBSA/GBSA)} to predict ligand binding},
  author={Massova, Irina and Kollman, Peter A},
  journal={Perspectives in drug discovery and design},
  volume={18},
  number={1},
  pages={113--135},
  year={2000},
  publisher={Springer}
}

@article{hermann1972theory,
  title={Theory of hydrophobic bonding. II. Correlation of hydrocarbon solubility in water with solvent cavity surface area},
  author={Hermann, Robert B},
  journal={The Journal of Physical Chemistry},
  volume={76},
  number={19},
  pages={2754--2759},
  year={1972},
  publisher={ACS Publications}
}

@article{huang2000temperature,
  title={Temperature and length scale dependence of hydrophobic effects and their possible implications for protein folding},
  author={Huang, David M and Chandler, David},
  journal={Proceedings of the National Academy of Sciences},
  volume={97},
  number={15},
  pages={8324--8327},
  year={2000},
  publisher={National Acad Sciences}
}

@article{kang1987free,
  title={Free energies of hydration of solute molecules. 1. { Improvement } of the hydration shell model by exact computations of overlapping volumes},
  author={Kang, Young Kee and Nemethy, George and Scheraga, Harold A},
  journal={Journal of Physical Chemistry},
  volume={91},
  number={15},
  pages={4105--4109},
  year={1987},
  publisher={ACS Publications}
}

@article{choudhury2005mechanism,
  title={On the mechanism of hydrophobic association of nanoscopic solutes},
  author={Choudhury, Niharendu and Pettitt, B Montgomery},
  journal={Journal of the American Chemical Society},
  volume={127},
  number={10},
  pages={3556--3567},
  year={2005},
  publisher={ACS Publications}
}

@article{pitera2001importance,
  title={The importance of solute-solvent van der Waals interactions with interior atoms of biopolymers},
  author={Pitera, Jed W and van Gunsteren, Wilfred F},
  journal={Journal of the American Chemical Society},
  volume={123},
  number={13},
  pages={3163--3164},
  year={2001},
  publisher={ACS Publications}
}

@article{jackson1994application,
  title={Application of scaled particle theory to model the hydrophobic effect: {Implications} for molecular association and protein stability},
  author={Jackson, Richard M and Sternberg, Michael JE},
  journal={Protein engineering},
  volume={7},
  number={3},
  pages={371--383},
  year={1994},
  publisher={Oxford Univ Press}
}

@article{sharp1991extracting,
  title={Extracting hydrophobic free energies from experimental data: relationship to protein folding and theoretical models},
  author={Sharp, Kim A and Nicholls, Anthony and Friedman, Richard and Honig, Barry},
  journal={Biochemistry},
  volume={30},
  number={40},
  pages={9686--9697},
  year={1991},
  publisher={ACS Publications}
}




@article{Grant:1995,
  title={A Gaussian Description of Molecular Shape},
  author={Grant, J. A. and Pickup, B. T. },
  journal={Journal of Physical Chemistry},
  volume={99},
  number={},
  pages={3503--3510},
  year={1995},
  publisher={}
}


@article{Kehoe:2012,
  title={Testing the semi-explicit assembly solvation model in the SAMPL3
community blind test},
  author={Charles W. Kehoe and  Christopher J. Fennell and
Ken A. Dill},
  journal={J Comput Aided Mol Des},
  volume={26},
  number={},
  pages={563--568},
  year={2012},
  publisher={}
}




@article{LinWang:2015,
  title={{pKa} predictions for proteins, {RNAs and DNAs with the Gaussian} dielectric function using {DelPhiPKa}},
  author={Lin Wang and  Lin Li and Emil Alexov },
  journal={Proteins},
  volume={83},
  number={},
  pages={2186--2197},
  year={2015},
  publisher={}
}



@article{LLi:2013,
  title={On the Dielectric "Constant'' of Proteins: Smooth Dielectric Function for Macromolecular Modeling and Its Implementation in {DelPhi}},
  author={   L. Li, C. Li, Z. Zhang and Emil Alexov },
  journal={J. Chem. Theory Comput.},
  volume={9},
  number={},
  pages={2126--2136},
  year={2013},
  publisher={}
}




@article{Truhlar:2009Sampl1,
    title     = {{Performance of SM6, SM8, and SMD on the SAMPL1} Test Set for the Prediction of Small-Molecule Solvation Free Energies},
  author    = {Aleksandr V. Marenich and Christopher J. Cramer and and Donald G. Truhlar},
  journal={Journal of Physical Chemistry B},
  volume={113},
  pages={4538–4543},
  year={2009}
}


@article{Gasteiger:1980,
    title     = {Iterative partial equalization of orbital electronegativity - a rapid access to atomic charges},
  author    = {J. Gasteiger and M. Marsili},
  journal={Tetrahedron},
  volume={36},
  pages={3219-3228},
  year={1980}
}


%%%%%%%%%%%%%%%%%%% Added by Bao Wang
@article{Mikhail:2001,
    title     = {Solvation Effect on Organic Compound Interactions in Soil Organic Matter},
  author    = {Mikhail Borisover and Minolen Reddy  and Ellen R. Graber},
  journal={Environ. Sci. Technol.},
  volume={35(12)},
  pages={2518–2524},
  year={2001}
}

@ARTICLE{Martins:2014,
  author = {Silvia A. Martins and Sergio F. Sousa and Maria Joao Ramos and Pedro A. Fernandes},
  title = {Prediction of Solvation Free Energies with Thermodynamic Integration Using the General Amber Force Field},
  journal = {Journal of Chemical Theory and Computation},
  year = {2014},
  volume = {10},
  pages = {3570--3577},
}

@article{BaoWangSolvationPredictionI:2016,
    title = {Hybrid physical and statistical models for the blind prediction of solvation free energies},
	author = {Bao Wang and Zhixiong Zhao and Guowei Wei},
  journal = {preprint},
     year = {2016},
	 volume={},
    pages = {}
}

@ARTICLE{Merz:2015Solvation,
  author = {Zheng, Zheng and Wang, Ting  and Li, Pengfei  and Merz Jr, Kenneth M.},
  title = {{KECSA-Movable} Type Implicit Solvation Model {(KMTISM)}},
  journal = {Journal of Chemical Theory and Computation},
  year = {2015},
  volume = {11},
  pages = {667--682},
}


@article{LambdaMart:2010,
    title = {From {RankNet to LambdaRank to LambdaMART: An} Overview},
	author = {Christopher J.C. Burges},
  journal = {Microsoft Research Technical Report},
     year = {2010},
	 volume={82},
    pages = {}
}

@article{RankSVM:2002,
    title = {Optimizing Search Engines Using Clickthrough Data},
	author = {T. Joachims},
  journal = {Proceedings of the ACM Conference on Knowledge Discovery and Data Mining (KDD)},
     year = {2002},
	 volume={},
    pages = {}
}

@article{RankSVM:2006,
    title = {Training Linear {SVMs} in Linear Time},
	author = {T. Joachims},
  journal = {Proceedings of the ACM Conference on Knowledge Discovery and Data Mining (KDD)},
     year = {2006},
	 volume={},
    pages = {}
}

@article{RankSVM:2014,
    title = {Large-scale Kernel {RankSVM}},
	author = {T.-M. Kuo and C.-P. Lee and C.-J. Lin.},
  journal = {SIAM International Conference on Data Mining},
     year = {2014},
	 volume={},
    pages = {}
}

@article{GBDT:2001,
    title = {Greedy function approximation: a gradient boosting machine},
	author = {Jerome H Friedman.},
  journal = {Annals of statistics},
     year = {2001},
	 volume={},
    pages = {1189-1232}
}

@article{RankNet:2005,
    title = {Learning to rank using gradient descent},
	author = {C.J.C. Burges and T. Shaked and E. Renshaw and A. Lazier and M. Deeds and N. Hamilton and G. Hullender.},
  journal = {In Proc. of ICML},
     year = {2005},
	 volume={},
    pages = {89-96}
}

@article{LambdaRank:2007,
    title = {Learning to rank with nonsmooth cost functions},
	author = {C. J. C. Burges and R. Ragno and Quoc Viet Le.},
  journal = {Advances in Neural Information Processing Systems},
     year = {2007},
	 volume={19},
    pages = {193-200}
}


@article{Truhlar:2009S1,
  title={Performance of {SM6 SM8 and SMD on the SAMPL1} Test Set for the Prediction of Small-Molecule Solvation Free Energies},
  author={Aleksandr V. Marenich and Christopher J. Cramer and and Donald G. Truhlar},
  journal={Journal of Physical Chemistry B},
  volume={113},
  number={},
  pages={4538–4543},
  year={2009},
  publisher={}
}


	@article{Boschitsch:2015,
  title={Chapter 4, The Adaptive Cartesian Grid-Based {Poisson--Boltzmann} Solver:
	Energy and Surface Electrostatic Properties, in {
	Computational Electrostatics for		Biological Applications: Geometric and Numerical Approaches to the		Description of Electrostatic Interaction Between Macromolecules,} Rocchia,~W., Spagnuolo,~M., Eds. },
  author={Boschitsch, A. H. and Fenley, M. O.},
  journal={Cham,	2015},
  volume={ },
  number={},
  pages={73--110},
  year={2015},
  publisher={Springer International Publishing}
}



	@article{Sorensen:2015,
  title={Chapter 3,
A Comprehensive Exploration of Physical
and Numerical Parameters
in the {Poisson-Boltzmann} Equation
for Applications to Receptor-Ligand Binding, in
	{Computational Electrostatics for		Biological Applications: Geometric and Numerical Approaches to the		Description of Electrostatic Interaction Between Macromolecules}, Rocchia,~W., Spagnuolo,~M., Eds. },
  author={Jesper Sorensen and Marcia O. Fenley and Rommie E. Amaro},
  journal={Cham,	2015},
  volume={ },
  number={},
  pages={39--71},
  year={2015},
  publisher={Springer International Publishing}
}

@article{CWang:2013,
  title={ Exploring accurate	{Poisson--Boltzmann} methods for biomolecular simulations},
  author={Wang, C. and Wang, J. and  Cai, Q. and Li, Z. and Zhao, H. -K. and Luo, R.},
  journal={Comput. Theor. Chem.},
  volume={1:2},
  number={},
  pages={34-44},
  year={2014},
  publisher={}
}


@article{Mirzadeh:2011,
  title={ A second-order discretization of the
	nonlinear {Poisson--Boltzmann} equation over irregular geometries using
	non-graded adaptive Cartesian grids},
  author={Mirzadeh, M. and Theillard, M. and Gibou, F.},
  journal={J. Comput. Phys.},
  volume={230},
  number={},
  pages={ 2125--2140},
  year={2011},
  publisher={}
}






@article{Fenley:2015b,
  title={ Features of {CPB: A	Poisson--Boltzmann} solver that uses an adaptive cartesian grid},
  author={Fenley, M. O. and Harris, R. C. and Mackoy, T. and  Boschitsch, A. H.},
  journal={J. Comput. Chem.},
  volume={36},
  number={},
  pages={235--243},
  year={2015},
  publisher={}
}



@article{DDNguyen:2014,
  title={High order {FDTD} methods for transverse magnetic modes with dispersive interfaces},
  author={D.D. Nguyen and S. Zhao},
  journal={Applied Mathematics and Computation},
  volume={226},
  number={},
  pages={ 699--707},
  year={2014},
  publisher={}
}



@article{DDNguyen:2016,
  title={A second order dispersive {FDTD} algorithm for transverse electric {Maxwell's} equations with complex interfaces},
  author={D.D. Nguyen and S. Zhao},
  journal={Computers and Mathematics with Applications},
  volume={71},
  number={},
  pages={21010--1035},
  year={2016},
  publisher={}
}


@article{Talley:2008,
  title={On the electrostatic component of protein-protein binding free energy},
  author={Kemper Talley and  Carmen Ng and  Michael Shoppell and  Petras Kundrotas and Emil Alexov},
  journal={PMC Biophysics},
  volume={1:2},
  number={},
  pages={1-23},
  year={2008},
  publisher={}
}


%%%% Added by Bao Wang for Binding
@article{BaoWang:2016FFTS,
  title={Feature functional theory - solvation  predictor (FFT-SP) for the blind prediction of solvation free energy},
  author={Bao Wang and Chengzhang Wang and G. W. Wei},
  journal={Journal of Chemical Information and Modeling},
  volume={},
  number={},
  pages={},
  year={submitted 2016},
  publisher={}
}

@article{BaoWang:2016FFTB,
  title={Feature functional theory - binding predictor (FFT-BP) for the blind prediction of binding free energy},
  author={Bao Wang and Zhixiong Zhao and G. W. Wei},
  journal={Journal of Chemical Thoery and Computation},
  volume={},
  number={},
  pages={},
  year={submitted 2016},
  publisher={}
}


@article{BaoWang:2016HPK,
  title={Automatic parametrization of non-polar implicit solvent models for the blind prediction of solvation free energies},
  author={Bao Wang and Zhixiong Zhao and G. W. Wei},
  journal={Journal of Chemical Physics },
  volume={145},
  number={},
  pages={124110},
  year={2016},
  publisher={}
}


#Add for binding affinity scoring
@article{BaoWang:2016LTR,
  title={Learning to Rank for Solvation Free Energy Prediction},
  author={Bao Wang and Chengzhang Wang and G. W. Wei},
  journal={Preprint},
  volume={},
  number={},
  pages={},
  year={2016},
  publisher={}
}


@article{WeiZhang:2015,
  title={When drug discovery meets web search: Learning to Rank for ligand-based virtual screening},
  author={Wei Zhang and Lijuan Ji and Yanan Chen and Kailin Tang and Haiping Wang and Ruixin Zhu and Wei Jia and Zhiwei Cao and Qi Liu},
  journal={Journal of Cheminformatics},
  volume={7},
  number={5},
  pages={},
  year={2015},
  publisher={}
}

@article{HongjianLi:2014RF,
  title={Substituting random forest for multiple linear regression improves binding affinity prediction of scoring functions: Cyscore as a case study},
  author={Hongjian Li and Kwong-Sak Leung and ManHon Wong and Pedro J Ballester},
  journal={BMC Bioinformatics},
  volume={15},
  number={291},
  pages={},
  year={2014},
  publisher={}
}

@article{RenxiaoWang:2003CompareSF,
  title={Comparative Evaluation of 11 Scoring Functions for Molecular Docking},
  author={Renxiao Wang and YiPin Lu and Shaomeng Wang},
  journal={J. Med. Chem.},
  volume={46},
  number={},
  pages={2287-2303},
  year={2003},
  publisher={}
}


@article{Pedro:2010Binding,
  title={A machine learning approach to predicting protein–ligand binding affinity with applications to molecular docking},
  author={Pedro J. Ballester  and John B. O. Mitchell},
  journal={Bioinformatics},
  volume={26},
  number={9},
  pages={1169-1175},
  year={2010},
  publisher={}
}

@article{PDBBind:2015,
  title={{{PDB}-wide collection of binding data: current status of the { PDBbind} database}},
  author={Liu, Z. H. and Li Y. and Han L. and Liu J. and Zhao Z. X. and Nie W. and Liu Y. C. and Wang R. X.},
  journal={Bioinformatics},
  volume={31},
  number={3},
  pages={405-412},
  year={2015},
  publisher={}
}

@article{Shivani:2010,
  title={Ranking Chemical Structure for Drug Discovery: A New Machine Learning Approach},
  author={Shivani Agarwal and Deepak Dugar and Shiladitya Sengupta},
  journal={Journal of Chemical Information and Model},
  volume={50},
  number={},
  pages={716-731},
  year={2010},
  publisher={}
}


@article{Bock:2002,
  title={A New Method to Estimate Ligand-Receptor Energetics},
  author={Joel R. Bock and David A. Gough},
  journal={Molecular and Cellular Proteomics},
  volume={1},
  number={11},
  pages={904-910},
  year={2002},
  publisher={}
}

@article{VirtualScreeningShoichet:2004,
  title={Virtual screening of chemical libraries},
  author={BK Schichet},
  journal={Nature},
  volume={432},
  number={7019},
  pages={862-865},
  year={2004},
  publisher={}
}

@article{Ballester:2014,
  title={Does a More Precise Chemical Description of Protein-Ligand Complexes Lead to More Accurate Prediction of Binding Affinity?},
  author={Pedro J. Ballester and Adrian Schreyer and Tom, L. Blundell},
  journal={Journal of Chemical Information and Model},
  volume={54},
  number={},
  pages={944-955},
  year={2014},
  publisher={}
}


@article{Leach:2006,
  title={Prediction of Protein-Ligand Interactions. Docking and Scoring: Successes and Gaps.},
  author={A. R. Leach and B. K. Shoichet and C. E. Peishoff},
  journal={J. Med. Chem.},
  volume={49},
  number={},
  pages={5851-5855},
  year={2006},
  publisher={}
}

@article{Novikov:2011,
  title={{CSAR Scoring} Challenge Reveals the Need for New Concepts in Estimating Protein-Ligand Binding Affinity},
  author={F. N. Novikov and A. A. Zeifman and O. V. Stroganov and V. S. Stroylov and V. Kulkov and G. G. Chilov},
  journal={Journal of Chemical Information and Model},
  volume={51},
  number={},
  pages={2090-2096},
  year={2011},
  publisher={}
}

@article{LiuJie:2014,
  title={Clasification of Current Scoring Functions},
  author={Jie Liu and Renxiao Wang},
  journal={Journal of Chemical Information and Model},
  volume={55},
  number={3},
  pages={475-482},
  year={2015},
  publisher={}
}

@article{Ortiz:1995,
  title={Prediction of Drug Binding Affinities by Comparative Binding Energy Analysis},
  author={A. R. Ortiz and M. T. Pisabarro and F. Gago and R. C. Wade },
  journal={J. Med. Chem},
  volume={38},
  number={},
  pages={2681-2691},
  year={1995},
  publisher={}
}

@article{Yin:2008,
  title={MedusaScore: An Acurate Force Field-Based Scoring Function for Virtual Drug Screening},
  author={S. Yin and L. Biedermannova and J. Vondrasek and N. V. Dokholyan},
  journal={Journal of Chemical Information and Model},
  volume={48},
  number={},
  pages={1656-1662},
  year={2008},
  publisher={}
}

@article{Su:2015,
  title={Comparison of Radii Sets, Entropy, QM Methods, and Sampling on {MM-PBSA, MM-GBSA, and QM/MM-GBSA} Ligand Binding Energies of F. tularensis Enoyl-ACP Reductase (Fabl)},
  author={Pin-Chih Su and Cheng-Chieh Tsai and Shahila Mehboob and Kirk E. Heveber and Michael E. Johnson},
  journal={Journal of Computational Chemistry},
  volume={36},
  number={},
  pages={1859-1873},
  year={2015},
  publisher={}
}

@article{Zheng:2015LISA,
  title={Ligand Identification Scoring Algorithm {(LISA)}},
  author={Zheng, Zheng and Merz Jr, Kenneth M. },
  journal={Journal of Chemical Information and Model},
  volume={51},
  number={},
  pages={1296-1306},
  year={2011},
  publisher={}
}

@article{Verkhivker:1995PLP,
  title={Empirical free energy calculations of ligand-protein crystallographic complexes. I. Knowledge based ligand-protein interaction potentials applied to the prediction of human immunodeficiency virus protease binding affinity.},
  author={G. Verkhivker and K. Appelt and S. T. Freer and J. E. Villafranca},
  journal={Protein Eng},
  volume={8},
  number={},
  pages={677-691},
  year={1995},
  publisher={}
}

@article{Eldridge:1997,
  title={Empirical scoring functions: I. The development of a fast empirical scoring function to estimate the binding affinity of ligands in receptor complexes.},
  author={M. D. Eldridge and C. W. Murray and T. R. Auton and G. V. Paolini and R. P. Mee},
  journal={J. Comput. Aided. Mol. Des},
  volume={11},
  number={},
  pages={425-445},
  year={1997},
  publisher={}
}


@article{WangRenXiao:2002,
  title={Further development and validation of empirical scoring functions for structure based binding affinity prediction},
  author={R. Wang and L. Lai and S. Wang},
  journal={J. Comput. Aided. Mol. Des},
  volume={16},
  number={},
  pages={11-26},
  year={2002},
  publisher={}
}

@article{Baum:2010,
  title={Non-additivity of functional group contributions in protein-ligand binding: a comprehensive study by crystallography and isothermal titration calorimetry},
  author={B. Baum and L. Muley and M. Smolinski and A. Heine and D. Hangauer and G. Klebe},
  journal={J. Mol. Bio},
  volume={397},
  number={4},
  pages={1042-1054},
  year={2010},
  publisher={}
}

@article{Sarah:2011,
  title={A machine learning based method to improve docking scoring functions and its application to drug repurposing},
  author={Sarah L. Kinnings and Nina Liu and Peter J. Tonge and Richard M. Jackson and Lei Xie and Philip E. Bourne},
  journal={Journal of Chemical Information and Model},
  volume={51},
  number={2},
  pages={408-419},
  year={2011},
  publisher={}
}

@article{Ashtawy:2012,
  title={A Comparative Assessment of Ranking Accuracies of Conventional and Machine-Learning-Based Scoring Functions for Protein-Ligand Binding Affinity Prediction},
  author={Hossam M. Ashtawy and Nihar R. Mahapatra},
  journal={IEEE/ACM Transactions on computational biology and bioinformatics},
  volume={9},
  number={5},
  pages={1301-1313},
  year={2012},
  publisher={}
}

@article{Zheng:2013KECSA,
  title={Development of the Knowledge-Based and Empirical Combined Scoring Algorithm {(KECSA)} To Score Protein-Ligand Interactions},
  author={Zheng, Zheng and Merz Jr, Kenneth M. },
  journal={Journal of Chemical Information and Model},
  volume={53},
  number={},
  pages={1073-1083},
  year={2013},
  publisher={}
}

@article{Zheng:2013MoveableType,
  title={The Movable Type Method Applied to Protein-Ligand Binding},
  author={Zheng, Zheng and Ucisik, Melek N.  and Merz Jr, Kenneth M.},
  journal={Journal of Chemical Theory and Computation},
  volume={9},
  number={},
  pages={5526-5538},
  year={2013},
  publisher={}
}


@article{DrugScore:2005,
  title={Knowledge-Based Scoring Function Derived from Small Molecule Crystal Data with Superior Recognition Rate of Near-Native Ligand Poses and Better Affinity Prediction.},
  author={H. F. G. Velec and H. Gohlke and G. Klebe},
  journal={J. Med. Chem},
  volume={48},
  number={},
  pages={6296-6303},
  year={2005},
  publisher={}
}

@article{ITScore:2006,
  title={An iterative knowledge-based scoring function to predict protein-ligand interactions: I. Derivation of interaction potentials.},
  author={S. Y. Huang and X. Zou},
  journal={J. Comput. Chem.},
  volume={27},
  number={},
  pages={1865-1875},
  year={2006},
  publisher={}
}

@article{Wassermann:2009,
  title={Searching for target-selective compounds using different combinations of multiclass support vector machine ranking methods, kernel functions, and fingerprint descriptors.},
  author={A. M. Wassermann and H. Geppert and J. R. Bajorath},
  journal={Journal of Chemical Information and Model},
  volume={49},
  number={3},
  pages={582-92},
  year={2009},
  publisher={}
}



@article{Wale:2009,
  title={Target Fishing for Chemical Compounds Using Target-Ligand Activity Data and Ranking Based Methods.},
  author={Wale, N. and Karypis, G.},
  journal={Journal of Chemical Information and Model},
  volume={49},
  number={10},
  pages={2190-201},
  year={2009},
  publisher={}
}


@article{Kollman:2000ACR,
  title={Calculating structures and free energies of complex molecules: combining molecular mechanics and continuum models.},
  author={P. A. Kollman and I. Massova and C. Reyes and B. Kuhn and S.H. Huo and L. Chong and M. Lee and T. Lee and Y. Duan and W. Wang and O. Donini and P. Cieplak and J. Srinivasan and D. A. Case and T. E. Cheatham},
  journal={Acc. Chem. Res},
  volume={33},
  number={},
  pages={889-897},
  year={2000},
  publisher={}
}


@article{Greenidge:2012,
  title={{MM/GBSA} Binding Energy Prediction on the { PDBBind} Data Set: Successes, Failures, and Directions for Further Improvement.},
  author={Paulette A. Greenidge and Christian Kramer and Jean-Christophe Mozziconacci and Romain M. Wolf},
  journal={Journal of Chemical Information and Model},
  volume={53},
  number={},
  pages={201-209},
  year={2013},
  publisher={}
}


@article{Cao:2014Cyscore,
  title={Improved protein-ligand binding affinity prediction by using a curvature-dependent surface-area model.},
  author={Y Cao and L Li},
  journal={Bioinformatics},
  volume={30},
  number={12},
  pages={1674-1680},
  year={2014},
  publisher={}
}

@article{Trott:2010AutoDock,
  title={{AutoDock Vina}: improving the speed and accuracy of docking with a new scoring function, efficient optimization, and multithreading},
  author={O. Trott and A. J. Olson},
  journal={J Computat Chem},
  volume={31},
  number={2},
  pages={455-461},
  year={2010},
  publisher={}
}

@article{Friesner:2004Schrodinger,
  title={Glide: a new approach for rapid, accurate docking and scoring. 1. Method and assessment of docking accuracy.},
  author={R. A. Friesner and J. L. Banks and R. B. Murphy and T. A. Halgren and J. J. Klicic and D. T. Mainz and M. P. Repasky and E. H. Knoll and M Shelley and J. K. Perry JK and D. E. Shaw and P. Francis and P. S. Shenkin},
  journal={J. Med. Chem.},
  volume={47},
  number={},
  pages={1739},
  year={2004},
  publisher={}
}


@article{Madhavi:2013Schrodinger,
  title={Protein and ligand preparation: parameters, protocols, and influence on virtual screening enrichments.},
  author={G. Madhavi Sastry and Matvey Adzhigirey and Tyler Day and Ramakrishna Annabhimoju and Woody Sherman},
  journal={J. Comput. Aid. Mol. Des.},
  volume={27},
  number={},
  pages={221-234},
  year={2013},
  publisher={}
}

@article{Michal:2011Schrodinger,
  title={Graphical analysis of {pH-dependent} properties of proteins predicted using {PROPKA}},
  author={Michal Rostkowski and Mats HM Olsson and Chresten R Sondergaard and Jan H Jensen},
  journal={BMC Structural Biology},
  volume={11},
  number={6},
  pages={},
  year={2011},
  publisher={}
}

@article{Olsson:2011Schrodinger,
  title={{PROPKA3:} Consistent Treatment of Internal and Surface Residues in Empirical pKa Predictions.},
  author={Mats H. M. Olsson and Chresten R. Sondergaard and Michal Rostkowski and Jan H. Jensen},
  journal={J. Chem. Theory Comput.},
  volume={7},
  number={2},
  pages={525-537},
  year={2011},
  publisher={}
}

@article{OPLS:1988,
  title={The {OPLS} optimized potentials for liquid simulations] potential functions for proteins, energy minimizations for crystals of cyclic peptides and crambin.},
  author={William L. Jorgensen and Julian. Tirado-Rives},
  journal={J. Am. Chem. Soc.},
  volume={110},
  number={6},
  pages={1657-1666},
  year={1988},
  publisher={}
}


@article{OPLS:2001,
  title={Evaluation and Reparametrization of the {OPLS-AA} Force Field for Proteins via Comparison with Accurate Quantum Chemical Calculations on Peptides.},
  author={George A. Kaminski and Richard A. Friesner and Julian Tirado-Rives and William L. Jorgensen},
  journal={The Journal of Physical Chemistry B},
  volume={105},
  number={28},
  pages={6474-6487},
  year={2001},
  publisher={}
}

@article{ITScoreSE:2010,
  title={Inclusion of Solvation and Entropy in the Knowledge-Based Scoring Function for Protein-Ligand Interactions.},
  author={Sheng-You Huang and Xiaoqin Zou},
  journal={J. Chem. Inf. Model.},
  volume={50},
  number={2},
  pages={262-273},
  year={2010},
  publisher={}
}


}

@article{XScore:2002,
  title={Further development and validation of empirical scoring functions for structural based binding affinity prediction.},
  author={R. Wang and L. Lai and S. Wang},
  journal={J. Comput-Aided Mol. Des},
  volume={16},
  number={},
  pages={11-26},
  year={2002},
  publisher={}
}

@article{DFIRE:2005,
  title={A knowledge-based energy function for protein-ligand, protein-protein, and protein-DNA complexes.},
  author={C Zhang and S Liu and Q Zhu and Y Zhou},
  journal={J Med Chem.},
  volume={48},
  number={7},
  pages={2325-35},
  year={2005},
  publisher={}
}

@article{DrugScoreCSD:2005,
  title={{DrugScore (CSD)}-knowledge-based scoring function derived from small molecule  crystal data with superior recognition rate of near-native ligand poses and better affinity prediction.},
  author={HF Velec and H Gohlke and G Klebe},
  journal={J Med Chem.},
  volume={48},
  number={20},
  pages={6296-303},
  year={2005},
  publisher={}
}

@article{DrugScorePDB:2000,
  title={Knowledge-based scoring function to predict protein-ligand interactions.},
  author={H Gohlke and M Hendlich and G Klebe},
  journal={J Mol Biol.},
  volume={295},
  number={2},
  pages={337-356},
  year={2000},
  publisher={}
}

@article{Cerius2:PLP1,
  title={Molecular recognition of the inhibitor {AG-1343} by {HIV-1} protease: conformationally flexible docking by evolutionary programming.},
  author={DK Gehlhaar and GM Verkhivker and PA Rejto and CJ Sherman and DB Fogel and LJ Fogel and ST Freer},
  journal={Chem Biol.},
  volume={2},
  number={5},
  pages={317-324},
  year={1995},
  publisher={}
}


@article{G-Score,
  title={Development and validation of a genetic algorithm for flexible docking.},
  author={Gareth Jones and Peter Willett and Robert C Glen and  Andrew R Leach and Robin Taylor},
  journal={Journal of Molecular Biology},
  volume={267},
  number={3},
  pages={727-748},
  year={1997},
  publisher={}
}

@article{D-Score,
  title={Automated docking with grid-based energy evaluation},
  author={Elaine C. Meng and Brian K. Shoichet and Irwin D. Kuntz},
  journal={Journal of Computational Chemistry},
  volume={13},
  number={},
  pages={505-524},
  year={1992},
  publisher={}
}


@article{AutoDock:1998,
  title={Automated Docking Using a Lamarckian Genetic Algorithm and an Empirical Binding Free Energy Function},
  author={Morris, G. M. and  Goodsell, D. S. and  Halliday, R. S. and Huey, R. and Hart, W. E. and Belew, R. K. and Olson, A. J.},
  journal={Journal of Computational Chemistry},
  volume={19},
  number={},
  pages={1639-62},
  year={1998},
  publisher={}
}

@article{PMFScore:1999,
  title={A general and fast scoring function for protein-ligand interactions: a simplified potential approach.},
  author={I Muegge and YC Martin},
  journal={J Med Chem.},
  volume={42},
  number={5},
  pages={791-804},
  year={1999},
  publisher={}
}


@article{F-Score,
  title={A fast flexible docking method using an incremental construction algorithm.},
  author={M Rarey and B Kramer and T Lengauer and G Klebe},
  journal={J Mol Biol.},
  volume={261},
  number={3},
  pages={470-489},
  year={1996},
  publisher={}
}


@article{CERIUS2:2000,
  title={{CERIUS2  LigandFit User Manual; Accelrys, Inc.: San Deigo, CA}},
  author={},
  journal={},
  volume={},
  number={},
  pages={3-48},
  year={2000},
  publisher={}
}

@article{CERIUS2LUDI,
  title={The development of a simple empirical scoring function to estimate the binding constant for a protein-ligand complex of known three-dimensional structure},
  author={H. J. Bohm},
  journal={Journal of Computer-Aided Molecular Design},
  volume={8},
  number={},
  pages={234-256},
  year={1994},
  publisher={}
}

@article{istar:2014,
  title={{iStar: A} Web Platform for Large-Scale Protein-Ligand Docking},
  author={H. Li and K.S. Leung and P.J. Ballester and M. H. Wong},
  journal={Plos One},
  volume={9},
  number={1},
  pages={},
  year={2014},
  publisher={}
}

@ARTICLE{HongJianLi:2015,
  AUTHOR =       {Hongjian Li and Kwong-Sak Leung and Man-Hon Wong  and Pedro J. Ballester},
  TITLE =        {{Low-Quality Structural and Interaction Data Improves Binding Affinity Prediction via Random Forest}},
  JOURNAL =      {Molecules},
  YEAR =         {2015},
  volume =       {20},
  pages =        {10947-10962},
}

@article{IDScore:2013,
  title={{ID-Score: A} New Empirical Scoring Function Based on a Comprehensive Set of Descriptors Related to Protein–Ligand Interactions},
  author={Guo-Bo Li and Ling-Ling Yang and Wen-Jing Wang and Lin-Li Li and Sheng-Yong Yang},
  journal={J. Chem. Inf. Model.},
  volume={53},
  number={3},
  pages={592-600},
  year={2013},
  publisher={}
}


@article{Pedro:2012New,
  title={Machine learning scoring functions based on random forest and support vector regression},
  author={Pedro J. Ballester},
  journal={Proceedings of the 7th IAPR international conference on Pattern Recognition in Bioinformatics},
  volume={},
  number={},
  pages={14-25},
  year={2012},
  publisher={}
}

@article{RenxiaoWang:2009Compare,
  title={Comparative Assesment of Scoring Functions on a Diverse Test Set},
  author={T. Cheng and X. Li and Y. Li and Z. Liu and R. Wang},
  journal={J. Chem. Inf. Model.},
  volume={49},
  number={},
  pages={1079-1093},
  year={2009},
  publisher={}
}

@article{Jorgensen:1991,
  title={Rusting of the lock and key model for protein-ligand binding},
  author={Jorgensen, W. L.},
  journal={Science},
  volume={254},
  number={},
  pages={954-955},
  year={1991},
  publisher={}
}


@article{Bursulaya:2003,
  title={Comparative study of several algorithms for flexible ligand docking},
  author={Bursulaya, B. D. and  Totrov, M. and  Abagyan, R. and Brooks, C. L.},
  journal={Journal of Computer-Aided Molecular Design},
  volume={17},
  number={},
  pages={755-763},
  year={2003},
  publisher={}
}

@article{Goodsell:1990,
  title={Automated docking of substrates to proteins by simulated
annealing},
  author={Goodsell,  D. S. and Olson, A. J.},
  journal={Protein Struct. Funct. Genet. },
  volume={8},
  number={},
  pages={195-202},
  year={1990},
  publisher={}
}

@article{DesJarlais:1986,
  title={ Docking flexible ligands to macromolecular receptors by molecular shape},
  author={DesJarlais, R. L. and  Sheridan, R. P. and  Dixon,  J. S. and  Kuntz, I. D. and  Venkataraghavan, R.},
  journal={J. Med. Chem. },
  volume={29},
  number={},
  pages={2149-2153},
  year={1986},
  publisher={}
}


@article{Kuntz:1982,
  title={ A geometric approach to macromolecule-ligand interactions},
  author={Kuntz, I. D. and  Blaney, J. M. and Oatley, S. J. and Langridge, R. and Ferrin, T. E.},
  journal={ J. Mol. Biol.},
  volume={161},
  number={},
  pages={269-288},
  year={1982},
  publisher={}
}

@article{ListNet:2007,
  title={ Learning to Rank: From Pairwise Approach to Listwise Approach},
  author={Cao, Z. and  Qin, T. and Liu, T. Y. and Tsai, M. F. and Li, F.},
  journal={ICML},
  volume={},
  number={},
  pages={},
  year={2007},
  publisher={}
}


%%%%%%%%%%%%%%%%%%% Kelin: AIM papers

@article{Bader:1985,
  title={Atoms in molecules},
  author={Bader, R. F.},
  journal={Accounts of Chemical Research},
  volume={18},
  number={1},
  pages={9--15},
  year={1985},
  publisher={ACS Publications}
}

@book{Bader:1990,
  title={Atoms in molecules},
  author={Bader, R. F.},
  year={1990},
   publisher={Wiley Online Library}
}


@article{Silvi:1994,
  title={Classification of chemical bonds based on topological analysis of electron localization functions},
  author={Silvi, B. and Savin, A.},
  journal={Nature},
  volume={371},
  number={6499},
  pages={683--686},
  year={1994}
}

@article{Bader:1988,
  title={A physical basis for the {VSEPR} model of molecular geometry},
  author={Bader, R. F. and Gillespie, R. J. and MacDougall, P. J.},
  journal={Journal of the American Chemical Society},
  volume={110},
  number={22},
  pages={7329--7336},
  year={1988},
  publisher={ACS Publications}
}

@article{Leboeuf:1999,
  title={Topological analysis of the molecular electrostatic potential},
  author={Leboeuf, M. and K{\"o}ster, A. M. and Jug, K. and Salahub, D. R.},
  journal={The Journal of chemical physics},
  volume={111},
  number={11},
  pages={4893--4905},
  year={1999},
  publisher={AIP Publishing}
}

@article{Kohout:2004,
  title={Electron localizability indicator for correlated wavefunctions. {I. Parallel-spin} pairs},
  author={Kohout, M. and Pernal, K. and Wagner, F. R. and Grin, Y.},
  journal={Theoretical Chemistry Accounts},
  volume={112},
  number={5-6},
  pages={453--459},
  year={2004},
  publisher={Springer}
}

@article{Schmider:2000,
  title={Chemical content of the kinetic energy density},
  author={Schmider, H. L. and Becke, A. D.},
  journal={Journal of Molecular Structure: THEOCHEM},
  volume={527},
  number={1},
  pages={51--61},
  year={2000},
  publisher={Elsevier}
}

@article{Keith:1996,
  title={Structural homeomorphism between the electron density and the virial field},
  author={Keith, T. A. and Bader, R. F. and Aray, Y.},
  journal={International journal of quantum chemistry},
  volume={57},
  number={2},
  pages={183--198},
  year={1996},
  publisher={Wiley Online Library}
}

@article{Keith:1993,
  title={Topological analysis of magnetically induced molecular current distributions},
  author={Keith, T. A. and Bader, R. F.},
  journal={The Journal of chemical physics},
  volume={99},
  number={5},
  pages={3669--3682},
  year={1993},
  publisher={AIP Publishing}
}

@article{Mezey:1981,
  title={Catchment region partitioning of energy hypersurfaces,{I}},
  author={Mezey, P. G.},
  journal={Theoretica chimica acta},
  volume={58},
  number={4},
  pages={309--330},
  year={1981},
  publisher={Springer}
}

@article{Cioslowski:1999,
  title={Topology of electron-electron interactions in atoms and molecules. {II}. The correlation cage},
  author={Cioslowski, J. and Liu, G. H.},
  journal={The Journal of chemical physics},
  volume={110},
  number={4},
  pages={1882--1887},
  year={1999},
  publisher={AIP Publishing}
}

@incollection{Popelier:2005,
  title={Quantum chemical topology: on bonds and potentials},
  author={Popelier, P. L.},
  booktitle={Intermolecular forces and clusters I},
  pages={1--56},
  year={2005},
  publisher={Springer}
}

@article{Popelier:2000,
  title={Atoms in molecules},
  author={Popelier, P. L. and Aicken, F. M. and O'Brien, S. E.},
  journal={Chemical Modelling: Applications and Theory},
  volume={1},
  pages={143--198},
  year={2000},
  publisher={Royal Society of Chemistry Specialist Periodical Report}
}


@article{Gunther:2014b,
  title={Characterizing molecular interactions in chemical systems},
  author={G{\"u}nther, D. and Boto, R. A. and Contreras-Garcia, J. and Piquemal, J. P. and Tierny, J.},
  journal={IEEE transactions on visualization and computer graphics},
  volume={20},
  number={12},
  pages={2476--2485},
  year={2014},
  publisher={IEEE}
}

@article{Johnson:2010,
  title={Revealing noncovalent interactions},
  author={Johnson, E. R. and Keinan, S. and Mori-Sanchez, P. and Contreras-Garcia, J. and Cohen, A. J. and Yang, W.T.},
  journal={Journal of the American Chemical Society},
  volume={132},
  number={18},
  pages={6498--6506},
  year={2010},
  publisher={ACS Publications}
}

@inproceedings{kindlmann2003curvature,
  title={Curvature-based transfer functions for direct volume rendering: Methods and applications},
  author={Kindlmann, Gordon and Whitaker, Ross and Tasdizen, Tolga and Moller, Torsten},
  booktitle={Visualization, 2003. VIS 2003. IEEE},
  pages={513--520},
  year={2003},
  organization={IEEE}
}


@article{Gillet:2012,
  title={Coupling quantum interpretative techniques: another look at chemical mechanisms in organic reactions},
  author={Gillet, N. and Chaudret, R. and Contreras-Garc{\i}a, J. and Yang, W. T. and Silvi, B. and Piquemal, J. P.},
  journal={Journal of chemical theory and computation},
  volume={8},
  number={11},
  pages={3993--3997},
  year={2012},
  publisher={ACS Publications}
}

@article{Biegler:2002,
  title={Update of the {AIM}2000-Program for atoms in molecules},
  author={Biegler-K{\"o}nig, F. and Sch{\"o}nbohm, J.},
  journal={Journal of computational chemistry},
  volume={23},
  number={15},
  pages={1489--1494},
  year={2002},
  publisher={Wiley Online Library}
}

@article{Henkelman:2006,
  title={A fast and robust algorithm for {Bader} decomposition of charge density},
  author={Henkelman, G. and Arnaldsson, A. and J{\'o}nsson, H.},
  journal={Computational Materials Science},
  volume={36},
  number={3},
  pages={354--360},
  year={2006},
  publisher={Elsevier}
}

@inproceedings{Beketayev:2011,
  title={Topology-based Visualization of Transformation Pathways in Complex Chemical Systems},
  author={Beketayev, K. and Weber, G. H. and Haranczyk, M. and Bremer, P.T. and Hlawitschka, M. and Hamann, B.},
  booktitle={Computer Graphics Forum},
  volume={30},
  number={3},
  pages={663-672},
  year={2011},
  organization={Wiley Online Library}
}

@article{Pendas:2003,
  title={Curvature of interatomic surfaces. I. Fundamentals},
  author={Pend{\'a}s, A. M. and Lua{\~n}a, V.},
  journal={The Journal of chemical physics},
  volume={119},
  number={15},
  pages={7633--7642},
  year={2003},
  publisher={AIP Publishing}
}

@article{Popelier:1996,
  title={On the differential geometry of interatomic surfaces},
  author={Popelier, P. L.},
  journal={Canadian journal of chemistry},
  volume={74},
  number={6},
  pages={829--838},
  year={1996},
  publisher={NRC Research Press}
}

@inproceedings{Verbeek:1993,
  title={Curvature and bending energy in digitized {2D and 3D} images},
  author={Verbeek, P. W. and Van Vliet, L. J.},
  booktitle={8th Scandinavian Conference on Image Analysis, Tromso, Norway},
  year={1993}
}

@article{Stokely:1992,
  title={Surface parametrization and curvature measurement of arbitrary {3-D} objects: five practical methods},
  author={Stokely, E. M. and Wu, S. Y.},
  journal={IEEE Transactions on pattern analysis and machine Intelligence},
  volume={14},
  number={8},
  pages={833--840},
  year={1992},
  publisher={IEEE Computer Society}
}

@article{Sander:1990,
  title={Inferring surface trace and differential structure from {3D} images},
  author={Sander, P. T. and Zucker, S. W.},
  journal={IEEE Transactions on Pattern Analysis and Machine Intelligence},
  volume={12},
  number={9},
  pages={833--854},
  year={1990},
  publisher={IEEE}
}

@BOOK{Kuhnel:2015,
  title={Differential Geometry: Curves-Surfaces-Manifolds, Student Math},
  publisher = {American mathematical Society},
  year = {2015},
  author={K{\"u}hnel, W.}
}

%%%%%%%%%%%%%%%%% spectral graph
@inproceedings{spielman2007spectral,
  title={Spectral graph theory and its applications},
  author={Spielman, D. A.},
  booktitle={48th Annual IEEE Symposium on Foundations of Computer Science {(FOCS'07)}},
  pages={29--38},
  year={2007},
  organization={IEEE}
}


@article{shi:2000,
  title={Normalized cuts and image segmentation},
  author={Shi, J. B. and Malik, J.},
  journal={{IEEE} Transactions on pattern analysis and machine intelligence},
  volume={22},
  number={8},
  pages={888--905},
  year={2000},
  publisher={IEEE}
}

@inproceedings{meila:2001,
  title={A random walks view of spectral segmentation},
  author={Meila, M. and Shi, J. B.},
  booktitle={In Tenth International Workshop on Artificial Intelligence and Statistics {AISTATS}},
  year={2001}
}

@article{ng:2002,
  title={On spectral clustering: {Analysis} and an algorithm},
  author={Ng, A. Y. and Jordan, M. I. and Weiss, Y.},
  journal={Advances in neural information processing systems},
  volume={2},
  pages={849--856},
  year={2002}
}

@inproceedings{azran:2006,
  title={A new approach to data driven clustering},
  author={Azran, A. and Ghahramani, Z.},
  booktitle={Proceedings of the 23rd international conference on Machine learning},
  pages={57--64},
  year={2006},
  organization={ACM}
}


@INPROCEEDINGS{zelnik:2005,
    author = {Lihi Zelnik-manor and Pietro Perona},
    title = {Self-tuning spectral clustering},
    booktitle = {Advances in Neural Information Processing Systems 17},
    year = {2004},
    pages = {1601--1608},
    publisher = {MIT Press}
}

%%%%%%%%%%%%%%%%%%%%%% Protein domain decomposition
@article{alexandrov:2003,
  title={{PDP}: protein domain parser},
  author={Alexandrov, N. and Shindyalov, I.},
  journal={Bioinformatics},
  volume={19},
  number={3},
  pages={429--430},
  year={2003}
}

@article{Guo:2003,
  title={Improving the performance of {DomainParser} for structural domain partition using neural network},
  author={Guo, J. T. and Xu, D. and Kim, D. and Xu, Y.},
  journal={Nucleic Acids Research},
  volume={31},
  number={3},
  pages={944--952},
  year={2003}
}

@article{holm:1996,
  title={Mapping the protein universe},
  author={Holm, L. and Sander, C.},
  journal={Science},
  volume={273},
  number={5275},
  pages={595},
  year={1996}
}

@article{SKundu:2004,
  title={Automatic domain decomposition of proteins by a {Gaussian} network model},
  author={Kundu, S. and Sorensen, D. C. and Phillips,  G. N.},
  journal={Proteins: Structure, Function, and Bioinformatics},
  volume={57},
  number={4},
  pages={725--733},
  year={2004}
}

@article{murzin:1995,
  title={{SCOP}: a structural classification of proteins database for the investigation of sequences and structures},
  author={Murzin, A. G. and Brenner, S. E. and Hubbard, T. and Chothia, C.},
  journal={Journal of molecular biology},
  volume={247},
  number={4},
  pages={536--540},
  year={1995}
}

@article{orengo:1997,
  title={{CATH}--a hierarchic classification of protein domain structures},
  author={Orengo, C. A. and Michie, A. D. and Jones, S. and Jones, D. T. and Swindells, M. B. and Thornton, J. M.},
  journal={Structure},
  volume={5},
  number={8},
  pages={1093--1109},
  year={1997}
}

@incollection{veretnik:2007,
  title={Computational methods for domain partitioning of protein structures},
  author={Veretnik, S. and Shindyalov, I.},
  booktitle={Computational Methods for Protein Structure Prediction and Modeling},
  pages={125--145},
	publisher={Springer New York},
  year={2007}
}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% Protein Interaction Map

@article{rain:2001,
  title={The protein-protein interaction map of {Helicobacter} pylori},
  author={Rain, J. C. and Selig, L. and De Reuse, H. and Battaglia, V. and Reverdy, C. and Simon, S. and Lenzen, G. and Petel, F. and Wojcik, J. and Sch{\"a}chter, V. and Chemama, Y. and Labigne, A. and Legrain, P.},
  journal={Nature},
  volume={409},
  number={6817},
  pages={211--215},
  year={2001}
}

@article{giot:2003,
  title={A protein interaction map of drosophila melanogaster},
  author={Giot, L. and Bader, J. S. and Brouwer, C. and Chaudhuri, A. and Kuang, B. and Li, Y. and Hao, Y.L. and Ooi, C.E. and Godwin, B. and Vitols, E. and others},
  journal={science},
  volume={302},
  number={5651},
  pages={1727--1736},
  year={2003}
}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% metabolic networks

@article{jeong:2000,
  title={The large-scale organization of metabolic networks},
  author={Jeong, H. and Tombor, B. and Albert, R. and Oltvai, Z. N. and Barab{\'a}si, A. L.},
  journal={Nature},
  volume={407},
  number={6804},
  pages={651--654},
  year={2000}
}

@article{overbeek:2000,
  title={{WIT}: integrated system for high-throughput genome sequence analysis and metabolic reconstruction},
  author={Overbeek, R. and Larsen, N. and Pusch, G. D. and D’Souza, M. and Selkov Jr, E. and Kyrpides, N. and Fonstein, M. and Maltsev, N. and Selkov, E.},
  journal={Nucleic Acids Research},
  volume={28},
  number={1},
  pages={123--125},
  year={2000}
}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% Transcriptional regulatory networks

@article{lee:2002,
  title={Transcriptional regulatory networks in Saccharomyces cerevisiae},
  author={Lee, T. I. and Rinaldi, N. J. and Robert, F. and Odom, D. T. and Bar-Joseph, Z. and Gerber, G. K. and Hannett, N. M. and Harbison, C. T. and Thompson, C. M. and Simon, I. and others},
  journal={science},
  volume={298},
  number={5594},
  pages={799--804},
  year={2002}
}

@article{salgado:2006,
  title={The comprehensive updated regulatory network of Escherichia coli K-12},
  author={Salgado, H. and Santos-Zavaleta, A. and Gama-Castro, S. and Peralta-Gil, M. and Pe{\~n}aloza-Sp{\'\i}nola, M. I. and Mart{\'\i}nez-Antonio, A. and Karp, P. D. and Collado-Vides, J.},
  journal={BMC bioinformatics},
  volume={7},
  number={1},
  pages={1},
  year={2006}
}

%%%%%%%%%%%%%%%%%% DNA KNOT

@book{vologodskii:1992,
  title={Topology and Physics of Circular {DNA}},
  author={Vologodskii, A.},
  year={1992},
  publisher={CRC Press}
}

@article{pohl:1980,
  title={{DNA} and differential geometry},
  author={Pohl, W. F.},
  journal={The Mathematical Intelligencer},
  volume={3},
  number={1},
  pages={20--27},
  year={1980}
}

@article{fuller:1971,
  title={The writhing number of a space curve},
  author={Fuller, F. B.},
  journal={Proceedings of the National Academy of Sciences},
  volume={68},
  number={4},
  pages={815--819},
  year={1971}
}

@book{ABates:2005,
  title={{DNA} topology},
  author={Bates, A. D. and Maxwell, A.},
  year={2005},
  publisher={Oxford University Press, USA}
}

@inproceedings{sumners:1992,
  title={Knot theory and {DNA}},
  author={Sumners, D. W.},
  booktitle={Proceedings of Symposia in Applied Mathematics},
  volume={45},
  pages={39--72},
  year={1992}
}

@article{darcy:2001,
  title={Biological distances on {DNA} knots and links: applications to {XER} recombination},
  author={Darcy, I. K.},
  journal={Journal of Knot Theory and its Ramifications},
  volume={10},
  number={02},
  pages={269--294},
  year={2001},
  publisher={World Scientific}
}

@article{arsuaga:2002,
  title={Knotting probability of {DNA} molecules confined in restricted volumes: {DNA} knotting in phage capsids},
  author={Arsuaga, J. and V{\'a}zquez, M. and Trigueros, S. and Sumners, D. W. and Roca, J.},
  journal={Proceedings of the National Academy of Sciences},
  volume={99},
  number={8},
  pages={5373--5377},
  year={2002},
  publisher={National Acad Sciences}
}

@article{buck:2007,
  title={Predicting knot or catenane type of site-specific recombination products},
  author={Buck, D. and Flapan, E.},
  journal={Journal of molecular biology},
  volume={374},
  number={5},
  pages={1186--1199},
  year={2007},
  publisher={Elsevier}
}

%%%%%%%%%%%%% Mapper

@inproceedings{singh:2007,
  title={Topological Methods for the Analysis of High Dimensional Data Sets and { 3D} Object Recognition.},
  author={Singh, G. and M{\'e}moli, F. and Carlsson, G. E.},
  booktitle={SPBG},
  pages={91--100},
  year={2007}
}

@article{Gameiro:2013,
title={Topological measurement of protein compressibility via persistence diagrams},
author={Gameiro, M. and Hiraoka, Y. and Izumi, S. and Kramar, M. and Mischaikow, K. and Nanda, V.},
journal={preprint},
year = {2013},
}

@article{Kovacev-Nikolic:2016,
title={Using persistent homology and dynamical  distances to analyze protein binding},
author={Violeta Kovacev-Nikolic and  Peter Bubenik and Dragan Nikoli\'c  and Giseon Heo},
journal={Stat. Appl. Genet. Mol. Biol.},
volume={15},
number={1},
pages={19--38},
year = {2016},
}


% added by Duan Chen 06/27

@Misc{UofIwebsite,
author = {University of Illinois at Urbana-Champaign},
title = {KcsA Potassium Channel.},
howpublished = {Online},
}

@Article{Egwolf-Roux-2010,
author = {{Egwolf, B.} and { Roux, B.}},
title={Ion selectivity of the KcsA channel: A perspective from multi-ion free energy landscapes},
journal = {J. Chem. Phys.},
volume = {401},
year = {2010},
pages = {831-842}
}

@ARTICLE{lixf:2014,
  AUTHOR =       {Flavell, Alan and Machen, Michael and Eisenberg, Bob and Kabre, Julienne and Liu, Chun and Li, Xiaofan},
  TITLE =        {{A Conservative Finite Difference Scheme for Poisson-Nernst-Planck Equations}},
  JOURNAL =      {Journal of Computational Electronics},
  YEAR =         {2014},
  volume =       {13},
  pages =        {235-249},
}

@ARTICLE{xied:2013,
  AUTHOR =       {Xie, D. and Jiang, Y. and Scott, L. R.},
  TITLE =        {{Efficient algorithms for solving a nonlocal dielectric model for protein in ionic solvent}},
  JOURNAL =      {SIAM Journal on Scientific Computing },
  YEAR =         {2013},
  volume =       {38 },
  pages =        {B1267-1284},
}

@ARTICLE{lintc:2014,
  AUTHOR =       {Lin, Tai-Chia and Eisenberg, Bob},
  TITLE =        {{A new approach to the Lennard-Jones potential and a new model: PNP-steric equations}},
  JOURNAL =      {Communications in Mathematical Sciences},
  YEAR =         {2014},
  volume =       {12},
  pages =        {149-173},

}@ARTICLE{liujl:2014,
  AUTHOR =       {Liu, Jinn-Liang and Eisenberg, Bob},
  TITLE =        {{Poisson-Nernst-Planck-Fermi Theory for Modeling Biological Ion Channels}},
  JOURNAL =      {Journal of Chemical Physics},
  YEAR =         {2014},
  volume =       {141},
  pages =        {22D532},
}
@ARTICLE{lub:2014,
  AUTHOR =       {Li, Hanlin and Lu, Benzhuo},
  TITLE =        {{An ionic concentration and size dependent dielectric permittivity Poisson-Boltzmann model for biomolecular solvation studies}},
  JOURNAL =      {J. Chem. Phys.},
  YEAR =         {2014},
  volume =       {141 },
  pages =        {024115},
}

@ARTICLE{Harguindey:2009,
  AUTHOR =       {Harguindey, Salvador and Arranz, Jose and Wahl, Miriam and Orives, Gorka and Reshkin, Stephan},
  TITLE =        {{Proton Transport Inhibitors as Potentially Selective Anticancer Drugs}},
  JOURNAL =      {Anticancer Research},
  YEAR =         {2009},
  volume =       {29},
  pages =        {2127-2136},
}
@ARTICLE{Chandra:2000,
  AUTHOR =       {Chandra, Amalendu },
  TITLE =        {{Static dielectric constant of aqueous electrolyte solutions: Is there any dynamic contribution?}},
  JOURNAL =      {Journal of Chemical Physics},
  YEAR =         {2000},
  volume =       {113},
  pages =        {903-905},
}

@ARTICLE{Ben-Yaakov:2011b,
  AUTHOR =       {Ben-Yaakov, D. and Andelman, D.  and Podgornik, R. and Podgornik, R.},
  TITLE =        {{Ion-specific hydration effects: Extending the Poisson-Boltzmann theory}},
  JOURNAL =      {Current Opinion in Colloid and Interface Science},
  YEAR =         {2011},
  volume =       {16},
  pages =        {542-550},
}


@ARTICLE{DuanChen:2016c,
  AUTHOR =       {Duan Chen},
  TITLE =        {{A New Poisson-Nernst-Planck Model with Ion-Water Interactions for Charge Transport in Ion Channels}},
  JOURNAL =      {Bulletin of Mathematical Biology},
  YEAR =         {2016},
  volume =       { },
  pages =        {accepted},
}

@ARTICLE{HH:1952,
  AUTHOR =       {Hodgkin, A. L. and Huxley, A. F.},
  TITLE =        {{A quantitative description of membrane current and its application to conduction and excitation in nerve.}},
  JOURNAL =      {The Journal of Physiology},
  YEAR =         {1952},
  volume =       { 117},
  pages =        {500-544},
}


@ARTICLE{ZhouHX:2014,
  AUTHOR =       {Dai, J. and Zhou, H.-X.},
  TITLE =        {{General rules for the arrangements and gating motions of pore-lining helices in homomeric ion channels.}},
  JOURNAL =      {Nat. Commun.},
  YEAR =         {2014},
  volume =       { 5},
  pages =        {4641},
}

@ARTICLE{ZhouHX:2013,
  AUTHOR =       {Heymann, G. and Dai, J. and Li, M. and Silberberg, S. D.  and Zhou, H.-X. and Swartz, K. J.},
  TITLE =        {{Inter- and intrasubunit interactions between transmembrane helices in the open state of P2X receptor channels.}},
  JOURNAL =      {Proc. Natl. Acad. Sci. USA},
  YEAR =         {2013},
  volume =       { 110},
  pages =        {E4045-E4054},
}


@ARTICLE{CaiW:2013,
  AUTHOR =       {Lin, Humin and Cho, Min-Hyung and Tang, Huazhong and Cai, Wei},
  TITLE =        {{icBIE: A Boundary Integral Equation Program for an Ion Channel in Layered Membrane/Electrolyte Media.}},
  JOURNAL =      {Computer Physics Communications},
  YEAR =         {2013},
  volume =       {},
  pages =        {To appear},
}

@ARTICLE{CaiW:2016,
  AUTHOR =       {Baker, K. and Chen, D. and Cai, Wei},
  TITLE =        {{Investigating the Selectivity of KcsA Channel by an Image Charge Solvation Method (ICSM) in Molecular Dynamics Simulations.}},
  JOURNAL =      {Communications in Computational Physics},
  YEAR =         {2016},
  volume =       {19},
  pages =        {927-943},
}

@ARTICLE{ShawD:2012,
  AUTHOR =       {Jensen, Morten and Jogini, Vishwanath and Borhani, David and Leffler, Abba and Dror, Ron and Shaw, David},
  TITLE =        {{Mechanism of Voltage Gating in Potassium Channels.}},
  JOURNAL =      {Science},
  YEAR =         {2012},
  volume =       {336},
  pages =        {229-233},
}

@ARTICLE{Bezanilla:2015,
  AUTHOR =       {Labro, Alain and Priest, Michael and Lacroix, Jerome and Snyders, Dirk and Bezanilla, Francisco},
  TITLE =        {{ K$_v$3.1 uses a timely resurgent  K$^+$ current to secure action potential repolarization}},
  JOURNAL =      {Nature communications},
  YEAR =         {2015},
  volume =       {6},
  pages =        {10173},
}

@ARTICLE{Catterall:2014,
  AUTHOR =       {Fu, Ying and Westenbroek, Ruth and Scheuer, Todd and Catterall, Willliam},
  TITLE =        {{Basal and $\beta$-adrenergic regulation of the cardiac calcium channel $\rm Ca_V 1.2$ requires phosphorylation of serine 1700.}},
  JOURNAL =      {Proc Natl Acad Sci USA},
  YEAR =         {2014},
  volume =       {111},
  pages =        {16598-16603},
}


@ARTICLE{MacKinnon:2014,
  AUTHOR =       {Brohawn, S.G. and Campbell, E.B. and MacKinnon, R.},
  TITLE =        {{Physical mechanism for gating and mechanosensitivity of the human TRAAK $K^+$ channel.}},
  JOURNAL =      {Nature},
  YEAR =         {2014},
  volume =       {516},
  pages =        {126-30},
}


@ARTICLE{DeCoursey:2014,
  AUTHOR =       {Hondares, E. and Brown, M. A. and Musset, B and Morgan, D. and  Cherny, V. V. and Taubert, C. and Bhamrah, M. K. and Coe, D. and Marelli-Berg, F. and Gribben, J.G. and Dyer,  M. J. and DeCoursey, T. E. and Capasso, M.},
  TITLE =        {{Enhanced activation of an amino-terminally truncated isoform of the voltage-gated proton channel HVCN1 enriched in malignant B cells.}},
  JOURNAL =      {Proc Natl Acad Sci USA.},
  YEAR =         {2014},
  volume =       {111},
  pages =        {18078-83},
}


@ARTICLE{ZhouHX:2015,
  AUTHOR =       {Dai, Jian and Wollmuth, Lonnie, P. and Zhou, Huan-Xiang},
  TITLE =        {{Mechanism-Based Mathematical Model for Gating of Ionotropic Glutamate Receptors.}},
  JOURNAL =      {J. Phys. Chem. B},
  YEAR =         {2015},
  volume =       {119},
  pages =        {10934-10940},
}


@ARTICLE{Lu:2011,
  AUTHOR =       {Lu, Benzhuo and Zhou, Y. C.},
  TITLE =        {{Poisson-Nernst-Planck Equations for Simulating Biomolecular Diffusion-Reaction Processes II: Size Effects on Ionic Distributions
and Diffusion-Reaction Rates}},
  JOURNAL =      {Biophysical Journal},
  YEAR =         {2011},
  volume =       {100},
  pages =        {2475-2485},
}

@ARTICLE{YMiao:2015,
  AUTHOR =       { Y. Miao and R. Fu and H.-X. Zhou and T. A. Cross },
  TITLE =        {{Dynamic short hydrogen bonds in histidine tetrad of full length M2 proton channel reveal tetrameric structural heterogeneity and functional mechanism}},
  JOURNAL =      {Structure},
  YEAR =         {2015},
  volume =       {23},
  pages =        {2300-2308},
}

@ARTICLE{HDong:2013,
  AUTHOR =       { H. Dong and M. Yi and T.A. Cross and H.-X. Zhou },
  TITLE =        {{Ab initio calculations and validation of the pH-dependent structures of the His37-Trp41 quartet, the heart of acid activation and proton conductance in the M2 protein of Influenza A virus}},
  JOURNAL =      {Chem. Sci.},
  YEAR =         {2013},
  volume =       {4},
  pages =        {2776-2787},
}


@ARTICLE{TACross:2012,
  AUTHOR =       { T. A. Cross and H. Dong and M. Sharma and D. D. Busath and H.-X. Zhou },
  TITLE =        {{ M2 protein from influenza A: from multiple structures to biophysical and functional insights}},
  JOURNAL =      {Curr. Opin. Virol.},
  YEAR =         {2012},
  volume =       {2},
  pages =        {128-133},
}


@ARTICLE{HXZhou:2011,
  AUTHOR =       { H.-X. Zhou },
  TITLE =        {{ A theory for the proton transport of the influenza virus M2 protein: extensive test against conductance data}},
  JOURNAL =      { Biophys.},
  YEAR =         {2011},
  volume =       {100},
  pages =        {912-921},
}


@ARTICLE{DMeng:2014,
  AUTHOR =       { Meng, D. and  Zheng, B. and  Lin, G. and  Sushko, M. L. },
  TITLE =        {{ Numerical Solution of 3D Poisson-Nernst-Planck Equations Coupled with Classical Density Functional Theory for Modeling Ion and Electron Transport in a Confined Environment}},
  JOURNAL =      {Communications in Computational Physics },
  YEAR =         {2014},
  volume =       {16},
  pages =        { 1298-1322 },
}



@ARTICLE{LiuHL:2014,
  AUTHOR =       {Liu, Hailiang and Wang, Zhongming},
  TITLE =        {{ A free energy satisfying finite difference method for Poisson-Nernst-Planck equations}},
  JOURNAL =      {Journal of Computational Physics },
  YEAR =         {2014},
  volume =       {268},
  pages =        { 363-376 },
}

@ARTICLE{Xuzl:2014,
  AUTHOR =       {Xu,Zhenli and Ma, Manman and Liu, Pei},
  TITLE =        {{ Self-energy-modified Poisson-Nernst-Planck equations: WKB approximation and finite-difference approaches}},
  JOURNAL =      {Physical Review E},
  YEAR =         {2014},
  volume =       {90},
  pages =        {013307},
}


 @ARTICLE{Chaudhry:2014,
  AUTHOR =       {Chaudhry, Jehanzeb Hameed and Comer, Jeffrey and Aksimentiev, Aleksei and Olson, Luke N.},
  TITLE =        {{ A Stabilized Finite Element Method for Modified Poisson-Nernst-Planck Equations to Determine Ion Flow Through a Nanopore}},
  JOURNAL =      {Communications in Computational Physics},
  YEAR =         {2014},
  volume =       {15},
  pages =        {93-125},
}


@ARTICLE{Sunyz:2016,
  AUTHOR =       {Sun, Yuzhou and Sun, Pengtao and Zheng, Bin and Lin, Guang},
  TITLE =        {{ Error analysis of finite element method for Poisson-Nernst-Planck equations}},
  JOURNAL =      {Journal of Computational and Applied Mathematics},
  YEAR =         {2016},
  volume =       {301},
  pages =        {28-43},
}

@ARTICLE{Metti:2016,
  AUTHOR =       {Metti, Maximilian S. and Xu, Jinchao and Liu, Chun},
  TITLE =        {{Energetically stable discretizations for charge transport and electrokinetic models}},
  JOURNAL =      {Journal of Computational Physics},
  YEAR =         {2016},
  volume =       {306},
  pages =        {1-18},
}


@ARTICLE{Mascagni:2013,
  AUTHOR =       {Mackoy, Travis and Harris, Robert C. and Johnson, Jesse and Mascagni, Michael and Fenley, Marcia O.},
  TITLE =        {{Numerical Optimization of a Walk-on-Spheres Solver for the Linear Poisson-Boltzmann Equation}},
  JOURNAL =      {Communications in Computational Physics},
  YEAR =         {2013},
  volume =       {13},
  pages =        {195-206},
}

@ARTICLE{Jerome:1990,
  AUTHOR =       {Jerome, Joseph and Kerkhoven, Thomas},
  TITLE =        {{A Finite Element Approximation Theory for the Drift Diffusion Semiconductor Model}},
  JOURNAL =      {SIAM J. Numer. Anal},
  YEAR =         {1990},
  volume =       {28},
  pages =        {403-422},
}


@ARTICLE{Zinser:2016,
  AUTHOR =       {Ziner, Brian and Cai, Wei},
  TITLE =        {{A well-conditioned hypersingular boundary element method for electrostatic potentials in the presence of inhomogeneities within layered media}},
  JOURNAL =      {Communication in Computational Physics},
  YEAR =         {2016},
  volume =       {19},
  pages =        {970-997},
}

@ARTICLE{Mascagni:2007,
  AUTHOR =       {Simonov, Nikolai and Mascagni, Michael and Fenley Marcia O},
  TITLE =        {{Monte Carlo-based linear Poisson-Boltzmann approach makes accurate salt-dependent solvation free energy predictions possible}},
  JOURNAL =      {Journal of Chemical Physics},
  YEAR =         {2007},
  volume =       {127},
  pages =        {185105},
}


@ARTICLE{Zhangmj:2016,
  AUTHOR =       {Jia, Yusheng and Liu, Weishi and Zhang, Mingji},
  TITLE =        {{Qualitative properties of ionic flows via Poisson-Nernst-Planck systems with Bikerman's local hard-sphere potential: Ion size effects}},
  JOURNAL =      {Discrete and Continuous Dynamical Systems-series B},
  YEAR =         {2016},
  volume =       {21},
  pages =        {1775-1802},
}


@ARTICLE{Zhangmj:2015,
  AUTHOR =       {Zhang, Mingji},
  TITLE =        {{Asymptotic expansions and numerical simulations of I-V relations via a steady state Poisson-Nernst-Planck system}},
  JOURNAL =      {Rocky Mountain Journal of Mathematics},
  YEAR =         {2015},
  volume =       {45},
  pages =        {1681-1708},
}


@ARTICLE{lintc:2015,
  AUTHOR =       {Lin, Tai-Chia and Eisenberg, Bob},
  TITLE =        {{Multiple solutions of steady-state Poisson-Nernst-Planck equations with steric effects}},
  JOURNAL =      {Nonlinearity},
  YEAR =         {2015},
  volume =       {28},
  pages =        {2053-2080},
}


@ARTICLE{Xusx:2014,
  AUTHOR =       {Xu, Shixin and Sheng, Ping and Liu, Chun},
  TITLE =        {{An energetic variational approach for ion transport}},
  JOURNAL =      {Communications in Mathematical Sciences},
  YEAR =         {2014},
  volume =       {12},
  pages =        {779-789},
}

@ARTICLE{Qiaoyu:2014,
  AUTHOR =       {Qiao,Yu and Tu,Bin and Lu, Benzhuo},
  TITLE =        {{Ionic size effects to molecular solvation energy and to ion current across a channel resulted from the nonuniform size-modified PNP equations}},
  JOURNAL =      {Journal of Chemical Physics},
  YEAR =         {2014},
  volume =       {140},
  pages =        {174102},
}


@ARTICLE{Lu:2010,
  AUTHOR =       {Lu, Benzhuo and Holst, Michael and McCammon, J. Andrew and  Zhou, Y. C.},
  TITLE =        {{Poisson-Nernst-Planck Equations for Simulating Biomolecular Diffusion-Reaction Processes I:  Finite element solutions}},
  JOURNAL =      {Journal of Computational Physics},
  YEAR =         {2010},
  volume =       {229},
  pages =        {6979-6994},
}

%% End of Duan Chen's refs


@ARTICLE{JRBrender:2016,
  AUTHOR =       {J R Brender and   Y. Zhang},
  TITLE =        {{Predicting the Effect of Mutations on Protein-Protein Binding Interactions through Structure-Based Interface Profiles }},
  JOURNAL =      {PLoS Comput Biol. },
  YEAR =         {2016},
  volume =       {11},
  pages =        {e1004494 },
}

@ARTICLE{LJQuan:2016,
  AUTHOR =       {Lijun Quan  and Qiang Lv and   Yang Zhang},
  TITLE =        {{STRUM: Structure-based prediction of protein stability changes upon single-point mutation}},
  JOURNAL =      {  Bioinformatics },
  YEAR =         {in press 2016},
  volume =       { },
  pages =        {  },
}



@ARTICLE{JYing:2015,
  AUTHOR =       {Ying, Jinyong and Xie, Dexuan},
  TITLE =        {{A New Finite Element and Finite Difference Hybrid Method for Computing Electrostatics of Ionic Solvated Biomolecule}},
  JOURNAL =      { Journal of Computational Physics },
  YEAR =         {2015},
  volume =       { 298},
  pages =        { 636-651 },
}

@article{jiang2015frame,
  title={Frame field generation through metric customization},
  author={Jiang, Tengfei and Fang, Xianzhong and Huang, Jin and Bao, Hujun and Tong, Yiying and Desbrun, Mathieu},
  journal={ACM Transactions on Graphics (TOG)},
  volume={34},
  number={4},
  pages={40},
  year={2015},
  publisher={ACM}
}



@article{liu2015model,
  title={Model-reduced variational fluid simulation},
  author={Liu, Beibei and Mason, Gemma and Hodgson, Julian and Tong, Yiying and Desbrun, Mathieu},
  journal={ACM Transactions on Graphics (TOG)},
  volume={34},
  number={6},
  pages={244},
  year={2015},
  publisher={ACM}
}



@article{liu2016discrete,
  title={Discrete connection and covariant derivative for vector field analysis and design},
  author={Liu, Beibei and Tong, Yiying and Goes, Fernando De and Desbrun, Mathieu},
  journal={ACM Transactions on Graphics (TOG)},
  volume={35},
  number={3},
  pages={23},
  year={2016},
  publisher={ACM}
}



@inproceedings{de2016vector,
  title={Vector field processing on triangle meshes},
  author={de Goes, Fernando and Desbrun, Mathieu and Tong, Yiying},
  booktitle={ACM SIGGRAPH 2016 Courses},
  pages={27},
  year={2016},
  organization={ACM}
}



%%%%%% Duc added on 08/05/16 %%%%%%%%%%%%

@Article{Breiman:2001,
author="Breiman, Leo",
title="Random Forests",
journal="Machine Learning",
year="2001",
volume="45",
number="1",
pages="5--32",
abstract="Random forests are a combination of tree predictors such that each tree depends on the values of a random vector sampled independently and with the same distribution for all trees in the forest. The generalization error for forests converges a.s. to a limit as the number of trees in the forest becomes large. The generalization error of a forest of tree classifiers depends on the strength of the individual trees in the forest and the correlation between them. Using a random selection of features to split each node yields error rates that compare favorably to Adaboost (Y. Freund {\&} R. Schapire, Machine Learning: Proceedings of the Thirteenth International conference, ***, 148--156), but are more robust with respect to noise. Internal estimates monitor error, strength, and correlation and these are used to show the response to increasing the number of features used in the splitting. Internal estimates are also used to measure variable importance. These ideas are also applicable to regression.",
issn="1573-0565",
doi="10.1023/A:1010933404324",
url="http://dx.doi.org/10.1023/A:1010933404324"
}

@book{Breiman:1984,
  title={Classification and regression trees},
  author={Breiman, Leo and Friedman, Jerome and Stone, Charles J and Olshen, Richard A},
  year={1984},
  publisher={CRC press}
}

@article{Breiman:1996,
  title={Bagging predictors},
  author={Breiman, Leo},
  journal={Machine learning},
  volume={24},
  number={2},
  pages={123--140},
  year={1996},
  publisher={Springer}
}

@inproceedings{Ho:1995,
  title={Random decision forests},
  author={Ho, Tin Kam},
  booktitle={Document Analysis and Recognition, 1995., Proceedings of the Third International Conference on},
  volume={1},
  pages={278--282},
  year={1995},
  organization={IEEE}
}

@article{Ho:1998,
  title={The random subspace method for constructing decision forests},
  author={Ho, Tin Kam},
  journal={IEEE transactions on pattern analysis and machine intelligence},
  volume={20},
  number={8},
  pages={832--844},
  year={1998},
  publisher={IEEE}
}

@article{Amit:1997,
  title={Shape quantization and recognition with randomized trees},
  author={Amit, Yali and Geman, Donald},
  journal={Neural computation},
  volume={9},
  number={7},
  pages={1545--1588},
  year={1997},
  publisher={MIT Press}
}


@article{Guerts:2006,
  title={Extremely randomized trees},
  author={Geurts, Pierre and Ernst, Damien and Wehenkel, Louis},
  journal={Machine learning},
  volume={63},
  number={1},
  pages={3--42},
  year={2006},
  publisher={Springer}
}

@article{HLi:2015,
  title={Improving AutoDock Vina using random forest: the growing accuracy of binding affinity prediction by the effective exploitation of larger data sets},
  author={Li, Hongjian and Leung, Kwong-Sak and Wong, Man-Hon and Ballester, Pedro J},
  journal={Molecular Informatics},
  volume={34},
  number={2-3},
  pages={115--126},
  year={2015},
  publisher={Wiley Online Library}
}

@article{Dill:1997b,
  title={Additivity principles in biochemistry},
  author={Dill, Ken A},
  journal={Journal of Biological Chemistry},
  volume={272},
  number={2},
  pages={701--704},
  year={1997},
  publisher={ASBMB}
}
@article{YLi:2014,
  title={Comparative assessment of scoring functions on an updated benchmark: 2. Evaluation methods and general results},
  author={Li, Yan and Han, Li and Liu, Zhihai and Wang, Renxiao},
  journal={Journal of chemical information and modeling},
  volume={54},
  number={6},
  pages={1717--1736},
  year={2014},
  publisher={ACS Publications}
}

@InProceedings{Simba,
  author =	{Tamal K. Dey and Dayu Shi and Yusu Wang},
  title =	{{SimBa: An Efficient Tool for Approximating  Rips-Filtration Persistence via Simplicial Batch-Collapse}},
  booktitle =	{24th Annual European Symposium on Algorithms (ESA 2016)},
  pages =	{35:1--35:16},
  series =	{Leibniz International Proceedings in Informatics (LIPIcs)},
  ISBN =	{978-3-95977-015-6},
  ISSN =	{1868-8969},
  year =	{2016},
  volume =	{57},
  editor =	{Piotr Sankowski and Christos Zaroliagis},
  publisher =	{Schloss Dagstuhl--Leibniz-Zentrum fuer Informatik},
  address =	{Dagstuhl, Germany},
  URL =		{http://drops.dagstuhl.de/opus/volltexte/2016/6386},
  URN =		{urn:nbn:de:0030-drops-63869},
  doi =		{http://dx.doi.org/10.4230/LIPIcs.ESA.2016.35},
  annote =	{Keywords: Rips filtration, Homology groups, Persistence, Topological data analysis}
}

@inproceedings{DMW16,
  author    = {Tamal K. Dey and
               Facundo M{\'{e}}moli and
               Yusu Wang},
  title     = {Multiscale Mapper: Topological Summarization via Codomain Covers},
  booktitle = {Proceedings of the Twenty-Seventh Annual {ACM-SIAM} Symposium on Discrete
               Algorithms, {SODA} 2016, Arlington, VA, USA, January 10-12, 2016},
  pages     = {997--1013},
  year      = {2016},
  url       = {http://dx.doi.org/10.1137/1.9781611974331.ch71},
  doi       = {10.1137/1.9781611974331.ch71},
  timestamp = {Thu, 07 Apr 2016 12:20:54 +0200},
  biburl    = {http://dblp.uni-trier.de/rec/bib/conf/soda/DeyMW16},
  bibsource = {dblp computer science bibliography, http://dblp.org}
}

@inproceedings{WWL15new,
  author    = {Suyi Wang and
               Yusu Wang and
               Yanjie Li},
  title     = {Efficient map reconstruction and augmentation via topological methods},
  booktitle = {Proceedings of the 23rd {SIGSPATIAL} International Conference on Advances
               in Geographic Information Systems, Bellevue, WA, USA, November 3-6,
               2015},
  pages     = {25:1--25:10},
  year      = {2015},
  crossref  = {DBLP:conf/gis/2015},
  url       = {http://doi.acm.org/10.1145/2820783.2820833},
  doi       = {10.1145/2820783.2820833},
  timestamp = {Thu, 07 Apr 2016 11:57:11 +0200},
  biburl    = {http://dblp.uni-trier.de/rec/bib/conf/gis/WangWL15},
  bibsource = {dblp computer science bibliography, http://dblp.org}
}

@article{RJing:2014,
  title={A Research of Predicting the B-factor Base on the Protein Sequence},
  author={Runyu Jing and  Yuelong Wang and Yiming Wu and Yongpan Hua and Xu Dai and Menglong Li},
  journal={Journal of Theoretical Computational  Science},
  volume={1},
  number={},
  pages={111},
  year={2014},
	doi  ={doi:10.4172/jtco.1000111}
}





@article{PYue:2005,
  title={Loss of protein structure stability as a major causative factor in monogenic disease},
  author={Yue, P. and Li, Z. and Moult, J.},
  journal={J. Mol. Biol.},
  volume={353},
  number={},
  pages={459-473},
  year={2005}	
}



@article{ZZhang:2012,
  title={Analyzing effects of naturally occurring missense mutations},
  author={Zhang, Z. and  Miteva, M. A. and Wang, L. and  Alexov, E. },
  journal={Comput. Math. Methods Med.},
  volume={2012},
  number={},
  pages={805827},
  year={2012}	
}



@article{Kucukkal:2015,
  title={Structural and physico-chemical effects of disease and non-disease nsSNPs on proteins},
  author={Kucukkal, T. G. and  Petukh, M. and Li, L. and Alexov, E. },
  journal={Curr. Opin. Struct. Biol.},
  volume={32},
  number={},
  pages={18-24},
  year={2015}	
}



@article{Dolzhanskaya:2014,
  title={A novel p.Leu(381)Phe mutation in presenilin 1 is associated with very early onset and unusually
fast progressing dementia as well as lysosomal inclusions typically seen in Kufs disease},
  author={ Dolzhanskaya, N. and Gonzalez, M.A. and Sperziani, F. and  Stefl, S. and  Messing, J. and  Wen, G.Y. and  Alexov, E. and  Zuchner, S. and Velinov, M.},
  journal={J. Alzheimers Dis.},
  volume={39},
  number={},
  pages={23-27},
  year={2014}	
}





@article{Boccuto:2014,
  title={ A mutation in a ganglioside biosynthetic enzyme, ST3GAL5, results in salt \&
pepper syndrome, a neurocutaneous disorder with altered glycolipid and glycoprotein glycosylation},
  author={Boccuto, L. and  Aoki, K. and  Flanagan-Steet, H. and  Chen, C. F. and  Fan, X. and  Bartel, F. and  Petukh, M. and  Pittman, A. and  Saul, R. and Chaubey, A. and  Alexov,  E. and  Tiemeyer,  M. and  Steet,  R. and  Schwartz,  C. E.},
  journal={Hum. Mol. Genet. },
  volume={23},
  number={},
  pages={418-433},
  year={2014}	
}

@article{ZZhang:2013,
  title={A Y328C missense mutation in spermine synthase causes a mild form of Snyder-Robinson syndrome},
  author={ Zhang, Z. and  Norris, J. and  Kalscheuer, V. and  Wood, T. and  Wang, L. and  Schwartz, C. and  Alexov, E. and  van Esch, H.},
  journal={Hum. Mol. Genet. },
  volume={22},
  number={},
  pages={3789-3797},
  year={2013}	
}



@article{Kucukkal:2015b,
  title={Impact of rett syndrome mutations on MeCP2 MBD Stability},
  author={Kucukkal, T.G. and  Yang, Y. and Uvarov, O. and Cao, W. and Alexov, E.},
  journal={Biochemistry },
  volume={54},
  number={},
  pages={6357-6368},
  year={2015}	
}

 @article{YPeng:2015,
  title={Mutations in the KDM5C ARID domain and their plausible association with syndromic Claes-Jensen-Type disease},
  author={Peng, Y. and Suryadi, J. and Yang, Y. and Kucukkal, T. G. and Cao, W. and  Alexov, E.},
  journal={Int. J. Mol. Sci.},
  volume={16},
  number={},
  pages={27270-27287},
  year={2015}	
}

@article{Fersht:2078,
  title={Dissection of the structure and activity of the tyrosyl-tRNA synthetase by site-directed mutagenesis},
  author={Alan R. Fersht},
  journal={Biochemistry},
  volume={26},
  number={},
  pages={8031-8037},
  year={1978}	
}



 @article{Capriotti:2005,
  title={I-Mutant2.0: predicting stability changes upon mutation from the protein sequence or structure},
  author={Emidio Capriotti and  Piero Fariselli and Rita Casadio},
  journal={Nucleic Acids Research},
  volume={33},
  number={},
  pages={W306-W310},
  year={2005}	
}

 @article{Guerois:2002,
  title={Predicting Changes in the Stability of Proteins and Protein Complexes: A Study of More Than 1000 Mutations},
  author={Raphael Guerois and  Jens Erik Nielsen and Luis Serrano},
  journal={J. Mol. Biol. },
  volume={320},
  number={},
  pages={369- 387},
  year={2002}	
}


 @article{Pires:2014,
  title={mCSM: predicting the effects of mutations in proteins using graph-based signatures},
  author={Douglas E. V. Pires and  David B. Ascher and Tom L. Blundell},
  journal={Structural Bioinformatics},
  volume={30},
  number={},
  pages={335 - 342},
  year={2014}	
}

@article{Giollo:2014,
  title={NeEMO: a method using residue interaction networks to improve prediction of protein stability upon mutation},
  author={Manuel Giollo and  Alberto JM Martin and  Ian Walsh and  Carlo Ferrari and  Silvio CE Tosatto},
  journal={BMC Genomics},
  volume={15},
  number={S4},
  pages={S7},
  year={2014}	
}

@article{Dehouck:2009,
  title={Fast and accurate predictions of protein stability changes upon mutations using statistical potentials and neural networks: PoPMuSiC-2.0},
  author={Yves Dehouck and  Aline Grosfils and  Benjamin Folch and  Dimitri Gilis and  Philippe Bogaerts and Marianne Rooman},
  journal={Structural Bioinformatics},
  volume={25},
  number={},
  pages={2537-2543},
  year={2009}	
}

@article{JTian:2010,
  title={Predicting changes in protein thermostability brought about by single- or multi-site mutations},
  author={Jian Tian and  Ningfeng Wu and  Xiaoyu Chu and Yunliu Fan},
  journal={MBC bioinformatics},
  volume={11},
  number={},
  pages={370},
  year={2010}	
}



@article{Getov:2016,
  title={SAAFEC: Predicting the Effect of Single Point Mutations on Protein Folding Free Energy Using a Knowledge-Modified MM/PBSA Approach},
  author={Ivan Getov and  Marharyta Petukh  and Emil Alexov},
  journal={International Journal of Molecular Sciences },
  volume={17},
  number={},
  pages={512},
  year={2016}	
}

@article{LQuan:2016,
  title={STRUM: structure-based prediction of protein stability changes upon single-point mutation},
  author={Lijun Quan and Qiang Lv and Yang Zhang},
  journal={Structural Bioinformatics},
  volume={},
  number={},
  pages={},
  year={In press, 2016}	
}


@article{Martinez:2000,
  title={Mutation Frequencies and Antibiotic Resistance},
  author={J. L. Martinez and F. Baquero},
  journal={Antimicrobial Agents and Chemotherapy},
  volume={44},
  number={},
  pages={1771-1777},
  year={2000}	
}



@article{Overington:2006,
  title={How many drug targets are there?},
  author={Overington JP and  Al-Lazikani B and  Hopkins A L},
  journal={Nat. Rev. Drug Discov.},
  volume={5},
  number={},
  pages={993-995},
  year={2005}	
}



@article{Liszewski:2015,
  title={Dissecting the Structure of Membrane Proteins},
  author={Liszewski, Kathy },
  journal={Genetic Engineering \& Biotechnology News},
  volume={35},
  number={},
  pages={16-17},
  year={2015}	
}

@inproceedings{evgeniou2004regularized,
  title={Regularized multi--task learning},
  author={Evgeniou, Theodoros and Pontil, Massimiliano},
  booktitle={Proceedings of the tenth ACM SIGKDD international conference on Knowledge discovery and data mining},
  pages={109--117},
  year={2004},
  organization={ACM}
}

@incollection{caruana1998multitask,
  title={Multitask learning},
  author={Caruana, Rich},
  booktitle={Learning to learn},
  pages={95--133},
  year={1998},
  publisher={Springer}
}

@article{evgeniou2007multi,
  title={Multi-task feature learning},
  author={Evgeniou, A and Pontil, Massimiliano},
  journal={Advances in neural information processing systems},
  volume={19},
  pages={41},
  year={2007}
}

@inproceedings{liu2009multi,
  title={Multi-task feature learning via efficient l 2, 1-norm minimization},
  author={Liu, Jun and Ji, Shuiwang and Ye, Jieping},
  booktitle={Proceedings of the twenty-fifth conference on uncertainty in artificial intelligence},
  pages={339--348},
  year={2009},
  organization={AUAI Press}
}

@article{pong2010trace,
  title={Trace norm regularization: Reformulations, algorithms, and multi-task learning},
  author={Pong, Ting Kei and Tseng, Paul and Ji, Shuiwang and Ye, Jieping},
  journal={SIAM Journal on Optimization},
  volume={20},
  number={6},
  pages={3465--3489},
  year={2010},
  publisher={SIAM}
}

@inproceedings{krizhevsky2012imagenet,
  title={Imagenet classification with deep convolutional neural networks},
  author={Krizhevsky, Alex and Sutskever, Ilya and Hinton, Geoffrey E},
  booktitle={Advances in neural information processing systems},
  pages={1097--1105},
  year={2012}
}

@article{hinton2012deep,
  title={Deep neural networks for acoustic modeling in speech recognition: The shared views of four research groups},
  author={Hinton, Geoffrey and Deng, Li and Yu, Dong and Dahl, George E and Mohamed, Abdel-rahman and Jaitly, Navdeep and Senior, Andrew and Vanhoucke, Vincent and Nguyen, Patrick and Sainath, Tara N and  Kingsbury, Brian},
  journal={IEEE Signal Processing Magazine},
  volume={29},
  number={6},
  pages={82--97},
  year={2012},
  publisher={IEEE}
}

@article{simonyan2014very,
  title={Very deep convolutional networks for large-scale image recognition},
  author={Simonyan, Karen and Zisserman, Andrew},
  journal={arXiv preprint arXiv:1409.1556},
  year={2014}
}

@article{zhou2011malsar,
  title={Malsar: Multi-task learning via structural regularization},
  author={Zhou, Jiayu and Chen, Jianhui and Ye, Jieping},
  journal={Arizona State University},
  year={2011}
}

@inproceedings{marcou2014compound,
  title={Tutorial: QSAR modeling of compounds profiling},
  author={Marcou, Gilles and Horvath, Dragos and Varnek, Alexandre},
  booktitle={Strasbourg Summer School in Chemoinformatics},
  year={2014},
  note={\url{http://infochim.u-strasbg.fr/spip.php?rubrique176}}
}

@inproceedings{chen2011integrating,
  title={Integrating low-rank and group-sparse structures for robust multi-task learning},
  author={Chen, Jianhui and Zhou, Jiayu and Ye, Jieping},
  booktitle={Proceedings of the 17th ACM SIGKDD international conference on Knowledge discovery and data mining},
  pages={42--50},
  year={2011},
  organization={ACM}
}

@inproceedings{zhou2011clustered,
  title={Clustered multi-task learning via alternating structure optimization},
  author={Zhou, Jiayu and Chen, Jianhui and Ye, Jieping},
  booktitle={Advances in neural information processing systems},
  pages={702--710},
  year={2011}
}

@inproceedings{gong2014efficient,
  title={Efficient multi-task feature learning with calibration},
  author={Gong, Pinghua and Zhou, Jiayu and Fan, Wei and Ye, Jieping},
  booktitle={Proceedings of the 20th ACM SIGKDD international conference on Knowledge discovery and data mining},
  pages={761--770},
  year={2014},
  organization={ACM}
}

@inproceedings{lin2016multi,
  title={Multi-Task Feature Interaction Learning},
  author={Lin, Kaixiang and Xu, Jianpeng and Ji, Shuiwang and Zhou, Jiayu},
  booktitle={Proceedings of the 22th ACM SIGKDD international conference on Knowledge discovery and data mining},
  year={2016},
  organization={ACM}
}

@inproceedings{lin2016interactive,
  title={Interactive Multi-Task Relationship Learning},
  author={Lin, Kaixiang and Zhou, Jiayu},
  booktitle={2016 IEEE International Conference on Data Mining},
  year={2016},
  organization={IEEE}
}

@inproceedings{baytas2016asynchronous,
  title={Asynchronous Multi-Task Learning},
  author={Baytas, Inci and Yan, Ming and Jain, Anil and Zhou, Jiayu},
  booktitle={2016 IEEE International Conference on Data Mining},
  year={2016},
  organization={IEEE}
}

@inproceedings{zhou2011multi,
  title={A multi-task learning formulation for predicting disease progression},
  author={Zhou, Jiayu and Yuan, Lei and Liu, Jun and Ye, Jieping},
  booktitle={Proceedings of the 17th ACM SIGKDD international conference on Knowledge discovery and data mining},
  pages={814--822},
  year={2011},
  organization={ACM}
}

@inproceedings{zhou2012modeling,
  title={Modeling disease progression via fused sparse group lasso},
  author={Zhou, Jiayu and Liu, Jun and Narayan, Vaibhav A and Ye, Jieping},
  booktitle={Proceedings of the 18th ACM SIGKDD international conference on Knowledge discovery and data mining},
  pages={1095--1103},
  year={2012},
  organization={ACM}
}

@article{zhou2013modeling,
  title={Modeling disease progression via multi-task learning},
  author={Zhou, Jiayu and Liu, Jun and Narayan, Vaibhav A and Ye, Jieping},
  journal={NeuroImage},
  volume={78},
  pages={233--248},
  year={2013},
  publisher={Elsevier}
}

@inproceedings{zhou2013feafiner,
  title={Feafiner: biomarker identification from medical data through feature generalization and selection},
  author={Zhou, Jiayu and Lu, Zhaosong and Sun, Jimeng and Yuan, Lei and Wang, Fei and Ye, Jieping},
  booktitle={Proceedings of the 19th ACM SIGKDD international conference on Knowledge discovery and data mining},
  pages={1034--1042},
  year={2013},
  organization={ACM}
}

@inproceedings{zhou2014micro,
  title={From micro to macro: data driven phenotyping by densification of longitudinal electronic medical records},
  author={Zhou, Jiayu and Wang, Fei and Hu, Jianying and Ye, Jieping},
  booktitle={Proceedings of the 20th ACM SIGKDD international conference on Knowledge discovery and data mining},
  pages={135--144},
  year={2014},
  organization={ACM}
}

@inproceedings{xu2015formula,
  title={Formula: FactORized MUlti-task LeArning for task discovery in personalized medical models},
  author={Xu, Jianpeng and Zhou, Jiayu and Tan, Pang-Ning},
  booktitle={Proceedings of the 15th SIAM International Conference on Data Mining},
  pages={496--504},
  year={2015},
  organization={SIAM}
	}


@article{Bava:2004,
  title={ProTherm, version 4.0: thermodynamic database for proteins and mutants},
  author={Bava, K Abdulla and Gromiha, M Michael and Uedaira, Hatsuho and Kitajima, Koji and Sarai, Akinori},
  journal={Nucleic acids research},
  volume={32},
  number={suppl 1},
  pages={D120--D121},
  year={2004},
  publisher={Oxford Univ Press}
}

@article{Berman:2000,
  title={The protein data bank},
  author={Berman, Helen M and Westbrook, John and Feng, Zukang and Gilliland, Gary and Bhat, Talapady N and Weissig, Helge and Shindyalov, Ilya N and Bourne, Philip E},
  journal={Nucleic acids research},
  volume={28},
  number={1},
  pages={35--242},
  year={2000},
  publisher={Oxford Univ Press}
}

@article{Ashtawy:2015,
  title={A Comparative Assessment of Predictive Accuracies of Conventional and Machine Learning Scoring Functions for Protein-Ligand Binding Affinity Prediction},
  author={Hossam M. Ashtawy and Nihar R. Mahapatra},
  journal={IEEE/ACM Transactions on Computational Biology and Bioinformatics},
  volume={12},
  number={},
  pages={335-347},
  year={2015},
  publisher={ }
}



@article{Ashtawy:2014,
  title={Molecular Docking for Drug Discovery: Machine-Learning Approaches for Native Pose Prediction of Protein-Ligand Complexes},
  author={Hossam M. Ashtawy and Nihar R. Mahapatra},
  journal={ Computational Intelligence Methods for Bioinformatics and Biostatistics, Lecture Notes in Computer Science},
  volume={8452},
  number={},
  pages={15-32},
  year={2014},
  publisher={ }
}



@BOOK{Conley:1978,
  title = {Isolated invariant sets and the Morse index. CBMS Regional Conference Series in Mathematics, 38},
  publisher = {American Mathematical Society,Providence, R.I},
  year = {1978},
  author = {Charles Conley}
}


@BOOK{Mischaikow:2002,
  title = {Conley index.  Chapter 9 in Handbook of Dynamical Systems, vol 2, pp 393-460},
  publisher = {Elsevier},
  year = {2002},
  author = {Konstantin Mischaikow and Marian Mrozek}
}

%%%%%%%%%%%%%%%%%%%%% Conley index

@article{Chen:2012morse,
  title={Morse set classification and hierarchical refinement using Conley index},
  author={Chen, Guoning and Deng, Qingqing and Szymczak, Andrzej and Laramee, Robert S and Zhang, Eugene},
  journal={IEEE transactions on visualization and computer graphics},
  volume={18},
  number={5},
  pages={767--782},
  year={2012},
  publisher={IEEE}
}

@article{Manolescu:2013conley,
  title={The Conley index, gauge theory, and triangulations},
  author={Manolescu, Ciprian},
  journal={Journal of Fixed Point Theory and Applications},
  volume={13},
  number={2},
  pages={431--457},
  year={2013},
  publisher={Springer}
}

%%%%%%%%%%%%% persistent landscape

@article{RBrasher:2013,
  title={New biologically motivated knot table},
  author={Brasher, R. and Scharein, R. G. and Vazquez, M.},
  journal={Biochemical Society Transactions},
  volume={41},
  number={},
  pages={606--611},
  year={2013}
}


@article{IKDarcy:2013,
  title={Determining the topology of stable { protein-DNA} complexes},
  author={Darcy, I. K. and Vazquez, M.},
  journal={Biochemical Society Transactions},
  volume={41},
  number={},
  pages={601--605},
  year={2013}
}


@article{CHeitsch:2014,
  title={ Combinatorial insights into RNA secondary structure, in { N. Jonoska and M. Saito}, editors},
  author={C. Heitsch and S. Poznanovic},
  journal={Discrete and Topological Models in Molecular Biology},
  volume={ Chapter 7},
  number={},
  pages={145-166},
  year={2014}
}

@article{SHarvey:2013,
  title={The icosahedral RNA virus as a grotto: organizing the genome into stalagmites and stalactite},
  author={S. C. Harvey and Y. Zeng and C. E. Heitsch},
  journal={J Biol Phys},
  volume={ Chapter 7},
  number={},
  pages={163-172},
  year={2013}
}



@article{Kroncke:2016,
  title={Documentation of an Imperative To Improve Methods for Predicting
Membrane Protein Stability},
  author={Brett M. Kroncke and Amanda M. Duran and Jeffrey L. Mendenhall and Jens Meiler and Jeffrey D. Blume and Charles R. Sanders},
  journal={Biochemistry},
  volume={55},
  number={},
  pages={5002-5009},
  year={2016}
}

@article{Kellogg:2011,
  title={Role of conformational sampling in computing mutation-induced changes in protein structure and stability},
  author={Kellogg, E. H. and Leaver-Fay, A. and Baker, D.},
  journal={ Proteins: Struct., Funct., Genet. },
  volume={79},
  number={},
  pages={830-838},
  year={2011}
}


@article{Guerois:2002,
  title={ Predicting changes in the stability of proteins and protein complexes: a study of
more than 1000 mutations},
  author={Guerois, R. and Nielsen, J. E. and Serrano, L.},
  journal={ J. Mol. Biol.},
  volume={320},
  number={},
  pages={369-387},
  year={2002}
}

@article{Worth:2011,
  title={ {SDM}-a server for predicting effects of mutations on protein stability and
malfunction},
  author={Worth, C. L. and Preissner, R. and Blundell, T. L.},
  journal={ Nucleic Acids Res.},
  volume={39},
  number={},
  pages={W215-W222},
  year={2011}
}


@article{Pires:2014,
  title={ { DUET:} a server for predicting effects of mutations on protein stability using an
integrated computational approach},
  author={Pires, D. E. V. and Ascher, D. B. and Blundell, T. L.},
  journal={ Nucleic Acids Res.},
  volume={42},
  number={},
  pages={W314-W319},
  year={2014}
}


@article{Berliner:2014,
  title={Combining structural modeling with ensemble machine learning to accurately predict protein fold stability and binding affinity effects upon mutation},
  author={Berliner, N. and Teyra, J. and Colak, R. and Garcia Lopez, S. and and Kim, P. M.},
  journal={PLoS One},
  volume={9},
  number={},
  pages={e107353},
  year={2014}
}



@article{YYang:2013,
  title={Structure-based prediction of the effects of a missense variant on
protein stability},
  author={Yang, Y. and Chen, B. and Tan, G. and Vihinen, M. and Shen, B.},
  journal={Amino Acids},
  volume={44},
  number={},
  pages={ 847-855},
  year={2013}
}


@article{YChoi:2012,
  title={Predicting the functional effect of amino acid substitutions and
indels},
  author={Choi, Y. and Sims, G. E. and Murphy, S. and Miller, J. R. and Chan, A. P.},
  journal={PLoS One},
  volume={7},
  number={},
  pages={e46688},
  year={2014}
}

@article{Folkman:2016,
  title={ {EASEMM:} Sequence-Based Prediction of Mutation-Induced Stability Changes with Feature-Based Multiple Models},
  author={Folkman, L. and Stantic, B. and Sattar, A. and Zhou, Y.},
  journal={J. Mol. Biol.},
  volume={428},
  number={},
  pages={1394-1405},
  year={2016}
}

@article{Puente:2003,
  title={ Human and mouse proteases: a comparative genomic approach},
  author={Puente, X. S. and  Sanchez, L.M. and  Overall, C. M. and Lopez-Otin, C. },
  journal={Nat Rev Genet.},
  volume={4},
  number={},
  pages={544-558},
  year={2003}
}


%%%%%%%%%%%%%%%%%%% Modularity
@article{Newman:2004,
  title={Finding and evaluating community structure in networks},
  author={Newman, M. E. J. and Girvan, M.},
  journal={Physical review E},
  volume={69},
  number={2},
  pages={026113},
  year={2004},
  publisher={APS}
}

@article{Newman:2006,
  title={Modularity and community structure in networks},
  author={Newman, M. E. J.},
  journal={Proceedings of the national academy of sciences},
  volume={103},
  number={23},
  pages={8577--8582},
  year={2006},
  publisher={National Acad Sciences}
}

@article{Fortunato:2010,
  title={Community detection in graphs},
  author={Fortunato, S.},
  journal={Physics reports},
  volume={486},
  number={3},
  pages={75--174},
  year={2010},
  publisher={Elsevier}
}

@article{Jain:2010,
  title={Data clustering: 50 years beyond K-means},
  author={Jain, A. K.},
  journal={Pattern recognition letters},
  volume={31},
  number={8},
  pages={651--666},
  year={2010},
  publisher={Elsevier}
}

%%%%%%%%%%%%%%%%%%%%%%%% spectral graph theory

@article{Mohar:1991laplacian,
  title={The Laplacian spectrum of graphs},
  author={Mohar, B. and Alavi, Y. and Chartrand, G. and Oellermann, O. R.},
  journal={Graph theory, combinatorics, and applications},
  volume={2},
  number={871-898},
  pages={12},
  year={1991}
}

@incollection{Mohar:1997some,
  title={Some applications of {Laplace} eigenvalues of graphs},
  author={Mohar, B.},
  booktitle={Graph symmetry},
  pages={225--275},
  year={1997},
  publisher={Springer}
}

@article{von:2007tutorial,
  title={A tutorial on spectral clustering},
  author={Von Luxburg, U.},
  journal={Statistics and computing},
  volume={17},
  number={4},
  pages={395--416},
  year={2007},
  publisher={Springer}
}

@article{Hagen:1992new,
  title={New spectral methods for ratio cut partitioning and clustering},
  author={Hagen, L. and Kahng, A. B.},
  journal={IEEE transactions on computer-aided design of integrated circuits and systems},
  volume={11},
  number={9},
  pages={1074--1085},
  year={1992},
  publisher={IEEE}
}

@inproceedings{Ding:2001min,
  title={A min-max cut algorithm for graph partitioning and data clustering},
  author={Ding, C. H. Q. and He, X. F. and Zha, H. Y. and Gu, M. and Simon, H. D.},
  booktitle={Data Mining, 2001. ICDM 2001, Proceedings IEEE International Conference on},
  pages={107--114},
  year={2001},
  organization={IEEE}
}

%%%%%% random walk

@article{Lovasz:1993,
  title={Random walks on graphs},
  author={Lov{\'a}sz, L.},
  journal={Combinatorics, Paul erdos is eighty},
  volume={2},
  pages={1--46},
  year={1993}
}

@misc{Aldous:2002,
  title={Reversible {Markov} chains and random walks on graphs},
  author={Aldous, D. and Fill, J.},
  year={2002},
  publisher={Berkeley}
}

%%% continuous Laplacian

@PHDTHESIS{Belkin:2003,
  title={Problems of learning on manifolds},
  author={Belkin, M.},
  School={The University of Chicago},
  year={2003},
}

@inproceedings{Belkin:2005,
  title={Towards a theoretical foundation for {Laplacian}-based manifold methods},
  author={Belkin, M. and Niyogi, P.},
  booktitle={International Conference on Computational Learning Theory},
  pages={486--500},
  year={2005},
  organization={Springer}
}

@phdthesis{Lafon:2004,
  title={Diffusion maps and geometric harmonics},
  author={Lafon, S. S.},
  year={2004},
  school={Yale University}
}

@inproceedings{Hein:2005graphs,
  title={From graphs to manifolds--weak and strong pointwise consistency of graph {Laplacian}},
  author={Hein, M. and Audibert, J. Y. and Von Luxburg, U.},
  booktitle={International Conference on Computational Learning Theory},
  pages={470--485},
  year={2005},
  organization={Springer}
}

@incollection{Gine:2006empirical,
  title={Empirical graph {Laplacian} approximation of {Laplace Beltrami} operators: Large sample results},
  author={Gin{\'e}, E. and Koltchinskii, V.},
  booktitle={High dimensional probability},
  pages={238--259},
  year={2006},
  publisher={Institute of Mathematical Statistics}
}

%%total variation

@article{Merkurjev:2013,
  title={An {MBO} scheme on graphs for classification and image processing},
  author={Merkurjev, E. and Kostic, T. and Bertozzi, A. L.},
  journal={SIAM Journal on Imaging Sciences},
  volume={6},
  number={4},
  pages={1903--1930},
  year={2013},
  publisher={SIAM}
}

@article{Hu:2013method,
  title={A method based on total variation for network modularity optimization using the {MBO} scheme},
  author={Hu, H. Y. and Laurent, T. and Porter, M. A. and Bertozzi, A. L.},
  journal={SIAM Journal on Applied Mathematics},
  volume={73},
  number={6},
  pages={2224--2246},
  year={2013},
  publisher={SIAM}
}

%%%%%%%%%%%%%%%%%  cryo-EM mode analysis
@article{Tama:2002exploring,
  title={Exploring global distortions of biological macromolecules and assemblies from low-resolution structural information and elastic network theory},
  author={Tama, F. and Wriggers, W. and Brooks, C. L.},
  journal={Journal of molecular biology},
  volume={321},
  number={2},
  pages={297--305},
  year={2002},
  publisher={Elsevier}
}

@article{Ming:2002describe,
  title={How to describe protein motion without amino acid sequence and atomic coordinates},
  author={Ming, D. M. and Kong, Y. F. and Lambert, M. A. and Huang, Z. and Ma, J. P.},
  journal={Proceedings of the National Academy of Sciences},
  volume={99},
  number={13},
  pages={8620--8625},
  year={2002},
  publisher={National Acad Sciences}
}

@article{Gray:1984vector,
  title={Vector quantization},
  author={Gray, R.},
  journal={IEEE Assp Magazine},
  volume={1},
  number={2},
  pages={4--29},
  year={1984},
  publisher={IEEE}
}

%%%%%%%%%%%%%  Harmonic analysis
@article{Brooks:1995harmonic,
  title={Harmonic analysis of large systems. {I. Methodology}},
  author={Brooks, B. R. and Jane{\v{z}}i{\v{c}}, D. and Karplus, M.},
  journal={Journal of computational chemistry},
  volume={16},
  number={12},
  pages={1522--1542},
  year={1995},
  publisher={Wiley Online Library}
}

@article{Lopez:2014normal,
  title={Normal Mode Analysis Techniques in Structural Biology},
  author={L{\'o}pez-Blanco, J. R. and Miyashita, O. and Tama, F. and Chac{\'o}n, P.},
  journal={eLS},
  year={2014},
  publisher={Wiley Online Library}
}

@article{Hayward:2008normal,
  title={Normal modes and essential dynamics},
  author={Hayward, S. and De Groot, B. L.},
  journal={Molecular Modeling of Proteins},
  pages={89--106},
  year={2008},
  publisher={Springer}
}

@article{Levitt:1983normal,
  title={The normal modes of a protein: Native bovine pancreatic trypsin inhibitor},
  author={Levitt, M. and Sander, C. and Stern, P. S.},
  journal={International Journal of Quantum Chemistry},
  volume={24},
  number={S10},
  pages={181--199},
  year={1983},
  publisher={Wiley Online Library}
}

@article{Brooks:1983harmonic,
  title={Harmonic dynamics of proteins: normal modes and fluctuations in bovine pancreatic trypsin inhibitor},
  author={Brooks, B. and Karplus, M.},
  journal={Proceedings of the National Academy of Sciences},
  volume={80},
  number={21},
  pages={6571--6575},
  year={1983},
  publisher={National Acad Sciences}
}


@article{Garcia:1992large,
  title={Large-amplitude nonlinear motions in proteins},
  author={Garc{\'\i}a, A. E.},
  journal={Physical review letters},
  volume={68},
  number={17},
  pages={2696},
  year={1992},
  publisher={APS}
}

@article{Amadei:1993essential,
  title={Essential dynamics of proteins},
  author={Amadei, A. and Linssen, A. and Berendsen, H. JC},
  journal={Proteins: Structure, Function, and Bioinformatics},
  volume={17},
  number={4},
  pages={412--425},
  year={1993},
  publisher={Wiley Online Library}
}

@article{Kitao:1991effects,
  title={The effects of solvent on the conformation and the collective motions of protein: normal mode analysis and molecular dynamics simulations of melittin in water and in vacuum},
  author={Kitao, A. and Hirata, F. and G{\=o}, N.},
  journal={Chemical physics},
  volume={158},
  number={2-3},
  pages={447--472},
  year={1991},
  publisher={Elsevier}
}

@article{Edelsbrunner:2008persistent,
  title={Persistent homology-a survey},
  author={Edelsbrunner, H. and Harer, J.},
  journal={Contemporary mathematics},
  volume={453},
  pages={257--282},
  year={2008},
  publisher={Providence, RI: American Mathematical Society}
}

%%%%%%%%%%%%%%%  Graph model of RNA
@article{Gan:2004rag,
  title={{RAG}: {RNA}-As-Graphs database—concepts, analysis, and features},
  author={Gan, H. H. and Fera, D. and Zorn, J. and Shiffeldrim, N. and Tang, M. and Laserson, U. and Kim, N. and Schlick, T.},
  journal={Bioinformatics},
  volume={20},
  number={8},
  pages={1285--1291},
  year={2004},
  publisher={Oxford Univ Press}
}

@article{Fera:2004rag,
  title={{RAG}: {RNA}-As-Graphs web resource},
  author={Fera, D. and Kim, N. and Shiffeldrim, N. and Zorn, J. and Laserson, U. and Gan, H. H. and Schlick, T.},
  journal={BMC bioinformatics},
  volume={5},
  number={1},
  pages={1},
  year={2004},
  publisher={BioMed Central}
}

@article{Kim2004:candidates,
  title={Candidates for novel {RNA} topologies},
  author={Kim, N. and Shiffeldrim, N. and Gan, H. H. and Schlick, T.},
  journal={Journal of molecular biology},
  volume={341},
  number={5},
  pages={1129--1144},
  year={2004},
  publisher={Elsevier}
}

@article{Schlick:1992trefoil,
  title={Trefoil knotting revealed by molecular dynamics simulations of supercoiled {DNA}},
  author={Schlick, T. and Olson, W. K.},
  journal={Science},
  volume={257},
  number={5073},
  pages={1110--1115},
  year={1992},
  publisher={American Association for the Advancement of Science}
}

@article{Quine:2006intensity,
  title={Intensity and mosaic spread analysis from {PISEMA} tensors in solid-state {NMR}},
  author={Quine, J. R. and Achuthan, S. and Asbury, T. and Bertram, R. and Chapman, M.S. and Hu, J. and Cross, T.A.},
  journal={Journal of Magnetic Resonance},
  volume={179},
  number={2},
  pages={190--198},
  year={2006},
  publisher={Elsevier}
}


@article{weisstein2011lemon,
  title={Lemon},
  author={Weisstein, Eric W},
  year={2011},
  publisher={Wolfram Research, Inc.}
}

@ARTICLE{Franz:1991,
  author = {Franz Aurenhammer},
  title = { Voronoi Diagrams - A Survey of a Fundamental Geometric Data Structure},
  journal = {ACM Computing Surveys},
  year = {1991},
  volume = {23},
  pages = {345-405},
  number = {3}
}

@ARTICLE{ZXiang:2001,
  author = {Xiang, Z and Honig, B},
  title = {Extending the accuracy limits of prediction for side-chain conformations},
  journal = {J Mol Biol},
  year = {2001},
  volume = {311},
  pages = {421-430-405},
  number = {2}
}

@article{quine2004mathematical,
  title={Mathematical aspects of protein structure determination with NMR orientational restraints},
  author={Quine, JR and Cross, Timothy A and Chapman, Michael S and Bertram, Richard},
  journal={Bulletin of mathematical biology},
  volume={66},
  number={6},
  pages={1705--1730},
  year={2004},
  publisher={Springer}
}

@article{hu2011discrete,
  title={Discrete Frenet frame, inflection point solitons, and curve visualization with applications to folded proteins},
  author={Hu, Shuangwei and Lundgren, Martin and Niemi, Antti J},
  journal={Physical Review E},
  volume={83},
  number={6},
  pages={061908},
  year={2011},
  publisher={APS}
}

@article{crenshaw1993orientation,
  title={Orientation by helical motion—II. Changing the direction of the axis of motion},
  author={Crenshaw, Hugh C and Edelstein-Keshet, Leah},
  journal={Bulletin of mathematical biology},
  volume={55},
  number={1},
  pages={213--230},
  year={1993},
  publisher={Springer}
}

@article{Zavodszky:2005,
  title={Side-chain flexibility in protein--ligand binding: The minimal rotation hypothesis},
  author={Zavodszky, Maria I and Kuhn, Leslie A},
  journal={Protein Science},
  volume={14},
  number={4},
  pages={1104--1114},
  year={2005},
  publisher={Wiley Online Library}
}

@article{Grunberg:2006,
  title={Flexibility and conformational entropy in protein-protein binding},
  author={Gr{\"u}nberg, Raik and Nilges, Michael and Leckner, Johan},
  journal={Structure},
  volume={14},
  number={4},
  pages={683--693},
  year={2006},
  publisher={Elsevier}
}

@article{Tuffery:2012,
  title={Flexibility and binding affinity in protein--ligand, protein--protein and multi-component protein interactions: limitations of current computational approaches},
  author={Tuffery, Pierre and Derreumaux, Philippe},
  journal={Journal of The Royal Society Interface},
  volume={9},
  number={66},
  pages={20--33},
  year={2012},
  publisher={The Royal Society}
}

@book{Jeffrey:2012,
  title={Hydrogen bonding in biological structures},
  author={Jeffrey, George A and Saenger, Wolfram},
  year={2012},
  publisher={Springer Science \& Business Media}
}

@book{Jeffrey:1997,
  title={An introduction to hydrogen bonding},
  author={Jeffrey, George A and Jeffrey, George A},
  volume={12},
  year={1997},
  publisher={Oxford university press New York}
}
@article{contreras2011analysis,
  title={Analysis of hydrogen-bond interaction potentials from the electron density: integration of noncovalent interaction regions},
  author={Contreras-Garc{\'\i}a, Julia and Yang, Weitao and Johnson, Erin R},
  journal={The Journal of Physical Chemistry A},
  volume={115},
  number={45},
  pages={12983--12990},
  year={2011},
  publisher={ACS Publications}
}

@article{contreras2011nciplot,
  title={NCIPLOT: a program for plotting noncovalent interaction regions},
  author={Contreras-Garc{\'\i}a, Julia and Johnson, Erin R and Keinan, Shahar and Chaudret, Robin and Piquemal, Jean-Philip and Beratan, David N and Yang, Weitao},
  journal={Journal of chemical theory and computation},
  volume={7},
  number={3},
  pages={625--632},
  year={2011},
  publisher={ACS Publications}
}



@article{LLi:2016,
  title={Multiscale method for modeling binding phenomena involving large objects: application to kinesin motor domains motion along microtubules},
  author={Li L, Alper J, Alexov E.},
  journal={ Sci Rep.},
  volume={6},
  number={},
  pages={23249},
  year={2016},
  publisher={}
}

@article{warshel1976theoretical,
  title={Theoretical studies of enzymic reactions: dielectric, electrostatic and steric stabilization of the carbonium ion in the reaction of lysozyme},
  author={Warshel, Arieh and Levitt, Michael},
  journal={Journal of Molecular Biology},
  volume={103},
  number={2},
  pages={227--249},
  year={1976},
  publisher={Elsevier}
}

@article{chen2016new,
  title={A New {Poisson--Nernst--Planck} Model with Ion--Water Interactions for Charge Transport in Ion Channels},
  author={Chen, Duan},
  journal={Bulletin of Mathematical Biology},
  volume={78},
  number={8},
  pages={1703--1726},
  year={2016},
  publisher={Springer}
}

@article{alipanahi2015predicting,
  title={Predicting the sequence specificities of {DNA-and RNA-binding} proteins by deep learning},
  author={Alipanahi, Babak and Delong, Andrew and Weirauch, Matthew T and Frey, Brendan J},
  journal={Nature Biotechnology},
  year={2015},
  publisher={Nature Publishing Group}
}

@book{rosner2015fundamentals,
  title={Fundamentals of biostatistics},
  author={Rosner, Bernard},
  year={2015},
  publisher={Nelson Education}
}

@ARTICLE{KLXia:2016,
  author = {Xia, K. L.  and Wei, G. W. },
  title = {A review of geometric, topological and graph theory apparatuses for
the modeling and analysis of biomolecular data},
  journal = {arXiv preprint arXiv:1611.04573},
  year = {2016},
  pages = {1 - 76},
  ty = {JOUR}
}


@article{singer2011three,
  title={Three-dimensional structure determination from common lines in {cryo-EM} by eigenvectors and semidefinite programming},
  author={Singer, Amit and Shkolnisky, Yoel},
  journal={SIAM Journal on Imaging Sciences},
  volume={4},
  number={2},
  pages={543--572},
  year={2011},
  publisher={SIAM}
}

@article{ESES:2015,
Author = {Beibei Liu and Bao Wang and Rundong Zhao and Yiying Tong and Guo Wei Wei},
Title = {{ESES:  software for Eulerian solvent excluded surface}},
Journal = {{Preprint}},
Year = {2015},
}

%%% chromosome

@article{Bolzer:2005three,
  title={Three-dimensional maps of all chromosomes in human male fibroblast nuclei and prometaphase rosettes},
  author={Bolzer, A. and Kreth, G. and Solovei, I. and Koehler, D. and Saracoglu, K. and Fauth, C. and M{\"u}ller, S. and Eils, R. and Cremer, C. and Speicher, M. R. and others},
  journal={PLoS biology},
  volume={3},
  number={5},
  pages={e157},
  year={2005},
  publisher={Public Library of Science}
}

%%%%%%%%%%%%%%%%%%%%%%%   Hi-C papers

@article{Dekker:2002capturing,
  title={Capturing chromosome conformation},
  author={Dekker, J. and Rippe, K. and Dekker, M. and Kleckner, N.},
  journal={science},
  volume={295},
  number={5558},
  pages={1306--1311},
  year={2002},
  publisher={American Association for the Advancement of Science}
}

@article{Zhao:2006circular,
  title={Circular chromosome conformation capture {(4C)} uncovers extensive networks of epigenetically regulated intra-and interchromosomal interactions},
  author={Zhao, Z. H. and Tavoosidana, G. and Sj{\"o}linder, M. and G{\"o}nd{\"o}r, A. and Mariano, P. and Wang, S. and Kanduri, C. and Lezcano, M. and Sandhu, K. S. and Singh, U. and others},
  journal={Nature genetics},
  volume={38},
  number={11},
  pages={1341--1347},
  year={2006},
  publisher={Nature Publishing Group}
}

@article{Simonis:2006nuclear,
  title={Nuclear organization of active and inactive chromatin domains uncovered by chromosome conformation {capture--on-chip (4C)}},
  author={Simonis, M. and Klous, P. and Splinter, E. and Moshkin, Y. and Willemsen, R. and De Wit, E. and Van Steensel, B. and De Laat, W.},
  journal={Nature genetics},
  volume={38},
  number={11},
  pages={1348--1354},
  year={2006},
  publisher={Nature Publishing Group}
}

@article{Dostie:2006chromosome,
  title={{Chromosome Conformation Capture Carbon Copy (5C)}: a massively parallel solution for mapping interactions between genomic elements},
  author={Dostie, J. and Richmond, T. A. and Arnaout, R. A. and Selzer, R. R. and Lee, W. L. and Honan, T. A. and Rubio, E. D. and Krumm, A. and Lamb, J. and Nusbaum, C. and others},
  journal={Genome research},
  volume={16},
  number={10},
  pages={1299--1309},
  year={2006},
  publisher={Cold Spring Harbor Lab}
}

@article{Fullwood:2009oestrogen,
  title={An oestrogen-receptor-$\alpha$-bound human chromatin interactome},
  author={Fullwood, M. J. and Liu, M. H. and Pan, Y. F. and Liu, J. and Xu, H. and Mohamed, Y. B. and Orlov, Y. L. and Velkov, S. and Ho, A. and Mei, P. H. and others},
  journal={Nature},
  volume={462},
  number={7269},
  pages={58--64},
  year={2009},
  publisher={Nature Publishing Group}
}

@article{sexton:2012three,
  title={Three-dimensional folding and functional organization principles of the {Drosophila} genome},
  author={Sexton, T. and Yaffe, E. and Kenigsberg, E. and Bantignies, F. and Leblanc, B. and Hoichman, M. and Parrinello, H. and Tanay, A. and Cavalli, G.},
  journal={Cell},
  volume={148},
  number={3},
  pages={458--472},
  year={2012},
  publisher={Elsevier}
}

@article{Tanizawa:2010mapping,
  title={Mapping of long-range associations throughout the fission yeast genome reveals global genome organization linked to transcriptional regulation},
  author={Tanizawa, H. and Iwasaki, O. and Tanaka, A. and Capizzi, J. R. and Wickramasinghe, P. and Lee, M. and Fu, Z. Y. and Noma, K.},
  journal={Nucleic acids research},
  volume={38},
  number={22},
  pages={8164--8177},
  year={2010},
  publisher={Oxford Univ Press}
}

@article{Zhang:2013chromatin,
  title={Chromatin connectivity maps reveal dynamic promoter-enhancer long-range associations},
  author={Zhang, Y. B. and Wong, C. H. and Birnbaum, R. Y. and Li, G. L. and Favaro, R. and Ngan, C. Y. and Lim, J. and Tai, E. and Poh, H. M. and Wong, E. and others},
  journal={Nature},
  volume={504},
  number={7479},
  pages={306--310},
  year={2013},
  publisher={Nature Research}
}

@article{Duan:2010three,
  title={A three-dimensional model of the yeast genome},
  author={Duan, Z. J. and Andronescu, M. and Schutz, K. and McIlwain, S. and Kim, Y. J. and Lee, C. and Shendure, J. and Fields, S. and Blau, C. A. and Noble, W. S.},
  journal={Nature},
  volume={465},
  number={7296},
  pages={363--367},
  year={2010},
  publisher={Nature Research}
}


@article{De2012:decade,
  title={A decade of {3C} technologies: insights into nuclear organization},
  author={de Wit, E. and de Laat, W.},
  journal={Genes \& development},
  volume={26},
  number={1},
  pages={11--24},
  year={2012},
  publisher={Cold Spring Harbor Lab}
}

@article{Lieberman:2009comprehensive,
  title={Comprehensive mapping of long-range interactions reveals folding principles of the human genome},
  author={Lieberman-Aiden, E. and Van Berkum, N. L. and Williams, L. and Imakaev, M. and Ragoczy, T. and Telling, A. and Amit, I. and Lajoie, B. R. and Sabo, P. J. and Dorschner, M. O. and others},
  journal={science},
  volume={326},
  number={5950},
  pages={289--293},
  year={2009},
  publisher={American Association for the Advancement of Science}
}

@article{Dixon2012:topological,
  title={Topological domains in mammalian genomes identified by analysis of chromatin interactions},
  author={Dixon, J. R. and Selvaraj, S. and Yue, F. and Kim, A. and Li, Y. and Shen, Y. and Hu, M. and Liu, J. S. and Ren, B.},
  journal={Nature},
  volume={485},
  number={7398},
  pages={376--380},
  year={2012},
  publisher={Nature Research}
}

@article{Nora2012:spatial,
  title={Spatial partitioning of the regulatory landscape of the {X-inactivation} centre},
  author={Nora, E. P. and Lajoie, B. R. and Schulz, E. G. and Giorgetti, L. and Okamoto, I. and Servant, N. and Piolot, T. and van Berkum, N. L. and Meisig, J. and Sedat, J. and others},
  journal={Nature},
  volume={485},
  number={7398},
  pages={381--385},
  year={2012},
  publisher={Nature Research}
}



@article{Jin2013:high,
  title={A high-resolution map of the three-dimensional chromatin interactome in human cells},
  author={Jin, F. and Li, Y. and Dixon, J. R. and Selvaraj, S. and Ye, Z. and Lee, A. Y. and Yen, C. A. and Schmitt, A. D. and Espinoza, C. A. and Ren, B.},
  journal={Nature},
  volume={503},
  number={7475},
  pages={290--294},
  year={2013},
  publisher={Nature Research}
}

@article{Ma:2015fine,
  title={Fine-scale chromatin interaction maps reveal the cis-regulatory landscape of human {lincRNA} genes},
  author={Ma, W. X.and Ay, F. and Lee, C. and Gulsoy, G. and Deng, X. X. and Cook, S. and Hesson, J. and Cavanaugh, C. and Ware, C. B. and Krumm, A. and others},
  journal={Nature methods},
  volume={12},
  number={1},
  pages={71--78},
  year={2015},
  publisher={Nature Research}
}

@article{Schoenfelder:2015pluripotent,
  title={The pluripotent regulatory circuitry connecting promoters to their long-range interacting elements},
  author={Schoenfelder, S. and Furlan-Magaril, M. and Mifsud, B. and Tavares-Cadete, F. and Sugar, R. and Javierre, B. M. and Nagano, T. and Katsman, Y. and Sakthidevi, M. and Wingett, S. W. and others},
  journal={Genome research},
  volume={25},
  number={4},
  pages={582--597},
  year={2015},
  publisher={Cold Spring Harbor Lab}
}

@article{Dryden:2014unbiased,
  title={Unbiased analysis of potential targets of breast cancer susceptibility loci by {Capture Hi-C}},
  author={Dryden, N. H. and Broome, L. R. and Dudbridge, F. and Johnson, N. and Orr, N. and Schoenfelder, S. and Nagano, T. and Andrews, S. and Wingett, S. and Kozarewa, I. and others},
  journal={Genome research},
  volume={24},
  number={11},
  pages={1854--1868},
  year={2014},
  publisher={Cold Spring Harbor Lab}
}

@article{Dixon:2015chromatin,
  title={Chromatin architecture reorganization during stem cell differentiation},
  author={Dixon, J. R. and Jung, I. and Selvaraj, S. and Shen, Y. and Antosiewicz-Bourget, J. E. and Lee, A. Y. and Ye, Z. and Kim, A. and Rajagopal, N. and Xie, W. and others},
  journal={Nature},
  volume={518},
  number={7539},
  pages={331--336},
  year={2015},
  publisher={Nature Research}
}

@article{Bonev2016:organization,
  title={Organization and function of the {3D} genome},
  author={Bonev, B. and Cavalli, G.},
  journal={Nature Reviews Genetics},
  volume={17},
  number={11},
  pages={661--678},
  year={2016},
  publisher={Nature Research}
}

@article{Schmitt:2016genome,
  title={Genome-wide mapping and analysis of chromosome architecture},
  author={Schmitt, A. D. and Hu, M. and Ren, B.},
  journal={Nature Reviews Molecular Cell Biology},
  volume={17},
  pages={743--755},
  year={2016},
  publisher={Nature Research}
}


@article{Rao:2014A3D,
  title={A {3D} map of the human genome at kilobase resolution reveals principles of chromatin looping},
  author={Rao, S. S. and Huntley, M. H. and Durand, N. C. and Stamenova, E. K. and Bochkov, I. D. and Robinson, J. T. and Sanborn, A. L. and Machol, I. and Omer, A. D. and Lander, E. S. and others},
  journal={Cell},
  volume={159},
  number={7},
  pages={1665--1680},
  year={2014},
  publisher={Elsevier}
}


@article{Nagano:2013single,
  title={Single-cell {Hi-C} reveals cell-to-cell variability in chromosome structure},
  author={Nagano, T. and Lubling, Y. and Stevens, T. J. and Schoenfelder, S. and Yaffe, E. and Dean, W. and Laue, E. D. and Tanay, A. and Fraser, P.},
  journal={Nature},
  volume={502},
  number={7469},
  pages={59--64},
  year={2013},
  publisher={Nature Publishing Group}
}

@article{Hou2012:gene,
  title={Gene density, transcription, and insulators contribute to the partition of the {Drosophila} genome into physical domains},
  author={Hou, C. H. and Li, L. and Qin, Z. S. and Corces, V. G.},
  journal={Molecular cell},
  volume={48},
  number={3},
  pages={471--484},
  year={2012},
  publisher={Elsevier}
}

@article{Cavalli:2013functional,
  title={Functional implications of genome topology},
  author={Cavalli, G. and Misteli, T.},
  journal={Nature structural \& molecular biology},
  volume={20},
  number={3},
  pages={290--299},
  year={2013},
  publisher={Nature Research}
}

@article{Chen2015:functional,
  title={Functional organization of the human 4D Nucleome},
  author={Chen, H. M. and Chen, J. and Muir, L. A. and Ronquist, S. and Meixner, W. and Ljungman, M. and Ried, T. and Smale, S. and Rajapakse, I.},
  journal={Proceedings of the National Academy of Sciences},
  volume={112},
  number={26},
  pages={8002--8007},
  year={2015},
  publisher={National Acad Sciences}
}

@article{Le:2014distinct,
  title={Distinct structural transitions of chromatin topological domains correlate with coordinated hormone-induced gene regulation},
  author={Le Dily, F. and Ba{\`u}, D. and Pohl, A. and Vicent, G. P. and Serra, F. and Soronellas, D. and Castellano, G. and Wright, R. H. and Ballare, C. and Filion, G. and others},
  journal={Genes \& development},
  volume={28},
  number={19},
  pages={2151--2162},
  year={2014},
  publisher={Cold Spring Harbor Lab}
}

@article{Pope:2014topologically,
  title={Topologically associating domains are stable units of replication-timing regulation},
  author={Pope, B. D. and Ryba, T. and Dileep, V. and Yue, F. and Wu, W. S. and Denas, O. and Vera, D. L. and Wang, Y. L. and Hansen, R. S. and Canfield, T. K. and others},
  journal={Nature},
  volume={515},
  number={7527},
  pages={402--405},
  year={2014},
  publisher={Nature Research}
}

%%% Sanyal's paper
@article{Phillips:2013architectural,
  title={Architectural protein subclasses shape 3D organization of genomes during lineage commitment},
  author={Phillips-Cremins, J. E. and Sauria, M. E. and Sanyal, A. and Gerasimova, T. I. and Lajoie, B. R. and Bell, J. S. and Ong, C. T. and Hookway, T. A. and Guo, C. Y. and Sun, Y. H. and others},
  journal={Cell},
  volume={153},
  number={6},
  pages={1281--1295},
  year={2013},
  publisher={Elsevier}
}

@article{Sanyal:2012long,
  title={The long-range interaction landscape of gene promoters},
  author={Sanyal, A. and Lajoie, B. R. and Jain, G. and Dekker, J.},
  journal={Nature},
  volume={489},
  number={7414},
  pages={109--113},
  year={2012},
  publisher={Nature Research}
}

@article{Sanyal:2011chromatin,
  title={Chromatin globules: a common motif of higher order chromosome structure?},
  author={Sanyal, A. and Ba{\`u}, D. and Mart{\'\i}-Renom, M. A. and Dekker, J.},
  journal={Current opinion in cell biology},
  volume={23},
  number={3},
  pages={325--331},
  year={2011},
  publisher={Elsevier}
}

@article{Bau:2011three,
  title={The three-dimensional folding of the $\alpha$-globin gene domain reveals formation of chromatin globules},
  author={Ba{\`u}, D. and Sanyal, A. and Lajoie, B. R. and Capriotti, E. and Byron, M. and Lawrence, J. B. and Dekker, J. and Marti-Renom, M. A.},
  journal={Nature structural \& molecular biology},
  volume={18},
  number={1},
  pages={107--114},
  year={2011},
  publisher={Nature Publishing Group}
}

%% Hi-C remove bias
@article{Imakaev:2012iterative,
  title={Iterative correction of {Hi-C} data reveals hallmarks of chromosome organization},
  author={Imakaev, M. and Fudenberg, G. and McCord, R. P. and Naumova, N. and Goloborodko, A. and Lajoie, B. R. and Dekker, J. and Mirny, L. A.},
  journal={Nature methods},
  volume={9},
  number={10},
  pages={999--1003},
  year={2012},
  publisher={Nature Publishing Group}
}

@article{Yaffe:2011probabilistic,
  title={Probabilistic modeling of {Hi-C} contact maps eliminates systematic biases to characterize global chromosomal architecture},
  author={Yaffe, E. and Tanay, A.},
  journal={Nature genetics},
  volume={43},
  number={11},
  pages={1059--1065},
  year={2011},
  publisher={Nature Publishing Group}
}

@article{Hu:2012hicnorm,
  title={{HiCNorm}: removing biases in {Hi-C} data via {Poisson} regression},
  author={Hu, M. and Deng, K. and Selvaraj, S. and Qin, Z. H. and Ren, B. and Liu, J. S.},
  journal={Bioinformatics},
  volume={28},
  number={23},
  pages={3131--3133},
  year={2012},
  publisher={Oxford Univ Press}
}

@article{Ay:2014statistical,
  title={Statistical confidence estimation for Hi-C data reveals regulatory chromatin contacts},
  author={Ay, F. and Bailey, T. L. and Noble, W. S.},
  journal={Genome research},
  volume={24},
  number={6},
  pages={999--1011},
  year={2014},
  publisher={Cold Spring Harbor Lab}
}

@article{Witten:2012assessment,
  title={On the assessment of statistical significance of three-dimensional colocalization of sets of genomic elements},
  author={Witten, D. M. and Noble, W. S.},
  journal={Nucleic acids research},
  volume={40},
  number={9},
  pages={3849–-3855},
  year={2012},
  publisher={Oxford Univ Press}
}

@article{Knight:2013fast,
  title={A fast algorithm for matrix balancing},
  author={Knight, P. A. and Ruiz, D.},
  journal={IMA Journal of Numerical Analysis},
  volume={33},
  number={3},
  pages={1029--1047},
  year={2013},
  publisher={Oxford University Press}
}

%%%%%%%%%%%%%%%%%%%%%%%% Hi-C algorithm

@article{Chen2016:spectral,
  title={Spectral identification of topological domains},
  author={Chen, J. and Hero, A. O. and Rajapakse, I.},
  journal={Bioinformatics},
  pages={1-7},
  year={2016},
  publisher={Oxford Univ Press}
}

@article{Filippova2014:identification,
  title={Identification of alternative topological domains in chromatin},
  author={Filippova, D. and Patro, R. and Duggal, G. and Kingsford, C.},
  journal={Algorithms for Molecular Biology},
  volume={9},
  number={1},
  pages={14},
  year={2014},
  publisher={BioMed Central}
}

@article{levy:2014two,
  title={{Two-dimensional} segmentation for analyzing {Hi-C} data},
  author={L{\'e}vy-Leduc, C. and Delattre, M. and Mary-Huard, T. and Robin, S.},
  journal={Bioinformatics},
  volume={30},
  number={17},
  pages={i386--i392},
  year={2014},
  publisher={Oxford Univ Press}
}

@article{Imakaev2015modeling,
  title={Modeling chromosomes: Beyond pretty pictures},
  author={Imakaev, M. V. and Fudenberg, G. and Mirny, L. A.},
  journal={FEBS letters},
  volume={589},
  number={20PartA},
  pages={3031--3036},
  year={2015},
  publisher={Wiley Online Library}
}


@article{Boulos:2013revealing,
  title={Revealing long-range interconnected hubs in human chromatin interaction data using graph theory},
  author={Boulos, R. E. and Arneodo, A. and Jensen, P. and Audit, B.},
  journal={Physical review letters},
  volume={111},
  number={11},
  pages={118102},
  year={2013},
  publisher={APS}
}

@inproceedings{Wang:2013topological,
  title={Topological properties of chromosome conformation graphs reflect spatial proximities within chromatin},
  author={Wang, H. and Duggal, G. and Patro, R. and Girvan, M. and Hannenhalli, S. and Kingsford, C.},
  booktitle={Proceedings of the International Conference on Bioinformatics, Computational Biology and Biomedical Informatics},
  pages={306},
  year={2013},
  organization={ACM}
}

@article{Libbrecht:2015joint,
  title={Joint annotation of chromatin state and chromatin conformation reveals relationships among domain types and identifies domains of cell-type-specific expression},
  author={Libbrecht, M. W. and Ay, F. and Hoffman, M. M. and Gilbert, D. M. and Bilmes, J. A. and Noble, W. S.},
  journal={Genome research},
  volume={25},
  number={4},
  pages={544--557},
  year={2015},
  publisher={Cold Spring Harbor Lab}
}

@article{Botta:2010intra,
  title={Intra-and inter-chromosomal interactions correlate with {CTCF} binding genome wide},
  author={Botta, M. and Haider, S. and Leung, I. X. and Lio, P. and Mozziconacci, J.},
  journal={Molecular systems biology},
  volume={6},
  number={1},
  pages={426},
  year={2010},
  publisher={EMBO Press}
}

@article{Siahpirani:2016multitask,
  title={A multi-task graph-clustering approach for chromosome conformation capture data sets identifies conserved modules of chromosomal interactions},
  author={Siahpirani, A. F. and Ay, F. and Roy, S.},
  journal={Genome biology},
  volume={17},
  number={1},
  pages={114},
  year={2016},
  publisher={BioMed Central}
}

%% repeat orginal structure
@article{Zhang:2015topology,
  title={Topology, structures, and energy landscapes of human chromosomes},
  author={Zhang, B. and Wolynes, P. G.},
  journal={Proceedings of the National Academy of Sciences},
  volume={112},
  number={19},
  pages={6062--6067},
  year={2015},
  publisher={National Acad Sciences}
}

@article{Hu:2013bayesian,
  title={Bayesian inference of spatial organizations of chromosomes},
  author={Hu, M. and Deng, K. and Qin, Z. H. and Dixon, J. and Selvaraj, S. and Fang, J. and Ren, B. and Liu, J. S.},
  journal={PLoS Comput Biol},
  volume={9},
  number={1},
  pages={e1002893},
  year={2013},
  publisher={Public Library of Science}
}

@article{Zhang:20133d,
  title={{3D} chromosome modeling with semi-definite programming and {Hi-C} data},
  author={Zhang, Z. Z. and Li, G. L. and Toh, K. C. and Sung, W. K.},
  journal={Journal of computational biology},
  volume={20},
  number={11},
  pages={831--846},
  year={2013},
  publisher={Mary Ann Liebert, Inc. 140 Huguenot Street, 3rd Floor New Rochelle, NY 10801 USA}
}

@article{Segal:2014reproducibility,
  title={Reproducibility of 3D chromatin configuration reconstructions},
  author={Segal, M. R. and Xiong, H. and Capurso, D. and Vazquez, M. and Arsuaga, J.},
  journal={Biostatistics},
  volume={15},
  number={3},
  pages={442--456},
  year={2014},
  publisher={Biometrika Trust}
}

@article{Lesne:20143d,
  title={{3D} genome reconstruction from chromosomal contacts},
  author={Lesne, A. and Riposo, J. and Roger, P. and Cournac, A. and Mozziconacci, J.},
  journal={Nature methods},
  volume={11},
  number={11},
  pages={1141--1143},
  year={2014},
  publisher={Nature Research}
}

%%%%%%%%%%%%%%%%%%%%%  ion aggregation

@article{zhang:2006interactions,
  title={Interactions between macromolecules and ions: the Hofmeister series},
  author={Zhang, Y. J. and Cremer, P. S.},
  journal={Current opinion in chemical biology},
  volume={10},
  number={6},
  pages={658--663},
  year={2006},
  publisher={Elsevier}
}

@article{Marcus:2009effect,
  title={Effect of ions on the structure of water: structure making and breaking},
  author={Marcus, Y.},
  journal={Chemical reviews},
  volume={109},
  number={3},
  pages={1346--1370},
  year={2009},
  publisher={ACS Publications}
}

@article{Lo:2012hofmeister,
  title={Hofmeister phenomena: an update on ion specificity in biology},
  author={Lo Nostro, P. and Ninham, B. W.},
  journal={Chemical reviews},
  volume={112},
  number={4},
  pages={2286--2322},
  year={2012},
  publisher={ACS Publications}
}

@article{Wallace:2013microscopic,
  title={Microscopic evidence for liquid-liquid separation in supersaturated CaCO3 solutions},
  author={Wallace, A. F. and Hedges, L. O. and Fernandez-Martinez, A. and Raiteri, P. and Gale, J. D. and Waychunas, G. A. and Whitelam, S. and Banfield, J. F. and De Yoreo, J. J.},
  journal={Science},
  volume={341},
  number={6148},
  pages={885--889},
  year={2013},
  publisher={American Association for the Advancement of Science}
}


%% experiments to prove ion has no effect

@article{Omta:2003negligible,
  title={Negligible effect of ions on the hydrogen-bond structure in liquid water},
  author={Omta, A. W. and Kropman, M. F. and Woutersen, S. and Bakker, H. J.},
  journal={Science},
  volume={301},
  number={5631},
  pages={347--349},
  year={2003},
  publisher={American Association for the Advancement of Science}
}


%%%%%%%%%%% Hydrogn network

@article{Xenides:2006hydrogen,
  title={Hydrogen bonding in liquid water: An ab initio {QM/MM MD} simulation study},
  author={Xenides, D. and Randolf, B. R. and Rode, B. M.},
  journal={Journal of molecular liquids},
  volume={123},
  number={2},
  pages={61--67},
  year={2006},
  publisher={Elsevier}
}


@article{kumar:2007hydrogen,
  title={Hydrogen bonding definitions and dynamics in liquid water},
  author={Kumar, R. and Schmidt, J. R. and Skinner, J. L.},
  journal={The Journal of chemical physics},
  volume={126},
  number={20},
  pages={05B611},
  year={2007},
  publisher={AIP}
}

@article{laage:2011water,
  title={Water jump reorientation: from theoretical prediction to experimental observation},
  author={Laage, D. and Stirnemann, G. and Sterpone, F. and Hynes, J. T.},
  journal={Accounts of chemical research},
  volume={45},
  number={1},
  pages={53--62},
  year={2011},
  publisher={ACS Publications}
}

@article{Oleinikova:2005formation,
  title={Formation of spanning water networks on protein surfaces via {2D} percolation transition},
  author={Oleinikova, A. and Smolin, N. and Brovchenko, I. and Geiger, A. and Winter, Roland},
  journal={The journal of physical chemistry B},
  volume={109},
  number={5},
  pages={1988--1998},
  year={2005},
  publisher={ACS Publications}
}


@article{Bako:2010hydrogen,
  title={Hydrogen bonded network properties in liquid formamide},
  author={Bak{\'o}, I. and Megyes, T. and B{\'a}lint, S. and Chihaia, V. and Bellissent-Funel, M. C. and Krienke, H. and Kopf, A. and Suh, S. H.},
  journal={The Journal of chemical physics},
  volume={132},
  number={1},
  pages={014506},
  year={2010},
  publisher={AIP}
}


@article{Shiraga:2016hydrogen,
  title={Hydrogen Bond Network of Water around Protein Investigated with Terahertz and Infrared Spectroscopy},
  author={Shiraga, K. and Ogawa, Y. and Kondo, N.},
  journal={Biophysical journal},
  volume={111},
  number={12},
  pages={2629--2641},
  year={2016},
  publisher={Elsevier}
}

@article{dillon:2003nmr,
  title={{NMR} evidence of weak continuous transitions in water and aqueous electrolyte solutions},
  author={Dillon, S. R. and Dougherty, R. C.},
  journal={The Journal of Physical Chemistry A},
  volume={107},
  number={47},
  pages={10217--10220},
  year={2003},
  publisher={ACS Publications}
}

@article{dixit2002molecular,
  title={Molecular segregation observed in a concentrated alcohol--water solution},
  author={Dixit, S. and Crain, J. and Poon, W. C. K. and Finney, J. L. and Soper, A. K.},
  journal={Nature},
  volume={416},
  number={6883},
  pages={829},
  year={2002},
  publisher={Nature Publishing Group}
}

@article{mason:2004structure,
  title={The structure of aqueous guanidinium chloride solutions},
  author={Mason, P. E. and Neilson, G. W. and Enderby, J. E. and Saboungi, M. L. and Dempsey, C. E. and MacKerell, A. D. and Brady, J. W.},
  journal={Journal of the American Chemical Society},
  volume={126},
  number={37},
  pages={11462--11470},
  year={2004},
  publisher={ACS Publications}
}

@article{mason:2005nanometer,
  title={Nanometer-scale ion aggregates in aqueous electrolyte solutions: guanidinium sulfate and guanidinium thiocyanate},
  author={Mason, P. E. and Dempsey, C. E. and Neilson, G. W. and Brady, J. W.},
  journal={The Journal of Physical Chemistry B},
  volume={109},
  number={50},
  pages={24185--24196},
  year={2005},
  publisher={ACS Publications}
}


@article{cerreta:1987structure,
  title={The structure of aqueous solutions of some dihydrogen orthophosphates by laser {Raman} spectroscopy},
  author={Cerreta, M. K. and Berglund, K. A.},
  journal={Journal of crystal growth},
  volume={84},
  number={4},
  pages={577--588},
  year={1987},
  publisher={Elsevier}
}

@article{rusli:1989raman,
  title={Raman spectroscopic study of $NaNO_3$ solution system-solute clustering in supersaturated solutions},
  author={Rusli, I. T. and Schrader, G. L. and Larson, M. A.},
  journal={Journal of crystal growth},
  volume={97},
  number={2},
  pages={345--351},
  year={1989},
  publisher={Elsevier}
}

@article{bian2011ion,
  title={Ion clustering in aqueous solutions probed with vibrational energy transfer},
  author={Bian, H. T. and Wen, X. W. and Li, J. B. and Chen, H. L. and Han, S. Z. and Sun, X. Q. and Song, J. and Zhuang, W. and Zheng, J. R.},
  journal={Proceedings of the National Academy of Sciences},
  volume={108},
  number={12},
  pages={4737--4742},
  year={2011},
  publisher={National Acad Sciences}
}

%%%%% graph for hydrogn-bond

@article{radhakrishnan:1991graph,
  title={Graph theoretical analysis of water clusters},
  author={Radhakrishnan, T. P. and Herndon, W. C.},
  journal={The Journal of Physical Chemistry},
  volume={95},
  number={26},
  pages={10609--10617},
  year={1991},
  publisher={ACS Publications}
}

@article{dos:2004topology,
  title={Topology of the hydrogen bond networks in liquid water at room and supercritical conditions: a small-world structure},
  author={dos Santos, V. M. L. and Moreira, F. G. B. and Longo, R. L.},
  journal={Chemical physics letters},
  volume={390},
  number={1},
  pages={157--161},
  year={2004},
  publisher={Elsevier}
}

@article{Bako:2008water,
  title={Water--methanol mixtures: topology of hydrogen bonded network},
  author={Bak{\'o}, I. and Megyes, T. and B{\'a}lint, S. and Gr{\'o}sz, T. and Chihaia, V.},
  journal={Physical Chemistry Chemical Physics},
  volume={10},
  number={32},
  pages={5004--5011},
  year={2008},
  publisher={Royal Society of Chemistry}
}

@article{Bako:2013hydrogen,
  title={Hydrogen bond network topology in liquid water and methanol: a graph theory approach},
  author={Bak{\'o}, I. and Bencsura, A. and Hermannson, K. and B{\'a}lint, S. and Gr{\'o}sz, T. and Chihaia, V. and Ol{\'a}h, J.},
  journal={Physical Chemistry Chemical Physics},
  volume={15},
  number={36},
  pages={15163--15171},
  year={2013},
  publisher={Royal Society of Chemistry}
}

@article{da:2011hydrogen,
  title={On the hydrogen bond networks in the water--methanol mixtures: topology, percolation and small-world},
  author={da Silva, J. A. B. and Moreira, F. G. B. and dos Santos, V. M. L. and Longo, R. L.},
  journal={Physical Chemistry Chemical Physics},
  volume={13},
  number={14},
  pages={6452--6461},
  year={2011},
  publisher={Royal Society of Chemistry}
}

@article{Wang:2017proton,
  title={Proton network flexibility enables robustness and large electric fields in the ketosteroid isomerase active site},
  author={Wang, L. and Fried, S. D. and Markland, T. E.},
  journal={The Journal of Physical Chemistry B},
  volume={121},
  number={42},
  pages={9807--9815},
  year={2017},
  publisher={ACS Publications}
}


@article{Kim:2014ionI,
  title={Ion aggregation in high salt solutions: Ion network versus ion cluster},
  author={Kim, S. and Kim, H. and Choi, J. and Cho, M.},
  journal={The Journal of chemical physics},
  volume={141},
  number={12},
  pages={124510},
  year={2014},
  publisher={AIP}
}

@article{Choi:2014ionII,
  title={Ion aggregation in high salt solutions. {II}. Spectral graph analysis of water hydrogen-bonding network and ion aggregate structures},
  author={Choi, J. and Cho, M.},
  journal={The Journal of chemical physics},
  volume={141},
  number={15},
  pages={154502},
  year={2014},
  publisher={AIP}
}


@article{choi:2015ion,
  title={Ion aggregation in high salt solutions. {IV}. Graph-theoretical analyses of ion aggregate structure and water hydrogen bonding network},
  author={Choi, J. and Cho, M.},
  journal={The Journal of chemical physics},
  volume={143},
  number={10},
  pages={104110},
  year={2015},
  publisher={AIP Publishing}
}

@article{choi2016ion,
  title={Ion aggregation in high salt solutions. {VI}. Spectral graph analysis of chaotropic ion aggregates},
  author={Choi, J. and Cho, M.},
  journal={The Journal of chemical physics},
  volume={145},
  number={17},
  pages={174501},
  year={2016},
  publisher={AIP Publishing}
}


@article{Tielrooij:2010cooperativity,
  title={Cooperativity in ion hydration},
  author={Tielrooij, K. J. and Garcia-Araez, N. and Bonn, M. and Bakker, H. J.},
  journal={Science},
  volume={328},
  number={5981},
  pages={1006--1009},
  year={2010},
  publisher={American Association for the Advancement of Science}
}


@article{Stirnemann:2013mechanisms,
  title={Mechanisms of acceleration and retardation of water dynamics by ions},
  author={Stirnemann, G. and Wernersson, E. and Jungwirth, P. and Laage, D.},
  journal={Journal of the American Chemical Society},
  volume={135},
  number={32},
  pages={11824--11831},
  year={2013},
  publisher={ACS Publications}
}

@article{Chen:2016electrolytes,
  title={Electrolytes induce long-range orientational order and free energy changes in the {H}-bond network of bulk water},
  author={Chen, Y. X. and Okur, H. I. and Gomopoulos, N. and Macias-Romero, C. and Cremer, P. S. and Petersen, P. B. and Tocci, G. and Wilkins, D. M. and Liang, C. W. and Ceriotti, M. and others},
  journal={Science advances},
  volume={2},
  number={4},
  pages={e1501891},
  year={2016},
  publisher={American Association for the Advancement of Science}
}

@article{choi2018graph,
  title={Graph theory and ion and molecular aggregation in aqueous solutions},
  author={Choi, J. H. and Lee, H. and Choi, H. R. and Cho, M.},
  journal={Annual review of physical chemistry},
  volume={69},
  pages={125--149},
  year={2018},
  publisher={Annual Reviews}
}


%%%%%%%%%%%%%
@book{gudhi:urm,
  title= {{GUDHI} User and Reference Manual},
  author = {The GUDHI Project},
  publisher= {GUDHI Editorial Board},
  year= {2015},
  url = {http://gudhi.gforge.inria.fr/doc/latest/}
}

@incollection{gudhi:FilteredComplexes,
   author={Maria, C. },
   title={Filtered Complexes},
   publisher={{GUDHI} Editorial Board},
   booktitle={{GUDHI} User and Reference Manual},
   url= {http://gudhi.gforge.inria.fr/doc/latest/group__simplex__tree.html},
   year={2015}
}

@article{fasy:2014introduction,
  title={Introduction to the R package TDA},
  author={Fasy, B. T. and Kim, J. and Lecci, F. and Maria, C.},
  journal={arXiv preprint arXiv:1411.1830},
  year={2014}
}

@article{bauer2017ripser,
  title={Ripser: a lean {C++} code for the computation of {Vietoris-Rips} persistence barcodes},
  author={Bauer, U.},
  journal={Software available at https://github. com/Ripser/ripser},
  year={2017}
}

@inproceedings{bauer2014phat,
  title={{PHAT}--Persistent Homology Algorithms Toolbox},
  author={Bauer, U. and Kerber, M. and Reininghaus, J. and Wagner, H.},
  booktitle={International Congress on Mathematical Software},
  pages={137--143},
  year={2014},
  organization={Springer}
}

@inproceedings{bauer2014distributed,
  title={Distributed computation of persistent homology},
  author={Bauer, U. and Kerber, M. and Reininghaus, J.},
  booktitle={2014 proceedings of the sixteenth workshop on algorithm engineering and experiments (ALENEX)},
  pages={31--38},
  year={2014},
  organization={SIAM}
}

%%%%%%%% topological similarity

@article{mate:2014topological,
  title={A topological similarity measure for proteins},
  author={M{\'a}t{\'e}, G. and Hofmann, A. and Wenzel, N. and Heermann, D. W.},
  journal={Biochimica et Biophysica Acta (BBA)-Biomembranes},
  volume={1838},
  number={4},
  pages={1180--1190},
  year={2014},
  publisher={Elsevier}
}

@article{feinauer:2013zinc,
  title={Zinc finger proteins and the {3D} organization of chromosomes},
  author={Feinauer, C. J. and Hofmann, A. and Goldt, S. and Liu, L. and Mate, G. and Heermann, D. W.},
  journal={Advances in Protein Chemistry and Structual Biology},
  volume={90},
  pages={67--117},
  year={2013}
}

@article{mate:2014statistical,
  title={Statistical analysis of protein ensembles},
  author={M{\'a}t{\'e}, G. and Heermann, D. W.},
  journal={Frontiers in Physics},
  volume={2},
  pages={20},
  year={2014},
  publisher={Frontiers}
}

@article{gelly:2011ipba,
  title={{iPBA}: a tool for protein structure comparison using sequence alignment strategies},
  author={Gelly, J. C. and Joseph, A. P. and Srinivasan, N. and de Brevern, A. G.},
  journal={Nucleic acids research},
  volume={39},
  number={suppl 2},
  pages={W18--W23},
  year={2011},
  publisher={Oxford Univ Press}
}

@article{koehl:2001protein,
  title={Protein structure similarities},
  author={Koehl, P.},
  journal={Current opinion in structural biology},
  volume={11},
  number={3},
  pages={348--353},
  year={2001},
  publisher={Elsevier}
}

%% network topological similarity

@article{erten2011:vavien,
  title={{Vavien}: an algorithm for prioritizing candidate disease genes based on topological similarity of proteins in interaction networks},
  author={Erten, S. and Bebek, G. and Koyut{\"u}rk, M.},
  journal={Journal of computational biology},
  volume={18},
  number={11},
  pages={1561--1574},
  year={2011},
  publisher={Mary Ann Liebert, Inc. 140 Huguenot Street, 3rd Floor New Rochelle, NY 10801 USA}
}

@article{lei2013:novel,
  title={A novel link prediction algorithm for reconstructing {protein--protein} interaction networks by topological similarity},
  author={Lei, C. and Ruan, J.},
  journal={Bioinformatics},
  volume={29},
  number={3},
  pages={355--364},
  year={2013},
  publisher={Oxford Univ Press}
}

%%% Protein structure
@article{Rogen2003:automatic,
  title={Automatic classification of protein structure by using {Gauss} integrals},
  author={R{\o}gen, P. and Fain, B.},
  journal={Proceedings of the National Academy of Sciences},
  volume={100},
  number={1},
  pages={119--124},
  year={2003},
  publisher={National Acad Sciences}
}

%%%% elastic network model and coarse-grained models

%%%%%%%%%%%%%%%%%  cryo-EM mode analysis
@article{Tama:2002exploring,
  title={Exploring global distortions of biological macromolecules and assemblies from low-resolution structural information and elastic network theory},
  author={Tama, F. and Wriggers, W. and Brooks, C. L.},
  journal={Journal of molecular biology},
  volume={321},
  number={2},
  pages={297--305},
  year={2002},
  publisher={Elsevier}
}

@article{Ming:2002describe,
  title={How to describe protein motion without amino acid sequence and atomic coordinates},
  author={Ming, D. M. and Kong, Y. F. and Lambert, M. A. and Huang, Z. and Ma, J. P.},
  journal={Proceedings of the National Academy of Sciences},
  volume={99},
  number={13},
  pages={8620--8625},
  year={2002},
  publisher={National Acad Sciences}
}

@article{Gray:1984vector,
  title={Vector quantization},
  author={Gray, R.},
  journal={IEEE Assp Magazine},
  volume={1},
  number={2},
  pages={4--29},
  year={1984},
  publisher={IEEE}
}

@article{chacon2003mega,
  title={{Mega-Dalton} biomolecular motion captured from electron microscopy reconstructions},
  author={Chac{\'o}n, P. and Tama, F. and Wriggers, W.},
  journal={Journal of molecular biology},
  volume={326},
  number={2},
  pages={485--492},
  year={2003},
  publisher={Elsevier}
}

@article{lu2005:role,
  title={The role of shape in determining molecular motions},
  author={Lu, M. Y. and Ma, J. P.},
  journal={Biophysical journal},
  volume={89},
  number={4},
  pages={2395--2401},
  year={2005},
  publisher={Elsevier}
}

@article{stember:2009bend,
  title={{Bend-twist-stretch} model for coarse elastic network simulation of biomolecular motion},
  author={Stember, J. N. and Wriggers, W.},
  journal={The Journal of chemical physics},
  volume={131},
  number={7},
  pages={074112},
  year={2009},
  publisher={AIP}
}

@article{tama2006symmetry,
  title={Symmetry, form, and shape: guiding principles for robustness in macromolecular machines},
  author={Tama, F. and Brooks III, C. L.},
  journal={Annu. Rev. Biophys. Biomol. Struct.},
  volume={35},
  pages={115--133},
  year={2006},
  publisher={Annual Reviews}
}

@article{xia:2012multiscale,
  title={Multiscale coarse-graining via normal mode analysis},
  author={Xia, F. and Lu, L. Y.},
  journal={Journal of chemical theory and computation},
  volume={8},
  number={11},
  pages={4797--4806},
  year={2012},
  publisher={ACS Publications}
}

@article{durand:1994new,
  title={A new approach for determining low-frequency normal modes in macromolecules},
  author={Durand, P. and Trinquier, G. and Sanejouand, Y. H.},
  journal={Biopolymers},
  volume={34},
  number={6},
  pages={759--771},
  year={1994},
  publisher={Wiley Online Library}
}

@article{van:2005normal,
  title={Normal mode calculations of icosahedral viruses with full dihedral flexibility by use of molecular symmetry},
  author={van V., Herman W. T. and Karplus, M.},
  journal={Journal of molecular biology},
  volume={350},
  number={3},
  pages={528--542},
  year={2005},
  publisher={Elsevier}
}


@article{xia:2012multiscale,
  title={Multiscale coarse-graining via normal mode analysis},
  author={Xia, F. and Lu, L. Y.},
  journal={Journal of chemical theory and computation},
  volume={8},
  number={11},
  pages={4797--4806},
  year={2012},
  publisher={ACS Publications}
}

@article{chu:2005allostery,
  title={Allostery of actin filaments: molecular dynamics simulations and coarse-grained analysis},
  author={Chu, J. W. and Voth, G. A.},
  journal={Proceedings of the National Academy of Sciences of the United States of America},
  volume={102},
  number={37},
  pages={13111--13116},
  year={2005},
  publisher={National Acad Sciences}
}

@article{chu:2006coarse,
  title={Coarse-grained modeling of the actin filament derived from atomistic-scale simulations},
  author={Chu, J. W. and Voth, G. A.},
  journal={Biophysical journal},
  volume={90},
  number={5},
  pages={1572--1582},
  year={2006},
  publisher={Elsevier}
}

@article{na:2015bridging,
  title={Bridging between {NMA} and elastic network models: preserving all-atom accuracy in coarse-grained models},
  author={Na, H. and Jernigan, R. L. and Song, G.},
  journal={PLoS computational biology},
  volume={11},
  number={10},
  pages={e1004542},
  year={2015},
  publisher={Public Library of Science}
}

@article{wriggers:1998self,
  title={Self-organizing neural networks bridge the biomolecular resolution gap},
  author={Wriggers, W. and Milligan, R. A. and Schulten, K. and McCammon, J. A.},
  journal={Journal of molecular biology},
  volume={284},
  number={5},
  pages={1247--1254},
  year={1998},
  publisher={Elsevier}
}

@article{ming:2002domain,
  title={Domain movements in human fatty acid synthase by quantized elastic deformational model},
  author={Ming, D. M. and Kong, Y. F. and Wakil, S. J. and Brink, J. and Ma, J. P.},
  journal={Proceedings of the National Academy of Sciences},
  volume={99},
  number={12},
  pages={7895--7899},
  year={2002},
  publisher={National Acad Sciences}
}

@article{na:2014bridging,
  title={Bridging between normal mode analysis and elastic network models},
  author={Na, H. and Song, G.},
  journal={Proteins: Structure, Function, and Bioinformatics},
  volume={82},
  number={9},
  pages={2157--2168},
  year={2014},
  publisher={Wiley Online Library}
}


@article{martinetz:1993neural,
  title={'Neural-gas' network for vector quantization and its application to time-series prediction},
  author={Martinetz, T. M. and Berkovich, S. G. and Schulten, K. J.},
  journal={IEEE transactions on neural networks},
  volume={4},
  number={4},
  pages={558--569},
  year={1993},
  publisher={IEEE}
}


@article{lyman2008systematic,
  title={Systematic multiscale parameterization of heterogeneous elastic network models of proteins},
  author={Lyman, Edward and Pfaendtner, Jim and Voth, Gregory A},
  journal={Biophysical journal},
  volume={95},
  number={9},
  pages={4183--4192},
  year={2008},
  publisher={Elsevier}
}

@article{zhang2008systematic,
  title={A systematic methodology for defining coarse-grained sites in large biomolecules},
  author={Zhang, Zhiyong and Lu, Lanyuan and Noid, Will G and Krishna, Vinod and Pfaendtner, Jim and Voth, Gregory A},
  journal={Biophysical journal},
  volume={95},
  number={11},
  pages={5073--5083},
  year={2008},
  publisher={Elsevier}
}


@article{zhang2010coarse,
  title={Coarse-grained representations of large biomolecular complexes from low-resolution structural data},
  author={Zhang, Zhiyong and Voth, Gregory A},
  journal={Journal of chemical theory and computation},
  volume={6},
  number={9},
  pages={2990--3002},
  year={2010},
  publisher={ACS Publications}
}

@book{frey2000mesh,
  title={Mesh generation: application to finite elements},
  author={Frey, Pascal Jean and George, Paul L},
  year={2000},
  publisher={Wiley Online Library}
}

%% EMDB

@article{Tagari:2002new,
  title={New electron microscopy database and deposition system},
  author={Tagari, M. and Newman, R. and Chagoyen, M. and Carazo, J. M. and Henrick, K.},
  journal={Trends in biochemical sciences},
  volume={27},
  number={11},
  pages={589},
  year={2002},
  publisher={Elsevier}
}

%%%%%%%  solvent effects on normal modes
@article{Zhou:2008effects,
  title={Effects of surface water on protein dynamics studied by a novel coarse-grained normal mode approach},
  author={Zhou, L. and Siegelbaum, S. A.},
  journal={Biophysical journal},
  volume={94},
  number={9},
  pages={3461--3474},
  year={2008},
  publisher={Elsevier}
}

@article{Zheng:2005probing,
  title={Probing the local dynamics of nucleotide-binding pocket coupled to the global dynamics: myosin versus kinesin},
  author={Zheng, W. J. and Brooks, B. R.},
  journal={Biophysical journal},
  volume={89},
  number={1},
  pages={167--178},
  year={2005},
  publisher={Elsevier}
}

@article{Moritsugu:2005langevin,
  title={Langevin model of the temperature and hydration dependence of protein vibrational dynamics},
  author={Moritsugu, K. and Smith, J. C.},
  journal={The Journal of Physical Chemistry B},
  volume={109},
  number={24},
  pages={12182--12194},
  year={2005},
  publisher={ACS Publications}
}

@article{Diehl:1997water,
  title={Water-coupled low-frequency modes of myoglobin and lysozyme observed by inelastic neutron scattering},
  author={Diehl, M. and Doster, W. and Petry, W. and Schober, H.},
  journal={Biophysical journal},
  volume={73},
  number={5},
  pages={2726--2732},
  year={1997},
  publisher={Elsevier}
}

@article{Hinsen:2008solvent,
  title={Solvent effects in the slow dynamics of proteins},
  author={Hinsen, K. and Kneller, G. R.},
  journal={Proteins: Structure, Function, and Bioinformatics},
  volume={70},
  number={4},
  pages={1235--1242},
  year={2008},
  publisher={Wiley Online Library}
}

@article{Ansari:1992role,
  title={The role of solvent viscosity in the dynamics of protein conformational changes},
  author={Ansari, A. and Jones, C. M. and Henry, E. R. and Hofrichter, J. and Eaton, W. A.},
  journal={Science},
  volume={256},
  number={5065},
  pages={1796--1798},
  year={1992},
  publisher={American Association for the Advancement of Science}
}

@article{Brooks:1989solvent,
  title={Solvent effects on protein motion and protein effects on solvent motion: dynamics of the active site region of lysozyme},
  author={Brooks III, C. L. and Karplus, M.},
  journal={Journal of molecular biology},
  volume={208},
  number={1},
  pages={159--181},
  year={1989},
  publisher={Elsevier}
}

@article{Bahar:2009normal,
  title={Normal mode analysis of biomolecular structures: functional mechanisms of membrane proteins},
  author={Bahar, I. and Lezon, T. R. and Bakan, A. and Shrivastava, I. H.},
  journal={Chemical reviews},
  volume={110},
  number={3},
  pages={1463--1497},
  year={2009},
  publisher={ACS Publications}
}

@article{Moritsugu:2006temperature,
  title={Temperature-dependent protein dynamics: a simulation-based probabilistic diffusion-vibration {Langevin} description},
  author={Moritsugu, K. and Smith, J. C.},
  journal={The Journal of Physical Chemistry B},
  volume={110},
  number={11},
  pages={5807--5816},
  year={2006},
  publisher={ACS Publications}
}

%% ferritin

@article{Qian:2012dna,
  title={{DNA} nanotube formation based on normal mode analysis},
  author={Qian, P. and Seo, S. and Kim, J. and Kim, S. and Lim, B. S. and Liu, W. K. and Kim, B. J. and LaBean, T. H. and Park, S. H. and Kim, M. K.},
  journal={Nanotechnology},
  volume={23},
  number={10},
  pages={105704},
  year={2012},
  publisher={IOP Publishing}
}

@article{Knowles:2014amyloid,
  title={The amyloid state and its association with protein misfolding diseases},
  author={Knowles, T. P. J. and Vendruscolo, M. and Dobson, C. M.},
  journal={Nature reviews Molecular cell biology},
  volume={15},
  number={6},
  pages={384},
  year={2014},
  publisher={Nature Publishing Group}
}

%%%% self-assembly

@article{Zhang:2003fabrication,
  title={Fabrication of novel biomaterials through molecular self-assembly},
  author={Zhang, S. G.},
  journal={Nature biotechnology},
  volume={21},
  number={10},
  pages={1171},
  year={2003},
  publisher={Nature Publishing Group}
}

@article{Mcmanus:2016physics,
  title={The physics of protein self-assembly},
  author={McManus, J. J. and Charbonneau, P. and Zaccarelli, E. and Asherie, N.},
  journal={Current Opinion in Colloid \& Interface Science},
  volume={22},
  pages={73--79},
  year={2016},
  publisher={Elsevier}
}

@article{Abe:2016design,
  title={Design of a confined environment using protein cages and crystals for the development of biohybrid materials},
  author={Abe, S. and Maity, B. and Ueno, T.},
  journal={Chemical Communications},
  volume={52},
  number={39},
  pages={6496--6512},
  year={2016},
  publisher={Royal Society of Chemistry}
}

@article{Negishi:2018supramolecular,
  title={Supramolecular protein cages constructed from a crystalline protein matrix},
  author={Negishi, H. and Abe, S. and Yamashita, K. and Hirata, K. and Niwase, K. and Boudes, M. and Coulibaly, F. and Mori, H. and Ueno, T.},
  journal={Chemical Communications},
  volume={54},
  number={16},
  pages={1988--1991},
  year={2018},
  publisher={Royal Society of Chemistry}
}

@article{Abe:2018functionalization,
  title={Functionalization of protein crystals with metal ions, complexes and nanoparticles},
  author={Abe, S. and Maity, B. and Ueno, T.},
  journal={Current opinion in chemical biology},
  volume={43},
  pages={68--76},
  year={2018},
  publisher={Elsevier}
}

@article{Sana:2015unique,
  title={The unique self-assembly/disassembly property of Archaeoglobus fulgidus ferritin and its implications on molecular release from the protein cage},
  author={Sana, B. and Johnson, E. and Lim, S.},
  journal={Biochimica et Biophysica Acta (BBA)-General Subjects},
  volume={1850},
  number={12},
  pages={2544--2551},
  year={2015},
  publisher={Elsevier}
}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%  Persistent homology distance measurement

@article{mileyko2011probability,
  title={Probability measures on the space of persistence diagrams},
  author={Mileyko, Y. and Mukherjee, S. and Harer, J.},
  journal={Inverse Problems},
  volume={27},
  number={12},
  pages={124007},
  year={2011},
  publisher={IOP Publishing}
}

@article{turner2014frechet,
  title={Fr{\'e}chet means for distributions of persistence diagrams},
  author={Turner, K. and Mileyko, Y. and Mukherjee, S. and Harer, J.},
  journal={Discrete \& Computational Geometry},
  volume={52},
  number={1},
  pages={44--70},
  year={2014},
  publisher={Springer}
}



@article{marchese2017signal,
  title={Signal classification with a point process distance on the space of persistence diagrams},
  author={Marchese, A. and Maroulas, V.},
  journal={Advances in Data Analysis and Classification},
  pages={1--26},
  year={2017},
  publisher={Springer}
}

@article{chazal2017robust,
  title={Robust topological inference: Distance to a measure and kernel distance},
  author={Chazal, F. and Fasy, B. and Lecci, F. and Michel, B. and Rinaldo, A. and Rinaldo, A. and Wasserman, L.},
  journal={The Journal of Machine Learning Research},
  volume={18},
  number={1},
  pages={5845--5884},
  year={2017},
  publisher={JMLR. org}
}

@inproceedings{anirudh2016riemannian,
  title={A {Riemannian} framework for statistical analysis of topological persistence diagrams},
  author={Anirudh, R. and Venkataraman, V. and Ramamurthy, K. N., and Turaga, P.},
  booktitle={Proceedings of the IEEE Conference on Computer Vision and Pattern Recognition Workshops},
  pages={68--76},
  year={2016}
}

@article{chazal2011geometric,
  title={Geometric inference for probability measures},
  author={Chazal, F. and Cohen-Steiner, D. and M{\'e}rigot, Q.},
  journal={Foundations of Computational Mathematics},
  volume={11},
  number={6},
  pages={733--751},
  year={2011},
  publisher={Springer}
}


%%%%%%%%%%%%%%%% Persistent homology based machine learning papers

%% kernnels

@inproceedings{reininghaus2015stable,
  title={A stable multi-scale kernel for topological machine learning},
  author={Reininghaus, J. and Huber, S. and Bauer, U. and Kwitt, R.},
  booktitle={Proceedings of the IEEE conference on computer vision and pattern recognition},
  pages={4741--4748},
  year={2015}
}


@inproceedings{kwitt2015statistical,
  title={Statistical topological data analysis-a kernel perspective},
  author={Kwitt, R. and Huber, S. and Niethammer, M. and Lin, W. and Bauer, U.},
  booktitle={Advances in neural information processing systems},
  pages={3070--3078},
  year={2015}
}

@article{carriere2017sliced,
  title={Sliced wasserstein kernel for persistence diagrams},
  author={Carriere, M. and Cuturi, M. and Oudot, S.},
  journal={arXiv preprint arXiv:1706.03358},
  year={2017}
}


@article{kusano2018kernel,
  title={Kernel method for persistence diagrams via kernel embedding and weight factor},
  author={Kusano, G. and Fukumizu, K. and Hiraoka, Y.},
  journal={Journal of Machine Learning Research},
  volume={18},
  number={189},
  pages={1--41},
  year={2018}
}

@inproceedings{kusano2016persistence,
  title={Persistence weighted Gaussian kernel for topological data analysis},
  author={Kusano, G. and Hiraoka, Y. and Fukumizu, K.},
  booktitle={International Conference on Machine Learning},
  pages={2004--2013},
  year={2016}
}

@article{le2018riemannian,
  title={Riemannian Manifold Kernel for Persistence Diagrams},
  author={Le, T. and Yamada, M.},
  journal={arXiv preprint arXiv:1802.03569},
  year={2018}
}

@article{carriere2018metric,
  title={On the Metric Distortion of Embedding Persistence Diagrams into Reproducing Kernel Hilbert Spaces},
  author={Carriere, M. and Bauer, U.},
  journal={arXiv preprint arXiv:1806.06924},
  year={2018}
}


@article{padellini2017supervised,
  title={Supervised Learning with Indefinite Topological Kernels},
  author={Padellini, T. and Brutti, P.},
  journal={arXiv preprint arXiv:1709.07100},
  year={2017}
}

@article{bubenik2018persistence,
  title={The persistence landscape and some of its properties},
  author={Bubenik, P.},
  journal={arXiv preprint arXiv:1810.04963},
  year={2018}
}

@inproceedings{zhu2016stochastic,
  title={Stochastic Multiresolution Persistent Homology Kernel},
  author={Zhu, X. J. and Vartanian, A. and Bansal, M. and Nguyen, D. and Brandl, L.},
  booktitle={IJCAI},
  pages={2449--2457},
  year={2016}
}


%% Deep learning top layer
@inproceedings{hofer2017deep,
  title={Deep learning with topological signatures},
  author={Hofer, C. and Kwitt, R. and Niethammer, M. and Uhl, A.},
  booktitle={Advances in Neural Information Processing Systems},
  pages={1634--1644},
  year={2017}
}


%%%%%%%%%%%% Topological feature selections

@article{adcock2016ring,
  title={The ring of algebraic functions on persistence bar codes},
  author={Adcock, A. and Carlsson, E. and Carlsson, G.},
  journal={Homology, Homotopy and Applications},
  volume={18},
  number={1},
  pages={381--402},
  year={2016},
  publisher={International Press of Boston}
}

@article{kalivsnik2018tropical,
  title={Tropical coordinates on the space of persistence barcodes},
  author={Kali{\v{s}}nik, S.},
  journal={Foundations of Computational Mathematics},
  pages={1--29},
  year={2018},
  publisher={Springer}
}

@inproceedings{li2014persistence,
  title={Persistence-based structural recognition},
  author={Li, C. and Ovsjanikov, M. and Chazal, F.},
  booktitle={Proceedings of the IEEE Conference on Computer Vision and Pattern Recognition},
  pages={1995--2002},
  year={2014}
}

@article{zielinski2018persistence,
  title={Persistence Codebooks for Topological Data Analysis},
  author={Zielinski, B. and Juda, M. and Zeppelzauer, M.},
  journal={arXiv preprint arXiv:1802.04852},
  year={2018}
}

@article{adams2017persistence,
  title={Persistence images: {A} stable vector representation of persistent homology},
  author={Adams, H. and Emerson, T. and Kirby, M. and Neville, R. and Peterson, C. and Shipman, P. and Chepushtanova, S. and Hanson, E. and Motta, F. and Ziegelmeier, L.},
  journal={The Journal of Machine Learning Research},
  volume={18},
  number={1},
  pages={218--252},
  year={2017},
  publisher={JMLR. org}
}

@inproceedings{carriere2015stable,
  title={Stable topological signatures for points on 3d shapes},
  author={Carriere, M. and Oudot, S. Y. and Ovsjanikov, M.},
  booktitle={Computer Graphics Forum},
  volume={34},
  number={5},
  pages={1--12},
  year={2015},
  organization={Wiley Online Library}
}


@article{bubenik2017persistence,
  title={A persistence landscapes toolbox for topological statistics},
  author={Bubenik, P. and D{\l}otko, P.},
  journal={Journal of Symbolic Computation},
  volume={78},
  pages={91--114},
  year={2017},
  publisher={Elsevier}
}


@article{chevyrev2018persistence,
  title={Persistence paths and signature features in topological data analysis},
  author={Chevyrev, I. and Nanda, V. and Oberhauser, H.},
  journal={arXiv preprint arXiv:1806.00381},
  year={2018}
}

%% Top Machine learning application

@inproceedings{bae2017beyond,
  title={Beyond Deep Residual Learning for Image Restoration: Persistent Homology-Guided Manifold Simplification.},
  author={Bae, W. and Yoo, J. J. and Ye, J. C.},
  booktitle={CVPR Workshops},
  pages={1141--1149},
  year={2017}
}

@article{han2016deep,
  title={Deep residual learning for compressed sensing CT reconstruction via persistent homology analysis},
  author={Han, Y. S. and Yoo, J. and Ye, J. C.},
  journal={arXiv preprint arXiv:1611.06391},
  year={2016}
}

@article{qaiser2018fast,
  title={Fast and Accurate Tumor Segmentation of Histology Images using Persistent Homology and Deep Convolutional Features},
  author={Qaiser, T. and Tsang, Y. W. and Taniyama, D. and Sakamoto, N. and Nakane, K. and Epstein, D. and Rajpoot, N.},
  journal={arXiv preprint arXiv:1805.03699},
  year={2018}
}

@article{makarenko2016texture,
  title={Texture recognition by the methods of topological data analysis},
  author={Makarenko, N. and Kalimoldayev, M. and Pak, I. and Yessenaliyeva, A.},
  journal={Open Engineering},
  volume={6},
  number={1},
  year={2016},
  publisher={De Gruyter Open}
}

@inproceedings{zhu2013persistent,
  title={Persistent Homology: An Introduction and a New Text Representation for Natural Language Processing.},
  author={Zhu, X. J.},
  booktitle={IJCAI},
  pages={1953--1959},
  year={2013}
}

@inproceedings{dey2018protein,
  title={Protein Classification with Improved Topological Data Analysis},
  author={Dey, T. K. and Mandal, S.},
  booktitle={LIPIcs-Leibniz International Proceedings in Informatics},
  volume={113},
  year={2018},
  organization={Schloss Dagstuhl-Leibniz-Zentrum fuer Informatik}
}

@article{pachauri2011topology,
  title={Topology-based kernels with application to inference problems in Alzheimer's disease},
  author={Pachauri, D. and Hinrichs, C. and Chung, M. K. and Johnson, S. C. and Singh, V.},
  journal={IEEE transactions on medical imaging},
  volume={30},
  number={10},
  pages={1760--1770},
  year={2011},
  publisher={IEEE}
}

@inproceedings{seversky2016time,
  title={On time-series topological data analysis: New data and opportunities},
  author={Seversky, L. M. and Davis, S. and Berger, M.},
  booktitle={Proceedings of the IEEE Conference on Computer Vision and Pattern Recognition Workshops},
  pages={59--67},
  year={2016}
}


@article{zeppelzauer2018study,
  title={A study on topological descriptors for the analysis of 3D surface texture},
  author={Zeppelzauer, M. and Zieli{\'n}ski, B. and Juda, M. and Seidl, M.},
  journal={Computer Vision and Image Understanding},
  volume={167},
  pages={74--88},
  year={2018},
  publisher={Elsevier}
}



@inproceedings{bonis2016persistence,
  title={Persistence-based pooling for shape pose recognition},
  author={Bonis, T. and Ovsjanikov, M. and Oudot, S. and Chazal, F.},
  booktitle={International Workshop on Computational Topology in Image Context},
  pages={19--29},
  year={2016},
  organization={Springer}
}

@article{guo2018sparse,
  title={Sparse-TDA: Sparse Realization of Topological Data Analysis for Multi-Way Classification},
  author={Guo, W. and Manohar, K. and Brunton, S. L. and Banerjee, A. G.},
  journal={IEEE Transactions on Knowledge and Data Engineering},
  volume={30},
  number={7},
  pages={1403--1408},
  year={2018},
  publisher={IEEE}
}

@article{zhou2017exploring,
  title={Exploring generalized shape analysis by topological representations},
  author={Zhou, Z. and Huang, Y. Z. and Wang, L. and Tan, T. N.},
  journal={Pattern Recognition Letters},
  volume={87},
  pages={177--185},
  year={2017},
  publisher={Elsevier}
}


@article{anirudh2016autism,
  title={Autism Spectrum Disorder Classification using Graph Kernels on Multidimensional Time Series},
  author={Anirudh, R. and Thiagarajan, J. J. and Kim, I. and Polonik, W.},
  journal={arXiv preprint arXiv:1611.09897},
  year={2016}
}

@inproceedings{zhang2015early,
  title={Early mastitis diagnosis through topological analysis of biosignals from low-voltage alternate current electrokinetics},
  author={Zhang, Z. F. and Song, Y. and Cui, H. C. and Wu, J. and Schwartz, F. and Qi, H. R.},
  booktitle={Engineering in Medicine and Biology Society (EMBC), 2015 37th Annual International Conference of the IEEE},
  pages={542--545},
  year={2015},
  organization={IEEE}
}

@article{obayashi2018persistence,
  title={Persistence diagrams with linear machine learning models},
  author={Obayashi, I. and Hiraoka, Y. and Kimura, M.},
  journal={Journal of Applied and Computational Topology},
  volume={1},
  number={3-4},
  pages={421--449},
  year={2018},
  publisher={Springer}
}

@article{wang2014persistence,
  title={Persistence landscape of functional signal and its application to epileptic electroencaphalogram data},
  author={Wang, Y. and Ombao, H. and Chung, M. K. and others},
  journal={ENAR Distinguished Student Paper Award},
  year={2014}
}


@article{giansiracusa2017persistent,
  title={Persistent homology machine learning for fingerprint classification},
  author={Giansiracusa, N. and Giansiracusa, R. and Moon, C.},
  journal={arXiv preprint arXiv:1711.09158},
  year={2017}
}

@article{umeda2017time,
  title={Time series classification via topological data analysis},
  author={Umeda, Y.},
  journal={Information and Media Technologies},
  volume={12},
  pages={228--239},
  year={2017},
  publisher={Information and Media Technologies Editorial Board}
}

@article{niyogi2011topological,
  title={A topological view of unsupervised learning from noisy data},
  author={Niyogi, P. and Smale, S. and Weinberger, S.},
  journal={SIAM Journal on Computing},
  volume={40},
  number={3},
  pages={646--663},
  year={2011},
  publisher={SIAM}
}

@article{robins2016principal,
  title={Principal component analysis of persistent homology rank functions with case studies of spatial point patterns, sphere packing and colloids},
  author={Robins, V. and Turner, K.},
  journal={Physica D: Nonlinear Phenomena},
  volume={334},
  pages={99--117},
  year={2016},
  publisher={Elsevier}
}

%%%%%%%%%%%%%%%%%%%% persistent local homology


@inproceedings{bendich2007inferring,
  title={Inferring local homology from sampled stratified spaces},
  author={Bendich, P. and Cohen-Steiner, D. and Edelsbrunner, H. and Harer, J. and Morozov, D.},
  booktitle={Foundations of Computer Science, 2007. FOCS'07. 48th Annual IEEE Symposium on},
  pages={536--546},
  year={2007},
  organization={IEEE}
}

@inproceedings{bendich2012local,
  title={Local homology transfer and stratification learning},
  author={Bendich, P. and Wang, B. and Mukherjee, S.},
  booktitle={Proceedings of the twenty-third annual ACM-SIAM symposium on Discrete Algorithms},
  pages={1355--1370},
  year={2012},
  organization={SIAM}
}

@inproceedings{ahmed2014local,
  title={Local persistent homology based distance between maps},
  author={Ahmed, M. and Fasy, B. T. and Wenk, C.},
  booktitle={Proceedings of the 22nd ACM SIGSPATIAL International Conference on Advances in Geographic Information Systems},
  pages={43--52},
  year={2014},
  organization={ACM}
}

@inproceedings{bendich2015multi,
  title={Multi-scale local shape analysis and feature selection in machine learning applications},
  author={Bendich, P. and Gasparovic, E. and Harer, J. and Izmailov, R. and Ness, L.},
  booktitle={Neural Networks (IJCNN), 2015 International Joint Conference on},
  pages={1--8},
  year={2015},
  organization={IEEE}
}

@inproceedings{fasy2016exploring,
  title={Exploring persistent local homology in topological data analysis},
  author={Fasy, B. T. and Wang, B.},
  booktitle={Acoustics, Speech and Signal Processing (ICASSP), 2016 IEEE International Conference on},
  pages={6430--6434},
  year={2016},
  organization={IEEE}
}
%%%%%%%%%%%%%%% Clique complex

@article{giusti2015clique,
  title={Clique topology reveals intrinsic geometric structure in neural correlations},
  author={Giusti, C. and Pastalkova, E. and Curto, C. and Itskov, V.},
  journal={Proceedings of the National Academy of Sciences},
  volume={112},
  number={44},
  pages={13455--13460},
  year={2015},
  publisher={National Acad Sciences}
}

@article{giusti2016two,
  title={Two’s company, three (or more) is a simplex},
  author={Giusti, C. and Ghrist, R. and Bassett, D. S.},
  journal={Journal of computational neuroscience},
  volume={41},
  number={1},
  pages={1--14},
  year={2016},
  publisher={Springer}
}


@inproceedings{zomorodian2010tidy,
  title={The tidy set: a minimal simplicial set for computing homology of clique complexes},
  author={Zomorodian, A.},
  booktitle={Proceedings of the twenty-sixth annual symposium on Computational geometry},
  pages={257--266},
  year={2010},
  organization={ACM}
}

@article{frohmader2008face,
  title={Face vectors of flag complexes},
  author={Frohmader, A.},
  journal={Israel Journal of Mathematics},
  volume={164},
  number={1},
  pages={153--164},
  year={2008},
  publisher={Springer}
}


%%%%%%%%%%%%%%%%%%%%% Loop motion

@article{kurkcuoglu2006loop,
  title={Loop motions of triosephosphate isomerase observed with elastic networks},
  author={Kurkcuoglu, O. and Jernigan, R. L. and Doruker, P.},
  journal={Biochemistry},
  volume={45},
  number={4},
  pages={1173--1182},
  year={2006},
  publisher={ACS Publications}
}

@article{lu2006new,
  title={A new method for coarse-grained elastic normal-mode analysis},
  author={Lu, M. Y. and Poon, B. and Ma, J. P.},
  journal={Journal of chemical theory and computation},
  volume={2},
  number={3},
  pages={464--471},
  year={2006},
  publisher={ACS Publications}
}

%%%%%%%%%%%% Gaussian surface by Benzuo Lu

@article{liu:2015parameterization,
  title={Parameterization for molecular {Gaussian} surface and a comparison study of surface mesh generation},
  author={Liu, T. T. and Chen, M. X. and Lu, B. Z.},
  journal={Journal of molecular modeling},
  volume={21},
  number={5},
  pages={113},
  year={2015},
  publisher={Springer}
}

%%%%%%%%%%%%%%%%%% weighted persistent homology
@article{dawson1990homology,
  title={Homology of weighted simplicial complexes},
  author={Dawson, R. J. M.},
  journal={Cahiers de Topologie et G{\'e}om{\'e}trie Diff{\'e}rentielle Cat{\'e}goriques},
  volume={31},
  number={3},
  pages={229--243},
  year={1990}
}
@article{ren2018weighted,
  title={Weighted persistent homology},
  author={Ren, S. Q. and Wu, C. Y. and Wu, J.},
  journal={Rocky Mountain Journal of Mathematics},
  volume={48},
  number={8},
  pages={2661--2687},
  year={2018},
  publisher={Rocky Mountain Mathematics Consortium}
}

@article{wu2018weighted,
  title={Weighted (co) homology and weighted laplacian},
  author={Wu, C. Y. and Ren, S. Q. and Wu, J. and Xia, K. L.},
  journal={arXiv preprint arXiv:1804.06990},
  year={2018}
}

@article{bell2017weighted,
  title={Weighted persistent homology},
  author={Bell, G. and Lawson, A. and Martin, J. and Rudzinski, J. and Smyth, C.},
  journal={arXiv preprint arXiv:1709.00097},
  year={2017}
}

@book{edelsbrunner1992weighted,
  title={Weighted alpha shapes},
  author={Edelsbrunner, H.},
  volume={92},
  year={1992},
  publisher={University of Illinois at Urbana-Champaign, Department of Computer Science}
}

@article{buchet2016efficient,
  title={Efficient and robust persistent homology for measures},
  author={Buchet, M. and Chazal, F. and Oudot, Steve Y. and Sheehy, D. R.},
  journal={Computational Geometry},
  volume={58},
  pages={70--96},
  year={2016},
  publisher={Elsevier}
}

@article{guibas2013witnessed,
  title={Witnessed k-distance},
  author={Guibas, L. and Morozov, D. and M{\'e}rigot, Q.},
  journal={Discrete \& Computational Geometry},
  volume={49},
  number={1},
  pages={22--45},
  year={2013},
  publisher={Springer}
}

@article{petri2013topological,
  title={Topological strata of weighted complex networks},
  author={Petri, G. and Scolamiero, M. and Donato, I. and Vaccarino, F.},
  journal={PloS one},
  volume={8},
  number={6},
  pages={e66506},
  year={2013},
  publisher={Public Library of Science}
}


%%%%%%%%%%%% DNA construction and simulation
@article{meng2018molecular,
  title={A Molecular Dynamics-Quantum Mechanics Theoretical Study of {DNA}-Mediated Charge Transport in Hydrated Ionic Liquids},
  author={Meng, Z. Y. and Kubar, T. and Mu, Y. G. and Shao, F. W.},
  journal={Journal of chemical theory and computation},
  volume={14},
  number={5},
  pages={2733--2742},
  year={2018},
  publisher={ACS Publications}
}

@article{lu20033dna,
  title={{3DNA}: a software package for the analysis, rebuilding and visualization of three-dimensional nucleic acid structures},
  author={Lu, X. J. and Olson, W. K.},
  journal={Nucleic acids research},
  volume={31},
  number={17},
  pages={5108--5121},
  year={2003},
  publisher={Oxford University Press}
}

@article{hess2008gromacs,
  title={{GROMACS} 4: algorithms for highly efficient, load-balanced, and scalable molecular simulation},
  author={Hess, B. and Kutzner, C. and Van Der Spoel, D. and Lindahl, E.},
  journal={Journal of chemical theory and computation},
  volume={4},
  number={3},
  pages={435--447},
  year={2008},
  publisher={ACS Publications}
}

@article{lu1997structure,
  title={Structure and conformation of helical nucleic acids: analysis program {(SCHNAaP)}},
  author={Lu, X. J. and El Hassan, M. A. and Hunter, C. A.},
  journal={Journal of molecular biology},
  volume={273},
  number={3},
  pages={668--680},
  year={1997},
  publisher={Elsevier}
}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%  Urea and TMAO

@article{rossky2008protein,
  title={Protein denaturation by urea: slash and bond},
  author={Rossky, P. J.},
  journal={Proceedings of the National Academy of Sciences},
  volume={105},
  number={44},
  pages={16825--16826},
  year={2008},
  publisher={National Acad Sciences}
}

@article{rezus2006effect,
  title={Effect of urea on the structural dynamics of water},
  author={Rezus, Y. L. A. and Bakker, H. J.},
  journal={Proceedings of the National Academy of Sciences},
  volume={103},
  number={49},
  pages={18417--18420},
  year={2006},
  publisher={National Acad Sciences}
}

@article{panuszko2009effects,
  title={Effects of urea and {trimethylamine-N-oxide} on the properties of water and the secondary structure of hen egg white lysozyme},
  author={Panuszko, A. and Bruzdziak, P. and Zielkiewicz, J. and Wyrzykowski, D. and Stangret, J.},
  journal={The Journal of Physical Chemistry B},
  volume={113},
  number={44},
  pages={14797--14809},
  year={2009},
  publisher={ACS Publications}
}

@article{idrissi2010effect,
  title={The effect of urea on the structure of water: A molecular dynamics simulation},
  author={Idrissi, A. and Gerard, M. and Damay, P. and Kiselev, M. and Puhovsky, Y. and Cinar, E. and Lagant, P. and Vergoten, G.},
  journal={The Journal of Physical Chemistry B},
  volume={114},
  number={13},
  pages={4731--4738},
  year={2010},
  publisher={ACS Publications}
}

@article{bandyopadhyay2014molecular,
  title={Molecular dynamics simulation of aqueous urea solution: is urea a structure breaker?},
  author={Bandyopadhyay, D. and Mohan, S. and Ghosh, S. K. and Choudhury, N.},
  journal={The Journal of Physical Chemistry B},
  volume={118},
  number={40},
  pages={11757--11768},
  year={2014},
  publisher={ACS Publications}
}

@article{abraham2015gromacs,
  title={{GROMACS}: High performance molecular simulations through multi-level parallelism from laptops to supercomputers},
  author={Abraham, M. J. and Murtola, T. and Schulz, R. and P{\'a}ll, S. and Smith, J. C. and Hess, B. and Lindahl, E.},
  journal={SoftwareX},
  volume={1},
  pages={19--25},
  year={2015},
  publisher={Elsevier}
}

@article{berendsen1995gromacs,
  title={{GROMACS}: a message-passing parallel molecular dynamics implementation},
  author={Berendsen, H. J. C. and van der Spoel, D. and van Drunen, R.},
  journal={Computer physics communications},
  volume={91},
  number={1-3},
  pages={43--56},
  year={1995},
  publisher={Elsevier}
}

@article{kast2003binary,
  title={Binary phases of aliphatic N-oxides and water: Force field development and molecular dynamics simulation},
  author={Kast, K. M. and Brickmann, J. and Kast, S. M. and Berry, R. S.},
  journal={The Journal of Physical Chemistry A},
  volume={107},
  number={27},
  pages={5342--5351},
  year={2003},
  publisher={ACS Publications}
}


@article{tseng1998natural,
  title={Natural methylamine osmolytes, trimethylamine {N}-oxide and betaine, increase tau-induced polymerization of microtubules},
  author={Tseng, H. C. and Graves, D. J.},
  journal={Biochemical and biophysical research communications},
  volume={250},
  number={3},
  pages={726--730},
  year={1998},
  publisher={Elsevier}
}

@article{baskakov1999trimethylamine,
  title={{Trimethylamine N-oxide-induced} cooperative folding of an intrinsically unfolded transcription-activating fragment of human glucocorticoid receptor},
  author={Baskakov, I. V. and Kumar, R. and Srinivasan, G. and Ji, Y. S. and Bolen, D. W. and Thompson, E. B.},
  journal={Journal of Biological Chemistry},
  volume={274},
  number={16},
  pages={10693--10696},
  year={1999},
  publisher={ASBMB}
}

@article{baskakov1998forcing,
  title={Forcing thermodynamically unfolded proteins to fold},
  author={Baskakov, I. and Bolen, D. W.},
  journal={Journal of Biological Chemistry},
  volume={273},
  number={9},
  pages={4831--4834},
  year={1998},
  publisher={ASBMB}
}


@article{uversky2001trimethylamine,
  title={{Trimethylamine-N-oxide-induced} folding of $\alpha$-synuclein},
  author={Uversky, V. N. and Li, J. and Fink, A. L.},
  journal={FEBS letters},
  volume={509},
  number={1},
  pages={31--35},
  year={2001},
  publisher={Wiley Online Library}
}

@article{rosgen2012volume,
  title={Volume exclusion and {H}-bonding dominate the thermodynamics and solvation of {trimethylamine-N-oxide} in aqueous urea},
  author={Rosgen, J. and Jackson-Atogi, R.},
  journal={Journal of the American Chemical Society},
  volume={134},
  number={7},
  pages={3590--3597},
  year={2012},
  publisher={ACS Publications}
}

@article{paul2007structure,
  title={Structure and interaction in aqueous {urea-trimethylamine-N-oxide} solutions},
  author={Paul, S. and Patey, G. N.},
  journal={Journal of the American Chemical Society},
  volume={129},
  number={14},
  pages={4476--4482},
  year={2007},
  publisher={ACS Publications}
}

@article{meersman2011x,
  title={An {X}-ray and neutron scattering study of the equilibrium between trimethylamine {N}-oxide and urea in aqueous solution},
  author={Meersman, F. and Bowron, D. and Soper, A. K. and Koch, M. H. J.},
  journal={Physical Chemistry Chemical Physics},
  volume={13},
  number={30},
  pages={13765--13771},
  year={2011},
  publisher={Royal Society of Chemistry}
}


@article{ganguly2015mutual,
  title={Mutual exclusion of urea and trimethylamine {N-oxide} from amino acids in mixed solvent environment},
  author={Ganguly, P. and Hajari, T. and Shea, J. E. and van der Vegt, N. F. A.},
  journal={The journal of physical chemistry letters},
  volume={6},
  number={4},
  pages={581--585},
  year={2015},
  publisher={ACS Publications}
}

@article{sahle2016influence,
  title={Influence of {TMAO} and urea on the structure of water studied by inelastic {X-ray} scattering},
  author={Sahle, C. J. and Schroer, M. A. and Juurinen, I. and Niskanen, J.},
  journal={Physical Chemistry Chemical Physics},
  volume={18},
  number={24},
  pages={16518--16526},
  year={2016},
  publisher={Royal Society of Chemistry}
}


@article{ganguly2017trimethylamine,
  title={Trimethylamine {N}-oxide Counteracts Urea Denaturation by Inhibiting Protein--Urea Preferential Interaction},
  author={Ganguly, P. and Boserman, P. and van der Vegt, N. F. and Shea, J. E.},
  journal={Journal of the American Chemical Society},
  volume={140},
  number={1},
  pages={483--492},
  year={2017},
  publisher={ACS Publications}
}

@article{hunger2015water,
  title={Water-mediated interactions between trimethylamine-{N}-oxide and urea},
  author={Hunger, J. and Ottosson, N. and Mazur, K. and Bonn, M. and Bakker, H. J.},
  journal={Physical Chemistry Chemical Physics},
  volume={17},
  number={1},
  pages={298--306},
  year={2015},
  publisher={Royal Society of Chemistry}
}

@article{liao2017trimethylamine,
  title={Trimethylamine {N}-oxide stabilizes proteins via a distinct mechanism compared with betaine and glycine},
  author={Liao, Y. T. and Manson, A. C. and DeLyser, M. R. and Noid, W. G. and Cremer, P. S.},
  journal={Proceedings of the National Academy of Sciences},
  volume={114},
  number={10},
  pages={2479--2484},
  year={2017},
  publisher={National Acad Sciences}
}

@article{ganguly2016hydrophobic,
  title={Hydrophobic association in mixed urea--{TMAO} solutions},
  author={Ganguly, P. and van der Vegt, N. F. and Shea, J. E.},
  journal={The journal of physical chemistry letters},
  volume={7},
  number={15},
  pages={3052--3059},
  year={2016},
  publisher={ACS Publications}
}

@article{zetterholm2018noncovalent,
  title={Noncovalent Interactions between {Trimethylamine N-Oxide (TMAO)}, Urea, and Water},
  author={Zetterholm, S. G. and Verville, G. A. and Boutwell, L. and Boland, C. and Prather, J. C. and Bethea, J. and Cauley, J. and Warren, K. E. and Smith, S. A. and Magers, D. H. and others},
  journal={The Journal of Physical Chemistry B},
  volume={122},
  number={38},
  pages={8805--8811},
  year={2018},
  publisher={ACS Publications}
}

@article{xie2018large,
  title={Large hydrogen-bond mismatch between {TMAO} and urea promotes their hydrophobic association},
  author={Xie, W. J. and Cha, S. and Ohto, T. and Mizukami, W. and Mao, Y. and Wagner, M. and Bonn, M. and Hunger, J. and Nagata, Y.},
  journal={Chem},
  volume={4},
  number={11},
  pages={2615--2627},
  year={2018},
  publisher={Elsevier}
}

%%%%%%%%%%%%%%%%%%% MD simulation of TMAO and UREA
@article{pearlman1995amber,
  title={{AMBER}, a package of computer programs for applying molecular mechanics, normal mode analysis, molecular dynamics and free energy calculations to simulate the structural and energetic properties of molecules},
  author={Pearlman, D. A. and Case, D. A. and Caldwell, J. W. and Ross, W. S. and Cheatham III, T. E. and DeBolt, S. and Ferguson, D. and Seibel, G. and Kollman, P.},
  journal={Computer Physics Communications},
  volume={91},
  number={1-3},
  pages={1--41},
  year={1995},
  publisher={Elsevier}
}

@article{horn2004development,
  title={Development of an improved four-site water model for biomolecular simulations: {TIP4P-Ew}},
  author={Horn, H. W. and Swope, W. C. and Pitera, J. W. and Madura, J. D. and Dick, T. J. and Hura, G. L. and Head-Gordon, T.},
  journal={The Journal of chemical physics},
  volume={120},
  number={20},
  pages={9665--9678},
  year={2004},
  publisher={AIP}
}

@article{hess1997lincs,
  title={LINCS: a linear constraint solver for molecular simulations},
  author={Hess, B. and Bekker, H. and Berendsen, H. J. C. and Fraaije, J. G. E. M.},
  journal={Journal of computational chemistry},
  volume={18},
  number={12},
  pages={1463--1472},
  year={1997},
  publisher={Wiley Online Library}
}

@article{essmann1995smooth,
  title={A smooth particle mesh {Ewald} method},
  author={Essmann, U. and Perera, L. and Berkowitz, M. L. and Darden, T. and Lee, H. and Pedersen, L. G.},
  journal={The Journal of chemical physics},
  volume={103},
  number={19},
  pages={8577--8593},
  year={1995},
  publisher={AIP}
}

%%%%%%%%%%%% Literature on Vault

@article{bhaskar:2017engineering,
	title={Engineering protein nanocages as carriers for biomedical applications},
	author={Bhaskar, S. and Lim, S.},
	journal={NPG Asia Materials},
	volume={9},
	number={4},
	pages={e371},
	year={2017},
	publisher={Nature Publishing Group}
}

@article{kong1999structure,
	title={Structure of the vault, a ubiquitous celular component},
	author={Kong, L. B. and Siva, A. C. and Rome, L. H. and Stewart, P. L.},
	journal={Structure},
	volume={7},
	number={4},
	pages={371--379},
	year={1999},
	publisher={Elsevier}
}

@article{poderycki2006vault,
	title={The vault exterior shell is a dynamic structure that allows incorporation of vault-associated proteins into its interior},
	author={Poderycki, M. J. and Kickhoefer, V. A. and Kaddis, C. S. and Raval-Fernandes, S. and Johansson, E. and Zink, J. I. and Loo, J. A. and Rome, L. H.},
	journal={Biochemistry},
	volume={45},
	number={39},
	pages={12184--12193},
	year={2006},
	publisher={ACS Publications}
}

@article{goldsmith2007vault,
	title={Vault nanocapsule dissociation into halves triggered at low {pH}},
	author={Goldsmith, L. E. and Yu, M. and Rome, L. H. and Monbouquette, H. G.},
	journal={Biochemistry},
	volume={46},
	number={10},
	pages={2865--2875},
	year={2007},
	publisher={ACS Publications}
}

@article{esfandiary2009structural,
	title={Structural stability of vault particles},
	author={Esfandiary, R. and Kickhoefer, V. A. and Rome, L. H. and Joshi, S. B. and Middaugh, C. R.},
	journal={Journal of pharmaceutical sciences},
	volume={98},
	number={4},
	pages={1376--1386},
	year={2009},
	publisher={Wiley Online Library}
}

@article{querol2009mechanism,
	title={The mechanism of vault opening from the high resolution structure of the {N}-terminal repeats of {MVP}},
	author={Querol-Aud{\'\i}, J. and Casa{\~n}as, A. and Us{\'o}n, I. and Luque, D. and Cast{\'o}n, J. R. and Fita, I. and Verdaguer, N.},
	journal={The EMBO journal},
	volume={28},
	number={21},
	pages={3450--3457},
	year={2009},
	publisher={EMBO Press}
}

@article{goldsmith2009utilization,
	title={Utilization of a protein shuttle to load vault nanocapsules with gold probes and proteins},
	author={Goldsmith, L. E. and Pupols, M. and Kickhoefer, V. A. and Rome, L. H. and Monbouquette, H. G.},
	journal={Acs Nano},
	volume={3},
	number={10},
	pages={3175--3183},
	year={2009},
	publisher={ACS Publications}
}

@article{casanas2013new,
	title={New features of vault architecture and dynamics revealed by novel refinement using the deformable elastic network approach},
	author={Casa{\~n}as, A. and Querol-Aud{\'\i}, J. and Guerra, P. and Pous, J. and Tanaka, H. and Tsukihara, T. and Verdaguer, N. and Fita, I.},
	journal={Acta Crystallographica Section D: Biological Crystallography},
	volume={69},
	number={6},
	pages={1054--1061},
	year={2013},
	publisher={International Union of Crystallography}
}

@article{casanas2012vault,
	title={Vault particles: a new generation of delivery nanodevices},
	author={Casa{\~n}as, A. and Guerra, P. and Fita, I. and Verdaguer, N.},
	journal={Current opinion in biotechnology},
	volume={23},
	number={6},
	pages={972--977},
	year={2012},
	publisher={Elsevier}
}

@article{kedersha1986isolation,
	title={Isolation and characterization of a novel ribonucleoprotein particle: large structures contain a single species of small {RNA}},
	author={Kedersha, N. L. and Rome, L. H.},
	journal={The Journal of cell biology},
	volume={103},
	number={3},
	pages={699--709},
	year={1986},
	publisher={Rockefeller University Press}
}

@article{yang2010vaults,
	title={Vaults are dynamically unconstrained cytoplasmic nanoparticles capable of half vault exchange},
	author={Yang, J. and Kickhoefer, V. A. and Ng, B. C. and Gopal, A. and Bentolila, L. A. and John, S. and Tolbert, S. H. and Rome, L. H.},
	journal={Acs Nano},
	volume={4},
	number={12},
	pages={7229--7240},
	year={2010},
	publisher={ACS Publications}
}

@article{anderson2007draft,
	title={Draft crystal structure of the vault shell at 9-{\AA} resolution},
	author={Anderson, D. H. and Kickhoefer, V. A. and Sievers, S. A. and Rome, L. H. and Eisenberg, D.},
	journal={PLoS biology},
	volume={5},
	number={11},
	pages={e318},
	year={2007},
	publisher={Public Library of Science}
}

@article{ding2018solution,
	title={Solution structures of engineered vault particles},
	author={Ding, K. and Zhang, X. and Mrazek, J. and Kickhoefer, V. A. and Lai, M. and Ng, H. L. and Yang, O. O. and Rome, L. H. and Zhou, Z. H.},
	journal={Structure},
	volume={26},
	number={4},
	pages={619--626},
	year={2018},
	publisher={Elsevier}
}

%%%%%%%%%%%%%%%%%%%%%%%%%% Voronoi diagram

@article{petvrek2007mole,
  title={{MOLE}: a Voronoi diagram-based explorer of molecular channels, pores, and tunnels},
  author={Pet{\v{r}}ek, M. and Ko{\v{s}}inov{\'a}, P. and Ko{\v{c}}a, J. and Otyepka, M.},
  journal={Structure},
  volume={15},
  number={11},
  pages={1357--1363},
  year={2007},
  publisher={Elsevier}
}

@article{edelsbrunner2005geometry,
  title={The geometry of biomolecular solvation},
  author={Edelsbrunner, H. and Koehl, P.},
  journal={Combinatorial and computational geometry},
  volume={52},
  pages={243--275},
  year={2005},
  publisher={Cmbridge Univ. Press, New York}
}

@article{chalikian1998thermodynamic,
  title={Thermodynamic analysis of biomolecules: a volumetric approach},
  author={Chalikian, T. V. and Breslauer, K. J.},
  journal={Current opinion in structural biology},
  volume={8},
  number={5},
  pages={657--664},
  year={1998},
  publisher={Elsevier}
}

@article{cazals2006revisiting,
  title={Revisiting the Voronoi description of protein--protein interfaces},
  author={Cazals, F. and Proust, F. and Bahadur, R. P. and Janin, J.},
  journal={Protein Science},
  volume={15},
  number={9},
  pages={2082--2092},
  year={2006},
  publisher={Wiley Online Library}
}

@article{smolin2017tmao,
  title={{TMAO} and urea in the hydration shell of the protein SNase},
  author={Smolin, N. and Voloshin, V. P. and Anikeenko, A. V. and Geiger, A. and Winter, R. and Medvedev, N. N.},
  journal={Physical Chemistry Chemical Physics},
  volume={19},
  number={9},
  pages={6345--6357},
  year={2017},
  publisher={Royal Society of Chemistry}
}

%%% radial distribution function
@book{chandler1987introduction,
  publisher={Oxford University Press},
  title={Introduction to Modern Statistical Mechanics},
  year={1987},
  author={Chandler, D.},
  pages={288}
}

%%%%%%%%%%%%% TDA in ion aggregation

@article{steinberg2019new,
  title={A new topological descriptor for water network structure},
  author={Steinberg, L. and Russo, J. and Frey, J. G.},
  journal={Journal of cheminformatics},
  volume={11},
  number={1},
  pages={48},
  year={2019},
  publisher={BioMed Central}
}

@article{pirashvili2018improved,
  title={Improved understanding of aqueous solubility modeling through topological data analysis},
  author={Pirashvili, M. and Steinberg, L. and Guillamon, F. B. and Niranjan, M. and Frey, J. G. and Brodzki, J.},
  journal={Journal of cheminformatics},
  volume={10},
  number={1},
  pages={54},
  year={2018},
  publisher={Nature Publishing Group}
}

%%%%%%%%%%%%%%%%%%%%%%% perovskite review

@article{grancini2018dimensional,
  title={Dimensional tailoring of hybrid perovskites for photovoltaics},
  author={Grancini, G. and Nazeeruddin, M. K.},
  journal={Nature Reviews Materials},
  pages={1},
  year={2018},
  publisher={Nature Publishing Group}
}

@article{mao2018two,
  title={Two-dimensional hybrid halide perovskites: principles and promises},
  author={Mao, L. and Stoumpos, C. C. and Kanatzidis, M. G.},
  journal={Journal of the American Chemical Society},
  volume={141},
  number={3},
  pages={1171--1190},
  year={2018},
  publisher={ACS Publications}
}

@article{ahmad2019dion,
  title={{Dion-Jacobson} Phase {2D} Layered Perovskites for Solar Cells with Ultrahigh Stability},
  author={Ahmad, S. and Fu, P. and Yu, S. W. and Yang, Q. and Liu, X. and Wang, X. C. and Wang, X. L. and Guo, X. and Li, C.},
  journal={Joule},
  volume={3},
  number={3},
  pages={794--806},
  year={2019},
  publisher={Elsevier}
}


@article{stoumpos2016ruddlesden,
  title={{Ruddlesden-Popper} hybrid lead iodide perovskite {2D} homologous semiconductors},
  author={Stoumpos, C. C. and Cao, D. H. and Clark, D. J. and Young, J. and Rondinelli, J. M. and Jang, J. I. and Hupp, J. T. and Kanatzidis, M. G.},
  journal={Chemistry of Materials},
  volume={28},
  number={8},
  pages={2852--2867},
  year={2016},
  publisher={ACS Publications}
}

%%%%%%%%%%%%%%%%%%%%%%% photovoltaics

@article{goldschmidt2015upconversion,
  title={Upconversion for photovoltaics--a review of materials, devices and concepts for performance enhancement},
  author={Goldschmidt, J. C. and Fischer, S.},
  journal={Advanced Optical Materials},
  volume={3},
  number={4},
  pages={510--535},
  year={2015},
  publisher={Wiley Online Library}
}

%%%%%%%%%%%% HOIP history
@article{kojima2009organometal,
  title={Organometal halide perovskites as visible-light sensitizers for photovoltaic cells},
  author={Kojima, Akihiro and Teshima, Kenjiro and Shirai, Yasuo and Miyasaka, Tsutomu},
  journal={Journal of the American Chemical Society},
  volume={131},
  number={17},
  pages={6050--6051},
  year={2009},
  publisher={ACS Publications}
}

@article{yang2017iodide,
  title={Iodide management in formamidinium-lead-halide-based perovskite layers for efficient solar cells},
  author={Yang, Woon Seok and Park, Byung-Wook and Jung, Eui Hyuk and Jeon, Nam Joong and Kim, Young Chan and Lee, Dong Uk and Shin, Seong Sik and Seo, Jangwon and Kim, Eun Kyu and Noh, Jun Hong and others},
  journal={Science},
  volume={356},
  number={6345},
  pages={1376--1379},
  year={2017},
  publisher={American Association for the Advancement of Science}
}

@article{jung2019efficient,
  title={Efficient, stable and scalable perovskite solar cells using poly (3-hexylthiophene)},
  author={Jung, Eui Hyuk and Jeon, Nam Joong and Park, Eun Young and Moon, Chan Su and Shin, Tae Joo and Yang, Tae-Youl and Noh, Jun Hong and Seo, Jangwon},
  journal={Nature},
  volume={567},
  number={7749},
  pages={511--515},
  year={2019},
  publisher={Nature Publishing Group}
}

%% HOIP dataset

@article{kim2017hybrid,
  title={A hybrid organic-inorganic perovskite dataset},
  author={Kim, Chiho and Huan, Tran Doan and Krishnan, Sridevi and Ramprasad, Rampi},
  journal={Scientific data},
  volume={4},
  number={1},
  pages={1--11},
  year={2017},
  publisher={Nature Publishing Group}
}

%%%%%%%%%%%%%%%%%%%%%%% perovskite machine learning

%%%% Review
@article{gu2019machine,
  title={Machine learning for renewable energy materials},
  author={Gu, Geun Ho and Noh, Juhwan and Kim, Inkyung and Jung, Yousung},
  journal={Journal of Materials Chemistry A},
  volume={7},
  number={29},
  pages={17096--17117},
  year={2019},
  publisher={Royal Society of Chemistry}
}

@article{yilmaz2020critical,
  title={Critical review of machine learning applications in perovskite solar research},
  author={Y{\i}lmaz, Beyza and Y{\i}ld{\i}r{\i}m, Ramazan},
  journal={Nano Energy},
  pages={105546},
  year={2020},
  publisher={Elsevier}
}

@article{odabacsi2019performance,
  title={Performance analysis of perovskite solar cells in 2013--2018 using machine-learning tools},
  author={Odaba{\c{s}}{\i}, {\c{C}}a{\u{g}}la and Y{\i}ld{\i}r{\i}m, Ramazan},
  journal={Nano Energy},
  volume={56},
  pages={770--791},
  year={2019},
  publisher={Elsevier}
}

%%%% single perovskite
@article{pilania2016finding,
  title={Finding new perovskite halides via machine learning},
  author={Pilania, Ghanshyam and Balachandran, Prasanna V and Kim, Chiho and Lookman, Turab},
  journal={Frontiers in Materials},
  volume={3},
  pages={19},
  year={2016},
  publisher={Frontiers}
}

%% GCN
@article{xie2018crystal,
  title={Crystal graph convolutional neural networks for an accurate and interpretable prediction of material properties},
  author={Xie, Tian and Grossman, Jeffrey C},
  journal={Physical review letters},
  volume={120},
  number={14},
  pages={145301},
  year={2018},
  publisher={APS}
}

@article{balachandran2018predictions,
  title={Predictions of new {ABO3} perovskite compounds by combining machine learning and density functional theory},
  author={Balachandran, P. V. and Emery, A. A. and Gubernatis, J. E. and Lookman, T. and Wolverton, C. and Zunger, A.},
  journal={Physical Review Materials},
  volume={2},
  number={4},
  pages={043802},
  year={2018},
  publisher={APS}
}

@article{xu2018rationalizing,
  title={Rationalizing perovskite data for machine learning and materials design},
  author={Xu, Q. C. and Li, Z. Z. and Liu, M. and Yin, W. J.},
  journal={The journal of physical chemistry letters},
  volume={9},
  number={24},
  pages={6948--6954},
  year={2018},
  publisher={ACS Publications}
}

@article{li2018stability,
  title={Stability engineering of halide perovskite via machine learning},
  author={Li, Z. Z. and Xu, Q. C. and Sun, Q. D. and Hou, Z. F. and Yin, W. J.},
  journal={arXiv preprint arXiv:1803.06042},
  year={2018}
}

@article{park2019exploring,
  title={Exploring new approaches towards the formability of mixed-ion perovskites by {DFT} and machine learning},
  author={Park, Heesoo and Mall, Raghvendra and Alharbi, Fahhad H and Sanvito, Stefano and Tabet, Nouar and Bensmail, Halima and El-Mellouhi, Fedwa},
  journal={Physical Chemistry Chemical Physics},
  volume={21},
  number={3},
  pages={1078--1088},
  year={2019},
  publisher={The Royal Society of Chemistry}
}

@article{jacobs2019materials,
  title={Materials Discovery of stable and nontoxic halide perovskite materials for high-efficiency solar cells},
  author={Jacobs, Ryan and Luo, Guangfu and Morgan, Dane},
  journal={Advanced Functional Materials},
  volume={29},
  number={23},
  pages={1804354},
  year={2019},
  publisher={Wiley Online Library}
}

@article{schmidt2017predicting,
  title={Predicting the thermodynamic stability of solids combining density functional theory and machine learning},
  author={Schmidt, Jonathan and Shi, Jingming and Borlido, Pedro and Chen, Liming and Botti, Silvana and Marques, Miguel AL},
  journal={Chemistry of Materials},
  volume={29},
  number={12},
  pages={5090--5103},
  year={2017},
  publisher={ACS Publications}
}

%%% double perovskite
@article{pilania2016machine,
  title={Machine learning bandgaps of double perovskites},
  author={Pilania, G. and Mannodi-Kanakkithodi, A. and Uberuaga, B. P. and Ramprasad, R. and Gubernatis, J. E. and Lookman, T.},
  journal={Scientific reports},
  volume={6},
  pages={19375},
  year={2016},
  publisher={Nature Publishing Group}
}

@article{askerka2019learning,
  title={Learning-in-Templates Enables Accelerated Discovery and Synthesis of New Stable Double Perovskites},
  author={Askerka, M. and Li, Z. L. and Lempen, M. and Liu, Y. N. and Johnston, A. and Saidaminov, M. I. and Zajacz, Z. and Sargent, E. H.},
  journal={Journal of the American Chemical Society},
  volume={141},
  number={8},
  pages={3682--3690},
  year={2019},
  publisher={ACS Publications}
}


@article{im2019identifying,
  title={Identifying {Pb}-free perovskites for solar cells by machine learning},
  author={Im, J. and Lee, S. and Ko, T. W. and Kim, H. W. and Hyon, Y. and Chang, H.},
  journal={npj Computational Materials},
  volume={5},
  number={1},
  pages={37},
  year={2019},
  publisher={Nature Publishing Group}
}

@article{l2019machine,
  title={Machine Learning Augmented Discovery of Chalcogenide Double Perovskites for Photovoltaics},
  author={L. Agiorgousis, M. and Sun, Y. Y. and Choe, D. H. and West, D. and Zhang, S. B.},
  journal={Advanced Theory and Simulations},
  volume={2},
  number={5},
  pages={1800173},
  year={2019},
  publisher={Wiley Online Library}
}

@article{li2019thermodynamic,
  title={Thermodynamic stability landscape of halide double perovskites via high-throughput computing and machine learning},
  author={Li, Zhenzhu and Xu, Qichen and Sun, Qingde and Hou, Zhufeng and Yin, Wan-Jian},
  journal={Advanced Functional Materials},
  volume={29},
  number={9},
  pages={1807280},
  year={2019},
  publisher={Wiley Online Library}
}
%%%% HOIP machine learning
@article{wu2019global,
  title={Global discovery of stable and non-toxic hybrid organic-inorganic perovskites for photovoltaic systems by combining machine learning method with first principle calculations},
  author={Wu, Tianmin and Wang, Jian},
  journal={Nano Energy},
  volume={66},
  pages={104070},
  year={2019},
  publisher={Elsevier}
}

@article{lu2018accelerated,
  title={Accelerated discovery of stable lead-free hybrid organic-inorganic perovskites via machine learning},
  author={Lu, Shuaihua and Zhou, Qionghua and Ouyang, Yixin and Guo, Yilv and Li, Qiang and Wang, Jinlan},
  journal={Nature communications},
  volume={9},
  number={1},
  pages={1--8},
  year={2018},
  publisher={Nature Publishing Group}
}

%%%% design and fabrication

@article{sun2018accelerating,
  title={Accelerating Photovoltaic Materials Development via High-Throughput Experiments and Machine-Learning-Assisted Diagnosis},
  author={Sun, S. J. and Hartono, N. T. P. and Ren, Z. D. and Oviedo, F. and Buscemi, A. M. and Layurova, M. and Chen, D. X. and Ogunfunmi, T. and Thapa, J. and Ramasamy, S. and others},
  journal={arXiv preprint arXiv:1812.01025},
  year={2018}
}


@article{howard2018machine,
  title={Machine Learning for Perovskites' Reap-Rest-Recovery Cycle},
  author={Howard, J. M. and Tennyson, E. M. and Neves, B. R. A. and Leite, M. S.},
  journal={Joule},
  year={2018},
  publisher={Elsevier}
}


@article{li2019machine,
  title={Machine Learning ({ML})-Assisted Design and Fabrication for Solar Cells},
  author={Li, Fan and Peng, Xiaoqi and Wang, Zuo and Zhou, Yi and Wu, Yuxia and Jiang, Minlin and Xu, Min},
  journal={Energy \& Environmental Materials},
  volume={2},
  number={4},
  pages={280--291},
  year={2019},
  publisher={Wiley Online Library}
}

@article{yu2019machine,
  title={Machine Learning for Understanding Compatibility of Organic--Inorganic Hybrid Perovskites with Post-Treatment {Amines}},
  author={Yu, Yongze and Tan, Xuanheng and Ning, Shougui and Wu, Yiying},
  journal={ACS Energy Letters},
  volume={4},
  number={2},
  pages={397--404},
  year={2019},
  publisher={ACS Publications}
}

%%%% Perovskite solar cell setting

@article{li2019predictions,
  title={Predictions and Strategies Learned from Machine Learning to Develop High-Performing Perovskite Solar Cells},
  author={Li, Jinxin and Pradhan, Basudev and Gaur, Surya and Thomas, Jayan},
  journal={Advanced Energy Materials},
  volume={9},
  number={46},
  pages={1901891},
  year={2019},
  publisher={Wiley Online Library}
}

@article{odabacsi2020assessment,
  title={Assessment of Reproducibility, Hysteresis, and Stability Relations in Perovskite Solar Cells Using Machine Learning},
  author={Odaba{\c{s}}{\i}, {\c{C}}a{\u{g}}la and Y{\i}ld{\i}r{\i}m, Ramazan},
  journal={Energy Technology},
  volume={8},
  number={12},
  pages={1901449},
  year={2020},
  publisher={Wiley Online Library}
}

@article{odabacsi2020machine,
  title={Machine learning analysis on stability of perovskite solar cells},
  author={Odaba{\c{s}}{\i}, {\c{C}}a{\u{g}}la and Y{\i}ld{\i}r{\i}m, Ramazan},
  journal={Solar Energy Materials and Solar Cells},
  volume={205},
  pages={110284},
  year={2020},
  publisher={Elsevier}
}
%%%%%%%%%%%%%%%  material featurization

@article{schutt2014represent,
  title={How to represent crystal structures for machine learning: Towards fast prediction of electronic properties},
  author={Sch{\"u}tt, K. T. and Glawe, H. and Brockherde, F. and Sanna, A. and M{\"u}ller, K. R.and Gross, E. K. U.},
  journal={Physical Review B},
  volume={89},
  number={20},
  pages={205118},
  year={2014},
  publisher={APS}
}

@article{isayev2015materials,
  title={Materials cartography: representing and mining materials space using structural and electronic fingerprints},
  author={Isayev, O. and Fourches, D. and Muratov, E. N. and Oses, C. and Rasch, K. and Tropsha, A. and Curtarolo, S.},
  journal={Chemistry of Materials},
  volume={27},
  number={3},
  pages={735--743},
  year={2015},
  publisher={ACS Publications}
}

@article{huan2015accelerated,
  title={Accelerated materials property predictions and design using motif-based fingerprints},
  author={Huan, T. D. and Mannodi-Kanakkithodi, A. and Ramprasad, R.},
  journal={Physical Review B},
  volume={92},
  number={1},
  pages={014106},
  year={2015},
  publisher={APS}
}

%%%%%%%%%%%%%%%%%%%%%%% material informatics
@article{rajan2005materials,
  title={Materials informatics},
  author={Rajan, K.},
  journal={Materials Today},
  volume={8},
  number={10},
  pages={38--45},
  year={2005},
  publisher={Elsevier}
}

@book{rajan2013informatics,
  title={Informatics for materials science and engineering: data-driven discovery for accelerated experimentation and application},
  author={Rajan, K.},
  year={2013},
  publisher={Butterworth-Heinemann}
}

@article{ward2017atomistic,
  title={Atomistic calculations and materials informatics: A review},
  author={Ward, L. and Wolverton, C.},
  journal={Current Opinion in Solid State and Materials Science},
  volume={21},
  number={3},
  pages={167--176},
  year={2017},
  publisher={Elsevier}
}


@article{schleder2019dft,
  title={From {DFT} to machine learning: recent approaches to materials science--a review},
  author={Schleder, G. R. and Padilha, A. C. and Acosta, C. M. and Costa, M. and Fazzio, A.},
  journal={Journal of Physics: Materials},
  volume={2},
  number={3},
  pages={032001},
  year={2019},
  publisher={IOP Publishing}
}

@article{green2017fulfilling,
  title={Fulfilling the promise of the materials genome initiative with high-throughput experimental methodologies},
  author={Green, M. L. and Choi, C. L. and Hattrick-Simpers, J. R. and Joshi, A. M. and Takeuchi, I. and Barron, S. C. and others},
  journal={Applied Physics Reviews},
  volume={4},
  number={1},
  pages={011105},
  year={2017},
  publisher={AIP Publishing}
}

@article{agrawal2016perspective,
  title={Perspective: Materials informatics and big data: Realization of the "fourth paradigm" of science in materials science},
  author={Agrawal, A. and Choudhary, A.},
  journal={Apl Materials},
  volume={4},
  number={5},
  pages={053208},
  year={2016},
  publisher={AIP Publishing}
}

@article{ramprasad2017machine,
  title={Machine learning in materials informatics: recent applications and prospects},
  author={Ramprasad, R. and Batra, R. and Pilania, G. and Mannodi-Kanakkithodi, A. and Kim, C.},
  journal={npj Computational Materials},
  volume={3},
  number={1},
  pages={54},
  year={2017},
  publisher={Nature Publishing Group}
}

@article{butler2018machine,
  title={Machine learning for molecular and materials science},
  author={Butler, K. T. and Davies, D. W. and Cartwright, H. and Isayev, O. and Walsh, A.},
  journal={Nature},
  volume={559},
  number={7715},
  pages={547},
  year={2018},
  publisher={Nature Publishing Group}
}

@article{brockherde2017bypassing,
  title={Bypassing the {Kohn-Sham} equations with machine learning},
  author={Brockherde, F. and Vogt, L. and Li, L. and Tuckerman, M. E. and Burke, K. and M{\"u}ller, K. R.},
  journal={Nature communications},
  volume={8},
  number={1},
  pages={872},
  year={2017},
  publisher={Nature Publishing Group}
}


@article{pilania2013accelerating,
  title={Accelerating materials property predictions using machine learning},
  author={Pilania, G. and Wang, C. C. and Jiang, X. and Rajasekaran, S. and Ramprasad, R.},
  journal={Scientific reports},
  volume={3},
  pages={2810},
  year={2013},
  publisher={Nature Publishing Group}
}

%%%%%%%%%%%%%%%%%%%%% Material geomone project

@book{national2011materials,
  title={Materials genome initiative for global competitiveness},
  author={National Science and Technology Council (US)},
  year={2011},
  publisher={Executive Office of the President, National Science and Technology Council}
}


@article{jain2013commentary,
  title={Commentary: The Materials Project: A materials genome approach to accelerating materials innovation},
  author={Jain, Anubhav and Ong, Shyue Ping and Hautier, Geoffroy and Chen, Wei and Richards, William Davidson and Dacek, Stephen and Cholia, Shreyas and Gunter, Dan and Skinner, David and Ceder, Gerbrand and others},
  journal={Apl Materials},
  volume={1},
  number={1},
  pages={011002},
  year={2013},
  publisher={AIP}
}

@article{ong2013python,
  title={Python Materials Genomics (pymatgen): A robust, open-source python library for materials analysis},
  author={Ong, S. P. and Richards, W. D. and Jain, A.v and Hautier, G. and Kocher, M. and Cholia, S. and Gunter, D. and Chevrier, V. L. and Persson, K. A. and Ceder, G.},
  journal={Computational Materials Science},
  volume={68},
  pages={314--319},
  year={2013},
  publisher={Elsevier}
}

%%%%%%%%%%%% computional material sciences

@book{hergert2004computational,
  title={Computational materials science: from basic principles to material properties},
  author={Hergert, W. and Ernst, A. and D{\"a}ne, M.},
  volume={642},
  year={2004},
  publisher={Springer Science \& Business Media}
}

@techreport{crabtree2010computational,
  title={Computational materials science and chemistry: accelerating discovery and innovation through simulation-based engineering and science},
  author={Crabtree, G. and Glotzer, S. and McCurdy, B. and Roberto, J.},
  year={2010},
  institution={USDOE Office of Science (SC)(United States)}
}

@book{moskowitz2014advanced,
  title={The advanced materials revolution: technology and economic growth in the age of globalization},
  author={Moskowitz, S. L.},
  year={2014},
  publisher={John Wiley \& Sons}
}

%%%%%%%%%%% The fourth paradigm
@book{hey2009fourth,
  title={The fourth paradigm: data-intensive scientific discovery},
  author={Hey, A. and Tansley, S. and Tolle, K. M. and others},
  volume={1},
  year={2009},
  publisher={Microsoft research Redmond, WA}
}

%%%%%%% material innovation

@article{magee2012towards,
  title={Towards quantification of the role of materials innovation in overall technological development},
  author={Magee, C. L.},
  journal={Complexity},
  volume={18},
  number={1},
  pages={10--25},
  year={2012},
  publisher={Wiley Online Library}
}

@Online{Darroch2012,
 author = {Boren, M., Chan, V., and Musso, C.},
 year = {2012},
 title = {The path to improved returns in materials commercialization },
 journal = {McKinsey & Company},
 url = {https://www.mckinsey.com/business-functions/operations/our-insights/the-path-to-improved-returns-in-materials-commercialization},
 urldate = {2012-08}
}

%%%%%%%%%%% DFT application in material sciences

@article{castelli2012new,
  title={New cubic perovskites for one-and two-photon water splitting using the computational materials repository},
  author={Castelli, I. E. and Landis, D. D. and Thygesen, K. S. and Dahl, S. and Chorkendorff, I. and Jaramillo, T. F. and Jacobsen, K. W.},
  journal={Energy \& Environmental Science},
  volume={5},
  number={10},
  pages={9034--9043},
  year={2012},
  publisher={Royal Society of Chemistry}
}

@article{yu2012identification,
  title={Identification of potential photovoltaic absorbers based on first-principles spectroscopic screening of materials},
  author={Yu, L. P. and Zunger, A.},
  journal={Physical review letters},
  volume={108},
  number={6},
  pages={068701},
  year={2012},
  publisher={APS}
}

@article{yang2012search,
  title={A search model for topological insulators with high-throughput robustness descriptors},
  author={Yang, K. S. and Setyawan, W. and Wang, S. D. and Nardelli, M. B. and Curtarolo, S.},
  journal={Nature materials},
  volume={11},
  number={7},
  pages={614},
  year={2012},
  publisher={Nature Publishing Group}
}

@article{lin2012silico,
  title={In silico screening of carbon-capture materials},
  author={Lin, L. C. and Berger, A. H. and Martin, R. L. and Kim, J. and Swisher, J. A. and others},
  journal={Nature materials},
  volume={11},
  number={7},
  pages={633},
  year={2012},
  publisher={Nature Publishing Group}
}


%%%%%%%%%%%%%%%% chemical informatics

@book{puzyn2010recent,
  title={Recent advances in {QSAR} studies: methods and applications},
  author={Puzyn, T. and Leszczynski, J. and Cronin, M. T.},
  volume={8},
  year={2010},
  publisher={Springer Science \& Business Media}
}

@article{lo2018machine,
  title={Machine learning in chemoinformatics and drug discovery},
  author={Lo, Y. C. and Rensi, S. E. and Torng, W. and Altman, R. B.},
  journal={Drug discovery today},
  volume={23},
  number={8},
  pages={1538--1546},
  year={2018},
  publisher={Elsevier}
}

@book{bajorath2011chemoinformatics,
  title={Chemoinformatics and computational chemical biology},
  author={Bajorath, J. and Bajorath, J.},
  year={2011},
  publisher={Springer}
}

@book{bajorath2004chemoinformatics,
  title={Chemoinformatics: concepts, methods, and tools for drug discovery},
  author={Bajorath, J.},
  volume={275},
  year={2004},
  publisher={Springer Science \& Business Media}
}

%%%%%%%%%%%% Bioinformatics

@book{mount2004bioinformatics,
  title={Bioinformatics: sequence and genome analysis},
  author={Mount, D. W.},
  volume={692},
  year={2004},
  publisher={Cold Spring Harbor, NY: Cold Spring Harbor Laboratory Press. xii}
}

@book{baxevanis2004bioinformatics,
  title={Bioinformatics: a practical guide to the analysis of genes and proteins},
  author={Baxevanis, A. D. and Ouellette, B. F. F.},
  volume={43},
  year={2004},
  publisher={John Wiley \& Sons}
}

%%%%%%%%%%%%%%%%%%% high throughput ab inition

@article{curtarolo2005high,
  title={High-throughput ab initio analysis of the {Bi--In}, {Bi--Mg}, {Bi--Sb}, {In--Mg}, {In--Sb}, and {Mg--Sb} systems},
  author={Curtarolo, S. and Kolmogorov, A. N. and Cocks, F. H.},
  journal={Calphad},
  volume={29},
  number={2},
  pages={155--161},
  year={2005},
  publisher={Elsevier}
}

@article{oganov2006crystal,
  title={Crystal structure prediction using ab initio evolutionary techniques: Principles and applications},
  author={Oganov, A. R. and Glass, C. W.},
  journal={The Journal of chemical physics},
  volume={124},
  number={24},
  pages={244704},
  year={2006},
  publisher={AIP}
}

@article{pickard2011ab,
  title={Ab initio random structure searching},
  author={Pickard, C. J. and Needs, R. J.},
  journal={Journal of Physics: Condensed Matter},
  volume={23},
  number={5},
  pages={053201},
  year={2011},
  publisher={IOP Publishing}
}

@article{morgan2004high,
  title={High-throughput and data mining with ab initio methods},
  author={Morgan, D. and Ceder, G. and Curtarolo, S.},
  journal={Measurement Science and Technology},
  volume={16},
  number={1},
  pages={296},
  year={2004},
  publisher={IOP Publishing}
}

@article{kang2006electrodes,
  title={Electrodes with high power and high capacity for rechargeable lithium batteries},
  author={Kang, K. and Meng, Y. S. and Br{\'e}ger, J. and Grey, C. P. and Ceder, G.},
  journal={Science},
  volume={311},
  number={5763},
  pages={977--980},
  year={2006},
  publisher={American Association for the Advancement of Science}
}

%%%%%%%%%%%%%% QM MM

@book{bohm1986quantum,
  title={Quantum mechanics: foundations and applications},
  author={Bohm, A. and Loewe, M.},
  volume={3},
  year={1986},
  publisher={Springer}
}

@book{baym2018lectures,
  title={Lectures on quantum mechanics},
  author={Baym, G.},
  year={2018},
  publisher={CRC Press}
}

@article{haile1993molecular,
  title={Molecular dynamics simulation: elementary methods},
  author={Haile, J.M. and Johnston, I. and Mallinckrodt, A. J. and McKay, S.},
  journal={Computers in Physics},
  volume={7},
  number={6},
  pages={625--625},
  year={1993},
  publisher={AIP}
}

@book{binder1995monte,
  title={{Monte Carlo} and molecular dynamics simulations in polymer science},
  author={Binder, K.},
  year={1995},
  publisher={Oxford University Press}
}

%%%%%%%%%%%%%%%%%%% TDA

@article{wasserman2018topological,
  title={Topological data analysis},
  author={Wasserman, L.},
  journal={Annual Review of Statistics and Its Application},
  volume={5},
  pages={501--532},
  year={2018},
  publisher={Annual Reviews}
}

@article{zomorodian2012topological,
  title={Topological data analysis},
  author={Zomorodian, A.},
  journal={Advances in applied and computational topology},
  volume={70},
  pages={1--39},
  year={2012}
}

@book{pascucci2010topological,
  title={Topological Methods in Data Analysis and Visualization: Theory, Algorithms, and Applications},
  author={Pascucci, V. and Tricoche, X. and Hagen, H. and Tierny, J.},
  year={2010},
  publisher={Springer Science \& Business Media}
}

%%%%%%%% PH material

@article{nakamura2015persistent,
  title={Persistent homology and many-body atomic structure for medium-range order in the glass},
  author={Nakamura, T. and Hiraoka, Y. and Hirata, A. and Escolar, E. G. and Nishiura, Y.},
  journal={Nanotechnology},
  volume={26},
  number={30},
  pages={304001},
  year={2015},
  publisher={IOP Publishing}
}

@article{hiraoka2016hierarchical,
  title={Hierarchical structures of amorphous solids characterized by persistent homology},
  author={Hiraoka, Y. and Nakamura, T. and Hirata, A. and Escolar, E. G. and Matsue, K. and Nishiura, Y.},
  journal={Proceedings of the National Academy of Sciences},
  volume={113},
  number={26},
  pages={7035--7040},
  year={2016},
  publisher={National Acad Sciences}
}

@article{ichinomiya2017persistent,
  title={Persistent homology analysis of craze formation},
  author={Ichinomiya, T. and Obayashi, I. and Hiraoka, Y.},
  journal={Physical Review E},
  volume={95},
  number={1},
  pages={012504},
  year={2017},
  publisher={APS}
}


@article{saadatfar:2017pore,
  title={Pore configuration landscape of granular crystallization},
  author={Saadatfar, M. and Takeuchi, H. and Robins, V. and Francois, N. and Hiraoka, Y.},
  journal={Nature communications},
  volume={8},
  pages={15082},
  year={2017},
  publisher={Nature Publishing Group}
}

@article{lee2018high,
  title={High-throughput screening approach for nanoporous materials genome using topological data analysis: application to zeolites},
  author={Lee, Yongjin and Barthel, Senja D and D{\l}otko, Pawe{\l} and Moosavi, Seyed Mohamad and Hess, Kathryn and Smit, Berend},
  journal={Journal of chemical theory and computation},
  volume={14},
  number={8},
  pages={4427--4437},
  year={2018},
  publisher={ACS Publications}
}

@article{lee2017quantifying,
  title={Quantifying similarity of pore-geometry in nanoporous materials},
  author={Lee, Yongjin and Barthel, Senja D and D{\l}otko, Pawe{\l} and Moosavi, S Mohamad and Hess, Kathryn and Smit, Berend},
  journal={Nature communications},
  volume={8},
  number={1},
  pages={1--8},
  year={2017},
  publisher={Nature Publishing Group}
}

@article{krishnapriyan2020topological,
  title={Topological descriptors help predict guest adsorption in nanoporous materials},
  author={Krishnapriyan, Aditi S and Haranczyk, Maciej and Morozov, Dmitriy},
  journal={The Journal of Physical Chemistry C},
  volume={124},
  number={17},
  pages={9360--9368},
  year={2020},
  publisher={ACS Publications}
}


%%%%%%%%%%%%%%%%% Persistent cohomology

@article{rybakken2019decoding,
  title={Decoding of neural data using cohomological feature extraction},
  author={Rybakken, E. and Baas, N. and Dunn, B.},
  journal={Neural computation},
  volume={31},
  number={1},
  pages={68--93},
  year={2019},
  publisher={MIT Press}
}

@article{vejdemo2015cohomological,
  title={Cohomological learning of periodic motion},
  author={Vejdemo-Johansson, M. and Pokorny, F. T. and Skraba, P. and Kragic, D.},
  journal={Applicable Algebra in Engineering, Communication and Computing},
  volume={26},
  number={1-2},
  pages={5--26},
  year={2015},
  publisher={Springer}
}




%%%%%%%%%%%%% databank

@article{gaulton2011chembl,
  title={{ChEMBL}: a large-scale bioactivity database for drug discovery},
  author={Gaulton, A. and Bellis, L. J. and Bento, A. P. and Chambers, J. and Davies, M. and Hersey, A. and Light, Y. and McGlinchey, S. and Michalovich, D. and Al-Lazikani, B. and others},
  journal={Nucleic acids research},
  volume={40},
  number={D1},
  pages={D1100--D1107},
  year={2011},
  publisher={Oxford University Press}
}

@article{oughtred2018biogrid,
  title={The {BioGRID} interaction database: 2019 update},
  author={Oughtred, R. and Stark, C. and Breitkreutz, B. J. and Rust, J. and Boucher, L. and Chang, C. and Kolas, N. and O’Donnell, L. and Leung, G. and McAdam, R. and others},
  journal={Nucleic acids research},
  volume={47},
  number={D1},
  pages={D529--D541},
  year={2018},
  publisher={Oxford University Press}
}


@article{benson2008genbank,
  title={GenBank},
  author={Benson, D. A. and Karsch-Mizrachi, I. and Lipman, D. J. and Ostell, J. and Sayers, E. W.},
  journal={Nucleic acids research},
  volume={37},
  number={suppl\_1},
  pages={D26--D31},
  year={2008},
  publisher={Oxford University Press}
}

%%%%%%%%%%%%%% inphone vs appollo

@Online{Kendall2019,
 author = {Kendall, G. },
 year = {2019},
 title = {Would your mobile phone be powerful enough to get you to the moon? },
 journal = {The Conversation},
 url = {http://theconversation.com/would-your-mobile-phone-be-powerful-enough-to-get-you-to-the-moon-115933},
 urldate = {2019-07-01}
}

%%%%%%%%%% alpha fold
@Online{Hutson2019,
 author = {Hutson, M. },
 year = {2019},
 title = {{AI} protein-folding algorithms solve structures faster than ever },
 journal = {Nature news},
 url = {https://www.nature.com/articles/d41586-019-01357-6},
 urldate = {2019-07-22}
}

%%%%%%%% Drug design papers, scoring function, protein-ligand binding

@article{liu2015classification,
  title={Classification of current scoring functions},
  author={Liu, J. and Wang, R. X.},
  journal={Journal of chemical information and modeling},
  volume={55},
  number={3},
  pages={475--482},
  year={2015},
  publisher={ACS Publications}
}

@article{wojcikowski2019development,
  title={Development of a protein--ligand extended connectivity ({PLEC}) fingerprint and its application for binding affinity predictions},
  author={W{\'o}jcikowski, M. and Kukie{\l}ka, M. and Stepniewska-Dziubinska, M. M. and Siedlecki, P.},
  journal={Bioinformatics},
  volume={35},
  number={8},
  pages={1334--1341},
  year={2019},
  publisher={Oxford University Press}
}


@article{stepniewska2018development,
  title={Development and evaluation of a deep learning model for protein--ligand binding affinity prediction},
  author={Stepniewska-Dziubinska, M. M. and Zielenkiewicz, P. and Siedlecki, P.},
  journal={Bioinformatics},
  volume={34},
  number={21},
  pages={3666--3674},
  year={2018},
  publisher={Oxford University Press}
}

@article{su2018comparative,
  title={Comparative assessment of scoring functions: The {CASF}-2016 update},
  author={Su, M. Y. and Yang, Q. F. and Du, Y. and Feng, G. Q. and Liu, Z. H. and Li, Y and Wang, R. X.},
  journal={Journal of chemical information and modeling},
  volume={59},
  number={2},
  pages={895--913},
  year={2018},
  publisher={ACS Publications}
}

@article{zheng2019onionnet,
  title={{OnionNet}: a Multiple-Layer Intermolecular-Contact-Based Convolutional Neural Network for Protein--Ligand Binding Affinity Prediction},
  author={Zheng, L. Z. and Fan, J. R. and Mu, Y. G.},
  journal={ACS omega},
  volume={4},
  number={14},
  pages={15956--15965},
  year={2019},
  publisher={ACS Publications}
}

@article{afifi2018improving,
  title={Improving classical scoring functions using random forest: The non-additivity of free energy terms' contributions in binding},
  author={Afifi, K. and Al-Sadek, A. F.},
  journal={Chemical biology \& drug design},
  volume={92},
  number={2},
  pages={1429--1434},
  year={2018},
  publisher={Wiley Online Library}
}

@article{feinberg2018potentialnet,
  title={PotentialNet for molecular property prediction},
  author={Feinberg, E. N. and Sur, D. and Wu, Z. Q. and Husic, B. E. and Mai, H. H. and Li, Y. and Sun, S. S. and Yang, J. Y. and Ramsundar, B. and Pande, V. S.},
  journal={ACS central science},
  volume={4},
  number={11},
  pages={1520--1530},
  year={2018},
  publisher={ACS Publications}
}

@article{boyles2020learning,
  title={Learning from the ligand: using ligand-based features to improve binding affinity prediction},
  author={Boyles, F. and Deane, C. M. and Morris, G. M.},
  journal={Bioinformatics},
  volume={36},
  number={3},
  pages={758--764},
  year={2020},
  publisher={Oxford University Press}
}

%% Ballester

@article{ain2015machine,
  title={Machine-learning scoring functions to improve structure-based binding affinity prediction and virtual screening},
  author={Ain, Q. U. and Aleksandrova, A. and Roessler, F. D. and Ballester, P. J.},
  journal={Wiley Interdisciplinary Reviews: Computational Molecular Science},
  volume={5},
  number={6},
  pages={405--424},
  year={2015},
  publisher={Wiley Online Library}
}

@article{li2015improving,
  title={Improving {AutoDock Vina} using random forest: the growing accuracy of binding affinity prediction by the effective exploitation of larger data sets},
  author={Li, H. J. and Leung, K. S. and Wong, M. H. and Ballester, P. J.},
  journal={Molecular informatics},
  volume={34},
  number={2-3},
  pages={115--126},
  year={2015},
  publisher={Wiley Online Library}
}


%%%%%%%% ADDED BY Liu Xiang, PDBbind for protein-ligand binding affinity prediction

@article{karlov2020graphdelta,
  title={{graphDelta}: {MPNN} scoring function for the affinity prediction of protein--ligand complexes},
  author={Karlov, Dmitry S and Sosnin, Sergey and Fedorov, Maxim V and Popov, Petr},
  journal={ACS omega},
  volume={5},
  number={10},
  pages={5150--5159},
  year={2020},
  publisher={ACS Publications}
}

@article{sanchez2021extended,
  title={Extended connectivity interaction features: Improving binding affinity prediction through chemical description},
  author={S{\'a}nchez-Cruz, Norberto and Medina-Franco, Jos{\'e} L and Mestres, Jordi and Barril, Xavier},
  journal={Bioinformatics},
  volume={37},
  number={10},
  pages={1376--1382},
  year={2021},
  publisher={Oxford University Press}
}

@article{wang2021onionnet,
  title={{OnionNet-2: A Convolutional Neural Network Model for Predicting Protein-Ligand Binding Affinity based on Residue-Atom Contacting Shells}},
  author={Wang, Zechen and Zheng, Liangzhen and Liu, Yang and Qu, Yuanyuan and Li, Yong-Qiang and Zhao, Mingwen and Mu, Yuguang and Li, Weifeng},
  journal={arXiv preprint arXiv:2103.11664},
  year={2021}
}

@article{rezaei2020deep,
  title={{Deep Learning in Drug Design: Protein-Ligand Binding Affinity Prediction}},
  author={Rezaei, Mohammad Ali and Li, Yanjun and Wu, Dapeng Oliver and Li, Xiaolin and Li, Chenglong},
  journal={IEEE/ACM Transactions on Computational Biology and Bioinformatics},
  year={2020},
  publisher={IEEE}
}

@article{boyles2020learning,
  title={Learning from the ligand: using ligand-based features to improve binding affinity prediction},
  author={Boyles, Fergus and Deane, Charlotte M and Morris, Garrett M},
  journal={Bioinformatics},
  volume={36},
  number={3},
  pages={758--764},
  year={2020},
  publisher={Oxford University Press}
}

@article{song2020se,
  title={{SE-OnionNet: A }convolution neural network for protein-ligand binding affinity prediction},
  author={Song, Tao and Wang, Shudong and Liu, Dayan and Ding, Mao and Du, Zhenzhen and Zhong, Yue and Rodr{\'\i} Guez-Pat{\'o}n, Alfonso},
  journal={Frontiers in Genetics},
  volume={11},
  pages={1805},
  year={2020},
  publisher={Frontiers}
}

@article{zhu2020binding,
  title={{Binding Affinity Prediction by Pairwise Function Based on Neural Network}},
  author={Zhu, Fangqiang and Zhang, Xiaohua and Allen, Jonathan E and Jones, Derek and Lightstone, Felice C},
  journal={Journal of chemical information and modeling},
  volume={60},
  number={6},
  pages={2766--2772},
  year={2020},
  publisher={ACS Publications}
}

@article{wang2021deepdtaf,
  title={{DeepDTAF}: a deep learning method to predict protein--ligand binding affinity},
  author={Wang, Kaili and Zhou, Renyi and Li, Yaohang and Li, Min},
  journal={Briefings in Bioinformatics},
  year={2021}
}

@article{zhou2020distance,
  title={{Distance-aware Molecule Graph Attention Network for Drug-Target Binding Affinity Prediction}},
  author={Zhou, Jingbo and Li, Shuangli and Huang, Liang and Xiong, Haoyi and Wang, Fan and Xu, Tong and Xiong, Hui and Dou, Dejing},
  journal={arXiv preprint arXiv:2012.09624},
  year={2020}
}

@article{jones2021improved,
  title={{Improved Protein--Ligand Binding Affinity Prediction with Structure-Based Deep Fusion Inference}},
  author={Jones, Derek and Kim, Hyojin and Zhang, Xiaohua and Zemla, Adam and Stevenson, Garrett and Bennett, WF Drew and Kirshner, Daniel and Wong, Sergio E and Lightstone, Felice C and Allen, Jonathan E},
  journal={Journal of Chemical Information and Modeling},
  volume={61},
  number={4},
  pages={1583--1592},
  year={2021},
  publisher={ACS Publications}
}

@article{hassan2020rosenet,
  title={{RosENet: improving binding affinity prediction by leveraging molecular mechanics energies with an ensemble of 3D convolutional neural networks}},
  author={Hassan-Harrirou, Hussein and Zhang, Ce and Lemmin, Thomas},
  journal={Journal of chemical information and modeling},
  volume={60},
  number={6},
  pages={2791--2802},
  year={2020},
  publisher={ACS Publications}
}


@article{sagi2018ensemble,
  title={Ensemble learning: A survey},
  author={Sagi, Omer and Rokach, Lior},
  journal={Wiley Interdisciplinary Reviews: Data Mining and Knowledge Discovery},
  volume={8},
  number={4},
  pages={e1249},
  year={2018},
  publisher={Wiley Online Library}
}

@article{wang2019stacking,
  title={Stacking-based ensemble learning of decision trees for interpretable prostate cancer detection},
  author={Wang, Yuyan and Wang, Dujuan and Geng, Na and Wang, Yanzhang and Yin, Yunqiang and Jin, Yaochu},
  journal={Applied Soft Computing},
  volume={77},
  pages={188--204},
  year={2019},
  publisher={Elsevier}
}

@article{rosen1996ensemble,
  title={Ensemble learning using decorrelated neural networks},
  author={Rosen, Bruce E},
  journal={Connection science},
  volume={8},
  number={3-4},
  pages={373--384},
  year={1996},
  publisher={Taylor \& Francis}
}

@article{yang2010review,
  title={A review of ensemble methods in bioinformatics},
  author={Yang, Pengyi and Hwa Yang, Yee and B Zhou, Bing and Y Zomaya, Albert},
  journal={Current Bioinformatics},
  volume={5},
  number={4},
  pages={296--308},
  year={2010},
  publisher={Bentham Science Publishers}
}



%%%%%%%%% fignerprint softwares

@misc{landrum2006rdkit,
  title={{RDKit}: {Open}-source cheminformatics},
  author={Landrum, G.},
  year={2006}
}

@article{oboyle2011open,
  title={{Open Babel}: An open chemical toolbox},
  author={O'Boyle, N. M. and Banck, M. and James, C. A. and Morley, C. and Vandermeersch, T. and Hutchison, G. R.},
  journal={Journal of cheminformatics},
  volume={3},
  number={1},
  pages={33},
  year={2011},
  publisher={BioMed Central}
}

@article{cao2013chemopy,
  title={{ChemoPy}: freely available python package for computational biology and chemoinformatics},
  author={Cao, D. S. and Xu, Q. S. and Hu, Q. N. and Liang, Y. Z.},
  journal={Bioinformatics},
  volume={29},
  number={8},
  pages={1092--1094},
  year={2013},
  publisher={Oxford University Press}
}

%%%% spectral models

@article{eckmann1944harmonische,
  title={Harmonische funktionen und randwertaufgaben in einem komplex},
  author={Eckmann, B.},
  journal={Commentarii Mathematici Helvetici},
  volume={17},
  number={1},
  pages={240--255},
  year={1944},
  publisher={Springer}
}

@article{horak2013spectra,
  title={Spectra of combinatorial {Laplace} operators on simplicial complexes},
  author={Horak, D. and Jost, J.},
  journal={Advances in Mathematics},
  volume={244},
  pages={303--336},
  year={2013},
  publisher={Elsevier}
}

@article{mukherjee2016random,
  title={Random walks on simplicial complexes and harmonics},
  author={Mukherjee, S. and Steenbergen, J.},
  journal={Random structures \& algorithms},
  volume={49},
  number={2},
  pages={379--405},
  year={2016},
  publisher={Wiley Online Library}
}

@article{parzanchevski2017simplicial,
  title={Simplicial complexes: spectrum, homology and random walks},
  author={Parzanchevski, O. and Rosenthal, R.},
  journal={Random Structures \& Algorithms},
  volume={50},
  number={2},
  pages={225--261},
  year={2017},
  publisher={Wiley Online Library}
}

@article{shukla2020spectral,
  title={Spectral gap bounds for the simplicial {Laplacian} and an application to random complexes},
  author={Shukla, S. and Yogeshwaran, D.},
  journal={Journal of Combinatorial Theory, Series A},
  volume={169},
  pages={105134},
  year={2020},
  publisher={Elsevier}
}

@article{torres2020simplicial,
  title={Simplicial complexes: higher-order spectral dimension and dynamics},
  author={Torres, Joaqu{\'\i}n J and Bianconi, Ginestra},
  journal={Journal of Physics: Complexity},
  volume={1},
  number={1},
  pages={015002},
  year={2020},
  publisher={IOP Publishing}
}

@article{barbarossa2020topological,
  title={Topological signal processing over simplicial complexes},
  author={Barbarossa, Sergio and Sardellitti, Stefania},
  journal={IEEE Transactions on Signal Processing},
  volume={68},
  pages={2992--3007},
  year={2020},
  publisher={IEEE}
}

@inproceedings{muhammad2006control,
  title={Control using higher order {Laplacians} in network topologies},
  author={Muhammad, A. and Egerstedt, M.},
  booktitle={Proc. of 17th International Symposium on Mathematical Theory of Networks and Systems},
  pages={1024--1038},
  year={2006},
  organization={Citeseer}
}

%% hypergraph spectral

@article{feng1996spectra,
  title={Spectra of hypergraphs and applications},
  author={Feng, K. Q. and Li, W. C. W.},
  journal={Journal of number theory},
  volume={60},
  number={1},
  pages={1--22},
  year={1996},
  publisher={Elsevier}
}


@inproceedings{sun2008hypergraph,
  title={Hypergraph spectral learning for multi-label classification},
  author={Sun, L. and Ji, S. W. and Ye, J. P.},
  booktitle={Proceedings of the 14th ACM SIGKDD international conference on Knowledge discovery and data mining},
  pages={668--676},
  year={2008}
}

@article{cooper2012spectra,
  title={Spectra of uniform hypergraphs},
  author={Cooper, J. and Dutle, A.},
  journal={Linear Algebra and its applications},
  volume={436},
  number={9},
  pages={3268--3292},
  year={2012},
  publisher={Elsevier}
}

@inproceedings{lu2011high,
  title={High-ordered random walks and generalized {Laplacians} on hypergraphs},
  author={Lu, L. Y. and Peng, X.},
  booktitle={International Workshop on Algorithms and Models for the Web-Graph},
  pages={14--25},
  year={2011},
  organization={Springer}
}

@inproceedings{barbarossa2016introduction,
  title={An introduction to hypergraph signal processing},
  author={Barbarossa, Sergio and Tsitsvero, Mikhail},
  booktitle={2016 IEEE International Conference on Acoustics, Speech and Signal Processing (ICASSP)},
  pages={6425--6429},
  year={2016},
  organization={IEEE}
}

%%% Path complex

@article{grigor2019homology,
  title={Homology of path complexes and hypergraphs},
  author={Grigor'yan, A. and Jimenez, R. and Muranov, Y. and Yau, S. T. },
  journal={Topology and its Applications},
  volume={267},
  pages={106877},
  year={2019},
  publisher={Elsevier}
}

@article{grigor2018path,
  title={On the path homology theory of digraphs and {Eilenberg--Steenrod} axioms},
  author={Grigor'yan, A. and Jimenez, R. and Muranov, Y. and Yau, S. T.},
  journal={Homology, Homotopy and Applications},
  volume={20},
  number={2},
  pages={179--205},
  year={2018},
  publisher={International Press of Boston}
}

@article{grigor2014graphs,
  title={Graphs associated with simplicial complexes},
  author={Grigor'yan, A. and Muranov, Y. and Yau, S. T.},
  journal={Homology, Homotopy and Applications},
  volume={16},
  number={1},
  pages={295--311},
  year={2014},
  publisher={International Press of Boston}
}

@article{grigor2015cohomology,
  title={Cohomology of digraphs and (undirected) graphs},
  author={Grigor'yan, A. and Lin, Y. and Muranov, Y. and Yau, S. T.},
  journal={Asian Journal of Mathematics},
  volume={19},
  number={5},
  pages={887--932},
  year={2015},
  publisher={International Press of Boston}
}

%%%%%%%%%%%% drug design papers

@article{smalley2017ai,
  title={{AI}-powered drug discovery captures pharma interest},
  author={Smalley, Eric},
  journal={Nature},
  number={35},
  pages={604--605},
  year={2017},
  publisher={Nature Publishing Group}
}

@article{fleming2018computer,
  title={Computer-calculated compounds},
  author={Fleming, Nic},
  journal={Nature},
  volume={557},
  number={7707},
  pages={S55--S57},
  year={2018},
  publisher={Macmillan Publishers Ltd., London, England}
}

@article{yang2018silico,
  title={In silico prediction of chemical toxicity for drug design using machine learning methods and structural alerts},
  author={Yang, Hongbin and Sun, Lixia and Li, Weihua and Liu, Guixia and Tang, Yun},
  journal={Frontiers in chemistry},
  volume={6},
  pages={30},
  year={2018},
  publisher={Frontiers}
}

@article{schneider2019mind,
  title={Mind and machine in drug design},
  author={Schneider, Gisbert},
  journal={Nature Machine Intelligence},
  volume={1},
  number={3},
  pages={128--130},
  year={2019},
  publisher={Nature Publishing Group}
}

@misc{smietana2016trends,
  title={Trends in clinical success rates},
  author={Smietana, Katarzyna and Siatkowski, Marcin and M{\o}ller, Martin},
  year={2016},
  pages={379-380},
  publisher={Nature Publishing Group}
}

@article{mak2019artificial,
  title={Artificial intelligence in drug development: present status and future prospects},
  author={Mak, Kit-Kay and Pichika, Mallikarjuna Rao},
  journal={Drug discovery today},
  volume={24},
  number={3},
  pages={773--780},
  year={2019},
  publisher={Elsevier}
}

@article{chan2019advancing,
  title={Advancing drug discovery via artificial intelligence},
  author={Chan, HC Stephen and Shan, Hanbin and Dahoun, Thamani and Vogel, Horst and Yuan, Shuguang},
  journal={Trends in pharmacological sciences},
  volume={40},
  number={8},
  pages={592--604},
  year={2019},
  publisher={Elsevier}
}

@article{sellwood2018artificial,
  title={Artificial intelligence in drug discovery},
  author={Sellwood, Matthew A and Ahmed, Mohamed and Segler, Marwin HS and Brown, Nathan},
  journal={Future Medicinal Chemistry},
  volume={10},
  number={17},
  year={2018},
  publisher={Future Science}
}

@article{chen2018rise,
  title={The rise of deep learning in drug discovery},
  author={Chen, Hongming and Engkvist, Ola and Wang, Yinhai and Olivecrona, Marcus and Blaschke, Thomas},
  journal={Drug discovery today},
  volume={23},
  number={6},
  pages={1241--1250},
  year={2018},
  publisher={Elsevier}
}

@inproceedings{unterthiner2014deep,
  title={Deep learning as an opportunity in virtual screening},
  author={Unterthiner, Thomas and Mayr, Andreas and Klambauer, G{\"u}nter and Steijaert, Marvin and Wegner, J{\"o}rg K and Ceulemans, Hugo and Hochreiter, Sepp},
  booktitle={Proceedings of the deep learning workshop at NIPS},
  volume={27},
  pages={1--9},
  year={2014}
}

@article{zhang2017machine,
  title={From machine learning to deep learning: progress in machine intelligence for rational drug discovery},
  author={Zhang, Lu and Tan, Jianjun and Han, Dan and Zhu, Hao},
  journal={Drug discovery today},
  volume={22},
  number={11},
  pages={1680--1685},
  year={2017},
  publisher={Elsevier}
}

@article{ekins2016next,
  title={The next era: deep learning in pharmaceutical research},
  author={Ekins, Sean},
  journal={Pharmaceutical research},
  volume={33},
  number={11},
  pages={2594--2603},
  year={2016},
  publisher={Springer}
}


@article{shen2017deep,
  title={Deep learning in medical image analysis},
  author={Shen, Dinggang and Wu, Guorong and Suk, Heung-Il},
  journal={Annual review of biomedical engineering},
  volume={19},
  pages={221--248},
  year={2017},
  publisher={Annual Reviews}
}

@article{litjens2017survey,
  title={A survey on deep learning in medical image analysis},
  author={Litjens, Geert and Kooi, Thijs and Bejnordi, Babak Ehteshami and Setio, Arnaud Arindra Adiyoso and Ciompi, Francesco and Ghafoorian, Mohsen and Van Der Laak, Jeroen Awm and Van Ginneken, Bram and S{\'a}nchez, Clara I},
  journal={Medical image analysis},
  volume={42},
  pages={60--88},
  year={2017},
  publisher={Elsevier}
}

%%% AI_Drug_Design start-up
@Online{AI_Startup,
 author = {Smith, Simon},
 year = {2020},
 title = {230 Startups Using Artificial Intelligence in Drug Discovery},
 journal = {Benchsci},
 url = {https://blog.benchsci.com/startups-using-artificial-intelligence-in-drug-discovery},
 urldate = {2020-04-1}
}

%% Drug bank
@article{wishart2018drugbank,
  title={{DrugBank} 5.0: a major update to the {DrugBank} database for 2018},
  author={Wishart, David S and Feunang, Yannick D and Guo, An C and Lo, Elvis J and Marcu, Ana and Grant, Jason R and Sajed, Tanvir and Johnson, Daniel and Li, Carin and Sayeeda, Zinat and others},
  journal={Nucleic acids research},
  volume={46},
  number={D1},
  pages={D1074--D1082},
  year={2018},
  publisher={Oxford University Press}
}


%% CADD

@article{hassan2016computer,
  title={Computer aided drug design: success and limitations},
  author={Hassan Baig, Mohammad and Ahmad, Khurshid and Roy, Sudeep and Mohammad Ashraf, Jalaluddin and Adil, Mohd and Haris Siddiqui, Mohammad and Khan, Saif and Amjad Kamal, Mohammad and Provazn{\'\i}k, Ivo and Choi, Inho},
  journal={Current pharmaceutical design},
  volume={22},
  number={5},
  pages={572--581},
  year={2016},
  publisher={Bentham Science Publishers}
}


@article{marshall1987computer,
  title={Computer-aided drug design},
  author={Marshall, Garland R},
  journal={Annual review of pharmacology and toxicology},
  volume={27},
  number={1},
  pages={193--213},
  year={1987},
  publisher={Annual Reviews 4139 El Camino Way, PO Box 10139, Palo Alto, CA 94303-0139, USA}
}

@article{song2009recent,
  title={Recent advances in computer-aided drug design},
  author={Song, Chun Meng and Lim, Shen Jean and Tong, Joo Chuan},
  journal={Briefings in bioinformatics},
  volume={10},
  number={5},
  pages={579--591},
  year={2009},
  publisher={Oxford University Press}
}

@article{macalino2015role,
  title={Role of computer-aided drug design in modern drug discovery},
  author={Macalino, Stephani Joy Y and Gosu, Vijayakumar and Hong, Sunhye and Choi, Sun},
  journal={Archives of pharmacal research},
  volume={38},
  number={9},
  pages={1686--1701},
  year={2015},
  publisher={Springer}
}


@article{ballester2010machine,
  title={A machine learning approach to predicting protein--ligand binding affinity with applications to molecular docking},
  author={Ballester, Pedro J and Mitchell, John BO},
  journal={Bioinformatics},
  volume={26},
  number={9},
  pages={1169--1175},
  year={2010},
  publisher={Oxford University Press}
}

@article{khamis2015machine,
  title={Machine learning in computational docking},
  author={Khamis, Mohamed A and Gomaa, Walid and Ahmed, Walaa F},
  journal={Artificial intelligence in medicine},
  volume={63},
  number={3},
  pages={135--152},
  year={2015},
  publisher={Elsevier}
}

@article{ain2015machine,
  title={Machine-learning scoring functions to improve structure-based binding affinity prediction and virtual screening},
  author={Ain, Qurrat Ul and Aleksandrova, Antoniya and Roessler, Florian D and Ballester, Pedro J},
  journal={Wiley Interdisciplinary Reviews: Computational Molecular Science},
  volume={5},
  number={6},
  pages={405--424},
  year={2015},
  publisher={Wiley Online Library}
}

@article{mayr2016deeptox,
  title={DeepTox: toxicity prediction using deep learning},
  author={Mayr, Andreas and Klambauer, G{\"u}nter and Unterthiner, Thomas and Hochreiter, Sepp},
  journal={Frontiers in Environmental Science},
  volume={3},
  pages={80},
  year={2016},
  publisher={Frontiers}
}



%%%%% Reservoir computing RC papers


@article{lukovsevivcius2009reservoir,
  title={Reservoir computing approaches to recurrent neural network training},
  author={Luko{\v{s}}evi{\v{c}}ius, Mantas and Jaeger, Herbert},
  journal={Computer Science Review},
  volume={3},
  number={3},
  pages={127--149},
  year={2009},
  publisher={Elsevier}
}

@article{tanaka2019recent,
  title={Recent advances in physical reservoir computing: A review},
  author={Tanaka, Gouhei and Yamane, Toshiyuki and H{\'e}roux, Jean Benoit and Nakane, Ryosho and Kanazawa, Naoki and Takeda, Seiji and Numata, Hidetoshi and Nakano, Daiju and Hirose, Akira},
  journal={Neural Networks},
  year={2019},
  publisher={Elsevier}
}


@article{lipton2015critical,
  title={A critical review of recurrent neural networks for sequence learning},
  author={Lipton, Zachary C and Berkowitz, John and Elkan, Charles},
  journal={arXiv preprint arXiv:1506.00019},
  year={2015}
}

@article{prater2016reservoir,
  title={Reservoir computing for spatiotemporal signal classification without trained output weights},
  author={Prater, Ashley},
  journal={arXiv preprint arXiv:1604.03073},
  year={2016}
}

@article{kudithipudi2016design,
  title={Design and analysis of a neuromemristive reservoir computing architecture for biosignal processing},
  author={Kudithipudi, Dhireesha and Saleh, Qutaiba and Merkel, Cory and Thesing, James and Wysocki, Bryant},
  journal={Frontiers in neuroscience},
  volume={9},
  pages={502},
  year={2016},
  publisher={Frontiers}
}

%%%%% Hodge theory

@book{hodge1989theory,
  title={The theory and applications of harmonic integrals},
  author={Hodge, William Vallance Douglas},
  year={1989},
  publisher={CUP Archive}
}

@book{voisin2003hodge,
  title={Hodge theory and complex algebraic geometry {II}},
  author={Voisin, Claire},
  volume={2},
  year={2003},
  publisher={Cambridge University Press}
}

@book{greub1972connections,
  title={Connections, {Curvature}, and {Cohomology V1}: {De Rham} cohomology of manifolds and vector bundles},
  author={Greub, Werner and Halperin, Stephen and Vanstone, Ray},
  year={1972},
  publisher={Academic press}
}

@article{bartholdi2012hodge,
  title={Hodge theory on metric spaces},
  author={Bartholdi, Laurent and Schick, Thomas and Smale, Nat and Smale, Steve},
  journal={Foundations of Computational Mathematics},
  volume={12},
  number={1},
  pages={1--48},
  year={2012},
  publisher={Springer}
}

@article{lim2015hodge,
  title={Hodge {Laplacians} on graphs},
  author={Lim, Lek-Heng},
  journal={arXiv preprint arXiv:1507.05379},
  year={2015}
}

@article{friedman1998computing,
  title={Computing {Betti} numbers via combinatorial {Laplacians}},
  author={Friedman, Joel},
  journal={Algorithmica},
  volume={21},
  number={4},
  pages={331--346},
  year={1998},
  publisher={Springer}
}


@article{jiang2011statistical,
  title={Statistical ranking and combinatorial {Hodge} theory},
  author={Jiang, Xiaoye and Lim, Lek-Heng and Yao, Yuan and Ye, Yinyu},
  journal={Mathematical Programming},
  volume={127},
  number={1},
  pages={203--244},
  year={2011},
  publisher={Springer}
}

@article{candogan2011flows,
  title={Flows and decompositions of games: Harmonic and potential games},
  author={Candogan, Ozan and Menache, Ishai and Ozdaglar, Asuman and Parrilo, Pablo A},
  journal={Mathematics of Operations Research},
  volume={36},
  number={3},
  pages={474--503},
  year={2011},
  publisher={INFORMS}
}

@article{bhatia2012helmholtz,
  title={The {Helmholtz-Hodge} decomposition—a survey},
  author={Bhatia, Harsh and Norgard, Gregory and Pascucci, Valerio and Bremer, Peer-Timo},
  journal={IEEE Transactions on visualization and computer graphics},
  volume={19},
  number={8},
  pages={1386--1404},
  year={2012},
  publisher={IEEE}
}

@article{schaub2020random,
  title={Random walks on simplicial complexes and the normalized Hodge {1-Laplacian}},
  author={Schaub, M. T. and Benson, A. R. and Horn, P. and Lippner, G. and Jadbabaie, A.},
  journal={SIAM Review},
  volume={62},
  number={2},
  pages={353--391},
  year={2020},
  publisher={SIAM}
}

@article{wang2021hermes,
  title={HERMES: Persistent spectral graph software},
  author={Wang, Rui and Zhao, Rundong and Ribando-Gros, Emily and Chen, Jiahui and Tong, Yiying and Wei, Guo-Wei},
  journal={Foundations of data science (Springfield, Mo.)},
  volume={3},
  number={1},
  pages={67},
  year={2021},
  publisher={NIH Public Access}
}

%%%%%%%%%%%%% Learning and representation

@inproceedings{bengio2013deep,
  title={Deep learning of representations: Looking forward},
  author={Bengio, Yoshua},
  booktitle={International Conference on Statistical Language and Speech Processing},
  pages={1--37},
  year={2013},
  organization={Springer}
}

@article{bengio2013representation,
  title={Representation learning: A review and new perspectives},
  author={Bengio, Yoshua and Courville, Aaron and Vincent, Pascal},
  journal={IEEE transactions on pattern analysis and machine intelligence},
  volume={35},
  number={8},
  pages={1798--1828},
  year={2013},
  publisher={IEEE}
}

@article{pattanaik2020molecular,
  title={Molecular Representation: Going Long on Fingerprints},
  author={Pattanaik, Lagnajit and Coley, Connor W},
  journal={Chem},
  volume={6},
  number={6},
  pages={1204--1207},
  year={2020},
  publisher={Elsevier}
}

%%%%%%%%%% COVID 19

@article{zhou2020network,
  title={Network-based drug repurposing for novel coronavirus {2019-nCoV/SARS-CoV-2}},
  author={Zhou, Yadi and Hou, Yuan and Shen, Jiayu and Huang, Yin and Martin, William and Cheng, Feixiong},
  journal={Cell Discovery},
  volume={6},
  number={1},
  pages={1--18},
  year={2020},
  publisher={Nature Publishing Group}
}


@article{zhang2020crystal,
  title={Crystal structure of {SARS-CoV-2} main protease provides a basis for design of improved $\alpha$-ketoamide inhibitors},
  author={Zhang, Linlin and Lin, Daizong and Sun, Xinyuanyuan and Curth, Ute and Drosten, Christian and Sauerhering, Lucie and Becker, Stephan and Rox, Katharina and Hilgenfeld, Rolf},
  journal={Science},
  year={2020},
  publisher={American Association for the Advancement of Science}
}

%%%%%%%% ADMET
@article{hodgson2001admet,
  title={{ADMET}--turning chemicals into drugs},
  author={Hodgson, J.},
  journal={Nature Biotechnology},
  volume={19},
  number={8},
  pages={722--726},
  year={2001},
  publisher={Nature Publishing Group}
}

%%%%%%%%% symmetry function
@article{behler2007generalized,
  title={Generalized neural-network representation of high-dimensional potential-energy surfaces},
  author={Behler, J. and Parrinello, M.},
  journal={Physical review letters},
  volume={98},
  number={14},
  pages={146401},
  year={2007},
  publisher={APS}
}


%%%%%%%% Ricci Curvature

@book{jost2008riemannian,
  title={Riemannian geometry and geometric analysis},
  author={Jost, J{\"u}rgen and Jost, J{\`e}urgen},
  volume={42005},
  year={2008},
  publisher={Springer}
}

@book{najman2017modern,
  title={Modern approaches to discrete curvature},
  author={Najman, Laurent and Romon, Pascal},
  volume={2184},
  year={2017},
  publisher={Springer}
}

@article{perelman2003ricci,
  title={Ricci flow with surgery on three-manifolds},
  author={Perelman, Grisha},
  journal={arXiv preprint math/0303109},
  year={2003}
}



%%%%%%%%%%%%% Forman Ricci curvature



@article{forman2003bochner,
  title={Bochner's method for cell complexes and combinatorial {Ricci} curvature},
  author={Forman, Robin},
  journal={Discrete and Computational Geometry},
  volume={29},
  number={3},
  pages={323--374},
  year={2003},
  publisher={Springer}
}

%%%%%%%%% ORC theorem, Discrete Ricci curvature
@incollection{bakry1985diffusions,
  title={Diffusions hypercontractives},
  author={Bakry, Dominique and {\'E}mery, Michel},
  booktitle={S{\'e}minaire de Probabilit{\'e}s XIX 1983/84},
  pages={177--206},
  year={1985},
  publisher={Springer}
}

@article{sturm2006geometry,
  title={On the geometry of metric measure spaces},
  author={Sturm, Karl-Theodor and others},
  journal={Acta mathematica},
  volume={196},
  number={1},
  pages={65--131},
  year={2006},
  publisher={Institut Mittag-Leffler}
}

@article{ollivier2007ricci,
  title={Ricci curvature of metric spaces},
  author={Ollivier, Yann},
  journal={Comptes Rendus Mathematique},
  volume={345},
  number={11},
  pages={643--646},
  year={2007},
  publisher={Elsevier}
}

@article{ollivier2009ricci,
  title={Ricci curvature of Markov chains on metric spaces},
  author={Ollivier, Yann},
  journal={Journal of Functional Analysis},
  volume={256},
  number={3},
  pages={810--864},
  year={2009},
  publisher={Elsevier}
}

@article{lott2009ricci,
  title={Ricci curvature for metric-measure spaces via optimal transport},
  author={Lott, John and Villani, C{\'e}dric},
  journal={Annals of Mathematics},
  pages={903--991},
  year={2009},
  publisher={JSTOR}
}

@article{bonciocat2009mass,
  title={Mass transportation and rough curvature bounds for discrete spaces},
  author={Bonciocat, Anca-Iuliana and Sturm, Karl-Theodor},
  journal={Journal of Functional Analysis},
  volume={256},
  number={9},
  pages={2944--2966},
  year={2009},
  publisher={Elsevier}
}

@article{chung1996logarithmic,
  title={Logarithmic harnack inequalities},
  author={Chung, Fan RK and Yau, S-T},
  journal={Mathematical Research Letters},
  volume={3},
  number={6},
  pages={793--812},
  year={1996},
  publisher={International Press of Boston}
}

@article{lin2011ricci,
  title={Ricci curvature of graphs},
  author={Lin, Yong and Lu, Linyuan and Yau, Shing-Tung},
  journal={Tohoku Mathematical Journal, Second Series},
  volume={63},
  number={4},
  pages={605--627},
  year={2011},
  publisher={Mathematical Institute, Tohoku University}
}



@article{lin2010ricci,
	title={Ricci curvature and eigenvalue estimate on locally finite graphs},
	author={Lin, Yong and Yau, Shing-Tung},
	journal={Mathematical research letters},
	volume={17},
	number={2},
	pages={343--356},
	year={2010},
	publisher={International Press of Boston}
}

@article{jost2014ollivier,
	title={Ollivier's {Ricci} curvature, local clustering and curvature-dimension inequalities on graphs},
	author={Jost, J{\"u}rgen and Liu, Shiping},
	journal={Discrete \& Computational Geometry},
	volume={51},
	number={2},
	pages={300--322},
	year={2014},
	publisher={Springer}
}

@article{bhattacharya2015exact,
	title={Exact and asymptotic results on coarse {Ricci} curvature of graphs},
	author={Bhattacharya, Bhaswar B and Mukherjee, Sumit},
	journal={Discrete Mathematics},
	volume={338},
	number={1},
	pages={23--42},
	year={2015},
	publisher={Elsevier}
}

@article{cho2013ollivier,
	title={Ollivier's {Ricci} curvature and the coloring of graphs},
	author={Cho, Hee Je and Paeng, Seong-Hun},
	journal={European Journal of Combinatorics},
	volume={34},
	number={5},
	pages={916--922},
	year={2013},
	publisher={Elsevier}
}

@article{bourne2018ollivier,
  title={Ollivier-{Ricci} Idleness Functions of Graphs},
  author={Bourne, David P and Cushing, David and Liu, Shiping and Munch, F and Peyerimhoff, Norbert},
  journal={SIAM Journal on Discrete Mathematics},
  volume={32},
  number={2},
  pages={1408--1424},
  year={2018},
  publisher={SIAM}
}


%%%%%%%%%%%%%% Ollivier Ricci curvatur application
@article{ni2019community,
  title={Community detection on networks with {Ricci} flow},
  author={Ni, Chien-Chun and Lin, Yu-Yao and Luo, Feng and Gao, Jie},
  journal={Scientific reports},
  volume={9},
  number={1},
  pages={1--12},
  year={2019},
  publisher={Nature Publishing Group}
}

@article{sia2019ollivier,
  title={{Ollivier-Ricci} curvature-based method to community detection in complex networks},
  author={Sia, Jayson and Jonckheere, Edmond and Bogdan, Paul},
  journal={Scientific reports},
  volume={9},
  number={1},
  pages={1--12},
  year={2019},
  publisher={Nature Publishing Group}
}


@inproceedings{ni2015ricci,
  title={Ricci curvature of the internet topology},
  author={Ni, Chien-Chun and Lin, Yu-Yao and Gao, Jie and Gu, Xianfeng David and Saucan, Emil},
  booktitle={2015 IEEE Conference on Computer Communications (INFOCOM)},
  pages={2758--2766},
  year={2015},
  organization={IEEE}
}


@article{sandhu2016ricci,
  title={Ricci curvature: An economic indicator for market fragility and systemic risk},
  author={Sandhu, Romeil S and Georgiou, Tryphon T and Tannenbaum, Allen R},
  journal={Science advances},
  volume={2},
  number={5},
  pages={e1501495},
  year={2016},
  publisher={American Association for the Advancement of Science}
}


@article{sandhu2015graph,
  title={Graph curvature for differentiating cancer networks},
  author={Sandhu, Romeil and Georgiou, Tryphon and Reznik, Ed and Zhu, Liangjia and Kolesov, Ivan and Senbabaoglu, Yasin and Tannenbaum, Allen},
  journal={Scientific reports},
  volume={5},
  number={1},
  pages={1--13},
  year={2015},
  publisher={Nature Publishing Group}
}

@article{farooq2019network,
  title={Network curvature as a hallmark of brain structural connectivity},
  author={Farooq, Hamza and Chen, Yongxin and Georgiou, Tryphon T and Tannenbaum, Allen and Lenglet, Christophe},
  journal={Nature communications},
  volume={10},
  number={1},
  pages={1--11},
  year={2019},
  publisher={Nature Publishing Group}
}








%%%%%%%%%%%%%%%%%%% Protein Hinges
@article{khade2020characterizing,
	title={Characterizing and Predicting Protein Hinges for Mechanistic Insight},
	author={Khade, Pranav M and Kumar, Ambuj and Jernigan, Robert L},
	journal={Journal of molecular biology},
	volume={432},
	number={2},
	pages={508--522},
	year={2020},
	publisher={Elsevier}
}

@article{emekli2008hingeprot,
	title={HingeProt: automated prediction of hinges in protein structures},
	author={Emekli, Ugur and Schneidman-Duhovny, Dina and Wolfson, Haim J and Nussinov, Ruth and Haliloglu, Turkan},
	journal={Proteins: Structure, Function, and Bioinformatics},
	volume={70},
	number={4},
	pages={1219--1227},
	year={2008},
	publisher={Wiley Online Library}
}

%%%%%%%%%%%%%%%%%%%%%%% Forman Ricci Curvature
@article{samal2018comparative,
  title={Comparative analysis of two discretizations of Ricci curvature for complex networks},
  author={Samal, Areejit and Sreejith, RP and Gu, Jiao and Liu, Shiping and Saucan, Emil and Jost, J{\"u}rgen},
  journal={Scientific reports},
  volume={8},
  number={1},
  pages={1--16},
  year={2018},
  publisher={Nature Publishing Group}
}

@article{saucan2019discrete,
  title={Discrete Ricci curvatures for directed networks},
  author={Saucan, Emil and Sreejith, RP and Vivek-Ananth, RP and Jost, J{\"u}rgen and Samal, Areejit},
  journal={Chaos, Solitons \& Fractals},
  volume={118},
  pages={347--360},
  year={2019},
  publisher={Elsevier}
}

@inproceedings{saucan2018forman,
  title={Forman's Ricci curvature-From networks to hypernetworks},
  author={Saucan, Emil and Weber, Melanie},
  booktitle={International Conference on Complex Networks and their Applications},
  pages={706--717},
  year={2018},
  organization={Springer}
}

@article{sreejith2016forman,
  title={Forman curvature for complex networks},
  author={Sreejith, RP and Mohanraj, Karthikeyan and Jost, J{\"u}rgen and Saucan, Emil and Samal, Areejit},
  journal={Journal of Statistical Mechanics: Theory and Experiment},
  volume={2016},
  number={6},
  pages={063206},
  year={2016},
  publisher={IOP Publishing}
}

@article{forman1999combinatorial,
  title={Combinatorial Differential Topology and Geometry},
  author={Forman, Robin},
  journal={New Perspectives in Algebraic Combinatorics},
  volume={38},
  pages={177},
  year={1999},
  publisher={Cambridge University Press}
}

%%%%%%% Gephi
@article{bastian2009gephi,
  title={Gephi: an open source software for exploring and manipulating networks.},
  author={Bastian, Mathieu and Heymann, Sebastien and Jacomy, Mathieu and others},
  year={2009}
}


%%%%%%%%%%%%%%%%%  3D CNN for drug design

@article{wallach2015atomnet,
  title={{AtomNet}: a deep convolutional neural network for bioactivity prediction in structure-based drug discovery},
  author={Wallach, Izhar and Dzamba, Michael and Heifets, Abraham},
  journal={arXiv preprint arXiv:1510.02855},
  year={2015}
}

@article{ragoza2017protein,
  title={Protein--ligand scoring with convolutional neural networks},
  author={Ragoza, Matthew and Hochuli, Joshua and Idrobo, Elisa and Sunseri, Jocelyn and Koes, David Ryan},
  journal={Journal of chemical information and modeling},
  volume={57},
  number={4},
  pages={942--957},
  year={2017},
  publisher={ACS Publications}
}


@article{hassan2020rosenet,
  title={RosENet: Improving Binding Affinity Prediction by Leveraging Molecular Mechanics Energies with an Ensemble of 3D Convolutional Neural Networks},
  author={Hassan-Harrirou, Hussein and Zhang, Ce and Lemmin, Thomas},
  journal={Journal of Chemical Information and Modeling},
  year={2020},
  publisher={ACS Publications}
}

@article{jimenez2018k,
  title={K$_{DEEP}$: Protein--ligand absolute binding affinity prediction via {3D}-convolutional neural networks},
  author={Jim{\'e}nez, J. and Skalic, M. and Martinez-Rosell, G. and De Fabritiis, G.},
  journal={Journal of chemical information and modeling},
  volume={58},
  number={2},
  pages={287--296},
  year={2018},
  publisher={ACS Publications}
}

@article{hochuli2018visualizing,
  title={Visualizing convolutional neural network protein-ligand scoring},
  author={Hochuli, Joshua and Helbling, Alec and Skaist, Tamar and Ragoza, Matthew and Koes, David Ryan},
  journal={Journal of Molecular Graphics and Modelling},
  volume={84},
  pages={96--108},
  year={2018},
  publisher={Elsevier}
}

@article{zeng2019atom,
  title={Atom table convolutional neural networks for an accurate prediction of compounds properties},
  author={Zeng, Shuming and Zhao, Yinchang and Li, Geng and Wang, Ruirui and Wang, Xinming and Ni, Jun},
  journal={NPJ Computational Materials},
  volume={5},
  number={1},
  pages={1--7},
  year={2019},
  publisher={Nature Publishing Group}
}


@article{stepniewska2018development,
  title={Development and evaluation of a deep learning model for protein--ligand binding affinity prediction},
  author={Stepniewska-Dziubinska, Marta M and Zielenkiewicz, Piotr and Siedlecki, Pawel},
  journal={Bioinformatics},
  volume={34},
  number={21},
  pages={3666--3674},
  year={2018},
  publisher={Oxford University Press}
}


@article{imrie2018protein,
  title={Protein family-specific models using deep neural networks and transfer learning improve virtual screening and highlight the need for more data},
  author={Imrie, Fergus and Bradley, Anthony R and van der Schaar, Mihaela and Deane, Charlotte M},
  journal={Journal of chemical information and modeling},
  volume={58},
  number={11},
  pages={2319--2330},
  year={2018},
  publisher={ACS Publications}
}

%%%%%%%%%%%%%  Graph neural network for biomolecules


@article{lusci2013deep,
  title={Deep architectures and deep learning in chemoinformatics: the prediction of aqueous solubility for drug-like molecules},
  author={Lusci, Alessandro and Pollastri, Gianluca and Baldi, Pierre},
  journal={Journal of chemical information and modeling},
  volume={53},
  number={7},
  pages={1563--1575},
  year={2013},
  publisher={ACS Publications}
}

@article{pereira2016boosting,
  title={Boosting docking-based virtual screening with deep learning},
  author={Pereira, Janaina Cruz and Caffarena, Ernesto Raul and dos Santos, Cicero Nogueira},
  journal={Journal of chemical information and modeling},
  volume={56},
  number={12},
  pages={2495--2506},
  year={2016},
  publisher={ACS Publications}
}

@article{kearnes2016molecular,
  title={Molecular graph convolutions: moving beyond fingerprints},
  author={Kearnes, Steven and McCloskey, Kevin and Berndl, Marc and Pande, Vijay and Riley, Patrick},
  journal={Journal of computer-aided molecular design},
  volume={30},
  number={8},
  pages={595--608},
  year={2016},
  publisher={Springer}
}


@article{gomes2017atomic,
  title={Atomic convolutional networks for predicting protein-ligand binding affinity},
  author={Gomes, Joseph and Ramsundar, Bharath and Feinberg, Evan N and Pande, Vijay S},
  journal={arXiv preprint arXiv:1703.10603},
  year={2017}
}


@article{feinberg2018potentialnet,
  title={PotentialNet for molecular property prediction},
  author={Feinberg, Evan N and Sur, Debnil and Wu, Zhenqin and Husic, Brooke E and Mai, Huanghao and Li, Yang and Sun, Saisai and Yang, Jianyi and Ramsundar, Bharath and Pande, Vijay S},
  journal={ACS central science},
  volume={4},
  number={11},
  pages={1520--1530},
  year={2018},
  publisher={ACS Publications}
}

@article{tsubaki2019compound,
  title={Compound--protein interaction prediction with end-to-end learning of neural networks for graphs and sequences},
  author={Tsubaki, Masashi and Tomii, Kentaro and Sese, Jun},
  journal={Bioinformatics},
  volume={35},
  number={2},
  pages={309--318},
  year={2019},
  publisher={Oxford University Press}
}

@article{li2019deepchemstable,
  title={Deepchemstable: chemical stability prediction with an attention-based graph convolution network},
  author={Li, Xiuming and Yan, Xin and Gu, Qiong and Zhou, Huihao and Wu, Di and Xu, Jun},
  journal={Journal of chemical information and modeling},
  volume={59},
  number={3},
  pages={1044--1049},
  year={2019},
  publisher={ACS Publications}
}


@article{wang2019molecule,
  title={Molecule property prediction based on spatial graph embedding},
  author={Wang, Xiaofeng and Li, Zhen and Jiang, Mingjian and Wang, Shuang and Zhang, Shugang and Wei, Zhiqiang},
  journal={Journal of chemical information and modeling},
  volume={59},
  number={9},
  pages={3817--3828},
  year={2019},
  publisher={ACS Publications}
}



@article{jiang2021could,
  title={Could graph neural networks learn better molecular representation for drug discovery? A comparison study of descriptor-based and graph-based models},
  author={Jiang, Dejun and Wu, Zhenxing and Hsieh, Chang-Yu and Chen, Guangyong and Liao, Ben and Wang, Zhe and Shen, Chao and Cao, Dongsheng and Wu, Jian and Hou, Tingjun},
  journal={Journal of cheminformatics},
  volume={13},
  number={1},
  pages={1--23},
  year={2021},
  publisher={BioMed Central}
}

@article{stokes2020deep,
  title={A deep learning approach to antibiotic discovery},
  author={Stokes, Jonathan M and Yang, Kevin and Swanson, Kyle and Jin, Wengong and Cubillos-Ruiz, Andres and Donghia, Nina M and MacNair, Craig R and French, Shawn and Carfrae, Lindsey A and Bloom-Ackermann, Zohar and others},
  journal={Cell},
  volume={180},
  number={4},
  pages={688--702},
  year={2020},
  publisher={Elsevier}
}


@article{gaudelet2020utilising,
  title={Utilising graph machine learning within drug discovery and development},
  author={Gaudelet, Thomas and Day, Ben and Jamasb, Arian R and Soman, Jyothish and Regep, Cristian and Liu, Gertrude and Hayter, Jeremy BR and Vickers, Richard and Roberts, Charles and Tang, Jian and others},
  journal = {Briefings in Bioinformatics},
  year = {2021},
  month = {05},
  doi = {10.1093/bib/bbab159},
  url = {https://doi.org/10.1093/bib/bbab159},
  note = {bbab159},
}



%%% Reivew of graph neural networks

@article{wu2020comprehensive,
  title={A comprehensive survey on graph neural networks},
  author={Wu, Zonghan and Pan, Shirui and Chen, Fengwen and Long, Guodong and Zhang, Chengqi and Philip, S Yu},
  journal={IEEE transactions on neural networks and learning systems},
  volume={32},
  number={1},
  pages={4--24},
  year={2020},
  publisher={IEEE}
}

@article{zhang2019graph,
  title={Graph convolutional networks: a comprehensive review},
  author={Zhang, Si and Tong, Hanghang and Xu, Jiejun and Maciejewski, Ross},
  journal={Computational Social Networks},
  volume={6},
  number={1},
  pages={1--23},
  year={2019},
  publisher={Springer}
}

@article{zhou2020graph,
  title={Graph neural networks: A review of methods and applications},
  author={Zhou, Jie and Cui, Ganqu and Hu, Shengding and Zhang, Zhengyan and Yang, Cheng and Liu, Zhiyuan and Wang, Lifeng and Li, Changcheng and Sun, Maosong},
  journal={AI Open},
  volume={1},
  pages={57--81},
  year={2020},
  publisher={Elsevier}
}

%%%%%%%%%%%%%%%%%%% 2D molecular fingerprint

@article{durant2002reoptimization,
  title={Reoptimization of MDL keys for use in drug discovery},
  author={Durant, Joseph L and Leland, Burton A and Henry, Douglas R and Nourse, James G},
  journal={Journal of chemical information and computer sciences},
  volume={42},
  number={6},
  pages={1273--1280},
  year={2002},
  publisher={ACS Publications}
}

@article{oboyle2011open,
  title={{Open Babel}: An open chemical toolbox},
  author={O'Boyle, N. M. and Banck, M. and James, C. A. and Morley, C. and Vandermeersch, T. and Hutchison, G. R.},
  journal={Journal of cheminformatics},
  volume={3},
  number={1},
  pages={33},
  year={2011},
  publisher={BioMed Central}
}

@article{hall1995electrotopological,
  title={Electrotopological state indices for atom types: a novel combination of electronic, topological, and valence state information},
  author={Hall, Lowell H and Kier, Lemont B},
  journal={Journal of Chemical Information and Computer Sciences},
  volume={35},
  number={6},
  pages={1039--1045},
  year={1995},
  publisher={ACS Publications}
}

@article{rogers2010extended,
  title={Extended-connectivity fingerprints},
  author={Rogers, David and Hahn, Mathew},
  journal={Journal of chemical information and modeling},
  volume={50},
  number={5},
  pages={742--754},
  year={2010},
  publisher={ACS Publications}
}
@article{landrum2006rdkit,
  title={{RDKit}: {Open}-source cheminformatics},
  author={Landrum, G.},
  year={2006}
}

@article{stiefl2006erg,
  title={{ErG}: {2D} pharmacophore descriptions for scaffold hopping},
  author={Stiefl, Nikolaus and Watson, Ian A and Baumann, Knut and Zaliani, Andrea},
  journal={Journal of chemical information and modeling},
  volume={46},
  number={1},
  pages={208--220},
  year={2006},
  publisher={ACS Publications}
}

%%%%%%%%%%%%%%%%%%%%% GCN for molecular fingerprints


@article{merkwirth2005automatic,
  title={Automatic generation of complementary descriptors with molecular graph networks},
  author={Merkwirth, Christian and Lengauer, Thomas},
  journal={Journal of chemical information and modeling},
  volume={45},
  number={5},
  pages={1159--1168},
  year={2005},
  publisher={ACS Publications}
}

@inproceedings{duvenaud2015convolutional,
  title={Convolutional networks on graphs for learning molecular fingerprints},
  author={Duvenaud, David K and Maclaurin, Dougal and Iparraguirre, Jorge and Bombarell, Rafael and Hirzel, Timothy and Aspuru-Guzik, Al{\'a}n and Adams, Ryan P},
  booktitle={Advances in neural information processing systems},
  pages={2224--2232},
  year={2015}
}

@article{coley2017convolutional,
  title={Convolutional embedding of attributed molecular graphs for physical property prediction},
  author={Coley, Connor W and Barzilay, Regina and Green, William H and Jaakkola, Tommi S and Jensen, Klavs F},
  journal={Journal of chemical information and modeling},
  volume={57},
  number={8},
  pages={1757--1772},
  year={2017},
  publisher={ACS Publications}
}

@article{xu2017deep,
  title={Deep learning based regression and multiclass models for acute oral toxicity prediction with automatic chemical feature extraction},
  author={Xu, Youjun and Pei, Jianfeng and Lai, Luhua},
  journal={Journal of chemical information and modeling},
  volume={57},
  number={11},
  pages={2672--2685},
  year={2017},
  publisher={ACS Publications}
}

@article{winter2019learning,
  title={Learning continuous and data-driven molecular descriptors by translating equivalent chemical representations},
  author={Winter, Robin and Montanari, Floriane and No{\'e}, Frank and Clevert, Djork-Arn{\'e}},
  journal={Chemical science},
  volume={10},
  number={6},
  pages={1692--1701},
  year={2019},
  publisher={Royal Society of Chemistry}
}

@phdthesis{yang2019learned,
  title={Are learned molecular representations ready for prime time?},
  author={Yang, Kevin and others},
  year={2019},
  school={Massachusetts Institute of Technology}
}

%%%%%%%%%%%%% RNA

@article{singh2019rna,
  title={{RNA} secondary structure prediction using an ensemble of two-dimensional deep neural networks and transfer learning},
  author={Singh, Jaswinder and Hanson, Jack and Paliwal, Kuldip and Zhou, Yaoqi},
  journal={Nature communications},
  volume={10},
  number={1},
  pages={1--13},
  year={2019},
  publisher={Nature Publishing Group}
}

@article{liu2019bioseq,
  title={{BioSeq-Analysis}: a platform for {DNA}, {RNA} and protein sequence analysis based on machine learning approaches},
  author={Liu, Bin},
  journal={Briefings in bioinformatics},
  volume={20},
  number={4},
  pages={1280--1294},
  year={2019},
  publisher={Oxford University Press}
}


@article{puton2013comparna,
  title={{CompaRNA}: a server for continuous benchmarking of automated methods for {RNA} secondary structure prediction},
  author={Puton, Tomasz and Kozlowski, Lukasz P and Rother, Kristian M and Bujnicki, Janusz M},
  journal={Nucleic acids research},
  volume={41},
  number={7},
  pages={4307--4323},
  year={2013},
  publisher={Oxford University Press}
}

@article{bellaousov2010probknot,
  title={{ProbKnot}: fast prediction of {RNA} secondary structure including pseudoknots},
  author={Bellaousov, Stanislav and Mathews, David H},
  journal={Rna},
  volume={16},
  number={10},
  pages={1870--1880},
  year={2010},
  publisher={Cold Spring Harbor Lab}
}

%%% flexibility
@article{guruge2018b,
  title={B-factor profile prediction for {RNA} flexibility using support vector machines},
  author={Guruge, Ivantha and Taherzadeh, Ghazaleh and Zhan, Jian and Zhou, Yaoqi and Yang, Yuedong},
  journal={Journal of Computational Chemistry},
  volume={39},
  number={8},
  pages={407--411},
  year={2018},
  publisher={Wiley Online Library}
}

@article{wei2019rna,
  title={{RNA} flexibility prediction with sequence profile and predicted solvent accessibility},
  author={Wei, Hong and Wang, Boling and Yang, Jianyi and Gao, Jianzhao},
  journal={IEEE/ACM Transactions on Computational Biology and Bioinformatics},
  year={2019},
  publisher={IEEE}
}

%%%MD references
@article{blochl1994projector,
  title={Projector augmented-wave method},
  author={Bl{\"o}chl, Peter E},
  journal={Physical review B},
  volume={50},
  number={24},
  pages={17953},
  year={1994},
  publisher={APS}
}

@article{perdew1998perdew,
  title={Perdew, burke, and ernzerhof reply},
  author={Perdew, JP and Burke, K and Ernzerhof, M},
  journal={Physical Review Letters},
  volume={80},
  number={4},
  pages={891},
  year={1998},
  publisher={APS}
}

@article{kresse1996efficient,
  title = {Efficient iterative schemes for ab initio total-energy calculations using a plane-wave basis set},
  author = {Kresse, G. and Furthm\"uller, J.},
  journal = {Phys. Rev. B},
  volume = {54},
  issue = {16},
  pages = {11169--11186},
  numpages = {0},
  year = {1996},
  month = {Oct},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRevB.54.11169},
  url = {https://link.aps.org/doi/10.1103/PhysRevB.54.11169}
}

@article{tkatchenko2009accurate,
  title={Accurate molecular van der Waals interactions from ground-state electron density and free-atom reference data},
  author={Tkatchenko, Alexandre and Scheffler, Matthias},
  journal={Physical review letters},
  volume={102},
  number={7},
  pages={073005},
  year={2009},
  publisher={APS}
}


%%%%%%%%% geometric deep learning


@article{bronstein2021geometric,
  title={Geometric deep learning: Grids, groups, graphs, geodesics, and gauges},
  author={Bronstein, Michael M and Bruna, Joan and Cohen, Taco and Veli{\v{c}}kovi{\'c}, Petar},
  journal={arXiv preprint arXiv:2104.13478},
  year={2021}
}

@inproceedings{masci2015geodesic,
  title={Geodesic convolutional neural networks on riemannian manifolds},
  author={Masci, Jonathan and Boscaini, Davide and Bronstein, Michael and Vandergheynst, Pierre},
  booktitle={Proceedings of the IEEE international conference on computer vision workshops},
  pages={37--45},
  year={2015}
}

@article{gainza2020deciphering,
  title={Deciphering interaction fingerprints from protein molecular surfaces using geometric deep learning},
  author={Gainza, Pablo and Sverrisson, Freyr and Monti, Frederico and Rodola, Emanuele and Boscaini, D and Bronstein, MM and Correia, BE},
  journal={Nature Methods},
  volume={17},
  number={2},
  pages={184--192},
  year={2020},
  publisher={Nature Publishing Group}
}


%%%%%%%%%%%%%%%%%%%%%%%% Protein-protein interactions (PPI)
%% review

@article{gonzalez2012chapter,
  title={Chapter 4: Protein interactions and disease},
  author={Gonzalez, Mileidy W and Kann, Maricel G},
  journal={PLoS computational biology},
  volume={8},
  number={12},
  pages={e1002819},
  year={2012},
  publisher={Public Library of Science San Francisco, USA}
}

@article{rebsamen2013protein,
  title={Protein interaction networks in innate immunity},
  author={Rebsamen, Manuele and Kandasamy, Richard Kumaran and Superti-Furga, Giulio},
  journal={Trends in immunology},
  volume={34},
  number={12},
  pages={610--619},
  year={2013},
  publisher={Elsevier}
}


@article{mosca2013interactome3d,
  title={{Interactome3D:} adding structural details to protein networks},
  author={Mosca, Roberto and C{\'e}ol, Arnaud and Aloy, Patrick},
  journal={Nature methods},
  volume={10},
  number={1},
  pages={47--53},
  year={2013},
  publisher={Nature Publishing Group}
}


%% Datasets

@article{thorn2001asedb,
  title={{ASEdb:} a database of alanine mutations and their effects on the free energy of binding in protein interactions},
  author={Thorn, Kurt S and Bogan, Andrew A},
  journal={Bioinformatics},
  volume={17},
  number={3},
  pages={284--285},
  year={2001},
  publisher={Oxford University Press}
}

@article{kumar2006pint,
  title={{PINT:} protein--protein interactions thermodynamic database},
  author={Kumar, MD Shaji and Gromiha, M Michael},
  journal={Nucleic acids research},
  volume={34},
  number={suppl\_1},
  pages={D195--D198},
  year={2006},
  publisher={Oxford University Press}
}


@article{moal2012skempi,
  title={{SKEMPI:} a Structural Kinetic and Energetic database of Mutant Protein Interactions and its use in empirical models},
  author={Moal, Iain H and Fern{\'a}ndez-Recio, Juan},
  journal={Bioinformatics},
  volume={28},
  number={20},
  pages={2600--2607},
  year={2012},
  publisher={Oxford University Press}
}
@article{sirin2016ab,
  title={{AB-Bind:} antibody binding mutational database for computational affinity predictions},
  author={Sirin, Sarah and Apgar, James R and Bennett, Eric M and Keating, Amy E},
  journal={Protein Science},
  volume={25},
  number={2},
  pages={393--409},
  year={2016},
  publisher={Wiley Online Library}
}

@article{geng2016exploring,
  title={Exploring the interplay between experimental methods and the performance of predictors of binding affinity change upon mutations in protein complexes},
  author={Geng, Cunliang and Vangone, Anna and Bonvin, Alexandre MJJ},
  journal={Protein Engineering, Design and Selection},
  volume={29},
  number={8},
  pages={291--299},
  year={2016},
  publisher={Oxford University Press}
}

@article{jemimah2017proximate,
  title={{PROXiMATE:} a database of mutant protein--protein complex thermodynamics and kinetics},
  author={Jemimah, Sherlyn and Yugandhar, K and Michael Gromiha, M},
  journal={Bioinformatics},
  volume={33},
  number={17},
  pages={2787--2788},
  year={2017},
  publisher={Oxford University Press}
}

@article{liu2017dbmpikt,
  title={{dbMPIKT:} a web resource for the kinetic and thermodynamic database of mutant protein interactions},
  author={Liu, Quanya and Chen, Peng and Wang, Bing and Li, Jinyan},
  journal={arXiv preprint arXiv:1708.01857},
  year={2017}
}


@article{jankauskaite2019skempi,
  title={{SKEMPI 2.0:} an updated benchmark of changes in protein--protein binding energy, kinetics and thermodynamics upon mutation},
  author={Jankauskait{\.e}, Justina and Jim{\'e}nez-Garc{\'\i}a, Brian and Dapk{\=u}nas, Justas and Fern{\'a}ndez-Recio, Juan and Moal, Iain H},
  journal={Bioinformatics},
  volume={35},
  number={3},
  pages={462--469},
  year={2019},
  publisher={Oxford University Press}
}

%% PPI mutation methods MD

@article{guerois2002predicting,
  title={Predicting changes in the stability of proteins and protein complexes: a study of more than 1000 mutations},
  author={Guerois, Raphael and Nielsen, Jens Erik and Serrano, Luis},
  journal={Journal of molecular biology},
  volume={320},
  number={2},
  pages={369--387},
  year={2002},
  publisher={Elsevier}
}

@article{kortemme2002simple,
  title={A simple physical model for binding energy hot spots in protein--protein complexes},
  author={Kortemme, Tanja and Baker, David},
  journal={Proceedings of the National Academy of Sciences},
  volume={99},
  number={22},
  pages={14116--14121},
  year={2002},
  publisher={National Acad Sciences}
}

@article{dourado2014multiscale,
  title={A multiscale approach to predicting affinity changes in protein--protein interfaces},
  author={Dourado, Daniel FAR and Flores, Samuel Coulbourn},
  journal={Proteins: Structure, Function, and Bioinformatics},
  volume={82},
  number={10},
  pages={2681--2690},
  year={2014},
  publisher={Wiley Online Library}
}

@article{petukh2016saambe,
  title={SAAMBE: webserver to predict the charge of binding free energy caused by amino acids mutations},
  author={Petukh, Marharyta and Dai, Luogeng and Alexov, Emil},
  journal={International journal of molecular sciences},
  volume={17},
  number={4},
  pages={547},
  year={2016},
  publisher={Multidisciplinary Digital Publishing Institute}
}

%% PPI mutation methods statistical potential

@article{xiong2017bindprofx,
  title={BindProfX: assessing mutation-induced binding affinity change by protein interface profiles with pseudo-counts},
  author={Xiong, Peng and Zhang, Chengxin and Zheng, Wei and Zhang, Yang},
  journal={Journal of molecular biology},
  volume={429},
  number={3},
  pages={426--434},
  year={2017},
  publisher={Elsevier}
}

@article{dehouck2013beatmusic,
  title={{BeAtMuSiC:} prediction of changes in protein--protein binding affinity on mutations},
  author={Dehouck, Yves and Kwasigroch, Jean Marc and Rooman, Marianne and Gilis, Dimitri},
  journal={Nucleic acids research},
  volume={41},
  number={W1},
  pages={W333--W339},
  year={2013},
  publisher={Oxford University Press}
}

@article{moal2013intermolecular,
  title={Intermolecular contact potentials for protein--protein interactions extracted from binding free energy changes upon mutation},
  author={Moal, Iain H and Fernandez-Recio, Juan},
  journal={Journal of Chemical Theory and Computation},
  volume={9},
  number={8},
  pages={3715--3727},
  year={2013},
  publisher={ACS Publications}
}


@article{szilagyi2014template,
  title={Template-based structure modeling of protein--protein interactions},
  author={Szilagyi, Andras and Zhang, Yang},
  journal={Current opinion in structural biology},
  volume={24},
  pages={10--23},
  year={2014},
  publisher={Elsevier}
}

@article{liu2004physical,
  title={A physical reference state unifies the structure-derived potential of mean force for protein folding and binding},
  author={Liu, Song and Zhang, Chi and Zhou, Hongyi and Zhou, Yaoqi},
  journal={Proteins: Structure, Function, and Bioinformatics},
  volume={56},
  number={1},
  pages={93--101},
  year={2004},
  publisher={Wiley Online Library}
}


%% PPI mutation methods  AI

@article{geng2019finding,
  title={Finding the $\Delta$$\Delta$G spot: Are predictors of binding affinity changes upon mutations in protein--protein interactions ready for it?},
  author={Geng, Cunliang and Xue, Li C and Roel-Touris, Jorge and Bonvin, Alexandre MJJ},
  journal={Wiley Interdisciplinary Reviews: Computational Molecular Science},
  volume={9},
  number={5},
  pages={e1410},
  year={2019},
  publisher={Wiley Online Library}
}


@article{brender2015predicting,
  title={Predicting the effect of mutations on protein-protein binding interactions through structure-based interface profiles},
  author={Brender, Jeffrey R and Zhang, Yang},
  journal={PLoS computational biology},
  volume={11},
  number={10},
  pages={e1004494},
  year={2015},
  publisher={Public Library of Science San Francisco, CA USA}
}


@article{geng2019isee,
  title={{iSEE:} Interface structure, evolution, and energy-based machine learning predictor of binding affinity changes upon mutations},
  author={Geng, Cunliang and Vangone, Anna and Folkers, Gert E and Xue, Li C and Bonvin, Alexandre MJJ},
  journal={Proteins: Structure, Function, and Bioinformatics},
  volume={87},
  number={2},
  pages={110--119},
  year={2019},
  publisher={Wiley Online Library}
}


@article{rodrigues2019mcsm,
  title={{mCSM-PPI2:} predicting the effects of mutations on protein--protein interactions},
  author={Rodrigues, Carlos HM and Myung, Yoochan and Pires, Douglas EV and Ascher, David B},
  journal={Nucleic acids research},
  volume={47},
  number={W1},
  pages={W338--W344},
  year={2019},
  publisher={Oxford University Press}
}


@article{jemimah2020proaffimuseq,
  title={{ProAffiMuSeq}: sequence-based method to predict the binding free energy change of protein--protein complexes upon mutation using functional classification},
  author={Jemimah, Sherlyn and Sekijima, Masakazu and Gromiha, M Michael},
  journal={Bioinformatics},
  volume={36},
  number={6},
  pages={1725--1730},
  year={2020},
  publisher={Oxford University Press}
}

@article{zhou2020mutation,
  title={Mutation effect estimation on protein--protein interactions using deep contextualized representation learning},
  author={Zhou, Guangyu and Chen, Muhao and Ju, Chelsea JT and Wang, Zheng and Jiang, Jyun-Yu and Wang, Wei},
  journal={NAR genomics and bioinformatics},
  volume={2},
  number={2},
  pages={lqaa015},
  year={2020},
  publisher={Oxford University Press}
}

@article{zhang2020mutabind2,
  title={{MutaBind2:} predicting the impacts of single and multiple mutations on protein-protein interactions},
  author={Zhang, Ning and Chen, Yuting and Lu, Haoyu and Zhao, Feiyang and Alvarez, Roberto Vera and Goncearenco, Alexander and Panchenko, Anna R and Li, Minghui},
  journal={Iscience},
  volume={23},
  number={3},
  pages={100939},
  year={2020},
  publisher={Elsevier}
}

@article{strokach2021elaspic2,
  title={{ELASPIC2 (EL2):} {Combining} {Contextualized} {Language} {Models} and {Graph Neural Networks} to {Predict Effects} of {Mutations}},
  author={Strokach, Alexey and Lu, Tian Yu and Kim, Philip M},
  journal={Journal of molecular biology},
  volume={433},
  number={11},
  pages={166810},
  year={2021},
  publisher={Elsevier}
}

@article{liu2021deep,
  title={Deep geometric representations for modeling effects of mutations on protein-protein binding affinity},
  author={Liu, Xianggen and Luo, Yunan and Li, Pengyong and Song, Sen and Peng, Jian},
  journal={PLoS computational biology},
  volume={17},
  number={8},
  pages={e1009284},
  year={2021},
  publisher={Public Library of Science San Francisco, CA USA}
}

%%%%%%%%% deep learning for protein data

@article{shi2021deep,
  title={Deep learning for mining protein data},
  author={Shi, Qiang and Chen, Weiya and Huang, Siqi and Wang, Yan and Xue, Zhidong},
  journal={Briefings in bioinformatics},
  volume={22},
  number={1},
  pages={194--218},
  year={2021},
  publisher={Oxford University Press}
}

%%% dirac operator
@article{knill2013dirac,
  title={The {Dirac} operator of a graph},
  author={Knill, Oliver},
  journal={arXiv preprint arXiv:1306.2166},
  year={2013}
}

@article{knill2013mckean,
  title={The {McKean-Singer} Formula in Graph Theory},
  author={Knill, Oliver},
  journal={arXiv preprint arXiv:1301.1408},
  year={2013}
}

@article{Bianconi_2021,
	doi = {10.1088/2632-072x/ac19be},
	url = {https://doi.org/10.1088/2632-072x/ac19be},
	year = 2021,
	month = {sep},
	publisher = {{IOP} Publishing},
	volume = {2},
	number = {3},
	pages = {035022},
	author = {Ginestra Bianconi},
	title = {The topological {Dirac} equation of networks and simplicial complexes},
	journal = {Journal of Physics: Complexity},
	abstract = {We define the topological Dirac equation describing the evolution of a topological wave function on networks or on simplicial complexes. On networks, the topological wave function describes the dynamics of topological signals or cochains, i.e. dynamical signals defined both on nodes and on links. On simplicial complexes the wave function is also defined on higher-dimensional simplices. Therefore the topological wave function satisfies a relaxed condition of locality as it acquires the same value along simplices of dimension larger than zero. The topological Dirac equation defines eigenstates whose dispersion relation is determined by the spectral properties of the Dirac operator defined on networks and generalized network structures including simplicial complexes and multiplex networks. On simplicial complexes the Dirac equation leads to multiple energy bands. On multiplex networks the topological Dirac equation can be generalized to distinguish between different mutlilinks leading to a natural definition of rotations of the topological spinor. The topological Dirac equation is here initially formulated on a spatial network or simplicial complex for describing the evolution of the topological wave function in continuous time. This framework is also extended to treat the topological Dirac equation on 1 + d lattices describing a discrete space-time with one temporal dimension and d spatial dimensions with d ∈ {1, 2, 3}. It is found that in this framework space-like and time-like links are only distinguished by the choice of the directional Dirac operator and are otherwise structurally indistinguishable. This work includes also the discussion of numerical results obtained by implementing the topological Dirac equation on simplicial complex models and on real simple and multiplex network data.}
}

@article{PhysRevE.104.064303,
  title = {Spectral {D}etection of {S}implicial {C}ommunities via {H}odge {L}aplacians},
  author = {Krishnagopal, Sanjukta and Bianconi, Ginestra},
  journal = {Phys. Rev. E},
  volume = {104},
  issue = {6},
  pages = {064303},
  numpages = {18},
  year = {2021},
  month = {Dec},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRevE.104.064303},
  url = {https://link.aps.org/doi/10.1103/PhysRevE.104.064303}
}


@article{memoli2020persistent,
  title={Persistent {Laplacians: Properties}, algorithms and implications},
  author={M{\'e}moli, Facundo and Wan, Zhengchao and Wang, Yusu},
  journal={arXiv preprint arXiv:2012.02808},
  year={2020}
}

@article{wei2021persistent,
  title={Persistent {Sheaf} {Laplacians}},
  author={Wei, Xiaoqi and Wei, Guo-Wei},
  journal={arXiv preprint arXiv:2112.10906},
  year={2021}
}

%%%% Protein Interactions Simplicial Complexes
@article{estrada2018centralities,
  title={Centralities in simplicial complexes. Applications to protein interaction networks},
  author={Estrada, Ernesto and Ross, Grant J},
  journal={Journal of theoretical biology},
  volume={438},
  pages={46--60},
  year={2018},
  publisher={Elsevier}
}

%%%%% Higher-order Dynamics
@article{torres2020simplicial,
  title={Simplicial complexes: higher-order spectral dimension and dynamics},
  author={Torres, Joaqu{\'\i}n J and Bianconi, Ginestra},
  journal={Journal of Physics: Complexity},
  volume={1},
  number={1},
  pages={015002},
  year={2020},
  publisher={IOP Publishing}
}

@article{millan2020explosive,
  title={Explosive higher-order {K}uramoto dynamics on simplicial complexes},
  author={Mill{\'a}n, Ana P and Torres, Joaqu{\'\i}n J and Bianconi, Ginestra},
  journal={Physical Review Letters},
  volume={124},
  number={21},
  pages={218301},
  year={2020},
  publisher={APS}
}

@article{ghorbanchian2021higher,
  title={Higher-order simplicial synchronization of coupled topological signals},
  author={Ghorbanchian, Reza and Restrepo, Juan G and Torres, Joaqu{\'\i}n J and Bianconi, Ginestra},
  journal={Communications Physics},
  volume={4},
  number={1},
  pages={1--13},
  year={2021},
  publisher={Nature Publishing Group}
}

@article{calmon2021topological,
  title={Dirac syncrhonization is rhythmic and explosive},
  author={Calmon, Lucille and Restrepo, Juan G and Torres, Joaqu{\'\i}n J and Bianconi, Ginestra},
  journal={Communications Physics},
    volume={5},
  number={1},
  pages={253},
  year={2022},
   publisher={Nature Publishing Group}
}

%%% synchronization dynamics
@article{wu2015emergent,
  title={Emergent complex network geometry},
  author={Wu, Zhihao and Menichetti, Giulia and Rahmede, Christoph and Bianconi, Ginestra},
  journal={Scientific reports},
  volume={5},
  number={1},
  pages={1--12},
  year={2015},
  publisher={Nature Publishing Group}
}

@article{bianconi2017emergent,
  title={Emergent hyperbolic network geometry},
  author={Bianconi, Ginestra and Rahmede, Christoph},
  journal={Scientific reports},
  volume={7},
  number={1},
  pages={1--9},
  year={2017},
  publisher={Nature Publishing Group}
}

@article{bianconi2016network,
  title={Network geometry with flavor: {F}rom complexity to quantum geometry},
  author={Bianconi, Ginestra and Rahmede, Christoph},
  journal={Physical Review E},
  volume={93},
  number={3},
  pages={032315},
  year={2016},
  publisher={APS}
}

%%%% De-Rham Hodge

@article{chen2021evolutionary,
  title={Evolutionary de {Rham-Hodge} method},
  author={Chen, Jiahui and Zhao, Rundong and Tong, Yiying and Wei, Guo-Wei},
  journal={Discrete and continuous dynamical systems. Series B},
  volume={26},
  number={7},
  pages={3785},
  year={2021},
  publisher={NIH Public Access}
}

@article{zhao2020rham,
  title={The de {Rham--Hodge} analysis and modeling of biomolecules},
  author={Zhao, Rundong and Wang, Menglun and Chen, Jiahui and Tong, Yiying and Wei, Guo-Wei},
  journal={Bulletin of mathematical biology},
  volume={82},
  number={8},
  pages={1--38},
  year={2020},
  publisher={Springer}
}

@article{zhao20193d,
  title={{3D Hodge} {D}ecompositions of {E}dge-and {F}ace-based {V}ector {F}ields},
  author={Zhao, Rundong and Desbrun, Mathieu and Wei, Guo-Wei and Tong, Yiying},
  journal={ACM Transactions on Graphics (TOG)},
  volume={38},
  number={6},
  pages={1--13},
  year={2019},
  publisher={ACM New York, NY, USA}
}

@article{wei2022hodge,
  title={Hodge theory-based biomolecular data analysis},
  author={Wei, Ronald Koh Joon and Wee, Junjie and Laurent, Valerie Evangelin and Xia, Kelin},
  journal={Scientific Reports},
  volume={12},
  number={1},
  pages={1--16},
  year={2022},
  publisher={Nature Publishing Group}
}

%%%% Image
@article{crawford2020predicting,
  title={Predicting clinical outcomes in glioblastoma: an application of topological and functional data analysis},
  author={Crawford, Lorin and Monod, Anthea and Chen, Andrew X and Mukherjee, Sayan and Rabad{\'a}n, Ra{\'u}l},
  journal={Journal of the American Statistical Association},
  volume={115},
  number={531},
  pages={1139--1150},
  year={2020},
  publisher={Taylor \& Francis}
}

@article{saadatfar2017pore,
  title={Pore configuration landscape of granular crystallization},
  author={Saadatfar, Mohammad and Takeuchi, Hiroshi and Robins, Vanessa and Francois, Nicolas and Hiraoka, Yasuaki},
  journal={Nature communications},
  volume={8},
  number={1},
  pages={1--11},
  year={2017},
  publisher={Nature Publishing Group}
}

@article{turner2014persistent,
  title={Persistent homology transform for modeling shapes and surfaces},
  author={Turner, Katharine and Mukherjee, Sayan and Boyer, Doug M},
  journal={Information and Inference: A Journal of the IMA},
  volume={3},
  number={4},
  pages={310--344},
  year={2014},
  publisher={Oxford University Press}
}

@article{de2007homological,
  title={Homological sensor networks},
  author={De Silva, Vin and Ghrist, Robert and others},
  journal={Notices of the American mathematical society},
  volume={54},
  number={1},
  year={2007}
}

@inproceedings{skraba2010persistence,
  title={Persistence-based segmentation of deformable shapes},
  author={Skraba, Primoz and Ovsjanikov, Maks and Chazal, Frederic and Guibas, Leonidas},
  booktitle={2010 IEEE Computer Society Conference on Computer Vision and Pattern Recognition-Workshops},
  pages={45--52},
  year={2010},
  organization={IEEE}
}

@article{carlsson2008local,
  title={On the local behavior of spaces of natural images},
  author={Carlsson, Gunnar and Ishkhanov, Tigran and De Silva, Vin and Zomorodian, Afra},
  journal={International journal of computer vision},
  volume={76},
  number={1},
  pages={1--12},
  year={2008},
  publisher={Springer}
}

@article{qaiser2019fast,
  title={Fast and accurate tumor segmentation of histology images using persistent homology and deep convolutional features},
  author={Qaiser, Talha and Tsang, Yee-Wah and Taniyama, Daiki and Sakamoto, Naoya and Nakane, Kazuaki and Epstein, David and Rajpoot, Nasir},
  journal={Medical image analysis},
  volume={55},
  pages={1--14},
  year={2019},
  publisher={Elsevier}
}

@book{bianconi2018multilayer,
  title={Multilayer networks: structure and function},
  author={Bianconi, Ginestra},
  year={2018},
  publisher={Oxford university press}
}

@article{ameneyro2022quantumph,
  title={Quantum {Persistent Homology}},
  author={Ameneyro, Bernardo and Maroulas, Vasileios and Siopsis, George},
  journal={arXiv preprint arXiv:2202.12965},
  year={2022}
}

@inproceedings{ameneyro2022quantum,
  title={Quantum {Persistent Homology for Time Series}},
  author={Ameneyro, Bernardo and Siopsis, George and Maroulas, Vasileios},
  booktitle={2022 IEEE/ACM 7th Symposium on Edge Computing (SEC)},
  pages={387--392},
  year={2022},
  organization={IEEE}
}

@article{baccini2022weighted,
  title={Weighted simplicial complexes and their representation power of higher-order network data and topology},
  author={Baccini, Federica and Geraci, Filippo and Bianconi, Ginestra},
  journal={Physical Review E},
  volume={106},
  number={3},
  pages={034319},
  year={2022},
  publisher={APS}
}

@incollection{crane2011spin,
  title={Spin transformations of discrete surfaces},
  author={Crane, Keenan and Pinkall, Ulrich and Schr{\"o}der, Peter},
  booktitle={ACM SIGGRAPH 2011 papers},
  pages={1--10},
  year={2011}
}

@article{memoli2022persistent,
  title={Persistent {Laplacians}: {Properties}, algorithms and implications},
  author={M{\'e}moli, Facundo and Wan, Zhengchao and Wang, Yusu},
  journal={SIAM Journal on Mathematics of Data Science},
  volume={4},
  number={2},
  pages={858--884},
  year={2022},
  publisher={SIAM}
}

@article{lloyd2016quantum,
  title={Quantum algorithms for topological and geometric analysis of data},
  author={Lloyd, Seth and Garnerone, Silvano and Zanardi, Paolo},
  journal={Nature communications},
  volume={7},
  number={1},
  pages={1--7},
  year={2016},
  publisher={Nature Publishing Group}
}

@article{anand2022topological,
  title={Topological {F}eature {E}ngineering for {M}achine {L}earning based {H}alide {P}erovskite {M}aterials {D}esign},
  author={Anand, D Vijay and Xu, Qiang and Wee, JunJie and Xia, Kelin and Sum, Tze Chien},
  journal={npj Computational Materials},
  volume={8},
  number={1},
  pages={203},
  year={2022},
  publisher={Nature Publishing Group UK London}
}
